Tensor-restriction categories

Restriction categories were established to handle maps that are partially defined with respect to composition. Tensor topology realises that monoidal categories have an intrinsic notion of space, and deals with objects and maps that are partially defined with respect to this spatial structure. We introduce a construction that turns a firm monoidal category into a restriction category and axiomatise the monoidal restriction categories that arise this way, called tensor-restriction categories.

==> pgf.revision.tex <==
\begingroup
\catcode`\-=12
\catcode`\/=12
\catcode`\.=12
\catcode`\:=12
\catcode`\+=12
\catcode`\-=12
\gdef\pgfrevision{3.1.8b}
\gdef\pgfversion{3.1.8b}
\gdef\pgfversiondatetime{2020-12-27 19:52:45 +0100}
\gdef\pgfrevisiondatetime{2020-12-27 19:52:45 +0100}
\gdef\pgf@glob@TMPa#1-#2-#3 #4\relax{#1/#2/#3}
\xdef\pgfversiondate{\expandafter\pgf@glob@TMPa\pgfversiondatetime\relax}
\xdef\pgfrevisiondate{\expandafter\pgf@glob@TMPa\pgfrevisiondatetime\relax}
\endgroup


==> pgfcore.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgfcore.code.tex}

\newif\ifpgf@draftmode
\def\pgf@typeout{\immediate\write0}

\input pgfmath.code.tex
\input pgfint.code.tex

\input pgfcorepoints.code.tex
\input pgfcorepathconstruct.code.tex
\input pgfcorepathusage.code.tex
\input pgfcorescopes.code.tex
\input pgfcoregraphicstate.code.tex
\input pgfcoretransformations.code.tex
\input pgfcorequick.code.tex
\input pgfcoreobjects.code.tex
\input pgfcorepathprocessing.code.tex
\input pgfcorearrows.code.tex
\input pgfcoreshade.code.tex
\input pgfcoreimage.code.tex
\input pgfcorelayers.code.tex
\input pgfcoretransparency.code.tex
\input pgfcorepatterns.code.tex
\input pgfcorerdf.code.tex

\pgfutil@ifundefined{pgf@texdist@protect}{%
    \def\pgf@texdist@protect{}%
}{}
\endinput


==> pgfcorearrows.code.tex <==
% Copyright 2006, 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorearrows.code.tex}



% Define a new (meta) arrow or a shorthand
%
% #1 = key--value pairs
%
% Description:
%
% This command is used to define a new arrow tip kind. For more
% details on the description of the keys, please see the pgfmanual.
%
% name         = Name of the arrow. If the name contains a dash
%                (hyphen), the text before the hyphen is the start name
%                and the text behind it the end name.
%
% means        = If set, none of the below options may be
%                given. The effect is that whenever the arrow is
%                used, it gets replaced by this "text", which is
%                parsed by the parser.
%
% setup code   = Code that does "precomputations". These will be
%                executed only once for each combination of the
%                dependencies. At the end of this code, you can use
%                \savethe and \save to "save" computed values, which
%                will then be available inside the "code". Values needed
%                only for the "... end" keys and the convex hull do not
%                need to be saved since these are also executed only
%                once.
% drawing code = Code for drawing the arrow. When the cache key is set to
%                true, which is the default, the code will be protocolled
%                and the resulting code is inserted using \pgflowlevelobj.
% cache        = Boolean that decides whether the arrow can be cached. The
%                default is true, so you have to say cache=false to switch
%                caching off. In this case, each time the arrow is drawn,
%                its code is simply executed. This allows you to put things
%                like text or shadings in arrow tips.
% bending mode = Can be set to "orthogonal", "polar", or
%                "none". Defaults to "orthogonal".
% defaults     = A list of "default" options for the arrow tip. These
%                are executed as if they were given to the arrow tip in
%                brackets. This is useful for setting up default values.
% parameters   = A list of comma-separated macro names on whose values
%                the appearance of the arrow tip depends. When an arrow
%                tip is used, these macros are expanded. If an
%                arrow tip was already installed with the same macro
%                names (and caching is true), the cached code is
%                used. Note that when you use dimensions here, add \the.
%
% Inside the setup code, the following macros are available:
%
% \pgfarrowssettipend
%              The code should draw an arrow pointing "right along the x
%              axis". The "tip" key specifies how far the arrow goes
%              along the x axis, that is, it should be the x coordinate
%              of the very tip of the arrow. In previous versions this
%              was called the "right extend". The value passed to this
%              key should be some code that sets the dimension
%              "\pgfarrowresult", which is \let to be equal to
%              \pgf@x. A \relax will be added after the code provided
%              here, so you can write things like "\pgfarrowresult=1pt".
% \pgfarrowssetbackend
%              The leftmost x-coordinate that is still part of the
%              arrow tip (the "back end" of the arrow"). This coordinate
%              will be used when multiple arrow tips are
%              composed. Defaults to 0pt.
% \pgfarrowssetlineend
%              The x-coordinate where a line should stop inside the arrow
%              tip so that it gets "obscured" by the arrow. Defaults to 0pt.
% \pgfarrowssetvisualtipend
%              When the arrow tip is drawn in flex mode, it is rotated
%              such that the x-coordinates of "visual tip end" and "visual
%              back end" lie on the path. Defaults to \pgfarrowssettipend.
% \pgfarrowssetvisualbackend
%              See above. Defaults to \pgfarrowssetbackend

\def\pgfdeclarearrow#1{%
  \let\pgf@decl@arrow@defaults\pgfutil@empty%
  \let\pgf@decl@arrow@means\relax%
  \let\pgf@decl@arrow@code\relax%
  \pgfkeys{/pgf/@arrows decl/.cd,
    name=,
    setup code=,
    cache=true,
    bending mode=orthogonal,
    parameters=,%
    #1%
  }%
  \ifx\pgf@decl@arrow@name@end\pgfutil@empty%
    \pgferror{Declaring unnamed arrow}%
  \else%
    \pgf@arrow@letter{name@end}%
    \pgf@arrow@letter{name@start}%
    \expandafter\let\csname pgf@ar@start@\pgf@decl@arrow@name@start\endcsname\pgf@decl@arrow@name@end%
    \expandafter\let\expandafter\pgf@old@code\csname pgf@ar@code@\pgf@decl@arrow@name@end\endcsname%
    \expandafter\let\expandafter\pgf@old@means\csname pgf@ar@means@\pgf@decl@arrow@name@end\endcsname%
    \ifx\pgf@decl@arrow@code\relax%
      \ifx\pgf@decl@arrow@means\relax%
        \pgferror{You must set either the 'means' or the drawing code' keys for arrow tip '\pgf@decl@arrow@name@end'}%
      \else%
        \ifx\pgf@old@code\relax%
          \let\pgf@arrow@tip@sequence\pgfutil@empty%
          \let\pgf@arrow@translate\relax%
          \expandafter\let\expandafter\pgf@arrows@direct\csname pgf@arrows@direct@name@end@\pgf@decl@arrow@means\endcsname%
          \ifx\pgf@arrows@direct\relax%
            \let\pgf@arrows@options\pgfutil@empty%
            \expandafter\pgfarrows@initial@parser\pgf@decl@arrow@means[]\pgf@stop%
          \else%
            \let\pgf@arrow@tip@sequence\pgf@arrows@direct%
          \fi%
          \pgf@arrow@letter@\pgf@arrow@tip@sequence{means}%
          \expandafter\let\csname pgf@ar@code@\pgf@decl@arrow@name@end\endcsname\relax%
        \else%
          \pgferror{Arrow tip '\pgf@decl@arrow@name@end' was already
            defined with key 'drawing code' previously and you cannot change this}%
        \fi%
      \fi%
    \else%
      \ifx\pgf@decl@arrow@means\relax%
        \ifx\pgf@old@means\relax%
          \pgf@arrow@letter{code}%
          \pgf@arrow@letter{defaults}%
          \pgf@arrow@letter{setup}%
          \pgf@arrow@letter{bending@mode}%
          \pgf@arrow@letter{par}%
          \expandafter\let\csname pgf@ar@do@cache@\pgf@decl@arrow@name@end\endcsname\pgf@decl@arrow@cache%
        \else%
          \pgferror{Arrow tip '\pgf@decl@arrow@name@end' was already
            defined with key 'means' previously and you cannot change this}%
        \fi%
      \else%
        \pgferror{You cannot set both the 'means' and also the 'drawing code'
          keys for arrow tip '\pgf@decl@arrow@name@end'}%
      \fi%
    \fi%
  \fi%
}

\def\pgf@arrow@letter#1{%
  \expandafter\pgf@arrow@letter@\expandafter{\csname pgf@decl@arrow@#1\endcsname}{#1}%
}
\def\pgf@arrow@letter@#1#2{%
  \expandafter\let\csname pgf@ar@#2@\pgf@decl@arrow@name@end\endcsname#1%
}

\pgfkeys{
  /pgf/@arrows decl/.cd,
  name/.code={%
    \pgfutil@in@-{#1}%
    \ifpgfutil@in@%
      \pgf@arrows@name@decomp#1\pgf@stop%
    \else%
      \def\pgf@decl@arrow@name@end{#1}\let\pgf@decl@arrow@name@start\pgf@decl@arrow@name@end%
    \fi},
  means/.store in=\pgf@decl@arrow@means,
  setup code/.store in=\pgf@decl@arrow@setup,
  drawing code/.store in=\pgf@decl@arrow@code,
  cache/.store in=\pgf@decl@arrow@cache,
  bending mode/.is choice,
  bending mode/none/.code=\let\pgf@decl@arrow@bending@mode\pgfutil@empty,
  bending mode/orthogonal/.code=\def\pgf@decl@arrow@bending@mode{\pgfpointcurvilinearbezierorthogonal},
  bending mode/polar/.code=\def\pgf@decl@arrow@bending@mode{\pgfpointcurvilinearbezierpolar},
  parameters/.store in=\pgf@decl@arrow@par,
  defaults/.code={%
    \let\pgf@arrows@options\pgfutil@empty%
    \pgfkeys{/pgf/arrow keys/.cd,#1}%
    \let\pgf@decl@arrow@defaults\pgf@arrows@options%
  }
}

\def\pgf@arrows@name@decomp#1-#2\pgf@stop{%
  \def\pgf@decl@arrow@name@start{#1}%
  \def\pgf@decl@arrow@name@end{#2}%
}


% Handler for defining arrow tips:
%
% Description:
%
% When you write "my name/.tip = arrow spec", this has the same
% effect as writing \pgfdeclarearrow{name = my name, means = arrow spec}.

\pgfkeys{/handlers/.tip/.code=%
  \expandafter\expandafter\expandafter\pgf@arrows@unravel\pgfkeyscurrentpath/\pgf@stop%
  \expandafter\pgf@arrows@key@call\expandafter{\pgf@arrows@unravelled}{#1}}
\def\pgf@arrows@unravel#1/{\pgfutil@ifnextchar\pgf@stop{\def\pgf@arrows@unravelled{#1}\pgfutil@gobble}{\pgf@arrows@unravel}}
\def\pgf@arrows@key@call#1#2{\pgfdeclarearrow{name={#1},means={#2}}}




% Draw an arrow
%
% #1 = arrow specification
%
% Description:
%
% Draws the arrow in the given specification (and "end"
% specification). The arrow will be drawn such that it touches the
% origin "from the left", that is, the arrow will lie completely in
% the half plane with negative $x$ values and the tip will end exactly
% at the origin.

\def\pgfarrowdraw#1{%
  {%
    \pgfsetarrowsend{#1}%
    \pgf@arrow@compute@shortening\pgf@end@tip@sequence%
    \pgf@arrow@draw@arrow\pgf@end@tip@sequence\pgf@xb%
  }%
}



% Compute the length of an arrow
%
% #1 = arrow specification
%
% Description:
%
% In \pgf@x, this will return the total length of the arrow given as
% #1, in \pgf@xa it will return the distance from the tip to the line
% end.

\def\pgfarrowtotallength#1{%
  {%
    \pgfsetarrowsend{#1}%
    \pgf@arrow@compute@shortening\pgf@end@tip@sequence%
    \expandafter\expandafter\expandafter%
  }%
  \expandafter\expandafter\expandafter\pgf@x\expandafter\the\expandafter\pgf@xb\expandafter\pgf@xa\the\pgf@xa%
}





% Sets the end arrow tip
%
% #1 = An arrow specification
%
% Description:
%
% An "arrow specification" is a sequence of names of meta arrow tips
% together with options in brackets. In detail:
%
% In #1, consider the text from the start up to the first bracket. If
% this text is the name of a (meta) arrow tip, we use this arrow tip
% with the provided options. If it is the name of a arrow tip
% shorthand, this shorthand is expanded and the options are applied to
% each arrow tip inside the shorthand. If the text is neither or the
% above, the first letter of text is treated as a shorthand without
% options.
%
% The special arrow tip "." is used to indicate the end of the line.
%
% \pgfsetarrowsend{stealth[reversed]}
% \pgfsetarrowsend{stealth[length=1pt] . stealth[length=2pt]}
% \pgfsetarrowsend{>>>}
% \pgfsetarrowsend{>.>}

\def\pgfsetarrowsend#1{%
  \let\pgf@arrow@tip@sequence\pgfutil@empty%
  \pgf@arrows@translatefalse%
  \expandafter\let\expandafter\pgf@arrows@direct\csname pgf@arrows@direct@name@end@#1\endcsname%
  \ifx\pgf@arrows@direct\relax%
    \edef\pgf@marshal{\noexpand\pgfarrows@initial@parser#1[]\noexpand\pgf@stop}%
    \pgf@marshal%
  \else%
    \let\pgf@arrow@tip@sequence\pgf@arrows@direct%
  \fi%
  \let\pgf@end@tip@sequence\pgf@arrow@tip@sequence%
}

\newif\ifpgf@arrows@translate

\def\pgfarrows@initial@parser{%
  \pgfutil@ifnextchar[\pgfarrows@initial@parser@{\pgfarrows@initial@parser@[]}}%}

\def\pgfarrows@initial@parser@[#1]{%
  \let\pgf@arrows@options\pgfutil@empty%
  \pgfkeys{/pgf/arrow keys/.cd,#1}%
  \let\pgf@arrows@options@initial\pgf@arrows@options%
  \pgfarrows@parser%
}

\def\pgfarrows@parser#1[{%
  \pgfkeys@spdef\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
    \let\pgf@next\pgf@arrows@empty%
  \else%
    \ifx\pgf@temp\pgf@dot@text%
      \let\pgf@next\pgf@arrows@dot@parsed%
    \else%
      \let\pgf@untranslated\pgf@temp%
      \ifpgf@arrows@translate%
        \pgf@arrow@swapper%
      \fi%
      % Now, let's see what we do with this...
      \expandafter\ifx\csname pgf@ar@code@\pgf@temp\endcsname\relax
        \expandafter\ifx\csname pgf@ar@means@\pgf@temp\endcsname\relax
          % #1 should start with a single-char shorthands
          \let\pgf@next\pgf@arrows@single@char@parser%
          \let\pgf@temp\pgf@untranslated%
        \else%
          % #1 is a shorthand!
          \let\pgf@next\pgf@arrows@shorthand@parsed%
        \fi%
      \else%
        % #1 is a meta arrow!
        \let\pgf@next\pgf@arrows@meta@parsed%
      \fi%
    \fi%
  \fi%
  \expandafter\pgf@next\pgf@temp[%
}

\def\pgf@arrows@empty[#1]{%
  \pgfutil@ifnextchar\pgf@stop\pgf@arrows@parser@done\pgfarrows@parser%
}

\def\pgf@arrows@single@char@parser#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@dot@text%
    \let\pgf@next\pgf@arrows@dot@parsed%
  \else%
    \let\pgf@untranslated\pgf@temp%
    \ifpgf@arrows@translate%
      \pgf@arrow@swapper%
    \fi%
    \expandafter\ifx\csname pgf@ar@code@\pgf@temp\endcsname\relax
      \expandafter\ifx\csname pgf@ar@means@\pgf@temp\endcsname\relax
        \let\pgf@temp\pgf@untranslated%
        \let\pgf@next\pgf@arrows@unknown%
      \else%
        \let\pgf@next\pgf@arrows@shorthand@parsed%
      \fi%
    \else%
      \let\pgf@next\pgf@arrows@meta@parsed%
    \fi
  \fi
  \expandafter\pgf@next\pgf@temp[]%
}
\def\pgf@arrows@unknown#1[]#2[#3]{%
  \pgferror{Unknown arrow tip kind '#1#2'}%
}

\def\pgf@arrows@meta@parsed#1[#2]{%
  % Ok, run the keys #2. This will add commands to \pgf@arrows@options:
  %
  \let\pgf@arrows@options\pgf@arrows@options@initial%
  \pgfkeys{/pgf/arrow keys/.cd,#2}%
  % Append the arrow and its options to the arrow tip sequence:
  \expandafter\pgf@arrows@meta@set\expandafter{\pgf@arrows@options}{#1}{\pgf@arrow@handle}%
  \pgfutil@ifnextchar\pgf@stop\pgf@arrows@parser@done\pgfarrows@parser%
}

\def\pgf@arrows@parser@done#1{%
}

\def\pgf@arrows@dot@parsed#1[#2]{%
  \pgf@arrows@append@to@tips{\pgf@arrow@handle@dot}%
  \pgfutil@ifnextchar\pgf@stop\pgf@arrows@parser@done\pgfarrows@parser%
}

\def\pgf@arrows@meta@set#1#2#3{%
  \pgf@arrows@append@to@tips{#3{#2}{#1}}%
}
\def\pgf@arrows@append@to@tips#1{%
  \let\pgf@tempa\pgf@arrow@tip@sequence%
  \def\pgf@tempb{#1}%
  \ifpgf@arrows@translate%
    \let\pgf@tempa\pgf@tempb%
    \let\pgf@tempb\pgf@arrow@tip@sequence%
  \fi%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgf@arrow@tip@sequence%
  \expandafter\expandafter\expandafter{\expandafter\pgf@tempa\pgf@tempb}%
}

\def\pgf@arrows@shorthand@parsed#1[#2]{%
  \let\pgf@arrows@options\pgf@arrows@options@initial%
  \pgfkeys{/pgf/arrow keys/.cd,#2}%
  \ifx\pgf@arrows@options\pgfutil@empty%
    \expandafter\pgf@arrows@append@to@tips\expandafter{%
      \expandafter\pgf@arrow@handle@shorthand@empty\expandafter{\csname pgf@ar@means@#1\endcsname}}%
  \else%
    \expandafter\expandafter\expandafter\pgf@arrows@meta@set\expandafter\expandafter\expandafter{%
      \expandafter\pgf@arrows@options\expandafter}\expandafter{\csname pgf@ar@means@#1\endcsname}{\pgf@arrow@handle@shorthand}%
  \fi%
  \pgfutil@ifnextchar\pgf@stop\pgf@arrows@parser@done\pgfarrows@parser%
}


% General handler:

\def\pgf@arrow@handle@shorthand@empty#1{#1}

\def\pgf@arrow@handle@shorthand#1#2{%
  \def\pgf@temp@opt{#2}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgf@arrows@nested@options@temp%
  \expandafter\expandafter\expandafter{\expandafter\pgf@temp@opt\pgf@arrows@nested@options}%
  \expandafter\let\expandafter\pgf@arrows@nested@options\expandafter\pgf@arrows@nested@options@temp%
  \expandafter#1% all these expandafters to avoid creating groups, but having the options nest
  \expandafter\def\expandafter\pgf@arrows@nested@options\expandafter{\pgf@arrows@nested@options}%
}

\let\pgf@arrows@nested@options\pgfutil@empty




% Sets the start arrow tip
%
% #1 = An arrow specification
%
% Description:
%
% This works like \pgfsetarrowsend, only the order of the tips in the
% arrow specification is reversed and the "reversed names" are used.
%
% \pgfsetarrowsend{<<}
% \pgfsetarrowsend{>.>}

\def\pgfsetarrowsstart#1{%
  \let\pgf@arrow@tip@sequence\pgfutil@empty%
  \pgf@arrows@translatetrue%
  \expandafter\let\expandafter\pgf@arrows@direct\csname pgf@arrows@direct@name@start@#1\endcsname%
  \ifx\pgf@arrows@direct\relax%
    \edef\pgf@marshal{\noexpand\pgfarrows@initial@parser#1[]\noexpand\pgf@stop}%
    \pgf@marshal%
  \else%
    \let\pgf@arrow@tip@sequence\pgf@arrows@direct%
  \fi%
  \let\pgf@start@tip@sequence\pgf@arrow@tip@sequence%
}

\def\pgf@arrow@swapper{%
  \expandafter\let\expandafter\pgf@temp\csname pgf@ar@start@\pgf@temp\endcsname%
  \ifx\pgf@temp\relax%
    \def\pgf@temp{undefined}%
  \fi%
}

\let\pgf@start@tip@sequence\pgfutil@empty
\let\pgf@end@tip@sequence\pgfutil@empty


\expandafter\def\csname pgf@arrows@direct@name@start@\endcsname{}
\expandafter\def\csname pgf@arrows@direct@name@end@\endcsname{}


% Predefined lengths and ifs

\newdimen\pgfarrowsep

\newif\ifpgfarrowswap
\newif\ifpgfarrowreversed
\newif\ifpgfarrowharpoon
\newif\ifpgfarrowopen

\let\pgf@arrows@stroke@color\pgfutil@empty
\let\pgf@arrows@fill@color\pgfutil@empty

\def\pgfarrows@length@scale{1}
\def\pgfarrows@width@scale{1}
\def\pgfarrows@slant{0}

\let\pgfarrows@scale@list\pgfutil@empty
\def\pgfarrowsaddtolengthscalelist#1{\expandafter\def\expandafter\pgfarrows@scale@list\expandafter{\pgfarrows@scale@list#1\pgfarrows@length@scale#1}}
\def\pgfarrowsaddtowidthscalelist#1{\expandafter\def\expandafter\pgfarrows@scale@list\expandafter{\pgfarrows@scale@list#1\pgfarrows@width@scale#1}}

\pgfkeys{
  /pgf/arrow keys/.cd,
  scale/.code={%
    \pgfmathparse{#1}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrows@length@scale\expandafter{\pgfmathresult}}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrows@width@scale\expandafter{\pgfmathresult}}%
  },
  scale length/.code={\pgfmathparse{#1}\expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrows@length@scale\expandafter{\pgfmathresult}}},
  scale width/.code={\pgfmathparse{#1}\expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrows@width@scale\expandafter{\pgfmathresult}}},
  slant/.code={\pgfmathparse{#1}\expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrows@slant\expandafter{\pgfmathresult}}},
  sep/.code={
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\pgfarrowslinewidthdependent\pgfarrowstheparameters\pgfarrowsep\pgf@x}%
  },
  sep/.default=0.88pt .3 1,
  %
  swap/.code=\pgfarrowsaddtooptions{\ifpgfarrowswap\pgfarrowswapfalse\else\pgfarrowswaptrue\fi},
  reversed/.code=\pgfarrowsaddtooptions{\ifpgfarrowreversed\pgfarrowreversedfalse\else\pgfarrowreversedtrue\fi},
  harpoon/.is choice,
  harpoon/.default=true,
  harpoon/true/.code=\pgfarrowsaddtooptions{\pgfarrowharpoontrue},
  harpoon/false/.code=\pgfarrowsaddtooptions{\pgfarrowharpoonfalse},
  left/.style={harpoon},
  right/.style={harpoon,swap},
  %
  color/.code=\pgfarrowsaddtooptions{\def\pgf@arrows@stroke@color{#1}},
  fill/.code={%
    \def\pgf@temp{#1}%
    \ifx\pgf@temp\pgf@nonetext%
      \pgfarrowsaddtooptions{\pgfarrowopentrue}
    \else
      \pgfarrowsaddtooptions{\pgfarrowopenfalse\def\pgf@arrows@fill@color{#1}}
    \fi
  },
  fill/.value required,
  open/.style={fill=none},
  .unknown/.code={
    \expandafter\pgfutil@in@\expandafter!\expandafter{\pgfkeyscurrentname}%
    \ifpgfutil@in@%
      % this is a color!
      \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgf@arrows@stroke@color\expandafter{\pgfkeyscurrentname}}%
    \else%
      \pgfutil@doifcolorelse{\pgfkeyscurrentname}
      {%
        \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgf@arrows@stroke@color\expandafter{\pgfkeyscurrentname}}%
      }
      {%
        \edef\pgf@temp{\pgfkeyscurrentname}%
        \pgfkeys{/errors/unknown key/.expand once=\expandafter{\pgf@temp}{#1}}%
      }
      \fi
    }
}
\def\pgf@nonetext{none}

\def\pgfarrowsaddtooptions#1{\expandafter\def\expandafter\pgf@arrows@options\expandafter{\pgf@arrows@options#1}}
\def\pgfarrowsaddtolateoptions#1{\expandafter\def\expandafter\pgf@arrows@options\expandafter{\pgf@arrows@options\pgf@arrows@add@to@late@options{#1}}}
\def\pgf@arrows@add@to@late@options#1{\expandafter\def\expandafter\pgf@arrows@late@options\expandafter{\pgf@arrows@late@options#1}}



\def\pgfarrowsthreeparameters#1{%
  \pgfarrowsthreeparameters@#1 +0 +0 +0 \pgf@stop%
}
\def\pgfarrowsthreeparameters@#1 #2 #3 #4\pgf@stop{%
  \pgfmathsetlength\pgf@x{#1}%
  \pgfmathsetmacro\pgf@temp@a{#2}%
  \pgfmathsetmacro\pgf@temp@b{#3}%
  \edef\pgfarrowstheparameters{{\the\pgf@x}{\pgf@temp@a}{\pgf@temp@b}}%
}

\def\pgfarrowsfourparameters#1{%
  \pgfarrowsfourparameters@#1 +0 +0 +0 \pgf@stop%
}
\def\pgfarrowsfourparameters@#1:#2 #3 #4 #5\pgf@stop{%
  \pgfmathsetmacro\pgf@temp@z{#1}%
  \pgfmathsetlength\pgf@x{#2}%
  \pgfmathsetmacro\pgf@temp@a{#3}%
  \pgfmathsetmacro\pgf@temp@b{#4}%
  \edef\pgfarrowstheparameters{{\pgf@temp@z}{\the\pgf@x}{\pgf@temp@a}{\pgf@temp@b}}%
}

\def\pgfarrows@angle@setup#1#2#3#4{%
  \pgfarrowslinewidthdependent{#2}{#3}{#4}
  \pgf@xc\pgf@x
  \pgf@yc#1 pt%
  \pgf@yc.5\pgf@yc%
  \pgfpointpolar{\pgf@yc}{\pgf@xc}
  \pgfarrowlength\pgf@x%
  \pgf@y2\pgf@y%
  \expandafter\pgf@arrows@add@to@late@options\expandafter{\expandafter\pgfarrowwidth\the\pgf@y}%
}

\def\pgfarrows@angle@setup@prime#1{%
  \pgf@yc#1 pt %
  \pgf@yc=0.5\pgf@yc
  \pgfmathtan@{\pgf@sys@tonumber\pgf@yc}%
  \pgfarrowwidth\pgfmathresult\pgfarrowlength%
  \pgfarrowwidth2\pgfarrowwidth%
}

\def\pgfarrowslinewidthdependent#1#2#3{%
  \pgf@x#1%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgf@arrows@inner@line@width@dep{#2}{#3}%
  \else%
    \advance\pgf@x by#2\pgflinewidth%
  \fi%
}
\def\pgf@arrows@inner@line@width@dep#1#2{%
  % #1*((1-#2/2)*full line width - (#2/2) * inner line width)
  % Compute "real" line width
  \pgf@xa\pgflinewidth%
  \pgf@xb-.5\pgflinewidth%
  \pgf@xb#2\pgf@xb%
  \advance\pgf@xa by\pgf@xb%
  \pgf@xb\pgfinnerlinewidth%
  \pgf@xb-.5\pgf@xb
  \advance\pgf@xa by#2\pgf@xb%
  \advance\pgf@x by#1\pgf@xa%
}


\def\pgfarrowslengthdependent#1#2#3#4{%
  #4#1%
  \advance#4by#2\pgfarrowlength%
  \advance#4by#3\pgflinewidth%
}



% Build the full name:

\def\pgf@arrow@fullname#1{pgf@@ar@#1@\the\pgflinewidth @\pgfinnerlinewidth @\ifpgfarrowreversed r\fi @\pgf@arrows@stroke@color @\pgf@arrows@fill@color @\csname pgf@ar@par@#1\endcsname}
\def\pgf@arrow@id@count{0}%

% Compute the arrow id of an arrow
%
% #1 = arrow name
% #2 = options
%
% Description:
%
% Returns the an id in \pgf@arrow@id that identifies the instantiation
% of the given arrow. If the arrow was not instantiated, this happens now.

\def\pgfarrows@getid#1#2{%
  % Execute options:
  \let\pgf@arrows@late@options\pgfutil@empty%
  % 1. Defaults:
  \csname pgf@ar@defaults@#1\endcsname%
  % 2. Scope:
  \pgf@arrows@options@scope
  % 3. Local:
  #2\relax%
  % 4. Nested:
  \pgf@arrows@nested@options%
  % 5. Last options:
  \pgf@arrows@late@options%
  % 6. Scaling:
  \pgfarrows@scale@list%
  % Now, test:
  \expandafter\global\expandafter\let\expandafter\pgf@arrow@id\csname\pgf@arrow@fullname{#1}\endcsname\relax%
  \ifx\pgf@arrow@id\relax%
    \pgf@arrows@instantiate{#1}
  \fi%
}

\def\pgf@arrows@instantiate#1{%
  % Not defined. Rats!
  % Allocate new id:
  \pgfutil@tempcnta\pgf@arrow@id@count\relax%
  \advance\pgfutil@tempcnta by1\relax%
  \xdef\pgf@arrow@id@count{\the\pgfutil@tempcnta}%
  \expandafter\global\expandafter\let\csname\pgf@arrow@fullname{#1}\endcsname\pgf@arrow@id@count%
  \global\let\pgf@arrow@id\pgf@arrow@id@count%
  {%
    \pgfclearid%
    \csname pgf@ar@setup@#1\endcsname%
    % Handle reversal
    \ifpgfarrowreversed%
      % Compute transformation:
      \pgf@arrows@handle@reverse%
    \fi%
    % Save computed values
    \expandafter\global\expandafter\let\csname pgf@ar@saves@\pgf@arrow@id\endcsname\pgf@arrows@saves%
    \expandafter\global\expandafter\let\csname pgf@ar@hull@\pgf@arrow@id\endcsname\pgf@arrows@convexhull%
    \expandafter\xdef\csname pgf@ar@ends@\pgf@arrow@id\endcsname{{\pgf@arrows@the@tipend}{\pgf@arrows@the@backend}{\pgf@arrows@the@lineend}}%
    \expandafter\xdef\csname pgf@ar@visual@\pgf@arrow@id\endcsname{{\pgf@arrows@the@visualtipend}{\pgf@arrows@the@visualbackend}{}}%
    % Save code (needed for bending)
    \edef\pgf@arrow@code{%
      \ifpgfarrowreversed\noexpand\pgftransformxscale{-1}\fi%
      \expandafter\noexpand\csname pgf@ar@code@#1\endcsname%
    }%
    \expandafter\global\expandafter\let\csname pgf@ar@inst@code@\pgf@arrow@id\endcsname\pgf@arrow@code%
    % Should we cache?
    \expandafter\ifx\csname pgf@ar@do@cache@#1\endcsname\pgf@truetext%
      \pgfsysprotocol@getcurrentprotocol\pgf@arrow@temp%
      {%
        \pgfinterruptpath%
          \let\pgfusepath=\pgf@nousepath@here%
          \pgf@relevantforpicturesizefalse%
          \pgftransformreset%
          \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
          \pgfsysprotocol@bufferedtrue%
          \pgfscope%
          \pgf@arrow@code%
          \endpgfscope%
          \pgfsysprotocol@getcurrentprotocol\pgf@@arrow@temp%
          \expandafter\gdef\expandafter\pgf@arrow@code\expandafter{\expandafter\pgfsysprotocol@literal\expandafter{\pgf@@arrow@temp}}%
        \endpgfinterruptpath%
      }%
      \pgfsysprotocol@setcurrentprotocol\pgf@arrow@temp%
    \fi%
    \expandafter\global\expandafter\let\csname pgf@ar@cache@\pgf@arrow@id\endcsname\pgf@arrow@code%
  }%
}
\def\pgf@truetext{true}

% Ok, now run setup:
\def\pgf@arrows@copy@tipend{\pgf@arrows@the@tipend}
\def\pgf@arrows@copy@backend{\pgf@arrows@the@backend}
\def\pgf@arrows@copy@lineend{\pgf@arrows@the@lineend}
\def\pgf@arrows@zeropt{0pt}%

\let\pgf@arrows@saves\pgfutil@empty%
\let\pgf@arrows@convexhull\pgfutil@empty%
\let\pgf@arrows@the@tipend\pgf@arrows@zeropt%
\let\pgf@arrows@the@backend\pgf@arrows@zeropt%
\let\pgf@arrows@the@lineend\pgf@arrows@zeropt%
\let\pgf@arrows@the@visualtipend\pgf@arrows@copy@tipend%
\let\pgf@arrows@the@visualbackend\pgf@arrows@copy@backend%


\def\pgf@arrows@handle@reverse{%
  \pgf@x\pgf@arrows@the@visualtipend\pgf@x-\pgf@x%
  \pgf@y\pgf@arrows@the@visualbackend\pgf@y-\pgf@y
  \edef\pgf@arrows@the@visualtipend{\the\pgf@y}%
  \edef\pgf@arrows@the@visualbackend{\the\pgf@x}%
  \pgf@x\pgf@arrows@the@tipend\pgf@x-\pgf@x%
  \pgf@y\pgf@arrows@the@backend\pgf@y-\pgf@y
  \edef\pgf@arrows@the@tipend{\the\pgf@y}%
  \edef\pgf@arrows@the@backend{\the\pgf@x}%
  \pgf@x\pgf@arrows@the@lineend\pgf@x-\pgf@x\edef\pgf@arrows@the@lineend{\the\pgf@x}%
  \let\pgf@temp\pgf@arrows@convexhull%
  \let\pgf@arrows@convexhull\pgfutil@empty%
  \let\pgf@arrow@hull@point\pgf@arrow@hull@point@reverse%
  \pgf@temp%
}
\def\pgf@arrow@hull@point@reverse#1#2{%
  \pgf@x#1%
  \pgfarrowshullpoint{-\pgf@x}{#2}%
}

\def\pgf@nousepath@here#1{\pgferror{The definition of an arrow may not use \string\pgfusepath}}

\def\pgfarrowssavethe#1{%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgf@arrows@saves%
  \expandafter\expandafter\expandafter{\expandafter\pgf@arrows@saves\expandafter#1\the#1\relax}
}

\def\pgfarrowssave#1{%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgf@arrows@saves%
  \expandafter\expandafter\expandafter{\expandafter\pgf@arrows@saves\expandafter\def\expandafter#1\expandafter{#1}}
}

\def\pgfarrowshullpoint#1#2{%
  \pgf@x#1\relax%
  \pgf@y#2\relax%
  \edef\pgf@arrows@temp{\noexpand\pgf@arrows@convexhull\noexpand\pgf@arrow@hull@point{\the\pgf@x}{\the\pgf@y}}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgf@arrows@convexhull\expandafter\expandafter\expandafter{\pgf@arrows@temp}%
}

\def\pgfarrowsupperhullpoint#1#2{%
  \pgf@x#1\relax%
  \pgf@y#2\relax%
  \ifdim\pgf@y>0pt
    \edef\pgf@arrows@temp{\noexpand\pgf@arrows@convexhull\noexpand\pgf@arrow@hull@point{\the\pgf@x}{\the\pgf@y}\ifpgfarrowharpoon\else\noexpand\pgf@arrow@hull@point{\the\pgf@x}{-\the\pgf@y}\fi}%
  \else
    \edef\pgf@arrows@temp{\noexpand\pgf@arrows@convexhull\noexpand\pgf@arrow@hull@point{\the\pgf@x}{\the\pgf@y}}%
  \fi
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgf@arrows@convexhull\expandafter\expandafter\expandafter{\pgf@arrows@temp}%
}

\def\pgfarrowssettipend#1{\pgf@x#1\edef\pgf@arrows@the@tipend{\the\pgf@x}}
\def\pgfarrowssetbackend#1{\pgf@x#1\edef\pgf@arrows@the@backend{\the\pgf@x}}
\def\pgfarrowssetlineend#1{\pgf@x#1\edef\pgf@arrows@the@lineend{\the\pgf@x}}
\def\pgfarrowssetvisualtipend#1{\pgf@x#1\edef\pgf@arrows@the@visualtipend{\the\pgf@x}}
\def\pgfarrowssetvisualbackend#1{\pgf@x#1\edef\pgf@arrows@the@visualbackend{\the\pgf@x}}


% Internal computation of the line end (shortening) for an arrow
%
% #1 = arrow tip list
%
% Description:
%
% \pgf@xa will contain the necessary path shortening for the given
% arrow tip list, \pgf@xb will contain the total length of the arrow
% tip list (sum of the differences between tip end and back end plus
% the seps).

\def\pgf@arrow@compute@shortening#1{%
  \let\pgf@arrow@handle\pgf@arrow@compute@shortening@
  \let\pgf@arrow@handle@dot\pgf@arrow@after@line@endtrue%
  \pgf@arrow@after@line@endfalse%
  \pgf@xa0pt%
  \pgf@xb0pt%
  #1%
}
\newif\ifpgf@arrow@after@line@end

\def\pgf@arrow@compute@shortening@#1#2{%
  {\pgfarrows@getid{#1}{#2}\ifnum\pgf@arrow@flex@mode>0\relax\global\pgf@precise@shorteningtrue\fi\expandafter}\expandafter\pgf@x\the\pgfarrowsep%
  \expandafter\expandafter\expandafter\pgf@arrow@cont@short\csname pgf@ar@ends@\pgf@arrow@id\endcsname%
}
\def\pgf@dot@text{.}

\def\pgf@arrow@cont@short#1#2#3{% tip end, back end, line end, sep
  \advance\pgf@xb by#1%
  \pgf@xc#2%
  \advance\pgf@xb by-\pgf@xc%
  \advance\pgf@xb by\pgf@x%
  \ifpgf@arrow@after@line@end%
    \advance\pgf@xa by#1%
    \advance\pgf@xa by\pgf@x%
    \pgf@xc#2%
    \advance\pgf@xa by-\pgf@xc%
  \else%
    \pgf@xa#1%
    \advance\pgf@xa by\pgf@x%
    \pgf@xc#3%
    \advance\pgf@xa by-\pgf@xc%
  \fi%
}



\def\pgf@arrow@rigid@arrow#1#2{%
  {%
    \pgf@xb=#2%
    \pgftransformxshift{-\pgf@xb}%
    \let\pgf@arrow@handle\pgf@arrow@rigid
    \let\pgf@arrow@handle@dot\relax%
    #1%
  }%
}


\def\pgf@arrow@rigid#1#2{%
  % Prepare:
  {%
    \pgfarrows@getid{#1}{#2}%
    % Do shift:
    \expandafter\expandafter\expandafter\pgf@arrow@drawer@shift\csname pgf@ar@ends@\pgf@arrow@id\endcsname%
    % Do slant:
    \ifdim\pgfarrows@slant pt=0pt%
    \else%
      \pgftransformxslant{\pgfarrows@slant}%
    \fi%
    % do swap:
    \ifpgfarrowswap%
      \pgftransformyscale{-1}%
    \fi%
    {%
      \csname pgf@ar@saves@\pgf@arrow@id\endcsname%
      \pgf@arrows@rigid@hull%
    }%
  \expandafter}%
  % Transform to next tip:
  \expandafter\pgftransformxshift\expandafter{\the\pgf@xc}%
}




% Draw an arrow
%
% #1 = arrow tip list
% #2 = total length of the arrow (the value of \pgf@xb computed by
% \pgf@arrow@compute@shortening)
%
% Description:
%
% Draws an arrow tip list. The coordinate system must have been
% transformed so that the to-be-drawn arrow points right and should
% "end" at the origin.

\def\pgf@arrow@draw@arrow#1#2{%
  {%
    \pgf@xb=#2%
    \pgftransformxshift{-\pgf@xb}%
    \let\pgf@arrow@handle\pgf@arrow@drawer
    \let\pgf@arrow@handle@dot\relax%
    #1%
  }%
}


\def\pgf@arrow@drawer#1#2{%
  % Prepare:
  {%
    \pgfarrows@getid{#1}{#2}%
    % Do shift:
    \expandafter\expandafter\expandafter\pgf@arrow@drawer@shift\csname pgf@ar@ends@\pgf@arrow@id\endcsname%
    % Do slant:
    \ifdim\pgfarrows@slant pt=0pt%
    \else%
      \pgftransformxslant{\pgfarrows@slant}%
    \fi%
    % do swap:
    \ifpgfarrowswap%
      \pgftransformyscale{-1}%
    \fi%
    {%
      \csname pgf@ar@saves@\pgf@arrow@id\endcsname%
      \pgfscope%
        \pgf@arrows@color@setup%
        \pgflowlevelsynccm\csname pgf@ar@cache@\pgf@arrow@id\endcsname%
      \endpgfscope%
      \pgf@arrows@rigid@hull%
    }%
  \expandafter}%
  % Transform to next tip:
  \expandafter\pgftransformxshift\expandafter{\the\pgf@xc}%
}

\def\pgf@arrows@color@setup@restore@std@colors{%
  % we want to allow 'arrows={fill=pgffillcolor}'. To this end, we have to ensure that \string\color@pgffillcolor is known.
  % we can safely keep the macro in the current TeX group since it has global character anyway.
  %
  % Note that declaring \string\color@pgfstrokecolor as \global macro causes save stack issues and should be avoided.
  \pgfutil@namelet{\string\color@pgfstrokecolor}{pgf@strokecolor@global}%
  \pgfutil@namelet{\string\color@pgffillcolor}{pgf@fillcolor@global}%
  %
}%

\def\pgf@arrows@color@setup{%
  \ifx\pgf@arrows@stroke@color\pgfutil@empty\else\pgfsetstrokecolor{\pgf@arrows@stroke@color}\fi%
  \ifx\pgf@arrows@fill@color\pgfutil@empty%
    \ifx\pgf@strokecolor@global\pgf@fillcolor@global
    \else
      \pgf@arrows@color@setup@restore@std@colors
      \pgfsetfillcolor{pgfstrokecolor}%
    \fi%
  \else%
    \pgf@arrows@color@setup@restore@std@colors
    \pgfsetfillcolor{\pgf@arrows@fill@color}%
  \fi%
}

\def\pgf@arrow@drawer@shift#1#2#3{% tip end, back end, line end, sep
  \pgf@xb#2\pgftransformxshift{-\pgf@xb}%
  \pgf@xc#1%
  \advance\pgf@xc by\pgfarrowsep%
  \advance\pgf@xc by-\pgf@xb%
}

\def\pgf@arrows@rigid@hull{%
  \ifpgf@relevantforpicturesize%
    % Do bb update:
    \expandafter\let\expandafter\pgf@temp\csname pgf@ar@hull@\pgf@arrow@id\endcsname%
    \ifx\pgf@temp\pgfutil@empty\else%
      \let\pgf@arrow@hull@point\pgf@arrow@hull@point@first%
      \pgf@temp%
      \pgf@arrow@update@bb%
    \fi%
  \fi
}


% Convex hull stuff:

\def\pgf@arrow@hull@point@first#1#2{%
% {\pgfsys@beginscope\pgfpathcircle{\pgfqpoint{#1}{#2}}{0.5pt}\pgfusepathqfill\pgfsys@endscope}%
  \pgf@x#1\pgf@y#2%
  \pgf@xa\pgf@pt@aa\pgf@x%
  \advance\pgf@xa by\pgf@pt@ba\pgf@y%
  \pgf@ya\pgf@pt@ab\pgf@x%
  \advance\pgf@ya by\pgf@pt@bb\pgf@y%
  \pgf@xb\pgf@xa\pgf@yb\pgf@ya%
  \let\pgf@arrow@hull@point\pgf@arrow@hull@point@other%
}
\def\pgf@arrow@hull@point@other#1#2{%
%  {\pgfsys@beginscope\pgfpathcircle{\pgfqpoint{#1}{#2}}{0.5pt}\pgfusepathqfill\pgfsys@endscope}%
  \pgfutil@tempdima#1\pgfutil@tempdimb#2%
  \pgf@x\pgf@pt@aa\pgfutil@tempdima%
  \advance\pgf@x by\pgf@pt@ba\pgfutil@tempdimb%
  \pgf@y\pgf@pt@ab\pgfutil@tempdima%
  \advance\pgf@y by\pgf@pt@bb\pgfutil@tempdimb%
  \ifdim\pgf@x<\pgf@xa\pgf@xa\pgf@x\else\ifdim\pgf@x>\pgf@xb\pgf@xb\pgf@x\fi\fi%
  \ifdim\pgf@y<\pgf@ya\pgf@ya\pgf@y\else\ifdim\pgf@y>\pgf@yb\pgf@yb\pgf@y\fi\fi%
}

\def\pgf@arrow@update@bb{%
  \advance\pgf@xa by\pgf@pt@x%
  \advance\pgf@ya by\pgf@pt@y%
  \advance\pgf@xb by\pgf@pt@x%
  \advance\pgf@yb by\pgf@pt@y%
  \ifdim\pgf@picmaxx=-16000pt\relax%
    \global\pgf@picminx\pgf@xa%
    \global\pgf@picmaxx\pgf@xb%
    \global\pgf@picminy\pgf@ya%
    \global\pgf@picmaxy\pgf@yb%
  \else%
    \ifdim\pgf@xa<\pgf@picminx\global\pgf@picminx\pgf@xa\fi%
    \ifdim\pgf@ya<\pgf@picminy\global\pgf@picminy\pgf@ya\fi%
    \ifdim\pgf@xb>\pgf@picmaxx\global\pgf@picmaxx\pgf@xb\fi%
    \ifdim\pgf@yb>\pgf@picmaxy\global\pgf@picmaxy\pgf@yb\fi%
  \fi%
}



% Sets arrows
%
% #1 = An arrow specification of the form
%      <start spec>-<end spec>. This will call \pgfsetstartarrow{start
%        spec} and \pgfsetendarrow{end spec}.
%
%      Alternatively, it may be of the form [options]. In this case,
%      the arrow options are set for the local scope and all arrows in
%      the current scope will have these options set.
%
% Example:
%
% \pgfsetarrows{-to}

\def\pgfsetarrows#1{\pgf@arrows#1\pgf@stop}
\def\pgf@arrows{\pgfutil@ifnextchar[\pgf@arrows@test@opt\pgf@arrows@}%}
\def\pgf@arrows@#1-#2\pgf@stop{%
  \pgfsetarrowsstart{#1}%
  \pgfsetarrowsend{#2}%
}
\def\pgf@arrows@test@opt[{%
  \pgfutil@ifnextchar-{\pgf@arrows@[}%} go back to normal reading for compat. reasons.
  \pgf@arrows@test@opt@%
}
\def\pgf@arrows@test@opt@#1]{%
  \pgfutil@ifnextchar\pgf@stop{%
    \let\pgf@arrows@options\pgf@arrows@options@scope%
    \pgfkeys{/pgf/arrow keys/.cd,#1}%
    \let\pgf@arrows@options@scope\pgf@arrows@options%
    % Ok, setup the options
    \pgfutil@gobble%
  }{%
    \pgf@arrows@[#1]% Oops: go back to normal mode
  }%
}

\let\pgf@arrows@options@scope\pgfutil@empty




%
% Predefined arrows:
%


% A dot is used to indicate the end of the line:

\pgfdeclarearrow{
  name = .,
  drawing code =
}


% An underscore adds a space as in >_> or >_ >. However, it will be
% faster to say ">[sep] >" or ">[sep=2pt] >".

\pgfdeclarearrow{
  name = _,
  defaults = {sep},
  drawing code =
}



% Default shorthands:

\pgfdeclarearrow{ name = To,  means = } % forward declaration
\pgfdeclarearrow{ name = Bar, means = } % forward declaration
\pgfkeys{
  <-> /.tip           = {To},
  >-< /.tip           = {>[reversed]},
  | /.tip             = {Bar}
}



% Compatibility with old arrow system:

\pgfkeys {}

\def\pgf@arrows@direct@def#1#2{\expandafter\pgf@arrows@direct@def@\expandafter{\csname pgf@ar@means@#2\endcsname}{#1}}
\def\pgf@arrows@direct@def@#1#2{\expandafter\def\csname pgf@arrows@direct@name@#2\endcsname{\pgf@arrow@handle@shorthand@empty{#1}}}
\pgf@arrows@direct@def{start@[}{]}
\pgf@arrows@direct@def{start@]}{[}
\pgf@arrows@direct@def{start@spaced [}{spaced ]}
\pgf@arrows@direct@def{start@spaced ]}{spaced [}
\pgf@arrows@direct@def{end@[}{[}
\pgf@arrows@direct@def{end@]}{]}
\pgf@arrows@direct@def{end@spaced [}{spaced [}
\pgf@arrows@direct@def{end@spaced ]}{spaced ]}

\def\pgfsetarrowoptions#1#2{\expandafter\def\csname pgf@arrow@compat@opt@#1\endcsname{#2}}
\def\pgfgetarrowoptions#1{\csname pgf@arrow@compat@opt@#1\endcsname}
\def\pgfarrowsdeclare#1#2#3#4{%
  \pgfdeclarearrow{ name  ={#1}-{#2}, setup code ={#3}, drawing code={#4}, parameters/.expand once={\csname pgf@arrow@compat@opt@#2\endcsname}}%
  \expandafter\def\csname pgf@arrow@compat@opt@#2\endcsname{0}}
\def\pgfarrowsleftextend#1{\pgfmathsetlength\pgf@xa{#1}\pgfarrowssetbackend{\pgf@xa}}
\def\pgfarrowsrightextend#1{\pgfmathsetlength\pgf@xb{#1}\pgfarrowssettipend{\pgf@xb}}
\def\pgfarrowsdeclarealias#1#2#3#4{\pgfdeclarearrow{ name  ={#1}-{#2}, means ={#4} } }
\def\pgfarrowsdeclarereversed#1#2#3#4{\pgfdeclarearrow{ name ={#1}-{#2}, means={{#4}[reversed]}}}
\def\pgfarrowsdeclarecombine{\pgfutil@ifnextchar*{\pgfarrowsdeclarecombine@star}{\pgf@@arrowsdeclarecombine}}
\def\pgf@@arrowsdeclarecombine{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine}{\pgf@arrowsdeclarecombine[0pt]}}
\def\pgf@arrowsdeclarecombine[#1]#2#3#4#5#6#7{\def\pgf@@temp{#1}\ifx\pgf@@temp\pgf@linewidthtext\def\pgf@@temp{+0pt 1}\fi%
  \pgfdeclarearrow{name ={#2}-{#3}, means={#5[sep/.expand once=\pgf@@temp]#6}}}
\def\pgf@linewidth@text{\pgflinewidth}
\def\pgfarrowsdeclarecombine@star*{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine@star}{\pgf@arrowsdeclarecombine@star[0pt]}}
\def\pgf@arrowsdeclarecombine@star[#1]#2#3#4#5#6#7{\def\pgf@@temp{#1}\ifx\pgf@@temp\pgf@linewidthtext\def\pgf@@temp{+0pt 1}\fi%
  \pgfdeclarearrow{name ={#2}-{#3}, means={#5[sep/.expand once=\pgf@@temp].#6}}}
\def\pgfarrowsdeclaredouble{\pgfutil@ifnextchar[{\pgf@arrowsdeclaredouble}{\pgf@arrowsdeclaredouble[0pt]}}
\def\pgf@arrowsdeclaredouble[#1]#2#3#4#5{\pgfarrowsdeclarecombine[#1]{#2}{#3}{#4}{#5}{#4}{#5}}
\def\pgfarrowsdeclaretriple{\pgfutil@ifnextchar[{\pgf@arrowsdeclaretriple}{\pgf@arrowsdeclaretriple[0pt]}}
\def\pgf@arrowsdeclaretriple[#1]#2#3#4#5{ \pgfarrowsdeclarecombine[#1]{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}{#4}{#5}%
  \pgfarrowsdeclarecombine[#1]{#2}{#3}{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}}
\def\pgf@linewidthtext{\pgflinewidth}

\pgfarrowsdeclare{stealth}{stealth}
{
  \pgfutil@tempdima=0.28pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}
  \pgfarrowsrightextend{+5\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfpathmoveto{\pgfqpoint{5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqfill
}
\pgfarrowsdeclarereversed{stealth reversed}{stealth reversed}{stealth}{stealth}
\pgfarrowsdeclare{to}{to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}
\pgfkeys{To /.tip = to}
\pgfarrowsdeclare{to reversed}{to reversed}
{
  \pgfutil@tempdima=-0.21pt%
  \advance\pgfutil@tempdima by-0.475\pgflinewidth%
  \pgfutil@tempdimb=0.98pt%
  \advance\pgfutil@tempdimb by1.45\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{+0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{3.5\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.25\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{-0.25\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{3.25\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}
\pgfarrowsdeclare{latex}{latex}
{
  \pgfutil@tempdima=0.28pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfarrowsleftextend{+-1\pgfutil@tempdima}
  \pgfarrowsrightextend{+9\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfpathmoveto{\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{6.3333\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{2\pgfutil@tempdima}{2\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-1\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{2\pgfutil@tempdima}{-2\pgfutil@tempdima}}
  {\pgfqpoint{6.3333\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfusepathqfill
}
\pgfarrowsdeclarereversed{latex reversed}{latex reversed}{latex}{latex}
\pgfarrowsdeclare{@bar}{@bar}
{
  \pgfarrowsleftextend{+-0.25\pgflinewidth}
  \pgfarrowsrightextend{+.75\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetrectcap
  \pgfpathmoveto{\pgfqpoint{0.25\pgflinewidth}{-\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.25\pgflinewidth}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}
\pgfkeys{Bar /.tip = @bar}
\pgfarrowsdeclare{space}{space}
{
  \pgfutil@tempdima=0.88pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{0pt}
  \pgfarrowsrightextend{\pgfutil@tempdima}
}
{}



\endinput


==> pgfcoreexternal.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreexternal.code.tex}



\newif\ifpgfexternal@aux@in@dpth
\newif\ifpgfexternal@info

\pgfkeys{
    /pgf/images/include external/.code={\pgfimage{#1}},
    /pgf/images/aux in dpth/.is if=pgfexternal@aux@in@dpth,
    /pgf/images/aux in dpth/.default=true,
    /pgf/images/trim external/.code n args={4}{%
        \def\pgf@external@kern@left{#1}%
        \def\pgf@external@kern@bottom{#2}%
        \def\pgf@external@kern@right{#3}%
        \def\pgf@external@kern@top{#4}%
        \ifx\pgf@external@kern@left\pgfutil@empty\def\pgf@external@kern@left{0sp}\fi%
        \ifx\pgf@external@kern@bottom\pgfutil@empty\def\pgf@external@kern@bottom{0sp}\fi%
        \ifx\pgf@external@kern@right\pgfutil@empty\def\pgf@external@kern@right{0sp}\fi%
        \ifx\pgf@external@kern@top\pgfutil@empty\def\pgf@external@kern@top{0sp}\fi%
    },
    /pgf/images/trim external={1truein}{1truein}{1truein}{1truein},
    /pgf/images/external info/.is if=pgfexternal@info,
    /pgf/images/external info/.default=true,
}

% The external read/write mechanism is used as follows:
%
% In your document, you put a number or all of your pgfpicture (or
% tikzpicture) environments inside a pair of \beginpgfexternal and
% \endpgfexternal. The \beginpgfexternal gets one parameter called the
% graphics name.
%
% Once this is done, the next step is to declare the names of your
% graphics in the document at the beginning using the
% \pgfdeclaregraphicname command.
%
% Now, when you typeset your document, each time a \beginpgfexternal
% command is encountered, it will be checked whether the corresponding
% graphics file exists. If this is the case, it will be included and
% the code between \beginpgfexternal and \endpgfexternal is
% ignored. Otherwise, the code is executed normally.
%
% Things change when you run tex on your file with the \jobname set to
% the name of a declared graphics name. In this case, only your
% graphic will be typeset, the rest of the document will be "thrown away".
% To be more precise, everything is gobbled up to the beginning
% of the first \beginpgfexternal with the given graphics name. Then,
% the content of the "environment" is put in a box (this "environment"
% need not contain a graphics, it may contain anything that can be put
% in a box). Then a single page is output whose size is exactly the
% size of the picture.
%
% So, once you have run tex repeatedly, each time with the jobname set
% to each of the graphics, you can then run tex on the whole document
% and this will cause all graphics to be included rather than begin
% typeset.
%
% Finally, once all the graphics have been created, you can also say
% \input pgfexternal.tex instead of including pgf/TikZ.


\newif\ifpgfexternalreadmainaux
\pgfexternalreadmainauxtrue

% Tells pgf which jobname is the name of the real file
%
% #1 = name
%
% Description:
%
% This command is used to tell pgf that the file named #1 should be
% typeset normally. If \jobname is not equal to #1, only
% the graphic called \jobname will be typeset.
%
% Example:
%
% \pgfrealjobname{survey}
%
% Note that afterwards, \jobname will be set to the argument. In our
% example, \jobname will be 'survey'. This is to accomplish
% compatibility with aux-file generation.

\def\pgfrealjobname#1{%
  \global\let\pgfactualjobname=\jobname
  \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
  \edef\pgf@tempb{\expandafter\string\csname\jobname\endcsname}%
  \ifx\pgf@tempa\pgf@tempb%
  \else%
    \pgf@external@grabshipouttrue%
    \pgfexternal@nofiles% see also \pgf@external@init@aux@in@dpth
    \ifpgfexternalreadmainaux
        % and reset the jobname. This should allow to handle any
        % \label/\ref constructions which are stored in \jobname.aux (and
        % which won't be found otherwise)
        \gdef\jobname{#1}%
    \fi
    \ifpgfexternal@aux@in@dpth
        \csname newwrite\endcsname\w@pgfexternal@auxout
    \fi
    \pgfexternal@geometry@compatibility
  \fi%
  \gdef\pgfrealjobname##1{}% avoid multiple calls.
}

\def\pgfexternal@geometry@compatibility{%
    % check if \usepackage{geometry} is loaded:
    \pgfutil@ifundefined{geometry}{%
    }{%
        % The geometry package hooks into \begin{document}, evaluates
        % its driver -- and generates \special instructions to set the
        % paper size.
        %
        % Unfortunately, this confuses dvips utterly - and perhaps
        % other drivers as well.
        %
        % Thus, if we currently about to generate some external
        % graphics, we WANT to disable geometry (it has no purpose in
        % this context anyway).
        %
        % This here works well:
        \pgf@typeout{Package TikZ externalization: calling \string\geometry{driver=none} during externalization.^^J}%
        \geometry{driver=none}%
    }%
}%

\def\pgfexternal@nofiles{%
    % replace \relax. The \nofiles macros does
    % \let\makeglossary=\relax
    % but the glossary.sty calls \renewcommand\makeglossary (which
    % will fail if \makeglossary=\relax). Stupid, but it works.
    \let\pgfexternal@nofiles@=\relax
    \def\relax{\relax}%
    %
    % suppress generation of LaTeX .aux, .toc etc files.
    % generation of these files is not thread-safe.
    % the \csname \endcsname yields \relax if \nofiles doesn't exist.
    \csname nofiles\endcsname
    %
    \let\relax=\pgfexternal@nofiles@
}%

\newif\ifpgf@external@grabshipout
\newbox\pgfexternal@startupbox

\pgfutil@ifundefined{AtBeginDocument}{}{%
    \AtBeginDocument{%
      \ifpgf@external@grabshipout%
        \global\let\pgfexternal@originalshipout=\shipout%
        \global\def\shipout{\setbox\pgfpic=}%
        \maxdeadcycles=10000%
        % Ok, gather everything we have seen up to now in a box. This box
        % will contain any specials that have been used.
        {%
          \output{\global\setbox\pgfexternal@startupbox=\vbox{\csname @begindvi\endcsname\unvbox255}}%
          \hbox{}\eject%
        }%
      \fi%
    }
}%

\pgfutil@ifundefined{AtEndDocument}{}{%
    \AtEndDocument{%
      \ifpgf@external@grabshipout
        \pgfutil@ifundefined{pgfexternal@did@a@shipout}{%
          \pgfexternal@error@no@shipout
        }{}%
      \fi
    }%
}

% This will be overwritten by the tikz external lib if it is loaded.
\def\pgfexternal@error@no@shipout{%
    \pgferror{Sorry, image externalization failed: the resulting image was EMPTY. I tried to externalize '\pgfactualjobname'. Perhaps there was a typo somewhere? Please check that your document contains '\string\beginpgfgraphicnamed{\pgfactualjobname} ... \string\endpgfgraphicnamed'}%
}%


% "Environment" for an external graphic.
%
% #1 = graphic name
%
% Example:
%
% \beginpgfgraphicnamed{main-graphic2}
%   \begin{tikzpicture}
%     ...
%   \end{tikzpicture}
% \endpgfgraphicnamed

\def\pgf@externalbegin#1{%
  % First, check whether we wish to grab this graphic:
  \let\pgf@next=\pgf@external@normal%
  \ifpgf@external@grabshipout%
    \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
    \edef\pgf@tempb{\expandafter\string\csname\pgfactualjobname\endcsname}%
    \ifx\pgf@tempa\pgf@tempb%
      \let\pgf@next=\pgf@external@grab%
    \fi%
  \fi%
  \pgf@next{#1}%
}


\AtBeginDocument{
  \let\beginpgfgraphicnamed=\pgf@externalbegin% overwrite definition of pgfexternal.tex if necessary
  \let\endpgfgraphicnamed=\unskip
}


% Normal operation: Include an external graphic instead of the
% picture, if such an external picture exists.
\def\pgf@external@normal#1{%
  \let\pgf@filename=\pgfutil@empty%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#1}%
  \ifx\pgf@filename\pgfutil@empty%
    % Ok, no such image... Just typeset the picture normally.
    \let\pgf@next=\relax%
  \else%
    \let\pgf@next=\pgf@replacepicturebygraphic%
  \fi%
  \pgf@next%
}

\long\def\pgf@replacepicturebygraphic#1\endpgfgraphicnamed{%
    \expandafter\pgfincludeexternalgraphics\expandafter{\pgf@filename}\unskip
}

% This is almost the same as \includegraphics{#1}, but it checks
% whether '#1.dpth' exists. In such case, it restores the boxes depth
% stored in #1.dpth.
%
% Furthermore, the .dpth file may contain .aux related information
% collected for the external graphics (references). They start after
% the first line (if any).
\def\pgfincludeexternalgraphics#1{%
    \begingroup
    \pgfexternalreaddpth{#1}%
    \pgfkeysifdefined{/pgf/images/include external/#1/.@cmd}{%
        \pgfkeysgetvalue{/pgf/images/include external/#1/.@cmd}\pgf@tempa
        \pgfkeyslet{/pgf/images/include external/.@cmd}\pgf@tempa
    }{}%
    \setbox1=\hbox{\pgfkeysvalueof{/pgf/images/include external/.@cmd}{#1}\pgfeov}%
    \ifdim\pgfexternaltrimleft=0sp \else \kern\pgfexternaltrimleft\relax \fi
    \ifdim\pgfexternaldepth=0pt
        \box1
    \else
        \dimen0=\pgfexternaldepth\relax
        \hbox{\lower\dimen0 \box1 }%
    \fi
    \ifdim\pgfexternaltrimright=0sp \else \kern\pgfexternaltrimright\relax \fi
    \endgroup
}

% Reads the .dpth file which contains meta data of the external
% picture.
%
% This command handles the following stuff:
% - it defines \pgfexternaldepth . The macro contains the contents of
%   a line which does not start with a control sequence (for example a
%   line containing '50pt')
% - it defines \pgfexternaltrimleft and \pgfexternaltrimright
% - it checks if the .dpth file contains content stored by means of
%   \pgfexternalstorecommand. If so, the argument of
%   \pgfexternalstorecommand will be restored.
% - anything else will be appended to the main .aux file, assuming that
%   it contains \label or \ref information (only if the LaTeX switch
%   \if@filesw is \iftrue).
%
%
% #1: the image file name (such that #1.dpth exists)
\def\pgfexternalreaddpth#1{%
    % no \begingroup. Handle that manually:
    \edef\pgfexternalreaddpth@restore{%
        \noexpand\endlinechar=\the\endlinechar\space
        \noexpand\catcode`\noexpand\@=\the\catcode`\@\space
    }%
    %
    \def\pgfexternaldepth{0sp}%
    \def\pgfexternaltrimleft{0sp}%
    \def\pgfexternaltrimright{0sp}%
    \endlinechar=-1 % suppress white space at end
    \catcode`\@=11
    \openin\r@pgf@reada=#1.dpth
    \pgfincludeexternalgraphics@read@dpth
    %
    \pgfexternalreaddpth@restore
}%
%
% The .dpth consists of 0-N lines, where each is either a single
% dimension (the box' depth) or something which belongs to the .aux
% file (such lines will always start with a macro).
\def\pgfincludeexternalgraphics@read@dpth{%
    \ifeof\r@pgf@reada
        \closein\r@pgf@reada
    \else
        \read\r@pgf@reada to\pgfincludeexternalgraphics@auxline
        \ifx\pgfincludeexternalgraphics@auxline\pgfutil@empty
        \else
            \expandafter\pgfincludeexternalgraphics@read@dpth@line\pgfincludeexternalgraphics@auxline\pgfincludeexternalgraphics@read@dpth@line@EOI
        \fi
        \expandafter\pgfincludeexternalgraphics@read@dpth
    \fi
}%

\def\pgfexternal@restore#1{#1}%

\long\def\pgfincludeexternalgraphics@read@dpth@line@getfirst#1#2\pgfincludeexternalgraphics@read@dpth@line@EOI{%
    \def\pgf@first{#1}%
}%
\long\def\pgfincludeexternalgraphics@read@dpth@line#1\pgfincludeexternalgraphics@read@dpth@line@EOI{%
    \pgfincludeexternalgraphics@read@dpth@line@getfirst#1\pgfincludeexternalgraphics@read@dpth@line@EOI
    \expandafter\ifcat\expandafter\noexpand\pgf@first\relax
        % Ah -- the first token is a control sequence. It belongs to
        % the .aux file.
        %
        \expandafter\ifx\pgf@first\pgfexternal@restore
            % if the first line in the .dpth file starts with the
            % magic string \pgfexternal@restore, the complete line
            % will be executed as-is. Example:
            % \pgfexternal@restore{\def\somevalue{1}}
            #1%
        \else
            % do NOT execute #1! many LaTeX commands don't support it (\label for example)
            \pgfutil@ifundefined{if@filesw}{%
                % sorry, .aux file support only for latex
            }{%
                % append to main .aux file (for forward references)
                \if@filesw
                    {%
                    \toks0={#1}%
                    % believe it or not, but the
                    % \def\dpthimport{...}\dpthimport *makes* a
                    % difference! In ensures any occurring `##' characters are properly expanded to `#'.
                    \immediate\write\@auxout{%
                        \noexpand\def\noexpand\dpthimport{\the\toks0}\noexpand\dpthimport}%
                    }%
                \fi
            }%
        \fi
    \else% it is the depth (which is simply a number for backwards compatibility)
        \def\pgfexternaldepth{#1}%
    \fi
}%

% Stores '#1' (expanded!) into the .dpth file of the currently
% exported image.
%
% This command has only an effect if an image is being exported.
%
% The stored contents will be read in the context where
% /pgf/images/include external is active (i.e. by
% \pgfexternalreaddpth).
%
\def\pgfexternalstorecommand#1{%
}%
\def\pgfexternalstorecommand@isexporting#1{%
    \immediate\write\w@pgfexternal@auxout{\noexpand\pgfexternal@restore{#1}}%
}%



% Grab operation: If jobname matches the graphic name, typeset this
% picture normal.
% REMARK:
%   this method is also invoked from within the tikz external library.
\def\pgf@external@grab#1{%
  \def\pgf@filename{#1}%
  \ifpgfexternal@aux@in@dpth
    \begingroup
    \pgf@external@init@aux@in@dpth
    \let\G@refundefinedtrue=\pgf@external@grab@refundefinedtrue
  \fi
  \gdef\pgf@trimleft@final{0sp}%
  \gdef\pgf@trimright@final{0sp}%
  \setbox\pgfpic=\hbox\bgroup\bgroup%
    \let\endpgfgraphicnamed=\pgf@externalend%
}

{\catcode`\^=12 \gdef\pgfexternal@hat{^}}

\expandafter\let\expandafter\pgf@external@grab@refundefinedtrue@orig\csname G@refundefinedtrue\endcsname

\def\pgf@external@grab@refundefinedtrue{%
    \pgf@external@grab@refundefinedtrue@orig
    \begingroup
    \def\n{\pgfexternal@hat\pgfexternal@hat J}%
    \pgfexternalstorecommand{%
      \pgf@external@grab@refundefinedtrue@code
      \noexpand\immediate\noexpand\write16{\pgf@external@grab@refundefinedtrue@warning}%
      \noexpand\G@refundefinedtrue
    }%
    \endgroup
}%

% A hook. will be overwritten by \usetikzlibrary{external}
\def\pgf@external@grab@refundefinedtrue@code{}

\def\pgf@external@grab@refundefinedtrue@warning{%
    LaTeX Warning: External picture `\pgfactualjobname' contains undefined references\noexpand\on@line.\n
}%

\let\pgf@external@@protected@write@orig=\protected@write
\long\def\pgf@external@@protected@write@immediate#1#2#3{%
  \begingroup
    \let\pgf@write@=\write
    \def\write{\noexpand\immediate\pgf@write@}%
    \pgf@external@@protected@write@orig{#1}{#2}{#3}%
  \endgroup
}%

\def\pgf@external@init@aux@in@dpth{%
  \let\pgfexternalstorecommand=\pgfexternalstorecommand@isexporting
  %
  % tell LaTeX to write aux files...
  \csname @fileswtrue\endcsname
  % ... but redirect output to the .dpth file!
  \immediate\openout\w@pgfexternal@auxout=\pgf@filename.dpth
  \let\@auxout=\w@pgfexternal@auxout
  % ... and disable the correct page numbers. I can't get that
  % (because the correct page number is only available in the
  % shipout routine). Use immediate output:
  \let\protected@write=\pgf@external@@protected@write@immediate
}%

\def\pgf@externalend@storeshifts#1{%
  \immediate\write#1{\the\dp\pgfpic}% store the depth simply as number for backw. compat.
  \ifx\pgf@trimleft@final\pgfutil@empty\else
    \immediate\write#1{\noexpand\pgfexternal@restore{\noexpand\def\noexpand\pgfexternaltrimleft{\pgf@trimleft@final}}}%
  \fi
  \ifx\pgf@trimright@final\pgfutil@empty\else
    \immediate\write#1{\noexpand\pgfexternal@restore{\noexpand\def\noexpand\pgfexternaltrimright{\pgf@trimright@final}}}%
  \fi
  \ifpgfexternal@info
    \immediate\write#1{\noexpand\pgfexternal@restore{\noexpand\def\noexpand\pgfexternalwidth{\the\wd\pgfpic}}}%
    \immediate\write#1{\noexpand\pgfexternal@restore{\noexpand\def\noexpand\pgfexternalheight{\the\dimen0}}}%
  \fi
}
% REMARK:
%   this method is also invoked from within the tikz external library.
\def\pgf@externalend{%
  \unskip\egroup\egroup%
  {%
    \def\pgf@external@trim{0}%
    \def\pgf@external@store@dpth{0}%
    %
    \ifpgf@trim@lowlevel
      \gdef\pgf@trimleft@final{}%
      \gdef\pgf@trimright@final{}%
    \else
      \ifdim\pgf@trimleft@final=0sp  \gdef\pgf@trimleft@final{}  \else\def\pgf@external@trim{1}\fi
      \ifdim\pgf@trimright@final=0sp \gdef\pgf@trimright@final{} \else\def\pgf@external@trim{1}\fi
      \if1\pgf@external@trim
          % UNDO the trimming! export to pdf doesn't supported trimmed
          % bounding boxes (has to do with the mediabox/trimbox etc).
          % I'll keep the bounding box intact and store the trim information
          % into the .dpth file.
          \setbox\pgfpic=\hbox{%
              \ifx\pgf@trimleft@final\pgfutil@empty\else\kern-\pgf@trimleft@final\fi
              \box\pgfpic
              \ifx\pgf@trimright@final\pgfutil@empty\else\kern-\pgf@trimright@final\fi
          }%
          \def\pgf@external@store@dpth{1}%
      \fi
    \fi
    %
    \parindent0pt % leave the space
%    \leftmargin0pt%
%    \rightmargin0pt%
    \hoffset=0pt % reset to default
    \voffset=0pt
    \dimen0\ht\pgfpic%
    \advance\dimen0\dp\pgfpic%
    \ifdim\dp\pgfpic=0pt\relax
    \else% store the picture's depth. Otherwise, it would be lost.
      \def\pgf@external@store@dpth{1}%
    \fi
    \ifpgfexternal@info
      \def\pgf@external@store@dpth{1}%
    \fi
    %
    \if1\pgf@external@store@dpth
      \ifpgfexternal@aux@in@dpth
        \pgf@externalend@storeshifts\@auxout
        \immediate\closeout\@auxout
      \else
        \immediate\openout\pgf@plotwrite=\pgf@filename.dpth
        \pgf@externalend@storeshifts\pgf@plotwrite
        \immediate\closeout\pgf@plotwrite
      \fi
    \fi
    \pgfsys@prepare@papersize{\the\wd\pgfpic}{\the\dimen0}%
    %
    \setbox0=\vbox{%
      % I admit that I don't know why there is this kerning:
      \kern -\pgf@external@kern@top\relax%
      \hbox{%
        \kern -\pgf@external@kern@left\relax%
        \hbox to0pt{%
          \wd\pgfexternal@startupbox=0pt %
          \ht\pgfexternal@startupbox=0pt %
          \dp\pgfexternal@startupbox=0pt %
          \box\pgfexternal@startupbox%
          \pgfsys@atbegindocument\hss}%
        \box\pgfpic%
        \kern\pgf@external@kern@right\relax%
      }%
      \kern\pgf@external@kern@bottom\relax%
    }%
    %
    % compatibility with eso-pic package: \nointerlineskip is not
    % allowed here, but the eso-pic package uses \nointerlineskip in
    % its shipout routine.
    \let\pgfexternal@nointerlineskip@orig=\nointerlineskip
    \let\nointerlineskip=\pgfexternal@nointerlineskip
    %
    \pgfexternal@originalshipout\box0 %
    \gdef\pgfexternal@did@a@shipout{1}%
  }%
  \ifpgfexternal@aux@in@dpth
    \endgroup
  \fi
}

\def\pgfexternal@nointerlineskip{%
    \ifvmode
      \pgfexternal@nointerlineskip@orig
    \else
      \relax% \nointerlineskip in horizontal mode not allowed. Silently ignore the error message.
    \fi
}%

\endinput
% vi: tabstop=4 shiftwidth=2 expandtab


==> pgfcoregraphicstate.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoregraphicstate.code.tex}

% Globals

\newdimen\pgflinewidth


% Set the line width to #1.
% 
% #1 = new line width.
% 
% Example:
%
% \pgfsetlinewidth{3pt}

\def\pgfsetlinewidth#1{%
  \pgfmathsetlength\pgflinewidth{#1}%
  \global\pgflinewidth=\pgflinewidth%
  \pgfsys@setlinewidth{\the\pgflinewidth}%
  \ignorespaces}


% Set the inner line width to #1.
% 
% #1 = new inner line width.
% 
% Description:
%
% The inner line width is the width of a second line that is drawn on
% top of the main stroked line. If the inner line width is 0pt, no
% inner line is drawn. The main use of inner lines is for creating
% "double" lines.
%
% Inner lines are not drawn when a path is used for clipping.
%
% The inner line width is local to the current TeX group, it is not
% part of the graphic state.
%
% Example:
%
% \pgfsetinnerlinewidth{1pt}

\def\pgfsetinnerlinewidth#1{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgfinnerlinewidth{\the\pgf@x}%
}
\def\pgfinnerlinewidth{0pt}


% Set the inner line color to #1.
%
% #1 = color for the inner line
%
% Example:
%
% \pgfsetinnerlinecolor{green} % yikes!

\def\pgfsetinnerstrokecolor#1{\def\pgfinnerstrokecolor{#1}}
\def\pgfinnerstrokecolor{white}


% Set the miter limit to #1.
% 
% #1 = new miter limit factor.
% 
% Example:
%
% \pgfsetmiterlimit{3}

\def\pgfsetmiterlimit#1{%
  \ifdim#1pt<1pt\pgferror{miter limit cannot be less than 1}\fi%
  \pgfsys@setmiterlimit{#1}%
  \ignorespaces}


% Set the dash pattern to #1 with phase #2/
% 
% #1 = a row of numbers of length of ``on'' and ``off'' points.
% #2 = a phase
% 
% Example:
%
% \pgfsetdash{}          {0pt} % solid line
% \pgfsetdash{{.1cm}}    {0pt} % long dashes
% \pgfsetdash{{1pt}{1ex}}{0pt} % dotted

\def\pgfsetdash#1#2{%
  \def\pgf@temp{}%
  \def\pgf@next{\pgf@strip}%
  \pgf@strip#1{pgf@stop}%
  \pgfmathsetlength\pgf@x{#2}%
  \pgfsys@setdash{\pgf@temp}{\the\pgf@x}%
  \ignorespaces}

\def\pgf@strip#1{%
  \def\pgf@@temp{#1}%
  \ifx\pgf@@temp\pgf@stop%
    \let\pgf@next=\relax%
  \else%
    \pgfmathsetlength\pgf@x{#1}%
    \ifx\pgf@temp\pgfutil@empty%
      \edef\pgf@temp{\the\pgf@x}%
    \else%
      \edef\pgf@temp{\pgf@temp,\the\pgf@x}%
    \fi%
  \fi\pgf@next}

\def\pgf@stop{pgf@stop}


% Set color of strokes. This will overrule the normal color.
% 
% Example:
%
% \pgfsetstrokecolor{red}

\def\pgfsetstrokecolor#1{%
  \pgfutil@colorlet{pgfstrokecolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfstrokecolor}}%
  \expandafter\let\expandafter\pgf@temp\csname\string\color@pgfstrokecolor\endcsname
  % for arrow tips:
  \global\let\pgf@strokecolor@global=\pgf@temp
  \expandafter\pgf@setstrokecolor\pgf@temp%
}
\def\pgf@setstrokecolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@stroke\endcsname\relax%
    \pgferror{Unsupported color model `#4'. Sorry}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@stroke\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

\def\pgf@uncomma#1,{%
  \def\pgf@coltest{#1}%
  \ifx\pgf@coltest\pgfutil@empty%
    \let\pgf@colnext=\relax%
  \else%
    \expandafter\def\expandafter\pgf@colmarshal\expandafter{\pgf@colmarshal{#1}}%
    \let\pgf@colnext=\pgf@uncomma%
  \fi%
  \pgf@colnext%  
}


% Set color of fills. This will overrule the normal color.
% 
% Example:
%
% \pgfsetfillcolor{gray}

\def\pgfsetfillcolor#1{%
  \pgfutil@colorlet{pgffillcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgffillcolor}}%
  \expandafter\let\expandafter\pgf@temp\csname\string\color@pgffillcolor\endcsname
  % for arrow tips:
  \global\let\pgf@fillcolor@global=\pgf@temp
  \expandafter\pgf@setfillcolor\pgf@temp
}
\def\pgf@setfillcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@fill\endcsname\relax%
    \pgferror{Unsupported color model `#4'. Sorry}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@fill\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}



% Sets both the stroke and fill color.
% 
% Example:
%
% \pgfsetcolor{blue}

\def\pgfsetcolor#1{%
  \pgfutil@colorlet{pgfstrokecolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfstrokecolor}}%
  \expandafter\let\expandafter\pgf@temp\csname\string\color@pgfstrokecolor\endcsname
  % for arrow tips:
  \global\let\pgf@strokecolor@global=\pgf@temp
  \global\let\pgf@fillcolor@global=\pgf@temp
  \expandafter\pgf@setcolor\pgf@temp%
}
\def\pgf@setcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4\endcsname\relax%
    \pgferror{Unsupported color model `#4'. Sorry}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

% Code for ensuring the stroke/fill colors are correctly reset.
\def\XC@bcolor{\pgfsys@color@reset}

% Set a butt line cap.
% 
% Example:
%
% \pgfsetbuttcap

\def\pgfsetbuttcap{\pgfsys@buttcap\ignorespaces}


% Set a round line cap.
% 
% Example:
%
% \pgfsetroundcap

\def\pgfsetroundcap{\pgfsys@roundcap\ignorespaces}


% Set a rectangular line cap.
% 
% Example:
%
% \pgfsetrectcap

\def\pgfsetrectcap{\pgfsys@rectcap\ignorespaces}


% Set a miter line join.
% 
% Example:
%
% \pgfsetmiterjoin

\def\pgfsetmiterjoin{\pgfsys@miterjoin\ignorespaces}


% Set a bevel line join.
% 
% Example:
%
% \pgfsetbeveljoin

\def\pgfsetbeveljoin{\pgfsys@beveljoin\ignorespaces}


% Set a round line join.
% 
% Example:
%
% \pgfsetroundjoin

\def\pgfsetroundjoin{\pgfsys@roundjoin\ignorespaces}


% Sets the even-odd rule for filling and clipping.
% 
% Example:
%
% \pgfseteorule

\def\pgfseteorule{\pgfsys@eoruletrue\ignorespaces}


% Sets the non-zero winding number rule for filling and clipping.
% 
% Example:
%
% \pgfsetnonzerorule

\def\pgfsetnonzerorule{\pgfsys@eorulefalse\ignorespaces}



\endinput


==> pgfcoreimage.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreimage.code.tex}



% Declare an image
%
% #1 = optional argument: width, height, page specification
% #2 = name of the image for later use
% #4 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF and .ps, .eps, .epsi for postscript.
%
% Description:
%
% This command declares an image file for later use. Even if the image
% is used several times in the document, in PDF it will only be stored
% once.
%
% Example:
%
% \pgfdeclareimage[width=2cm,page=2]{myimage}{imagefilename}

\def\pgfdeclareimage{\pgfutil@ifnextchar[{\pgf@declareimage}{\pgf@declareimage[]}}
\def\pgf@declareimage[#1]#2#3{%
  \pgfqkeys{/pgf/images}{height=,width=,page=,interpolate=false,mask=,#1}%
  % Try to find the file
  \gdef\pgf@filename{}%
  % If page= parameter is not empty, try that file first:
  \ifx\pgf@imagepage\pgfutil@empty%
  \else%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3.page\pgf@imagepage}%
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \else%
    \pgfkeys{/pgf/images/page=}% make page empty
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \pgfwarning%
    {File "#3" not found when defining image "#2".
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
    \pgf@declaredraftimage{#2}{#3}%
  \else%
    \ifpgf@draftmode%
      \pgf@declaredraftimage{#2}{#3}%
    \else%
      \pgfsys@defineimage%
    \fi%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@image@#2!\endcsname=\pgf@image%
}


\pgfkeys{
    /pgf/images/draft/.is if=pgf@draftmode,
    /pgf/images/draft/.default=true}
\pgfkeys{/pgf/images/width/.estore in=\pgf@imagewidth}
\pgfkeys{/pgf/images/height/.estore in=\pgf@imageheight}
\pgfkeys{/pgf/images/page/.estore in=\pgf@imagepage}
\pgfkeys{/pgf/images/interpolate/.cd,.code=\edef\pgf@imageinterpolate{#1},.default=true}
\let\pgf@imageinterpolate\pgfutil@empty
\pgfkeys{/pgf/images/mask/.code=%
  {%
    \edef\pgf@imagemask{#1}%
    \ifx\pgf@imagemask\pgfutil@empty%
    \else%
      \pgfutil@ifundefined{pgf@mask@#1}%
      {\pgferror{Undefined mask "#1".}%
        \edef\pgf@imagemask{}}%
      {\edef\pgf@imagemask{\csname pgf@mask@#1\endcsname}%
      }%
    \fi%
  }}


\def\pgf@findfile#1:#2+#3{%
  \pgfutil@IfFileExists{#3#1}%
  {\xdef\pgf@filename{#3#1}}%
  {\def\pgf@mightbeempty{#2}%
    \ifx\pgf@mightbeempty\pgfutil@empty\else%
    \pgf@findfile#2+{#3}%
    \fi}}

% #1: image name
% #2: file name
\def\pgf@declaredraftimage#1#2{%
  \ifx\pgf@imagewidth\pgfutil@empty%
    \pgfwarning{Missing width for image "#1" ("#2") in draft mode. Using 1cm instead}%
    \edef\pgf@imagewidth{1cm}%
  \fi%
  \ifx\pgf@imageheight\pgfutil@empty%
    \pgfwarning{Missing height for image "#1" ("#2") in draft mode. Using 1cm instead}%
    \edef\pgf@imageheight{1cm}%
  \fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepagetext{ page \pgf@imagepage}\fi%
  \edef\pgf@image{%
    \hbox to \pgf@imagewidth{%
      \vrule\kern-0.4pt%
      \vbox to \pgf@imageheight{%
        \hrule\vfil%
        \hbox to \pgf@imagewidth{\hskip-10cm\hfil\noexpand\pgfutil@font@tiny#2\pgf@imagepage\hfil\hskip-10cm}%
        \vfil\hrule}%
      \kern-0.4pt\vrule}%
  }%
}



% Declare a soft mask
%
% #1 = optional argument: matte specification. default matte is
%      white.
% #2 = name of the mask for later use
% #3 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF. Postscript is not supported.
%
% Description:
%
% This command declares a soft mask for later masking an image. The
% declared mask should be used together with an image of exactly the
% same height/width if matte is defined. Matte should be the
% preblended background color (see pdf spec for details).
%
% Example:
%
% \pgfdeclaremask[matte=white]{maskname}{maskfilename}
% \pgfdeclareimage[mask=maskname]{image}{imagefilename}

\def\pgfdeclaremask{\pgfutil@ifnextchar[\pgf@declaremask{\pgf@declaremask[]}}
\def\pgf@declaremask[#1]#2#3{%
  \pgfqkeys{/pgf/images/mask}{matte={1 1 1},#1}% defaults
  \def\pgf@mask{}%
  % Try to find the file
  \gdef\pgf@filename{}%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \ifx\pgf@filename\pgfutil@empty%
    \pgfwarning%
    {File "#3" not found when defining mask "#2".
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
  \else%
    \pgfsys@definemask%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@mask@#2\endcsname=\pgf@mask%
}

\pgfkeys{/pgf/images/mask/matte/.cd,.estore in=\pgf@maskmatte,.value required}



% Create an alias name for an image
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfdeclareimage{image}{1cm}{1cm}{filename
% \pgfaliasimage{alias}{image}
% \pgfuseimage{alias}

\def\pgfaliasimage#1#2{%
  \expandafter\global\expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@image@#2!\endcsname%
  \expandafter\global\expandafter\let\csname pgf@image@#1!\endcsname=\pgf@temp%
  }


% Use an image
%
% #1 = name of a previously declared image
%
% Example:
%
% \pgfputat{\pgforigin}{\pgfbox[left,base]{\pgfuseimage{myimage}}}

\def\pgfuseimage#1{%
  \def\pgf@imagename{pgf@image@#1}%
  \pgf@tryextensions{\pgf@imagename}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@imagename}%
  {\pgferror{Undefined image "#1"}}%
  {{\leavevmode\csname\pgf@imagename\endcsname}}}

\def\pgf@tryextensions#1#2{%
  \edef\pgf@args{[#2!]}\expandafter\pgf@@tryextensions\pgf@args{#1}}
\def\pgf@@tryextensions[#1!#2]#3{%
  \expandafter\pgfutil@ifundefined\expandafter{#3#1!#2}%
  {\def\pgf@temp{#2}%
    \ifx\pgf@temp\pgfutil@empty%
    \edef#3{#3!}%
    \else%
    \pgf@@tryextensions[#2]{#3}%
    \fi}%
  {\edef#3{#3#1!#2}}}


% Alternate image
%
% Description:
%
% When an image is used, pgf first attempts to use the image with the
% alternate extension added. If this fails, the original image is
% used. If the alternate extension contains ``!'', then the text up to
% the ! is successively removed and the remainder is tried as an
% alternate extension.
%
% Example:
%
% \def\pgfalternateextension{20!white}

\def\pgfalternateextension{}



% Directly insert an image
%
% #1 = optional argument: width, height, page specification
% #2 = file name
%
% Description:
%
% Directly inserts an image without declaration. You can, however,
% still access this image using the name pgflastimage. By using
% pgfaliasimage, you can also save this image for later.
%
% Example:
%
% \pgfimage[height=2cm]{filename}

\def\pgfimage{\pgfutil@ifnextchar[\pgf@imagecom{\pgf@imagecom[]}}
\def\pgf@imagecom[#1]#2{%
  \pgfdeclareimage[#1]{pgflastimage}{#2}%
  \pgfuseimage{pgflastimage}}


\input pgfcoreexternal.code.tex

\endinput


==> pgfcorelayers.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorelayers.code.tex}


% Creates a new pgf layer
%
% #1 = layer name
%
% Declares a new layer for pgf.
%
% Example:
%
% \pgfdeclarelayer{background}

\def\pgfdeclarelayer#1{%
  \pgfutil@ifundefined{pgf@layerbox@#1}{%
    \expandafter\expandafter\csname pgf@newbox\endcsname\csname pgf@layerbox@#1\endcsname%
    \expandafter\expandafter\csname pgf@newbox\endcsname\csname pgf@layerboxsaved@#1\endcsname%
  }{}%
}
\let\pgf@newbox=\newbox % avoid plain TeX outer problem

% Sets the layers that compose the picture
%
% #1 = List of layers
%
% Description:
%
% Sets the list of layers that make up the picture. The layers will be
% put on top of each other in the order given. 
%
% This command can also be given inside of a picture in which case it
% applies only to that very picture.
%
% Example:
%
% \pgfsetlayers{background,main}

\def\pgfsetlayers#1{%
  \let\pgf@layerlist\pgfutil@empty%
  \pgf@dosetlayer#1,,\relax%
}

\def\pgf@dosetlayer#1,#2,\relax{%
  \ifx\pgf@layerlist\pgfutil@empty%
    \edef\pgf@layerlist{\pgfutil@trimspaces{#1}}%
  \else
    \edef\pgf@layerlist{\pgf@layerlist,\pgfutil@trimspaces{#1}}%
  \fi
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosetlayer#2,\relax%
  \fi%
}

\pgfsetlayers{main}

% Adds code to a layer
%
% #1 = layer name
%
% Note:
%
% You cannot add anything to the ``main'' layer using this command.
%
% Example:
%
% \begin{pgfonlayer}{background}
%   \fill[red] (0,0) -- (1,1);
% \end{pgfonlayer}

\def\pgfonlayer@name{main}

\def\pgfonlayer#1{%
  \pgfutil@ifundefined{pgf@layerbox@#1}{%
     \pgferror{Sorry, the requested layer '#1' could not be found. Maybe you misspelled it?}%
   \bgroup
     \begingroup
  }{%
      \begingroup
        \edef\pgf@temp{#1}%
        \ifx\pgf@temp\pgfonlayer@name
          % we are already on this layer.
          \def\pgf@temp{%
            \bgroup
            \begingroup
          }%
      \else
        \let\pgfonlayer@name=\pgf@temp
        \pgfonlayer@assert@is@active
        \def\pgf@temp{%
          \expandafter\global\expandafter%
          \setbox\csname pgf@layerbox@#1\endcsname=\hbox to 0pt%
            \bgroup%
              \expandafter\box\csname pgf@layerbox@#1\endcsname%
              \begingroup%
        }%
      \fi
   \pgfsetlinewidth{0.4pt}% always reset the line width
   \pgf@temp
  }%
}
\def\endpgfonlayer{%
      \endgroup%
      \hss
    \egroup%
  \endgroup
}

\let\startpgfonlayer=\pgfonlayer
\let\stoppgfonlayer=\endpgfonlayer

\def\pgfdiscardlayername{discard}

\def\pgfonlayer@assert@is@active{%
  \ifx\pgfonlayer@name\pgfdiscardlayername
     % this special layer name can be used as /dev/null without
   % warning.
  \else
    \begingroup
    \def\pgfonlayer@isactive{0}%
    \expandafter\pgf@assert@layer@is@active@loop\pgf@layerlist,,\relax%
    \if0\pgfonlayer@isactive
       \pgfonlayer@assert@fail
    \fi
    \endgroup
  \fi
}%
\def\pgfonlayer@assert@fail{%
  \pgferror{Sorry, the requested layer '\pgfonlayer@name' is not 
   part of the layer list. Please verify that you provided 
   \string\pgfsetlayers\space and that '\pgfonlayer@name' is part of this list}%
}%
\def\pgf@assert@layer@is@active@loop#1,#2,\relax{%
  \edef\pgf@test{#1}%
  \ifx\pgf@test\pgfonlayer@name
     \def\pgfonlayer@isactive{1}%
  \else
    \def\pgf@test{#2}%
    \ifx\pgf@test\pgfutil@empty%
    \else%
    \pgf@assert@layer@is@active@loop#2,\relax%
    \fi%
  \fi
}

% Hooks into the scoping:

\def\pgf@insertlayers{%
  \expandafter\pgf@dolayer\pgf@layerlist,,\relax%
}
\def\pgf@maintext{main}%
\def\pgf@dolayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \box\pgf@layerbox@main%
  \else%
    \pgfsys@beginscope%
      \expandafter\box\csname pgf@layerbox@#1\endcsname%
    \pgfsys@endscope%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dolayer#2,\relax%
  \fi%
}

\def\pgf@savelayers{%
  \expandafter\pgf@dosavelayer\pgf@layerlist,,\relax%
}
\def\pgf@dosavelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \setbox\csname pgf@layerboxsaved@#1\endcsname=\box\csname pgf@layerbox@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavelayer#2,\relax%
  \fi%
}

\def\pgf@restorelayers{%
  \expandafter\pgf@dorestorelayer\pgf@layerlist,,\relax%
}
\def\pgf@dorestorelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \global\setbox\csname pgf@layerbox@#1\endcsname=\box\csname pgf@layerboxsaved@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dorestorelayer#2,\relax%
  \fi%
}

\endinput


==> pgfcoreobjects.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreobjects.code.tex}


% Object reuse


% Define a pgf object for reuse. Such objects will be stored
% efficiently internally.
%
% #1 = name for later reuse
% #2 = lower left corner point of bounding box
% #3 = upper right left corner point of bounding box
% #4 = pure pgf code (nothing too fancy!)
%
% Description:
% 
% Used to define reusable objects. The object must be composed of
% basic pgf graphic primitives. Nothing fancy can be used. The
% created object will be stored as an xform object in pdf or as a
% postscript procedure in postscript.
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfpathqmoveto{0pt}{0pt}
%  \pgfpathqmoveto{10pt}{0pt}
%  \pgfpathqmoveto{10pt}{10pt}
%  \pgfpathqmoveto{0pt}{10pt}
%  \pgfpathclose
%  \pgfusepath{stroke}}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfdefobject#1#2#3#4{%
  \pgfinterruptpath%
    \pgf@relevantforpicturesizefalse%
    \pgfsys@defobject{#1}{#2}{#3}{#4}%
  \endpgfinterruptpath%
  \ignorespaces%
}


% Use an object that was previously defined using pgfdefobject
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfuseobject#1{\pgfsys@beginscope\pgfsys@useobject{#1}{}\pgfsys@endscope}


% Use an object that was previously defined using pgfdefobject, but
% magnify the object by the current x and y register values
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgf@x=2pt% Scale by factor two in x-direction
%   \pgf@y=2pt% Scale by factor two in y-direction
%   \pgfuseobjectmagnify{myrect}
% \end{pgfpicture}

\def\pgfuseobjectmagnify#1{%
  \pgfsys@beginscope%
  \pgfsys@useobject{#1}{\pgfsys@transformxyscale{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}}%
  \pgfsys@endscope%
}


\endinput


==> pgfcorepathconstruct.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorepathconstruct.code.tex}


\newdimen\pgf@path@lastx
\newdimen\pgf@path@lasty

\let\pgfgetpath=\pgfsyssoftpath@getcurrentpath
\let\pgfsetpath=\pgfsyssoftpath@setcurrentpath



% Replace corners by arcs.
%
% #1 = in-size of arc
% #2 = out-size of arc
%
% Description:
%
% This command influences path construction command like
% \pgfpathlineto or \pgfpatharc. It will cause the corners at the end
% of these commands to be replaced by little arcs. If the
% corner is a 90 degrees corner and if #1=#2, a quarter-circle of
% radius #1 is put in place of the corner. If #1 and #2 are different,
% the quarter circle will instead by a quarter ellipse. If the angle
% is different from 90 degrees, a deformed quarter circle will
% result, which may or may not be desirable. For a ``perfect'' arc you
% must use the \pgfpatharc command.
%
%
% Example: One rounded corner.
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfstroke
%
% Example: A rounded rectangle
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% \pgfstroke
%
% Example: A rounded triangles
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{1cm}{0cm}}
% \pgfpathlineto{\pgfpoint{1cm}{1cm}}
% \pgfpathclose
% \pgfstroke

\newif\ifpgf@arccorners

\def\pgfsetcornersarced#1{%
  \pgf@process{#1}%
  \edef\pgf@corner@arc{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@arccornerstrue%
  \ifdim\pgf@x=0pt%
    \ifdim\pgf@y=0pt\relax%
      \pgf@arccornersfalse%
    \fi%
  \fi%
}

\def\pgf@roundcornerifneeded{%
  \ifpgf@arccorners\expandafter\pgfsyssoftpath@specialround\pgf@corner@arc\fi%
}



% The following protocol the passed sizes and all the corresponding
% softpath commands. The nonlinear transformation (nlt) module
% overwrites these commands.

\def\pgf@lt@moveto#1#2{%
  \pgf@protocolsizes{#1}{#2}%
  \pgfsyssoftpath@moveto{\the#1}{\the#2}%
}
\def\pgf@lt@lineto#1#2{%
  \pgf@protocolsizes{#1}{#2}%
  \pgfsyssoftpath@lineto{\the#1}{\the#2}%
}
\def\pgf@lt@curveto#1#2#3#4#5#6{%
  \pgf@protocolsizes{#1}{#2}%
  \pgf@protocolsizes{#3}{#4}%
  \pgf@protocolsizes{#5}{#6}%
  \pgfsyssoftpath@curveto{\the#1}{\the#2}{\the#3}{\the#4}{\the#5}{\the#6}%
}

\let\pgf@lt@closepath\pgfsyssoftpath@closepath

\let\pgf@nlt@moveto\pgf@lt@moveto
\let\pgf@nlt@lineto\pgf@lt@lineto
\let\pgf@nlt@curveto\pgf@lt@curveto
\let\pgf@nlt@closepath\pgf@lt@closepath

\let\pgf@nlt@list\pgfutil@empty % If non-empty, the nlt module is active


% Move current point to #1.
%
% #1 = new current point
%
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathmoveto#1{%
  \pgfpointtransformed{#1}%
  \pgf@nlt@moveto{\pgf@x}{\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}

\def\pgf@protocolsizes#1#2{%
  \ifpgf@relevantforpicturesize%
    \ifdim#1<\pgf@picminx\global\pgf@picminx#1\fi%
    \ifdim#1>\pgf@picmaxx\global\pgf@picmaxx#1\fi%
    \ifdim#2<\pgf@picminy\global\pgf@picminy#2\fi%
    \ifdim#2>\pgf@picmaxy\global\pgf@picmaxy#2\fi%
    \ifpgf@size@hooked%
      \let\pgf@size@hook@x#1\let\pgf@size@hook@y#2\pgf@path@size@hook%
    \fi%
  \fi%
  \ifdim#1<\pgf@pathminx\global\pgf@pathminx#1\fi%
  \ifdim#1>\pgf@pathmaxx\global\pgf@pathmaxx#1\fi%
  \ifdim#2<\pgf@pathminy\global\pgf@pathminy#2\fi%
  \ifdim#2>\pgf@pathmaxy\global\pgf@pathmaxy#2\fi%
}
\newif\ifpgf@size@hooked
\let\pgf@path@size@hook=\pgfutil@empty%

\def\pgf@resetpathsizes{%
  \global\pgf@pathmaxx=-16000pt\relax%
  \global\pgf@pathminx=16000pt\relax%
  \global\pgf@pathmaxy=-16000pt\relax%
  \global\pgf@pathminy=16000pt\relax%
}

\def\pgf@getpathsizes#1{%
  \edef#1{{\the\pgf@pathmaxx}{\the\pgf@pathminx}{\the\pgf@pathmaxy}{\the\pgf@pathminy}}%
}
\def\pgf@setpathsizes#1{%
  \expandafter\pgf@@setpathsizes#1%
}
\def\pgf@@setpathsizes#1#2#3#4{%
  \global\pgf@pathmaxx=#1\relax%
  \global\pgf@pathminx=#2\relax%
  \global\pgf@pathmaxy=#3\relax%
  \global\pgf@pathminy=#4\relax%
}





% Append a line from the current point to #1 to the current path.
%
% #1 = end of line
%
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathlineto#1{%
  \pgfpointtransformed{#1}%
  \pgf@roundcornerifneeded%
  \pgf@nlt@lineto{\pgf@x}{\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}



% Close the current path.
%
% Example:
%
% % Draws two triangles
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfclosepath
% \pgfpathmoveto{\pgfxy(2,0)}
% \pgfpathlineto{\pgfxy(2,1)}
% \pgfpathlineto{\pgfxy(3,0)}
% \pgfpathclose
% \pgfstroke

\def\pgfpathclose{%
  \pgf@roundcornerifneeded%
  \pgf@nlt@closepath%
}


% Append a cubic bezier spline from the current point to #3 with control
% points #1 and #2 to the current path.
%
% #1 = first control point
% #2 = second control point
% #3 = end point
%
% Example:
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfpathcurveto{\pgfpointxy{0}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{1}{2}}
% \pgfstroke

\def\pgfpathcurveto#1#2#3{%
  \pgfpointtransformed{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgf@roundcornerifneeded%
  \pgf@nlt@curveto{\pgf@x}{\pgf@y}{\pgf@xa}{\pgf@ya}{\pgf@xb}{\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
}



% Append a quadratic bezier spline from the current point to #2 with
% control point #1 to the current path.
%
% #1 = control point
% #2 = end point
%
% Example:
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfpathquadraticcurveto{\pgfpointxy{1}{1}}{\pgfpointxy{2}{0}}
% \pgfstroke

\def\pgfpathquadraticcurveto#1#2{%
  \pgfpointtransformed{#2}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgf@xc=.6666666\pgf@x%
  \pgf@yc=.6666666\pgf@y%
  % compute second control point:
  \pgf@xa=.33333333\pgf@xb%
  \pgf@ya=.33333333\pgf@yb%
  \advance\pgf@xa by\pgf@xc%
  \advance\pgf@ya by\pgf@yc%
  % compute first control point
  \advance\pgf@xc by.3333333\pgf@path@lastx%
  \advance\pgf@yc by.3333333\pgf@path@lasty%
  \pgf@roundcornerifneeded%
  \pgf@nlt@curveto{\pgf@xc}{\pgf@yc}{\pgf@xa}{\pgf@ya}{\pgf@xb}{\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
}




% Append an arc to the current point, where the current point is at
% angle #1 and the end is at angle #2. If #2 > #1, the arc is drawn
% counter-clockwise, otherwise it is clockwise.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = radius or x-radius/y-radius
%
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharc{0}{90}{2cm}
% \pgfstroke

\def\pgfpatharc#1#2#3{%
  {%
    \pgfmathparse{#1}\let\pgf@temp@a=\pgfmathresult%
    \pgfmathparse{#2}\let\pgf@temp@b=\pgfmathresult%
    \pgfutil@in@{and }{#3}%
    \ifpgfutil@in@%
      \pgf@arc@get@radii#3\pgf@arc@stop%
    \else
      \pgf@arc@get@radii#3and #3\pgf@arc@stop%
    \fi%
    \pgf@arc@local@angle@a=\pgf@temp@a pt%
    \pgf@arc@local@angle@b=\pgf@temp@b pt%
    \loop%
      \pgfutil@tempdima=\pgf@arc@local@angle@a%
      \advance\pgfutil@tempdima by-\pgf@arc@local@angle@b\relax%
      \ifdim\pgfutil@tempdima<0pt\relax%
        \pgfutil@tempdima=-\pgfutil@tempdima\relax%
      \fi%
    \ifdim\pgfutil@tempdima>90pt\relax%
      \ifdim\pgfutil@tempdima>115pt\relax%
        \pgf@arc@temp=90pt% big skip
      \else%
        \pgf@arc@temp=60pt% smaller skip to ensure wide segments
                          % (important shortened end segments because
                          % of arrow tips)
      \fi%
      \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
        {%
          \pgf@arc@local@angle@b=\pgf@arc@local@angle@a\relax%
          \advance\pgf@arc@local@angle@b by\pgf@arc@temp\relax%
          \pgf@arc%
        }
        \advance\pgf@arc@local@angle@a by\pgf@arc@temp\relax%
      \else
        {%
          \pgf@arc@local@angle@b=\pgf@arc@local@angle@a\relax%
          \advance\pgf@arc@local@angle@b by-\pgf@arc@temp\relax%
          \pgf@arc%
        }%
        \advance\pgf@arc@local@angle@a by-\pgf@arc@temp\relax%
      \fi%
    \repeat%
    \pgf@roundcornerifneeded%
    \pgf@arc%
  }%
}
\dimendef\pgf@arc@local@angle@a=0
\dimendef\pgf@arc@local@angle@b=1
\dimendef\pgf@arc@temp=2

\def\pgf@arc@get@radii#1and #2\pgf@arc@stop{%
  \pgfmathparse{#1}\let\pgf@arc@radius@a=\pgfmathresult%
  \pgfmathparse{#2}\let\pgf@arc@radius@b=\pgfmathresult%
}


\def\pgf@arc{%
  {%
  \pgfutil@tempdima=\pgf@arc@radius@a pt%
  \pgfutil@tempdimb=\pgf@arc@radius@b pt%
  %
  \pgf@xa=\pgf@arc@local@angle@a\relax%
  \pgf@xb=\pgf@arc@local@angle@b\relax%
  \advance\pgf@xb by-\pgf@xa\relax%
  \ifdim\pgf@xb<0pt\relax%
    \pgf@xb=-\pgf@xb\relax%
  \fi%
  \ifdim\pgf@xb=90.0pt%
    \def\pgfmathresult{0.55228475}%
  \else%
    \pgfmathparse{1.333333333*tan(.25*\pgf@sys@tonumber{\pgf@xb})}% many thanks to Ken Starks
  \fi%
  \pgfutil@tempdima=\pgfmathresult\pgfutil@tempdima%
  \pgfutil@tempdimb=\pgfmathresult\pgfutil@tempdimb%
  %.. controls +(\pgf@xa+90:\pgfutil@tempdima) and +(\pgf@xb-90:\pgfutil@tempdima) .. +(-(#1:#3)+(#2:#3))%
  % store first support vector in xa/ya:
  \pgf@xa=\pgf@arc@local@angle@a\relax%
  \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
    \advance\pgf@xa by 90pt\relax%
  \else%
    \advance\pgf@xa by -90pt\relax%
  \fi%
  \edef\pgf@arc@angle{\pgf@sys@tonumber{\pgf@xa}}%
  \pgfpointtransformed{\pgfpointpolar{\pgf@arc@angle}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xa=\pgf@path@lastx%
  \pgf@ya=\pgf@path@lasty%
  \advance\pgf@xa by \pgf@x%
  \advance\pgf@ya by \pgf@y%
  % store target in xb/yb:
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@a}}{\pgf@arc@radius@a pt and \pgf@arc@radius@b pt}}%
  \pgf@xb=\pgf@path@lastx%
  \pgf@yb=\pgf@path@lasty%
  \advance\pgf@xb by -\pgf@x%
  \advance\pgf@yb by -\pgf@y%
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@b}}{\pgf@arc@radius@a pt and \pgf@arc@radius@b pt}}%
  \advance\pgf@xb by \pgf@x%
  \advance\pgf@yb by \pgf@y%
  % store second support xc/yc:
  \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
    \advance\pgf@arc@local@angle@b by -90pt\relax%
  \else%
    \advance\pgf@arc@local@angle@b by 90pt\relax%
  \fi%
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@b}}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xc=\pgf@xb\relax%
  \pgf@yc=\pgf@yb\relax%
  \advance \pgf@xc by \pgf@x\relax%
  \advance \pgf@yc by \pgf@y\relax%
  \pgf@nlt@curveto{\pgf@xa}{\pgf@ya}{\pgf@xc}{\pgf@yc}{\pgf@xb}{\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
  }%
}


% Append an arc to the current point, where the arc is on an ellipse
% given by two axis vectors.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = first axis
% #4 = second axis
%
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharcaxes{0}{90}{\pgfpointxy{2}{0}}{\pgfpointxy{0}{2}}
% \pgfstroke

\def\pgfpatharcaxes#1#2#3#4{%
  {%
    \pgftransformtriangle{\pgfpointorigin}{#3}{#4}%
    \pgfpatharc{#1}{#2}{1pt}%
  }%
}



% Append an arc to the current point that ends at a given position.
%
% #1 = x-radius
% #2 = y-radius
% #3 = x-axis-rotation (in degrees)
% #4 = large-arc-sweep-flag (0 or 1)
% #5 = sweep-flag (0 or 1)
% #6 = target point
%
% Description:
%
% This command implements an arc drawing where a given target
% coordinate (#6) is given and the task is to draw an arc of an
% ellipse with the given radii. The center point of the ellipse is not
% give, but computed automatically.
%
% This kind of "endpoint parameterization" of an arc is exactly the
% same as the one specified by the SVG-specification for the "A" and
% "a" path commands. Please see the SVG-specification for details.
%
% Note that the problem is internally converted to drawing an arc
% using \pgfpatharc. This means that there may be a heavy loss of
% accuracy.
%
% Example:
%
% \pgfpathmoveto{\pgfpoint{1cm}{1cm}}
% \pgfpatharcto{1cm}{1cm}{0}{0}{0}{\pgfpoint{0cm}{2cm}}

\def\pgfpatharcto#1#2#3#4#5#6{%
  {%
    % The following code is based on the transformation described in svg
    % 1.1 specification Section F.6.5
    %
    % Step 1: store the simple parameters (xa=x1 since TeX does not
    % allow numbers in names)
    %
    \pgfmathsetmacro\pgf@arcto@rx{abs(#1)}%
    \pgfmathsetmacro\pgf@arcto@ry{abs(#2)}%
    \ifdim\pgf@arcto@rx pt=0pt% special rule: zero radius=straight line
      \gdef\pgf@marshal{\pgfpathlineto{#6}}%
    \else
    \ifdim\pgf@arcto@ry pt=0pt% special rule: zero radius=straight line
      \gdef\pgf@marshal{\pgfpathlineto{#6}}%
    \else
    \pgfmathsetmacro\pgf@arcto@phi{#3}%
    \pgfmathsetmacro\pgf@arcto@fA{#4}%
    \ifdim\pgf@arcto@fA pt=0pt
    \else
      \pgfmathsetmacro\pgf@arcto@fA{1.0} % Special rule: every non-zero value is 1.
    \fi
    \pgfmathsetmacro\pgf@arcto@fS{#5}%
    \ifdim\pgf@arcto@fS pt=0pt
    \else
      \pgfmathsetmacro\pgf@arcto@fS{1.0} % Special rule: every non-zero value is 1.
    \fi
    \pgf@process{#6}
    \edef\pgf@arcto@xb{\the\pgf@x}%
    \edef\pgf@arcto@yb{\the\pgf@y}%
    %
    % Step 2: x1,y1 is more complicated to compute: It is given by lastx
    % and lasty, but these are transformed coordinates, we need the
    % untransformed ones. So, we inverse the transformation (arghh...)
    %
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{\pgfqpoint{\pgf@path@lastx}{\pgf@path@lasty}}}
    \edef\pgf@arcto@xa{\the\pgf@x}
    \edef\pgf@arcto@ya{\the\pgf@y}
    \edef\pgf@temp@a{\pgf@arcto@xa,\pgf@arcto@ya}
    \edef\pgf@temp@b{\pgf@arcto@xb,\pgf@arcto@yb}
    \ifx\pgf@temp@a\pgf@temp@b% special rule: skip!
      \global\let\pgf@marshal\pgfutil@empty
    \else
    %
    % Ok, now we got all the parameters setup. Now comes the
    % computation...
    %
    %
    % Step 3: Start with a new coordinate system and rotate everything
    % by the negated phi.
    %
    \pgftransformreset
    \pgftransformrotate{-\pgf@arcto@phi}
    % Ok, using \pgfpointtransformed we now get transformed points...
    %
    % Step 4: Compute x1' and y1' (xaprime and yaprime)
    %
    \pgf@process{
      \pgfpointtransformed{\pgfpointscale{.5}{\pgfpointdiff
          {\pgfqpoint{\pgf@arcto@xb}{\pgf@arcto@yb}}
          {\pgfqpoint{\pgf@arcto@xa}{\pgf@arcto@ya}}
        }
      }
    }
    \edef\pgf@arcto@xaprime{\pgf@sys@tonumber\pgf@x}
    \edef\pgf@arcto@yaprime{\pgf@sys@tonumber\pgf@y}
    %
    % Compute Lambda
    %
    \pgfmathsetmacro\pgf@arcto@frac@x{\pgf@arcto@xaprime/\pgf@arcto@rx}
    \pgfmathsetmacro\pgf@arcto@frac@y{\pgf@arcto@yaprime/\pgf@arcto@ry}
    \pgfmathsetmacro\pgf@arcto@lambda{
      \pgf@arcto@frac@x*\pgf@arcto@frac@x+\pgf@arcto@frac@y*\pgf@arcto@frac@y
    }
    \ifdim\pgf@arcto@lambda pt>1pt%
      \pgfmathsetmacro\pgf@arcto@sqrt@lambda{sqrt(\pgf@arcto@lambda)}
      \pgfmathsetmacro\pgf@arcto@rx{\pgf@arcto@sqrt@lambda*\pgf@arcto@rx}
      \pgfmathsetmacro\pgf@arcto@ry{\pgf@arcto@sqrt@lambda*\pgf@arcto@ry}
    \fi
    %
    % Do some scaling
    %
    \pgfmathsetmacro\pgf@arcto@xaprime@abs{abs(\pgf@arcto@xaprime)}
    \pgfmathsetmacro\pgf@arcto@yaprime@abs{abs(\pgf@arcto@yaprime)}
    \pgfmathmax@{\pgf@arcto@rx,\pgf@arcto@ry,\pgf@arcto@xaprime@abs,\pgf@arcto@yaprime@abs}
    \pgfmathsetmacro\pgf@arcto@scaling{20/\pgfmathresult}
    \pgfmathsetmacro\pgf@arcto@rx@scaled{\pgf@arcto@scaling*\pgf@arcto@rx}
    \pgfmathsetmacro\pgf@arcto@ry@scaled{\pgf@arcto@scaling*\pgf@arcto@ry}
    \pgfmathsetmacro\pgf@arcto@xaprime@scaled{\pgf@arcto@scaling*\pgf@arcto@xaprime}
    \pgfmathsetmacro\pgf@arcto@yaprime@scaled{\pgf@arcto@scaling*\pgf@arcto@yaprime}
    %
    % Step 5: Now comes the messy computation of c1' and c2'.
    %
    \ifdim\pgf@arcto@rx pt>\pgf@arcto@ry pt%
      \pgfmathsetmacro\pgf@arcto@rx@over@ry{\pgf@arcto@rx/\pgf@arcto@ry}
      \pgfmathsetmacro\pgf@arcto@ry@over@rx{\pgf@arcto@ry/\pgf@arcto@rx}
      \pgfmathsetmacro\pgf@arcto@temp{\pgf@arcto@ry@over@rx*\pgf@arcto@xaprime@scaled}
      \pgfmathsetmacro\pgf@arcto@numerator{
        \pgf@arcto@ry@scaled*\pgf@arcto@ry@scaled-
        \pgf@arcto@yaprime@scaled*\pgf@arcto@yaprime@scaled-
        \pgf@arcto@temp*\pgf@arcto@temp
      }
      \pgfmathsetmacro\pgf@arcto@denominator{
        \pgf@arcto@yaprime@scaled*\pgf@arcto@yaprime@scaled+
        \pgf@arcto@temp*\pgf@arcto@temp
      }
    \else
      \pgfmathsetmacro\pgf@arcto@rx@over@ry{\pgf@arcto@rx/\pgf@arcto@ry}
      \pgfmathsetmacro\pgf@arcto@ry@over@rx{\pgf@arcto@ry/\pgf@arcto@rx}
      \pgfmathsetmacro\pgf@arcto@temp{\pgf@arcto@rx@over@ry*\pgf@arcto@yaprime@scaled}
      \pgfmathsetmacro\pgf@arcto@numerator{
        \pgf@arcto@rx@scaled*\pgf@arcto@rx@scaled-
        \pgf@arcto@xaprime@scaled*\pgf@arcto@xaprime@scaled-
        \pgf@arcto@temp*\pgf@arcto@temp
      }
      \pgfmathsetmacro\pgf@arcto@denominator{
        \pgf@arcto@xaprime@scaled*\pgf@arcto@xaprime@scaled+
        \pgf@arcto@temp*\pgf@arcto@temp
      }
    \fi
    \pgfmathsetmacro\pgf@arcto@frac{
      \pgf@arcto@numerator/\pgf@arcto@denominator
    }
    \ifdim\pgf@arcto@frac pt<0pt
      \pgfmathsetmacro\pgf@arcto@factor{0}
    \else
      \pgfmathsetmacro\pgf@arcto@factor{sqrt(\pgf@arcto@frac)}
    \fi
    \ifx\pgf@arcto@fA\pgf@arcto@fS
      \pgfmathsetmacro\pgf@arcto@factor{-\pgf@arcto@factor}
    \fi
    \pgfmathsetmacro\pgf@arcto@cxprime{
      \pgf@arcto@factor*\pgf@arcto@rx@over@ry*\pgf@arcto@yaprime
    }
    \pgfmathsetmacro\pgf@arcto@cyprime{
      -\pgf@arcto@factor*\pgf@arcto@ry@over@rx*\pgf@arcto@xaprime
    }
    %
    % Step 6: Ok, now compute cx,cy
    %
    \pgftransformreset
    \pgftransformrotate{\pgf@arcto@phi}
    \pgf@process{
      \pgfpointtransformed{\pgfqpoint{\pgf@arcto@cxprime pt}{\pgf@arcto@cyprime pt}}
    }
    \edef\pgf@arcto@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
    \pgf@process{\pgfpointadd{\pgf@arcto@temp}{
        \pgfpointscale{.5}{
          \pgfpointadd
          {\pgfqpoint{\pgf@arcto@xa}{\pgf@arcto@ya}}
          {\pgfqpoint{\pgf@arcto@xb}{\pgf@arcto@yb}}        }
      }
    }
    \edef\pgf@arcto@cx{\the\pgf@x}
    \edef\pgf@arcto@cy{\the\pgf@y}
    %
    % Step 7: Compute start angle:
    %
    \pgfmathsetmacro\pgf@arcto@vec@x{(\pgf@arcto@xaprime-\pgf@arcto@cxprime)/\pgf@arcto@rx}
    \pgfmathsetmacro\pgf@arcto@vec@y{(\pgf@arcto@yaprime-\pgf@arcto@cyprime)/\pgf@arcto@ry}
    \pgfmathsetmacro\pgf@arcto@denominator{veclen(\pgf@arcto@vec@x,\pgf@arcto@vec@y)}
    \pgfmathsetmacro\pgf@arcto@frac{\pgf@arcto@vec@x/\pgf@arcto@denominator}
    \pgfmathsetmacro\pgf@arcto@theta@start{acos(\pgf@arcto@frac)}
    \ifdim\pgf@arcto@vec@y pt<0pt
      \pgfmathsetmacro\pgf@arcto@theta@start{-\pgf@arcto@theta@start}
    \fi
    %
    % Step 8: Compute end angle:
    %
    \pgfmathsetmacro\pgf@arcto@vec@x{(-\pgf@arcto@xaprime-\pgf@arcto@cxprime)/\pgf@arcto@rx}
    \pgfmathsetmacro\pgf@arcto@vec@y{(-\pgf@arcto@yaprime-\pgf@arcto@cyprime)/\pgf@arcto@ry}
    \pgfmathsetmacro\pgf@arcto@denominator{veclen(\pgf@arcto@vec@x,\pgf@arcto@vec@y)}
    \pgfmathsetmacro\pgf@arcto@frac{\pgf@arcto@vec@x/\pgf@arcto@denominator}
    \pgfmathsetmacro\pgf@arcto@theta@end{acos(\pgf@arcto@frac)}
    \ifdim\pgf@arcto@vec@y pt<0pt
      \pgfmathsetmacro\pgf@arcto@theta@end{-\pgf@arcto@theta@end}
    \fi
    \pgfmathsetmacro\pgf@arcto@delta@theta{abs(\pgf@arcto@theta@start-\pgf@arcto@theta@end)}
    \ifdim\pgf@arcto@fA pt=0pt%
      \ifdim\pgf@arcto@delta@theta pt>180pt%
        % Ok, we need to adjust the angle!
        \ifdim\pgf@arcto@theta@end pt>\pgf@arcto@theta@start pt
          \pgfmathsetmacro\pgf@arcto@theta@end{\pgf@arcto@theta@end-360}
        \else
          \pgfmathsetmacro\pgf@arcto@theta@end{\pgf@arcto@theta@end+360}
        \fi
      \fi
    \else
      \ifdim\pgf@arcto@delta@theta pt<180pt%
        % Ok, we need to adjust the angle!
        \ifdim\pgf@arcto@theta@end pt>\pgf@arcto@theta@start pt
          \pgfmathsetmacro\pgf@arcto@theta@end{\pgf@arcto@theta@end-360}
        \else
          \pgfmathsetmacro\pgf@arcto@theta@end{\pgf@arcto@theta@end+360}
        \fi
      \fi
    \fi
    \xdef\pgf@marshal{\noexpand
      \pgfpatharcaxes{\pgf@arcto@theta@start}{\pgf@arcto@theta@end}
      {\noexpand\pgfpointpolar{\pgf@arcto@phi}{\pgf@arcto@rx}}
      {\noexpand\pgfpointpolar{\pgf@arcto@phi+90}{\pgf@arcto@ry}}
    }
    \fi\fi\fi
  }
  \pgf@marshal
}



% the quality of arc approximation by means of Bezier splines is
% controlled by a mesh width.
%
% The mesh width is provided in (full!) degrees. The smaller the mesh
% width, the more precise the arc approximation.
%
% Use an empty value to disable spline approximation (uses a single
% cubic polynomial for the complete arc).
%
% The value must be an integer!
\def\pgfpatharctomaxstepsize{45}

% A specialized arc operation for an arc on an (axis--parallel) ellipse.
%
% In contrast to \pgfpatharc, it explicitly interpolates start- and end points.
%
% In contrast to \pgfpatharcto, this routine is numerically stable and
% quite fast since it relies on a lot of precomputed information.
%
% #1 center of ellipse
% #2 angle of last path position inside of the ellipse
% #3 end angle
% #4 end point (a \pgfpoint)
% #5 xradius
% #6 yradius
% #7 the ratio xradius/yradius of the ellipse
% #8 the ratio yradius/xradius of the ellipse
% Example:
%    \def\cx{1cm}% center x
%    \def\cy{1cm}% center y
%    \def\startangle{0}%
%    \def\endangle{45}%
%    \def\a{5cm}% xradius
%    \def\b{10cm}% yradius
%    \pgfmathparse{\a/\b}\let\abratio=\pgfmathresult
%    \pgfmathparse{\b/\a}\let\baratio=\pgfmathresult
%
% \pgfpathmoveto{\pgfpoint{\cx+\a*cos(\startangle)}{\cy+\b*sin(\startangle)}}%
% \pgfpatharctoprecomputed
%    {\pgfpoint{\cx}{\cy}}
%    {\startangle}
%    {\endangle}
%    {\pgfpoint{\cx+\a*cos(\endangle)}{\cy+\b*sin(\endangle)}}%
%    {\a}
%    {\b}
%    {\abratio}
%    {\baratio}
%
\def\pgfpatharctoprecomputed#1#2#3#4#5#6#7#8{%
    \begingroup
    % Implementation idea:
    %
    % let
    %   m = center (#1)
    %   \gamma_0 = start angle
    %   \gamma_1 = end angle
    %   a = x radius
    %   b = y radius
    %
    % an axis parallel ellipse is parameterized by
    % C(\gamma) = m + ( a cos(\gamma), b sin(\gamma) ), \gamma in [0,360].
    %
    % Now, consider the segment \gamma(t),
    %   \gamma:[0,1] -> [\gamma_0,\gamma_1],
    %            t   ->  \gamma_0 + t(\gamma_1 - \gamma_0)
    % and
    %   C(\gamma(t)) which is defined on [0,1].
    %
    % I'd like to approximate the arc by one or more cubic bezier
    % splines which interpolate through the last and first provided
    % points.
    %
    % In general, a Bezier spline C:[0,1] -> \R of order n fulfills
    % C'(0) = n ( P_1 - P_0 ),
    % C'(1) = n ( P_n - P_{n-1} ).
    % For n=3 and given P_0 and P_3, I can directly compute P_1 and P_2 once I know
    % the derivatives at t=0 and t=1.
    %
    % The derivatives in our case are
    %   ( C \circ \gamma )'(t) = C'[\gamma(t)] * \gamma'(t)
    %       = ( -a pi/180 sin(\gamma(t)),  b pi/180 cos(\gamma(t)) ) * (\gamma_1 - \gamma_0).
    % The pi/180 comes into play since we are working with degrees.
    %
    % Expression (C\circ\gamma)'(0) using P_0 and (C \circ \gamma)'(1)
    % using P_3 yields the expressions
    %   (C \circ \gamma)'(0) =
    %       pi/180 * (\gamma_1 - \gamma_0)* [ - a/b(P_0^y - my), b/a (P_0^x - mx) ]
    %   (C \circ \gamma)'(1) =
    %       pi/180 * (\gamma_1 - \gamma_0)* [ - a/b(P_3^y - my), b/a (P_3^x - mx) ]
    %
    % defining
    %  scaleA = a/b * pi / (3*180) * (\gamma_1 - \gamma_0)
    % and
    %  scaleB = b/a * pi / (3*180) * (\gamma_1 - \gamma_0)
    % yields the direct expressions for the intermediate bezier
    % control points
    %
    % P_1 = [
    %   P_0^x - scaleA* ( P_0^y -my),
    %   P_0^y + scaleB* ( P_0^x -mx) ]
    % and
    % P_2 = [
    %   P_3^x + scaleA* ( P_3^y -my),
    %   P_3^y - scaleB* ( P_3^x -mx) ].
    %
    % This works fast, with few operations, if
    % - a/b and b/a are known in advance
    % - P_0 and P_3 are known in advance
    % - \gamma_0 and \gamma_1 are known.
    %
    % It is also reliable if (\gamma_1 - \gamma_0) is small
    %
    \pgf@process{#1}%
    \edef\pgfpath@center@x{\the\pgf@x}%
    \edef\pgfpath@center@y{\the\pgf@y}%
    \def\pgfpath@completearcend{#4}%
    % compute scale (#3-#2) * pi/(3*180) = (#3 - #2) * pi/27 * 1/20
    % splitting pi/(3*180) into two scales has higher TeX accuracy
    \pgf@xa=#2pt
    \pgf@xb=#3pt
    \edef\pgfpath@startangle{#2pt}%
    \edef\pgfpath@endangle{\pgf@sys@tonumber\pgf@xb}%
    %
    \pgf@ya=\pgf@xb
    \advance\pgf@ya by-\pgf@xa
    %
    \ifx\pgfpatharctomaxstepsize\pgfutil@empty
        \def\pgfpath@N{1}%
        \pgf@xc=\pgf@ya
    \else
        \pgf@xc=\pgf@ya% compute N = floor((gamma_1 - gamma_0) / max) +1
        \ifdim\pgf@xc<0pt
            \multiply\pgf@xc by-1
        \fi
        \divide\pgf@xc by\pgfpatharctomaxstepsize\relax
        \afterassignment\pgfutil@gobble@until@relax
        \c@pgf@counta=\the\pgf@xc\relax
        \advance\c@pgf@counta by1
        \edef\pgfpath@N{\the\c@pgf@counta}%
        %
        \pgf@xc=\pgf@ya
        \divide\pgf@xc by\c@pgf@counta
    \fi
    %
    \edef\pgfpath@h{\pgf@sys@tonumber\pgf@xc}%
    %
%\message{pgfpathellipse: using N =\pgfpath@N\space spline points y0 = \pgfpath@startangle, y0+i*h, yN=\pgfpath@endangle, i=1,...,(\pgfpath@N-1), with h=\pgfpath@h\space mesh width (total arc angle \pgf@sys@tonumber\pgf@ya).}%
    %
    %
    \pgf@xc=0.116355283466289\pgf@xc % pi/27
    \divide\pgf@xc by20
    \pgf@xa=#7\pgf@xc
    \edef\pgfpath@scale@A{\pgf@sys@tonumber\pgf@xa}%
    \pgf@xa=#8\pgf@xc
    \edef\pgfpath@scale@B{\pgf@sys@tonumber\pgf@xa}%
    %
    % compute intermediate spline segments for
    %  i = 1,...,N-1
    % this is a no-op for N=1.
    \c@pgf@countd=1
    \pgfutil@loop
    \ifnum\c@pgf@countd<\pgfpath@N\relax
        %
        \pgf@xa=\pgfpath@startangle % compute \pgf@xa = y_0 + i*h
        \pgf@xb=\pgfpath@h pt
        \multiply\pgf@xb by\c@pgf@countd
        \advance\pgf@xa by\pgf@xb
        \edef\pgfpath@angle@i{\pgf@sys@tonumber\pgf@xa}%
%\message{angle \the\c@pgf@countd: \pgfpath@angle@i...}%
        %
        \pgfpatharcofellipse@{%
            \pgfpoint
                {\pgfpath@center@x + #5*cos(\pgfpath@angle@i)}
                {\pgfpath@center@y + #6*sin(\pgfpath@angle@i)}%
        }%
        %
        \advance\c@pgf@countd by1
    \pgfutil@repeat
    %
    % compute final spline segment. It only differs insofar as the
    % final point is already known explicitly and should be
    % interpolated without additional math error.
%\message{angle \pgfpath@N: \pgfpath@endangle...}%
    \pgfpatharcofellipse@{\pgfpath@completearcend}%
    \endgroup
}%
\def\pgfpatharcofellipse@#1{%
    \begingroup
    \pgf@process{#1}%
    \edef\pgfpath@endpt{\global\pgf@x=\the\pgf@x\space\global\pgf@y=\the\pgf@y\space}%
    %
    \pgfpathcurveto{
        \begingroup
        \global\pgf@x=\pgf@path@lastx
        \global\pgf@y=\pgf@path@lasty
        \pgf@xa=\pgf@x \advance\pgf@xa by-\pgfpath@center@x
        \pgf@ya=\pgf@y \advance\pgf@ya by-\pgfpath@center@y
        \global\advance\pgf@x by-\pgfpath@scale@A\pgf@ya
        \global\advance\pgf@y by \pgfpath@scale@B\pgf@xa
        \endgroup
    }{%
        \begingroup
        \pgfpath@endpt
        \pgf@xa=\pgf@x \advance\pgf@xa by-\pgfpath@center@x
        \pgf@ya=\pgf@y \advance\pgf@ya by-\pgfpath@center@y
        \global\advance\pgf@x by \pgfpath@scale@A\pgf@ya
        \global\advance\pgf@y by-\pgfpath@scale@B\pgf@xa
        \endgroup
    }{%
        \pgfpath@endpt
    }%
    \endgroup
}









% Append  an ellipse to the current path.
%
% #1 = center
% #2 = first axis
% #3 = second axis
%
% Example:
%
% % Add a circle of radius 3cm around the origin
% \pgfpathellipse{\pgforigin}{\pgfxy(2,0)}{\pgfxy(0,1)}
%
% % Draw a non-filled circle of radius 1cm around the point (1,1)
% \pgfpathellipse{\pgfxy(1,1)}{\pgfxy(1,1)}{\pgfxy(-2,2)}
% \pgfstroke

\def\pgfpathellipse#1#2#3{%
  \pgfpointtransformed{#1}% store center in xc/yc
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@xa=\pgf@x% store first axis in xa/ya
  \pgf@ya=\pgf@y%
  \advance\pgf@xa by-\pgf@pt@x%
  \advance\pgf@ya by-\pgf@pt@y%
  \pgfpointtransformed{#3}%
  \pgf@xb=\pgf@x% store second axis in xb/yb
  \pgf@yb=\pgf@y%
  \advance\pgf@xb by-\pgf@pt@x%
  \advance\pgf@yb by-\pgf@pt@y%
  {%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    \pgf@nlt@moveto{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@x=0.55228475\pgf@xb% first arc
  \pgf@y=0.55228475\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{\pgf@xc\the\pgf@x\pgf@yc\the\pgf@y}%
  \pgf@x=0.55228475\pgf@xa%
  \pgf@y=0.55228475\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%
    \pgf@temp%
    \pgf@nlt@curveto{\pgf@xc}{\pgf@yc}{\pgf@x}{\pgf@y}{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.55228475\pgf@xa% second arc
  \pgf@y=0.55228475\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{\pgf@xc\the\pgf@x\pgf@yc\the\pgf@y}%
  \pgf@x=0.55228475\pgf@xb%
  \pgf@y=0.55228475\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    \pgf@temp%
    \pgf@nlt@curveto{\pgf@xc}{\pgf@yc}{\pgf@x}{\pgf@y}{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@xb=-\pgf@xb% flip second axis
  \pgf@yb=-\pgf@yb%
  \pgf@x=0.55228475\pgf@xb% third arc
  \pgf@y=0.55228475\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{\pgf@xc\the\pgf@x\pgf@yc\the\pgf@y}%
  \pgf@x=0.55228475\pgf@xa%
  \pgf@y=0.55228475\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%
    \pgf@temp%
    \pgf@nlt@curveto{\pgf@xc}{\pgf@yc}{\pgf@x}{\pgf@y}{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis once more
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.55228475\pgf@xa% fourth arc
  \pgf@y=0.55228475\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{\pgf@xc\the\pgf@x\pgf@yc\the\pgf@y}%
  \pgf@x=0.55228475\pgf@xb%
  \pgf@y=0.55228475\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    \pgf@temp%
    \pgf@nlt@curveto{\pgf@xc}{\pgf@yc}{\pgf@x}{\pgf@y}{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@nlt@closepath%
  \pgf@nlt@moveto{\pgf@xc}{\pgf@yc}%
}



% Append a circle to the current path
%
% #1 = center
% #2 = radius
%
% Example:
%
% % Append a circle of radius 3cm around the point (1,1)
% \pgfpathcircle{\pgxy(1,1)}{3cm}

\def\pgfpathcircle#1#2{\pgfpathellipse{#1}{\pgfpoint{#2}{0pt}}{\pgfpoint{0pt}{#2}}}




% Append a rectangle to the current path
%
% #1 = lower left corner point of rectangle
% #2 = width and height vector
%
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectangle{\pgfpointxy{2}{2}}{\pgfpointxy{1}{1}}

\def\pgfpathrectangle{%
  \let\pgfrect@next=\pgf@specialrect%
  \ifpgf@pt@identity%
    \ifpgf@arccorners%
    \else%
      \ifx\pgf@nlt@list\pgfutil@empty%
        \let\pgfrect@next=\pgf@normalrect%
      \fi%
    \fi%
  \fi%
  \pgfrect@next%
}

\def\pgf@normalrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgfsyssoftpath@rect{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \advance\pgf@x by\pgf@xa\relax%
  \advance\pgf@y by\pgf@ya\relax%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
}

\def\pgf@specialrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \advance\pgf@xa by\pgf@xb%
  \advance\pgf@ya by\pgf@yb%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
}

% Append a rectangle to the current path
%
% #1 = one corner of the rectangle
% #2 = opposite corner of the rectangle
%
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectanglecorners{\pgfpointxy{2}{2}}{\pgfpointxy{3}{3}}

\def\pgfpathrectanglecorners#1#2{%
  \pgf@process{#2}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xc by-\pgf@x%
  \advance\pgf@yc by-\pgf@y%
  \pgfpathrectangle{#1}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
}


% Append a grid to the current path.
%
% #1 = first corner point of grid
% #2 = second corner point of grid
%
% Options:
%
% stepx = x-step dimension (default 1cm)
% stepy = y-step dimension (default 1cm)
% step  = dimension vector
%
% Example:
%
% \pgfsetlinewidth{0.8pt}
% \pgfgrid{\pgfxy(0,0)}{\pgfxy(3,2)}
% \pgfsetlinewidth{0.4pt}
% \pgfgrid[stepx=1cm,stepy=1cm]{\pgfxy(0,0)}{\pgfxy(3,2)}

\pgfkeys{
  /pgf/stepx/.initial=1cm,
  /pgf/stepy/.initial=1cm,
  /pgf/step/.code={\pgf@process{#1}\pgfkeysalso{/pgf/stepx/.expanded=\the\pgf@x,/pgf/stepy/.expanded=\the\pgf@y}},
  /pgf/step/.value required
}

\def\pgfpathgrid{\pgfutil@ifnextchar[{\pgf@pathgrid}{\pgf@pathgrid[]}}
\def\pgf@pathgrid[#1]#2#3{%
  \pgfset{#1}%
  \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/stepx}}%
  \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/stepy}}%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  % Swap coordinates if one of them is smaller than the other:
  \ifdim\pgf@xa>\pgf@xb%
    \pgf@x=\pgf@xb%
    \pgf@xb=\pgf@xa%
    \pgf@xa=\pgf@x%
  \fi%
  \ifdim\pgf@ya>\pgf@yb%
    \pgf@y=\pgf@yb%
    \pgf@yb=\pgf@ya%
    \pgf@ya=\pgf@y%
  \fi%
  \ifdim \pgf@yc > .01pt\relax% if to draw horizontal lines
    \c@pgf@counta=\pgf@ya\relax%
    \c@pgf@countb=\pgf@yc\relax%
    \divide\c@pgf@counta by\c@pgf@countb\relax%
    \pgfutil@tempdima=\c@pgf@counta\pgf@yc\relax%
    \ifdim\pgfutil@tempdima<\pgf@ya%
      \advance\pgfutil@tempdima by\pgf@yc%
    \fi%
    \pgfutil@tempdimb\pgf@x
    \pgfutil@loop% horizontal lines
      {%
        \pgf@xa=\pgfutil@tempdimb%
        \pgf@ya=\pgfutil@tempdima%
        \pgf@pos@transform{\pgf@xa}{\pgf@ya}
        \pgf@nlt@moveto{\pgf@xa}{\pgf@ya}%
        \pgf@xa=\pgf@xb%
        \pgf@ya=\pgfutil@tempdima%
        \pgf@pos@transform{\pgf@xa}{\pgf@ya}
        \pgf@nlt@lineto{\pgf@xa}{\pgf@ya}%
      }%
    \advance\pgfutil@tempdima by\pgf@yc%
    \ifdim\pgfutil@tempdima<\pgf@yb%
    \pgfutil@repeat%
    \advance\pgfutil@tempdima by-0.01pt\relax%
    \ifdim\pgfutil@tempdima<\pgf@yb%
      {%
        \pgf@xa=\pgfutil@tempdimb%
        \pgf@ya=\pgfutil@tempdima%
        \pgf@pos@transform{\pgf@xa}{\pgf@ya}
        \pgf@nlt@moveto{\pgf@xa}{\pgf@ya}%
        \pgf@xa=\pgf@xb%
        \pgf@ya=\pgfutil@tempdima%
        \pgf@pos@transform{\pgf@xa}{\pgf@ya}
        \pgf@nlt@lineto{\pgf@xa}{\pgf@ya}%
      }%
    \fi%
  \fi%
  \ifdim \pgf@xc > .01pt\relax% if to draw vertical lines
    \c@pgf@counta=\pgf@xa\relax%
    \c@pgf@countb=\pgf@xc\relax%
    \divide\c@pgf@counta by\c@pgf@countb\relax%
    \pgfutil@tempdimb=\c@pgf@counta\pgf@xc\relax%
    \ifdim\pgfutil@tempdimb<\pgf@xa%
      \advance\pgfutil@tempdimb by\pgf@xc%
    \fi%
    \pgfutil@loop% vertical lines
      {%
        \pgf@xc=\pgfutil@tempdimb%
        \pgf@yc=\pgf@ya%
        \pgf@pos@transform{\pgf@xc}{\pgf@yc}
        \pgf@nlt@moveto{\pgf@xc}{\pgf@yc}%
        \pgf@xc=\pgfutil@tempdimb%
        \pgf@yc=\pgf@yb%
        \pgf@pos@transform{\pgf@xc}{\pgf@yc}
        \pgf@nlt@lineto{\pgf@xc}{\pgf@yc}%
      }%
      \advance\pgfutil@tempdimb by\pgf@xc%
    \ifdim\pgfutil@tempdimb<\pgf@xb%
    \pgfutil@repeat%
    \advance\pgfutil@tempdimb by-0.01pt\relax%
    \ifdim\pgfutil@tempdimb<\pgf@xb%
      {%
        \pgf@xc=\pgfutil@tempdimb%
        \pgf@yc=\pgf@ya%
        \pgf@pos@transform{\pgf@xc}{\pgf@yc}
        \pgf@nlt@moveto{\pgf@xc}{\pgf@yc}%
        \pgf@xc=\pgfutil@tempdimb%
        \pgf@yc=\pgf@yb%
        \pgf@pos@transform{\pgf@xc}{\pgf@yc}
        \pgf@nlt@lineto{\pgf@xc}{\pgf@yc}%
      }%
    \fi%
  \fi%
  \pgf@process{#3}%
  \pgf@pos@transform{\pgf@x}{\pgf@y}%
  \pgf@nlt@moveto{\pgf@x}{\pgf@y}%
}



% Append two half-parabolas to the path
%
% #1 = bend (relative to current point)
% #2 = end point (relative to bend point)
%
% Description:
%
% This command appends a half-parabola that starts at the current point
% and has its bend at #1+current point. Then, a second parabola is
% appended that starts at #1+current point, where it also has its
% minimum/maximum, and ends at #1+current point+#2, which becomes the
% new current point.
%
% By setting #2 = (0,0) you draw only a half parabola that goes from the
% current point to the bend; by setting #1 = (0,0)
% you draw a half parabola that going to current point + #2 and has its
% bend at the current point.
%
% Examples:
%
% % Half-parabola going ``up and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpointorigin}{\pgfpoint{2cm}{4cm}}
%
% % Half-parabola going ``down and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}}{\pgfpointorigin}
%
% % Full parabola
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}{\pgfpoint{2cm}{4cm}}

\def\pgfpathparabola#1#2{%
  {%
    \pgf@process{#2}% untransformed
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempswatrue%
    \ifdim\pgf@xb=0pt\relax%
      \ifdim\pgf@yb=0pt\relax%
        \pgfutil@tempswafalse%
      \fi%
    \fi%
    {%
      \ifpgfutil@tempswa%
        \pgf@arccornersfalse
      \else%
      \fi%
      \pgfutil@tempswatrue%
      \ifdim\pgf@xc=0pt\relax%
        \ifdim\pgf@yc=0pt\relax%
          \pgfutil@tempswafalse%
        \fi%
      \fi%
      \ifpgfutil@tempswa
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.1125\pgf@xc}{.225\pgf@yc}}% found by trial and error
          {\pgfqpoint{.5\pgf@xc}{\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
      \fi%
    }%
    \ifpgfutil@tempswa%
      \pgf@xc=\pgf@xb%
      \pgf@yc=\pgf@yb%
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.5\pgf@xc}{0\pgf@yc}}% found by trial and error
          {\pgfqpoint{.8875\pgf@xc}{.775\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
    \fi%
  }%
}




% Append a sine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%
% Description:
%
% This command appends a sine curve in the interval 0 and \pi/2 to the
% current path. The sine curve ends at currentpoint+#1.
%
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathsine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.3260\pgf@xc}{.5120\pgf@yc}}%
      {\pgfqpoint{.6380\pgf@xc}{\pgf@yc}}%
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%
}

% Append a cosine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathcosine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.3620\pgf@xc}{0pt}}%
      {\pgfqpoint{.6740\pgf@xc}{.4880\pgf@yc}}%
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%
}



% Draw part of a curve between two specified times s and t.
%
% #1 - a start time s.
% #2 - an end time t.
% #3 - start point of the curve
% #4 - first control
% #5 - second control
% #6 - end point of the curve
%
% There are two versions, \pgfpathcurvebetweentime and
% \pgfpathcurvebetweentimecontinue. The latter does not insert a
% moveto to the first point.
%
\def\pgfpathcurvebetweentime{\pgf@ignoremovetofalse\pgf@@pathcurvebetweentime}
\def\pgfpathcurvebetweentimecontinue{\pgf@ignoremovetotrue\pgf@@pathcurvebetweentime}
\newif\ifpgf@ignoremoveto

\def\pgf@@pathcurvebetweentime#1#2#3#4#5#6{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgf@time@t=\pgfmathresult%
  \ifdim\pgf@time@s pt>\pgf@time@t pt\relax%
    \pgfmathsetmacro\pgf@time@s{1-#1}%
    \pgfmathsetmacro\pgf@time@t{1-#2}%
    \pgf@@@pathcurvebetweentime{\pgf@time@t}{#6}{#5}{#4}{#3}%
  \else%
    \pgf@@@pathcurvebetweentime{\pgf@time@t}{#3}{#4}{#5}{#6}%
  \fi%
}

\def\pgf@@@pathcurvebetweentime#1#2#3#4#5{%
  % Q1 = P1.
  \pgf@process{#2}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  % Q2 = P1 + t*(P2-P1).
  \pgf@process{%
    \pgf@process{#3}%
    \pgf@xa=#1\pgf@x%
    \pgf@ya=#1\pgf@y%
    \pgf@process{#2}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \advance\pgf@x by-#1\pgf@xb%
    \advance\pgf@y by-#1\pgf@yb%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Q3 = Q2 + t*((P2 + t*(P3-P2)) - Q2).
  \pgf@process{%
    \pgf@process{#4}%
    \pgf@xa=#1\pgf@x%
    \pgf@ya=#1\pgf@y%
    %
    \pgf@process{#3}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xc by-#1\pgf@x%
    \advance\pgf@yc by-#1\pgf@y%
    %
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by#1\pgf@xa%
    \advance\pgf@y by#1\pgf@ya%
    \advance\pgf@x by-#1\pgf@xb%
    \advance\pgf@y by-#1\pgf@yb%
    \advance\pgf@x by#1\pgf@xc%
    \advance\pgf@y by#1\pgf@yc%
  }%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  % Q4 = (1-t)^3*P1 + 3*t(1-t)^2*P2 + 3*t^2(1-t)*P3 + t^3*P4.
  \pgf@process{\pgfpointcurveattime{#1}{#2}{#3}{#4}{#5}}%
  \ifx#1\pgf@time@t%
    % First time round...
    \pgfmathdivide@{\pgf@time@s}{\pgf@time@t}%
    \pgfmathadd@{-\pgfmathresult}{1}%
    \let\pgf@time@s=\pgfmathresult%
    \edef\pgf@marshal{%
      \noexpand\pgf@@@pathcurvebetweentime{\noexpand\pgf@time@s}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
        {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
  \else%
    % ...second time round.
    \ifpgf@ignoremoveto%
      \edef\pgf@marshal{%
        \noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
          {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      }%
    \else%
      \edef\pgf@marshal{%
        \noexpand\pgfpathmoveto{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
          {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      }%
    \fi%
  \fi%
  \pgf@marshal%
}


\endinput


==> pgfcorepathprocessing.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorepathprocessing.code.tex}


% Split a path at the last subpath of a path
%
% #1 = a macro that stores a path
%
% Description:
%
% This command will split the path into two parts:
%
% \pgfprocessresultpathprefix
%   The part of the path before the last subpath.
%
% \pgfprocessresultpathsuffix
%   The last subpath on the path.
%
% #1 will always be equal to the contents of the two above macros
% concatenated. Normally, your objective will be to modify the
% \pgfprocessresultpathsuffix and then concatenate the result.

\def\pgfprocesssplitpath#1{%
  \let\pgfprocessresultpathprefix\pgfutil@empty%
  \let\pgfprocessresultpathsuffix\pgfutil@empty%
  \let\pgf@next\pgf@process@split%
  \expandafter\pgf@process@split#1\pgfsyssoftpath@movetotoken{}{}\pgf@stop%
}

\def\pgf@process@split#1\pgfsyssoftpath@movetotoken#2#3#4{%
  \ifx#4\pgf@stop% ok, end reached!
    \expandafter\def\expandafter\pgfprocessresultpathsuffix\expandafter{\pgfprocessresultpathsuffix#1}%
    \let\pgf@next\pgfutil@gobble%
  \else%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\pgfprocessresultpathprefix%
    \expandafter\expandafter\expandafter{\expandafter\pgfprocessresultpathprefix\pgfprocessresultpathsuffix#1}%
    \def\pgfprocessresultpathsuffix{\pgfsyssoftpath@movetotoken{#2}{#3}}%
  \fi%
  \pgf@next#4%
}



% Split a subpath at the end
%
% #1 = a macro that stores an open subpath that contains at least two
%      path commands (so, not just a moveto);
%
% Description:
%
% Splits the subpath into two parts:
%
% \pgfprocessresultsubpathsuffix
%   This macro contains the last two "relevant" path commands: The end
%   of the path command that led to the last path command and this
%   last path command. In essence, this macro contains everything you
%   "need to modify" if you wish to modify the end of the path.
%
% \pgfprocessresultsubpathprefix
%   Everything before the previous macro on the subpath.

\def\pgfprocesssplitsubpath#1{%
  % First, we need to find the end:
  \let\pgf@tempa\pgfutil@emtpy%
  \let\pgf@tempb\pgfutil@emtpy%
  \let\pgf@tempc\pgfutil@emtpy%
  \let\pgf@tempd\pgfutil@emtpy%
  \let\pgfprocessresultsubpathprefix\pgfutil@empty%
  \let\pgfprocessresultsubpathsuffix\pgfutil@empty%
  \let\pgf@next\pgf@split@subpath%
  \expandafter\pgf@split@subpath#1\pgf@stop%
}

\newif\ifpgf@split@move

\def\pgf@split@subpath#1#2#3#4{%
  \ifx#4\pgf@stop%
    \expandafter\def\expandafter\pgfprocessresultsubpathsuffix\expandafter{\pgfprocessresultsubpathsuffix#1{#2}{#3}}%
    \let\pgf@next\pgfutil@gobble%
  \else%
    \pgf@split@movetrue%
    \ifx#1\pgfsyssoftpath@curvetosupportatoken%
      \pgf@split@movefalse%
    \else
      \ifx#1\pgfsyssoftpath@curvetosupportbtoken%
        \pgf@split@movefalse%
      \fi%
    \fi%
    \ifpgf@split@move%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\pgfprocessresultsubpathprefix%
      \expandafter\expandafter\expandafter{%
        \expandafter\pgfprocessresultsubpathprefix\pgfprocessresultsubpathsuffix}%
      \def\pgfprocessresultsubpathsuffix{#1{#2}{#3}}%
    \else%
      \expandafter\def\expandafter\pgfprocessresultsubpathsuffix\expandafter{\pgfprocessresultsubpathsuffix#1{#2}{#3}}%
    \fi%
  \fi%
  \pgf@next#4%
}




% Extract start and end vectors of a path
%
% #1 = a macro that stores a path
%
% Description:
%
% This command will extract the first and second coordinate on the
% path as well as the last and second-last. These coordinates will be
% put in the pgfpoint-macros \pgfpointfirstonpath,
% \pgfpointsecondonpath, \pgfpointsecondlastonpath, and
% \pgfpointlastonpath. If the path is empty, these macros are set to
% \pgfpointorigin.
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesspathextractpoints\mypath
%
% % \pgfpointfirstonpath is now \pgfpoint{0}{0}
% % \pgfpointsecondonpath is now \pgfpoint{10bp}{10bp}
% % \pgfpointsecondlastonpath is now \pgfpoint{30bp}{30bp}
% % \pgfpointlastonpath is now \pgfpoint{40bp}{40bp}

\def\pgfprocesspathextractpoints#1{%
  \ifx#1\pgfutil@empty%
    \let\pgfpointfirstonpath=\pgfpointorigin%
    \let\pgfpointsecondonpath=\pgfpointorigin%
    \let\pgfpointsecondlastonpath=\pgfpointorigin%
    \let\pgfpointlastonpath=\pgfpointorigin%
  \else%
    \expandafter\pgf@extractprocessorfirst#1\pgf@stop%
  \fi%
}

\def\pgf@extractprocessorfirst#1#2#3#4{%
  \def\pgfpointfirstonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % pretty short path...
    \let\pgfpointsecondonpath=\pgfpointfirstonpath%
    \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
    \let\pgfpointlastonpath=\pgfpointfirstonpath%
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorsecond%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorsecond#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorsecond%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorsecond#1#2#3#4{%
  \def\pgfpointsecondonpath{\pgfqpoint{#2}{#3}}%
  \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
  \let\pgfpointlastonpath=\pgfpointsecondonpath%
  \ifx#4\pgf@stop%
    % short path...
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorother%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorother%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorother#1#2#3#4{%
  \let\pgfpointsecondlastonpath=\pgfpointlastonpath%
  \def\pgfpointlastonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % end!
    \let\next=\pgfutil@gobble%
  \fi%
  \next#4%
}



% Check for closepath and rectangles
%
% #1 = a macro that stores a path
% #2 = command to be executed when a closepath or a rectangle is encountered
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesscheckclosed{\mypath}{\pgf@drawarrowsfalse}

\def\pgfprocesscheckclosed#1#2{%
  {%
    \global\let\pgf@proc@todo=\relax%
    \let\pgfsyssoftpath@movetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@linetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportatoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportbtoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetotoken=\pgfutil@gobbletwo%
    \def\pgfsyssoftpath@rectcornertoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@rectsizetoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@closepathtoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    #1%
  }%
  \pgf@proc@todo%
}


% Resolve specialround
%
% #1 = a macro that stores a path
% #2 = a macro that stores the new path
%
% Description:
%
% Resolves all specialround tokens. When such a token is encountered,
% the objective is to replace the next corner by a rounded corner.
%

\def\pgfprocessround#1#2{%
  % first, check whether #1 contains \pgfsyssoftpath@specialroundtoken.
  % if not, do quick assignment!
  \expandafter\pgf@processroundcheck\expandafter#1\expandafter#2#1\pgfsyssoftpath@specialroundtoken\pgf@stop%
}

\def\pgf@processroundcheck#1#2#3\pgfsyssoftpath@specialroundtoken#4\pgf@stop{%
  \def\pgf@test{#4}%
  \ifx\pgf@test\pgfutil@empty%
    % ok, nothing to be done!
    \let#2=#1%
  \else%
    % very well...
    \pgf@@processround#1#2%
  \fi%
}


\def\pgf@@processround#1#2{%
  \let\pgfprocess@newpath\pgfutil@empty%
  \let\pgfprocess@moveto\pgfutil@empty%
  \let\pgfprocess@firstto\pgfutil@empty%
  \let\pgfprocess@segment\pgfutil@empty%
  \pgf@xa=0pt%
  \pgf@ya=0pt%
  \expandafter\pgfprocess@round#1\pgf@stop{0pt}{0pt}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
  \let#2=\pgfprocess@newpath%
}

\def\pgfprocess@round#1#2#3{%
  \ifx#1\pgf@stop%
    \let\next=\relax%
  \else%
    \ifx#1\pgfsyssoftpath@specialroundtoken%
      \def\pgfprocess@savex{#2}%
      \def\pgfprocess@savey{#3}%
      \let\next=\pgfprocess@specialround%
      \ifdim#2=0pt%
        \ifdim#3=0pt%
          \let\next=\pgfprocess@round% skip!
        \fi%
      \fi%
    \else%
      \ifx\pgfprocess@firstto\pgfutil@empty%
        \def\pgfprocess@firstto{{#2}{#3}}%
      \fi%
      \pgf@xa=#2%
      \pgf@ya=#3%
      \ifx#1\pgfsyssoftpath@movetotoken%
        % ok, move old segment to newpath
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
        \def\pgfprocess@moveto{#1{#2}{#3}}%
        \let\pgfprocess@firstto=\pgfutil@empty%
        \let\pgfprocess@segment=\pgfutil@empty%
      \else%
        \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}}%
      \fi%
      \let\next=\pgfprocess@round%
    \fi%
  \fi%
  \next%
}

\def\pgfprocess@specialround#1#2#3{%
  \ifx\pgfprocess@firstto\pgfutil@empty%
    \def\pgfprocess@firstto{{#2}{#3}}%
  \fi%
  \let\next=\pgfprocess@round% default: do nothing
  \ifx#1\pgfsyssoftpath@linetotoken%
    % Ok, round a lineto
    \let\next=\pgfprocess@specialroundcope%
  \else%
    \ifx#1\pgfsyssoftpath@curvetosupportatoken%
      % Ok, round a curveto.
      \let\next=\pgfprocess@specialroundcurveto%
    \else%
      \ifx#1\pgfsyssoftpath@closepathtoken%
        % Ok, round a closepath (this is tricky...)
        \let\next=\pgfprocess@specialroundclose%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}%
}%

\def\pgfprocess@specialroundcope#1#2#3#4#5#6{%
  \let\next=\pgfprocess@round% do nothing by default
  \let\pgfprocess@continueafterrounding=\pgfprocess@round%
  \ifx#4\pgfsyssoftpath@linetotoken%
    % ok, let's get kicking...
    \pgf@xc=#5%
    \pgf@yc=#6%
    \let\next=\pgfprocess@@specialround%
  \else%
    \ifx#4\pgfsyssoftpath@curvetosupportatoken%
      \pgf@xc=#5%
      \pgf@yc=#6%
      \let\next=\pgfprocess@@specialround%
    \else%
      \ifx#4\pgfsyssoftpath@closepathtoken%
        \pgf@xc=#5%
        \pgf@yc=#6%
        \let\next=\pgfprocess@@specialround%
      \else
        \ifx#4\pgfsyssoftpath@specialroundtoken%
          \let\next=\pgfprocess@@findrightcoordinates%
        \fi%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}#4{#5}{#6}%
}

\def\pgfprocess@@findrightcoordinates#1#2#3#4#5#6#7#8#9{%
  \pgf@xc=#8%
  \pgf@yc=#9%
  \pgfprocess@@specialround#1{#2}{#3}#4{#5}{#6}#7{#8}{#9}%
}

\def\pgfprocess@@specialround#1#2#3{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1}%
  % calculate start coordinate of the curve
  \pgf@xb=#2%
  \pgf@yb=#3%
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savex}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xa=\pgf@x% save start point of added curve
  \pgf@ya=\pgf@y%
  \edef\pgfprocess@addition{{\the\pgf@x}{\the\pgf@y}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % now add curve
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savey}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xc=\pgf@x% save end point of added curve
  \pgf@yc=\pgf@y%
  % calculate first support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \advance\pgf@xa by 0.5522847\pgf@x%
    \advance\pgf@ya by 0.5522847\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportatoken{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % calculate second support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xc%
    \advance\pgf@y by-\pgf@yc%
    \advance\pgf@xc by 0.5522847\pgf@x%
    \advance\pgf@yc by 0.5522847\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportbtoken{\the\pgf@xc}{\the\pgf@yc}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % add end:
  \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % continue!
  %
  \pgf@xa=#2%
  \pgf@ya=#3%
  \pgfprocess@continueafterrounding%
}

\def\pgfprocess@specialroundcurveto#1#2#3#4#5#6{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}#4{#5}{#6}}% supports
  \pgf@xa=#5%
  \pgf@ya=#6%
  \pgfprocess@specialroundcope}

\def\pgfprocess@specialroundclose{%
  \let\next=\pgfprocess@round%
  \ifx\pgfprocess@moveto\pgfutil@empty%
  \else%
    \ifx\pgfprocess@firstto\pgfutil@empty%
    \else%
      \expandafter\pgfprocess@@specialclosetarget\pgfprocess@firstto%
      \let\pgfprocess@continueafterrounding=\pgfprocess@cleanupafterclose%
      \edef\next{%
        \noexpand\pgfprocess@@specialround%
        \expandafter\expandafter\expandafter\noexpand\expandafter\pgfprocess@@specialclosemoveto\pgfprocess@moveto%
      }%
    \fi%
  \fi%
  \next%
}

\def\pgfprocess@@specialclosetarget#1#2{%
  \pgf@xc=#1%
  \pgf@yc=#2%
}

\def\pgfprocess@@specialclosemoveto#1#2#3{%
  \pgfsyssoftpath@linetotoken{#2}{#3}%
}


\def\pgfprocess@cleanupafterclose#1#2#3{%
  \edef\pgfprocess@moveto{\noexpand\pgfsyssoftpath@movetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \edef\pgf@marshal{\noexpand\pgfprocess@round\noexpand\pgfsyssoftpath@closepathtoken{\the\pgf@xc}{\the\pgf@yc}}%
  \pgf@marshal%
}


% Replace start and end coordinates of a path
%
% #1 = new start coordinate
% #2 = new end coordinate
%
% Description:
%
% This command will replace the first and last coordinates on a path
% by the given coordinates.
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{10}{40}{0}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfsetlinewidth{2pt}
% \pgfusepath{stroke}
% \pgfprocesspathextractpoints{\mypath}
% \pgfprocesspathreplacestartandend{\mypath}
%   {\pgfpointlineatdistance{2pt}{\pgfpointfirstonpath}{\pgfpointsecondonpath}}%
%   {\pgfpointlineatdistance{2pt}{\pgfpointlastonpath}{\pgfpointsecondlastonpath}}%
% \pgfsyssoftpath@setcurrentpath\mypath
% \pgfsetlinewidth{1pt}
% \color{red}
% \pgfusepath{stroke}

\def\pgfprocesspathreplacestartandend#1#2#3{%
  \ifx#1\pgfutil@empty%
  \else%
  {%
    % We (mis)use the current path to store (in a buffered manner) the
    % rest path.
    \pgfsyssoftpath@getcurrentpath\pgf@replace@origpath%
    \let\pgf@prepath=\pgfutil@empty%
    \pgf@process{#3}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \expandafter\pgf@replaceprocessfirst#1\pgf@stop%
    \pgfsyssoftpath@getcurrentpath\pgf@restpath%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\pgf@prepath%
      \expandafter\pgf@newstart\pgf@restpath}%
    % Restore current path
    \pgfsyssoftpath@setcurrentpath\pgf@replace@origpath%
  }%
  \fi%
}

\def\pgf@replaceprocessfirst#1#2#3#4{%
  \def\pgf@origstart{#1{#2}{#3}}%
  \edef\pgf@newstart{\noexpand#1{\the\pgf@x}{\the\pgf@y}}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \ifx#4\pgf@stop%
    \let\pgf@next=\pgfutil@gobble%
  \else%
    \let\pgf@next=\pgf@replaceprocessother%
    \let\pgf@@next=\pgf@@replaceprocessother%
  \fi%
  \pgf@next#4%
}

\def\pgf@replaceprocessother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    \pgf@replace@handle@move%
  \fi%
  \pgf@@next#1%
}
\def\pgf@@replaceprocessother#1#2#3#4{%
  \ifx#4\pgf@stop%
    \edef\pgf@restpathaddition{{\noexpand#1{\the\pgf@xa}{\the\pgf@ya}}}%
    \expandafter\pgfsyssoftpath@addtocurrentpath\pgf@restpathaddition%
    \let\pgf@next=\pgfutil@gobble%
  \else%
    \pgfsyssoftpath@addtocurrentpath{#1{#2}{#3}}%
  \fi%
  \pgf@next#4%
}

\def\pgf@replace@handle@move{%
  \pgfsyssoftpath@getcurrentpath\pgf@restpath%
  % Arggghh! Must reset everything!
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgf@prepath%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\pgf@prepath%
    \expandafter\pgf@origstart\pgf@restpath}%
  % Redo first.
  \let\pgf@@next=\pgf@replaceprocessfirst%
}

\endinput


==> pgfcorepathusage.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorepathusage.code.tex}


% Stroke/fill/clip/etc. the current path. Depending on the options,
% the current path will be stroked/filled/clipped/etc. If no options
% are given, the path is stroked. If multiple options are given, all
% of them are performed (in a sensible order).
%
% #1 = action(s) to be applied to the current path. Valid actions are:
%      stroke -  strokes the path.
%      draw -    strokes the path and adds arrow tips.
%      tips -    adds arrow tips.
%      fill -    fills the path.
%      clip -    clip the path.
%      discard - Discards the path. Same effect as having an empty
%                options list.
%
% Example:
%
% % Draws an edge.
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfusepath{stroke}

\pgfkeys{
  /pgf/stroke/.code=\let\pgf@up@stroke\pgf@up@stroke@text\pgf@up@path@neededtrue,
  /pgf/draw/.code=\let\pgf@up@stroke\pgf@up@stroke@text\pgf@up@path@neededtrue,
  /pgf/fill/.code=\let\pgf@up@fill\pgf@up@fill@text\pgf@up@path@neededtrue,
  /pgf/clip/.code=\let\pgf@up@clip\pgf@up@clip@text\pgf@up@path@neededtrue,
  /pgf/discard/.code=,
  /pgf/use as bounding box/.code=\let\pgf@up@bb\pgf@do@up@bb,
  /pgf/arrow keys/flex/.code=\pgferror{You need to say \string\usetikzlibrary{bending} for flexing and bending arrows},
  /pgf/arrow keys/flex'/.code=\pgferror{You need to say \string\usetikzlibrary{bending} for flexing and bending arrows},
  /pgf/arrow keys/bend/.code=\pgferror{You need to say \string\usetikzlibrary{bending} for flexing and bending arrows},
  /pgf/arrow keys/quick/.code=\pgfarrowsaddtooptions{\let\pgf@arrow@flex@mode\pgf@arrow@mode@is@quick},
}

\pgfkeys{
  /pgf/.cd,
  tips/.is choice,
  tips/.default=true,
  tips/proper/.code=\let\pgf@tips@mode\pgf@tips@mode@onproper,
  tips/on proper draw/.code=\let\pgf@tips@mode\pgf@tips@mode@onproperdraw,
  tips/true/.code=\let\pgf@tips@mode\pgf@tips@mode@true,
  tips/on draw/.code=\let\pgf@tips@mode\pgf@tips@mode@ondraw,
  tips/never/.code=\let\pgf@tips@mode\pgf@tips@mode@false,
  tips/false/.code=\let\pgf@tips@mode\pgf@tips@mode@false,
}
\def\pgf@tips@mode@onproper{4}
\def\pgf@tips@mode@onproperdraw{3}
\def\pgf@tips@mode@true{2}
\def\pgf@tips@mode@ondraw{1}
\def\pgf@tips@mode@false{0}
\let\pgf@tips@mode\pgf@tips@mode@ondraw


% The following can only be set to "true" using the options in the
% module "bending"
\newif\ifpgf@precise@shortening
\def\pgf@arrow@mode@is@quick{0}
\let\pgf@arrow@flex@mode\pgf@arrow@mode@is@quick

\newif\ifpgf@up@path@needed
\newif\ifpgf@up@draw@arrows
\def\pgf@up@stroke@text{stroke}
\def\pgf@up@fill@text{fill}
\def\pgf@up@clip@text{clip}
\def\pgf@do@up@bb{\pgf@relevantforpicturesizefalse}

\def\pgfusepath#1{%
  \pgf@up@path@neededfalse%
  \pgf@up@draw@arrowsfalse%
  \let\pgf@up@stroke\pgfutil@empty%
  \let\pgf@up@fill\pgfutil@empty%
  \let\pgf@up@clip\pgfutil@empty%
  \let\pgf@up@bb\pgfutil@empty%
  \pgfset{#1}%
  \expandafter\def\expandafter\pgf@up@action\expandafter{\csname pgfsys@\pgf@up@fill\pgf@up@stroke\endcsname}%
  \ifnum\pgf@tips@mode=2\relax%
    \pgf@up@path@neededtrue%
  \fi%
  \ifnum\pgf@tips@mode=4\relax%
    \pgf@up@path@neededtrue%
  \fi%
  \ifpgf@up@path@needed%
  \else%
    \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \fi%
  \ifx\pgf@up@stroke\pgfutil@empty%
    \ifx\pgf@up@fill\pgfutil@empty%
      \let\pgf@up@action=\pgfutil@empty%
      \ifx\pgf@up@clip\pgfutil@empty%
      \else%
        % only clipping
        \let\pgf@up@action=\pgfsys@discardpath%
      \fi%
    \fi%
  \fi%
  \pgfsyssoftpath@getcurrentpath\pgf@last@processed@path
  \pgfprocessround{\pgf@last@processed@path}{\pgf@last@processed@path}% change the path
  \pgfsyssoftpath@setcurrentpath\pgf@last@processed@path%
  %
  % Check whether the path is stroked. If so, add half the line width
  % to the bounding box.
  %
  \ifpgf@relevantforpicturesize%
    \ifx\pgf@up@stroke\pgfutil@empty%
    \else%
      \ifdim\pgf@picmaxx=-16000pt\relax%
      \else%
        \pgf@x=\pgf@pathminx\advance\pgf@x by-.5\pgflinewidth%
        \ifdim\pgf@x<\pgf@picminx\global\pgf@picminx\pgf@x\fi%
        \pgf@y=\pgf@pathminy\advance\pgf@y by-.5\pgflinewidth%
        \ifdim\pgf@y<\pgf@picminy\global\pgf@picminy\pgf@y\fi%
        \pgf@x=\pgf@pathmaxx\advance\pgf@x by.5\pgflinewidth%
        \ifdim\pgf@x>\pgf@picmaxx\global\pgf@picmaxx\pgf@x\fi%
        \pgf@y=\pgf@pathmaxy\advance\pgf@y by.5\pgflinewidth%
        \ifdim\pgf@y>\pgf@picmaxy\global\pgf@picmaxy\pgf@y\fi%
      \fi%
    \fi%
  \fi%
  %
  \ifx\pgf@up@clip\pgfutil@empty%
    \ifx\pgf@up@stroke\pgfutil@empty%
      \ifx\pgf@up@action\pgfutil@empty%
        \ifnum\pgf@tips@mode=2\relax%
          \pgf@up@draw@arrows@only%
        \fi%
        \ifnum\pgf@tips@mode=4\relax%
          \pgf@up@draw@arrows@only%
        \fi%
      \else%
        \pgfsyssoftpath@invokecurrentpath%
        \pgf@up@action%
      \fi%
    \else%
      \pgfgetpath\pgf@arrowpath%
      \pgf@path@setup@tempswa%
      \pgfprocesscheckclosed{\pgf@arrowpath}{\pgfutil@tempswafalse}%
      \pgf@path@check@proper%
      \ifpgfutil@tempswa%
        \pgf@check@for@arrow@and@animation%
        \pgf@prepare@end@of@path%
        \begingroup%
          \pgf@prepare@start@of@path%
      \fi%
          \pgfsyssoftpath@invokecurrentpath%
          \pgf@up@action%
          \ifdim\pgfinnerlinewidth>0pt\relax%
            \pgf@stroke@inner@line%
          \fi%
      \ifpgfutil@tempswa%
          \pgf@add@arrow@at@start%
        \endgroup%
        \pgf@add@arrow@at@end%
      \fi%
    \fi%
  \else%
    \pgfsyssoftpath@invokecurrentpath%
    \pgfsys@clipnext%
    \pgf@up@action%
    \pgf@relevantforpicturesizefalse%
  \fi%
  \pgf@up@bb%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgf@resetpathsizes%
  \ignorespaces%
}
\def\pgf@path@setup@tempswa{%
  \ifnum\pgf@tips@mode>0\relax
    \pgfutil@tempswatrue%
  \else
    \pgfutil@tempswafalse%
  \fi%
}
\def\pgf@up@draw@arrows@only{%
  \pgfgetpath\pgf@arrowpath%
  \pgfutil@tempswatrue%
  \pgfprocesscheckclosed{\pgf@arrowpath}{\pgfutil@tempswafalse}%
  \pgf@path@check@proper%
  \ifpgfutil@tempswa%
    \pgf@check@for@arrow@and@animation%
    \pgf@prepare@end@of@path%
    \begingroup%
      \pgf@prepare@start@of@path%
      \pgf@add@arrow@at@start%
    \endgroup%
    \pgf@add@arrow@at@end%
  \fi%
}

\def\pgf@check@for@arrow@and@animation{\pgfsys@if@fresh@currentid{\pgf@check@for@arrow@and@animation@}{}}%
\def\pgf@check@for@arrow@and@animation@{%
  \expandafter\ifx\csname pgfsysanim@path@is@animated@\pgf@sys@id@current@id @\pgfsys@current@type\endcsname\pgfutil@empty%
    % Ok, an animation is here!
    \ifx\pgf@end@tip@sequence\pgfutil@empty%
      \ifx\pgf@start@tip@sequence\pgfutil@empty%
      \else%
        \pgf@check@for@arrow@and@animation@error%
      \fi%
    \else%
      \pgf@check@for@arrow@and@animation@error%
    \fi%
  \fi%
}
\def\pgf@check@for@arrow@and@animation@error{\pgferror{Animated path may not have normal arrow tips. Use a base path with arrow tips}}

\def\pgf@path@check@proper{%
  \ifpgfutil@tempswa%
    \ifnum\pgf@tips@mode>2\relax%
      \pgf@path@check@proper@%
    \fi%
  \fi%
}

\def\pgf@path@check@proper@{%
  {%
    \pgf@x0pt\pgf@y\pgf@x%
    \pgfutil@tempswatrue%
    \let\pgfsyssoftpath@movetotoken\pgf@path@proper@init%
    \let\pgfsyssoftpath@linetotoken\pgf@path@proper@test%%
    \let\pgfsyssoftpath@curvetosupportatoken\pgf@path@proper@test%
    \let\pgfsyssoftpath@curvetosupportbtoken=\pgf@path@proper@test%
    \let\pgfsyssoftpath@curvetotoken\pgf@path@proper@test%
    \let\pgfsyssoftpath@rectcornertoken\pgf@path@proper@test%
    \let\pgfsyssoftpath@rectsizetoken\pgf@path@proper@zero@test%
    \let\pgfsyssoftpath@closepathtoken\pgf@path@proper@test%
    % Execute the path:
    \pgf@arrowpath%
    \expandafter
  }%
  \ifpgfutil@tempswa\pgfutil@tempswafalse\else\pgfutil@tempswatrue\fi%
}

\def\pgf@path@proper@init#1#2{\pgfutil@tempswatrue\pgf@x#1\pgf@y#2}%
\def\pgf@path@proper@test#1#2{%
  \ifdim\pgf@x=#1\relax\else\pgfutil@tempswafalse\fi%
  \ifdim\pgf@y=#2\relax\else\pgfutil@tempswafalse\fi}
\def\pgf@path@proper@zero@test#1#2{%
  \ifdim\pgf@x=0pt\relax\else\pgfutil@tempswafalse\fi%
  \ifdim\pgf@y=0pt\relax\else\pgfutil@tempswafalse\fi}




\def\pgf@stroke@inner@line{%
  \let\pgf@temp@save=\pgf@strokecolor@global
  \pgfsys@beginscope%
  {%
    \pgfsys@setlinewidth{\pgfinnerlinewidth}%
    \pgfsetstrokecolor{\pgfinnerstrokecolor}%
    \pgfsyssoftpath@invokecurrentpath%
    \pgfsys@stroke%
  }%
  \pgfsys@endscope%
  \global\let\pgf@strokecolor@global=\pgf@temp@save
}

\let\pgf@prepare@start@of@path\relax%




% Shorten start/end of paths by a certain amount.
%
% #1 = amount by which paths should be shortened.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{10pt}{0pt}
%
% % The following has the same effect:
% \pgfsetshortenstart{1pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{11pt}{0pt}

\def\pgfsetshortenstart#1{\pgfmathsetlength\pgf@shorten@start@additional{#1}}
\def\pgfsetshortenend#1{\pgfmathsetlength\pgf@shorten@end@additional{#1}}

\newdimen\pgf@shorten@end@additional
\newdimen\pgf@shorten@start@additional



%
%
% Handling the end of a path
%
%
% The "handling" consists of first testing whether we need to do
% anything at all, namely because either an arrow tip should be drawn
% at the end or because the path should be shortened at the end. If
% so, we shorten the path if needed and, later on, add the arrow tip.
%

\newif\ifpgf@worry


% Prepare the end of the path: Test whether anything must be done
% (step 0) and, if so, split the path (step 1), extract the interesting points from
% the path (step 2), prepare further computations (step 3), shorten
% the path (step 4) if necessary, and add the arrow tip (step 4 in
% macro \pgf@add@arrow@at@end, which is called later).

\def\pgf@prepare@end@of@path{%
  \let\pgfprocessresultpathsuffix\relax% flag that nothing has happened...
  \let\pgfprocessresultsubpathsuffix\relax%
  \pgfsyssoftpath@getcurrentpath\pgf@arrowpath%
  %
  % Step 0 start:
  %
  % Do we need to worry about the end?
  %
  \ifx\pgf@arrowpath\pgfutil@empty\else%
    \pgf@worryfalse%
    \ifx\pgf@end@tip@sequence\pgfutil@empty%
    \else%
      \pgf@worrytrue% Yes, worry if we have to draw an arrow
    \fi%
    \pgf@precise@shorteningfalse%
    \pgf@arrow@compute@shortening\pgf@end@tip@sequence%
    \advance\pgf@xa by\pgf@shorten@end@additional%
    \advance\pgf@xb by\pgf@shorten@end@additional%
    \ifdim\pgf@xa=0pt\relax\else\pgf@worrytrue\fi% Also, worry if shortening is requested
    \edef\pgf@path@shortening@distance{\the\pgf@xa}%
    \edef\pgf@arrow@tip@total@length{\the\pgf@xb}%
    %
    % Step 0 done.
    %
    \ifpgf@worry%
      % Ok, need to "worry" about the end, either because we need to
      % shorten it or to draw an arrow head.
      %
      % Step 1: Split
      %
      \pgfprocesssplitpath{\pgf@arrowpath}%
      \pgfprocesssplitsubpath{\pgfprocessresultpathsuffix}%
      %
      % Step 2: extract
      %
      \expandafter\pgf@parse@end\pgfprocessresultsubpathsuffix\pgf@stop\pgf@stop\pgf@stop%
      %
      % Step 3: prep
      %
      \pgf@prep@end%
      %
      % Step 4: shorten
      %
      \ifdim\pgf@path@shortening@distance=0pt\else\pgf@do@shorten@end\fi%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\pgf@arrowpath%
      \expandafter\expandafter\expandafter{\expandafter\pgfprocessresultpathprefix\pgfprocessresultpathsuffix}%
      \pgfsyssoftpath@setcurrentpath\pgf@arrowpath%
    \fi%
  \fi%
}

\def\pgf@parse@end#1#2#3#4#5#6{%
  \ifx#4\pgf@stop% Only a moveto! -> do nothing!
    \def\pgfpointlastonpath{\pgfqpoint{#2}{#3}}%
    \let\pgf@next\relax%
    \let\pgf@do@shorten@end\relax%
    \let\pgf@do@draw@end\pgf@do@draw@straightend%
    \let\pgf@prep@end\pgf@prep@movetoend%
  \else\ifx#4\pgfsyssoftpath@curvetosupportatoken% A curve -> this will get complicated...
    \def\pgfsubpathfourthlasttoken{#1}%
    \def\pgfpointfourthlastonpath{\pgfqpoint{#2}{#3}}%
    \def\pgfpointthirdlastonpath{\pgfqpoint{#5}{#6}}%
    \ifpgf@precise@shortening%
      \let\pgf@do@shorten@end\pgf@do@shorten@curvedend%
      \let\pgf@do@draw@end\pgf@do@draw@curvedend%
      \let\pgf@prep@end\pgf@prep@curveend%
    \else%
      \def\pgfsubpathstart{\noexpand#1{#2}{#3}\noexpand#4{#5}{#6}}%
      \let\pgf@do@shorten@end\pgf@do@shorten@straightend%
      \let\pgf@do@draw@end\pgf@do@draw@straightend%
      \let\pgf@prep@end\pgf@prep@straightend%
    \fi%
    \let\pgf@next\pgf@parse@end@curve@cont%
  \else% A straight line -> great!
    \def\pgfsubpathstart{\noexpand#1{#2}{#3}\noexpand#4}%
    \def\pgfpointsecondlastonpath{\pgfqpoint{#2}{#3}}%
    \def\pgfpointlastonpath{\pgfqpoint{#5}{#6}}%
    \let\pgfpointfourthlastonpath\relax%
    \let\pgfpointthirdlastonpath\relax%
    \let\pgf@next\pgf@parse@end@gobble@three%
    \let\pgf@do@shorten@end\pgf@do@shorten@straightend%
    \let\pgf@do@draw@end\pgf@do@draw@straightend%
    \let\pgf@prep@end\pgf@prep@straightend%
  \fi\fi%
  \pgf@next% Needed for reading rest of path...
}

\def\pgf@parse@end@gobble@three#1#2#3{}%
\def\pgf@parse@end@curve@cont#1#2#3#4#5#6#7#8#9{%
  \def\pgfpointsecondlastonpath{\pgfqpoint{#2}{#3}}%
  \def\pgfpointlastonpath{\pgfqpoint{#5}{#6}}%
  \ifpgf@precise@shortening%
  \else%
    \expandafter\def\expandafter\pgfsubpathstart\expandafter{\pgfsubpathstart\noexpand#1{#2}{#3}\noexpand#4}%
  \fi%
}

%
% Preps
%
\def\pgf@prep@movetoend{%
  \pgf@process{\pgfpointlastonpath}%
  \pgf@xb\pgf@x
  \pgf@yb\pgf@y
  \pgf@xc\pgf@x
  \pgf@yc\pgf@y
}
\def\pgf@prep@straightend{%
  \let\pgf@ref\pgfpointsecondlastonpath
  \ifx\pgfpointlastonpath\pgfpointsecondlastonpath% degenerate!
    \ifx\pgfpointthirdlastonpath\relax% cannot help it: really a zero-length path
    \else%
      \ifx\pgfpointlastonpath\pgfpointthirdlastonpath% double degenerate!
        \let\pgf@ref\pgfpointfourthlastonpath% Use third point for reference.
      \else
        \let\pgf@ref\pgfpointthirdlastonpath% Use third point for reference.
      \fi%
    \fi%
  \fi%
  \pgfpointlineatdistance{\pgf@path@shortening@distance}{\pgfpointlastonpath}{\pgf@ref}%
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
}


%
% Line shortening for straight lines:
%
\def\pgf@do@shorten@straightend{%
  \edef\pgfprocessresultsubpathsuffix{\pgfsubpathstart{\the\pgf@xa}{\the\pgf@ya}}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgfprocessresultpathsuffix%
  \expandafter\expandafter\expandafter{\expandafter\pgfprocessresultsubpathprefix\pgfprocessresultsubpathsuffix}%
}


%
% Draw an end arrow by calling an appropriate subfunction, if necessary
%

\def\pgf@add@arrow@at@end{%
  \ifx\pgf@arrowpath\pgfutil@empty\else%
    \ifx\pgf@end@tip@sequence\pgfutil@empty\else%
      \pgf@do@draw@end%
    \fi%
  \fi%
}

%
% Draw an end arrow at the end of a straight line
%
\def\pgf@do@draw@straightend{%
  {%
    \pgftransformreset%
    \pgftransformarrow{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
    \pgf@arrow@draw@arrow\pgf@end@tip@sequence\pgf@arrow@tip@total@length%
  }%
}





%
%
% Handling the start of a path
%
%
% The "handling" is similar to the case for the start of the path. We
% may be able to skip the splitting if that was done already for the
% end. Otherwise, things are basically the same.
%

% Prepare the start of the path: Test whether anything must be done
% (step 0) and, if so, split the path (step 1) if necessary, extract
% the interesting points from the path (step 2), prepare computations
% (step 3) needed for both shortening and tip adding, shorten the path
% (step 4), and add the arrow tip (step 5 in macro
% \pgf@add@arrow@at@start, which is called later).

\def\pgf@prepare@start@of@path{%
  %
  % Step 0 start:
  %
  % Do we need to worry about the start?
  %
  \ifx\pgf@arrowpath\pgfutil@empty\else%
    \pgf@worryfalse%
    \ifx\pgf@start@tip@sequence\pgfutil@empty\else\pgf@worrytrue\fi% Yes, worry if we have to draw an arrow
    \pgf@precise@shorteningfalse%
    \pgf@arrow@compute@shortening\pgf@start@tip@sequence%
    \advance\pgf@xa by\pgf@shorten@start@additional%
    \advance\pgf@xb by\pgf@shorten@start@additional%
    \ifdim\pgf@xa=0pt\relax\else\pgf@worrytrue\fi% Also, worry if shortening is requested
    \edef\pgf@path@shortening@distance{\the\pgf@xa}%
    \edef\pgf@arrow@tip@total@length{\the\pgf@xb}%
    %
    % Step 0 done.
    %
    \ifpgf@worry%
      % Ok, need to "worry" about the start, either because we need to
      % shorten it or to draw an arrow head.
      %
      % Step 1: Split
      %
      \ifx\pgfprocessresultpathsuffix\relax%
        % Ok, still need to compute the split:
        \pgfprocesssplitpath{\pgf@arrowpath}%
      \fi%
      %
      % Step 2: extract
      %
      \expandafter\pgf@parse@start\pgfprocessresultpathsuffix\pgf@stop\pgf@stop\pgf@stop%
      %
      % Step 3: prep
      %
      \pgf@prep@start%
      %
      % Step 4: shorten
      %
      \ifdim\pgf@path@shortening@distance=0pt\else\pgf@do@shorten@start\fi%
      \expandafter\expandafter\expandafter\def%
      \expandafter\expandafter\expandafter\pgf@arrowpath%
      \expandafter\expandafter\expandafter{\expandafter\pgfprocessresultpathprefix\pgfprocessresultpathsuffix}%
      \pgfsyssoftpath@setcurrentpath\pgf@arrowpath%
    \fi%
  \fi%
}

\def\pgf@parse@start#1#2#3#4#5#6{%
  \def\pgfpointfirstonpath{\pgfqpoint{#2}{#3}}%
  \def\pgfpointsecondonpath{\pgfqpoint{#5}{#6}}%
  \let\pgfpointthirdonpath\relax%
  \let\pgfpointfourthonpath\relax%
  \def\pgfsubpathfirsttoken{\noexpand#1}%
  \def\pgfsubpathsecondtoken{\noexpand#4}%
  \ifx#4\pgf@stop% Only a moveto! -> do nothing!
    \let\pgf@next\relax%
    \let\pgf@do@shorten@start\relax%
    \let\pgf@prep@start\pgf@prep@movetostart%
    \let\pgf@do@draw@start\pgf@do@draw@straightstart%
  \else\ifx#4\pgfsyssoftpath@curvetosupportatoken% A curve -> this will get complicated...
    \ifpgf@precise@shortening%
      \let\pgf@next\pgf@parse@start@curve@cont%
      \let\pgf@do@shorten@start\pgf@do@shorten@curvedstart%
      \let\pgf@do@draw@start\pgf@do@draw@curvedstart%
      \let\pgf@prep@start\pgf@prep@curvedstart%
    \else% can treat the end like a straight line...
      \let\pgf@next\pgf@parse@start@curve@cont@straight%
      \let\pgf@do@shorten@start\pgf@do@shorten@straightstart%
      \let\pgf@do@draw@start\pgf@do@draw@straightstart%
      \let\pgf@prep@start\pgf@prep@straightstart%
    \fi%
  \else% A straight line -> great!
    \let\pgf@next\pgf@parse@start@till@stop%
    \let\pgf@do@shorten@start\pgf@do@shorten@straightstart%
    \let\pgf@do@draw@start\pgf@do@draw@straightstart%
    \let\pgf@prep@start\pgf@prep@straightstart%
  \fi\fi%
  \pgf@next% Needed for reading rest of path...
}

\def\pgf@parse@start@till@stop#1\pgf@stop\pgf@stop\pgf@stop{\def\pgfsubpathend{#1}}%

\def\pgf@parse@start@curve@cont#1#2#3#4#5#6#7\pgf@stop\pgf@stop\pgf@stop{%
  \def\pgfpointthirdonpath{\pgfqpoint{#2}{#3}}%
  \def\pgfpointfourthonpath{\pgfqpoint{#5}{#6}}%
  \def\pgfsubpathend{#7}%
}

\def\pgf@parse@start@curve@cont@straight#1#2#3#4#5#6#7\pgf@stop\pgf@stop\pgf@stop{%
  \def\pgfpointthirdonpath{\pgfqpoint{#2}{#3}}%
  \def\pgfpointfourthonpath{\pgfqpoint{#5}{#6}}%
  \def\pgfsubpathend{#1{#2}{#3}#4{#5}{#6}#7}%
}

%
% Preps
%
\def\pgf@prep@movetostart{%
  \pgf@process{\pgfpointfirstonpath}%
  \pgf@xb\pgf@x
  \pgf@yb\pgf@y
  \pgf@xc\pgf@x
  \pgf@yc\pgf@y
}
\def\pgf@prep@straightstart{%
  \let\pgf@ref\pgfpointsecondonpath
  \ifx\pgfpointfirstonpath\pgfpointsecondonpath% degenerate!
    \ifx\pgfpointthirdonpath\relax% cannot help it: really a zero-length path
    \else%
      \ifx\pgfpointfirstonpath\pgfpointthirdonpath% double degenerate!
        \let\pgf@ref\pgfpointfourthonpath% Use third point for reference.
      \else
        \let\pgf@ref\pgfpointthirdonpath% Use third point for reference.
      \fi%
    \fi%
  \fi%
  \pgfpointlineatdistance{\pgf@path@shortening@distance}{\pgfpointfirstonpath}{\pgf@ref}%
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
}

%
% Line shortening for straight lines:
%
\def\pgf@do@shorten@straightstart{%
  \edef\pgfprocessresultpathsuffix{\pgfsubpathfirsttoken{\the\pgf@xa}{\the\pgf@ya}\pgfsubpathsecondtoken{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\pgfprocessresultpathsuffix%
  \expandafter\expandafter\expandafter{\expandafter\pgfprocessresultpathsuffix\pgfsubpathend}%
}


%
% Draw a start arrow by calling an appropriate subfunction, if necessary
%

\def\pgf@add@arrow@at@start{%
  \ifx\pgf@arrowpath\pgfutil@empty\else%
    \ifx\pgf@start@tip@sequence\pgfutil@empty\else%
      \pgf@do@draw@start%
    \fi%
  \fi%
}

%
% Draw an start arrow at the start of a straight line
%
\def\pgf@do@draw@straightstart{%
  {%
    \pgftransformreset%
    \pgftransformarrow{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
    \pgf@arrow@draw@arrow\pgf@start@tip@sequence\pgf@arrow@tip@total@length%
  }%
}



\let\pgf@shorten@end=\pgfutil@empty
\let\pgf@shorten@start=\pgfutil@empty


\endinput%


==> pgfcorepatterns.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorepatterns.code.tex}

% Creates a new uncolored pattern
%
% [#1] = optional list of variables.
% #2   = pattern name
% #3   = lower left of bounding box
% #4   = upper right of bounding box
% #5   = step vector
% #6   = pattern code
%
% Description:
%
% Declares a new uncolored pattern. An uncolored pattern is a pattern
% that has no inherent color. When the pattern is used, a color for
% the pattern must be supplied.
%
% See the pdf-manual for more details on uncolored patterns.
%
% Specifying a variable list makes the pattern ``mutable''.
%
% The bounding box must be a bounding box of the pattern cell.
%
% The step vector must provide the x- and y-step by which the cells
% are spaced.
%
% The pattern code should be pgf code that can be protocolled.
%
% The transformation matrix will be reset prior to invoking the
% pattern code.
%
% Example:
%
% \pgfdeclarepatternformonly{stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke}
% }
%
\def\pgfdeclarepatternformonly{%
  \def\pgf@pattern@type{formonly}%
  \pgfutil@ifnextchar[{\pgf@declarepattern@checkarg}{\pgf@declarepattern@checkarg[]}%
}


% Creates a new colored pattern
%
% [#1] = optional list of variables.
% #2   = pattern name
% #3   = lower left of bounding box
% #4   = upper right of bounding box
% #5   = step vector
% #6   = pattern code
%
% Description:
%
% Declares a new colored pattern. Such patterns have a one or more
% fixed inherent colors. See the pdf-manual for more details on
% uncolored patterns.
%
% The parameters have the same effect as for uncolored patterns.
%
% Example:
%
% \pgfdeclarepatterninherentlycolored{red stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgfsetfillcolor{red}
%   \pgfsetstrokecolor{black}
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke,fill}
% }
%
\def\pgfdeclarepatterninherentlycolored{%
  \def\pgf@pattern@type{inherentlycolored}%
  \pgfutil@ifnextchar[{\pgf@declarepattern@checkarg}{\pgf@declarepattern@checkarg[]}%
}





\def\pgf@declarepattern@checkarg[#1]{%
  \def\pgf@pattern@tempvars{#1}%
  \ifx\pgf@pattern@tempvars\pgfutil@empty%
    \expandafter\let\expandafter\pgf@next\csname pgf@declarepattern\pgf@pattern@type\endcsname%
  \else%
    \expandafter\let\expandafter\pgf@next\csname pgf@declarepattern\pgf@pattern@type @mutable\endcsname%
  \fi%
  \pgf@next}

\long\def\pgf@declarepatternformonly#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{0}}

\long\def\pgf@declarepatterninherentlycolored#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{1}}

\long\def\pgf@declarepatternformonly@mutable#1#2#3#4#5{%
  \def\pgf@marshal{\pgf@declarepatternmutable{#1}}%
  \expandafter\pgf@marshal\expandafter{\pgf@pattern@tempvars}{#2}{#3}{#4}{#5}{2}%
}

\long\def\pgf@declarepatterninherentlycolored@mutable#1#2#3#4#5#6{%
  \def\pgf@marshal{\pgf@declarepatternmutable{#1}}%
  \expandafter\pgf@marshal\expandafter{\pgf@pattern@tempvars}{#2}{#3}{#4}{#5}{3}%
}

\def\pgfsys@patternmatrix{{1.0}{0.0}{0.0}{1.0}{0.0pt}{0.0pt}}
\def\pgf@declarepattern#1#2#3#4#5#6{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
  \pgfsysprotocol@getcurrentprotocol\pgf@pattern@temp%
  {%
    \pgfinterruptpath%
      \pgfpicturetrue%
      \pgf@relevantforpicturesizefalse%
      \pgftransformreset%
      \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
      \pgfsysprotocol@bufferedtrue%
      \pgfsys@beginscope%
      \pgfsetarrows{-}%
      #5%
      \pgfsys@endscope%
      \pgfsysprotocol@getcurrentprotocol\pgf@pattern@code%
      \global\let\pgf@pattern@code=\pgf@pattern@code%
    \endpgfinterruptpath%
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#3}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#4}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    % Now, build a name for the pattern
    \pgfutil@tempcnta=\pgf@pattern@number%
    \advance\pgfutil@tempcnta by1\relax%
    \xdef\pgf@pattern@number{\the\pgfutil@tempcnta}%
    \expandafter\xdef\csname pgf@pattern@name@#1\endcsname{\the\pgfutil@tempcnta}%
    \expandafter\gdef\csname pgf@pattern@type@#1\endcsname{#6}%
    \xdef\pgf@marshal{\noexpand\pgfsys@declarepattern
      {\csname pgf@pattern@name@#1\endcsname}% name
      {\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}% bbox
      {\the\pgf@xc}{\the\pgf@yc}% x/y step
      \pgfsys@patternmatrix% transformation matrix
      {\pgf@pattern@code}{#6}}%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgf@pattern@temp%
  \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\pgf@marshal%
  }
  {%
    \pgferror{Pattern `#1' already defined}%
  }%
}

\def\pgf@pattern@number{0}%

\def\pgf@declarepatternmutable#1#2#3#4#5#6#7{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
    \expandafter\gdef\csname pgf@pattern@name@#1\endcsname{#1}%
    \expandafter\gdef\csname pgf@pattern@variables@#1\endcsname{#2}%
    \expandafter\gdef\csname pgf@pattern@lowerleft@#1\endcsname{#3}%
    \expandafter\gdef\csname pgf@pattern@upperright@#1\endcsname{#4}%
    \expandafter\gdef\csname pgf@pattern@tilesize@#1\endcsname{#5}%
    \expandafter\long\expandafter\gdef\csname pgf@pattern@code@#1\endcsname{#6}%
    \expandafter\gdef\csname pgf@pattern@type@#1\endcsname{7}%
  }{\pgferror{The pattern `#1' is already defined}}%
}

\def\pgf@ifpatternisinherentlycolored#1#2#3{%
  \expandafter\ifodd\csname pgf@pattern@type@#1\endcsname\relax#2\else#3\fi%
}

\def\pgf@ifpatternismutable#1#2#3{%
  \expandafter\ifnum\csname pgf@pattern@type@#1\endcsname>1\relax#2\else#3\fi%
}

\def\pgfpatternreleasename#1{\expandafter\let\csname pgf@pattern@name@#1\endcsname\relax}






% Set an pattern as fill color
%
% #1 = Name of the pattern
% #2 = Color to be used for the pattern. If the pattern is already
%      colored, this parameter is ignored.
%
% Description:
%
% Sets the pattern for subsequent filling operations.
%
% Example:
%
% \pgfsetfillpattern{stars}{red}
%
\def\pgfsetfillpattern#1#2{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}%
  {%
    \pgferror{Undefined pattern `#1'}%
  }%
  {%
    \pgf@ifpatternismutable{#1}%
    {%
      % So, a mutable pattern. Check to see if the pattern
      % has been used with the current variable values...
      \let\pgf@pattern@tempvars\pgfutil@empty%
      \expandafter\expandafter\expandafter\pgf@pattern@check@vars%
        \csname pgf@pattern@variables@#1\endcsname,\pgf@stop,%
      \edef\pgf@pattern@nametemp{pgf@pattern@#1@\pgf@pattern@tempvars}%
      \expandafter\pgfutil@ifundefined\expandafter{\pgf@pattern@nametemp}%
      {%
        % ...Nope. So declare a new instance of the mutable pattern.
        \pgf@ifpatternisinherentlycolored{#1}%
          {\let\pgf@set@fillpattern@declare\pgfdeclarepatterninherentlycolored}%
          {\let\pgf@set@fillpattern@declare\pgfdeclarepatternformonly}%
        \pgf@set@fillpattern@declare%
          {\pgf@pattern@nametemp}%
          {\csname pgf@pattern@lowerleft@#1\endcsname}%
          {\csname pgf@pattern@upperright@#1\endcsname}%
          {\csname pgf@pattern@tilesize@#1\endcsname}%
          {\csname pgf@pattern@code@#1\endcsname}%
      }%
      {%
        % ...Yep. So do nothing.
      }%
      \expandafter\pgf@set@fillpattern\expandafter{\pgf@pattern@nametemp}{#2}%
      \expandafter\gdef\csname\pgf@pattern@nametemp\endcsname{#1}%
    }%
    {%
      % A non-mutable pattern.
      \pgf@set@fillpattern{#1}{#2}%
    }%
  }%
}


\def\pgf@set@fillpattern#1#2{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
    \pgferror{Undefined pattern `#1'}}
  {%
    \csname pgf@pattern@instantiate@#1\endcsname%
    \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\relax%
    \pgf@ifpatternisinherentlycolored{#1}{%
      \pgfsys@setpatterncolored{\csname pgf@pattern@name@#1\endcsname}%
    }{%
      \pgfutil@colorlet{pgf@tempcolor}{#2}%
      \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
      \pgfutil@extractcolorspec{pgf@tempcolor}{\pgf@tempcolor}%
      \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
      \expandafter\pgf@set@fill@patternuncolored\pgf@rgbcolor\relax{#1}%
    }%
  }%
}

\def\pgf@set@fill@patternuncolored#1,#2,#3\relax#4{%
  \pgfsys@setpatternuncolored{\csname pgf@pattern@name@#4\endcsname}{#1}{#2}{#3}%
}

\def\pgf@pattern@check@vars#1,{%
  \ifx#1\pgf@stop%
    \let\pgf@next\relax%
  \else%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    \expandafter\let\expandafter\pgf@pattern@char#1#1\pgfmath@%
    \ifx\pgf@pattern@char/%
      \edef\pgf@pattern@tempvar{(\pgfkeysvalueof{#1})}%
    \else%
      \expandafter\ifcat\pgf@pattern@char\relax%
        \edef\pgf@pattern@tempvar{(\the#1)}%
      \else%
        \edef\pgf@pattern@tempvar{(#1)}%
      \fi%
    \fi%
    \edef\pgf@pattern@tempvars{\pgf@pattern@tempvars\pgf@pattern@tempvar}%
    \let\pgf@next\pgf@pattern@check@vars%
  \fi%
  \pgf@next%
}

\endinput


==> pgfcorepoints.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorepoints.code.tex}

\newdimen\pgf@picminx
\newdimen\pgf@picmaxx
\newdimen\pgf@picminy
\newdimen\pgf@picmaxy

\newdimen\pgf@pathminx
\newdimen\pgf@pathmaxx
\newdimen\pgf@pathminy
\newdimen\pgf@pathmaxy

\newif\ifpgf@relevantforpicturesize

\def\pgf@process#1{{#1\global\pgf@x=\pgf@x\global\pgf@y=\pgf@y}}

% Save a point.
%
% #1 = macro for storing point.
% #2 = code for point (should define x and y)
%
% Example:
%
% \pgfextract@process\mypoint{\pgf@x=10pt \pgf@y10pt}
% \pgfextract@process\myarcpoint{\pgfpointpolar{30}{5cm and 2cm}}

\def\pgfextract@process#1#2{%
    \pgf@process{#2}%
    \edef#1{\noexpand\global\pgf@x=\the\pgf@x\noexpand\relax\noexpand\global\pgf@y=\the\pgf@y\noexpand\relax}%
}
% This needed until old shapes code changed.
\let\pgfsavepgf@process\pgfextract@process%


% Return a point
%
% #1 = x-coordinate of the point
% #2 = y-coordinate of the point
%
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfpoint{2pt+3cm}{3cm}}

\def\pgfpoint#1#2{%
  \pgfmathsetlength\pgf@x{#1}%
  \pgfmathsetlength\pgf@y{#2}\ignorespaces}


% Quickly a point
%
% #1 = x-coordinate of the point (no calculations done)
% #2 = y-coordinate of the point (no calculations done)
%
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfqpoint{2pt}{3cm}}

\def\pgfqpoint#1#2{\global\pgf@x=#1\relax\global\pgf@y=#2\relax}



% Return the origin.
%
% x = 0
% y = 0
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}

\def\pgfpointorigin{\global\pgf@x=0pt \global\pgf@y=\pgf@x\ignorespaces}



% Return a transformed point
%
% #1 = a point
%
% Description:
%
% This command applies pgf's current transformation matrix to the
% given point. Normally, this is done automatically by commands like
% lineto or moveto, but sometimes you may wish to access a transformed
% point yourself. In the below example, this command is used for a low level
% coordinate system shift.
%
% Example:
%
% \begin{pgflowleveltransformshiftscope}{\pgfpointtransformed{\pgfpointorigin}}
%   \pgfbox[center,center]{Hi!}
% \end{pgflowleveltransformshiftscope}

\def\pgfpointtransformed#1{%
  \pgf@process{%
    #1%
    \pgf@pos@transform@glob%
  }%
}


% Return the difference vector of two points.
%
% #1 = start of vector
% #2 = end of vector
%
% x = x-component of difference
% y = y-component of difference
%
% Example:
%
% \pgfpathmoveto{\pgfpointdiff{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointdiff#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \global\advance\pgf@x by-\pgf@xa\relax%
  \global\advance\pgf@y by-\pgf@ya\relax\ignorespaces}

% Add two vectors.
%
% #1 = first vector
% #2 = second vector
%
% x = x-component of addition
% y = y-component of addition
%
% Example:
%
% \pgfpathmoveto{\pgfpointadd{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointadd#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \global\advance\pgf@x by\pgf@xa%
  \global\advance\pgf@y by\pgf@ya}



% Multiply a vector by a factor.
%
% #1 = factor
% #2 = vector
%
% Example:
%
% \pgfpointscale{2}{\pgfpointxy{0}{1}}

\def\pgfpointscale#1#2{%
  \pgf@process{#2}%
  \pgfmathparse{#1}%
  \global\pgf@x=\pgfmathresult\pgf@x%
  \global\pgf@y=\pgfmathresult\pgf@y%
}
% A "quick" variant of \pgfpointscale which doesn't invoke the math parser for '#1'.
% #1 must be a number without units, no registers are accepted.
\def\pgfqpointscale#1#2{%
  \pgf@process{#2}%
  \global\pgf@x=#1\pgf@x%
  \global\pgf@y=#1\pgf@y%
}


% The intersection of two lines
%
% #1 = point on first line
% #2 = another point on first line
% #3 = point on second line
% #4 = another point on second line
%
% Returns the intersection of the two lines. If there is no
% intersection or if the points #1 and #2 or the points #3 and #4 are
% identical, the behaviour is not specified.
%
% Example:
%
% \pgfpointintersectionoflines{\pgfpointxy{0}{1}}{\pgfpointxy{1}{0}}{\pgfpointxy{2}{2}}{\pgfpointxy{3}{4}}

\def\pgfpointintersectionoflines#1#2#3#4{%
  {%
    %
    % Compute orthogonal vector to #1--#2
    %
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#1}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@ya=-\pgf@ya%
    % Normalise a bit
    \c@pgf@counta=\pgf@xa%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@ya%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xa by\c@pgf@counta\relax%
      \divide\pgf@ya by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@xc=\pgf@sys@tonumber{\pgf@ya}\pgf@x%
    \advance\pgf@xc by\pgf@sys@tonumber{\pgf@xa}\pgf@y%
    %
    % The orthogonal vector is (\pgf@ya,\pgf@xa)
    %
    %
    % Compute orthogonal vector to #3--#4
    %
    \pgf@process{#4}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#3}%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    \pgf@yb=-\pgf@yb%
    % Normalise a bit
    \c@pgf@counta=\pgf@xb%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@yb%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xb by\c@pgf@counta\relax%
      \divide\pgf@yb by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@yc=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
    \advance\pgf@yc by\pgf@sys@tonumber{\pgf@xb}\pgf@y%
    %
    % The orthogonal vector is (\pgf@yb,\pgf@xb)
    %
    % Setup transformation matrix (this is just to use the matrix
    % inversion)
    %
    \pgfsettransform{{\pgf@sys@tonumber\pgf@ya}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@xb}{0pt}{0pt}}%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{\pgfpoint{\pgf@xc}{\pgf@yc}}}%
  }%
}


% The intersection of two circles
%
% #1 = center of first circle
% #2 = center of second circle
% #3 = radius of first circle
% #4 = radius of second circle
% #5 = solution number
%
% Returns the intersection of the two circles. If #5 is to "1", the
% first intersection is returned, otherwise the second. If the circles
% do not intersect, an error may occur.
%
% Example:
%
% \pgfpointintersectionofcircles{\pgfpointxy{0}{1}}{\pgfpointxy{1}{0}}{1cm}{1cm}{1}

\def\pgfpointintersectionofcircles#1#2#3#4#5{%
  {%
    % Store first point in (xa,ya) and radius in xc.
    \pgf@process{#1}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgfmathsetlength{\pgf@xc}{#3}%
    % Store second point in (xb,yb) and radius in yc.
    \pgf@process{#2}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgfmathsetlength{\pgf@yc}{#4}%
    %
    % Ok, now make numbers smaller, in case they are too large
    %
    \c@pgf@counta=1\relax%
    \loop%
      \pgf@scale@downfalse%
      \ifdim\pgf@xc>50pt\relax%
        \pgf@scale@downtrue%
      \fi%
      \ifdim\pgf@yc>50pt\relax%
        \pgf@scale@downtrue%
      \fi%
    \ifpgf@scale@down%
      \multiply\c@pgf@counta by2\relax%
      \divide\pgf@xa by2\relax%
      \divide\pgf@ya by2\relax%
      \divide\pgf@xb by2\relax%
      \divide\pgf@yb by2\relax%
      \divide\pgf@xc by2\relax%
      \divide\pgf@yc by2\relax%
    \repeat%
    % The following code is taken from the Dr. Math internet forum:
    %
    % Let the centers be: (a,b), (c,d)
    % Let the radii be: r, s
    %
    % e = c - a                          [difference in x coordinates]
    % f = d - b                          [difference in y coordinates]
    % p = sqrt(e^2 + f^2)                [distance between centers]
    % k = (p^2 + r^2 - s^2)/(2p)         [distance from center 1 to line
    %                                     joining points of intersection]
    % x = a + ek/p + (f/p)sqrt(r^2 - k^2)
    % y = b + fk/p - (e/p)sqrt(r^2 - k^2)
    % OR
    % x = a + ek/p - (f/p)sqrt(r^2 - k^2)
    % y = b + fk/p + (e/p)sqrt(r^2 - k^2)
    %
    % Since we are running low on registers, use
    % \dimen0 for e
    % \dimen1 for f
    % \dimen2 for p
    % \dimen3 for p^2
    % \dimen4 for k
    % \dimen5 for 1/p
    % \dimen6 for sqrt(r^2 - k^2)
    % \dimen7 for k^2
    % \dimen8 for k/p
    % \dimen9 for sqrt(r^2 - k^2)/p
    % Also note that:
    % \pgf@xa for a
    % \pgf@ya for b
    % \pgf@xb for c
    % \pgf@yb for d
    % \pgf@xc for r
    % \pgf@yc for s
    %
    % Now:
    % e = c - a
    \dimen0=\pgf@xb%
    \advance\dimen0 by-\pgf@xa%
    % f = d - b
    \dimen1=\pgf@yb%
    \advance\dimen1 by-\pgf@ya%
    % p^2 = e^2 + f^2
    \pgf@x=\dimen0\relax%
    \pgf@x=\pgf@sys@tonumber{\pgf@x}\pgf@x%
    \dimen3=\pgf@x%
    \pgf@x=\dimen1\relax%
    \advance\dimen3 by\pgf@sys@tonumber{\pgf@x}\pgf@x%
    % p = sqrt(p^2)
    \pgfmathparse{sqrt(\the\dimen3)}%
    \dimen2=\pgfmathresult pt%
    % 1/p = 1/p
    \pgfmathreciprocal@{\pgfmathresult}%
    \dimen5=\pgfmathresult pt%
    % k = (p^2 + r^2 - s^2)/(2p)
    \dimen4=\dimen3\relax%
    \pgf@x=\pgf@xc%
    \advance\dimen4 by\pgf@sys@tonumber{\pgf@x}\pgf@x\relax%
    \pgf@x=\pgf@yc%
    \advance\dimen4 by-\pgf@sys@tonumber{\pgf@x}\pgf@x\relax%
    \dimen4=.5\dimen4%
    \dimen4=\pgf@sys@tonumber{\dimen5}\dimen4%
    % dimen7 is k^2
    \dimen7=\pgf@sys@tonumber{\dimen4}\dimen4\relax%
    % dimen6 is sqrt(r^2 - k^2)
    \pgfmathparse{sqrt(\pgf@sys@tonumber{\pgf@xc}\pgf@xc-\the\dimen7)}%
    \dimen6=\pgfmathresult pt%
    % dimen8 is k/p
    \dimen8=\pgf@sys@tonumber{\dimen4}\dimen5\relax%
    % dimen9 is sqrt(r^2 - k^2)/p
    \dimen9=\pgf@sys@tonumber{\dimen6}\dimen5\relax%
    \ifnum#5=1\relax%
      % x = a + ek/p + (f/p)sqrt(r^2 - k^2)
      \pgf@x=\pgf@xa%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen0}\dimen8\relax%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen1}\dimen9\relax%
      % y = b + fk/p - (e/p)sqrt(r^2 - k^2)
      \pgf@y=\pgf@ya%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen1}\dimen8\relax%
        %temp
        \pgf@xb=\pgf@sys@tonumber{\dimen0}\dimen9%
        \pgf@xb=-\pgf@xb%
      \advance\pgf@y by\pgf@xb\relax%
    \else%
      % x = a + ek/p - (f/p)sqrt(r^2 - k^2)
      \pgf@x=\pgf@xa%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen0}\dimen8\relax%
        %temp
        \pgf@xb=\pgf@sys@tonumber{\dimen1}\dimen9%
        \pgf@xb=-\pgf@xb%
      \advance\pgf@x by\pgf@xb\relax%
      % y = b + fk/p + (e/p)sqrt(r^2 - k^2)
      \pgf@y=\pgf@ya%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen1}\dimen8\relax%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen0}\dimen9\relax%
    \fi%
    \pgf@x=\c@pgf@counta\pgf@x%
    \pgf@y=\c@pgf@counta\pgf@y%
    \pgf@process{}% get results outside
  }%
}
\newif\ifpgf@scale@down


% Returns point on a line from #2 to #3 at time #1.
%
% #1 = a time, where 0 is the start and 1 is the end
% #2 = start point
% #3 = end point
%
% x = x-component of #1*start + (1-#1)*end
% y = y-component of #1*start + (1-#1)*end
% xa/ya = #1*start + (1-#1)*end
% xb/yb = start point
% xc/yc = end point
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointlineattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointlineattime#1#2#3{%
  \pgf@process{#3}%
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
  \pgf@xc\pgf@x%
  \pgf@yc\pgf@y%
  \pgf@process{#2}%
  \pgf@xb\pgf@x%
  \pgf@yb\pgf@y%
  \pgfmathsetmacro\pgf@temp{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \global\advance\pgf@x by\pgf@temp\pgf@xa%
  \global\advance\pgf@y by\pgf@temp\pgf@ya%
}


% Move point #2 #1 many units in the direction of #3.
%
% #1 = a distance
% #2 = start point
% #3 = end point
%
% Description:
%
% Computes
%
% x/y = start + #1*(normalise(end-start))
%
% and additionally
%
% xa/ya = #1*(normalise(end-start))
% xb/yb = start
% xc/yc = end
%
% Example:
%
% \pgfpathmoveto{\pgfpointlineatdistance{2pt}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}
% \pgfpathlineto{\pgfpointlineatdistance{3pt}{\pgfpointxy{2}{3}}{\pgfpointxy{0}{1}}}

\def\pgfpointlineatdistance#1#2#3{%
  \pgfmathsetlength\pgf@xa{#1}%
  \pgf@process{#2}%
  \pgf@xb\pgf@x% xb/yb = start point
  \pgf@yb\pgf@y%
  \pgf@process{#3}%
  \pgf@xc\pgf@x%
  \pgf@yc\pgf@y%
  \global\advance\pgf@x by-\pgf@xb\relax%
  \global\advance\pgf@y by-\pgf@yb\relax%
  \pgf@process{\pgfpointnormalised{}}% x/y = normalised vector
  \pgf@ya=\pgf@xa\relax%
  \pgf@xa=\pgf@sys@tonumber{\pgf@x}\pgf@xa%
  \pgf@ya=\pgf@sys@tonumber{\pgf@y}\pgf@ya%
  \global\pgf@x=\pgf@xb\relax%
  \global\pgf@y=\pgf@yb\relax%
  \global\advance\pgf@x by\pgf@xa\relax%
  \global\advance\pgf@y by\pgf@ya\relax%
}


% Returns point on a curve from #2 to #5 with controls #3 and #4 at time #1.
%
% #1 = a time
% #2 = start point
% #3 = first control point
% #4 = second control point
% #5 = end point
%
% x = x-component of place on the curve at time t
% y = y-component of place on the curve at time t
%
% Additionally, (\pgf@xa,\pgf@ya) and (\pgf@xb,\pgf@yb) will be on a
% tangent to the point on the curve (this can be useful for computing
% a label rotation). (\pgf@xc,\pgf@yc) will be equal to the end
% point. \pgf@time@s will equal the value of #1 and \pgf@time@t will
% equal 1-#1.
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointcurveattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointcurveattime#1#2#3#4#5{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \global\pgf@x=\pgfmathresult pt%
  \global\pgf@x=-\pgf@x%
  \advance\pgf@x by 1pt%
  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@process{#5}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#4}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  % First iteration:
  \global\pgf@x=\pgf@time@t\pgf@x\global\advance\pgf@x by\pgf@time@s\pgf@xa%
  \global\pgf@y=\pgf@time@t\pgf@y\global\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
  % Second iteration:
  \global\pgf@x=\pgf@time@t\pgf@x\global\advance\pgf@x by\pgf@time@s\pgf@xa%
  \global\pgf@y=\pgf@time@t\pgf@y\global\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  % Save x/y
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Third iteration:
  \global\pgf@x=\pgf@time@t\pgf@x\global\advance\pgf@x by\pgf@time@s\pgf@xa%
  \global\pgf@y=\pgf@time@t\pgf@y\global\advance\pgf@y by\pgf@time@s\pgf@ya%
}



% Returns point on an arc at a certain "time"
%
% #1 = a time
% #2 = center of a ellipse
% #3 = 0-degree axis of the ellipse
% #4 = 90-degree axis of the ellipse
% #5 = start angle of an arc on the ellipse
% #6 = end angle of an arc on the ellipse
%
% Result:
%
% \pgf@x = x-component of place on the arc at time t
% \pgf@y = y-component of place on the arc at time t
%
% Additionally, (\pgf@xa,\pgf@ya) will be a tangent to the
% point on the arc (this can be useful for computing a label rotation).
%
% Example:
%
% \pgfpointarcaxesattime{0.25}{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{0cm}}{\pgfpoint{0cm}{1cm}}{1cm}{30}{40}

\def\pgfpointarcaxesattime#1#2#3#4#5#6{%
  \pgfmathsetmacro\pgf@angle@start{#5}%
  \pgfmathsetmacro\pgf@angle@end{#6}%
  \pgfmathparse{#1}%
  \global\pgf@x=\pgfmathresult pt%
  \global\pgf@x=-\pgf@x%
  \advance\pgf@x by 1pt%
  \pgfmathsetmacro\pgf@angle@mid{\pgf@angle@end*\pgfmathresult+\pgf@angle@start*\pgf@sys@tonumber{\pgf@x}}%
  \pgfmathcos@{\pgf@angle@mid}%
  \let\pgf@angle@cos\pgfmathresult%
  \pgfmathsin@{\pgf@angle@mid}%
  \let\pgf@angle@sin\pgfmathresult%
  \pgf@process{#3}%
  \edef\pgf@angle@zero@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
  \pgf@process{#4}%
  \edef\pgf@angle@ninety@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
  % Compute tangent
  \pgf@process{\pgfpointadd{\pgfpointscale{\pgf@angle@sin}{\pgf@angle@zero@axis}}%
    {\pgfpointscale{-\pgf@angle@cos}{\pgf@angle@ninety@axis}}}%
  \ifdim\pgf@angle@start pt>\pgf@angle@end pt%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
  \else%
    \pgf@xa=-\pgf@x%
    \pgf@ya=-\pgf@y%
  \fi%
  % Compute position
  \pgf@process{\pgfpointadd{#2}{%
      \pgfpointadd{\pgfpointscale{\pgf@angle@cos}{\pgf@angle@zero@axis}}%
    {\pgfpointscale{\pgf@angle@sin}{\pgf@angle@ninety@axis}}}}%
}



% Internal registers
\newdimen\pgf@xx
\newdimen\pgf@xy
\newdimen\pgf@yx
\newdimen\pgf@yy
\newdimen\pgf@zx
\newdimen\pgf@zy



% A polar coordinate
%
% #1 = a degree
% #2 = a radius -- either a dimension or two dimensions separated by
%      " and ".
%
% x = (first dimension in #2) * cos(#1)
% y = (second dimension in #2) * sin(#2)
%
% Example:
%
% \pgfpathmoveto{\pgfpointpolar{30}{1cm}}
% \pgfpathlineto{\pgfpointpolar{30}{1cm and 2cm}}

\def\pgfpointpolar#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polar@#2\@@%
  \else%
    \pgf@polar@#2 and #2\@@%
  \fi%
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \global\pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{\pgfpoint@angle}%
  \global\pgf@y=\pgfmathresult\pgf@y%
}

\def\pgf@polar@#1and #2\@@{%
  \pgfmathsetlength{\pgf@y}{#2}%
  \pgfmathsetlength{\pgf@x}{#1}%
}

% Quick version of the polar coordinate method

\def\pgfqpointpolar#1#2{%
  \global\pgf@x=#2%
  \global\pgf@y=\pgf@x%
  \pgfmathcos@{#1}%
  \global\pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{#1}%
  \global\pgf@y=\pgfmathresult\pgf@y\relax%
}




% A polar coordinate in the xy plane.
%
% #1 = a degree
% #2 = a radius given as a number or two radii
%
% result = (first dim in #2) * x-vector * cos(#1) +
%          (second dim in #2) * y-vector * sin(#1)
%
% Example:
%
% \pgfpathmoveto{\pgfpointpolarxy{30}{2}}

\def\pgfpointpolarxy#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polarxy@#2\@@%
  \else%
    \pgf@polarxy@#2and #2\@@%
  \fi%
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xa=\pgfmathresult\pgf@xa%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@ya=\pgfmathresult\pgf@ya%
  \global\pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@xx%
  \global\advance\pgf@x by \pgf@sys@tonumber{\pgf@ya}\pgf@yx%
  \global\pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@xy%
  \global\advance\pgf@y by \pgf@sys@tonumber{\pgf@ya}\pgf@yy}

\def\pgf@polarxy@#1and #2\@@{%
  \pgfmathsetlength{\pgf@xa}{#1}%
  \pgfmathsetlength{\pgf@ya}{#2}%
}



% A cylindrical coordinate.
%
% #1 = a degree
% #2 = a radius given as a number
% #3 = a height given as a number
%
% result = #2*(x-vector * cos(#1) + y-vector * sin(#1)) + #3*z-vector
%
% Example:
%
% \pgfpathmoveto{\pgfpointcylindrical{30}{2}{1}}

\def\pgfpointcylindrical#1#2#3{%
  \pgfpointpolarxy{#1}{#2}%
  \pgfmathparse{#3}%
  \global\advance\pgf@x by \pgfmathresult\pgf@zx%
  \global\advance\pgf@y by \pgfmathresult\pgf@zy}


% A spherical coordinate.
%
% #1 = a longitude
% #2 = a latitude
% #3 = a radius
%
% result = #3*(cos(#2)*(x-vector * cos(#1) + y-vector * sin(#1)) + sin(#2)*z-vector)
%
% Example:
%
% \pgfpathmoveto{\pgfpointspherical{30}{30}{2}}

\def\pgfpointspherical#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@xb=\pgfmathresult\pgf@xx%
  \pgf@yb=\pgfmathresult\pgf@xy%
  \pgfmathcos@{\pgfpoint@angle}%
  \advance\pgf@xb by \pgfmathresult\pgf@yx%
  \advance\pgf@yb by \pgfmathresult\pgf@yy%
  %
  \pgfmathparse{#2}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xc=\pgfmathresult\pgf@xb%
  \pgf@yc=\pgfmathresult\pgf@yb%
  \pgfmathsin@{\pgfpoint@angle}%
  \advance\pgf@xc by \pgfmathresult\pgf@zx%
  \advance\pgf@yc by \pgfmathresult\pgf@zy%
  \pgfmathparse{#3}%
  \global\pgf@x=\pgfmathresult\pgf@xc%
  \global\pgf@y=\pgfmathresult\pgf@yc\relax%
}


% Store the vector #1 * x-vec + #2 * y-vec
%
% #1 = a factor for the x-vector
% #2 = a factor for the y-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
% Description:
%
% This command can be used to create a new coordinate system
% without using the rotate/translate/scale commands. This
% may be useful, if you do not want arrows and line width to
% be scaled/transformed together with the coordinate system.
%
% Example:
%
% % Create a slanted rectangle
%
% \pgfsetxvec{\pgfpoint{1cm}{1cm}}
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfpathlineto{\pgfpointxy{1}{0}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfclosestroke

\def\pgfpointxy#1#2{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \global\pgf@x=\pgftemp@x\pgf@xx%
  \global\advance\pgf@x by \pgftemp@y\pgf@yx%
  \global\pgf@y=\pgftemp@x\pgf@xy%
  \global\advance\pgf@y by \pgftemp@y\pgf@yy}


% "Quick" variant for \pgfpointxy.
%
% Only numbers without unit are allowed here.
\def\pgfqpointxy#1#2{%
  \global\pgf@x=#1\pgf@xx%
  \global\advance\pgf@x by #2\pgf@yx%
  \global\pgf@y=#1\pgf@xy%
  \global\advance\pgf@y by #2\pgf@yy}

% Store the vector #1 * x-vec + #2 * y-vec + #3 * z-vec
%
% #1 = a factor for the x-vector
% #2 = a factor for the y-vector
% #3 = a factor for the z-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
%
% Description:
%
% This command allows you to use a 3d coordinate system.
%
%
% Example:
%
% % Draw a cubus
%
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{1}{1}{0}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{1}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{1}{0}{1}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{1}{0}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{0}{1}{1}}{\pgfpointxyz{1}{1}{1}}

\def\pgfpointxyz#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \pgfmathparse{#3}%
  \let\pgftemp@z=\pgfmathresult%
  \global\pgf@x=\pgftemp@x\pgf@xx%
  \global\advance\pgf@x by \pgftemp@y\pgf@yx%
  \global\advance\pgf@x by \pgftemp@z\pgf@zx%
  \global\pgf@y=\pgftemp@x\pgf@xy%
  \global\advance\pgf@y by \pgftemp@y\pgf@yy%
  \global\advance\pgf@y by \pgftemp@z\pgf@zy}

% "Quick" variant for \pgfpointxyz.
%
% Only numbers without unit are allowed.
\def\pgfqpointxyz#1#2#3{%
  \global\pgf@x=#1\pgf@xx%
  \global\advance\pgf@x by #2\pgf@yx%
  \global\advance\pgf@x by #3\pgf@zx%
  \global\pgf@y=#1\pgf@xy%
  \global\advance\pgf@y by #2\pgf@yy%
  \global\advance\pgf@y by #3\pgf@zy}



% Set the x-vector
%
% #1 = a point the is the new x-vector
%
% Example:
%
% \pgfsetxvec{\pgfpoint{1cm}{0cm}}

\def\pgfsetxvec#1{%
  \pgf@process{#1}%
  \pgf@xx=\pgf@x%
  \pgf@xy=\pgf@y%
  \ignorespaces}


% Set the y-vector
%
% #1 = a point the is the new y-vector
%
% Example:
%
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}

\def\pgfsetyvec#1{%
  \pgf@process{#1}%
  \pgf@yx=\pgf@x%
  \pgf@yy=\pgf@y%
  \ignorespaces}


% Set the z-vector
%
% #1 = a point the is the new z-vector
%
% Example:
%
% \pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}

\def\pgfsetzvec#1{%
  \pgf@process{#1}%
  \pgf@zx=\pgf@x%
  \pgf@zy=\pgf@y%
  \ignorespaces}



% Default values
\pgfsetxvec{\pgfpoint{1cm}{0cm}}
\pgfsetyvec{\pgfpoint{0cm}{1cm}}
\pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}




% Normalise a point.
%
% #1 = point with coordinates (a,b)
%
% x  = a/\sqrt(a*a+b*b)
% y  = b/\sqrt(a*a+b*b)
%
% Example:
%
% \pgfpointnormalised{\pgfpointxy{2}{1}}

\def\pgfpointnormalised#1{%
  \pgf@process{#1}%
  \pgfmathatantwo{\the\pgf@y}{\the\pgf@x}%
  \let\pgf@tmp=\pgfmathresult%
  \pgfmathcos@{\pgf@tmp}%
  \pgf@x=\pgfmathresult pt\relax%
  \pgfmathsin@{\pgf@tmp}%
  \pgf@y=\pgfmathresult pt\relax%
}





% A point on a rectangle in a certain direction.
%
% #1 = a point pointing in some direction (length should be about 1pt,
%      but need not be exact)
% #2 = upper right corner of a rectangle centered at the origin
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the rectangle's border.
%
% Example:
%
% \pgfpointborderrectangle{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderrectangle#1#2{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  % Ok, let's find out about the direction:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifnum\pgf@xa<0\relax% move into first quadrant
    \global\pgf@x=-\pgf@x%
  \fi%
  \ifnum\pgf@ya<0\relax%
    \global\pgf@y=-\pgf@y%
  \fi%
  \pgf@xc=.125\pgf@x%
  \pgf@yc=.125\pgf@y%
  \c@pgf@counta=\pgf@xc%
  \c@pgf@countb=\pgf@yc%
  \ifnum\c@pgf@countb<\c@pgf@counta%
    \ifnum\c@pgf@counta<255\relax%
      \global\pgf@y=\pgf@yb\relax%
      \global\pgf@x=0pt\relax%
    \else%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
      \global\pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \global\pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
      \ifnum\pgf@y<\pgf@yb%
        \global\pgf@x=\pgf@xb%
      \else% rats, calculate intersection on upper side
        \ifnum\c@pgf@countb<255\relax%
          \global\pgf@x=\pgf@xb\relax%
          \global\pgf@y=0pt\relax%
        \else%
          \pgf@yc=8192pt%
          \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
          \global\pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
          \global\pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
          \global\pgf@y=\pgf@yb%
        \fi%
      \fi%
    \fi%
  \else%
    \ifnum\c@pgf@countb<255\relax%
      \global\pgf@x=\pgf@xb\relax%
      \global\pgf@y=0pt\relax%
    \else%
      \pgf@yc=8192pt%
      \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
      \global\pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \global\pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
      \ifnum\pgf@x<\pgf@xb%
        \global\pgf@y=\pgf@yb%
      \else%
        \ifnum\c@pgf@counta<255\relax%
          \global\pgf@y=\pgf@yb\relax%
          \global\pgf@x=0pt\relax%
        \else%
          \pgf@xc=8192pt%
          \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
          \global\pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
          \global\pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
          \global\pgf@x=\pgf@xb%
        \fi%
      \fi%
    \fi%
  \fi%
  \ifnum\pgf@xa<0\relax\global\pgf@x=-\pgf@x\fi%
  \ifnum\pgf@ya<0\relax\global\pgf@y=-\pgf@y\fi%
}




% An approximation to a point on an ellipse in a certain
% direction. Will be exact only if the ellipse is a circle.
%
% #1 = a point pointing in some direction
% #2 = upper right corner of a bounding box for the ellipse
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the ellipses border.
%
% Example:
%
% \pgfpointborderellipse{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderellipse#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@xa=\pgf@ya% circle. that's easy!
    \pgf@process{\pgfpointnormalised{#1}}%
    \global\pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \global\pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@y%
  \else%
    \ifdim\pgf@xa<\pgf@ya%
      % Ok, first, let's compute x/y:
      \c@pgf@countb=\pgf@ya%
      \divide\c@pgf@countb by65536\relax%
      \global\divide\pgf@x by\c@pgf@countb%
      \global\divide\pgf@y by\c@pgf@countb%
      \pgf@xc=\pgf@x%
      \pgf@yc=8192pt%
      \global\pgf@y=.125\pgf@y%
      \c@pgf@countb=\pgf@y%
      \divide\pgf@yc by\c@pgf@countb%
      \pgf@process{#1}%
      \global\pgf@y=\pgf@sys@tonumber{\pgf@yc}\pgf@y%
      \global\pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@process{\pgfpointnormalised{}}%
      \global\pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \global\pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \else%
      % Ok, now let's compute y/x:
      \c@pgf@countb=\pgf@xa%
      \divide\c@pgf@countb by65536\relax%
      \global\divide\pgf@x by\c@pgf@countb%
      \global\divide\pgf@y by\c@pgf@countb%
      \pgf@yc=\pgf@y%
      \pgf@xc=8192pt%
      \global\pgf@x=.125\pgf@x%
      \c@pgf@countb=\pgf@x%
      \divide\pgf@xc by\c@pgf@countb%
      \pgf@process{#1}%
      \global\pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \global\pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
      \pgf@process{\pgfpointnormalised{}}%
      \global\pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \global\pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \fi%
  \fi%
}





% Extract the x-coordinate of a point to a dimensions
%
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextractx{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 2cm

\def\pgfextractx#1#2{%
  \pgf@process{#2}%
  #1=\pgf@x\relax}


% Extract the y-coordinate of a point to a dimensions
%
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextracty{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 4pt

\def\pgfextracty#1#2{%
  \pgf@process{#2}%
  #1=\pgf@y\relax}


% Stores the most recently used (x,y) coordinates into two macros, #1 and #2.
\def\pgfgetlastxy#1#2{%
    \edef#1{\the\pgf@x}%
    \edef#2{\the\pgf@y}%
}%


\def\pgf@def#1#2#3{\expandafter\def\csname pgf@#1#2\endcsname{#3}}
\pgf@def{cosfrac}{0}{1}
\pgf@def{cosfrac}{1}{0.99995}    \pgf@def{cosfrac}{2}{0.9998}
\pgf@def{cosfrac}{3}{0.99955}    \pgf@def{cosfrac}{4}{0.999201}
\pgf@def{cosfrac}{5}{0.998752}   \pgf@def{cosfrac}{6}{0.998205}
\pgf@def{cosfrac}{7}{0.997559}   \pgf@def{cosfrac}{8}{0.996815}
\pgf@def{cosfrac}{9}{0.995974}   \pgf@def{cosfrac}{10}{0.995037}
\pgf@def{cosfrac}{11}{0.994004}  \pgf@def{cosfrac}{12}{0.992877}
\pgf@def{cosfrac}{13}{0.991656}  \pgf@def{cosfrac}{14}{0.990342}
\pgf@def{cosfrac}{15}{0.988936}  \pgf@def{cosfrac}{16}{0.987441}
\pgf@def{cosfrac}{17}{0.985856}  \pgf@def{cosfrac}{18}{0.984183}
\pgf@def{cosfrac}{19}{0.982424}  \pgf@def{cosfrac}{20}{0.980581}
\pgf@def{cosfrac}{21}{0.978653}  \pgf@def{cosfrac}{22}{0.976644}
\pgf@def{cosfrac}{23}{0.974555}  \pgf@def{cosfrac}{24}{0.972387}
\pgf@def{cosfrac}{25}{0.970143}  \pgf@def{cosfrac}{26}{0.967823}
\pgf@def{cosfrac}{27}{0.965429}  \pgf@def{cosfrac}{28}{0.962964}
\pgf@def{cosfrac}{29}{0.960429}  \pgf@def{cosfrac}{30}{0.957826}
\pgf@def{cosfrac}{31}{0.955157}  \pgf@def{cosfrac}{32}{0.952424}
\pgf@def{cosfrac}{33}{0.949629}  \pgf@def{cosfrac}{34}{0.946773}
\pgf@def{cosfrac}{35}{0.943858}  \pgf@def{cosfrac}{36}{0.940887}
\pgf@def{cosfrac}{37}{0.937862}  \pgf@def{cosfrac}{38}{0.934784}
\pgf@def{cosfrac}{39}{0.931655}  \pgf@def{cosfrac}{40}{0.928477}
\pgf@def{cosfrac}{41}{0.925252}  \pgf@def{cosfrac}{42}{0.921982}
\pgf@def{cosfrac}{43}{0.918669}  \pgf@def{cosfrac}{44}{0.915315}
\pgf@def{cosfrac}{45}{0.911922}  \pgf@def{cosfrac}{46}{0.90849}
\pgf@def{cosfrac}{47}{0.905024}  \pgf@def{cosfrac}{48}{0.901523}
\pgf@def{cosfrac}{49}{0.89799}   \pgf@def{cosfrac}{50}{0.894427}
\pgf@def{cosfrac}{51}{0.890835}  \pgf@def{cosfrac}{52}{0.887217}
\pgf@def{cosfrac}{53}{0.883573}  \pgf@def{cosfrac}{54}{0.879905}
\pgf@def{cosfrac}{55}{0.876216}  \pgf@def{cosfrac}{56}{0.872506}
\pgf@def{cosfrac}{57}{0.868777}  \pgf@def{cosfrac}{58}{0.865031}
\pgf@def{cosfrac}{59}{0.861269}  \pgf@def{cosfrac}{60}{0.857493}
\pgf@def{cosfrac}{61}{0.853704}  \pgf@def{cosfrac}{62}{0.849903}
\pgf@def{cosfrac}{63}{0.846092}  \pgf@def{cosfrac}{64}{0.842271}
\pgf@def{cosfrac}{65}{0.838444}  \pgf@def{cosfrac}{66}{0.834609}
\pgf@def{cosfrac}{67}{0.83077}   \pgf@def{cosfrac}{68}{0.826927}
\pgf@def{cosfrac}{69}{0.82308}   \pgf@def{cosfrac}{70}{0.819232}
\pgf@def{cosfrac}{71}{0.815383}  \pgf@def{cosfrac}{72}{0.811534}
\pgf@def{cosfrac}{73}{0.807687}  \pgf@def{cosfrac}{74}{0.803842}
\pgf@def{cosfrac}{75}{0.8}       \pgf@def{cosfrac}{76}{0.796162}
\pgf@def{cosfrac}{77}{0.792329}  \pgf@def{cosfrac}{78}{0.788502}
\pgf@def{cosfrac}{79}{0.784682}  \pgf@def{cosfrac}{80}{0.780869}
\pgf@def{cosfrac}{81}{0.777064}  \pgf@def{cosfrac}{82}{0.773268}
\pgf@def{cosfrac}{83}{0.769481}  \pgf@def{cosfrac}{84}{0.765705}
\pgf@def{cosfrac}{85}{0.761939}  \pgf@def{cosfrac}{86}{0.758185}
\pgf@def{cosfrac}{87}{0.754443}  \pgf@def{cosfrac}{88}{0.750714}
\pgf@def{cosfrac}{89}{0.746997}  \pgf@def{cosfrac}{90}{0.743294}
\pgf@def{cosfrac}{91}{0.739605}  \pgf@def{cosfrac}{92}{0.735931}
\pgf@def{cosfrac}{93}{0.732272}  \pgf@def{cosfrac}{94}{0.728628}
\pgf@def{cosfrac}{95}{0.724999}  \pgf@def{cosfrac}{96}{0.721387}
\pgf@def{cosfrac}{97}{0.717792}  \pgf@def{cosfrac}{98}{0.714213}
\pgf@def{cosfrac}{99}{0.710651}  \pgf@def{cosfrac}{100}{0.707107}




% Forward declarations for nonlinear stuff (have no effect till module
% nonlineartransformations is loaded)

\let\pgfpointtransformednonlinear\pgfpointtransformed


\endinput


==> pgfcorequick.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorequick.code.tex}

% Quick version of basic drawing commands. Most high-level commands
% are not available if these commands are used.

% Move current point to (#1,#2).
%
% #1 = x dimension of new current point
% #2 = y dimension of new current point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqmoveto#1#2{\pgfsyssoftpath@moveto{#1}{#2}}


% Append a line to (#1,#2) to the current path.
%
% #1 = x dimension of target
% #2 = y dimension of target
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqlineto#1#2{\pgfsyssoftpath@lineto{#1}{#2}}


% Append a bezier spline to the current path.
%
% #1 = x dimension of first support point
% #2 = y dimension of first support point
% #3 = x dimension of second support point
% #4 = y dimension of second support point
% #5 = x dimension of target point
% #6 = y dimension of target point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqcurveto#1#2#3#4#5#6{\pgfsyssoftpath@curveto{#1}{#2}{#3}{#4}{#5}{#6}}




% Append a circle of the given radius around the origin.
%
% #1 = radius
% 
% Example:
%
% \pgfpathqcircle{10pt}
% is quicker than
% \pgfpathcircle{\pgforigin}{10pt}

\def\pgfpathqcircle#1{%
  {%
    \pgf@x=#1%
    \pgf@y=0.5522847\pgf@x%
    \pgfsyssoftpath@moveto{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@y}{\the\pgf@x}{0pt}{\the\pgf@x}%
    \pgfsyssoftpath@curveto{-\the\pgf@y}{\the\pgf@x}{-\the\pgf@x}{\the\pgf@y}{-\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{-\the\pgf@x}{-\the\pgf@y}{-\the\pgf@y}{-\the\pgf@x}{0pt}{-\the\pgf@x}%
    \pgfsyssoftpath@curveto{\the\pgf@y}{-\the\pgf@x}{\the\pgf@x}{-\the\pgf@y}{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@closepath%
  }%
}



% Stroke current path. No hooks called.
% 
% Example:
%
% \pgfpathqmoveto{0cm}{0cm}
% \pgfpathqlineto{1cm}{1cm}
% \pgfpathqcurveto{2cm}{1cm}{2cm}{2cm}{3cm}{2cm}
% \pgfqstroke

\def\pgfusepathqstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@stroke%
  \pgf@resetpathsizes%
}


% Quickly fill current path.

\def\pgfusepathqfill{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fill%
  \pgf@resetpathsizes%
}


% Quickly fill and stroke current path.

\def\pgfusepathqfillstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fillstroke%
  \pgf@resetpathsizes%
}

% Quickly clip current path.

\def\pgfusepathqclip{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@clipnext%
  \pgfsys@discardpath%
  \pgf@resetpathsizes%
}


\endinput


==> pgfcorerdf.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorerdf.code.tex}



% 
%
% The Resource Description Framework (RDF) is a method of enriching
% output files with semantic information. In PGF, you can use the
% following commands to create RDF information that will be inserted
% into the output, provided the output format allows this (SVG
% does). You call any of these commands before an ID-scope and it will
% attach the attribute(s) to this id scope.
%
%
% Example:
%
% ...
% \pgfrdftypeof{http://purl.org/dc/dcmitype/Image}
% \pgfrdfresource{/paper/figures/1}
% \pgfidscope
%   % This ID scope will be flagged as the resource "/paper/figures/1"
%   % and typeof "Image" from the Dublin Core.
%   ...
% \endidscope





% Adds the rdf attribute "about" with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a SafeCURIEorCURIEorIRI, used for stating what
% the data is about (a 'subject' in RDF terminology);" 

\def\pgfrdfabout#1{\pgfsys@rdf@about{#1}}



% Adds the rdf attribute content with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a CDATA string, for supplying machine-readable
% content for a literal (a 'literal object', in RDF terminology);"  

\def\pgfrdfcontent#1{\pgfsys@rdf@content{#1}}



% Adds the rdf attribute datatype with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a TERMorCURIEorAbsIRI representing a datatype,
% to express the datatype of a literal;" 

\def\pgfrdfdatatype#1{\pgfsys@rdf@datatype{#1}}



% Adds the rdf attribute href with value #1 to the next idscope
% The RDF-spec says: "a traditionally navigable IRI for
% expressing the partner resource of a relationship (a 'resource object', in RDF terminology);" 

\def\pgfrdfhref#1{\pgfsys@rdf@href{#1}}



% Adds the rdf attribute inlist to the next idscope.
%
% Description:
%
% The RDF-spec says: "An attribute used to indicate that the object
% associated with a rel or property attribute on the same element is
% to be added to the list for that predicate. Presence of this
% attribute causes a list to be created if it does not already exist."   

\def\pgfrdfinlist{\pgfsys@rdf@inlist}




% Adds #1 to the list of the rdf prefix attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called several times, in which case all values of #1 are
% concatenated with whitespaces. The RDF-spec says: "a white space
% separated list of prefix-name IRI pairs of the form NCName ':' ' '+
% xsd:anyURI"  

\def\pgfrdfprefix#1{\pgfsys@rdf@prefix{#1}}




% Adds #1 to the list of the rdf property attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between a subject and either a resource object if
% given or some literal text (also a 'predicate');"  

\def\pgfrdfproperty#1{\pgfsys@rdf@property{#1}}



% Adds #1 to the list of the rdf rel attribute to the next
% next idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between two resources ('predicates' in RDF
% terminology);" 

\def\pgfrdfrel#1{\pgfsys@rdf@rel{#1}}


% Adds the rdf attribute resource with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a SafeCURIEorCURIEorIRI for expressing the
% partner resource of a relationship that is not intended to be
% navigable (e.g., a 'clickable' link) (also an 'object');"  

\def\pgfrdfresource#1{\pgfsys@rdf@resource{#1}}




% Adds #1 to the list of the rdf rev attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing reverse
% relationships between two resources (also 'predicates');

\def\pgfrdfrev#1{\pgfsys@rdf@rev{#1}}




% Adds an rdf attribute src with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "an IRI for expressing the partner resource of a
% relationship when the resource is embedded (also a 'resource object');" 

\def\pgfrdfsrc#1{\pgfsys@rdf@src{#1}}




% Adds #1 to the list of the rdf typeof attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs that indicate the RDF type(s)
% to associate with a subject;" 

\def\pgfrdftypeof#1{\pgfsys@rdf@typeof{#1}}




% Adds an rdf attribute vocab with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "an IRI that defines the mapping to use when a
% TERM is referenced in an attribute value. See General Use of Terms
% in Attributes and the section on Vocabulary Expansion."  

\def\pgfrdfvocab#1{\pgfsys@rdf@vocab{#1}}





\endinput


==> pgfcorescopes.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorescopes.code.tex}

% Globals

\newbox\pgfpic
\newbox\pgf@hbox

\newbox\pgf@layerbox@main

\newcount\pgf@picture@serial@count



% This if decides whether the position of pictures on the page is
% protocolled or not. Normally,
% this is switched off as it works only with certain drivers and it
% causes external files to be written. When switched on, the position
% of pgfpictures are protocolled and can be referenced using
% \pgfsys@getposition{XXX} where XXX is the value of \pgfpictureid
% inside the picture.
\newif\ifpgfrememberpicturepositiononpage




% Scopes


% Pgf scope environment. All changes of the graphic state are local to
% the scope.
%
% Example:
%
% \begin{pgfscope}
%    \pgfsetlinewidth{3pt}
%    \pgfline{\pgfxy(0,0)}{\pgfxy(3,3)}
% \end{pgfscope}

\def\pgfscope{%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgfsys@beginscope%
    \pgf@resetpathsizes%
    \edef\pgfscope@linewidth{\the\pgflinewidth}%
    \let\pgfscope@stroke@color=\pgf@strokecolor@global%
    \let\pgfscope@fill@color=\pgf@fillcolor@global%
    \begingroup}
\def\endpgfscope{%
    \endgroup%
    \global\pgflinewidth=\pgfscope@linewidth%
    \global\let\pgf@strokecolor@global=\pgfscope@stroke@color%
    \global\let\pgf@fillcolor@global=\pgfscope@fill@color%
  \pgfsys@endscope}




% Quickly insert a box can contain normal TeX text at the origin.
%
% #1 = box of width/height and depth 0pt
%
% Example:
%
% \pgfqbox{\mybox}

\def\pgfqbox#1{%
  \pgfsys@hbox#1%
}


% Insert a box that can contain normal TeX text at the origin, but
% with the current coordinate transformation matrix synced with the
% low-level transformation matrix.
%
% #1 = box of width/height and depth 0pt
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfqbox. However, pgf will use a
% ``TeX-translation'' for the translation part of the transformation
% cm. This will ensure that hyperlinks ``survive'' at least
% translations.
%
% Example:
%
% \pgfqboxsynced{\mybox}

\def\pgfqboxsynced#1{%
  \pgfsys@hboxsynced#1%
}


% Puts some text in a box and inserts it with the current
% transformations applied.
%
% #1 = List of optional positioning. Possible values are ``left'', ``right'',
%      ``top'', ``bottom'' and ``base''.
% #2 = TeX text. May contain verbatims.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{0cm}}
% \pgftext{Hello World!}

\def\pgftext{\pgfutil@ifnextchar[\pgf@text{\pgf@text[]}}%
\def\pgf@text[#1]{%
  \def\pgf@text@options{#1}%
  \pgf@maketext\pgf@after@text}
\def\pgf@after@text{%
  {%
  \def\pgf@text@hshift{center}%
  \def\pgf@text@vshift{center}%
  \expandafter\pgf@text@setkeys\expandafter{\pgf@text@options}%
  \csname pgf@halign\pgf@text@hshift\endcsname%
  \csname pgf@valign\pgf@text@vshift\endcsname%
  %
  \pgfapproximatenonlineartransformation%
  % Protocol sizes:
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgfqboxsynced{\pgf@hbox}%
  }%
}
\def\pgf@text@setkeys{\pgfqkeys{/pgf/text}}%

\pgfkeys{/pgf/text/left/.code=\def\pgf@text@hshift{left}}
\pgfkeys{/pgf/text/center/.code=}
\pgfkeys{/pgf/text/right/.code=\def\pgf@text@hshift{right}}
\pgfkeys{/pgf/text/top/.code=\def\pgf@text@vshift{top}}
\pgfkeys{/pgf/text/bottom/.code=\def\pgf@text@vshift{bottom}}
\pgfkeys{/pgf/text/base/.code=\def\pgf@text@vshift{base}}
\pgfkeys{/pgf/text/at/.cd,.code=\pgftransformshift{#1},.value required}
\pgfkeys{/pgf/text/x/.cd,.code=\pgftransformxshift{#1},.value required}
\pgfkeys{/pgf/text/y/.cd,.code=\pgftransformyshift{#1},.value required}
\pgfkeys{/pgf/text/rotate/.cd,.code=\pgftransformrotate{#1},.value required}

\def\pgf@halignleft{}% do nothing
\def\pgf@haligncenter{\pgftransformxshift{+-.5\wd\pgf@hbox}}
\def\pgf@halignright{\pgftransformxshift{+-\wd\pgf@hbox}}%
\def\pgf@valignbase{}% do nothing
\def\pgf@valignbottom{\pgftransformyshift{+\dp\pgf@hbox}}%
\def\pgf@valigncenter{\pgftransformyshift{+.5\dp\pgf@hbox}\pgftransformyshift{+-.5\ht\pgf@hbox}}%
\def\pgf@valigntop{\pgftransformyshift{+-\ht\pgf@hbox}}%


% Internal function for creating a hbox.
\def\pgf@maketext#1{%
  \def\pgf@@maketextafter{#1}%
  \setbox\pgf@hbox=\hbox\bgroup%
    \pgfinterruptpicture%
      \bgroup%
        \aftergroup\pgf@collectresetcolor%
        \let\next=%
}
\def\pgf@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\pgf@collectresetcolor\let\pgf@temp=}%
  {\pgf@textdone}%
}
\def\pgf@textdone{%
    \endpgfinterruptpicture%
  \egroup%
  \pgf@@maketextafter%
}

\long\def\pgf@makehbox#1{%
  \setbox\pgf@hbox=\hbox{{%
    \pgfinterruptpicture%
      #1%
    \endpgfinterruptpicture%
    }}}



% Picture environment
%
% Example:
%
% \begin{pgfpicture}
%   \pgfsetendarrow{\pgfarrowto}
%   \pgfpathmoveto{\pgfpointxy{-0.9}{0.2}}
%   \pgfpathlineto{\pgfpointxy{0.9}{0.4}}
%   \pgfusepath{stroke}
% \end{pgfpicture}

\def\pgfresetboundingbox{%
    \global\pgf@picmaxx=-16000pt\relax%
    \global\pgf@picminx=16000pt\relax%
    \global\pgf@picmaxy=-16000pt\relax%
    \global\pgf@picminy=16000pt\relax%
}%

\def\pgfpicture{%
  \begingroup%
    \pgfpicturetrue%
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
    \let\pgf@nodecallback=\pgfutil@gobble%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
    \pgf@relevantforpicturesizetrue%
    \pgf@resetpathsizes%
    \pgfutil@ifnextchar\bgroup\pgf@oldpicture\pgf@picture}
\def\pgf@oldpicture#1#2#3#4{%
  \pgfmathsetlength\pgf@picminx{#1}%
  \pgfmathsetlength\pgf@picminy{#2}%
  \pgfmathsetlength\pgf@picmaxx{#3}%
  \pgfmathsetlength\pgf@picmaxy{#4}%
  \pgf@relevantforpicturesizefalse%
  \pgf@picture}

\def\pgf@picture{%
  \setbox\pgfpic\hbox to0pt\bgroup%
    \begingroup%
    \pgfsys@beginpicture%
      \pgfsys@beginscope%
        \begingroup%
        \pgfsetcolor{.}%
        \pgfsetlinewidth{0.4pt}%
        \pgftransformreset%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
        \begingroup%
          \let\pgf@setlengthorig=\setlength%
          \let\pgf@addtolengthorig=\addtolength%
          \let\pgf@selectfontorig=\selectfont%
          \let\setlength=\pgf@setlength%
          \let\addtolength=\pgf@addtolength%
          \let\selectfont=\pgf@selectfont%
          \nullfont\spaceskip0pt\xspaceskip0pt%
          \setbox\pgf@layerbox@main\hbox to0pt\bgroup%
            \begingroup%
  }
\def\endpgfpicture{%
              \ifpgfrememberpicturepositiononpage%
                \hbox to0pt{\pgfsys@markposition{\pgfpictureid}}%
              \fi%
              % ok, now let's position the box
              \ifdim\pgf@picmaxx=-16000pt\relax%
                % empty picture. make size 0.
                \global\pgf@picmaxx=0pt\relax%
                \global\pgf@picminx=0pt\relax%
                \global\pgf@picmaxy=0pt\relax%
                \global\pgf@picminy=0pt\relax%
              \fi%
              % Shift baseline outside:
              \pgf@relevantforpicturesizefalse%
              \pgf@process{\pgf@baseline}%
              \xdef\pgf@shift@baseline{\the\pgf@y}%
              %
              \pgf@process{\pgf@trimleft}%
              \global\advance\pgf@x by-\pgf@picminx
              % prepare \hskip\pgf@trimleft@final.
              % note that \pgf@trimleft@final is also queried
              % by the pgf image externalization.
              \xdef\pgf@trimleft@final{-\the\pgf@x}%
              %
              \pgf@process{\pgf@trimright}%
              \global\advance\pgf@x by-\pgf@picmaxx
              % prepare \hskip\pgf@trimright@final.
              % note that \pgf@trimright@final is also queried
              % by the pgf image externalization.
              \xdef\pgf@trimright@final{\the\pgf@x}%
        %
        \pgf@remember@layerlist@globally
            \endgroup%
            \hss%
          \egroup%
      \pgf@restore@layerlist@from@global
          \pgf@insertlayers%
        \endgroup%
        \pgfsys@discardpath%
        \endgroup%
      \pgfsys@endscope%
    \pgfsys@endpicture%
    \endgroup%
    \hss
  \egroup%
  \pgfsys@typesetpicturebox\pgfpic%
  \endgroup%
}

\def\pgf@remember@layerlist@globally{%
  \global\let\pgf@layerlist@=\pgf@layerlist
}%
\def\pgf@restore@layerlist@from@global{%
  \let\pgf@layerlist=\pgf@layerlist@
}%
\def\pgf@insertlayers{%
  \box\pgf@layerbox@main%
}

\def\pgf@selectfont{\pgf@selectfontorig\nullfont}

\def\pgf@setlength#1#2{% these will be used only when \nullfont is active
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@setlengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}
\def\pgf@addtolength#1#2{%
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@addtolengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}


% Sets the baseline at the y-coordinate of a given point
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point. However, the point will be evaluated *at the end of the
% picture*.
%
% Example:
%
% \pgfsetbaselinepointlater{\pgfpointanchor{mynode}{base}}

\def\pgfsetbaselinepointlater#1{\def\pgf@baseline{#1}}


% Sets the baseline at the y-coordinate of a given point, now
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point.
%
% Example:
%
% \pgfsetbaselinepointnow{\pgfpoint{1cm}{2pt}}

\def\pgfsetbaselinepointnow#1{%
  \pgf@process{#1}%
  \edef\pgf@setter@baseline{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfsetbaselinepointlater{\pgf@setter@baseline}%
}

\def\pgf@default@text{default}%

% Sets the baseline
%
% #1 = baseline
%
% Sets the baseline of the picture. Default is the lower border, which
% is the same as \pgf@picminy
%
% Example:
%
% \pgfsetbaseline{1cm+2pt}
% \pgfsetbaseline{default}% resets to default value

\def\pgfsetbaseline#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@default@text
    \pgfsetbaseline{\pgf@picminy}%
  \else
    \pgfsetbaselinepointlater{\pgfpoint{0pt}{#1}}%
  \fi
}
\pgfsetbaseline{\pgf@picminy}

% controls how the image externalization implements trim:
\newif\ifpgf@trim@lowlevel
\pgfkeys{
  /pgf/trim lowlevel/.is if=pgf@trim@lowlevel,
  /pgf/trim lowlevel/.default=true,
}

% Same as the y-baseline for horizontal alignment.
% The effect is different, though: it is some kind of trimming which
% leaves the bounding box intact.
\def\pgfsettrimleftpointlater#1{\def\pgf@trimleft{#1}}
\def\pgfsettrimleftpointnow#1{%
  \pgf@process{#1}%
  \edef\pgf@setter@baseline{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfsettrimleftpointlater{\pgf@setter@baseline}%
}
% \pgfsettrimleft{<x coord>}
% or
% \pgfsettrimleft{default}
\def\pgfsettrimleft#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@default@text
    \pgfsettrimleft{\pgf@picminx}
  \else
    \pgfsettrimleftpointlater{\pgfpoint{#1}{0pt}}%
  \fi
}
\pgfsettrimleft{\pgf@picminx}

\def\pgfsettrimrightpointlater#1{\def\pgf@trimright{#1}}
\def\pgfsettrimrightpointnow#1{%
  \pgf@process{#1}%
  \edef\pgf@setter@baseline{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfsettrimrightpointlater{\pgf@setter@baseline}%
}
% \pgfsettrimright{<x coord>}
% or
% \pgfsettrimright{default}
\def\pgfsettrimright#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@default@text
    \pgfsettrimright{\pgf@picmaxx}%
  \else
    \pgfsettrimrightpointlater{\pgfpoint{#1}{0pt}}%
  \fi
}
\pgfsettrimright{\pgf@picmaxx}


% Interrupt path
%
% Description:
%
% The environment can be used to insert some drawing commands while
% constructing a path. The drawing commands inside the environment
% will not interfere with the path being constructed ``outside.''
% However, you must ward against graphic state changes using a scope.
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \begin{pgfinterruptpath}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptpath}
% \pgflineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpath
{%
  \begingroup%
  % save all sorts of things...
  \edef\pgf@interrupt@savex{\the\pgf@path@lastx}%
  \edef\pgf@interrupt@savey{\the\pgf@path@lasty}%
  \pgf@getpathsizes\pgf@interrupt@pathsizes%
  \pgfsyssoftpath@getcurrentpath\pgf@interrupt@path%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \let\pgf@interrupt@lastmoveto=\pgfsyssoftpath@lastmoveto%
  \begingroup%
}
\def\endpgfinterruptpath
{%
  \endgroup%
  \pgfsyssoftpath@setcurrentpath\pgf@interrupt@path%
  \pgf@setpathsizes\pgf@interrupt@pathsizes%
  \global\pgf@path@lastx\pgf@interrupt@savex%
  \global\pgf@path@lasty\pgf@interrupt@savey%
  \global\let\pgfsyssoftpath@lastmoveto\pgf@interrupt@lastmoveto%
  \endgroup%
}



% Interrupt bounding box
%
% Description:
%
% The environment can be used to temporarily setup a new bounding box
% computation. The bounding box will be made empty at the beginning of
% the environment and will be reset to its old value after the
% environment.
%
% Example:
%
% \begin{pgfinterruptboundinbox}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptboundinbox}

\def\pgfinterruptboundingbox
{%
  \begingroup%
    \edef\pgf@interrupt@savemaxx{\the\pgf@picmaxx}%
    \edef\pgf@interrupt@saveminx{\the\pgf@picminx}%
    \edef\pgf@interrupt@savemaxy{\the\pgf@picmaxy}%
    \edef\pgf@interrupt@saveminy{\the\pgf@picminy}%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
    \pgf@size@hookedfalse%
    \let\pgf@path@size@hook=\pgfutil@empty%
}
\def\endpgfinterruptboundingbox
{%
    \global\pgf@picmaxx=\pgf@interrupt@savemaxx%
    \global\pgf@picmaxy=\pgf@interrupt@savemaxy%
    \global\pgf@picminx=\pgf@interrupt@saveminx%
    \global\pgf@picminy=\pgf@interrupt@saveminy%
  \endgroup%
}




% Creates an id scope.
%
% Description:
%
% An id scope is not (conceptually) a graphic scope, but a scope that
% has a unique name or "id". This id can be used as a reference point
% for instance for a hyperlink or for an animation (currently, only
% SVG supports ids, all other drivers ignore id scopes).
%
% Prior to using \pgfidscope, call \pgfuseid to install an
% id (and possibly \pgfusetype). The scope will then get this id and,
% likely, a graphic scope is installed. If \pgfuseid has not been
% called or if you try to call \pgfidscope again for the same id,
% nothing happens (except for a \TeX\ group being established).

\def\pgfidscope{\pgfsys@begin@idscope}
\def\endpgfidscope{\pgfsys@end@idscope}

\let\startpgfidscope\pgfidscope
\let\stoppgfidscope\pgfendidscope




% Use an id on the next graphic object
%
% #1 = a name
%
% The next scope or path can be the target of an animation command or
% a hyperlink.

\def\pgfuseid#1{%
  \edef\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgf@lookup@id{#1}%
    \pgfsys@use@id{\pgf@next@id}%
    \expandafter\xdef\csname pgf@id@names@#1\endcsname{{\pgf@next@id}{}}%
  \fi%
}

\def\pgf@lookup@id#1{%
  \expandafter\let\expandafter\pgf@id@name\csname pgf@id@names@#1\endcsname%
  \ifx\pgf@id@name\relax%
    \let\pgf@prev@id\pgfutil@empty%
    \let\pgf@next@id\pgfutil@empty%
  \else%
    \expandafter\pgf@id@parse\pgf@id@name%
  \fi%
  \ifx\pgf@next@id\pgfutil@empty%
    \pgfsys@new@id\pgf@next@id%
    \expandafter\xdef\csname pgf@id@names@#1\endcsname{{\pgf@prev@id}{\pgf@next@id}}%
  \fi%
}
\def\pgf@id@parse#1#2{%
  \def\pgf@prev@id{#1}%
  \def\pgf@next@id{#2}%
}



% Clear the current id
%
% Description:
%
% Sets the current id to be empty so that it cannot be referenced.

\def\pgfclearid{%
  \pgfsys@clear@id%
}


% Get the id that will be given to a name upon the next use
%
% #1 = a macro
% #2 = a name
%
% Description:
%
% #1 will get the id that will be used by \pgfuseid next time for the
% given name.

\def\pgfidrefnextuse#1#2{%
  \edef\pgf@temp{#2}\ifx\pgf@temp\pgfutil@empty\pgferror{Missing name reference for ``\string#1''}\fi%
  \pgf@lookup@id{#2}%
  \let#1\pgf@next@id%
}


% Get the id was last used
%
% #1 = a macro
% #2 = a name
%
% Description:
%
% #1 will get the id that was last used by \pgfuseid for #2.

\def\pgfidrefprevuse#1#2{%
  \edef\pgf@temp{#2}\ifx\pgf@temp\pgfutil@empty\pgferror{Missing name reference for ``\string#1''}\fi%
  \pgf@lookup@id{#2}%
  \let#1\pgf@prev@id%
}


% Use a type
%
% #1 = an id type; when starting with a dot, it is added to the
% current type.
%
% The next scope or path can be the target of an animation command or
% a hyperlink.

\def\pgfusetype#1{%
  \edef\pgf@temp{#1}%
  \expandafter\pgfutil@ifnextchar\expandafter.\expandafter\pgf@id@use@type@add\expandafter\pgf@id@use@type@replace\pgf@temp\pgf@stop
}
\def\pgf@id@use@type@add.#1\pgf@stop{\pgfsys@append@type{#1}}
\def\pgf@id@use@type@replace#1\pgf@stop{\pgfsys@use@type{#1}}

% Push the current type on a global stack
%
% Description:
%
% The current type is pushed onto a global type stack. It can be
% restored using \pgfpoptype.

\def\pgfpushtype{\pgfsys@push@type}


% Pop a type from the type stack
%
% Description:
%
% Restores the most current value from the type stack.

\def\pgfpoptype{\pgfsys@pop@type}




% Alias an id locally or globally
%
% #1 = the alias name
% #2 = a existing id name
%
% Description:
%
% Creates an alias of a name

\def\pgfaliasid#1#2{%
  \expandafter\let\expandafter\pgf@temp\csname pgf@id@names@#2\endcsname%
  \expandafter\let\csname pgf@id@names@#1\endcsname\pgf@temp%
}
\def\pgfgaliasid#1#2{%
  \expandafter\let\expandafter\pgf@temp\csname pgf@id@names@#2\endcsname%
  \expandafter\global\expandafter\let\csname pgf@id@names@#1\endcsname\pgf@temp%
}


% Check whether a name has been forward-referenced
%
% #1 = a name
% #2 = what to do, when has been forward-referenced
% #3 = what to do otherwise
%
% Description:
%
% Depending on whether #1 has been forward-referenced, #2 or #3 will be executed.

\def\pgfifidreferenced#1#2#3{%
  \expandafter\let\expandafter\pgf@id@name\csname pgf@id@names@#1\endcsname%
  \ifx\pgf@id@name\relax%
    #3%
  \else
    \expandafter\pgf@id@parse\pgf@id@name%
    \ifx\pgf@next@id\pgfutil@empty%
      #3%
    \else%
      #2%
    \fi%
  \fi%
}


% Interrupts a picture
%
% Description:
%
% This environment interrupts a picture and temporarily returns to
% normal TeX mode. All sorts of things are saved and restored by this
% environment.
%
% WARNING: Using this environment in conjunction with low level
% transformations can *strongly* upset the typesetting. Typically, the
% contents of this environment should have size/height/depth 0pt in
% the end.
%
% WARNING: This environment should only be used inside typesetting a
% box and this box must in turn be inserted using \pgfqbox.
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \setbox\mybox=\hbox{
%    \begin{pgfinterruptpicture}
%      This is normal text.
%      \begin{pgfpicture} % a subpicture
%        \pgfmoveto{\pgfpoint{1cm}{0cm}}
%        \pgfmoveto{\pgfpoint{1cm}{1cm}}
%        \pgfusepath{stroke}
%      \end{pgfpicture}
%      More text.
%    \end{pgfinterruptpicture}
%  }
% \ht\mybox=0pt
% \wd\mybox=0pt
% \dp\mybox=0pt
% \pgfqbox{\mybox}%
% \pgfpathlineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpicture
{%
  \begingroup%
    \csname tikz@inside@picturefalse\endcsname%
    \pgfinterruptboundingbox%
      \pgftransformreset%
      \pgfinterruptpath%
        \ifx\pgf@selectfontorig\@undefined%
        \else%
          \let\setlength\pgf@setlengthorig%
          \let\addtolength\pgf@addtolengthorig%
          \let\selectfont\pgf@selectfontorig%
        \fi%
        \pgfutil@selectfont%
        \pgfpicturefalse%
        \let\pgf@positionnodelater@macro\relax%
        \pgf@savelayers%
}
\def\endpgfinterruptpicture
{%
        \pgf@restorelayers%
      \endpgfinterruptpath%
    \endpgfinterruptboundingbox%
  \endgroup%
}

\let\pgf@savelayers=\relax
\let\pgf@restorelayers=\relax

\endinput


==> pgfcoreshade.code.tex <==
% Copyright 2019 by Till Tantau
% CMYK and grayscale shadings adaptation copyright 2019 by David Purton
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreshade.code.tex}

%
% Parsing functions
%
\newdimen\pgf@max
\newcount\pgf@sys@shading@range@num
\def\pgf@parsefunc#1{%
  \edef\temp{{#1}}%
  \expandafter\pgf@convertstring\temp%
  \edef\temp{{\pgf@conv}}%
  \expandafter\pgf@@parsefunc\temp}
\def\pgf@@parsefunc#1{%
  \let\pgf@bounds=\pgfutil@empty%
  \let\pgf@funcs=\pgfutil@empty%
  \let\pgf@psfuncs=\pgfutil@empty%
  \let\pgf@encode=\pgfutil@empty%
  \let\pgf@sys@shading@ranges=\pgfutil@empty%
  \pgf@sys@shading@range@num=0\relax%
  \csname pgf@parsefirst\pgf@shading@model\endcsname[#1; ]%
  \csname pgf@parselastdom\pgf@shading@model\endcsname[#1; ]%
  \csname pgf@parsemid\pgf@shading@model\endcsname[#1; ]%
  \ifx\pgf@bounds\pgfutil@empty%
    \edef\pgf@pdfparseddomain{0 1}%
    \edef\pgf@pdfparsedfunction{\pgf@singlefunc\space}%
  \else%
    \edef\pgf@pdfparseddomain{\pgf@doma\space\pgf@domb}%
    \edef\pgf@pdfparsedfunction{%
      << /FunctionType 3 /Domain [\pgf@doma\space\pgf@domb] /Functions
      [\pgf@funcs\space] /Bounds [\pgf@bounds] /Encode [0 1 \pgf@encode]
      >> }% <<
  \fi%
  \xdef\pgf@psfuncs{\pgf@psfuncs}%
  }
\def\pgf@parsefirstrgb[rgb(#1)=(#2,#3,#4)#5]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
  \edef\pgf@sys@shading@start@rgb{\pgf@sys@rgb}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@rgb%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@rgb}%
  \edef\pgf@firstcolor{\pgf@rgb}}
\def\pgf@parselastdomrgb[rgb(#1)=(#2,#3,#4); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@end@rgb{\pgf@sys@rgb}%
    \pgfutil@gobble}{\pgf@parselastdomrgb[}}
\def\pgf@parsemidrgb[rgb(#1)=(#2,#3,#4); {\pgf@parserestrgb[}
\def\pgf@parserestrgb[rgb(#1)=(#2,#3,#4); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@rgb}%
    \pgf@parserestrgb[}}

\def\pgf@getrgbtuplewithmixin#1#2#3{%
  \pgfutil@definecolor{pgfshadetemp}{rgb}{#1,#2,#3}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@getrgb@@\pgf@rgbcolor!}
\def\pgf@getrgb@@#1,#2,#3!{%
  \def\pgf@rgb{#1 #2 #3}%
  \def\pgf@sys@rgb{{#1}{#2}{#3}}%
}

\def\pgf@parsefirstcmyk[cmyk(#1)=(#2,#3,#4,#5)#6]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
  \edef\pgf@sys@shading@start@cmyk{\pgf@sys@cmyk}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@cmyk%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@cmyk}%
  \edef\pgf@firstcolor{\pgf@cmyk}}
\def\pgf@parselastdomcmyk[cmyk(#1)=(#2,#3,#4,#5); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@sys@shading@end@cmyk{\pgf@sys@cmyk}%
    \pgfutil@gobble}{\pgf@parselastdomcmyk[}}
\def\pgf@parsemidcmyk[cmyk(#1)=(#2,#3,#4,#5); {\pgf@parserestcmyk[}
\def\pgf@parserestcmyk[cmyk(#1)=(#2,#3,#4,#5); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space
      \pgf@cmyk\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@cmyk}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@cmyk%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@cmyk}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@cmyk%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@cmyk\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@cmyk}%
    \pgf@parserestcmyk[}}

\def\pgf@getcmyktuplewithmixin#1#2#3#4{%
  \pgfutil@definecolor{pgfshadetemp}{cmyk}{#1,#2,#3,#4}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{cmyk}{\pgf@cmykcolor}%
  \expandafter\pgf@getcmyk@@\pgf@cmykcolor!}
\def\pgf@getcmyk@@#1,#2,#3,#4!{%
  \def\pgf@cmyk{#1 #2 #3 #4}%
  \def\pgf@sys@cmyk{{#1}{#2}{#3}{#4}}%
}

\def\pgf@parsefirstgray[gray(#1)=(#2)#3]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getgraytuplewithmixin{#2}%
  \edef\pgf@sys@shading@start@gray{\pgf@sys@gray}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@gray%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@gray}%
  \edef\pgf@firstcolor{\pgf@gray}}
\def\pgf@parselastdomgray[gray(#1)=(#2); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@sys@shading@end@gray{\pgf@sys@gray}%
    \pgfutil@gobble}{\pgf@parselastdomgray[}}
\def\pgf@parsemidgray[gray(#1)=(#2); {\pgf@parserestgray[}
\def\pgf@parserestgray[gray(#1)=(#2); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@gray\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@gray}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@gray%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@gray}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@gray%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@gray\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@gray}%
    \pgf@parserestgray[}}

\def\pgf@getgraytuplewithmixin#1{%
  \pgfutil@definecolor{pgfshadetemp}{gray}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{gray}{\pgf@graycolor}%
  \expandafter\pgf@getgray@@\pgf@graycolor!}
\def\pgf@getgray@@#1!{%
  \def\pgf@gray{#1}%
  \def\pgf@sys@gray{{#1}}%
}

% Normalized a <color specification> argument for shadings into a
% series of color specifications in the current xcolor color model and write
% the result into \pgf@conv.
%
% Example:
% \pgf@convertstring{rgb(0cm)=(1,0,0); rgb(2cm)=(0,1,0); cmyk(4cm)=(1,0,0,0); gray(1cm)=(3);  color(2cm)=(green); }
% ->
% \pgf@conv = macro:->'rgb(0cm)=(1,0,0); rgb(2cm)=(0,1,0); rgb(4cm)=(0,1,1); rgb(1cm)=(3,3,3); rgb(2cm)=(0,1,0); '
\def\pgf@convertstring#1{%
  \def\pgf@conv{}%
  \pgf@convert#1]%
  }
\def\pgf@convert{%
  \pgfutil@ifnextchar]{\pgfutil@gobble}%done!
  {%
    \pgfutil@ifnextchar;{\pgf@grabsemicolor}%
    {%
      \pgfutil@ifnextchar c{\pgf@gobblec}%
      {%
        \pgfutil@ifnextchar g{\pgf@grabgray}%
        {%
          \pgfutil@ifnextchar o{\pgf@grabcolor}%
          {%
            \pgfutil@ifnextchar m{\pgf@grabcmyk}%
            {%
              \pgfutil@ifnextchar r{\pgf@grabrgb}%
                {\pgferror{Illformed shading
                 specification}\pgf@convert}%
            }%
          }%
        }%
      }%
    }%
  }%
}
\def\pgf@savecolor#1{%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor
    {\pgf@shading@model}{\pgf@color}%
  \expandafter\pgf@convget@\expandafter{\pgf@color}{#1}%
}
\def\pgf@grabsemicolor;{%
  \edef\pgf@conv{\pgf@conv; }\pgf@convert}
\def\pgf@gobblec c{\pgf@convert}
\def\pgf@grabrgb rgb(#1)=(#2,#3,#4){%
  \pgfutil@definecolor{pgf@tempcol}{rgb}{#2,#3,#4}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabcmyk myk(#1)=(#2,#3,#4,#5){%
  \pgfutil@definecolor{pgf@tempcol}{cmyk}{#2,#3,#4,#5}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabgray gray(#1)=(#2){%
  \pgfutil@definecolor{pgf@tempcol}{gray}{#2}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabcolor olor(#1)=(#2){%
  \pgfutil@colorlet{pgf@tempcol}{#2}%
  \pgf@savecolor{#1}%
}
\def\pgf@convget@#1#2{%
  \edef\pgf@conv{\pgf@conv \pgf@shading@model(#2)=(#1)}\pgf@convert}


\newcount\pgf@shadingcount
\pgf@shadingcount=0
{
  \catcode`\/=0
  \catcode`\\=12
  /gdef/pgf@shadingnum{\/the/pgf@shadingcount\}
}

% Set up shading properties based on the current xcolor color model. This is
% called when shadings are declared and used. \ifpgfshadingmodelrgb,
% \ifpgfshadingmodelcmyk, and \ifpgfshadingmodelgray are set so that the type
% 4 function in functional shadings can be converted to the current color
% model. See \pgffuncshading*to* macros.

\newif\ifpgfshadingmodelrgb
\newif\ifpgfshadingmodelcmyk
\newif\ifpgfshadingmodelgray
\def\pgf@setup@shading@model{%
  \pgfshadingmodelrgbtrue
  \pgfshadingmodelcmykfalse
  \pgfshadingmodelgrayfalse
  \XC@sdef\pgf@mod@test{\XC@tgt@mod{natural}}%
  \def\pgf@shading@device{/DeviceRGB}%
  \def\pgf@shading@ps@device{setrgbcolor}%
  \def\pgf@shading@functional@range{0 1 0 1 0 1}%
  \def\pgf@shading@model{rgb}%
  \ifx\pgf@mod@test\XC@mod@cmyk
    \def\pgf@shading@device{/DeviceCMYK}%
    \def\pgf@shading@ps@device{setcmykcolor}%
    \def\pgf@shading@functional@range{0 1 0 1 0 1 0 1}%
    \def\pgf@shading@model{cmyk}%
    \pgfshadingmodelrgbfalse
    \pgfshadingmodelcmyktrue
  \fi
  \ifx\pgf@mod@test\XC@mod@gray
    \def\pgf@shading@device{/DeviceGray}%
    \def\pgf@shading@ps@device{setgray}%
    \def\pgf@shading@functional@range{0 1}%
    \def\pgf@shading@model{gray}%
    \pgfshadingmodelrgbfalse
    \pgfshadingmodelgraytrue
  \fi
  \edef\pgf@sys@driver@dvisvgm{pgfsys-dvisvgm.def}%
  \ifx\pgfsysdriver\pgf@sys@driver@dvisvgm
    \def\pgf@shading@model{rgb}%
  \fi
  \edef\pgf@sys@driver@texforht{pgfsys-tex4ht.def}%
  \ifx\pgfsysdriver\pgf@sys@driver@texforht
    \def\pgf@shading@model{rgb}%
  \fi
}


% Declares a horizontal shading for later use. The shading is a
% horizontal bar that changes its color.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification in the following format: A list of colors
%      that the bar should have at certain points. If the bar should
%      be red at 1cm, this is specified as
%      "rgb(1cm)=(1,0,0)". Multiple specifications are separated by a
%      semicolon and a space. At least two specifications must be
%      given. The specified positions must be given in increasing
%      order.
%
% Description:
%
% The optional dependencies have the following effect: If present, it
% should consist of a list of colors, separated by commas. Each time
% the shading is used, these colors will be reevaluated. It will be
% checked whether the colors still have their "original meaning". If
% the colors have changed, a new shading will be created internally to
% reflect the changed color's values.
%
% Example:
%
% \pgfdeclarehorizontalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm long: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclarehorizontalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declarehorizontalshading{\pgf@declarehorizontalshading[]}}
\def\pgf@declarehorizontalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname\pgfutil@empty
    \pgfsys@horishading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@horishading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a vertical shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification
%
% Example:
%
% \pgfdeclareverticalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm high: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareverticalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declareverticalshading{\pgf@declareverticalshading[]}}
\def\pgf@declareverticalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfsys@vertshading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@vertshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a radial shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = center of inner circle
% #4 = color specification
%
% Description:
%
% A radial shading creates a smooth color transition between two
% circles. The center of the inner circle is at the give position. Its
% radius is the start of the color specification. The
% center of the outer circle is at the center of the whole shading,
% whose radius is the end of the color specification. For example,
% suppose the color specification is "rgb(1cm)=(1,1,1); rgb(2cm)=(0,0,0)".
% Then the shading would be 4cm times 4cm large. The inner circle would
% have diameter 1cm and the outer circle would have diameter 2cm. The
% outer circle would be centered in the middle of the shading, whereas
% the outer circle would be centered at the given position.
%
% Example:
%
% \pgfdeclareradialshading{redtogreentoblue}{\pgfpoint{2cm}{2cm}}{%
%   rgb(10pt)=(1,0,0); % red
%   rgb(2cm)=(0,1,0); % green
%   rgb(3cm)=(0,0,1)}
%
% \begin{document}
%   The following ball has diameter 3cm: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareradialshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declareradialshading{\pgf@declareradialshading[]}}
\def\pgf@declareradialshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfsys@radialshading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@radialshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}




% Declares a functional shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = lower left corner of the shading as a pgfpoint.
% #4 = upper right corner of the shading as a pgfpoint.
% #5 = Preparation code
% #6 = a PDF type 4 function (restricted Postscript function), see the
%      PDF-specification 1.7, section 3.9.4
%
% Description:
%
% This command creates a so-called functional shading. For such a
% shading the color of each point is calculated by calling a function
% for each point that gets the coordinates as input and yields the
% color as an output. Note that the function is evaluated by the
% *renderer*, not by PGF or TeX or someone else at compile-time. This
% means that the evaluation of this function has to be done *extremely
% quickly* and the function should be *very simple*. For this reason,
% only a very restricted set of operations are possible in the
% function (see 3.9.4 of the PDF-spec 1.7). Also functions should be
% kept small. Any errors in the function will only be noticed by the
% renderer.
%
% The function gets the coordinates of a point as input (as bp). This
% input consists of the top two elements of an otherwise empty
% (virtual, PostScript) stack. The function should then replace these
% two values by one value representing the gray color of the point for a
% grayscale shading, three values, representing the red, green, and blue color
% of the point for an RGB shading, or four values, representing the cyan,
% magenta, yellow, and black color of the point for a CMYK shading. The
% numbers should be real values, not integers since Apple's PDF renderer is
% broken in this regard (use cvr at the end if necessary).
%
% Conceptually, the function will be evaluated once for each point of
% the rectangle (#3) to (#4). A renderer may choose to evaluate the
% function at less points, but, in principle, the function will be
% evaluated for each pixel independently.
%
% Because of the rather difficult PostScript syntax, use this macro
% only *if you know what you are doing* (or if you are adventurous, of
% course).
%
% As for other shadings, the optional dependencies argument is used to
% determine whether a shading needs to be recalculated when a color
% has changed.
%
% The code #5 is executed each time a shading is
% (re)calculated. Typically, it will contain code to extract
% coordinates from colors (see below).
%
% Inside the PostScript function #6 you cannot use colors
% directly. Rather, you must push the color components on the
% stack. For this, it is useful to call \pgfshadecolortorgb,
% \pgfshadecolortocmyk, or \pgfshadecolortogray in the startup
% code #4. The macro takes a color name as input and stores the color's
% component real numbers between 0.0 and 1.0 separated
% by spaces (which is exactly what you need if you want to push it on
% a stack) in a macro.
%
% Example:
%
%\pgfdeclarefunctionalshading{twospots}{\pgfpointorigin}{\pgfpoint{200bp}{200bp}}{}{
%  2 copy
%  90 sub dup mul exch
%  80 sub dup mul add sqrt
%  dup mul neg 1.0005 exch exp 1.0 exch sub
%  3 1 roll
%  120 sub dup mul exch
%  100 sub dup mul add sqrt
%  dup mul neg 1.002 exch exp 1.0 exch sub
%  1.0
%}
%
% \pgfdeclarefunctionalshading[mycol]{sweep}{\pgfpointorigin}{\pgfpoint{100bp}{100bp}}
% {\pgfshadecolortorgb{mycol}{\myrgb}}{
%   add 150 div   % not very useful...
%   dup
%   \myrgb        % push mycol
%   5 4 roll      % multiply all components by calculated value
%   mul
%   3 1 roll
%   3 index
%   mul
%   3 1 roll
%   4 3 roll
%   mul
%   3 1 roll
% }
%
% \begin{document}
%   Have a look at this: \pgfuseshading{twospots}.
%   Here is \colorlet{mycol}{green!50}\pgfuseshading{sweep} in green
%   and in \colorlet{mycol}{red!50!blue}\pgfuseshading{sweep} in red/blue.
% \end{document}

\def\pgfdeclarefunctionalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declarefunctionalshading{\pgf@declarefunctionalshading[]}}
\def\pgf@declarefunctionalshading[#1]#2#3#4#5#6{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfshade@functionaldo{#2}{#3}{#4}{#5}{#6}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfshade@functionaldo}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}{#5}{#6}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}
\def\pgfshade@functionaldo#1#2#3#4#5{%
  \begingroup
    #4%
    \pgfsys@functionalshading{#1}{#2}{#3}{#5}%
    \expandafter\pgfmath@smuggleone\csname @pgfshading#1!\endcsname
  \endgroup
}

\def\pgfshadecolortorgb#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgfshading@rgb\pgf@rgbcolor\relax%
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space\pgf@sys@tonumber{\pgf@xb}\space\pgf@sys@tonumber{\pgf@xc}\space}%
  \c@pgf@counta\escapechar%
  \escapechar-1\relax%
  \expandafter\edef\csname\string#2red\endcsname{\pgf@sys@tonumber{\pgf@xa}\space}%
  \expandafter\edef\csname\string#2green\endcsname{\pgf@sys@tonumber{\pgf@xb}\space}%
  \expandafter\edef\csname\string#2blue\endcsname{\pgf@sys@tonumber{\pgf@xc}\space}%
  \escapechar\c@pgf@counta%
}
\def\pgfshading@rgb#1,#2,#3\relax{%
  \pgf@xa=#1pt%
  \pgf@xb=#2pt%
  \pgf@xc=#3pt%
}

\def\pgfshadecolortocmyk#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{cmyk}{\pgf@cmykcolor}%
  \expandafter\pgfshading@cmyk\pgf@cmykcolor\relax%
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space\pgf@sys@tonumber{\pgf@xb}\space
    \pgf@sys@tonumber{\pgf@xc}\space\pgf@sys@tonumber{\pgf@xd}\space}%
  \c@pgf@counta\escapechar%
  \escapechar-1\relax%
  \expandafter\edef\csname\string#2cyan\endcsname{%
    \pgf@sys@tonumber{\pgf@xa}\space}%
  \expandafter\edef\csname\string#2magenta\endcsname{%
    \pgf@sys@tonumber{\pgf@xb}\space}%
  \expandafter\edef\csname\string#2yellow\endcsname{%
    \pgf@sys@tonumber{\pgf@xc}\space}%
  \expandafter\edef\csname\string#2black\endcsname{%
    \pgf@sys@tonumber{\pgf@xd}\space}%
  \escapechar\c@pgf@counta
}
\def\pgfshading@cmyk#1,#2,#3,#4\relax{%
  \pgf@xa=#1pt%
  \pgf@xb=#2pt%
  \pgf@xc=#3pt%
  \pgf@xd=#4pt%
}

\def\pgfshadecolortogray#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{gray}{\pgf@graycolor}%
  \expandafter\pgfshading@gray\pgf@graycolor\relax
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space}%
  \c@pgf@counta\escapechar
  \escapechar-1\relax
  \expandafter\edef\csname\string#2gray\endcsname{%
    \pgf@sys@tonumber{\pgf@xa}\space}%
  \escapechar\c@pgf@counta
}
\def\pgfshading@gray#1\relax{%
  \pgf@xa=#1pt%
}

% Functions to convert between color models in the type 4 PostScript data of
% functional shadings.

\def\pgffuncshadingrgbtocmyk{%
  1.0 exch sub 3 1 roll
  1.0 exch sub 3 1 roll
  1.0 exch sub 3 1 roll
  3 copy
  2 copy gt { exch } if pop
  2 copy gt { exch } if pop
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
}

\def\pgffuncshadingrgbtogray{%
  0.11 mul exch 0.59 mul add exch 0.3 mul add
}

\def\pgffuncshadingcmyktorgb{%
  % covert to CMY
  dup 3 1 roll add
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll add
  1.0 2 copy gt { exch } if pop
  4 1 roll
  add
  1.0 2 copy gt { exch } if pop
  3 1 roll
  % covert to RGB
  1.0 exch sub
  3 1 roll
  1.0 exch sub
  3 1 roll
  1.0 exch sub
  3 1 roll
}

\def\pgffuncshadingcmyktogray{%
  exch 0.11 mul add exch 0.59 mul add exch 0.3 mul add
  1.0 2 copy gt { exch } if pop
  1.0 exch sub
}

\def\pgffuncshadinggraytorgb{%
  dup dup
}

\def\pgffuncshadinggraytocmyk{%
  0.0 0.0 0.0
  4 3 roll
}

% Inserts a box into the text that contains a previously defined
% shading.
%
% #1 = Name of a shading
%
% Example:
%
% \pgfuseshading{redtogreentoblue}

\def\pgfuseshading#1{%
  \edef\pgf@shadingname{@pgfshading#1}%
  \pgf@tryextensions{\pgf@shadingname}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@shadingname}%
  {\pgferror{Undefined shading "#1"}}%
  {%
    \edef\pgf@shade@adds{\csname pgf@num\pgf@shadingname\endcsname}%
    \pgfutil@ifundefined{pgf@deps\pgf@shadingname}%
    {}%
    {%
      \pgf@setup@shading@model
      \begingroup
        \pgfutil@globalcolorsfalse
        \edef\@list{\csname pgf@deps\pgf@shadingname\endcsname}%
        \pgfutil@for\@temp:=\@list\do{%
          \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{\@temp}}%
          \pgfutil@extractcolorspec{\@temp}{\pgf@tempcolor}%
          \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{\pgf@shading@model}{\pgf@color}%
          \edef\pgf@shade@adds{\pgf@shade@adds,\pgf@color}%
        }%
        \pgfmath@smuggleone\pgf@shade@adds
      \endgroup
    }%
    \expandafter\pgf@strip@shadename\pgf@shadingname!!%
    \edef\pgf@shadingxname{@pgfshading\pgf@basename\pgf@shade@adds!}%
    \pgfutil@ifundefined{\pgf@shadingxname}%
    {%
      \begingroup
        \edef\@temp{\expandafter\noexpand\csname pgf@func\pgf@shadingname\endcsname}%
        \edef\@args{{\pgf@basename\pgf@shade@adds}}%
        \expandafter\expandafter\expandafter\def
        \expandafter\expandafter\expandafter\@@args
        \expandafter\expandafter\expandafter{\csname pgf@args\pgf@shadingname\endcsname}%
        \expandafter\expandafter\expandafter\@temp\expandafter\@args\@@args
        \expandafter\pgfmath@smuggleone\csname\pgf@shadingxname\endcsname
      \endgroup
    }%
    {}%
    \pgf@invokeshading{\csname\pgf@shadingxname\endcsname}%
  }%
}

\def\pgf@strip@shadename @pgfshading#1!!!{\def\pgf@basename{#1}}

\def\pgf@invokeshading#1{%
  \ifpgfpicture%
    \pgfsys@shadinginsidepgfpicture{#1}%
  \else%
    \pgfsys@shadingoutsidepgfpicture{#1}%
  \fi%
}


% Create an alias name for a shading
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfaliasshading{shading!25}{shadingshaded}

\def\pgfaliasshading#1#2{%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname @pgfshading#2!\endcsname%
  \expandafter\let\csname @pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@num@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@num@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@deps@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@deps@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@func@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@func@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@args@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@args@pgfshading#1!\endcsname=\pgf@temp%
}




% Shades the current path, but does not discard it.
%
% #1 - a shading (see below)
% #2 - an angle
%
% Description:
%
% \pgfshadepath  ``tries'' to fill the
% current path with a shading. The shading's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% shading will be rotated by #2 and then rescaled so that it
% completely covers the path. Then the path will be used (locally) for
% clipping and the shading is drawn.
%
% In addition to the rotation, any transformation set by the
%\pgfsetadditionalshadetransform will also be applied.
%
% After all this, the path can still be used for the normal
% stroking/clipping operations.
%
% The shading is rotated around its middle. If no rotation occurs, the
% lower left corner of the path will lie on (25bp, 25bp), the upper
% right corner on (75bp, 75bp).
%
% Example:
%
% \pgfdeclareverticalshading{myshading}{100bp}{color(0pt)=(red); color(100bp)=(green)}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfshadepath{myshading}{0}
% \pgfusepath{stroke}

\def\pgfshadepath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    \pgfwarning{No path specified that can be filled}%
  \else%
    \begingroup%
      % Calculate center:
      \pgf@xb=.5\pgf@pathmaxx%
      \advance\pgf@xb by.5\pgf@pathminx%
      \pgf@yb=.5\pgf@pathmaxy%
      \advance\pgf@yb by.5\pgf@pathminy%
      % Calculate rotation:
      \pgfmathparse{#2}%
      \let\pgfshade@angle=\pgfmathresult
      \pgfmathsin@\pgfshade@angle
      \let\pgfshade@sin=\pgfmathresult
      \pgfmathcos@\pgfshade@angle
      \let\pgfshade@cos=\pgfmathresult
      % width and height of the bounding box
      \pgf@xa=\pgf@pathmaxx
      \advance\pgf@xa by-\pgf@pathminx
      \pgf@ya=\pgf@pathmaxy
      \advance\pgf@ya by-\pgf@pathminy
      % Calculate scaling:
      % xscale = 1pt/50bp * (w*|cos(a)|+h*|sin(a)|)/(|cos(a)|+|sin(a)|)
      % yscale = 1pt/50bp * (w*|sin(a)|+h*|cos(a)|)/(|cos(a)|+|sin(a)|)
      % 1pt/50bp = .01992528
      \pgfmathabs@\pgfshade@sin
      \let\pgfshade@abssin=\pgfmathresult
      \pgfmathabs@\pgfshade@cos
      \let\pgfshade@abscos=\pgfmathresult
      \pgf@xc=\pgfshade@abscos\pgf@xa
      \advance\pgf@xc by\pgfshade@abssin\pgf@ya
      \pgf@yc=\pgfshade@abssin\pgf@xa
      \advance\pgf@yc by\pgfshade@abscos\pgf@ya
      \pgfmathadd@\pgfshade@abscos\pgfshade@abssin
      \pgfmathdivide@{.01992528}{\pgfmathresult}%
      \pgf@xc=\pgfmathresult\pgf@xc
      \pgf@yc=\pgfmathresult\pgf@yc
      \ifdim\pgf@xc<0.0001pt
        \ifdim\pgf@xc>-0.0001pt
          \pgf@no@shadetrue
        \fi
      \fi
      \ifdim\pgf@yc<0.0001pt
        \ifdim\pgf@yc>-0.0001pt
          \pgf@no@shadetrue
        \fi
      \fi
      \ifpgf@no@shade\else
        \pgfsys@beginscope
          \pgfsyssoftpath@invokecurrentpath
          \pgfsys@clipnext
          \pgfsys@discardpath
          % Compute new transformation matrix:
          % shift
          \pgfsys@transformcm{1}{0}{0}{1}{\the\pgf@xb}{\the\pgf@yb}%
          % rotation
          \pgf@x=\pgfshade@sin pt%
          \pgf@xa=-\pgf@x%
          \pgfsys@transformcm{\pgfshade@cos}{\pgfshade@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgfshade@cos}{0pt}{0pt}%
          % scaling
          \pgfsys@transformcm{\pgf@sys@tonumber{\pgf@xc}}{0}{0}{\pgf@sys@tonumber{\pgf@yc}}{0pt}{0pt}%
          % This will actually be the first transformation of the shading.
          % Should it be applied first so that it becomes the last one?
          \ifx\pgf@shade@extra@transform\pgfutil@empty%
          \else%
            \pgflowlevel{\pgf@shade@extra@transform}%
          \fi%
          \pgfuseshading{#1}%
        \pgfsys@endscope%
      \fi%
    \endgroup%
  \fi%
}

\newif\ifpgf@no@shade

% Additionally transform shade paths
%
% #1 = Transformation code that is used in addition to the normal
%      shading transformation.
%
% Example:
%
% \pgfsetadditionalshadetransform{\pgftransformrotate{30}}

\def\pgfsetadditionalshadetransform#1{\def\pgf@shade@extra@transform{#1}}
\let\pgf@shade@extra@transform=\pgfutil@empty





\endinput


==> pgfcoretransformations.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoretransformations.code.tex}


% Position transformations

\newdimen\pgf@pt@x
\newdimen\pgf@pt@y

\newdimen\pgf@pt@temp

\newif\ifpgf@pt@identity
\pgf@pt@identitytrue

\def\pgf@pt@aa{1.0} \def\pgf@pt@ab{0.0}
\def\pgf@pt@ba{0.0} \def\pgf@pt@bb{1.0}



% Store the current transformation matrix in a macro.
%
% #1 = macro name
%
% Example:
%
% \pgfgettransform\mytransform

\def\pgfgettransform#1{%
  \edef#1{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}}%
}

% Store the current transformation matrix in a set of macros, one for
% each single entry.
%
% #1-#4 are macro which store the matrix entries (0,0), (0,1), (1,0),
% (1,1) (in this order). It is the same order as for \pgftransformcm.
%
% #5 is a macro which will be filled with the x shift and
% #6 is a macro which will be filled with the y shift.
%
% Example:
% \pgfgettransform\aa\ab\ba\bb\shiftx\shifty
%
% ->
%
% \pgftransformcm\aa\ab\ba\bb{\pgfqpoint{\shiftx}{\shifty}}
%
% or
%
% \pgfsettransformentries\aa\ab\ba\bb\shiftx\shifty
\def\pgfgettransformentries#1#2#3#4#5#6{%
  \edef#1{\pgf@pt@aa}%
  \edef#2{\pgf@pt@ab}% attention: this is (1,0), i.e. the point which is usually labelled 'ba'!
  \edef#3{\pgf@pt@ba}% attention: this is (0,1), i.e. the point which is usually labelled 'ab'!
  \edef#4{\pgf@pt@bb}%
  \edef#5{\the\pgf@pt@x}%
  \edef#6{\the\pgf@pt@y}%
}%
\def\pgfsettransformentries#1#2#3#4#5#6{%
  \pgfsettransform{{#1}{#2}{#3}{#4}{#5}{#6}}%
}%

% Restore the current transformation matrix from a macro.
%
% #1 = macro name, previously used with \pgfgettransform
%
% Example:
%
% \pgfsettransform\mytransform

\def\pgfsettransform#1{%
  \edef\pgf@temp{#1}%
  \expandafter\pgf@settransform\pgf@temp%
}
\def\pgf@settransform#1#2#3#4#5#6{%
  \def\pgf@pt@aa{#1}%
  \def\pgf@pt@ab{#2}%
  \def\pgf@pt@ba{#3}%
  \def\pgf@pt@bb{#4}%
  \pgf@pt@x=#5%
  \pgf@pt@y=#6%
  \edef\pgf@idtest{#1,#2,#3,#4}%
  \ifx\pgf@idtest\pgf@idmatrixtext%
    \pgf@pt@identitytrue%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}

\def\pgf@idmatrixtext{1.0,0.0,0.0,1.0}
\def\pgf@zerozerotext{0.0,0.0}
\def\pgf@one@text{1.0}
\def\pgf@zero@text{0.0}

% Transformation command
%
% #1 = x dimension
% #2 = y dimension
%
% Description:
%
% Applies the pgfs transformation matrix to the point (#1,#2). The
% result is once more stored in the point.
%
%
% Example:
%
% \pgf@pos@transform{\pgf@x}{\pgf@y}

\def\pgf@pos@transform#1#2{%
  \ifpgf@pt@identity%
  \else%
    \pgf@pt@temp=#1%
    #1=\pgf@pt@aa#1%
    \advance#1 by\pgf@pt@ba#2%
    #2=\pgf@pt@bb#2%
    \advance#2 by\pgf@pt@ab\pgf@pt@temp%
  \fi%
  \advance#1 by\pgf@pt@x%
  \advance#2 by\pgf@pt@y%
}
\def\pgf@pos@transform@glob{%
  \ifpgf@pt@identity%
  \else%
    \pgf@pt@temp=\pgf@x%
    \global\pgf@x=\pgf@pt@aa\pgf@x%
    \global\advance\pgf@x by\pgf@pt@ba\pgf@y%
    \global\pgf@y=\pgf@pt@bb\pgf@y%
    \global\advance\pgf@y by\pgf@pt@ab\pgf@pt@temp%
  \fi%
  \global\advance\pgf@x by\pgf@pt@x%
  \global\advance\pgf@y by\pgf@pt@y%
}


% Invert the current transformation matrix
%
% Description:
%
% This command replaces the current transformation matrix by its
% inverse. The inversion is not very exact if the matrix is nearly
% singular.
%
% Example:
%
% \pgftransforminvert

\def\pgftransforminvert{%
  % First, invert the shift. That's easy
  \pgf@pt@x=-\pgf@pt@x
  \pgf@pt@y=-\pgf@pt@y
  \ifpgf@pt@identity%
  \else%
    % Sigh. Have to calculate the inverse of the matrix.
    % Perhaps we are lucky and ba and bb are zero?
    \edef\pgf@zerotest{\pgf@pt@ab,\pgf@pt@ba}%
    \ifx\pgf@zerotest\pgf@zerozerotext%
      % Ha! Just invert aa and bb
      \pgfmathreciprocal@{\pgf@pt@aa}%
      \let\pgf@pt@aa\pgfmathresult%
      \pgfmathreciprocal@{\pgf@pt@bb}%
      \let\pgf@pt@bb\pgfmathresult%
    \else%
      % Start with determinant
      % Matrix = (aa ab
      %           ba bb)
      {%
        \pgfutil@tempdima=\pgf@pt@aa pt%
        \pgfutil@tempdima=\pgf@pt@bb\pgfutil@tempdima% aa * bb
        \pgfutil@tempdimb=\pgf@pt@ba pt%
        \pgfutil@tempdimb=\pgf@pt@ab\pgfutil@tempdimb% ba * ab
        \advance\pgfutil@tempdima by -\pgfutil@tempdimb% aa*bb - ba*ab
        % Invert
        \pgfmathreciprocal@{\pgf@sys@tonumber{\pgfutil@tempdima}}%
        \pgfutil@tempdima=\pgfmathresult pt%
        \pgf@x=\pgf@pt@bb\pgfutil@tempdima% bb/(det A)
        \xdef\pgf@new@pt@aa{\pgf@sys@tonumber{\pgf@x}}%
        \pgf@x=\pgf@pt@aa\pgfutil@tempdima% aa/(det A)
        \xdef\pgf@new@pt@bb{\pgf@sys@tonumber{\pgf@x}}%
        \pgfutil@tempdima=-\pgfutil@tempdima%
        \pgf@x=\pgf@pt@ba\pgfutil@tempdima% -ba/(det A)
        \xdef\pgf@new@pt@ba{\pgf@sys@tonumber{\pgf@x}}%
        \pgf@x=\pgf@pt@ab\pgfutil@tempdima% -ab/(det A)
        \xdef\pgf@new@pt@ab{\pgf@sys@tonumber{\pgf@x}}%
      }%
      \let\pgf@pt@aa\pgf@new@pt@aa%
      \let\pgf@pt@ab\pgf@new@pt@ab%
      \let\pgf@pt@ba\pgf@new@pt@ba%
      \let\pgf@pt@bb\pgf@new@pt@bb%
    \fi%
    \pgf@pt@temp=\pgf@pt@x%
    \pgf@pt@x=\pgf@pt@aa\pgf@pt@x%
    \advance\pgf@pt@x by\pgf@pt@ba\pgf@pt@y%
    \pgf@pt@y=\pgf@pt@bb\pgf@pt@y%
    \advance\pgf@pt@y by\pgf@pt@ab\pgf@pt@temp%
  \fi%
}




% PGF-Level concatenation of the transformation matrix with a given
% matrix.
%
% #1 - #5 = a concatenation matrix (see pdf spec). Entry #5 is a
%           translation point.
%
% Description:
%
% All coordinates given to subsequent path construction commands will
% be transformed additionally by the given transformation matrix. If
% the command is followed by a 6th argument, the transformation is
% only applied to this argument.
%
%
% Example:
%
% \pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}} % 100pt to the right.
%
% \pgftransformcm{2}{0}{0}{2}{\pgfpointorigin} % double in size
% \pgfpathmoveto{\pgfpoint{0cm}{0cm}}
% \pgfpathlineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm

\def\pgftransformcm#1#2#3#4#5{%
  \edef\pgf@marshal{\noexpand\pgf@transformcm{#1}{#2}{#3}{#4}}%
  \pgf@marshal{#5}%
}
\def\pgf@transformcm#1#2#3#4#5{%
  {%
    \pgf@process{#5}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    %
    \pgfmathsetlength\pgf@x{#1}%
    \pgfmathsetlength\pgf@y{#2}%
    %
    \pgf@xa=\pgf@pt@aa\pgf@x%
    \advance\pgf@xa by \pgf@pt@ba\pgf@y%
    %
    \pgf@ya=\pgf@pt@ab\pgf@x%
    \advance\pgf@ya by \pgf@pt@bb\pgf@y%
    %
    \pgfmathsetlength\pgf@x{#3}%
    \pgfmathsetlength\pgf@y{#4}%
    %
    \pgf@xb=\pgf@pt@aa\pgf@x%
    \advance\pgf@xb by \pgf@pt@ba\pgf@y%
    %
    \pgf@yb=\pgf@pt@ab\pgf@x%
    \advance\pgf@yb by \pgf@pt@bb\pgf@y%
    %
    \pgf@x=\pgf@pt@aa\pgf@xc%
    \advance\pgf@x by\pgf@pt@ba\pgf@yc%
    \advance\pgf@x by\pgf@pt@x%
    %
    \pgf@y=\pgf@pt@ab\pgf@xc%
    \advance\pgf@y by\pgf@pt@bb\pgf@yc%
    \advance\pgf@y by\pgf@pt@y%
    %
    \global\pgf@x=\pgf@x%
    \global\pgf@y=\pgf@y%
    \xdef\pgf@tempaa{\pgf@sys@tonumber{\pgf@xa}}%
    \xdef\pgf@tempab{\pgf@sys@tonumber{\pgf@ya}}%
    \xdef\pgf@tempba{\pgf@sys@tonumber{\pgf@xb}}%
    \xdef\pgf@tempbb{\pgf@sys@tonumber{\pgf@yb}}%
  }%
  \pgf@pt@x=\pgf@x%
  \pgf@pt@y=\pgf@y%
  \let\pgf@pt@aa=\pgf@tempaa%
  \let\pgf@pt@ba=\pgf@tempba%
  \let\pgf@pt@ab=\pgf@tempab%
  \let\pgf@pt@bb=\pgf@tempbb%
  \edef\pgf@idtest{\pgf@pt@aa,\pgf@pt@ba,\pgf@pt@ab,\pgf@pt@bb}%
  \ifx\pgf@idtest\pgf@idmatrixtext%
    \pgf@pt@identitytrue%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}



% Transformation into a given triangle. The three corners of the
% triangle are called "origin", "x" and "y" are given. After this
% transformation has been applied, the canvas origin is at "origin",
% the vector (1pt,0pt) lies at "x" and the vector (0pt,1pt) lies at
% "y".
%
% #1 = origin
% #2 = x
% #3 = y
%
% Example:
%
% \pgftransformtriangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}{\pgfpoint{-1cm}{1cm}}

\def\pgftransformtriangle#1#2#3{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \advance\pgf@xb by-\pgf@x%
  \advance\pgf@yb by-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
  {\pgf@sys@tonumber\pgf@xb}{\pgf@sys@tonumber\pgf@yb}%
  {\pgfpoint{\pgf@x}{\pgf@y}}%
}



% Undo all transformations
%
% Example:
%
% \pgftansformreset

\def\pgftransformreset{%
  \pgf@pt@x=0pt%
  \pgf@pt@y=0pt%
  \let\pgf@pt@aa\pgf@one@text%
  \let\pgf@pt@ba\pgf@zero@text%
  \let\pgf@pt@ab\pgf@zero@text%
  \let\pgf@pt@bb\pgf@one@text%
  \pgf@pt@identitytrue%
}


% Undo all slanting/rotation, but not translations
%
% Example:
%
% \pgftansformreset

\def\pgftransformresetnontranslations{%
  \let\pgf@pt@aa\pgf@one@text%
  \let\pgf@pt@ba\pgf@zero@text%
  \let\pgf@pt@ab\pgf@zero@text%
  \let\pgf@pt@bb\pgf@one@text%
  \pgf@pt@identitytrue%
}




% Shifting command and environment
%
% #1 = vector by which all subsequent points should be moved.
%
% Example:
%
% \pgftansformshift{\pgfpoint{1cm}{1cm}}

\def\pgftransformshift#1{\pgftransformcm{1}{0}{0}{1}{#1}}
\def\pgftransformxshift#1{\pgftransformcm{1}{0}{0}{1}{\pgfpoint{#1}{+0pt}}}
\def\pgftransformyshift#1{\pgftransformcm{1}{0}{0}{1}{\pgfpoint{+0pt}{#1}}}




% Scaling commands
%
% #1 = scaling for all subsequent points.
%
% Example:
%
% \pgftransformscale{2}
% \pgftransformxscale{2}
% \pgftransformyscale{2}

\def\pgftransformscale#1{\pgftransformcm{#1}{0}{0}{#1}{\pgfpointorigin}}
\def\pgftransformxscale#1{\pgftransformcm{#1}{0}{0}{1.0}{\pgfpointorigin}}
\def\pgftransformyscale#1{\pgftransformcm{1.0}{0}{0}{#1}{\pgfpointorigin}}



% Slanting commands
%
% #1 = slanting in x-direction. 1 means 45 degrees.
%
% Example:
%
% \pgftransformxslant{2}
% \pgftransformyslant{2}

\def\pgftransformxslant#1{\pgftransformcm{1.0}{0}{#1}{1.0}{\pgfpointorigin}}
\def\pgftransformyslant#1{\pgftransformcm{1.0}{#1}{0}{1.0}{\pgfpointorigin}}



% Rotation commands
%
% #1 = degrees for the rotation
%
% Example:
%
% \pgftransformrotate{30}

\def\pgftransformrotate#1{%
  \pgfmathparse{#1}%
  \let\pgftransform@angle=\pgfmathresult%
  \pgfmathsin@{\pgftransform@angle}%
  \let\pgftransform@sin=\pgfmathresult%
  \pgfmathcos@{\pgftransform@angle}%
  \let\pgftransform@cos=\pgfmathresult%
  \pgf@x=\pgftransform@sin pt%
  \pgf@xa=-\pgf@x%
  \pgftransformcm{\pgftransform@cos}{\pgftransform@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgftransform@cos}{\pgfpointorigin}%
}



% The following if's have the following effect:
%
% \ifpgfslopedattime decides whether the coordinate system of an
% xxxattime transformation command should be rotated such that text
% drawn on the line should be tangent to the line
%
% \ifpgfallowupsidedowattime decides whether the transformation should
% be done in such a way that the text is always ``upright,'' that is,
% text drawn in this coordinate system is never upside-down.
%
% \ifpgfresetnontranslationattime decides whether the coordinate
% system of an xxxattime transformation command should be reset
% (concerning the non-translations) before a possible rotation is
% applied. This is useful, for example, if the main coordinate system
% is scaled by, say, a factor of 2 and you do not want that to apply
% to the text, but you do want the rotation to apply.

\newif\ifpgfslopedattime
\newif\ifpgfallowupsidedownattime
\newif\ifpgfresetnontranslationattime


% Transform to the coordinate system of a point on a line
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = end of line
%
% Example:
%
% {
%   \pgftransformlineattime{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformlineattime{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformlineattime#1#2#3{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x% xb/yb = start point
  \pgf@yb=\pgf@y%
  \pgf@process{#3}%
  \pgf@xc=\pgf@x% xc/yc = end point
  \pgf@yc=\pgf@y%
  \pgftransformshift{\pgfpointlineattime{#1}{\pgfqpoint{\pgf@xb}{\pgf@yb}}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \advance\pgf@xc by-\pgf@xb%
    \advance\pgf@yc by-\pgf@yb%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@xc<0pt%
        \pgf@xc=-\pgf@xc%
        \pgf@yc=-\pgf@yc%
      \fi%
    \fi%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}


% Transform to the coordinate system of a point on an arc
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = center of an ellipse
% #3 = 0-degree axis of the ellipse
% #4 = 90-degree axis of the ellipse
% #4 = start angle of the arc on this ellipse
% #5 = end angle of the arc on this ellipse
%
% Example:
%
% {
%   \pgftransformlineattime{.5}{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{0cm}}{\pgfpoint{0cm}{1cm}}{30}{40}
%   \pgftext{Hi!}
% }

\def\pgftransformarcaxesattime#1#2#3#4#5#6{%
  \pgfpointarcaxesattime{#1}{#2}{#3}{#4}{#5}{#6}%
  \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \pgf@process{\pgfpointnormalised{}}%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}




% Transform to the coordinate system of a point on a curve
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = first control
% #4 = second control
% #5 = end of line
%
% Example:
%
% {
%   \pgftransformcurveattime{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformcurveattime{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformcurveattime#1#2#3#4#5{%
  \pgfpointcurveattime{#1}{#2}{#3}{#4}{#5}%
  \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \advance\pgf@x by-\pgf@xb%
    \advance\pgf@y by-\pgf@yb%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}





% Transform to the coordinate system of an arrow at the end of the
% line going from point #1 to point #2 with the correct rotation.
%
% #1 = a start point an (invisible) line
% #2 = an end point an (invisible) line
%
% Example:
%
% \pgftransformarrow{\pgfpointorigin}{\pgfpoint{1cm}{0cm}}

\def\pgftransformarrow#1#2{%
  \pgf@process{#2}%
  \pgftransformshift{}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \pgf@x=\pgf@xa%
  \pgf@y=\pgf@ya%
  \pgfpointnormalised{}%
  \pgf@ya=-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
  {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfqpoint{0pt}{0pt}}%
}




% Computes transformations adjustments for the current transformation
% matrix
%
% Description:
%
% This command is used when you install a transformation matrix that
% scales everything by a certain factor, but you still wish to draw
% something with "an absolute size". Suppose for instance that you
% install a transformation matrix that scales everything by a factor
% of 4 and you now wish to draw a horizontal line of length 1cm. Then,
% if you do not reset the transformation matrix, you can draw a line
% of logical length 2.5mm, which will then get scaled to a line of
% 1cm.
%
% Things get more difficult in case you scale things only, say,
% vertically. In this case, the adjustment necessary for horizontal
% lines is different from the one needed for vertical lines.
%
% This function computes the necessary scaling factors and puts them
% in the macros \pgfhorizontaltransformationadjustment and
% \pgfverticaltransformationadjustment.
%
% Note that the "right" way to draw a line of absolute length 1cm in a
% transformed coordinate system is to first compute the start point
% and to then reset the transformation matrix. The transformation
% adjustments computed here are important only in situations where you
% cannot do this, for instance when an "outer xsep" must be set.

\def\pgftransformationadjustments{%
  \ifpgf@pt@identity%
    \let\pgfhorizontaltransformationadjustment\pgf@one@text%
    \let\pgfverticaltransformationadjustment\pgf@one@text%
  \else%
    {%
      \pgf@pt@x0pt%
      \pgf@pt@y0pt%
      \pgfpointtransformed{\pgfqpoint{1pt}{0pt}}%
      \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
      \pgfmathreciprocal@{\pgfmathresult}%
      \global\let\pgf@temp@hori\pgfmathresult
      \pgfpointtransformed{\pgfqpoint{0pt}{1pt}}%
      \pgfmathveclen@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
      \pgfmathreciprocal@{\pgfmathresult}%
      \global\let\pgf@temp@vert\pgfmathresult
      \xdef\pgf@marshal@b{\def\noexpand\pgfverticaltransformationadjustment{\pgfmathresult}}
    }%
    \let\pgfhorizontaltransformationadjustment\pgf@temp@hori%
    \let\pgfverticaltransformationadjustment\pgf@temp@vert%
  \fi%
}

\let\pgfhorizontaltransformationadjustment\pgf@one@text
\let\pgfverticaltransformationadjustment\pgf@one@text


% Low-level transformations

% Causes the current high-level transformation command to be applied
% to the low-level.
%
% Description:
%
% All subsequent drawing will be transformed additionally by the
% current high-level transformation. Thus, the high-level
% transformation becomes the low-level transformation. The high-level
% transformation is reset at this point.

\def\pgflowlevelsynccm{%
  \pgfsys@transformcm%
  {\pgf@pt@aa}{\pgf@pt@ab}%
  {\pgf@pt@ba}{\pgf@pt@bb}%
  {\pgf@pt@x}{\pgf@pt@y}%
  \pgftransformreset%
  \pgf@relevantforpicturesizefalse%
}



% Causes a transformation command to be applied to the ``lowlevel''
% transformation matrix.
%
% #1 - a high-level transformation command
%
% Description:
%
% All subsequent drawing will be transformed additionally by the given
% transformation matrix. Note that PGF will no longer be able to
% ``keep track'' of the coordinates. Also, transformations are applied
% to *everything*, including line thickness and line endings. Most
% often, this is not desirable.
%
% Example:
%
% \pgflowlevel{\pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}}} % 100bp to the right.
%
% \begin{pgflowlevelscope}{\pgftransformcm{2}{0}{0}{2}{\pgfpointorigin}} % double in size
%  \pgfmoveto{\pgfpoint{0cm}{0cm}}
%  \pgflineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm
% \end{pgflowlevelscope}

\def\pgflowlevel#1{%
  {%
    \pgftransformreset%
    #1%
    \pgflowlevelsynccm%
  }%
  \pgf@relevantforpicturesizefalse%
}

\def\pgflowlevelscope#1{\pgfscope\pgflowlevel{#1}}
\def\endpgflowlevelscope{\endpgfscope}

\long\def\pgflowlevelobj#1#2{\pgfscope{\pgflowlevel{#1}#2}\endpgfscope}



% View boxes

% Establishes a view box scope
%
% #1 and #2 = two opposite corners of the source rectangle
% #3 and #4 = two opposite corners of the target rectangle
% #5        = "meet" or "slice"
%
% Description:
%
% Inside the viewbox scope, the source rectangle will be translated
% and scaled so that it becomes centered on the target rectangle and
% will, for "meet", be as large as possible so that it fits inside the
% target and, for "slice", be as small as possible so that it
% encompasses the target.

\def\pgfviewboxscope#1#2#3#4#5{%
  {% Compute rectangle corners
    \pgf@process{#1}%
    \pgf@pos@transform@glob
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \pgf@pos@transform@glob
    \ifdim\pgf@x<\pgf@xa%
      \pgf@xb\pgf@x%
      \pgf@xc\pgf@xa%
    \else%
      \pgf@xb\pgf@xa%
      \pgf@xc\pgf@x%
    \fi%
    \ifdim\pgf@y<\pgf@ya%
      \pgf@yb\pgf@y%
      \pgf@yc\pgf@ya%
    \else%
      \pgf@yb\pgf@ya%
      \pgf@yc\pgf@y%
    \fi%
    \pgf@process{#3}%
    \pgf@pos@transform@glob
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#4}%
    \pgf@pos@transform@glob
    \ifdim\pgf@x<\pgf@xa%
    \else%
      \pgfutil@tempdima\pgf@x
      \pgf@x\pgf@xa%
      \pgf@xa\pgfutil@tempdima%
    \fi%
    \ifdim\pgf@y<\pgf@ya%
    \else%
      \pgfutil@tempdima\pgf@y
      \pgf@y\pgf@ya%
      \pgf@ya\pgfutil@tempdima%
    \fi%
    \pgfusetype{.view}%
    \edef\pgf@marshal{\expandafter\noexpand\csname pgfsys@viewbox#5\endcsname{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}{\the\pgf@xc}{\the\pgf@yc}}%
    \pgf@marshal%
  }%
  \pgf@relevantforpicturesizefalse%
}

\def\endpgfviewboxscope{\pgfsys@endviewbox}

\let\startpgfviewboxscope=\pgfviewboxscope
\let\stoppgfviewboxscope=\endpgfviewboxscope

% Forward declarations for nonlinear stuff (have no effect till module
% nonlineartransformations is loaded)

\let\pgfapproximatenonlineartranslation\relax
\let\pgfapproximatenonlineartransformation\relax
\def\pgftransformnonlinear#1{\pgferror{You need to say
    \string\usepgfmodule{nonlineartransformations} to use nonlinear transformations}}


\endinput


==> pgfcoretransparency.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoretransparency.code.tex}


% Sets the opacity of stroking operations.
%
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent.
%
% Example:
%
% \pgfsetstrokeopacity{0.5}

\def\pgfsetstrokeopacity#1{%
  \pgfmathparse{#1}%
  \expandafter\pgfsys@stroke@opacity\expandafter{\pgfmathresult}}


% Sets the opacity of stroking operations.
%
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent.
%
% Example:
%
% \pgfsetfillopacity{0.5}

\def\pgfsetfillopacity#1{%
  \pgfmathparse{#1}%
  \expandafter\pgfsys@fill@opacity\expandafter{\pgfmathresult}}



% Sets the current blend mode. See Section 7.2.4 of the PDF
% Specification 1.7 for an introduction to blend modes in general.
%
% #1 = One of the following modes, see also section 7.2.4 of the
% PDF Specification 1.7. (The PGF names, which are all lowercase with
% spaces as usual, must be mapped to the PDF or SVG by the drivers.)
%
% normal
% multiply
% screen
% overlay
% darken
% lighten
% color dodge
% color burn
% hard light
% soft light
% difference
% exclusion
% saturation
% color
% hue
% luminosity
%
% Example:
%
% \pgfsetblendmode{multiply}

\def\pgfsetblendmode#1{\pgfsys@blend@mode{#1}}


% Declares a new fading based on the contents of a box.
%
% #1 = name of the fading
% #2 = content of a TeX box that specifies the fading
%
% Description:
%
% This command declares a new fading based on the contents of
% the TeX box. The mask can later be used to mask other graphics.
%
% The box is used to determine where the mask is opaque: At the
% beginning, the mask is completely transparent. Wherever the box
% contains something (like text or a picture or whatever), the
% luminosity of the text/graphic is used to determine how opaque the
% point will be. The greater the luminosity, the more opaque. The net
% effect is that white corresponds to "completely opaque" and black to
% "completely transparent". This is rather counterintuitive. Because
% of this, the special color "pgftransparent" is defined, which is the
% same as black. By setting the color to, say,
% \color{pgftransparent!10} you get something that is 10% transparent
% and \color{pgftransparent!90} gives you 90% transparency.
%
% By default, the drawing color is set to opaque.
%
% Example:
%
% \pgfdeclarefading{mymask}{
%  \fontsize{200}{200}\bfseries
%  Ti\emph{k}Z
% }
% \pgfdeclarefading{myothermask}{
%  \tikz \shade [left color=transparent,right color=transparent!0]
%    (0,0) rectangle (5,5);
% }

\def\pgfdeclarefading#1#2{%
  \setbox\pgfutil@tempboxa=\hbox{{\pgfsys@beginscope\pgfutil@color{white}\ignorespaces#2\pgfsys@endscope}}%
  \pgfsys@fadingfrombox{#1}\pgfutil@tempboxa%
}

\pgfutil@colorlet{pgftransparent}{black}


% Use a previously declared fading.
%
% #1 = name of the fading
% #2 = transformation code
%
% Description:
%
% The command should be used *inside* a pgfpicture to install a
% fading. The fading is a part of the graphic state. (This command
% works much like \pgfsetstrokeopacity).
%
% The mask will be centered on the origin. The transformation code #2 is
% applied to the mask (but not the contents of the actual picture).

\def\pgfsetfading#1#2{%
  {%
    \pgftransformreset%
    #2%
    \pgfgettransform{\pgftrans@temp}%
    \edef\pgf@marshal{\noexpand\pgfsys@usefading{#1}\pgftrans@temp}%
    \pgf@marshal%
  }%
}



% Use a previously declared fading scaled for the current path.
%
% #1 - an fading
% #2 - extra transformations
%
% Description:
%
% This command works a bit like \pgfshadepath. "Works a bit like"
% means the following: The masks's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% mask is then rescaled so that it completely covers the path. Then
% the additional transformation #2 is applied. Finally, the mask is
% made part of the graphic state (as with \pgfsetfading). The path
% used for computation purposes only -- it is not drawn or otherwise
% used.
%
% If no transformations occur, the lower left corner of the path will
% lie on (25bp, 25bp), the upper right corner on (75bp, 75bp).
%
% If the path was empty, the fading will be used at its natural size,
% centered on the origin.
%
% Example:
%
% \pgfdeclarefading{fade right}
% {\tikz[left color=transparent!0,right color=transparent!100]
%    (0,0) rectangle (100bp,100bp);}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfsetfadingforcurrentpath{fade right}{}
% \pgfusepath{fill}

\def\pgfsetfadingforcurrentpath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    % Path was empty -> use natural size
    \pgfsetfading{#1}{#2}%
  \else%
    \pgfsetfading{#1}{%
      % Calculate center:
      \pgf@xb=.5\pgf@pathmaxx%
      \advance\pgf@xb by.5\pgf@pathminx%
      \pgf@yb=.5\pgf@pathmaxy%
      \advance\pgf@yb by.5\pgf@pathminy%
      % Calculate scaling:
      \pgf@xc=\pgf@pathmaxx%
      \advance\pgf@xc by-\pgf@pathminx%
      \ifdim\pgf@xc<0.1pt\pgf@xc=0.1pt\fi%
      \pgf@yc=\pgf@pathmaxy%
      \advance\pgf@yc by-\pgf@pathminy%
      \ifdim\pgf@yc<0.1pt\pgf@yc=0.1pt\fi%
      \pgf@xc=.02\pgf@xc%
      \pgf@yc=.02\pgf@yc%
      % Compute new transformation matrix:
      \pgftransformcm{1}{0}{0}{1}{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
      \pgftransformcm{\pgf@sys@tonumber{\pgf@xc}}{0}{0}{\pgf@sys@tonumber{\pgf@yc}}{\pgfpointorigin}%
      \pgfsys@clipfading%
      #2%
    }%
  \fi%
}




% Use a previously declared fading scaled for the current path.
%
% #1 - an fading
% #2 - extra transformations
%
% Description:
%
% This command works like \pgfsetfadingforcurrentpath, only it takes
% the current line width into account: Before the path is considered,
% it is enlarged by half the line width in all directions.

\def\pgfsetfadingforcurrentpathstroked#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    % Path was empty -> use natural size
    \pgfsetfading{#1}{#2}%
  \else%
    \pgfsetfading{#1}{%
      % Calculate center:
      \pgf@xb=.5\pgf@pathmaxx%
      \advance\pgf@xb by.5\pgf@pathminx%
      \pgf@yb=.5\pgf@pathmaxy%
      \advance\pgf@yb by.5\pgf@pathminy%
      % Calculate scaling:
      \pgf@xc=\pgf@pathmaxx%
      \advance\pgf@xc by-\pgf@pathminx%
      \advance\pgf@xc by\pgflinewidth%
      \ifdim\pgf@xc<0.1pt\pgf@xc=0.1pt\fi%
      \pgf@yc=\pgf@pathmaxy%
      \advance\pgf@yc by-\pgf@pathminy%
      \advance\pgf@yc by\pgflinewidth%
      \ifdim\pgf@yc<0.1pt\pgf@yc=0.1pt\fi%
      \pgf@xc=.02\pgf@xc%
      \pgf@yc=.02\pgf@yc%
      % Compute new transformation matrix:
      \pgftransformcm{1}{0}{0}{1}{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
      \pgftransformcm{\pgf@sys@tonumber{\pgf@xc}}{0}{0}{\pgf@sys@tonumber{\pgf@yc}}{\pgfpointorigin}%
      \pgfsys@clipfading%
      #2%
    }%
  \fi%
}


% Group things in a a transparency group
%
% Description:
%
% This takes groups pgf commands inside a pgfpicture in a transparency
% group. This means that any transparency settings apply to commands a
% whole. For instance, if a box contains two overlapping black
% circles and you draw them normally with 50% transparency, then the
% overlap will be darker than the rest. By comparison, if the circles
% are part of a transparency group, the overlap will get the same
% color as the rest.
%
%

\def\pgftransparencygroup{%
  \pgfutil@ifnextchar[{\pgftransparencygroup@}{\pgftransparencygroup@[]}%
}
\def\pgftransparencygroup@[#1]{%
  \begingroup%
    \pgfkeys{/pgf/transparency group options/.cd,%
      isolated=false,
      knockout=false,
      #1}%
    \setbox\pgfutil@tempboxa=\hbox\bgroup%
}
\pgfkeys{
  /pgf/transparency group options/.cd,
  isolated/.is if=pgfsys@transparency@group@isolated,
  knockout/.is if=pgfsys@transparency@group@knockout
}

\def\endpgftransparencygroup{%
    \egroup%
    % Now compute the correct position. This is a bit tricky...
    \ifdim\pgf@picminx=16000pt%
      % Nothing needs to be done
    \else%
      % Safety margin to avoid clipping:
      \advance\pgf@picminx by-1cm%
      \advance\pgf@picmaxx by1cm%
      \advance\pgf@picminy by-1cm%
      \advance\pgf@picmaxy by1cm%
      % Ok, set the box size to current picture size.
      \setbox\pgfutil@tempboxa=\hbox{%
        \vrule width0pt height\pgf@picmaxy depth-\pgf@picminy%
        \hskip-\pgf@picminx%
        \box\pgfutil@tempboxa%
        \hskip\pgf@picmaxx%
      }%
      \pgfsys@transparencygroupfrombox\pgfutil@tempboxa%
      \wd\pgfutil@tempboxa=0pt%
      \ht\pgfutil@tempboxa=0pt%
      \dp\pgfutil@tempboxa=0pt%
      \hskip\pgf@picminx\box\pgfutil@tempboxa\hskip-\pgf@picminx%
    \fi%
  \endgroup%
}

\let\startpgftransparencygroup=\pgftransparencygroup
\let\stoppgftransparencygroup=\endpgftransparencygroup

\endinput


==> pgffor.code.tex <==
% Copyright 2019 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgffor.code.tex}

% pgfmath is needed
\input pgfmath.code.tex

\newdimen\pgffor@iter
\newdimen\pgffor@skip
\newif\ifpgffor@continue


\def\pgffor@reset@hooks{%
  \let\pgffor@beginhook=\relax%
  \let\pgffor@endhook=\relax%
  \let\pgffor@afterhook=\relax%
}
\pgffor@reset@hooks


% Stack emulation
%
\newtoks\pgffor@stack
\pgffor@stack={{}{}{}}

\def\pgffor@stackpush#1{%
    \def\pgffor@stacktemp{#1}%
    \expandafter\expandafter\expandafter\pgffor@stack\expandafter\expandafter\expandafter=%
    \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
        {\expandafter\pgffor@stacktemp\expandafter}\the\pgffor@stack}%
}

\def\pgffor@stackpop{\expandafter\pgffor@@stackpop\the\pgffor@stack\pgffor@stackstop}
\def\pgffor@@stackpop#1#2\pgffor@stackstop{\pgffor@stack{#2}#1}

\def\pgffor@emptyvalues{, \pgffor@stop,}%

\def\pgffor@foreach{%
    \pgffor@atbeginforeach%
    \let\pgffor@assign@before@code=\pgfutil@empty%
    \let\pgffor@assign@after@code=\pgfutil@empty%
    \let\pgffor@assign@once@code=\pgfutil@empty%
    \let\pgffor@remember@code=\pgfutil@empty%
    \let\pgffor@remember@once@code=\pgfutil@empty%
    \pgffor@alphabeticsequencefalse%
    \pgffor@contextfalse%
    %
    \let\pgffor@var=\pgfutil@empty
    %
    \pgffor@vars%
}

\let\foreach=\pgffor@foreach

\def\pgffor@vars{%
    \pgfutil@ifnextchar i{\pgffor@@vars@end}{%
        \pgfutil@ifnextchar[{\pgffor@@vars@opt}{%]
            \pgfutil@ifnextchar/{\pgffor@@vars@slash@gobble}{%
                \pgffor@@vars}}}}%

\def\pgffor@@vars@end in{\pgfutil@ifnextchar\bgroup{\pgffor@normal@list}{\pgffor@macro@list}}
\def\pgffor@@vars@opt[#1]{\pgfkeys{/pgf/foreach/.cd,#1}\pgffor@vars}
\def\pgffor@@vars#1{\pgffor@var@add#1\pgffor@stop\pgffor@vars}
\def\pgffor@@vars@slash@gobble/{\pgffor@@vars}

\def\pgffor@var@add#1#2\pgffor@stop{%
    \ifx\pgffor@var\pgfutil@empty%
        \def\pgffor@var{#1}%
        \def\pgffor@mainvar{#1}%
    \else%
        \expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@var/#1}%
    \fi%
}

\def\pgffor@expand@list@true{\let\pgffor@expand@list\edef}
\def\pgffor@expand@list@false{\let\pgffor@expand@list\def}
\def\pgffor@macro@list#1{%
  \expandafter\pgffor@normal@list\expandafter{#1}}
\def\pgffor@normal@list#1{%
  \pgffor@expand@list\pgffor@values{#1}%
  \expandafter\def\expandafter\pgffor@values\expandafter{\pgffor@values, \pgffor@stop,}%
  \ifx\pgffor@values\pgffor@emptyvalues
    \def\pgffor@values{\pgffor@stop,}%
  \fi%
  \let\pgffor@body=\pgfutil@empty%
  \global\pgffor@continuetrue%
  \pgffor@collectbody}
\def\pgffor@collectbody{%
  \pgfutil@ifnextchar\foreach{\pgffor@collectforeach}{%
    \pgfutil@ifnextchar\bgroup{\pgffor@collectargument}{\pgffor@collectsemicolon}}%
}

\def\pgffor@collectforeach\foreach#1in{%
  \pgfutil@ifnextchar\bgroup{\pgffor@collectforeach@normal{#1}}{\pgffor@collectforeach@macro{#1}}}
\def\pgffor@collectforeach@macro#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in#2}%
  \pgffor@collectbody%
}
\def\pgffor@collectforeach@normal#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in{#2}}%
  \pgffor@collectbody%
}
\long\def\pgffor@collectargument#1{%
    \expandafter\pgfutil@in@\expandafter\foreach\expandafter{\pgffor@body}%
    \ifpgfutil@in@%
        \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter%
    {\pgffor@body{#1}}%
    \else%
        \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter%
    {\pgffor@body#1}%
    \fi%
  \pgffor@iterate%
}

\def\pgffor@collectsemicolon{%
  \let\pgffor@next=\pgffor@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\pgffor@next=\pgffor@collectactivesemicolon%
  \fi%
  \pgffor@next%
}

\def\pgffor@collectnormalsemicolon#1;{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
  \pgffor@iterate%
}

{
  \catcode`\;=\active

  \gdef\pgffor@collectactivesemicolon#1;{%
    \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
    \pgffor@iterate%
  }
}

\def\pgffor@iterate{%
  % Must do all of these in case the internal stack is used.
  \let\pgffor@last=\pgfutil@empty%
  \let\pgffor@prevlast=\pgfutil@empty%
  \let\pgffor@dotsend=\pgfutil@empty%
  \let\pgffor@dots@pre=\pgfutil@empty%
  \let\pgffor@dots@post=\pgfutil@empty%
  %
  \expandafter\pgffor@scan\pgffor@values}

\def\pgffor@stop{\pgffor@stop}%
\def\pgffor@dots{...}%

\def\pgffor@scan{\pgfutil@ifnextchar({\pgffor@scanround}{\pgffor@scanone}}
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)#2}\pgffor@scanned}
\def\pgffor@scanone#1,{\def\pgffor@value{#1}\pgffor@scanned}


% Check for dots.
\newif\ifpgffor@dots@in@
\def\pgffor@dots@in@#1...#2#3\pgffor@stop{%
    \ifx\pgffor@dots@@#2%
        \pgffor@dots@in@false%
    \else%
        \pgffor@dots@in@true%
    \fi%
}

\def\pgffor@dots@@{\pgffor@dots@@}

\def\pgffor@scanned{%
  \ifx\pgffor@value\pgffor@stop%
    \let\pgffor@next=\pgffor@after% Done!
  \else%
    % Check for dots. Quicker than \pgfutil@in@ and not suceptable
        % to false-positives when a token sequence ends in a single full-stop.
    \expandafter\pgffor@dots@in@\pgffor@value\pgffor@dots@...\pgffor@dots@@\pgffor@stop%
    \ifpgffor@dots@in@%
      \let\pgffor@next=\pgffor@handledots%
    \else%
      \let\pgffor@next=\pgffor@handlevalue%
    \fi%
    \ifpgffor@continue%
    \else%
      \let\pgffor@next=\pgffor@scan% Done!
    \fi%
  \fi%
  \pgffor@next}


\def\pgffor@after{%
  \global\pgffor@continuetrue%
  \pgffor@atendforeach%
  \pgffor@afterhook}

\def\pgffor@handlevalue{%
    \let\pgffor@prevlast=\pgffor@last%
  \let\pgffor@last=\pgffor@value%
  \pgffor@invokebody%
  \pgffor@scan%
}


\def\pgffor@invokebody{%
  \pgffor@begingroup%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@value//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@value}%
    \fi%
    % Execute assign once code.
    \ifx\pgffor@assign@once@code\pgfutil@empty%
    \else%
        \pgffor@assign@once@code%
    \fi%
    % Execute assign before code.
    \ifx\pgffor@assign@before@code\pgfutil@empty%
    \else%
        \pgffor@assign@before@code%
    \fi%
    %
    \expandafter\expandafter\expandafter\pgffor@reset@hooks\expandafter\pgffor@beginhook\expandafter\pgffor@body\pgffor@endhook%
    % Execute assign after code.
    \ifx\pgffor@assign@after@code\pgfutil@empty%
    \else%
        \pgffor@assign@after@code%
    \fi%
    %
  \pgffor@endgroup%
}


\def\pgffor@multiassign#1/#2/\relax{%
  \def\pgffor@currentvar{#1}%
  \def\pgffor@rest{#2}%
  \ifx\pgffor@currentvar\pgffor@stop%
    \let\pgffor@next=\relax%
  \else%
    \let\pgffor@next=\pgffor@multiassignrest%
  \fi%
  \pgffor@next%
}

\def\pgffor@multiassignrest{\expandafter\pgffor@multiassignfinal\pgffor@valuerest}
\def\pgffor@multiassignfinal#1/#2/\relax{%
    \def\pgffor@temp{#1}%
    \ifx\pgffor@currentvar\pgffor@mainvar%
        \ifpgffor@alphabeticsequence%
        \pgffor@makealphabetic\pgffor@temp%
    \fi%
  \fi%
  \def\pgffor@test{#2}%
  \ifx\pgffor@test\pgfutil@empty%
    \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}% repeat
  \else%
    \def\pgffor@valuerest{#2/\relax}%
  \fi%
  \expandafter\expandafter\expandafter\def\expandafter\pgffor@currentvar\expandafter{\pgffor@temp}%
    %
  \expandafter\pgffor@multiassign\pgffor@rest/\relax%
}

\def\pgffor@gobblespaces#1{\pgfutil@ifnextchar x{#1}{#1}}

\def\pgffor@handledots{%
    \pgffor@gobblespaces{\expandafter\pgffor@@handledots\pgffor@value\pgffor@@stop}%
}

\newif\ifpgffor@context

\def\pgffor@@handledots#1...#2\pgffor@@stop{%
    % Define the context if any.
    \def\pgffor@dots@pre{#1}%
    \def\pgffor@dots@post{#2}%
    \def\pgffor@dots@stripcontext#1##1#2\pgffor@@stop{\def\pgffor@dotsvalue{##1}}%
    \pgffor@contexttrue%
    \ifx\pgffor@dots@pre\pgfutil@empty%
        \ifx\pgffor@dots@post\pgfutil@empty%
            \pgffor@contextfalse%
            \def\pgffor@dots@stripcontext##1\pgffor@@stop{\def\pgffor@dotsvalue{##1}}%
        \fi%
    \fi%
    \pgffor@gobblespaces{\pgffor@dotsscanend}%
}

\def\pgffor@dots@value@process#1{%
    \expandafter\pgffor@dots@stripcontext#1\pgffor@@stop%
    \expandafter\pgffor@dots@charcheck\pgffor@dotsvalue\pgffor@@stop%
  \ifpgffor@alphabeticsequence
  \else
    \ifpgffor@assign@parse
      \begingroup
      \pgfkeys{/pgf/fpu/false/.try}%
      \pgfmathparse{\pgffor@dotsvalue}%
      \pgfmath@smuggleone\pgfmathresult
      \endgroup
      \let\pgffor@dotsvalue=\pgfmathresult
    \fi
  \fi
  \let#1=\pgffor@dotsvalue%
}

\def\pgffor@dotsscanend#1,{%
    \pgffor@alphabeticsequencefalse%
    % Strip context and check for a character sequence.
    \def\pgffor@dotsend{#1}%
    \pgffor@dots@value@process{\pgffor@dotsend}%
  %
  \pgffor@dots@value@process{\pgffor@last}%
  %
  % calculate skip%
  \ifx\pgffor@prevlast\pgfutil@empty%
    \ifdim\pgffor@dotsend pt>\pgffor@last pt%
      \pgffor@skip=1pt%
    \else%
      \pgffor@skip=-1pt%
    \fi%
  \else%
    \pgffor@dots@value@process{\pgffor@prevlast}%
    \pgffor@skip=\pgffor@last pt%
    \pgffor@iter=\pgffor@prevlast pt%
    \advance\pgffor@skip by-\pgffor@iter%
  \fi%
  \pgffor@iter=\pgffor@last pt%
  % do loop
  \pgffor@loop%
}

\def\pgffor@loop{%
  \advance\pgffor@iter by\pgffor@skip%
  \let\pgffor@next=\pgffor@doloop%
  \ifdim\pgffor@skip<0pt%
    \ifdim\pgffor@iter<\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \else%
    \ifdim\pgffor@iter>\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \fi%
  \ifpgffor@continue%
  \else%
    \let\pgffor@next=\pgffor@endloop% Done!
  \fi%
  \pgffor@next%
}

\def\pgffor@endloop{%
    \pgffor@alphabeticsequencefalse%
    \pgffor@scan%
}

{\catcode`\p=12\catcode`\t=12\gdef\Pgffor@geT#1pt{#1}}

\def\pgffor@doloop{%
  \pgffor@begingroup
    \edef\pgffor@temp{\expandafter\Pgffor@geT\the\pgffor@iter}%
    \edef\pgffor@incheck{{.0/}{\pgffor@temp/}}%
    \expandafter\pgfutil@in@\pgffor@incheck%
    \ifpgfutil@in@%
      \expandafter\pgffor@strip\pgffor@temp%
    \fi%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
        % Convert to alphabetic sequence, if necessary.
        \ifpgffor@alphabeticsequence%
            \pgffor@makealphabetic\pgffor@temp%
            \expandafter\let\pgffor@var=\pgffor@temp%
        \else%
            \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@temp}%
      \fi%
    \fi%
    % Insert any context, if any.
    \ifpgffor@context%
      \let\pgffor@temp=\pgffor@dots@pre%
        \expandafter\pgfutil@append@macrotomacro\expandafter%
            {\expandafter\pgffor@temp\expandafter}\expandafter{\pgffor@var}%
        \expandafter\pgfutil@append@macrotomacro\expandafter%
            {\expandafter\pgffor@temp\expandafter}\expandafter{\pgffor@dots@post}%
        \expandafter\let\pgffor@var=\pgffor@temp%
      \fi%
      % Perform assignments before loop body.
      \ifx\pgffor@assign@before@code\pgfutil@empty%
    \else%
        \pgffor@assign@before@code%
    \fi%
    %
    \expandafter\expandafter\expandafter\pgffor@reset@hooks\expandafter\pgffor@beginhook\expandafter\pgffor@body\pgffor@endhook%
    %
    % Perform assignments after loop body.
      \ifx\pgffor@assign@after@code\pgfutil@empty%
    \else%
        \pgffor@assign@after@code%
    \fi%
  \pgffor@endgroup%
  \pgffor@loop%
}

\def\pgffor@strip#1.0{\def\pgffor@temp{#1}}

\def\breakforeach{\global\pgffor@continuefalse}

\def\pgffor@gobbletil@pgffor@@stop#1\pgffor@@stop{}


\newif\ifpgffor@registeriscount

\def\pgffor@ifcsregister#1{%
    \expandafter\pgffor@@ifcsregister\meaning#1\pgffor@stop}

\def\pgffor@@ifcsregister#1#2#3#4#5\pgffor@stop{%
    \if#1m% It is an ordinary (m)acro.
        \pgffor@registeriscountfalse%
        \let\pgffor@csnext=\pgfutil@secondoftwo%
    \else%
        \if#1u% It is (u)ndefined.
            \let\pgffor@csnext=\pgfutil@secondoftwo%
            \pgffor@registeriscountfalse%
        \else%
            \let\pgffor@csnext=\pgfutil@firstoftwo%
            \if#4u% It is a co(u)nt
                \pgffor@registeriscounttrue%
            \else% Assume it is a dimen or skip (bad assumption in the general case).
                \pgffor@registeriscountfalse%
                \let\pgffor@csnext=\pgfutil@firstoftwo%
            \fi%
        \fi%
    \fi%
    \pgffor@csnext}

\newif\ifpgffor@alphabeticsequence

%
\def\pgffor@dots@charcheck#1\pgffor@@stop{%
  \edef\pgffor@dots@charcheck@temp{#1}%
  \expandafter\expandafter\expandafter\pgffor@@dotscharcheck\expandafter\meaning\pgffor@dots@charcheck@temp\pgffor@@stop%
}
\def\pgffor@@dotscharcheck#1#2\pgffor@@stop{%
    \if#1t%
    \afterassignment\pgffor@gobbletil@pgffor@@stop%
      \expandafter\chardef\expandafter\pgffor@char\expandafter=\expandafter`\pgffor@dots@charcheck@temp\relax\pgffor@@stop%
      \edef\pgffor@char{\the\pgffor@char}%
      \ifnum\pgffor@char>64\relax% From A-Z?
        \ifnum\pgffor@char<91\relax%
          \let\pgffor@dotsvalue=\pgffor@char%
          \pgffor@alphabeticsequencetrue%
        \else%
          \ifnum\pgffor@char>96\relax% From a-z?
            \ifnum\pgffor@char<123\relax%
              \let\pgffor@dotsvalue=\pgffor@char%
              \pgffor@alphabeticsequencetrue%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
}

\def\pgffor@makealphabetic#1{%
    % Convert the number in the macro passed as #1 to a-z or A-Z.
    \pgfutil@tempcnta=#1\relax%
    \ifnum\pgfutil@tempcnta>95\relax%
        \advance\pgfutil@tempcnta by-96\relax%
        \edef#1{\pgffor@alpha\pgfutil@tempcnta}%
    \else%
        \advance\pgfutil@tempcnta by-64 %
        \edef#1{\pgffor@Alpha\pgfutil@tempcnta}%
    \fi%
}

\def\pgffor@Alpha#1{%
    \ifcase#1\relax\or A\or B\or C\or D\or E\or F\or G\or H\or I\or J\or K\or L\or M%
    \or N\or O\or P\or Q\or R\or S\or T\or U\or V\or W\or X\or Y\or Z\else?\fi%
}

\def\pgffor@alpha#1{%
    \ifcase#1\relax\or a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\or m%
    \or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or y\or z\else?\fi%
}

\newtoks\pgffor@toks

\def\pgffor@addcstotoks#1{%
    \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\expandafter\def\expandafter#1\expandafter{#1}}%
    \pgffor@@addcstotoks}

\def\pgffor@addregtotoks#1{%
    \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\expandafter#1\expandafter=\the#1}%
    \pgffor@@addcstotoks}

\def\pgffor@addiftotoks#1{%
    \begingroup%
        \escapechar=-1\relax%
            \expandafter\pgffor@@addiftotoks\string#1\pgffor@stop}
\def\pgffor@@addiftotoks#1#2#3#4\pgffor@stop{%
    \endgroup
    \csname if#3#4\endcsname%
        \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\csname#3#4true\endcsname}%
    \else%
        \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\csname#3#4false\endcsname}%
    \fi%
    \pgffor@@addcstotoks%
}

\def\pgffor@@addcstotoks{%
    \expandafter\expandafter\expandafter\pgffor@toks\expandafter\expandafter\expandafter=%
    \expandafter\expandafter\expandafter{\expandafter\pgffor@tokstemp\the\pgffor@toks}%
}

% Set up the pgffor scopes.

\def\pgffor@atbeginforeach{%
    \begingroup%
}

\def\pgffor@atendforeach{%
        \global\edef\pgffor@remember@expanded{\pgffor@remember@code}%
        \ifx\pgffor@remember@expanded\pgfutil@empty%
        \else%
          \pgffor@remember@expanded%
          \global\let\pgffor@remember@expanded=\pgfutil@empty%
        \fi%
    \endgroup%
}
\def\pgffor@default@begingroup{%
    \begingroup%
}

\let\pgffor@remember@once@expanded=\pgfutil@empty
\let\pgffor@remember@expanded=\pgfutil@empty

\def\pgffor@default@endgroup{%
   \ifx\pgffor@remember@once@code\pgfutil@empty
   \else
     \xdef\pgffor@remember@once@expanded{\pgffor@remember@once@code}%
   \fi
   \ifx\pgffor@remember@code\pgfutil@empty
   \else
     \xdef\pgffor@remember@expanded{\pgffor@remember@code}%
   \fi
 \endgroup
 %
 \ifx\pgffor@remember@once@expanded\pgfutil@empty
 \else
   \pgffor@remember@once@expanded%
   % \let\pgffor@assign@once@code=\pgfutil@empty % Not needed anymore? (CJ)
   \global\let\pgffor@remember@once@expanded=\pgfutil@empty
 \fi
 \ifx\pgffor@assign@once@code\pgfutil@empty
 \else
   \global\let\pgffor@assign@once@code=\pgfutil@empty
 \fi
 %
 \ifx\pgffor@remember@expanded\pgfutil@empty
 \else
   \pgffor@remember@expanded%
   \global\let\pgffor@remember@expanded=\pgfutil@empty
 \fi
}

\let\pgffor@begingroup=\pgffor@default@begingroup
\let\pgffor@endgroup=\pgffor@default@endgroup


\def\pgffor@stack@begingroup{%
    \pgffor@toks={}%
    \pgffor@addcstotoks{\pgffor@mainvar}%
    \pgffor@addcstotoks{\pgffor@var}%
    \pgffor@addcstotoks{\pgffor@body}%
    %
    \pgffor@addcstotoks{\pgffor@last}%
    \pgffor@addcstotoks{\pgffor@prevlast}%
    \pgffor@addcstotoks{\pgffor@dotsend}%
    %
    \pgffor@addcstotoks{\pgffor@assign@before@code}%
    \pgffor@addcstotoks{\pgffor@assign@after@code}%
    \pgffor@addcstotoks{\pgffor@remember@code}%
    \pgffor@addcstotoks{\pgffor@remember@once@code}%
    \pgffor@addcstotoks{\pgffor@dots@pre}%
    \pgffor@addcstotoks{\pgffor@dots@post}%
    %
    \pgffor@addregtotoks{\pgffor@iter}%
    \pgffor@addregtotoks{\pgffor@skip}%
    %
    \pgffor@addiftotoks{\ifpgffor@alphabeticsequence}%
    \pgffor@addiftotoks{\ifpgffor@context}%
    \expandafter\pgffor@stackpush\expandafter{\the\pgffor@toks}%
}

\def\pgffor@stack@endgroup{\pgffor@stackpop}

% Keys stuff.

\newif\ifpgffor@assign@evaluate
\newif\ifpgffor@assign@once
\newif\ifpgffor@assign@parse

\pgfkeys{/pgf/foreach/.cd,
    var/.code=\pgffor@var@add#1\pgffor@stop,
    scope iterations/.code={
        \csname if#1\endcsname%
            \let\pgffor@begingroup=\pgffor@default@begingroup%
            \let\pgffor@endgroup=\pgffor@default@endgroup%
        \else%
            \let\pgffor@begingroup=\pgffor@stack@begingroup%
            \let\pgffor@endgroup=\pgffor@stack@endgroup%
        \fi%
    },
    evaluate/.code=\pgffor@assign@evaluatetrue\pgffor@assign@oncefalse\pgffor@assign@parse{#1},%
    assign/.code=\pgffor@assign@evaluatefalse\pgffor@assign@oncefalse\pgffor@assign@parse{#1},%
    evaluate once/.code=\pgffor@assign@evaluatetrue\pgffor@assign@oncetrue\pgffor@assign@parse{#1},%
    assign once/.code=\pgffor@assign@evaluatefalse\pgffor@assign@oncetrue\pgffor@assign@parse{#1},%
    remember/.code=\pgffor@remember@parse{#1},%
    count/.code=\pgffor@count@parse#1\pgffor@stop,
    parse/.is if=pgffor@assign@parse,
    parse/.default=false,
    expand list/.is if=pgffor@expand@list@,
    expand list/.default=true,
    expand list=false,
}

\def\pgffor@assign@parse#1{%
    \pgfutil@in@;{#1}%
    \ifpgfutil@in@%
    \else%
        \pgfutil@in@={#1}%
    \fi%
    \ifpgfutil@in@%
        \pgffor@assign@@parse#1;\pgffor@stop;%
    \else%
        \pgffor@assign@parse@old#1\pgffor@stop%%
    \fi%
}

\def\pgffor@stop{\pgffor@stop}
\def\pgffor@assign@@parse#1;{%
    \def\pgffor@test{#1}%
    \ifx\pgffor@test\pgffor@stop%
        \let\pgffor@next=\relax%
    \else%
        \let\pgffor@next=\pgffor@assign@@parse%
        \ifx\pgffor@test\pgfutil@empty%
        \else%
            \pgfutil@in@={#1}%
            \ifpgfutil@in@%
                \pgffor@assign@@@parse#1\pgffor@stop%
            \else%
                \pgffor@assign@@@parse#1=#1\pgffor@stop%
            \fi%
        \fi%
    \fi%
    \pgffor@next}

\def\pgffor@assign@@@parse#1=#2\pgffor@stop{%
    \ifpgffor@assign@evaluate%
        \ifpgffor@assign@once%
            \pgfutil@append@tomacro{\pgffor@assign@once@code}{\pgfmathparse{#2}\let#1=\pgfmathresult}%
            \pgfutil@append@tomacro{\pgffor@remember@once@code}{\noexpand\def\noexpand#1{#2}}%
        \else
            \pgfutil@append@tomacro{\pgffor@assign@before@code}{\pgfmathparse{#2}\let#1=\pgfmathresult}%
        \fi%
    \else%
        \ifpgffor@assign@once%
            \pgfutil@append@tomacro{\pgffor@assign@once@code}{\def#1{#2}}%
            \pgfutil@append@tomacro{\pgffor@remember@once@code}{\noexpand\def\noexpand#1{#2}}%
        \else
            \pgfutil@append@tomacro{\pgffor@assign@before@code}{\def#1{#2}}%
        \fi%
    \fi%
}

\def\pgffor@assign@parse@old#1#2\pgffor@stop{%
    \pgffor@assign@@parse@old#2\pgffor@stop as#1using #1\pgffor@@stop}

\def\pgffor@assign@@parse@old#1as#2#3\pgffor@@stop{%
    \pgffor@assign@@@parse@old{#2}#1#3\pgffor@stop\pgffor@@stop}

\def\pgffor@assign@@@parse@old#1#2using #3\pgffor@stop#4\pgffor@@stop{%
    \pgffor@assign@@@parse#1=#3\pgffor@stop}



\def\pgffor@remember@parse#1{%
    \pgfutil@in@ a{#1}% This matches the 'a' in 'as' or 'initially'.
    \ifpgfutil@in@%
        \pgffor@remember@parse@old#1\pgffor@stop%
    \else%
        \pgffor@remember@@parse#1;\pgffor@stop;%
    \fi%
}

\def\pgffor@remember@@parse#1;{%
    \def\pgffor@test{#1}%
    \ifx\pgffor@test\pgffor@stop%
        \let\pgffor@next=\relax%
    \else%
        \let\pgffor@next=\pgffor@remember@@parse%
        \ifx\pgffor@test\pgfutil@empty%
        \else%
            \pgfutil@in@={#1}%
            \ifpgfutil@in@%
                \pgffor@remember@@@parse#1\pgffor@stop%
            \else%
                \pgffor@ifcsregister{#1}{%
                    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand#1=\the#1\noexpand\relax}%
                }%
                {%
                    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
                }%
            \fi%
        \fi%
    \fi%
    \pgffor@next%
}

\def\pgffor@remember@@@parse#1=#2\pgffor@stop{%
    \pgffor@ifcsregister{#2}{%
        \pgfutil@append@tomacro{\pgffor@assign@after@code}{\expandafter\def\expandafter#1\expandafter{\the#2}}%
        \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
    }%
    {%
        \pgfutil@append@tomacro{\pgffor@assign@after@code}{\expandafter\def\expandafter#1\expandafter{#2}}%
        \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
    }%
}

\def\pgffor@remember@parse@old#1#2\pgffor@stop{%
    \pgffor@remember@@parse@old#1#2\pgffor@stop as#1(initially 0)\pgffor@@stop}

\def\pgffor@remember@@parse@old#1#2as#3#4\pgffor@@stop{%
    \pgffor@remember@@@parse@old{#1}{#3}#2#4\pgffor@stop\pgffor@@stop}

\def\pgffor@remember@@@parse@old#1#2#3(initially #4)#5\pgffor@stop#6\pgffor@@stop{%
    \pgfutil@append@tomacro{\pgffor@assign@after@code}{\edef#2{#1}}%
    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#2{#2}}%
    \pgfutil@append@tomacro{\pgffor@assign@once@code}{\def#2{#4}}%
}

\def\pgffor@count@parse#1#2\pgffor@stop{%
    \pgffor@count@@parse#1#2\pgffor@stop from 1\pgffor@stop\pgffor@@stop}

\def\pgffor@count@@parse#1#2from#3\pgffor@stop#4\pgffor@@stop{%
    \pgfutil@append@tomacro\pgffor@remember@code{\noexpand\def\noexpand#1{#1}}%
    \pgfutil@append@tomacro\pgffor@assign@before@code{\pgfmathparse{int(#1+1)}\let#1=\pgfmathresult}%
    \pgfmathparse{int(#3-1)}\let#1=\pgfmathresult%
}


\def\pgfutil@append@macrotomacro#1#2{%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
        #1\expandafter\expandafter\expandafter{\expandafter#1#2}}

\def\pgfutil@append@tomacro#1#2{%
    \expandafter\def\expandafter#1\expandafter{#1#2}}


\endinput


==> pgfint.code.tex <==
% Copyright 2019 by Henri Menke
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% Guard against reading twice
\ifx\pgfintloaded\pgfutil@undefined
  \let\pgfintloaded=\relax
\else
  \expandafter\endinput
\fi

% This module is pretty much a rip-off of the LaTeX3 l3int module for integer
% calculations.  Since PGF supports e-TeX now, we can make use of those
% extended facilities.

% In contrast to l3int we will just admit that integers are regular TeX \count
% register and will not implement an extra "integer datatype".

% Evaluate an integer expression using \numexpr
\def\pgfinteval#1{\number\numexpr#1\relax}

% Get the absolute value of an integer by stripping off a leading minus sign
\def\pgfintabs#1{\number\expandafter\pgfint@abs\number\numexpr#1\relax}
\def\pgfint@abs#1{\ifx-#1\else\expandafter#1\fi}

% Minimum and maximum
\def\pgfintmax#1#2{%
  \number\expandafter\pgfint@minmax
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  >
}
\def\pgfintmin#1#2{%
  \number\expandafter\pgfint@minmax
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  <
}
\def\pgfint@minmax#1;#2;#3{%
  \ifnum#1#3#2
    #1%
  \else
    #2%
  \fi
}

% \numexpr has the annoying property to round divisions rather than truncating
% (as you would expect for integer arithmetic).  Therefore we need a truncating
% division function.
\def\pgfintdivtruncate#1#2{%
  \number\numexpr\expandafter\pgfint@divtruncate
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@divtruncate#1#2;#3#4;{%
  \ifx0#1
    0%
  \else
    (#1#2%
      \ifx-#1 +\else-\fi
      (\ifx-#3 -\fi#3#4-1)/2%
    )%
  \fi
  /#3#4%
}

% \pgfintdivtruncate always truncates the result which leads to a rounding
% towards zero.  Donald Knuth defines in TAoCP, Vol 1, 3rd Ed, Section 1.2.4
% that the modulo operation is
%
%    x mod y = x - y * floor(x/y)
%
% In contrast to truncated division, floored division always rounds towards
% -inf, i.e. floor(1/2) = 0 and floor(-1/2) = -1.  This is also how integer
% division is done in Lua.
\def\pgfintdivfloor#1#2{%
  \number\numexpr\expandafter\pgfint@divfloor
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@divfloor#1#2;#3#4;{%
  \ifx0#1
    0%
  \else
    \ifnum
      0\ifx-#1\ifx#3-\else1\fi\fi
      0\ifx-#3\ifx#1-\else1\fi\fi
      >0
      \pgfint@@divfloor#1#2;#3#4;-+%
    \else
      \pgfint@@divfloor#1#2;#3#4;+-%
    \fi
  \fi
  /#3#4%
}
\def\pgfint@@divfloor#1#2;#3#4;#5#6{%
  (#1#2%
  \ifx-#1 #5\else#6\fi
    (\ifx-#3 -\fi#3#4#61)/2%
  )%
}

% Round
\def\pgfintdivround#1#2{\number\numexpr(#1)/(#2)\relax}

% Modulo
\def\pgfintmod#1#2{%
  \number\numexpr\expandafter\pgfint@mod%
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@mod#1;#2;{#1-(\pgfint@divfloor#1;#2;)*#2}

% Setter function so we don't always have to write \pgfinteval
\def\pgfintset#1#2{#1 \numexpr#2\relax}

\endinput


==> pgfkeys.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% The files pgfkeys.code.tex and pgfkeysfiltered.code.tex are
% perfectly self-contained, except that the catcode of @
% should be made a letter.


% Guard against reading twice
\ifx\pgfkeysloaded\undefined
  \let\pgfkeysloaded=\relax
\else
  \expandafter\endinput
\fi

% The purpose of this file is to provide a general settings engine that
% works with all TeX formats and has no save-stack impact

\def\pgfkeys@empty{}
\long\def\pgfkeys@firstoftwo#1#2{#1}
\long\def\pgfkeys@secondoftwo#1#2{#2}

% This is useful:

\ifx\PackageError\undefined
  \def\pgfkeys@error#1{\errmessage{Package pgfkeys Error: #1}}%
\else
  \def\pgfkeys@error#1{\PackageError{pgfkeys}{#1}{}}%
\fi

\ifx\eTeXrevision\undefined%
  \pgfkeys@error{PGF requires etex in extended mode}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

\ifnum\eTeXversion<2
  \pgfkeys@error{PGF requires etex version 2}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

% Set a key to a value
%
% #1 = key
% #2 = tokens
%
% Description:
%
% This command sets the key to the given tokens. The tokens are stored as
% is and can even contain things like #9.
%
% Keys are organized hierarchically using something similar to Unix
% paths. Thus, a typically key might be called "/tikz/length" or
% "/tikz/length dimension/.@cmd". Some keys starting with a dot are
% special, so they should not be used as normal key names (they are
% similar to Unix files starting with a dot -- you can use them, but
% be careful).
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyssetvalue{/tikz/length}{2cm-3cm}
% \pgfkeyssetvalue{/algo/swap}{{#2}{#1}}

\long\def\pgfkeyssetvalue#1#2{%
  \pgfkeys@temptoks{#2}\expandafter\edef\csname pgfk@#1\endcsname{\the\pgfkeys@temptoks}%
}

\long\def\pgfkeyssetevalue#1#2{%
  \edef\pgfkeys@temp##1##2##3##4##5##6##7##8##9{#2}%
  \pgfkeys@temptoks=\expandafter{\pgfkeys@temp{##1}{##2}{##3}{##4}{##5}{##6}{##7}{##8}{##9}}%
  \expandafter\edef\csname pgfk@#1\endcsname{\the\pgfkeys@temptoks}%
}

% Add text to a key at the end
%
% #1 = key
% #2 = a value to be added at the beginning
% #3 = a value to be added at the end
%
% Description:
%
% This command adds #2 to the definition of the key. The key should
% have been set previously using \pgfkeyssetvalue.
%
% Example:
%
% \pgfkeysaddvalue{/tikz/length}{}{-3cm}

\long\def\pgfkeysaddvalue#1#2#3{%
  {%
    \toks0{#2}%
    \pgfkeysifdefined{#1}
    {\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@#1\endcsname}}%
    {\pgfkeys@temptoks{}}%
    \toks1{#3}%
    \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1}% believe or don't: the spaces are important
  }%
  \pgfkeyslet{#1}\pgfkeys@global@temp%
}



% Makes a key equal a given code
%
% #1 = key
% #2 = a code name
%
% Description:
%
% This command executes a \let command so that a key gets the same
% value as the parameter #2.
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyslet{/algo/swap}{\myswap}

\def\pgfkeyslet#1#2{%
  \expandafter\let\csname pgfk@#1\endcsname#2%
}


% Retrieve the code stored in a key into a code
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will set #2 to "point" to the value stored in the key.
%
% Example:
%
% \pgfkeysgetvalue{/tikz/swap}{\myswap}

\def\pgfkeysgetvalue#1#2{\expandafter\let\expandafter#2\csname pgfk@#1\endcsname}



% Retrieve the value stored in a key
%
% #1 = key
%
% Description:
%
% This command will expand to the value stored in the key. The key
% should previously have been set using \pgfkeyasetkey or \pgfkeyslet.
%
% Example:
%
% The length is \pgfkeysvalue{/tikz/length}.

\def\pgfkeysvalueof#1{\csname pgfk@#1\endcsname}



% If for testing whether a key exists
%
% #1 = key
% #2 = if-case
% #3 = else-case
%
% Description:
%
% This if will be executed if the key exists. In eTeX mode this works
% like a normal if, in normal TeX mode you need to provide an \else.
%
% Example:
%
% \pgfkeysifdefined{/tikz/length}{key exists}{does not exist}

\long\def\pgfkeysifdefined#1{%
  \ifcsname pgfk@#1\endcsname
    \expandafter\pgfkeys@firstoftwo
  \else
    \expandafter\pgfkeys@secondoftwo
  \fi
}

% Tests whether a key is assignable. For standard keys which just
% store their value, this is identical to \pgfkeysifdefined.
%
% But \pgfkeysifassignable is true for command keys as well (but not
% for handled keys).
\long\def\pgfkeysifassignable#1#2#3{%
  \pgfkeysifdefined{#1}%
    {#2}
  {\pgfkeysifdefined{#1/.@cmd}%
    {#2}%
    {#3}}%
}%



% Execute settings
%
% #1 = list of settings
%
% Description:
%
% The list of settings should contain comma-separated settings. Each
% setting has the following form:
%
% /path/key=value
%
% The parts "/path/" and "=value" are optional. When the path is not
% specified, the value of the token register "\pgfkeypath" is used. If
% "=value" is missing, the value of the setting "/path/key/.@def" is used
% instead. If this key is set to "\pgfvaluerequired", the key
% "/errors/value required/.@cmd" is executed. This error handler,
% like all other error handlers, will get the current key as its first
% parameter (unexpanded) and the current value as its second value
% (also unexpanded).
%
% Any spaces at the beginning and at the end and around the
% equals-sign are removed. The key with the complete path is set to
% the code \pgfcurrentkey.
%
% The setting is then processed according to the following rules:
%
% 1) If the key /path/key/.@cmd" is present, its code is executed
%    with the value computed above, followed by \pgfeov (end of
%    value). So, to handle
%
%    "/stuff/height=  1.5 ,"
%
%    /stuff/height/.@cmd should be set to some code, that can
%    handle the parameter
%
%    "1.5\pgfeov"
%
%    For instance, saying
%
%    \pgfkeys{/stuff/height/.@cmd}{#1\pgfeov}{\def\myheight{#1}}
%
%    will do nicely.
%
% 2) Otherwise, if the key /path/key is present, this key is
%    set to the value computed above.
%
% 3) Otherwise, if the key /handlers/key/.@cmd is present, it is executed
%    with the same parameters as in 1). Additionally, the
%    token register \pgfcurrentkeypath will be set to "/path/" and the
%    macro \pgfcurrentkeywithoutpath to "key". So, in the above
%    example if neither "/stuff/height/.@cmd" nor
%    "/stuff/height" is present, but "/handlers/height" is,
%    then "/handlers/height" is executed with the parameters:
%
%    "1.5\pgfeov"
%
%    and \pgfcurrentkey is set to "/stuff/height" and \pgfcurrentkeypath
%    is set to "/stuff/" and \pgfcurrentkeywithoutpath to "height".
%
% 4) Otherwise, if the key "/path/.unknown/.@cmd" is present, its code is
%    executed with the same parameters as in 3).
%
% 5) Otherwise, the key "/handlers/.unknown/.@cmd" is executed with the same
%    parameters as in 1).
%
% After all settings have been processed, the value of the token
% register \pgfdefaultkeypath is set to its original value. Thus, any local
% change of this token register has no effect outside the call.
%
% Example:
%
% \pgfkeys{/tikz/.is family}
% \pgfkeys{/tikz/line width/.cd,
%         .def=\pgfsetlinewidth{##1},
%         .set default=.4pt}
% \pgfkeys{tikz,line width=1pt}

\newtoks\pgfkeys@pathtoks
\def\pgfkeyscurrentpath{\the\pgfkeys@pathtoks}
\newtoks\pgfkeys@temptoks

\def\pgfkeys@root{/}
\let\pgfkeysdefaultpath\pgfkeys@root

\def\pgfkeys{\expandafter\pgfkeys@@set\expandafter{\pgfkeysdefaultpath}}%
\long\def\pgfkeys@@set#1#2{%
  \let\pgfkeysdefaultpath\pgfkeys@root%
  \pgfkeys@parse#2,\pgfkeys@mainstop%
  \def\pgfkeysdefaultpath{#1}}

\def\pgfkeys@parse{\futurelet\pgfkeys@possiblerelax\pgfkeys@parse@main}
\def\pgfkeys@parse@main{%
  \ifx\pgfkeys@possiblerelax\pgfkeys@mainstop%
    \expandafter\pgfkeys@cleanup%
  \else%
    \expandafter\pgfkeys@normal%
  \fi%
}
\newif\ifpgfkeys@syntax@handlers
\def\pgfkeys@normal{%
  \ifpgfkeys@syntax@handlers%
    \expandafter\pgfkeys@syntax@handlers%
  \else%
    \expandafter\pgfkeys@@normal%
  \fi%
}
\def\pgfkeys@syntax@handlers{\pgf@keys@utilifnextchar\relax\pgfkeys@syntax@@handlers\pgfkeys@syntax@@handlers}%get rid of spaces
\def\pgfkeys@syntax@@handlers{\futurelet\pgfkeys@first@char\pgfkeys@syntax@handlers@test}
\def\pgfkeys@syntax@handlers@test{%
  \pgfkeysgetvalue{/handlers/first char syntax/\meaning\pgfkeys@first@char}\pgfkeys@the@handler%
  \ifx\pgfkeys@the@handler\relax%
    \expandafter\pgfkeys@@normal%
  \else%
    \expandafter\pgfkeys@use@handler%
  \fi%
}
\long\def\pgfkeys@use@handler#1,{%
  \pgfkeys@the@handler{#1}%
  \pgfkeys@parse%
}

\long\def\pgfkeys@@normal#1,{%
  \pgfkeys@unpack#1=\pgfkeysnovalue=\pgfkeys@stop%
  \pgfkeys@parse%
}
\def\pgfkeys@cleanup\pgfkeys@mainstop{}

\def\pgfkeys@mainstop{\pgfkeys@mainstop} % equals only itself
\def\pgfkeys@novalue{}
\def\pgfkeysnovalue{\pgfkeys@novalue} % equals only itself
\def\pgfkeysnovalue@text{\pgfkeysnovalue}
\def\pgfkeysvaluerequired{\pgfkeysvaluerequired} % equals only itself

\long\def\pgfkeys@unpack#1=#2=#3\pgfkeys@stop{%
  \pgfkeys@spdef\pgfkeyscurrentkey{#1}%
  \edef\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
  \ifx\pgfkeyscurrentkey\pgfkeys@empty%
    % Skip
  \else%
    \pgfkeys@add@path@as@needed%
    \pgfkeys@spdef\pgfkeyscurrentvalue{#2}%
    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
      \pgfkeysifdefined{\pgfkeyscurrentkey/.@def}%
      {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@def}{\pgfkeyscurrentvalue}}
      {}% no default, so leave it
    \fi%
    \ifx\pgfkeyscurrentvalue\pgfkeysvaluerequired%
      \def\pgf@marshal{\pgfkeysvalueof{/errors/value required/.@cmd}}%
      \expandafter\pgf@marshal\expandafter{\pgfkeyscurrentkey}{}\pgfeov%
    \else%
      \pgfkeys@case@one%
    \fi%
  \fi}

\def\pgfkeys@case@one{%
  \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}%
  {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
   \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@case@two}%
}

\def\pgfkeys@case@two{%
  \pgfkeysifdefined{\pgfkeyscurrentkey}%
  {\pgfkeys@case@two@extern}%
  {\pgfkeys@case@three}%
}

\def\pgfkeys@case@two@extern{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
    \pgfkeysvalueof{\pgfkeyscurrentkey}%
  \else%
    \pgfkeyslet{\pgfkeyscurrentkey}\pgfkeyscurrentvalue%
  \fi%
}


% either handled key or unknown.
%
% This macro will be replaced by the /handler config/handle only existing
% configuration, see below.
\def\pgfkeys@case@three{%
  \pgfkeys@split@path%
  \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}%
  {\pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@unknown}%
}
\let\pgfkeys@case@three@handleall=\pgfkeys@case@three
\def\pgfkeys@case@three@handle@restricted{%
  \pgfkeys@split@path%
  \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
    \pgfkeys@ifexecutehandler{%
    \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
      \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
  }{%
      % this here is necessary:  /my search path/key/.code
      % won't be called, so \pgfkeyscurrentpath == '/my search path/key'
      % -> it should be one directory higher! We want to invoke the
    %  .unknown handler in
    % '/my search path'
    %
    % Idea:
    % set
    % - path := '/my search path'
    % - name := 'key/.code'
    % - key = '/my search path/key/.code'
    \let\pgfkeys@tempa=\pgfkeyscurrentkey
    \let\pgfkeys@tempb=\pgfkeyscurrentname
      \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}%
      \pgfkeys@split@path%
    \let\pgfkeyscurrentkey=\pgfkeys@tempa
    \edef\pgfkeyscurrentname{\pgfkeyscurrentname/\pgfkeys@tempb}%
      \pgfkeys@unknown
  }%
  }{%
    \pgfkeys@unknown
  }%
}

% this macro is to implement the |handle only existing| key in key filtering:
% #1: the code to invoke IF the key handler shall be executed
% #2: the code to invoke if it shall not run.
\def\pgfkeys@ifexecutehandler#1#2{#1}%
\let\pgfkeys@ifexecutehandler@handleall=\pgfkeys@ifexecutehandler
\def\pgfkeys@ifexecutehandler@handleonlyexisting#1#2{%
  \ifcsname pgfk@excpt@\pgfkeyscurrentname\endcsname%
     #1% ok, this particular key handler is known and should be processed in any case (for example .try)
  \else
     % implement the 'only existing' feature here:
     \pgfkeysifdefined{\pgfkeyscurrentpath}{#1}{%
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}{#1}{#2}%
     }{}%
  \fi%
}%
\def\pgfkeys@ifexecutehandler@handlefullorexisting#1#2{%
  \ifpgfkeysaddeddefaultpath
    \ifcsname pgfk@excpt@\pgfkeyscurrentname\endcsname%
       #1% ok, this particular key handler is known and be processed in any case (for example .try)
    \else
       % implement the 'only existing' feature here:
       \pgfkeysifdefined{\pgfkeyscurrentpath}{%
         #1%
       }{%
         \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}{%
           #1%
         }{%
           #2%
         }%
       }%
    \fi%
  \else
    #1% ok, always true if the USER explicitly provided the full key path.
  \fi
}%
\def\pgfkeysaddhandleonlyexistingexception#1{\expandafter\def\csname pgfk@excpt@#1\endcsname{1}}%

\def\pgfkeys@unknown{%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.unknown/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {%
    \pgfkeysgetvalue{/handlers/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
  }%
}


\long\def\pgfkey@argumentisspace#1{%
  \long\def\pgfkeys@spdef##1##2{%
    \futurelet\pgfkeys@possiblespace\pgfkeys@sp@a##2\pgfkeys@stop\pgfkeys@stop#1\pgfkeys@stop\relax##1}%
  \def\pgfkeys@sp@a{%
    \ifx\pgfkeys@possiblespace\pgfkeys@sptoken%
      \expandafter\pgfkeys@sp@b%
    \else%
      \expandafter\pgfkeys@sp@b\expandafter#1%
    \fi}%
  \long\def\pgfkeys@sp@b#1##1 \pgfkeys@stop{\pgfkeys@sp@c##1}%
}
\pgfkey@argumentisspace{ }
\long\def\pgfkeys@sp@c#1\pgfkeys@stop#2\relax#3{\pgfkeys@temptoks{#1}\edef#3{\the\pgfkeys@temptoks}}
{\def\:{\global\let\pgfkeys@sptoken= } \: }



\def\pgfkeys@add@path@as@needed{% Should add the path if the
  % \pgfkeyscurrentkey does not start with /
  \expandafter\futurelet\expandafter\pgfkeys@possibleslash\expandafter\pgfkeys@check@slash\pgfkeyscurrentkey\relax%
}
\newif\ifpgfkeysaddeddefaultpath
\def\pgfkeys@check@slash{%
  \ifx\pgfkeys@possibleslash/%
    \expandafter\pgfkeys@nevermind%
  \else%
    \expandafter\pgfkeys@addpath%
  \fi%
}

\def\pgfkeys@nevermind#1\relax{%
  \pgfkeysaddeddefaultpathfalse
  \let\pgfkeyscurrentkeyRAW\pgfkeyscurrentkey
}
\def\pgfkeys@addpath#1\relax{%
  \pgfkeysaddeddefaultpathtrue
  \def\pgfkeyscurrentkeyRAW{#1}%
  \edef\pgfkeyscurrentkey{\pgfkeysdefaultpath#1}%
}


\def\pgfkeys@split@path{% Should assign the two codes
                       % \pgfkeyscurrentname and \pgfcurrentlkeypath
  \pgfkeys@pathtoks{}%
  \expandafter\pgfkeys@splitter\pgfkeyscurrentkey//%
}
\def\pgfkeys@splitter#1/#2/{%
  \def\pgfkeys@temp{#2}%
  \ifx\pgfkeys@temp\pgfkeys@empty%
    % Ah. done
    \def\pgfkeyscurrentname{#1}%
    \expandafter\pgfkeys@gobbletoslash%
  \else%
    \expandafter\pgfkeys@pathtoks\expandafter{\the\pgfkeys@pathtoks#1/}%
  \fi%
  \pgfkeys@splitter#2/%
}
\def\pgfkeys@gobbletoslash\pgfkeys@splitter/{%
  \if\relax\detokenize\expandafter{\the\pgfkeys@pathtoks}\relax\else
    \expandafter\pgfkeys@remove@slash\the\pgfkeys@pathtoks\relax
  \fi
}%
\def\pgfkeys@remove@slash#1/\relax{\pgfkeys@pathtoks{#1}}



% Quickly set keys
%
% #1 = default path
% #2 = key-value pairs
%
% Description:
%
% This command starts the execution with the default path set to
% #1. This command should only be used when speed is important (like
% in a heavily used macro like \tikzset). Normally, keys should be
% used to set the path. Note that if #1 equals /, then \pgfkeys will
% actually be quicker!
%
% Example:
%
% \pgfqkeys{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\def\pgfqkeys{\expandafter\pgfkeys@@qset\expandafter{\pgfkeysdefaultpath}}%
\long\def\pgfkeys@@qset#1#2#3{\def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}}


% Sets keys while setting keys
%
% #1 = key-value pairs
%
% Description:
%
% This code may only be called inside the code that is executed for a
% key. The #1 should be a list of settings pairs. They will be executed
% as if they had been given as the argument to the \pgfkeys command.
%
% Example:
%
% \pgfkeys{tikz,myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\long\def\pgfkeysalso#1{\pgfkeys@parse#1,\pgfkeys@mainstop}



% Quickly sets keys while setting keys
%
% #1 = default path
% #2 = key-value pairs
%
% Description:
%
% This command executes #2 with the default path set to #1. This
% command will cause chaos if used incorrectly. The only safe
% place to use it instead of \pgfkeys is at the beginning of a TeX group.
%
% Example:
%
% \begingroup
%   \pgfqkeysalso{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\long\def\pgfqkeysalso#1#2{\def\pgfkeysdefaultpath{#1/}\pgfkeys@parse#2,\pgfkeys@mainstop}




% Now setup the default handlers and keys:

% Define a key macro with one argument (\def or \edef)
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes one parameter and has #2 as its code.
%
% Example:
%
% \pgfkeysdef{/my key}{\show#1}

\long\def\pgfkeysdef#1#2{%
  \long\def\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@body}{#2}%
}
\long\def\pgfkeysedef#1#2{%
  \long\edef\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetevalue{#1/.@body}{#2}%
}


% Define a key macro with multiple arguments (\def or \edef)
%
% #1 = key
% #2 = argument pattern
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes #2 as its parameter pattern and has #3 as its code.
%
% Example:
%
% \pgfkeysdefargs{/swap}{#1#2}{#2#1}

\long\def\pgfkeysdefargs#1#2#3{%
  \long\def\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetvalue{#1/.@body}{#3}%
}

\long\def\pgfkeysedefargs#1#2#3{%
  \long\edef\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetevalue{#1/.@body}{#3}%
}

% Like \pgfkeysdefargs, but `#2' is an integer denoting the expected
% *number* of arguments.
%
% There is a subtle difference between the 'args' command, when it
% comes to spaces:
%  a key defined with defargs{#1#2} must not have spaces between the
%  arguments when it is used.
%
% See this:
%
%--------------------------------------------------
% % defnargs:
% \pgfkeysdefnargs{/a}{2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /a=
%     {1}
%     {2}
% }
% ->defnargs: 1=`1', 2=`2'
%
% defargs:
% \pgfkeysdefargs{/b}{#1#2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /b=
%     {1}
%     {2}
% }
% ->defargs: 1=`1', 2=` 2'  (note the space!)
%
% defargs:
% \pgfkeysdefargs{/b}{#1#2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /b=
%     {1}%
%     {2}
% }
% ->defargs: 1=`1', 2=`2'
% --------------------------------------------------
\long\def\pgfkeysdefnargs#1#2#3{\pgfkeysdefnargs@{#1}{#2}{#3}{\def}{\pgfkeyssetvalue}}%
\long\def\pgfkeysedefnargs#1#2#3{\pgfkeysdefnargs@{#1}{#2}{#3}{\edef}{\pgfkeyssetevalue}}%
\long\def\pgfkeysdefnargs@#1#2#3#4#5{%
  \ifcase#2\relax
    \pgfkeyssetvalue{#1/.@args}{}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7##8}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7##8##9}%
  \else
    \pgfkeys@error{\string\pgfkeysdefnargs: expected  <= 9 arguments, got #2}%
  \fi
  \pgfkeysgetvalue{#1/.@args}\pgfkeys@tempargs
  \def\pgfkeys@temp{\expandafter\long\expandafter#4\csname pgfk@#1/.@@body\endcsname}%
  \expandafter\pgfkeys@temp\pgfkeys@tempargs{#3}%
  % eliminate the \pgfeov at the end such that TeX gobbles spaces
  % by using
  % \pgfkeysdef{#1}{\pgfkeysvalueof{#1/.@@body}##1}
  % (with expansion of '#1'):
  \edef\pgfkeys@tempargs{\noexpand\pgfkeysvalueof{#1/.@@body}}%
  \def\pgfkeys@temp{\pgfkeysdef{#1}}%
  \ifnum#2=1\relax
    \expandafter\pgfkeys@temp\expandafter{\pgfkeys@tempargs{##1}}%
  \else
    \expandafter\pgfkeys@temp\expandafter{\pgfkeys@tempargs##1}%
  \fi
  #5{#1/.@body}{#3}%
}

% Defining a key command

\pgfkeysdef{/handlers/.code}{\pgfkeysdef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.code 2 args}{\pgfkeysdefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdef{/handlers/.ecode}{\pgfkeysedef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.ecode 2 args}{\pgfkeysedefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdefnargs{/handlers/.code args}{2}{\pgfkeysdefargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.ecode args}{2}{\pgfkeysedefargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.code n args}{2}{\pgfkeysdefnargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.ecode n args}{2}{\pgfkeysedefnargs{\pgfkeyscurrentpath}{#1}{#2}}

% Adding to a key command

\pgfkeys{/handlers/.add code/.code 2 args=%
  % Find out, whether with args or not.
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@args}%
  {% Yes, so add to body and reuse args
  \pgfkeysaddvalue{\pgfkeyscurrentpath/.@body}{#1}{#2}%
  % Redefine code
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@args}{\pgfkeys@tempargs}%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@body}{\pgfkeys@tempbody}%
    \def\pgfkeys@marshal{\expandafter\long\expandafter\gdef\expandafter\pgfkeys@global@temp\pgfkeys@tempargs}%
    \expandafter\pgfkeys@marshal\expandafter{\pgfkeys@tempbody}%
  }%
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@@body}{%
    % support for \pgfkeysndefargs:
    \pgfkeyslet{\pgfkeyscurrentpath/.@@body}{\pgfkeys@global@temp}%
  }{%
    % support for \pgfkeysdefargs:
      \pgfkeyslet{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@global@temp}%
  }%
  }%
  {%
    % No, so single argument (simple \pgfkeysdef). Redefine accordingly.
    \edef\pgf@expanded@path{\pgfkeyscurrentpath}%
    {%
      \toks0{#1}%
      \pgfkeysifdefined{\pgf@expanded@path/.@cmd}%
      {\expandafter\expandafter\expandafter\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@\pgf@expanded@path/.@body\endcsname}}%
      {\expandafter\pgfkeys@temptoks\expandafter{\expandafter\pgfkeyssetvalue\expandafter{\pgf@expanded@path}{##1}}}%
      \toks1{#2}%
      \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1 }%
    }%
    \def\pgf@temp{\pgfkeyssetvalue{\pgf@expanded@path/.@body}}%
    \expandafter\pgf@temp\expandafter{\pgfkeys@global@temp}%
    \expandafter\long\expandafter\def\expandafter\pgfkeys@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
    \pgfkeyslet{\pgf@expanded@path/.@cmd}\pgfkeys@temp%
  }%
}
\pgfkeys{/handlers/.prefix code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={#1}{}}}%
\pgfkeys{/handlers/.append code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{#1}}}%


% Defining a style

\pgfkeys{/handlers/.style/.code=\pgfkeys{\pgfkeyscurrentpath/.code=\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.estyle/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\noexpand\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.style args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.code args={#1}{\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.estyle args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.ecode args={#1}{\noexpand\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.style 2 args/.code=\pgfkeys{\pgfkeyscurrentpath/.code 2 args=\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.style n args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.code n args={#1}{\pgfkeysalso{#2}}}}

% Adding to a style

\pgfkeys{/handlers/.add style/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{\pgfkeysalso{#2}}}}%
\pgfkeys{/handlers/.prefix style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{}}}%
\pgfkeys{/handlers/.append style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{\pgfkeysalso{#1}}}}%


% Defining a value

\pgfkeys{/handlers/.initial/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/handlers/.add/.code 2 args=\pgfkeysaddvalue{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeys{/handlers/.prefix/.code=\pgfkeysaddvalue{\pgfkeyscurrentpath}{#1}{}}
\pgfkeys{/handlers/.append/.code=\pgfkeysaddvalue{\pgfkeyscurrentpath}{}{#1}}
\pgfkeys{/handlers/.get/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/handlers/.link/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath}{\pgfkeysvalueof{#1}}}


% Defining a default

\pgfkeys{/handlers/.default/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{#1}}
\pgfkeys{/handlers/.value required/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeysvaluerequired}}
\pgfkeys{/handlers/.value forbidden/.code=\pgfkeys{\pgfkeyscurrentpath/.add code=%
{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
  \else%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/value forbidden/.@cmd}}%
    \expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkey\expandafter}\expandafter{\pgfkeyscurrentvalue}\pgfeov%
  \fi%
}{}}}


% High-level cmds

\pgfkeys{/handlers/.store in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\def#1{##1}}}
\pgfkeys{/handlers/.estore in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\edef#1{##1}}}

\pgfkeys{/handlers/.is if/.code=\pgfkeysalso{%
    \pgfkeyscurrentpath/.code=\pgfkeys@handle@boolean{#1}{##1},
    \pgfkeyscurrentpath/.default=true%
  }%
}
\def\pgfkeys@handle@boolean#1#2{%
  \ifcsname#1#2\endcsname%
    \csname#1#2\endcsname%
  \else%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/boolean expected/.@cmd}}%
    \expandafter\pgf@marshal\expandafter{\pgfkeyscurrentkey}{#2}\pgfeov%
  \fi
}

\pgfkeys{/handlers/.is choice/.code=%
  \pgfkeys{%
    \pgfkeyscurrentpath/.cd,%
    .code=\def\pgfkeys@was@choice{##1}\expandafter\pgfkeysalso\expandafter{\pgfkeyscurrentkey/##1},
    .unknown/.code={%
      \def\pgf@marshal{\pgfkeysvalueof{/errors/unknown choice value/.@cmd}}%
      {\expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@pathtoks\expandafter}\expandafter{\pgfkeys@was@choice}\pgfeov}%
    }%
  }%
}


% Repeatedly setting a key

\pgfkeys{/handlers/.list/.code=%
  {%
    \ifx\foreach\@undefined%
      \pgfkeys@error{You need to load the pgffor package to use the .list key syntax.}%
    \fi%
    % Use foreach to unfold the list
    \def\pgf@keys@temp{}%
    \foreach \pgf@keys@key in{#1}%
    {\expandafter\expandafter\expandafter\gdef%
      \expandafter\expandafter\expandafter\pgf@keys@temp%
      \expandafter\expandafter\expandafter{\expandafter\pgf@keys@temp\expandafter{\pgf@keys@key}}}%
    \edef\pgf@keys@list@path{\pgfkeyscurrentpath}%
    \expandafter\expandafter\expandafter\pgf@keys@do@list%
    \expandafter\expandafter\expandafter{\expandafter\pgf@keys@list@path\expandafter}\pgf@keys@temp\pgf@stop%
  }%
}
\def\pgf@keys@do@list#1{\pgf@keys@utilifnextchar\bgroup{\pgf@keys@do@list@item{#1}}\pgf@keys@gobble}
\def\pgf@keys@do@list@item#1#2{\pgfkeysalso{#1={#2}}\pgf@keys@do@list{#1}}


% Forwarding

\pgfkeys{/handlers/.forward to/.code=%
  \pgfkeys{\pgfkeyscurrentpath/.add code={}{\pgfkeys{#1={##1}}}}
}


% Inspection handlers

\pgfkeys{/handlers/.show value/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{\pgfkeysshower}\show\pgfkeysshower} % inspect the value
\pgfkeys{/handlers/.show code/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeysshower}\show\pgfkeysshower} % inspect the body of the command


% First char syntax handlers
\pgfkeys{/handlers/first char syntax/.is if=pgfkeys@syntax@handlers}

% Path handling

% Prepares the .unknown handler used by '.search also'.
% It will be stored into \pgfkeys@global@temp.
\def\pgfkeys@searchalso@prepare@unknown@handler#1{%
  \global\def\pgfkeys@global@temp##1\pgfeov{}%
  \pgfkeys@searchalso@parse#1,\pgfkeys@mainstop
  {%
    \toks0=\expandafter{\pgfkeys@global@temp##1\pgfeov}%
  \toks1={%
    \pgfkeysgetvalue{/handlers/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeys@searchalso@temp@value\pgfeov
  }%
  \xdef\pgfkeys@global@temp{%
    \noexpand\def\noexpand\pgfkeys@searchalso@temp@value{####1}%
    \noexpand\ifpgfkeysaddeddefaultpath
      \noexpand\expandafter\noexpand\pgfkeys@firstoftwo
    \noexpand\else
      \noexpand\expandafter\noexpand\pgfkeys@secondoftwo
    \noexpand\fi{%
      \noexpand\pgfkeyssuccessfalse
      \noexpand\let\noexpand\pgfkeys@searchalso@name=\noexpand\pgfkeyscurrentkeyRAW
      \the\toks0 % one or more /.try things; one for each path. The last element won't have a /.try
      %\noexpand\ifpgfkeyssuccess
      %\noexpand\else
      %  \the\toks1 % invoke /handlers/.unknown handler
      %\noexpand\fi
    }{%
      \the\toks1 % invoke /handlers/.unknown handler
    }%
  }%
  \expandafter\gdef\expandafter\pgfkeys@global@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
  }%
}%

\def\pgfkeys@searchalso@parse{\futurelet\pgfkeys@possiblerelax\pgfkeys@searchalso@parse@main}
\def\pgfkeys@searchalso@parse@main{%
  \ifx\pgfkeys@possiblerelax\pgfkeys@mainstop%
    \expandafter\pgfkeys@cleanup%
  \else%
    \expandafter\pgfkeys@searchalso@appendentry%
  \fi%
}
\def\pgfkeys@searchalso@appendentry#1,#2{%
  \def\pgfkeys@searchalso@nexttok{#2}%
  \pgfkeys@spdef\pgfkeys@temp{#1}%
  {%
    \toks0=\expandafter{\pgfkeys@global@temp##1\pgfeov}%
  \toks1=\expandafter{\pgfkeys@temp}%
  \xdef\pgfkeys@global@temp{%
    \the\toks0 % the space is important!
    \noexpand\ifpgfkeyssuccess\noexpand\else
      \noexpand\pgfqkeys{\the\toks1 }{\noexpand\pgfkeys@searchalso@name
               \ifx\pgfkeys@searchalso@nexttok\pgfkeys@mainstop\else/.try\fi /.expand once=\noexpand\pgfkeys@searchalso@temp@value}%
    \noexpand\fi}%
  \expandafter\gdef\expandafter\pgfkeys@global@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
  }%
  \pgfkeys@searchalso@parse#2%
}
\pgfkeys{%
  /handlers/.is family/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\edef\noexpand\pgfkeysdefaultpath{\pgfkeyscurrentpath/}},%
  /handlers/.cd/.code=\edef\pgfkeysdefaultpath{\pgfkeyscurrentpath/},%
  /handlers/.search also/.code={%
    \pgfkeys@searchalso@prepare@unknown@handler{#1}%
%\message{I prepared the '\pgfkeyscurrentpath/.unknown' handler \meaning\pgfkeys@global@temp\space for '#1'.}%
    \pgfkeyslet{\pgfkeyscurrentpath/.unknown/.@cmd}{\pgfkeys@global@temp}%
  }
}%


% Value expansion

\pgfkeys{/handlers/.expand once/.code=\expandafter\pgfkeys@exp@call\expandafter{#1}}
\pgfkeys{/handlers/.expand twice/.code=\expandafter\expandafter\expandafter\pgfkeys@exp@call\expandafter\expandafter\expandafter{#1}}
\pgfkeys{/handlers/.expanded/.code=\edef\pgfkeys@temp{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfkeys@temp}}

\long\def\pgfkeys@exp@call#1{\pgfkeysalso{\pgfkeyscurrentpath={#1}}}

\def\pgfkeys@mathparse{%
  \ifcsname pgfmathparse\endcsname
    \expandafter\pgfmathparse
  \else
    \pgfkeys@error{You have to load `pgfmath' to use \string\pgfmathparse}%
    \expandafter\def\expandafter\pgfmathresult
  \fi
}
\pgfkeys{/handlers/.evaluated/.code=\pgfkeys@mathparse{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}

% Try to set a key and do nothing if not define

\newif\ifpgfkeyssuccess
\pgfkeys{/handlers/.try/.code=\pgfkeys@try}
\pgfkeys{/handlers/.retry/.code=\ifpgfkeyssuccess\else\pgfkeys@try\fi}
\def\pgfkeys@try{%
  \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}% make sure that \pgfkeys@code doesn't know about 'try'. Important for .is choice
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
    {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
    {}% no default, so leave it
  \fi%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
    \pgfkeyssuccesstrue%
  }%
  {%
    \pgfkeysifdefined{\pgfkeyscurrentpath}%
    {%
      \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
        \pgfkeysvalueof{\pgfkeyscurrentpath}%
      \else%
        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
      \fi%
      \pgfkeyssuccesstrue%
    }%
    {%
      \pgfkeys@split@path%
      \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
      % in the standard configuration, this check here is redundant
      % because pgfkeys@ifexecutehandler === true.
    % It is only interesting for 'handle only existing'.
        \pgfkeys@ifexecutehandler{%
        \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
          \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
          \pgfkeyssuccesstrue%
      }{%
        \pgfkeyssuccessfalse
      }%
      }{%
      \pgfkeyssuccessfalse
      }%
  }%
  }%
}

% Utilities

\pgfkeys{/utils/exec/.code=#1} % simply execute the given code directly.


% Errors

\pgfkeys{
  /errors/boolean expected/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      Boolean parameter of key '\the\toks1' must be 'true' or 'false', not
      '\the\toks2'. I am going to ignore it%
    }%
  },
  /errors/value required/.code 2 args=%
  {%
    \toks1={#1}%
    \pgfkeys@error{%
      The key '\the\toks1' requires a value. I am going to ignore this
      key%
    }%
  },
  /errors/value forbidden/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      You may not specify a value for the key '\the\toks1'. I am going to ignore
      the value '\the\toks2' that you provided%
    }%
  },
  /errors/unknown choice value/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      Choice '\the\toks2' unknown in choice key '\the\toks1'. I am
      going to ignore this key%
    }%
  },
  /errors/unknown key/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \def\pgf@temp{#2}%
    \pgfkeys@error{%
      I do not know the key '\the\toks1'\ifx\pgf@temp\pgfkeysnovalue@text\space\else, to which you passed
      '\the\toks2', \fi and I am going to ignore it. Perhaps you
      misspelled it%
    }%
  }
}

\pgfkeys{/handlers/.unknown/.code=%
  {%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/unknown key/.@cmd}}%
    {\expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkey\expandafter}\expandafter{\pgfkeyscurrentvalue}\pgfeov}%
  }%
}

\pgfkeys{
  /handler config/.is choice,
  /handler config/all/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handleall
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handleall
  },
  /handler config/only existing/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handle@restricted
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handleonlyexisting
  },
  /handler config/full or existing/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handle@restricted
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handlefullorexisting
  },
  /handler config/only existing/add exception/.code={\pgfkeysaddhandleonlyexistingexception{#1}},
}%
\pgfkeysaddhandleonlyexistingexception{.cd}%
\pgfkeysaddhandleonlyexistingexception{.try}%
\pgfkeysaddhandleonlyexistingexception{.retry}%
\pgfkeysaddhandleonlyexistingexception{.lastretry}%
\pgfkeysaddhandleonlyexistingexception{.unknown}%
\pgfkeysaddhandleonlyexistingexception{.expand once}%
\pgfkeysaddhandleonlyexistingexception{.expand twice}%
\pgfkeysaddhandleonlyexistingexception{.expanded}%


% Utilities for self-containment
\def\pgf@keys@gobble#1{}
\long\def\pgf@keys@utilifnextchar#1#2#3{%
  \let\pgf@keys@utilreserved@d=#1%
  \def\pgf@keys@utilreserved@a{#2}%
  \def\pgf@keys@utilreserved@b{#3}%
  \futurelet\pgf@keys@utillet@token\pgf@keys@utilifnch}
\def\pgf@keys@utilifnch{%
  \ifx\pgf@keys@utillet@token\pgf@keys@utilsptoken
    \let\pgf@keys@utilreserved@c\pgf@keys@utilxifnch
  \else
    \ifx\pgf@keys@utillet@token\pgf@keys@utilreserved@d
      \let\pgf@keys@utilreserved@c\pgf@keys@utilreserved@a
    \else
      \let\pgf@keys@utilreserved@c\pgf@keys@utilreserved@b
    \fi
  \fi
  \pgf@keys@utilreserved@c}
{%
  \def\:{\global\let\pgf@keys@utilsptoken= } \:
  \def\:{\pgf@keys@utilxifnch} \expandafter\gdef\: {\futurelet\pgf@keys@utillet@token\pgf@keys@utilifnch}
}


\input pgfkeysfiltered.code.tex

\endinput


==> pgfkeysfiltered.code.tex <==
% Copyright 2019 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file contains additions to pgfkeys.code.tex (loaded
% automatically at the end of pgfkeys.code.tex)
%
% Improvements:
%
% - option filtering
%   you provide
%     - a boolean predicate
%     - a "filter handler" which will be invoked for non-matching options,
%     - a key=value list as usual.
%   The filter sets only matching options and invokes the handler for
%   unmatching ones.
%
% - Fast family support as in xkeyval.
%   - A key like /my tree/my option  can be associated with /my family
%   - You can efficiently set keys which belong to a set of "active"
%     families.
%  Remaining options can be collected into a macro.

% WARNING:
% this file overwrites
% \pgfkeys@addpath
% \pgfkeys@nevermind
%
% all other features are 'additive'


% these implementations will be switched dynamically with their
% filtered versions (in \pgfkeys@install@filter@and@invoke)
\let\pgfkeys@orig@case@one=\pgfkeys@case@one
\let\pgfkeys@orig@@set=\pgfkeys@@set
\let\pgfkeys@orig@@qset=\pgfkeys@@qset
\let\pgfkeys@orig@try=\pgfkeys@try
\let\pgfkeys@orig@unknown=\pgfkeys@unknown

\newif\ifpgfkeysfilteringisactive
\newif\ifpgfkeysfiltercontinue
\let\pgfkeys@key@predicate=\pgfkeys@empty
\let\pgfkeys@filtered@handler=\pgfkeys@empty
\newtoks\pgfkeys@tmptoks

% Performs 'filtered' key settings.
%
% For every option for which the path prefixing has already been done,
% the current key filter predicate will be invoked. If the predicate
% returns true, pgfkeys will process this key in the normal manner.
% If not, a key filter handler will be invoked.
%
% The *predicate* and *handler* semantics are as follows:
% PRECONDITION:
%         1. The variables
%             \pgfkeyscurrentkey (full path including name)
%             \pgfkeyscurrentkeyRAW (the current key as it has been
%                                    found in the key=value list
%                                    without path modification)
%             \pgfkeyscurrentvalue
%             are all set. If the current key is a handler variable,
%                 \pgfkeyscurrentname
%             and
%                 \pgfkeyscurrentpath
%             are also set.
%         2. The type of option has already been checked, that means
%             case (1) whether '.@cmd' exists
%             case (2) whether the key as such has its value
%             case (3) it is a handler like '.code', '.cd' or whatever.
%             case (0) it is unknown.
%             The actual case number (0-3) will be provided as contents
%             of the macro
%                 \pgfkeyscasenumber.
%             It is always a one-character token, so it may be compared
%             with both, \ifnum or \if.
%             Please note that unknown options will be processed with
%             the usual '.unknown' handlers unless the key filter takes
%             control over unknown options as well.
%
% POSTCONDITION:
%         the predicate sets
%             \pgfkeysfiltercontinuetrue
%         or
%             \pgfkeysfiltercontinuefalse
%         (the boolean \ifpgfkeysfiltercontinue).
% Depending on this 'if', option processing will be continued or
% skipped.
%
% The handler can do anything with the option, for example collect
% unmatched ones.
%
% ATTENTION: \pgfkeysfiltered can't be nested (yet). Use the
% \pgfkeyspredicateAND if you need multiple predicates at once.
% Nesting would produce unexpected results because the current filter
% state can't be stored/restored without TeX-groups, therefor it is
% disabled.
%
% ATTENTION: you can't filter error messages.
%
% REMARK: In case (3), the macros \pgfkeyscurrentpath and
% \pgfkeyscurrentname have already been computed, you do not need to
% invoke \pgfkeyssplitpath. In any other case, neither path nor name
% are required for the options processing - if you need them for
% predicates/handlers, you need to compute them by hand.
%
%
% Example:
%   \def\unmatched{}
%   \pgfkeys{/pgf/key filters/is descendant of/.install key filter=/my group}
%   \pgfkeys{/pgf/key filter handlers/append filtered to/.install key filter handler=\unmatched}
%   \pgfkeysfiltered%
%       {/my group/option 1=value 1,/tikz/option 2=value 2}
% ->
%  will set '/my group/option 1' as usual, but '/tikz/option 2' will not
%  be set. Instead, it will be appended to '\unmatched' such that
%  \unmatched = {/tikz/option 2=value2}
%  after the operation.
%
% Arguments:
% #1:  key-value list.
\def\pgfkeysfiltered{%
    % produce
    % '{<default path>}'
    % each expanded exactly one time into the register:
    \expandafter\pgfkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}%
}

% #1: old value of default path.
% #2: key-value-list.
\long\def\pgfkeysfiltered@@install#1#2{%
    \pgfkeys@install@filter@and@invoke{%
        \let\pgfkeysdefaultpath\pgfkeys@root%
        \pgfkeys@parse#2,\pgfkeys@mainstop%
        \def\pgfkeysdefaultpath{#1}%
    }%
}

% Assuming that macro #1 contains a key=value list, this command
% performs an \pgfkeysalso command for the content of macro #1.
%
% It can be used in conjunction with
%   - \pgfkeysfiltered and
%   - \pgfkeysappendfilterednamestomacro:
% the first pass fill only process options matching the filter, then,
% a \pgfkeysalsofrom can be used at a later time to set the remaining
% options.
%
% Example:
% \pgfkeys{/my group/.cd,/utils/exec=\pgfkeysalsofrom\filtered}
\long\def\pgfkeysalsofrom#1{%
    \expandafter\pgfkeysalso\expandafter{#1}%
}

% The same as \pgfkeysalsofrom, but it invokes \pgfkeysalsofiltered.
\long\def\pgfkeysalsofilteredfrom#1{%
    \expandafter\pgfkeysalsofiltered\expandafter{#1}%
}

% #1 = options
\long\def\pgfkeysalsofiltered#1{%
    \pgfkeys@install@filter@and@invoke{\pgfkeysalso{#1}}%
}%

% The same like \pgfkeysfiltered, but with quick search path setting.
%
% #1: default path
% #2: key-value-pairs
\long\def\pgfqkeysfiltered#1{%
    \expandafter\pgfqkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}{#1}%
}

% #1: old value of default path.
% #2: default path
% #3: key-value-list.
\long\def\pgfqkeysfiltered@@install#1#2#3{%
    \pgfkeys@install@filter@and@invoke{%
        \def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}%
    }%
}

% Family management
%
% The family code provides the following features:
% 1. every key can be associated with 0 or 1 'family'.
% 2. Families are a loose association which are independent of the key
% hierarchy.
%   For example, /my tree/key1  can belong to family /tikz.
%
% 3. It is possible to "activate" or "deactivate" single families.
%    Furthermore, it is possible to set only keys which belong to
%    active families (using \pgfkeysfiltered).
% 4. Runtime complexities:
%    If you have N options and you only want to process K active
%    families, the runtime is O( N + K ):
%      - activate every family O(K)
%      - use \pgfkeyshasactivefamily as filter predicate O(N)
%      - deactivate every family O(K)


% Activates family #1.
%
% #1 maybe a macro.
\def\pgfkeysactivatefamily#1{%
    \pgfkeysiffamilydefined
        {#1}%
        {\csname pgfk@#1/familyactivetrue\endcsname}%
        {\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[ACTIVATING FAMILY #1]}%
}

% Deactivates family #1.
%
% #1 maybe a macro.
\def\pgfkeysdeactivatefamily#1{%
    \pgfkeysiffamilydefined
        {#1}%
        {\csname pgfk@#1/familyactivefalse\endcsname}%
        {\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[DEACTIVATING FAMILY #1]}%
}

% Activates all families in the comma separated list #1.
%
% It will also generate code for deactivation of all those families
% into the command #2.
%
% #1: a comma-separated list of fully qualified family names.
% #2: a command which will be filled with a deactivate-all command.
\def\pgfkeysactivatefamilies#1#2{%
    \pgfkeyssavekeyfilterstateto\pgfkeys@cur@state
    \expandafter\pgfkeysactivatefamilies@impl\expandafter{\pgfkeys@cur@state}{#1}{#2}%
}
% #1: commands needed to restore the old filtering state
% #2: family name list
% #3: macro name for de-activate command
\def\pgfkeysactivatefamilies@impl#1#2#3{%
    \pgfkeysinstallkeyfilter{/pgf/key filters/false}{}%
    \let#3=\pgfkeys@empty%
    \def\pgfkeys@filtered@handler{\pgfkeys@family@activate@handler{#3}}%
    \pgfkeysalsofiltered{#2}%
    #1%
}

\def\pgfkeys@family@activate@handler#1{%
    \pgfkeysactivatefamily{\pgfkeyscurrentkey}%
    % produce
    %   <old list> '\pgfkeysdeactivatefamily{' <current key> '}'
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter\pgfkeysdeactivatefamily\expandafter{\pgfkeyscurrentkey}}%
    \edef#1{\the\pgfkeys@tmptoks}%
}

% If for testing whether a family exists.
%
% #1 = fully qualified family name
% #2 = if-case
% #3 = else-case
%
% Description:
%
% If the family exists, #2 will be executed. Otherwise, #3 will be
% called.
\long\def\pgfkeysiffamilydefined#1#2#3{\ifcsname ifpgfk@#1/familyactive\endcsname#2\else#3\fi}

% Sets the TeX boolean
%   \ifpgfkeysfiltercontinue := ( family #1 is active )
%
% Argument:
% #1 the family name. Maybe a macro.
\def\pgfkeysisfamilyactive#1{%
    \pgfkeysiffamilydefined{#1}{%
        \expandafter\let\expandafter\ifpgfkeysfiltercontinue\csname ifpgfk@#1/familyactive\endcsname
    }{%
        \pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov%
        \expandafter\expandafter\expandafter\let\csname ifpgfkeysfiltercontinue\endcsname\csname iffalse\endcsname
    }%
}%

% Retrieve the family of full key #1 into macro #2.
%
% Will set the TeX boolean \ifpgfkeyssuccess to whether the full key
% really has a family.
%
% The family for any key is stored in the sub-key #1/family.
%
% Parameters:
% #1:  the full key name for which the family is requested. Maybe a
%      macro.
% #2:  a macro name which will be filled with the result.
\def\pgfkeysgetfamily#1#2{%
    \pgfkeysifdefined{#1/family}{\pgfkeysgetvalue{#1/family}{#2}\pgfkeyssuccesstrue}{\pgfkeyssuccessfalse}%
}

% Equivalent to \pgfkeys{#1/.belongs to family=#2}
\def\pgfkeyssetfamily#1#2{%
    \pgfkeysiffamilydefined{#2}{%
        \pgfkeyssetvalue{#1/family}{#2}%
    }{%
        \pgfkeysalso{/errors/family unknown=#2}%
    }%
}%


% Sets \ifpgfkeysfiltercontinue to true iff the current key belongs to
% the /errors tree.
\long\def\pgfkeys@cur@is@descendant@of@errors{%
    \expandafter\pgfkeys@cur@is@descendant@of@errors@impl\pgfkeyscurrentkey/errors\pgf@@eov
}%
\long\def\pgfkeys@cur@is@descendant@of@errors@impl#1/errors#2\pgf@@eov{%
    \def\pgfkeyspred@TMP{#1}%
    \ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': TRUE.}%
        \pgfkeysfiltercontinuetrue
    \else
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': FALSE.}%
        \pgfkeysfiltercontinuefalse
    \fi
}%

% \pgfkeysinterruptkeyfilter
% ...
% \endpgfkeysinterruptkeyfilter
% temporarily interrupts key filtering and enables it in
% \endpgfkeysinterruptkeyfilter.
%
% If key filtering it not active, this has no effect at all.
%
% REMARK:
% \pgfkeysinterruptkeyfilter...\endpgfkeysinterruptkeyfilter does NOT
% introduce a \TeX-group.
\def\pgfkeysinterruptkeyfilter{%
    \ifpgfkeysfilteringisactive
        \let\pgfkeys@case@one=\pgfkeys@orig@case@one
        \let\pgfkeys@try=\pgfkeys@orig@try
        \let\pgfkeys@unknown=\pgfkeys@orig@unknown
    \fi
}

\def\endpgfkeysinterruptkeyfilter{%
    \ifpgfkeysfilteringisactive
        \let\pgfkeys@case@one=\pgfkeys@case@one@filtered
        \let\pgfkeys@try=\pgfkeys@try@filtered
        \let\pgfkeys@unknown=\pgfkeys@unknown@filtered
    \fi
}

% Activates families #1, calls \pgfkeysfiltered and deactivates the
% families afterwards.
%
% REMARK: you need to install a family-based key filter predicate
% manually to benefit from the activated families!
%
% #1: comma separated family list
% #2: key-value pairs
%
% @see \pgfkeysactivatefamiliesandfilteroptions
\def\pgfkeysactivatefamiliesandfilteroptions#1#2{%
    \pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
    \pgfkeysfiltered{#2}%
    \pgfkeys@family@deactivation
}

% The "quick" variant of \pgfkeysactivatefamiliesandfilteroptions: it
% also assigns a default path.
%
% #1: comma separated family list
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatefamiliesandfilteroptions#1#2#3{%
    \pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
    \pgfqkeysfiltered{#2}{#3}%
    \pgfkeys@family@deactivation
}

% Public version of split path:
\def\pgfkeyssplitpath{\pgfkeys@split@path}%


% The same as \pgfkeysactivatefamiliesandfilteroptions but just for
% ONE family.
%
% #1: family (maybe a macro)
% #2: key-value pairs
\def\pgfkeysactivatesinglefamilyandfilteroptions#1#2{%
    \pgfkeysactivatefamily{#1}%
    \pgfkeysfiltered{#2}%
    \pgfkeysdeactivatefamily{#1}%
}

% The "quick" variant of \pgfkeysactivatesinglefamilyandfilteroptions
%
% #1: family (maybe a macro)
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatesinglefamilyandfilteroptions#1#2#3{%
    \pgfkeysactivatefamily{#1}%
    \pgfqkeysfiltered{#2}{#3}%
    \pgfkeysdeactivatefamily{#1}%
}

% Installs the key filter '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter=#2}
%
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilter
% and
% \pgfkeyscurrentkeyfilterargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the key. If the key expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilter#1#2{%
    \pgfkeysifdefined{#1/.@cmd}{%
        \edef\pgfkeyscurrentkeyfilter{#1}%
        \def\pgfkeyscurrentkeyfilterargs{#2}%
        \pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@key@predicate@}%
        \def\pgfkeys@key@predicate{\pgfkeys@key@predicate@#2\pgfeov}%
    }{%
        \pgfkeysvalueof{/errors/no such key filter/.@cmd}{#1}{#2}\pgfeov%
    }%
}

% Installs the key filter handler '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter handler=#2}
%
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilterhandler
% and
% \pgfkeyscurrentkeyfilterhandlerargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the handler. If the handler expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilterhandler#1#2{%
    \pgfkeysifdefined{#1/.@cmd}{%
        \edef\pgfkeyscurrentkeyfilterhandler{#1}%
        \def\pgfkeyscurrentkeyfilterhandlerargs{#2}%
        \pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@filtered@handler@}%
        \def\pgfkeys@filtered@handler{\pgfkeys@filtered@handler@#2\pgfeov}%
    }{%
        \pgfkeysvalueof{/errors/no such key filter handler/.@cmd}{#1}{#2}\pgfeov%
    }%
}

% Creates a macro which contains commands to re-activate the current
% key filter and key filter handler. It can be used to temporarily
% switch the key filter.
\def\pgfkeyssavekeyfilterstateto#1{%
    % produce the string
    % \pgfkeysinstallkeyfilter{...}{...}
    % \pgfkeysinstallkeyfilterhandler{...}{...}
    % where each argument is expanded once
    % FIXME: Do the same with less overhead!
    \pgfkeys@tmptoks={\pgfkeysinstallkeyfilter}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilter}}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterargs}\pgfkeysinstallkeyfilterhandler}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandler}}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandlerargs}}%
    \edef#1{%
        \the\pgfkeys@tmptoks
    }%
}


\pgfkeys{%
    /errors/family unknown/.code=\pgfkeys@error{%
        Sorry, I do not know family '#1' and can't work with any assoicated family handling. Perhaps you misspelled it?},
    /errors/no such key filter/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter '#1'.},
    /errors/no such key filter handler/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter handler '#1'.},
    % HANDLERS:
    %
    % .is family should
    %  1. '.cd' into the families' path,
    %  2. define booleans to activate/deactive the family
    %     (see \pgfkeysisfamilyactive)
    %  3. make sure that \pgfkeyshasactivefamily returns true for
    %     the family itself.
    /handlers/.is family/.append code={%
        %\newif is an \outer macro in plain tex, so this here is not portable:
        %\expandafter\newif\csname if\pgfkeyscurrentpath/familyactive\endcsname
        \edef\pgfkeyspred@TMP{pgfk@\pgfkeyscurrentpath/familyactive}%
        \expandafter\pgfkeys@non@outer@newif\expandafter{\pgfkeyspred@TMP}%
        \edef\pgfkeyspred@TMP{\pgfkeyscurrentpath/.belongs to family=\pgfkeyscurrentpath}%
        \expandafter\pgfkeysalso\expandafter{\pgfkeyspred@TMP}%
    },%
    /handlers/.activate family/.code=\pgfkeysactivatefamily{\pgfkeyscurrentpath},
    /handlers/.deactivate family/.code=\pgfkeysdeactivatefamily{\pgfkeyscurrentpath},
    /handlers/.belongs to family/.code={\pgfkeyssetfamily{\pgfkeyscurrentpath}{#1}},%
    %
    %
    % An addition to the '.try' and '.retry' handlers:
    %
    % It is the same as '.retry', but if the option is still unknown, the
    % usual handlers for unknown keys will be invoked.
    /handlers/.lastretry/.code={%
        \ifpgfkeyssuccess\else
            \pgfkeys@try
            \ifpgfkeyssuccess\else
                \pgfkeys@split@path%
                \pgfkeys@unknown
            \fi
        \fi
    },
    %
    %
    /handlers/.install key filter/.code={%
        \pgfkeysinstallkeyfilter{\pgfkeyscurrentpath}{#1}%
    },%
    /handlers/.install key filter handler/.code={%
        \pgfkeysinstallkeyfilterhandler{\pgfkeyscurrentpath}{#1}%
    },%
    %
    %
    % KEY FILTER HANDLERS:
    %
    /pgf/key filter handlers/append filtered to/.code={%
        % Produce
        %  <orig key> '={' <value> '}'
        % where both, the key and the value are expanded just ONCE:
        \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkeyRAW\expandafter=\expandafter{\pgfkeyscurrentvalue}}%
        \ifx#1\pgfkeys@empty
        \else
            % Produce <old list> ','  <orig key> '={' <value> '}'
            \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter,\the\pgfkeys@tmptoks}%
        \fi
        \edef#1{\the\pgfkeys@tmptoks}%
    },%
    /pgf/key filter handlers/ignore/.code={},
    /pgf/key filter handlers/ignore/.install key filter handler,
    /pgf/key filter handlers/log/.code={%
        \pgf@typeout{LOG: the option '\pgfkeyscurrentkey' (was originally '\pgfkeyscurrentkeyRAW') (case \pgfkeyscasenumber) has not been processed due to pgfkeysfiltered.}%
    },
    %
    %
    % KEY FILTER PREDICATES:
    %
    % Returns true if the currently processed key belongs to an active family.
    % A family is active if it has been activated before.
    /pgf/key filters/active families/.code={%
        \if\pgfkeyscasenumber0%
            % unknown options shall be processed with the
            % unknown-handlers.
            \pgfkeysfiltercontinuetrue
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },%
    %
    %
    %
    % This filter works as follows:
    % 1. if the current key belongs to a family:
    %    return whether its family is active,
    % 2. if the current key does NOT belong to a family:
    %    return the result of criterion '#1',
    % 3. the current key is unknown:
    %    return the result of criterion '#2'.
    %
    % Arguments:
    % #1: the predicate which will be invoked in case 2.
    %     It will be invoked with the current case number as argument.
    % #2: the predicate which will be invoked in case 3 with
    %     the current case number as argument.
    /pgf/key filters/active families or no family/.code 2 args={%
        \if\pgfkeyscasenumber0%
            \pgfkeysevalkeyfilterwith{#2}%
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysevalkeyfilterwith{#1}%
            \fi
        \fi
    },
    /pgf/key filters/active families or no family DEBUG/.code 2 args={%
        \if\pgfkeyscasenumber0%
            \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking unknown handler '#2']}%
            \pgfkeysevalkeyfilterwith{#2}%
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
                \ifpgfkeysfiltercontinue
                    \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is ACTIVE]}%
                \else
                    \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is NOT active.]}%
                \fi
            \else% Ok, it does not belong to any family.
                \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking has-no-family-handler '#1']}%
                \pgfkeysevalkeyfilterwith{#1}%
            \fi
        \fi
    },
    %
    % A (faster) shortcut for
    % /pgf/key filters/active families or no family=
    %   {/pgf/keys filters/false}
    %   {/pgf/keys filters/false}
    /pgf/key filters/active families and known/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },
    % A (faster) shortcut for
    % /pgf/key filters/active families or no family=
    %   {/pgf/key filters/is descendant of=#1}% for keys without family
    %   {/pgf/keys filters/false}
    /pgf/key filters/active families or descendants of/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                % the 'is descendant of' implementation has been
                % COPY PASTED here:
                %
                % string prefix comparison:
                \def\pgfkeysisdescendantof@impl##1#1##2\pgf@@eov{%
                    \def\pgfkeyspred@TMP{##1}%
                    \ifx\pgfkeyspred@TMP\pgfkeys@empty
                        \pgfkeysfiltercontinuetrue
                    \else
                        \pgfkeysfiltercontinuefalse
                    \fi
                }%
                \expandafter\pgfkeysisdescendantof@impl\pgfkeyscurrentkey#1\pgf@@eov
            \fi
        \fi
    },
    %
    % Processes only options which are children of #1.
    % Example:
    %   is descendant of/.install key filter=/foo
    % will be true for
    %   /foo/bar/x=y
    %   /foo/.cd
    %   /foo/bar/.style=...
    % but not for
    %   /bar/foo/...
    /pgf/key filters/is descendant of/.code={%
        \if\pgfkeyscasenumber0%
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is UNKNOWN. Calling unknown handler.}%
            % unknown options shall be processed with the
            % unknown-handlers.
            \pgfkeysfiltercontinuetrue
        \else
            % string prefix comparison:
            % [ note : this has been COPY-PASTED to
            %   |active families or descendants of| ]
            \def\pgfkeysisdescendantof@impl##1#1##2\pgf@@eov{%
                \def\pgfkeyspred@TMP{##1}%
                \ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': TRUE.}%
                    \pgfkeysfiltercontinuetrue
                \else
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': FALSE.}%
                    \pgfkeysfiltercontinuefalse
                \fi
            }%
            \expandafter\pgfkeysisdescendantof@impl\pgfkeyscurrentkey#1\pgf@@eov
        \fi
    },%
    %
    %
    %
    % Returns true if the currently processed full key equals #2.
    /pgf/key filters/equals/.code={%
        \if\pgfkeyscasenumber0%
            % Unknown option:
            \pgfkeysfiltercontinuetrue
        \else
            \def\pgfkeyspred@TMP{#1}%
            \ifx\pgfkeyscurrentkey\pgfkeyspred@TMP
                \pgfkeysfiltercontinuetrue
            \else
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },%
    %
    %
    % Argument #1 can be any other (evaluated) filter predicate, its logical return
    % value will be inverted.
    % Example:
    %   not/.install key filter={is descendant of=/tikz}
    % will install a key filter which evaluates 'is descendant of' with argument
    % '/tikz' and returns the logical negation of the result.
    %
    /pgf/key filters/not/.code={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
            \pgfkeysfiltercontinuefalse
        \else
            \pgfkeysfiltercontinuetrue
        \fi
    },%
    /pgf/key filters/and/.code 2 args={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
            \pgfkeysevalkeyfilterwith{#2}%
        \fi
    },%
    /pgf/key filters/or/.code 2 args={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
        \else
            \pgfkeysevalkeyfilterwith{#2}%
        \fi
    },%
    /pgf/key filters/true/.code={\pgfkeysfiltercontinuetrue},%
    /pgf/key filters/true/.install key filter,
    /pgf/key filters/false/.code={%
        \pgfkeysfiltercontinuefalse
    },%
    %
    % Returns false if the current key is unknown, which avoids calling
    % the unknown handlers.
    /pgf/key filters/defined/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \pgfkeysfiltercontinuetrue
        \fi
    },
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Private IMPLEMENTATION
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% This command does THE SAME work as \pgfkeys@case@one,
% but it applies filtering whenever it identified the type of an
% option.
\def\pgfkeys@case@one@filtered{%
    \pgfkeys@cur@is@descendant@of@errors
    \ifpgfkeysfiltercontinue
        \pgfkeys@orig@case@one
    \else
        \pgfkeysfiltercontinuetrue
        \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
            % CASE ONE: a command option
            \def\pgfkeyscasenumber{1}%
            \pgfkeys@key@predicate%
            \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
                \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
            \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                \pgfkeys@filtered@handler%
            \fi
        }{%
            % CASE TWO: a normal value option
            \pgfkeysifdefined{\pgfkeyscurrentkey}{%
                \def\pgfkeyscasenumber{2}%
                \pgfkeys@key@predicate%
                \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                    \pgfkeys@case@two@extern
                \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                    \pgfkeys@filtered@handler%
                \fi
            }{%
                \pgfkeys@split@path
                % CASE THREE: a handler
                \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
                    \pgfkeys@ifexecutehandler{%
                        \def\pgfkeyscasenumber{3}%
                        \pgfkeys@key@predicate%
                        \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                            \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
                            \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
                        \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                            \pgfkeys@filtered@handler%
                        \fi
                    }{%
                        \pgfkeys@unknown
                    }%
                }{%
                    \pgfkeys@unknown
                }%
            }%
        }%
    \fi
}%

\def\pgfkeys@unknown@filtered{%
    % CASE ZERO: an unknown option.
    \def\pgfkeyscasenumber{0}%
    \pgfkeys@key@predicate%
    \ifpgfkeysfiltercontinue
%\message{PROCESSING  KEY \pgfkeyscurrentkey!}%
        % start normal 'unknown' handlers:
        \pgfkeys@orig@unknown
    \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
        \pgfkeys@filtered@handler%
    \fi
}

% Does the same as \pgfkeys@try, but it also invokes the key filters.
\def\pgfkeys@try@filtered{%
    \ifpgfkeysfiltercontinue
        \pgfkeys@orig@try
    \else
        \pgfkeysfiltercontinuetrue
        \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}% make sure that \pgfkeys@code doesn't know about 'try'. Important for .is choice
        \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
            \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
            {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
            {}% no default, so leave it
        \fi%
        \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
        {%
            % CASE ONE: a command option
            \def\pgfkeyscasenumber{1}%
            \pgfkeys@key@predicate%
            \ifpgfkeysfiltercontinue
                \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
                \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
            \else
                \pgfkeys@filtered@handler%
            \fi
            \pgfkeyssuccesstrue%
        }%
        {%
            \pgfkeysifdefined{\pgfkeyscurrentpath}%
            {% CASE TWO: a normal value option
                \def\pgfkeyscasenumber{2}%
                \pgfkeys@key@predicate%
                \ifpgfkeysfiltercontinue
                    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
                        \pgfkeysvalueof{\pgfkeyscurrentpath}%
                    \else%
                        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
                    \fi%
                \else
                    \pgfkeys@filtered@handler%
                \fi
                \pgfkeyssuccesstrue%
            }%
            {%
                \pgfkeys@split@path%
                \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
                    % CASE THREE: a handled key
                    %
                    % in the standard configuration, this check here is redundant
                    % because pgfkeys@ifexecutehandler === true.
                    % It is only interesting for 'handle only existing'.
                    \pgfkeys@ifexecutehandler{%
                        \def\pgfkeyscasenumber{3}%
                        \pgfkeys@key@predicate%
                        \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                            \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
                            \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
                        \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                            \pgfkeys@filtered@handler%
                        \fi
                        \pgfkeyssuccesstrue%
                    }{%
                        \pgfkeyssuccessfalse
                    }%
                }{%
                    \pgfkeyssuccessfalse
                }%
            }%
        }%
    \fi
}


% #1 the code to invoke after init and before cleanup
\long\def\pgfkeys@install@filter@and@invoke#1{%
    \ifpgfkeysfilteringisactive
        \pgfkeys@error{Sorry, nested calls to key filtering routines are not allowed. (reason: It is not possible to properly restore the previous filtering state after returning from the nested call)}%
    \fi
    \pgfkeysfilteringisactivetrue
    \let\pgfkeys@case@one=\pgfkeys@case@one@filtered
    \let\pgfkeys@try=\pgfkeys@try@filtered
    \let\pgfkeys@unknown=\pgfkeys@unknown@filtered
    #1%
    \let\pgfkeys@case@one=\pgfkeys@orig@case@one
    \let\pgfkeys@try=\pgfkeys@orig@try
    \let\pgfkeys@unknown=\pgfkeys@orig@unknown
    \pgfkeysfilteringisactivefalse
}


%--------------------------------------------------
% \def\pgfkeys@eval@key@filter@subroutine@case@one{%
%     \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
%         \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
%         \let\pgfkeyspred@TMP=\pgfkeyscurrentvalue
%         \pgfkeys@eval@key@filter@subroutine@restorestate
%         \expandafter\pgfkeys@code\pgfkeyspred@TMP\pgfeov
%     }{%
%         \pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyscurrentkey\pgfkeyscurrentvalue\pgfeov%
%     }%
% }
% % THIS VERSION IS TOO SLOW. See below.
% \def\pgfkeysevalkeyfilterwith#1{%
%     \edef\pgfkeys@eval@key@filter@subroutine@restorestate{%
%         \noexpand\def\noexpand\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
%         \noexpand\def\noexpand\pgfkeyscurrentkeyRAW{\pgfkeyscurrentkeyRAW}%
%         \noexpand\def\noexpand\pgfkeyscurrentname{\pgfkeyscurrentname}%
%         \noexpand\def\noexpand\pgfkeyscurrentvalue{\pgfkeyscurrentvalue}%
%         \noexpand\pgfkeys@pathtoks={\pgfkeyscurrentpath}%
%     }%
%     \pgfkeysinterruptkeyfilter
%     \let\pgfkeys@case@one=\pgfkeys@eval@key@filter@subroutine@case@one
%     \pgfkeysalso{#1}%
%     \endpgfkeysinterruptkeyfilter% this here also restored \pgfkeys@case@one.
%     \pgfkeys@eval@key@filter@subroutine@restorestate
% }%
%--------------------------------------------------


% Evaluates a key filter '#1'. Example:
% \pgfkeysevalkeyfilterwith{/pgf/key filters/equals=/tikz}
%
% \pgfkeysevalkeyfilterwith works only if key filtering is
% active.
%
% The argument '#1' MUST be a FULL KEY.
%
% The implementation employs a subset of the \pgfkeysalso code.
\long\def\pgfkeysevalkeyfilterwith#1{%
    \pgfkeys@eval@key@filter@subroutine@unpack#1=\pgfkeysnovalue=\pgfkeys@stop
}%
\long\def\pgfkeys@eval@key@filter@subroutine@unpack#1=#2=#3\pgfkeys@stop{%
    \pgfkeys@spdef\pgfkeyspred@TMP{#1}%
    \edef\pgfkeyspred@TMP{\pgfkeyspred@TMP}%
    \pgfkeys@spdef\pgfkeyspred@TMPB{#2}% TMPB=value
    \ifx\pgfkeyspred@TMPB\pgfkeysnovalue@text% Hmm... no value
        \pgfkeysifdefined{\pgfkeyspred@TMP/.@def}%
        {\pgfkeysgetvalue{\pgfkeyspred@TMP/.@def}{\pgfkeyspred@TMPB}}
        {}% no default, so leave it
    \fi%
    \ifx\pgfkeyspred@TMPB\pgfkeysvaluerequired%
        \pgfkeysvalueof{/errors/value required/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
    \else%
        \pgfkeysifdefined{\pgfkeyspred@TMP/.@cmd}{%
            \pgfkeysgetvalue{\pgfkeyspred@TMP/.@cmd}{\pgfkeys@code}%
            \expandafter\pgfkeys@code\pgfkeyspred@TMPB\pgfeov
        }{%
            \pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
        }%
    \fi%
}


\def\pgfkeys@non@outer@newif@#1#2{%
    \expandafter\edef\csname #2true\endcsname{\noexpand\let\noexpand#1=\noexpand\iftrue}%
    \expandafter\edef\csname #2false\endcsname{\noexpand\let\noexpand#1=\noexpand\iffalse}%
    \csname #2false\endcsname
}%

% For latex and context, this here has the same effect as a \newif
% applied to 'if#1'. For plain tex, it has also the same effect, but
% it is not an \outer macro as the plain-tex \newif.
\def\pgfkeys@non@outer@newif#1{%
    \expandafter\pgfkeys@non@outer@newif@\csname if#1\endcsname{#1}%
}
\endinput


==> pgflibraryarrows.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryarrows.code.tex}


% A square bracket shaped arrow

\pgfarrowsdeclare{square bracket}{square bracket}
{
  \pgfutil@tempdima=1pt%
  \advance\pgfutil@tempdima by1.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdima}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=\pgfutil@tempdima%
  \advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdimb}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-.5\pgfutil@tempdimb}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}%
\pgfdeclarearrow{name=[-], means=square bracket}%

\pgfarrowsdeclarereversed{]}{[}{[}{]}%


% A round bracket shaped arrow

\pgfarrowsdeclare{(}{)}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=0.0625\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \pgfutil@tempdimb=0.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{.25\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{.25\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-.5\pgfutil@tempdima}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}%

\pgfarrowsdeclarereversed{)}{(}{(}{)}%




% A pointed bracket shaped arrow

\pgfarrowsdeclare{angle 90}{angle 90}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=5.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke
}%

\pgfarrowsdeclarereversed{angle 90 reversed}{angle 90 reversed}{angle 90}{angle 90}%


\pgfarrowsdeclare{angle 60}{angle 60}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfusepathqstroke
}%

\pgfarrowsdeclarereversed{angle 60 reversed}{angle 60 reversed}{angle 60}{angle 60}%



\pgfarrowsdeclare{angle 45}{angle 45}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfusepathqstroke
}%

\pgfarrowsdeclarereversed{angle 45 reversed}{angle 45 reversed}{angle 45}{angle 45}%



% A dot shaped arrow

\pgfarrowsdeclare{*}{*}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfutil@tempdimb=7.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=1.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{-3\pgfutil@tempdima}{0pt}}{+4.5\pgfutil@tempdima}
  \pgfusepathqfillstroke
}%


% An open dot shaped arrow

\pgfarrowsdeclare{o}{o}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfutil@tempdimb=9\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{4.5\pgfutil@tempdima}{0bp}}{4.5\pgfutil@tempdima}
  \pgfusepathqstroke
}%



% A diamond shaped arrow

\pgfarrowsdeclare{diamond}{diamond}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfutil@tempdimb=13\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=1\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}%

\pgfarrowsdeclare{open diamond}{open diamond}%{{-.5bp}{14.5bp}}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=14\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{14\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}%


% A square shaped arrow
\newdimen\arrowsize
\pgfarrowsdeclare{square}{square}
{
 \arrowsize=0.4pt
 \advance\arrowsize by.275\pgflinewidth%
 \pgfarrowsleftextend{-7\arrowsize-.5\pgflinewidth}
 \advance\arrowsize by.5\pgflinewidth
 \pgfarrowsrightextend{+\arrowsize}
}
{
 \arrowsize=0.4pt
 \advance\arrowsize by.275\pgflinewidth%
 \pgfsetdash{}{+0pt}
 \pgfsetroundjoin
 \pgfpathmoveto{\pgfqpoint{1\arrowsize}{4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{-7\arrowsize}{4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{-7\arrowsize}{-4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{1\arrowsize}{-4\arrowsize}}
 \pgfpathclose
 \pgfusepathqfillstroke
}%
% A open square shaped arrow

\pgfarrowsdeclare{open square}{open square}%{{-.5bp}{8.5bp}}
{
 \arrowsize=0.4pt
 \advance\arrowsize by.275\pgflinewidth%
 \pgfarrowsleftextend{+-.5\pgflinewidth}
 \advance\arrowsize by7\arrowsize
 \advance\arrowsize by.5\pgflinewidth
 \pgfarrowsrightextend{+\arrowsize}
}
{
 \arrowsize=0.4pt
 \advance\arrowsize by.275\pgflinewidth%
 \pgfsetdash{}{+0pt}
 \pgfsetroundjoin
 \pgfpathmoveto{\pgfqpoint{8\arrowsize}{4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{0\arrowsize}{4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{0\arrowsize}{-4\arrowsize}}
 \pgfpathlineto{\pgfqpoint{8\arrowsize}{-4\arrowsize}}
 \pgfpathclose
 \pgfusepathqstroke
}%



% A triangle shaped arrow

\pgfarrowsdeclare{triangle 90}{triangle 90}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=5.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}%

\pgfarrowsdeclarereversed{triangle 90 reversed}{triangle 90 reversed}{triangle 90}{triangle 90}%


\pgfarrowsdeclare{triangle 60}{triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}%

\pgfarrowsdeclarereversed{triangle 60 reversed}{triangle 60 reversed}{triangle 60}{triangle 60}%




\pgfarrowsdeclare{triangle 45}{triangle 45}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}%

\pgfarrowsdeclarereversed{triangle 45 reversed}{triangle 45 reversed}{triangle 45}{triangle 45}%




\pgfarrowsdeclare{open triangle 90}{open triangle 90}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}%

\pgfarrowsdeclare{open triangle 90 reversed}{open triangle 90 reversed}%
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.707\pgflinewidth}
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}%



\pgfarrowsdeclare{open triangle 60}{open triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=7.794\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}%



\pgfarrowsdeclare{open triangle 60 reversed}{open triangle 60 reversed}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgflinewidth}
  \pgfutil@tempdimb=7.794\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpointpolar{30}{9\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpointpolar{-30}{9\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}%



\pgfarrowsdeclare{open triangle 45}{open triangle 45}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=9.205\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}%



\pgfarrowsdeclare{open triangle 45 reversed}{open triangle 45 reversed}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-1.28\pgflinewidth}
  \pgfutil@tempdimb=9.205\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpointpolar{23}{10\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpointpolar{-23}{10\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}%



% A less fleshy variant of LaTeX's ordinal arrow type

\pgfarrowsdeclare{latex'}{latex'}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-4\pgfutil@tempdima}
  \pgfarrowsrightextend{+6\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfill
}%

\pgfarrowsdeclarereversed{latex' reversed}{latex' reversed}{latex'}{latex'}%


% A rounded variant of the stealth arrow

\pgfarrowsdeclare{stealth'}{stealth'}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=2\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-6\pgfutil@tempdima}{3.25\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-3\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-6\pgfutil@tempdima}{-3.25\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-3\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{-.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}%

\pgfarrowsdeclarereversed{stealth' reversed}{stealth' reversed}{stealth'}{stealth'}%



% The two half of the $\to$ arrow

\pgfarrowsdeclare{left to}{left to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0.55\pgfutil@tempdima}{-0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  \pgfusepathqstroke
}%


\pgfarrowsdeclare{right to}{right to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0.55\pgfutil@tempdima}{0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0pt}{0.125\pgflinewidth}}
  \pgfusepathqstroke
}%



% The halfs of the $\to$ arrow reversed

\pgfarrowsdeclare{left to reversed}{left to reversed}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}%

\pgfarrowsdeclare{right to reversed}{right to reversed}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}%



% A left hook

\pgfarrowsdeclare{left hook}{left hook}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}%

\pgfarrowsdeclarereversed{left hook reversed}{left hook reversed}{left hook}{left hook}%



% A right hook

\pgfarrowsdeclare{right hook}{right hook}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}%

\pgfarrowsdeclarereversed{right hook reversed}{right hook reversed}{right hook}{right hook}%


% Hooks in both directions

\pgfarrowsdeclare{hooks}{hooks}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathmoveto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}%

\pgfarrowsdeclarereversed{hooks reversed}{hooks reversed}{hooks}{hooks}%


% An arrow that looks like a serif of the computer modern font

\pgfarrowsdeclare{serif cm}{serif cm}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgfarrowsleftextend{+-.75\pgfutil@tempdima}
  \pgfarrowsrightextend{+.04\pgflinewidth}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgftransformxshift{.04\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{-.75\pgfutil@tempdima}{.5\pgflinewidth}}
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{.5\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{1.95\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{1.95\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.04\pgflinewidth}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.04\pgflinewidth}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-1.95\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-.375\pgfutil@tempdima}{-1.95\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.5\pgflinewidth}}
    {\pgfqpoint{-.75\pgfutil@tempdima}{-.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}%



% Round cap

\pgfarrowsdeclare{round cap}{round cap}
{\pgfarrowsleftextend{+0pt}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}%


% Butt cap

\pgfarrowsdeclare{butt cap}{butt cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+.5\pgflinewidth}}
{
  \pgfsetdash{}{+0pt}
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}%



% 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap}{triangle 90 cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}%


% reversed 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap reversed}{triangle 90 cap reversed}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}%



% fast

\pgfarrowsdeclare{fast cap}{fast cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}%


\pgfarrowsdeclare{fast cap reversed}{fast cap reversed}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}%





% Mathematical arrows


% The arrow tip of an \implies arrow, to be used with an inner line.
%
% Example:
%
% \pgfsetarrow{-implies}
% \pgfsetlinewidth{1.8pt}
% \pgfsetinnerlinewidth{1pt}

\pgfarrowsdeclare{implies}{implies}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgfarrowsrightextend{2.06\pgfutil@tempdima+.5\pgfutil@tempdimb}
  \pgfarrowsleftextend{-1.36\pgfutil@tempdima-.5\pgfutil@tempdimb}
}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgftransformxshift{.06\pgfutil@tempdima}
  \pgfsetlinewidth{\pgfutil@tempdimb}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-1.4\pgfutil@tempdima}{2.65\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-0.75\pgfutil@tempdima}{1.25\pgfutil@tempdima}}
  {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
  {\pgfpoint{2\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
  {\pgfpoint{-.75\pgfutil@tempdima}{-1.25\pgfutil@tempdima}}
  {\pgfpoint{-1.4\pgfutil@tempdima}{-2.65\pgfutil@tempdima}}
  \pgfusepathqstroke
}%



\endinput


==> pgflibraryarrows.meta.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryarrows.meta.code.tex}



%
%
% Meta keys
%
%


\newdimen\pgfarrowinset
\newdimen\pgfarrowlength
\newdimen\pgfarrowwidth
\newdimen\pgfarrowlinewidth
\newif\ifpgfarrowroundcap
\newif\ifpgfarrowroundjoin

\pgfarrowsaddtolengthscalelist\pgfarrowlength
\pgfarrowsaddtolengthscalelist\pgfarrowinset
\pgfarrowsaddtowidthscalelist\pgfarrowwidth


\pgfkeys{
  /pgf/arrow keys/.cd,
  length/.code={%
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\pgfarrowslinewidthdependent\pgfarrowstheparameters\pgfarrowlength\pgf@x}%
  },
  inset/.code={%
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslinewidthdependent\pgfarrowstheparameters\pgfarrowinset\pgf@x}%
  },
  inset'/.code={
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslengthdependent\pgfarrowstheparameters\pgfarrowinset}%
  },
  line width/.code={%
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslinewidthdependent\pgfarrowstheparameters\pgfarrowlinewidth\pgf@x}%
  },
  line width'/.code={
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslengthdependent\pgfarrowstheparameters\pgfarrowlinewidth}%
  },
  width/.code={%
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslinewidthdependent\pgfarrowstheparameters\pgfarrowwidth\pgf@x}%
  },
  width'/.code={%
    \pgfarrowsthreeparameters{#1}%
    \expandafter\pgfarrowsaddtolateoptions\expandafter{\expandafter\pgfarrowslengthdependent\pgfarrowstheparameters\pgfarrowwidth}%
  },
  angle/.code={%
    \pgfarrowsfourparameters{#1}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\pgfarrows@angle@setup\pgfarrowstheparameters}%
  },
  angle'/.code={
    \pgfarrowsaddtolateoptions{\pgfarrows@angle@setup@prime{#1}}%
  },
  %
  line cap/.is choice,
  line cap/butt/.code=\pgfarrowsaddtooptions{\pgfarrowroundcapfalse},
  line cap/round/.code=\pgfarrowsaddtooptions{\pgfarrowroundcaptrue},
  line join/.is choice,
  line join/miter/.code=\pgfarrowsaddtooptions{\pgfarrowroundjoinfalse},
  line join/round/.code=\pgfarrowsaddtooptions{\pgfarrowroundjointrue},
  round/.style={line cap=round,line join=round},
  sharp/.style={line cap=butt,line join=miter},
}%
%
%
% Classification of arrow tips:
%
%
% Barbs
% -----
%
% These arrow tips consisting of stroked lines starting at the tip,
% typically going backward. They cannot be filled, only stroked
%
% A special case are the arrows mimicking the tip at the end of a
% \rightarrow command.
%
%
% Geometric
% ---------
%
% The arrow tips have a geometric form like a triangle or a
% "stealth" fighter or a kite. They can be filled and/or stroked.
%
%
% Caps
% ----
%
% These arrow tips have their width fixed to the line width and
% provide different ways of adding a "cap" to the end of a line. This
% allows one to use more than just the standard "round cap", "butt
% cap" and "rect cap" and, additionally, one can one kind of cap at
% one end and another at the other end.
%
%
% Other
% -----
%
% Special purpose arrow tips.
%



%
%
% Barbs arrow tips
%
%


% An Straight Barb yields a simple angle

\pgfdeclarearrow{
  name = Straight Barb,
  defaults = {
    length = +1.5pt 2,
    width'  = +0pt 2,
    line width = +0pt 1 1,
  },
  setup code = {
    % Compute front miter length:
    \pgfmathdivide@{\pgf@sys@tonumber\pgfarrowlength}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x4\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@xc\pgfmathresult\pgfarrowlinewidth% xc is front miter
    \pgf@xc.5\pgf@xc
    \pgf@xa\pgf@temp@quot\pgfarrowlinewidth% xa is extra harpoon miter
    % Set ends
    \ifpgfarrowroundjoin
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by\pgf@xc\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi}
    \fi
    \pgfarrowssetvisualbackend{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}
    \pgfarrowssetbackend{-.5\pgfarrowlinewidth}
    % harpoon miter correction
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\ifpgfarrowharpoon\advance\pgf@x by.5\pgfarrowlinewidth\fi}
    \else
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \fi
    % The hull:
    \ifpgfarrowroundjoin
      \pgfarrowshullpoint{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else0pt\fi}%
    \else%
      \ifpgfarrowharpoon
        \pgfarrowshullpoint{\pgfarrowlength\advance\pgf@x by\pgf@xc\advance\pgf@x by\pgf@xa}{-.5\pgfarrowlinewidth}%
      \else
        \pgfarrowshullpoint{\pgfarrowlength\advance\pgf@x by\pgf@xc\advance\pgf@x by\pgf@xa}{0pt}%
      \fi%
    \fi
    \pgfarrowsupperhullpoint{.5\pgfarrowlinewidth}{.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}%
    \pgfarrowsupperhullpoint{-.5\pgfarrowlinewidth}{.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}%
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{-.5\pgfarrowlinewidth}{-.5\pgfarrowlinewidth}%
    \fi
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \ifpgfarrowharpoon
      \pgfpathlineto{\pgfqpoint{\pgfarrowlength\advance\pgf@x by\ifpgfarrowreversed\else-\fi\pgfarrowlinewidth}{0pt}}
    \else
      \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \fi
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundjoin j\fi%
    \ifpgfarrowroundcap c\fi%
  },
}%
%
%
% Hooks are barbs that consist of an arc going forward from the line
% end and curving back by a given angle specified using the |arc|
% key.

\pgfkeys{
  /pgf/arrow keys/.cd,
  arc/.code={%
    \pgfmathparse{#1}%
    \expandafter\pgfarrowsaddtooptions\expandafter{\expandafter\def\expandafter\pgfarrowarc\expandafter{\pgfmathresult}}
  }
}%

\def\pgfarrowarc{180}%

\pgfdeclarearrow{
  name = Hooks,
  defaults = {
    length = +0.75pt 1.25,
    width'  = +0pt 4 -1,
    line width = +0pt 1 1,
  },
  setup code = {
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{.5\pgfarrowlength}{-.5\pgfarrowlinewidth}
      \pgfarrowshullpoint{\pgfarrowlength}{-.5\pgfarrowlinewidth\advance\pgf@y by.125\pgfarrowwidth}
    \fi
    \ifdim\pgfarrowarc pt<90.1pt
      \pgfarrowsupperhullpoint{0pt}{.25\pgfarrowwidth\ifpgfarrowroundcap\else\advance\pgf@y by-.25\pgfarrowlinewidth\fi}
      \pgfarrowsupperhullpoint{\pgfarrowlength}{.25\pgfarrowwidth\ifpgfarrowroundcap\else\advance\pgf@y by-.25\pgfarrowlinewidth\fi}
    \else%
      \pgfarrowsupperhullpoint{\pgfarrowlength}{.375\pgfarrowwidth}
      \pgfarrowsupperhullpoint{.5\pgfarrowlength}{.5\pgfarrowwidth}
      \ifdim\pgfarrowarc pt>180pt
        \pgfarrowsupperhullpoint{-.5\pgfarrowlength}{.5\pgfarrowwidth}
        \pgfarrowsupperhullpoint{-\pgfarrowlength}{.375\pgfarrowwidth}
        \pgfarrowsupperhullpoint{-\pgfarrowlength}{.25\pgfarrowwidth}
      \else
        \pgfarrowsupperhullpoint{\ifpgfarrowroundcap-.5\pgfarrowlinewidth\else0pt\fi}{.25\pgfarrowwidth}
        \pgfarrowsupperhullpoint{\ifpgfarrowroundcap-.5\pgfarrowlinewidth\else0pt\fi}{.5\pgfarrowwidth}
      \fi
    \fi
    % Adjust width and length: Take line thickness into account:
    \advance\pgfarrowlength by-.5\pgfarrowlinewidth
    \advance\pgfarrowwidth by-\pgfarrowlinewidth
    \ifpgfarrowreversed
      \ifpgfarrowroundjoin
        \pgfarrowssetbackend{-.5\pgfarrowlinewidth}
      \fi
    \fi
    % There are four different intervals for the values of
    % \pgfarrowsarc that give rise to four different settings of tip
    % ends and so on:
    %
    % Case 1: 0 <= Angle < 90
    %
    \ifdim\pgfarrowarc pt<90pt%
      % Tip end is given by sin(pgfarrowarc)*length
      \pgfmathsin@{\pgfarrowarc}
      \pgfarrowssettipend{\pgfmathresult\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}%
    \else\ifdim\pgfarrowarc pt<180pt%
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}%
      \ifpgfarrowroundcap\pgfarrowssetbackend{-.5\pgfarrowlinewidth}\fi%
    \else\ifdim\pgfarrowarc pt<270pt%
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}%
      \ifdim\pgfarrowarc pt>180pt
        % Back end is given by sin(pgfarrowarc)*length
        \pgfmathsin@{\pgfarrowarc}
        \pgfarrowssetbackend{\pgfmathresult\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}%
      \else
        \ifpgfarrowroundcap\pgfarrowssetbackend{-.5\pgfarrowlinewidth}\fi%
      \fi%
    \else%
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by.5\pgfarrowlinewidth}%
      \pgfarrowssetbackend{-\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}%
    \fi\fi\fi%
    \ifpgfarrowreversed
      \pgfarrowssetlineend{.5\pgfarrowlinewidth}
    \else%
      \ifpgfarrowharpoon
        \pgfarrowssetlineend{0pt}
      \else
        \pgfarrowssetlineend{.25\pgfarrowlinewidth}
      \fi
    \fi
    % Adjust arc:
    \pgf@x\pgfarrowarc pt%
    \advance\pgf@x by-90pt%
    \edef\pgfarrowarc{\pgf@sys@tonumber\pgf@x}%
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
    \pgfarrowssave\pgfarrowarc
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    {%
      \pgftransformxscale{+\pgfarrowlength}
      \pgftransformyscale{+.25\pgfarrowwidth}
      \pgfpathmoveto{\pgfpointpolar{+\pgfarrowarc}{+1pt}\advance\pgf@y by1pt}
      \pgfpatharc{\pgfarrowarc}{+-90}{+1pt}
      \ifpgfarrowharpoon
      \else
        \pgfpatharc{+90}{+-\pgfarrowarc}{+1pt}
      \fi
    }
    \ifpgfarrowharpoon\ifpgfarrowreversed
    \pgfpathlineto{\pgfqpoint{\pgflinewidth}{0pt}}
    \fi\fi
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \pgfarrowarc,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundjoin j\fi%
    \ifpgfarrowroundcap c\fi%
  },
}%


\pgfdeclarearrow{
  name = Arc Barb,
  defaults = {
    length = +1.5pt 2,
    width'  = +0pt 2,
    line width = +0pt 1 1,
  },
  setup code = {
    % Adjust arc:
    \pgf@x\pgfarrowarc pt%
    \pgf@x.5\pgf@x%
    \edef\pgfarrowarc{\pgf@sys@tonumber\pgf@x}%
    % The tips:
    \pgfarrowssettipend{\pgfarrowlength}
    \pgfarrowssetvisualbackend{\pgfarrowlength}
    \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    % The hull:
    \pgfarrowsupperhullpoint{\pgfarrowlength}{.25\pgfarrowwidth}
    \ifpgfarrowharpoon\pgfarrowshullpoint{\pgfarrowlength}{-.5\pgflinewidth}\fi
    \pgfmathsincos@{\pgfarrowarc}%
    \pgf@xa.5\pgfarrowwidth%
    \pgfarrowsupperhullpoint{\pgfmathresultx\pgfarrowlength}{\pgfmathresulty\pgf@xa}
    \ifdim\pgfarrowarc pt>60pt
      \pgfarrowsupperhullpoint{.5\pgfarrowlength}{\ifdim\pgfarrowarc pt<90pt\pgfmathresulty\pgf@xa\else.5\pgfarrowwidth\fi}
    \fi
    \ifdim\pgfarrowarc pt>90pt
      \ifdim\pgfarrowarc pt<120pt
        \pgfarrowsupperhullpoint{\pgfmathresultx\pgfarrowlength}{.5\pgfarrowwidth}
      \else
        \pgfarrowsupperhullpoint{-.5\pgfarrowlength}{.5\pgfarrowwidth}
        \ifdim\pgfarrowarc pt>150pt
          \pgfarrowsupperhullpoint{-\pgfarrowlength}{.25\pgfarrowwidth}
        \fi
      \fi
    \fi
    \pgfutil@tempswafalse
    \ifdim\pgfarrowarc pt<90pt
      \pgfutil@tempswatrue
    \fi
    \ifpgfarrowharpoon
      \pgfutil@tempswatrue
    \fi
    \ifpgfutil@tempswa
      \pgf@xa.5\pgfarrowwidth\advance\pgf@xa by-\pgfarrowlinewidth%
      \pgf@ya\pgfarrowlength\advance\pgf@ya by-\pgfarrowlinewidth%
      \pgfarrowsupperhullpoint{\pgfmathresultx\pgf@ya}{\pgfmathresulty\pgf@xa}
    \fi
    % Compute back end
    \ifpgfarrowroundcap
      \pgf@y\pgfarrowlength
      \advance\pgf@y by-.5\pgfarrowlinewidth
      \pgf@x\pgfmathresultx\pgf@y%
    \else
      \ifdim\pgfarrowarc pt<90pt
        \pgf@y\pgfarrowlength
        \advance\pgf@y by-\pgfarrowlinewidth
        \pgf@x\pgfmathresultx\pgf@y%
      \else
        \pgf@x\pgfmathresultx\pgfarrowlength%
      \fi
    \fi
    \pgfarrowssetbackend{\pgf@x\ifpgfarrowroundcap\advance\pgf@x by-.5\pgfarrowlinewidth\fi}
    % Adjust width and length: Take line thickness into account:
    \advance\pgfarrowlength by-.5\pgfarrowlinewidth
    \advance\pgfarrowwidth by-\pgfarrowlinewidth
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
    \pgfarrowssave\pgfarrowarc
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    {%
      \pgftransformxscale{+\pgfarrowlength}
      \pgftransformyscale{+.5\pgfarrowwidth}
      \pgfpathmoveto{\pgfpointpolar{+\pgfarrowarc}{+1pt}}
      \ifpgfarrowharpoon
        \pgfpatharc{+\pgfarrowarc}{0pt}{+1pt}
      \else
        \pgfpatharc{+\pgfarrowarc}{+-\pgfarrowarc}{+1pt}
      \fi
    }
    \ifpgfarrowharpoon
      \pgfpathlineto{\pgfqpoint{\pgfarrowlength\advance\pgf@x by\ifpgfarrowreversed\else-\fi.5\pgflinewidth}{0pt}}
    \fi
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \pgfarrowarc,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundcap c\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%



% Tee Barb are barb arrows heads that look like a T

\pgfdeclarearrow{
  name = Tee Barb,
  defaults = {
    length = +1.5pt 2,
    width = +3pt 4,
    inset' = +0pt .5,
    line width = +0pt 1 1,
  },
  bending mode=polar,
  setup code = {
    % Two useful numbers...
    \pgfutil@tempswafalse%
    \pgfutil@tempswbfalse%
    \pgfutil@tempdima\pgfarrowlength\advance\pgfutil@tempdima by-\pgfarrowinset\ifdim\pgfutil@tempdima<.5\pgfarrowlinewidth\pgfutil@tempdima.5\pgfarrowlinewidth\pgfutil@tempswatrue\fi%
    \pgfutil@tempdimb-\pgfarrowinset\ifdim\pgfutil@tempdimb>-.5\pgfarrowlinewidth\pgfutil@tempdimb-.5\pgfarrowlinewidth\pgfutil@tempswbtrue\fi
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowwidth
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
    % Infos:
    \pgfarrowssettipend{\pgfutil@tempdima\ifpgfarrowroundcap\ifpgfutil@tempswa\else\advance\pgf@x by.5\pgfarrowlinewidth\fi\fi}
    \pgfarrowssetvisualbackend{.5\pgfarrowlinewidth}
    \pgfarrowssetbackend{\pgfutil@tempdimb\ifpgfarrowroundcap\ifpgfutil@tempswb\else\advance\pgf@x by-.5\pgfarrowlinewidth\fi\fi}
    \pgfarrowssetlineend{\ifpgfarrowreversed\else-\fi.25\pgfarrowlinewidth}%
    % The hull:
    \pgfarrowsupperhullpoint{\pgfutil@tempdima\ifpgfarrowroundcap\ifpgfutil@tempswa\else\advance\pgf@x by.5\pgfarrowlinewidth\fi\fi}{.5\pgfarrowwidth}%
    \pgfarrowsupperhullpoint{\pgfutil@tempdimb\ifpgfarrowroundcap\ifpgfutil@tempswb\else\advance\pgf@x by-.5\pgfarrowlinewidth\fi\fi}{.5\pgfarrowwidth}%
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{.5\pgfarrowlinewidth}{-.5\pgfarrowlinewidth}%
    \fi
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \pgf@yc\pgflinewidth% save...
    \ifdim\pgflinewidth=\pgfarrowlinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \pgf@x\pgfutil@tempdima\advance\pgf@x by-.5\pgfarrowlinewidth%
    \pgf@y\pgfutil@tempdimb\advance\pgf@y by.5\pgfarrowlinewidth%
    % Case 1: No bar atop the I:
    \ifdim\pgf@x=\pgf@y%
      \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
      \pgfpathlineto{\pgfqpoint{0pt}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else-.5\pgfarrowwidth\fi}}
    \else
      % Case 2: Bar, but only in one direction:
      \ifdim\pgfutil@tempdima=.5\pgfarrowlinewidth%
        \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdimb}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
        \pgfpathlineto{\pgfqpoint{0pt}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
        \ifpgfarrowharpoon%
          \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgf@yc}}%
        \else%
          \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}}
          \pgfpathlineto{\pgfqpoint{\pgfutil@tempdimb}{-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}}
        \fi
      \else% Case 3: Complete I:
        \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdimb}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
        \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
        \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
        \ifpgfarrowharpoon%
          \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgf@yc}}%
        \else%
          \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}}
          \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdimb}{-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}}
          \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth}}
        \fi
      \fi
    \fi
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowwidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowinset,%
    \the\pgfarrowlinewidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundjoin j\fi%
    \ifpgfarrowroundcap c\fi%
  },
}%


% Math barbs that resemble \rightarrow in different fonts:



% The original default arrow head used in TikZ. It is modeled on an
% old version of the \rightarrow head of the *old* Computer Modern
% fonts.

\pgfdeclarearrow{
  name = Classical TikZ Rightarrow,
  defaults = {
    length  = +1.05pt 1.925,
    width'  = +0pt 1.9237,
    line width = 0pt 0.8 1,
    round
  },
  setup code =
  {
    \ifpgfarrowharpoon\pgfarrowroundjointrue\fi
    % inner length:
    \pgfutil@tempdima\pgfarrowlength
    \advance\pgfutil@tempdima by-\pgfarrowlinewidth
    \pgfutil@tempdimb\pgfarrowwidth
    \advance\pgfutil@tempdimb by-\pgfarrowlinewidth
    \ifpgfarrowroundjoin%
    \else%
      \pgfmathdivide@{\pgf@sys@tonumber\pgfutil@tempdima}{\pgf@sys@tonumber\pgfutil@tempdimb}%
      \let\pgf@temp@quot\pgfmathresult%
      \pgf@x\pgfmathresult pt%
      \pgf@x\pgfmathresult\pgf@x%
      \pgf@x40.96\pgf@x%
      \advance\pgf@x by1pt%  \pgflinewidth^2 + (6.4 \pgftempdim@a / \pgfutil@tempdimb) \pgflinewidth^2
      \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
      \pgf@xc\pgfmathresult\pgfarrowlinewidth% xc is front miter
      \pgf@xc.5\pgf@xc
    \fi%
     % The following are needed in the code:
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
    % The extend:
    \pgfarrowssettipend{\pgfutil@tempdima\ifpgfarrowroundjoin\advance\pgf@x by.5\pgfarrowlinewidth\else\advance\pgf@x by\pgf@xc\fi}%
    \pgfarrowssetvisualbackend{\pgfutil@tempdima\advance\pgf@x by.5\pgfarrowlinewidth}%
    \ifpgfarrowreversed%
      \ifpgfarrowharpoon%
        % A reversed arrow needs a slightly different line end:
        \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by.5\pgflinewidth}%
      \else%
        % A reversed arrow needs a slightly different line end:
        \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by-.25\pgflinewidth}%
      \fi%
    \else%
      \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by-.6\pgflinewidth}%
    \fi%
    \pgfarrowssetbackend{-.5\pgfarrowlinewidth}%
    % The hull:
    %  Tip:
    \pgfarrowshullpoint{\pgfutil@tempdima\ifpgfarrowroundjoin\advance\pgf@x by.5\pgfarrowlinewidth\else\advance\pgf@x by\pgf@xc\fi}{.5\pgfarrowlinewidth}%
    \pgfarrowshullpoint{\pgfutil@tempdima\ifpgfarrowroundjoin\advance\pgf@x by.5\pgfarrowlinewidth\else\advance\pgf@x by\pgf@xc\fi}{-.5\pgfarrowlinewidth}%
    %  Upper end:
    \pgfarrowsupperhullpoint{.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by.5\pgfarrowlinewidth}%
    \pgfarrowsupperhullpoint{-.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by.5\pgfarrowlinewidth}%
    %  Lower end:
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{\pgfutil@tempdima\advance\pgf@x by-\pgflinewidth}{-.5\pgflinewidth}%
      \pgfarrowshullpoint{-.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by-.5\pgflinewidth}%
    \fi
  },
  drawing code =
  {
    \pgfsetdash{}{+0pt}
    \edef\pgf@orig@linewidth{\the\pgflinewidth}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \ifpgfarrowharpoon\pgfarrowroundjointrue\fi
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \pgfpathmoveto
          {\pgfqpoint{0pt}{.5\pgfutil@tempdimb}}
    \ifpgfarrowharpoon
      \pgf@arrows@old@tikz@harpoon
    \else
      \pgfpathcurveto
          {\pgfqpoint{0.066666\pgfutil@tempdima}{0.3125\pgfutil@tempdimb}}
          {\pgfqpoint{.8\pgfutil@tempdima}{0.03125\pgfutil@tempdimb}}
          {\pgfqpoint{\pgfutil@tempdima}{0pt}}
      \pgfpathcurveto
          {\pgfqpoint{.8\pgfutil@tempdima}{-.03125\pgfutil@tempdimb}}
          {\pgfqpoint{0.066666\pgfutil@tempdima}{-.3125\pgfutil@tempdimb}}
          {\pgfqpoint{0pt}{-.5\pgfutil@tempdimb}}
      \pgfsetlinewidth{+\pgfarrowlinewidth}
      \pgfusepathqstroke
    \fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundjoin j\fi%
    \ifpgfarrowroundcap c\fi%
  },
}%

\def\pgf@arrows@old@tikz@harpoon{
  \ifpgfarrowreversed
    \pgf@arrows@old@tikz@harpoon@reversed
  \else
    \pgfpathcurveto
      {\pgfqpoint{0.066666\pgfutil@tempdima}{0.3125\pgfutil@tempdimb}}
      {\pgfqpoint{.8\pgfutil@tempdima}{0.03125\pgfutil@tempdimb}}
      {\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathcurveto
      {\pgfqpoint{0.95\pgfutil@tempdima}{-0.125\pgflinewidth}}
      {\pgfqpoint{0.933333\pgfutil@tempdima}{-0.125\pgflinewidth}}
      {\pgfqpoint{0.933333\pgfutil@tempdima}{-0.125\pgflinewidth}}
    \pgfpathlineto
      {\pgfqpoint{0.8\pgfutil@tempdima\advance\pgf@x by-.5\pgflinewidth}{-0.125\pgflinewidth}}
    \pgfusepathqstroke
  \fi
}%
\def\pgf@arrows@old@tikz@harpoon@reversed{
    \pgfpathcurveto
      {\pgfqpoint{0.066666\pgfutil@tempdima}{0.3125\pgfutil@tempdimb}}
      {\pgfqpoint{.8\pgfutil@tempdima}{0.03125\pgfutil@tempdimb}}
      {\pgfqpoint{\pgfutil@tempdima}{0.125\pgflinewidth}}
    \pgfpathmoveto
      {\pgfqpoint{0pt}{.5\pgfutil@tempdimb}}
    \pgfpathcurveto
      {\pgfqpoint{0.066666\pgfutil@tempdima}{0.3125\pgfutil@tempdimb}}
      {\pgfqpoint{.8\pgfutil@tempdima}{0.03125\pgfutil@tempdimb}}
      {\pgfqpoint{\pgfutil@tempdima}{-0.125\pgflinewidth}}
    \pgfusepathqstroke
    \pgfsetlinewidth{+\pgf@orig@linewidth}
    \pgfsetroundcap
    \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdima\advance\pgf@x by0.6\pgflinewidth}{0pt}}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfusepathqstroke
}%


% An approximation to the new (past 1992) Computer Modern math arrow
% heads. This would be a better version of "to", so consider saying
% to/.tips=Computer Modern Rightarrow

\pgfdeclarearrow{
  name = Computer Modern Rightarrow,
  defaults = {
    length = +1.6pt 2.2, % 0pt 5.2
    width' = +0pt 2.096774,
    line width = 0pt 1 1,
    round
  },
  setup code =
  {
    % inner length:
    \pgfutil@tempdima\pgfarrowlength
    \advance\pgfutil@tempdima by-\pgfarrowlinewidth
    \pgfutil@tempdimb\pgfarrowwidth
    \advance\pgfutil@tempdimb by-\pgfarrowlinewidth
    % The following are needed in the code:
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
    % Front miter:
    \ifpgfarrowroundjoin%
    \else%
      \pgfmathdivide@{\pgf@sys@tonumber\pgfutil@tempdima}{\pgf@sys@tonumber\pgfutil@tempdimb}%
      \let\pgf@temp@quot\pgfmathresult%
      \pgf@x\pgfmathresult pt%
      \pgf@x\pgfmathresult\pgf@x%
      \pgf@x49.44662\pgf@x%
      \advance\pgf@x by1pt%  \pgfarrowlinewidth^2 + (0.41019/0.0583333 \pgftempdim@a / \pgfutil@tempdimb) \pgfarrowlinewidth^2
      \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
      \pgf@xc\pgfmathresult\pgfarrowlinewidth% xc is front miter
      \pgf@xc.5\pgf@xc
      \pgf@xa\pgf@temp@quot\pgfarrowlinewidth% xa is extra harpoon miter
      \pgf@xa3.51591\pgf@xa% xa is extra harpoon miter
    \fi%
    % The extend:
    \pgfarrowssettipend{\ifpgfarrowroundjoin.5\pgfarrowlinewidth\else\pgf@xc\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi\fi}%
    \pgfarrowssetvisualbackend{.5\pgfarrowlinewidth}%
    \ifpgfarrowreversed%
      \ifpgfarrowharpoon%
        \pgfarrowssetlineend{.5\pgfarrowlinewidth}%
      \else%
        \pgfarrowssetlineend{-.5\pgfarrowlinewidth}%
      \fi%
    \else%
      \pgfarrowssetlineend{-.5\pgfarrowlinewidth}%
    \fi%
    \pgfarrowssetbackend{-\pgfutil@tempdima\advance\pgf@x by-.5\pgfarrowlinewidth}%
    % The hull:
    %  Tip:
    \pgfarrowshullpoint{\ifpgfarrowroundjoin.5\pgfarrowlinewidth\else\pgf@xc\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi\fi}{.5\pgfarrowlinewidth}%
    \pgfarrowshullpoint{\ifpgfarrowroundjoin.5\pgfarrowlinewidth\else\pgf@xc\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi\fi}{-.5\pgfarrowlinewidth}%
    %  Upper end:
    \pgfarrowsupperhullpoint{-\pgfutil@tempdima\advance\pgf@x by.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by.5\pgfarrowlinewidth}%
    \pgfarrowsupperhullpoint{-\pgfutil@tempdima\advance\pgf@x by-.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by.5\pgfarrowlinewidth}%
    %  Lower end:
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{-\pgfarrowlinewidth}{-.5\pgfarrowlinewidth}%
      \pgfarrowshullpoint{-\pgfutil@tempdima\advance\pgf@x by-.5\pgfarrowlinewidth}{.5\pgfutil@tempdimb\advance\pgf@y by-.5\pgfarrowlinewidth}%
    \fi
  },
  drawing code =
  {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto
        {\pgfqpoint{-\pgfutil@tempdima}{.5\pgfutil@tempdimb}}
    \pgfpathcurveto
        {\pgfqpoint{-0.81731\pgfutil@tempdima}{.2\pgfutil@tempdimb}}
        {\pgfqpoint{-0.41019\pgfutil@tempdima}{0.05833333\pgfutil@tempdimb}}
        {\pgfpointorigin}
    \ifpgfarrowharpoon
      \pgfpathlineto
        {\pgfqpoint{\ifpgfarrowreversed.5\else-\fi\pgfarrowlinewidth}{0pt}}
    \else
      \pgfpathcurveto
        {\pgfqpoint{-0.41019\pgfutil@tempdima}{-0.05833333\pgfutil@tempdimb}}
        {\pgfqpoint{-0.81731\pgfutil@tempdima}{-.2\pgfutil@tempdimb}}
        {\pgfqpoint{-\pgfutil@tempdima}{-.5\pgfutil@tempdimb}}
    \fi
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi
    \ifpgfarrowharpoon r\fi
    \ifpgfarrowroundjoin j\fi%
    \ifpgfarrowroundcap c\fi%
  },
}%



% The arrow tip of an \implies arrow, to be used with an inner
% line. Cannot be configured otherwise.

\pgfdeclarearrow{
  name = Implies,
  setup code = {
    \pgf@xa\pgfinnerlinewidth
    \pgfutil@tempdima.25\pgflinewidth
    \advance\pgfutil@tempdima by.25\pgf@xa%
    \pgfutil@tempdimb.5\pgflinewidth
    \advance\pgfutil@tempdimb by-.5\pgf@xa%
    \pgfarrowssettipend{2.06\pgfutil@tempdima\advance\pgf@x by.5\pgfutil@tempdimb}
    \pgfarrowssetbackend{-1.36\pgfutil@tempdima\advance\pgf@x by.5\pgfutil@tempdimb}
    \pgfarrowsupperhullpoint{-1.4\pgfutil@tempdima}{2.8\pgfutil@tempdima}
    \pgfarrowsupperhullpoint{2\pgfutil@tempdima}{.5\pgfutil@tempdimb}
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
  },
  drawing code = {
    \pgftransformxshift{.06\pgfutil@tempdima}
    \pgfsetlinewidth{\pgfutil@tempdimb}
    \pgfsetdash{}{+0pt}
    \pgfsetroundcap
    \pgfsetroundjoin
    \pgfpathmoveto{\pgfpoint{-1.4\pgfutil@tempdima}{2.65\pgfutil@tempdima}}
    \pgfpathcurveto
    {\pgfpoint{-0.75\pgfutil@tempdima}{1.25\pgfutil@tempdima}}
    {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
    {\pgfpoint{2\pgfutil@tempdima}{0pt}}
    \pgfpathcurveto
    {\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
    {\pgfpoint{-.75\pgfutil@tempdima}{-1.25\pgfutil@tempdima}}
    {\pgfpoint{-1.4\pgfutil@tempdima}{-2.65\pgfutil@tempdima}}
    \pgfusepathqstroke
  },
  parameters = {\the\pgfarrowlength}
}%




%
%
% Geometric arrow tips
%
%


% Generic "latex-like" arrow tip. This is the basic arrow tip used in
% latex's picture environment. You can configure its length and width.

\pgfdeclarearrow{
  name = Latex,
  defaults = {
    length  = +3pt 4.5 .8,% +2.8pt 3 0.8,
    width' = +0pt .75,
    line width = +0pt 1 1,
  },
  setup code = {
    % Cap the line width at 1/4th distance from inset to tip
    \pgf@x.2\pgfarrowlength
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    \pgfarrowssavethe\pgfarrowlinewidth%
    % Compute front miter length:
    \pgfmathdivide@{\pgf@sys@tonumber\pgfarrowlength}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x9\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@xc\pgfmathresult\pgfarrowlinewidth%
    \pgf@xa\pgf@temp@quot\pgfarrowlinewidth
    % Inner length (pgfutil@tempdima) is now arrowlength - front miter
    % - 0.5 linewidth (back thickness)
    \pgfutil@tempdima\pgfarrowlength%
    \advance\pgfutil@tempdima by-.5\pgf@xc%
    \advance\pgfutil@tempdima by-.5\pgfarrowlinewidth%
    % harpoon miter correction
    \pgfarrowssetbackend{-.5\pgfarrowlinewidth}
    \ifpgfarrowreversed
      \ifdim\pgfinnerlinewidth>0pt
        \pgfarrowssetlineend{0pt}
      \else
        \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by-.5\pgflinewidth}
      \fi
    \else
      \pgfarrowssetlineend{0pt}
    \fi
    \ifpgfarrowroundjoin
      \pgfarrowssettipend{\pgfutil@tempdima\advance\pgf@x by.5\pgfarrowlinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth\ifpgfarrowharpoon\advance\pgf@x  by1.5\pgf@xa\fi}
    \fi
    % The following are needed in the code:
    \pgfarrowssavethe\pgfutil@tempdima
    % Now, compute back tip miter limit:
    \pgf@process{\pgfpointnormalised{\pgfqpoint{.3\pgfarrowlength}{.2333333\pgfarrowwidth}}}%
    \advance\pgf@y by1pt%
    \pgf@yc\pgf@y\pgf@xc\pgf@x%
    \pgfmathdivide@{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@xc}%
    \pgfutil@tempdimb\pgfmathresult\pgfarrowlinewidth%
    \pgfutil@tempdimb-.5\pgfutil@tempdimb%
    \advance\pgfutil@tempdimb by.5\pgfarrowwidth%
    \pgfarrowssavethe\pgfutil@tempdimb%
    % The hull:
    \pgfarrowshullpoint{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth\ifpgfarrowroundjoin\else\ifpgfarrowharpoon\advance\pgf@x  by1.5\pgf@xa\fi\fi}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else0pt\fi}%
    \pgfarrowshullpoint{-.5\pgfarrowlinewidth}{.5\pgfarrowwidth\ifpgfarrowharpoon\advance\pgf@y by-.5\pgfarrowlinewidth\fi}%
    \pgfarrowshullpoint{-.5\pgfarrowlinewidth}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else-.5\pgfarrowwidth\fi}%
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto    {\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathcurveto   {\pgfqpoint{.877192\pgfutil@tempdima}{.077922\pgfutil@tempdimb}}
                      {\pgfqpoint{.337381\pgfutil@tempdima}{.519480\pgfutil@tempdimb}}
                      {\pgfqpoint{0pt}{\pgfutil@tempdimb}}
    \ifpgfarrowharpoon
      \pgfpathlineto  {\pgfpointorigin}
    \else
      \pgfpathlineto  {\pgfqpoint{0pt}{-\pgfutil@tempdimb}}
      \pgfpathcurveto {\pgfqpoint{.337381\pgfutil@tempdima}{-.519480\pgfutil@tempdimb}}
                      {\pgfqpoint{.877192\pgfutil@tempdima}{-.077922\pgfutil@tempdimb}}
                      {\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \fi
    \pgfpathclose
    \ifpgfarrowopen\pgfusepathqstroke\else\ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi\fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowopen o\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%



% A basic stealth-fighter-like pointed arrow

\pgfdeclarearrow{
  name = Stealth,
  defaults = {
    length  = +3pt 4.5 .8,
    width'  = +0pt .75,
    inset'  = +0pt 0.325,
    line width = +0pt 1 1,
  },
  setup code = {
    % Cap the line width at 1/4th distance from inset to tip
    \pgf@x\pgfarrowlength
    \advance\pgf@x by-\pgfarrowinset
    \pgf@x.25\pgf@x
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    % Compute front miter length:
    \pgfmathdivide@{\pgf@sys@tonumber\pgfarrowlength}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x4\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@xc\pgfmathresult\pgfarrowlinewidth% xc is front miter
    \pgf@xc.5\pgf@xc
    \pgf@xa\pgf@temp@quot\pgfarrowlinewidth% xa is extra harpoon miter
    % Compute back miter length:
    \pgf@ya.5\pgfarrowwidth%
    \csname pgfmathatan2@\endcsname{\pgfmath@tonumber\pgfarrowlength}{\pgfmath@tonumber\pgf@ya}%
    \pgf@yb\pgfmathresult pt%
    \csname pgfmathatan2@\endcsname{\pgfmath@tonumber\pgfarrowinset}{\pgfmath@tonumber\pgf@ya}%
    \pgf@ya\pgfmathresult pt%
    \advance\pgf@yb by-\pgf@ya%
    \pgf@yb.5\pgf@yb% half angle in yb
    \pgfmathtan@{\pgf@sys@tonumber\pgf@yb}%
    \pgfmathreciprocal@{\pgfmathresult}%
    \pgf@yc\pgfmathresult\pgfarrowlinewidth%
    \pgf@yc.5\pgf@yc%
    \advance\pgf@ya by\pgf@yb%
    \pgfmathsincos@{\pgf@sys@tonumber\pgf@ya}%
    \pgf@ya\pgfmathresulty\pgf@yc% ya is the back miter
    \pgf@yb\pgfmathresultx\pgf@yc% yb is the top miter
    \ifdim\pgfarrowinset=0pt%
      \pgf@ya.5\pgfarrowlinewidth% easy: back miter is half linewidth
    \fi
    % Compute inset miter length:
    \pgfmathdivide@{\pgf@sys@tonumber\pgfarrowinset}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x4\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@yc\pgfmathresult\pgfarrowlinewidth% yc is inset miter
    \pgf@yc.5\pgf@yc%
    % Inner length (pgfutil@tempdima) is now arrowlength - front miter - back miter
    \pgfutil@tempdima\pgfarrowlength%
    \advance\pgfutil@tempdima by-\pgf@xc%
    \advance\pgfutil@tempdima by-\pgf@ya%
    \pgfutil@tempdimb.5\pgfarrowwidth%
    \advance\pgfutil@tempdimb by-\pgf@yb%
    % harpoon miter correction
    \ifpgfarrowroundjoin
      \pgfarrowssetbackend{\pgf@ya\advance\pgf@x by-.5\pgfarrowlinewidth}
    \else
      \pgfarrowssetbackend{0pt}
    \fi
    \ifpgfarrowharpoon
      \pgfarrowssetlineend{\pgfarrowinset\advance\pgf@x
        by\pgf@yc\advance\pgf@x by.5\pgfarrowlinewidth}
    \else
      \pgfarrowssetlineend{\pgfarrowinset\advance\pgf@x by\pgf@yc\advance\pgf@x by-.25\pgfarrowlinewidth}
      \ifpgfarrowreversed
        \ifdim\pgfinnerlinewidth>0pt
          \pgfarrowssetlineend{\pgfarrowinset}
        \else
          \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by\pgf@ya\advance\pgf@x by-.25\pgfarrowlinewidth}
        \fi
      \fi
    \fi
    \ifpgfarrowroundjoin
      \pgfarrowssettipend{\pgfutil@tempdima\advance\pgf@x by\pgf@ya\advance\pgf@x by.5\pgfarrowlinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi}
    \fi
    % The hull:
    \pgfarrowshullpoint{\pgfarrowlength\ifpgfarrowroundjoin\else\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi\fi}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else0pt\fi}%
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}%
    \pgfarrowshullpoint{\pgfarrowinset}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else 0pt\fi}%
    % Adjust inset
    \pgfarrowssetvisualbackend{\pgfarrowinset}
    \advance\pgfarrowinset by\pgf@yc%
    % The following are needed in the code:
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgf@ya
    \pgfarrowssavethe\pgfarrowinset
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdima\advance\pgf@x by\pgf@ya}{0pt}}
    \pgfpathlineto{\pgfqpoint{\pgf@ya}{\pgfutil@tempdimb}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{0pt}}
    \ifpgfarrowharpoon \else
    \pgfpathlineto{\pgfqpoint{\pgf@ya}{-\pgfutil@tempdimb}}
    \fi
    \pgfpathclose
    \ifpgfarrowopen\pgfusepathqstroke\else\ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi\fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowopen o\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%



% A Kite is like a Stealth, only the inset counts in the other direction

\pgfdeclarearrow{
  name = Kite,
  defaults = {
    length  = +3.6pt +5.4,
    width'  = +0pt +0.5,
    inset'  = +0pt 0.25,
    line width = +0pt 1 1,
  },
  setup code = {
    % Cap the line width at 1/4th of the length
    \pgf@x.4\pgfarrowlength
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    \pgf@x.4\pgfarrowwidth
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    % Compute front miter length:
    \pgf@xa\pgfarrowlength%
    \advance\pgf@xa by-\pgfarrowinset%
    \pgfmathdivide@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x4\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@xc\pgfmathresult\pgfarrowlinewidth% xc is front miter
    \pgf@xc.5\pgf@xc
    \pgf@xa\pgf@temp@quot\pgfarrowlinewidth% xa is extra harpoon miter
    % Compute back miter length:
    \pgfmathdivide@{\pgf@sys@tonumber\pgfarrowinset}{\pgf@sys@tonumber\pgfarrowwidth}%
    \let\pgf@temp@quot\pgfmathresult%
    \pgf@x\pgfmathresult pt%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@x4\pgf@x%
    \advance\pgf@x by1pt%
    \pgfmathsqrt@{\pgf@sys@tonumber\pgf@x}%
    \pgf@yc\pgfmathresult\pgfarrowlinewidth% yc is back miter
    \pgf@yc.5\pgf@yc
    \pgf@ya\pgf@temp@quot\pgfarrowlinewidth% ya is extra harpoon miter
    % Compute top miter length:
    {%
      \pgfutil@tempdimb.5\pgfarrowwidth%
      \pgfutil@tempdima\pgfarrowlength\advance\pgfutil@tempdima by-\pgfarrowinset%
      \csname pgfmathatan2@\endcsname{\pgfmath@tonumber\pgfutil@tempdima}{\pgfmath@tonumber\pgfutil@tempdimb}%
      \pgf@yb\pgfmathresult pt%
      \csname pgfmathatan2@\endcsname{\pgfmath@tonumber\pgfarrowinset}{\pgfmath@tonumber\pgfutil@tempdimb}%
      \pgf@ya\pgfmathresult pt%
      \advance\pgf@yb by\pgf@ya%
      \pgf@yb.5\pgf@yb% half angle in yb
      \ifdim\pgf@yb=45pt%
        \def\pgfmathresult{1.414213}%
      \else%
        \pgfmathsin@{\pgf@sys@tonumber\pgf@yb}%
        \pgfmathreciprocal@{\pgfmathresult}%
      \fi%
      \pgf@yc\pgfmathresult\pgfarrowlinewidth%
      \pgf@yc.5\pgf@yc%
      \pgf@ya-\pgf@ya%
      \advance\pgf@ya by-90pt%
      \advance\pgf@ya by\pgf@yb%
      \pgfmathsincos@{\pgf@sys@tonumber\pgf@ya}%
      \pgf@xb\pgfmathresultx\pgf@yc% ya is the back miter
      \pgf@yb\pgfmathresulty\pgf@yc% yb is the top miter
      \expandafter\expandafter\expandafter%
    }\expandafter\expandafter\expandafter\pgf@xb\expandafter\the\expandafter\pgf@xb\expandafter\pgf@yb\the\pgf@yb%
    % Inner length (pgfutil@tempdima) is now arrowlength - front miter - back miter
    \pgfutil@tempdima\pgfarrowlength%
    \advance\pgfutil@tempdima by-\pgf@xc%
    \pgfutil@tempdimb.5\pgfarrowwidth%
    \advance\pgfutil@tempdimb by\pgf@yb%
    % Set back end
    \ifpgfarrowroundjoin
      \pgfarrowssetbackend{\pgf@ya\advance\pgf@x by-.5\pgfarrowlinewidth}
    \else
      \pgfarrowssetbackend{0pt}
    \fi
    % harpoon miter correction
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfutil@tempdima\advance\pgf@x by-\pgflinewidth\advance\pgf@x by\pgfarrowlinewidth}
    \else
      \pgfarrowssetlineend{\pgf@yc\advance\pgf@x by\pgflinewidth\advance\pgf@x by-\pgfarrowlinewidth}
    \fi
    \ifpgfarrowroundjoin
      \pgfarrowssettipend{\pgfutil@tempdima\advance\pgf@x by.5\pgfarrowlinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi}
    \fi
    % The hull:
    \pgfarrowshullpoint{\pgfarrowlength\ifpgfarrowroundjoin\else\ifpgfarrowharpoon\advance\pgf@x by\pgf@xa\fi\fi}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else0pt\fi}%
    \pgfarrowsupperhullpoint{\pgfarrowinset}{.5\pgfarrowwidth}%
    \pgfarrowshullpoint{0pt}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else0pt\fi}%
    % Adjust the inset:
    \advance\pgfarrowinset by\pgf@xb%
    % The following are needed in the code:
    \pgfarrowssavethe\pgfutil@tempdima
    \pgfarrowssavethe\pgfutil@tempdimb
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgf@yc
    \pgfarrowssavethe\pgfarrowinset
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{\pgfutil@tempdimb}}
    \pgfpathlineto{\pgfqpoint{\pgf@yc}{0pt}}
    \ifpgfarrowharpoon \else
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{-\pgfutil@tempdimb}}
    \fi
    \pgfpathclose
    \ifpgfarrowopen\pgfusepathqstroke\else\ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi\fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowopen o\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%




% A simple rectangle shape

\pgfdeclarearrow{
  name = Square,
  defaults = {
    length  = +2.12132pt +2.828427,
    width'  = +0pt +1,
    line width = +0pt +1 +1,
  },
  setup code = {
    % Cap the line width at 1/2th of the length
    \pgf@x.5\pgfarrowlength
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \else
      \pgfarrowssetlineend{.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % The hull:
    \pgfarrowshullpoint{\pgfarrowlength}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{0pt}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{\pgfarrowlength}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else-.5\pgfarrowwidth\fi}
    \pgfarrowshullpoint{0pt}{\ifpgfarrowharpoon-.5\pgfarrowlinewidth\else-.5\pgfarrowwidth\fi}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
    \pgfpathlineto{\pgfqpoint{.5\pgfarrowlinewidth}{.5\pgfarrowwidth\advance\pgf@y by-.5\pgfarrowlinewidth}}
    \pgfpathlineto{\pgfqpoint{.5\pgfarrowlinewidth}{\ifpgfarrowharpoon0pt\else-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth\fi}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}{\ifpgfarrowharpoon0pt\else-.5\pgfarrowwidth\advance\pgf@y by.5\pgfarrowlinewidth\fi}}
    \pgfpathclose
    \ifpgfarrowopen\pgfusepathqstroke\else\ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi\fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowopen o\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%


% A simple rectangle shape

\pgfdeclarearrow{
  name = Circle,
  defaults = {
    length  = +2.39365pt +3.191538,
    width'  = +0pt 1,
    line width = +0pt 1 1,
  },
  setup code = {
    % Cap the line width at 1/2th of the length
    \pgf@x.5\pgfarrowlength
    \ifdim\pgf@x<\pgfarrowlinewidth
      \pgfarrowlinewidth\pgf@x
    \fi
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \else
      \pgfarrowssetlineend{.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % The hull:
    \pgfarrowsupperhullpoint{\pgfarrowlength}{.25\pgfarrowwidth}
    \pgfarrowsupperhullpoint{.75\pgfarrowlength}{.5\pgfarrowwidth}
    \pgfarrowsupperhullpoint{.25\pgfarrowlength}{.5\pgfarrowwidth}
    \pgfarrowsupperhullpoint{0pt}{.25\pgfarrowwidth}
    \ifpgfarrowharpoon%
      \pgfarrowshullpoint{0pt}{-.5\pgfarrowlinewidth}
      \pgfarrowshullpoint{\pgfarrowlength}{-.5\pgfarrowlinewidth}
    \fi%
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundjoin\pgfsetroundjoin\else\pgfsetmiterjoin\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \ifpgfarrowharpoon
      \pgfpathmoveto{\pgfqpoint{\pgfarrowlength\advance\pgf@x
          by-.5\pgfarrowlinewidth}{0pt}}
      {%
        \pgf@xa.5\pgfarrowlength
        \advance\pgf@xa by-.5\pgfarrowlinewidth
        \pgftransformxscale{+\the\pgf@xa}
        \pgf@xa.5\pgfarrowwidth
        \advance\pgf@xa by-.5\pgfarrowlinewidth
        \pgftransformyscale{+\the\pgf@xa}
        \pgfpatharc{0}{180}{1pt}
      }
      \pgfpathclose
    \else%
      \pgfpathellipse{\pgfqpoint{.5\pgfarrowlength}{0pt}}{\pgfqpoint{.5\pgfarrowlength\advance\pgf@x
          by-.5\pgfarrowlinewidth}{0pt}}{\pgfqpoint{0pt}{.5\pgfarrowwidth\advance\pgf@y
          by-.5\pgfarrowlinewidth}}
    \fi
    \ifpgfarrowopen\pgfusepathqstroke\else\ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi\fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowopen o\fi%
    \ifpgfarrowroundjoin j\fi%
  },
}%

% Round cap

\pgfdeclarearrow{
  name = Round Cap,
  defaults = {
    length = +0pt .5
  },
  setup code = {
    \ifpgfarrowreversed
      \pgfarrowssettipend{\pgfarrowlength}
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by.5\pgflinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength}
      \pgfarrowssetlineend{-.5\pgflinewidth}
    \fi
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowsupperhullpoint{0pt}{.5\pgflinewidth}
    \pgfarrowsupperhullpoint{\pgfarrowlength}{.5\pgflinewidth}
  },
  drawing code = {
    \ifpgfarrowreversed
      \pgftransformxscale{-1}
      \pgftransformxshift{-\pgfarrowlength}
    \fi
    \pgfutil@tempdima.5\pgflinewidth
    \pgfpathmoveto   {\pgfqpoint{-0.75\pgflinewidth}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \ifpgfarrowreversed
      \pgfpathlineto {\pgfqpoint{\pgfarrowlength}{\pgfutil@tempdima}}
      \begingroup
      \pgftransformxshift{\pgfarrowlength}
      \pgftransformxscale{-1}
    \fi
    \pgfpathcurveto  {\pgfqpoint{0.55228475\pgfarrowlength}{\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathcurveto  {\pgfqpoint{\pgfarrowlength}{-0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{0.55228475\pgfarrowlength}{-\pgfutil@tempdima}}
                     {\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \ifpgfarrowreversed
      \endgroup
    \fi
    \pgfpathlineto   {\pgfqpoint{-.75\pgflinewidth}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfill
  },
  parameters = {\the\pgfarrowlength}
}%



\pgfdeclarearrow{
  name = Butt Cap,
  defaults = {
    length = +0pt .5
  },
  setup code = {
    \pgfarrowssettipend{\pgfarrowlength}
    \pgfarrowssetlineend{-.5\pgflinewidth}
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowsupperhullpoint{0pt}{.5\pgflinewidth}
    \pgfarrowsupperhullpoint{\pgfarrowlength}{.5\pgflinewidth}
  },
  drawing code = {
    \pgfutil@tempdima.5\pgflinewidth
    \pgfpathmoveto   {\pgfqpoint{-0.75\pgflinewidth}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowlength}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowlength}{-\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{-.75\pgflinewidth}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfill
  },
  parameters = {\the\pgfarrowlength}
}%



\pgfkeys{
  /pgf/arrow keys/.cd,
  cap angle/.code={%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@x.5\pgf@x
    \pgfmathtan@{\pgf@sys@tonumber\pgf@x}%
    \pgfmathreciprocal@{\pgfmathresult}%
    \pgf@x\pgfmathresult pt%
    \pgf@x.5\pgf@x%
    \edef\pgf@marshal{\noexpand\pgfarrowsaddtooptions{\noexpand\pgfarrowslinewidthdependent{+0pt}{\pgf@sys@tonumber\pgf@x}{0}\pgfarrowlength\pgf@x}}
    \pgf@marshal
  }
}%


\pgfdeclarearrow{
  name = Triangle Cap,
  defaults = {
    length = +0pt .5
  },
  setup code = {
    \ifpgfarrowreversed
      \pgfarrowssettipend{\pgfarrowlength}
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by.5\pgflinewidth}
    \else
      \pgfarrowssettipend{\pgfarrowlength}
      \pgfarrowssetlineend{-.5\pgflinewidth}
    \fi
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowsupperhullpoint{0pt}{.5\pgflinewidth}
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
  },
  drawing code = {
    \ifpgfarrowreversed
      \pgftransformxscale{-1}
      \pgftransformxshift{-\pgfarrowlength}
    \fi
    \pgfutil@tempdima.5\pgflinewidth
    \pgfpathmoveto   {\pgfqpoint{-0.75\pgflinewidth}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \ifpgfarrowreversed
      \pgfpathlineto {\pgfqpoint{\pgfarrowlength}{\pgfutil@tempdima}}
      \begingroup
      \pgftransformxshift{\pgfarrowlength}
      \pgftransformxscale{-1}
    \fi
    \pgfpathlineto   {\pgfqpoint{\pgfarrowlength}{0pt}}
    \ifpgfarrowreversed
      \endgroup
      \pgfpathlineto {\pgfqpoint{\pgfarrowlength}{-\pgfutil@tempdima}}
    \fi
    \pgfpathlineto   {\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{-.75\pgflinewidth}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfill
  },
  parameters = {\the\pgfarrowlength}
}%



\pgfdeclarearrow{
  name = Fast Triangle,
  defaults = {
    length = +0pt .5,
    inset = +0pt .5,
  },
  setup code = {
    \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}
    \ifpgfarrowreversed\pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}\fi
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowsupperhullpoint{0pt}{.5\pgflinewidth}
    \pgfarrowsupperhullpoint{\pgfarrowinset}{.5\pgflinewidth}
    \pgfarrowshullpoint{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}{0pt}
  },
  drawing code = {
    \pgfutil@tempdima.5\pgflinewidth
    \pgfpathmoveto   {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowinset}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowinset\advance\pgf@x by\pgfarrowlength}{0pt}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowinset}{-\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathclose
    \pgfusepathqfill
  },
  parameters = {\the\pgfarrowlength,\the\pgfarrowinset}
}%


\pgfdeclarearrow{
  name = Fast Round,
  defaults = {
    length = +0pt .5,
    inset = +0pt .5,
  },
  setup code = {
    \pgfarrowssettipend{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}
    \ifpgfarrowreversed\pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}\fi
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowsupperhullpoint{0pt}{.5\pgflinewidth}
    \pgfarrowsupperhullpoint{\pgfarrowlength\advance\pgf@x by\pgfarrowinset}{.5\pgflinewidth}
  },
  drawing code = {
    \pgfutil@tempdima.5\pgflinewidth
    \pgfpathmoveto   {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto   {\pgfqpoint{\pgfarrowinset}{\pgfutil@tempdima}}
    {
      \pgftransformxshift{\pgfarrowinset}
      \pgfpathcurveto{\pgfqpoint{0.55228475\pgfarrowlength}{\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{0pt}}
      \pgfpathcurveto{\pgfqpoint{\pgfarrowlength}{-0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{0.55228475\pgfarrowlength}{-\pgfutil@tempdima}}
                     {\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    }
    \pgfpathlineto   {\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathcurveto  {\pgfqpoint{0.55228475\pgfarrowlength}{-\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{-0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathcurveto  {\pgfqpoint{\pgfarrowlength}{0.55228475\pgfutil@tempdima}}
                     {\pgfqpoint{0.55228475\pgfarrowlength}{\pgfutil@tempdima}}
                     {\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfill
  },
  parameters = {\the\pgfarrowlength,\the\pgfarrowinset}
}%




%
%
% Other arrow tips.
%
%


\pgfkeys{
  /pgf/arrow keys/.cd,
  n/.code={%
    \pgfmathparse{#1}%
    \expandafter\pgf@lib@meta@strip@dot\pgfmathresult.\relax%
  }
}%
\def\pgf@lib@meta@strip@dot#1.#2\relax{%
  \pgfarrowsaddtooptions{\def\pgfarrown{#1}}%
}%

\def\pgfarrown{4}%

\pgfdeclarearrow{
  name = Rays,
  defaults = {
    length = +3pt 4,
    width'  = +0pt 1,
    line width = +0pt 1 1,
  },
  setup code = {
    \pgfmathdivide@{360}{\pgfarrown}%
    \let\pgfarrow@inc\pgfmathresult%
    % Compute tips:
    \pgf@xa\pgfarrow@inc pt%
    \ifodd\pgfarrown\pgf@ya.25\pgf@xa\else\pgf@ya.5\pgf@xa\fi%
    \pgfmathsincos@{\pgf@sys@tonumber\pgf@ya}%
    \pgf@x.5\pgfarrowlength%
    \pgf@xa\pgfmathresultx\pgf@x%
    \ifpgfarrowroundcap
      \advance\pgf@xa by.5\pgfarrowlinewidth
    \else
      \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgfmathresultx\pgfarrowlength}{\pgfmathresulty\pgfarrowwidth}}}%
      \pgf@x.5\pgfarrowlinewidth%
      \advance\pgf@xa by\pgf@sys@tonumber{\pgf@y}\pgf@x%
    \fi%
    \pgfarrowssettipend{\pgf@xa}
    \pgfarrowssetbackend{-\pgf@xa}
    % Hull is always 8-point hull, except for tip
    % The following are needed in the code:
    \pgfarrowsupperhullpoint{\pgf@xa}{.25\pgfarrowwidth}
    \pgfarrowsupperhullpoint{.25\pgfarrowlength}{.5\pgfarrowwidth\ifpgfarrowroundcap\advance\pgf@y by.5\pgfarrowlinewidth\fi}
    \pgfarrowsupperhullpoint{-.25\pgfarrowlength}{.5\pgfarrowwidth\ifpgfarrowroundcap\advance\pgf@y by.5\pgfarrowlinewidth\fi}
    \pgfarrowsupperhullpoint{-\pgf@xa}{.25\pgfarrowwidth}
    \ifpgfarrowharpoon
      \pgfarrowshullpoint{-.5\pgfarrowlength\ifpgfarrowroundcap\advance\pgf@x by-.5\pgfarrowlinewidth\fi}{-.5\pgfarrowlinewidth}
      \pgfarrowshullpoint{.5\pgfarrowlength\ifpgfarrowroundcap\advance\pgf@x by.5\pgfarrowlinewidth\fi}{-.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
    \pgfarrowssave\pgfarrow@inc
    \pgfarrowssave\pgfarrown
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifpgfarrowroundcap\pgfsetroundcap\else\pgfsetbuttcap\fi
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    {%
      \pgfgettransform\pgf@temp@trans
      \pgftransformxscale{+.5\pgfarrowlength}
      \pgftransformyscale{+.5\pgfarrowwidth}
      \pgf@xa\pgfarrow@inc pt%
      \ifodd\pgfarrown\pgf@ya.25\pgf@xa\else\pgf@ya.5\pgf@xa\fi%
      \ifpgfarrowharpoon\pgf@yb180pt\else\pgf@yb360pt\fi
      \pgfutil@loop%
      \ifdim\pgf@ya<\pgf@yb%
        \pgfpathmoveto{\pgfpointpolar{+\pgf@ya}{+1pt}}
        \pgfpathlineto{\pgfpointorigin}
        \ifpgfarrowharpoon\ifdim\pgf@ya>\pgf@xa\else{\pgfsettransform\pgf@temp@trans\pgfpathlineto{\pgfqpoint{-.5\pgflinewidth}{0pt}}}\fi\fi
        \advance\pgf@ya by\pgf@xa\relax%
      \pgfutil@repeat%
    }
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \pgfarrown,%
    \ifpgfarrowharpoon h\fi%
    \ifpgfarrowroundcap c\fi%
  }
}%



% Shorthands and Aliases:

\pgfkeys{
  LaTeX /.tip         = {Latex},
  Triangle /.tip      = {Stealth[inset=+0pt, angle=+60:+2.7pt +3.6]},
  Rectangle /.tip     = {Square[length=+3pt +4.5,width'=+0pt +.5]},
  Ellipse /.tip       = {Circle[length=+3.3pt +4.95, width'=+0pt +0.5]},
  Diamond /.tip       = {Kite[inset'=+0pt .5]},
  Turned Square /.tip = {Kite[length=+3pt 4,width'= +0pt 1,inset'= +0pt 0.5]},
  To /.tip            = {Computer Modern Rightarrow},
  Bar /.tip           = {Tee Barb[length=+0pt]},
  Bracket /.tip       = {Tee Barb[inset'=+0pt +1,length=+0.75pt +1]},
  Parenthesis /.tip   = {Arc Barb[arc=+120,length=+1.725pt +2.3]}
}%




\endinput


==> pgflibrarydecorations.pathreplacing.code.tex <==
% Copyright 2018 by Mark Wibrow and Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}%


%
% Path replacing decorations
%
% These decorations change the path by replacing it by another path.
% For instance, a line in the path might be replaced by small
% ticks or unconnected curves or crosses. Applying a chopping
% decoration to a path means that the path can no longer be used for
% filling in the original manner.
%



%
%
% Kind 1: Path chopping with open subpaths
%
%


% ticks decoration
%
% Parameters: \pgfdecorationsegmentlength, \pgfdecorationsegmentamplitude

\pgfdeclaredecoration{ticks}{ticks}
{%
  \state{ticks}[width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfdecorationsegmentamplitude}}
  }%
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfdecorationsegmentamplitude}}
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }%
}%



% expanding waves decoration
%
% Parameters: \pgfdecorationsegmentangle, \pgfdecorationsegmentlength

\pgfdeclaredecoration{expanding waves}{initial}
{%
  \state{initial}[width=+\pgfdecorationsegmentlength,next state=wave]
  {}%

  \state{wave}[switch if less than=+\pgfdecorationsegmentlength to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfdecoratedcompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}%
  }%
  \state{last}[width=+0pt,next state=final]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfdecoratedcompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}%
  }%
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }%
}%



% waves decoration

\pgfdeclaredecoration{waves}{wave}
{%
  \state{wave}[width=\pgfdecorationsegmentlength]
  {
    \pgftransformxshift{+\pgfdecorationsegmentlength}
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfkeysvalueof{/pgf/decoration/start radius}}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}%
  }%
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }%
}%



% border decoration
%
% Parameters: \pgfdecorationsegmentlength, \pgfdecorationsegmentamplitude, \pgfdecorationsegmentangle

\pgfdeclaredecoration{border}{tick}
{%
  \state{tick}[switch if less than=+\pgfdecorationsegmentlength to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecorationsegmentamplitude}}
  }%
  \state{last}[width=+\pgfdecorationsegmentamplitude,next state=final]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecorationsegmentamplitude}}
  }%
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }%
}%






% brace decorations
%
% Parameters: \pgfdecorationsegmentamplitude

\pgfdeclaredecoration{brace}{brace}
{%
  \state{brace}[width=+\pgfdecoratedremainingdistance,next state=final]
  {
    \pgf@yc=\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance
    \ifdim2\pgfdecorationsegmentamplitude>\pgf@yc
      \pgf@yc=0.5\pgf@yc
    \else
      \pgf@yc=\pgfdecorationsegmentamplitude
    \fi
    \pgf@xc=\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance
    \advance\pgf@xc-\pgfdecoratedremainingdistance
    \ifdim-2\pgfdecorationsegmentamplitude<\pgf@xc
      \pgf@xc=-0.5\pgf@xc
    \else
      \pgf@xc=\pgfdecorationsegmentamplitude
    \fi
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
    {\pgfqpoint{.15\pgf@yc}{.3\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.5\pgf@yc}{.5\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{\pgf@yc}{.5\pgfdecorationsegmentamplitude}}
    {
      \pgftransformxshift{+\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgf@yc}{.5\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgf@yc}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{-.15\pgf@yc}{.7\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{0\pgf@yc}{1\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{.15\pgf@xc}{.7\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{.5\pgf@xc}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{\pgf@xc}{.5\pgfdecorationsegmentamplitude}}
    }
    {
      \pgftransformxshift{+\pgfdecoratedremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgf@xc}{.5\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgf@xc}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{-.15\pgf@xc}{.3\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{0pt}{0pt}}
    }
  }%
  \state{final}
  {}%
}%




% show path construction decoration
%
\pgfdeclaredecoration{show path construction}{check for moveto}{%
    \state{check for moveto}[width=0pt, next state=segment,
      persistent precomputation={%
        \begingroup%
            \pgf@lib@decoraions@installinputsegmentpoints%
              \ifx\pgfdecorationpreviousinputsegment\pgfdecorationinputsegmentmoveto%
                  \pgfdecoratedinputsegmentmovetocode%
              \fi%
            \endgroup%
        }]{}%
    \state{segment}[width=\pgfdecoratedinputsegmentremainingdistance, next state=check for moveto,
      persistent precomputation={%
        \begingroup%
            \pgf@lib@decoraions@installinputsegmentpoints%
                \csname pgfdecoratedinputsegment\pgfdecorationcurrentinputsegment code\endcsname%
            \endgroup%
        }]{}%
    \state{final}{%
        \egroup%
        \begingroup%
        \pgf@lib@decoraions@installinputsegmentpoints%
            \csname pgfdecoratedinputsegment\pgfdecorationcurrentinputsegment code\endcsname%
        \endgroup%
        \bgroup%
    }%
}%

\pgfkeys{
    /pgf/decoration/.cd,
        moveto code/.code=\def\pgfdecoratedinputsegmentmovetocode{#1},
        lineto code/.code=\def\pgfdecoratedinputsegmentlinetocode{#1},
        curveto code/.code=\def\pgfdecoratedinputsegmentcurvetocode{#1},
      closepath code/.code=\def\pgfdecoratedinputsegmentclosepathcode{#1}
}%

\let\pgfdecoratedinputsegmentmovetocode\pgfutil@empty%
\let\pgfdecoratedinputsegmentlinetocode\pgfutil@empty%
\let\pgfdecoratedinputsegmentcurvetocode\pgfutil@empty%
\let\pgfdecoratedinputsegmentclosepathcode\pgfutil@empty%

\def\pgf@lib@decoraions@installinputsegmentpoints{%
    \let\pgfpointdecoratedinputsegmentfirst\pgf@decorate@inputsegment@first%
    \let\pgfpointdecoratedinputsegmentlast\pgf@decorate@inputsegment@last%
    \let\pgfpointdecoratedinputsegmentsupporta\pgf@decorate@inputsegment@supporta%
    \let\pgfpointdecoratedinputsegmentsupportb\pgf@decorate@inputsegment@supportb%
}%


\endinput


==> pgflibrarypatterns.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibrarypatterns.code.tex}


% Lines in different directions

\pgfdeclarepatternformonly{horizontal lines}{\pgfpointorigin}{\pgfqpoint{100pt}{1pt}}{\pgfqpoint{100pt}{3pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{0pt}{0.5pt}}%
  \pgfpathlineto{\pgfqpoint{100pt}{0.5pt}}%
  \pgfusepath{stroke}%
}%

\pgfdeclarepatternformonly{vertical lines}{\pgfpointorigin}{\pgfqpoint{1pt}{100pt}}{\pgfqpoint{3pt}{100pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{0.5pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{0.5pt}{100pt}}%
  \pgfusepath{stroke}%
}%

\pgfdeclarepatternformonly{north east lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}%
  \pgfusepath{stroke}%
}%

\pgfdeclarepatternformonly{north west lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{0pt}{3pt}}%
  \pgfpathlineto{\pgfqpoint{3.1pt}{-0.1pt}}%
  \pgfusepath{stroke}%
}%

% Crossed lines in different directions

\pgfdeclarepatternformonly{grid}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}%
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{3.1pt}{0pt}}%
  \pgfusepath{stroke}%
}%

\pgfdeclarepatternformonly{crosshatch}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfsetlinewidth{0.4pt}%
  \pgfpathmoveto{\pgfqpoint{3.1pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}%
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}%
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}%
  \pgfusepath{stroke}%
}%


% Dotted regions

\pgfdeclarepatternformonly{dots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{1pt}{1pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatternformonly{crosshatch dots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2.5pt}{2.5pt}}{\pgfqpoint{3pt}{3pt}}%
{%
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}%
  \pgfpathcircle{\pgfqpoint{1.5pt}{1.5pt}}{.5pt}%
  \pgfusepath{fill}%
}%




% Star shaped patterns

\pgfdeclarepatternformonly{fivepointed stars}{\pgfpointorigin}{\pgfqpoint{3mm}{3mm}}{\pgfqpoint{3mm}{3mm}}%
{%
  \pgftransformshift{\pgfqpoint{1mm}{1mm}}%
  \pgfpathmoveto{\pgfqpointpolar{18}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{162}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{306}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{90}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{234}{1mm}}%
  \pgfpathclose%%
  \pgfusepath{fill}%
}%

\pgfdeclarepatternformonly{sixpointed stars}{\pgfpointorigin}{\pgfqpoint{3mm}{3mm}}{\pgfqpoint{3mm}{3mm}}%
{%
  \pgftransformshift{\pgfqpoint{1mm}{1mm}}%
  \pgfpathmoveto{\pgfqpointpolar{30}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{150}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{270}{1mm}}%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpointpolar{-30}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{-270}{1mm}}%
  \pgfpathlineto{\pgfqpointpolar{-150}{1mm}}%
  \pgfpathclose%
  \pgfsetnonzerorule%
  \pgfusepath{fill}%
}%



% Bricks

\pgfdeclarepatternformonly{bricks}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{5mm}{5mm}}{\pgfqpoint{4mm}{4mm}}%
{%
  \pgfsetlinewidth{0.8pt}%
  \pgfpathmoveto{\pgfqpoint{0mm}{1mm}}%
  \pgfpathlineto{\pgfqpoint{4mm}{1mm}}%
  \pgfpathmoveto{\pgfqpoint{0mm}{3mm}}%
  \pgfpathlineto{\pgfqpoint{4mm}{3mm}}%
  \pgfpathmoveto{\pgfqpoint{1mm}{0mm}}%
  \pgfpathlineto{\pgfqpoint{1mm}{1mm}}%
  \pgfpathmoveto{\pgfqpoint{3mm}{1mm}}%
  \pgfpathlineto{\pgfqpoint{3mm}{3mm}}%
  \pgfpathmoveto{\pgfqpoint{1mm}{3mm}}%
  \pgfpathlineto{\pgfqpoint{1mm}{4mm}}%
  \pgfusepath{stroke}%
}%


% Checkerboards

\pgfdeclarepatternformonly{checkerboard}{\pgfpointorigin}{\pgfqpoint{4mm}{4mm}}{\pgfqpoint{4mm}{4mm}}%
{%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{2mm}{2mm}}%
  \pgfpathrectangle{\pgfqpoint{2mm}{2mm}}{\pgfqpoint{2mm}{2mm}}%
  \pgfusepath{fill}%
}%



% Backgrounds

\pgfdeclarepatterninherentlycolored{checkerboard light gray}
{\pgfpointorigin}{\pgfqpoint{4mm}{4mm}}{\pgfqpoint{4mm}{4mm}}%
{%
%  \pgfsetfillcolor{black!10}
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{4.1mm}{4.1mm}}% make
                                % slightly larger to ensure that tiles
                                % are really solid
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!20}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{2mm}{2mm}}%
  \pgfpathrectangle{\pgfqpoint{2mm}{2mm}}{\pgfqpoint{2mm}{2mm}}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatterninherentlycolored{horizontal lines light gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{%
  \pgfsetfillcolor{black!10}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!15}%
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatterninherentlycolored{horizontal lines gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{%
  \pgfsetfillcolor{black!30}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!35}%
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatterninherentlycolored{horizontal lines dark gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{%
  \pgfsetfillcolor{black!90}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!85}%
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatterninherentlycolored{horizontal lines light blue}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{%
  \pgfsetfillcolor{blue!10}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{blue!15}%
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
}%

\pgfdeclarepatterninherentlycolored{horizontal lines dark blue}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{%
  \pgfsetfillcolor{blue!90}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{blue!85}%
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}%
  \pgfusepath{fill}%
}%


\pgfdeclarepatterninherentlycolored{crosshatch dots gray}
{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
{\pgfpoint{8pt}{8pt}}
{%
  \pgfsetfillcolor{black!20}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!10}%
  \pgfpathcircle{\pgfpoint{2pt}{1.75pt}}{1pt}%
  \pgfpathcircle{\pgfpoint{6pt}{5.75pt}}{1pt}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{black!70}%
  \pgfpathcircle{\pgfpoint{2pt}{2.25pt}}{1pt}%
  \pgfpathcircle{\pgfpoint{6pt}{6.25pt}}{1pt}%
  \pgfusepath{fill}%
}%

\pgfutil@definecolor{pgf@lightsteelblue}{rgb}{0.6875,0.765625,0.8671875}%
\pgfutil@colorlet{pgf@darklightsteelblue}{black!50!pgf@lightsteelblue}%

\pgfdeclarepatterninherentlycolored{crosshatch dots light steel blue}
{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
{\pgfpoint{8pt}{8pt}}
{%
  \pgfsetfillcolor{pgf@lightsteelblue}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{pgf@darklightsteelblue!10}%
  \pgfpathcircle{\pgfpoint{2pt}{1.75pt}}{1pt}%
  \pgfpathcircle{\pgfpoint{6pt}{5.75pt}}{1pt}%
  \pgfusepath{fill}%
  \pgfsetfillcolor{pgf@darklightsteelblue!70}%
  \pgfpathcircle{\pgfpoint{2pt}{2.25pt}}{1pt}%
  \pgfpathcircle{\pgfpoint{6pt}{6.25pt}}{1pt}%
  \pgfusepath{fill}%
}%


\endinput


==> pgflibraryplothandlers.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryplothandlers.code.tex}


% This handler converts each plot stream command into a curveto
% command, except for the first, which is converted to the previously
% specified action.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfsetlinetofirstplotpoint
% \pgfplothandlercurveto
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlercurveto}{}{%
  point macro=\pgf@plot@curveto@handler@initial,
  jump macro=\pgf@plot@smooth@next@moveto,
  end macro=\pgf@plot@curveto@handler@finish
}%

\def\pgf@plot@smooth@next@moveto{%
  \pgf@plot@curveto@handler@finish%
  \global\pgf@plot@startedfalse%
  \global\let\pgf@plotstreampoint\pgf@plot@curveto@handler@initial%
}%

\def\pgf@plot@curveto@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@plot@first@action{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@curveto@first{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plot@curveto@first@support=\pgf@plot@curveto@first%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@second%
}%

\def\pgf@plot@curveto@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@second{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@third%
  \global\pgf@plot@startedtrue%
}%

\def\pgf@plot@curveto@handler@third#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@curveto@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@curveto@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@curveto@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@curveto@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@curveto@first=\pgf@plot@curveto@second%
  \global\let\pgf@plot@curveto@second=\pgf@plot@curveto@current%
  \xdef\pgf@plot@curveto@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}%

\def\pgf@plot@curveto@handler@finish{%
  \ifpgf@plot@started%
    \pgfpathcurveto{\pgf@plot@curveto@first@support}{\pgf@plot@curveto@second}{\pgf@plot@curveto@second}%
  \fi%
}%


% This commands sets the tension for smoothing of plots.
%
% #1 = tension of curves. A value of 1 will yield a circle when the
%      control points are at quarters of a circle. A smaller value
%      will result in a tighter curve. Default is 0.5.
%
% Example:
%
% \pgfsetplottension{0.2}

\def\pgfsetplottension#1{%
  \pgf@x=#1pt\relax%
  \pgf@x=0.2775\pgf@x\relax%
  \edef\pgf@plottension{\pgf@sys@tonumber\pgf@x}}%
\pgfsetplottension{0.5}%


% This handler converts the plot stream command into a curveto
% command that is closed using a closepath.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfplothandlerclosedcurve
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerclosedcurve}{}{%
  point macro=\pgf@plot@closedcurve@handler@initial,
  end macro=\pgf@plot@closedcurve@handler@finish,
  jump macro=\pgf@plot@closedsmooth@next@moveto
}%

\def\pgf@plot@closedsmooth@next@moveto{%
  \pgf@plot@closedcurve@handler@finish%
  \global\pgf@plot@startedfalse%
  \global\let\pgf@plotstreampoint\pgf@plot@closedcurve@handler@initial%
}%

\def\pgf@plot@closedcurve@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@closedcurve@initial{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@second%
  \global\pgf@plot@startedfalse%
}%

\def\pgf@plot@closedcurve@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@after@initial{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {\pgfpathmoveto{}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@third%
}%

\def\pgf@plot@closedcurve@handler@third#1{%
  \global\pgf@plot@startedtrue%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@initial}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@after@initial}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@after@initial%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@after@initial@presupport{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@fourth%
}%

\def\pgf@plot@closedcurve@handler@fourth#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@second%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}%

\def\pgf@plot@closedcurve@handler@finish{%
  \ifpgf@plot@started
    %
    % first, draw line from 2nd last to last:
    %
    \pgf@process{\pgf@plot@closedcurve@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@first}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@second}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
    {\pgf@marshal}%
    \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    %
    % second, draw line from last point to start:
    %
    \pgf@process{\pgf@plot@closedcurve@after@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@second}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@initial}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@initial}}%
    {\pgf@marshal}%
    %
    % third, draw line from first to second point:
    %
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgf@plot@closedcurve@after@initial@presupport}{\noexpand\pgf@plot@closedcurve@after@initial}}%
    {\pgf@marshal}%
    \pgfpathclose%
  \fi%
}%





% This handler converts each point in a stream into a line from the
% $y$-axis to the given points coordinate, resulting in a
% ``comb.''
%
% Example:
%
% \pgfplothandlerxcomb
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerxcomb}{}{%
  start macro=\pgfplotxzerolevelstreamstart,
  point macro=\pgf@plot@xcomb@handler,
  end macro=\pgfplotxzerolevelstreamend,
}%

\def\pgf@plot@xcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \pgfpathmoveto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}%


% This handler converts each point in a stream into a line from the
% $x$-axis straight up to the given points coordinate, resulting in a
% ``comb.''
%
% Example:
%
% \pgfplothandlerycomb
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerycomb}{}{%
  start macro=\pgfplotyzerolevelstreamstart,
  point macro=\pgf@plot@ycomb@handler,
  end macro=\pgfplotyzerolevelstreamend
}%

\def\pgf@plot@ycomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}%

% PGF Bar or comb plots usually draw something from zero to the current plot's coordinate.
%
% The 'zero' offset can be changed using an input stream.
%
% There are two such streams which can be configured independently.
% The first one returns "zeros" for coordinate x, the second one
% returns "zeros" for coordinate y.
%
% \pgfplotxzerolevelstreamstart
% \pgfplotxzerolevelstreamnext % assigns \pgf@x globally
% \pgfplotxzerolevelstreamnext
% \pgfplotxzerolevelstreamnext
% \pgfplotxzerolevelstreamend
%
% and
% \pgfplotyzerolevelstreamstart
% \pgfplotyzerolevelstreamnext % assigns \pgf@x globally
% \pgfplotyzerolevelstreamend
%
\def\pgfplotxzerolevelstreamstart{\pgf@plotxzerolevelstreamstart}%
\def\pgfplotxzerolevelstreamend{\pgf@plotxzerolevelstreamend}%
\def\pgfplotxzerolevelstreamnext{\pgf@plotxzerolevelstreamnext}
\def\pgfplotyzerolevelstreamstart{\pgf@plotyzerolevelstreamstart}%
\def\pgfplotyzerolevelstreamend{\pgf@plotyzerolevelstreamend}%
\def\pgfplotyzerolevelstreamnext{\pgf@plotyzerolevelstreamnext}%

% This zero level stream always returns '#1' (a dimension).
\def\pgfplotxzerolevelstreamconstant#1{%
    \edef\pgfplotxzerolevelstreamconstant@val{#1}%
    \def\pgf@plotxzerolevelstreamstart{%
        \global\let\pgf@plotxzerolevelstreamend=\relax
        \gdef\pgf@plotxzerolevelstreamnext{\global\pgf@x=\pgfplotxzerolevelstreamconstant@val\relax}%
    }%
}%
\pgfplotxzerolevelstreamconstant{0pt}%

% This zero level stream always returns '#1'.
\def\pgfplotyzerolevelstreamconstant#1{%
    \edef\pgfplotyzerolevelstreamconstant@val{#1}%
    \def\pgf@plotyzerolevelstreamstart{%
        \global\let\pgf@plotyzerolevelstreamend=\relax
        \gdef\pgf@plotyzerolevelstreamnext{\global\pgf@x=\pgfplotyzerolevelstreamconstant@val\relax}%
    }%
}%
\pgfplotyzerolevelstreamconstant{0pt}%

\def\pgfplotbarwidth{\pgfkeysvalueof{/pgf/bar width}}%
\def\pgfplotbarshift{\pgfkeysvalueof{/pgf/bar shift}}%

\pgfqkeys{/pgf}{%
    bar width/.initial=10pt,
    bar shift/.initial=0pt,
    bar interval width/.initial=1,
    bar interval shift/.initial=0.5,
    %
    % hook which is executed right before a new bar is begun.
    at begin bar/.initial=,
    % hook which is executed right after a bar path has been finished.
    % In this context, the bar's path has not been used.
    at end bar/.initial=,
}%

% This handler places a rectangle at each point in the plot stream, a
% rectangle which touches the x-axis at one end and the current point
% at the other end:
%    --(X)--
%    |     |
%    |     |
%    |     |
%    --(0)--
% Example:
%
% \pgfplothandlerybar
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerybar}{}{%
  start={
    \pgfmathparse{\pgfplotbarwidth}%
    \xdef\pgfplotbarwidth@{\pgfmathresult pt}%
    \pgfmathparse{\pgfplotbarshift}%
    \xdef\pgfplotbarshift@{\pgfmathresult pt}%
    \pgfplotyzerolevelstreamstart
  },
  end macro=\pgfplotyzerolevelstreamend,
  point macro=\pgf@plot@ybar@handler
}%

\def\pgf@plot@ybar@handler#1{%
  \pgfkeysvalueof{/pgf/at begin bar}%
  \pgf@process{#1}%
  \pgf@ya=\pgf@y
  \expandafter\pgf@xb\pgfplotbarwidth@\relax
  \pgf@xc=\pgf@x
  \advance\pgf@xc by-.5\pgf@xb
  \advance\pgf@xc by\pgfplotbarshift@\relax
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
    {\pgfqpoint{\pgf@xc}{\pgf@yb}}%
    {\pgfqpoint{\pgf@xb}{\pgf@ya}}%
  \pgfkeysvalueof{/pgf/at end bar}%
}%

% This handler places a rectangle at each point in the plot stream, a
% rectangle which touches the y-axis at one end and the current point
% at the other end:
%    ---------
%    |       |
%   (0)     (X)
%    |       |
%    ---------
% Example:
%
% \pgfplothandlerxbar
% \pgfplotxyfile{mytable}
\pgfdeclareplothandler{\pgfplothandlerxbar}{}{%
  start={
    \pgfmathparse{\pgfplotbarwidth}%
    \xdef\pgfplotbarwidth@{\pgfmathresult pt}%
    \pgfmathparse{\pgfplotbarshift}%
    \xdef\pgfplotbarshift@{\pgfmathresult pt}%
    \pgfplotxzerolevelstreamstart
  },
  end macro=\pgfplotxzerolevelstreamend,
  point macro=\pgf@plot@xbar@handler
}%

\def\pgf@plot@xbar@handler#1{%
  \pgfkeysvalueof{/pgf/at begin bar}%
  \pgf@process{#1}%
  \pgf@ya=\pgf@x
  \expandafter\pgf@xb\pgfplotbarwidth@\relax
  \pgf@xc=\pgf@y
  \advance\pgf@xc by-.5\pgf@xb
  \advance\pgf@xc by\pgfplotbarshift@\relax
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
    {\pgfqpoint{\pgf@yb}{\pgf@xc}}%
    {\pgfqpoint{\pgf@ya}{\pgf@xb}}%
  \pgfkeysvalueof{/pgf/at end bar}%
}%

% This handler is a variant of \pgfplothandlerybar which works with
% intervals instead of points.
%
% Bars are drawn between successive input coordinates and the width is
% determined relatively to the interval length.
%
% It looks like this:
%
%    |---|      |-----|
%    |   |      |     |
%    |   |      |     |
%    |   |      |     |
% (X)------(X)-----------(X)
%
% where (X) denotes the x-axis offsets of input coordinates.
%
% In more detail, if (x_i,y_i) and (x_{i+1},y_{i+1}) denote successive
% input coordinates, the bar will be placed above the
% interval [x_i,x_{i+1}], centered at
%
%    x_i + \pgfkeysvalueof{/pgf/bar interval shift} * (x_{i+1} - x_i)
%
% with width
%
%    \pgfkeysvalueof{/pgf/bar interval width} * (x_{i+1} - x_i).
%
% If you have N+1 input points, you will get N bars (one for each
% interval). The y_i value of the last bar will be ignored.
%
% Example:
%
% \pgfplothandlerybarinterval
% \pgfplotxyfile{mytable}
\pgfdeclareplothandler{\pgfplothandlerybarinterval}{}{%
  start={
    \pgfmathparse{\pgfkeysvalueof{/pgf/bar interval width}}%
    \xdef\pgfplotbarintervalwidth@{\pgfmathresult}%
    \pgfmathparse{\pgfkeysvalueof{/pgf/bar interval shift}}%
    \xdef\pgfplotbarintervalshift@{\pgfmathresult}%
    \pgfplotyzerolevelstreamstart
  },
  end macro=\pgfplotyzerolevelstreamend,
  point macro=\pgf@plot@ybarinterval@handler@first
}%

\def\pgf@plot@ybarinterval@handler@first#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@x}%
  \xdef\pgf@plot@barinterval@bar{\the\pgf@y}%
  \global\let\pgf@plotstreampoint=\pgf@plot@ybarinterval@handler%
}%
\def\pgf@plot@ybarinterval@handler#1{%
  \pgfkeysvalueof{/pgf/at begin bar}%
  \pgf@process{#1}%
  \pgf@ya=\pgf@plot@barinterval@bar
  \xdef\pgf@plot@barinterval@bar{\the\pgf@y}%
  \pgf@xc=\pgf@plot@barinterval@intervalstart\relax
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@x}%
  \pgf@xb=\pgf@x
  \advance\pgf@xb by-\pgf@xc
  \advance\pgf@xc by\pgfplotbarintervalshift@\pgf@xb
  \pgf@xb=\pgfplotbarintervalwidth@\pgf@xb
  \advance\pgf@xc by-.5\pgf@xb% center
  \begingroup
  \pgfplotyzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
    {\pgfqpoint{\pgf@xc}{\pgf@yb}}%
    {\pgfqpoint{\pgf@xb}{\pgf@ya}}%
  \pgfkeysvalueof{/pgf/at end bar}%
}%

% Like \pgfplothandlerybarinterval but for xbar.
\pgfdeclareplothandler{\pgfplothandlerxbarinterval}{}{%
  start={
    \pgfmathparse{\pgfkeysvalueof{/pgf/bar interval width}}%
    \xdef\pgfplotbarintervalwidth@{\pgfmathresult}%
    \pgfmathparse{\pgfkeysvalueof{/pgf/bar interval shift}}%
    \xdef\pgfplotbarintervalshift@{\pgfmathresult}%
    \pgfplotxzerolevelstreamstart
  },
  end macro=\pgfplotxzerolevelstreamend,
  point macro=\pgf@plot@xbarinterval@handler@first
}%

\def\pgf@plot@xbarinterval@handler@first#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@y}%
  \xdef\pgf@plot@barinterval@bar{\the\pgf@x}%
  \global\let\pgf@plotstreampoint=\pgf@plot@xbarinterval@handler%
}%
\def\pgf@plot@xbarinterval@handler#1{%
  \pgfkeysvalueof{/pgf/at begin bar}%
  \pgf@process{#1}%
  \pgf@ya=\pgf@plot@barinterval@bar
  \xdef\pgf@plot@barinterval@bar{\the\pgf@x}%
  \pgf@xc=\pgf@plot@barinterval@intervalstart\relax
  \xdef\pgf@plot@barinterval@intervalstart{\the\pgf@y}%
  \pgf@xb=\pgf@y
  \advance\pgf@xb by-\pgf@xc
  \advance\pgf@xc by\pgfplotbarintervalshift@\pgf@xb
  \pgf@xb=\pgfplotbarintervalwidth@\pgf@xb
  \advance\pgf@xc by-.5\pgf@xb% center
  \begingroup
  \pgfplotxzerolevelstreamnext
  \endgroup
  \pgf@yb=\pgf@x
  \advance\pgf@ya by-\pgf@yb
  \pgfpathrectangle
    {\pgfqpoint{\pgf@yb}{\pgf@xc}}%
    {\pgfqpoint{\pgf@ya}{\pgf@xb}}%
  \pgfkeysvalueof{/pgf/at end bar}%
}%


% This handler is very similar to \pgfplothandlerlineto, but it
% produces CONSTANT connected pieces of the form
%
%          x
%          |
%   x---   |
%   |  x----
% x-|
%
% Example:
%
% \pgfplothandlerconstantlineto
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerconstantlineto}{}{%
  point macro=\pgf@plot@const@line@handler
}%

\def\pgf@plot@const@line@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@y}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@const@line@handler@@%
}%
\def\pgf@plot@const@line@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@yb\pgf@plot@const@line@handler@last\relax
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@ya}%
}%

% A variant of \pgfplothandlerconstantlineto which places its mark on
% the right line ends.
%
%       |---x
% ---x  |
%    |--x
% x
%
% Example:
%
% \pgfplothandlerconstantlinetomarkright
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerconstantlinetomarkright}{}{%
  point macro=\pgf@plot@const@line@mark@right@handler
}%

\def\pgf@plot@const@line@mark@right@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@x}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@const@line@mark@right@handler@@%
}%
\def\pgf@plot@const@line@mark@right@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@yb\pgf@plot@const@line@handler@last\relax
  \pgfpathlineto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@xa}%
}%

% A variant of \pgfplothandlerconstantlineto which places its mark on
% the middle of the line segment.
%
%               ----x
%               |
%   --x---      |
%   |    |--x----
% x--
%
% Example:
%
% \pgfplothandlerconstantlinetomarkmid
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerconstantlinetomarkmid}{}{%
  point macro=\pgf@plot@const@line@mark@mid@handler
}%

\def\pgf@plot@const@line@mark@mid@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\global\pgf@x=\the\pgf@x\space\global\pgf@y=\the\pgf@y\space}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@const@line@mark@mid@handler@@%
}%
\def\pgf@plot@const@line@mark@mid@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@plot@const@line@handler@last
  \pgf@xc=.5\pgf@xa
  \advance\pgf@xc by.5\pgf@x
  \pgfpathlineto{\pgfqpoint{\pgf@xc}{\pgf@y}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xc}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\global\pgf@x=\the\pgf@x\space\global\pgf@y=\the\pgf@y\space}%
}%

% This handler is in fact a variant of \pgfplothandlerconstantlineto,
% but it does not draw vertical lines. It produces a sequence of
% line-to and move-to operations such that plot marks are placed at
% each right end:
%
%          ---x
%   ---x
%       ---x
% --x
%
% Example:
%
% \pgfplothandlerjumpmarkright
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerjumpmarkright}{}{%
  point macro=\pgf@plot@jumpmarkright@handler
}%

\def\pgf@plot@jumpmarkright@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@x}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkright@handler@@%
}%
\def\pgf@plot@jumpmarkright@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@yb\pgf@plot@const@line@handler@last\relax
  \pgfpathmoveto{\pgfqpoint{\pgf@yb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@xa}%
}%

% This handler is in fact a variant of \pgfplothandlerconstantlineto,
% but it does not draw vertical lines. It produces a sequence of
% line-to and move-to operations such that plot marks are placed at
% each left end:
%
%          x---
%   x---
%       x---
% x--
%
% Example:
%
% \pgfplothandlerjumpmarkleft
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerjumpmarkleft}{}{%
  point macro=\pgf@plot@jumpmarkleft@handler
}%
\def\pgf@plot@jumpmarkleft@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@y}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@jumpmarkleft@handler@@%
}%
\def\pgf@plot@jumpmarkleft@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@yb\pgf@plot@const@line@handler@last\relax
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\the\pgf@ya}%
}%

% This handler is in fact a variant of
% \pgfplothandlerconstantlinetomarkmid,
% but it does not draw vertical lines. It produces a sequence of
% line-to and move-to operations such that plot marks are placed like
%
%             ----x
%
%   --x--
%       --x----
% x--
%
% Example:
%
% \pgfplothandlerjumpmarkmid
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerjumpmarkmid}{}{%
  point macro=\pgf@plot@jump@mark@mid@handler
}%

\def\pgf@plot@jump@mark@mid@handler#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@const@line@handler@last{\global\pgf@x=\the\pgf@x\space\global\pgf@y=\the\pgf@y\space}%
  \pgf@plot@first@action{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@jump@mark@mid@handler@@%
}%
\def\pgf@plot@jump@mark@mid@handler@@#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgf@plot@const@line@handler@last
  \pgf@xc=.5\pgf@xa
  \advance\pgf@xc by.5\pgf@x
  \pgfpathlineto{\pgfqpoint{\pgf@xc}{\pgf@y}}%
  \pgfpathmoveto{\pgfqpoint{\pgf@xc}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@const@line@handler@last{\global\pgf@x=\the\pgf@x\space\global\pgf@y=\the\pgf@y\space}%
}%


% This handler converts each point in a stream into a line from the
% origin to the point's coordinate, resulting in a ``star''.
%
% Example:
%
% \pgfplothandlerpolarcomb
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerpolarcomb}{}{%
  point macro=\pgf@plot@polarcomb@handler
}%

\def\pgf@plot@polarcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}%




% This handler draws a given mark at each point.
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
%
% Example:
%
% \pgfplothandlermark{\pgfuseplotmark{*}}
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlermark}{#1}{%
  start={
    \def\pgf@plot@mark{%
      \ifnum\pgf@plot@mark@count<\pgf@plot@mark@repeat\relax%
      \else%
        \global\pgf@plot@mark@count=0\relax%
        #1%
      \fi%
    }%
    \global\pgf@plot@mark@count=\pgf@plot@mark@repeat\relax%
    \global\advance\pgf@plot@mark@count by-\pgf@plot@mark@phase\relax%
  },
  point macro=\pgf@plot@mark@handler
}%

\newcount\pgf@plot@mark@count
\def\pgf@plot@mark@phase{0}%

\def\pgf@plot@mark@handler#1{%
  \global\advance\pgf@plot@mark@count by1\relax%
  {\pgftransformshift{#1}\pgf@plot@mark}%
}%


% Set the repeat count for marks. For example, if 3 is given as a
% value, only every third point will get a mark.
%
% #1 = repeat count
%
% Example:
%
% \pgfsetplotmarkrepeat{2}

\def\pgfsetplotmarkrepeat#1{\def\pgf@plot@mark@repeat{#1}}%
\pgfsetplotmarkrepeat{1}%


% Set the phase for marks. For example, if 3 is the repeat and 3 is
% the phase, already the first point will be marked.
%
% #1 = the index of the first point that should be marked.
%
% Example:
%
% \pgfsetplotmarkphase{3}

\def\pgfsetplotmarkphase#1{\def\pgf@plot@mark@phase{#1}}%
\pgfsetplotmarkphase{1}%



% This handler draws a given mark at those points whose number is
% given in the (pgffor-like) list.
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
% #2 = list of positions like "1,2,4,...,9,10"
%
% Example:
%
% \pgfplothandlermarklisted{\pgfuseplotmark{*}}{1,2,4,...,9}
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlermarklisted}{#1#2}{%
  start={
    \let\pgf@plot@mark@list=\pgfutil@empty%
    \edef\pgf@marshal{\noexpand\foreach\noexpand\pgf@temp in{#2}}
    \pgf@marshal{\xdef\pgf@plot@mark@list{\pgf@plot@mark@list(\pgf@temp)}}%
    \def\pgf@plot@mark{%
      \edef\pgf@marshal{\noexpand\pgfutil@in@{(\the\pgf@plot@mark@count)}{\pgf@plot@mark@list}}%
      \pgf@marshal%
      \ifpgfutil@in@#1\fi%
    }%
    \global\pgf@plot@mark@count=\pgf@plot@mark@repeat\relax%
    \global\advance\pgf@plot@mark@count by-\pgf@plot@mark@phase\relax%
  },
  point macro=\pgf@plot@mark@handler
}%

% \def\pgfplothandlermarklisted#1#2{%
%   \let\pgf@plot@mark@list=\pgfutil@empty%
%   \edef\pgf@marshal{\noexpand\foreach\noexpand\pgf@temp in{#2}}
%   \pgf@marshal{\xdef\pgf@plot@mark@list{\pgf@plot@mark@list(\pgf@temp)}}%
%   \pgf@plothandlermark{%
%     \edef\pgf@marshal{\noexpand\pgfutil@in@{(\the\pgf@plot@mark@count)}{\pgf@plot@mark@list}}%
%     \pgf@marshal%
%     \ifpgfutil@in@#1\fi}%
% }%


% Define a new plot mark for use with \pgfplotmark.
%
% #1 = a plot mark mnemonic
% #2 = code for drawing the mark
%
% Example:
%
% \pgfdeclareplotmark{*}{\pgfpathcircle{\pgfpointorigin}{2pt}\pgfusepathqfill}

\def\pgfdeclareplotmark#1#2{\expandafter\def\csname pgf@plot@mark@#1\endcsname{#2}}%


% Set the size of plot marks. For circles, this will be the radius,
% for other shapes it should be about half the width/height.
%
% Example:
%
% \pgfsetplotmarksize{1pt}

\def\pgfsetplotmarksize#1{\pgfmathsetlength\pgfplotmarksize{#1}}%

\newdimen\pgfplotmarksize
\pgfplotmarksize=2pt


% Insert a plot mark's code at the origin.
%
% #1 = plot mark mnemonic
%
% Example:
%
% \pgfuseplotmark{*}

\def\pgfuseplotmark#1{\csname pgf@plot@mark@#1\endcsname}%


% A stroke-filled circle mark

\pgfdeclareplotmark{*}
{%
  \pgfpathellipse{\pgfpointorigin}{\pgfqpoint{\pgfplotmarksize}{0sp}}{\pgfqpoint{0sp}{\pgfplotmarksize}}%
  \pgfusepathqfillstroke
}%


% A plus-sign like mark

\pgfdeclareplotmark{+}
{%
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}%
  \pgfusepathqstroke
}%


% An x-shaped mark

\pgfdeclareplotmark{x}
{%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
  \pgfusepathqstroke
}%

% See pgflibraryplotmarks for more plot marks




% This handler turns creates a series of straight line segments
% between consecutive points, but leaving /pgf/gap around stream point
% space.
%
% Example:
%
% \pgfplothandlergaplineto
% \pgfplotxyfile{mytable}

\pgfkeys{/pgf/gap around stream point/.initial=1.5pt}%

\pgfdeclareplothandler{\pgfplothandlergaplineto}{}{%
  point macro=\pgf@plot@gap@lineto@handler@initial,
  jump macro=\pgf@plot@gap@next@moveto
}%

\def\pgf@plot@gap@next@moveto{%
  \global\let\pgf@plotstreampoint=\pgf@plot@gap@lineto@handler@initial%
}%

\def\pgf@plot@gap@lineto@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@gap@lineto@last{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@gap@lineto@handler%
}%

\def\pgf@plot@gap@lineto@handler#1{%
  % Ok, compute normalized line vector
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@gap@lineto@next{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \pgf@process{\pgfpointnormalised{\pgfpointdiff{\pgf@plot@gap@lineto@last}{\pgf@plot@gap@lineto@next}}}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgfpathmoveto{\pgfpointadd{\pgfpointscale{\pgfkeysvalueof{/pgf/gap
          around stream point}}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}{\pgf@plot@gap@lineto@last}}%
  \pgfpathlineto{\pgfpointadd{\pgfpointscale{\pgfkeysvalueof{/pgf/gap
          around stream point}}{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}}{\pgf@plot@gap@lineto@next}}%
  \global\let\pgf@plot@gap@lineto@last=\pgf@plot@gap@lineto@next%
}%




% This handler works like \pgfplothandlergaplineto, only the last
% point is connected to the first point, creating a closed curve
% space.
%
% Example:
%
% \pgfplothandlergapcycle
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlergapcycle}{}{%
  point macro=\pgf@plot@gap@cycle@handler@initial,
  jump macro=\pgf@plot@gapcycle@next@moveto,
  end macro=\pgf@plot@gap@cycle@handler@finish,
  start={\global\let\pgf@plot@gap@cycle@first\relax}
}%

\def\pgf@plot@gapcycle@next@moveto{%
  \pgf@plot@gap@cycle@handler@finish%
  \global\let\pgf@plot@gap@cycle@first=\relax%
  \global\let\pgf@plotstreampoint=\pgf@plot@gap@cycle@handler@initial%
}%

\def\pgf@plot@gap@cycle@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@gap@cycle@last{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plot@gap@cycle@first=\pgf@plot@gap@cycle@last%
  \global\let\pgf@plotstreampoint=\pgf@plot@gap@cycle@handler%
}%

\def\pgf@plot@gap@cycle@handler#1{%
  % Ok, compute normalized line vector
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@gap@cycle@next{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \pgf@process{\pgfpointnormalised{\pgfpointdiff{\pgf@plot@gap@cycle@last}{\pgf@plot@gap@cycle@next}}}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgfpathmoveto{\pgfpointadd{\pgfpointscale{\pgfkeysvalueof{/pgf/gap
          around stream point}}{\pgfqpoint{\pgf@xc}{\pgf@yc}}}{\pgf@plot@gap@cycle@last}}%
  \pgfpathlineto{\pgfpointadd{\pgfpointscale{\pgfkeysvalueof{/pgf/gap
          around stream point}}{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}}{\pgf@plot@gap@cycle@next}}%
  \global\let\pgf@plot@gap@cycle@last=\pgf@plot@gap@cycle@next%
}%

\def\pgf@plot@gap@cycle@handler@finish{%
  \ifx\pgf@plot@gap@cycle@first\relax%
  \else
    \pgf@plot@gap@cycle@handler{\pgf@plot@gap@cycle@first}%
  \fi
}%



\endinput

% Local Variables:
% tab-width: 2
% End:


==> pgflibraryshapes.arrows.code.tex <==
% Copyright 2018 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryshapes.arrows.code.tex}


% keys for shape single arrow
%
% /pgf/single arrow tip angle
% /pgf/single arrow head extend
% /pgf/single arrow head indent

\pgfkeys{/pgf/.cd,
    single arrow tip angle/.initial=90,
    single arrow head extend/.initial=.25cm,
    single arrow head indent/.initial=0cm,
}%

% Shape single arrow
%
%
\pgfdeclareshape{single arrow}{%
    \savedmacro\getsinglearrowpoints{%
        %
        % Get the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \edef\xoutersep{\the\pgf@x}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \edef\youtersep{\the\pgf@y}%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@xa.5\wd\pgfnodeparttextbox%
        \advance\pgf@xa.5\pgflinewidth%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@ya.5\ht\pgfnodeparttextbox%
        \advance\pgf@ya.5\dp\pgfnodeparttextbox%
        \advance\pgf@ya.5\pgflinewidth%
        \ifpgfshapeborderusesincircle%
            \ifdim\pgf@xa<\pgf@ya%
                \pgf@xa\pgf@ya%
            \fi%
            \pgf@xa1.41421\pgf@xa%
            \pgf@ya\pgf@xa%
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \ifdim\xoutersep>\youtersep\relax%
                \let\youtersep\xoutersep%
            \else%
                \let\xoutersep\youtersep%
            \fi%
        \else%
            %
            % Round the rotation.
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \pgfmathmod@{\rotate}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Calculate the width and height of the node
            % contents, according to any border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@x\pgf@xa%
                \pgf@xa\pgf@ya%
                \pgf@ya\pgf@x%
                \let\pgfmathresult\xoutersep%
                \let\xoutersep\youtersep%
                \let\youtersep\pgfmathresult%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@x\pgf@xa%
                    \pgf@xa\pgf@ya%
                    \pgf@ya\pgf@x%
                    \let\pgfmathresult\xoutersep%
                    \let\xoutersep\youtersep%
                    \let\youtersep\pgfmathresult%
                \fi%
            \fi%
        \fi%
        \addtosavedmacro\rotate%
        %
        % Get some useful trig stuff.
        %
        \pgfmathdivide{\pgfkeysvalueof{/pgf/single arrow tip angle}}{2}%
        \let\halftipangle\pgfmathresult%
        \pgfmathcosec@{\halftipangle}%
        \let\cosechalftipangle\pgfmathresult%
        \pgfmathcos@{\halftipangle}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima\cosechalftipangle\pgfutil@tempdima%
        \edef\cothalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgfmathreciprocal@{\pgfmathresult}%
        \let\sechalftipangle\pgfmathresult%
        \pgfmathsin@{\halftipangle}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima\sechalftipangle\pgfutil@tempdima%
        \edef\tanhalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
        %
        % Get the single arrow head extend, and adjust for minimum width.
        %
        \pgf@xb\pgf@ya%
        \pgf@xb\cothalftipangle\pgf@xb%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/single arrow head extend}}%
        \pgf@yc\pgf@xc%
        \advance\pgf@xc\pgf@ya%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@xc<.5\pgfutil@tempdimb%
            \pgfutil@tempdimb.5\pgfutil@tempdimb%
            \pgfmathdivide@{\pgfmath@tonumber{\pgfutil@tempdimb}}{\pgfmath@tonumber{\pgf@xc}}%
            \pgf@ya\pgfmathresult\pgf@ya%
            \pgf@xc\pgfmathresult\pgf@xc%
            \pgf@yc\pgfmathresult\pgf@yc%
            \pgf@xb\pgfmathresult\pgf@xb%
        \fi%
        %
        % Now calculate the height of the arrow and adjust for minimum height.
        %
        \advance\pgf@xc-\pgf@ya%
        \pgf@xc\cothalftipangle\pgf@xc%
        \pgf@xa2.0\pgf@xa%
        \advance\pgf@xa\pgf@xb%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@xa<\pgfutil@tempdimb%
            \pgf@xa\pgfutil@tempdimb%
        \fi%
        \advance\pgf@xa-\pgf@xb%
        \pgf@xa.5\pgf@xa%
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/single arrow head indent}}%
        %
        % Now:
        %
        % xa - .5 * width of the node minus xb.
        % ya - .5 * height of the node contents.
        % xb - distance from the end of the node contents to the arrow tip.
        % xc - distance from the end of the node contents to the back end of the arrow head.
        % yc - distance from the top of the node contents to the top end of the arrow head.
        %
        \pgfsavepgf@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \pgfsavepgf@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt%
        }%
        \pgfsavepgf@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        %
        % As the arrow is symmetrical it can be described by only four points:
        %
        \pgfsavepgf@process\arrowtip{%
            \pgf@x\pgf@xa%
            \advance\pgf@x\pgf@xb%
            \pgf@y0pt\relax%
        }%
        \pgfsavepgf@process\beforearrowtip{%
            \pgf@x\pgf@xa%
            \advance\pgf@x-\pgf@xc%
            \pgf@y\pgf@ya%
            \advance\pgf@y\pgf@yc%
        }%
        \pgfsavepgf@process\beforearrowhead{%
            \pgf@x\pgf@xa%
            \advance\pgf@x-\pgf@xc%
            \advance\pgf@x\pgfutil@tempdima%
            \pgf@y\pgf@ya%
        }%
        \pgfsavepgf@process\afterarrowtail{%
            \pgf@x-\pgf@xa%
            \pgf@y\pgf@ya%
        }%
        %
        % Calculate the anchor point at the arrow tip...
        %
        \pgfsavepgf@process\arrowtipanchor{%
            \pgfpointadd{\centerpoint}{\arrowtip}%
            \pgf@xa\xoutersep\relax%
            \advance\pgf@x\cosechalftipangle\pgf@xa%
        }%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \edef\externalradius{\the\pgf@x}%
        \addtosavedmacro\externalradius%
        %
        % ...and the rest of the points.
        %
        \pgfmathanglebetweenlines{\beforearrowtip}{\beforearrowhead}{\beforearrowtip}{\arrowtip}%
        \pgf@xa\xoutersep\relax%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima.5\pgfutil@tempdima%
        \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \advance\pgfutil@tempdima-\halftipangle pt\relax%
        %
        \pgfsavepgf@process\beforearrowtipanchor{%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
            \pgf@xb\pgf@x%
            \pgf@yb\pgf@y%
            \pgf@process{\pgfpointadd{\centerpoint}{\beforearrowtip}}%
            \advance\pgf@x\pgf@xb%
            \advance\pgf@y\pgf@yb%
        }%
        \pgfmathanglebetweenpoints{\beforearrowhead}{\beforearrowtip}%
        \pgfutil@tempdima-\pgfmathresult pt\relax%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfutil@tempdima.5\pgfutil@tempdima%
        \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgf@xa\xoutersep\relax%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfsavepgf@process\beforearrowheadanchor{%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
            \pgf@xb\pgf@x%
            \pgf@yb\pgf@y%
            \pgf@process{\pgfpointadd{\centerpoint}{\beforearrowhead}}%
            \advance\pgf@x\pgf@xb%
            \advance\pgf@y\pgf@yb%
        }%
        \pgfsavepgf@process\afterarrowtailanchor{%
            \pgfpointadd{\centerpoint}{\afterarrowtail}%
            \advance\pgf@x-\xoutersep\relax%
            \advance\pgf@y\youtersep\relax%
        }%
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\beforearrowtipanchor}%
        \let\center@angle@beforearrowtip\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\beforearrowheadanchor}%
        \let\center@angle@beforearrowhead\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\afterarrowtailanchor}%
        \let\center@angle@afterarrowtail\pgfmathresult%
        \addtosavedmacro\center@angle@beforearrowtip%
        \addtosavedmacro\center@angle@beforearrowhead%
        \addtosavedmacro\center@angle@afterarrowtail%
        %
        \pgfmathanglebetweenpoints{\midpoint}{\beforearrowtipanchor}%
        \let\mid@angle@beforearrowtip\pgfmathresult%
        \pgfmathanglebetweenpoints{\midpoint}{\beforearrowheadanchor}%
        \let\mid@angle@beforearrowhead\pgfmathresult%
        \pgfmathanglebetweenpoints{\midpoint}{\afterarrowtailanchor}%
        \let\mid@angle@afterarrowtail\pgfmathresult%
        \addtosavedmacro\mid@angle@beforearrowtip%
        \addtosavedmacro\mid@angle@beforearrowhead%
        \addtosavedmacro\mid@angle@afterarrowtail%
        %
        \pgfmathanglebetweenpoints{\basepoint}{\beforearrowtipanchor}%
        \let\base@angle@beforearrowtip\pgfmathresult%
        \pgfmathanglebetweenpoints{\basepoint}{\beforearrowheadanchor}%
        \let\base@angle@beforearrowhead\pgfmathresult%
        \pgfmathanglebetweenpoints{\basepoint}{\afterarrowtailanchor}%
        \let\base@angle@afterarrowtail\pgfmathresult%
        \addtosavedmacro\base@angle@beforearrowtip%
        \addtosavedmacro\base@angle@beforearrowhead%
        \addtosavedmacro\base@angle@afterarrowtail%
        %
        \addtosavedmacro\arrowtipanchor%
        \addtosavedmacro\beforearrowtipanchor%
        \addtosavedmacro\beforearrowheadanchor%
        \addtosavedmacro\afterarrowtailanchor%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+0.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \getsinglearrowpoints%
        \let\pgf@singlearrow@referencepoint\midpoint%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid west}{%
        \getsinglearrowpoints%
        \let\pgf@singlearrow@referencepoint\midpoint%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \getsinglearrowpoints%
        \let\pgf@singlearrow@referencepoint\basepoint%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{base west}{%
        \getsinglearrowpoints%
        \let\pgf@singlearrow@referencepoint\basepoint%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south east}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{south west}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \getsinglearrowpoints%
        \csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{before head}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{\beforearrowheadanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{before tip}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{\beforearrowtipanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{tip}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{\arrowtipanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{after tip}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{after head}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{before tail}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{after tail}{%
        \getsinglearrowpoints%
        \pgfmathrotatepointaround{\afterarrowtailanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{tail}{%
        \getsinglearrowpoints%
        \pgfpointlineattime{0.5}{%
            \pgfmathrotatepointaround{\afterarrowtailanchor}{\centerpoint}{\rotate}%
        }%
        {%
            \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
            {\centerpoint}{\rotate}%
        }%
    }%
    \backgroundpath{%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            \pgfpathmoveto{\arrowtip}%
            \pgfpathlineto{\beforearrowtip}%
            \pgfpathlineto{\beforearrowhead}%
            \pgfpathlineto{\afterarrowtail}%
            \pgfpathlineto{\afterarrowtail\pgf@y-\pgf@y}%
            \pgfpathlineto{\beforearrowhead\pgf@y-\pgf@y}%
            \pgfpathlineto{\beforearrowtip\pgf@y-\pgf@y}%
        }%
        \pgfpathclose%
    }%
    \anchorborder{%
        \pgfsavepgf@process\externalpoint{}%
        \getsinglearrowpoints%
        \pgfutil@ifundefined{pgf@singlearrow@referencepoint}{\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@singlearrow@referencepoint}%
        \pgfsavepgf@process\externalpoint{%
            \externalpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \referencepoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya}%
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        \pgf@x\externalangle pt\relax%
        \ifx\referencepoint\midpoint%
            \pgf@xa\mid@angle@beforearrowtip pt\relax%
            \pgf@xb\mid@angle@beforearrowhead pt\relax%
            \pgf@xc\mid@angle@afterarrowtail pt\relax%
        \else%
            \ifx\referencepoint\basepoint%
                \pgf@xa\base@angle@beforearrowtip pt\relax%
                \pgf@xb\base@angle@beforearrowhead pt\relax%
                \pgf@xc\base@angle@afterarrowtail pt\relax%
            \else%
                \pgf@xa\center@angle@beforearrowtip pt\relax%
                \pgf@xb\center@angle@beforearrowhead pt\relax%
                \pgf@xc\center@angle@afterarrowtail pt\relax%
            \fi%
        \fi%
        \ifdim\pgf@x<\pgf@xa%
            \let\firstpoint\arrowtipanchor%
            \let\secondpoint\beforearrowtipanchor%
        \else%
            \ifdim\pgf@x<\pgf@xb%
                \ifdim\pgf@xb<\pgf@xa%
                    \let\firstpoint\arrowtipanchor%
                    \let\secondpoint\beforearrowtipanchor%
                \else%
                    \let\firstpoint\beforearrowheadanchor%
                    \let\secondpoint\beforearrowtipanchor%
                \fi%
            \else%
                \ifdim\pgf@x<\pgf@xc%
                    \let\firstpoint\beforearrowheadanchor%
                    \let\secondpoint\afterarrowtailanchor%
                \else%
                    \pgf@xc-\pgf@xc%
                    \advance\pgf@xc360pt\relax%
                    \ifdim\pgf@x<\pgf@xc%
                        \let\firstpoint\afterarrowtailanchor%
                        \pgfsavepgf@process\secondpoint{%
                            \pgfpointadd{%
                                \pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
                                \pgf@y-\pgf@y%
                            }{\centerpoint}%
                        }%
                    \else%
                        \pgf@xa-\pgf@xa%
                        \advance\pgf@xa360pt\relax%
                        \pgf@xb-\pgf@xb%
                        \advance\pgf@xb360pt\relax%
                        \ifdim\pgf@x<\pgf@xa%
                            \ifdim\pgf@x<\pgf@xb%
                                \pgfsavepgf@process\firstpoint{%
                                    \pgfpointadd{%
                                            \pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
                                            \pgf@y-\pgf@y%
                                    }{\centerpoint}%
                                }%
                                \pgfsavepgf@process\secondpoint{%
                                    \pgfpointadd{%
                                        \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                                        \pgf@y-\pgf@y%
                                    }{\centerpoint}%
                                }%
                            \else%
                                \ifdim\pgf@xb<\pgf@xa%
                                    \pgfsavepgf@process\firstpoint{%
                                        \pgfpointadd{%
                                                \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                                                \pgf@y-\pgf@y%
                                        }{\centerpoint}%
                                    }%
                                \else%
                                    \pgfsavepgf@process\firstpoint{%
                                        \pgfpointadd{%
                                                \pgfpointdiff{\centerpoint}{\arrowtipanchor}%
                                                \pgf@y-\pgf@y%
                                        }{\centerpoint}%
                                    }%
                                \fi%
                                \pgfsavepgf@process\secondpoint{%
                                        \pgfpointadd{%
                                            \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                                            \pgf@y-\pgf@y%
                                        }{\centerpoint}%
                                    }%
                            \fi%
                        \else%
                            \pgfsavepgf@process\firstpoint{%
                                \pgfpointadd{%
                                    \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                                    \pgf@y-\pgf@y%
                                }{\centerpoint}%
                            }%
                            \let\secondpoint\arrowtipanchor%
                        \fi%
                    \fi%
                \fi%
            \fi%
        \fi%
        \pgfsavepgf@process\firstpoint{%
            \pgfmathrotatepointaround{\firstpoint}{\centerpoint}{\rotate}%
        }%
        \pgfsavepgf@process\secondpoint{%
            \pgfmathrotatepointaround{\secondpoint}{\centerpoint}{\rotate}%
        }%
        \pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
            {\firstpoint}{\secondpoint}%
    }%
}%







% keys for shape double arrow
%
% /pgf/double arrow tip angle
% /pgf/double arrow head sep

\pgfkeys{/pgf/.cd,
    double arrow tip angle/.initial=90,
    double arrow head extend/.initial=.25cm,
    double arrow head indent/.initial=0cm,
}%

% Shape double arrow
%
%
\pgfdeclareshape{double arrow}{%
    \savedmacro\getdoublearrowpoints{%
        %
        % Get the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \edef\xoutersep{\the\pgf@x}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \edef\youtersep{\the\pgf@y}%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@xa.5\wd\pgfnodeparttextbox%
        \advance\pgf@xa.5\pgflinewidth%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@ya.5\ht\pgfnodeparttextbox%
        \advance\pgf@ya.5\dp\pgfnodeparttextbox%
        \advance\pgf@ya.5\pgflinewidth%
        \ifpgfshapeborderusesincircle%
            \ifdim\pgf@xa<\pgf@ya%
                \pgf@xa\pgf@ya%
            \fi%
            \pgf@xa1.41421\pgf@xa%
            \pgf@ya\pgf@xa%
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \ifdim\xoutersep>\youtersep\relax%
                \let\youtersep\xoutersep%
            \else%
                \let\xoutersep\youtersep%
            \fi%
        \else%
            %
            % Round the rotation.
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}
            \pgfmathmod@{\rotate}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Calculate the width and height of the node
            % contents, according to any border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@x\pgf@xa%
                \pgf@xa\pgf@ya%
                \pgf@ya\pgf@x%
                \let\pgfmathresult\xoutersep%
                \let\xoutersep\youtersep%
                \let\youtersep\pgfmathresult%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@x\pgf@xa%
                    \pgf@xa\pgf@ya%
                    \pgf@ya\pgf@x%
                    \let\pgfmathresult\xoutersep%
                    \let\xoutersep\youtersep%
                    \let\youtersep\pgfmathresult%
                \fi%
            \fi%
        \fi%
        \addtosavedmacro\rotate%
        %
        % Get some useful trig stuff.
        %
        \pgfmathdivide{\pgfkeysvalueof{/pgf/double arrow tip angle}}{2}%
        \let\halftipangle\pgfmathresult%
        \pgfmathcosec@{\halftipangle}%
        \let\cosechalftipangle\pgfmathresult%
        \pgfmathcos@{\halftipangle}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima\cosechalftipangle\pgfutil@tempdima%
        \edef\cothalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgfmathreciprocal@{\pgfmathresult}%
        \let\sechalftipangle\pgfmathresult%
        \pgfmathsin@{\halftipangle}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima\sechalftipangle\pgfutil@tempdima%
        \edef\tanhalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
        %
        % Get the double arrow head extend, and adjust for minimum width.
        %
        \pgf@xb\pgf@ya%
        \pgf@xb\cothalftipangle\pgf@xb%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/double arrow head extend}}%
        \pgf@yc\pgf@xc%
        \advance\pgf@xc\pgf@ya%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@xc<.5\pgfutil@tempdimb%
            \pgfutil@tempdimb.5\pgfutil@tempdimb%
            \pgfmathdivide@{\pgfmath@tonumber{\pgfutil@tempdimb}}{\pgfmath@tonumber{\pgf@xc}}%
            \pgf@ya\pgfmathresult\pgf@ya%
            \pgf@xc\pgfmathresult\pgf@xc%
            \pgf@yc\pgfmathresult\pgf@yc%
            \pgf@xb\pgfmathresult\pgf@xb%
        \fi%
        %
        % Now calculate the height of the arrow and adjust for minimum height.
        %
        \advance\pgf@xc-\pgf@ya%
        \pgf@xc\cothalftipangle\pgf@xc%
        \advance\pgf@xa\pgf@xb%
        \pgf@xa2.0\pgf@xa%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@xa<\pgfutil@tempdimb%
            \pgf@xa\pgfutil@tempdimb%
        \fi%
        \pgf@xa.5\pgf@xa%
        \advance\pgf@xa-\pgf@xb%
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/double arrow head indent}}%
        %
        % Now:
        %
        % xa - .5 * width of the node minus xb.
        % ya - .5 * height of the node contents.
        % xb - distance from the end of the node contents to the arrow tip.
        % xc - distance from the end of the node contents to the back end of the arrow head.
        % yc - distance from the top of the node contents to the top end of the arrow head.
        %
        \pgfsavepgf@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \pgfsavepgf@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt%
        }%
        \pgfsavepgf@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        %
        % As the arrow is symmetrical it can be described by only 3 points:
        %
        \pgfsavepgf@process\arrowtip{%
            \pgf@x\pgf@xa%
            \advance\pgf@x\pgf@xb%
            \pgf@y0pt\relax%
        }%
        \pgfsavepgf@process\beforearrowtip{%
            \pgf@x\pgf@xa%
            \advance\pgf@x-\pgf@xc%
            \pgf@y\pgf@ya%
            \advance\pgf@y\pgf@yc%
        }%
        \pgfsavepgf@process\beforearrowhead{%
            \pgf@x\pgf@xa%
            \advance\pgf@x-\pgf@xc%
            \advance\pgf@x\pgfutil@tempdima%
            \pgf@y\pgf@ya%
        }%
        %
        % Calculate the anchor point at the arrow tip.
        %
        \pgfsavepgf@process\arrowtipanchor{%
            \pgfpointadd{\centerpoint}{\arrowtip}%
            \pgf@xa\xoutersep\relax%
            \advance\pgf@x\cosechalftipangle\pgf@xa%
        }%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \edef\externalradius{\the\pgf@x}%
        \addtosavedmacro\externalradius%
        %
        %
        \pgfmathanglebetweenlines{\beforearrowtip}{\beforearrowhead}{\beforearrowtip}{\arrowtip}%
        \pgf@xa\xoutersep\relax%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \pgfutil@tempdima.5\pgfutil@tempdima%
        \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \advance\pgfutil@tempdima-\halftipangle pt\relax%
        \pgfsavepgf@process\beforearrowtipanchor{%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
            \pgf@xb\pgf@x%
            \pgf@yb\pgf@y%
            \pgf@process{\pgfpointadd{\centerpoint}{\beforearrowtip}}%
            \advance\pgf@x\pgf@xb%
            \advance\pgf@y\pgf@yb%
        }%
        \pgfmathanglebetweenpoints{\beforearrowhead}{\beforearrowtip}%
        \pgfutil@tempdima-\pgfmathresult pt\relax%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfutil@tempdima.5\pgfutil@tempdima%
        \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgf@xa\xoutersep\relax%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfsavepgf@process\beforearrowheadanchor{%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
            \pgf@xb\pgf@x%
            \pgf@yb\pgf@y%
            \pgf@process{\pgfpointadd{\centerpoint}{\beforearrowhead}}%
            \advance\pgf@x\pgf@xb%
            \advance\pgf@y\pgf@yb%
        }%
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\beforearrowtipanchor}%
        \let\center@angle@beforearrowtip\pgfmathresult%
        \addtosavedmacro\center@angle@beforearrowtip%
        %
        \pgfmathanglebetweenpoints{\midpoint}{\beforearrowtipanchor}%
        \let\mid@angle@beforearrowtip\pgfmathresult%
        \addtosavedmacro\mid@angle@beforearrowtip%
        %
        \pgfmathanglebetweenpoints{\basepoint}{\beforearrowtipanchor}%
        \let\base@angle@beforearrowtip\pgfmathresult%
        \addtosavedmacro\base@angle@beforearrowtip%
        %
        \addtosavedmacro\arrowtipanchor%
        \addtosavedmacro\beforearrowtipanchor%
        \addtosavedmacro\beforearrowheadanchor%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+0.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \getdoublearrowpoints%
        \let\pgf@singlearrow@referencepoint\midpoint%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid west}{%
        \getdoublearrowpoints%
        \let\pgf@singlearrow@referencepoint\midpoint%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \getdoublearrowpoints%
        \let\pgf@singlearrow@referencepoint\basepoint%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{base west}{%
        \getdoublearrowpoints%
        \let\pgf@singlearrow@referencepoint\basepoint%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south east}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{south west}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \getdoublearrowpoints%
        \csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{before head 1}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{\beforearrowheadanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{before tip 1}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{\beforearrowtipanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{tip 1}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{\arrowtipanchor}{\centerpoint}{\rotate}%
    }%
    \anchor{after tip 1}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{after head 1}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{before head 2}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{before tip 2}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{tip 2}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\arrowtipanchor}%
                \pgf@x-\pgf@x%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{after tip 2}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                \pgf@x-\pgf@x%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \anchor{after head 2}{%
        \getdoublearrowpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                \pgf@x-\pgf@x%
            }{\centerpoint}}%
        {\centerpoint}{\rotate}%
    }%
    \backgroundpath{%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            \pgfpathmoveto{\arrowtip}%
            \pgfpathlineto{\beforearrowtip}%
            \pgfpathlineto{\beforearrowhead}%
            \pgfpathlineto{\beforearrowhead\pgf@x-\pgf@x}%
            \pgfpathlineto{\beforearrowtip\pgf@x-\pgf@x}%
            \pgfpathlineto{\arrowtip\pgf@x-\pgf@x}%
            \pgfpathlineto{\beforearrowtip\pgf@x-\pgf@x\pgf@y-\pgf@y}%
            \pgfpathlineto{\beforearrowhead\pgf@x-\pgf@x\pgf@y-\pgf@y}%
            \pgfpathlineto{\beforearrowhead\pgf@y-\pgf@y}%
            \pgfpathlineto{\beforearrowtip\pgf@y-\pgf@y}%
        }%
        \pgfpathclose%
    }%
    \anchorborder{%
        \pgfsavepgf@process\externalpoint{}%
        \getdoublearrowpoints%
        \pgfutil@ifundefined{pgf@singlearrow@referencepoint}{\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@singlearrow@referencepoint}%
        \pgfsavepgf@process\externalpoint{%
            \externalpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \referencepoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya}%
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        \pgf@x\externalangle pt\relax%
        \ifx\referencepoint\midpoint%
            \pgf@xa\mid@angle@beforearrowtip pt\relax%
        \else%
            \ifx\referencepoint\basepoint%
                \pgf@xa\base@angle@beforearrowtip pt\relax%
            \else%
                \pgf@xa\center@angle@beforearrowtip pt\relax%
            \fi%
        \fi%
        \ifdim\pgf@x<180pt\relax%
            \ifdim\pgf@x<\pgf@xa%
                \let\firstpoint\arrowtipanchor%
                \let\secondpoint\beforearrowtipanchor%
            \else%
                \pgf@xa-\pgf@xa%
                \advance\pgf@xa180pt\relax%
                \ifdim\pgf@x<\pgf@xa%
                    \let\firstpoint\beforearrowheadanchor%
                    \pgfsavepgf@process\secondpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                            \pgf@x-\pgf@x
                            }{\centerpoint}}%
                \else%
                    \pgfsavepgf@process\firstpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                            \pgf@x-\pgf@x
                            }{\centerpoint}}%
                    \pgfsavepgf@process\secondpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\arrowtipanchor}%
                            \pgf@x-\pgf@x%
                            \pgf@y-\pgf@y%
                        }{\centerpoint}}%
                \fi%
            \fi%
        \else%
            \pgf@xa-\pgf@xa%
            \advance\pgf@xa360pt\relax%
            \ifdim\pgf@x<\pgf@xa%
                \pgf@xa-\pgf@xa%
                \advance\pgf@xa540pt\relax%
                \ifdim\pgf@x<\pgf@xa%
                    \pgfsavepgf@process\firstpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\arrowtipanchor}%
                            \pgf@x-\pgf@x%
                        }{\centerpoint}}%
                    \pgfsavepgf@process\secondpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
                            \pgf@x-\pgf@x%
                            \pgf@y-\pgf@y%
                        }{\centerpoint}}%
                \else%
                    \pgfsavepgf@process\firstpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                            \pgf@x-\pgf@x%
                            \pgf@y-\pgf@y%
                        }{\centerpoint}}%
                    \pgfsavepgf@process\secondpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
                            \pgf@y-\pgf@y%
                        }{\centerpoint}}%
                \fi%
            \else%
                \pgfsavepgf@process\firstpoint{%
                        \pgfpointadd{%
                            \pgfpointdiff{\beforearrowtipanchor}{\centerpoint}%
                            \pgf@x-\pgf@x%
                        }{\centerpoint}}%
                \let\secondpoint\arrowtipanchor%
            \fi%
        \fi%
        \pgfsavepgf@process\firstpoint{%
            \pgfmathrotatepointaround{\firstpoint}{\centerpoint}{\rotate}%
        }%
        \pgfsavepgf@process\secondpoint{%
            \pgfmathrotatepointaround{\secondpoint}{\centerpoint}{\rotate}%
        }%
        \pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
            {\firstpoint}{\secondpoint}%
    }%
}%




%
% Internal macros for the arrow box/shape.
%
\def\pgf@lib@arrowbox@parsearrowlength#1#2#3{%
    \edef\pgf@lib@temp{#3}%
    \edef\pgf@lib@marshal{%
        \noexpand\pgfutil@in@{none}{\pgf@lib@temp}%
    }%
    \pgf@lib@marshal%
    \ifpgfutil@in@%
        #10pt\relax%
    \else%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \expandafter#1\pgf@lib@temp\relax\pgfmath@%
        %
        \edef\pgf@lib@marshal{%
            \noexpand\pgfutil@in@{from center}{\pgf@lib@temp}%
        }%
        \pgf@lib@marshal%
        \ifpgfutil@in@%
        \else%
            \ifdim#1>0pt\relax%
                \advance#1#2\relax%
            \fi%
        \fi%
    \fi}%

\def\pgf@lib@arrowbox@parsearrows#1{%
    \pgfkeys{/pgf/.cd,%
        arrow box west arrow=0pt,
        arrow box east arrow=0pt,
        arrow box south arrow=0pt,
        arrow box north arrow=0pt
    }%
    \def\pgf@lib@arrowbox@extend{0pt}%
    \edef\pgf@lib@temp{#1}%
    \expandafter\pgf@lib@arrowbox@@parsearrows\pgf@lib@temp,\pgf@lib@arrowbox@parsearrows,
}%


\def\pgf@lib@arrowbox@@parsearrows#1,{%
    \ifx\pgf@lib@arrowbox@parsearrows#1%
        \let\pgflib@next\relax%
    \else%
        \pgfutil@in@:{#1}%
        \ifpgfutil@in@%
            \pgf@lib@arrowbox@getextend#1\pgf@lib%
        \else%
            \def\pgf@lib@arrowbox@direction{#1}%
        \fi%
        \edef\pgf@marshal{%
            \noexpand\pgfkeys{/pgf/arrow box  \pgf@lib@arrowbox@direction\space arrow=\pgf@lib@arrowbox@extend}%
        }%
        \pgf@marshal%
        \let\pgflib@next\pgf@lib@arrowbox@@@parsearrows%
    \fi%
    \pgflib@next%
}%
\def\pgf@lib@arrowbox@@@parsearrows{%
    \pgfutil@ifnextchar x{\relax\pgf@lib@arrowbox@@parsearrows}{\relax\pgf@lib@arrowbox@@parsearrows}%
}%

\def\pgf@lib@arrowbox@getextend#1:#2\pgf@lib{%
    \def\pgf@lib@arrowbox@direction{#1}%
    \def\pgf@lib@arrowbox@extend{#2}%
}%

%
% /pgf/arrow box north arrow
% /pgf/arrow box south arrow
% /pgf/arrow box west arrow
% /pgf/arrow box east arrow
% /pgf/arrow box arrows
% /pgf/arrow box shaft width
% /pgf/arrow box head extend
% /pgf/arrow box head indent
% /pgf/arrow box tip angle
%
\pgfkeys{/pgf/.cd,
    arrow box west arrow/.initial=.5cm,
    arrow box east arrow/.initial=.5cm,
    arrow box south arrow/.initial=.5cm,
    arrow box north arrow/.initial=.5cm,
    arrow box shaft width/.initial=.125cm,
    arrow box head extend/.initial=.125cm,
    arrow box head indent/.initial=0cm,
    arrow box tip angle/.initial=90,
}%

%
% arrow box/Shape.
%
\pgfdeclareshape{arrow box}{%
    \saveddimen\shaftwidth{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box shaft width}}%
    }%
    %
    % Calculate far the arrows extend from the center of the node.
    %
    \savedmacro\arrowboxpoints{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@x<.5\pgf@xa%
            \pgf@x.5\pgf@xa%
        \fi%
        \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@y<.5\pgf@ya%
            \pgf@y.5\pgf@ya%
        \fi%
        \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        %
        \edef\halfboxwidth{\the\pgf@x}%
        \edef\halfboxheight{\the\pgf@y}%
        \pgfextract@process\arrowboxcorner{}%
        \addtosavedmacro\arrowboxcorner%
        %
        \pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxwidth}%
            {\pgfkeysvalueof{/pgf/arrow box west arrow}}%
        \edef\westextend{\the\pgf@x}%
        \addtosavedmacro\westextend%
        %
        \pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxwidth}%
            {\pgfkeysvalueof{/pgf/arrow box east arrow}}%
        \edef\eastextend{\the\pgf@x}%
        \addtosavedmacro\eastextend%
        %
        \pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxheight}%
            {\pgfkeysvalueof{/pgf/arrow box north arrow}}%
        \edef\northextend{\the\pgf@x}%
        \addtosavedmacro\northextend%
        %
        \pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxheight}%
            {\pgfkeysvalueof{/pgf/arrow box south arrow}}%
        \edef\southextend{\the\pgf@x}%
        \addtosavedmacro\southextend%
    }%
    \saveddimen\arrowheadextend{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head extend}}%
    }%
    \saveddimen\arrowheadindent{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head indent}}%
    }%
    %
    % Calculate the `miter' angle for the outer sep at the arrow tip.
    %
    \savedmacro\arrowtipmiterangle{%
        \pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\arrowtipmiterangle\pgfmathresult%
    }%
    %
    % Calculate the `miter' angle for the outer sep at the point just
    % before the arrow tip.
    %
    \savedmacro\arrowheadangles{%
        %
        % Calculate the `miter' angle and its cosecant at the arrow tip...
        %
        \pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\arrowtipmiterangle\pgfmathresult%
        \addtosavedmacro\arrowtipmiterangle%
        \pgfmathcosec@{\arrowtipmiterangle}%
        \let\cosecarrowtipmiterangle\pgfmathresult%
        \addtosavedmacro\cosecarrowtipmiterangle%
        %
        % ...before the arrow head...
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head extend}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/arrow box head indent}}%
        \ifdim\pgf@y=0pt\relax%
            \def\pgfmathresult{90}%
        \else%
            \ifdim\pgf@y<0pt\relax%
                \pgfmathdivide@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
                \pgfmathatan@{\pgfmathresult}%
                \pgfmathadd@{\pgfmathresult}{180}%
            \else%
                \pgfmathdivide@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
                \pgfmathatan@{\pgfmathresult}%
            \fi%
        \fi%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\beforearrowheadmiterangle\pgfmathresult%
        \addtosavedmacro\beforearrowheadmiterangle%
        \pgfmathcosec@{\beforearrowheadmiterangle}%
        \let\cosecbeforearrowheadmiterangle\pgfmathresult%
        \addtosavedmacro\cosecbeforearrowheadmiterangle%
        %
        % ...and before the arrow tip.
        %
        \pgfutil@tempdima-\arrowtipmiterangle pt\relax%
        \advance\pgfutil@tempdima90pt\relax%
        \pgfutil@tempdimb\beforearrowheadmiterangle pt\relax%
        \pgfutil@tempdimb2.0\pgfutil@tempdimb%
        \advance\pgfutil@tempdimb-90pt\relax%
        \advance\pgfutil@tempdima\pgfutil@tempdimb%
        \divide\pgfutil@tempdima2\relax%
        \edef\beforearrowtipmiterangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \addtosavedmacro\beforearrowtipmiterangle%
        \pgfmathcosec@{\beforearrowtipmiterangle}%
        \let\cosecbeforearrowtipmiterangle\pgfmathresult%
        \addtosavedmacro\cosecbeforearrowtipmiterangle%
    }%
    \saveddimen\outerxsep{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    }%
    \saveddimen\outerysep{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer ysep}}%
    }%
    %
    % Calculate the (path) point immediately prior to an arrow tip.
    %
    \savedanchor\beforearrowtip{%
        \pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \pgfmathcot@{\pgfmathresult}%
        \let\cothalfangle\pgfmathresult%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/arrow box shaft width}}%
        \pgf@y.5\pgf@y%
        \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/arrow box head extend}}%
        \pgf@y\pgf@y%
        \pgf@x\cothalfangle\pgf@y%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \let\pgf@lib@shapes@arrowbox@referencepoint\midpoint%
            \csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{\eastextend}{0pt}};
        \else%
            \arrowboxcorner%
            \pgf@xa\pgf@x%
            \midpoint%
            \advance\pgf@x\pgf@xa%
        \fi%
    }%
    \anchor{mid west}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \let\pgf@lib@shapes@arrowbox@referencepoint\midpoint%
            \csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{-\westextend}{0pt}};
        \else%
            \arrowboxcorner%
            \pgf@xa\pgf@x%
            \midpoint%
            \advance\pgf@x-\pgf@xa%
        \fi%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \let\pgf@lib@shapes@arrowbox@referencepoint\basepoint%
            \csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{\eastextend}{0pt}};
        \else%
            \arrowboxcorner%
            \pgf@xa\pgf@x%
            \basepoint%
            \advance\pgf@x\pgf@xa%
        \fi%
    }%
    \anchor{base west}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \let\pgf@lib@shapes@arrowbox@referencepoint\basepoint%
            \csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{-\westextend}{0pt}};
        \else%
            \arrowboxcorner%
            \pgf@xa\pgf@x%
            \basepoint%
            \advance\pgf@x-\pgf@xa%
        \fi%
    }%
    \anchor{north}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \csname pgf@anchor@arrow box@north arrow tip\endcsname%
        \else%
            \pgfpointadd{\centerpoint}{\arrowboxcorner}%
            \pgf@ya\pgf@y%
            \centerpoint%
            \pgf@y\pgf@ya%
        \fi%
    }%
    \anchor{south}{%
        \arrowboxpoints%
        \ifdim\southextend>0pt\relax%
            \csname pgf@anchor@arrow box@south arrow tip\endcsname%
        \else%
            \pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@y-\pgf@y}%
            \pgf@ya\pgf@y%
            \centerpoint%
            \pgf@y\pgf@ya%
        \fi%
    }%
    \anchor{east}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \csname pgf@anchor@arrow box@east arrow tip\endcsname%
        \else%
            \pgfpointadd{\centerpoint}{\arrowboxcorner}%
            \pgf@xa\pgf@x%
            \centerpoint%
            \pgf@x\pgf@xa%
        \fi%
    }%
    \anchor{west}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \csname pgf@anchor@arrow box@west arrow tip\endcsname%
        \else%
            \pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x}%
            \pgf@xa\pgf@x%
            \centerpoint%
            \pgf@x\pgf@xa%
        \fi%
    }%
    \anchor{north east}{%
        \arrowboxpoints%
        \pgfpointadd{\centerpoint}{\arrowboxcorner}%
    }%
    \anchor{north west}{%
        \arrowboxpoints%
        \pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x}%
    }%
    \anchor{south west}{%
        \arrowboxpoints%
        \pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x\pgf@y-\pgf@y}%
    }%
    \anchor{south east}{%
        \arrowboxpoints%
        \pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@y-\pgf@y}%
    }%
    \anchor{before east arrow}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@y\shaftwidth\relax%
                \pgf@y.5\pgf@y%
                \advance\pgf@y\outerysep\relax%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{before east arrow head}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{before east arrow tip}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                }%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{east arrow tip}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \centerpoint%
            \advance\pgf@x\eastextend\relax%
            \pgf@xa\outerxsep\relax%
            \pgfmathcosec@{\arrowtipmiterangle}%
            \advance\pgf@x\pgfmathresult\pgf@xa%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{after east arrow tip}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                }%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{after east arrow head}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{after east arrow}{%
        \arrowboxpoints%
        \ifdim\eastextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@y\shaftwidth\relax%
                \pgf@y.5\pgf@y%
                \advance\pgf@y\outerysep\relax%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    %
    \anchor{before west arrow}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@x-\pgf@x%
                \pgf@y\shaftwidth\relax%
                \pgf@y.5\pgf@y%
                \advance\pgf@y\outerysep\relax%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{before west arrow head}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\westextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{before west arrow tip}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\westextend\relax%
                }%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{west arrow tip}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \centerpoint%
            \advance\pgf@x-\westextend\relax%
            \pgf@xa\outerxsep\relax%
            \pgfmathcosec@{\arrowtipmiterangle}%
            \advance\pgf@x-\pgfmathresult\pgf@xa%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{after west arrow tip}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\westextend\relax%
                }%
                \pgf@x-\pgf@x%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{after west arrow head}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima180pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\westextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgf@x-\pgf@x%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    \anchor{after west arrow}{%
        \arrowboxpoints%
        \ifdim\westextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@y\shaftwidth\relax%
                \pgf@y.5\pgf@y%
                \advance\pgf@y\outerysep\relax%
                \pgf@x-\pgf@x%
            }%
        \else%
            \csname pgf@anchor@arrow box@west\endcsname%
        \fi%
    }%
    %
    \anchor{before north arrow}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@x-\shaftwidth\relax%
                \pgf@x.5\pgf@x%
                \advance\pgf@x-\outerxsep\relax%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{before north arrow head}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima270pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x-\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{before north arrow tip}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-90pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y-\pgf@xa%
                    \advance\pgf@y\northextend\relax%
                }%
                \pgf@x-\pgf@x%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{north arrow tip}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \centerpoint%
            \advance\pgf@y\northextend\relax%
            \pgf@ya\outerysep\relax%
            \pgfmathcosec@{\arrowtipmiterangle}%
            \advance\pgf@y\pgfmathresult\pgf@ya%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{after north arrow tip}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-90pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y-\pgf@xa%
                    \advance\pgf@y\northextend\relax%
                }%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{after north arrow head}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima270pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x-\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
                \pgf@x-\pgf@x%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    \anchor{after north arrow}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@x\shaftwidth\relax%
                \pgf@x.5\pgf@x%
                \advance\pgf@x\outerxsep\relax%
            }%
        \else%
            \csname pgf@anchor@arrow box@north\endcsname%
        \fi%
    }%
    %
    \anchor{before south arrow}{%
        \arrowboxpoints%
        \ifdim\southextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@x\shaftwidth\relax%
                \pgf@x.5\pgf@x%
                \advance\pgf@x\outerxsep\relax%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    \anchor{before south arrow head}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima270pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x-\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    \anchor{before south arrow tip}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-90pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y-\pgf@xa%
                    \advance\pgf@y\northextend\relax%
                }%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    \anchor{south arrow tip}{%
        \arrowboxpoints%
        \ifdim\southextend>0pt\relax%
            \centerpoint%
            \advance\pgf@y-\southextend\relax%
            \pgf@ya\outerysep\relax%
            \pgfmathcosec@{\arrowtipmiterangle}%
            \advance\pgf@y-\pgfmathresult\pgf@ya%
        \else%
            \csname pgf@anchor@arrow box@east\endcsname%
        \fi%
    }%
    \anchor{after south arrow tip}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima\arrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
                    \advance\pgfutil@tempdima-90pt\relax%
                    \pgfutil@tempdimb\outerxsep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y-\pgf@xa%
                    \advance\pgf@y\northextend\relax%
                }%
                \pgf@x-\pgf@x%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    \anchor{after south arrow head}{%
        \arrowboxpoints%
        \ifdim\northextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \pgfpointadd{%
                    \arrowheadangles%
                    \pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
                    \advance\pgfutil@tempdima270pt\relax%
                    \pgfutil@tempdimb\outerysep\relax%
                    \pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
                    \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x-\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    \anchor{after south arrow}{%
        \arrowboxpoints%
        \ifdim\southextend>0pt\relax%
            \pgfpointadd{\centerpoint}{%
                \arrowboxcorner%
                \pgf@x-\shaftwidth\relax%
                \pgf@x.5\pgf@x%
                \advance\pgf@x-\outerxsep\relax%
                \pgf@y-\pgf@y%
            }%
        \else%
            \csname pgf@anchor@arrow box@south\endcsname%
        \fi%
    }%
    %
    \backgroundpath{%
        \arrowboxpoints%
        \pgfextract@process\arrowboxcorner{%
            \arrowboxcorner%
            \pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
            \pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
        }%
        {%
            \pgftransformshift{\centerpoint}%
            \pgfpathmoveto{\arrowboxcorner}%
            \ifdim\eastextend>0pt\relax%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                }%
                \pgfpathlineto{%
                    \pgf@x\eastextend\relax%
                    \pgf@y0pt\relax%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                    \pgf@y-\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@x-\pgf@x%
                    \advance\pgf@x\eastextend\relax%
                    \advance\pgf@x\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y-.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y-.5\pgf@y%
                }%
            \fi%
            \pgfpathlineto{\arrowboxcorner\pgf@y-\pgf@y}%
            \ifdim\southextend>0pt\relax%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                    \pgf@y-\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@y\pgf@x%
                    \advance\pgf@y-\southextend\relax%
                    \advance\pgf@y-\arrowheadindent\relax%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@xa\pgf@y%
                    \pgf@y\pgf@x%
                    \advance\pgf@y-\southextend\relax%
                    \pgf@x\pgf@xa%
                }%
                \pgfpathlineto{%
                    \pgf@x0pt\relax%
                    \pgf@y-\southextend\relax%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@xa\pgf@y%
                    \pgf@y\pgf@x%
                    \advance\pgf@y-\southextend\relax%
                    \pgf@x-\pgf@xa%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@y\pgf@x%
                    \advance\pgf@y-\southextend\relax%
                    \advance\pgf@y-\arrowheadindent\relax%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x-.5\pgf@x%
                }%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x-.5\pgf@x%
                    \pgf@y-\pgf@y%
                }%
            \fi%
            \pgfpathlineto{\arrowboxcorner\pgf@x-\pgf@x\pgf@y-\pgf@y}%
            \ifdim\westextend>0pt\relax%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x-\pgf@x
                    \pgf@y\shaftwidth\relax%
                    \pgf@y-.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \advance\pgf@x-\westextend\relax%
                    \advance\pgf@x-\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y-.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \advance\pgf@x-\westextend\relax%
                    \pgf@y-\pgf@y%
                }%
                \pgfpathlineto{%
                    \pgf@x-\westextend\relax%
                    \pgf@y0pt\relax%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \advance\pgf@x-\westextend\relax%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \advance\pgf@x-\westextend\relax%
                    \advance\pgf@x-\arrowheadindent\relax%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x-\pgf@x%
                    \pgf@y\shaftwidth\relax%
                    \pgf@y.5\pgf@y%
                }%
            \fi%
            \pgfpathlineto{\arrowboxcorner\pgf@x-\pgf@x}%
            \ifdim\northextend>0pt\relax%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x-.5\pgf@x%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x-.5\pgf@x%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@xa\pgf@y%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \pgf@x-\pgf@xa%
                }%
                \pgfpathlineto{%
                    \pgf@x0pt\relax%
                    \pgf@y\northextend\relax%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@xa\pgf@y%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \pgf@x\pgf@xa%
                }%
                \pgfpathlineto{%
                    \beforearrowtip%
                    \pgf@y-\pgf@x%
                    \advance\pgf@y\northextend\relax%
                    \advance\pgf@y\arrowheadindent\relax%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
                \pgfpathlineto{%
                    \arrowboxcorner%
                    \pgf@x\shaftwidth\relax%
                    \pgf@x.5\pgf@x%
                }%
            \fi%
            \pgfpathclose%
        }%
    }%
    \anchorborder{%
        \pgfextract@process\externalpoint{}%
        \pgfutil@ifundefined{pgf@lib@shapes@arrowbox@referencepoint}%
            {\let\referencepoint\centerpoint}{\let\referencepoint\pgf@lib@shapes@arrowbox@referencepoint}%
        \pgfextract@process\externalpoint{%
            \pgfpointadd{\referencepoint}{\externalpoint}%
        }%
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \let\externalangle\pgfmathresult%
        \pgfmathanglebetweenpoints{\referencepoint}%
            {\csname pgf@anchor@arrow box@west\endcsname}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
            \pgfmathanglebetweenpoints{\referencepoint}%
                {\csname pgf@anchor@arrow box@north\endcsname}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                \pgfmathanglebetweenpoints{\referencepoint}%
                    {\csname pgf@anchor@arrow box@north east\endcsname}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@before east arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \def\firstpoint{east arrow tip}%
                        \def\secondpoint{before east arrow tip}%
                    \else%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@before east arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{before east arrow head}%
                            \def\secondpoint{before east arrow}%
                        \else%
                            \def\firstpoint{before east arrow}%
                            \def\secondpoint{north east}%
                        \fi%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@after north arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@after north arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{north east}%
                            \def\secondpoint{after north arrow}%
                        \else%
                            \def\firstpoint{after north arrow}%
                            \def\secondpoint{after north arrow head}%
                        \fi%
                    \else%
                        \def\firstpoint{after north arrow tip}%
                        \def\secondpoint{north arrow tip}%
                    \fi%
                \fi%
            \else%
                \pgfmathanglebetweenpoints{\referencepoint}%
                    {\csname pgf@anchor@arrow box@north west\endcsname}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@before north arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \def\firstpoint{north arrow tip}%
                        \def\secondpoint{before north arrow tip}%
                    \else%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@before north arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{before north head}%
                            \def\secondpoint{before north arrow}%
                        \else%
                            \def\firstpoint{before north arrow}%
                            \def\secondpoint{north west}%
                        \fi%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@after west arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@after west arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{north west}%
                            \def\secondpoint{after west arrow}%
                        \else%
                            \def\firstpoint{after west arrow}%
                            \def\secondpoint{after west arrow head}%
                        \fi%
                    \else%
                        \def\firstpoint{after west arrow tip}%
                        \def\secondpoint{west arrow tip}%
                    \fi%
                \fi%
            \fi%
        \else%
            \pgfmathanglebetweenpoints{\referencepoint}%
                {\csname pgf@anchor@arrow box@south arrow tip\endcsname}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                \pgfmathanglebetweenpoints{\referencepoint}%
                    {\csname pgf@anchor@arrow box@south west\endcsname}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@before west arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \def\firstpoint{west arrow tip}%
                        \def\secondpoint{before west arrow tip}%
                    \else%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@before west arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{before west arrow head}%
                            \def\secondpoint{before west arrow}%
                        \else%
                            \def\firstpoint{before west arrow}%
                            \def\secondpoint{south west}%
                        \fi%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@after south arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@after south arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{south west}%
                            \def\secondpoint{after south arrow}%
                        \else%
                            \def\firstpoint{after south arrow}%
                            \def\secondpoint{after south arrow head}%
                        \fi%
                    \else%
                        \def\firstpoint{after south arrow tip}%
                        \def\secondpoint{south arrow tip}%
                    \fi%
                \fi%
            \else%
                \pgfmathanglebetweenpoints{\referencepoint}%
                    {\csname pgf@anchor@arrow box@south east\endcsname}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@before south arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \def\firstpoint{south arrow tip}%
                        \def\secondpoint{before south arrow tip}%
                    \else%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@before south arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{before south arrow head}%
                            \def\secondpoint{before south arrow}%
                        \else%
                            \def\firstpoint{before south arrow}%
                            \def\secondpoint{south east}%
                        \fi%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\referencepoint}%
                        {\csname pgf@anchor@arrow box@after east arrow tip\endcsname}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax%
                        \pgfmathanglebetweenpoints{\referencepoint}%
                            {\csname pgf@anchor@arrow box@after east arrow\endcsname}%
                        \ifdim\externalangle pt<\pgfmathresult pt\relax%
                            \def\firstpoint{south east}%
                            \def\secondpoint{after east arrow}%
                        \else%
                            \def\firstpoint{after east arrow}%
                            \def\secondpoint{after east arrow head}%
                        \fi%
                    \else%
                        \def\firstpoint{after east arrow tip}%
                        \def\secondpoint{east arrow tip}%
                    \fi%
                \fi%
            \fi%
        \fi%
        \pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
            {\csname pgf@anchor@arrow box@\firstpoint\endcsname}%
            {\csname pgf@anchor@arrow box@\secondpoint\endcsname}%
    }%
}%




\endinput


==> pgflibraryshapes.callouts.code.tex <==
% Copyright 2018 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.symbols}%

% Keys for callouts
%
% Common to all callouts:
%    /pgf/callout absolute pointer
%    /pgf/callout relative pointer
%
% ellipse callout only:
%    /pgf/callout pointer arc
%
% rectangle callout only:
%    /pgf/callout pointer width
%
% cloud callout only:
%    /pgf/callout pointer start size
%    /pgf/callout pointer end size
%    /pgf/callout pointer segments
%
\newif\ifpgf@lib@callout@absolutepointer
\pgfkeys{/pgf/.cd,
    callout pointer arc/.initial=15,
    callout pointer width/.initial=.25cm,
    callout pointer start size/.initial=.2 of callout,
    callout pointer end size/.initial=.1 of callout,
    callout pointer segments/.initial=2,
    callout absolute pointer/.code={\pgf@lib@callout@makeabsolutepointer{#1}},
    callout relative pointer/.code={\pgf@lib@callout@makerelativepointer{#1}},
    callout pointer shorten/.initial=0cm,
}%



\def\pgf@lib@callout@makeabsolutepointer#1{%
    \pgf@lib@callout@absolutepointertrue%
    {%
        \pgftransformshift{#1}%
        \pgfmultipartnode{coordinate}{center}{pgf@lib@callout@pointer}{}%
    }%
}%

\def\pgf@lib@callout@makerelativepointer#1{%
    \pgf@lib@callout@absolutepointerfalse%
    \def\pgf@lib@callout@relativepointer{#1}%
}%
\pgfkeys{/pgf/callout relative pointer=\pgfpointpolar{300}{.5cm}}%


% Shape ellipse callout
%
%
\pgfdeclareshape{ellipse callout}{%
    \savedmacro\ellipsecalloutpoints{%
        %
        % Get the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@x>\pgf@y%
            \edef\outersep{\the\pgf@x}%
        \else%
            \edef\outersep{\the\pgf@y}%
        \fi%
        \addtosavedmacro\outersep%
        %
        % Calculate the node dimensions...
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@x1.4142136\pgf@x%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<.5\pgf@xa%
      \pgf@x.5\pgf@xa%
    \fi%
    %
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y.5\dp\pgfnodeparttextbox%
    \pgf@y1.4142136\pgf@y%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<.5\pgf@ya%
      \pgf@y.5\pgf@ya%
    \fi%
    %
    % ...without outer sep...
    %
    \edef\xpathradius{\the\pgf@x}%
    \edef\ypathradius{\the\pgf@y}%
    %
    % ...and width outer sep.
    %
    \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \edef\xradius{\the\pgf@x}%
    \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \edef\yradius{\the\pgf@y}%
    %
    \addtosavedmacro\xradius%
    \addtosavedmacro\xpathradius%
    \addtosavedmacro\yradius%
    \addtosavedmacro\ypathradius%
    %
      \pgfmathsetmacro\pointerarc{\pgfkeysvalueof{/pgf/callout pointer arc}}%
        \addtosavedmacro\pointerarc%
      %
      \pgfextract@process\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
      }%
      %
      % Get the relative pointer.
      %
      \ifpgf@lib@callout@absolutepointer%
      \else%
        \pgfextract@process\calloutpointer{%
                \pgfextract@process\borderpoint{%
                    \expandafter\pgfpointborderellipse\expandafter{\pgf@lib@callout@relativepointer}{\pgfqpoint{\xpathradius}{\ypathradius}}%
                }%
                \pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
                \let\pointerangle\pgfmathresult%
                \expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
                \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
                \edef\pointerradius{\pgfmathresult pt}%
                \pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
                \pgf@xa\pgf@x%
                \pgf@ya\pgf@y%
                \centerpoint%
                \advance\pgf@x\pgf@xa%
                \advance\pgf@y\pgf@ya%
            }%
            %
            \addtosavedmacro\calloutpointer%
            \pgf@lib@callouts@shortenpointer%
            \pgf@lib@ellipsecallout@getpoints%
        \addtosavedmacro\calloutpointeranchor%
        \addtosavedmacro\beforecalloutangle%
        \addtosavedmacro\aftercalloutangle%
    \fi%
  }%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt\relax%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
    \ellipsecalloutpoints%
    \pgfmathpointintersectionoflineandarc{\midpoint\advance\pgf@x\xradius}{\midpoint}%
        {\centerpoint}{270}{450}{\xradius and \yradius}%
  }%
  \anchor{mid west}{%
    \ellipsecalloutpoints%
    \pgfmathpointintersectionoflineandarc{\midpoint\advance\pgf@x-\xradius}{\midpoint}%
        {\centerpoint}{90}{270}{\xradius and \yradius}%
  }%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
    \ellipsecalloutpoints%
    \pgfmathpointintersectionoflineandarc{\basepoint\advance\pgf@x\xradius}{\basepoint}%
        {\centerpoint}{270}{450}{\xradius and \yradius}%
  }%
  \anchor{base west}{%
    \ellipsecalloutpoints%
    \pgfmathpointintersectionoflineandarc{\basepoint\advance\pgf@x-\xradius}{\basepoint}%
        {\centerpoint}{90}{270}{\xradius and \yradius}%
  }%
  \anchor{north}{%
    \ellipsecalloutpoints%
    \centerpoint%
    \advance\pgf@y\yradius\relax%
  }%
  \anchor{south}{%
    \ellipsecalloutpoints%
    \centerpoint%
    \advance\pgf@y-\yradius\relax%
  }%
  \anchor{east}{%
    \ellipsecalloutpoints%
    \centerpoint%
    \advance\pgf@x\xradius\relax%
  }%
  \anchor{west}{%
    \ellipsecalloutpoints%
    \centerpoint%
    \advance\pgf@x-\xradius\relax%
  }%
  \anchor{north west}{%
    \ellipsecalloutpoints%
    \pgf@xa\xradius\relax%
    \pgf@ya\yradius\relax%
    \centerpoint%
    \advance\pgf@y0.7071067\pgf@ya%
    \advance\pgf@x-0.7071067\pgf@xa%
  }%
  \anchor{north east}{%
    \ellipsecalloutpoints%
    \pgf@xa\xradius\relax%
    \pgf@ya\yradius\relax%
    \centerpoint%
    \advance\pgf@y0.7071067\pgf@ya%
    \advance\pgf@x0.7071067\pgf@xa%
  }%
  \anchor{south west}{%
    \ellipsecalloutpoints%
    \pgf@xa\xradius\relax%
    \pgf@ya\yradius\relax%
    \centerpoint%
    \advance\pgf@y-0.7071067\pgf@ya%
    \advance\pgf@x-0.7071067\pgf@xa%
  }%
  \anchor{south east}{%
    \ellipsecalloutpoints%
    \pgf@xa\xradius\relax%
    \pgf@ya\yradius\relax%
    \centerpoint%
    \advance\pgf@y-0.7071067\pgf@ya%
    \advance\pgf@x0.7071067\pgf@xa%
  }%
  \anchor{pointer}{%
    \ellipsecalloutpoints%
    \calloutpointeranchor%
    }%
  \backgroundpath{%
    \ellipsecalloutpoints%
    \ifpgf@lib@callout@absolutepointer%
        \pgfextract@process\calloutpointer{%
                \pgfpointanchor{pgf@lib@callout@pointer}{center}%
            }%
            \pgf@lib@callouts@shortenpointer%
            \pgf@lib@ellipsecallout@getpoints%
            \calloutpointeranchor%
            \ifx\pgf@node@name\pgfutil@empty%
            \else%
                \edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@node@name\noexpand\endcsname}%
                \edef\pgf@sh@@@temp{%
                    \noexpand\def\noexpand\calloutpointeranchor{%
                        \noexpand\pgf@x\the\pgf@x%
                        \noexpand\pgf@y\the\pgf@y%
                    }%
                }%
                \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}
            \fi%
        \fi%
        \pgfpathmoveto{\calloutpointer}%
        \pgfpathlineto{\aftercalloutpointer}%
        \ifdim\aftercalloutangle pt<\beforecalloutangle pt\relax%
            \pgfpatharc{\aftercalloutangle}{\beforecalloutangle}{\xpathradius and \ypathradius}%
        \else%
            \pgfpatharc{\aftercalloutangle}{360}{\xpathradius and \ypathradius}%
            \pgfpatharc{0}{\beforecalloutangle}{\xpathradius and \ypathradius}%
        \fi%
        \pgfpathclose%
  }%
  \anchorborder{%
    \pgfextract@process\externalpoint{}%
    \ellipsecalloutpoints%
    \pgfpointadd{\pgfpointborderellipse{\externalpoint}{\pgfpoint{\xradius}{\yradius}}%
    }{\centerpoint}%
  }%
}%

% Internal macro for calculating the points for the
% ellipse callout pointer.
%
% The following must be set up:
%
% \centerpoint    - the center of the ellipse.
% \calloutpointer - the location of the callout point.
% \pointerarc     - the width of the pointer.
% \xpathradius    - the x radius of the ellipse.
% \ypathradius    - the y radius of the ellipse.
%
\def\pgf@lib@ellipsecallout@getpoints{%
    \pgfextract@process\borderpoint{%
        \pgfpointborderellipse{%
            \centerpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \calloutpointer%
            \advance\pgf@x-\pgf@xa%
            \advance\pgf@y-\pgf@ya%
        }{\pgfqpoint{\xpathradius}{\ypathradius}}%
    }%
    \pgfmathangleonellipse{\borderpoint}{\xpathradius and \ypathradius}%
    \pgfutil@tempdima\pointerarc pt\relax%
    \pgfutil@tempdimb\pgfmathresult pt\relax%
    \advance\pgfutil@tempdimb-.5\pgfutil@tempdima%
    \ifdim\pgfutil@tempdimb<0pt\relax%
        \advance\pgfutil@tempdimb360pt\relax%
    \fi%
    \edef\beforecalloutangle{\pgfmath@tonumber{\pgfutil@tempdimb}}%
    \advance\pgfutil@tempdimb\pgfutil@tempdima%
    \ifdim\pgfutil@tempdimb<360pt\relax%
    \else%
        \advance\pgfutil@tempdimb-360pt\relax%
    \fi%
    \edef\aftercalloutangle{\pgfmath@tonumber{\pgfutil@tempdimb}}%
    %
    \pgfextract@process\beforecalloutpointer{%
        \pgfpointadd{\centerpoint}{%
            \pgfpointpolar{\beforecalloutangle}{\xpathradius and \ypathradius}%
        }%
    }%
    \pgfextract@process\aftercalloutpointer{%
        \pgfpointadd{\centerpoint}{%
            \pgfpointpolar{\aftercalloutangle}{\xpathradius and \ypathradius}%
        }%
    }%
    %
    % Calculate the pointer anchor.
    %
    \pgf@lib@callouts@pointeranchor%
}%


% If the callout pointer is very pointed and stroked, the anchor will be
% miles away from the end of the pointer which will (typically) be
% bevelled.
% Using outer sep=0pt is one solution, however, another is provided
% using this special key:
%
% /pgf/callout pointer anchor aspect
%
% which takes a value from 0 (ignore any outer sep) to 1 (use
% the full outer sep).

\pgfkeys{/pgf/callout pointer anchor aspect/.initial=1}%

% Internal macro for calculating the anchor for the callout pointer.
%
% Requires the following to be set up (points are anti-clockwise)
%
% \beforecalloutpointer - point on the border before the callout pointer
% \calloutpointer
% \aftercalloutpointer  - point on the border after the callout pointer
% \outersep             - the largest of the outer xsep or ysep.
%
\def\pgf@lib@callouts@pointeranchor{%
    \pgfutil@tempdimb\outersep\relax%
    %
    \pgfmathanglebetweenlines{\calloutpointer}{\aftercalloutpointer}{\calloutpointer}{\beforecalloutpointer}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \pgfutil@tempdima\pgfmathresult pt\relax%
    \pgfmathcosec@{\pgfmathresult}%
    \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
    \pgfmathanglebetweenpoints{\calloutpointer}{\aftercalloutpointer}%
    \advance\pgfutil@tempdima\pgfmathresult pt\relax%
    \advance\pgfutil@tempdima180pt\relax%
    %
    \pgfextract@process\calloutpointeranchor{%
        \pgfpointadd{%
            \pgfmathparse{\pgfkeysvalueof{/pgf/callout pointer anchor aspect}}%
            \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
        }{%
            \calloutpointer%
        }%
    }%
}%

\def\pgf@lib@callouts@shortenpointer{%
    \pgfextract@process\calloutpointer{%
        \pgfmathanglebetweenpoints{\calloutpointer}{\centerpoint}%
        \let\angle\pgfmathresult%
        \pgfmathsin@{\angle}%
        \let\sinpointerangle\pgfmathresult%
        \pgfmathcos@{\angle}%
        \let\cospointerangle\pgfmathresult%
        \pgfpointadd{\calloutpointer}{%
            \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/callout pointer shorten}}%
            \pgf@x\cospointerangle\pgfutil@tempdima%
            \pgf@y\sinpointerangle\pgfutil@tempdima%
        }%
    }%
}%


\pgfdeclareshape{rectangle callout}{%
    \savedmacro\rectanglecalloutpoints{%
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@x<.5\pgf@xa%
            \pgf@x.5\pgf@xa%
        \fi%
        \edef\xtemp{\the\pgf@x}%
        \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@y<.5\pgf@ya%
            \pgf@y.5\pgf@ya%
        \fi%
        \edef\ytemp{\the\pgf@y}%
        \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        %
        \edef\xlength{\the\pgf@x}%
        \edef\ylength{\the\pgf@y}%
        \addtosavedmacro\xlength%
        \addtosavedmacro\ylength%
        %
        \pgfmathsetlengthmacro\pointerwidth{\pgfkeysvalueof{/pgf/callout pointer width}}%
        \addtosavedmacro\pointerwidth%
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        %
        % Process the relative callout pointer.
        %
        \ifpgf@lib@callout@absolutepointer%
        \else%
            \pgfextract@process\calloutpointer{%
                \pgfextract@process\borderpoint{%
                    \expandafter\pgfpointborderrectangle\expandafter{\pgf@lib@callout@relativepointer}%
                        {\pgfqpoint{\xtemp}{\ytemp}}%
                }%
                \pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
                \let\pointerangle\pgfmathresult%
                \expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
                \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
                \edef\pointerradius{\pgfmathresult pt}%
                \pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
                \pgf@xa\pgf@x%
                \pgf@ya\pgf@y%
                \centerpoint%
                \advance\pgf@x\pgf@xa%
                \advance\pgf@y\pgf@ya%
            }%
            \pgf@lib@callouts@shortenpointer%
            \addtosavedmacro\calloutpointer%
            \pgf@lib@rectanglecallout@pointer%
            \addtosavedmacro\calloutpointeranchor%
            \addtosavedmacro\beforecalloutpointer%
            \addtosavedmacro\aftercalloutpointer%
            \addtosavedmacro\firstpoint%
            \addtosavedmacro\secondpoint%
            \addtosavedmacro\thirdpoint%
            \addtosavedmacro\fourthpoint%
        \fi%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5em}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \rectanglecalloutpoints%
        \midpoint%
        \advance\pgf@x\xlength\relax%
    }%
    \anchor{mid west}{%
        \rectanglecalloutpoints%
        \midpoint%
        \advance\pgf@x-\xlength\relax%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \rectanglecalloutpoints%
        \basepoint%
        \advance\pgf@x\xlength\relax%
    }%
    \anchor{base west}{%
        \rectanglecalloutpoints%
        \basepoint%
        \advance\pgf@x-\xlength\relax%
    }%
    \anchor{north}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@y\ylength\relax%
    }%
    \anchor{south}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@y-\ylength\relax%
    }%
    \anchor{east}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x\xlength\relax%
    }%
    \anchor{west}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x-\xlength\relax%
    }%
    \anchor{north east}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x\xlength\relax%
        \advance\pgf@y\ylength\relax%
    }%
    \anchor{south west}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x-\xlength\relax%
        \advance\pgf@y-\ylength\relax%
    }%
    \anchor{south east}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x\xlength\relax%
        \advance\pgf@y-\ylength\relax%
    }%
    \anchor{north west}{%
        \rectanglecalloutpoints%
        \centerpoint%
        \advance\pgf@x-\xlength\relax%
        \advance\pgf@y\ylength\relax%
    }%
    \anchor{pointer}{%
        \rectanglecalloutpoints%
        \calloutpointeranchor%
    }%
    \backgroundpath{%
        \rectanglecalloutpoints%
        \pgf@x\xlength\relax%
        \pgf@y\ylength\relax%
        \pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
        \edef\xtemp{\the\pgf@x}%
        \edef\ytemp{\the\pgf@y}%
        %
        % The absolute pointer must be calculated here because the
        % anchor of the shape (which is calculated after the saved
        % macros and points) affects how the pointer joins the
        % main rectangle.
        %
        \ifpgf@lib@callout@absolutepointer%
            \pgfextract@process\calloutpointer{%
                \pgfpointanchor{pgf@lib@callout@pointer}{center}%
            }%
            \pgf@lib@callouts@shortenpointer%
            \pgfmathsetlengthmacro\pointerwidth{\pgfkeysvalueof{/pgf/callout pointer width}}%
            \pgf@lib@rectanglecallout@pointer%
            %
            % \pgf@node@name = the shape name (from \pgfmultipartnode)
            %
            \ifx\pgf@node@name\pgfutil@empty%
            \else%
                %
                % Now hack an extra saved anchor \calloutpointeranchor,
                % with the new anchor for the callout pointer.
                %
                \edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@node@name\noexpand\endcsname}%
                \edef\pgf@sh@@@temp{%
                    \noexpand\def\noexpand\calloutpointeranchor{%
                        \noexpand\pgf@x\the\pgf@x%
                        \noexpand\pgf@y\the\pgf@y%
                    }%
                }%
                \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}%
            \fi%
        \fi%
        {%
            \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
            \pgfpathmoveto{\beforecalloutpointer}%
        }%
        \pgfpathlineto{\calloutpointer}%
        {%
            \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
            \pgfpathlineto{\aftercalloutpointer}%
        }%
        {%
            \pgftransformshift{\centerpoint}%
            \pgfpathlineto{\firstpoint}%
            \pgfpathlineto{\secondpoint}%
            \pgfpathlineto{\thirdpoint}%
            \pgfpathlineto{\fourthpoint}%
            {%
                \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
                \pgfpathclose%
            }%
        }
    }%
    \anchorborder{%
        \pgfextract@process\externalpoint{}%
        \rectanglecalloutpoints%
        \pgfpointadd{\centerpoint}%
        {%
            \pgfpointborderrectangle{\pgfpointadd{\centerpoint}{\externalpoint}}%
            {\pgfqpoint{\xlength}{\ylength}}%
        }%
    }%
}%



% \pgf@lib@rectanglecallout@pointer
%
% Internal macro for calculations relating to the rectangle callout.
%
% Requires the following to be set up:
%
% \calloutpointer - the location of the callout point.
% \xtemp          - the half width of the rectangle
% \ytemp          - the half height of the rectangle
% \pointerwidth   - the width of the pointer.
%
\def\pgf@lib@rectanglecallout@pointer{%
    %
    % Ensure that the pointer never connects to the main shape
    % too near to a corner. This is done for two reasons:
    % 1. It can look ugly.
    % 2. If the corners are rounded, a mess can result.
    %
    \pgfextract@process\borderpoint{%
            \pgfpointborderrectangle{%
                \centerpoint%
                \pgf@xa\pgf@x%
                \pgf@ya\pgf@y%
                \calloutpointer%
                \advance\pgf@x-\pgf@xa%
                \advance\pgf@y-\pgf@ya%
            }{\pgfqpoint{\xtemp}{\ytemp}}%
        }%
    \pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
    \let\borderangle\pgfmathresult%
    %
    \pgfutil@tempdima\pointerwidth\relax%
    \pgf@xa\xtemp\relax%
    \advance\pgf@xa-\pgfutil@tempdima%
    \pgf@ya\ytemp\relax%
    \advance\pgf@ya-\pgfutil@tempdima%
    %
    \pgf@process{%
        \pgfutil@ifundefined{pgf@corner@arc}{\pgfpointorigin}{%
            \expandafter\pgfqpoint\pgf@corner@arc}%
    }%
    \advance\pgf@xa-\pgf@x%
    \advance\pgf@ya-\pgf@y%
    %
    \borderpoint%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    %
    \pgf@xc0pt\relax%
    \pgf@yc0pt\relax%
    %
    \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{\ytemp}}%
    \ifdim\borderangle pt<\pgfmathresult pt\relax%
        \pgf@yc.5\pgfutil@tempdima%
        \ifdim\pgf@yb>\pgf@ya%
            \pgf@yb\pgf@ya%
        \fi%
        %
        % Establish the order for drawing the rectangle corners.
        %
        \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
        \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
        \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
        \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
    \else%
        \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{\ytemp}}%
        \ifdim\borderangle pt<\pgfmathresult pt\relax%
            \pgf@xc-.5\pgfutil@tempdima%
            \ifdim\pgf@xb>\pgf@xa%
                \pgf@xb\pgf@xa%
            \else%
                \ifdim\pgf@xb<-\pgf@xa%
                    \pgf@xb-\pgf@xa%
                \fi%
            \fi%
            \edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
            \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
            \edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
            \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
        \else%
            \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{-\ytemp}}%
            \ifdim\borderangle pt<\pgfmathresult pt\relax%
                \pgf@yc-.5\pgfutil@tempdima%
                \ifdim\pgf@yb>\pgf@ya%
                    \pgf@yb\pgf@ya%
                \else%
                    \ifdim\pgf@yb<-\pgf@ya%
                        \pgf@yb-\pgf@ya%
                    \fi%
                \fi%
                \edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                \edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                \edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                \edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
            \else%
                \pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{-\ytemp}}%
                \ifdim\borderangle pt<\pgfmathresult pt\relax%
                    \pgf@xc.5\pgfutil@tempdima%
                    \ifdim\pgf@xb>\pgf@xa%
                        \pgf@xb\pgf@xa%
                    \else%
                        \ifdim\pgf@xb<-\pgf@xa%
                            \pgf@xb-\pgf@xa%
                        \fi%
                    \fi%
                    \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                    \edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                    \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
                    \edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                \else%
                    \pgf@yc.5\pgfutil@tempdima%
                    \ifdim\pgf@yb<-\pgf@ya%
                        \pgf@yb-\pgf@ya%
                    \fi%
                    \edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
                    \edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
                    \edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
                    \edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
                \fi%
            \fi%
        \fi%
    \fi%
    \pgfextract@process\beforecalloutpointer{%
        \centerpoint%
        \advance\pgf@x\pgf@xb%
        \advance\pgf@y\pgf@yb%
        \advance\pgf@x-\pgf@xc%
        \advance\pgf@y-\pgf@yc%
    }%
    \pgfextract@process\aftercalloutpointer{%
        \centerpoint%
        \advance\pgf@x\pgf@xb%
        \advance\pgf@y\pgf@yb%
        \advance\pgf@x\pgf@xc%
        \advance\pgf@y\pgf@yc%
    }%
    %
    % Now calculate the pointer anchor.
    %
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@x>\pgf@y%
        \edef\outersep{\the\pgf@x}%
    \else%
        \edef\outersep{\the\pgf@y}%
    \fi%
    \pgf@lib@callouts@pointeranchor%
}%


% Internal macro for parsing the size of
% the cloud callout pointer.
%
% \pgf@x and \pgf@y should be set up as the
% width and height of the main shape.
%
% \pgf@xa and \pgf@ya are returned appropriately.
%
\def\pgf@lib@callout@setpointersize#1{%
    \edef\pgf@lib@callout@temp{#1}%
    \edef\pgf@marshall{\noexpand\pgfutil@in@{of callout}{\pgf@lib@callout@temp}}%
    \pgf@marshall%
    \ifpgfutil@in@%
        \expandafter\pgf@xa\expandafter\pgf@lib@callout@setpointerrelativesize%
            \pgf@lib@callout@temp\pgf@lib@stop\pgf@x%
        \expandafter\pgf@ya\expandafter\pgf@lib@callout@setpointerrelativesize%
            \pgf@lib@callout@temp\pgf@lib@stop\pgf@y%
    \else%
        \edef\pgf@marshall{\noexpand\pgfutil@in@{and}{\pgf@lib@callout@temp}}%
        \pgf@marshall%
        \ifpgfutil@in@%
            \expandafter\pgf@lib@callout@setpointerbothsizes\pgf@lib@callout@temp\pgf@lib@stop%
        \else%
            \pgfmathsetlength\pgf@xa{#1}%
            \pgfmathsetlength\pgf@ya{#1}%
        \fi%
    \fi%
}%
\def\pgf@lib@callout@setpointerrelativesize#1of callout#2\pgf@lib@stop{#1}%
\def\pgf@lib@callout@setpointerbothsizes#1and#2\pgf@lib@stop{%
    \pgfmathsetlength\pgf@xa{#2}%
    \pgfmathsetlength\pgf@ya{#2}%
}%

% Shape: cloud callout.
%
\pgfdeclareshape{cloud callout}{%
    \savedanchor\calloutpointer{%
        \pgfutil@ifundefined{pgf@sh@s@cloud}{%
            \pgferror{I cannot find the cloud shape. Please load the `symbol shapes' library}}{}%
        \pgf@sh@s@cloud%
        \pgf@sh@savedmacros%
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \ifpgf@lib@callout@absolutepointer%
      \else%
        \pgfextract@process\calloutpointer{%
                \pgfextract@process\borderpoint{%
                    \expandafter\pgfpointborderellipse\expandafter{\pgf@lib@callout@relativepointer}%
                        {\pgfqpoint{\xouterradius}{\youterradius}}%
                }%
                \pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
                \let\pointerangle\pgfmathresult%
                \expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
                \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
                \edef\pointerradius{\pgfmathresult pt}%
                \pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
                \pgf@xa\pgf@x%
                \pgf@ya\pgf@y%
                \centerpoint%
                \advance\pgf@x\pgf@xa%
                \advance\pgf@y\pgf@ya%
            }%
            \pgf@lib@callouts@shortenpointer%
        \fi%
    }%
    \anchor{pointer}{%
        \calloutpointer%
    }%
    \inheritsavedanchors[from=cloud]%
    \inheritanchor[from=cloud]{center}%
    \inheritanchor[from=cloud]{base}%
    \inheritanchor[from=cloud]{mid}%
    \inheritanchor[from=cloud]{north}%
    \inheritanchor[from=cloud]{south}%
    \inheritanchor[from=cloud]{east}%
    \inheritanchor[from=cloud]{west}%
    \inheritanchor[from=cloud]{north east}%
    \inheritanchor[from=cloud]{south west}%
    \inheritanchor[from=cloud]{south east}%
    \inheritanchor[from=cloud]{north west}%
    \inheritanchorborder[from=cloud]%
    \backgroundpath{%
        \pgf@sh@bg@cloud%
        \ifpgf@lib@callout@absolutepointer%
        \pgfextract@process\calloutpointer{%
                \pgfpointanchor{pgf@lib@callout@pointer}{center}%
            }%
            \ifx\pgf@node@name\pgfutil@empty%
            \else%
                \edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@node@name\noexpand\endcsname}%
                \edef\pgf@sh@@@temp{%
                    \noexpand\def\noexpand\calloutpointeranchor{%
                        \noexpand\pgf@x\the\pgf@x%
                        \noexpand\pgf@y\the\pgf@y%
                    }%
                }%
                \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}
            \fi%
        \fi%
        %
        \pgfextract@process\borderpoint{%
            \pgfpointadd{%
                \pgfpointborderellipse{\pgfpointdiff{\centerpoint}{\calloutpointer}}%
                        {\pgfqpoint{\xouterradius}{\youterradius}}%
            }{\centerpoint}%
        }%
        \pgf@lib@callouts@shortenpointer%
        \pgfmathanglebetweenpoints{\calloutpointer}{\centerpoint}%
        \let\angle\pgfmathresult%
        \pgfmathsin@{\angle}%
        \let\sinpointerangle\pgfmathresult%
        \pgfmathcos@{\angle}%
        \let\cospointerangle\pgfmathresult%
        %
        \pgf@x\xouterradius\relax%
        \pgf@x2.0\pgf@x%
        \pgf@y\yinnerradius\relax%
        \pgf@y2.0\pgf@y%
        \pgf@lib@callout@setpointersize{\pgfkeysvalueof{/pgf/callout pointer start size}}%
        \pgf@xb\pgf@xa%
        \pgf@yb\pgf@ya%
        \pgf@lib@callout@setpointersize{\pgfkeysvalueof{/pgf/callout pointer end size}}%
        \advance\pgf@xb-\pgf@xa%
        \advance\pgf@yb-\pgf@ya%
        %
        \pgfmathsetcount\c@pgf@counta{\pgfkeysvalueof{/pgf/callout pointer segments}}%
        \divide\pgf@xb\c@pgf@counta%
        \divide\pgf@yb\c@pgf@counta%
        %
        \pgf@process{\pgfpointdiff{\borderpoint}{\calloutpointer}}%
        \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \divide\pgfutil@tempdima\c@pgf@counta%
        %
        \pgfutil@tempdimb0pt\relax%
        \pgfmathloop%
        \ifnum\pgfmathcounter>\c@pgf@counta%
        \else%
            {%
                \pgf@xa.5\pgf@xa%
                \pgf@ya.5\pgf@ya%
                \edef\tempxradius{\the\pgf@xa}%
                \edef\tempyradius{\the\pgf@ya}%
                \pgfpathellipse%
                    {%
                        \calloutpointer%
                        \advance\pgf@x\cospointerangle\pgfutil@tempdimb%
                        \advance\pgf@y\sinpointerangle\pgfutil@tempdimb%
                    }%
                    {\pgfqpoint{\tempxradius}{0pt}}{\pgfqpoint{0pt}{\tempyradius}}%
            }%
            \advance\pgf@xa\pgf@xb%
            \advance\pgf@ya\pgf@yb%
            \advance\pgfutil@tempdimb\pgfutil@tempdima%
        \repeatpgfmathloop%
    }%
    %
    % Hack the puff anchors for the callout.
    %
    \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@cloud callout\endcsname{%
        \c@pgf@counta\puffs\relax%
        \pgfmathloop%
            \ifnum\c@pgf@counta>0\relax%
                \pgfutil@ifundefined{pgf@anchor@cloud callout@puff\space\the\c@pgf@counta}{%
                \expandafter\xdef\csname pgf@anchor@cloud callout@puff\space\the\c@pgf@counta\endcsname{%
                    \noexpand\pgf@sh@@cloudpuffanchor{\the\c@pgf@counta}%
                }%
            }{\c@pgf@counta0\relax}%
            \advance\c@pgf@counta-1\relax%
        \repeatpgfmathloop%
    }%
}%

\endinput


==> pgflibraryshapes.geometric.code.tex <==
% Copyright 2018 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryshapes.geometric.code.tex}

\pgfdeclareshape{ellipse}
%
% Draws a circle around the text
%
{%
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\radius{%
    %
    % Calculate ``height radius''
    %
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by\pgf@yb%
    %
    % Calculate ``width radius''
    %
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by\pgf@xb%
    %
    % Adjust
    %
    \pgf@x=1.4142136\pgf@x%
    \pgf@y=1.4142136\pgf@y%
    %
    % Adjust height, if necessary
    %
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<.5\pgf@yc%
      \pgf@y=.5\pgf@yc%
    \fi%
    %
    % Adjust width, if necessary
    %
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<.5\pgf@xc%
      \pgf@x=.5\pgf@xc%
    \fi%
    %
    % Add outer sep
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@x by\pgf@xb%
    \advance\pgf@y by\pgf@yb%
  }%

  %
  % Anchors
  %
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base}{\centerpoint\pgf@y=0pt}%
  \anchor{north}
  {
    \pgf@process{\radius}
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@y by\pgf@ya
  }%
  \anchor{south}
  {
    \pgf@process{\radius}
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@y by-\pgf@ya
  }%
  \anchor{west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa
  }%
  \anchor{mid west}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa%
    \pgfmathsetlength\pgf@y{.5ex}
  }%
  \anchor{base west}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa%
    \pgf@y=0pt
  }%
  \anchor{north west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@ya
  }%
  \anchor{south west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@ya
  }%
  \anchor{east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa
  }%
  \anchor{mid east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@y{.5ex}
  }%
  \anchor{base east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa%
    \pgf@y=0pt
  }%
  \anchor{north east}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@ya
  }%
  \anchor{south east}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@ya
  }%
  \anchorborder{%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      {\noexpand\radius}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%

  %
  % Background path
  %
  \backgroundpath
  {
    \pgf@process{\radius}%
    \pgfutil@tempdima=\pgf@x%
    \pgfutil@tempdimb=\pgf@y%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgfutil@tempdima by-\pgf@xb%
    \advance\pgfutil@tempdimb by-\pgf@yb%
    \pgfpathellipse{\centerpoint}{\pgfqpoint{\pgfutil@tempdima}{0pt}}{\pgfqpoint{0pt}{\pgfutil@tempdimb}}%
  }%
}%




% Set the recommended shape aspect ratio
%
% #1 = aspect ratio
%
% Example:
%
% \pgfsetshapeaspect{1.5}

% Keys for shape aspect ratio.
%
% /pgf/aspect         : recommended width/height quotient.
%
\pgfkeys{/pgf/.cd,
    aspect/.code={\pgfsetshapeaspect{#1}},% this for tikz...
    shape aspect/.initial=1,% but this is consistent with other pgfset stuff.
    shape aspect/.code={%
        \pgfkeys{/pgf/aspect=#1}%
        \pgfkeyssetvalue{/pgf/shape aspect}{#1}
    }%
}%


\def\pgfsetshapeaspect#1{%
  \def\pgfshapeaspect{#1}%
  % Invert
  \pgfutil@tempdima=#1pt%
  \pgfutil@tempdima=.125\pgfutil@tempdima%
  \c@pgf@counta=\pgfutil@tempdima\relax% 8192*determinant
  \pgfutil@tempdima=8192pt%
  \divide\pgfutil@tempdima by\c@pgf@counta%
  \edef\pgfshapeaspectinverse{\pgf@sys@tonumber{\pgfutil@tempdima}}%
}%

\pgfsetshapeaspect{1}%

\pgfdeclareshape{diamond}
{%
  \savedanchor\outernortheast{%
    %
    % Calculate width and height of the inner rectangle
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xc%
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yc%
    %
    % Calculate width and height of diamond
    %
    \pgf@x=\pgf@xa%
    \advance\pgf@x by\pgfshapeaspect\pgf@ya%
    \pgf@y=\pgfshapeaspectinverse\pgf@xa%
    \advance\pgf@y by\pgf@ya%
    %
    % Check against minimum height/width
    %
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgf@xb=.5\pgf@xb%
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \pgf@yb=.5\pgf@yb%
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    %
    % Add outer border
    %
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }%
  \savedanchor\text{%
    \pgf@x=-.5\wd\pgfnodeparttextbox%
    \pgf@y=-.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by.5\dp\pgfnodeparttextbox%
  }%

  %
  % Anchors
  %
  \anchor{text}{\text}%
  \anchor{center}{\pgfpointorigin}%
  \anchor{mid}{%
    \pgf@process{\text}%
    \pgf@x=0pt%
    \pgfmathsetlength\pgf@ya{.5ex}%
    \advance\pgf@y by\pgf@ya%
  }%
  \anchor{base}{\pgf@process{\text}\pgf@x=0pt}%
  \anchor{north}{\pgf@process{\outernortheast}\pgf@x=0pt}%
  \anchor{south}{\pgf@process{\outernortheast}\pgf@x=0pt\pgf@y=-\pgf@y}%
  \anchor{west}{\pgf@process{\outernortheast}\pgf@x=-\pgf@x\pgf@y=0pt}%
  \anchor{north west}{\pgf@process{\outernortheast}\pgf@x=-.5\pgf@x\pgf@y=.5\pgf@y}%
  \anchor{south west}{\pgf@process{\outernortheast}\pgf@x=-.5\pgf@x\pgf@y=-.5\pgf@y}%
  \anchor{east}{\pgf@process{\outernortheast}\pgf@y=0pt}%
  \anchor{north east}{\pgf@process{\outernortheast}\pgf@x=.5\pgf@x\pgf@y=.5\pgf@y}%
  \anchor{south east}{\pgf@process{\outernortheast}\pgf@x=.5\pgf@x\pgf@y=-.5\pgf@y}%
  \anchorborder{%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\outernortheast}%
    \ifdim\pgf@xa>0pt%
    \else%
      \pgf@x=-\pgf@x%
    \fi%
    \ifdim\pgf@ya>0pt%
    \else%
      \pgf@y=-\pgf@y%
    \fi%
    \edef\pgf@marshal{%
      \noexpand\pgfpointintersectionoflines
      {\noexpand\pgfpointorigin}
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\the\pgf@x}{0pt}}
      {\noexpand\pgfqpoint{0pt}{\the\pgf@y}}%
    }%
    \pgf@process{\pgf@marshal}%
  }%

  %
  % Background path
  %
  \backgroundpath{
    \pgf@process{\outernortheast}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@xc by-1.414213\pgf@xa%
    \advance\pgf@yc by-1.414213\pgf@ya%
    \pgfpathmoveto{\pgfqpoint{\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{-\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@yc}}%
    \pgfpathclose%
  }%
}%






\newif\ifpgf@lib@shapes@starouterradiususesratio
\pgf@lib@shapes@starouterradiususesratiotrue

% Keys for star shape
%
% /pgf/star points       : Number of points on the star.
% /pgf/star point height : The height of the outer star points.
% /pgf/star point ratio  : The ratio of the outer point and inner point radii.

\pgfkeys{/pgf/.cd,
    star points/.initial=5,
    star point height/.initial=.5cm,
    star point height/.code={%
        \def\pgf@lib@temp{#1}%
        \pgfkeyslet{/pgf/star point height}{\pgf@lib@temp}%
        \pgf@lib@shapes@starouterradiususesratiofalse%
    },
    star point ratio/.initial=1.5,
    star point ratio/.code={%
        \def\pgf@lib@temp{#1}%
        \pgfkeyslet{/pgf/star point ratio}{\pgf@lib@temp}%
        \pgf@lib@shapes@starouterradiususesratiotrue%
    },%
    star rotate/.style={/pgf/shape border rotate=#1},% For compatibility with 1.18
}%


% Shape star.
%
\pgfdeclareshape{star}{%
    \savedmacro\totalstarpoints{%
        \pgfmathsetcounter{pgf@counta}{\pgfkeysvalueof{/pgf/star points}}%
        \multiply\c@pgf@counta2\relax%
        \edef\totalstarpoints{\the\c@pgf@counta}%
    }%
    \savedmacro\anglestep{%
        \pgfmathdivide{180}{\pgfkeysvalueof{/pgf/star points}}%
        \let\anglestep\pgfmathresult%
    }%
    \savedmacro\calculateradii{%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \ifdim\pgf@y>\pgf@x%
            \pgf@x\pgf@y%
        \fi%
        %
        % Calculate the incircle radius.
        %
        \pgf@x1.41421\pgf@x%
        \edef\innerradius{\the\pgf@x}%
        %
        % Calculate the circumcircle radius.
        %
        % Use the star point height or the star point ratio?
        %
        \ifpgf@lib@shapes@starouterradiususesratio%
            \pgfmathparse{\pgfkeysvalueof{/pgf/star point ratio}}%
            \expandafter\pgf@x\pgfmathresult\pgf@x%
        \else%
            \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/star point height}}%
        \fi%
        \pgf@xc\pgf@x%
        %
        % Accommodate the larger of the minimum height/width.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@ya>\pgf@xa%
            \pgf@xa\pgf@ya%
        \fi%
        \ifdim\pgf@x<.5\pgf@xa%
        \pgf@x.5\pgf@xa%
       \fi%
       \edef\outerradius{\the\pgf@x}%
       %
       % If the outer radius has been enlarged, adjust the inner radius...
       %
       \ifdim\pgf@x>\pgf@xc%
        %
        % ...using the star point ratio, or...
        %
        \ifpgf@lib@shapes@starouterradiususesratio%
            \pgfmathreciprocal{\pgfkeysvalueof{/pgf/star point ratio}}%
            \pgf@xa\pgfmathresult\pgf@x\relax%
            \edef\innerradius{\the\pgf@xa}%
            \else%
                %
                % The star point height.
                %
                \pgf@xa\pgf@x\relax%
                \pgfmathaddtolength\pgf@xa{-\pgfkeysvalueof{/pgf/star point height}}%
                \edef\innerradius{\the\pgf@xa}%
            \fi%
        \fi%
        \edef\outerradius{\the\pgf@x}%
        %
        % Now calculate the anchor radii from the outer sep.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@ya>\pgf@xa%
            \pgf@xa\pgf@ya%
        \fi
        %
        % Take into account the miter length...
        %
        \pgfmathdivide{180}{\pgfkeysvalueof{/pgf/star points}}%
        \let\angletofirstpoint\pgfmathresult%
        \pgfmathmultiply@{\angletofirstpoint}{2}%
        \let\angletosecondpoint\pgfmathresult%
        %
        % ...for the outer radius...
        %
        \pgfmathanglebetweenlines%
            {\pgfqpointpolar{\angletofirstpoint}{\outerradius}}%
            {\pgfqpointpolar{\angletosecondpoint}{\innerradius}}%
            {\pgfqpointpolar{\angletofirstpoint}{\outerradius}}%
            {\pgfqpointpolar{0}{\innerradius}}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \pgfmathcosec@{\pgfmathresult}%
        \pgf@x\outerradius\relax%
        \advance\pgf@x\pgfmathresult\pgf@xa%
        \edef\anchorouterradius{\the\pgf@x}%
        %
        % ...and for the inner radius.
        %
        \pgfmathanglebetweenlines%
            {\pgfqpointpolar{\angletofirstpoint}{\innerradius}}%
            {\pgfqpointpolar{0}{\outerradius}}%
            {\pgfqpointpolar{\angletofirstpoint}{\innerradius}}%
            {\pgfqpointpolar{\angletosecondpoint}{\outerradius}}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \pgfmathcosec@{\pgfmathresult}%
        \pgf@x\innerradius\relax%
        \advance\pgf@x\pgfmathresult\pgf@xa%
        \edef\anchorinnerradius{\the\pgf@x}%
        %
        % Save all radii.
        %
        \addtosavedmacro{\innerradius}%
        \addtosavedmacro{\outerradius}%
        \addtosavedmacro{\anchorinnerradius}%
        \addtosavedmacro{\anchorouterradius}%
    }%
    \savedmacro\startangle{%
        \pgfmathadd{90}{\pgfkeysvalueof{/pgf/shape border rotate}}%
        \let\startangle\pgfmathresult%
    }%
    %
    % Saved anchors.
    %
    \savedanchor{\centerpoint}{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor{\midpoint}{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    %
    %
    % Other anchors.
    %
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}%
    \anchor{base}{\centerpoint\pgf@y=0pt}%
    \anchor{north}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{0pt}{\anchorouterradius}}}%
    \anchor{south}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{0pt}{-\anchorouterradius}}}%
    \anchor{east}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{0pt}}}%
    \anchor{west}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{0pt}}}%
    \anchor{north east}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{\anchorouterradius}}}%
    \anchor{north west}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{\anchorouterradius}}}%
    \anchor{south east}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{-\anchorouterradius}}}%
    \anchor{south west}{%
        \calculateradii%
        \csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{-\anchorouterradius}}}%
    %
    % Background path.
    %
    \backgroundpath{%
        \calculateradii%
        \let\angle\startangle%
        \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\startangle}{\outerradius}}}%
        \pgfmathloop%
            \pgfmathadd@{\angle}{\anglestep}%
            \let\angle\pgfmathresult%
        \ifnum\pgfmathcounter=\totalstarpoints%
            \pgfpathclose%
        \else%
            \ifodd\pgfmathcounter
                \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\innerradius}}}%
            \else%
                \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\outerradius}}}%
            \fi%
        \repeatpgfmathloop%
    }%
    %
    % Define points on the anchor border.
    %
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % Adjust the location of the external
        % point relative to \centerpoint.
        %
        \centerpoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Get the angle of the external point to the \centerpoint.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
        %
        % Locate the appropriate sides on the star border...
        %
        \pgfmathsubtract@{\pgfmathresult}{\startangle}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \pgfmathdivide@{\pgfmathresult}{\anglestep}%
        \pgfmathfloor@{\pgfmathresult}%
        \afterassignment\pgfmath@gobbletilpgfmath@
        \c@pgf@counta\pgfmathresult\relax\pgfmath@
        \pgfmathmultiply@{\pgfmathresult}{\anglestep}%
        \pgfmathadd@{\pgfmathresult}{\startangle}%
        \let\firstangle\pgfmathresult%
        \pgfmathadd@{\pgfmathresult}{\anglestep}%
        \let\secondangle\pgfmathresult%
        \calculateradii%
        %
        % ...and thus, the point on the star border.
        %
        \ifodd\c@pgf@counta
            \pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
                {%
                    \pgfpointadd{\centerpoint}%
                        {\pgfqpointpolar{+\firstangle}{+\anchorinnerradius}}%
                    }%
                    {%
                        \pgfpointadd{\centerpoint}%
                            {\pgfqpointpolar{+\secondangle}{+\anchorouterradius}}%
                    }%
        \else%
            \pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
                {%
                    \pgfpointadd{\centerpoint}%
                        {\pgfqpointpolar{+\firstangle}{+\anchorouterradius}}%
                    }%
                    {%
                        \pgfpointadd{\centerpoint}%
                            {\pgfqpointpolar{+\secondangle}{+\anchorinnerradius}}%
                    }%
        \fi%
    }%
    %
    % Some hackery. This is needed if a star is positioned using
    % a `...point <n+1>' anchor, where n is the maximum number of
    % points of any previously drawn star.
    %
    \pgfutil@g@addto@macro\pgf@sh@s@star{%
        \c@pgf@counta\totalstarpoints\relax%
        \divide\c@pgf@counta2\relax%
        \pgfmathloop%
            \ifnum\c@pgf@counta>0\relax%
                \c@pgf@countb\c@pgf@counta\relax%
                \advance\c@pgf@countb-1\relax%
                \pgfutil@ifundefined{pgf@anchor@star@inner point\space\the\c@pgf@counta}{%
                    \expandafter\xdef\csname pgf@anchor@star@inner point\space\the\c@pgf@counta\endcsname{%
                        \noexpand\calculateradii%
                        \noexpand\pgfmathmultiply@{\the\c@pgf@countb}{\noexpand\anglestep}%
                        \noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{2}%
                        \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
                        \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
                        \noexpand\let\noexpand\angle\noexpand\pgfmathresult%
                        \noexpand\pgfpointadd{\noexpand\centerpoint}%
                            {\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorinnerradius}}%
                    }%
                    \expandafter\xdef\csname pgf@anchor@star@outer point\space\the\c@pgf@counta\endcsname{%
                        \noexpand\calculateradii%
                        \noexpand\pgfmathmultiply@{\the\c@pgf@countb}{\noexpand\anglestep}%
                        \noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{2}%
                        \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
                        \noexpand\let\noexpand\angle\noexpand\pgfmathresult%
                        \noexpand\pgfpointadd{\noexpand\centerpoint}%
                            {\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorouterradius}}%
                    }%
                }{\c@pgf@counta0\relax}%
            \advance\c@pgf@counta-1\relax%
        \repeatpgfmathloop%
    }%
}%




% Keys for shape regular polygon
%
% /pgf/regular polygon sides
%
\pgfkeys{/pgf/.cd,
    regular polygon sides/.initial=5,
    regular polygon rotate/.style={/pgf/shape border rotate=#1}% For compatibility with 1.18
}%


% Shape Regular Polygon.
%
\pgfdeclareshape{regular polygon}{%
    \savedmacro\sides{%
        \pgfmathtruncatemacro\sides{\pgfkeysvalueof{/pgf/regular polygon sides}}%
    }%
    \savedmacro\anglestep{%
        \pgfmathdivide{360}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
        \let\anglestep\pgfmathresult%
    }%
    \savedmacro\calculateradii{%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \ifdim\pgf@y>\pgf@x%
            \pgf@x\pgf@y%
        \fi%
        %
        % Calculate i, the incircle radius
        %
        \pgf@x1.41421\pgf@x%
        %
        % Calculate r, the polygon radius
        %
        % r = i / cos(360 / s / 2)
        %
        % (s = polygon sides)
        %
        \pgfmathdivide{180}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
        \pgfmathsec@{\pgfmathresult}%
        \pgf@x\pgfmathresult\pgf@x%
        %
        % Accommodate the minimum width/height.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@ya>\pgf@xa%
            \pgf@xa\pgf@ya%
        \fi%
        \ifdim\pgf@x<.5\pgf@xa%
            \pgf@x.5\pgf@xa%
        \fi%
        \edef\radius{\the\pgf@x}%
        %
        % Now calculate the anchor radius from the outer sep.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@ya>\pgf@xa%
            \pgf@xa\pgf@ya%
        \fi
        %
        % Take into account the miter length.
        %
        % m = o / sin (90 - (360 / s / 2))
        %
        % (o = outer sep, s = sides)
        %
        \pgfmathdivide{180}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
        \pgfmathsubtract@{90}{\pgfmathresult}%
        \pgfmathcosec@{\pgfmathresult}%
        \advance\pgf@x\pgfmathresult\pgf@xa%
        \edef\anchorradius{\the\pgf@x}%
        %
        % Save both radii.
        %
        \addtosavedmacro{\radius}%
        \addtosavedmacro{\anchorradius}%
    }%
    \savedmacro\startangle{%
        \pgfmathdivide{360}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
        \let\anglestep\pgfmathresult%
        \pgfmathtruncatemacro\sides{\pgfkeysvalueof{/pgf/regular polygon sides}}%
        \expandafter\ifodd\sides\relax%
            \edef\pgfmathresult{90}%
        \else%
            \pgfmathdivide@{\anglestep}{2}%
            \pgfmathsubtract@{90}{\pgfmathresult}%
        \fi%
        \pgfmathadd{\pgfmathresult}{\pgfkeysvalueof{/pgf/shape border rotate}}%
        \let\startangle\pgfmathresult%
    }%
    %
    % Saved anchors.
    %
    \savedanchor{\centerpoint}{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor{\midpoint}{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    %
    % Other anchors.
    %
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{base}{\centerpoint\pgf@y=0pt}%
    \anchor{north}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{0pt}{\anchorradius}}}%
    \anchor{south}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{0pt}{-\anchorradius}}}%
    \anchor{east}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{0pt}}}%
    \anchor{west}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{0pt}}}%
    \anchor{north east}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{\anchorradius}}}%
    \anchor{north west}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{\anchorradius}}}%
    \anchor{south east}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{-\anchorradius}}}%
    \anchor{south west}{%
        \calculateradii%
        \csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{-\anchorradius}}}%
    %
    % Background path.
    %
    \backgroundpath{%
        \calculateradii%
        \pgfpathmoveto{%
            \pgfpointadd{\centerpoint}{\pgfqpointpolar{\startangle}{\radius}}%
        }%
        \let\angle\startangle%
        \pgfmathloop%
            \ifnum\pgfmathcounter=\sides\relax%
                \pgfpathclose%
            \else%
                \pgfmathadd@{\angle}{\anglestep}%
                \let\angle\pgfmathresult%
                \pgfpathlineto{%
                    \pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\radius}}%
                }%
        \repeatpgfmathloop%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % Adjust the location of the external
        % point relative to \centerpoint.
        %
        \centerpoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Get the angle of the external point to the \centerpoint.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
        %
        % Locate the appropriate sides on the polygon border...
        %
        \pgfmathsubtract@{\pgfmathresult}{\startangle}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \pgfmathdivide@{\pgfmathresult}{\anglestep}%
        \pgfmathfloor@{\pgfmathresult}%
        \pgfmathmultiply@{\pgfmathresult}{\anglestep}%
        \pgfmathadd@{\pgfmathresult}{\startangle}%
        \let\firstangle\pgfmathresult%
        \pgfmathadd@{\pgfmathresult}{\anglestep}%
        \let\secondangle\pgfmathresult%
        \calculateradii%
        %
        % ...and thus, the point on the polygon border.
        %
        \pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
            {%
                \pgfpointadd{\centerpoint}%
                    {\pgfqpointpolar{+\firstangle}{+\anchorradius}}%
                }%
                {%
                    \pgfpointadd{\centerpoint}%
                        {\pgfqpointpolar{+\secondangle}{+\anchorradius}}%
                }%
    }%
    %
    % More hackery for when the rectangular polygon is positioned using
    % a `corner <n+1>' or `side <n+1>' anchor, where n is the maximum
    % number of sides of any previously drawn regular polygon.
    %
    \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@regular polygon\endcsname{%
        \c@pgf@counta\sides\relax%
        \pgfmathloop%
            \ifnum\c@pgf@counta>0\relax%
                \pgfutil@ifundefined{pgf@anchor@regular polygon@corner\space\the\c@pgf@counta}{%
                %
                % ...(manually \xdef as \gdef is normally used by \anchor)...
                %
                \expandafter\xdef\csname pgf@anchor@regular polygon@corner\space\the\c@pgf@counta\endcsname{%
                    \noexpand\calculateradii%
                    \noexpand\pgfmathsubtract@{\the\c@pgf@counta}{1}%
                    \noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
                    \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
                    \noexpand\let\noexpand\angle\noexpand\pgfmathresult%
                    \noexpand\pgfpointadd{\noexpand\centerpoint}%
                        {\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorradius}}%
                }%
                \expandafter\xdef\csname pgf@anchor@regular polygon@side\space\the\c@pgf@counta\endcsname{%
                    \noexpand\calculateradii%
                    \noexpand\pgfmathsubtract@{\the\c@pgf@counta}{1}%
                    \noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
                    \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
                    \noexpand\let\noexpand\firstangle\noexpand\pgfmathresult%
                    \noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
                    \noexpand\let\noexpand\secondangle\noexpand\pgfmathresult%
                    \noexpand\pgfpointlineattime{0.5}%
                        {\noexpand\pgfpointadd{\noexpand\centerpoint}%
                            {\noexpand\pgfqpointpolar{\noexpand\firstangle}{\noexpand\anchorradius}}}%
                        {\noexpand\pgfpointadd{\noexpand\centerpoint}%
                            {\noexpand\pgfqpointpolar{\noexpand\secondangle}{\noexpand\anchorradius}}}%
                }%
            }{\c@pgf@counta0\relax}%
            \advance\c@pgf@counta-1\relax%
        \repeatpgfmathloop%
    }%
}%



% Keys for shape trapezium
%
% /pgf/trapezium left angle  : angle of the left side.
% /pgf/trapezium right angle : angle of the right side.

\pgfkeys{/pgf/.cd,
    trapezium left angle/.initial=60,
    trapezium right angle/.initial=60,
    trapezium angle/.style={
        /pgf/trapezium left angle=#1,
        /pgf/trapezium right angle=#1
    },%
    trapezium stretches/.is if=pgf@lib@sh@trapeziumstretches,%
    trapezium stretches body/.is if=pgf@lib@sh@trapeziumstretchesbody,%
}%

\newif\ifpgf@lib@sh@trapeziumstretchesbody
\newif\ifpgf@lib@sh@trapeziumstretches


% Shape trapezium.
%
\pgfdeclareshape{trapezium}{%
    \savedmacro\installtrapeziumparameters{%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \ifpgfshapeborderusesincircle%
            %
            % Get the rotation (no rounding).
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            %
            % Use the radius of the incircle if required...
            %
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \fi%
            \pgf@x1.41421\pgf@x%
            \pgf@y\pgf@x%
        \else%
            %
            % Get the rotation (with rounding).
            %
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Calculate the width and height of the node
            % contents, according to any border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xc\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xc\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xc%
                \fi%
            \fi%
        \fi%
        \pgfmathmod{\pgfkeysvalueof{/pgf/trapezium left angle}}{360}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\leftangle\pgfmathresult%
        \ifdim\leftangle pt=0pt\relax%
            \def\pgfmathresult{0}%
        \else%
            \pgfmathcot@{\leftangle}%
        \fi%
        \pgf@xa2\pgf@y%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfmathmod{\pgfkeysvalueof{/pgf/trapezium right angle}}{360}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\rightangle\pgfmathresult%
        \ifdim\rightangle pt=0pt\relax%
            \def\pgfmathresult{0}%
        \else%
            \pgfmathcot@{\rightangle}%
        \fi%
        \pgf@xb2\pgf@y%
        \pgf@xb\pgfmathresult\pgf@xb%
        %
        % Take into account minimum height and width.
        %
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@y<.5\pgf@ya%
            \ifpgf@lib@sh@trapeziumstretches%
                \pgf@y.5\pgf@ya%
            \else%
                \ifpgf@lib@sh@trapeziumstretchesbody%
                    \pgf@y.5\pgf@ya%
                \else%
                    \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@y}}%
                    \pgf@yb.5\pgf@ya%
                    \pgf@yb\pgfmathresult\pgf@yb%
                    \pgf@y.5\pgf@ya%
                    \pgf@x\pgfmath@tonumber{\pgf@yb}\pgf@x%
                    \pgf@xa\pgfmath@tonumber{\pgf@yb}\pgf@xa%
                    \pgf@xb\pgfmath@tonumber{\pgf@yb}\pgf@xb%
                \fi%
            \fi%
        \fi%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgf@xc2\pgf@x%
        \ifdim\pgf@xa<0pt\relax%
            \advance\pgf@xc-\pgf@xa%
        \else%
            \advance\pgf@xc\pgf@xa%
        \fi%
        \ifdim\pgf@xb<0pt\relax%
            \advance\pgf@xc-\pgf@xb%
        \else%
            \advance\pgf@xc\pgf@xb%
        \fi%
        \ifdim\pgf@xc<\pgf@ya%
            \ifpgf@lib@sh@trapeziumstretchesbody%
                \pgf@xc-\pgf@xc%
                \advance\pgf@xc\pgf@ya%
                \advance\pgf@x.5\pgf@xc%
            \else%
                \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xc}}%
                \pgf@ya\pgfmathresult\pgf@ya%
                \pgf@x\pgfmath@tonumber{\pgf@ya}\pgf@x%
                \pgf@xa\pgfmath@tonumber{\pgf@ya}\pgf@xa%
                \pgf@xb\pgfmath@tonumber{\pgf@ya}\pgf@xb%
                \ifpgf@lib@sh@trapeziumstretches%
                \else%
                    \pgf@y\pgfmath@tonumber{\pgf@ya}\pgf@y%
                \fi%
            \fi%
        \fi%
        \edef\halfheight{\the\pgf@y}%
        \edef\halfwidth{\the\pgf@x}%
        \edef\leftextension{\the\pgf@xa}%
        \edef\rightextension{\the\pgf@xb}%
        \pgf@xc2\pgf@x%
        %
        % Take the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@y>\pgf@x%
            \pgf@x\pgf@y%
        \fi%
        \edef\outersep{\the\pgf@x}%
        %
        % The \externalradius is a length that is
        % guarenteed to produce a point outside the trapezium.
        %
        \advance\pgf@xc2.0\pgf@x%
        \pgf@yc\halfheight\relax%
        \multiply\pgf@yc2\relax%
        \advance\pgf@yc2.0\pgf@x%
        \ifdim\pgf@xc<\pgf@yc%
            \edef\externalradius{\the\pgf@yc}%
        \else%
            \edef\externalradius{\the\pgf@xc}%
        \fi%
        %
        % Calculate the centre base and mid poins of the node.
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \pgfextract@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt\relax%
        }%
        \pgfextract@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        %
        % Calculate each point on the trapezium (without rotation).
        %
        \pgfextract@process\lowerleftpoint{%
            \centerpoint%
            \advance\pgf@x-\halfwidth\relax%
            \ifdim\leftextension>0pt\relax%
                \advance\pgf@x-\leftextension\relax%
            \fi%
            \advance\pgf@y-\halfheight\relax%
        }%
        \pgfextract@process\upperleftpoint{%
            \centerpoint%
            \advance\pgf@x-\halfwidth\relax%
            \ifdim\leftextension<0pt\relax%
                \advance\pgf@x\leftextension\relax%
            \fi%
            \advance\pgf@y\halfheight\relax%
        }%
        \pgfextract@process\upperrightpoint{%
            \centerpoint%
            \advance\pgf@x\halfwidth\relax%
            \ifdim\rightextension<0pt\relax%
                \advance\pgf@x-\rightextension\relax%
            \fi%
            \advance\pgf@y\halfheight\relax%
        }%
        \pgfextract@process\lowerrightpoint{%
            \centerpoint%
            \advance\pgf@x\halfwidth\relax%
            \ifdim\rightextension>0pt\relax%
                \advance\pgf@x\rightextension\relax%
            \fi%
            \advance\pgf@y-\halfheight\relax%
        }%
        %
        % Now calculate the adjustment for the miter length at each corner
        % of the trapezium. This ensures more accurate anchor positioning
        % when the line width is particularly thick.
        %
        \pgfextract@process\lowerleftmiter{%
            \pgfmathanglebetweenlines{\lowerleftpoint}{\lowerrightpoint}{\lowerleftpoint}{\upperleftpoint}%
            \pgfmathmultiply@{\pgfmathresult}{.5}%
            \pgfmathtan@{\pgfmathresult}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@x-\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y-\outersep\relax%
        }%
        \pgfextract@process\upperleftmiter{%
            \pgfmathanglebetweenlines{\upperleftpoint}{\lowerleftpoint}{\upperleftpoint}{\upperrightpoint}%
            \pgfmathmultiply@{\pgfmathresult}{.5}%
            \pgfmathtan@{\pgfmathresult}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@x-\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y\outersep\relax%
        }%
        \pgfextract@process\upperrightmiter{%
            \pgfmathanglebetweenlines{\upperrightpoint}{\upperleftpoint}{\upperrightpoint}{\lowerrightpoint}%
            \pgfmathmultiply@{\pgfmathresult}{.5}%
            \pgfmathtan@{\pgfmathresult}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@x\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y\outersep\relax%
        }%
        \pgfextract@process\lowerrightmiter{%
            \pgfmathanglebetweenlines{\lowerrightpoint}{\upperrightpoint}{\lowerrightpoint}{\lowerleftpoint}%
            \pgfmathmultiply@{\pgfmathresult}{.5}%
            \pgfmathtan@{\pgfmathresult}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@x\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y-\outersep\relax%
        }%
        %
        % Now calculate the corners for determining anchor border
        % points, by adding the adjustment for the miter length.
        %
        \pgfextract@process\lowerleftborderpoint{%
            \pgfpointadd{\lowerleftpoint}{\lowerleftmiter}%
        }%
        \pgfextract@process\upperleftborderpoint{%
            \pgfpointadd{\upperleftpoint}{\upperleftmiter}%
        }%
        \pgfextract@process\upperrightborderpoint{%
            \pgfpointadd{\upperrightpoint}{\upperrightmiter}%
        }%
        \pgfextract@process\lowerrightborderpoint{%
            \pgfpointadd{\lowerrightpoint}{\lowerrightmiter}%
        }%
        %
        % Calculate the angle from the centerpoint to each corner.
        % Rotation is not important here (see \anchorborder code).
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\lowerleftborderpoint}%
        \let\angletolowerleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\upperleftborderpoint}%
        \let\angletoupperleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\upperrightborderpoint}%
        \let\angletoupperright\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\lowerrightborderpoint}%
        \let\angletolowerright\pgfmathresult%
        %
        % Do the same for the *inversely rotated* base point...
        %
        \pgfextract@process\rotatedbasepoint{%
            \pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\lowerleftborderpoint}%
        \let\baseangletolowerleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\upperleftborderpoint}%
        \let\baseangletoupperleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\upperrightborderpoint}%
        \let\baseangletoupperright\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\lowerrightborderpoint}%
        \let\baseangletolowerright\pgfmathresult%
        %
        % And the *inversely rotated* mid point...
        %
        \pgfextract@process\rotatedmidpoint{%
            \pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\lowerleftborderpoint}%
        \let\midangletolowerleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\upperleftborderpoint}%
        \let\midangletoupperleft\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\upperrightborderpoint}%
        \let\midangletoupperright\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\lowerrightborderpoint}%
        \let\midangletolowerright\pgfmathresult%
        %
        % Now rotate the border points around the centerpoint...
        %
        \pgfextract@process\lowerleftborderpoint{%
            \pgfmathrotatepointaround%
                {\lowerleftborderpoint}%
                {\centerpoint}%
                {\rotate}%
        }%
        \pgfextract@process\upperleftborderpoint{%
            \pgfmathrotatepointaround%
                {\upperleftborderpoint}%
                {\centerpoint}%
                {\rotate}%
        }%
        \pgfextract@process\upperrightborderpoint{%
            \pgfmathrotatepointaround%
                {\upperrightborderpoint}%
                {\centerpoint}%
                {\rotate}%
        }%
        \pgfextract@process\lowerrightborderpoint{%
            \pgfmathrotatepointaround%
                {\lowerrightborderpoint}%
                {\centerpoint}%
                {\rotate}%
        }%
        %
        % ...and the points for drawing the border (i.e. no outer sep).
        %
        \pgfextract@process\lowerleftpoint{%
            \pgfmathrotatepointaround{\lowerleftpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\upperleftpoint{%
            \pgfmathrotatepointaround{\upperleftpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\upperrightpoint{%
            \pgfmathrotatepointaround{\upperrightpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\lowerrightpoint{%
            \pgfmathrotatepointaround{\lowerrightpoint}{\centerpoint}{\rotate}%
        }%
        %
        % And finally, save all the relevant stuff.
        %
        \addtosavedmacro{\lowerleftpoint}%
        \addtosavedmacro{\upperleftpoint}%
        \addtosavedmacro{\upperrightpoint}%
        \addtosavedmacro{\lowerrightpoint}%
        %
        \addtosavedmacro{\lowerleftborderpoint}%
        \addtosavedmacro{\upperleftborderpoint}%
        \addtosavedmacro{\upperrightborderpoint}%
        \addtosavedmacro{\lowerrightborderpoint}%
        %
        \addtosavedmacro{\angletolowerleft}%
        \addtosavedmacro{\angletoupperleft}%
        \addtosavedmacro{\angletoupperright}%
        \addtosavedmacro{\angletolowerright}%
        %
        \addtosavedmacro{\baseangletolowerleft}%
        \addtosavedmacro{\baseangletoupperleft}%
        \addtosavedmacro{\baseangletoupperright}%
        \addtosavedmacro{\baseangletolowerright}%
        %
        \addtosavedmacro{\midangletolowerleft}%
        \addtosavedmacro{\midangletoupperleft}%
        \addtosavedmacro{\midangletoupperright}%
        \addtosavedmacro{\midangletolowerright}%
        %
        \addtosavedmacro{\rotate}%
        \addtosavedmacro{\externalradius}%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \installtrapeziumparameters%
        \let\pgf@trapeziumanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{base west}{%
        \installtrapeziumparameters%
        \let\pgf@trapeziumanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \installtrapeziumparameters%
        \let\pgf@trapeziumanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid west}{%
        \installtrapeziumparameters%
        \let\pgf@trapeziumanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south west}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{south east}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \installtrapeziumparameters%
        \csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{bottom left corner}{%
        \installtrapeziumparameters%
        \lowerleftborderpoint%
    }%
    \anchor{top left corner}{%
        \installtrapeziumparameters%
        \upperleftborderpoint%
    }%
    \anchor{top right corner}{%
        \installtrapeziumparameters%
        \upperrightborderpoint%
    }%
    \anchor{bottom right corner}{%
        \installtrapeziumparameters%
        \lowerrightborderpoint%
    }%
    \anchor{left side}{%
        \installtrapeziumparameters%
        \pgfpointlineattime{0.5}{\lowerleftborderpoint}{\upperleftborderpoint}%
    }%
    \anchor{right side}{%
        \installtrapeziumparameters%
        \pgfpointlineattime{0.5}{\lowerrightborderpoint}{\upperrightborderpoint}%
    }%
    \anchor{top side}{%
        \installtrapeziumparameters%
        \pgfpointlineattime{0.5}{\upperleftborderpoint}{\upperrightborderpoint}%
    }%
    \anchor{bottom side}{%
        \installtrapeziumparameters%
        \pgfpointlineattime{0.5}{\lowerleftborderpoint}{\lowerrightborderpoint}%
    }%
    \backgroundpath{%
        \installtrapeziumparameters%
        \pgfpathmoveto{\lowerleftpoint}%
        \pgfpathlineto{\upperleftpoint}%
        \pgfpathlineto{\upperrightpoint}%
        \pgfpathlineto{\lowerrightpoint}%
        \pgfpathclose%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % This allows anchors base east, base west, mid east and mid west,
        % to redefine the `center' of the node to correctly calculate the
        % border points.
        %
        \pgfutil@ifundefined{pgf@trapeziumanchorborderreferencepoint}%
            {\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@trapeziumanchorborderreferencepoint}%
        %
        % Adjust the location of the external
        % point relative to the reference point.
        %
        \referencepoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Install the required points and angles.
        %
        \installtrapeziumparameters%
        %
        % Get the angle of the external point to the \referencepoint.
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
        %
        % *Subtract* the rotation from the external angle. This is
        % why the border point angles do not neeed to be rotated.
        %
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        %
        % Get the relevant angles for the reference point.
        %
        \let\externalangle\pgfmathresult%
        \ifx\referencepoint\basepoint%
            \let\angletoupperright\baseangletoupperright%
            \let\angletoupperleft\baseangletoupperleft%
            \let\angletolowerright\baseangletolowerright%
            \let\angletolowerleft\baseangletolowerleft%
        \else%
            \ifx\referencepoint\midpoint%
                \let\angletoupperright\midangletoupperright%
                \let\angletoupperleft\midangletoupperleft%
                \let\angletolowerright\midangletolowerright%
                \let\angletolowerleft\midangletolowerleft%
        \fi\fi%
        %
        % Find the line on the border...
        %
        \ifdim\externalangle pt<\angletoupperright pt\relax%
            \let\firstpoint\upperrightborderpoint%
            \let\secondpoint\lowerrightborderpoint%
        \else%
            \ifdim\externalangle pt<\angletoupperleft pt\relax%
                \let\firstpoint\upperleftborderpoint%
                \let\secondpoint\upperrightborderpoint%
            \else%
                \ifdim\externalangle pt<\angletolowerleft pt\relax%
                    \let\firstpoint\upperleftborderpoint%
                    \let\secondpoint\lowerleftborderpoint%
                \else%
                    \ifdim\externalangle pt<\angletolowerright pt\relax%
                        \let\firstpoint\lowerleftborderpoint%
                        \let\secondpoint\lowerrightborderpoint%
                    \else%
                        \let\firstpoint\upperrightborderpoint%
                        \let\secondpoint\lowerrightborderpoint%
                    \fi%
                \fi%
            \fi%
        \fi%
        %
        % ...and thus the point on the border.
        %
        \pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\firstpoint}{\secondpoint}%
    }%
}%




% Shape semicircle.
%
\pgfdeclareshape{semicircle}{%
    \savedmacro\installsemicircleparameters{%
        %
        % Get the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@x<\pgf@y%
            \pgf@x\pgf@y%
        \fi%
        \edef\outersep{\the\pgf@x}%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x+.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y+.5\ht\pgfnodeparttextbox%
        \advance\pgf@y+.5\dp\pgfnodeparttextbox%
        %
        % Use the radius of the incircle if required...
        %
        \ifpgfshapeborderusesincircle%
            %
            % Get the rotation (no rounding).
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \fi%
            \pgf@x1.41421\pgf@x%
            \edef\halfheight{\the\pgf@x}%
            \advance\pgf@x\pgf@x%
        \else%
            %
            % Get the rotation (with rounding).
            %
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Calculate the width and height of the node
            % contents, according to any border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xc\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xc\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xc%
                \fi%
            \fi%
            \advance\pgf@y\pgf@y%
            \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
            \pgf@x\pgfmathresult pt\relax%
            \pgf@y.5\pgf@y%
            \edef\halfheight{\the\pgf@y}%
        \fi%
        \edef\defaultradius{\the\pgf@x}%
        %
        % Take into account minimum height and width.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@x<.5\pgf@xa%
            \pgf@x.5\pgf@xa%
        \fi%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@x<\pgf@ya%
            \pgf@x\pgf@ya%
        \fi%
        \edef\semicircleradius{\the\pgf@x}%
        %
        % Find the center/base/mid of the semi circle node.
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y+-.5\dp\pgfnodeparttextbox%
        }%
        \pgfextract@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt\relax%
        }%
        \pgfextract@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        \pgfextract@process\semicirclecenterpoint{%
            \centerpoint%
            \pgf@ya\semicircleradius\relax%
            \advance\pgf@ya-\defaultradius\relax%
            %
            % The point is adjusted to make the node contents
            % appear more centered if the node is enlarged to
            % some minimum size. The factor .4 just seems OK.
            %
            \pgf@ya.4\pgf@ya%
            \advance\pgf@y-\pgf@ya%
            \pgf@ya\halfheight\relax%
            \advance\pgf@y-\pgf@ya%
        }%
        %
        % Add the outer sep to the radius here.
        %
        \pgf@x\semicircleradius\relax%
        \advance\pgf@x\outersep\relax%
        \edef\semicircleradius{\the\pgf@x}%
        \pgfpointdiff{\centerpoint}{\semicirclecenterpoint}%
        \ifdim\pgf@y<0pt\pgf@y-\pgf@y\fi%
        \edef\centerpointdiff{\the\pgf@y}%
        %
        % Calculate the start and end points on the border.
        %
        \pgfextract@process\arcstartborder{%
            \semicirclecenterpoint%
            \advance\pgf@x\semicircleradius\relax%
        }%
        \pgfextract@process\arcendborder{%
            \semicirclecenterpoint%
            \advance\pgf@x-\semicircleradius\relax%
        }%
        %
        % Calculate the start and end *corner* points on the border.
        % This is needed to accommodate the outer sep.
        %
        \pgfextract@process\arcstartcorner{%
            \arcstartborder%
            \advance\pgf@y-\outersep\relax%
        }%
        \pgfextract@process\arcendcorner{%
            \arcendborder%
            \advance\pgf@y-\outersep\relax%
        }
        %
        % Now calculate all the relevant angles.
        %
        % For the center point.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\arcstartborder}%
        \let\angletoarcstartborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcendborder}%
        \let\angletoarcendborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcstartcorner}%
        \let\angletoarcstartcorner\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcendcorner}%
        \let\angletoarcendcorner\pgfmathresult%
        %
        % For the basepoint (rotated about the center point).
        %
        \pgfextract@process\rotatedbasepoint{%
            \pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcstartborder}%
        \let\baseangletoarcstartborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcendborder}%
        \let\baseangletoarcendborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcstartcorner}%
        \let\baseangletoarcstartcorner\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcendcorner}%
        \let\baseangletoarcendcorner\pgfmathresult%
        %
        % For the midpoint (rotated about the center point).
        %
        \pgfextract@process\rotatedmidpoint{%
            \pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcstartborder}%
        \let\midangletoarcstartborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcendborder}%
        \let\midangletoarcendborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcstartcorner}%
        \let\midangletoarcstartcorner\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcendcorner}%
        \let\midangletoarcendcorner\pgfmathresult%
        %
        % Now, rotate the semicircle points around the centerpoint.
        %
        \pgfextract@process\semicirclecenterpoint{%
            \pgfmathrotatepointaround{\semicirclecenterpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcstartborder{%
            \pgfmathrotatepointaround{\arcstartborder}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcendborder{%
            \pgfmathrotatepointaround{\arcendborder}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcstartcorner{%
            \pgfmathrotatepointaround{\arcstartcorner}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcendcorner{%
            \pgfmathrotatepointaround{\arcendcorner}{\centerpoint}{\rotate}%
        }%
        %
        % Calculate the distance between the base point and the (rotated) semicircle center.
        %
        \pgfpointdiff{\basepoint}{\semicirclecenterpoint}%
        \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
        \edef\basesemicirclecenterdiff{\pgfmathresult pt}%
        %
        % Calculate the distance between the base point and the (rotated) semicircle center.
        %
        \pgfpointdiff{\midpoint}{\semicirclecenterpoint}%
        \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
        \edef\midsemicirclecenterdiff{\pgfmathresult pt}%
        %
        % And save all the stuff.
        %
        \addtosavedmacro{\rotate}%
        \addtosavedmacro{\outersep}%
        \addtosavedmacro{\semicircleradius}%
        %
        \addtosavedmacro{\arcstartborder}%
        \addtosavedmacro{\arcendborder}%
        \addtosavedmacro{\arcstartcorner}%
        \addtosavedmacro{\arcendcorner}%
        \addtosavedmacro{\semicirclecenterpoint}%
        %
        \addtosavedmacro{\angletoarcstartborder}%
        \addtosavedmacro{\angletoarcendborder}%
        \addtosavedmacro{\angletoarcstartcorner}%
        \addtosavedmacro{\angletoarcendcorner}%
        %
        \addtosavedmacro{\centerpointdiff}%
        \addtosavedmacro{\basesemicirclecenterdiff}%
        \addtosavedmacro{\midsemicirclecenterdiff}%
        %
        \addtosavedmacro{\baseangletoarcstartborder}%
        \addtosavedmacro{\baseangletoarcendborder}%
        \addtosavedmacro{\baseangletoarcstartcorner}%
        \addtosavedmacro{\baseangletoarcendcorner}%
        %
        \addtosavedmacro{\midangletoarcstartborder}%
        \addtosavedmacro{\midangletoarcendborder}%
        \addtosavedmacro{\midangletoarcstartcorner}%
        \addtosavedmacro{\midangletoarcendcorner}%
    }%
    \savedanchor{\centerpoint}{%
        \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
        \pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
        \pgfmathaddtolength\pgf@y{-.5\dp\pgfnodeparttextbox}%
    }%
    \savedanchor{\basepoint}{%
        \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
        \pgf@y0pt\relax%
    }%
    \savedanchor{\midpoint}{%
        \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{base}{\basepoint}%
    \anchor{base west}{%
        \installsemicircleparameters%
        \let\pgf@semicirclereferencepoint\basepoint%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{-\semicircleradius}{0pt}}%
    }%
    \anchor{base east}{%
        \installsemicircleparameters%
        \let\pgf@semicirclereferencepoint\basepoint%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{\semicircleradius}{0pt}}%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid west}{%
        \installsemicircleparameters%
        \let\pgf@semicirclereferencepoint\midpoint%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{-\semicircleradius}{0pt}}%
    }%
    \anchor{mid east}{%
        \installsemicircleparameters%
        \let\pgf@semicirclereferencepoint\midpoint%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{\semicircleradius}{0pt}}%
    }%
    \anchor{apex}{%
        \installsemicircleparameters%
        \pgfmathadd@{\rotate}{90}%
        \let\angle\pgfmathresult%
        \pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\angle}{\semicircleradius}}%
    }%
    \anchor{arc start}{%
        \installsemicircleparameters%
        \arcstartcorner%
    }%
    \anchor{arc end}{%
        \installsemicircleparameters%
        \arcendcorner%
    }%
    \anchor{chord center}{%
        \installsemicircleparameters%
        \pgfpointlineattime{0.5}{\arcstartcorner}{\arcendcorner}%
    }%
    \anchor{north}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{90}{\semicircleradius}}%
    }%
    \anchor{south}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{270}{\semicircleradius}}%
    }%
    \anchor{east}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{0}{\semicircleradius}}%
    }%
    \anchor{west}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{180}{\semicircleradius}}%
    }%
    \anchor{north west}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{135}{\semicircleradius}}%
    }%
    \anchor{south west}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{225}{\semicircleradius}}%
    }%
    \anchor{north east}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{45}{\semicircleradius}}%
    }%
    \anchor{south east}{%
        \installsemicircleparameters%
        \csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{315}{\semicircleradius}}%
    }%
    \backgroundpath{%
        \installsemicircleparameters%
        \pgf@x\semicircleradius\relax%
        \advance\pgf@x-\outersep\relax%
        \edef\semicircleradius{\the\pgf@x}%
        \pgfpathmoveto{\pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\rotate}{\semicircleradius}}}%
        {%
            \pgftransformrotate{\rotate}%
            \pgfpatharc{0}{180}{\semicircleradius}%
            \pgfpathclose%
        }%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % Check if a reference point has been defined (i.e. \midpoint or \basepoint).
        %
        \pgfutil@ifundefined{pgf@semicirclereferencepoint}%
            {\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@semicirclereferencepoint}%
        %
        % Adjust the location of the external  point relative to the reference point.
        %
        \referencepoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Install the required points and angles.
        %
        \installsemicircleparameters%
        %
        % Get the angle of the external point to the \referencepoint.
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
        \let\externalangle\pgfmathresult%
        %
        % *Subtract* the rotation from the external angle.
        %
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\angle\pgfmathresult%
        \ifx\referencepoint\basepoint%
            \let\angletoarcstartborder\baseangletoarcstartborder%
            \let\angletoarcendborder\baseangletoarcendborder%
            \let\angletoarcstartcorner\baseangletoarcstartcorner%
            \let\angletoarcendcorner\baseangletoarcendcorner%
            \let\centerpointdiff\basesemicirclecenterdiff%
        \else%
            \ifx\referencepoint\midpoint%
                \let\angletoarcstartborder\midangletoarcstartborder%
                \let\angletoarcendborder\midangletoarcendborder%
                \let\angletoarcstartcorner\midangletoarcstartcorner%
                \let\angletoarcendcorner\midangletoarcendcorner%
                \let\centerpointdiff\midsemicirclecenterdiff%
        \fi\fi%
        %
        % Determine if the line will cross the semicircle arc, or the chord.
        %
        \ifdim\angle pt>\angletoarcstartborder pt\relax%
            \let\firstpoint\pgfutil@empty%
            \let\secondpoint\pgfutil@empty%
        \else%
            \ifdim\angle pt>\angletoarcstartcorner pt\relax%
                \let\firstpoint\arcstartcorner%
                \let\secondpoint\arcstartborder%
            \else%
                \ifdim\angle pt>\angletoarcendcorner pt\relax%
                    \let\firstpoint\arcendcorner%
                    \let\secondpoint\arcstartcorner%
                \else%
                    \ifdim\angle pt>\angletoarcendborder pt\relax%
                        \let\firstpoint\arcendborder%
                        \let\secondpoint\arcendcorner%
                    \else%
                        \let\firstpoint\pgfutil@empty%
                        \let\secondpoint\pgfutil@empty%
                    \fi%
                \fi%
            \fi%
        \fi%
        \ifx\firstpoint\pgfutil@empty
            %
            % Calculate the angle from the centre of the semicircle to the
            % point on the semicircle arc which intersects the line from
            % the external point to the reference point...
            %
            \pgfmathanglebetweenlines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\semicirclecenterpoint}{\referencepoint}%
            \pgfmathsin@{\pgfmathresult}%
            \let\sineangle\pgfmathresult%
            \pgf@x\semicircleradius\relax%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
            \let\reciprocalradius\pgfmathresult%
            \pgf@x\centerpointdiff\relax%
            \pgf@x\sineangle\pgf@x%
            \pgf@x\reciprocalradius\pgf@x%
            \pgfmathasin@{\pgfmath@tonumber{\pgf@x}}%
            \pgf@x\pgfmathresult pt\relax%
            \advance\pgf@x\externalangle pt\relax%
            \edef\angle{\pgfmath@tonumber{\pgf@x}}%
            %
            % ...and thus the point on the border.
            %
            \pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\angle}{\semicircleradius}}%
        \else%
            %
            % Calculate the the point where the semicircle chord intersects
            % the line from the external point to the reference point.
            %
            \pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\firstpoint}{\secondpoint}%
        \fi%
    }%
}%


% Keys for shape isosceles triangle
%
% /pgf/isosceles triangle apex angle : angle at the apex of the triangle.
\pgfkeys{/pgf/.cd,
    isosceles triangle apex angle/.initial=45,
    isosceles triangle stretches/.is if=pgf@lib@sh@isosceslestrianglestretches
}%
\newif\ifpgf@lib@sh@isosceslestrianglestretches

\pgfdeclareshape{isosceles triangle}{%
    \savedmacro\trianglepoints{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/isosceles triangle apex angle}}%
        \divide\pgf@x2\relax%
        \edef\halfapexangle{\pgfmath@tonumber{\pgf@x}}%
        \addtosavedmacro\halfapexangle%
        %
        \pgfmathtan@{\halfapexangle}%
        \let\tanhalfapexangle\pgfmathresult%
        %
        \pgfmathcot@{\halfapexangle}%
        \let\cothalfapexangle\pgfmathresult%
        %
        \pgfmathsin@{\halfapexangle}%
        \let\sinhalfapexangle\pgfmathresult%
        %
        \pgfmathreciprocal@{\pgfmathresult}%
        \let\cosechalfapexangle\pgfmathresult%
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        %
        \ifpgfshapeborderusesincircle%
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \else%
                \pgf@y\pgf@x%
            \fi%
            \pgf@x1.414213\pgf@x%
            \pgf@y1.414213\pgf@y%
            %
            \pgf@xa\pgf@x%
            \advance\pgf@xa\cosechalfapexangle\pgf@x%
            \pgf@ya\tanhalfapexangle\pgf@xa%
        \else%
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \ifdim\pgfmathresult pt<0pt\relax%
                \pgfmathadd@{\pgfmathresult}{360}%
            \fi%
            \pgfmathsetcount\c@pgf@counta{+\pgfmathresult}%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \edef\rotate{\the\c@pgf@counta}%
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xa\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xa%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xa%
                \fi%
            \fi%
            %
            \pgf@xa2.0\pgf@x%
            \pgf@ya\tanhalfapexangle\pgf@xa%
            \advance\pgf@xa\cothalfapexangle\pgf@y%
            \advance\pgf@ya\pgf@y%
        \fi%
        \addtosavedmacro\rotate%
        \ifdim\pgf@xa=0pt\relax%
            \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum height}}%
        \fi%
        % Adjust for minimum height and width.
        %
        \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@ya<.5\pgf@yb%
            \ifpgf@lib@sh@isosceslestrianglestretches%
                \pgf@ya.5\pgf@yb%
                %
                \pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
                \pgfmathatan@{\pgfmathresult}%
                \let\halfapexangle\pgfmathresult%
                %
            \else%
                \pgf@ya.5\pgf@yb%
                \pgf@xa\cothalfapexangle\pgf@ya%
            \fi%
        \fi%
        %
        \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@xa<\pgf@xb%
            \ifpgf@lib@sh@isosceslestrianglestretches%
                \pgf@xa\pgf@xb%
                %
                \pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
                \pgfmathatan@{\pgfmathresult}%
                \let\halfapexangle\pgfmathresult%
                %
            \else%
                \pgf@xa\pgf@xb%
                \pgf@ya\tanhalfapexangle\pgf@xa%
            \fi%
        \fi%
        %
        %
        % Now find the ``offset height'' (h'). This is the distance from the
        % center of the node contents to the base of the triangle.
        %
        \ifpgfshapeborderusesincircle%
            %
            % h' = H*sin(a/2) / (1+sin(a/2))
            %
            % where:
            %   H = the height of the triangle.
            %   a = the apex angle.
            %
            \pgf@xc\pgf@xa%
            \pgfmathsin@{\halfapexangle}%
            \pgf@xc\pgfmathresult\pgf@xc%
            \pgf@yc1pt\relax%
            \advance\pgf@yc\pgfmathresult pt\relax%
            \pgfmathdivide@{\pgfmath@tonumber{\pgf@xc}}{\pgfmath@tonumber{\pgf@yc}}
            \pgfutil@tempdima\pgfmathresult pt\relax%
        \else%
            %
            % h' = 0.5*h + (0.5*(W-w)*cos(a/2) - h*sin(a/2))/(1+sin(a/2))
            %
            % where:
            %   h = the height of the node contents.
            %   w = the width of the node contents.
            %   W = the width of the triangle.
            %   a = the apex angle.
            %
            \pgf@xc\pgf@ya%
            \advance\pgf@xc-\pgf@y%
            \pgfmathcos@{\halfapexangle}%
            \pgf@xc\pgfmathresult\pgf@xc%
            \pgfmathsin@{\halfapexangle}%
            \advance\pgf@xc-\pgfmathresult\pgf@x%
            \advance\pgf@xc-\pgfmathresult\pgf@x%
            \pgf@yc\pgfmathresult pt\relax%
            \advance\pgf@yc1pt\relax%
            \pgfmathdivide@{\pgfmath@tonumber{\pgf@xc}}{\pgfmath@tonumber{\pgf@yc}}%
            \pgfutil@tempdima\pgfmathresult pt\relax%
            \advance\pgfutil@tempdima\pgf@x%
        \fi%
        \pgfextract@process\apex{%
            \pgf@y0pt%
            \pgf@x\pgf@xa%
            \advance\pgf@x-\pgfutil@tempdima%
        }%
        \addtosavedmacro\apex%
        %
        \pgfextract@process\lowerleft{%
            \pgf@y\pgf@ya%
            \pgf@x-\pgfutil@tempdima%
        }%
        \addtosavedmacro\lowerleft%
        %
        \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@xb<\pgf@yb%
            \pgf@xb\pgf@yb%
        \fi%
        \pgfextract@process\apexanchor{%
            \apex%
            \advance\pgf@x\cosechalfapexangle\pgf@xb%
        }%
        \addtosavedmacro\apexanchor%
        %
        \pgf@yc-\halfapexangle pt\relax%
        \advance\pgf@yc90pt\relax%
        \divide\pgf@yc2\relax%
        \pgfmathcot@{\pgfmath@tonumber{\pgf@yc}}%
        \pgfextract@process\lowerleftanchor{%
            \lowerleft%
            \advance\pgf@y\pgfmathresult\pgf@xb%
            \advance\pgf@x-\pgf@xb%
        }%
        \addtosavedmacro\lowerleftanchor%
        %
        \pgfextract@process\lowerrightanchor{%
            \lowerleftanchor%
            \pgf@y-\pgf@y%
        }%
        \addtosavedmacro\lowerrightanchor%
    }%
    \anchor{apex}{%
        \trianglepoints%
        \pgfpointadd{\centerpoint}{%
            \pgfmathrotatepointaround{\apexanchor}{\pgfpointorigin}{\rotate}%
        }%
    }%
    \anchor{left corner}{%
        \trianglepoints%
        \pgfpointadd{\centerpoint}{%
            \pgfmathrotatepointaround{\lowerleftanchor}{\pgfpointorigin}{\rotate}%
        }%
    }%
    \anchor{right corner}{%
        \trianglepoints%
        \pgfpointadd{\centerpoint}{%
            \pgfmathrotatepointaround{\lowerrightanchor}{\pgfpointorigin}{\rotate}%
        }%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid west}{%
        \trianglepoints%
        \let\pgf@isoscelestriangle@referencepoint\midpoint%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
    }%
    \anchor{mid east}{%
        \trianglepoints%
        \let\pgf@isoscelestriangle@referencepoint\midpoint%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base west}{%
        \trianglepoints%
        \let\pgf@isoscelestriangle@referencepoint\basepoint%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
    }%
    \anchor{base east}{%
        \trianglepoints%
        \let\pgf@isoscelestriangle@referencepoint\basepoint%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
    }%
    \anchor{north}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{0pt}{1pt}}%
    }%
    \anchor{south}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{0pt}{-1pt}}%
    }%
    \anchor{east}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
    }%
    \anchor{west}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
    }%
    \anchor{north east}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{1pt}}%
    }%
    \anchor{south west}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{-1pt}}%
    }%
    \anchor{south east}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{-1pt}}%
    }%
    \anchor{north west}{%
        \trianglepoints%
        \csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{1pt}}%
    }%
    \anchor{left side}{%
        \trianglepoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{\pgfpointlineattime{0.5}{\lowerleftanchor}{\apexanchor}}{\centerpoint}}%
                {\centerpoint}{\rotate}%
    }%
    \anchor{right side}{%
        \trianglepoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{\pgfpointlineattime{0.5}{\lowerrightanchor}{\apexanchor}}{\centerpoint}}%
                {\centerpoint}{\rotate}%
    }%
    \anchor{lower side}{%
        \trianglepoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{\pgfpointlineattime{0.5}{\lowerleftanchor}{\lowerrightanchor}}{\centerpoint}}%
                {\centerpoint}{\rotate}%
    }%
    \backgroundpath{%
        \trianglepoints%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            \pgfpathmoveto{\apex}%
            \pgfpathlineto{\lowerleft}%
            \pgfpathlineto{\lowerleft\pgf@y-\pgf@y}%
            \pgfpathclose%
        }%
    }%
    \anchorborder{%
        \pgfutil@ifundefined{pgf@isoscelestriangle@referencepoint}{\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@isoscelestriangle@referencepoint}%
        \pgfextract@process\externalpoint{%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \referencepoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \trianglepoints%
        \pgfmathanglebetweenpoints{\referencepoint}{\externalpoint}%
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
            \pgfmathmod@{\pgfmathresult}{360}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\lowerrightanchor}}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
            \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\lowerleftanchor}}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\apexanchor}}%
                \ifdim\externalangle pt>\pgfmathresult pt\relax%
                    \let\firstpoint\apexanchor%
                    \let\secondpoint\lowerleftanchor%
                \else%
                    \let\firstpoint\apexanchor%
                    \let\secondpoint\lowerrightanchor%
                \fi%
            \else%
                \let\firstpoint\lowerleftanchor%
                \let\secondpoint\lowerrightanchor%
            \fi%
        \else%
            \let\firstpoint\lowerrightanchor%
            \let\secondpoint\apexanchor%
        \fi%
        \pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
            {\pgfmathrotatepointaround{\pgfpointadd{\centerpoint}{\firstpoint}}{\centerpoint}{\rotate}}%
            {\pgfmathrotatepointaround{\pgfpointadd{\centerpoint}{\secondpoint}}{\centerpoint}{\rotate}}%
    }%
}%




% Keys for shape kite
%
%
\pgfkeys{/pgf/.cd,
    kite upper vertex angle/.initial=120,
    kite lower vertex angle/.initial=60,
    kite vertex angles/.code={%
        \pgfutil@in@{and}{#1}%
        \ifpgfutil@in@%
            \def\pgf@marshal##1and##2\@@{%
                \pgfkeys{/pgf/kite upper vertex angle=##1}%
                \pgfkeys{/pgf/kite lower vertex angle=##2}%
            }%
            \expandafter\pgf@marshal#1\@@%
        \else%
            \pgfkeys{/pgf/kite upper vertex angle=#1}%
            \pgfkeys{/pgf/kite lower vertex angle=#1}%
        \fi%
    }%
}%

% Shape kite.
%
\pgfdeclareshape{kite}{%
    \savedmacro\installkiteparameters{%
        %
        % Get the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@x<\pgf@y%
            \pgf@x\pgf@y%
        \fi%
        \edef\outersep{\the\pgf@x}%
        %
        % Calculate the centre, base and mid points of the node.
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \pgfextract@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt\relax%
        }%
        \pgfextract@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        %
        % Halve the vertex angles.
        %
        \pgfmathdivide{\pgfkeysvalueof{/pgf/kite upper vertex angle}}{2}%
        \let\halfuppervertexangle\pgfmathresult%
        \pgfmathdivide{\pgfkeysvalueof{/pgf/kite lower vertex angle}}{2}%
        \let\halflowervertexangle\pgfmathresult%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \ifpgfshapeborderusesincircle%
            %
            % Get the rotation.
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            %
            % Get the radius of the incircle.
            %
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \fi%
            \pgf@x1.41421\pgf@x%
            %
            % Get the distances from the upper and lower vertices
            % to the center of the incircle.
            %
            \pgfmathsin@{\halfuppervertexangle}%
            \let\sinehalfuppervertexangle\pgfmathresult%
            \pgfmathreciprocal@{\pgfmathresult}%
            \let\cosechalfuppervertexangle\pgfmathresult%
            \pgf@ya\pgfmathresult\pgf@x%
            \pgfmathsin@{\halflowervertexangle}%
            \let\sinehalflowervertexangle\pgfmathresult%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@yb\pgfmathresult\pgf@x%
            %
            % Now calculate vertical offset (yc) between the center of
            % the incircle, and the intersection of the kite diagonals.
            %
            % yc = x * cosec(a/2) - x * cot(a/2) * (sin(a/2) + sin(b/2)) * cosec(a/2 + b/2)
            %
            % where:
            %   x = the incircle radius.
            %   a = the upper vertex angle.
            %   b = the lower vertex angle.
            %
            \pgf@yc\pgf@x%
            \pgfmathadd@{\halfuppervertexangle}{\halflowervertexangle}%
            \pgfmathcosec@{\pgfmathresult}%
            \pgf@yc\pgfmathresult\pgf@yc%
            \pgfmathadd@{\sinehalfuppervertexangle}{\sinehalflowervertexangle}%
        \pgf@yc\pgfmathresult\pgf@yc%
            \pgfmathcos@{\halfuppervertexangle}%
            \pgf@yc\pgfmathresult\pgf@yc%
            \pgf@yc-\cosechalfuppervertexangle\pgf@yc%
            \advance\pgf@yc\cosechalfuppervertexangle\pgf@x%
            \edef\deltay{\the\pgf@yc}%
            %
            % Now calculate the height of the kite...
            %
            \advance\pgf@ya-\pgf@yc%
            %
            % ...and the depth.
            %
            \advance\pgf@yb\pgf@yc%
            %
            % Get the half width of the widest part of the kite.
            %
            \pgfmathtan@{\halfuppervertexangle}%
            \pgf@xa\pgfmathresult\pgf@ya%
        \else%
            \multiply\pgf@x2\relax%
            \multiply\pgf@y2\relax%
            %
            % Get the rotation (with rounding).
            %
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Calculate the width and height of the node
            % contents, according to any border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xc\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xc\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xc%
                \fi%
            \fi%
            %
            % The node contents (total height y) extends a distance ya into the
            % upper isosceles triangle of the kite and a distance yb into the
            % lower isosceles triangle. Thus, the following relationships hold:
            %
            %   ya/yb = tan(b/2)/tan(a/2)
            %
            % and   y = ya + yb
            %
            % so   ya = y * sin(a/2 + b/2) / (cos(a/2) * sin(b/2))
            %
            % where:
            %   a = upper vertex angle.
            %   b = lower vertex angle.
            %
            \pgfmathadd@{\halfuppervertexangle}{\halflowervertexangle}%
            \pgfmathsin@{\pgfmathresult}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \pgf@ya\pgfmathresult\pgf@y%
            \pgfmathcos@{\halfuppervertexangle}%
            \pgf@ya\pgfmathresult\pgf@ya%
            \pgfmathsin@{\halflowervertexangle}%
            \pgf@ya\pgfmathresult\pgf@ya%
            \pgf@yb\pgf@y%
            \advance\pgf@yb-\pgf@ya%
            %
            % The vertical offset between the center of the node, and
            % the intersection of the kite diagonals is given by:
            %
            % yc = y/2 - ya
            %
            \pgf@yc.5\pgf@y%
            \advance\pgf@yc-\pgf@ya%
            \edef\deltay{\the\pgf@yc}%
            %
            % Get the half width of the widest part of the kite.
            %
            \pgfmathtan@{\halfuppervertexangle}%
            \pgf@xa.5\pgf@x%
            \advance\pgf@xa\pgfmathresult\pgf@ya%
            %
            % Now calculate the height of the kite...
            %
            \pgf@xb.5\pgf@x%
            \pgfmathreciprocal@{\pgfmathresult}%
            \advance\pgf@ya\pgfmathresult\pgf@xb%
            %
            % ...and the depth.
            %
            \pgfmathtan@{\halflowervertexangle}%
            \pgfmathreciprocal@{\pgfmathresult}%
            \advance\pgf@yb\pgfmathresult\pgf@xb%
        \fi%
        %
        % Take into account minimum height and width.
        %
        % ya is the kite height.
        % yb is the kite depth.
        % xa is the kite (half) width.
        %
        \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
        \pgf@y\pgf@ya%
        \advance\pgf@y\pgf@yb%
        \ifdim\pgf@y<\pgf@yc%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@y}}%
            \pgf@yc\pgfmathresult\pgf@yc%
            \pgf@xa\pgfmath@tonumber{\pgf@yc}\pgf@xa%
            \pgf@ya\pgfmath@tonumber{\pgf@yc}\pgf@ya%
            \pgf@yb\pgfmath@tonumber{\pgf@yc}\pgf@yb%
        \fi%
        \pgf@x2.0\pgf@xa%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgf@x<\pgf@xc%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
            \pgf@xc\pgfmathresult\pgf@xc%
            \pgf@xa\pgfmath@tonumber{\pgf@xc}\pgf@xa%
            \pgf@ya\pgfmath@tonumber{\pgf@xc}\pgf@ya%
            \pgf@yb\pgfmath@tonumber{\pgf@xc}\pgf@yb%
        \fi%
        \edef\kitehalfwidth{\the\pgf@xa}%
        \edef\kiteheight{\the\pgf@ya}%
        \edef\kitedepth{\the\pgf@yb}%
        %
        % Calculate the basic points on the kite (for the background path).
        %
        \pgfextract@process\toppoint{%
            \centerpoint%
            \advance\pgf@y\deltay\relax%
            \advance\pgf@y\kiteheight%
        }%
        \pgfextract@process\bottompoint{%
            \centerpoint%
            \advance\pgf@y\deltay\relax%
            \advance\pgf@y-\kitedepth%
        }%
        \pgfextract@process\leftpoint{%
            \centerpoint%
            \advance\pgf@y\deltay\relax%
            \advance\pgf@x-\kitehalfwidth%
        }%
        \pgfextract@process\rightpoint{%
            \centerpoint%
            \advance\pgf@y\deltay\relax%
                \advance\pgf@x\kitehalfwidth%
        }%
        %
        % Now calculate the miter length. At the top...
        %
        \pgfmathsin@{\halfuppervertexangle}%
        \pgfmathreciprocal@{\pgfmathresult}%
        \pgf@y\outersep\relax%
        \pgf@y\pgfmathresult\pgf@y%
        \edef\topmiter{\the\pgf@y}%
        %
        % ...at the bottom...
        %
        \pgfmathsin@{\halflowervertexangle}%
        \pgfmathreciprocal@{\pgfmathresult}%
        \pgf@y\outersep\relax%
        \pgf@y\pgfmathresult\pgf@y%
        \edef\bottommiter{\the\pgf@y}%
        %
        % ...to the right...
        %
        \pgfmathsubtract@{180}{\halflowervertexangle}%
        \pgfmathsubtract@{\pgfmathresult}{\halfuppervertexangle}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \pgfmathsin@{\pgfmathresult}%
        \pgfmathreciprocal@{\pgfmathresult}%
        \pgf@xa\outersep\relax%
        \pgf@xa\pgfmathresult\pgf@xa%
        \pgfmathsubtract@{\halfuppervertexangle}{\halflowervertexangle}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\angle\pgfmathresult%
        \pgfextract@process\rightmiter{%
            \pgfqpointpolar{\angle}{\the\pgf@xa}%
        }%
        %
        % ...and to the left.
        %
        \pgfmathsubtract@{180}{\angle}%
        \let\angle\pgfmathresult%
        \pgfextract@process\leftmiter{%
            \pgfqpointpolar{\angle}{\the\pgf@xa}%
        }%
        %
        % Create the border points.
        %
        \pgfextract@process\topborderpoint{%
            \toppoint%
            \advance\pgf@y\topmiter\relax%
        }%
        \pgfextract@process\bottomborderpoint{%
            \bottompoint%
            \advance\pgf@y-\bottommiter\relax%
        }%
        \pgfextract@process\leftborderpoint{%
            \leftpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \leftmiter%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfextract@process\rightborderpoint{%
            \rightpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \rightmiter%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        %
        % Get the angle from the \centerpoint to the *unrotated points*.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\topborderpoint}%
        \let\angletotoppoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\leftborderpoint}%
        \let\angletoleftpoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\bottomborderpoint}%
        \let\angletobottompoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\rightborderpoint}%
        \let\angletorightpoint\pgfmathresult%
        %
        % ...from the *inversely rotated* \basepoint...
        %
        \pgfextract@process\rotatedbasepoint{%
            \pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\topborderpoint}%
        \let\baseangletotoppoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\leftborderpoint}%
        \let\baseangletoleftpoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\bottomborderpoint}%
        \let\baseangletobottompoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\rightborderpoint}%
        \let\baseangletorightpoint\pgfmathresult%
        %
        % ...and from the *inversely rotated* \midpoint.
        %
        \pgfextract@process\rotatedmidpoint{%
            \pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\topborderpoint}%
        \let\midangletotoppoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\leftborderpoint}%
        \let\midangletoleftpoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\bottomborderpoint}%
        \let\midangletobottompoint\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\rightborderpoint}%
        \let\midangletorightpoint\pgfmathresult%
        %
        % Calculate a radius guaranteed to be outside the kite.
        %
        \pgfextractx\pgf@xa{\pgfpointdiff{\leftborderpoint}{\rightborderpoint}}%
        \ifdim\pgf@xa<0pt\relax%
            \pgf@xa-\pgf@xa%
        \fi%
        \pgfextracty\pgf@ya{\pgfpointdiff{\topborderpoint}{\bottomborderpoint}}%
        \ifdim\pgf@ya<0pt\relax%
            \pgf@ya-\pgf@ya%
        \fi%
        \ifdim\pgf@ya>\pgf@xa%
            \edef\externalradius{\the\pgf@ya}%
        \else%
            \edef\externalradius{\the\pgf@xa}%
        \fi%
        %
        % Now rotate the points...
        %
        \pgfextract@process\toppoint{%
            \pgfmathrotatepointaround{\toppoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\bottompoint{%
            \pgfmathrotatepointaround{\bottompoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\leftpoint{%
            \pgfmathrotatepointaround{\leftpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\rightpoint{%
            \pgfmathrotatepointaround{\rightpoint}{\centerpoint}{\rotate}%
        }%
        %
        % ...and the border points.
        %
        \pgfextract@process\topborderpoint{%
            \pgfmathrotatepointaround{\topborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\bottomborderpoint{%
            \pgfmathrotatepointaround{\bottomborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\leftborderpoint{%
            \pgfmathrotatepointaround{\leftborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\rightborderpoint{%
            \pgfmathrotatepointaround{\rightborderpoint}{\centerpoint}{\rotate}%
        }%
        %
        % Now save it all.
        %
        \addtosavedmacro{\rotate}%
        \addtosavedmacro{\externalradius}%
        %
        \addtosavedmacro\toppoint%
        \addtosavedmacro\bottompoint%
        \addtosavedmacro\leftpoint%
        \addtosavedmacro\rightpoint%
        %
        \addtosavedmacro\topborderpoint%
        \addtosavedmacro\bottomborderpoint%
        \addtosavedmacro\leftborderpoint%
        \addtosavedmacro\rightborderpoint%
        %
        \addtosavedmacro\angletotoppoint%
        \addtosavedmacro\angletobottompoint%
        \addtosavedmacro\angletoleftpoint%
        \addtosavedmacro\angletorightpoint%
        %
        \addtosavedmacro\baseangletotoppoint%
        \addtosavedmacro\baseangletobottompoint%
        \addtosavedmacro\baseangletoleftpoint%
        \addtosavedmacro\baseangletorightpoint%
        %
        \addtosavedmacro\midangletotoppoint%
        \addtosavedmacro\midangletobottompoint%
        \addtosavedmacro\midangletoleftpoint%
        \addtosavedmacro\midangletorightpoint%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{base}{\basepoint}%
    \anchor{base west}{%
        \installkiteparameters%
        \let\pgf@kiteanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{base east}{%
        \installkiteparameters%
        \let\pgf@kiteanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid west}{%
        \installkiteparameters%
        \let\pgf@kiteanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{mid east}{%
        \installkiteparameters%
        \let\pgf@kiteanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south west}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{south east}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \installkiteparameters%
        \csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{upper vertex}{%
        \installkiteparameters%
        \topborderpoint}%
    \anchor{lower vertex}{%
        \installkiteparameters%
        \bottomborderpoint}%
    \anchor{left vertex}{%
        \installkiteparameters%
        \leftborderpoint}%
    \anchor{right vertex}{%
        \installkiteparameters%
        \rightborderpoint}%
    \anchor{upper left side}{%
        \installkiteparameters%
        \pgfpointlineattime{0.5}{\topborderpoint}{\leftborderpoint}}%
    \anchor{lower left side}{%
        \installkiteparameters%
        \pgfpointlineattime{0.5}{\bottomborderpoint}{\leftborderpoint}}%
    \anchor{upper right side}{%
        \installkiteparameters%
        \pgfpointlineattime{0.5}{\topborderpoint}{\rightborderpoint}}%
    \anchor{lower right side}{%
        \installkiteparameters%
        \pgfpointlineattime{0.5}{\bottomborderpoint}{\rightborderpoint}}%
    \backgroundpath{%
        \installkiteparameters%
        \pgfpathmoveto{\toppoint}%
        \pgfpathlineto{\leftpoint}%
        \pgfpathlineto{\bottompoint}%
        \pgfpathlineto{\rightpoint}%
        \pgfpathclose%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % This allows anchors base east, base west, mid east and mid west,
        % to redefine the `center' of the node to correctly calculate the
        % border points.
        %
        \pgfutil@ifundefined{pgf@kiteanchorborderreferencepoint}%
            {\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@kiteanchorborderreferencepoint}%
        %
        % Adjust the location of the external
        % point relative to the reference point.
        %
        \referencepoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Install the required points and angles.
        %
        \installkiteparameters%
        %
        % Get the angle of the external point relative to \referencepoint.
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
        %
        % *Subtract* the rotation from the external angle.
        %
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        \ifx\referencepoint\basepoint%
            \let\angletotoppoint\baseangletotoppoint%
            \let\angletobottompoint\baseangletobottompoint%
            \let\angletoleftpoint\baseangletoleftpoint%
            \let\angletorightpoint\baseangletorightpoint%
        \else%
            \ifx\referencepoint\midpoint%
                \let\angletotoppoint\midangletotoppoint%
                \let\angletobottompoint\midangletobottompoint%
                \let\angletoleftpoint\midangletoleftpoint%
                \let\angletorightpoint\midangletorightpoint%
        \fi\fi%
        %
        %  Depending on the rotation, the angle to \rightborderpoint
        %  may be smaller than the angle to \topborderpoint.
        %
        \ifdim\angletorightpoint pt<\angletotoppoint pt\relax%
            \ifdim\externalangle pt<\angletorightpoint pt\relax%
                \let\firstpoint\rightborderpoint%
                \let\secondpoint\bottomborderpoint%
            \else%
                \ifdim\externalangle pt<\angletotoppoint pt\relax%
                    \let\firstpoint\rightborderpoint%
                    \let\secondpoint\topborderpoint%
                \else%
                    \ifdim\externalangle pt<\angletoleftpoint pt\relax%
                        \let\firstpoint\topborderpoint%
                        \let\secondpoint\leftborderpoint%
                    \else%
                        \ifdim\externalangle pt<\angletobottompoint pt\relax%
                            \let\firstpoint\leftborderpoint%
                            \let\secondpoint\bottomborderpoint%
                        \else%
                            \let\firstpoint\rightborderpoint%
                            \let\secondpoint\bottomborderpoint%
                        \fi%
                    \fi%
                \fi%
            \fi%
        \else%
            \ifdim\externalangle pt<\angletotoppoint pt\relax%
                \let\firstpoint\rightborderpoint%
                \let\secondpoint\topborderpoint%
            \else%
                \ifdim\externalangle pt<\angletoleftpoint pt\relax%
                    \let\firstpoint\leftborderpoint%
                    \let\secondpoint\topborderpoint%
                \else%
                    \ifdim\externalangle pt<\angletobottompoint pt\relax%
                        \let\firstpoint\bottomborderpoint%
                        \let\secondpoint\leftborderpoint%
                    \else%
                        \ifdim\externalangle pt<\angletorightpoint pt\relax%
                            \let\firstpoint\rightborderpoint%
                            \let\secondpoint\bottomborderpoint%
                        \else%
                            \let\firstpoint\rightborderpoint%
                            \let\secondpoint\topborderpoint%
                        \fi%
                    \fi%
                \fi%
            \fi%
        \fi%
        \pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\firstpoint}{\secondpoint}%
    }%
}%




% Keys for shape dart.
%
%

\pgfkeys{/pgf/.cd,
    dart tip angle/.initial=45,
    dart tail angle/.initial=135,
}%

% Shape dart.
%
\pgfdeclareshape{dart}{%
    \savedmacro\installdartparameters{%
        %
        % Get the halved angles (more useful).
        %
        \pgfmathdivide{\pgfkeysvalueof{/pgf/dart tip angle}}{2}%
        \let\halftipangle\pgfmathresult%
        \pgfmathdivide{\pgfkeysvalueof{/pgf/dart tail angle}}{2}%
        \let\halftailangle\pgfmathresult%
        %
        % Calculate some common results.
        %
        \pgfmathcot@{\halftipangle}%
        \let\cothalftipangle\pgfmathresult%
        %
        % Get the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@x<\pgf@y%
            \pgf@x\pgf@y%
        \fi%
        \edef\outersep{\the\pgf@x}%
        %
        % Calculate the centre, base and mid points of the node.
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        \pgfextract@process\basepoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y0pt\relax%
        }%
        \pgfextract@process\midpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgfmathsetlength\pgf@y{+.5ex}%
        }%
        %
        % Get the (halved) dimension of the node.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        %
        % Get the length of the dart tip.
        %
        \ifpgfshapeborderusesincircle%
            %
            % Get the (unrounded) rotation.
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            %
            % Get the radius of the incircle.
            %
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \fi%
            \pgf@x1.41421\pgf@x%
            %
            % Calculate the length of the dart tip.
            %
            \pgf@xa\cothalftipangle\pgf@x%
            \advance\pgf@xa\pgf@x%
        \else%
            %
            % Get the rotation (with rounding).
            %
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Flip the width and height of the node contents,
            % according to the appropriate border rotation.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xc\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xc\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xc%
                \fi%
            \fi%
            %
            % Calculate the length of the dart tip.
            %
            \pgf@xa\cothalftipangle\pgf@y%
            \advance\pgf@xa2.0\pgf@x%
        \fi%
        %
        % Get the (half) separation of the dart tails.
        %
        \pgfmathsubtract@{\halftailangle}{\halftipangle}%
        \pgfmathcosec@{\pgfmathresult}%
        \pgf@ya\pgfmathresult\pgf@xa%
        \pgfmathsin@{\halftipangle}%
        \pgf@ya\pgfmathresult\pgf@ya%
        \pgfmathcos@{\halftipangle}%
        \pgf@ya\pgfmathresult\pgf@ya%
        %
        % Get the total length of the dart...
        %
        \pgf@xb\cothalftipangle\pgf@ya%
        %
        % and hence the length of the tails.
        %
        \pgf@xc-\pgf@xa%
        \advance\pgf@xc\pgf@xb%
        %
        % Adjust for minimum height (length of the dart).
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@xb<\pgf@y%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xb}}%
            \pgf@y\pgfmathresult\pgf@y%
            \pgf@xa\pgfmath@tonumber{\pgf@y}\pgf@xa%
            \pgf@xc\pgfmath@tonumber{\pgf@y}\pgf@xc%
            \pgf@ya\pgfmath@tonumber{\pgf@y}\pgf@ya%
            \pgf@x\pgfmath@tonumber{\pgf@y}\pgf@x%
        \fi%
        %
        % Adjust for minimum width (tail separation length).
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgf@y.5\pgf@y%
        \ifdim\pgf@ya<\pgf@y%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@ya}}%
            \pgf@ya\pgf@y%
            \pgf@y\pgfmathresult\pgf@y%
            \pgf@xa\pgfmath@tonumber{\pgf@y}\pgf@xa%
            \pgf@xc\pgfmath@tonumber{\pgf@y}\pgf@xc%
            \pgf@x\pgfmath@tonumber{\pgf@y}\pgf@x%
        \fi%
        \edef\dartlength{\the\pgf@xa}%
        \edef\deltax{\the\pgf@x}%
        \edef\taillength{\the\pgf@xc}%
        \edef\halftailseparation{\the\pgf@ya}
        %
        % Create the basic points on the dart (for the background path).
        %
        \pgfextract@process\tippoint{%
            \centerpoint%
            \advance\pgf@x\dartlength\relax%
            \advance\pgf@x-\deltax\relax%
        }%
        \pgfextract@process\tailcenterpoint{%
            \centerpoint%
            \advance\pgf@x-\deltax\relax%
        }%
        \pgfextract@process\lefttailpoint{%
            \centerpoint%
            \advance\pgf@x-\deltax\relax%
            \advance\pgf@x-\taillength\relax%
            \advance\pgf@y\halftailseparation\relax%
        }%
        \pgfextract@process\righttailpoint{%
            \centerpoint%
            \advance\pgf@x-\deltax\relax%
            \advance\pgf@x-\taillength\relax%
            \advance\pgf@y-\halftailseparation\relax%
        }%
        %
        % Calculate the miter vectors. At the dart tip...
        %
        \pgfextract@process\tipmiter{%
            \pgfmathcosec@{\halftipangle}%
            \pgf@x\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y0pt\relax%
        }%
        %
        % ...at the tail center...
        %
        \pgfextract@process\tailcentermiter{%
            \pgfmathcosec@{\halftailangle}%
            \pgf@x-\outersep\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y0pt\relax%
        }%
        %
        % ...at the left tail...
        %
        \pgfmathsubtract@{\halftailangle}{\halftipangle}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\angle\pgfmathresult%
        \pgfmathcosec@{\pgfmathresult}%
        \pgf@x\outersep\relax%
        \pgf@x\pgfmathresult\pgf@x%
        \pgfmathadd@{\angle}{90}%
        \pgfmathsubtract{\pgfmathresult}{\halftailangle}%
        \pgfmathsincos@{\pgfmathresult}%
        \pgf@ya\pgfmathresultx\pgf@x%
        \pgf@xa\pgfmathresulty\pgf@x%
        \pgfextract@process\lefttailmiter{%
            \pgf@x-\pgf@xa%
            \pgf@y\pgf@ya%
        }%
        %
        % ...and the right tail.
        %
        \pgfextract@process\righttailmiter{%
            \pgf@x-\pgf@xa%
            \pgf@y-\pgf@ya%
        }%
        %
        % Create the border points.
        %
        \pgfextract@process\tipborderpoint{%
            \pgfpointadd{\tippoint}{\tipmiter}
        }%
        \pgfextract@process\tailcenterborderpoint{%
            \pgfpointadd{\tailcenterpoint}{\tailcentermiter}%
        }%
        \pgfextract@process\lefttailborderpoint{%
            \pgfpointadd{\lefttailpoint}{\lefttailmiter}%
        }%
        \pgfextract@process\righttailborderpoint{%
            \pgfpointadd{\righttailpoint}{\righttailmiter}%
        }%
        %
        % Calculate the angles between the centerpoint
        % and the *unrotated* borderpoints.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\tipborderpoint}%
        \let\angletotip\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\tailcenterborderpoint}%
        \let\angletotailcenter\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\lefttailborderpoint}%
        \let\angletolefttail\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\righttailborderpoint}%
        \let\angletorighttail\pgfmathresult%
        %
        % Calculate the angles between the *inversely rotated*
        % basepoint and the *unrotated* borderpoints.
        %
        \pgfextract@process\rotatedbasepoint{%
            \pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\tipborderpoint}%
        \let\baseangletotip\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\tailcenterborderpoint}%
        \let\baseangletotailcenter\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\lefttailborderpoint}%
        \let\baseangletolefttail\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedbasepoint}{\righttailborderpoint}%
        \let\baseangletorighttail\pgfmathresult%
        %
        % Calculate the angles between the *inversely rotated*
        % midpoint and the *unrotated* borderpoints.
        %
        \pgfextract@process\rotatedmidpoint{%
            \pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
        }%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\tipborderpoint}%
        \let\midangletotip\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\tailcenterborderpoint}%
        \let\midangletotailcenter\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\lefttailborderpoint}%
        \let\midangletolefttail\pgfmathresult%
        \pgfmathanglebetweenpoints{\rotatedmidpoint}{\righttailborderpoint}%
        \let\midangletorighttail\pgfmathresult%
        %
        % Rotate the background path points.
        %
        \pgfextract@process\tippoint{%
            \pgfmathrotatepointaround{\tippoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\tailcenterpoint{%
            \pgfmathrotatepointaround{\tailcenterpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\lefttailpoint{%
            \pgfmathrotatepointaround{\lefttailpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\righttailpoint{%
            \pgfmathrotatepointaround{\righttailpoint}{\centerpoint}{\rotate}%
        }%
        %
        % Calculate a radius guaranteed to be outside the dart.
        %
        \pgfextractx\pgf@xa{\pgfpointdiff{\lefttailborderpoint}{\tipborderpoint}}%
        \pgfextracty\pgf@ya{\pgfpointdiff{\lefttailborderpoint}{\righttailborderpoint}}%
        \ifdim\pgf@xa<0pt\relax%
            \pgf@xa-\pgf@xa%
        \fi%
        \ifdim\pgf@ya<0pt\relax%
            \pgf@ya-\pgf@ya%
        \fi%
        \ifdim\pgf@xa>\pgf@ya%
            \edef\externalradius{\the\pgf@xa}%
        \else%
            \edef\externalradius{\the\pgf@ya}%
        \fi%
        %
        % Rotate the border anchor points.
        %
        \pgfextract@process\tipborderpoint{%
            \pgfmathrotatepointaround{\tipborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\tailcenterborderpoint{%
            \pgfmathrotatepointaround{\tailcenterborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\lefttailborderpoint{%
            \pgfmathrotatepointaround{\lefttailborderpoint}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\righttailborderpoint{%
            \pgfmathrotatepointaround{\righttailborderpoint}{\centerpoint}{\rotate}%
        }%
        %
        % Save everything.
        %
        \addtosavedmacro{\rotate}%
        \addtosavedmacro{\externalradius}%
        %
        \addtosavedmacro{\tippoint}%
        \addtosavedmacro{\tailcenterpoint}%
        \addtosavedmacro{\lefttailpoint}%
        \addtosavedmacro{\righttailpoint}%
        %
        \addtosavedmacro{\tipborderpoint}%
        \addtosavedmacro{\tailcenterborderpoint}%
        \addtosavedmacro{\lefttailborderpoint}%
        \addtosavedmacro{\righttailborderpoint}%
        %
        \addtosavedmacro{\angletotip}%
        \addtosavedmacro{\angletotailcenter}%
        \addtosavedmacro{\angletolefttail}%
        \addtosavedmacro{\angletorighttail}%
        %
        \addtosavedmacro{\baseangletotip}%
        \addtosavedmacro{\baseangletotailcenter}%
        \addtosavedmacro{\baseangletolefttail}%
        \addtosavedmacro{\baseangletorighttail}%
        %
        \addtosavedmacro{\midangletotip}%
        \addtosavedmacro{\midangletotailcenter}%
        \addtosavedmacro{\midangletolefttail}%
        \addtosavedmacro{\midangletorighttail}%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{base}{\basepoint}%
    \anchor{base west}{%
        \installdartparameters%
        \let\pgf@dartanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{base east}{%
        \installdartparameters%
        \let\pgf@dartanchorborderreferencepoint\basepoint%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid west}{%
        \installdartparameters%
        \let\pgf@dartanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{mid east}{%
        \installdartparameters%
        \let\pgf@dartanchorborderreferencepoint\midpoint%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south west}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{south east}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \installdartparameters%
        \csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{tip}{%
        \installdartparameters%
        \tipborderpoint}%
    \anchor{left tail}{%
        \installdartparameters%
        \lefttailborderpoint}%
    \anchor{right tail}{%
        \installdartparameters%
        \righttailborderpoint}%
    \anchor{tail center}{%
        \installdartparameters%
        \tailcenterborderpoint}%
    \anchor{left side}{%
        \installdartparameters%
        \pgfpointlineattime{0.5}{\tipborderpoint}{\lefttailborderpoint}}%
    \anchor{right side}{%
        \installdartparameters%
        \pgfpointlineattime{0.5}{\tipborderpoint}{\righttailborderpoint}}%
    \backgroundpath{%
        \installdartparameters%
        \pgfpathmoveto{\tippoint}%
        \pgfpathlineto{\lefttailpoint}%
        \pgfpathlineto{\tailcenterpoint}%
        \pgfpathlineto{\righttailpoint}%
        \pgfpathclose%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % This allows anchors base east, base west, mid east and mid west,
        % to redefine the `center' of the node to correctly calculate the
        % border points.
        %
        \pgfutil@ifundefined{pgf@dartanchorborderreferencepoint}%
            {\let\referencepoint\centerpoint}%
            {\let\referencepoint\pgf@dartanchorborderreferencepoint}%
        %
        % Adjust the location of the external
        % point relative to the reference point.
        %
        \referencepoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Install the required points and angles.
        %
        \installdartparameters%
        %
        % Get the angle of the external point relative to \referencepoint.
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
        %
        % *Subtract* the rotation from the external angle.
        %
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        %
        % Get the set of angles for the appropriate border point.
        %
        \ifx\referencepoint\basepoint%
            \let\angletotip\baseangletotip%
            \let\angletotailcenter\baseangletotailcenter%
            \let\angletolefttail\baseangletolefttail%
            \let\angletorighttail\baseangletorighttail%
        \else%
            \ifx\referencepoint\midpoint%
                \let\angletotip\midangletotip%
                \let\angletotailcenter\midangletotailcenter%
                \let\angletolefttail\midangletolefttail%
                \let\angletorighttail\midangletorighttail%
        \fi\fi%
        %
        % Locate the appropriate line on the border...
        %
        \ifdim\externalangle pt<\angletotip pt\relax%
            \let\firstpoint\tipborderpoint%
            \let\secondpoint\righttailborderpoint%
        \else%
            \ifdim\externalangle pt<\angletolefttail pt\relax%
                \let\firstpoint\lefttailborderpoint%
                \let\secondpoint\tipborderpoint%
            \else%
                \ifdim\externalangle pt<\angletotailcenter pt\relax%
                    \let\firstpoint\lefttailborderpoint%
                    \let\secondpoint\tailcenterborderpoint%
                \else%
                    \ifdim\externalangle pt<\angletorighttail pt\relax%
                        \let\firstpoint\righttailborderpoint%
                        \let\secondpoint\tailcenterborderpoint%
                    \else%
                        \let\firstpoint\tipborderpoint%
                        \let\secondpoint\righttailborderpoint%
                    \fi%
                \fi%
            \fi%
        \fi%
        %
        % ...and thus the point on the border.
        %
        \pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\firstpoint}{\secondpoint}%
    }%
}%



% Keys for shape circular sector:
%
% /pgf/circular sector angle : the angle at the center of the sector.
%
\pgfkeys{/pgf/circular sector angle/.initial=60}%

% Shape circular sector
%
\pgfdeclareshape{circular sector}{%
    \savedmacro\installcircularsectorparameters{%
        %
        % Define a \centerpoint, \basepoint and \midpoint.
        %
        \pgfextract@process\centerpoint{%
            \pgf@x.5\wd\pgfnodeparttextbox%
            \pgf@y.5\ht\pgfnodeparttextbox%
            \advance\pgf@y-.5\dp\pgfnodeparttextbox%
        }%
        %
        % Get the larger of the outer sep.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@x<\pgf@y%
            \pgf@x\pgf@y%
        \fi%
        \edef\outersep{\the\pgf@x}%
        %
        % Half of the sector angle is more useful.
        %
        \pgfmathmod{\pgfkeysvalueof{/pgf/circular sector angle}}{360}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\angle\pgfmathresult%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\halfangle\pgfmathresult%
        %
        % Get some useful trigonometric stuff.
        %
        \pgfmathsin@{\halfangle}%
        \let\sinehalfangle\pgfmathresult%
        \pgfmathreciprocal@{\pgfmathresult}%
        \let\cosechalfangle\pgfmathresult%
        \pgfmathabs@{\halfangle}%
        \pgfmathcos@{\pgfmathresult}%
        \let\coshalfangle\pgfmathresult%
        \pgf@x\pgfmathresult pt\relax%
        \pgf@x\cosechalfangle\pgf@x%
        \edef\cothalfangle{\pgfmath@tonumber{\pgf@x}}%
        %
        % Calculate the miter length at the center,
        % according to the outer sep.
        %
        \pgf@x\outersep\relax%
        \pgf@x\cosechalfangle\pgf@x%
        \edef\centermiter{\the\pgf@x}%
        %
        % Get the start and end angles of the arc.
        %
        \pgfmathsubtract@{180}{\halfangle}%
        \let\startangle\pgfmathresult%
        \pgfmathadd@{180}{\halfangle}%
        \let\endangle\pgfmathresult%
        %
        % Get (half) the node dimensions.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        %
        % Calculate the radius of the sector and the `center offset',
        % which is the distance between the center of the node and the
        % center of the sector.
        %
        \ifpgfshapeborderusesincircle%
            %
            % Get the rotation.
            %
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            %
            % Calculate the incircle radius.
            %
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \fi%
            \pgf@x1.41421\pgf@x%
            \pgf@xa\cosechalfangle\pgf@x%
            %
            % xa is the radius, xb the offset.
            %
            \pgf@xb\pgf@xa%
            \advance\pgf@xa\pgf@x%
        \else%
            %
            % Get the rotation (with rounding).
            %
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \afterassignment\pgfmath@gobbletilpgfmath@%
            \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \ifnum\c@pgf@counta<0\relax%
                \advance\c@pgf@counta360\relax%
            \fi%
            \edef\rotate{\the\c@pgf@counta}%
            %
            % Swap the height and width for relevant angles.
            %
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xc\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xc\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xc%
                \fi%
            \fi%
            %
            % xa is the radius, xb the offset.
            %
            \pgf@xa\cosechalfangle\pgf@y%
            \pgf@xa\coshalfangle\pgf@xa%
            \advance\pgf@xa\pgf@x%
            \pgf@xb\pgf@xa%
            \advance\pgf@xa\pgf@x%
            \pgfmathveclen@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@y}}%
            \pgf@xa\pgfmathresult pt\relax%
        \fi%
        %
        % Adjust for minimum height and width.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgf@x.5\pgf@x%
        \pgfmathsec@{\halfangle}%
        \pgf@xc\pgfmathresult\pgf@xb%
        \ifdim\pgf@xc<0pt\relax%
            \pgf@xc-\pgf@xc%
        \fi%
        \ifdim\pgf@xc<\pgf@x%
            \pgfmathreciprocal{\pgfmath@tonumber{\pgf@xc}}%
            \pgf@xc\pgfmathresult\pgf@x% Increase by ratio.
            \pgf@xa\pgfmath@tonumber{\pgf@xc}\pgf@xa%
            \pgf@xb\pgfmath@tonumber{\pgf@xc}\pgf@xb%
        \fi%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@xa<\pgf@y%
            \pgfmathreciprocal{\pgfmath@tonumber{\pgf@xa}}%
            \pgf@xc\pgfmathresult\pgf@y% Increase by ratio.
            \pgf@xa\pgf@y%
            \pgf@xb\pgfmath@tonumber{\pgf@xc}\pgf@xb%
        \fi%
        \edef\centeroffset{\the\pgf@xb}%
        \edef\radius{\the\pgf@xa}%
        %
        % Calculate the radius at sector border and the arc corners.
        %
        \advance\pgf@xa\outersep\relax%
        \edef\borderradius{\the\pgf@xa}%
        \pgf@x\outersep\relax%
        \pgf@x\cosechalfangle\pgf@x%
        \pgf@x\coshalfangle\pgf@x%
        \advance\pgf@xa\pgf@x%
        \edef\cornerradius{\the\pgf@xa}%
        %
        % Calculate the *unrotated* points for the background path.
        %
        \pgfextract@process\sectorcenter{%
            \centerpoint%
            \advance\pgf@x\centeroffset%
        }%
        \pgfextract@process\arcstart{%
            \pgfqpointpolar{\startangle}{\radius}%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \sectorcenter%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        %
        % Calculate the *unrotated* points for the anchor border.
        %
        \pgfextract@process\sectorcenterborder{%
            \sectorcenter%
            \advance\pgf@x\centermiter\relax%
        }%
        \pgfextract@process\arcstartborder{%
            \pgfqpointpolar{\startangle}{\borderradius}%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \sectorcenter%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfextract@process\arcendborder{%
            \pgfqpointpolar{\endangle}{\borderradius}%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \sectorcenter%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfextract@process\arcstartcorner{%
            \pgfqpointpolar{\startangle}{\cornerradius}%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \sectorcenterborder%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfextract@process\arcendcorner{%
            \pgfqpointpolar{\endangle}{\cornerradius}%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \sectorcenterborder%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        %
        % Calculate the *unrotated* corner angles to the \centerpoint.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\sectorcenterborder}%
        \let\angletosectorcenterborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcstartborder}%
        \let\angletoarcstartborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcendborder}%
        \let\angletoarcendborder\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcstartcorner}%
        \let\angletoarcstartcorner\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\arcendcorner}%
        \let\angletoarcendcorner\pgfmathresult%
        %
        % Rotate the background path points around the note center.
        %
        \pgfextract@process\sectorcenter{%
            \pgfmathrotatepointaround{\sectorcenter}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcstart{%
            \pgfmathrotatepointaround{\arcstart}{\centerpoint}{\rotate}%
        }%
        %
        % Rotate the border points around the note center.
        %
        \pgfextract@process\sectorcenterborder{%
            \pgfmathrotatepointaround{\sectorcenterborder}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcstartborder{%
            \pgfmathrotatepointaround{\arcstartborder}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcendborder{%
            \pgfmathrotatepointaround{\arcendborder}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcstartcorner{%
            \pgfmathrotatepointaround{\arcstartcorner}{\centerpoint}{\rotate}%
        }%
        \pgfextract@process\arcendcorner{%
            \pgfmathrotatepointaround{\arcendcorner}{\centerpoint}{\rotate}%
        }%
        %
        % Add the rotation to the start and end angles.
        %
        \pgfmathadd@{\startangle}{\rotate}%
        \let\startangle\pgfmathresult%
        \pgfmathadd@{\endangle}{\rotate}%
        \let\endangle\pgfmathresult%
        %
        % Save everything.
        %
        % NB \addtosavedmacro is currently experimental. May get changed.
        %
        \addtosavedmacro{\rotate}%
        \addtosavedmacro{\centeroffset}%
        %
        \addtosavedmacro{\radius}%
        \addtosavedmacro{\borderradius}%
        \addtosavedmacro{\cornerradius}%
        %
        \addtosavedmacro{\endangle}%
        \addtosavedmacro{\startangle}%
        %
        \addtosavedmacro{\sectorcenter}%
        \addtosavedmacro{\arcstart}%
        %
        \addtosavedmacro{\sectorcenterborder}%
        \addtosavedmacro{\arcstartborder}%
        \addtosavedmacro{\arcendborder}%
        \addtosavedmacro{\arcstartcorner}%
        \addtosavedmacro{\arcendcorner}%
        %
        \addtosavedmacro{\angletosectorcenterborder}%
        \addtosavedmacro{\angletoarcstartborder}%
        \addtosavedmacro{\angletoarcendborder}%
        \addtosavedmacro{\angletoarcstartcorner}%
        \addtosavedmacro{\angletoarcendcorner}%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{base}{\basepoint}%
    \anchor{mid}{\midpoint}%
    \anchor{arc start}{%
        \installcircularsectorparameters%
        \arcstartcorner%
    }%
    \anchor{arc end}{%
        \installcircularsectorparameters%
        \arcendcorner%
    }%
    \anchor{sector center}{%
        \installcircularsectorparameters%
        \sectorcenterborder%
    }%
    \anchor{arc center}{%
        \installcircularsectorparameters%
        \pgfmathadd@{\rotate}{180}%
        \let\angle\pgfmathresult%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpointpolar{\angle}{\cornerradius}}%
    }%
    \anchor{north}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{0pt}{\cornerradius}}%
    }%
    \anchor{south}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{0pt}{-\cornerradius}}%
    }%
    \anchor{east}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{0pt}}%
    }%
    \anchor{west}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{0pt}}%
    }%
    \anchor{north west}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{\cornerradius}}%
    }%
    \anchor{south west}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{-\cornerradius}}%
    }%
    \anchor{north east}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{\cornerradius}}%
    }%
    \anchor{south east}{%
        \installcircularsectorparameters%
        \csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{-\cornerradius}}%
    }%
    \backgroundpath{%
        \installcircularsectorparameters%
        \pgfpathmoveto{\sectorcenter}%
        \pgfpathlineto{\arcstart}%
        \ifdim\endangle pt>360pt\relax%
            \ifdim\startangle pt>360pt\relax%
                \pgfpatharc{\startangle}{\endangle}{\radius}%
            \else%
                \pgfpatharc{\startangle}{360}{\radius}%
                \pgfpatharc{0}{\endangle}{\radius}%
            \fi%
        \else%
            \pgfpatharc{\startangle}{\endangle}{\radius}%
        \fi%
        \pgfpathclose%
    }%
    \anchorborder{%
        %
        % Save x and y.
        %
        \edef\externalx{\the\pgf@x}%
        \edef\externaly{\the\pgf@y}%
        %
        % Adjust the location of the external  point relative to \centerpoint.
        %
        \centerpoint%
        \pgf@xa\externalx\relax%
        \pgf@ya\externaly\relax%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@ya\pgf@y%
        \edef\externalx{\the\pgf@xa}%
        \edef\externaly{\the\pgf@ya}%
        %
        % Install the required points and angles.
        %
        \installcircularsectorparameters%
        %
        % Get the angle of the external point to the \centerpoint.
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
        \let\externalangle\pgfmathresult%
        %
        % *Subtract* the rotation from the external angle.
        %
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\angle\pgfmathresult%
        %
        % Determine if the line will cross the sector arc.
        %
        \ifdim\angle pt>\angletoarcendcorner pt\relax%
            \let\firstpoint\arcendcorner%
            \let\secondpoint\sectorcenterborder%
        \else%
            \ifdim\angle pt>\angletoarcendborder pt\relax%
                \let\firstpoint\arcendborder%
                \let\secondpoint\arcendcorner%
            \else%
                \ifdim\angle pt>\angletoarcstartborder pt\relax%
                    \let\firstpoint\pgfutil@empty%
                    \let\secondpoint\pgfutil@empty%
                \else%
                    \ifdim\angle pt>\angletoarcstartcorner pt\relax%
                        \let\firstpoint\arcstartborder
                        \let\secondpoint\arcstartcorner
                    \else%
                        \let\firstpoint\sectorcenterborder%
                        \let\secondpoint\arcstartcorner%
                    \fi%
                \fi%
            \fi%
        \fi%
        \ifx\firstpoint\pgfutil@empty
            %
            % Calculate the angle from the centre of the semicircle to the
            % point on the semicircle arc which intersects the line from
            % the external point to the reference point...
            %
            \pgfmathanglebetweenlines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\sectorcenter}{\centerpoint}%
            \pgfmathsin@{\pgfmathresult}%
            \let\sineangle\pgfmathresult%
            \pgf@x\borderradius\relax%
            \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
            \let\reciprocalradius\pgfmathresult%
            \pgf@x\centeroffset\relax%
            \pgf@x\sineangle\pgf@x%
            \pgf@x\reciprocalradius\pgf@x%
            \pgfmathasin@{\pgfmath@tonumber{\pgf@x}}%
            \pgf@x\pgfmathresult pt\relax%
            \advance\pgf@x\externalangle pt\relax%
            \edef\angle{\pgfmath@tonumber{\pgf@x}}%
            %
            % ...and thus the point on the border.
            %
            \pgfpointadd{\sectorcenter}{\pgfqpointpolar{\angle}{\borderradius}}%
        \else%
            %
            % Calculate the the point where the semicircle chord intersects
            % the line from the external point to the reference point.
            %
            \pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
                {\firstpoint}{\secondpoint}%
        \fi%
    }%
}%



% Keys for shape cylinder
%
% /pgf/shape aspect              : Ratio between the x and y radii of the cylinder end.
% /pgf/cylinder uses custom fill : Use a custom fill for the cylinder.
% /pgf/cylinder end fill         : Custom color for the cylinder end.
% /pgf/cylinder body fill        : Custom color for the cylinder body.
%

\newif\ifpgfcylinderusescustomfill
\pgfkeys{/pgf/.cd,
    cylinder uses custom fill/.is if=pgfcylinderusescustomfill,
    cylinder end fill/.initial=white,
    cylinder body fill/.initial=white,
}%


\pgfdeclareshape{cylinder}{%
    \savedmacro\getcylinderpoints{%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
        \pgf@x\pgf@xc%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
        \pgf@y\pgf@yc%
        \advance\pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y.5\dp\pgfnodeparttextbox%
        \ifpgfshapeborderusesincircle%
            \pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
            \ifdim\pgf@x<\pgf@y%
                \pgf@x\pgf@y%
            \else%
                \pgf@y\pgf@x%
            \fi%
            \pgf@x1.414213\pgf@x%
            \pgf@y1.414213\pgf@y%
        \else%
            \pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
            \ifdim\pgfmathresult pt<0pt\relax%
                \pgfmathadd@{\pgfmathresult}{360}%
            \fi%
            \pgfmathsetcount\c@pgf@counta{+\pgfmathresult}%
            \advance\c@pgf@counta45\relax%
            \divide\c@pgf@counta90\relax%
            \multiply\c@pgf@counta90\relax%
            \edef\rotate{\the\c@pgf@counta}%
            \ifnum\c@pgf@counta=90\relax%
                \pgf@xa\pgf@x%
                \pgf@x\pgf@y%
                \pgf@y\pgf@xa%
                \pgf@yc\pgf@xc%
            \else%
                \ifnum\c@pgf@counta=270\relax%
                    \pgf@xa\pgf@x%
                    \pgf@x\pgf@y%
                    \pgf@y\pgf@xa%
                    \pgf@yc\pgf@xc%
                \fi%
            \fi%
        \fi%
        \addtosavedmacro\rotate%
        \pgf@xa\pgf@x%
        \pgf@ya\pgf@y%
        \pgfutil@tempdima\pgfshapeaspect\pgf@ya%
        \pgfutil@tempdimb\pgf@ya%
        %
        % Adjust for minimum height.
        %
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgfutil@tempdimb<.5\pgf@xc\relax%
            \pgfutil@tempdimb.5\pgf@xc%
            \pgf@ya\pgfutil@tempdimb%
        \fi%
        %
        % Calculate how far the node contents can extend into the cylinder bottom.
        %
        \pgf@yb\pgfutil@tempdimb%
        \advance\pgf@yb-\pgf@yc%
        \pgfmathdivide@{\pgfmath@tonumber{\pgf@yb}}{\pgfmath@tonumber{\pgfutil@tempdimb}}%
        \pgfmathasin@{\pgfmathresult}%
        \pgfmathcos@{\pgfmathresult}%
        \let\angle\pgfmathresult%
        \pgf@xb\pgfmathresult\pgfutil@tempdima%
        %
        % Adjust for minimum width.
        %
        \pgf@x.5\pgflinewidth%
        \advance\pgf@x2.0\pgf@xa%
        \advance\pgf@x3.0\pgfutil@tempdima%
        \advance\pgf@x-\pgf@xb%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@x<\pgf@xc%
            \advance\pgf@xc-\pgf@x%
            \advance\pgf@xa.5\pgf@xc%
        \fi%
        %
        % Add the larger of the outer sep to the radii.
        %
        \pgf@x\pgfutil@tempdima\relax%
        \pgf@y\pgfutil@tempdimb\relax%
        \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgf@xc>\pgf@yc%
            \advance\pgf@x\pgf@xc%
            \advance\pgf@y\pgf@xc%
            \edef\outersep{\the\pgf@xc}%
        \else%
            \advance\pgf@x\pgf@yc%
            \advance\pgf@y\pgf@yc%
            \edef\outersep{\the\pgf@yc}%
        \fi%
        \edef\xradius{\the\pgf@x}%
        \edef\yradius{\the\pgf@y}%
        \addtosavedmacro\xradius%
        \addtosavedmacro\yradius%
        \addtosavedmacro\outersep%
        %
        \pgfextract@process\cylindercenter{%
            \pgf@x\pgfutil@tempdima%
            \advance\pgf@x.5\pgflinewidth%
            \advance\pgf@x\pgf@xb%
            \pgf@x.5\pgf@x%
            \pgf@y0pt%
        }%
        \addtosavedmacro\cylindercenter%
        %
        \pgfextract@process\beforetop{%
            \pgf@x\pgf@xa%
            \advance\pgf@x\pgfutil@tempdima%
            \advance\pgf@x.5\pgflinewidth%
            \pgf@y\pgf@ya%
        }%
        \pgfextract@process\afterbottom{%
            \pgf@x-\pgf@xa%
            \advance\pgf@x\pgf@xb%
            \pgf@y\pgf@ya%
        }%
        \addtosavedmacro\beforetop%
        \addtosavedmacro\afterbottom%
        \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/outer ysep}}%
        \pgfextract@process\beforetopanchor{%
            \beforetop%
            \advance\pgf@y\pgf@yc%
        }%
        \pgfextract@process\afterbottomanchor{%
            \afterbottom%
            \advance\pgf@y\pgf@yc%
        }%
        \addtosavedmacro\beforetopanchor%
        \addtosavedmacro\afterbottomanchor%
        %
        \beforetopanchor%
        \advance\pgf@x\xradius\relax%
        \ifdim\pgf@x>\pgf@y%
            \edef\externalradius{\the\pgf@x}%
        \else%
            \edef\externalradius{\the\pgf@y}%
        \fi%
        \addtosavedmacro\externalradius%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+0.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{shape center}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{\pgfpointadd{\cylindercenter}{\centerpoint}}%
            {\centerpoint}{\rotate}%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \getcylinderpoints%
        \let\pgf@cylinder@referencepoint\midpoint%
        \pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{mid west}{%
        \getcylinderpoints%
        \let\pgf@cylinder@referencepoint\midpoint%
        \pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \getcylinderpoints%
        \let\pgf@cylinder@referencepoint\basepoint%
        \pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{base west}{%
        \getcylinderpoints%
        \let\pgf@cylinder@referencepoint\basepoint%
        \pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{0pt}{\externalradius}}%
    }%
    \anchor{south}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{0pt}{-\externalradius}}%
    }%
    \anchor{east}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
    }%
    \anchor{west}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
    }%
    \anchor{north east}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{\externalradius}}%
    }%
    \anchor{south west}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{-\externalradius}}%
    }%
    \anchor{south east}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{-\externalradius}}%
    }%
    \anchor{north west}{%
        \getcylinderpoints%
        \pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{\externalradius}}%
    }%
    \anchor{before top}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor}{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \anchor{top}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \beforetop%
                \pgf@y0pt\relax%
                \advance\pgf@x\xradius\relax%
            }{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \anchor{after top}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \anchor{before bottom}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \anchor{bottom}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{%
            \pgfpointadd{%
                \afterbottom%
                \pgf@y0pt\relax%
                \advance\pgf@x-\xradius\relax%
            }{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \anchor{after bottom}{%
        \getcylinderpoints%
        \pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor}{\centerpoint}}{\centerpoint}{\rotate}%
    }%
    \backgroundpath{%
        \getcylinderpoints%
        {%
            \pgf@x\xradius\relax%
            \advance\pgf@x-\outersep\relax%
            \edef\xradius{\the\pgf@x}%
            \pgf@y\yradius\relax%
            \advance\pgf@y-\outersep\relax%
            \edef\yradius{\the\pgf@y}%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            \pgfpathmoveto{\afterbottom}%
            \pgfpatharc{90}{270}{\xradius and \yradius}%
            \pgfpathlineto{\beforetop\pgf@y-\pgf@y}%
            \pgfpatharc{-90}{90}{\xradius and \yradius}%
            \pgfpathclose%
            \pgfpathmoveto{\beforetop}%
            \pgfpatharc{90}{270}{\xradius and \yradius}%
        }%
    }%
    \behindbackgroundpath{%
        \ifpgfcylinderusescustomfill%
            \getcylinderpoints%
            \pgf@x\xradius\relax%
            \advance\pgf@x-\outersep\relax%
            \edef\xradius{\the\pgf@x}%
            \pgf@y\yradius\relax%
            \advance\pgf@y-\outersep\relax%
            \edef\yradius{\the\pgf@y}%
            {%
                \pgftransformshift{\centerpoint}%
                \pgftransformrotate{\rotate}%
                \pgfpathmoveto{\afterbottom}%
                \pgfpatharc{90}{270}{\xradius and \yradius}%
                \pgfpathlineto{\beforetop\pgf@y-\pgf@y}%
                \pgfpatharc{270}{90}{\xradius and \yradius}%
                \pgfpathclose%
                \expandafter\pgfsetfillcolor\expandafter{\pgfkeysvalueof{/pgf/cylinder body fill}}%
                \pgfusepath{fill}%
                %
                \pgfpathmoveto{\beforetop}%
                \pgfpatharc{90}{-270}{\xradius and \yradius}%
                \pgfpathclose
                \expandafter\pgfsetfillcolor\expandafter{\pgfkeysvalueof{/pgf/cylinder end fill}}%
                \pgfusepath{fill}%
            }%
        \fi%
    }%
    \anchorborder{%
        \pgfextract@process\externalpoint{}%
        \getcylinderpoints%
        \pgfutil@ifundefined{pgf@cylinder@referencepoint}{\let\referencepoint\centerpoint}{%
            \let\referencepoint\pgf@cylinder@referencepoint}%
        \pgfextract@process\externalpoint{%
            \externalpoint%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \referencepoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \pgfmathsubtract@{\pgfmathresult}{\rotate}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathadd@{\pgfmathresult}{360}%
        \fi%
        \let\externalangle\pgfmathresult%
        %
        \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\afterbottomanchor}{\centerpoint}}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
            \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\beforetopanchor}{\centerpoint}}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                \pgfmathrotatepointaround{%
                    \pgfmathpointintersectionoflineandarc%
                        {\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
                        {\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
                        {%
                            \beforetop%
                            \pgf@xa\pgf@x%
                            \centerpoint%
                            \advance\pgf@x\pgf@xa%
                        }%
                        {0}{90}{\xradius and \yradius}%
                    }{\centerpoint}{\rotate}%
            \else%
                \pgfpointintersectionoflines{%
                    \pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor}{\centerpoint}}%
                        {\centerpoint}{\rotate}}{%
                    \pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor}{\centerpoint}}%
                        {\centerpoint}{\rotate}}%
                    {\referencepoint}{\externalpoint}%
            \fi%
        \else%
            \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}%
            \ifdim\externalangle pt>\pgfmathresult pt\relax%
                \pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}%
                \ifdim\externalangle pt>\pgfmathresult pt\relax%
                    \pgfmathrotatepointaround{%
                        \pgfmathpointintersectionoflineandarc%
                            {\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
                            {\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
                            {%
                                \beforetop%
                                \pgf@xa\pgf@x%
                                \centerpoint
                                \advance\pgf@x\pgf@xa%
                            }%
                            {270}{360}{\xradius and \yradius}%
                        }{\centerpoint}{\rotate}%
                \else%
                    \pgfpointintersectionoflines{%
                        \pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}%
                            {\centerpoint}{\rotate}}{%
                        \pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}%
                            {\centerpoint}{\rotate}}%
                        {\referencepoint}{\externalpoint}%
                \fi%
            \else%
                \pgfmathrotatepointaround{%
                    \pgfmathpointintersectionoflineandarc%
                        {\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
                        {\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
                        {%
                            \afterbottom%
                            \pgf@xa\pgf@x%
                            \centerpoint
                            \advance\pgf@x\pgf@xa%
                        }%
                        {90}{270}{\xradius and \yradius}%
                    }{\centerpoint}{\rotate}%
            \fi%
        \fi%
    }%
}%


==> pgflibraryshapes.misc.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryshapes.misc.code.tex}


\pgfdeclareshape{cross out}
{%
  \inheritsavedanchors[from=rectangle]% % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]%
  \inheritanchor[from=rectangle]{north}%
  \inheritanchor[from=rectangle]{north west}%
  \inheritanchor[from=rectangle]{north east}%
  \inheritanchor[from=rectangle]{center}%
  \inheritanchor[from=rectangle]{west}%
  \inheritanchor[from=rectangle]{east}%
  \inheritanchor[from=rectangle]{mid}%
  \inheritanchor[from=rectangle]{mid west}%
  \inheritanchor[from=rectangle]{mid east}%
  \inheritanchor[from=rectangle]{base}%
  \inheritanchor[from=rectangle]{base west}%
  \inheritanchor[from=rectangle]{base east}%
  \inheritanchor[from=rectangle]{south}%
  \inheritanchor[from=rectangle]{south west}%
  \inheritanchor[from=rectangle]{south east}%
  \foregroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }%
}%


\pgfdeclareshape{strike out}
{%
  \inheritsavedanchors[from=rectangle]% % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]%
  \inheritanchor[from=rectangle]{north}%
  \inheritanchor[from=rectangle]{north west}%
  \inheritanchor[from=rectangle]{north east}%
  \inheritanchor[from=rectangle]{center}%
  \inheritanchor[from=rectangle]{west}%
  \inheritanchor[from=rectangle]{east}%
  \inheritanchor[from=rectangle]{mid}%
  \inheritanchor[from=rectangle]{mid west}%
  \inheritanchor[from=rectangle]{mid east}%
  \inheritanchor[from=rectangle]{base}%
  \inheritanchor[from=rectangle]{base west}%
  \inheritanchor[from=rectangle]{base east}%
  \inheritanchor[from=rectangle]{south}%
  \inheritanchor[from=rectangle]{south west}%
  \inheritanchor[from=rectangle]{south east}%
  \foregroundpath{
    \pgfpathmoveto{\southwest}
    \pgfpathlineto{\northeast}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }%
}%


% Rounded rectangle


\pgfkeys{/pgf/.cd,
    rounded rectangle west arc/.initial=convex,
    rounded rectangle east arc/.initial=convex,
    rounded rectangle left arc/.style={/pgf/rounded rectangle west arc=#1},%
    rounded rectangle right arc/.style={/pgf/rounded rectangle east arc=#1},%
    rounded rectangle arc length/.initial=180%
}%

\def\pgf@lib@sh@misc@rr@text@concave{concave}%
\def\pgf@lib@sh@misc@rr@text@convex{convex}%

\pgfdeclareshape{rounded rectangle}{%
    \savedmacro\westarc{%
        \edef\westarc{\pgfkeysvalueof{/pgf/rounded rectangle west arc}}%
    }%
    \savedmacro\eastarc{%
        \edef\eastarc{\pgfkeysvalueof{/pgf/rounded rectangle east arc}}%
    }%
    \savedmacro\roundedrectanglepoints{%
        %
        % Get half the arc angle, a.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/rounded rectangle arc length}}%
        \pgf@x=.5\pgf@x%
        \edef\halfarcangle{\pgfmath@tonumber{\pgf@x}}%
        \addtosavedmacro\halfarcangle%
        %
        % Get the (half) node dimensions x & y.
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \edef\innerxsep{\the\pgf@x}%
        \pgf@xa=0.5\wd\pgfnodeparttextbox%
        \edef\halftextwidth{\the\pgf@xa}%
        \addtosavedmacro\halftextwidth%
        \advance\pgf@x by\pgf@xa%
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \edef\innerysep{\the\pgf@y}%
        \pgf@ya=.5\ht\pgfnodeparttextbox%
        \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
        \edef\halftextheight{\the\pgf@ya}%
        \addtosavedmacro\halftextheight%
        \advance\pgf@y by\pgf@ya%
        %
        % Adjust for minimum height
        %
        \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@y<.5\pgf@yb%
          \pgf@y=.5\pgf@yb%
        \fi%
        \edef\halfheight{\the\pgf@y}%
        \addtosavedmacro\halfheight%
        %
        % Calculate the radius of the arc ends.
        %
        \pgfmathcosec@{\halfarcangle}%
        \pgf@ya=\pgfmathresult\pgf@y%
        \edef\radius{\the\pgf@ya}%
        \addtosavedmacro\radius%
        %
        % Arc width = r - r*cos(a/2).
        %
        \pgfmathcos@{\halfarcangle}%
        \pgf@xa=\pgf@ya%
        \advance\pgf@xa by-\pgfmathresult\pgf@ya%
        %
        % When the node contents are pushed inside a convex arc,
        % the resulting chord has a height r - r*cos(asin(0.5*h/r)).
        %
        \pgfmathdivide{\halftextheight}{\radius}%
        \pgfmathasin@{\pgfmathresult}%
        \pgfmathcos@{\pgfmathresult}%
        \pgf@xb=\pgf@ya%
        \advance\pgf@xb by-\pgfmathresult\pgf@ya%
        %
        % Adjust for minimum width.
        %
        \edef\westarc{\pgfkeysvalueof{/pgf/rounded rectangle west arc}}%
        \edef\eastarc{\pgfkeysvalueof{/pgf/rounded rectangle east arc}}%
        %
        \pgfutil@tempdima=2.0\pgf@x% x still holds the half width.
        \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
            \advance\pgfutil@tempdima by\pgf@xa%
        \else%
            \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
                \advance\pgfutil@tempdima by\pgf@xb%
            \fi%
        \fi%
        %
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
            \advance\pgfutil@tempdima by\pgf@xa%
        \else%
            \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
                \advance\pgfutil@tempdima by\pgf@xb%
            \fi%
        \fi%
        %
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgfutil@tempdima<\pgfutil@tempdimb%
            \advance\pgfutil@tempdimb by-\pgfutil@tempdima%
            \divide\pgfutil@tempdimb by2\relax%
            \edef\xoffset{\the\pgfutil@tempdimb}%
        \else%
            \let\xoffset=\innerxsep%
        \fi%
        %
        % The node is made wider if convex arcs overlap.
        %
        \pgf@x=\halftextwidth\relax%
        \advance\pgf@x by\xoffset\relax%
        \pgf@xc=\pgf@ya%
        \advance\pgf@xc by-\pgf@xb%
        \ifdim\pgf@xc>\pgf@x\relax%
            \advance\pgf@xc by-\pgf@x%
            \advance\pgf@xc by\xoffset\relax%
            \edef\xoffset{\the\pgf@xc}%
        \fi%
        \addtosavedmacro\xoffset%
        %
        \pgf@x=\halftextwidth\relax%
        \advance\pgf@x by\xoffset\relax%
        \edef\halfwidth{\the\pgf@x}%
        \addtosavedmacro\halfwidth%
        %
        \edef\arcwidth{\the\pgf@xa}%
        \addtosavedmacro\arcwidth%
        %
        \edef\chordwidth{\the\pgf@xb}%
        \addtosavedmacro\chordwidth%
        %
        \pgfmathsetlengthmacro\outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathsetlengthmacro\outerysep{\pgfkeysvalueof{/pgf/outer ysep}}%
        \addtosavedmacro\outerxsep%
        \addtosavedmacro\outerysep%
        %
        % calculate some horizontal adjustments made for the default miter
        % drawn when an arc meets the north or south side of the node path.
        %
        \ifdim\halfarcangle pt=90pt\relax% Avoid division by zero.
            \def\concavexshift{0pt}%
        \else%
            % For a concave arc: outer xsep * cosec((90-a/2)/2)*cos((90-a/2)/2).
            \pgfmathsubtract@{90}{\halfarcangle}%
            \pgfmathdivide@{\pgfmathresult}{2}%
            \let\angletemp=\pgfmathresult%
            \pgf@x=\outerxsep\relax%
            \pgfmathcosec@{\angletemp}%
            \pgf@x=\pgfmathresult\pgf@x%
            \pgfmathcos@{\angletemp}%
            \pgf@x=\pgfmathresult\pgf@x%
            \edef\concavexshift{\the\pgf@x}%
        \fi%
        \addtosavedmacro\concavexshift%
        %
        \ifdim\halfarcangle pt=90pt\relax% Avoid division by zero.
            \def\convexxshift{0pt}%
        \else%
            % For a convex arc: outer xsep * cosec((90+a/2)/2)*cos((90+a/2)/2).
            \pgfmathadd@{90}{\halfarcangle}%
            \pgfmathdivide@{\pgfmathresult}{2}%
            \let\angletemp=\pgfmathresult%
            \pgf@x=\outerxsep\relax%
            \pgfmathcosec@{\angletemp}%
            \pgf@x=\pgfmathresult\pgf@x%
            \pgfmathcos@{\angletemp}%
            \pgf@x=\pgfmathresult\pgf@x%
            \edef\convexxshift{\the\pgf@x}%
        \fi%
        \addtosavedmacro\convexxshift%
    }%
    \saveddimen\halflinewidth{\pgf@x.5\pgflinewidth}%
    \savedanchor\centerpoint{%
        \pgf@x=.5\wd\pgfnodeparttextbox%
        \pgf@y=.5\ht\pgfnodeparttextbox%
        \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x=.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+0.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x=.5\wd\pgfnodeparttextbox%
        \pgf@y=0pt\relax%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid west}{%
        \csname pgf@anchor@rounded rectangle@west\endcsname%
        \pgf@xc=\pgf@x%
        \midpoint%
        \pgf@x=\pgf@xc%
    }%
    \anchor{mid east}{%
        \csname pgf@anchor@rounded rectangle@east\endcsname%
        \pgf@xc=\pgf@x%
        \midpoint%
        \pgf@x=\pgf@xc%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base west}{%
        \csname pgf@anchor@rounded rectangle@west\endcsname%
        \pgf@xc=\pgf@x%
        \basepoint%
        \pgf@x=\pgf@xc%
    }%
    \anchor{base east}{%
        \csname pgf@anchor@rounded rectangle@east\endcsname%
        \pgf@xc=\pgf@x%
        \basepoint%
        \pgf@x=\pgf@xc%
    }%
    \anchor{north}{%
        \roundedrectanglepoints%
        \pgfpointadd{\centerpoint}{\pgfpoint{+0pt}{\halfheight+\outerysep}}%
    }%
    \anchor{south}{%
        \roundedrectanglepoints%
        \pgfpointadd{\centerpoint}{\pgfpoint{+0pt}{-\halfheight-\outerysep}}%
    }%
    \anchor{west}{%
        \roundedrectanglepoints%
        \pgfpointadd{\centerpoint}{%
            \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
                \pgfpoint{-\halfwidth-\arcwidth-\concavexshift}{+0pt}%
            \else%
                \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfpoint{-\halfwidth-\chordwidth-\outerxsep}{+0pt}%
                \else%
                    \pgfpoint{-\halfwidth-\outerxsep}{+0pt}%
                \fi%
            \fi%
        }%
    }%
    \anchor{north west}{%
        \roundedrectanglepoints%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth-\convexxshift}{+0pt}}%
        \else%
            \csname pgf@anchor@rounded rectangle@west\endcsname%
        \fi%
        \pgf@xc=\pgf@x%
        \csname pgf@anchor@rounded rectangle@north\endcsname%
        \pgf@x=\pgf@xc%
    }%
    \anchor{south west}{%
        \roundedrectanglepoints%
        \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
            \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth-\convexxshift}{+0pt}}%
        \else%
            \csname pgf@anchor@rounded rectangle@west\endcsname%
        \fi%
        \pgf@xc=\pgf@x%
        \csname pgf@anchor@rounded rectangle@south\endcsname%
        \pgf@x=\pgf@xc%
    }%
    \anchor{east}{%
        \roundedrectanglepoints%
        \pgfpointadd{\centerpoint}{%
            \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
                \pgfpoint{\halfwidth+\arcwidth+\concavexshift}{+0pt}%
            \else%
                \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfpoint{\halfwidth+\chordwidth+\outerxsep}{+0pt}%
                \else%
                    \pgfpoint{\halfwidth+\outerxsep}{+0pt}%
                \fi%
            \fi%
        }%
    }%
    \anchor{north east}{%
        \roundedrectanglepoints%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\arcwidth+\convexxshift}{+0pt}}%
        \else%
            \csname pgf@anchor@rounded rectangle@east\endcsname%
        \fi%
        \pgf@xc=\pgf@x%
        \csname pgf@anchor@rounded rectangle@north\endcsname%
        \pgf@x=\pgf@xc%
    }%
    \anchor{south east}{%
        \roundedrectanglepoints%
        \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\arcwidth+\convexxshift}{+0pt}}%
        \else%
            \csname pgf@anchor@rounded rectangle@east\endcsname%
        \fi%
        \pgf@xc=\pgf@x%
        \csname pgf@anchor@rounded rectangle@south\endcsname%
        \pgf@x=\pgf@xc%
    }%
    \backgroundpath{%
        {%
            \roundedrectanglepoints%
            \pgftransformshift{\centerpoint}%
            \pgfpathmoveto{\pgfpoint{0pt}{\halfheight}}%
            \ifx\eastarc\pgf@lib@sh@misc@rr@text@concave%
                \pgfpathlineto{\pgfpoint{\halfwidth+\arcwidth}{+\halfheight}}%
                \pgfpatharc{180-\halfarcangle}{180+\halfarcangle}{+\radius}%
            \else%
                \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfpathlineto{\pgfpoint{\halfwidth+\chordwidth-\arcwidth}{+\halfheight}}%
                    \pgfpatharc{+\halfarcangle}{+-\halfarcangle}{+\radius}%
                \else%
                    \pgfpathlineto{\pgfqpoint{\halfwidth}{\halfheight}}%
                    \pgfpathlineto{\pgfqpoint{\halfwidth}{-\halfheight}}%
                \fi%
            \fi%
            \ifx\westarc\pgf@lib@sh@misc@rr@text@concave%
                \pgfpathlineto{\pgfpoint{-\halfwidth-\arcwidth}{+-\halfheight}}%
                \pgfpatharc{+-\halfarcangle}{+\halfarcangle}{+\radius}%
            \else%
                \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfpathlineto{\pgfpoint{-\halfwidth-\chordwidth+\arcwidth}{+-\halfheight}}%
                    \pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{+\radius}%
                \else%
                    \pgfpathlineto{\pgfqpoint{-\halfwidth}{-\halfheight}}%
                    \pgfpathlineto{\pgfqpoint{-\halfwidth}{\halfheight}}%
                \fi%
            \fi%
            \pgfpathclose%
        }%
    }%
    \anchorborder{%
    \pgfextract@process\externalpoint{%
        \pgfextract@process\externalpoint{}%
            \pgfpointadd{\centerpoint}{\externalpoint}%
        }%
        \roundedrectanglepoints%
        %
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \let\externalangle=\pgfmathresult%
        \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
            \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                % Between north east and east.
                \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfextract@process\arccenter{%
                        \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
                    }%
                    \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
                        {\arccenter}{0}{\halfarcangle}{\radius+\outerxsep and \radius+\outerysep}%
                \else%
                    \pgfpointintersectionoflines%
                        {\csname pgf@anchor@rounded rectangle@north east\endcsname}%
                        {\csname pgf@anchor@rounded rectangle@south east\endcsname}%
                        {\externalpoint}{\centerpoint}%
                \fi%
            \else%
                % Between north west and north east.
                \pgfpointintersectionoflines%
                    {\csname pgf@anchor@rounded rectangle@north east\endcsname}%
                    {\csname pgf@anchor@rounded rectangle@north west\endcsname}%
                    {\externalpoint}{\centerpoint}%
            \fi%
        \else%
            \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax%
                % Between south west and north west.
                \ifx\westarc\pgf@lib@sh@misc@rr@text@convex%
                    \pgfextract@process\arccenter{%
                        \pgfpointadd{\centerpoint}{\pgfpoint{-\halfwidth-\chordwidth+\radius}{+0pt}}%
                    }%
                    \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
                        {\arccenter}{180-\halfarcangle}{180+\halfarcangle}{\radius+\outerxsep and \radius+\outerysep}%
                \else%
                    \pgfpointintersectionoflines%
                        {\csname pgf@anchor@rounded rectangle@north west\endcsname}%
                        {\csname pgf@anchor@rounded rectangle@south west\endcsname}%
                        {\externalpoint}{\centerpoint}%
                \fi%
            \else%
                \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax%
                    % Between south east and south west.
                    \pgfpointintersectionoflines%
                        {\csname pgf@anchor@rounded rectangle@south east\endcsname}%
                        {\csname pgf@anchor@rounded rectangle@south west\endcsname}%
                        {\externalpoint}{\centerpoint}%
                \else%
                    % Between east and south east.
                    \ifx\eastarc\pgf@lib@sh@misc@rr@text@convex%
                        \pgfextract@process\arccenter{%
                            \pgfpointadd{\centerpoint}{\pgfpoint{\halfwidth+\chordwidth-\radius}{+0pt}}%
                        }%
                        \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
                            {\arccenter}{360-\halfarcangle}{360}{\radius+\outerxsep and \radius+\outerysep}%
                    \else%
                        \pgfpointintersectionoflines%
                            {\csname pgf@anchor@rounded rectangle@north east\endcsname}%
                            {\csname pgf@anchor@rounded rectangle@south east\endcsname}%
                            {\externalpoint}{\centerpoint}%
                    \fi%
                \fi%
            \fi%
        \fi%
    }%
}%



% Keys for chamfered rectangle
%
% /pgf/chamfered rectangle corners : specify the corners to chamfer.
% /pgf/chamfered rectangle angle   : set the angle of the chamfer.
% /pgf/chamfered rectangle xsep    : set the extent of the x chamferling.
% /pgf/chamfered rectangle ysep    : set the extent of the y chamferling.

\pgfkeys{/pgf/chamfered rectangle corners/.store in=\pgf@lib@sh@misc@cr@corners}%
\pgfkeys{/tikz/chamfered rectangle corners/.store in=\pgf@lib@sh@misc@cr@corners}%

\def\pgf@lib@sh@misc@cr@chamferall{chamfer all}%
\def\pgf@lib@sh@misc@cr@chamfer{chamfer}%
\let\pgf@lib@sh@misc@cr@corners\pgf@lib@sh@misc@cr@chamferall


\def\pgf@lib@sh@misc@cr@getcorners{%
    \let\northeastcorner\pgfutil@empty%
    \let\southeastcorner\pgfutil@empty%
    \let\southwestcorner\pgfutil@empty%
    \let\northwestcorner\pgfutil@empty%
    \expandafter\pgfutil@in@\expandafter{\pgf@lib@sh@misc@cr@corners}{chamfer all}%
    \ifpgfutil@in@%
        \let\northeastcorner\pgf@lib@sh@misc@cr@round%
        \let\southeastcorner\pgf@lib@sh@misc@cr@round%
        \let\southwestcorner\pgf@lib@sh@misc@cr@round%
        \let\northwestcorner\pgf@lib@sh@misc@cr@round%
        \let\pgf@next\relax%
    \else%
        \let\pgf@next\pgf@lib@sh@misc@cr@parsecorners%
    \fi%
    \pgf@next}%

\def\pgf@lib@sh@misc@cr@parsecorners{%
    \expandafter\pgf@@chamferedrectangle@parsecorners\pgf@lib@sh@misc@cr@corners,\pgf@stop,%
}%

\def\pgf@@chamferedrectangle@parsecorners#1,{%
    \ifx#1\pgf@stop%
        \let\pgf@next\relax%
    \else%
        \pgfutil@in@{@#1@}{@north east@@top left@}%
        \ifpgfutil@in@%
            \let\northeastcorner\pgf@lib@sh@misc@cr@chamfer%
        \else%
            \pgfutil@in@{@#1@}{@south east@@bottom right@}%
            \ifpgfutil@in@%
                \let\southeastcorner\pgf@lib@sh@misc@cr@chamfer%
            \else%
                \pgfutil@in@{@#1@}{@south west@@bottom left@}%
                \ifpgfutil@in@%
                    \let\southwestcorner\pgf@lib@sh@misc@cr@chamfer%
                \else%
                    \pgfutil@in@{@#1@}{@north west@@top right@}%
                    \ifpgfutil@in@%
                        \let\northwestcorner\pgf@lib@sh@misc@cr@round%
                    \fi%
                \fi%
            \fi%
        \fi%
        \let\pgf@next\pgf@@@chamferedrectangle@parsecorners%
    \fi%
    \pgf@next%
}%
\def\pgf@@@chamferedrectangle@parsecorners{%
    \pgfutil@ifnextchar x{\pgf@@chamferedrectangle@parsecorners}{\pgf@@chamferedrectangle@parsecorners}%
}%

\pgfkeys{/pgf/.cd,
    chamfered rectangle angle/.initial=45,%
    chamfered rectangle xsep/.initial=.666ex,%
    chamfered rectangle ysep/.initial=.666ex%
}%
 \pgfkeys{/pgf/chamfered rectangle sep/.style={%
    /pgf/chamfered rectangle xsep=#1,/pgf/chamfered rectangle ysep=#1}%
}%




% Shape chamfered rectangle.
%
%
\pgfdeclareshape{chamfered rectangle}{%
    \savedmacro\getchamferedrectanglepoints{%
        \pgf@lib@sh@misc@cr@getcorners%
        %
        % Get the node dimensions.
        %
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
        \advance\pgf@xa.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@ya.5\ht\pgfnodeparttextbox%
        \advance\pgf@ya.5\dp\pgfnodeparttextbox%
        %
        % Get chamfer stuff.
        %
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/chamfered rectangle angle}}%
        \ifdim\pgfutil@tempdima<89pt\relax%
            \ifdim\pgfutil@tempdima<1pt\relax%
                \pgfutil@tempdima1pt\relax%
            \fi%
        \else%
            \pgfutil@tempdima89pt\relax%
        \fi%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima90pt\relax%
        \pgfmathtan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \let\tanangle\pgfmathresult%
        \pgfmathcot@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \let\cotangle\pgfmathresult%
        \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/chamfered rectangle xsep}}%
        \pgf@yc\tanangle\pgf@xb%
        \ifdim\pgf@yc>\pgf@ya%
            \pgf@yc\pgf@ya%
            \pgf@xb\cotangle\pgf@yc%
        \fi%
        \pgfmathcot@{\pgfmath@tonumber{\pgfutil@tempdima}}%
        \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/chamfered rectangle ysep}}%
        \pgf@xc\cotangle\pgf@yb%
            \ifdim\pgf@xc>\pgf@xa%
            \pgf@xc\pgf@xa%
            \pgf@yb\tanangle\pgf@xc%
        \fi%
        %
        % Check for minimum width and height%
        %
        \pgfutil@tempdima\pgf@xa%
        \advance\pgfutil@tempdima\pgf@xb%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
        \ifdim\pgfutil@tempdima<.5\pgfutil@tempdimb%
            \pgf@xa.5\pgfutil@tempdimb%
            \advance\pgf@xa-\pgf@xb%
        \fi%
        \pgfutil@tempdima\pgf@ya%
        \advance\pgfutil@tempdima\pgf@yb%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgfutil@tempdima<.5\pgfutil@tempdimb%
            \pgf@ya.5\pgfutil@tempdimb%
            \advance\pgf@ya-\pgf@yb%
        \fi%
        %
        % Define the background path points.
        %
        \pgfextract@process\centerpoint{%
            \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
            \pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
            \pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
        }%
        \pgfextract@process\beforenortheast{%
            \centerpoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@x\pgf@xb%
            \advance\pgf@y\pgf@ya%
            \advance\pgf@y-\pgf@yc%
        }%
        \pgfextract@process\northeast{%
            \centerpoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
            \ifx\northeastcorner\pgfutil@empty%
                \advance\pgf@x\pgf@xb%
                \advance\pgf@y\pgf@yb%
            \fi%
        }%
        \pgfextract@process\afternortheast{%
            \centerpoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@x-\pgf@xc%
            \advance\pgf@y\pgf@ya%
            \advance\pgf@y\pgf@yb%
        }%
        \pgfextract@process\northwest{%
            \centerpoint%
            \advance\pgf@x-\pgf@xa%
            \advance\pgf@y\pgf@ya%
            \ifx\northwestcorner\pgfutil@empty%
                \advance\pgf@x-\pgf@xb%
                \advance\pgf@y\pgf@yb%
            \fi%
        }%
        \pgfextract@process\beforesouthwest{%
            \centerpoint%
            \advance\pgf@x-\pgf@xa%
            \advance\pgf@x-\pgf@xb%
            \advance\pgf@y-\pgf@ya%
            \advance\pgf@y\pgf@yc%
        }%
        \pgfextract@process\southwest{%
            \centerpoint%
            \advance\pgf@x-\pgf@xa%
            \advance\pgf@y-\pgf@ya%
            \ifx\southwestcorner\pgfutil@empty%
                \advance\pgf@x-\pgf@xb%
                \advance\pgf@y-\pgf@yb%
            \fi%
        }%
        \pgfextract@process\aftersouthwest{%
            \centerpoint%
            \advance\pgf@x-\pgf@xa%
            \advance\pgf@x\pgf@xc%
            \advance\pgf@y-\pgf@ya%
            \advance\pgf@y-\pgf@yb%
        }%
        \pgfextract@process\southeast{%
            \centerpoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y-\pgf@ya%
            \ifx\southeastcorner\pgfutil@empty%
                \advance\pgf@x\pgf@xb%
                \advance\pgf@y-\pgf@yb%
            \fi%
        }%
        %
        % Calculate the `miter' vectors.
        %
        \pgfmathanglebetweenlines{\beforenortheast}{\afternortheast}{\beforenortheast}%
            {\beforesouthwest\pgf@ya\pgf@y\beforenortheast\pgf@y\pgf@ya}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \ifdim\pgfutil@tempdima>180pt\relax%
            \advance\pgfutil@tempdima-180pt\relax%
        \fi%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/outer xsep}}%
        \ifdim\pgfutil@tempdima<90pt\relax%
            \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
            \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
            \pgfutil@tempdima0pt\relax%
        \else%
            \pgfutil@tempdima.5\pgfutil@tempdima%
            \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
            \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
            \pgfutil@tempdima-\pgfutil@tempdima%
            \advance\pgfutil@tempdima90pt\relax%
        \fi%
        \pgfextract@process\before@ne@anchor{%
            \beforenortheast%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfextract@process\before@sw@anchor{%
            \beforesouthwest%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \pgfqpointpolar{-\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        %
        \pgfmathanglebetweenlines{\afternortheast}{\aftersouthwest\pgf@xa\pgf@x\afternortheast\pgf@x\pgf@xa}%
            {\afternortheast}{\beforenortheast}%
        \pgfutil@tempdima\pgfmathresult pt\relax%
        \ifdim\pgfutil@tempdima>270pt\relax%
            \advance\pgfutil@tempdima-270pt\relax%
        \fi%
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/outer ysep}}%
        \ifdim\pgfutil@tempdima<90pt\relax%
            \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
            \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
            \pgfutil@tempdima90pt\relax%
        \else%
            \pgfutil@tempdima.5\pgfutil@tempdima%
            \pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
            \pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
        \fi%
        %
        \pgfextract@process\after@ne@anchor{%
            \afternortheast%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfutil@tempdima-\pgfutil@tempdima%
        \advance\pgfutil@tempdima180pt\relax%
        \pgfextract@process\after@sw@anchor{%
            \aftersouthwest
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \pgfqpointpolar{-\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \addtosavedmacro\before@ne@anchor%
        \addtosavedmacro\after@ne@anchor%
        \addtosavedmacro\before@sw@anchor%
        \addtosavedmacro\after@sw@anchor%
        \pgfextract@process\ne@anchor{%
            \ifx\northeastcorner\pgfutil@empty%
                \northeast%
                \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
                \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
            \else%
                \pgfpointlineattime{0.5}{\before@ne@anchor}{\after@ne@anchor}%
            \fi%
        }%
        \pgfextract@process\nw@anchor{%
            \ifx\northwestcorner\pgfutil@empty%
                \northwest%
                \pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
                \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
            \else%
                \pgfpointlineattime{0.5}{%
                    \before@ne@anchor%
                    \pgf@ya\pgf@y
                    \before@sw@anchor%
                    \pgf@y\pgf@ya%
                }{%
                    \after@ne@anchor%
                    \pgf@ya\pgf@y
                    \after@sw@anchor%
                    \pgf@y\pgf@ya%
                }%
            \fi%
        }%
        \pgfextract@process\sw@anchor{%
            \ifx\southwestcorner\pgfutil@empty%
                \southwest%
                \pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
                \pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
            \else%
                \pgfpointlineattime{0.5}{\before@sw@anchor}{\after@sw@anchor}%
            \fi%
        }%
        \pgfextract@process\se@anchor{%
            \ifx\southeastcorner\pgfutil@empty%
                \southeast%
                \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
                \pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
            \else%
                \pgfpointlineattime{0.5}{%
                    \before@ne@anchor%
                    \pgf@xa\pgf@x
                    \before@sw@anchor%
                    \pgf@x\pgf@xa%
                }{%
                    \after@ne@anchor%
                    \pgf@xa\pgf@x
                    \after@sw@anchor%
                    \pgf@x\pgf@xa%
                }%
            \fi%
        }%
        \addtosavedmacro\ne@anchor%
        \addtosavedmacro\nw@anchor%
        \addtosavedmacro\sw@anchor%
        \addtosavedmacro\se@anchor%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y.5\ht\pgfnodeparttextbox%
        \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+.5ex}%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \getchamferedrectanglepoints%
        \midpoint%
        \pgf@ya\pgf@y%
        \pgf@process{%
            \before@sw@anchor%
            \pgf@ya\pgf@y%
            \before@ne@anchor%
            \pgf@y\pgf@ya%
        }%
        \ifdim\pgf@ya<\pgf@y%
            \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                {\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                {\after@sw@anchor\pgf@ya\pgf@y\after@ne@anchor\pgf@y\pgf@ya}%
        \else%
            \pgf@process{\before@ne@anchor}%
            \ifdim\pgf@ya<\pgf@y%
                \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor}%
            \else%
                \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor}%
                    {\after@ne@anchor}%
            \fi%
        \fi%
    }%
    \anchor{mid west}{%
        \getchamferedrectanglepoints%
        \midpoint%
        \pgf@ya\pgf@y%
        \pgf@process{\before@sw@anchor}%
        \ifdim\pgf@ya<\pgf@y%
            \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                {\before@sw@anchor}{\after@sw@anchor}%
        \else%
            \pgf@process{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
            \ifdim\pgf@ya<\pgf@y%
                \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@sw@anchor}%
            \else%
                \pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\after@ne@anchor\pgf@ya\pgf@y\after@sw@anchor\pgf@y\pgf@ya}%
            \fi%
        \fi%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \getchamferedrectanglepoints%
        \basepoint%
        \pgf@ya\pgf@y%
        \pgf@process{%
            \before@sw@anchor%
            \pgf@ya\pgf@y%
            \before@ne@anchor%
            \pgf@y\pgf@ya%
        }%
        \ifdim\pgf@ya<\pgf@y%
            \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                {\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                {\after@sw@anchor\pgf@ya\pgf@y\after@ne@anchor\pgf@y\pgf@ya}%
        \else%
            \pgf@process{\before@ne@anchor}%
            \ifdim\pgf@ya<\pgf@y%
                \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor}%
            \else%
                \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor}%
                    {\after@ne@anchor}%
            \fi%
        \fi%
    }%
    \anchor{base west}{%
        \getchamferedrectanglepoints%
        \basepoint%
        \pgf@ya\pgf@y%
        \pgf@process{\before@sw@anchor}%
        \ifdim\pgf@ya<\pgf@y%
            \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                {\before@sw@anchor}{\after@sw@anchor}%
        \else%
            \pgf@process{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
            \ifdim\pgf@ya<\pgf@y%
                \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@sw@anchor}%
            \else%
                \pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
                    {\after@ne@anchor\pgf@ya\pgf@y\after@sw@anchor\pgf@y\pgf@ya}%
            \fi%
        \fi%
    }%
    \anchor{before north east}{\getchamferedrectanglepoints\before@ne@anchor}%
    \anchor{north east}{\getchamferedrectanglepoints\ne@anchor}%
    \anchor{after north east}{\getchamferedrectanglepoints\after@ne@anchor}%
    \anchor{north}{%
        \getchamferedrectanglepoints%
        \centerpoint%
        \pgf@xa\pgf@x%
        \after@ne@anchor%
        \pgf@x\pgf@xa}%
    \anchor{before north west}{%
        \getchamferedrectanglepoints%
        \after@sw@anchor%
        \pgf@xa\pgf@x%
        \after@ne@anchor%
        \pgf@x\pgf@xa}%
    \anchor{north west}{\getchamferedrectanglepoints\nw@anchor}%
    \anchor{after north west}{%
        \getchamferedrectanglepoints%
        \before@sw@anchor%
        \pgf@xa\pgf@x%
        \before@ne@anchor%
        \pgf@x\pgf@xa}%
    \anchor{west}{%
        \getchamferedrectanglepoints%
        \centerpoint%
        \pgf@ya\pgf@y%
        \before@sw@anchor%
        \pgf@y\pgf@ya}%
    \anchor{before south west}{\getchamferedrectanglepoints\before@sw@anchor}%
    \anchor{south west}{\getchamferedrectanglepoints\sw@anchor}%
    \anchor{after south west}{\getchamferedrectanglepoints\after@sw@anchor}%
        \anchor{south}{%
        \getchamferedrectanglepoints%
        \centerpoint%
        \pgf@xa\pgf@x%
        \after@sw@anchor%
        \pgf@x\pgf@xa}%
    \anchor{before south east}{%
        \getchamferedrectanglepoints%
        \after@sw@anchor%
        \pgf@ya\pgf@y%
        \after@ne@anchor%
        \pgf@y\pgf@ya}%
    \anchor{south east}{\getchamferedrectanglepoints\se@anchor}%
    \anchor{after south east}{%
        \getchamferedrectanglepoints%
        \before@sw@anchor%
        \pgf@ya\pgf@y%
        \before@ne@anchor%
        \pgf@y\pgf@ya}%
    \anchor{east}{%
        \getchamferedrectanglepoints%
        \centerpoint%
        \pgf@ya\pgf@y%
        \before@ne@anchor%
        \pgf@y\pgf@ya}%
    \backgroundpath{%
        \pgfpathmoveto{\beforenortheast}%
        \pgfpathlineto{\northeast}%
        \pgfpathlineto{\afternortheast}%
        \pgfpathlineto{\aftersouthwest\pgf@xa\pgf@x\afternortheast\pgf@x\pgf@xa}%
        \pgfpathlineto{\northwest}%
        \pgfpathlineto{\beforesouthwest\pgf@xa\pgf@x\beforenortheast\pgf@x\pgf@xa}%
        \pgfpathlineto{\beforesouthwest}%
        \pgfpathlineto{\southwest}%
        \pgfpathlineto{\aftersouthwest}%
        \pgfpathlineto{\aftersouthwest\pgf@ya\pgf@y\afternortheast\pgf@y\pgf@ya}%
        \pgfpathlineto{\southeast}%
        \pgfpathlineto{\beforesouthwest\pgf@ya\pgf@y\beforenortheast\pgf@y\pgf@ya}%
        \pgfpathclose%
    }%
    \anchorborder{%
        \pgfextract@process\externalpoint{%
            \pgf@xa\pgf@x%
            \pgf@ya\pgf@y%
            \centerpoint%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
        }%
        \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
        \let\externalangle\pgfmathresult%
        \getchamferedrectanglepoints%
        \pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax% west.
            \pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax% north.
                \pgfmathanglebetweenpoints{\centerpoint}{\ne@anchor}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax% north east.
                    \pgfmathanglebetweenpoints{\centerpoint}{\before@ne@anchor}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% before north east.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\centerpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}{\before@ne@anchor}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\before@ne@anchor}{\ne@anchor}%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\centerpoint}{\after@ne@anchor}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% after north east.
                            \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\ne@anchor}{\after@ne@anchor}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\after@ne@anchor}{\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
                    \fi%
                \fi%
            \else%
                \pgfmathanglebetweenpoints{\centerpoint}{\nw@anchor}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax% north west.
                    \pgfmathanglebetweenpoints{\centerpoint}{\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% before north west.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
                            {\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
                            {\nw@anchor}%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\centerpoint}{\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% after north west.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\nw@anchor}{\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
                            {\before@sw@anchor\pgf@xa\pgf@x\centerpoint\pgf@x\pgf@xa}%
                    \fi%
                \fi%
            \fi%
        \else%
            \pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
            \ifdim\externalangle pt<\pgfmathresult pt\relax% south.
                \pgfmathanglebetweenpoints{\centerpoint}{\sw@anchor}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax% south west.
                    \pgfmathanglebetweenpoints{\centerpoint}{\before@sw@anchor}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% before south west.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\before@sw@anchor\pgf@xa\pgf@x\centerpoint\pgf@x\pgf@xa}%
                            {\before@sw@anchor}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\before@sw@anchor}{\sw@anchor}%
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\centerpoint}{\after@sw@anchor}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% after south west.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\sw@anchor}{\after@sw@anchor}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\after@sw@anchor}{\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
                    \fi%
                \fi%
            \else%
                \pgfmathanglebetweenpoints{\centerpoint}{\se@anchor}%
                \ifdim\externalangle pt<\pgfmathresult pt\relax% south east.
                    \pgfmathanglebetweenpoints{\centerpoint}{\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% before south east.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
                            {\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}{\se@anchor}
                    \fi%
                \else%
                    \pgfmathanglebetweenpoints{\centerpoint}{\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%
                    \ifdim\externalangle pt<\pgfmathresult pt\relax% after south east.
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\se@anchor}{\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%
                    \else%
                        \pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
                            {\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%
                            {\centerpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
                    \fi%
                \fi%
            \fi%
        \fi%
    }%
}%


\endinput


==> pgflibraryshapes.multipart.code.tex <==
% Copyright 2018 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryshapes.multipart.code.tex}

\newbox\pgfnodepartlowerbox

%
% A circle that is split in the middle into an upper and a lower part.
%
% This node consists of two parts: The upper (main) part is shown in
% the upper half of the circle. The second part is the (optional)
% lower part.
%
% Parts: text, lower

\pgfdeclareshape{circle split}
{%
  %
  % Node parts
  %
  \nodeparts{text,lower}%

  %
  % Anchors
  %
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgf@y=-\pgf@y%
    \advance\pgf@y by-\dp\pgfnodeparttextbox%
    \advance\pgf@y by-.5\pgflinewidth%
  }%
  \savedanchor\loweranchor{%
    \pgf@x=-.5\wd\pgfnodepartlowerbox%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgf@y=-2\pgf@y%
    \advance\pgf@y by-\ht\pgfnodepartlowerbox%
    \advance\pgf@y by-.5\pgflinewidth%
    \advance\pgf@y by-\dp\pgfnodeparttextbox%
    \advance\pgf@y by-.5\pgflinewidth%
  }%

  \saveddimen\radius{%
    %
    % Calculate ``height radius''
    %
    %\pgf@ya=.5\ht\pgfnodeparttextbox%
%    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
%    \advance\pgf@ya by.5\ht\pgfnodepartlowerbox%
%    \advance\pgf@ya by.5\dp\pgfnodepartlowerbox%
%    \advance\pgf@ya by.5\pgflinewidth%
        %
        % MW: Suggested correction for above calculation:    Use the tallest box * 2.
        %
        \pgf@ya=.5\ht\pgfnodeparttextbox%
        \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
        \pgf@yb=.5\ht\pgfnodepartlowerbox%
        \advance\pgf@yb by.5\dp\pgfnodepartlowerbox%
        \ifdim\pgf@ya>\pgf@yb\relax%
            \pgf@ya2.0\pgf@ya\relax%
        \else%
            \pgf@ya2.0\pgf@yb\relax%
        \fi%
        \advance\pgf@ya by.5\pgflinewidth%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by2\pgf@yb%
    %
    % Calculate ``width radius''
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \ifdim\pgf@xa<.5\wd\pgfnodepartlowerbox%
      \pgf@xa=.5\wd\pgfnodepartlowerbox%
    \fi%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    %
    % Calculate length of radius vector:
    %
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    %
    % If necessary, adjust radius so that the size requirements are
    % met:
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    %
    % Now, add larger of outer separations.
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }%

  %
  % Anchors
  %
  \inheritanchorborder[from=circle]%
  \inheritanchor[from=circle]{north}%
  \inheritanchor[from=circle]{north west}%
  \inheritanchor[from=circle]{north east}%
  \inheritanchor[from=circle]{center}%
  \inheritanchor[from=circle]{west}%
  \inheritanchor[from=circle]{east}%
  \inheritanchor[from=circle]{mid}%
  \inheritanchor[from=circle]{mid west}%
  \inheritanchor[from=circle]{mid east}%
  \inheritanchor[from=circle]{base}%
  \inheritanchor[from=circle]{base west}%
  \inheritanchor[from=circle]{base east}%
  \inheritanchor[from=circle]{south}%
  \inheritanchor[from=circle]{south west}%
  \inheritanchor[from=circle]{south east}%
  \anchor{lower}{\loweranchor}%

  %
  % Background path
  %
  \inheritbackgroundpath[from=circle]%
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \advance\pgfutil@tempdima by-.5\pgflinewidth%
    \pgfsetshortenstart{0pt}%
    \pgfsetshortenend{0pt}%
    \pgfsetarrows{-}%
    \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpoint{-1\pgfutil@tempdima}{0pt}}}%
    \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpoint{\pgfutil@tempdima}{0pt}}}%
    \pgfusepath{stroke}%
  }%
}%


%
% A circle that is split diagonally into an upper and a lower part.
%
% Parts: text, lower

\pgfdeclareshape{circle solidus}{%
  % Node parts
  \nodeparts{text,lower}%
  % Anchors
  % solidus slants at 45 degrees
  % text placement minimizes the required radius,
  % this is achieved placing the "outer" corner
  % of each box in the line orthogonal to the
  % solidus which passes through circle center
  \savedanchor\centerpoint{%
    \pgf@x=0.5\wd\pgfnodeparttextbox%
    \advance\pgf@x by0.5\dp\pgfnodeparttextbox%
    \advance\pgf@x by0.5\ht\pgfnodeparttextbox%
    \pgf@y=-\pgf@x%
    \advance\pgf@y by\ht\pgfnodeparttextbox%
    \advance\pgf@x by0.3536\pgflinewidth%
    \advance\pgf@y by-0.3536\pgflinewidth%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by-\pgf@ya%
  }%
  \savedanchor\loweranchor{%
    \pgf@x=0.5\wd\pgfnodeparttextbox%
    \advance\pgf@x by0.5\dp\pgfnodeparttextbox%
    \advance\pgf@x by0.5\ht\pgfnodeparttextbox%
    \pgf@y=-\pgf@x%
    \advance\pgf@y by\ht\pgfnodeparttextbox%
    \advance\pgf@x by0.5\ht\pgfnodepartlowerbox%
    \advance\pgf@x by0.5\dp\pgfnodepartlowerbox%
    \advance\pgf@x by-0.5\wd\pgfnodepartlowerbox%
    \advance\pgf@y by-0.5\ht\pgfnodepartlowerbox%
    \advance\pgf@y by0.5\dp\pgfnodepartlowerbox%
    \advance\pgf@y by-0.5\wd\pgfnodepartlowerbox%
    \advance\pgf@x by0.7071\pgflinewidth%
    \advance\pgf@y by-0.7071\pgflinewidth%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by2\pgf@xa%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by-2\pgf@ya%
  }%
  \saveddimen\radius{%
    % "top" radius
    \pgf@x=\ht\pgfnodeparttextbox%
    \advance\pgf@x by\dp\pgfnodeparttextbox%
    \advance\pgf@x by\wd\pgfnodeparttextbox%
    % "bottom" radius
    \pgf@y=\ht\pgfnodepartlowerbox%
    \advance\pgf@y by\dp\pgfnodepartlowerbox%
    \advance\pgf@y by\wd\pgfnodepartlowerbox%
    % use the larger
    \ifdim\pgf@x<\pgf@y%
      \pgf@x=\pgf@y%
    \fi%
    \pgf@x=0.7071\pgf@x%
    % add spacings
    \advance\pgf@x by0.5\pgflinewidth%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/inner xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgfmathaddtolength{\pgf@x}{veclen(2\pgf@xa,2\pgf@ya)}%
    % If necessary, adjust radius so that the size requirements are
    % met:
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xa%
      \pgf@x=.5\pgf@xa%
    \fi%
    \ifdim\pgf@x<.5\pgf@ya%
      \pgf@x=.5\pgf@ya%
    \fi%
    % Now, add larger of outer separations.
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xa<\pgf@ya%
      \advance\pgf@x by\pgf@ya%
    \else%
      \advance\pgf@x by\pgf@xa%
    \fi%
  }%
  % Anchors
  \inheritanchorborder[from=circle]%
  \inheritanchor[from=circle]{north}%
  \inheritanchor[from=circle]{north west}%
  \inheritanchor[from=circle]{north east}%
  \inheritanchor[from=circle]{center}%
  \inheritanchor[from=circle]{west}%
  \inheritanchor[from=circle]{east}%
  \inheritanchor[from=circle]{mid}%
  \inheritanchor[from=circle]{mid west}%
  \inheritanchor[from=circle]{mid east}%
  \inheritanchor[from=circle]{base}%
  \inheritanchor[from=circle]{base west}%
  \inheritanchor[from=circle]{base east}%
  \inheritanchor[from=circle]{south}%
  \inheritanchor[from=circle]{south west}%
  \inheritanchor[from=circle]{south east}%
  \anchor{lower}{\loweranchor}%
  % Background path
  \inheritbackgroundpath[from=circle]%
  \beforebackgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xa<\pgf@ya%
      \advance\pgfutil@tempdima by-\pgf@ya%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xa%
    \fi%
    \advance\pgfutil@tempdima by-.5\pgflinewidth%
    \pgfsetshortenstart{0pt}%
    \pgfsetshortenend{0pt}%
    \pgfsetarrows{-}%
    % solidus slants at 45 degrees and its length is
    % the golden section of the diameter
    \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpoint{-0.437\pgfutil@tempdima}{-0.437\pgfutil@tempdima}}}%
    \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpoint{0.437\pgfutil@tempdima}{0.437\pgfutil@tempdima}}}%
    \pgfusepath{stroke}%
  }%
}%


\def\pgf@lib@sh@newbox{\csname newbox\endcsname}% Get round outer.

\def\pgf@lib@sh@toalpha#1{%
    \ifcase#1\relax%
        \or one\or two\or three\or four\or five\or six\or seven\or eight\or nine\or ten%
        \or eleven\or twelve\or thirteen\or fourteen\or fifteen%
        \or sixteen\or seventeen\or eighteen\or nineteen\or twenty%
    \else%
        twenty%
    \fi%
}%


\def\pgf@lib@sh@getalpha#1#2{\expandafter\edef\expandafter#1\expandafter{\pgf@lib@sh@toalpha{#2}}}%

\newbox\pgfnodeparttwobox
\newbox\pgfnodepartthreebox
\newbox\pgfnodepartfourbox

\let\pgfnodepartonebox=\pgfnodeparttextbox
\let\pgfnodepartsecondbox=\pgfnodeparttwobox
\let\pgfnodepartthirdbox=\pgfnodepartthreebox
\let\pgfnodepartfourthbox=\pgfnodepartfourbox

\def\pgf@lib@sh@allocateboxes#1{%
    \c@pgf@counta=#1\relax%
    \pgfmathloop%
        \ifnum\c@pgf@counta>4\relax%
        \pgfutil@ifundefined{pgfnodepart\pgf@lib@sh@toalpha{\c@pgf@counta}box}%
        {%
            \expandafter\pgf@lib@sh@newbox\csname pgfnodepart\pgf@lib@sh@toalpha{\c@pgf@counta}box\endcsname%
        }%
        {}%
        \advance\c@pgf@counta by-1\relax%
    \repeatpgfmathloop%
}%

\def\pgf@lib@sh@rs@lefttext{left}%
\def\pgf@lib@sh@rs@righttext{right}%
\def\pgf@lib@sh@rs@centertext{center}%
\def\pgf@lib@sh@rs@bottomtext{bottom}%
\def\pgf@lib@sh@rs@toptext{top}%
\def\pgf@lib@sh@rs@basetext{base}%
\def\pgf@lib@sh@rs@nonetext{none}%


\newif\ifpgfrectanglesplithorizontal
\newif\ifpgfrectanglesplitdrawsplits\pgfrectanglesplitdrawsplitstrue
\newif\ifpgfrectanglesplitignoreemptyparts
\newif\ifpgfrectanglesplitusecustomfill

\let\pgf@lib@sh@rs@every@emptypart=\pgfutil@empty
\let\pgf@lib@sh@rs@every@part=\pgfutil@empty
\def\pgf@lib@sh@rs@list@fill{none}%

\pgfkeys{/pgf/.cd,
    rectangle split parts/.initial=4,
    rectangle split part align/.initial=center,
    rectangle split horizontal/.is if=pgfrectanglesplithorizontal,
    rectangle split ignore empty parts/.is if=pgfrectanglesplitignoreemptyparts,
    rectangle split empty part width/.code={%
        \pgfmathsetlength\pgf@x{#1}
        \edef\pgf@lib@sh@rs@temp{\noexpand\vrule width\the\pgf@x height0ptdepth0pt\relax}%
        \def\pgf@lib@sh@rs@@temp{\def\pgf@lib@sh@rs@every@emptypart}%
        \expandafter\expandafter\expandafter\pgf@lib@sh@rs@@temp\expandafter\expandafter\expandafter{%
            \expandafter\pgf@lib@sh@rs@every@emptypart\pgf@lib@sh@rs@temp}%
    },%
    rectangle split empty part width=1ex,
    rectangle split empty part height/.code={%
        \pgfmathsetlength\pgf@x{#1}
        \edef\pgf@lib@sh@rs@temp{\noexpand\vrule width0ptheight\the\pgf@x depth0pt\relax}%
        \def\pgf@lib@sh@rs@@temp{\def\pgf@lib@sh@rs@every@emptypart}%
        \expandafter\expandafter\expandafter\pgf@lib@sh@rs@@temp\expandafter\expandafter\expandafter{%
            \expandafter\pgf@lib@sh@rs@every@emptypart\pgf@lib@sh@rs@temp}%
    },%
    rectangle split empty part height=1ex,
    rectangle split empty part depth/.code={%
        \pgfmathsetlength\pgf@x{#1}
        \edef\pgf@lib@sh@rs@temp{\noexpand\vrule width0ptheight0ptdepth\the\pgf@x\relax}%
        \def\pgf@lib@sh@rs@@temp{\def\pgf@lib@sh@rs@every@emptypart}%
        \expandafter\expandafter\expandafter\pgf@lib@sh@rs@@temp\expandafter\expandafter\expandafter{%
            \expandafter\pgf@lib@sh@rs@every@emptypart\pgf@lib@sh@rs@temp}%
    },%
    rectangle split empty part depth=0ex,
    rectangle split every empty part/.store in=\pgf@lib@sh@rs@every@emptypart,
    rectangle split part fill/.code=\def\pgf@lib@sh@rs@list@fill{#1}\pgfrectanglesplitusecustomfilltrue,
    rectangle split uses custom fill/.is if=pgfrectanglesplitusecustomfill,
    rectangle split draw splits/.is if=pgfrectanglesplitdrawsplits,
    rectangle split allocate boxes/.code=\pgf@lib@sh@allocateboxes{#1},
}%


\def\pgf@lib@sh@rs@process@list#1#2{%
    \c@pgf@counta=1\relax%
    \c@pgf@countb=#2\relax%
    \edef\pgf@lib@sh@rs@temp{#1}%
    \expandafter\pgf@lib@sh@rs@@process@list\pgf@lib@sh@rs@temp,\pgf@stop,
}%

\def\pgf@lib@sh@rs@@process@list{%
    \pgfutil@ifnextchar x{\pgf@lib@sh@rs@@@process@list}%
        {\pgf@lib@sh@rs@@@process@list}
}%

\def\pgf@lib@sh@rs@@@process@list#1,{%
    \ifx#1\pgf@stop%
        \let\pgf@next\pgf@lib@sh@rs@@@@process@list%
    \else%
        \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\c@pgf@counta}%
        \def\pgf@lib@sh@rs@lastalign{#1}%
        \pgfutil@namedef{pgf@lib@sh@rs@\pgf@lib@sh@toalpha{\c@pgf@counta}@item}{#1}%
        \let\pgf@next\pgf@lib@sh@rs@@process@list%
        \advance\c@pgf@counta by1\relax%
    \fi%
    \pgf@next}%

\def\pgf@lib@sh@rs@@@@process@list{%
    \pgfmathloop%
        \ifnum\c@pgf@counta>\c@pgf@countb%
        \else%
            \expandafter\edef\csname pgf@lib@sh@rs@\pgf@lib@sh@toalpha{\c@pgf@counta}@item\endcsname%
                {\pgf@lib@sh@rs@lastalign}%
            \advance\c@pgf@counta by1\relax%
    \repeatpgfmathloop%
}%

\pgf@lib@sh@allocateboxes{20}%

\pgfdeclareshape{rectangle split}{%
    \savedmacro\rectanglesplitparameters{%
        \pgfmathsetcount\c@pgf@counta{\pgfkeysvalueof{/pgf/rectangle split parts}}%
        \edef\parts{\the\c@pgf@counta}%
        \addtosavedmacro\parts%
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \edef\innerxsep{\the\pgf@x}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \edef\innerysep{\the\pgf@y}%
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \edef\outerxsep{\the\pgf@x}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
        \edef\outerysep{\the\pgf@y}%
        \addtosavedmacro\outerxsep%
        \addtosavedmacro\outerysep%
        %
        \pgf@x=0pt\relax% Widest box.
        \pgf@y=0pt\relax% Tallest box.
        %
        \pgfutil@tempdima=0pt\relax% Maximum box height.
        \pgfutil@tempdimb=0pt\relax% Maximum box depth.
        %
        % Get the dimensions of the boxes...
        %
        \pgfmathloop%
            \ifnum\pgfmathcounter>\parts%
            \else%
                \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                %
                \expandafter\let\expandafter\pgf@lib@sh@box\expandafter=%
                    \csname pgfnodepart\pgf@lib@sh@rs@number box\endcsname%
                \pgf@xa=\wd\pgf@lib@sh@box%
                \pgf@ya=\ht\pgf@lib@sh@box%
                \pgf@yb=\dp\pgf@lib@sh@box%
                %
                % Test to see if the box is empty...
                %
                \expandafter\def\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname{\relax}%
                \ifdim\pgf@xa=0pt\relax%
                    \ifdim\pgf@ya=0pt\relax%
                        \ifdim\pgf@yb=0pt\relax%
                            %
                            % ...It is. So...
                            %
                            \ifpgfrectanglesplitignoreemptyparts%
                                %
                                % ...flag this if we are ignoring parts...
                                %
                                \expandafter\let\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname=\pgfutil@empty%
                            \else%
                                %
                                % ...otherwise insert the code for every empty part.
                                %
                                \setbox\pgf@lib@sh@box=\hbox{{\pgf@lib@sh@rs@every@emptypart}}%
                                \pgf@xa=\wd\pgf@lib@sh@box%
                                \pgf@ya=\ht\pgf@lib@sh@box%
                                \pgf@yb=\dp\pgf@lib@sh@box%
                            \fi%
                        \fi%
                    \fi%
                \fi%
                \expandafter\edef\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@number\endcsname{\the\pgf@xa}%
                \expandafter\edef\csname pgf@lib@sh@rs@height@\pgf@lib@sh@rs@number\endcsname{\the\pgf@ya}%
                \expandafter\edef\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@number\endcsname{\the\pgf@yb}%
                \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname%
                %
                % ...saving the widest box...
                %
                \ifdim\pgf@xa>\pgf@x%
                    \pgf@x=\pgf@xa%
                \fi%
                %
                % ...the maximum height and depth...
                %
                \ifdim\pgf@ya>\pgfutil@tempdima%
                    \pgfutil@tempdima=\pgf@ya%
                \fi%
                \ifdim\pgf@yb>\pgfutil@tempdimb%
                    \pgfutil@tempdimb=\pgf@yb%
                \fi%
                %
                % ...and the tallest box.
                %
                \pgf@yc=\pgfutil@tempdima%
                \advance\pgf@yc by\pgfutil@tempdimb%
                \ifdim\pgf@yc>\pgf@y%
                    \pgf@y=\pgf@yc%
                \fi%
        \repeatpgfmathloop%
        %
        \edef\pgf@lib@sh@rs@max@width{\the\pgf@x}%
        \edef\pgf@lib@sh@rs@max@totalheight{\the\pgf@y}%
        %
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
        \advance\pgf@x by-\innerxsep\relax%
        \advance\pgf@x by-\innerxsep\relax%
        \pgf@xa=\pgf@x%
        \advance\pgf@xa by-\pgf@lib@sh@rs@max@width\relax%
        \ifdim\pgf@xa>0pt\relax%
            \edef\pgf@lib@sh@rs@max@width{\the\pgf@x}%
        \fi%
        %
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
        \advance\pgf@y by-\innerysep\relax%
        \advance\pgf@y by-\innerysep\relax%
        \pgf@ya=\pgf@y%
        \advance\pgf@ya by-\pgf@lib@sh@rs@max@totalheight\relax%
        \ifdim\pgf@ya>0pt\relax%
            \edef\pgf@lib@sh@rs@max@totalheight{\the\pgf@y}%
        \fi%
        %
        % Get the alignment of each node part box.
        %
        \pgf@lib@sh@rs@process@list{\pgfkeysvalueof{/pgf/rectangle split part align}}{\parts}%
        %
        % Are we splitting horizontally or vertically?
        %
        \ifpgfrectanglesplithorizontal%
            %
            % Calculate the origins of each node part box.
            %
            \pgf@x=0pt\relax%
            \pgfmathloop%
                \ifnum\pgfmathcounter>\parts%
                \else%
                    \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                    %
                    \expandafter\let\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname=\pgfutil@empty%
                    \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                        \ifpgfrectanglesplitignoreemptyparts%
                            \expandafter\let\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname=%
                                \pgf@lib@sh@rs@lastanchor%
                        \fi%
                    \fi%
                    %
                    % Adjust for alignment.
                    %
                    \expandafter\ifx\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                        \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname%
                                \pgf@lib@sh@rs@bottomtext%
                            \pgf@y=\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@number\endcsname\relax%
                        \else%
                            \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname%
                                    \pgf@lib@sh@rs@toptext%
                                \pgf@y=-\csname pgf@lib@sh@rs@height@\pgf@lib@sh@rs@number\endcsname\relax%
                                \advance\pgf@y by\pgf@lib@sh@rs@max@totalheight\relax%
                            \else%
                                \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname%
                                        \pgf@lib@sh@rs@basetext%
                                    \pgf@y=\pgf@lib@sh@rs@max@totalheight\relax%
                                    \advance\pgf@y by-\pgfutil@tempdima%
                                    \advance\pgf@y by\pgfutil@tempdimb%
                                    \divide\pgf@y by2\relax%
                                \else%
                                    \pgf@y=\pgf@lib@sh@rs@max@totalheight\relax%
                                    \advance\pgf@y by-\csname pgf@lib@sh@rs@height@\pgf@lib@sh@rs@number\endcsname\relax%
                                    \advance\pgf@y by\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@number\endcsname\relax%
                                    \divide\pgf@y by2\relax%
                                \fi%
                            \fi%
                        \fi%
                        %
                        % Re-adjust as the first box is at the origin.
                        %
                        \ifnum\pgfmathcounter=1\relax%
                            \edef\pgf@lib@sh@rs@yoffset{\the\pgf@y}%
                            \pgf@y=0pt\relax%
                            \pgfextract@process\pgf@lib@sh@rs@anchor@one{}%
                            \addtosavedmacro\pgf@lib@sh@rs@anchor@one%
                            \let\pgf@lib@sh@rs@lastanchor=\pgf@lib@sh@rs@anchor@one%
                            \let\pgf@lib@sh@rs@lastnumber=\pgf@lib@sh@rs@number%
                        \else
                            \advance\pgf@y by-\pgf@lib@sh@rs@yoffset\relax%
                            \advance\pgf@x by\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@lastnumber\endcsname\relax%
                            \advance\pgf@x by\innerxsep\relax%
                            \advance\pgf@x by\pgflinewidth%
                            \advance\pgf@x by\innerxsep\relax%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname{}%
                            \expandafter\let\expandafter\pgf@lib@sh@rs@lastanchor\expandafter=%
                                \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                            \let\pgf@lib@sh@rs@lastnumber=\pgf@lib@sh@rs@number%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                        \fi%
                    \fi%
            \repeatpgfmathloop%
            %
            % Calculate some anchors.
            %
            \pgfextract@process\northeast{%
                \pgf@lib@sh@rs@lastanchor%
                \advance\pgf@x by\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@lastnumber\endcsname\relax%
                \advance\pgf@x by\innerxsep\relax%
                \advance\pgf@x by\outerxsep\relax%
                \pgf@y=\pgf@lib@sh@rs@max@totalheight\relax%
                \advance\pgf@y by-\pgf@lib@sh@rs@yoffset\relax%
                \advance\pgf@y by\innerysep\relax%
                \advance\pgf@y by\outerysep\relax%
            }%
            \addtosavedmacro\northeast%
            \pgfextract@process\southwest{%
                \pgf@lib@sh@rs@anchor@one%
                \advance\pgf@x by-\innerxsep\relax%
                \advance\pgf@x by-\outerxsep\relax%
                \pgf@y=-\pgf@lib@sh@rs@yoffset\relax%
                \advance\pgf@y by-\innerysep\relax%
                \advance\pgf@y by-\outerysep\relax%
            }%
            \addtosavedmacro\southwest%
            %
            \pgfextract@process\centerpoint{%
                \pgfpointadd{\southwest}{\northeast}%
                \divide\pgf@x by2\relax%
                \divide\pgf@y by2\relax%
            }%
            \addtosavedmacro\centerpoint%
            %
            \pgfmathloop%
                \ifnum\pgfmathcounter>\parts%
                \else%
                    \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                    %
                    \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                    \else%
                        \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                        \pgf@xa=\pgf@x%
                        \pgf@xb=\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@number\endcsname\relax%
                        \advance\pgf@xa by0.5\pgf@xb%
                        \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @south\endcsname{%
                            \southwest%
                            \pgf@x=\pgf@xa%
                        }%
                        \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @north\endcsname{%
                            \northeast%
                            \pgf@x=\pgf@xa%
                        }%
                        \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @north\endcsname%
                        \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @south\endcsname%
                        \ifnum\pgfmathcounter=\parts%
                        \else%
                            \advance\pgf@xa by0.5\pgf@xb%
                            \advance\pgf@xa by\innerxsep\relax%
                            \advance\pgf@xa by.5\pgflinewidth%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@south\endcsname{%
                                \southwest%
                                \pgf@x=\pgf@xa%
                            }%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@north\endcsname{%
                                \northeast%
                                \pgf@x=\pgf@xa%
                            }%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split\endcsname{%
                                \centerpoint%
                                \pgf@x=\pgf@xa%
                            }%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@north\endcsname%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@south\endcsname%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split\endcsname%
                        \fi%
                    \fi%
            \repeatpgfmathloop%
        \else%
            %
            % Calculate the origins of each node part box.
            %
            \pgf@y=0pt\relax%
            \pgfmathloop%
                \ifnum\pgfmathcounter>\parts%
                \else%
                    \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                    %
                    \expandafter\let\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname=\pgfutil@empty%
                    \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                        \ifpgfrectanglesplitignoreemptyparts%
                            \expandafter\let\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname=%
                                \pgf@lib@sh@rs@lastanchor%
                        \fi%
                    \fi%
                    %
                    % Adjust for alignment.
                    %
                    \expandafter\ifx\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                        \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname%
                                \pgf@lib@sh@rs@lefttext%
                            \pgf@x=0pt\relax%
                        \else%
                            \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname%
                                    \pgf@lib@sh@rs@righttext%
                                \pgf@x=-\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@number\endcsname\relax%
                                \advance\pgf@x by\pgf@lib@sh@rs@max@width\relax%
                            \else%
                                \pgf@x=-\csname pgf@lib@sh@rs@width@\pgf@lib@sh@rs@number\endcsname\relax%
                                \advance\pgf@x by\pgf@lib@sh@rs@max@width\relax%
                                \divide\pgf@x by2\relax%
                        \fi%
                    \fi%
                    %
                    % Re-adjust as the first box is at the origin.
                    %
                    \ifnum\pgfmathcounter=1\relax%
                        \edef\pgf@lib@sh@rs@xoffset{\the\pgf@x}%
                        \pgf@x=0pt\relax%
                        \pgfextract@process\pgf@lib@sh@rs@anchor@one{}%
                        \addtosavedmacro\pgf@lib@sh@rs@anchor@one%
                        \let\pgf@lib@sh@rs@lastanchor=\pgf@lib@sh@rs@anchor@one%
                        \let\pgf@lib@sh@rs@lastnumber=\pgf@lib@sh@rs@number%
                    \else
                        \advance\pgf@x by-\pgf@lib@sh@rs@xoffset\relax%
                        \advance\pgf@y by-\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@lastnumber\endcsname\relax%
                        \advance\pgf@y by-\innerysep\relax%
                        \advance\pgf@y by-\pgflinewidth%
                        \advance\pgf@y by-\innerysep\relax%
                        \advance\pgf@y by-\csname pgf@lib@sh@rs@height@\pgf@lib@sh@rs@number\endcsname\relax%
                        \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname{}%
                        \expandafter\let\expandafter\pgf@lib@sh@rs@lastanchor\expandafter=%
                            \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                        \let\pgf@lib@sh@rs@lastnumber=\pgf@lib@sh@rs@number%
                        \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                    \fi%
                \fi%
            \repeatpgfmathloop%
            %
            % Calculate some anchors.
            %
            \pgfextract@process\northeast{%
                \pgf@x=\pgf@lib@sh@rs@max@width\relax%
                \advance\pgf@x by-\pgf@lib@sh@rs@xoffset\relax%
                \advance\pgf@x by\innerxsep\relax%
                \advance\pgf@x by\outerxsep\relax%
                \pgf@y=\pgf@lib@sh@rs@height@one\relax%
                \advance\pgf@y by\innerysep\relax%
                \advance\pgf@y by\outerysep\relax%
                \advance\pgf@y by.5\pgflinewidth%
            }%
            \addtosavedmacro\northeast%
            \pgfextract@process\southwest{%
                \pgf@lib@sh@rs@lastanchor%
                \pgf@x=-\pgf@lib@sh@rs@xoffset\relax%
                \advance\pgf@x by-\innerxsep\relax%
                \advance\pgf@x by-\outerxsep\relax%
                \advance\pgf@y by-\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@lastnumber\endcsname\relax%
                \advance\pgf@y by-\innerysep\relax%
                \advance\pgf@y by-\outerysep\relax%
                \advance\pgf@y by-.5\pgflinewidth%
            }%
            \addtosavedmacro\southwest%
            %
            \pgfextract@process\centerpoint{%
                \pgfpointadd{\southwest}{\northeast}%
                \divide\pgf@x by2\relax%
                \divide\pgf@y by2\relax%
            }%
            \addtosavedmacro\centerpoint%
            %
            \pgfmathloop%
                \ifnum\pgfmathcounter>\parts%
                \else%
                    \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                    %
                    \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                    \else%
                        \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                        \pgf@ya=\csname pgf@lib@sh@rs@height@\pgf@lib@sh@rs@number\endcsname\relax%
                        \advance\pgf@y by0.5\pgf@ya%
                        \pgf@ya=\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@number\endcsname\relax%
                        \advance\pgf@y by-0.5\pgf@ya%
                        \pgf@ya=\pgf@y%
                        \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @west\endcsname{%
                            \southwest%
                            \pgf@y=\pgf@ya%
                        }%
                        \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @east\endcsname{%
                            \northeast%
                            \pgf@y=\pgf@ya%
                        }%
                        \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @east\endcsname%
                        \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @west\endcsname%
                        \ifnum\pgfmathcounter=\parts%
                        \else%
                            \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number\endcsname%
                            \pgf@ya=\pgf@y%
                            \advance\pgf@ya by-\csname pgf@lib@sh@rs@depth@\pgf@lib@sh@rs@number\endcsname\relax%
                            \advance\pgf@ya by-\innerysep\relax%
                            \advance\pgf@ya by-.5\pgflinewidth%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@west\endcsname{%
                                \southwest%
                                \pgf@y=\pgf@ya%
                            }%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@east\endcsname{%
                                \northeast%
                                \pgf@y=\pgf@ya%
                            }%
                            \expandafter\pgfextract@process\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split\endcsname{%
                                \centerpoint%
                                \pgf@y=\pgf@ya%
                            }%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@east\endcsname%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@west\endcsname%
                            \expandafter\addtosavedmacro\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split\endcsname%
                        \fi%
                    \fi%
            \repeatpgfmathloop%
        \fi%
    }%
    \savedanchor\basepoint{%
        \pgf@x=0.5\wd\pgfnodeparttextbox%
        \pgf@y=0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x=0.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{+0.5ex}%
    }%
    \anchor{center}{%
        \rectanglesplitparameters%
        \centerpoint%
    }%
    \anchor{base}{\basepoint}%
    \anchor{base east}{%
        \rectanglesplitparameters%
        \northeast%
        \pgf@y=0pt\relax%
    }%
    \anchor{base west}{%
        \rectanglesplitparameters%
        \southwest%
        \pgf@y=0pt\relax%
    }%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{%
        \rectanglesplitparameters%
        \northeast%
        \pgf@xa=\pgf@x%
        \midpoint%
        \pgf@x=\pgf@xa%
    }%
    \anchor{mid west}{%
        \rectanglesplitparameters%
        \southwest%
        \pgf@xa=\pgf@x%
        \midpoint%
        \pgf@x=\pgf@xa%
    }%
    \anchor{north}{%
        \rectanglesplitparameters%
        \centerpoint%
        \pgf@xa=\pgf@x%
        \northeast%
        \pgf@x=\pgf@xa%
    }%
    \anchor{south}{%
        \rectanglesplitparameters%
        \centerpoint%
        \pgf@xa=\pgf@x%
        \southwest%
        \pgf@x=\pgf@xa%
    }%
    \anchor{east}{%
        \rectanglesplitparameters%
        \centerpoint%
        \pgf@ya=\pgf@y%
        \northeast%
        \pgf@y=\pgf@ya%
    }%
    \anchor{west}{%
        \rectanglesplitparameters%
        \centerpoint%
        \pgf@ya=\pgf@y%
        \southwest%
        \pgf@y=\pgf@ya%
    }%
    \anchor{north east}{%
        \rectanglesplitparameters%
        \northeast%
    }%
    \anchor{north west}{%
        \rectanglesplitparameters%
        \northeast%
        \pgf@ya=\pgf@y%
        \southwest%
        \pgf@y=\pgf@ya%
    }%
    \anchor{south west}{%
        \rectanglesplitparameters%
        \southwest%
    }%
    \anchor{south east}{%
        \rectanglesplitparameters%
        \southwest%
        \pgf@ya=\pgf@y%
        \northeast%
        \pgf@y=\pgf@ya%
    }%
    \behindbackgroundpath{%
        \ifpgfrectanglesplitusecustomfill%
            \pgf@lib@sh@rs@process@list{\pgf@lib@sh@rs@list@fill}{\parts}%
            {%
                \ifpgfrectanglesplithorizontal%
                    \expandafter\let\expandafter\pgf@lib@sh@rs@fill@bottomleft\expandafter=%
                        \csname pgf@anchor@rectangle split@south west\endcsname%
                    \pgfmathloop%
                        \ifnum\pgfmathcounter>\parts%
                        \else%
                            \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                            \ifnum\pgfmathcounter=\parts%
                                \expandafter\let\expandafter\pgf@lib@sh@rs@fill@topright\expandafter=%
                                    \csname pgf@anchor@rectangle split@north east\endcsname%
                            \else%
                                \expandafter\let\expandafter\pgf@lib@sh@rs@fill@topright\expandafter=%
                                    \csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@number\space split north\endcsname%
                            \fi%
                            \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                            \else%
                                \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname\pgf@lib@sh@rs@nonetext%
                                \else%
                                    \pgfextract@process\pgf@lib@sh@rs@fill@bottomleft{%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \advance\pgf@y by\outerysep\relax%
                                        \ifnum\pgfmathcounter=1\relax%
                                            \advance\pgf@x by\outerxsep\relax%
                                        \fi%
                                    }%
                                    \pgfextract@process\pgf@lib@sh@rs@fill@topright{%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \advance\pgf@y by-\outerysep\relax%
                                        \ifnum\pgfmathcounter=\parts\relax%
                                            \advance\pgf@x by-\outerxsep\relax%
                                        \fi%
                                    }%
                                    \ifnum\pgfmathcounter>1\relax%
                                        \begingroup\pgfsetcornersarced{\pgfpointorigin}%
                                    \fi%
                                    \pgfpathmoveto{%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \pgf@xa=\pgf@x%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \pgf@x=\pgf@xa%
                                    }%
                                    \pgfpathlineto{\pgf@lib@sh@rs@fill@bottomleft}%
                                    \pgfpathlineto{%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \pgf@xa=\pgf@x%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \pgf@x=\pgf@xa%
                                    }%
                                    \ifnum\pgfmathcounter>1\relax%
                                        \endgroup%
                                    \fi%
                                    \ifnum\pgfmathcounter<\parts%
                                        \begingroup\pgfsetcornersarced{\pgfpointorigin}%
                                    \fi%
                                    \pgfpathlineto{\pgf@lib@sh@rs@fill@topright}%
                                    \pgfpathclose%
                                    \ifnum\pgfmathcounter<\parts%
                                        \endgroup%
                                    \fi%
                                    \pgfsetfillcolor{\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname}%
                                    \pgfusepath{fill}%
                                \fi%
                            \fi%
                            \pgfextract@process\pgf@lib@sh@rs@fill@bottomleft{%
                                \pgf@lib@sh@rs@fill@bottomleft%
                                \pgf@ya=\pgf@y%
                                \pgf@lib@sh@rs@fill@topright%
                                \pgf@y=\pgf@ya%
                                \advance\pgf@y by-\outerysep%
                            }%
                    \repeatpgfmathloop%
                \else%
                    \expandafter\let\expandafter\pgf@lib@sh@rs@fill@topright\expandafter=%
                        \csname pgf@anchor@rectangle split@north east\endcsname%
                    \pgfmathloop%
                        \ifnum\pgfmathcounter>\parts%
                        \else%
                            \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                            \ifnum\pgfmathcounter=\parts%
                                \expandafter\let\expandafter\pgf@lib@sh@rs@fill@bottomleft\expandafter=%
                                    \csname pgf@anchor@rectangle split@south west\endcsname%
                            \else%
                                \expandafter\let\expandafter\pgf@lib@sh@rs@fill@bottomleft\expandafter=%
                                    \csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@number\space split west\endcsname%
                            \fi%
                            \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                            \else%
                                \expandafter\ifx\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname\pgf@lib@sh@rs@nonetext%
                                \else%
                                    \pgfextract@process\pgf@lib@sh@rs@fill@bottomleft{%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \advance\pgf@x by\outerxsep\relax%
                                        \ifnum\parts=1\relax%
                                            \advance\pgf@y by\outerysep\relax%
                                        \else%
                                            \ifnum\pgfmathcounter=\parts
                                                \advance\pgf@y by\outerysep\relax%
                                            \fi%
                                        \fi%
                                    }%
                                    \pgfextract@process\pgf@lib@sh@rs@fill@topright{%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \advance\pgf@x by-\outerxsep\relax%
                                        \ifnum\parts=1\relax%
                                            \advance\pgf@y by-\outerysep\relax%
                                        \else%
                                            \ifnum\pgfmathcounter=1\relax%
                                                \advance\pgf@y by-\outerysep\relax%
                                            \fi%
                                        \fi%
                                    }%
                                    \pgfpathmoveto{\pgf@lib@sh@rs@fill@bottomleft}%
                                    \ifnum\pgfmathcounter>1\relax%
                                        \begingroup\pgfsetcornersarced{\pgfpointorigin}%
                                    \fi%
                                    \pgfpathlineto{%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \pgf@xa=\pgf@x%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \pgf@x=\pgf@xa%
                                    }%
                                    \pgfpathlineto{\pgf@lib@sh@rs@fill@topright}%
                                    \ifnum\pgfmathcounter>1\relax%
                                        \endgroup%%
                                    \fi%
                                    \ifnum\pgfmathcounter<\parts%
                                        \begingroup\pgfsetcornersarced{\pgfpointorigin}%
                                    \fi%
                                    \pgfpathlineto{%
                                        \pgf@lib@sh@rs@fill@topright%
                                        \pgf@xa=\pgf@x%
                                        \pgf@lib@sh@rs@fill@bottomleft%
                                        \pgf@x=\pgf@xa%
                                    }%
                                    \pgfpathclose%
                                    \ifnum\pgfmathcounter<\parts%
                                        \endgroup%
                                    \fi%
                                    \pgfsetfillcolor{\csname pgf@lib@sh@rs@\pgf@lib@sh@rs@number @item\endcsname}%
                                    \pgfusepath{fill}%
                                \fi%
                            \fi%
                            \pgfextract@process\pgf@lib@sh@rs@fill@topright{%
                                \pgf@lib@sh@rs@fill@topright%
                                \pgf@xa=\pgf@x%
                                \pgf@lib@sh@rs@fill@bottomleft%
                                \pgf@x=\pgf@xa%
                                \advance\pgf@x by\outerxsep\relax%
                            }%
                    \repeatpgfmathloop%
                \fi%
            }%
        \fi%
    }%
    \backgroundpath{%
        \begingroup%
            \pgfextract@process\southwest{%
                \southwest%
                \advance\pgf@x by\outerxsep\relax%
                \advance\pgf@y by\outerysep\relax%
            }%
            \pgfextract@process\northeast{%
                \northeast%
                \advance\pgf@x by-\outerxsep\relax%
                \advance\pgf@y by-\outerysep\relax%
            }%
            \pgfpathrectangle{\southwest}{\pgfpointdiff{\southwest}{\northeast}}%
        \endgroup%
        \ifpgfrectanglesplitdrawsplits%
            \pgfmathloop%
                \ifnum\pgfmathcounter=\parts%
                \else%
                    \pgf@lib@sh@getalpha\pgf@lib@sh@rs@number{\pgfmathcounter}%
                    %
                    \expandafter\ifx\csname pgf@lib@sh@rs@empty@\pgf@lib@sh@rs@number\endcsname\pgfutil@empty%
                    \else%
                        \pgfpathmoveto{%
                            \ifpgfrectanglesplithorizontal%
                                \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@north\endcsname%
                                \advance\pgf@y by-\outerysep\relax%
                            \else%
                                \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@east\endcsname%
                                \advance\pgf@x by-\outerxsep\relax%
                            \fi%
                        }%
                        \pgfpathlineto{%
                            \ifpgfrectanglesplithorizontal%
                                \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@south\endcsname%
                                \advance\pgf@y by\outerysep\relax%
                            \else%
                                \csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@number @split@west\endcsname%
                                \advance\pgf@x by\outerxsep\relax%
                            \fi%
                        }%
                    \fi%
            \repeatpgfmathloop%
        \fi%
    }%
    \anchorborder{%
        \pgfutil@tempdima\pgf@x%
        \pgfutil@tempdimb\pgf@y%
        \rectanglesplitparameters%
        \pgfpointdiff{\southwest}{\northeast}%
        \pgf@x.5\pgf@x%
        \pgf@y.5\pgf@y%
        \edef\pgf@marshall{%
            \noexpand\pgfpointborderrectangle{%
                    \noexpand\pgfqpoint{\the\pgfutil@tempdima}{\the\pgfutil@tempdimb}%
                }%
                {%
                    \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}%
                }%
        }%
        \pgf@marshall%
        \pgf@xa\pgf@x%
        \pgf@ya\pgf@y%
        \centerpoint%
        \advance\pgf@x\pgf@xa%
        \advance\pgf@y\pgf@ya%
    }%
    %
    % Hackery to install the correct number of node parts.
    %
    \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@rectangle split\endcsname{%
        \let\pgf@lib@sh@rs@temp=\pgfutil@empty%
        \pgfmathloop%
            \ifnum\pgfmathcounter=\parts%
                \expandafter\edef\csname pgf@sh@boxes@rectangle split\endcsname%
                    {\pgf@lib@sh@rs@temp\pgf@lib@sh@toalpha{\pgfmathcounter}}%
            \else%
                \edef\pgf@lib@sh@rs@temp{\pgf@lib@sh@rs@temp\pgf@lib@sh@toalpha{\pgfmathcounter},}%
        \repeatpgfmathloop%
    }%
}%

\pgfutil@for\pgf@lib@sh@rs@temp:={one,two,three,four,five,six,seven,eight,nine,ten,eleven,twelve,thirteen,fourteen,fifteen,sixteen,seventeen,eighteen,nineteen,twenty}\do{%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp}{\noexpand\pgf@lib@sh@rs@anchor@one}%
            {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space split\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split}%
        {\noexpand\centerpoint}%
        {\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space split north\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@north}%
        {\noexpand\csname pgf@anchor@rectangle split@north\noexpand\endcsname}%
        {\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@north\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space split south\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@south}%
        {\noexpand\csname pgf@anchor@rectangle split@south\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@south\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space north\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @north}%
        {\noexpand\csname pgf@anchor@rectangle split@north\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @north\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space south\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @south}%
        {\noexpand\csname pgf@anchor@rectangle split@south\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @south\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space split east\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@east}%
        {\noexpand\csname pgf@anchor@rectangle split@east\noexpand\endcsname}%
        {\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@east\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space split west\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@west}%
        {\noexpand\csname pgf@anchor@rectangle split@west\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @split@west\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space east\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @east}%
        {\noexpand\csname pgf@anchor@rectangle split@east\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @east\noexpand\endcsname}%
    }%
    \expandafter\xdef\csname pgf@anchor@rectangle split@\pgf@lib@sh@rs@temp\space west\endcsname{%
        \noexpand\rectanglesplitparameters%
        \noexpand\pgfutil@ifundefined{pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @west}%
        {\noexpand\csname pgf@anchor@rectangle split@west\noexpand\endcsname}%
        {\noexpand\csname pgf@lib@sh@rs@anchor@\pgf@lib@sh@rs@temp @west\noexpand\endcsname}%
    }%
}%


\pgfutil@namelet{pgf@anchor@rectangle split@text east}{pgf@anchor@rectangle split@one east}%
\pgfutil@namelet{pgf@anchor@rectangle split@text west}{pgf@anchor@rectangle split@one west}%
\pgfutil@namelet{pgf@anchor@rectangle split@text split}{pgf@anchor@rectangle split@one split}%
\pgfutil@namelet{pgf@anchor@rectangle split@text split east}{pgf@anchor@rectangle split@one split east}%
\pgfutil@namelet{pgf@anchor@rectangle split@text split west}{pgf@anchor@rectangle split@one split west}%

\pgfutil@namelet{pgf@anchor@rectangle split@second}{pgf@anchor@rectangle split@two}%
\pgfutil@namelet{pgf@anchor@rectangle split@second east}{pgf@anchor@rectangle split@two east}%
\pgfutil@namelet{pgf@anchor@rectangle split@second west}{pgf@anchor@rectangle split@two west}%
\pgfutil@namelet{pgf@anchor@rectangle split@second split}{pgf@anchor@rectangle split@two split}%
\pgfutil@namelet{pgf@anchor@rectangle split@second split east}{pgf@anchor@rectangle split@two split east}%
\pgfutil@namelet{pgf@anchor@rectangle split@second split west}{pgf@anchor@rectangle split@two split west}%

\pgfutil@namelet{pgf@anchor@rectangle split@third}{pgf@anchor@rectangle split@three}%
\pgfutil@namelet{pgf@anchor@rectangle split@third east}{pgf@anchor@rectangle split@three east}%
\pgfutil@namelet{pgf@anchor@rectangle split@third west}{pgf@anchor@rectangle split@three west}%
\pgfutil@namelet{pgf@anchor@rectangle split@third split}{pgf@anchor@rectangle split@three split}%
\pgfutil@namelet{pgf@anchor@rectangle split@third split east}{pgf@anchor@rectangle split@three split east}%
\pgfutil@namelet{pgf@anchor@rectangle split@third split west}{pgf@anchor@rectangle split@three split west}%

\pgfutil@namelet{pgf@anchor@rectangle split@fourth}{pgf@anchor@rectangle split@four}%
\pgfutil@namelet{pgf@anchor@rectangle split@fourth east}{pgf@anchor@rectangle split@four east}%
\pgfutil@namelet{pgf@anchor@rectangle split@fourth west}{pgf@anchor@rectangle split@four west}%
\pgfutil@namelet{pgf@anchor@rectangle split@fourth split}{pgf@anchor@rectangle split@four split}%
\pgfutil@namelet{pgf@anchor@rectangle split@fourth split east}{pgf@anchor@rectangle split@four split east}%
\pgfutil@namelet{pgf@anchor@rectangle split@fourth split west}{pgf@anchor@rectangle split@four split west}%




% Shape: ellipse split.
%
\pgfdeclareshape{ellipse split}{%
    \nodeparts{text,lower}%
    \savedanchor\radii{%
        \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \pgf@y2.0\pgf@y%
        \advance\pgf@y.5\pgflinewidth%
        \pgf@xa.5\wd\pgfnodeparttextbox%
        \pgf@xb.5\wd\pgfnodepartlowerbox%
        \advance\pgf@xa\pgf@x%
        \advance\pgf@xb\pgf@x%
        \pgf@ya\ht\pgfnodeparttextbox%
        \advance\pgf@ya\dp\pgfnodeparttextbox%
        \pgf@yb\ht\pgfnodepartlowerbox%
        \advance\pgf@yb\dp\pgfnodepartlowerbox%
        \advance\pgf@ya\pgf@y%
        \advance\pgf@yb\pgf@y%
        \ifdim\pgf@xa>\pgf@xb%
            \pgf@x1.414213\pgf@xa%
        \else%
            \pgf@x1.414213\pgf@xb%
        \fi%
        \ifdim\pgf@ya>\pgf@yb%
            \pgf@y1.414213\pgf@ya%
        \else%
            \pgf@y1.414213\pgf@yb%
        \fi%
        \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
        \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
        \ifdim\pgf@x<.5\pgf@xa%
            \pgf@x.5\pgf@xa%
        \fi%
        \ifdim\pgf@y<.5\pgf@ya%
            \pgf@y.5\pgf@ya%
        \fi%
        \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    }%
    \savedanchor\lower{%
        \pgf@x-.5\wd\pgfnodepartlowerbox%
        \advance\pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
        \pgf@y-2.0\pgf@y%
        \advance\pgf@y-\pgflinewidth%
        \advance\pgf@y-\dp\pgfnodeparttextbox%
        \advance\pgf@y-\ht\pgfnodepartlowerbox%
    }%
    \savedanchor\centerpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{-\pgfkeysvalueof{/pgf/inner ysep}}%
        \advance\pgf@y-\dp\pgfnodeparttextbox%
        \advance\pgf@y-.5\pgflinewidth%
    }%
    \savedanchor\basepoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgf@y0pt\relax%
    }%
    \savedanchor\midpoint{%
        \pgf@x.5\wd\pgfnodeparttextbox%
        \pgfmathsetlength\pgf@y{.5ex}%
    }%
    \anchor{center}{\centerpoint}%
    \anchor{lower}{\lower}%
    \anchor{mid}{\midpoint}%
    \anchor{mid east}{\radii\pgf@xa\pgf@x\midpoint\advance\pgf@x\pgf@xa}%
    \anchor{mid west}{\radii\pgf@xa\pgf@x\midpoint\advance\pgf@x-\pgf@xa}%
    \anchor{base}{\basepoint}%
    \anchor{base east}{\radii\pgf@xa\pgf@x\basepoint\advance\pgf@x\pgf@xa}%
    \anchor{base west}{\radii\pgf@xa\pgf@x\basepoint\advance\pgf@x-\pgf@xa}%
    \anchor{north}{\pgfpointadd{\centerpoint}{\radii\pgf@x0pt}}%
    \anchor{south}{\pgfpointadd{\centerpoint}{\radii\pgf@x0pt\pgf@y-\pgf@y}}%
    \anchor{east}{\pgfpointadd{\centerpoint}{\radii\pgf@y0pt}}%
    \anchor{west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-\pgf@x\pgf@y0pt}}%
    \anchor{north west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
    \anchor{south west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
    \anchor{north east}{\pgfpointadd{\centerpoint}{\radii\pgf@x0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
    \anchor{south east}{\pgfpointadd{\centerpoint}{\radii\pgf@x0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
    \backgroundpath{%
        \radii%
        \pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
        \pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
        \pgfutil@tempdima\pgf@x%
        \pgfutil@tempdimb\pgf@y%
        \pgfpathellipse{\centerpoint}{\pgfqpoint{\the\pgfutil@tempdima}{0pt}}{\pgfqpoint{0pt}{\the\pgfutil@tempdimb}}%
        \pgfpathmoveto{\centerpoint\advance\pgf@x-\pgfutil@tempdima}%
        \pgfpathlineto{\centerpoint\advance\pgf@x\pgfutil@tempdima}%
    }%
    \anchorborder{%
        \pgfextract@process\externalpoint{}%
        \radii%
        \edef\pgf@marshal{%
            \noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
                {\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\centerpoint}%
        }%
       \pgf@marshal%
    }%
}%

\endinput


==> pgflibraryshapes.symbols.code.tex <==
% Copyright 2018 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgflibraryshapes.symbols.code.tex}

\pgfdeclareshape{forbidden sign}
{%
  \inheritsavedanchors[from=circle]% this is nearly a circle
  \inheritanchorborder[from=circle]%
  \inheritanchor[from=circle]{north}%
  \inheritanchor[from=circle]{north west}%
  \inheritanchor[from=circle]{north east}%
  \inheritanchor[from=circle]{center}%
  \inheritanchor[from=circle]{west}%
  \inheritanchor[from=circle]{east}%
  \inheritanchor[from=circle]{mid}%
  \inheritanchor[from=circle]{mid west}%
  \inheritanchor[from=circle]{mid east}%
  \inheritanchor[from=circle]{base}%
  \inheritanchor[from=circle]{base west}%
  \inheritanchor[from=circle]{base east}%
  \inheritanchor[from=circle]{south}%
  \inheritanchor[from=circle]{south west}%
  \inheritanchor[from=circle]{south east}%
  \inheritbackgroundpath[from=circle]%
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.707107\pgfutil@tempdima}{-0.707107\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{0.707107\pgfutil@tempdima}{0.707107\pgfutil@tempdima}}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
  }%
}%


\pgfdeclareshape{correct forbidden sign}
{%
  \inheritsavedanchors[from=circle]% this is nearly a circle
  \inheritanchorborder[from=circle]%
  \inheritanchor[from=circle]{north}%
  \inheritanchor[from=circle]{north west}%
  \inheritanchor[from=circle]{north east}%
  \inheritanchor[from=circle]{center}%
  \inheritanchor[from=circle]{west}%
  \inheritanchor[from=circle]{east}%
  \inheritanchor[from=circle]{mid}%
  \inheritanchor[from=circle]{mid west}%
  \inheritanchor[from=circle]{mid east}%
  \inheritanchor[from=circle]{base}%
  \inheritanchor[from=circle]{base west}%
  \inheritanchor[from=circle]{base east}%
  \inheritanchor[from=circle]{south}%
  \inheritanchor[from=circle]{south west}%
  \inheritanchor[from=circle]{south east}%
  \inheritbackgroundpath[from=circle]%
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{0.707107\pgfutil@tempdima}{-0.707107\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.707107\pgfutil@tempdima}{0.707107\pgfutil@tempdima}}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
  }%
}%





% Keys for starburst shape
%
% /pgf/starburst point height : The maximum height of the outer points.
% /pgf/starburst points       : The number of points.
% /pgf/random starburst       : The seed for the random number generator.
%
\pgfkeys{/pgf/random starburst/%
  .code={%
    \ifx\pgfkeysnovalue#1%
      \pgfmathgeneratepseudorandomnumber%
    \else%
      \pgfmathtruncatemacro\pgfmathresult{#1}%
    \fi%
    \pgfkeyslet{/pgf/random starburst}{\pgfmathresult}%
  }%
}%
\pgfkeys{/pgf/random starburst=100}%

\pgfkeys{/pgf/starburst point height/.value required}%
\pgfkeys{/pgf/starburst point height/.code={%
    \pgfmathparse{#1}%
    \edef\pgfmathresult{\pgfmathresult pt}%
    \pgfkeyslet{/pgf/starburst point height}{\pgfmathresult}%
  }%
}%
\pgfkeys{/pgf/starburst point height=.5cm}%

\pgfkeys{/pgf/starburst points/.value required}%
\pgfkeys{/pgf/starburst points/.code={%
    \pgfmathtruncatemacro\pgfmathresult{#1}%
    \pgfkeyslet{/pgf/starburst points}{\pgfmathresult}%
  }%
}%
\pgfkeys{/pgf/starburst points=17}%

\pgfdeclareshape{starburst}{%
  \savedmacro\anglestep{%
    \pgfmathdivide@{180}{\pgfkeysvalueof{/pgf/starburst points}}%
    \let\anglestep\pgfmathresult%
  }%
  \savedmacro\calculatestarburstpoints{%
    %
    % Get the angle step.
    %
    \pgfmathdivide@{180}{\pgfkeysvalueof{/pgf/starburst points}}%
    \let\anglestep\pgfmathresult%
    %
    % Get the total number of points.
    %
    \pgfmathsetcounter{pgf@counta}{\pgfkeysvalueof{/pgf/starburst points}}%
    \multiply\c@pgf@counta2\relax%
    \edef\totalpoints{\the\c@pgf@counta}%
    \addtosavedmacro{\totalpoints}%
    %
    % Calculate the centerpoint.
    %
    \pgfextract@process\centerpoint{%
      \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
      \pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
      \pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
    }%
    %
    % Get the larger of the outer sep.
    %
    \pgfmathsetlength\pgf@x{+\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@y{+\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@x<\pgf@y%
      \pgf@x\pgf@y%
    \fi%
    \edef\outersep{\the\pgf@x}%
    %
    % Get the node dimensions.
    %
    \pgfmathsetlength\pgf@x{+\pgfkeysvalueof{/pgf/inner xsep}}%
    \pgfmathaddtolength\pgf@x{+.5\wd\pgfnodeparttextbox}%
    \pgfmathsetlength\pgf@y{+\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgfmathaddtolength\pgf@y{+.5\ht\pgfnodeparttextbox}%
    \pgfmathaddtolength\pgf@y{+.5\dp\pgfnodeparttextbox}%
    %
    %  Calculate the inner radii.
    %
    \ifpgfshapeborderusesincircle%
      \pgfkeysgetvalue{/pgf/shape border rotate}{\rotate}%
      %
      % Use the incircle...
      %
      \ifdim\pgf@y>\pgf@x%
        \pgf@x\pgf@y%
      \fi%
      \pgf@x1.41421\pgf@x%
      \pgf@y\pgf@x%
    \else%
      %
      % Get the rotation (with rounding).
      %
      \pgfkeysgetvalue{/pgf/shape border rotate}{\rotate}%
      \pgfmathmod@{\rotate}{360}%
      \afterassignment\pgfmath@gobbletilpgfmath@%
      \expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
      \advance\c@pgf@counta45\relax%
      \divide\c@pgf@counta90\relax%
      \multiply\c@pgf@counta90\relax%
      \ifnum\c@pgf@counta<0\relax%
        \advance\c@pgf@counta360\relax%
      \fi%
      %
      % Calculate the width and height of the node
      % contents, according to any border rotation.
      %
      \ifnum\c@pgf@counta=90\relax%
        \pgf@xc\pgf@x%
        \pgf@x\pgf@y%
        \pgf@y\pgf@xc%
      \else%
        \ifnum\c@pgf@counta=270\relax%
          \pgf@xc\pgf@x%
          \pgf@x\pgf@y%
          \pgf@y\pgf@xc%
        \fi%
      \fi%
      \edef\rotate{\the\c@pgf@counta}%
      %
      % ...or not.
      %
      \pgf@x=1.41421\pgf@x%
      \pgf@y=1.41421\pgf@y%
    \fi%
    \addtosavedmacro{\rotate}%
    %
    % Adjust innerradius for minimum width and height.
    %
    \pgf@xa\pgf@x%
    \pgfmathsetlength\pgf@xb{+\pgfkeysvalueof{/pgf/starburst point height}}%
    \advance\pgf@xa\pgf@xb%
    \pgfmathsetlength\pgf@xc{+\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@xa<.5\pgf@xc%
      \pgf@x.5\pgf@xc%
      \advance\pgf@x-\pgf@xb%
    \fi%
    \pgf@ya\pgf@y%
    \pgfmathsetlength\pgf@yb{+\pgfkeysvalueof{/pgf/starburst point height}}%
    \advance\pgf@ya\pgf@yb%
    \pgfmathsetlength\pgf@yc{+\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@ya<.5\pgf@yc%
      \pgf@y.5\pgf@yc%
      \advance\pgf@y-\pgf@yb%
    \fi%
    \edef\xinnerradius{\the\pgf@x}%
    \edef\yinnerradius{\the\pgf@y}%
    \addtosavedmacro{\xinnerradius}%
    \addtosavedmacro{\yinnerradius}%
    %
    % Calculate a radius outside the starburst.
    %
    \ifdim\pgf@y>\pgf@x%
      \pgf@x\pgf@y%
    \fi%
    \pgfmathaddtolength\pgf@x{+\pgfkeysvalueof{/pgf/starburst point height}}%
    \edef\externalradius{\the\pgf@x}%
    \addtosavedmacro{\externalradius}%
    %
    % Set the seed for the random number generator.
    %
    \pgfmathsetseed{\pgfkeysvalueof{/pgf/random starburst}}%
    %
    % Now create the points on the shape and also
    % the miter length and angle for each point.
    %
    \def\angle{90}% Start at the top.
    %
    % At point a, the miter length and angle are calculated for point b = a - 1.
    %
    \c@pgf@counta1\relax%
    \c@pgf@countb0\relax%
    %
    % As 3 consecutive points are required to be defined for miter
    % calculations, it is necessary to go over the first two points
    % again.
    %
    \c@pgf@countc\totalpoints\relax%
    \advance\c@pgf@countc2\relax%
    \edef\looppoints{\the\c@pgf@countc}%
    \let\secondpoint\pgfutil@empty%
    \let\thirdpoint\pgfutil@empty%
    \pgfmathloop%
      %
      % Cycle the point definitions.
      %
      \let\firstpoint\secondpoint%
      \let\secondpoint\thirdpoint%
      \ifnum\pgfmathcounter>\looppoints%
      \else%
        \ifnum\pgfmathcounter>\totalpoints%
          \expandafter\let\expandafter\thirdpoint\csname point@\the\c@pgf@counta @\endcsname%
        \else%
          \ifodd\pgfmathcounter%
            %
            % An outer point.
            %
            \ifnum\pgfkeysvalueof{/pgf/random starburst}=0\relax%
              \pgf@xa\pgfkeysvalueof{/pgf/starburst point height}\relax%
            \else%
              \pgf@x\pgfkeysvalueof{/pgf/starburst point height}\relax%
              \pgf@xa.75\pgf@x%
              \pgf@xb.25\pgf@x%
              \pgfmathrnd%
              \pgf@xa\pgfmathresult\pgf@xa%
              \advance\pgf@xa\pgf@xb%
            \fi%
            \pgf@x\xinnerradius\relax%
            \advance\pgf@x\pgf@xa%
            \pgf@y\yinnerradius\relax%
            \advance\pgf@y\pgf@xa%
            \expandafter\pgfextract@process\csname point@\the\c@pgf@counta @\endcsname{%
              \pgfpointpolar{\angle}{\the\pgf@x and \the\pgf@y}%
              \pgf@xa\pgf@x%
              \pgf@ya\pgf@y%
              \centerpoint%
              \advance\pgf@x\pgf@xa%
              \advance\pgf@y\pgf@ya%
            }%
          \else%
            %
            % An inner point.
            %
            \expandafter\pgfextract@process\csname point@\the\c@pgf@counta @\endcsname{%
              \pgfpointpolar{\angle}{\xinnerradius and \yinnerradius}%
              \pgf@xa\pgf@x%
              \pgf@ya\pgf@y%
              \centerpoint%
              \advance\pgf@x\pgf@xa%
              \advance\pgf@y\pgf@ya%
            }%
          \fi%
          %
          % Add the points to the saved macro.
          %
          \expandafter\let\expandafter\thirdpoint\csname point@\the\c@pgf@counta @\endcsname%
          \expandafter\addtosavedmacro\expandafter{\csname point@\the\c@pgf@counta @\endcsname}%
        \fi%
        %
        % It is only possible to do the miter calculations if three points are defined.
        %
        \ifx\firstpoint\pgfutil@empty%
        \else%
          %
          % Calculate the miter length...
          %
          \pgfmathanglebetweenlines{\secondpoint}{\thirdpoint}{\secondpoint}{\firstpoint}%
          \pgfmathdivide@{\pgfmathresult}{2}%
          \let\defaultmiterangle\pgfmathresult%
          \pgfmathcosec@{\pgfmathresult}%
          \pgf@x\outersep\relax%
          \pgf@x\pgfmathresult\pgf@x%
          \edef\miterlength{\the\pgf@x}%
          %
          % ...the miter angle...
          %
          \pgfmathanglebetweenlines{\firstpoint}{\secondpoint}{\firstpoint}{\thirdpoint}%
          \pgfmathadd@{\pgfmathresult}{\defaultmiterangle}%
          \pgfmathsubtract@{180}{\pgfmathresult}%
          \let\angletemp\pgfmathresult%
          \pgfmathanglebetweenpoints{\firstpoint}{\thirdpoint}%
          \pgfmathsubtract@{180}{\pgfmathresult}%
          \pgfmathsubtract@{\angletemp}{\pgfmathresult}%
          \edef\miterangle{\pgfmathresult}%
          %
          % ...and thus the border point.
          %
          \pgfextract@process\borderpoint{%
            \secondpoint%
            \pgf@xa\pgf@x
            \pgf@ya\pgf@y%
            \pgfpointpolar{\miterangle}{\miterlength}%
            \advance\pgf@x\pgf@xa%
            \advance\pgf@y\pgf@ya%
          }%
          %
          % Get the angle from the centerpoint to the *unrotated* border points.
          %
          \pgfmathanglebetweenpoints{\centerpoint}{\borderpoint}%
          \expandafter\edef\csname angletoborderpoint@\the\c@pgf@countb @\endcsname{\pgfmathresult}%
          \expandafter\addtosavedmacro\expandafter{\csname angletoborderpoint@\the\c@pgf@countb @\endcsname}%
          %
          % Rotate the border points and save.
          %
          \expandafter\pgfextract@process\csname borderpoint@\the\c@pgf@countb @\endcsname{%
            \pgfmathrotatepointaround{\borderpoint}{\centerpoint}{\rotate}%
          }%
          \expandafter\addtosavedmacro\expandafter{\csname borderpoint@\the\c@pgf@countb @\endcsname}%
          %
          % Now create the anchors.
          %
          \c@pgf@countc\c@pgf@countb%
          \advance\c@pgf@countc1\relax%
          \divide\c@pgf@countc2\relax%
          \ifodd\c@pgf@countb\relax%
            \pgfutil@ifundefined{pgf@anchor@starburst@outer point\space\the\c@pgf@countc}{%
              \expandafter\xdef\csname pgf@anchor@starburst@outer point\space\the\c@pgf@countc\endcsname{%
                \noexpand\calculatestarburstpoints%
                \noexpand\csname borderpoint@\the\c@pgf@countb @\noexpand\endcsname%
              }%
            }{}%
          \else%
            \pgfutil@ifundefined{pgf@anchor@starburst@inner point\space\the\c@pgf@countc}{%
              \expandafter\xdef\csname pgf@anchor@starburst@inner point\space\the\c@pgf@countc\endcsname{%
                \noexpand\calculatestarburstpoints%
                \noexpand\csname borderpoint@\the\c@pgf@countb @\noexpand\endcsname%
              }%
            }{}%
          \fi%
        \fi%
        \pgfmathadd@{\angle}{\anglestep}%
        \pgfmathmod@{\pgfmathresult}{360}%
        \let\angle\pgfmathresult%
        \advance\c@pgf@counta1\relax%
        \ifnum\c@pgf@counta>\totalpoints%
          \c@pgf@counta1\relax%
        \fi%
        \advance\c@pgf@countb1\relax%
        \ifnum\c@pgf@countb>\totalpoints%
          \c@pgf@countb1\relax%
        \fi%
    \repeatpgfmathloop%
  }%
  \savedanchor\centerpoint{%
    \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
    \pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
    \pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
  }%
  \savedanchor\midpoint{%
    \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
    \pgfmathsetlength\pgf@y{+.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
    \pgf@y0pt\relax%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{base}{\basepoint}%
  \anchor{mid}{\midpoint}%
  \anchor{north}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
  }%
  \anchor{south}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
  }%
  \anchor{east}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
  }%
  \anchor{west}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
  }%
  \anchor{north west}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
  }%
  \anchor{south west}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
  }%
  \anchor{north east}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
  }%
  \anchor{south east}{%
    \calculatestarburstpoints%
    \csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
  }%
  \backgroundpath{%
    \calculatestarburstpoints%
    \pgfmathloop%
      \ifnum\pgfmathcounter>\totalpoints%
      \else%
        \ifnum\pgfmathcounter=1\relax%
          \let\starburstaction\pgfpathmoveto%
        \else%
          \let\starburstaction\pgfpathlineto%
        \fi%
        \starburstaction{%
          %\pgfmathrotatepointaround{\csname point@\pgfmathcounter @\endcsname}{\centerpoint}{\rotate}}%
          \csname point@\pgfmathcounter @\endcsname}
      \repeatpgfmathloop%
    \pgfpathclose%
  }%
  \anchorborder{%
    %
    % Save x and y.
    %
    \edef\externalx{\the\pgf@x}%
    \edef\externaly{\the\pgf@y}%
    %
    % Adjust the location of the external
    % point relative to \centerpoint.
    %
    \centerpoint%
    \pgf@xa\externalx\relax%
    \pgf@ya\externaly\relax%
    \advance\pgf@xa\pgf@x%
    \advance\pgf@ya\pgf@y%
    \edef\externalx{\the\pgf@xa}%
    \edef\externaly{\the\pgf@ya}%
    %
    % Get the starburst points.
    %
    \calculatestarburstpoints%
    %
    % Get the angle of the external point to the \centerpoint.
    %
    \pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
    \pgfmathsubtract@{\pgfmathresult}{\rotate}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\externalangle\pgfmathresult%
    %
    % Locate the appropriate sides on the starburst border...
    %
    \ifdim\externalangle pt<90pt\relax%
      \c@pgf@counta0\relax%
      \c@pgf@countb\totalpoints\relax%
      \pgfmathloop%
      \ifnum\c@pgf@counta>0\relax%
      \else%
        \ifdim\csname angletoborderpoint@\the\c@pgf@countb @\endcsname pt>90pt\relax%
          \c@pgf@counta\c@pgf@countb%
        \else%
          \ifdim\externalangle pt>\csname angletoborderpoint@\the\c@pgf@countb @\endcsname pt\relax%
            \c@pgf@counta\c@pgf@countb%
          \fi%
        \fi%
        \advance\c@pgf@countb-1\relax%
      \repeatpgfmathloop%
      \edef\first{\the\c@pgf@counta}%
      \advance\c@pgf@counta1\relax%
      \ifnum\c@pgf@counta>\totalpoints\relax%
        \c@pgf@counta1\relax%
      \fi%
      \edef\second{\the\c@pgf@counta}%
    \else%
      \c@pgf@counta0\relax%
      \pgfmathloop%
      \ifnum\c@pgf@counta>0\relax%
      \else%
        \ifdim\csname angletoborderpoint@\pgfmathcounter @\endcsname pt<90pt\relax%
          \c@pgf@counta\pgfmathcounter%
        \else%
          \ifdim\externalangle pt<\csname angletoborderpoint@\pgfmathcounter @\endcsname pt\relax%
            \c@pgf@counta\pgfmathcounter%
          \fi%
        \fi%
      \repeatpgfmathloop%
      \edef\first{\the\c@pgf@counta}%
      \advance\c@pgf@counta-1\relax%
      \ifnum\c@pgf@counta=0\relax%
        \c@pgf@counta\totalpoints\relax%
      \fi%
      \edef\second{\the\c@pgf@counta}%
    \fi%
    %
    % ...and thus, the point on the star border.
    %
    \pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
        {\csname borderpoint@\first @\endcsname}{\csname borderpoint@\second @\endcsname}%
  }%
}%




% Keys for shape cloud.
%
% /pgf/cloud puffs    : the number of cloud puffs.
% /pgf/cloud puff arc : the length of the cloud puff arc.

\newif\ifpgfcloudanchorsuseellipse%
\newif\ifpgfcloudignoresaspect%
\pgfcloudignoresaspectfalse%
\pgfkeys{/pgf/.cd,
  cloud puffs/.initial=10,
  cloud puff arc/.initial=150,
  cloud ignores aspect/.is if=pgfcloudignoresaspect,
  cloud anchors use ellipse/.is if=pgfcloudanchorsuseellipse,
}%


% If symbol library is loaded separately these need to be defined.
%
\pgfkeys{/pgf/.cd,
  aspect/.code={\pgfsetshapeaspect{#1}},% this for tikz...
  shape aspect/.initial=1,% but this is consistent with other pgfset stuff.
  shape aspect/.code={%
    \pgfkeys{/pgf/aspect=#1}%
    \pgfkeyssetvalue{/pgf/shape aspect}{#1}
  }%
}%

\def\pgfsetshapeaspect#1{%
  \def\pgfshapeaspect{#1}%
  % Invert
  \pgfutil@tempdima=#1pt%
  \pgfutil@tempdima=.125\pgfutil@tempdima%
  \c@pgf@counta=\pgfutil@tempdima\relax% 8192*determinant
  \pgfutil@tempdima=8192pt%
  \divide\pgfutil@tempdima by\c@pgf@counta%
  \edef\pgfshapeaspectinverse{\pgf@sys@tonumber{\pgfutil@tempdima}}%
}%

\pgfsetshapeaspect{1}%


% Shape cloud.
%
\pgfdeclareshape{cloud}{%
  \savedmacro\getradii{%
    \pgfmathtruncatemacro\puffs{\pgfkeysvalueof{/pgf/cloud puffs}}%
    \addtosavedmacro\puffs%
    \pgfmathdivide{360}{\pgfkeysvalueof{/pgf/cloud puffs}}%
    \let\anglestep\pgfmathresult%
    \addtosavedmacro\anglestep%
    \pgfmathsetmacro\arc{\pgfkeysvalueof{/pgf/cloud puff arc}}%
    \addtosavedmacro\arc%
    %
    % x radius.
    %
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@x1.4142135\pgf@x%
    %
    % y radius.
    %
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y.5\dp\pgfnodeparttextbox%
    \pgf@y1.4142135\pgf@y%
    %
    % Adjust for shape aspect.
    %
    \ifpgfcloudignoresaspect%
      \pgf@xc\pgf@x%
      \pgf@yc\pgf@y%
    \else%
      \pgf@xc\pgfshapeaspect\pgf@y%
      \ifdim\pgf@xc<\pgf@x%
        \pgf@xc\pgf@x%
      \fi%
      \pgf@yc\pgfshapeaspectinverse\pgf@xc%
      \ifdim\pgf@yc<\pgf@y%
        \pgf@yc\pgf@y%
        \pgf@xc\pgfshapeaspect\pgf@y%
      \fi%
    \fi%
    %
    \edef\xinnerradius{\the\pgf@xc}%
    \edef\yinnerradius{\the\pgf@yc}%
    %
    % Get the larger of the outer sep.
    %
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@x<\pgf@y%
      \pgf@x\pgf@y%
    \fi%
    \edef\outersep{\the\pgf@x}%
    \addtosavedmacro\outersep%
    %
    % For a given cloud, with puff arc length a, the quotient of the
    % distance between the start and end point of a puffs circular arc
    % and the radius of that arc, is constant:
    %
    % g = .5 * sec((180-a)/2)
    %
    \pgfmathsubtract{180}{\arc}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\tempangle\pgfmathresult%
    \pgfmathsec@{\pgfmathresult}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\arcradiusquotient\pgfmathresult%
    \addtosavedmacro\arcradiusquotient%
    %
    % In addition, the quotient of the distance between the start and
    % end point of a puffs circular arc and the height of that arc
    % (ignoring rotation), is also constant:
    %
    % h = .5 * (1-sin((180-a)/2))/cos((180-a)/2)
    %   = g  * (1 - sin((180-a)/2))
    \pgfmathsin@{\tempangle}%
    \pgfmathsubtract@{1}{\pgfmathresult}%
    \pgfmathmultiply@{\pgfmathresult}{\arcradiusquotient}%
    \let\archeightquotient\pgfmathresult%
    \addtosavedmacro\archeightquotient%
    %
    % Minimum size is applied to the circum-ellipse (i.e. the ellipse
    % that passes through the extremities of each puff). Thus, the
    % relationship between the radii of the elliptical incircle ("inellipse"?)
    % of the cloud (x and y) and the radii of the circum-ellipse (X and Y),
    % is given by
    %
    % X = 2(x*cos(p/2) + ky)
    % Y = 2(y*cos(p/2) + kx)
    %
    % where:
    % k = sin(p/2)*((1-cos(a/2))/sin(a/2))
    % p = the angle between each puff (i.e. 360/<puffs>)
    % a = the length of arc of the puff.
    %
    \pgfmathdivide{\arc}{2}%
    \let\halfarcangle\pgfmathresult%
    \pgfmathcos@{\pgfmathresult}%
    \pgfmathsubtract@{1}{\pgfmathresult}%
    \let\pgf@temp\pgfmathresult%
    \pgfmathsin@{\halfarcangle}%
    \pgfmathdivide@{\pgf@temp}{\pgfmathresult}%
    \let\pgf@temp\pgfmathresult%
    \pgfmathdivide@{\anglestep}{2}%
    \pgfmathsin@{\pgfmathresult}%
    \pgfmathmultiply@{\pgfmathresult}{\pgf@temp}%
    \let\k\pgfmathresult%
    %
    \pgfmathdivide@{\anglestep}{2}%
    \pgfmathcos@{\pgfmathresult}%
    \let\coshalfanglestep\pgfmathresult%
    %
    % Calculate the actual radii of the circum-ellipse.
    %
    \pgf@x\xinnerradius\relax%
    \pgf@y\yinnerradius\relax%
    \pgf@xa\coshalfanglestep\pgf@x%
    \advance\pgf@xa\k\pgf@y%
    \pgf@ya\coshalfanglestep\pgf@y%
    \advance\pgf@ya\k\pgf@x%
    %
    % Adjust for minimum height (Y').
    %
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@ya<.5\pgf@yb%
      \pgf@ya.5\pgf@yb%
    \fi%
    %
    % Adjust for minimum width (X').
    %
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@xa<.5\pgf@xb%
      \pgf@xa.5\pgf@xb%
    \fi%
    %
    \edef\xouterradius{\the\pgf@xa}%
    \addtosavedmacro\xouterradius%
    \edef\youterradius{\the\pgf@ya}%
    \addtosavedmacro\youterradius%
    %
    % Now recalculate `in-ellipse' radii:
    %
    % x = (X'cos(p/2)-kY')/cos^2(p/2)-k^2,
    % y = (Y'cos(p/2)-kX')/cos^2(p/2)-k^2,
    %
    \pgf@xc\k pt\relax%
    \pgf@xc-\k\pgf@xc%
    \pgf@yc\coshalfanglestep pt\relax%
    \pgf@yc\coshalfanglestep\pgf@yc%
    \advance\pgf@xc\pgf@yc\relax%
    \pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xc}}% cos^2(p/2)-k^2
    %
    \pgf@x\coshalfanglestep\pgf@xa%
    \advance\pgf@x-\k\pgf@ya%
    \pgf@x\pgfmathresult\pgf@x%
    \pgf@y\coshalfanglestep\pgf@ya%
    \advance\pgf@y-\k\pgf@xa%
    \pgf@y\pgfmathresult\pgf@y%
    %
    \edef\xinnerradius{\the\pgf@x}%
    \edef\yinnerradius{\the\pgf@y}%
    \addtosavedmacro\xinnerradius%
    \addtosavedmacro\yinnerradius%
    %
    % Get some useful trig. constants.
    %
    \pgfmathdivide@{\arc}{4}%
    \let\quarterarc\pgfmathresult%
    \pgfmathsubtract@{180}{\arc}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\halfcomplementarc\pgfmathresult%
    %
    \addtosavedmacro\arc%
    \addtosavedmacro\quarterarc%
    \addtosavedmacro\halfcomplementarc%
    %
    \pgfmathsec@{\halfcomplementarc}% 1/cos((180-a)/2)
    \let\sechalfcomplementarc\pgfmathresult%
    \pgfmathsin@{\halfcomplementarc}% sin((180-a)/2)
    \let\sinhalfcomplementarc\pgfmathresult%
    %
    \addtosavedmacro\sechalfcomplementarc%
    \addtosavedmacro\sinhalfcomplementarc%
    %
    \pgfmathsin@{\quarterarc}% sin(a/4)
    \let\sinquarterarc\pgfmathresult%
    \pgfmathcos@{\quarterarc}% cos(a/4)
    \let\cosquarterarc\pgfmathresult%
    \pgfmathreciprocal@{\cosquarterarc}%
    \pgfmathmultiply@{\pgfmathresult}{\sinquarterarc}% tan(a/4)
    \let\tanquarterarc\pgfmathresult%
    %
    \addtosavedmacro\sinquarterarc%
    \addtosavedmacro\cosquarterarc%
    \addtosavedmacro\tanquarterarc%
    %
  }%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+.5ex}%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{base}{\basepoint}%
  \anchor{north}{%
    \getradii%
    \csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{0pt}{\youterradius}}%
  }%
  \anchor{south}{%
    \getradii%
    \csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{0pt}{-\youterradius}}%
  }%
  \anchor{east}{%
    \getradii%
    \csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{\xouterradius}{0pt}}%
  }%
  \anchor{west}{%
    \getradii%
    \csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{-\xouterradius}{0pt}}%
  }%
  \anchor{north west}{%
    \getradii%
    \pgfextract@process\pgf@sh{%
      \pgf@x\xouterradius\relax%
      \pgf@x-0.707106\pgf@x%
      \pgf@y\youterradius\relax%
      \pgf@y0.707106\pgf@y%
    }%
    \csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
  }%
  \anchor{north east}{%
    \getradii%
    \pgfextract@process\pgf@sh{%
      \pgf@x\xouterradius\relax%
      \pgf@x0.707106\pgf@x%
      \pgf@y\youterradius\relax%
      \pgf@y0.707106\pgf@y%
    }%
    \csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
  }%
  \anchor{south west}{%
    \getradii%
    \pgfextract@process\pgf@sh{%
      \pgf@x\xouterradius\relax%
      \pgf@x-0.707106\pgf@x%
      \pgf@y\youterradius\relax%
      \pgf@y-0.707106\pgf@y%
    }%
    \csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
  }%
  \anchor{south east}{%
    \getradii%
    \pgfextract@process\pgf@sh{%
      \pgf@x\xouterradius\relax%
      \pgf@x0.707106\pgf@x%
      \pgf@y\youterradius\relax%
      \pgf@y-0.707106\pgf@y%
    }%
    \csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
  }%
  %
  % Each `puff' is a circular arc of length a, drawn using two a/2
  % arcs (a < 180), approximated by Bezier curves.
  % Due to TeX rounding errors, it is sometimes necessary to `force'
  % the arc to end at a specific point. So...
  %
  % @article{riskus2006,
  %   author  = {Aleskus Ri\v{s}kus},
  %   title   = {Approximation of a cubic Bezier curve by circular arcs and vice versa},
  %   journal = {Information Technology and Control},
  %   year    = {2006},
  %   volume  = {35},
  %   number  = {4}
  % }
  %
  \backgroundpath{%
    {%
    \getradii%
    %
    % Get the start angle.
    %
    \pgfmathdivide@{\anglestep}{2}%
    \pgfmathsubtract@{90}{\pgfmathresult}%
    \let\angle\pgfmathresult%
    %
    % Calculate the first arc point.
    %
    \pgfextract@process\arcfirstpoint{%
      \pgfpointadd{\centerpoint}{%
        \pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
      }%
    }%
    \pgfpathmoveto{\arcfirstpoint}%
    \let\arcendpoint\arcfirstpoint%
    %
    \pgfmathloop%
    \ifnum\pgfmathcounter>\puffs\relax%
    \else
      \let\arcstartpoint\arcendpoint%
      %
      % Make sure beginning and end of path are exactly the same.
      %
      \ifnum\pgfmathcounter=\puffs\relax%
        \let\arcendpoint\arcfirstpoint%
      \else%
        \pgfmathadd@{\angle}{\anglestep}%
        \let\angle\pgfmathresult%
        \pgfextract@process\arcendpoint{%
          \pgfpointadd{\centerpoint}{%
            \pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
          }%
        }%
      \fi%
      %
      % Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
      %
      \pgf@sh@getcloudpuffparameters%
      %
      % Get the rotation for the Bezier curve.
      %
      \pgfmathsubtract@{90}{\quarterarc}%
      \pgfmathadd@{\pgfmathresult}{\arcslope}%
      \let\arcrotate\pgfmathresult%
      \pgfmathsin@{\arcrotate}%
      \let\sinarcrotate\pgfmathresult%
      \pgfmathcos@{\arcrotate}%
      \let\cosarcrotate\pgfmathresult%
      %
      % Calculate the amount by which to scale the control
      % points, in order to approximate an a/2 arc with radius x.
      %
      \pgf@x\arcradius\relax%
      \pgf@x\tanquarterarc\pgf@x% tan(a/4)
      \edef\controlscale{\pgfmath@tonumber{\pgf@x}}%
      %
      % Get the first control point for the first arc (length a/2)...
      %
      \pgfextract@process\controlone{%
        %
        % k = 0.552284745 (a `magic' number)...
        %
        \pgf@x0.55228475pt\relax%
        \pgf@x\sinquarterarc\pgf@x% k * sin(a/2)
        \pgf@y0.55228475pt\relax%
        \pgf@y\cosquarterarc\pgf@y% k * cos(a/2)
        %
        % ...scale the control points up...
        %
        \pgf@x\controlscale\pgf@x%
        \pgf@y\controlscale\pgf@y%
        %
        % ...rotate...
        %
        \pgf@xa\cosarcrotate\pgf@x%
        \advance\pgf@xa-\sinarcrotate\pgf@y%
        \pgf@ya\cosarcrotate\pgf@y%
        \advance\pgf@ya\sinarcrotate\pgf@x%
        %
        % ...and shift.
        %
        \arcstartpoint%
        \advance\pgf@x\pgf@xa%
        \advance\pgf@y\pgf@ya%
      }%
      %
      % Get the midpoint of the 150� arc.
      %
      \pgfextract@process\arcmidpoint{%
        \pgfextract@process\arcmidpoint{%
          \pgf@x-\halfchordlength\relax%
          \pgf@y\segmentheight\relax%
        }%
        \pgfpointadd{\arcstartpoint}{%
          \pgfmathrotatepointaround{\arcmidpoint}{\pgfpointorigin}{\arcslope}%
        }%
      }%
      %
      % Get the second control point for the first arc (length a/2)...
      %
      \pgfextract@process\controltwo{%
        \pgf@x0.55228475pt\relax%
        \pgf@x\sinquarterarc\pgf@x%  k * sin(a/2)
        \pgf@y-0.55228475pt\relax%
        \pgf@y\cosquarterarc\pgf@y% -k * cos(a/2)
        %
        % ...scale, rotate and shift.
        %
        \pgf@x\controlscale\pgf@x%
        \pgf@y\controlscale\pgf@y%
        %
        \pgf@xa\cosarcrotate\pgf@x%
        \advance\pgf@xa-\sinarcrotate\pgf@y%
        \pgf@ya\cosarcrotate\pgf@y%
        \advance\pgf@ya\sinarcrotate\pgf@x%
        %
        \arcmidpoint%
        \advance\pgf@x\pgf@xa%
        \advance\pgf@y\pgf@ya%
      }%
      {%
        \pgfsetcornersarced{\pgfpointorigin}%
        \pgfpathcurveto{\controlone}{\controltwo}{\arcmidpoint}%
      }%
      %
      % Do the same for the second arc...
      %
      \pgfmathadd@{\quarterarc}{90}%
      \pgfmathadd@{\pgfmathresult}{\arcslope}%
      \let\arcrotate\pgfmathresult%
      \pgfmathsin@{\arcrotate}%
      \let\sinarcrotate\pgfmathresult%
      \pgfmathcos@{\arcrotate}%
      \let\cosarcrotate\pgfmathresult%
      %
      % First control point for the second arc...
      %
      \pgfextract@process\controlone{%
        \pgf@x0.55228475pt\relax%
        \pgf@x\sinquarterarc\pgf@x% k * sin(a/2)
        \pgf@y0.55228475pt\relax%
        \pgf@y\cosquarterarc\pgf@y% k * cos(a/2)
        %
        % ...scale, rotate and shift.
        %
        \pgf@x\controlscale\pgf@x%
        \pgf@y\controlscale\pgf@y%
        %
        \pgf@xa\cosarcrotate\pgf@x%
        \advance\pgf@xa-\sinarcrotate\pgf@y%
        \pgf@ya\cosarcrotate\pgf@y%
        \advance\pgf@ya\sinarcrotate\pgf@x%
        %
        \arcmidpoint%
        \advance\pgf@x\pgf@xa%
        \advance\pgf@y\pgf@ya%
      }%
      %
      % Second control point for the second arc.
      %
      \pgfextract@process\controltwo{%
        \pgf@x0.55228475pt\relax%
        \pgf@x\sinquarterarc\pgf@x%  k * sin(a/2)
        \pgf@y-0.55228475pt\relax%
        \pgf@y\cosquarterarc\pgf@y% -k * cos(a/2)
        %
        % ...scale, rotate and shift.
        %
        \pgf@x\controlscale\pgf@x%
        \pgf@y\controlscale\pgf@y%
        %
        \pgf@xa\cosarcrotate\pgf@x%
        \advance\pgf@xa-\sinarcrotate\pgf@y%
        \pgf@ya\cosarcrotate\pgf@y%
        \advance\pgf@ya\sinarcrotate\pgf@x%
        %
        \arcendpoint%
        \advance\pgf@x\pgf@xa%
        \advance\pgf@y\pgf@ya%
      }%
      \pgfpathcurveto{\controlone}{\controltwo}{\arcendpoint}%
      \repeatpgfmathloop%
    \pgfpathclose% Phew!
    }%
  }%
  %
  % Calculate a point on the border of the cloud. This is a two-stage process:
  %
  % 1. Locate the correct puff.
  % 2. Locate the angle on the circular arc which forms the puff.
  %
  \anchorborder{%
    %
    % Save x and y.
    %
    \edef\externalx{\the\pgf@x}%
    \edef\externaly{\the\pgf@y}%
     %
    % Get the inner radii and trig. constants.
    %
    \getradii%
    %
    %
    %
    \ifpgfcloudanchorsuseellipse%
      \pgfpointadd{\centerpoint}{%
        \pgfpointborderellipse{%
          \pgfpoint{\externalx}{\externaly}
          }{%
            \pgfpoint{\xouterradius}{\youterradius}
          }%
      }%
    \else%
      \pgfextract@process\externalpoint{%
        \centerpoint%
        \advance\pgf@x\externalx\relax%
        \advance\pgf@y\externaly\relax%
      }%
      \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
      \let\externalangle\pgfmathresult%
      %
      % 1. Locate the correct puff:
      %
      % Get end angle of the relevant puff arc.
      %
      \pgfmathdivide@{\anglestep}{2}%
      \let\halfanglestep\pgfmathresult%
      \pgfmathsubtract@{90}{\halfanglestep}%
      \let\endangle\pgfmathresult%
      \pgfmathloop%
        \pgfmathsubtract@{\endangle}{\anglestep}%
        \ifdim\pgfmathresult pt<-\anglestep pt\relax%
        \else%
          \let\endangle\pgfmathresult%
      \repeatpgfmathloop%
      \def\angle{0}%
      \let\lastangle\angle%
      \pgfmathloop%
        \pgfmathadd@{\endangle}{\anglestep}%
        \let\endangle\pgfmathresult%
        %
        % Calculate the `miter point'. This is the point between
        % each puff, and takes into account the outer sep.
        %
        \pgfextract@process\miterpoint{%
          %
          \pgfextract@process\secondpoint{%
            \pgfpointpolar{+\endangle}{+\xinnerradius and +\yinnerradius}%
          }%
          %
          \pgfmathadd@{\endangle}{\anglestep}%
          \let\angletemp\pgfmathresult%
          \pgfextract@process\thirdpoint{%
            \pgfpointpolar{+\angletemp}{+\xinnerradius and +\yinnerradius}%
          }%
          %
          \pgfmathsubtract@{\endangle}{\anglestep}%
          \let\angletemp\pgfmathresult%
          \pgfextract@process\firstpoint{%
            \pgfpointpolar{+\angletemp}{+\xinnerradius and +\yinnerradius}%
          }%
          %
          \pgfmathanglebetweenpoints{\firstpoint}{\secondpoint}%
          \let\anglealpha\pgfmathresult%
          \pgfmathanglebetweenpoints{\secondpoint}{\thirdpoint}%
          \let\anglebeta\pgfmathresult%
          %
          \pgfmathsubtract@{\anglebeta}{\anglealpha}%
          \pgfmathdivide@{\pgfmathresult}{2}%
          \pgfmathadd@{\pgfmathresult}{\halfcomplementarc}%
          \pgfmathcosec@{\pgfmathresult}%
          \pgf@x\outersep\relax%
          \pgf@x\pgfmathresult\pgf@x%
          \edef\miterradius{\the\pgf@x}%
          %
          \pgfmathadd@{\anglealpha}{\anglebeta}%
          \pgfmathsubtract@{\pgfmathresult}{180}%
          \pgfmathdivide@{\pgfmathresult}{2}%
          \let\miterangle\pgfmathresult%
          \pgfpointadd{\secondpoint}{%
            \pgfqpointpolar{\miterangle}{\miterradius}%
          }%
        }%
        %
        % Get the angle of the miter point...
        %
        \pgfmathanglebetweenpoints{\pgfpointorigin}{\miterpoint}%
        \let\angle\pgfmathresult%
        \ifdim\angle pt<\lastangle pt\relax% Guard against 360� = 0�
          \pgfmathadd@{\angle}{360}%
          \let\angle\pgfmathresult%
        \fi%
        \let\lastangle\angle%
        %
        % ...and see if it is greater than the external point.
        %
      \ifdim\externalangle pt>\angle pt\relax%
      \repeatpgfmathloop%
      %
      % Get the start angle of the relevant arc and ensure angles are in the range.
      %
      \pgfmathmod@{\endangle}{360}%
      \let\endangle\pgfmathresult%
      \pgfmathsubtract@{\endangle}{\anglestep}%
      \ifdim\pgfmathresult pt<0pt\relax%
        \pgfmathadd@{\pgfmathresult}{360}%
      \fi%
      \let\startangle\pgfmathresult%
      %
      % Now, get the start and end points of the arc.
      %
      \pgfextract@process\arcstartpoint{%
        \pgfpointadd{\centerpoint}{%
          \pgfpointpolar{+\startangle}{+\xinnerradius and +\yinnerradius}%
        }%
      }%
      \pgfextract@process\arcendpoint{%
        \pgfpointadd{\centerpoint}{%
          \pgfpointpolar{+\endangle}{+\xinnerradius and +\yinnerradius}%
        }%
      }%
      %
      % Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
      %
      \pgf@sh@getcloudpuffparameters%
      %
      % Hackery, for when an arc straddles 0�.
      %
      \ifdim\endangle pt<\startangle pt\relax%
        \pgfmathadd@{\externalangle}{180}%
        \pgfmathmod@{\pgfmathresult}{360}%
        \let\x\pgfmathresult%
      \else%
        \let\x\externalangle%
      \fi%
      %
      % 2. Locate the angle on the circular arc which forms the puff.
      %
      % Essentially a binary search to find the angle on the circular
      % arc, which provides the nearest estimate to the border point.
      %
      \let\s\halfcomplementarc% The start of the arc.
      \pgfmathadd@{\s}{\arc}%
      \let\e\pgfmathresult% The end of the arc.
      \pgfmathadd@{\e}{\s}%
      \pgfmathdivide@{\pgfmathresult}{2}%
      \let\n\pgfmathresult% The nearest estimate (default to middle of arc).
      \def\m{360}% Measure of `nearness'.
      \pgfmathloop%
        \pgfmathadd@{\e}{\s}%
        \pgfmathdivide@{\pgfmathresult}{2}%
        \let\p\pgfmathresult% The point halfway between \s and \e.
        \ifdim\p pt=\s pt\relax%
        \else%
          %
          % Get the point on the circular arc.
          %
          \pgfmathadd@{\p}{\arcslope}%
          \let\a\pgfmathresult%
          \pgfextract@process\arcpoint{%
            \pgfpointadd{\circlecenterpoint}{%
              \pgfqpointpolar{\a}{\outerarcradius}%
            }%
          }%
          %
          % Find the angle between the node centre and the point on the arc.
          %
          \pgfmathanglebetweenpoints{\centerpoint}{\arcpoint}%
          %
          % Hackery, for when an arc straddles 0�.
          %
          \ifdim\endangle pt<\startangle pt\relax%
            \pgfmathadd@{\pgfmathresult}{180}%
            \pgfmathmod@{\pgfmathresult}{360}%
          \fi%
          \let\q\pgfmathresult%
          \ifdim\x pt=\q pt% Found it!
            \pgfmathbreakloop% Breaks after current iteration is complete.
          \else
            \ifdim\x pt<\q pt\relax%
              \let\e\p%
            \else%
              \let\s\p%
            \fi%
          \fi%
          \pgfmathsubtract@{\x}{\q}%
          \pgfmathabs@{\pgfmathresult}%
          %
          % Save the estimate if it is better than any previous estimate.
          %
          \ifdim\pgfmathresult pt<\m pt\relax%
            \let\m\pgfmathresult%
            \let\n\p%
          \fi%
      \repeatpgfmathloop%
      %
      % Use the nearest estimate as the anchor angle.
      %
      \pgfmathadd@{\n}{\arcslope}%
      \let\anchorangle\pgfmathresult%
      %
      % Finally, the required point.
      %
      \pgfpointadd{\circlecenterpoint}{%
        \pgfqpointpolar{\anchorangle}{\outerarcradius}%
      }%
    \fi%
  }% Again, Phew!
  %
  % Now, a sneaky hack. This means an arbitrary `puff' anchors
  % can be used for positioning the cloud shape. This is needed
  % if a cloud is positioned using the `puff <n+1>' anchor, where
  % n is the number of puffs of any previously drawn cloud.
  %
  \pgfutil@g@addto@macro\pgf@sh@s@cloud{%
    \c@pgf@counta\puffs\relax%
    \pgfmathloop%
      \ifnum\c@pgf@counta>0\relax%
        \pgfutil@ifundefined{pgf@anchor@cloud@puff\space\the\c@pgf@counta}{%
        \expandafter\xdef\csname pgf@anchor@cloud@puff\space\the\c@pgf@counta\endcsname{%
          \noexpand\pgf@sh@@cloudpuffanchor{\the\c@pgf@counta}%
        }%
      }{\c@pgf@counta0\relax}%
      \advance\c@pgf@counta-1\relax%
    \repeatpgfmathloop%
  }%
}%

% \pgf@sh@@cloudpuffanchor
%
% Internal macro for calculating the anchors puff 1, puff 2, ... etc.
%
\def\pgf@sh@@cloudpuffanchor#1{%
    \getradii%
    \pgfmathdivide@{\anglestep}{2}%
    \let\halfanglestep\pgfmathresult%
    \c@pgf@counta#1\relax%
    \advance\c@pgf@counta-1\relax%
    \pgfmathmultiply@{\anglestep}{\the\c@pgf@counta}%
    \pgfmathadd@{\pgfmathresult}{90}%
    \pgfmathsubtract@{\pgfmathresult}{\halfanglestep}%
    \let\angle\pgfmathresult%
    %
    % Calculate the first arc point.
    %
    \pgfextract@process\arcstartpoint{%
      \pgfpointadd{\centerpoint}{%
        \pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
      }%
    }%
    %
    \pgfmathadd@{\angle}{\anglestep}%
    \let\angle\pgfmathresult%
    \pgfextract@process\arcendpoint{%
      \pgfpointadd{\centerpoint}{%
        \pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
      }%
    }%
    %
    % Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
    %
    \pgf@sh@getcloudpuffparameters%
    %
    % Calculate the point.
    %
    \pgfmathadd@{\arcslope}{90}%
    \let\anchorangle\pgfmathresult%
    \pgfpointadd{\circlecenterpoint}{%
      \pgfqpointpolar{\anchorangle}{\outerarcradius}%
    }%
}%

% \pgf@sh@cloudpuffparameters
%
% Internal macro to calculate some common arc parameters which
% are required when calculating radii, drawing the background
% path and calculating border anchors.
%
\def\pgf@sh@getcloudpuffparameters{%
  %
  % Calculate the angle to which the entire arc is sloped.
  %
  \pgfmathanglebetweenpoints{\arcendpoint}{\arcstartpoint}%
  \let\arcslope\pgfmathresult%
  %
  % Calculate the chord length and arc radius.
  %
  \pgfpointdiff{\arcendpoint}{\arcstartpoint}%
  \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}
  \pgf@x\pgfmathresult pt\relax%
  \pgf@xa.5\pgf@x%
  \edef\halfchordlength{\the\pgf@xa}%
  \pgf@x\arcradiusquotient\pgf@x%
  \edef\arcradius{\the\pgf@x}%
  \pgf@xa\outersep\relax%
  \advance\pgf@xa\pgf@x%
  \edef\outerarcradius{\the\pgf@xa}%
  %
  % Calculate the height of the resulting segment.
  %
  \pgf@y-\sinhalfcomplementarc\pgf@x% sin((180-a)/2)
  \advance\pgf@y\pgf@x%
  \edef\segmentheight{\the\pgf@y}%
  %
  % Calculate the center of the circle of which the arc is a part.
  %
  \pgfextract@process\circlecenterpoint{%
    \pgfextract@process\circlecenterpoint{%
      \pgf@x-\halfchordlength\relax%
      \pgf@y\segmentheight\relax%
      \advance\pgf@y-\arcradius
    }%
    \pgfpointadd{\arcstartpoint}{%
      \pgfmathrotatepointaround{\circlecenterpoint}{\pgfpointorigin}{\arcslope}%
    }%
  }%
}%





% Internal macros for signal shape.
%
\def\pgf@lib@sh@signal@nowhere{nowhere}%
\def\pgf@lib@sh@signal@from{from}%
\def\pgf@lib@sh@signal@to{to}%

\def\pgf@lib@sh@signal@parsedirection#1#2{%
  %
  \let\pgf@lib@sh@signal@direction=#2%
  \edef\pgf@lib@sh@temp{#1}%
  \expandafter\pgf@lib@sh@signal@@parsedirection\pgf@lib@sh@temp\pgf@stop}%

\def\pgf@lib@sh@signal@@parsedirection#1\pgf@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@%
    \pgf@lib@sh@signal@@@parsedirection#1\pgf@lib%
  \else%
    \pgf@lib@sh@signal@@@parsedirection#1 and #1\pgf@lib%
  \fi
}%
\def\pgf@lib@sh@signal@@@parsedirection#1 and #2\pgf@lib{%
  \pgfutil@in@{nowhere}{#1}%
  \ifpgfutil@in@
  \else%
    \pgf@lib@sh@signal@@@@parsedirection{#1}%
    \pgf@lib@sh@signal@@@@parsedirection{#2}%
  \fi%
}%
\def\pgf@lib@sh@signal@@@@parsedirection#1{%
  \pgfutil@in@{ #1 }{ east right }%
  \ifpgfutil@in@%
    \let\pgf@lib@sh@signal@east=\pgf@lib@sh@signal@direction%
    \let\pgf@lib@sh@signal@north=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@south=\pgf@lib@sh@signal@nowhere%
  \fi%
  \pgfutil@in@{ #1 }{ left west }%
  \ifpgfutil@in@%
    \let\pgf@lib@sh@signal@west=\pgf@lib@sh@signal@direction%
    \let\pgf@lib@sh@signal@north=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@south=\pgf@lib@sh@signal@nowhere%
  \fi%
  \pgfutil@in@{ #1 }{ above up north }%
  \ifpgfutil@in@%
    \let\pgf@lib@sh@signal@north=\pgf@lib@sh@signal@direction%
    \let\pgf@lib@sh@signal@east=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@west=\pgf@lib@sh@signal@nowhere%
  \fi%
  \pgfutil@in@{ #1 }{ below down south }%
  \ifpgfutil@in@%
    \let\pgf@lib@sh@signal@south=\pgf@lib@sh@signal@direction%
    \let\pgf@lib@sh@signal@east=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@west=\pgf@lib@sh@signal@nowhere%
  \fi%
}%


% Keys for signal shape:
%
\pgfkeys{/pgf/.cd,
  signal pointer angle/.initial=90,
  signal to/.initial=east,
  signal from/.initial=nowhere,
}%

\pgfdeclareshape{signal}{%
  \savedmacro\installsignalparameters{%
    %
    \let\pgf@lib@sh@signal@north=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@south=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@east=\pgf@lib@sh@signal@nowhere%
    \let\pgf@lib@sh@signal@west=\pgf@lib@sh@signal@nowhere%
    %
    \pgf@lib@sh@signal@parsedirection{\pgfkeysvalueof{/pgf/signal from}}{\pgf@lib@sh@signal@from}%
    \pgf@lib@sh@signal@parsedirection{\pgfkeysvalueof{/pgf/signal to}}{\pgf@lib@sh@signal@to}%
    %
    % Define a centerpoint.
    %
    \pgfextract@process\centerpoint{%
      \pgf@x.5\wd\pgfnodeparttextbox%
      \pgf@y.5\ht\pgfnodeparttextbox%
      \advance\pgf@y-.5\dp\pgfnodeparttextbox%
    }%
    %
    % Get some useful trig. stuff
    %
    \pgfmathsetmacro\pointerangle{\pgfkeysvalueof{/pgf/signal pointer angle}}%
    %
    \pgfmathdivide@{\pointerangle}{2}%
    \let\halfpointerangle=\pgfmathresult%
    %
    \pgfmathcosec@{\halfpointerangle}%
    \let\cosechalfpointerangle=\pgfmathresult%
    %
    \pgfmathdivide@{\halfpointerangle}{2}%
    \let\quarterpointerangle=\pgfmathresult%
    %
    \pgfmathcosec@{\quarterpointerangle}%
    \let\cosecquarterpointerangle=\pgfmathresult%
    %
    \pgfmathsec@{\quarterpointerangle}%
    \let\secquarterpointerangle=\pgfmathresult%
    %
    \pgfmathsubtract@{90}{\quarterpointerangle}%
    \let\complementquarterpointerangle\pgfmathresult%
    %
    % Get the larger of the outer sep.
    %
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@x>\pgf@y%
      \pgf@y\pgf@x%
    \fi%
    \pgf@yc=\pgf@y%
    %
    % Calculate the miter due to the line width, at the pointer apex...
    %
    \pgf@x=\cosechalfpointerangle\pgf@y%
    \edef\pointerapexmiter{\the\pgf@x}%
    %
    % ...at a corner by a `to' pointer (i.e. sticks out)...
    %
    \pgf@x=\secquarterpointerangle\pgf@y%
    \edef\tocornermiter{\the\pgf@x}%
    %
    % ...at a corner by a `from' pointer (i.e. sticks in).
    %
    \pgf@x=\cosecquarterpointerangle\pgf@y
    \edef\fromcornermiter{\the\pgf@x}%
    %
    % Get the (half) dimensions of the node.
    %
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya.5\dp\pgfnodeparttextbox%
    %
    % Get the distance a pointer sticks out to the side...
    %
    \pgfmathsubtract@{90}{\halfpointerangle}%
    \pgfmathtan@{\pgfmathresult}%
    \pgf@xb=\pgfmathresult\pgf@ya%
    %
    % ...and up.
    %
    \pgf@yb=\pgfmathresult\pgf@xa%
    %
    % Adjust for minimum height.
    %
    \pgfutil@tempdima=2.0\pgf@ya%
    \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@nowhere%
    \else%
      \advance\pgfutil@tempdima by\pgf@yb%
    \fi%
    \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@nowhere%
    \else%
      \advance\pgfutil@tempdima by\pgf@yb%
    \fi%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgfutil@tempdima<\pgf@y%
      \pgfutil@tempdima=\pgf@y%
      %
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@nowhere%
      \else%
        \advance\pgfutil@tempdima by-\pgf@yb%
      \fi%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@nowhere%
      \else%
        \advance\pgfutil@tempdima by-\pgf@yb%
      \fi%
      \pgf@ya=0.5\pgfutil@tempdima%
      \pgfmathsubtract@{90}{\halfpointerangle}%
      \pgfmathtan@{\pgfmathresult}%
      \pgf@xb=\pgfmathresult\pgf@ya%
    \fi%
    %
    % Adjust for minimum width.
    %
    \pgfutil@tempdima=2.0\pgf@xa%
    \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@nowhere%
    \else%
      \advance\pgfutil@tempdima by\pgf@xb%
    \fi%
    \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@nowhere%
    \else%
      \advance\pgfutil@tempdima by\pgf@xb%
    \fi%
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgfutil@tempdima<\pgf@x%
      \pgfutil@tempdima=\pgf@x%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@nowhere%
      \else%
        \advance\pgfutil@tempdima by-\pgf@xb%
      \fi%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@nowhere%
      \else%
        \advance\pgfutil@tempdima by-\pgf@xb%
      \fi%
      \pgf@xa=0.5\pgfutil@tempdima%
      \pgfmathsubtract@{90}{\halfpointerangle}%
      \pgfmathtan@{\pgfmathresult}%
      \pgf@yb=\pgfmathresult\pgf@xa%
    \fi%
    %
    % So, define the points for the background path.
    %
    \pgfextract@process\north{%
      \centerpoint%
      \advance\pgf@y\pgf@ya%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@to%
        \advance\pgf@y\pgf@yb%
      \fi%
    }%
    \pgfextract@process\south{%
      \centerpoint%
      \advance\pgf@y-\pgf@ya%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@to%
        \advance\pgf@y-\pgf@yb%
      \fi%
    }%
    \pgfextract@process\east{%
      \centerpoint%
      \advance\pgf@x\pgf@xa%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@to%
        \advance\pgf@x\pgf@xb%
      \fi%
    }%
    \pgfextract@process\west{%
      \centerpoint%
      \advance\pgf@x-\pgf@xa%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@to%
        \advance\pgf@x-\pgf@xb%
      \fi%
    }%
    \pgfextract@process\northeast{%
      \centerpoint%
      \advance\pgf@y\pgf@ya%
      \advance\pgf@x\pgf@xa%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@from%
        \advance\pgf@y\pgf@yb%
      \fi%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@from%
        \advance\pgf@x\pgf@xb%
      \fi%
    }%
    \pgfextract@process\southeast{%
      \centerpoint%
      \advance\pgf@y-\pgf@ya%
      \advance\pgf@x\pgf@xa%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@from%
        \advance\pgf@y-\pgf@yb%
      \fi%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@from%
        \advance\pgf@x\pgf@xb%
      \fi%
    }%
    \pgfextract@process\southwest{%
      \centerpoint%
      \advance\pgf@y-\pgf@ya%
      \advance\pgf@x-\pgf@xa%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@from%
        \advance\pgf@y-\pgf@yb%
      \fi%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@from%
        \advance\pgf@x-\pgf@xb%
      \fi%
    }%
    \pgfextract@process\northwest{%
      \centerpoint%
      \advance\pgf@y\pgf@ya%
      \advance\pgf@x-\pgf@xa%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@from%
        \advance\pgf@y\pgf@yb%
      \fi%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@from%
        \advance\pgf@x-\pgf@xb%
      \fi%
    }%
    \addtosavedmacro{\north}%
    \addtosavedmacro{\south}%
    \addtosavedmacro{\east}%
    \addtosavedmacro{\west}%
    \addtosavedmacro{\northeast}%
    \addtosavedmacro{\southwest}%
    \addtosavedmacro{\southeast}%
    \addtosavedmacro{\northwest}%
    %
    % Calculate the `miter vectors' (i.e. +outer sep).
    %
    \pgfextract@process\northmiter{%
      \pgf@x0pt%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@nowhere%
        \pgf@y\pgf@yc%
      \else%
        \pgf@y\pointerapexmiter\relax%
      \fi%
    }%
    \pgfextract@process\southmiter{%
      \pgf@x0pt%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@nowhere%
        \pgf@y-\pgf@yc%
      \else%
        \pgf@y-\pointerapexmiter\relax%
      \fi%
    }%
    \pgfextract@process\eastmiter{%
      \pgf@y0pt%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@nowhere%
        \pgf@x\pgf@yc%
      \else%
        \pgf@x\pointerapexmiter\relax%
      \fi%
    }%
    \pgfextract@process\westmiter{%
      \pgf@y0pt%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@nowhere%
        \pgf@x-\pgf@yc%
      \else%
        \pgf@x-\pointerapexmiter\relax%
      \fi%
    }%
    \pgfextract@process\northeastmiter{%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@nowhere%
        \pgf@x\pgf@yc
        \pgf@y\pgf@yc%
      \else
        \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@from%
          \pgfqpointpolar{\quarterpointerangle}{\fromcornermiter}
        \else%
          \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@to%
            \pgfqpointpolar{\complementquarterpointerangle}{\tocornermiter}%
          \fi%
        \fi%
      \fi%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@from%
        \pgfqpointpolar{\complementquarterpointerangle}{\fromcornermiter}%
      \else%
        \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@to%
          \pgfqpointpolar{\quarterpointerangle}{\tocornermiter}%
        \fi%
      \fi%
    }%
    \pgfextract@process\southeastmiter{%
      \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@nowhere%
        \pgf@x\pgf@yc%
        \pgf@y\pgf@yc%
      \else
        \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@from%
          \pgfqpointpolar{-\quarterpointerangle}{\fromcornermiter}
        \else%
          \ifx\pgf@lib@sh@signal@east\pgf@lib@sh@signal@to%
            \pgfqpointpolar{-\complementquarterpointerangle}{\tocornermiter}%
          \fi%
        \fi%
      \fi%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@from%
        \pgfqpointpolar{-\complementquarterpointerangle}{\fromcornermiter}
      \else%
        \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@to%
          \pgfqpointpolar{-\quarterpointerangle}{\tocornermiter}%
        \fi%
      \fi%
    }%
    \pgfextract@process\southwestmiter{%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@nowhere%
        \pgf@x-\pgf@yc
        \pgf@y-\pgf@yc%
      \else
        \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@from%
          \pgfmathadd@{\quarterpointerangle}{180}%
          \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}
        \else%
          \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@to%
            \pgfmathadd@{\complementquarterpointerangle}{180}%
            \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
          \fi%
        \fi%
      \fi%
      \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@from%
        \pgfmathadd@{\complementquarterpointerangle}{180}%
        \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}%
      \else%
        \ifx\pgf@lib@sh@signal@south\pgf@lib@sh@signal@to%
          \pgfmathadd@{\quarterpointerangle}{180}%
          \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
        \fi%
      \fi%
    }%
    \pgfextract@process\northwestmiter{%
      \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@nowhere%
        \pgf@x-\pgf@yc%
        \pgf@y\pgf@yc%
      \else
        \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@from%
          \pgfmathsubtract@{180}{\quarterpointerangle}%
          \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}
        \else%
          \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@to%
            \pgfmathsubtract@{180}{\complementquarterpointerangle}%
            \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
          \fi%
        \fi%
      \fi%
      \ifx\pgf@lib@sh@signal@north\pgf@lib@sh@signal@from%
        \pgfmathsubtract@{180}{\complementquarterpointerangle}%
        \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}%
      \else%
        \ifx\pgf@lib@sh@signal@west\pgf@lib@sh@signal@to%
          \pgfmathsubtract@{180}{\quarterpointerangle}%
          \expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
        \fi%
      \fi%
    }%
    \addtosavedmacro{\northmiter}%
    \addtosavedmacro{\southmiter}%
    \addtosavedmacro{\eastmiter}%
    \addtosavedmacro{\westmiter}%
    \addtosavedmacro{\northeastmiter}%
    \addtosavedmacro{\southeastmiter}%
    \addtosavedmacro{\southwestmiter}%
    \addtosavedmacro{\northwestmiter}%
    %
    % Now calculate the anchor points
    %
    \pgfextract@process\anchornorth{%
      \pgfpointadd{\north}{\northmiter}%
    }%
    \pgfextract@process\anchorsouth{%
      \pgfpointadd{\south}{\southmiter}%
    }%
    \pgfextract@process\anchoreast{%
      \pgfpointadd{\east}{\eastmiter}%
    }%
    \pgfextract@process\anchorwest{%
      \pgfpointadd{\west}{\westmiter}%
    }%
    \pgfextract@process\anchornortheast{%
      \pgfpointadd{\northeast}{\northeastmiter}%
    }%
    \pgfextract@process\anchorsoutheast{%
      \pgfpointadd{\southeast}{\southeastmiter}%
    }%
    \pgfextract@process\anchorsouthwest{%
      \pgfpointadd{\southwest}{\southwestmiter}%
    }%
    \pgfextract@process\anchornorthwest{%
      \pgfpointadd{\northwest}{\northwestmiter}%
    }%
    \addtosavedmacro{\anchornorth}%
    \addtosavedmacro{\anchorsouth}%
    \addtosavedmacro{\anchoreast}%
    \addtosavedmacro{\anchorwest}%
    \addtosavedmacro{\anchornortheast}%
    \addtosavedmacro{\anchorsouthwest}%
    \addtosavedmacro{\anchorsoutheast}%
    \addtosavedmacro{\anchornorthwest}%
  }%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+.5ex}%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
    \installsignalparameters%
    \anchoreast%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \anchorsoutheast%
    \ifdim\pgf@xa>\pgf@x%
      \pgfutil@tempdima\pgf@xa%
    \else%
      \pgfutil@tempdima\pgf@x%
    \fi%
    \pgfextract@process\externalpoint{%
      \basepoint%
      \pgf@x\pgfutil@tempdima%
    }
    \basepoint%
    \let\firstpoint\anchoreast%
    \ifdim\pgf@y<\pgf@ya%
      \let\secondpoint\anchorsoutheast%
    \else%
      \let\secondpoint\anchornortheast%
    \fi%
    \pgfpointintersectionoflines{\basepoint}{\externalpoint}%
      {\firstpoint}{\secondpoint}%
  }%
  \anchor{base west}{%
    \installsignalparameters%
    \anchorwest%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \anchorsouthwest%
    \ifdim\pgf@xa<\pgf@x%
      \pgfutil@tempdima\pgf@xa%
    \else%
      \pgfutil@tempdima\pgf@x%
    \fi%
    \pgfextract@process\externalpoint{%
      \basepoint%
      \pgf@x\pgfutil@tempdima%
    }
    \basepoint%
    \let\firstpoint\anchorwest%
    \ifdim\pgf@y<\pgf@ya%
      \let\secondpoint\anchorsouthwest%
    \else%
      \let\secondpoint\anchornorthwest%
    \fi%
    \pgfpointintersectionoflines{\basepoint}{\externalpoint}%
      {\firstpoint}{\secondpoint}%
  }%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
    \installsignalparameters%
    \anchoreast%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \anchorsoutheast%
    \ifdim\pgf@xa>\pgf@x%
      \pgfutil@tempdima\pgf@xa%
    \else%
      \pgfutil@tempdima\pgf@x%
    \fi%
    \pgfextract@process\externalpoint{%
      \midpoint%
      \pgf@x\pgfutil@tempdima%
    }
    \midpoint%
    \let\firstpoint\anchoreast%
    \ifdim\pgf@y<\pgf@ya%
      \let\secondpoint\anchorsoutheast%
    \else%
      \let\secondpoint\anchornortheast%
    \fi%
    \pgfpointintersectionoflines{\midpoint}{\externalpoint}%
      {\firstpoint}{\secondpoint}%
  }%
  \anchor{mid west}{%
    \installsignalparameters%
    \anchorwest%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \anchorsouthwest%
    \ifdim\pgf@xa<\pgf@x%
      \pgfutil@tempdima\pgf@xa%
    \else%
      \pgfutil@tempdima\pgf@x%
    \fi%
    \pgfextract@process\externalpoint{%
      \midpoint%
      \pgf@x\pgfutil@tempdima%
    }
    \midpoint%
    \let\firstpoint\anchorwest%
    \ifdim\pgf@y<\pgf@ya%
      \let\secondpoint\anchorsouthwest%
    \else%
      \let\secondpoint\anchornorthwest%
    \fi%
    \pgfpointintersectionoflines{\midpoint}{\externalpoint}%
      {\firstpoint}{\secondpoint}%
  }%
  \anchor{north}{\installsignalparameters\anchornorth}%
  \anchor{south}{\installsignalparameters\anchorsouth}%
  \anchor{east}{\installsignalparameters\anchoreast}%
  \anchor{west}{\installsignalparameters\anchorwest}%
  \anchor{north east}{\installsignalparameters\anchornortheast}%
  \anchor{south east}{\installsignalparameters\anchorsoutheast}%
  \anchor{south west}{\installsignalparameters\anchorsouthwest}%
  \anchor{north west}{\installsignalparameters\anchornorthwest}%
  \backgroundpath{%
    \installsignalparameters%
    \pgfpathmoveto{\north}%
    \pgfpathlineto{\northeast}%
    \pgfpathlineto{\east}%
    \pgfpathlineto{\southeast}%
    \pgfpathlineto{\south}%
    \pgfpathlineto{\southwest}%
    \pgfpathlineto{\west}%
    \pgfpathlineto{\northwest}%
    \pgfpathclose%
  }%
  \anchorborder{%
    %
    % Save x and y.
    %
    \edef\externalx{\the\pgf@x}%
    \edef\externaly{\the\pgf@y}%
    %
    % Adjust the location of the external
    % point relative to \centerpoint.
    %
    \centerpoint%
    \pgf@xa\externalx\relax%
    \pgf@ya\externaly\relax%
    \advance\pgf@xa\pgf@x%
    \advance\pgf@ya\pgf@y%
    \edef\externalx{\the\pgf@xa}%
    \edef\externaly{\the\pgf@ya}%
    %
    % Get the shape parameters.
    %
    \installsignalparameters%
    %
    % Get the angle of the external point to the \centerpoint.
    %
    \pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
    \let\externalangle\pgfmathresult%
    %
    %
    %
    \pgfmathanglebetweenpoints{\centerpoint}{\anchorwest}%
    \ifdim\externalangle pt<\pgfmathresult pt\relax%
      \pgfmathanglebetweenpoints{\centerpoint}{\anchornorth}%
      \ifdim\externalangle pt<\pgfmathresult pt\relax%
        \pgfmathanglebetweenpoints{\centerpoint}{\anchornortheast}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
          \let\firstpoint\anchoreast%
          \let\secondpoint\anchornortheast%
        \else%
          \let\secondpoint\anchornortheast%
          \let\firstpoint\anchornorth%
        \fi%
      \else%
        \pgfmathanglebetweenpoints{\centerpoint}{\anchornorthwest}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
          \let\firstpoint\anchornorth%
          \let\secondpoint\anchornorthwest%
        \else%
          \let\secondpoint\anchornorthwest%
          \let\firstpoint\anchorwest%
        \fi%
      \fi%
    \else%
      \pgfmathanglebetweenpoints{\centerpoint}{\anchorsouth}%
      \ifdim\externalangle pt<\pgfmathresult pt\relax%
        \pgfmathanglebetweenpoints{\centerpoint}{\anchorsouthwest}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
          \let\firstpoint\anchorwest%
          \let\secondpoint\anchorsouthwest%
        \else%
          \let\secondpoint\anchorsouthwest%
          \let\firstpoint\anchorsouth%
        \fi%
      \else%
        \pgfmathanglebetweenpoints{\centerpoint}{\anchorsoutheast}%
        \ifdim\externalangle pt<\pgfmathresult pt\relax%
          \let\firstpoint\anchorsouth%
          \let\secondpoint\anchorsoutheast%
        \else%
          \let\secondpoint\anchorsoutheast%
          \let\firstpoint\anchoreast%
        \fi%
      \fi%
    \fi%
    %
    % Now locate the point.
    %
    \pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
      {\firstpoint}{\secondpoint}%
  }%
}%






% Keys for shape tape
%
% /pgf/tape bend top : Type of bend for north side.
% /pgf/tape bend bottom : Type of bend for south side.
% /pgf/tape bend height : The height of the bends.
\pgfkeys{/pgf/.cd,
  tape bend top/.initial=in and out,
  tape bend bottom/.initial=in and out,
  tape bend/.style={/pgf/tape bend top=#1, /pgf/tape bend bottom=#1},
  tape bend height/.initial=5pt,
}%

\def\pgf@lib@sh@inandouttext{in and out}%
\def\pgf@lib@sh@outandintext{out and in}%
\def\pgf@lib@sh@nonetext{none}%

\pgfdeclareshape{tape}{%
  \savedmacro\tapedimensions{%
    \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y.5\dp\pgfnodeparttextbox%
    %
    \pgfmathsetlengthmacro\outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlengthmacro\outerysep{\pgfkeysvalueof{/pgf/outer ysep}}%
    \addtosavedmacro\outerxsep%
    \addtosavedmacro\outerysep%
    %
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/tape bend height}}%
    \pgfutil@tempdima.5\pgfutil@tempdima%
    \edef\halfbendheight{\the\pgfutil@tempdima}%
    \addtosavedmacro\halfbendheight%
    %
    \pgfkeysgetvalue{/pgf/tape bend top}{\topbendstyle}%
    \pgfkeysgetvalue{/pgf/tape bend bottom}{\bottombendstyle}%
    \addtosavedmacro\topbendstyle%
    \addtosavedmacro\bottombendstyle%
    %
    \ifx\topbendstyle\pgf@lib@sh@nonetext%
    \else%
      \advance\pgf@y\pgfutil@tempdima%
    \fi%
    \ifx\bottombendstyle\pgf@lib@sh@none%
    \else%
      \advance\pgf@y\pgfutil@tempdima%
    \fi%
    %
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xa%
      \pgf@x.5\pgf@xa%
    \fi%
    \ifdim\pgf@y<.5\pgf@ya%
      \pgf@y.5\pgf@ya%
    \fi%
    \ifx\topbendstyle\pgf@lib@sh@nonetext%
    \else%
      \advance\pgf@y-\pgfutil@tempdima%
    \fi%
    \ifx\bottombendstyle\pgf@lib@sh@nonetext%
    \else%
      \advance\pgf@y-\pgfutil@tempdima%
    \fi%
    %
    \pgfutil@tempdima3.414213\pgfutil@tempdima% 1 / (1-sin(45))
    \edef\bendyradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\bendyradius%
    \advance\pgfutil@tempdima\outerysep%
    \edef\outerbendyradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\outerbendyradius%
    \advance\pgfutil@tempdima-\outerysep%
    \advance\pgfutil@tempdima-\outerysep%
    \edef\innerbendyradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\innerbendyradius%
    %
    \pgfutil@tempdima0.707106\pgf@x% cos(45)
    \edef\bendxradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\bendxradius%
    \advance\pgfutil@tempdima\outerxsep%
    \edef\outerbendxradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\outerbendxradius%
    \advance\pgfutil@tempdima-\outerxsep%
    \advance\pgfutil@tempdima-\outerxsep%
    \edef\innerbendxradius{\the\pgfutil@tempdima}%
    \addtosavedmacro\innerbendxradius%
    %
    \edef\halfwidth{\the\pgf@x}%
    \edef\halfheight{\the\pgf@y}%
    \addtosavedmacro\halfwidth%
    \addtosavedmacro\halfheight%
    %
    \advance\pgf@x\outerxsep%
    \edef\outerhalfwidth{\the\pgf@x}%
    \addtosavedmacro\outerhalfwidth%
    %
    \pgf@xc\bendxradius%
    \pgf@yc\bendyradius%
    \pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@xc}}%
    \pgfmathatan{\pgfmathresult}%
    \pgf@xc\pgfmathresult pt\relax%
    \pgf@xc.5\pgf@xc%
    \edef\halfangle{\pgfmath@tonumber{\pgf@xc}}%
    \addtosavedmacro\halfangle%
    %
    \pgf@xc45pt\relax%
    \advance\pgf@xc-\halfangle pt%
    \pgfmathcot@{\pgfmath@tonumber{\pgf@xc}}%
    \let\cothalfanglein\pgfmathresult%
    \addtosavedmacro\cothalfanglein%
    %
    \pgf@xc90pt\relax%
    \advance\pgf@xc-\halfangle pt%
    \pgfmathcot@{\pgfmath@tonumber{\pgf@xc}}%
    \let\cothalfangleout\pgfmathresult%
    \addtosavedmacro\cothalfangleout%
    %
  }%
  \savedanchor{\centerpoint}{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }%
    \savedanchor{\midpoint}{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+0.5ex}%
  }%
  \savedanchor{\basepoint}{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt%
  }%
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{\tapedimensions\midpoint\advance\pgf@x\outerhalfwidth}%
  \anchor{mid west}{\tapedimensions\midpoint\advance\pgf@x-\outerhalfwidth}%
  \anchor{base}{\basepoint}%
  \anchor{base east}{\tapedimensions\basepoint\advance\pgf@x\outerhalfwidth}%
  \anchor{base west}{\tapedimensions\basepoint\advance\pgf@x-\outerhalfwidth}%
  \anchor{north}{%
    \csname pgf@anchor@tape@north east\endcsname%
    \pgf@ya\pgf@y%
    \csname pgf@anchor@tape@north west\endcsname%
    \advance\pgf@ya\pgf@y%
    \centerpoint%
    \pgf@y.5\pgf@ya%
  }%
  \anchor{south}{%
    \csname pgf@anchor@tape@south east\endcsname%
    \pgf@ya\pgf@y%
    \csname pgf@anchor@tape@south west\endcsname%
    \advance\pgf@ya\pgf@y%
    \centerpoint%
    \pgf@y.5\pgf@ya%
  }%
  \anchor{east}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x\outerhalfwidth%
  }%
  \anchor{west}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x-\outerhalfwidth%
  }%
  \anchor{north east}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x\outerhalfwidth%
    \advance\pgf@y\halfheight%
    \pgf@yc\outerysep%
    \ifx\topbendstyle\pgf@lib@sh@inandouttext%
      \advance\pgf@y\halfbendheight%
      \advance\pgf@y\cothalfangleout\pgf@yc%
    \else%
      \ifx\topbendstyle\pgf@lib@sh@outandintext%
        \advance\pgf@y\halfbendheight%
        \advance\pgf@y\cothalfanglein\pgf@yc%
      \else%
        \advance\pgf@y\pgf@yc%
      \fi%
    \fi%
  }%
  \anchor{north west}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x-\outerhalfwidth%
    \advance\pgf@y\halfheight%
    \pgf@yc\outerysep%
    \ifx\topbendstyle\pgf@lib@sh@inandouttext%
      \advance\pgf@y\halfbendheight%
      \advance\pgf@y\cothalfanglein\pgf@yc%
    \else%
      \ifx\topbendstyle\pgf@lib@sh@outandintext%
        \advance\pgf@y\halfbendheight%
        \advance\pgf@y\cothalfangleout\pgf@yc%
      \else%
        \advance\pgf@y\pgf@yc%
      \fi%
    \fi%
  }%
  \anchor{south east}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x\outerhalfwidth%
    \advance\pgf@y-\halfheight%
    \pgf@yc\outerysep%
    \ifx\topbendstyle\pgf@lib@sh@outandintext%
      \advance\pgf@y-\halfbendheight%
      \advance\pgf@y-\cothalfangleout\pgf@yc%
    \else%
      \ifx\topbendstyle\pgf@lib@sh@inandouttext%
        \advance\pgf@y-\halfbendheight%
        \advance\pgf@y-\cothalfanglein\pgf@yc%
      \else%
        \advance\pgf@y-\pgf@yc%
      \fi%
    \fi%
  }%
  \anchor{south west}{%
    \tapedimensions%
    \centerpoint%
    \advance\pgf@x-\outerhalfwidth%
    \advance\pgf@y-\halfheight%
    \pgf@yc\outerysep%
    \ifx\topbendstyle\pgf@lib@sh@outandintext%
      \advance\pgf@y-\halfbendheight%
      \advance\pgf@y-\cothalfanglein\pgf@yc%
    \else%
      \ifx\topbendstyle\pgf@lib@sh@inandouttext%
        \advance\pgf@y-\halfbendheight%
        \advance\pgf@y-\cothalfangleout\pgf@yc%
      \else%
        \advance\pgf@y-\pgf@yc%
      \fi%
    \fi%
  }%
  \backgroundpath{%
    \tapedimensions%
    %
    \pgf@xc\halfwidth%
    \pgf@yc\halfheight%
    %
    \pgf@xc\bendxradius%
    \pgf@yc\bendyradius%
    {%
      \pgftransformshift{\centerpoint}%
      \pgfpathmoveto{\pgfqpoint{-\halfwidth}{0pt}}%
      \pgfpathlineto{\pgfqpoint{-\halfwidth}{\halfheight}}%
      \ifx\topbendstyle\pgf@lib@sh@inandouttext%
        \pgfpathlineto{\pgf@x-\halfwidth\pgf@y\halfheight\advance\pgf@y\halfbendheight}%
        \pgfpatharc{225}{315}{\bendxradius and \bendyradius}%
        \pgfpatharc{135}{45}{\bendxradius and \bendyradius}%
      \else%
        \ifx\topbendstyle\pgf@lib@sh@outandintext%
          \pgfpathlineto{\pgf@x-\halfwidth\pgf@y\halfheight\advance\pgf@y\halfbendheight}%
          \pgfpatharc{135}{45}{\bendxradius and \bendyradius}%
          \pgfpatharc{225}{315}{\bendxradius and \bendyradius}%
        \else%
          \pgfpathlineto{\pgfqpoint{\halfwidth}{\halfheight}}%
        \fi%
      \fi%
      \pgfpathlineto{\pgfqpoint{\halfwidth}{-\halfheight}}%
      \ifx\bottombendstyle\pgf@lib@sh@inandouttext%
        \pgfpathlineto{\pgf@x\halfwidth\pgf@y-\halfheight\advance\pgf@y-\halfbendheight}%
        \pgfpatharc{45}{135}{\bendxradius and \bendyradius}%
        \pgfpatharc{315}{225}{\bendxradius and \bendyradius}%
      \else%
        \ifx\bottombendstyle\pgf@lib@sh@outandintext%
          \pgfpathlineto{\pgf@x\halfwidth\pgf@y-\halfheight\advance\pgf@y-\halfbendheight}%
          \pgfpatharc{315}{225}{\bendxradius and \bendyradius}%
          \pgfpatharc{45}{135}{\bendxradius and \bendyradius}%
        \else%
          \pgfpathlineto{\pgfqpoint{-\halfwidth}{-\halfheight}}%
        \fi%
      \fi%
      \pgfpathclose%
    }%
  }%
  \anchorborder{%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgfextract@process\externalpoint{%
      \centerpoint%
      \advance\pgf@x\pgf@xa%
      \advance\pgf@y\pgf@ya%
    }%
    \pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
    \let\externalangle\pgfmathresult%
    \tapedimensions%
    %
    \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@north west\endcsname}%
    \ifdim\externalangle pt<\pgfmathresult pt%
      \ifdim\externalangle pt<90pt%
        \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@north east\endcsname}%
        \ifdim\externalangle pt<\pgfmathresult pt%
          \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
            {\csname pgf@anchor@tape@north east\endcsname}%
            {\csname pgf@anchor@tape@south east\endcsname}%
        \else%
          % Between north and north east.
          \ifx\topbendstyle\pgf@lib@sh@inandouttext%
            % in and out.
            \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
            {%
              \centerpoint%
              \pgf@xc\halfwidth%
              \advance\pgf@x.5\pgf@xc%
              \advance\pgf@y\halfheight%
              \advance\pgf@y\halfbendheight%
              \pgf@yc\bendyradius%
              \advance\pgf@y-.707106\pgf@yc%
            }%
            {5}{175}{\outerbendxradius and \outerbendyradius}%
          \else%
            \ifx\topbendstyle\pgf@lib@sh@outandintext%
              % out and in.
              \pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
              {%
                \centerpoint%
                \pgf@xc\halfwidth%
                \advance\pgf@x.5\pgf@xc%
                \advance\pgf@y\halfheight%
                \advance\pgf@y\halfbendheight%
                \pgf@yc\bendyradius%
                \advance\pgf@y.707106\pgf@yc%
              }%
              {185}{355}{\innerbendxradius and \innerbendyradius}%
            \else%
              \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
                {\csname pgf@anchor@tape@north east\endcsname}%
                {\csname pgf@anchor@tape@north west\endcsname}%
            \fi%
          \fi%
        \fi%
      \else%
        % Between north and north west.
        \ifx\topbendstyle\pgf@lib@sh@inandouttext%
          % in and out.
          \pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
            {%
              \centerpoint%
              \pgf@xc\halfwidth%
              \advance\pgf@x-.5\pgf@xc%
              \advance\pgf@y\halfheight%
              \advance\pgf@y\halfbendheight%
              \pgf@yc\bendyradius%
              \advance\pgf@y.707106\pgf@yc%
            }%
            {185}{355}{\innerbendxradius and \innerbendyradius}%
        \else%
          \ifx\topbendstyle\pgf@lib@sh@outandintext%
            % out and in.
            \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
            {%
              \centerpoint%
              \pgf@xc\halfwidth%
              \advance\pgf@x-.5\pgf@xc%
              \advance\pgf@y\halfheight%
              \advance\pgf@y\halfbendheight%
              \pgf@yc\bendyradius%
              \advance\pgf@y-.707106\pgf@yc%
            }%
            {5}{175}{\outerbendxradius and \outerbendyradius}%
          \else%
            \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
              {\csname pgf@anchor@tape@north east\endcsname}%
              {\csname pgf@anchor@tape@north west\endcsname}%
          \fi%
        \fi%
      \fi%
    \else%
      \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@south west\endcsname}%
        \ifdim\externalangle pt>\pgfmathresult pt%
        \ifdim\externalangle pt>270pt%
          \pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@south east\endcsname}%
          \ifdim\externalangle pt>\pgfmathresult pt%
            \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
              {\csname pgf@anchor@tape@north east\endcsname}%
              {\csname pgf@anchor@tape@south east\endcsname}%
          \else%
            % Between south and south east.
            \ifx\bottombendstyle\pgf@lib@sh@inandouttext%
              % in and out.
              \pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
              {%
                \centerpoint%
                \pgf@xc\halfwidth%
                \advance\pgf@x.5\pgf@xc%
                \advance\pgf@y-\halfheight%
                \advance\pgf@y-\halfbendheight%
                \pgf@yc\bendyradius%
                \advance\pgf@y-.707106\pgf@yc%
              }%
              {5}{175}{\innerbendxradius and \innerbendyradius}%
            \else%
              \ifx\bottombendstyle\pgf@lib@sh@outandintext%
                % out and in.
                \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
              {%
                \centerpoint%
                \pgf@xc\halfwidth%
                \advance\pgf@x.5\pgf@xc%
                \advance\pgf@y-\halfheight%
                \advance\pgf@y-\halfbendheight%
                \pgf@yc\bendyradius%
                \advance\pgf@y.707106\pgf@yc%
              }%
              {185}{355}{\outerbendxradius and \outerbendyradius}%
              \else%
                \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
                  {\csname pgf@anchor@tape@south east\endcsname}%
                  {\csname pgf@anchor@tape@south west\endcsname}%
              \fi%
            \fi%
          \fi%
        \else%
          % Between south and south west.
          \ifx\bottombendstyle\pgf@lib@sh@inandouttext%
            % in and out.
            \pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
              {%
                \centerpoint%
                \pgf@xc\halfwidth%
                \advance\pgf@x-.5\pgf@xc%
                \advance\pgf@y-\halfheight%
                \advance\pgf@y-\halfbendheight%
                \pgf@yc\bendyradius%
                \advance\pgf@y.707106\pgf@yc%
              }%
              {185}{355}{\outerbendxradius and \outerbendyradius}%
          \else%
            \ifx\bottombendstyle\pgf@lib@sh@outandintext%
              % out and in.
              \pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
              {%
                \centerpoint%
                \pgf@xc\halfwidth%
                \advance\pgf@x-.5\pgf@xc%
                \advance\pgf@y-\halfheight%
                \advance\pgf@y-\halfbendheight%
                \pgf@yc\bendyradius%
                \advance\pgf@y-.707106\pgf@yc%
              }%
              {5}{175}{\innerbendxradius and \innerbendyradius}%
            \else%
              \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
                {\csname pgf@anchor@tape@south east\endcsname}%
                {\csname pgf@anchor@tape@south west\endcsname}%
            \fi%
          \fi%
        \fi%
      \else%
        \pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
          {\csname pgf@anchor@tape@north west\endcsname}%
          {\csname pgf@anchor@tape@south west\endcsname}%
      \fi%
    \fi%
  }%
}%




% Keys for magnifying glass shape
%
% /pgf/magnifying glass handle angle  : The angle of handle
% /pgf/magnifying glass handle aspect : The length of the handle as a multiple
%                               of the radius of the circle
%

\pgfkeys{/pgf/.cd,
  magnifying glass handle angle/.initial=-45,
  magnifying glass handle aspect/.initial=1.5,
}%

\pgfdeclareshape{magnifying glass}
{%
  \inheritsavedanchors[from=circle]% this is nearly a circle
  \inheritanchorborder[from=circle]%
  \inheritanchor[from=circle]{north}%
  \inheritanchor[from=circle]{north west}%
  \inheritanchor[from=circle]{north east}%
  \inheritanchor[from=circle]{center}%
  \inheritanchor[from=circle]{west}%
  \inheritanchor[from=circle]{east}%
  \inheritanchor[from=circle]{mid}%
  \inheritanchor[from=circle]{mid west}%
  \inheritanchor[from=circle]{mid east}%
  \inheritanchor[from=circle]{base}%
  \inheritanchor[from=circle]{base west}%
  \inheritanchor[from=circle]{base east}%
  \inheritanchor[from=circle]{south}%
  \inheritanchor[from=circle]{south west}%
  \inheritanchor[from=circle]{south east}%
  \inheritbackgroundpath[from=circle]%
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}
      {\pgfpointpolar{\pgfkeysvalueof{/pgf/magnifying glass handle angle}}{\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}
      {\pgfpointpolar{\pgfkeysvalueof{/pgf/magnifying glass handle angle}}{\pgfutil@tempdima+\pgfutil@tempdima*(\pgfkeysvalueof{/pgf/magnifying glass handle aspect})}}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
  }%
}%


\pgfkeys{%
  /pgf/magnetic tape tail/.initial=0.15,
  /pgf/magnetic tape tail extend/.initial=0cm,
}%
\pgfdeclareshape{magnetic tape}{%
  \nodeparts{text}%
  \savedmacro\installparameters{%
    %
    \pgf@x=0.5\wd\pgfnodeparttextbox%
    \pgf@y=0.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-0.5\dp\pgfnodeparttextbox%
    \edef\centerpoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    %
    \pgf@x=\wd\pgfnodeparttextbox%
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@x by2.0\pgf@xa%
    \advance\pgf@y by2.0\pgf@ya%
    \ifdim\pgf@y>\pgf@x%
      \pgf@x=\pgf@y%
    \fi%
    \pgf@x=1.414213\pgf@x%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<\pgf@xa%
      \pgf@x=\pgf@xa%
    \fi%
    \ifdim\pgf@x<\pgf@ya%
      \pgf@x=\pgf@ya%
    \fi%
    \pgf@x=0.5\pgf@x%
    \edef\radius{\the\pgf@x}%
    %
    \pgfmathparse{max(\pgfkeysvalueof{/pgf/magnetic tape tail extend},0)}%
    \edef\tailextend{\pgfmathresult pt}%
    %
    \pgfmathparse{min(max(\pgfkeysvalueof{/pgf/magnetic tape tail},0),1)}%
    \pgf@xa=\pgfmathresult\pgf@x%
    \edef\tailheight{\the\pgf@xa}%
    %
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xa<\pgf@ya%
      \pgf@xa=\pgf@ya%
    \fi%
    \edef\outersep{\the\pgf@xa}%
    %
    \pgfmathparse{\outersep+\radius}%
    \edef\outerradius{\pgfmathresult pt}%
    %
    \pgfmathparse{(\radius-\tailheight)/\radius}%
    \pgfmathasin@{\pgfmathresult}%
    \pgfmathadd@{-\pgfmathresult}{360}%
    \let\tailangle=\pgfmathresult%
    %
    \pgfmathparse{\outerradius/(\outerradius+\tailextend)}%
    \pgfmathatan@{\pgfmathresult}%
    \pgfmathadd@{-\pgfmathresult}{360}%
    \let\tailbottomangle=\pgfmathresult%
    %
    \pgfmathparse{(\outerradius-\outersep-\tailheight-\outersep)/(\outerradius+\tailextend)}%
    \pgfmathatan@{\pgfmathresult}%
    \pgfmathadd@{-\pgfmathresult}{360}%
    \let\tailtopangle=\pgfmathresult%
    %
    \addtosavedmacro\radius%
    \addtosavedmacro\outerradius%
    \addtosavedmacro\outersep%
    \addtosavedmacro\tailheight%
    \addtosavedmacro\tailextend
    \addtosavedmacro\tailangle%
    \addtosavedmacro\tailtopangle%
    \addtosavedmacro\tailbottomangle%
    \addtosavedmacro\centerpoint%
  }%
  \savedanchor{\base}{\pgfqpoint{0.5\wd\pgfnodeparttextbox}{0pt}}%
  \savedanchor{\mid}{\pgfqpoint{0.5\wd\pgfnodeparttextbox}{0pt}\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{center}{\installparameters\centerpoint}%  \addtosavedmacro\outerradius%
  \anchor{base}{\base}%
  \anchor{mid}{\mid}%
  \anchor{base west}{\installparameters\pgfpointadd{\base}{\pgfqpoint{-\outerradius}{0pt}}}%
  \anchor{base east}{\installparameters\pgfpointadd{\base}{\pgfqpoint{\outerradius}{0pt}}}%
  \anchor{mid west}{\installparameters\pgfpointadd{\mid}{\pgfqpoint{-\outerradius}{0pt}}}%
  \anchor{mid east}{\installparameters\pgfpointadd{\mid}{\pgfqpoint{\outerradius}{0pt}}}%
  \anchor{north}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpoint{0pt}{\outerradius}}}%
  \anchor{north east}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpointpolar{45}{\outerradius}}}%
  \anchor{south}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpoint{0pt}{-\outerradius}}}%
  \anchor{south east}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpoint{\outerradius}{-\outerradius}}}%
  \anchor{east}{\installparameters%
      \pgfpointadd{\centerpoint}{\pgfqpoint{\outerradius}{0pt}}}%
  \anchor{south west}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpointpolar{225}{\outerradius}}}%
  \anchor{west}{\installparameters%
    \pgfpointadd{\centerpoint}{\pgfqpoint{-\outerradius}{0pt}}}%
  \anchor{north west}{\installparameters%
      \pgfpointadd{\centerpoint}{\pgfqpointpolar{135}{\outerradius}}}%
  \anchor{tail east}{\installparameters%
        \pgfpointadd{\centerpoint}{\pgfpoint{\radius+\tailextend+\outersep}{-\outerradius+\outersep+\tailheight/2}}}%
  \anchor{tail south east}{\installparameters%
          \pgfpointadd{\centerpoint}{\pgfpoint{\radius+\tailextend+\outersep}{-\outerradius}}}%
  \anchor{tail north east}{\installparameters%
            \pgfpointadd{\centerpoint}{\pgfpoint{\radius+\tailextend+\outersep}{-\outerradius+\outersep+\tailheight+\outersep}}}%
  \backgroundpath{
  %
    \installparameters%
    {%
    \pgftransformshift{\centerpoint}%
    \pgfpathmoveto{\pgfpointpolar{\tailangle}{\radius}}%
    \pgfpatharc{\tailangle}{360}{\radius}%
    \pgfpatharc{0}{270}{\radius}%
    \pgfpathlineto{\pgfpoint{\radius+\tailextend}{-\radius}}%
    \pgfpathlineto{\pgfpoint{\radius+\tailextend}{-\radius+\tailheight}}%
    \pgfpathclose%
    }%
  }%
  \anchorborder{%
    \pgfextract@process\externalpoint{}%
    \installparameters%
    \pgfmathanglebetweenpoints{\pgfpointorigin}{\externalpoint}
    \ifdim\pgfmathresult pt<270pt\relax%
      \pgfpointadd{\centerpoint}{%
        \pgfpointborderellipse%
          {\externalpoint}%
          {\pgfqpoint{\outerradius}{\outerradius}}%
      }%
    \else%
      \ifdim\pgfmathresult pt<\tailbottomangle pt\relax%
        \pgfpointadd{\centerpoint}{%
          \pgfpointintersectionoflines%
            {\externalpoint}{\pgfpointorigin}%
            {\pgfqpoint{0pt}{-\outerradius}}{\pgfqpoint{\outerradius}{-\outerradius}}%
        }%
      \else%
        \ifdim\pgfmathresult pt<\tailtopangle pt\relax%
          \pgfpointadd{\centerpoint}{%
            \pgfpointintersectionoflines%
              {\externalpoint}{\pgfpointorigin}%
              {\pgfqpoint{\outerradius}{\outerradius}}{\pgfqpoint{\outerradius}{-\outerradius}}%
          }%
        \else%
          \pgfpointadd{\centerpoint}{%
            \pgfpointborderellipse%
              {\externalpoint}%
              {\pgfqpoint{\outerradius}{\outerradius}}%
            }%
        \fi%
      \fi%
    \fi%
  }%
}%

% Local Variables:
% tab-width: 2
% End:


==> pgfmath.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% Guard against reading twice
\ifx\pgfmathloaded\pgfutil@undefined
  \let\pgfmathloaded=\relax
\else
  \expandafter\endinput
\fi

% We need keys:
\ifx\pgfkeysloaded\pgfutil@undefined
  \input pgfkeys.code.tex
\fi

\input pgfmathcalc.code.tex
\input pgfmathfloat.code.tex

\endinput


==> pgfmathcalc.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file loads all the parsing, functions and operator stuff
%
% Version 1.414213 29/9/2007

\input pgfmathutil.code.tex
\input pgfmathparser.code.tex
\input pgfmathfunctions.code.tex
%\input pgfmathbase.code.tex

% \pgfmathsetlength, \pgfmathaddtolength
%
% #1 = dimension register
% #2 = expression
%
% Description:
%
% These functions work similar to \setlength and \addtolength. Only,
% they allow #2 to contain an expression, which is evaluated before
% assignment. Furthermore, the font is setup before the assignment is
% done, so that dimensions like 1em are evaluated correctly.
%
% If #2 starts with "+", then a simple assignment is done (but the
% font is still setup). This is orders of magnitude faster than a
% parsed assignment.

\def\pgfmathsetlength#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    % Ok, quick version:
    \begingroup%
      \pgfmath@selectfont%
      #1#2\unskip%
    \expandafter\endgroup%
    \expandafter#1\the#1\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \ifpgfmathmathunitsdeclared%
      #1\pgfmathresult mu\relax%
    \else%
      #1\pgfmathresult pt\relax%
    \fi%
  }%
  \ignorespaces%
}

% \pgfmathaddtolength
%
% Add to #1 the result of evaluating #2.
%
% #1 - a dimension register
% #2 - an expression
%
\def\pgfmathaddtolength#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \begingroup%
      \pgfmath@selectfont%
      \advance#1#2\unskip%
      \expandafter%
    \endgroup%
    \expandafter#1\the#1\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \ifpgfmathmathunitsdeclared%
      \advance#1\pgfmathresult mu\relax%
    \else%
      \advance#1\pgfmathresult pt\relax%
    \fi%
  }%
  \ignorespaces%
}

% \pgfmathsetcount
%
% Assign #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathsetcount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1#2\relax\pgfmath@%
  }%
  {%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
  }%
  \ignorespaces%
}

% \pgfmathaddtocount
%
% Add to #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathaddtocount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1#2\relax\pgfmath@%
    \advance#1\pgfmath@addtocounttemp\relax%
  }%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
    \advance#1\pgfmath@addtocounttemp\relax%
  }%
  \ignorespaces%
}

% \pgfmathnewcounter
%
% LaTeX style counter which also works in plain TeX. Defines
% \c@<name> as a count register and also defines \the<name>.
%
% #1 the name of the counter.
%
% Example:
%
% \pgfmathnewcounter{counter}
% \pgfmathsetcounter{counter}{12}
% \thecounter  (same as \the\c@counter)
%
\def\pgfmathnewcounter#1{%
  \expandafter\ifx\csname c@#1\endcsname\relax%
    \def\pgfmath@marshal{\csname newcount\endcsname}% Ha! Who cares about \outer?
    \expandafter\pgfmath@marshal\csname c@#1\endcsname%
    \expandafter\def\csname the#1\endcsname{\expandafter\the\csname c@#1\endcsname}%
  \fi%
}

% \pgfmathsetcounter
%
% Set the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathsetcounter#1#2{%
   \expandafter\pgfmathsetcount\csname c@#1\endcsname{#2}%
}

% \pgfmathaddtocounter
%
% Add the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathaddtocounter#1#2{%
  \expandafter\pgfmathaddtocount\csname c@#1\endcsname{#2}%
}

% \pgfmathmakecounterglobal
%
% Make the current value of a counter globally defined.
%
% #1 - a (valid) counter name.
%
\def\pgfmath@pgftext{pgf}
\def\pgfmath@tikztext{tikz}
\def\pgfmathmakecounterglobal#1{%
  \pgfmath@ifundefined{c@#1}{}{%
    \expandafter\pgfmath@in@\expandafter{\pgfmath@pgftext}{#1}%
    \ifpgfmath@in@%
    \else%
      \expandafter\pgfmath@in@\expandafter{\pgfmath@tikztext}{#1}%
      \ifpgfmath@in@%
      \else%
        \expandafter\global\csname c@#1\endcsname\csname c@#1\endcsname\relax%
      \fi%
    \fi%
  }%
}

% \pgfmathsetmacro
%
% \edef#1 as the result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetmacro#1#2{%
  \begingroup%
    \pgfmathparse{#2}%
    \let#1=\pgfmathresult
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% \pgfmathsetlengthmacro
%
% \edef#1 as the result of evaluating #2 with pt.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetlengthmacro#1#2{%
  \begingroup%
    \pgfmathsetlength\pgfmath@x{#2}%
    \edef#1{\the\pgfmath@x}%
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% \pgfmathtruncatemacro
%
% \edef#1 as the truncated result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathtruncatemacro#1#2{%
  \begingroup%
    \pgfmathsetcount\c@pgfmath@counta{#2}%
    \edef#1{\the\c@pgfmath@counta}%
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% Check whether a given parameter starts with quick.
%
% The command should be followed by nonempty text, ending with
% \pgfmath@ as a stop-token. Then should follow
%
% #1 - code to execute if text starts with +
% #2 - code to execute if text does not
%
% Example:
%
% \pgfmath@onquick+0pt\pgfmath@{is quick}{is slow}

\def\pgfmath@onquick{%
  \futurelet\pgfmath@next%
  \pgfmath@@onquick}
\def\pgfmath@@onquick#1\pgfmath@{%
  \ifx\pgfmath@next+%
    \let\pgfmath@next=\pgfmath@firstoftwo%
  \else%
    \let\pgfmath@next=\pgfmath@secondoftwo%
  \fi%
  \pgfmath@next%
}

% *** The following commands DO NOT WORK without the rest of PGF ***
%
% (a dumping ground for stuff that doesn't really belong anywhere else)

% \pgfmathanglebetweenpoints
%
% Define \pgfmathresult as the angle between points #1 and #2
% Should get the quadrants right as well.
%
\def\pgfmathanglebetweenpoints#1#2{%
  \begingroup%
    \pgf@process{\pgfpointdiff{#1}{#2}}%
    \edef\pgf@marshall{\expandafter\noexpand\csname pgfmathatan2@\endcsname{\expandafter\Pgf@geT\the\pgf@y}{\expandafter\Pgf@geT\the\pgf@x}}%
    \pgf@marshall%
    \ifdim\pgfmathresult pt<0pt%
      \pgfmathparse{\pgfmathresult+360}%
    \fi%
    \expandafter%
  \endgroup\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult}%
}

%
% \pgfmathrotatepointaround
%
% Rotate point #1 about point #2 by #3 degrees.
%
\def\pgfmathrotatepointaround#1#2#3{%
  \pgf@process{%
    \pgf@process{#1}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@process{#2}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \advance\pgf@x-\pgf@xa%
    \advance\pgf@y-\pgf@ya%
    \pgfmathsetmacro\angle{#3}%
    \pgfmathsin@{\angle}%
    \let\sineangle\pgfmathresult%
    \pgfmathcos@{\angle}%
    \let\cosineangle\pgfmathresult%
    \pgf@xa\cosineangle\pgf@x%
    \advance\pgf@xa-\sineangle\pgf@y%
    \pgf@ya\sineangle\pgf@x%
    \advance\pgf@ya\cosineangle\pgf@y%
    \pgf@x\pgf@xb%
    \pgf@y\pgf@yb%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
  }%
}

% \pgfmathanglebetweenlines
%
% Calculate the clockwise angle between a line from point #1
% to point #2 and a line from #3 to point #4.
%
\def\pgfmathanglebetweenlines#1#2#3#4{%
  \begingroup%
    \pgfmathanglebetweenpoints{#1}{#2}%
    \let\firstangle\pgfmathresult%
    \pgfmathanglebetweenpoints{#3}{#4}%
    \let\secondangle\pgfmathresult%
    \ifdim\firstangle pt>\secondangle pt\relax%
      \pgfmathadd@{\secondangle}{360}%
      \let\secondangle\pgfmathresult%
    \fi%
    \pgfmathsubtract@{\secondangle}{\firstangle}%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% \pgfmathpointreflectalongaxis
%
% Reflects point #1 around an axis centered on #2 at an angle #3.
%
\def\pgfmathreflectpointalongaxis#1#2#3{%
  \pgf@process{%
    \pgfmathanglebetweenpoints{#2}{#1}%
    \pgfmath@tempdima\pgfmathresult pt\relax%
    \pgfmathparse{#3}%
    \advance\pgfmath@tempdima-\pgfmathresult pt\relax%
    \pgfmath@tempdima-2.0\pgfmath@tempdima%
    \pgfmathrotatepointaround{#1}{#2}{\pgfmath@tonumber{\pgfmath@tempdima}}%
  }%
}



% \pgfmathpointintersectionoflineandarc
%
% A bit experimental at the moment:
%
% Locates the point where a line crosses an eliptical arc. If the line
% does not cross the arc, a meaningless point will result.
%
% #1 the point of the line on the "convex" side of the arc.
% #2 the point of the line on the "concave" side of the arc.
% #3 the center of the eliptical arc.
% #4 start angle of the arc.
% #5 end angle of the arc.
% #6 radii of the arc.
%
\def\pgfmathpointintersectionoflineandarc#1#2#3#4#5#6{%
  \pgf@process{%
    %
    % Get the required angle.
    %
    \pgfmathanglebetweenpoints{#2}{#1}%
    \let\x\pgfmathresult%
    %
    % Get the radii of the arc.
    %
    \pgfmath@in@{and }{#6}%
    \ifpgfmath@in@%
      \pgf@polar@#6\@@%
    \else%
      \pgf@polar@#6 and #6\@@%
    \fi%
    \edef\xarcradius{\the\pgf@x}%
    \edef\yarcradius{\the\pgf@y}%
     %
    % Get the start and end angles of the arc...
    %
    \pgfmathsetmacro\s{#4}%
    \pgfmathsetmacro\e{#5}%
    %
    % ...and also with rounding.
    %
    \pgfmathmod@{\s}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\ss\pgfmathresult%
    \pgfmathmod@{\e}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\ee\pgfmathresult%
    %
    % Hackery for when arc straddles zero.
    %
    \ifdim\ee pt<\ss pt\relax%
      \pgfmathadd@{\x}{180}%
      \pgfmathmod@{\pgfmathresult}{360}%
      \let\x\pgfmathresult%
    \fi%
    \def\m{360}% Measure of nearness.
    \pgfmathadd@{\s}{\e}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\n\pgfmathresult% The best estimate (default to middle of arc).
    \pgfmathloop%
      \pgfmathadd@{\s}{\e}%
      \pgfmathdivide@{\pgfmathresult}{2}%
      \let\p\pgfmathresult%
      \ifdim\p pt=\s pt\relax%
      \else%
        \pgfmathanglebetweenpoints{#2}{%
          \pgfpointadd{#3}{%
            \pgf@x\xarcradius\relax%
            \pgfmathcos@{\p}%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y\yarcradius\relax%
            \pgfmathsin@{\p}%
            \pgf@y\pgfmathresult\pgf@y%
          }%
        }%
        %
        % Hackery for when arc straddles zero.
        %
        \ifdim\ee pt<\ss pt\relax%
          \pgfmathadd@{\pgfmathresult}{180}%
          \pgfmathmod@{\pgfmathresult}{360}%
        \fi%
        \let\q\pgfmathresult%
        %
        % More hackery...
        %
        \ifdim\x pt>335pt\relax%
          \ifdim\q pt<45pt\relax%
            \pgfmathadd@{\q}{360}%
            \let\q\pgfmathresult%
          \fi%
        \fi%
        \ifdim\x pt=\q pt% Found it!
            \pgfmathbreakloop% Breaks after current iteration is complete.
          \else
            \ifdim\x pt<\q pt\relax%
              \let\e\p%
            \else%
              \let\s\p%
            \fi%
          \fi%
          \pgfmathsubtract@{\x}{\q}%
          \pgfmathabs@{\pgfmathresult}%
          %
          % Save the estimate if it is better than any previous estimate.
          %
          \ifdim\pgfmathresult pt<\m pt\relax%
            \let\m\pgfmathresult%
            \let\n\p%
          \fi%
    \repeatpgfmathloop%
    \pgfpointadd{#3}{\pgfpointpolar{\n}{\xarcradius and \yarcradius}}%
  }%
}

% \pgfmathangleonellipse
%
% Find the angle corresponding to a point on the border of an ellispe.
%
% #1 - the point on the border.
% #2 - the radii of the ellipse.
%
\def\pgfmathangleonellipse#1#2{%
  \begingroup%
    \pgfmath@in@{and }{#2}%
    \ifpgfmath@in@%
      \pgf@polar@#2\@@%
    \else%
      \pgf@polar@#2 and #2\@@%
    \fi%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@process{#1}%
    \ifdim\pgf@x=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else%
      \pgfutil@tempdima\pgf@x%
      \pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgfutil@tempdima}}%
      \pgfutil@tempdima\pgfmathresult pt\relax%
    \fi%
    \ifdim\pgf@y=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else%
      \pgfmathdivide@{\pgfmath@tonumber{\pgf@y}}{\pgfmath@tonumber{\pgf@ya}}%
      \pgfutil@tempdima\pgfmathresult\pgfutil@tempdima%
      \pgfmathatan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
    \fi%
    %
    \pgfutil@tempdima\pgfmathresult pt\relax%
    \ifdim\pgfutil@tempdima<0pt\relax%
      \advance\pgfutil@tempdima360pt\relax%
    \fi%
    \ifdim\pgf@x<0pt\relax%
      \ifdim\pgf@y=0pt\relax%
        \pgfutil@tempdima180pt\relax%
      \else%
        \ifdim\pgf@y<0pt\relax%
          \advance\pgfutil@tempdima180pt\relax%
        \else%
          \advance\pgfutil@tempdima-180pt\relax%
        \fi%
      \fi%
    \else%
      \ifdim\pgf@x=0pt\relax%
        \ifdim\pgf@y<0pt\relax%
          \pgfutil@tempdima270pt\relax%
        \else%
          \pgfutil@tempdima90pt\relax%
        \fi%
      \else%
        \ifdim\pgf@y=0pt\relax%
          \pgfutil@tempdima0pt\relax%
        \fi%
      \fi%
    \fi%
    \pgfmath@returnone\pgfutil@tempdima%
  \endgroup%
}


% Local Variables:
% tab-width: 2
% End:


==> pgfmathfloat.code.tex <==
% Copyright 2019 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file contains methods for basic floating point arithmetics, rounding
% to arbitrary precision and number pretty printing.
%


\pgfkeys{
    % The bug 3430171 (wrong minus sign spacing in pgfmathprintnumber)
    % has been fixed in 2.10 CVS. Since it changes the spacing, its
    % effects can be undone with this compatibility switch.
    /pgf/compat/number printer/.is choice,
    /pgf/compat/number printer/2.10/.code={%
        \def\pgfmathprintnumber@begingroup{\bgroup}%
        \def\pgfmathprintnumber@endgroup{\egroup}%
    },
    % I do not know the version number of the next release at this
    % time. Please be so kind and KEEP THIS NAME INTACT. Add an alias
    % if needed.
    /pgf/compat/number printer/next after 2.10/.code={%
        \def\pgfmathprintnumber@begingroup{\begingroup}%
        \def\pgfmathprintnumber@endgroup{\endgroup}%
    },
    % activate the fix by default.
    /pgf/compat/number printer/next after 2.10,%
}


\global\newif\ifpgfmathfloatcomparison
\newif\ifpgfmathfloatroundhasperiod
\newif\ifpgfmathprintnumberskipzeroperiod


% used internally in grouped macros:
\toksdef\pgfmathfloat@tmptoks=1
\newif\ifpgfmathfloat@fixed@digits@after@period
\newif\ifpgfmathfloatroundmayneedrenormalize
\toksdef\pgfmathfloat@a@Mtok=0

%% WARNING: avoid conflicting register names!
\let\pgfmathfloat@a@S=\c@pgf@counta
\let\pgfmathfloat@a@M=\pgf@xa
\let\pgfmathfloat@a@E=\c@pgf@countb
\let\pgfmathfloat@b@S=\c@pgf@countc
\let\pgfmathfloat@b@M=\pgf@xb
\let\pgfmathfloat@b@E=\c@pgf@countd

% can be changed with options.
\def\pgfmathfloat@round@precision{2}

% I introduced this to access the "original" precision in case a
% formatted changes it locally... in this case, the formatter may
% overwrite \pgfmathfloat@round@precision@orig to provide the original
% one.
% The default implementation here does nothing:
\def\pgfmathfloat@round@precision@orig{\pgfmathfloat@round@precision}%

\gdef\pgfmathfloat@glob@TMP{}


% Computes a normalised floating point representation for #1 of the
% form
%   [FLAGS] MANTISSE EXPONENT
% meaning
%   [+-]X.XXXXXXX*10^C
% where
%   X.XXXXXX is a mantissa with first number != 0, C is an integer and
% FLAGS contains the sign and some other special cases.
%
% This method does NOT use TeX Registers to represent the numbers! The
% computation is COMPLETELY STRING BASED.
% This allows numbers such at 10000000 or 5.23e-10 to be represented
% properly, although TeX-registers would produce overflow/underflow
% errors in these cases.
%
% It is to be used to compute logs, because log(X*10^Y) = log(X) + log(10)*Y
%
% Arguments:
% #1:  an arbitrary number which shall be parsed. Maybe a macro.
%     Examples:
%     [+-]XXXXX.XXXXXX
%     [+-]XXXXX.XXXXXXeXXXX
%     [+-]0.0000XXXXXX
%     [+-]0.0000XXXXXXeXXXX
%     [+-]inf
%     nan
%    Maybe a macro containing such a number.
%
% Return value:
% \pgfmathresult will be \def'ed to
%  FLAGS MANTISSE 'e' EXPONENT
% where
% FLAGS is a number in [0-5] where
%     0 == '0' (the number is +- 0.0),
%     1 == '+',
%     2 == '-',
%     3 == 'not a number'
%     4 == '+ infinity'
%     5 == '- infinity'
%
% MANTISSE is a normalised number 1 <= M < 10. It always contains a
% period and at least one digit after the period.
%
% EXPONENT is an integer value.
%
% Example:
% \pgfmathfloatparsenumber{1}
% -> \pgfmathresult = 11.0e0
% \pgfmathfloatparsenumber{141.212}
% -> \pgfmathresult = 11.41212e2
\def\pgfmathfloatparsenumber#1{%
    \begingroup
    \edef\pgfmathresult{#1}%
    \expandafter\pgfflt@impl\pgfmathresult\pgfflt@EOI
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.0}%
    \fi
    \pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% The same as \pgfmathfloatparsenumber, but does not perform sanity checking.
% FIXME: there is no longer any difference here.
\let\pgfmathfloatqparsenumber=\pgfmathfloatparsenumber

% Takes a floating point number #1 as input and writes flags to count
% register #2, mantissa to dimen register #3 and exponent to count
% register #4.
\def\pgfmathfloattoregisters#1#2#3#4{%
    \expandafter\pgfmathfloat@decompose#1\relax{#2}{#3}{#4}%
}

% the same, but writes the mantissa into a token register.
\def\pgfmathfloattoregisterstok#1#2#3#4{%
    \expandafter\pgfmathfloat@decompose@tok#1\relax{#2}{#3}{#4}%
}

% Extracts the flags of #1 into the count register #2.
\def\pgfmathfloatgetflags#1#2{%
    \expandafter\pgfmathfloat@decompose@F#1\relax{#2}%
}
% Extracts the flags of #1 into the macro #2.
\def\pgfmathfloatgetflagstomacro#1#2{%
    \expandafter\pgfmathfloat@decompose@Fmacro#1\relax{#2}%
}%

% Extracts the mantissa of #1 into the dimen register #2.
\def\pgfmathfloatgetmantissa#1#2{%
    \expandafter\pgfmathfloat@decompose@M#1\relax{#2}%
}
\let\pgfmathfloatgetmantisse=\pgfmathfloatgetmantissa
% Extracts the mantissa of #1 into the token register #2.
\def\pgfmathfloatgetmantissatok#1#2{%
    \expandafter\pgfmathfloat@decompose@Mtok#1\relax{#2}%
}
\let\pgfmathfloatgetmantissetok=\pgfmathfloatgetmantissatok
% Extracts the exponent of #1 into the count register #2.
\def\pgfmathfloatgetexponent#1#2{%
    \expandafter\pgfmathfloat@decompose@E#1\relax{#2}%
}


% Assigns \pgfmathresult to be a float encoded as
% <FLAGS><MANTISSE>e<EXPONENT>
%
% example:
% \pgfmathfloatcreate{1}{2.0}{10}
% \pgfmathfloat@to@FMeE@style\pgfmathresult
% ->
% \pgfmathresult is now '12.0e10' regardless of the internal float
% format.
\def\pgfmathfloat@to@FMeE@style#1{\expandafter\pgfmathfloat@to@FMeE@style@#1\relax\relax}%
\def\pgfmathfloat@to@FMeE@style@#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@to@FMeE@style@@%
    \else
        \expandafter\pgfmathfloat@to@FMeE@style@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@to@FMeE@style@@#1Y#2e#3]\relax\relax{\def\pgfmathresult{#1#2e#3}}%
\def\pgfmathfloat@to@FMeE@style@error#1\relax\relax{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%


% decomposes a lowlevel floating point representation into flags,
% mantissa and exponent.
%
% #4: integer register for the flags.
% #5: dimen registers for the mantissa.
% #6: integer register for the exponent.
%
% \expandafter\pgfmathfloat@decompose\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@M\pgfmathfloat@a@E
% -> the three temp registers contain flags, mantissa and exponent
\def\pgfmathfloat@decompose#1#2{% sanitize!
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@%
    \else
        \expandafter\pgfmathfloat@decompose@error%
    \fi
    #1#2%
}
\def\pgfmathfloat@decompose@#1Y#2e#3]\relax#4#5#6{%
   #4=#1\relax
   #5=#2pt % keep space here.
   #6=#3\relax%
}

% overloaded, #5 needs to be a token register for the mantissa.
% @see also \pgfmathfloatvalueof  which does also employ the load
% level repr.
% \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
% -> the three temp registers contain flags, mantissa and exponent
\def\pgfmathfloat@decompose@tok#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@tok@%
    \else
        \expandafter\pgfmathfloat@decompose@tok@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@tok@#1Y#2e#3]\relax#4#5#6{%
   #4=#1\relax
   #5={#2}%
   #6=#3\relax%
}
% overloaded, returns only ONE of the three components into #4:
% \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S
% -> \pgfmathfloat@a@S contains the flags field.
\def\pgfmathfloat@decompose@F#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@F@%
    \else
        \expandafter\pgfmathfloat@decompose@F@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@Fmacro#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@Fmacro@%
    \else
        \expandafter\pgfmathfloat@decompose@F@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@M#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@M@%
    \else
        \expandafter\pgfmathfloat@decompose@M@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@E#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@E@%
    \else
        \expandafter\pgfmathfloat@decompose@E@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@Mtok#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@Mtok@%
    \else
        \expandafter\pgfmathfloat@decompose@Mtok@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@F@#1Y#2e#3]\relax#4{#4=#1\relax}%
\def\pgfmathfloat@decompose@Fmacro@#1Y#2e#3]\relax#4{\def#4{#1}}%
\def\pgfmathfloat@decompose@M@#1Y#2e#3]\relax#4{#4=#2pt}%
\def\pgfmathfloat@decompose@Mtok@#1Y#2e#3]\relax#4{#4={#2}}%
\def\pgfmathfloat@decompose@E@#1Y#2e#3]\relax#4{#4=#3\relax}%

\def\pgfmathfloat@decompose@error#1\relax#2#3#4{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand#2=\the\pgfmathfloat@a@S\space
        \noexpand#3=\the\pgfmathfloat@a@Mtok pt
        \noexpand#4=\the\pgfmathfloat@a@E\space
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@tok@error#1\relax#2#3#4{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand#2=\the\pgfmathfloat@a@S\space
        \noexpand#3={\the\pgfmathfloat@a@Mtok}%
        \noexpand#4=\the\pgfmathfloat@a@E\space
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@F@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@S\space}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@M@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@Mtok pt }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@Mtok@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2={\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@E@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@E\space}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
% Takes a floating point number #1 as input and writes flags to macro
% #2, mantissa to macro #3 and exponent to macro #4.
\def\pgfmathfloattomacro#1#2#3#4{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\def\noexpand#2{\the\pgfmathfloat@a@S}%
        \noexpand\def\noexpand#3{\the\pgfmathfloat@a@Mtok}%
        \noexpand\def\noexpand#4{\the\pgfmathfloat@a@E}%
    }%
    \endgroup
    \pgfmathfloat@glob@TMP
}


% Defines \pgfmathresult as the floating point number encoded by
% the flags #1, mantissa #2 and exponent #3.
%
% All arguments are characters and will be expanded using '\edef'.
\def\pgfmathfloatcreate#1#2#3{%
    \edef\pgfmathresult{#1Y#2e#3]}%
}%
% This is the character present in any low-level floating point
% number. It is assumed to be the SECOND character of a float (after
% the flags integer).
\def\pgfmathfloat@POSTFLAGSCHAR{Y}



% Converts a composed floating point representation to fixed point.
%
% Example:
% \pgfmathfloattofixed{142e1}
% -> \pgfmathresult = 42.0
\def\pgfmathfloattofixed@#1{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifcase\pgfmathfloat@a@S
        \def\pgfmathresult{0.0}%
    \or
        \expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
    \or
        \expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
        \pgfmathfloat@a@Mtok=\expandafter{\pgfmathresult}%
        \edef\pgfmathresult{-\the\pgfmathfloat@a@Mtok}%
    \or\def\pgfmathresult{nan}%
    \or\def\pgfmathresult{inf}%
    \or\def\pgfmathresult{-inf}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\let\pgfmathfloattofixed=\pgfmathfloattofixed@

% Converts a float to an integer (in integer format).
%
% @see \pgfmathfloatint
\def\pgfmathfloattoint#1{%
    \pgfmathfloattofixed{#1}%
    \expandafter\pgfmathfloattoint@@\pgfmathresult\relax
}%
\def\pgfmathfloattoint@@#1.#2\relax{%
    \def\pgfmathresult{#1}%
}%

% Converts a floating point number to scientific format 1.234e5.
%
% This operation is very fast.
\def\pgfmathfloattosci@#1{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifcase\pgfmathfloat@a@S
        \def\pgfmathresult{0.0e0}%
    \or
        \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
    \or
        \edef\pgfmathresult{-\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
    \or\def\pgfmathresult{nan}%
    \or\def\pgfmathresult{inf}%
    \or\def\pgfmathresult{-inf}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%
\let\pgfmathfloattosci=\pgfmathfloattosci@

% Expands a floating point number to scientific format 1.234e5.
%
% This operation is very fast.
\def\pgfmathfloatvalueof#1{\expandafter\pgfmathfloatvalueof@@#1@@}%

% Make it fool proof such that the following arguments work:
%     \pgfmathfloatvalueof{1Y1.0e1} -> 1.0e1
%     \pgfmathfloatvalueof{2Y1.0e1} -> -1.0e1
% and wrong arguments as well:
%     \pgfmathfloatvalueof{1} -> 1
%     \pgfmathfloatvalueof{1e2} -> 1e2
\def\pgfmathfloatvalueof@@#1#2{%
    \if#2Y%
        % keep in mind that \pgfmathfloatvalueof should be expandable!
        % We must not use \let here. Let's hope that #1 and #2 are
        % single tokens (not something which was enclosed by curly
        % braces...)
        \expandafter\pgfmathfloatvalueof@@@\expandafter#1\expandafter#2%
    \else
        % Oh - no float!? Ok, we cannot report errors in this context.
        % So: make it a feature and return the input argument as-is.
        % Might be useful, in fact...
        \expandafter\pgfmathfloatvalueof@abort\expandafter#1\expandafter#2%
    \fi
}
\def\pgfmathfloatvalueof@@@#1Y#2e#3]@@{%
    \ifcase#1 %
        0.0e0%
    \or
        #2e#3%
    \or
        -#2e#3%
    \or nan%
    \or inf%
    \or -inf%
    \fi
}%
\def\pgfmathfloatvalueof@abort#1@@{#1}%



% Rounds a fixed point number #1 to \pgfmathfloat@round@precision digits precision and returns
% the result into \pgfmathresult.
%
% Any trailing zeros after the period are discarded.
% See \pgfmathroundtozerofill if you want trailing zeros and fixed
% width.
%
% This method is PURELY text based and can work with arbitrary
% precision (well, limited to TeX's stack size and integer size).
%
% Examples:
% \pgfmathroundto{1}
% -> \pgfmathresult = '1'
%
% \pgfmathroundto{19999.9996}
% -> \pgfmathresult = '20000'
%
% Arguments:
% #1 may be either a number or a macro (\pgfmathresult is allowed) expanding to a number.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundto#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodfalse
    \pgfmathroundto@impl{#1}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}


% Overloaded method.
%
% This variant always uses a FIXED number behind the period and fills
% in zeros if necessary.
% Examples:
% \pgfmathroundtozerofill{1}
% -> \pgfmathresult = '1.00'
%
% \pgfmathroundtozerofill{19999.9996}
% -> \pgfmathresult = '20000.00'
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundtozerofill#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodtrue
    \pgfmathroundto@impl{#1}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% see \pgfmathprintnumber@fixed@style for docs
\def\pgfmathprintnumber@fixed@styleDEFAULT#1#2#3e#4\relax{%
    \begingroup
    \pgfkeysgetvalue{/pgf/number format/set decimal separator}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP
    \pgfkeysgetvalue{/pgf/number format/@dec sep mark}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK
    \pgfkeysgetvalue{/pgf/number format/set thousands separator}\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP
    \c@pgf@counta=#4\relax % it is the exponent here.
    \ifnum#2=0
        \c@pgf@counta=0
    \fi
    \def\pgfmathresult{}%
    \ifpgfmathfloatroundhasperiod
        \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1\pgfmathfloat@EOI
    \else
        \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI%
        \begingroup
        \toks0=\expandafter{\pgfmathresult}%
        \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
        \endgroup
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1.#2\pgfmathfloat@EOI{%
    \ifpgfmathprintnumberskipzeroperiod
        \def\pgfmathfloat@loc@TMPb{#1}%
        \ifx\pgfmathfloatparsenumber@tok@ZERO\pgfmathfloat@loc@TMPb
        \else
            \def\pgfmathfloat@loc@TMPc{-0}%
            \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
                \def\pgfmathresult{-}%
            \else
                \def\pgfmathfloat@loc@TMPc{+0}%
                \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
                    \def\pgfmathresult{+}%
                \else
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
                \fi
            \fi
        \fi
    \else
        \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
    \fi
    \ifpgfmathprintnumber@thousand@sep@in@fractional
        \let\pgfmathresultfractional\pgfutil@empty%
        \pgfmathprintnumber@thousand@sep@in@fractional#2MMMM\@@
    \else
        \def\pgfmathresultfractional{#2}%
    \fi
    \begingroup
    \toks0=\expandafter{\pgfmathresult}%
    \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
    \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP}%
    \toks3=\expandafter{\pgfmathresultfractional}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 \the\toks3 }%
    \endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}%

% assigns \pgfmathresult such that it contains the formatted result.
% It assumes that none of the following tokens contains a period.
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod{%
    \ifx\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP\pgfutil@empty
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
    \else
        \ifnum\c@pgf@counta<0\relax % exponent of the number in this context
            \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
        \else
            \ifnum\c@pgf@counta<\pgfkeysvalueof{/pgf/number format/min exponent for 1000 sep}\relax
                \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
            \else
                \advance\c@pgf@counta by1 % counta:= total number of digits, N.
                \c@pgf@countb=\c@pgf@counta
                \divide\c@pgf@countb by3 %  countb := N DIV 3
                \c@pgf@countc=\c@pgf@countb
                \multiply\c@pgf@countc by3
                \advance\c@pgf@counta by-\c@pgf@countc% now counta := N MOD 3
                \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign
                }%
            \fi
        \fi
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign#1{%
    \def\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
        \let\pgfmathfloat@loc@TMPb=\pgfutil@empty
    \else
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
            \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
            \let\pgfmathfloat@loc@TMPb=\pgfutil@empty
        \else
            \ifpgfmathprintnumber@showpositive
                \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult +}%
            \fi
        \fi
    \fi
    \ifnum\c@pgf@counta>0 % \c@pgf@counta = N MOD 3 in this context
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits\pgfmathfloat@loc@TMPb
        }%
    \else
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird\pgfmathfloat@loc@TMPb
        }%
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits#1#2{%
    \ifcase\c@pgf@counta % = N MOD 3 in this context
        % does not happen per construction
    \or
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#2%
        }%
    \or
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2}%
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
        }%
    \fi
    \ifnum\c@pgf@countb>0\relax % \c@pgf@countb = N DIV 3 in this context
        \begingroup
        \toks0=\expandafter{\pgfmathresult}%
        \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
        \endgroup
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#1#2#3{%
    \ifnum\c@pgf@countb>0\relax
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2#3}%
        \advance\c@pgf@countb by-1
        \ifnum\c@pgf@countb>0\relax
            \begingroup
            \toks0=\expandafter{\pgfmathresult}%
            \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
            \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
            \endgroup
            \let\pgfmathresult=\pgfmathfloat@glob@TMP
        \fi
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
        }%
    \else
        % in this case, #1#2#3 are expected to be
        % \pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
        %--------------------------------------------------
        % \def\pgfmathfloat@loc@TMPb{\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI}%
        % \def\pgfmathfloat@loc@TMPc{#1#2#3}%
        % \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
        % \else
        %     \pgfmath@error{INTERNAL ERROR in fixed style - The input sequence did not terminate as expected; which indicates a wrong exponent argument provided to \string\pgfmathprintnumber@fixed@style}{}%
        % \fi
        %--------------------------------------------------
        \let\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT=\relax
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}

% \pgfmathprintnumber@thousand@sep@in@fractional 01234525MMMM\@@
% ->
% 012<sep>345<sep>25
\def\pgfmathprintnumber@thousand@sep@in@fractional#1#2#3#4{%
    \if#4M%
        % Ok, no further separator
        \def\pgfmathprint@next{\pgfmathprintnumber@thousand@sep@in@fractional@finish#1#2#3#4}%
    \else
        \begingroup
        \toks0=\expandafter{\pgfmathresultfractional}%
        \toks1={#1#2#3}%
        \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 }%
        \endgroup
        \let\pgfmathresultfractional=\pgfmathfloat@glob@TMP
        \def\pgfmathprint@next{\pgfmathprintnumber@thousand@sep@in@fractional#4}%
    \fi
    \pgfmathprint@next
}%
\def\pgfmathprintnumber@thousand@sep@in@fractional@finish#1M{%
    \expandafter\def\expandafter\pgfmathresultfractional\expandafter{\pgfmathresultfractional #1}%
    \pgfmathprintnumber@thousand@sep@in@fractional@finish@
}%
\def\pgfmathprintnumber@thousand@sep@in@fractional@finish@#1\@@{}%

\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall#1{%
    \def\pgfmathfloat@loc@TMPb{#1}%
    \let\pgfmathfloat@loc@TMPc=\pgfutil@empty
    \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
    \else
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
        \else
            \ifpgfmathprintnumber@showpositive
                \def\pgfmathfloat@loc@TMPc{+}%
            \fi
        \fi
    \fi
    \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@\pgfmathfloat@loc@TMPc#1%
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI{%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
}%

% @deprecated. It has been replaced by \pgfmathprintnumber@fixed@styleDEFAULT
% #1 maybe a macro
\def\pgfmathprintnumber@fixed@stylePERIOD#1#2#3e#4\relax{%
    \def\pgfmathresult{#1}%
}

% @deprecated. It has been replaced by \pgfmathprintnumber@fixed@styleDEFAULT
% #1 maybe a macro
\def\pgfmathprintnumber@fixed@styleCOMMA#1#2#3e#4\relax{%
    \ifpgfmathfloatroundhasperiod
        \expandafter\pgfmathprintnumber@fixed@styleCOMMA@impl#1\pgfmathfloat@EOI
    \else
        \def\pgfmathresult{#1}%
    \fi
}
\def\pgfmathprintnumber@fixed@styleCOMMA@impl#1.#2\pgfmathfloat@EOI{\def\pgfmathresult{#1{,}#2}}

% The default style to display fixed point numbers.
%
% It does not apply numerics, but it is responsible for typesetting the
% rounded number.
% It can access the \ifpgfmathfloatroundhasperiod boolean.
%
% Arguments:
% #1#2#3e#4\relax

% Input:
% #1  the fixed point number to be displayed (maybe a macro).
% #2#3e#4:  the (possibly unformatted) floating point representation
%     which belongs to #1. This format is returned (only!) by
%     \pgfmathfloat@to@FMeE@style.
%     It is used to determine sign and exponent.
\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT


% Rounds a normalized floating point number to \pgfmathfloat@round@precision
% digits precision and writes the result to \pgfmathresult.
%
% This method uses \pgfmathroundto for the mantissa.
%
% @see pgfmathfloatroundzerofill
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantissa #5 has a period or not.
\def\pgfmathfloatround#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodfalse
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \pgfmathfloatround@impl
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% Overload.
%
% This method uses a fixed width for the mantissa and fills in zeros
% if necessary.
%
% This method uses \pgfmathroundtozerofill for the mantissa.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantissa #5 has a period or not.
\def\pgfmathfloatroundzerofill#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodtrue
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \pgfmathfloatround@impl
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\newif\ifpgfmathfloatround@allow@empty@mantissa
\def\pgfmathfloatround@mantissa@ONE{1pt }%

% #1: sign
% #2: mantissa
% #3: exponent
% #4: CODE to display if the mantissa is drawn.
%     This code will be shown just before the exponent.
%     Example: #4=\cdot
% #5: CODE to display if the mantissa is NOT draw. (unused currently)
%     Might be used to display '10^1' instead of '1*10^1'.
% #6: CODE to display the exponent.
\def\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax#4#5#6{%
    \pgfkeysgetvalue{/pgf/number format/@sci exponent mark}\pgfmathfloatrounddisplaystyle@e@mark
    \ifcase#1\relax
        \pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
        \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
    \or
        \def\pgfmathfloat@loc@TMPa{1}% "should draw mantissa=1"
        \ifpgfmathfloatround@allow@empty@mantissa
        \else
            \ifdim#2pt=\pgfmathfloatround@mantissa@ONE
                \def\pgfmathfloat@loc@TMPa{0}% do not draw it.
            \fi
        \fi
        %
        \if1\pgfmathfloat@loc@TMPa
            \pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
            \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
        \else
            \def\pgfmathfloat@loc@TMPa{0}%
            \pgfmathfloatrounddisplaystyle@shared@impl@{#5}{#6}%
        \fi
    \or
        \def\pgfmathfloat@loc@TMPa{1}% "should draw mantissa=1"
        \ifpgfmathfloatround@allow@empty@mantissa
        \else
            \ifdim#2pt=\pgfmathfloatround@mantissa@ONE
                \def\pgfmathfloat@loc@TMPa{0}% do not draw it.
            \fi
        \fi
        %
        \if1\pgfmathfloat@loc@TMPa
            \pgfmathprintnumber@fixed@style{-#2}#1#2e0\relax%
            \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
        \else
            \def\pgfmathfloat@loc@TMPa{0}%
            \pgfmathfloatrounddisplaystyle@shared@impl@{-#5}{#6}%
        \fi
    \or
        \pgfmathfloatrounddisplaystyle@shared@impl@@{\hbox{NaN}}{}%
    \or
        \ifpgfmathprintnumber@showpositive
            \pgfmathfloatrounddisplaystyle@shared@impl@@{+\infty}{}%
        \else
            \pgfmathfloatrounddisplaystyle@shared@impl@@{\infty}{}%
        \fi
    \or
        \pgfmathfloatrounddisplaystyle@shared@impl@@{-\infty}{}%
    \fi
}

% #1: the part before the exponent code
% #2: the part for the exponent code.
\def\pgfmathfloatrounddisplaystyle@shared@impl@#1#2{%
    \pgfmathprintnumber@begingroup
    \toks0={#1}%
    \toks1=\expandafter{\pgfmathfloatrounddisplaystyle@e@mark #2}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
    \pgfmathprintnumber@endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}%
% Same as \pgfmathfloatrounddisplaystyle@shared@impl@, but it also
% inserts the '@dec sep mark' at the end.
\def\pgfmathfloatrounddisplaystyle@shared@impl@@#1#2{%
    \pgfmathprintnumber@begingroup
    \toks0={#1}%
    \toks1=\expandafter{\pgfmathfloatrounddisplaystyle@e@mark #2}%
    \pgfkeysgetvalue{/pgf/number format/@dec sep mark}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK
    \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 }%
    \pgfmathprintnumber@endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}

\def\pgfmathfloatrounddisplaystyle@std#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{\cdot}{}{10^{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@subscript#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}{_{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@superscript#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}{^{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@e#1#2e#3\relax{%
    \ifnum#3<0\relax
        \pgfmathprintnumber@begingroup
        \count0=#3\relax
        \multiply\count0 by-1
        \xdef\pgfmathfloat@glob@TMP{e{-}\the\count0}%
        \pgfmathprintnumber@endgroup%
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \else
        \def\pgfmathresult{e{+}#3}%
    \fi
    \def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
    \expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}
\def\pgfmathfloatrounddisplaystyle@E#1#2e#3\relax{%
    \ifnum#3<0\relax
        \pgfmathprintnumber@begingroup
        \count0=#3\relax
        \multiply\count0 by-1
        \xdef\pgfmathfloat@glob@TMP{E{-}\the\count0}%
        \pgfmathprintnumber@endgroup%
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \else
        \def\pgfmathresult{E{+}#3}%
    \fi
    \def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
    \expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}

\def\pgfmathfloatrounddisplaystyle@generic#1#2e#3\relax{%
    \begingroup
    \pgfkeysvalueof {/pgf/number format/sci generic/@/.@cmd}{#3}{#1}{#2}\pgfeov
    \pgfkeysgetvalue{/pgf/number format/sci generic/mantissa sep}\pgfmathdisplay@aftermantissa
    \pgfkeysgetvalue{/pgf/number format/sci generic/empty mantissa sep}\pgfmathdisplay@nomantissa
    \pgfkeysgetvalue{/pgf/number format/sci generic/exponent}\pgfmathdisplay@e
    \toks0=\expandafter{\pgfmathdisplay@aftermantissa}%
    \toks1=\expandafter{\pgfmathdisplay@nomantissa}%
    \toks2=\expandafter{\pgfmathdisplay@e}%
    \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\noexpand\relax{\the\toks0}{\the\toks1}{\the\toks2}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}

% A macro which takes the argument '<SIGN><MANTISSE>e<EXPONENT>' and
% expands to the final TeX-representation for that floating point
% number.
%
% PRECONDITION:
%   the floating point number has already been rounded properly and
%   the mantissa has been rounded correctly.
%
% The argument needs to be in the format returned by
% \pgfmathfloat@to@FMeE@style and terminated by '\relax'.
\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std
\newif\ifpgfmathfloat@usezerofill@sci
\newif\ifpgfmathfloat@usezerofill@fixed
\newif\ifpgfmathprintnumber@assumemathmode
\newif\ifpgfmathprintnumber@showpositive
\newif\ifpgfmathprintnumber@frac@warn
\newif\ifpgfmathprintnumber@frac@whole
\newif\ifpgfmathparsenumber@comma@as@period

\long\def\pgfmathfloatfrac@verbatim#1#2{#1/#2}%

\let\pgfmathround@@orig=\pgfmathround@

% 2 = compatible
% 0 = no
% 1 = yes
\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{2}%

\newif\ifpgfmathprintnumber@thousand@sep@in@fractional
\pgfkeys{%
    /pgf/number format/.is family,
    /pgf/number format,
    fixed/.code=           \pgfmath@set@number@printer{pgfmathprintnumber@FIXED},
    sci/.code=             \pgfmath@set@number@printer{pgfmathprintnumber@SCI},
    std/.code=             {\pgfmath@set@number@printer{pgfmathprintnumber@STD}\pgfmathprintnumber@STD@setparam{#1}},
    std/.default=,%
    relative round mode/.is choice,
    relative round mode/fixed/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{1}},
    relative round mode/mantissa/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{0}},
    relative round mode/compatible/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{2}},
    % relative={<exponent base 10>}
    relative/.code={%
        \pgfmath@set@number@printer{pgfmathprintnumber@RELATIVE}%
        \pgfmathround@@orig{#1}%
        \expandafter\pgfmathfloattoint@@\pgfmathresult\relax
        \let\pgfmathprintnumber@RELATIVE@param=\pgfmathresult
    },%
    relative/.value required,
    relative*/.style={/pgf/number format/relative={#1},/pgf/number format/relative round mode=fixed},
    every relative/.style=std,
    relative style/.style={/pgf/number format/every relative/.append style={#1}},
    fixed relative/.code=  \pgfmath@set@number@printer{pgfmathprintnumber@FIXED@RELATIVE},
    int detect/.code=      \pgfmath@set@number@printer{pgfmathprintnumber@INT@DETECT},
    int trunc/.code=       \pgfmath@set@number@printer{pgfmathprintnumber@INT@TRUNC},
    frac/.code=            \pgfmath@set@number@printer{pgfmathprintnumber@frac},%
    frac TeX/.initial=\frac,
    frac whole format/.code={\def\pgfmathresult{#1}},
    frac denom/.initial=,
    frac whole/.is if=pgfmathprintnumber@frac@whole,
    frac whole=true,
    frac shift/.initial=4,
    frac warning/.is if=pgfmathprintnumber@frac@warn,
    frac warning=true,
    assume math mode/.is if=pgfmathprintnumber@assumemathmode,
    assume math mode/.default=true,
    fixed zerofill/.is if= pgfmathfloat@usezerofill@fixed,
    fixed zerofill/.default=true,
    sci zerofill/.is if=   pgfmathfloat@usezerofill@sci,
    sci zerofill/.default=true,
    zerofill/.style=       {/pgf/number format/fixed zerofill=#1,/pgf/number format/sci zerofill=#1},
    zerofill/.default=     true,
    precision/.store in=   \pgfmathfloat@round@precision,
    sci precision/.code={%
        \edef\pgfmathfloat@loc@TMPa{#1}%
        \ifx\pgfmathfloat@loc@TMPa\pgfutil@empty
            \def\pgfmathprintnumber@sci@precision{\pgfmathfloat@round@precision}%
        \else
            \let\pgfmathprintnumber@sci@precision=\pgfmathfloat@loc@TMPa
        \fi
    },%
    sci precision/.default=,
    sci precision=,
    fixed default/.code=   {\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT},
    set decimal separator/.initial=,
    dec sep/.style={/pgf/number format/set decimal separator={#1}},
    @dec sep mark/.initial=,
    @sci exponent mark/.initial=,
    set thousands separator/.initial=,
    1000 sep in fractionals/.is if=pgfmathprintnumber@thousand@sep@in@fractional,
    1000 sep in fractionals/.default=true,
    1000 sep/.style={/pgf/number format/set thousands separator={#1}},
    min exponent for 1000 sep/.initial=0,
    use period/.style=     {/pgf/number format/set decimal separator={.},/pgf/number format/set thousands separator={{{,}}}},
    use comma/.style=      {/pgf/number format/set decimal separator={{{,}}},/pgf/number format/set thousands separator={.}},
    showpos/.is if=pgfmathprintnumber@showpositive,
    showpos/.default=true,
    print sign/.is if=pgfmathprintnumber@showpositive,
    print sign/.default=true,
    read comma as period/.is if=pgfmathparsenumber@comma@as@period,
    read comma as period/.default=true,
    skip 0./.is if=pgfmathprintnumberskipzeroperiod,
    skip 0./.default=true,
    skip 0.= false,
    use period,
    sci 10^e/.code=        {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
    sci 10e/.code=         {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
    sci e/.code=           {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@e},
    sci E/.code=           {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@E},
    sci subscript/.code=   {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@subscript},
    sci superscript/.code= {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@superscript},
    sci generic/.code=     {%
        \let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@generic
        \pgfkeysdefargs{/pgf/number format/sci generic/@}%
            {##1##2##3}%
            {\pgfqkeys{/pgf/number format/sci generic}{#1}}%
    },
    sci generic/mantissa sep/.initial=,%
    sci generic/empty mantissa sep/.initial=,%
    sci generic/mantisse sep/.style={/pgf/number format/sci generic/mantissa sep={#1}},%
    sci generic/empty mantisse sep/.style={/pgf/number format/sci generic/empty mantissa sep={#1}},%
    sci generic/exponent/.initial=,%
    sci generic/.value required,
    verbatim/.code={%
        \pgfqkeys{/pgf/number format}{%
            sci generic={mantissa sep=,exponent={e##1}},
            1000 sep=,
            skip 0.=false,
            print sign=false,
            dec sep=.,
            assume math mode,
            frac TeX=\pgfmathfloatfrac@verbatim,
            frac whole format/.code={\def\pgfmathresult{##1 }},
            @dec sep mark=,
            @sci exponent mark=,
        }%
    },
    retain unit mantissa/.is if=pgfmathfloatround@allow@empty@mantissa,
    retain unit mantissa/.default=true,
    retain unit mantissa=true,
    %
    % allows to replace the implementation, for example
    % 'implementation=\num'. This is experimental -- it is unclear
    % if all consumers work well since they rely on the keys in
    % /pgf/number format.
    implementation/.code={\def\pgfmathprintnumber@protected{#1}},
}



\def\pgfmathprintnumber@STD#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@STD@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@STD@setparam#1{%
    \edef\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfutil@empty
        % DEFAULT for lower and upper bound.
        \def\pgfmathprintnumber@STD@getlowerbound{%
            \c@pgf@counta=\pgfmathfloat@round@precision@orig\relax
            \divide\c@pgf@counta by-2\relax
        }%
        \def\pgfmathprintnumber@STD@upperbound{4}%
    \else
        \expandafter\pgfutil@in@\expandafter:\expandafter{\pgfmathfloat@loc@TMPb}%
        \ifpgfutil@in@
            % we have -4:5 or something like that.
            % parse both values:
            \def\pgfmathfloat@loc@TMPa##1:##2\relax{%
                \edef\pgfmathprintnumber@STD@getlowerbound{%
                    \noexpand\c@pgf@counta=##1\space
                }%
                \edef\pgfmathprintnumber@STD@upperbound{##2}%
            }%
            \expandafter\pgfmathfloat@loc@TMPa\pgfmathfloat@loc@TMPb\relax
        \else
            % we have just the lower bound:
            \def\pgfmathprintnumber@STD@upperbound{4}%
            \edef\pgfmathprintnumber@STD@getlowerbound{%
                \noexpand\c@pgf@counta=\pgfmathfloat@loc@TMPb\space
            }%
        \fi
    \fi
}%

\def\pgfmathprintnumber@STD@issci#1#2e#3\relax{%
    \expandafter\ifnum#1<3
        \expandafter\ifnum#3>\pgfmathprintnumber@STD@upperbound\relax
            \pgfmathprintnumber@SCI@issci#1#2e#3\relax%
        \else
            \begingroup
            \pgfmathprintnumber@STD@getlowerbound
            \ifnum#3<\c@pgf@counta
                \pgfmathprintnumber@SCI@issci#1#2e#3\relax%
            \else
                \pgfmathprintnumber@FIXED@issci#1#2e#3\relax%
            \fi
            \pgfmath@smuggleone\pgfmathresult
            \endgroup
        \fi
    \else% nan or inf:
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
}

\def\pgfmathprintnumber@RELATIVE#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@RELATIVE@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn{%
    \pgf@typeout{! Package pgf warning: the use of /pgf/number format/relative is discouraged (buggy). Please use 'relative*' instead or type \string\pgfkeys{/pgf/number format/relative round mode=fixed} into your preamble.}%
    \global\let\pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn=\relax
}

\def\pgfmathprintnumber@RELATIVE@issci#1#2e#3\relax{%
    \begingroup
        % format X / 10^{relative}:
        \c@pgf@counta=#3\relax
        \advance\c@pgf@counta by-\pgfmathprintnumber@RELATIVE@param\relax
        \pgfmathfloatcreate{#1}{#2}{\the\c@pgf@counta}%
        % OK, round it to the desired precision:
        \if0\pgfmathprintnumber@RELATIVE@choice@roundtofixed
            % relative round mode=mantissa
            \def\b@round@fixed{0}%
        \else
            \if1\pgfmathprintnumber@RELATIVE@choice@roundtofixed
                % relative round mode=fixed
                \def\b@round@fixed{1}%
            \else
                \pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn
                % relative round mode=compatible
                \ifnum\c@pgf@counta>0
                    % hm. for positive exponents, we should round the
                    % mantissa rather than only the fractional part.
                    \def\b@round@fixed{0}%
                \else
                    % negative exponent -> round fixed representation:
                    \def\b@round@fixed{1}%
                \fi
            \fi
        \fi
        \if1\b@round@fixed
            % round fixed representation:
            \pgfmathfloattofixed\pgfmathresult
            \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
            \pgfmathfloatparsenumber{\pgfmathresult}%
            \pgfmathfloatroundhasperiodtrue% make sure the code below works:
        \else
            % round the mantissa:
            \expandafter\pgfmathfloatround\expandafter{\pgfmathresult}%
        \fi
        % Now, compute result * 10^{relative} and format the result:
        \pgfmathfloattoregisterstok\pgfmathresult\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
        \ifnum\pgfmathfloat@a@S=0
            \pgfmathfloat@a@E=\pgfmathfloat@a@S % avoid 0 * 10^8
        \else
            \advance\pgfmathfloat@a@E by+\pgfmathprintnumber@RELATIVE@param\relax
        \fi
        \edef\pgfmathresultX{%
            \the\pgfmathfloat@a@S
            \the\pgfmathfloat@a@Mtok
            \ifpgfmathfloatroundhasperiod\else.0\fi
            e\the\pgfmathfloat@a@E}%
        % call another formatter for the result (but avoid rounding inside of it):
        \pgfqkeys{/pgf/number format}{/pgf/number format/every relative,
            fixed zerofill=false,% useless here!
            sci zerofill=false}%
        \ifx\pgfmathprintnumber@issci\pgfmathprintnumber@RELATIVE@issci
            \pgfmath@error{The '/pgf/number format/every relative' style should set a valid display style}{}%
        \fi
        \let\pgfmathfloat@round@precision@orig=\pgfmathfloat@round@precision
        \def\pgfmathfloat@round@precision{9999}%
        \expandafter\pgfmathprintnumber@issci\pgfmathresultX\relax%
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@FIXED@RELATIVE#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@FIXED@RELATIVE@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@FIXED@RELATIVE@issci#1#2e#3\relax{%
    \begingroup
    \pgfmathfloatcreate{#1}{#2}{#3}%
    % we want the first <precision> digits - not the first
    % <precision>+1 digits:
    \c@pgf@counta=\pgfmathfloat@round@precision\relax
    \advance\c@pgf@counta by-1
    \edef\pgfmathfloat@round@precision{\the\c@pgf@counta}%
    \pgfmathfloatround{\pgfmathresult}%
    \pgfmathfloattoregisterstok\pgfmathresult\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifnum\pgfmathfloat@a@S=0
        \pgfmathfloat@a@E=\pgfmathfloat@a@S % avoid 0 * 10^8
    \fi
    \edef\pgfmathresultX{%
        \the\pgfmathfloat@a@S
        \the\pgfmathfloat@a@Mtok
        \ifpgfmathfloatroundhasperiod\else.0\fi
        e\the\pgfmathfloat@a@E}%
    \let\pgfmathfloat@round@precision@orig=\pgfmathfloat@round@precision
    \pgfmathfloat@usezerofill@fixedfalse
    \def\pgfmathfloat@round@precision{9999}% typeset all remaining digits!
    \expandafter\pgfmathprintnumber@FIXED@issci\pgfmathresultX\relax%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@frac#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloatgetfrac{\pgfmathresult}%
    \expandafter\pgfmathprintnumber@frac@formatresult\pgfmathresult
}
\def\pgfmathprintnumber@frac@issci#1#2e#3\relax{%
    \pgfmathfloatcreate{#1}{#2}{#3}%
    \pgfmathfloatgetfrac{\pgfmathresult}%
    \expandafter\pgfmathprintnumber@frac@formatresult\pgfmathresult
}
\def\pgfmathprintnumber@frac@formatresult#1#2#3{%
    \begingroup
    \pgfkeysgetvalue{/pgf/number format/frac TeX}\pgfmathresult
    \toks0=\expandafter{\pgfmathresult}%
    \def\pgfmathfloat@loc@TMPa{#1}%
    \ifx\pgfmathfloat@loc@TMPa\pgfutil@empty
        \ifpgfmathprintnumber@showpositive
            \def\pgfmathfloat@loc@TMPa{+}%
        \fi
    \else
        \ifx\pgfmathfloat@loc@TMPa-%
        \else
            \ifx\pgfmathfloat@loc@TMPa+%
            \else
                \ifpgfmathprintnumber@showpositive
                    \edef\pgfmathfloat@loc@TMPa{+\pgfmathfloat@loc@TMPa}%
                \fi
                \def\pgfmathfloat@loc@TMPb{\pgfkeysvalueof{/pgf/number format/frac whole format/.@cmd}}%
                \expandafter\pgfmathfloat@loc@TMPb\pgfmathfloat@loc@TMPa\pgfeov
                \let\pgfmathfloat@loc@TMPa=\pgfmathresult
            \fi
        \fi
    \fi
    \toks1=\expandafter{\pgfmathfloat@loc@TMPa}%
    \edef\pgfmathresult{%
        \the\toks1 \ifnum#2=0 \else\the\toks0 {#2}{#3}\fi%
    }%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%

% Defines \pgfmathresult to contain three sets of braces containing
% the sign (optionally containing any components >1), the numerator and the denominator for #1.
%
% \pgfmathfloatgetfrac{0.5}  -> \pgfmathresult contains {}{1}{2}
% \pgfmathfloatgetfrac{-0.5} -> \pgfmathresult contains {-}{1}{2}
% \pgfmathfloatgetfrac{1.5} ->  \pgfmathresult contains {1}{1}{2}
%
% special cases:
% \pgfmathfloatgetfrac{0}   ->  \pgfmathresult contains {0}{0}{1}
% \pgfmathfloatgetfrac{1}   ->  \pgfmathresult contains {1}{0}{1}
%
% The numerator and denominator is always a number (not empty)
\def\pgfmathfloatgetfrac#1{%
    \pgfutil@ifundefined{pgfmathfloatmultiply@}{%
        \pgfmath@error{Sorry, the number format 'frac' requires '\string\usetikzlibrary{fpu}' (and, optionally, \string\usepackage{fp}) in order to work correctly}{}%
        \edef\pgfmathresult{{#1}{0}{1}}%
    }{%
        \pgfmathfloatgetfrac@{#1}%
    }%
}%
\def\pgfmathfloatgetfrac@#1{%
    \begingroup
        \edef\pgfmathfloat@arg{#1}%
        \expandafter\pgfmathfloat@decompose@tok\pgfmathfloat@arg\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
        \def\pgfmathfloat@loc@TMPa{0}%
        \ifcase\pgfmathfloat@a@S
        % #1 = 0:
            \def\pgfmathresult{{0}{0}{1}}%
        \or% #1 > 0
            \pgfmathfloat@a@S=1
            \def\pgfmathfloat@loc@TMPa{1}%
        \or% #1 < 0
            \pgfmathfloat@a@S=-1
            \def\pgfmathfloat@loc@TMPa{1}%
        \or
            \edef\pgfmathresult{{}{NaN}{1}}%
        \or
            \edef\pgfmathresult{{}{\infty}{1}}%
        \or
            \edef\pgfmathresult{{-}{\infty}{1}}%
        \fi
        \if1\pgfmathfloat@loc@TMPa
            \ifnum\pgfmathfloat@a@E<0
                \def\pgfmathfloat@wholenumber{}%
            \else
                \pgfmathfloatcreate{1}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
                \pgfmathfloattofixed\pgfmathresult%
                \def\pgfmathfloat@loc@TMPa##1.##2\relax{%
                    \def\pgfmathfloat@wholenumber{##1}%
                    \pgfmathfloatparsenumber{0.##2}%
                }%
                \expandafter\pgfmathfloat@loc@TMPa\pgfmathresult\relax
                \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@b@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
            \fi
            %
            \def\pgfmathfloat@loc@TMPa##1.##2\relax{%
                \def\pgfmathfloat@mantissa@first{##1}%
                \def\pgfmathfloat@mantissa@ltone{0.##2}%
            }%
            \expandafter\pgfmathfloat@loc@TMPa\the\pgfmathfloat@a@Mtok\relax
            %
            \def\pgfmathfloat@loc@@to@int##1.##2\relax##3{%
                ##3=##1
                \ifdim0.##2pt>0.5pt
                    \advance##3 by1
                \fi
            }%
            %
            % alias registers names:
            \let\pgfmathresultnumerator=\pgfmathfloat@b@S
            \let\pgfmathresultdenom=\pgfmathfloat@b@E
            %
            \pgfkeysgetvalue{/pgf/number format/frac denom}\pgfmath@target@denominator
            \ifx\pgfmath@target@denominator\pgfutil@empty
            %
                \pgfmathfloat@a@E=-\pgfmathfloat@a@E
                \ifdim\pgfmathfloat@mantissa@ltone pt=0pt
                    \def\pgfmathfloat@factor{1}%
                    \edef\pgfmathfloat@scaled@numerator{\the\pgfmathfloat@a@Mtok}%
                \else
                    % FIXME : this here is numerically instable.
                    %
                    % The errors of 1/r are magnified by 10^k which
                    % doesn't work.
                    \pgfutil@ifundefined{FPdiv}{%
                        \pgfmathfloatparsenumber{\pgfmathfloat@mantissa@ltone}%
                        \pgfmathfloatreciprocal@{\pgfmathresult}%
                    }{%
                        % \usepackage{fp}.
                        % yields higher absolute precision.
                        \FPmessagesfalse%
                        \FPdebugfalse%
                        \FPdiv\pgfmathresult{1}{\pgfmathfloat@mantissa@ltone}%
                        \pgfmathfloatparsenumber{\pgfmathresult}%
                    }%
                    \let\pgfmathfloat@inv=\pgfmathresult
                    \pgfmathfloatcreate{1}{1.0}{\pgfkeysvalueof{/pgf/number format/frac shift}}%
                    \let\pgfmathfloat@scalebaseten=\pgfmathresult
                    \pgfmathfloatmultiply@{\pgfmathfloat@inv}{\pgfmathfloat@scalebaseten}%
                    \let\pgfmathfloat@factor=\pgfmathresult
                    %
                    \expandafter\pgfmathfloatparsenumber\expandafter{\the\pgfmathfloat@a@Mtok}%
                    \let\pgfmathfloat@loc@TMPa=\pgfmathresult
                    \pgfmathfloatmultiply@{\pgfmathfloat@factor}{\pgfmathfloat@loc@TMPa}%
                    \pgfmathfloattofixed\pgfmathresult
                    \let\pgfmathfloat@scaled@numerator=\pgfmathresult
                    %
                    \pgfmathfloattofixed\pgfmathfloat@factor
                    \expandafter\pgfmathfloat@loc@@to@int\pgfmathresult\relax{\pgfmathfloat@b@S}%
                    \edef\pgfmathfloat@factor{\the\pgfmathfloat@b@S}%
                \fi
                %
                %
                \pgfmathresultdenom=\pgfmathfloat@factor\relax
                \pgfmathfloat@multiply@ten@to@the@E\pgfmathresultdenom
                %
                \expandafter\pgfmathfloat@loc@@to@int\pgfmathfloat@scaled@numerator\relax{\pgfmathresultnumerator}%
    %\message{scale = \pgfmathfloat@factor;  Z = \the\pgfmathresultnumerator\space ( von \pgfmathfloat@scaled@numerator), N = \the\pgfmathresultdenom.}%
                %
                \pgfmathgreatestcommondivisor{\pgfmathresultnumerator}{\pgfmathresultdenom}%
                \divide\pgfmathresultnumerator by\pgfmathresult\relax
                \divide\pgfmathresultdenom by\pgfmathresult\relax
                \ifpgfmathprintnumber@frac@warn
                    \ifnum\pgfmathresultdenom>1000
                        \pgfutil@ifundefined{FPdiv}{%
                            \pgfmathfloattosci@\pgfmathfloat@arg
                            \pgf@typeout{! Package pgf /pgf/number format/frac warning=true: /pgf/number format/frac of `\pgfmathresult' = \the\pgfmathresultnumerator\space / \the\pgfmathresultdenom\space might be large due to instabilities. Try \string\usepackage{fp} to improve accuracy.}%
                        }{}%
                    \fi
                \fi
            \else
                % use target denominator:
                \pgfmathresultdenom=\pgfmath@target@denominator\relax
                \pgfmathfloatcreate{1}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
                \pgfmathfloattofixed\pgfmathresult
                \pgf@xa=\pgfmathresult pt
                \multiply\pgf@xa by\pgfmathresultdenom
                \edef\pgfmathfloat@scaled@numerator{\pgfmath@tonumber\pgf@xa}%
                \expandafter\pgfmathfloat@loc@@to@int\pgfmathfloat@scaled@numerator\relax{\pgfmathresultnumerator}%
            \fi
            \ifpgfmathprintnumber@frac@whole
            \else
                \ifx\pgfmathfloat@wholenumber\pgfutil@empty
                \else
                    \count0=\pgfmathfloat@wholenumber\relax
                    \multiply\count0 by\pgfmathresultdenom
                    \advance\pgfmathresultnumerator by\count0
                    \def\pgfmathfloat@wholenumber{}%
                \fi
            \fi
            \ifnum\pgfmathfloat@a@S<0
                \edef\pgfmathresult{{-\pgfmathfloat@wholenumber}{\the\pgfmathresultnumerator}{\the\pgfmathresultdenom}}%
            \else
                \edef\pgfmathresult{{\pgfmathfloat@wholenumber}{\the\pgfmathresultnumerator}{\the\pgfmathresultdenom}}%
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%
\def\pgfmathfloat@gobble@until@relax#1\relax{}

% computes the greatest common divisor of two integer numbers (in
% integer arithmetics).
\def\pgfmathgreatestcommondivisor#1#2{%
    \begingroup
        \count0=#1\relax
        \count1=#2\relax
        \ifnum\count0=0
            \edef\pgfmathresult{\the\count1}%
        \else
            \pgfmathgreatestcommondivisor@loop
            \edef\pgfmathresult{\the\count0}%
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\def\pgfmathgreatestcommondivisor@loop{%
    \ifnum\count1=0
    \else
        \ifnum\count0>\count1
            \advance\count0 by-\count1
        \else
            \advance\count1 by-\count0
        \fi
        \expandafter\pgfmathgreatestcommondivisor@loop
    \fi
}%

% multiplies a TeX register by 10^E where E is stored in the register
% \pgfmathfloat@a@E (and it should be positive!)%
%
% #1 a TeX register
\def\pgfmathfloat@multiply@ten@to@the@E#1{%
    \ifnum\pgfmathfloat@a@E>0
        \multiply#1 by10
        \advance\pgfmathfloat@a@E by-1
        \def\pgfmathfloat@multiply@ten@to@the@E@next{\pgfmathfloat@multiply@ten@to@the@E{#1}}%
    \else
        \let\pgfmathfloat@multiply@ten@to@the@E@next=\relax%
    \fi
    \pgfmathfloat@multiply@ten@to@the@E@next
}%

\def\pgfmathprintnumber@INT@TRUNC#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@INT@TRUNC@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@TRUNC@impl#1.#2\relax#3#4e#5\relax{%
    \pgfmathfloatroundhasperiodfalse
    \pgfmathprintnumber@fixed@style{#1}#3#4e#5\relax%
}
\def\pgfmathprintnumber@INT@TRUNC@issci#1#2e#3\relax{%
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \expandafter\pgfmathprintnumber@INT@TRUNC@impl\pgfmathresult\relax#1#2e#3\relax
    \else
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
}

% Invokes '#2' if '#1' is actually an integer or '#3' if not.
%
% As a side-effect, \pgfretval will be set to the integer value if it
% actually *is* an integer. Otherwise, \pgfretval will contain the
% parsed floating point number.
%
% #1 a number constant (not necessarily a parsed float).
\def\pgfmathifisint#1#2#3{%
    \gdef\pgfmathfloatisint@@{0}%
    \begingroup
    \pgfmathfloatparsenumber{#1}%
    \let\pgfretval\pgfmathresult
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathfloatisint@\pgfmathresult\relax
    \pgfmath@smuggleone\pgfretval
    \endgroup
    \if1\pgfmathfloatisint@@ #2\else #3\fi
}%
\def\pgfmathfloatisint@#1#2e#3\relax{%
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \def\pgfmathfloat@round@precision{6}%
        \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \ifpgfmathfloatroundhasperiod
        \else
            \let\pgfretval\pgfmathresult%
            \gdef\pgfmathfloatisint@@{1}%
        \fi
    \fi
}

\def\pgfmathprintnumber@INT@DETECT#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@INT@DETECT@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@DETECT@issci#1#2e#3\relax{%
    \begingroup
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \let\pgfmathfloat@round@precision@=\pgfmathfloat@round@precision
        \def\pgfmathfloat@round@precision{6}%
        \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \let\pgfmathfloat@round@precision=\pgfmathfloat@round@precision@
        \ifpgfmathfloatroundhasperiod
            \pgfmathprintnumber@SCI@issci#1#2e#3\relax
        \else
            \expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax
        \fi
    \else
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@FIXED#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@FIXED@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@FIXED@issci#1#2e#3\relax{%
    \begingroup
    \ifnum#1<3
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \ifpgfmathfloat@usezerofill@fixed
            \expandafter\pgfmathroundtozerofill\expandafter{\pgfmathresult}%
        \else
            \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \fi
        \ifpgfmathfloatroundmayneedrenormalize
            \pgfmathfloat@a@E=#3\relax
            \advance\pgfmathfloat@a@E by1
            \edef\pgfmathfloat@loc@TMPb{\noexpand\pgfmathprintnumber@fixed@style{\pgfmathresult}#1#2e\the\pgfmathfloat@a@E}%
            \pgfmathfloat@loc@TMPb\relax%
        \else
            \expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax%
        \fi
    \else% nan or inf:
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}


\def\pgfmathprintnumber@SCI#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@SCI@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@SCI@issci#1#2e#3\relax{%
    \begingroup
    \pgfmathfloatcreate{#1}{#2}{#3}%
    \edef\pgfmathfloat@round@precision{\pgfmathprintnumber@sci@precision}%
    \ifpgfmathfloat@usezerofill@sci
        \pgfmathfloatroundzerofill{\pgfmathresult}%
    \else
        \pgfmathfloatround{\pgfmathresult}%
    \fi
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathfloatrounddisplaystyle\pgfmathresult\relax
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% Prints argument #1 using the current pretty printer environment (all
% variables in /pgf/number format).
%
% You may specify optional arguments with \pgfmathprintnumber[...].
\def\pgfmathprintnumber{%
    % \protect allows to supply \pgfmathprintnumber inside of latex
    % captions. The \csname yields \relax in case protect is undefined.
    \pgf@texdist@protect\pgfmathprintnumber@protected
}%
\def\pgfmathprintnumber@protected{%
    \pgfutil@ifnextchar[%
        {\pgfmathprintnumber@OPT}%
        {\pgfmathprintnumber@noopt}%
}

\def\pgfmathprintnumber@noopt#1{%
    \pgfmathprintnumber@{#1}%
    \ifpgfmathprintnumber@assumemathmode
        \pgfmathresult
    \else
        \pgfutilensuremath{\pgfmathresult}%
    \fi
}%
\def\pgfmathprintnumber@OPT[#1]#2{%
    \begingroup
    \pgfqkeys{/pgf/number format}{#1}%
    \pgfmathprintnumber@{#2}%
    \ifpgfmathprintnumber@assumemathmode
        \pgfmathresult
    \else
        \pgfutilensuremath{\pgfmathresult}%
    \fi
    \endgroup
}%

% As \pgfmathprintnumber, but it produces its output into the second
% argument.
\def\pgfmathprintnumberto{%
    \pgfutil@ifnextchar[%
        {\pgfmathprintnumberto@OPT}%
        {\pgfmathprintnumberto@noopt}%
}

\def\pgfmathprintnumberto@noopt#1#2{%
    \begingroup
    \pgfmathprintnumber@{#1}%
    \ifpgfmathprintnumber@assumemathmode
        \global\let\pgfmathfloat@glob@TMP=\pgfmathresult
    \else
        \toks0=\expandafter{\pgfmathresult}%
        \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
    \fi
    \endgroup
    \let#2=\pgfmathfloat@glob@TMP
}%
\def\pgfmathprintnumberto@OPT[#1]#2#3{%
    \begingroup
    \pgfqkeys{/pgf/number format}{#1}%
    \pgfmathprintnumber@{#2}%
    \ifpgfmathprintnumber@assumemathmode
        \global\let\pgfmathfloat@glob@TMP=\pgfmathresult
    \else
        \toks0=\expandafter{\pgfmathresult}%
        \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
    \fi
    \endgroup
    \let#3=\pgfmathfloat@glob@TMP
}%


% Changes the current number pretty printer to #1.
%
% #1 is the macro base name for the pretty print routine, without the
% leading '\'.
\def\pgfmath@set@number@printer#1{%
    \expandafter\let\expandafter\pgfmathprintnumber@\csname #1\endcsname
    \expandafter\let\expandafter\pgfmathprintnumber@issci\csname #1@issci\endcsname
}

\pgfkeys{/pgf/number format/std}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% IMPL
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% equals only itself when compared with \ifx:
\def\pgfmathfloat@EOI{\pgfmathfloat@EOI}%

% Re-use counters internally.
%
% They are always grouped and only used inside of the rounding
% routines.
\let\c@pgfmathroundto@prec=\pgfmathfloat@b@S% ATTENTION: DOUBLE-USED REGISTERS!
\let\c@pgfmathroundto@offsetbehindperiod=\pgfmathfloat@b@E
\newcount\c@pgfmathroundto@lastzeros

\newif\ifpgfmathround@impl@PREPERIOD@is@negative@zero

% PRECONDITION:
% \ifpgfmathfloatroundhasperiod=\iftrue  holds outside of the current TeX group.
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set correctly AFTER the
%   current TeX group.
%   \ifpgfmathfloatroundmayneedrenormalize will be set globally
\def\pgfmathroundto@impl#1{%
    \edef\pgfmathround@input{#1}%
    \global\pgfmathfloatroundmayneedrenormalizefalse
    \pgfmathfloat@tmptoks={}%
    \let\pgfmathround@next=\pgfutil@empty
    \let\pgfmathround@cur=\pgfutil@empty
    \let\pgfmathresult=\pgfutil@empty
    \expandafter\c@pgfmathroundto@prec\pgfmathfloat@round@precision\relax
    \c@pgfmathroundto@lastzeros=0
    \c@pgfmathroundto@offsetbehindperiod=-1 % means: no period found so far
    \pgfmathround@impl@PREPERIOD@is@negative@zerotrue
    \expandafter\pgfmathroundto@impl@ITERATE@NODOT@firstcall\pgfmathround@input\pgfmathfloat@EOI
}

% \pgfmathroundto implementation in WORDS:
%
% coarse idea:
%     1. collect all digits/sign BEFORE the first period in REVERSE order
%     2. then, collect UP TO \prec digits after the period in REVERSE order
% Steps 1. and 2. lead to the digit [sign] sequence
%     "x_{-p} x_{-p+1} ... x_{-2} x_{-1} '.' x_0 ... x_r"
% where 'r' is the total number of digits. The integer 'p' denotes the
% ACTUALLY collected number of digits behind the period.
%
% Let 'k' be the desired precision.
%
% Please note that pgfmathroundto rounds the mantissa, that means |abs(x)|.
%
% There are exactly TWO cases:
% 1. The case with p<=k and x_{-p-1} = end of input.
% 2. The case with p=k and x_{-p-1} is a further, next character.
%
% Then, for case 1.):
%     discard any unused zeros at the tail of our number (possibly
%     including the period)
%
% and in case 2.)
%   if NEXT DIGIT < 5:
%       do exactly the same as in case 1.) above and discard any
%       following digits.
%   else
%       let q := -p
%       while(x_q = 9 and q<=r )
%           if q>=0
%               set x_q = '0'
%           else
%               discard digit x_q='9'
%           fi
%           ++q
%           if q=0
%               discard the period
%           fi
%       end while
%       if q = r+1
%           insert a '1'
%       else
%           set x_q = x_q + 1
%       fi
%   fi
%
% All these loops have been implemented in spaghetti-code below.
% Sorry, I fear its hard to understand. In principle, everything is
% realised using more or less finite state machines (with some number
% counting logic).
%
% Some comments:
%     - The token register \pgfmathfloat@tmptoks is used to accumulate the REVERSED input number.
%     - \pgfmathfloat@EOI always denotes 'END OF INPUT'.
%     - in the second stage, we need to reverse \pgfmathfloat@tmptoks.
%       This is -- again -- done with \pgfmathfloat@tmptoks.

\def\pgfmathroundto@impl@discard@period#1.#2\pgfmathfloat@EOI{%
    \pgfmathfloatroundhasperiodfalse
    \aftergroup\pgfmathfloatroundhasperiodfalse
    \def\pgfmathresult{#1}%
}

\def\pgfmathroundto@impl@gobble@rest@and@start#1\pgfmathfloat@EOI{%
    \pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble@and@start\pgfmathfloat@EOI{%
    \pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble\pgfmathfloat@EOI{}%
\def\pgfmathroundto@impl@gobble@rest#1\pgfmathfloat@EOI{}%

% This method will be invoked as soon as the first step, the reverse
% collection of up to PREC digits after the period, has finished.
\def\pgfmathroundto@impl@start{%
    \ifx\pgfmathround@next\pgfutil@empty
        \ifnum\c@pgfmathroundto@offsetbehindperiod<0
            % no period found.
            \ifpgfmathfloat@fixed@digits@after@period
                \ifnum\c@pgfmathroundto@prec=0\relax
                    \pgfmathfloatroundhasperiodfalse
                    \aftergroup\pgfmathfloatroundhasperiodfalse
                    \edef\pgfmathresult{\pgfmathround@input}%
                \else
                    \pgfmathfloat@tmptoks=\expandafter{\pgfmathround@input.}%
                    \c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
                    \pgfmathroundto@impl@append@zeros
                    \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
                \fi
            \else
                \pgfmathfloatroundhasperiodfalse
                \aftergroup\pgfmathfloatroundhasperiodfalse
                \edef\pgfmathresult{\pgfmathround@input}%
            \fi
        \else
            %\ifnum\c@pgfmathroundto@offsetbehindperiod>\c@pgfmathroundto@prec
            %    \pgfmath@error{Internal logic error in pgfmathroundto at [I] - should not have happened!?}{}%
            %\fi
            \pgfmathroundto@impl@finish@with@truncation
        \fi
    \else
        %\ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
        %\else
        %    \pgfmath@error{Internal logic error in pgfmathroundto at [II] - should not have happened!? I have offsetbehindperiod=\the\c@pgfmathroundto@offsetbehindperiod and prec = \the\c@pgfmathroundto@prec}{}%
        %\fi
        \expandafter\ifnum\pgfmathround@next<5\relax
            \pgfmathroundto@impl@finish@with@truncation
        \else
            \multiply\c@pgfmathroundto@offsetbehindperiod by-1
            \expandafter\pgfmathroundto@impl@ADD@ONE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \fi
    \fi
}

% takes the current input and decides whether trailing zeros shall be
% discarded or more zeros need to be filled in.
\def\pgfmathroundto@impl@finish@with@truncation{%
    \ifpgfmathfloat@fixed@digits@after@period
        \expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
            \ifpgfmathround@impl@PREPERIOD@is@negative@zero
                % write '0.0000' instead of '-0.0000':
                \expandafter\pgfmathroundto@impl@discard@minus\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
            \fi
        \fi
        \ifnum\c@pgfmathroundto@prec=0\relax
            \expandafter\pgfmathroundto@impl@discard@period\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \else
            \advance\c@pgfmathroundto@prec by-\c@pgfmathroundto@offsetbehindperiod
            \c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
            \pgfmathroundto@impl@append@zeros
            \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
        \fi
    \else
        \pgfmathroundto@impl@discard@suffix@zeros
    \fi
}

\def\pgfmathroundto@impl@discard@minus-#1\pgfmathfloat@EOI{\pgfmathfloat@tmptoks={#1}}%

% appends \c@pgfmathroundto@offsetbehindperiod zeros at the end of \pgfmathfloat@tmptoks.
\def\pgfmathroundto@impl@append@zeros{%
    \ifnum\c@pgfmathroundto@offsetbehindperiod>0
        \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
        \advance\c@pgfmathroundto@offsetbehindperiod by-1
        \pgfmathroundto@impl@append@zeros
    \fi
}

\def\pgfmathroundto@impl@ADD@ONE{%
    \pgfmathfloat@tmptoks={}% no longer needed because its old value will be read from input
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@ITERATE{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        \global\pgfmathfloatroundmayneedrenormalizetrue
        \edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
        \pgfmathroundto@impl@gobble
    }{%
        \pgfutil@ifnextchar.{%
            \ifnum\c@pgfmathroundto@prec=0
                % silently discard period in special case precision=0
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
            \else
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT}%
            \fi
            \pgfmathround@nextcmd
        }{%
            \pgfutil@ifnextchar+{%
                \global\pgfmathfloatroundmayneedrenormalizetrue
                \edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
                \pgfmathroundto@impl@gobble@rest
            }{%
                \pgfutil@ifnextchar-{%
                    \global\pgfmathfloatroundmayneedrenormalizetrue
                    \edef\pgfmathresult{-1\the\pgfmathfloat@tmptoks}%
                    \pgfmathroundto@impl@gobble@rest
                }{%
                    \pgfmathroundto@impl@ADD@ONE@NEXT
                }%
            }%
        }%
    }%
}

\def\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot.{%
    \pgfmathfloatroundhasperiodfalse
    \aftergroup\pgfmathfloatroundhasperiodfalse
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}

\def\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT#1{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@NEXT#1{%
    \ifnum#1=9
        \ifnum\c@pgfmathroundto@offsetbehindperiod<0
            \ifpgfmathfloat@fixed@digits@after@period
                \pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
            \else
                % silently DROP digit
            \fi
        \else
            \pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
        \fi
        \advance\c@pgfmathroundto@offsetbehindperiod by1
        \ifnum\c@pgfmathroundto@offsetbehindperiod=0
            \ifpgfmathfloat@fixed@digits@after@period
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
            \else
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
            \fi
        \else
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
        \fi
    \else
        % re-use this counter:
        \c@pgfmathroundto@lastzeros=#1
        \advance\c@pgfmathroundto@lastzeros by1
        \edef\pgfmathresult{\the\c@pgfmathroundto@lastzeros\the\pgfmathfloat@tmptoks}%
        \pgfmathfloat@tmptoks=\expandafter{\pgfmathresult}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE@ITERATE}%
    \fi
    \pgfmathround@nextcmd
}


\def\pgfmathroundto@impl@discard@suffix@zeros{%
    \ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
        \ifpgfmathround@impl@PREPERIOD@is@negative@zero
            \pgfmathfloatroundhasperiodfalse
            \aftergroup\pgfmathfloatroundhasperiodfalse
            \def\pgfmathresult{0}% write '0' instead of '-0'
        \else
            \expandafter\pgfmathroundto@impl@discard@period\pgfmathround@input\pgfmathfloat@EOI
        \fi
    \else
        \ifnum\c@pgfmathroundto@lastzeros=0
            \expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \else
            \expandafter\pgfmathroundto@impl@discard@suffix@zeros@ITERATE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \fi
    \fi
}

% PRECONDITION:
%     \c@pgfmathroundto@lastzeros > 0
\def\pgfmathroundto@impl@discard@suffix@zeros@ITERATE#1{%
    \advance\c@pgfmathroundto@lastzeros by-1
    \ifnum\c@pgfmathroundto@lastzeros=0
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE}%
    \else
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@discard@suffix@zeros@ITERATE}%
    \fi
    \pgfmathround@nextcmd
}

% Usage:
% \pgfmathroundto@impl@REVERSE#1\pgfmathfloat@EOI
% -> writes #1 reversed into \pgfmathfloat@tmptoks
\def\pgfmathroundto@impl@REVERSE{%
    \pgfmathfloat@tmptoks={}%
    \pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@REVERSE@ITERATE{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
        \pgfmathroundto@impl@gobble
    }{%
        \pgfmathroundto@impl@REVERSE@NEXT
    }%
}

\def\pgfmathroundto@impl@REVERSE@NEXT#1{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
    \pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@BEGIN@DOT.{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter.\the\pgfmathfloat@tmptoks}%
    \c@pgfmathroundto@offsetbehindperiod=0
    \pgfmathroundto@impl@ITERATE@DOT
}
\def\pgfmathroundto@impl@ITERATE@DOT{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        % finished.
        \pgfmathroundto@impl@gobble@and@start
    }{%
        \pgfmathroundto@impl@NEXT@DOT
    }%
}
\def\pgfmathroundto@impl@NEXT@DOT#1{%
    \ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
        \def\pgfmathround@next{#1}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@gobble@rest@and@start}%
    \else
        \advance\c@pgfmathroundto@offsetbehindperiod by1
        \ifnum#1=0
            \advance\c@pgfmathroundto@lastzeros by1
        \else
            \c@pgfmathroundto@lastzeros=0
        \fi
        \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@DOT}%
    \fi
    \pgfmathround@nextcmd
}%

% in contrast to pgfmathroundto@impl@ITERATE@NODOT, this method here
% checks also for signs
\def\pgfmathroundto@impl@ITERATE@NODOT@firstcall#1{%
    \def\pgfmathround@cur{#1}%
    \ifx\pgfmathround@cur\pgfmathfloat@EOI
        \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
    \else
        \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
            \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
        \else
            \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@MINUS
            \else
                \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \fi
            \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
        \fi
    \fi
    \pgfmathround@nextcmd
}

\def\pgfmathroundto@impl@ITERATE@NODOT#1{%
    \def\pgfmathround@cur{#1}%
    \ifx\pgfmathround@cur\pgfmathfloat@EOI
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
    \else
        \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
        \else
            \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@ZERO
            \else
                \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \fi
            \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
        \fi
    \fi
    \pgfmathround@nextcmd
}

%--------------------------------------------
% END of pgfmathroundto implementation.
%--------------------------------------------


% flags, mantissa and exponent has already been stored into
% \pgfmathfloat@a@* [using ...@Mtok]
%
% PRECONDITION:
%   \ifpgfmathfloatroundhasperiod = \iftrue outside of the current
%   group
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set after the current TeX
%   group.
\def\pgfmathfloatround@impl{%
    \expandafter\pgfmathroundto@impl\expandafter{\the\pgfmathfloat@a@Mtok}%
    \ifpgfmathfloatroundmayneedrenormalize
        \ifpgfmathfloatroundhasperiod
            \expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult\pgfmathfloat@EOI%
        \else
            \expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult.\pgfmathfloat@EOI%
        \fi
        \advance\pgfmathfloat@a@E by1
    \fi
    \pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\pgfmathresult}{\the\pgfmathfloat@a@E}%
}

\def\pgfmathfloatround@impl@renormalize#1#2.#3\pgfmathfloat@EOI{%
    \pgfmathroundto@impl{#1.#2#3}%
}





% ATTENTION: this thing REQUIRES a period in the mantissa!
% collects everything into \pgfmathresult
\def\pgfmathfloattofixed@impl#1.#2\relax{%
    \ifnum\pgfmathfloat@a@E<0
        \ifcase-\pgfmathfloat@a@E
        \or%e-1
            \pgfmathfloat@a@Mtok={0.}%
        \or%e-2
            \pgfmathfloat@a@Mtok={0.0}%
        \or%e-3
            \pgfmathfloat@a@Mtok={0.00}%
        \or%e-4
            \pgfmathfloat@a@Mtok={0.000}%
        \or%e-5
            \pgfmathfloat@a@Mtok={0.0000}%
        \or%e-6
            \pgfmathfloat@a@Mtok={0.00000}%
        \or%e-7
            \pgfmathfloat@a@Mtok={0.000000}%
        \or%e-8
            \pgfmathfloat@a@Mtok={0.0000000}%
        \or%e-9
            \pgfmathfloat@a@Mtok={0.00000000}%
        \or%e-10
            \pgfmathfloat@a@Mtok={0.000000000}%
        \else%<= -11
            \pgfmathfloat@a@Mtok={0.0000000000}%
            \advance\pgfmathfloat@a@E by10
            \pgfutil@loop
            \ifnum\pgfmathfloat@a@E<-1
                \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
                \advance\pgfmathfloat@a@E by1
            \pgfutil@repeat
        \fi
        \def\pgfmathfloat@loc@TMPb{#2}%
        \def\pgfmathfloat@loc@TMPc{0}%
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloat@loc@TMPc
            \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1}%
        \else
            \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1#2}%
        \fi
    \else
        %--------------------------------------------------
        % \ifnum\pgfmathfloat@a@E=0%
        %     \edef\pgfmathresult{#1.#2}%
        % \else
        %     \pgfmathfloat@a@Mtok={#1}%
        %     \pgfmathfloattofixed@impl@collectmantissa#2\count\pgfmathfloat@a@E
        %     \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok}%
        % \fi
        %--------------------------------------------------
        \pgfmathfloat@a@Mtok{#1}%
        \pgfmathfloattofixed@impl@pos#2000000000\pgfmathfloat@EOI
        \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok}%
    \fi
}

% FIXME: this implementation here is very fast, but it introduces trailing zeros. Is that acceptable?
\def\pgfmathfloattofixed@impl@pos#1#2#3#4#5#6#7#8#9\pgfmathfloat@EOI{%
    \ifcase\pgfmathfloat@a@E
    % e+0
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok .#1#2#3#4#5#6#7#8#9}%
    \or%e+1
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1.#2#3#4#5#6#7#8#9}%
    \or%e+2
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2.#3#4#5#6#7#8#9}%
    \or%e+3
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3.#4#5#6#7#8#9}%
    \or%e+4
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4.#5#6#7#8#9}%
    \or%e+5
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5.#6#7#8#9}%
    \or%e+6
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6.#7#8#9}%
    \or%e+7
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7.#8#9}%
    \or%e+8
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7#8.#9}%
    \else%>=9
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7#8}%
        \advance\pgfmathfloat@a@E by-8
        \pgfmathfloattofixed@impl@collectmantissa#9\count\pgfmathfloat@a@E
    \fi
}%

\def\pgfmathfloattofixed@impl@collectmantissa#1#2\count#3{%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok #1}%
    \advance\pgfmathfloat@a@E by-1%
    \def\pgfmathfloat@loc@TMPb{#2}%
    \ifx\pgfmathfloat@loc@TMPb\pgfutil@empty
        \pgfutil@loop
        \ifnum\pgfmathfloat@a@E>0%
            \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
            \advance\pgfmathfloat@a@E by-1%
        \pgfutil@repeat
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .0}%
    \else
        \ifnum\pgfmathfloat@a@E=0
            \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .#2}%
        \else
            \pgfmathfloattofixed@impl@collectmantissa#2\count#3%
        \fi
    \fi
}


% ============================================
%
%
% \pgfmathfloatparsenumber implementation
%
%
% ============================================

% accepted parser tokens:
\def\pgfmathfloatparsenumber@tok@ZERO{0}
\def\pgfmathfloatparsenumber@tok@PLUS{+}
\def\pgfmathfloatparsenumber@tok@MINUS{-}
\def\pgfmathfloatparsenumber@tok@PERIOD{.}

\newif\ifpgfmathfloatparsenumberpendingperiod

\def\pgfflt@EOI{p@EOI}%
\def\pgfflt@EOI@unexpanded{\pgfflt@EOI}%

% Starts a finite-start-machine parser to read a number.
%
% The machine's state is represented by the macro which is currently
% processed; state transitions are realised using \csname...#1\endcsname
% constructions.
%
% It assigns \pgfmathfloat@a@S, \pgfmathfloat@a@Mtok, \pgfmathfloat@a@E.
\def\pgfflt@impl#1{%
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfmathfloat@tmptoks={}% this register is used to collect PENDING ZEROS
    \pgfmathfloat@a@E=0
    % start parsing: check for sign:
    \expandafter\ifx\csname pgfflt@#1\endcsname\relax
        \pgfmathfloat@a@S=1
        \expandafter\pgfflt@init\expandafter#1%
    \else
        \expandafter\expandafter\csname pgfflt@#1\endcsname
    \fi
}
% State transitions:
\expandafter\def\csname pgfflt@+\endcsname{%
    \pgfmathfloat@a@S=1 %
    \pgfflt@init}%
\expandafter\def\csname pgfflt@-\endcsname{%
    \pgfmathfloat@a@S=2 %
    \pgfflt@init}%
\expandafter\def\csname pgfflt@\pgfflt@EOI\endcsname{%
    \pgfmathfloatparsenumber@handleerror{empty number}{}{}}%

\pgfkeys{
    /pgf/fpu/handlers/empty number/.style 2 args={%
        /pgf/fpu/handlers/invalid number={#1}{#2}%
    },
    /pgf/fpu/empty number is zero/.style={%
        /pgf/fpu/handlers/empty number/.code 2 args={%
            \pgfmathfloatcreate{0}{0.0}{0}%
        }%
    },%
    /pgf/fpu/handlers/invalid separator/.code 2 args={%
        \pgfmath@error{Could not parse input '#1' as a floating point number, sorry. The unreadable part was near the decimal separator '#2'. Do you need the option 'read comma as period'?}{}%
    },
    /pgf/fpu/handlers/invalid number/.code 2 args={%
        \pgfmath@error{Could not parse input '#1' as a floating point number, sorry. The unreadable part was near '#2'.}{}%
    },
    /pgf/fpu/handlers/wrong lowlevel format/.code 2 args={%
        \pgfmath@error{Sorry, an internal routine of the floating point unit got an ill-formatted floating point number `#1'. The unreadable part was near '#2'.}{}%
        \let\pgfmathresult=\pgfutil@empty
    },
}

% #1 the error handler
% #2 the number which was invalid.
% #3 the part which produced the error
%
% POSTCONDITION: the three registers
%     \pgfmathfloat@a@S
%     \pgfmathfloat@a@Mtok
%     \pgfmathfloat@a@E
% will contain the number which results from the error handler.
\def\pgfmathfloatparsenumber@handleerror#1#2#3{%
    \let\pgfmathresult=\pgfutil@empty
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfkeys{/pgf/fpu/handlers/#1={#2}{#3}}%
    \ifx\pgfmathresult\pgfutil@empty
        \pgfmathfloat@a@S=3
        \pgfmathfloat@a@Mtok={0.0}%
        \pgfmathfloat@a@E=0
    \else
        \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \fi
}
\def\pgfflt@error#1\pgfflt@EOI{%
    \begingroup
    \pgfmathfloat@a@Mtok={#1}%
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\pgfmathfloatparsenumber@handleerror
            {invalid number}{\pgfmathresult}{\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}%



% FROM: checksign.
%
\def\pgfflt@init#1{%
    \expandafter\ifx\csname pgffltA@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltA@#1\endcsname
    \fi}
% state transitions:
\expandafter\def\csname pgffltA@0\endcsname{\pgfflt@leadingzero}% FIXME: inline optimization!
\expandafter\def\csname pgffltA@1\endcsname{\pgfflt@nonzerodigit1}%
\expandafter\def\csname pgffltA@2\endcsname{\pgfflt@nonzerodigit2}%
\expandafter\def\csname pgffltA@3\endcsname{\pgfflt@nonzerodigit3}%
\expandafter\def\csname pgffltA@4\endcsname{\pgfflt@nonzerodigit4}%
\expandafter\def\csname pgffltA@5\endcsname{\pgfflt@nonzerodigit5}%
\expandafter\def\csname pgffltA@6\endcsname{\pgfflt@nonzerodigit6}%
\expandafter\def\csname pgffltA@7\endcsname{\pgfflt@nonzerodigit7}%
\expandafter\def\csname pgffltA@8\endcsname{\pgfflt@nonzerodigit8}%
\expandafter\def\csname pgffltA@9\endcsname{\pgfflt@nonzerodigit9}%
\def\pgfflt@nonzerodigit#1{%
    \pgfmathfloat@a@Mtok={#1}%
    \pgfmathfloatparsenumberpendingperiodtrue
    \pgfflt@positiveexp}%
\expandafter\def\csname pgffltA@n\endcsname{\pgfflt@readnan}% FIXME: inlining?
\expandafter\def\csname pgffltA@N\endcsname{\pgfflt@readnan}% FIXME: inlining?
\expandafter\def\csname pgffltA@i\endcsname{\pgfflt@readinf}% FIXME: inlining?
\expandafter\def\csname pgffltA@I\endcsname{\pgfflt@readinf}% FIXME: inlining?
\expandafter\def\csname pgffltA@.\endcsname{% read '.9' like '0.9'
    \pgfmathfloat@a@E=-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltA@,\endcsname{% read ',9' like '0,9'
    \pgfmathfloat@frenchinput{%
        \pgfmathfloat@a@E=-1
        \pgfflt@leadingzero@foundperiod
    }%
}%

\def\pgfmathfloat@frenchinput#1{%
    \ifpgfmathparsenumber@comma@as@period
        \def\pgf@marshal{#1}%
        \expandafter\pgf@marshal
    \else
        \expandafter\pgfflt@error@separator\expandafter,%
    \fi
}%
\def\pgfflt@error@separator#1\pgfflt@EOI{%
    \begingroup
    \pgfmathfloat@a@Mtok={#1}%
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\pgfmathfloatparsenumber@handleerror
            {invalid separator}{\pgfmathresult}{\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}%

\def\pgfflt@finish#1\pgfflt@EOI{}

\def\pgfflt@readnan #1#2{%
    \def\pgfflt@readnan@ok{1}%
    \if#1a\else\if#1A\else\def\pgfflt@readnan@ok{0}\fi\fi
    \if#2n\else\if#2N\else\def\pgfflt@readnan@ok{0}\fi\fi
    \if\pgfflt@readnan@ok1%
        \pgfmathfloat@a@S=3\relax%
        \pgfmathfloat@a@Mtok={0.0}%
        \pgfmathfloat@a@E=0%
        \expandafter\pgfflt@finish
    \else
        \def\pgfflt@readnan@{\pgfflt@error #1#2}%
        \expandafter\pgfflt@readnan@
    \fi
}
\def\pgfflt@readinf #1#2{%
    \def\pgfflt@readinf@ok{1}%
    \if#1n\else\if#1N\else\def\pgfflt@readinf@ok{0}\fi\fi
    \if#2f\else\if#2F\else\def\pgfflt@readinf@ok{0}\fi\fi
    \if\pgfflt@readinf@ok1%
        \ifnum\pgfmathfloat@a@S=1 %
            \pgfmathfloat@a@S=4 %
            \pgfmathfloat@a@Mtok={0.0}%
        \else
            \pgfmathfloat@a@S=5 %
            \pgfmathfloat@a@Mtok={0.0}%
        \fi
        \pgfmathfloat@a@E=0 %
        \expandafter\pgfflt@finish
    \else
        \def\pgfflt@readinf@{\pgfflt@error #1#2}%
        \expandafter\pgfflt@readinf@
    \fi
}
\def\pgfflt@leadingzero#1{%
    \expandafter\ifx\csname pgffltB@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltB@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltB@0\endcsname{\pgfflt@leadingzero}%
\expandafter\def\csname pgffltB@1\endcsname{\pgfmathfloat@a@Mtok={1}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@2\endcsname{\pgfmathfloat@a@Mtok={2}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@3\endcsname{\pgfmathfloat@a@Mtok={3}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@4\endcsname{\pgfmathfloat@a@Mtok={4}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@5\endcsname{\pgfmathfloat@a@Mtok={5}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@6\endcsname{\pgfmathfloat@a@Mtok={6}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@7\endcsname{\pgfmathfloat@a@Mtok={7}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@8\endcsname{\pgfmathfloat@a@Mtok={8}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@9\endcsname{\pgfmathfloat@a@Mtok={9}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@\pgfmathfloat@POSTFLAGSCHAR\endcsname{\pgfmathfloat@a@Mtok={0}\pgfflt@readlowlevelfloat}%
\expandafter\def\csname pgffltB@.\endcsname{%
    \pgfmathfloat@a@E=-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltB@,\endcsname{%
    \pgfmathfloat@frenchinput{%
        \pgfmathfloat@a@E=-1
        \pgfflt@leadingzero@foundperiod
    }%
}%
\expandafter\def\csname pgffltB@e\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0%
    \pgfflt@readexponent}%
\let\pgffltB@E=\pgffltB@e
\expandafter\def\csname pgffltB@\pgfflt@EOI\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0}%

\def\pgfflt@leadingzero@foundperiod#1{%
    \expandafter\ifx\csname pgffltC@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltC@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltC@0\endcsname{%
    \advance\pgfmathfloat@a@E by-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltC@1\endcsname{\pgfmathfloat@a@Mtok={1}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@2\endcsname{\pgfmathfloat@a@Mtok={2}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@3\endcsname{\pgfmathfloat@a@Mtok={3}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@4\endcsname{\pgfmathfloat@a@Mtok={4}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@5\endcsname{\pgfmathfloat@a@Mtok={5}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@6\endcsname{\pgfmathfloat@a@Mtok={6}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@7\endcsname{\pgfmathfloat@a@Mtok={7}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@8\endcsname{\pgfmathfloat@a@Mtok={8}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@9\endcsname{\pgfmathfloat@a@Mtok={9}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@e\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0%
    \pgfflt@readexponent}%
\let\pgffltC@E=\pgffltC@e
\expandafter\def\csname pgffltC@\pgfflt@EOI\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0}%


\def\pgfflt@positiveexp#1{%
    \expandafter\ifx\csname pgffltD@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltD@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltD@0\endcsname{%
    \advance\pgfmathfloat@a@E by1
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros@positiveexp}%
\expandafter\def\csname pgffltD@1\endcsname{\pgffltD@nonzerodigit1}%
\expandafter\def\csname pgffltD@2\endcsname{\pgffltD@nonzerodigit2}%
\expandafter\def\csname pgffltD@3\endcsname{\pgffltD@nonzerodigit3}%
\expandafter\def\csname pgffltD@4\endcsname{\pgffltD@nonzerodigit4}%
\expandafter\def\csname pgffltD@5\endcsname{\pgffltD@nonzerodigit5}%
\expandafter\def\csname pgffltD@6\endcsname{\pgffltD@nonzerodigit6}%
\expandafter\def\csname pgffltD@7\endcsname{\pgffltD@nonzerodigit7}%
\expandafter\def\csname pgffltD@8\endcsname{\pgffltD@nonzerodigit8}%
\expandafter\def\csname pgffltD@9\endcsname{\pgffltD@nonzerodigit9}%
\expandafter\def\csname pgffltD@\pgfmathfloat@POSTFLAGSCHAR\endcsname{\pgfflt@readlowlevelfloat}%
\expandafter\def\csname pgffltD@.\endcsname{\pgfflt@finish@number@after@period}% FIXME : inlining?
\expandafter\def\csname pgffltD@,\endcsname{\pgfmathfloat@frenchinput{\pgfflt@finish@number@after@period}}%
\expandafter\def\csname pgffltD@e\endcsname{\pgfflt@readexponent}% FIXME : inlining?
\let\pgffltD@E=\pgffltD@e
\expandafter\def\csname pgffltD@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltD@nonzerodigit#1{%
    \advance\pgfmathfloat@a@E by1
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@positiveexp}%

% Read a low-level floating point.
% Since we are in the second state, \pgfmathfloat@a@Mtok contains the
% FLAGS. The post-flags-char has also been read.
\def\pgfflt@readlowlevelfloat#1e#2]\pgfflt@EOI{%
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfmathfloat@a@S=\the\pgfmathfloat@a@Mtok\relax
    \pgfmathfloat@a@Mtok={#1}%
    \pgfmathfloat@a@E=#2
}%

\def\pgfflt@readexponent#1\pgfflt@EOI{%
    \afterassignment\pgfflt@readexponent@
    \pgfmathfloat@b@E=#1 \pgfflt@EOI% the white space is important, otherwise \pgfflt@EOI will be expanded.
}
\def\pgfflt@readexponent@#1{%
    \advance\pgfmathfloat@a@E by\pgfmathfloat@b@E\relax
    %
    % sanity checking:
    \def\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfflt@EOI@unexpanded
    \else
        \def\pgfmathfloat@loc@TMPb{\pgfflt@error#1}%
        \expandafter\pgfmathfloat@loc@TMPb
    \fi
}

\def\pgfflt@pendingzeros@positiveexp#1{%
    \expandafter\ifx\csname pgffltE@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltE@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltE@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \advance\pgfmathfloat@a@E by1
    \pgfflt@pendingzeros@positiveexp}%
\expandafter\def\csname pgffltE@1\endcsname{\pgffltE@nonzerodigit1}%
\expandafter\def\csname pgffltE@2\endcsname{\pgffltE@nonzerodigit2}%
\expandafter\def\csname pgffltE@3\endcsname{\pgffltE@nonzerodigit3}%
\expandafter\def\csname pgffltE@4\endcsname{\pgffltE@nonzerodigit4}%
\expandafter\def\csname pgffltE@5\endcsname{\pgffltE@nonzerodigit5}%
\expandafter\def\csname pgffltE@6\endcsname{\pgffltE@nonzerodigit6}%
\expandafter\def\csname pgffltE@7\endcsname{\pgffltE@nonzerodigit7}%
\expandafter\def\csname pgffltE@8\endcsname{\pgffltE@nonzerodigit8}%
\expandafter\def\csname pgffltE@9\endcsname{\pgffltE@nonzerodigit9}%
\expandafter\def\csname pgffltE@.\endcsname{\pgfflt@finish@number@after@period}% FIXME : inlining?
\expandafter\def\csname pgffltE@,\endcsname{\pgfmathfloat@frenchinput{\pgfflt@finish@number@after@period}}% FIXME : inlining?
\def\pgffltE@e{\pgfflt@readexponent}% FIXME : inlining?
\let\pgffltE@E=\pgffltE@e
\expandafter\def\csname pgffltE@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltE@nonzerodigit#1{%
    \advance\pgfmathfloat@a@E by1
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@positiveexp}%

\def\pgfflt@finish@number@after@period#1{%
    \expandafter\ifx\csname pgffltF@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltF@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltF@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros}%
\expandafter\def\csname pgffltF@1\endcsname{\pgffltF@nonzerodigit1}%
\expandafter\def\csname pgffltF@2\endcsname{\pgffltF@nonzerodigit2}%
\expandafter\def\csname pgffltF@3\endcsname{\pgffltF@nonzerodigit3}%
\expandafter\def\csname pgffltF@4\endcsname{\pgffltF@nonzerodigit4}%
\expandafter\def\csname pgffltF@5\endcsname{\pgffltF@nonzerodigit5}%
\expandafter\def\csname pgffltF@6\endcsname{\pgffltF@nonzerodigit6}%
\expandafter\def\csname pgffltF@7\endcsname{\pgffltF@nonzerodigit7}%
\expandafter\def\csname pgffltF@8\endcsname{\pgffltF@nonzerodigit8}%
\expandafter\def\csname pgffltF@9\endcsname{\pgffltF@nonzerodigit9}%
\def\pgffltF@e{\pgfflt@readexponent}%
\let\pgffltF@E=\pgffltF@e
\expandafter\def\csname pgffltF@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltF@nonzerodigit#1{%
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@finish@number@after@period}%


\def\pgfflt@pendingzeros#1{%
    \expandafter\ifx\csname pgffltG@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltG@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltG@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros}%
\expandafter\def\csname pgffltG@1\endcsname{\pgffltG@nonzerodigit1}%
\expandafter\def\csname pgffltG@2\endcsname{\pgffltG@nonzerodigit2}%
\expandafter\def\csname pgffltG@3\endcsname{\pgffltG@nonzerodigit3}%
\expandafter\def\csname pgffltG@4\endcsname{\pgffltG@nonzerodigit4}%
\expandafter\def\csname pgffltG@5\endcsname{\pgffltG@nonzerodigit5}%
\expandafter\def\csname pgffltG@6\endcsname{\pgffltG@nonzerodigit6}%
\expandafter\def\csname pgffltG@7\endcsname{\pgffltG@nonzerodigit7}%
\expandafter\def\csname pgffltG@8\endcsname{\pgffltG@nonzerodigit8}%
\expandafter\def\csname pgffltG@9\endcsname{\pgffltG@nonzerodigit9}%
\def\pgffltG@e{\pgfflt@readexponent}% FIXME: inlining?
\let\pgffltG@E=\pgffltG@e
\expandafter\def\csname pgffltG@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltG@nonzerodigit#1{%
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@finish@number@after@period}%

\endinput


==> pgfmathfunctions.base.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file provides basic macros for converting between bases.
%
% Version 1.4142135 8/11/2008

% Base conversion operations for the parser.
%
\pgfmathdeclarefunction{bin}{1}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=#1\relax\pgfmath@%
        \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\the\c@pgfmath@counta}{10}{2}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}
\pgfmathdeclarefunction{hex}{1}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=#1\relax\pgfmath@%
        \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\the\c@pgfmath@counta}{10}{16}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

\pgfmathdeclarefunction{Hex}{1}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=#1\relax\pgfmath@%
        \expandafter\pgfmathbasetoBase\expandafter\pgfmathresult\expandafter{\the\c@pgfmath@counta}{10}{16}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

\pgfmathdeclarefunction{oct}{1}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=#1\relax\pgfmath@%
        \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\the\c@pgfmath@counta}{10}{8}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% Additional macros:

% \pgfmathbasetodec
%
% Convert a representation of an integer from
% the specified base to base 10.
%
% #1 - a macro to store the result.
% #2 - the representation of a number (i.e. not a register)
% #3 - the current base.
%
% e.g.
%
% \pgfmathbasetodec\mynumber{10111}{2}
%
% \mynumber <- 23
%
\def\pgfmathbasetodec#1#2#3{%
    \pgfmath@checknumber{#2}%
    \pgfmath@checkbase{#3}%
    \def\pgfmath@base{#3}%
    \def\pgfmath@base@macro{#1}%
    \c@pgfmath@counta=1\relax%
    \let\pgfmath@reversed=\pgfmath@empty%
    \expandafter\pgfmathbasetodec@#2\pgfmath@base@stop}

\def\pgfmathbasetodec@#1{%
    \ifx#1\pgfmath@base@stop%
        \c@pgfmath@countb=0%
        \divide\c@pgfmath@counta by\pgfmath@base\relax%
        \expandafter\pgfmathbasetodec@@%
    \else%
        \edef\pgfmath@reversed{\pgfmath@reversed#1}%
        \expandafter\multiply\expandafter\c@pgfmath@counta\pgfmath@base\relax%
        \expandafter\pgfmathbasetodec@%
    \fi}

\def\pgfmathbasetodec@@{\expandafter\pgfmathbasetodec@@@\pgfmath@reversed\pgfmathbasetodec}

\def\pgfmathbasetodec@@@#1{%
    \ifx\pgfmathbasetodec#1\relax%
        \expandafter\edef\pgfmath@base@macro{\the\c@pgfmath@countb}%
        \let\pgfmath@next=\pgfmathbasetodec@@@@%
    \else%
        \chardef\pgfmath@charnum`#1\relax%
        \c@pgfmath@countc=\pgfmath@charnum\relax%
        \ifnum\c@pgfmath@countc>96\relax%
            \advance\c@pgfmath@countc by-87\relax%
        \else
            \ifnum\c@pgfmath@countc>64\relax%
                \advance\c@pgfmath@countc by-55\relax%
            \else
                \advance\c@pgfmath@countc by-48\relax%
            \fi%
        \fi%
        \ifnum\c@pgfmath@countc<\pgfmath@base\relax%
            \multiply\c@pgfmath@countc by\c@pgfmath@counta%
            \advance\c@pgfmath@countb by\c@pgfmath@countc%
            \divide\c@pgfmath@counta by\pgfmath@base\relax%
            \let\pgfmath@next\pgfmathbasetodec@@@%
        \else
            \pgfmath@error{Digit `#1' invalid for base \pgfmath@base}{}%
            \let\pgfmath@next=\relax%
        \fi%
    \fi%
    \pgfmath@next}
\def\pgfmathbasetodec@@@@{%
    \expandafter\pgfmath@ensurenumberlength\expandafter{\pgfmath@base@macro}%
}

% \pgfmathdectobase
%
% Convert a representation of an integer from
% base 10 to the specified base. Letters for bases
% greater than 10 are in lowercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectobase\mynumber{127}{16}
%
% \mynumber <- 7f
%
\def\pgfmathdectobase#1#2#3{%
    \pgfmath@checknumber{#2}%
    \pgfmath@checkbase{#3}%
    \c@pgfmath@counta=#2\relax%
    \let#1=\pgfmath@empty%
    \pgfmathloop
        \ifnum\c@pgfmath@counta>0\relax%
            \c@pgfmath@countb=\c@pgfmath@counta%
            \divide\c@pgfmath@countb by#3\relax%
            \multiply\c@pgfmath@countb by-#3\relax%
            \advance\c@pgfmath@countb by\c@pgfmath@counta%
            \edef#1{\csname pgfmath@lowercase digit@\the\c@pgfmath@countb\endcsname#1}%
            \divide\c@pgfmath@counta by#3\relax%
    \repeatpgfmathloop%
    \pgfmath@ensurenumberlength{#1}}

% \pgfmathdectoBase
%
% Convert a representation of an integer from
% base 10 to the specified base. Letters for bases
% greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectoBase\mynumber{127}{16}
%
% \mynumber <- 7F
%
\def\pgfmathdectoBase#1#2#3{%
    \pgfmath@checkbase{#3}%
    \pgfmath@checknumber{#2}%
    \c@pgfmath@counta=#2\relax%
    \let#1=\pgfmath@empty%
    \pgfmathloop
        \ifnum\c@pgfmath@counta>0\relax%
            \c@pgfmath@countb=\c@pgfmath@counta%
            \divide\c@pgfmath@countb by#3\relax%
            \multiply\c@pgfmath@countb by-#3\relax%
            \advance\c@pgfmath@countb by\c@pgfmath@counta%
            \edef#1{\csname pgfmath@uppercase digit@\the\c@pgfmath@countb\endcsname#1}%
            \divide\c@pgfmath@counta by#3\relax%
    \repeatpgfmathloop%
    \pgfmath@ensurenumberlength{#1}}

\def\pgfmath@base@digits@create{%
    \def\pgfmath@base@digit@style{lowercase digit}%
    \c@pgfmath@counta=0\relax%
    \pgfmath@base@digits@create@0123456789abcdefghijklmnopqrstuvwxyz\pgfmath@base@digits@create%
    \def\pgfmath@base@digit@style{uppercase digit}%
    \c@pgfmath@counta=0\relax%
    \pgfmath@base@digits@create@0123456789ABCDEFGHIJKLMNOPQRSTUVWXYZ\pgfmath@base@digits@create}

\def\pgfmath@base@digits@create@#1{%
    \ifx\pgfmath@base@digits@create#1\relax%
    \else%
        \expandafter\pgfmath@def\expandafter{\pgfmath@base@digit@style}{\the\c@pgfmath@counta}{#1}%
        \advance\c@pgfmath@counta by1\relax%
        \expandafter\pgfmath@base@digits@create@%
    \fi}
\pgfmath@base@digits@create

% \pgfmathbasetobase
%
% Convert a representation of an integer from
% between the specified bases. Letters for target
% bases greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{4321}{5}{9}
%
% \mynumber <- 721
%
\def\pgfmathbasetobase#1#2#3#4{%
    \pgfmathbasetodec{\pgfmath@base@temp}{#2}{#3}%
    \pgfmathdectobase{#1}{\pgfmath@base@temp}{#4}%
}

% \pgfmathbasetobase
%
% Convert a representation of an integer from
% between the specified bases. Letters for target
% bases greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{1234}{5}{12}
%
% \mynumber <- 142
%
\def\pgfmathbasetoBase#1#2#3#4{%
    \pgfmathbasetodec{\pgfmath@base@temp}{#2}{#3}%
    \pgfmathdectoBase{#1}{\pgfmath@base@temp}{#4}%
}

\def\pgfmath@checkbase#1{%
    \ifnum#1<2\relax%
        \pgfmath@error{Cannot process numbers in base `#1'.}{}%
    \else%
        \ifnum#1>36\relax%
            \pgfmath@error{Cannot process numbers in base `#1'.}{}%
        \fi%
    \fi}

\def\pgfmath@checknumber#1{%
    \expandafter\pgfmath@checknumber@#1\pgfmath@}
\def\pgfmath@checknumber@#1#2\pgfmath@{%
    \ifx#1-%
        \pgfmath@error{Cannot process negative numbers.}{}%
    \fi}

% \pgfmath@ensurenumberlength
%
% Internal macro for making a representation of a number have
% a specific length, byte prefixing zeros to the number.
%
% #1 - a macro containing a representation of an integer.
% #2 - the number of digits to ensure.
%
% e.g.
%
% \foo <- 7FF
%
% \pgfmathsetnumberlength{8}%
% \pgfmath@ensurenumberlength\foo
%
% \foo <- 000007FF
%
\def\pgfmath@ensurenumberlength#1{%
    \def\pgfmath@base@tempa{#1}%
    \expandafter\c@pgfmath@counta\pgfmath@basenumberlength\relax%
    \expandafter\pgfmath@ensurenumberlength@#1\pgfmath@ensurenumberlength}
\def\pgfmath@ensurenumberlength@#1{%
    \ifx\pgfmath@ensurenumberlength#1\relax%
        \expandafter\pgfmath@ensurenumberlength@@%
    \else%
        \advance\c@pgfmath@counta by-1\relax%
        \expandafter\pgfmath@ensurenumberlength@
    \fi}

\def\pgfmath@ensurenumberlength@@{%
    \edef\pgfmath@base@tempb{\pgfmath@base@tempa}%
    \pgfmath@ensurenumberlength@@@}
\def\pgfmath@ensurenumberlength@@@{%
    \ifnum\c@pgfmath@counta>0\relax%
        \advance\c@pgfmath@counta by-1\relax%
        \edef\pgfmath@base@tempb{0\pgfmath@base@tempb}%
        \expandafter\pgfmath@ensurenumberlength@@@%
    \fi%
    \expandafter\edef\pgfmath@base@tempa{\pgfmath@base@tempb}}

\def\pgfmathsetbasenumberlength#1{\def\pgfmath@basenumberlength{#1}}
\pgfmathsetbasenumberlength{1}%

% \pgfmathtodigitlist\marg{macro}\marg{number}}
%
%    This command converts \meta{number} into a comma-separated
%    list of digits and stores the result in \meta{macro}.
%    The \marg{number} is \emph{not} parsed before processing.
%
\def\pgfmathtodigitlist#1#2{%
    \def\pgfmath@temp{#1}%
    \let\pgfmath@digitlist=\pgfutil@empty%
    \edef\pgfmath@@tmp{#2}%
    \expandafter\pgfmath@todigitlist\pgfmath@@tmp @%
}
\def\pgfmath@base@atchar{@}
\def\pgfmath@todigitlist#1{%
    \def\pgfmath@digit{#1}%
    \ifx\pgfmath@digit\pgfmath@base@atchar%
        \expandafter\let\pgfmath@temp=\pgfmath@digitlist%
    \else%
        \ifx\pgfmath@digitlist\pgfutil@empty%
            \edef\pgfmath@digitlist{#1}%
        \else%
            \edef\pgfmath@digitlist{\pgfmath@digitlist,#1}%
        \fi%
        \expandafter\pgfmath@todigitlist%
    \fi%
}


==> pgfmathfunctions.basic.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 1.4142135 25/8/2008

% add function.
%
\pgfmathdeclarefunction{add}{2}{%
    \begingroup%
    \pgfmath@x=#1pt\relax%
    \pgfmath@y=#2pt\relax%
    \advance\pgfmath@x by\pgfmath@y%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}


% subtract function.
%
\pgfmathdeclarefunction{subtract}{2}{%
    \begingroup%
    \pgfmath@x=#1pt\relax%
    \pgfmath@y=#2pt\relax%
    \advance\pgfmath@x by-\pgfmath@y%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% neg function.
%
\pgfmathdeclarefunction{neg}{1}{%
    \begingroup%
        \pgfmath@x=-#1pt\relax%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}
% change the precedence for neg.
% Otherwise, unary minus and exponentiation won't have the correct precedence
% (test '-2^2')
\def\pgfmath@operation@neg@precedence{500}

% multiply function.
%
\pgfmathdeclarefunction{multiply}{2}{%
  \begingroup%
    \pgfmath@x=#1pt\relax%
    \pgfmath@y=#2pt\relax%
    \pgfmath@x=\pgfmath@tonumber{\pgfmath@y}\pgfmath@x%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% divide function.
%
\newif\ifpgfmath@divide@period

\pgfmathdeclarefunction{divide}{2}{%
    \begingroup%
        \pgfmath@x=#1pt\relax%
        \pgfmath@y=#2pt\relax%
        \let\pgfmath@sign=\pgfmath@empty%
        \ifdim0pt=\pgfmath@y%
            \pgfmath@error{You've asked me to divide `#1' by `#2', %
                but I cannot divide any number by `#2'}{}%
        \fi%
        \afterassignment\pgfmath@xa%
        \c@pgfmath@counta\the\pgfmath@y\relax%
        \ifdim0pt=\pgfmath@xa%
            \divide\pgfmath@x by\c@pgfmath@counta%
        \else%
            \ifdim0pt>\pgfmath@x%
                \def\pgfmath@sign{-}%
                \pgfmath@x=-\pgfmath@x%
            \fi%
            \ifdim0pt>\pgfmath@y%
                \expandafter\def\expandafter\pgfmath@sign\expandafter{\pgfmath@sign-}%
                \pgfmath@y=-\pgfmath@y%
            \fi%
            \ifdim1pt>\pgfmath@y%
                \pgfmathreciprocal@{\pgfmath@tonumber{\pgfmath@y}}%
                \pgfmath@x=\pgfmath@sign\pgfmathresult\pgfmath@x%
            \else%
                \def\pgfmathresult{0}%
                \pgfmath@divide@periodtrue%
                \c@pgfmath@counta=0\relax%
                \pgfmathdivide@@%
                \pgfmath@x=\pgfmath@sign\pgfmathresult pt\relax%
            \fi%
        \fi%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

\def\pgfmath@small@number{0.00002}

\def\pgfmathdivide@@{%
    \let\pgfmath@next=\relax%
    \ifdim\pgfmath@small@number pt<\pgfmath@x%
        \ifdim\pgfmath@small@number pt<\pgfmath@y%
            \ifdim\pgfmath@y>\pgfmath@x%
                \ifpgfmath@divide@period%
                    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult.}%
                    \pgfmath@divide@periodfalse%
                \fi%
                \pgfmathdivide@dimenbyten\pgfmath@y%
                \ifdim\pgfmath@y>\pgfmath@x%
                    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult0}%
                \fi%
            \else%
                \c@pgfmath@counta=\pgfmath@x%
                \c@pgfmath@countb=\pgfmath@y%
                \divide\c@pgfmath@counta by\c@pgfmath@countb%
                \pgfmath@ya=\c@pgfmath@counta\pgfmath@y%
                \advance\pgfmath@x by-\pgfmath@ya%
                \def\pgfmath@next{%
                    \toks0=\expandafter{\pgfmathresult}%
                    \edef\pgfmathresult{\the\toks0 \the\c@pgfmath@counta}%
                }%
                \ifpgfmath@divide@period
                \else
                    % we are behind the period. It may happen that the
                    % result is more than one digit - in that case,
                    % introduce special handling:
                    \ifnum\c@pgfmath@counta>9 %
                        \expandafter\pgfmathdivide@advance@last@digit\pgfmathresult CCCCC\@@
                        \advance\c@pgfmath@counta by-10 %
                        \ifnum\c@pgfmath@counta=0
                            \let\pgfmath@next=\relax
                        \fi
                    \fi
                \fi
                \pgfmath@next
            \fi%
            \let\pgfmath@next=\pgfmathdivide@@%
        \fi%
    \fi%
    \pgfmath@next%
}

% advances the last digit found in the number. Any missing digits are
% supposed to be filled with 'C'.
\def\pgfmathdivide@advance@last@digit#1.#2#3#4#5#6#7\@@{%
    \pgfmath@ya=\pgfmathresult pt %
    \if#2C%
        \pgfmath@xa=1pt %
    \else
        \if#3C%
            \pgfmath@xa=0.1pt %
        \else
            \if#4C%
                \pgfmath@xa=0.01pt %
            \else
                \if#5C%
                    \pgfmath@xa=0.001pt %
                \else
                    \if#6C%
                        \pgfmath@xa=0.0001pt %
                    \else
                        \pgfmath@xa=0.00001pt %
                    \fi
                \fi
            \fi
        \fi
    \fi
    \advance\pgfmath@ya by\pgfmath@xa
    \edef\pgfmathresult{\pgfmath@tonumber@notrailingzero\pgfmath@ya}%
}%

{
\catcode`\p=12
\catcode`\t=12
\gdef\Pgf@geT@NO@TRAILING@ZERO#1.#2pt{%
    #1.%
    \ifnum#2=0 \else #2\fi
}
}
\def\pgfmath@tonumber@notrailingzero#1{\expandafter\Pgf@geT@NO@TRAILING@ZERO\the#1}


\def\pgfmathdivide@dimenbyten#1{%
    \edef\pgfmath@temp{\pgfmath@tonumber{#1}}%
    \expandafter\pgfmathdivide@@dimenbyten\pgfmath@temp\@@#1\@@}
\def\pgfmathdivide@@dimenbyten#1.#2\@@#3\@@{%
    \pgfmath@tempcnta=#1\relax%
    \divide\pgfmath@tempcnta by10\relax%
    \pgfmath@tempcntb=\pgfmath@tempcnta%
    \multiply\pgfmath@tempcnta by-10\relax%
    \advance\pgfmath@tempcnta by#1\relax%
    #3=\the\pgfmath@tempcntb.\the\pgfmath@tempcnta#2pt\relax%
}


% reciprocal function.
%
\pgfmathdeclarefunction{reciprocal}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x=0pt\relax%
            \pgfmath@error{You asked me to calculate `1/#1', but I cannot divide any number by zero}{}%
        \fi%
        \edef\pgfmath@reciprocaltemp{\pgfmath@tonumber{\pgfmath@x}}%
        \expandafter\pgfmathreciprocal@@\pgfmath@reciprocaltemp0000000\pgfmath@}
\def\pgfmathreciprocal@@#1.#2#3#4#5#6#7\pgfmath@{%
        \c@pgfmath@counta#2#3#4#5#6\relax%
        % If the number is an integer, use TeX arithmetic.
        \ifnum\c@pgfmath@counta=0\relax%
            \pgfmath@x1pt\relax%
            \divide\pgfmath@x#1\relax%
        \else%
            \ifnum#1>100\relax%
                \c@pgfmath@counta#1#2#3#4\relax%
                \c@pgfmath@countb1000000000\relax%
                \divide\c@pgfmath@countb\c@pgfmath@counta%
                \c@pgfmath@counta\c@pgfmath@countb%
                \divide\c@pgfmath@counta10000\relax%
                \pgfmath@x\c@pgfmath@counta pt\relax%
                \multiply\c@pgfmath@counta-10000\relax%
                \advance\c@pgfmath@countb\c@pgfmath@counta%
                \pgfmath@y\c@pgfmath@countb pt\relax%
                \divide\pgfmath@y1000000\relax%
                \advance\pgfmath@x\pgfmath@y%
            \else%
                \c@pgfmath@counta#1#2#3#4#5#6\relax%
                \c@pgfmath@countb1000000000\relax%
                \divide\c@pgfmath@countb\c@pgfmath@counta%
                \c@pgfmath@counta\c@pgfmath@countb%
                \divide\c@pgfmath@counta10000\relax%
                \pgfmath@x\c@pgfmath@counta pt\relax%
                \multiply\c@pgfmath@counta-10000\relax%
                \advance\c@pgfmath@countb\c@pgfmath@counta%
                \pgfmath@y\c@pgfmath@countb pt\relax%
                \pgfmath@y.1\pgfmath@y% Yes! This way is more accurate. Go figure...
                \pgfmath@y.1\pgfmath@y%
                \pgfmath@y.1\pgfmath@y%
                \pgfmath@y.1\pgfmath@y%
                \advance\pgfmath@x\pgfmath@y%
            \fi%
        \fi%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% div function.
%
\pgfmathdeclarefunction{div}{2}{%
    \begingroup%
        \pgfmathdivide@{#1}{#2}%
        \ifdim\pgfmathresult pt<0pt\relax%
            \pgfmathceil@{\pgfmathresult}%
        \else%
            \pgfmathfloor@{\pgfmathresult}%
        \fi%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=\pgfmathresult\relax\pgfmath@%
        \edef\pgfmathresult{\the\c@pgfmath@counta}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% mod function.
%
\pgfmathdeclarefunction{mod}{2}{%
  \begingroup%
    \pgfmath@xa#1pt%
    \pgfmath@xb#2pt%
    \pgfmath@x\pgfmath@xa%
    \c@pgfmath@counta\pgfmath@xa%
    \c@pgfmath@countb\pgfmath@xb%
    \divide\c@pgfmath@counta\c@pgfmath@countb%
    \multiply\pgfmath@xb\c@pgfmath@counta%
    \advance\pgfmath@x-\pgfmath@xb%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% Mod function (never negative).
%
\pgfmathdeclarefunction{Mod}{2}{%
    \begingroup%
        \pgfmathmod@{#1}{#2}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \advance\pgfmath@x by#2pt\relax%
        \fi%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% abs function.
%
\pgfmathdeclarefunction{abs}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \pgfmath@x-\pgfmath@x%
        \fi%
    \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% sign(x)
\pgfmathdeclarefunction{sign}{1}{%
  \begingroup
    \ifdim#1pt>0sp %
      \def\pgfmathresult{1}%
    \else
      \ifdim#1pt=0sp %
        \def\pgfmathresult{0}%
      \else
        \def\pgfmathresult{-1}%
      \fi
    \fi
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}

% e constant.
%
\pgfmathdeclarefunction{e}{0}{\def\pgfmathresult{2.718281828}}

% ln function.
%
% This is based on an algorithm due to Rouben Rostamian and
% uses coefficients contributed by Alain Matthes.
%
\pgfmathdeclarefunction{ln}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x>0pt\else%
            \pgfmath@error{I cannot calculate the logarithm of `#1'}{}%
        \fi%
        \c@pgfmath@counta=0\relax%
        \ifdim\pgfmath@x>2pt\relax%
            \ifdim\pgfmath@x<128pt\relax%
                \ifdim\pgfmath@x<8pt\relax%
                    \ifdim\pgfmath@x<4pt\relax%
                        \divide\pgfmath@x by2\relax%
                        \c@pgfmath@counta=1\relax%
                    \else%
                        \divide\pgfmath@x by4\relax%
                        \c@pgfmath@counta=2\relax%
                    \fi%
                \else%
                    \ifdim\pgfmath@x<32pt\relax%
                        \ifdim\pgfmath@x<16pt\relax%
                            \divide\pgfmath@x by8\relax%
                            \c@pgfmath@counta=3\relax%
                        \else%
                            \divide\pgfmath@x by16\relax%
                            \c@pgfmath@counta=4\relax%
                        \fi%
                    \else%
                        \ifdim\pgfmath@x<64pt\relax%
                            \divide\pgfmath@x by32\relax%
                            \c@pgfmath@counta=5\relax%
                        \else%
                            \divide\pgfmath@x by64\relax%
                            \c@pgfmath@counta=6\relax%
                        \fi%
                    \fi%
                \fi%
            \else%
                \ifdim\pgfmath@x<2048pt\relax%
                    \ifdim\pgfmath@x<512pt\relax%
                        \ifdim\pgfmath@x<256pt\relax%
                            \divide\pgfmath@x by128\relax%
                            \c@pgfmath@counta=7\relax%
                        \else%
                            \divide\pgfmath@x by256\relax%
                            \c@pgfmath@counta=8\relax%
                        \fi%
                    \else%
                        \ifdim\pgfmath@x<1024pt\relax%
                            \divide\pgfmath@x by512\relax%
                            \c@pgfmath@counta=9\relax%
                        \else%
                            \divide\pgfmath@x by1024\relax%
                            \c@pgfmath@counta=10\relax%
                        \fi%
                    \fi%
                \else%
                    \ifdim\pgfmath@x<8192pt\relax%
                        \ifdim\pgfmath@x<4096pt\relax%
                            \divide\pgfmath@x by2048\relax%
                            \c@pgfmath@counta=11\relax%
                        \else%
                            \divide\pgfmath@x by4096\relax%
                            \c@pgfmath@counta =12\relax%
                        \fi%
                    \else%
                        \divide\pgfmath@x by8192\relax%
                        \c@pgfmath@counta=13\relax%
                    \fi%
                \fi%
            \fi%
        \else%
            \ifdim\pgfmath@x<1pt\relax%
                \ifdim\pgfmath@x>0.0078125pt\relax% 2^-7
                    \ifdim\pgfmath@x>0.125pt\relax% 2^-3
                        \ifdim\pgfmath@x>0.5pt\relax% 2^-1
                            \multiply\pgfmath@x by2\relax%
                            \c@pgfmath@counta=-1\relax%
                        \else%
                            \multiply\pgfmath@x by4\relax%
                            \c@pgfmath@counta=-2\relax%
                        \fi%
                    \else%
                        \ifdim\pgfmath@x>0.03125pt\relax% 2^-5
                            \ifdim\pgfmath@x>0.0625pt\relax%
                                \multiply\pgfmath@x by8\relax%
                                \c@pgfmath@counta=-3\relax%
                            \else%
                                \multiply\pgfmath@x by16\relax%
                                \c@pgfmath@counta=-4\relax%
                            \fi%
                        \else%
                            \ifdim\pgfmath@x>0.015625pt\relax% 2^-6
                                \multiply\pgfmath@x by32\relax%
                                \c@pgfmath@counta=-5\relax%
                            \else%
                                \multiply\pgfmath@x by64\relax%
                                \c@pgfmath@counta=-6\relax%
                            \fi%
                        \fi%
                    \fi%
                \else%
                    \ifdim\pgfmath@x>0.00048828125pt\relax% 2^-11
                        \ifdim\pgfmath@x>0.001953125pt\relax% 2^-9
                            \ifdim\pgfmath@x>0.00390625pt\relax% 2^-8
                                \multiply\pgfmath@x by128\relax%
                                \c@pgfmath@counta=-7\relax%
                            \else%
                                \multiply\pgfmath@x by256\relax%
                                \c@pgfmath@counta=-8\relax%
                            \fi%
                        \else%
                            \ifdim\pgfmath@x>0.0009765625pt\relax% 2^-10
                                \multiply\pgfmath@x by512\relax%
                                \c@pgfmath@counta=-9\relax%
                            \else%
                                \multiply\pgfmath@x by1024\relax%
                                \c@pgfmath@counta=-10\relax%
                            \fi%
                        \fi%
                    \else%
                        \ifdim\pgfmath@x>0.0001220703125pt\relax% 2^13
                            \ifdim\pgfmath@x>0.0002441406256pt\relax% 2^12
                                \multiply\pgfmath@x by2048\relax%
                                \c@pgfmath@counta=-11\relax%
                            \else%
                                \multiply\pgfmath@x by4096\relax%
                                \c@pgfmath@counta=-12\relax%
                            \fi%
                        \else%
                            \multiply\pgfmath@x by8192\relax%
                            \c@pgfmath@counta=-13\relax%
                        \fi%
                    \fi%
                \fi%
            \fi%
        \fi%
        %
        % Use A+(B+(C+(D+(E+F*x)*x)*x)*x)*x
        %
        % where:
        % A = -2.787927935
        % B =  5.047861502
        % C = -3.489886985
        % D =  1.589480044
        % E = -.4025153233
        % F =  0.04300521312
        %
        \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@x=0.04300521312\pgfmath@x%
        \advance\pgfmath@x by-.4025153233pt\relax%
        \pgfmath@x=\pgfmath@temp\pgfmath@x%
        \advance\pgfmath@x by1.589480044pt\relax%
        \pgfmath@x=\pgfmath@temp\pgfmath@x%
        \advance\pgfmath@x by-3.489886985pt\relax%
        \pgfmath@x=\pgfmath@temp\pgfmath@x%
        \advance\pgfmath@x by5.047861502pt\relax%
        \pgfmath@x=\pgfmath@temp\pgfmath@x%
        \advance\pgfmath@x by-2.787927935pt\relax%
        \advance\pgfmath@x by\c@pgfmath@counta pt\relax%
        \pgfmath@x=0.6931471806\pgfmath@x%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% log2 function.
%
\pgfmathdeclarefunction{log2}{1}{%
    \begingroup%
        \pgfmathln@{#1}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmath@x=1.442695041\pgfmath@x% 1/ln(2).
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% log10 function
%
\pgfmathdeclarefunction{log10}{1}{%
    \begingroup%
        \pgfmathln@{#1}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmath@x=0.43429441\pgfmath@x% 1/ln(10).
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% This is needed since \pgfmathlog2 and \pgfmathlog10 are not legal macro names
\expandafter\let\expandafter\pgfmathlogtwo\csname pgfmathlog2\endcsname
\expandafter\let\expandafter\pgfmathlogtwo@\csname pgfmathlog2@\endcsname
\expandafter\let\expandafter\pgfmathlogten\csname pgfmathlog10\endcsname
\expandafter\let\expandafter\pgfmathlogten@\csname pgfmathlog10@\endcsname

% exp function.
%
\pgfmathdeclarefunction{exp}{1}{%
  \begingroup
    \pgfmath@xc=#1pt\relax
    \pgfmath@yc=#1pt\relax
    \ifdim\pgfmath@xc<-9pt
      \pgfmath@x=1sp\relax
    \else
      \ifdim\pgfmath@xc<0pt
        \pgfmath@xc=-\pgfmath@xc
      \fi
      \pgfmath@x=1pt\relax
      \pgfmath@xa=1pt\relax
      \pgfmath@xb=\pgfmath@x
      \pgfmathloop%
        \divide\pgfmath@xa by\pgfmathcounter
        \pgfmath@xa=\pgfmath@tonumber\pgfmath@xc\pgfmath@xa%
        \advance\pgfmath@x by\pgfmath@xa
      \ifdim\pgfmath@x=\pgfmath@xb
      \else
        \pgfmath@xb=\pgfmath@x
      \repeatpgfmathloop%
      \ifdim\pgfmath@yc<0pt
        \pgfmathreciprocal@{\pgfmath@tonumber\pgfmath@x}%
        \pgfmath@x=\pgfmathresult pt\relax
      \fi
    \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup
}

% sqrt function.
%
\pgfmathdeclarefunction{sqrt}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \pgfmath@error{I cannot calculate the square-root of the negative number `#1'}{}%
        \else%
            \ifdim\pgfmath@x<10pt\relax%
                \def\pgfmath@zeros{0}%
                \def\pgfmath@targetiterations{1}%
            \else%
                \ifdim\pgfmath@x<100pt\relax%
                    \def\pgfmath@zeros{}%
                    \def\pgfmath@targetiterations{1}%
                \else%
                    \ifdim\pgfmath@x<1000pt\relax%
                        \def\pgfmath@zeros{0}%
                        \def\pgfmath@targetiterations{2}%
                    \else%
                        \ifdim\pgfmath@x<10000pt\relax%
                            \def\pgfmath@zeros{}%
                            \def\pgfmath@targetiterations{2}%
                    \else%
                            \def\pgfmath@zeros{0}%
                            \def\pgfmath@targetiterations{3}%
        \fi\fi\fi\fi\fi%
        \edef\pgfmath@temp{\pgfmath@zeros\pgfmath@tonumber{\pgfmath@x}}%
        \expandafter\pgfmath@sqrt@\pgfmath@temp\pgfmath@%
}
\def\pgfmath@sqrt@#1.#2\pgfmath@{\pgfmath@@sqrt@#1#2\pgfmath@empty\pgfmath@empty\pgfmath@}

\def\pgfmath@@sqrt@#1#2{%
        \c@pgfmath@countb=#1#2\relax%
        \ifnum\c@pgfmath@countb>35\relax%
            \ifnum\c@pgfmath@countb>63\relax%
                \ifnum\c@pgfmath@countb>80\relax%
                    \c@pgfmath@counta=9\relax%
                \else%
                    \c@pgfmath@counta=8\relax%
                \fi%
            \else%
                \ifnum\c@pgfmath@countb>48\relax%
                    \c@pgfmath@counta=7\relax%
                \else%
                    \c@pgfmath@counta=6\relax%
                \fi%
            \fi%
        \else%
            \ifnum\c@pgfmath@countb>15\relax%
                \ifnum\c@pgfmath@countb>24\relax%
                    \c@pgfmath@counta5\relax%
                \else%
                    \c@pgfmath@counta=4\relax%
                \fi%
            \else%
                \ifnum\c@pgfmath@countb>3\relax%
                    \ifnum\c@pgfmath@countb>8\relax%
                        \c@pgfmath@counta=3\relax%
                    \else%
                        \c@pgfmath@counta=2\relax%
                    \fi%
                \else%
                    \ifnum\c@pgfmath@countb>0\relax%
                        \c@pgfmath@counta=1\relax%
                    \else%
                        \c@pgfmath@counta=0\relax%
                    \fi%
                \fi%
            \fi%
        \fi%
        \edef\pgfmath@root{\the\c@pgfmath@counta}%
        \edef\pgfmath@rootspecial{\the\c@pgfmath@counta}%
        \multiply\c@pgfmath@counta by-\c@pgfmath@counta\relax%
        \advance\c@pgfmath@counta by#1#2\relax%
        \edef\pgfmath@remainder{\the\c@pgfmath@counta}%
        \pgfmath@@@sqrt@%
}

\def\pgfmath@@@sqrt@#1#2{%
        \ifx\pgfmath@empty#1%
            \edef\pgfmath@remainder{\pgfmath@remainder00}%
            \def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
        \else%
            \ifx\pgfmath@empty#2%
                \edef\pgfmath@remainder{\pgfmath@remainder#10}%
                \def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
            \else%
                \edef\pgfmath@remainder{\pgfmath@remainder#1#2}%
                \def\pgfmath@tokens{}%
        \fi\fi%
        \c@pgfmath@counta=\pgfmath@rootspecial\relax%
        \multiply\c@pgfmath@counta by20\relax%
        \c@pgfmath@countb=\c@pgfmath@counta%
        \multiply\c@pgfmath@countb by6\relax%
        \advance\c@pgfmath@countb by36\relax%
        \c@pgfmath@countc=\c@pgfmath@counta%
        \multiply\c@pgfmath@countc by2\relax%
        \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
            \advance\c@pgfmath@countb by-\c@pgfmath@countc%
            \advance\c@pgfmath@countb by-20\relax%
            \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                \advance\c@pgfmath@countb by-\c@pgfmath@countc%
                \advance\c@pgfmath@countb by-12\relax%
                \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                    \advance\c@pgfmath@countb by-\c@pgfmath@counta%
                    \advance\c@pgfmath@countb by-3\relax%
                    \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                        \def\pgfmath@digit{0}%
                    \else%
                        \def\pgfmath@digit{1}%
                    \fi%
                \else%
                    \advance\c@pgfmath@countb by\c@pgfmath@counta%
                    \advance\c@pgfmath@countb by5\relax%
                    \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                        \def\pgfmath@digit{2}%
                    \else%
                        \def\pgfmath@digit{3}%
                    \fi%
                \fi%
            \else%
                \advance\c@pgfmath@countb by\c@pgfmath@counta%
                \advance\c@pgfmath@countb by9\relax%
                \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                    \def\pgfmath@digit{4}%
                \else%
                    \def\pgfmath@digit{5}%
                \fi%
            \fi%
        \else%
            \advance\c@pgfmath@countb by\c@pgfmath@countc%
            \advance\c@pgfmath@countb by28\relax%
            \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                \advance\c@pgfmath@countb by-\c@pgfmath@counta%
                \advance\c@pgfmath@countb by-15\relax%
                \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                    \def\pgfmath@digit{6}%
                \else%
                    \def\pgfmath@digit{7}%
                \fi%
            \else%
                \advance\c@pgfmath@countb by\c@pgfmath@counta%
                \advance\c@pgfmath@countb by17\relax%
                \ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
                    \def\pgfmath@digit{8}%
                \else%
                    \def\pgfmath@digit{9}%
                \fi%
            \fi%
        \fi%
        \edef\pgfmath@rootspecial{\pgfmath@rootspecial\pgfmath@digit}%
        \advance\c@pgfmath@counta by\pgfmath@digit\relax%
        \multiply\c@pgfmath@counta by-\pgfmath@digit\relax%
        \advance\c@pgfmath@counta by\pgfmath@remainder\relax%
        \edef\pgfmath@remainder{\the\c@pgfmath@counta}%
        \c@pgfmath@counta=\pgfmath@targetiterations\relax%
        \advance\c@pgfmath@counta by-1\relax%
        \edef\pgfmath@targetiterations{\the\c@pgfmath@counta}%
        \ifnum\c@pgfmath@counta=0\relax%
            \edef\pgfmath@root{\pgfmath@root.\pgfmath@digit}%
        \else%
            \edef\pgfmath@root{\pgfmath@root\pgfmath@digit}%
        \fi%
        \ifnum\c@pgfmath@counta=-4\relax% -n+1 digits of precision.
            \let\pgfmath@next\pgfmath@sqrt@end%
        \else%
            \let\pgfmath@next\pgfmath@@@sqrt@%
        \fi%
        \expandafter\pgfmath@next\pgfmath@tokens%
}

\def\pgfmath@sqrt@end#1\pgfmath@{%
        \edef\pgfmathresult{\pgfmath@root}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup}

% \pgfmathpow
%
% Calculates #1 ^ #2
%
\pgfmathdeclarefunction{pow}{2}{%
  \begingroup%
    \pgfmath@xa=#1pt%
    \pgfmath@xb=#2pt%
    \ifdim\pgfmath@xa=0pt\relax%
      \ifdim\pgfmath@xb=0pt\relax%
        \pgfmath@x=1pt\relax%
      \else%
        \pgfmath@x=0pt\relax%
      \fi%
    \else%
      \afterassignment\pgfmath@x%
      \expandafter\c@pgfmath@counta\the\pgfmath@xb\relax%
      \ifnum\c@pgfmath@counta<0\relax%
        \c@pgfmath@counta=-\c@pgfmath@counta%
        \pgfmathreciprocal@{#1}%
        \pgfmath@xa=\pgfmathresult pt\relax%
      \fi
      \ifdim\pgfmath@x=0pt\relax%
        \pgfmath@x=1pt\relax%
        \pgfmathloop%
          \ifnum\c@pgfmath@counta>0\relax%
            \ifodd\c@pgfmath@counta%
              \pgfmath@x=\pgfmath@tonumber{\pgfmath@x}\pgfmath@xa%
            \fi
            \ifnum\c@pgfmath@counta>1\relax%
              \pgfmath@xa=\pgfmath@tonumber{\pgfmath@xa}\pgfmath@xa%
            \fi%
            \divide\c@pgfmath@counta by2\relax%
        \repeatpgfmathloop%
      \else%
        \pgfmathln@{#1}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmath@x=\pgfmath@tonumber{\pgfmath@xb}\pgfmath@x%
        \pgfmathexp@{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@x=\pgfmathresult pt\relax%
      \fi%
    \fi
    \pgfmath@returnone\pgf@x%
  \endgroup%
}

% factorial function.
%
\pgfmathdeclarefunction{factorial}{1}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \c@pgfmath@counta=#1\relax\pgfmath@%
        \pgfmath@x=1pt\relax%
        \pgfmathloop%
        \ifnum\c@pgfmath@counta<2\relax%
        \else%
            \multiply\pgfmath@x by\c@pgfmath@counta%
            \advance\c@pgfmath@counta by-1\relax%
        \repeatpgfmathloop%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% Local Variables:
% coding: undecided-unix
% End:


==> pgfmathfunctions.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% Declare a function for the parser.
%
% #1 - the name of the function.
% #2 - arity (or ... for variable arguments).
% #3 - the code for the function.
%
% Use \pgfmathdeclarefunction* to force a redefinition if the function exists already.
\def\pgfmathdeclarefunction{\pgfmath@ifnextchar*\pgfmathdeclarefunction@force\pgfmathdeclarefunction@check}
\def\pgfmathdeclarefunction@check#1{%
    \expandafter\ifx\csname pgfmath@function@#1\endcsname\relax\else%
        \pgfmath@error{The function `#1' already exists}{}%
    \fi%
    \pgfmath@declarefunction{#1}%
}
\def\pgfmathdeclarefunction@force*{\pgfmath@declarefunction}%

\def\pgfmathredeclarefunction#1#2{%
    \expandafter\ifx\csname pgfmath@function@#1\endcsname\relax%
        \pgfmath@error{The function `#1' does not exist}{}%
    \else%
    % was: \pgfmath@namedef{pgfmath#1@}{#2}% TT
    \edef\pgf@marshal{\noexpand\pgfmathdeclarefunction*{#1}{\csname    pgfmath@operation@#1@arity\endcsname}}%
    \pgf@marshal{#2}%
    \fi%
}

\def\pgfmath@declarefunction#1#2{%
    \pgfmath@namedef{pgfmath@function@#1}{#1}%
    \pgfmath@namedef{pgfmath@operation@#1@type}{function}%
    \pgfmath@namedef{pgfmath@operation@#1@arity}{#2}%
    \pgfmath@namedef{pgfmath@operation@#1@infix}{#1}%
    \pgfmath@namedef{pgfmath@operation@#1@precedence}{1000}%
    \expandafter\ifx\csname pgfmath@operation@#1@arity\endcsname\pgfmath@dots%
        \pgfmath@namedef{pgfmath@operation@#1@arity}{1}%
    \else%
        \ifnum\csname pgfmath@operation@#1@arity\endcsname>9\relax%
                \pgfmath@namedef{pgfmath@operation@#1@arity}{1}%
        \fi%
    \fi%
    \edef\pgfmath@marshal{%
        \noexpand\pgfmath@@declarefunction%
        {\expandafter\noexpand\csname pgfmath#1\endcsname}%
        {\expandafter\noexpand\csname pgfmath#1@\endcsname}%
        {\csname pgfmath@operation@#1@arity\endcsname}%
    }%
    \pgfkeysvalueof{/pgf/declare function/execute at begin function}%
    \pgfmath@marshal%
}

% #1 - \pgfmath<name>.
% #2 - \pgfmath<name>@.
% #3 - arity.
% #4 - code for function <name>.
%
\def\pgfmath@@declarefunction#1#2#3#4{% Function of arity 0 - 9.
    \pgfkeysvalueof{/pgf/declare function/execute at end function}%
    \ifcase#3\relax%
        \def#1{#2}%
        \def\pgfmath@@head{\def#2}%
    \or
        \def#1##1{\pgfmathparse{##1}\expandafter#2\expandafter{\pgfmathresult}}%
        \def\pgfmath@@head{\def#2####1}%
    \else%
        \pgfmath@toks={}%
        \pgfmathloop%
        \ifnum\pgfmathcounter>#3\relax%
        \else%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@char@hash}%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmathcounter}%
        \repeatpgfmathloop%
        \edef\pgfmath@head{\noexpand\def\noexpand#1\the\pgfmath@toks}%
        \edef\pgfmath@@head{\noexpand\def\noexpand#2\the\pgfmath@toks}%
        \pgfmath@toks={}%
        \def\pgfmath@arguments{}%
        \pgfmathloop%
        \ifnum\pgfmathcounter>#3\relax%
        \else%
            \pgfmath@addto@toks{\pgfmathparse}%
            \expandafter\expandafter\expandafter\pgfmath@addto@toks%
                \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
                    {\expandafter\pgfmath@char@hash\pgfmathcounter}}%
            \pgfmath@addto@toks{\let}%
            \expandafter\pgfmath@addto@toks\expandafter{%
                \csname pgfmath@argument@\pgfmathcounter\endcsname=\pgfmathresult}%
            \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
                \pgfmath@arguments\expandafter\expandafter\expandafter{\expandafter%
                    \pgfmath@arguments\expandafter{\csname pgfmath@argument@\pgfmathcounter\endcsname}}%
        \repeatpgfmathloop%
        \expandafter\pgfmath@addto@toks\expandafter{\expandafter#2\pgfmath@arguments}%
        \edef\pgfmath@body{{\the\pgfmath@toks}}%
        \expandafter\pgfmath@head\pgfmath@body%
    \fi%
    \pgfmath@@head{#4}%
}

\def\pgfmath@addto@toks#1{%
    \edef\pgfmath@toks@expanded{\the\pgfmath@toks}%
    \expandafter\pgfmath@toks\expandafter{\pgfmath@toks@expanded#1}}

% Key for declaring local functions.
%
\pgfkeys{%
    /pgf/declare function/.code={%
        \pgfmath@local@functions#1@=@;%
    },
    /pgf/declare function/execute at begin function/.initial={},
    /pgf/declare function/execute at end function/.initial={},
    /pgf/declare function/ignore spaces/.is choice,
    /pgf/declare function/ignore spaces/.default=true,
    /pgf/declare function/ignore spaces/true/.style={%
        /pgf/declare function/execute at begin function={%
            \begingroup
            \catcode`\^^I=9\relax
            \catcode`\ =9\relax
            \catcode`\~=10\relax
            \endlinechar=`\ \relax
        },
        /pgf/declare function/execute at end function={%
            \endgroup
        },
    },
    /pgf/declare function/ignore spaces/false/.style={%
        /pgf/declare function/execute at begin function={},
        /pgf/declare function/execute at end function={},
    },
}

\def\pgfmath@local@gobbleone#1{}
\def\pgfmath@local@at{@}%

\def\pgfmath@local@functions{%
    \pgfutil@ifnextchar x{\pgfmath@local@@functions}{\pgfmath@local@@functions}%
}

\def\pgfmath@local@@functions#1=#2;{%
    \def\pgfmath@local@temp{#1}%
    \ifx\pgfmath@local@temp\pgfmath@local@at%
        \let\pgfmath@local@next=\relax%
    \else%
        \pgfmath@local@function#1=#2;%
        \let\pgfmath@local@next=\pgfmath@local@functions%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function{%
    \let\pgfmath@local@name=\pgfutil@empty%
    \let\pgfmath@local@args=\pgfutil@empty%
    \let\pgfmath@local@body=\pgfutil@empty%
    \pgfmath@local@@function}

\def\pgfmath@local@@function#1{%
    \if#1=%
        \let\pgfmath@local@next=\pgfmath@local@function@body%
    \else%
        \if#1(%
            \let\pgfmath@local@next=\pgfmath@local@function@args%
        \else%
            \expandafter\def\expandafter\pgfmath@local@name\expandafter{\pgfmath@local@name#1}%
            \let\pgfmath@local@next=\pgfmath@local@@function%
        \fi%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function@args#1){%
    \def\pgfmath@local@args{#1}%
    \pgfmath@local@@function}

\def\pgfmath@local@function@body#1;{%
    \def\pgfmath@local@body{#1}%
    \begingroup%
        \c@pgf@counta=0\relax%
        \ifx\pgfmath@local@args\pgfmath@empty%
            \expandafter\pgfmath@toks\expandafter=\expandafter{\pgfmath@local@body}%
        \else%
            \pgfmath@toks={}%
            \expandafter\pgfmath@local@function@@body\pgfmath@local@args,,%
        \fi%
        \xdef\pgfmath@local@temp{%
            \noexpand\pgfmathnotifynewdeclarefunction{\pgfmath@local@name}{\the\c@pgf@counta}%
                {\the\pgfmath@toks}%
        }%
    \endgroup%
    \pgfmath@local@temp%
}

% #1: the name
% #2: the number of arguments <n>
% #3: a math expression containing '#1', '#2', ... ,'#'<n>
% This callback is overwritten by pgflibraryluamath.
\def\pgfmathnotifynewdeclarefunction#1#2#3{%
    \pgfmathdeclarefunction{#1}{#2}{\pgfmathparse{#3}}%
}%

\def\pgfmath@local@function@@body#1,{%
    \def\pgfmath@local@test{#1}%
    \ifx\pgfmath@local@test\pgfutil@empty%
        \let\pgfmath@local@next=\relax%
    \else%
        \edef\pgfmath@local@var@string{@\expandafter\pgfmath@local@gobbleone\string#1}%
        \advance\c@pgf@counta by1\relax%
        \expandafter\expandafter\expandafter\pgfmath@toks\expandafter\expandafter\expandafter=%
            \expandafter\expandafter\expandafter{\expandafter\pgfmath@char@hash\the\c@pgf@counta}%
        \edef#1{\the\pgfmath@toks}%
        \pgfmath@toks={}%
        \expandafter\pgfmath@local@function@@@body\pgfmath@local@body @%
        \edef\pgfmath@local@body{\the\pgfmath@toks}%
        \let\pgfmath@local@next=\pgfmath@local@function@@body%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function@@@body{%
    \pgfutil@ifnextchar\bgroup{\pgfmath@local@function@@@body@bgroup}%
        {\pgfmath@local@function@@@body@nobgroup}}%

\def\pgfmath@local@function@@@body@bgroup#1{%
    \begingroup%
        \pgfmath@toks={}%
        \pgfmath@local@function@@@body#1 @%
        \xdef\pgfmath@local@temp{{\the\pgfmath@toks}}%
    \endgroup%
    \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@local@temp}%
    \pgfmath@local@function@@@body%
}

\def\pgfmath@local@function@@@body@nobgroup#1{%
    \ifx#1@%
        \let\pgfmath@local@next=\relax%
    \else%
        \let\pgfmath@local@next=\pgfmath@local@function@@@body%
        \edef\pgfmath@local@var@@string{@\expandafter\pgfmath@local@gobbleone\string#1}%
        \ifx\pgfmath@local@var@@string\pgfmath@local@var@string%
            \expandafter\pgfmath@addto@toks\expandafter{#1}%
        \else%
            \edef\pgfmath@local@temp{\the\pgfmath@toks}%
            \pgfmath@toks={#1}%
            \edef\pgfmath@local@@temp{\the\pgfmath@toks}%
            \expandafter\pgfmath@toks\expandafter=\expandafter{\pgfmath@local@temp}%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@local@@temp}%
        \fi%
    \fi%
    \pgfmath@local@next%
}

% Allows to define 'x' as some \TeX command '#2'.
\def\pgfmathdeclarepseudoconstant#1#2{%
    \pgfmathdeclarefunction*{#1}{0}{#2}%
}%
% Redefines a pseudo constant '#1'.
\def\pgfmathredeclarepseudoconstant#1#2{%
    \pgfmathredeclarefunction{#1}{#2}%
}%

\input pgfmathfunctions.basic.code.tex
\input pgfmathfunctions.trigonometric.code.tex
\input pgfmathfunctions.random.code.tex
\input pgfmathfunctions.comparison.code.tex
\input pgfmathfunctions.base.code.tex
\input pgfmathfunctions.round.code.tex
\input pgfmathfunctions.misc.code.tex
\input pgfmathfunctions.integerarithmetics.code.tex



% Local Variables:
% tab-width: 2
% End:


==> pgfmathfunctions.comparison.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 1.4142135 11/8/2008

\pgfmathdeclarefunction{greater}{2}{%
  \begingroup%
    \ifdim#1pt>#2pt\relax%
        \def\pgfmathresult{1}%
    \else%
      \def\pgfmathresult{0}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}
\let\pgfmathgreaterthan=\pgfmathgreater

\pgfmathdeclarefunction{less}{2}{%
  \begingroup%
    \ifdim#1pt<#2pt\relax%
        \def\pgfmathresult{1}%
    \else%
      \def\pgfmathresult{0}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}
\let\pgfmathlessthan=\pgfmathless

\pgfmathdeclarefunction{equal}{2}{%
  \begingroup%
    \ifdim#1pt=#2pt\relax%
        \def\pgfmathresult{1}%
    \else%
      \def\pgfmathresult{0}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}
\let\pgfmathequalto=\pgfmathequal


% approxequalto function from Christian Feuersaenger.
%
\newif\ifpgfmathcomparison
\pgfmathdeclarefunction{approxequalto}{2}{%
    \begingroup%
        \pgfmath@x=#1pt\relax%
        \pgfmath@y=#2pt\relax%
        \advance\pgfmath@x by-\pgfmath@y%
        \ifdim\pgfmath@x<0pt\relax%
            \multiply\pgfmath@x by-1\relax%
        \fi
        \ifdim\pgfmath@x<0.0001pt\relax%
            \def\pgfmathresult{1.0}%
            \global\pgfmathcomparisontrue%
        \else%
            \def\pgfmathresult{0.0}%
            \global\pgfmathcomparisonfalse%
        \fi%
    \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}



% ifthenelse function.
%
\pgfmathdeclarefunction{ifthenelse}{3}{%
    \begingroup%
        \ifdim#1pt=0.0pt\relax%
            \expandafter\def\expandafter\pgfmathresult\expandafter{#3}%
        \else%
            \expandafter\def\expandafter\pgfmathresult\expandafter{#2}%
        \fi%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% notequal function.
%
\pgfmathdeclarefunction{notequal}{2}{%
  \begingroup%
    \ifdim#1pt=#2pt\relax%
            \def\pgfmathresult{0}%
    \else%
      \def\pgfmathresult{1}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% notless function.
%
\pgfmathdeclarefunction{notless}{2}{%
  \begingroup%
    \ifdim#1pt<#2pt\relax%
            \def\pgfmathresult{0}%
    \else%
      \def\pgfmathresult{1}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% notgreater function.
%
\pgfmathdeclarefunction{notgreater}{2}{%
  \begingroup%
    \ifdim#1pt>#2pt\relax%
            \def\pgfmathresult{0}%
    \else%
      \def\pgfmathresult{1}%
    \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% and function.
%
\pgfmathdeclarefunction{and}{2}{%
  \begingroup%
      \def\pgfmathresult{1}%
    \ifdim#1pt=0pt\relax%
            \def\pgfmathresult{0}%
        \else%
            \ifdim#2pt=0pt\relax%
                \def\pgfmathresult{0}%
            \fi%
        \fi%
     \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% or function.
%
\pgfmathdeclarefunction{or}{2}{%
  \begingroup%
    \def\pgfmathresult{0}%
    \ifdim#1pt=0pt\relax%
            \ifdim#2pt=0pt\relax%
            \else%
                \def\pgfmathresult{1}%
            \fi%
        \else%
            \def\pgfmathresult{1}%
        \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% not function.
%
\pgfmathdeclarefunction{not}{1}{%
  \begingroup%
    \ifdim#1pt=0pt\relax%
            \def\pgfmathresult{1}%
        \else%
            \def\pgfmathresult{0}%
        \fi%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% true function.
%
\pgfmathdeclarefunction{true}{0}{\def\pgfmathresult{1}}

% false function.
%
\pgfmathdeclarefunction{false}{0}{\def\pgfmathresult{0}}


==> pgfmathfunctions.integerarithmetics.code.tex <==
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% Macros contributed by Alain Matthes and adapted by CJ
\pgfmathdeclarefunction{gcd}{2}{%
  \begingroup
    \pgfmathcontinuelooptrue
    \pgfmath@xa=#1pt
    \pgfmath@xb=#2pt
    \ifdim\pgfmath@xa=0pt\relax
      \pgfmathcontinueloopfalse
      \pgfmath@xa=\pgfmath@xb
    \fi
    \ifdim\pgfmath@xb=0pt\relax
      \pgfmathcontinueloopfalse
      \pgfmath@xb=\pgfmath@xa
    \fi
    \ifdim\pgfmath@xa<0pt\relax
      \pgfmath@xa=-\pgfmath@xa
    \fi
    \ifdim\pgfmath@xb<0pt\relax
      \pgfmath@xb=-\pgfmath@xb
    \fi
    \loop
      \ifpgfmathcontinueloop
      \ifdim\pgfmath@xa=\pgfmath@xb
        \pgfmathcontinueloopfalse
      \else
        \ifdim\pgfmath@xa>\pgfmath@xb
          \advance\pgfmath@xa by-\pgfmath@xb
        \else
          \advance\pgfmath@xb by-\pgfmath@xa
        \fi
      \fi
    \repeat
    \pgfmathparse{int(\pgfmath@xa)}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup}

\newif\ifpgfmath@isprime@unknown
\newif\ifpgfmath@isprime

\pgfmathdeclarefunction{isprime}{1}{%
  \begingroup
    \pgfmath@isprime@unknowntrue
    \pgfmathsetcount\c@pgfmath@counta{abs(int(#1))}%
    \ifcase\c@pgfmath@counta\relax
      % |#1| = 0
      \pgfmath@isprimefalse
      \pgfmath@isprime@unknownfalse
    \or
      % |#1| = 1
      \pgfmath@isprimefalse
      \pgfmath@isprime@unknownfalse
    \or
      % |#1| = 2
      \pgfmath@isprimetrue
      \pgfmath@isprime@unknownfalse
    \or
      % |#1| = 3
      \pgfmath@isprimetrue
      \pgfmath@isprime@unknownfalse
    \else
      % |#1| > 3
      \ifodd\c@pgfmath@counta\relax
      \else
        \pgfmath@isprimefalse
        \pgfmath@isprime@unknownfalse
      \fi
    \fi
    \ifpgfmath@isprime@unknown
      \c@pgfmath@countd=3
      \pgfmath@isprimetrue
      \pgfmathloop
        \c@pgfmath@countb=\c@pgfmath@counta
        \divide\c@pgfmath@countb by\c@pgfmath@countd
        \ifnum\c@pgfmath@countb>\c@pgfmath@countd
          \pgfmath@isprime@unknowntrue
        \else
          \pgfmath@isprime@unknownfalse
        \fi
        \multiply\c@pgfmath@countb by\c@pgfmath@countd
        \ifnum\c@pgfmath@countb=\c@pgfmath@counta
          \global\pgfmath@isprimefalse
          \pgfmath@isprime@unknownfalse
        \fi
      \ifpgfmath@isprime@unknown\advance\c@pgfmath@countd by 2
      \repeatpgfmathloop
    \fi
    \ifpgfmath@isprime
      \def\pgfmathresult{1}%
    \else
      \def\pgfmathresult{0}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
  \endgroup}

\pgfmathdeclarefunction{isodd}{1}{%
  \begingroup
    \pgfmathsetcount\c@pgfmath@counta{abs(int(#1))}%
    \ifodd\c@pgfmath@counta
      \def\pgfmathresult{1}%
    \else
      \def\pgfmathresult{0}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
  \endgroup}

\pgfmathdeclarefunction{iseven}{1}{%
  \begingroup
    \pgfmathsetcount\c@pgfmath@counta{abs(int(#1))}%
    \ifodd\c@pgfmath@counta
      \def\pgfmathresult{0}%
    \else
      \def\pgfmathresult{1}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
  \endgroup}

\endinput


==> pgfmathfunctions.misc.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 1.414213 29/9/2007

% veclen function adapted from ideas due to Rouben Rostamian.
%
% Calculate the Euclidean length of a 2D vector.
%
%
\pgfmathdeclarefunction{veclen}{2}{%
  \begingroup%
    \pgfmath@x#1pt\relax%
    \pgfmath@y#2pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \pgfmath@x-\pgfmath@x%
        \fi%
        \ifdim\pgfmath@y<0pt\relax%
            \pgfmath@y-\pgfmath@y%
        \fi%
        \ifdim\pgfmath@x=0pt\relax%
            \pgfmath@x\pgfmath@y%
        \else%
            \ifdim\pgfmath@y=0pt\relax%
            \else%
                \ifdim\pgfmath@x>\pgfmath@y%
                    \pgfmath@xa\pgfmath@x%
                    \pgfmath@x\pgfmath@y%
                    \pgfmath@y\pgfmath@xa%
                \fi%
                % We use a scaling factor to reduce errors.
                \ifdim\pgfmath@y>10000pt\relax%
                    \c@pgfmath@counta1500\relax%
                \else%
                    \ifdim\pgfmath@y>1000pt\relax%
                        \c@pgfmath@counta150\relax%
                    \else%
                        \ifdim\pgfmath@y>100pt\relax%
                            \c@pgfmath@counta50\relax%
                        \else%
                            \c@pgfmath@counta1\relax%
                        \fi%
                    \fi%
                \fi%
                \divide\pgfmath@x\c@pgfmath@counta\relax%
                \divide\pgfmath@y\c@pgfmath@counta\relax%
                \pgfmathreciprocal@{\pgfmath@tonumber{\pgfmath@y}}%
                \pgfmath@x\pgfmathresult\pgfmath@x%
                \pgfmath@xa\pgfmath@tonumber{\pgfmath@x}\pgfmath@x%
                \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@xa}}%
                %
                % Use A+x^2*(B+x^2*(C+x^2*(D+E*x^2)))
                % where
                % A = +1.000012594
                % B = +0.4993615349
                % C = -0.1195159052
                % D = +0.04453994279
                % E = -0.01019210944
                %
                \pgfmath@x-0.01019210944\pgfmath@xa%
                \advance\pgfmath@x0.04453994279pt\relax%
                \pgfmath@x\pgfmath@temp\pgfmath@x%
                \advance\pgfmath@x-0.1195159052pt\relax%
                \pgfmath@x\pgfmath@temp\pgfmath@x%
                \advance\pgfmath@x0.4993615349pt\relax%
                \pgfmath@x\pgfmath@temp\pgfmath@x%
                \advance\pgfmath@x1.000012594pt\relax%
                \ifdim\pgfmath@y<0pt\relax%
                    \pgfmath@y-\pgfmath@y%
                \fi%
                \pgfmath@x\pgfmath@tonumber{\pgfmath@y}\pgfmath@x%
                % Invert the scaling factor.
                \multiply\pgfmath@x\c@pgfmath@counta\relax%
            \fi%
        \fi%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}

% Hyperbolic functions contributed by Martin Heller.
%
\pgfmathdeclarefunction{cosh}{1}{%
    \begingroup
        \edef\pgfmath@arg{#1}%
        \pgfmathexp@{\pgfmath@arg}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmathexp@{-\pgfmath@arg}%
        \advance\pgfmath@x by\pgfmathresult pt\relax%
        \divide\pgfmath@x by2\relax%
        \pgfmath@returnone\pgfmath@x%
    \endgroup}

\pgfmathdeclarefunction{sinh}{1}{%
    \begingroup
        \edef\pgfmath@arg{#1}%
        \pgfmathexp@{\pgfmath@arg}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmathexp@{-\pgfmath@arg}%
        \advance\pgfmath@x by-\pgfmathresult pt\relax%
        \divide\pgfmath@x by2\relax%
        \pgfmath@returnone\pgfmath@x%
    \endgroup
}%

\pgfmathdeclarefunction{tanh}{1}{%
    \begingroup
        \edef\pgfmath@arg{#1}%
        \pgfmathsinh@{\pgfmath@arg}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmathcosh@{\pgfmath@arg}%
        \pgfmath@y=\pgfmathresult pt\relax%
        \pgfmathdivide@{\pgfmath@tonumber{\pgfmath@x}}{\pgfmath@tonumber{\pgfmath@y}}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \pgfmath@returnone\pgfmath@x%
    \endgroup
}%

% \pgfmathscientific
%
% Return the value of #1e#2
%
% e.g. \pgfmathscientific{1.23456789123}{4}
%
% defines \pgfmathresult as 12345.67891
%
% NB These arguments *are not parsed*, as the long mantissa would be lost.
%
\def\pgfmathscientific#1#2{%
    \begingroup%
        \edef\pgfmath@sci@exponent{#2}%
        \pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \pgfmath@x-\pgfmath@x%
            \edef\pgfmath@sci@sign{-}%
            \expandafter\edef\expandafter\pgfmath@temp\expandafter{\expandafter\pgfmath@gobbleone#1}%
        \else%
            \edef\pgfmath@sci@sign{+}%
            \edef\pgfmath@temp{#1}%
        \fi%
        \expandafter\pgfmath@in@\expandafter.\expandafter{#1}%
        \ifpgfmath@in@%
        \else%
            \edef\pgfmath@temp{\pgfmath@temp.0}%
        \fi%
        \expandafter\pgfmath@scientific@@\pgfmath@temp00000000000\pgfmath@}

\def\pgfmath@scientific@@#1.#2#3#4#5#6{%
        \edef\pgfmath@sci@int{#1}%
        \edef\pgfmath@sci@mantissaA{#2#3#4#5#6}%
        \pgfmath@scientific@@@}

\def\pgfmath@scientific@@@#1#2#3#4#5#6\pgfmath@{%
        \edef\pgfmath@sci@mantissaB{#1#2#3#4#5}%
        \c@pgfmath@counta\pgfmath@sci@exponent\relax%
                \ifnum\c@pgfmath@counta<-4\relax%
                  \pgfmath@x0pt\relax%
                \else%
        \c@pgfmath@countb\c@pgfmath@counta%
        \ifnum\c@pgfmath@counta<0\relax%
            \c@pgfmath@counta-\c@pgfmath@counta%
        \fi%
        \pgfmathpow@{10}{\the\c@pgfmath@counta}%
        \afterassignment\pgfmath@gobbletilpgfmath@
        \c@pgfmath@countc\pgfmathresult\relax\pgfmath@
        \edef\pgfmath@sci@factor{\the\c@pgfmath@countc}%
        \ifnum\c@pgfmath@countb<0\relax%
            % xE-y: easy...
            \pgfmath@x\pgfmath@sci@int.\pgfmath@sci@mantissaA pt\relax%
            \divide\pgfmath@x\pgfmath@sci@factor\relax%
        \else%
            % xE+y:
            % Must do this way so as not lose digits in a long mantissa. Sigh...
            \c@pgfmath@counta\pgfmath@sci@int%
            \c@pgfmath@countb\pgfmath@sci@mantissaA%
            \multiply\c@pgfmath@counta\pgfmath@sci@factor\relax%
            \multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
            \c@pgfmath@countc\c@pgfmath@countb%
            \divide\c@pgfmath@countb100000\relax%
            \advance\c@pgfmath@counta\c@pgfmath@countb%
            \multiply\c@pgfmath@countb100000\relax%
            \advance\c@pgfmath@countc-\c@pgfmath@countb%
            \c@pgfmath@countb\pgfmath@sci@mantissaB\relax%
            \multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
            \divide\c@pgfmath@countb100000\relax%
            \advance\c@pgfmath@countc\c@pgfmath@countb%
            \advance\c@pgfmath@countc100000\relax%
            \edef\pgfmath@sci@result{\pgfmath@sci@sign\the\c@pgfmath@counta.\expandafter\pgfmath@gobbleone\the\c@pgfmath@countc pt}%
            \pgfmath@x\pgfmath@sci@result\relax%
        \fi\fi%
        \pgfmath@returnone\pgfmath@x%
    \endgroup}



% width function.
%
\pgfmathdeclarefunction{width}{1}{%
    \begingroup%
        \setbox\pgfmath@box=\hbox{{\pgfmath@selectfont{#1}}}%
        \pgfmath@x=\wd\pgfmath@box%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}


% height function.
%
\pgfmathdeclarefunction{height}{1}{%
    \begingroup%
        \setbox\pgfmath@box=\hbox{{\pgfmath@selectfont{#1}}}%
        \pgfmath@x=\ht\pgfmath@box%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}

% depth function.
%
\pgfmathdeclarefunction{depth}{1}{%
    \begingroup%
        \setbox\pgfmath@box=\hbox{{\pgfmath@selectfont{#1}}}%
        \pgfmath@x=\dp\pgfmath@box%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}


% array function.
%
\pgfmathdeclarefunction{array}{2}{%
    \begingroup%
        \afterassignment\pgfmath@gobbletilpgfmath@\pgfmath@count=#2\relax\pgfmath@%
        \expandafter\pgfmatharray@@#1\pgfmath@stop%
}

\def\pgfmath@token@stop{\pgfmath@stop}%
\def\pgfmatharray@@#1{%
    \def\pgfmath@temp{#1}%
    \advance\pgfmath@count by-1\relax%
    \ifx\pgfmath@temp\pgfmath@token@stop%
        \pgfmath@error{Array index out of bounds.}{}%
        \def\pgfmathresult{0}%
        \pgfmath@smuggleone\pgfmathresult\endgroup%
        \let\pgfmath@next=\relax%
    \else%
        \ifnum\pgfmath@count=-1\relax%
            \def\pgfmathresult{#1}%
            \let\pgfmath@next=\pgfmatharray@@@%
        \else%
            \let\pgfmath@next=\pgfmatharray@@%
        \fi%
    \fi%
    \pgfmath@next}

\def\pgfmatharray@@@#1\pgfmath@stop{%
    \pgfmath@smuggleone\pgfmathresult\endgroup%
}

% dim function: return dimension of an array
% dim({1,2,3}) return 3
% dim({{1,2,3},{4,5,6}}) return 2
\pgfmathdeclarefunction{dim}{1}{%
  \begingroup
    \pgfmath@count=0\relax
    \expandafter\pgfmath@dim@i\pgfutil@firstofone#1\pgfmath@token@stop
    \edef\pgfmathresult{\the\pgfmath@count}%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup}

\def\pgfmath@dim@i#1{%
    \ifx\pgfmath@token@stop#1%
    \else
      \advance\pgfmath@count by 1\relax
      \expandafter\pgfmath@dim@i
    \fi}


% max function.
%
\pgfmathdeclarefunction{max}{...}{%
    \begingroup%
        \pgfmath@x=-16383pt\relax%
        \pgfmathmax@@#1{}}

\def\pgfmathmax@@#1{%
    \def\pgfmath@temp{#1}%
    \ifx\pgfmath@temp\pgfmath@empty%
        \let\pgfmath@next=\pgfmathmax@@@%
    \else%
        \ifdim#1pt>\pgfmath@x%
            \pgfmath@x=#1pt\relax%
        \fi%
        \let\pgfmath@next=\pgfmathmax@@%
    \fi%
    \pgfmath@next}

\def\pgfmathmax@@@{\pgfmath@returnone\pgfmath@x\endgroup}%

% For computability with old code.
\def\pgfmathmax#1#2{%
    \pgfmathparse{#1,#2}%
    \expandafter\pgfmathmax@\expandafter{\pgfmathresult}%
}

% min function.
%
\pgfmathdeclarefunction{min}{...}{%
    \begingroup%
        \pgfmath@x=16383pt\relax%
        \pgfmathmin@@#1{}}

\def\pgfmathmin@@#1{%
    \def\pgfmath@temp{#1}%
    \ifx\pgfmath@temp\pgfmath@empty%
        \let\pgfmath@next=\pgfmathmin@@@%
    \else%
        \ifdim#1pt<\pgfmath@x%
            \pgfmath@x=#1pt\relax%
        \fi%
        \let\pgfmath@next=\pgfmathmin@@%
    \fi%
    \pgfmath@next}

\def\pgfmathmin@@@{\pgfmath@returnone\pgfmath@x\endgroup}%

% For computability with old code.
\def\pgfmathmin#1#2{%
    \pgfmathparse{#1,#2}%
    \expandafter\pgfmathmin@\expandafter{\pgfmathresult}%
}



% scalar function.
%
\pgfmathdeclarefunction{scalar}{1}{%
  \def\pgfmathresult{#1}%
  \global\pgfmathunitsdeclaredfalse%
}


==> pgfmathfunctions.random.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the pseudorandom numbers.
%
% Version 1.414213 29/9/2007

% Pseudo-random number generation.
%
% See:
% \book@{pressetal1992,
%    author    = {William H. Press and Brian P. Flannery and Saul A.
%                 Teukolsky and William T. Vetterling},
%    title     = {Numerical Recipies in C},
%    edition   = {Second},
%    publisher = {Cambridge University Press}
% }
%
% See also, the documentation for the lcg package by Erich Janka:
% (http://www.ctan.org/tex-archive/macros/latex/contrib/lcg/lcg.pdf)
%
\def\pgfmath@rnd@m{2147483647}% LaTeX Maximum.

\begingroup
\c@pgfmath@counta=\time%
\multiply\c@pgfmath@counta by\year%
\ifnum\c@pgfmath@counta=0
  \c@pgfmath@counta=1
\fi
\xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}% The seed.
\endgroup

% \pgfmathsetseed
%
% Explicitly set the seed for the generator
%
% #1 -> the new seed.
%
\def\pgfmathsetseed#1{%
    % Attention pgflibraryluamath.code.tex relies on the fact that
    % this method also modifies \pgfmathresult:
    \pgfmathparse{#1}\expandafter\pgfmath@setseed\pgfmathresult.0\pgfmath@stop
}%
\def\pgfmath@setseed#1.#2\pgfmath@stop{\def\pgfmath@rnd@z{#1}}%

% Alternative parameters - see Press et al (1992) p278-279,
% for discussion.
%
% a=16807 q=127773 r=2836
% a=48271 q=4488   r=3399
%
\def\pgfmath@rnd@a{69621}
\def\pgfmath@rnd@r{23902}
\def\pgfmath@rnd@q{30845}

% \pgfmathgeneratepseudorandomnumber
%
% A linear congruency generator for generating
% pseudo-random numbers. Generates numbers in
% the range 1 - 2^31-1.
%
\def\pgfmathgeneratepseudorandomnumber{%
    \begingroup%
        \c@pgfmath@counta=\pgfmath@rnd@z%
        \c@pgfmath@countb=\pgfmath@rnd@z%
        \c@pgfmath@countc=\pgfmath@rnd@q%
        \divide\c@pgfmath@counta by\c@pgfmath@countc%
        \multiply\c@pgfmath@counta by-\c@pgfmath@countc%
        \advance\c@pgfmath@counta by\c@pgfmath@countb
        \c@pgfmath@countc=\pgfmath@rnd@a%
        \multiply\c@pgfmath@counta by\c@pgfmath@countc%
        \c@pgfmath@countc=\pgfmath@rnd@q%
        \divide\c@pgfmath@countb by\c@pgfmath@countc%
        \c@pgfmath@countc=\pgfmath@rnd@r%
        \multiply\c@pgfmath@countb by\c@pgfmath@countc%
        \advance\c@pgfmath@counta by-\c@pgfmath@countb%
        \ifnum\c@pgfmath@counta<0\relax%
            \c@pgfmath@countb=\pgfmath@rnd@m%
            \advance\c@pgfmath@counta by\c@pgfmath@countb%
        \fi%
        \xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}%
    \endgroup%
    \edef\pgfmathresult{\pgfmath@rnd@z}%
}

% \pgfmathrnd
%
% Generates a pseudo-random number between 0 and 1.
%
\pgfmathdeclarefunction{rnd}{0}{%
    \begingroup%
        \pgfmathgeneratepseudorandomnumber%
        \c@pgfmath@counta\pgfmathresult%
        \c@pgfmath@countb\c@pgfmath@counta%
        \divide\c@pgfmath@countb100001\relax% To get one.
        \multiply\c@pgfmath@countb-100001\relax%
        \advance\c@pgfmath@countb\c@pgfmath@counta%
        \advance\c@pgfmath@countb1000000\relax%
        \expandafter\pgfmathrnd@@\the\c@pgfmath@countb\pgfmath@%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}%

\def\pgfmathrnd@@#1#2#3\pgfmath@{%
    \edef\pgfmath@temp{#2.#3}%
    \pgfmath@x=\pgfmath@temp pt\relax%
}%

% \pgfmathrand
%
% Generates a pseudo-random number between -1 and 1.
%
\pgfmathdeclarefunction{rand}{0}{%
    \begingroup%
        \pgfmathgeneratepseudorandomnumber%
        \c@pgfmath@counta\pgfmathresult%
        \c@pgfmath@countb\c@pgfmath@counta%
        \divide\c@pgfmath@countb200001\relax%
        \multiply\c@pgfmath@countb-200001\relax%
        \advance\c@pgfmath@countb\c@pgfmath@counta%
        \advance\c@pgfmath@countb-100000\relax%
        \ifnum\c@pgfmath@countb<0\relax%
            \advance\c@pgfmath@countb-1000000\relax%
        \else%
            \advance\c@pgfmath@countb1000000\relax%
        \fi%
        \expandafter\pgfmathrand@@\the\c@pgfmath@countb\pgfmath@%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}%

\def\pgfmathrand@@#1#2#3#4\pgfmath@{%
    \ifx#1-%
        \edef\pgfmath@temp{-#3.#4}%
    \else%
        \edef\pgfmath@temp{#2.#3#4}%
    \fi%
    \pgfmath@x=\pgfmath@temp pt\relax%
}%

\pgfmathdeclarefunction{random}{...}{%
    \begingroup%
        \def\pgfmath@temp{#1}%
        \ifx\pgfmath@temp\pgfmath@empty%
            \pgfmathrnd@%
        \else%
            \expandafter\pgfmathrandom@@#1\pgfmath@stop%
        \fi%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup}

\def\pgfmathrandom@@{\futurelet\pgfmath@token\pgfmathrandom@@@}
\def\pgfmathrandom@@@{%
    \ifx\pgfmath@token\bgroup%
        \expandafter\pgfmath@random@@@@%
    \else%
        \expandafter\pgfmath@random@@@@@%
    \fi%
}
\def\pgfmath@random@@@@@#1\pgfmath@stop{%
    \pgfmathrandominteger\pgfmathresult{1}{#1}%
}
\def\pgfmath@random@@@@#1#2\pgfmath@stop{%
    \pgfmathrandominteger\pgfmathresult{#1}{#2}%
}

% \pgfmathrandominteger
%
% Return a 'randomly' selected integer in the range #2 - #3 (inclusive).
%
% #1 - a macro to store the integer (not a count register).
% #2 - the lower limit of the range.
% #3 - the upper limit of the range.
%
\def\pgfmathrandominteger#1#2#3{%
    \begingroup%
        \pgfmathsetcount\c@pgfmath@counta{#2}%
        \pgfmathsetcount\c@pgfmath@countb{#3}%
        \c@pgfmath@countc\c@pgfmath@countb%
        % OK. Maybe #2 > #3.
        \ifnum\c@pgfmath@counta>\c@pgfmath@countb\relax%
            \c@pgfmath@countc\c@pgfmath@counta%
            \c@pgfmath@counta\c@pgfmath@countb%
            \c@pgfmath@countb\c@pgfmath@countc%
        \fi%
        \c@pgfmath@countd\c@pgfmath@counta
        \advance\c@pgfmath@countc1\relax%
        \advance\c@pgfmath@countc-\c@pgfmath@counta%
        \pgfmathgeneratepseudorandomnumber%
        \c@pgfmath@counta\pgfmathresult\relax%
        \c@pgfmath@countb\c@pgfmath@counta%
        \divide\c@pgfmath@countb\c@pgfmath@countc%
        \multiply\c@pgfmath@countb-\c@pgfmath@countc%
        \advance\c@pgfmath@counta\c@pgfmath@countb%
        \advance\c@pgfmath@counta\c@pgfmath@countd
        \edef\pgfmathresult{\the\c@pgfmath@counta}%
        \pgfmath@smuggleone{\pgfmathresult}%
    \endgroup%
    \edef#1{\pgfmathresult}%
}

% \pgfmathdeclarerandomlist
%
% Create a list to be used with \pgfmathrandomelement.
%
% #1 - the name of the list
% #2 - a list of elements (e.g., {item-1}{item-2}...{item-n}).
%
\def\pgfmathdeclarerandomlist#1#2{%
    \def\pgfmath@randomlistname{#1}%
    \begingroup%
        \c@pgfmath@counta=1\relax%
        % {} is a possible random element so (locally)
        % redefine \pgfmath@empty.
        \def\pgfmath@empty{pgfmath@empty}%
        \expandafter\pgfmath@scanrandomlist#2{pgfmath@empty}}
\def\pgfmath@scanrandomlist#1{%
    \def\pgfmath@scanneditem{#1}%
    \ifx\pgfmath@scanneditem\pgfmath@empty%
        \advance\c@pgfmath@counta-1\relax%
        \expandafter\xdef\csname pgfmath@randomlist@\pgfmath@randomlistname\endcsname{\the\c@pgfmath@counta}%
        \endgroup%
    \else%
        \expandafter\gdef\csname pgfmath@randomlist@\pgfmath@randomlistname @\the\c@pgfmath@counta\endcsname{#1}%
        \advance\c@pgfmath@counta1\relax%
        \expandafter\pgfmath@scanrandomlist%
    \fi}

% \pgfmathrandomitem
%
% Return a 'randomly' selected element from a list.
%
% #1 - a macro to store the item.
% #2 - the name of the list.
%
\def\pgfmathrandomitem#1#2{%
    \pgfmath@ifundefined{pgfmath@randomlist@#2}{\pgfmath@error{Unknown random list `#2'}{}}{%
        \edef\pgfmath@randomlistlength{\csname pgfmath@randomlist@#2\endcsname}%
        \pgfmathrandominteger{\pgfmath@randomtemp}{1}{\pgfmath@randomlistlength}%
        \def#1{\csname pgfmath@randomlist@#2@\pgfmath@randomtemp\endcsname}}}


==> pgfmathfunctions.round.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 1.414213 29/9/2007

% round function. Uses asymmetric half-up rounding.
%
\pgfmathdeclarefunction{round}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \afterassignment\pgfmath@xa%
        \expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
        \pgfmath@xb\pgfmath@x%
        \ifdim\pgfmath@xb<0pt\relax%
            \ifdim\pgfmath@xa<0.5pt\relax%
            \else%
                \advance\c@pgfmath@counta-1\relax%
            \fi%
        \else%
            \ifdim\pgfmath@xa<0.5pt\relax%
            \else%
                \advance\c@pgfmath@counta1\relax%
            \fi%
        \fi%
        \pgfmath@returnone\the\c@pgfmath@counta pt%
    \endgroup%
}%

% floor function.
%
\pgfmathdeclarefunction{floor}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \afterassignment\pgfmathfloor@collect@remainder%
        \expandafter\c@pgfmath@counta\the\pgfmath@x\pgfmath@%
        \expandafter\pgfmath@x#1pt\relax%
        \ifdim\pgfmath@x<0pt\relax%
            \ifdim\pgfmathfloor@remainder>0pt
                \advance\c@pgfmath@counta by -1\relax%
            \else
                % ok, we stripped only '0'.
            \fi
        \fi%
        \pgfmath@x\c@pgfmath@counta pt\relax%
        \pgfmath@returnone\pgfmath@x%
    \endgroup%
}%

\def\pgfmathfloor@collect@remainder#1\pgfmath@{%
    \def\pgfmathfloor@remainder{#1}%
    \ifx\pgfmathfloor@remainder\pgfutil@empty
        \def\pgfmathfloor@remainder{0}%
    \fi
}%

% ceil function.
%
\pgfmathdeclarefunction{ceil}{1}{%
    \begingroup%
        \expandafter\pgfmath@x#1pt\relax%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
        \pgfmath@y\pgfmath@x%
        \advance\pgfmath@y-\c@pgfmath@counta pt\relax%
        \pgfmath@x\c@pgfmath@counta pt\relax%
        \ifdim\pgfmath@y>0pt\relax%
            \advance\pgfmath@x1pt\relax%
        \fi%
    \pgfmath@returnone\pgfmath@x%
    \endgroup%
}%

% int function
%
\pgfmathdeclarefunction{int}{1}{%
    \begingroup%
        \expandafter\pgfmathint@@#1.\pgfmath@stop
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup}

\def\pgfmathint@@#1.#2\pgfmath@stop{%
    \def\pgfmath@temp{#1}%
    \ifx\pgfmath@temp\pgfmath@empty%
        \def\pgfmathresult{0}%
    \else%
        \pgfmath@in@{#1}{+-+0-0}%
        \ifpgfmath@in@
            \def\pgfmathresult{0}%
        \else%
            \def\pgfmathresult{#1}%
        \fi%
    \fi}

% frac function.
%
\pgfmathdeclarefunction{frac}{1}{%
    \begingroup%
        \expandafter\pgfmathfrac@@#1.\pgfmath@stop%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup}

\def\pgfmathfrac@@#1.{%
    \pgfmath@ifnextchar\pgfmath@stop{\def\pgfmathresult{0.0}\pgfmath@gobbleone}{\pgfmathfrac@@@}%
}
\def\pgfmathfrac@@@#1.\pgfmath@stop{\def\pgfmathresult{0.#1}}

% real function.
%
\pgfmathdeclarefunction{real}{1}{%
    \begingroup%
        \pgfmath@x=#1pt\relax%
        \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
        \pgfmath@smuggleone\pgfmathresult%
    \endgroup%
}


==> pgfmathfunctions.trigonometric.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the trigonometric functions/functions.
%
% Much of this file is based on ideas and code (particularly
% the old \pgfcoremath.code.tex) due to Till Tantau.
%
% Version 1.414213 29/9/2007

% \pgfmathpi
%
\pgfmathdeclarefunction{pi}{0}{\def\pgfmathresult{3.141592654}}

\pgfkeys{
    /pgf/trig format/.is choice,
    % attention: the luamath library will hook into these code keys.
    /pgf/trig format/deg/.code={\def\pgfmath@trig@format@choice{0}},
    /pgf/trig format/rad/.code={\def\pgfmath@trig@format@choice{1}},
    /pgf/trig format/deg,
}

% Executes #1 if 'trig format=deg' and #2 otherwise.
\def\pgfmathiftrigonometricusesdeg#1#2{%
    \if0\pgfmath@trig@format@choice
        #1%
    \else
        #2%
    \fi
}%

% \pgfmathradians
% (for compatibility with 1.18 beta, will be deprecated)
%
% Convert #1 from radians to degrees (accurate to 1 deg).
%
\pgfmathdeclarefunction{radians}{1}{%
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \pgfmath@x57.29577\pgfmath@x\relax% 57.29577 = 360/(2*pi)
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}%

% \pgfmathdeg
%
% Convert #1 from radians to degrees.
%
\pgfmathdeclarefunction{deg}{1}{%
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \pgfmath@scale@rad@to@deg\pgfmath@x
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}%

\def\pgfmath@scale@rad@to@deg#1{%
    #1=57.29577#1\relax% 57.29577 = 360/(2*pi)
}%

% \pgfmathrad
%
% Convert #1 from degrees to radians.
%
\pgfmathdeclarefunction{rad}{1}{%
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \pgfmath@scale@deg@to@rad\pgfmath@x
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}%

\def\pgfmath@scale@deg@to@rad#1{%
    #1=3.14159#1%
    \divide#1180\relax%
}%

% \pgfmathsin
%
% Calculate the sine of #1 (in degrees).
%
\pgfmathdeclarefunction{sin}{1}{%
  % Let #1 = a.b
  % Then sin(#1) \approx (1-b)*sin(a) + b*sin(a+1)
  %
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \if1\pgfmath@trig@format@choice
        % trig format=rad
        \pgfmath@scale@rad@to@deg\pgfmath@x
    \fi
    \advance\pgfmath@x-90pt\relax%
    \afterassignment\pgfmath@gobbletilpgfmath@
    \expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@
    \divide\c@pgfmath@counta360\relax%
    \multiply\c@pgfmath@counta-360\relax%
    \advance\pgfmath@x\c@pgfmath@counta pt\relax%
    \ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
    \ifdim\pgfmath@x<180pt\relax%
    \else
      \pgfmath@x-\pgfmath@x%
      \advance\pgfmath@x360pt\relax%
    \fi%
    % Now 0 <= x < 179. So split x into integer and decimal...
    %
    \afterassignment\pgfmath@xa%
    \expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
    %
    % ...if #1 is an integer, don't do anything fancy.
    \ifdim\pgfmath@xa=0pt%
      \expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt\relax%
    \else%
      \pgfmath@x-\pgfmath@xa%
      \advance\pgfmath@x1pt\relax%
      \expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
      \advance\c@pgfmath@counta1\relax%
      \ifnum\c@pgfmath@counta=181\relax\c@pgfmath@counta179\relax\fi%
      \expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
    \fi%
    \pgfmath@returnone\pgfmath@x%
  \endgroup
}

% \pgfmathcos
%
% Calculate the cosine of #1 (in degrees).
%
\pgfmathdeclarefunction{cos}{1}{%
  % Let x = a.b
  % Then cos(x) \approx (1-b)*cos(a) + b*cos(a+1)
  %
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \if1\pgfmath@trig@format@choice
        % trig format=rad
        \pgfmath@scale@rad@to@deg\pgfmath@x
    \fi
    \afterassignment\pgfmath@gobbletilpgfmath@%
    \expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
    \divide\c@pgfmath@counta360\relax%
    \multiply\c@pgfmath@counta-360\relax%
    \advance\pgfmath@x\c@pgfmath@counta pt\relax%
    \ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
    \ifdim\pgfmath@x<180pt\relax%
    \else%
      \pgfmath@x-\pgfmath@x%
      \advance\pgfmath@x360pt\relax%
    \fi%
    % Now 0 <= x < 179. So split x into integer and decimal...
    %
    \afterassignment\pgfmath@xa%
    \expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
    %
    % ...if #1 is an integer, don't do anything fancy.
    \ifdim\pgfmath@xa=0pt%
      \expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt%
    \else%
      \pgfmath@x-\pgfmath@xa%
      \advance\pgfmath@x1pt\relax%
      \expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
      \advance\c@pgfmath@counta1\relax%
      \ifnum\c@pgfmath@counta=181\relax\c@pgfmath@counta179\relax\fi%
      \expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
    \fi%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathsincos
%
% Calculate the sin and cosine of #1 (in degrees).
%
\def\pgfmathsincos#1{%
  \pgfmathparse{#1}%
  \expandafter\pgfmathsincos@\expandafter{\pgfmathresult}}
\def\pgfmathsincos@#1{%
  \edef\pgfmath@temparg{#1}%
  \pgfmathsin@{\pgfmath@temparg}\edef\pgfmathresulty{\pgfmathresult}%
  \pgfmathcos@{\pgfmath@temparg}\edef\pgfmathresultx{\pgfmathresult}%
}

% \pgfmathtan
%
% Calculate the tangent of #1 (in degrees).
%
\pgfmathdeclarefunction{tan}{1}{%
  \begingroup%
    \edef\pgfmath@temparg{#1}%
    \pgfmathcos@{\pgfmath@temparg}%
    \expandafter\pgfmathreciprocal@\expandafter{\pgfmathresult}%
    \edef\pgfmath@tantemp{\pgfmathresult}%
    \pgfmathsin@{\pgfmath@temparg}%
    \pgfmath@x\pgfmathresult pt\relax%
    \pgfmath@x\pgfmath@tantemp\pgfmath@x%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathcosec
%
% Calculate the cosec of #1 (in degrees).
%
\pgfmathdeclarefunction{cosec}{1}{%
  \expandafter\pgfmathsin@\expandafter{#1}%
  \pgfmathreciprocal@{\pgfmathresult}%
}

% \pgfmathsec
%
% Calculate the sec of #1 (in degrees).
%
\pgfmathdeclarefunction{sec}{1}{%
  \expandafter\pgfmathcos@\expandafter{#1}%
  \pgfmathreciprocal@{\pgfmathresult}%
}

% \pgfmathcot
%
% Calculate the cotangent of #1 (in degrees).
%
\pgfmathdeclarefunction{cot}{1}{%
  \begingroup%
    \edef\pgfmath@temparg{#1}%
    \pgfmathsin@{\pgfmath@temparg}%
    \expandafter\pgfmathreciprocal@\expandafter{\pgfmathresult}%
    \edef\pgfmath@tantemp{\pgfmathresult}%
    \pgfmathcos@{\pgfmath@temparg}%
    \pgfmath@x\pgfmathresult pt\relax%
    \pgfmath@x\pgfmath@tantemp\pgfmath@x%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

\def\pgfmath@multiply@thousand#1.#2#3#4#5\relax{%
  \edef\pgfmathresult{#1#2#3#4.#5}%
}%

% \pgfmathasin
%
% The asin of #1
%
\pgfmathdeclarefunction{asin}{1}{%
  \begingroup%
    \pgfmath@x=#1pt %
    \pgfmath@xa\pgfmath@x%
    \edef\pgf@temp{\pgfmath@tonumber\pgfmath@x}%
    % compute lossless '*1000' operation:
    \expandafter\pgfmath@multiply@thousand\pgf@temp 000\relax
    \pgfmath@x=\pgfmathresult pt %
    \ifdim\pgfmath@x<0pt\relax%
      \pgfmath@x-\pgfmath@x%
    \fi%
    \pgfmath@table@lookup{\pgfmath@x}{pgfmath@acos@}{1001}%
    \pgfmath@x=-\pgfmath@x
    \advance\pgfmath@x90pt\relax%
    \ifdim\pgfmath@xa<0pt\relax%
      \pgfmath@x-\pgfmath@x%
    \fi%
    \if1\pgfmath@trig@format@choice
        % trig format=rad
        \pgfmath@scale@deg@to@rad\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% Defines \pgfmath@x to be the result of the table lookup for value
% '#1' in table '#2'
%
% #1: a value for which lookup should be performed
% #2: the table's prefix name
% #3: the table's size
\def\pgfmath@table@lookup#1#2#3{%
  \pgfmath@x=#1\relax
  \expandafter\pgfmath@table@lookup@\the\pgfmath@x\relax{#2}{#3}%
}
\def\pgfmath@table@lookup@#1.#2\relax#3#4{%
  \edef\pgf@temp{\Pgf@geT#2}% strip 'pt' suffix.
  %
  % prepare constant interpolant (i.e. the value at node '#1'):
  \pgfmath@x=\csname #3#1\endcsname pt %
  %
  \c@pgfmath@countc=#1 %
  \advance\c@pgfmath@countc by1 %
  \ifnum\c@pgfmath@countc<#4 %
    % Ah - we have enough elements in the table.
    %
    % perform linear interpolation:
    \pgfmath@ya=\csname #3\the\c@pgfmath@countc\endcsname pt %
    \advance\pgfmath@ya by-\pgfmath@x %
    \advance\pgfmath@x by0.\pgf@temp\pgfmath@ya
  \fi
}%

% \pgfmathacos
%
% The acos of #1
%
\pgfmathdeclarefunction{acos}{1}{%
  \begingroup%
    \pgfmath@x#1pt\relax%
    \pgfmath@xa\pgfmath@x%
    \edef\pgf@temp{\pgfmath@tonumber\pgfmath@x}%
    % compute lossless '*1000' operation:
    \expandafter\pgfmath@multiply@thousand\pgf@temp 000\relax
    \pgfmath@x=\pgfmathresult pt %
    \ifdim\pgfmath@x<0pt\relax%
      \pgfmath@x-\pgfmath@x%
    \fi%
    \pgfmath@table@lookup{\pgfmath@x}{pgfmath@acos@}{1001}%
    \ifdim\pgfmath@xa<0pt\relax%
      \pgfmath@x-\pgfmath@x%
      \advance\pgfmath@x by180pt\relax%
    \fi%
    \if1\pgfmath@trig@format@choice
        % trig format=rad
        \pgfmath@scale@deg@to@rad\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

\pgfmathdeclarefunction{atan}{1}{%
  \begingroup%
    \expandafter\pgfmath@x#1pt\relax%
    \pgfmath@xa\pgfmath@x%
    \ifdim\pgfmath@x<0pt\relax%
      \pgfmath@x-\pgfmath@x%
    \fi%
    \pgfmath@xb\pgfmath@x%
    \ifdim\pgfmath@x>1pt\relax%
      \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
      \pgfmathreciprocal@{\pgfmath@temp}%
      \pgfmath@x\pgfmathresult pt\relax%
    \fi%
    % compute lossless '*1000' operation:
    \edef\pgf@temp{\pgfmath@tonumber\pgfmath@x}%
    \expandafter\pgfmath@multiply@thousand\pgf@temp 000\relax
    \pgfmath@x=\pgfmathresult pt %
    \pgfmath@table@lookup{\pgfmath@x}{pgfmath@atan@}{1001}%xxx
    \ifdim\pgfmath@xb>1pt\relax%
      \pgfmath@x=-\pgfmath@x%
      \advance\pgfmath@x90pt%
    \fi%
    \ifdim\pgfmath@xa<0pt\relax%
      \pgfmath@x-\pgfmath@x%
    \fi%
    \if1\pgfmath@trig@format@choice
        % trig format=rad
        \pgfmath@scale@deg@to@rad\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

\pgfmathdeclarefunction{atan2}{2}{%
  % Note: first parameter is y (!), second is x (!)
  \begingroup%
    \let\pgfmath@trig@format@choice@@=\pgfmath@trig@format@choice
    \def\pgfmath@trig@format@choice{0}%
    \pgfmath@y=#1pt\relax%
    \ifdim\pgfmath@y<0pt\relax%
      \pgfmath@y=-\pgfmath@y%
    \fi%
    \ifdim\pgfmath@y<0.001pt\relax%
      \ifdim#2pt<0pt\relax%
        \pgfmath@x=+180pt\relax%
      \else%
        \ifdim#2pt>0pt\relax%
          \pgfmath@x=0pt\relax%
        \else%
          \ifdim#1pt<0pt%
            \pgfmath@x=-90pt\relax%
          \else%
            \pgfmath@x=90pt\relax%
          \fi%
        \fi%
      \fi%
    \else%
      \pgfmathabs@{#1}\let\pgfmath@tempa\pgfmathresult%
      \pgfmathabs@{#2}\let\pgfmath@tempb\pgfmathresult%
      \ifdim\pgfmath@tempa pt>\pgfmath@tempb pt%
        \pgfmathdivide@{#2}{\pgfmath@tempa}%
        \expandafter\pgfmathatan@\expandafter{\pgfmathresult}%
        \pgfmath@x=90pt%
        \advance\pgfmath@x by-\pgfmathresult pt\relax%
      \else%
        \pgfmathdivide@{\pgfmath@tempa}{#2}%
        \expandafter\pgfmathatan@\expandafter{\pgfmathresult}%
        \pgfmath@x=\pgfmathresult pt\relax%
        \ifdim#2pt<0pt%
          \advance\pgfmath@x by180pt\relax%
        \fi%
      \fi%
      \ifdim#1pt<0pt\relax%
        \pgfmath@x=-\pgfmath@x%
      \fi%
    \fi%
    \if1\pgfmath@trig@format@choice@@
        % trig format=rad
        \pgfmath@scale@deg@to@rad\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% This is needed since \pgfmathatan2 is not a legal macro name
\expandafter\let\expandafter\pgfmathatantwo\csname pgfmathatan2\endcsname
\expandafter\let\expandafter\pgfmathatantwo@\csname pgfmathatan2@\endcsname

\def\pgfmath@def#1#2#3{\expandafter\def\csname pgfmath@#1@#2\endcsname{#3}}
\pgfmath@def{cos}{0}{1.00000}    \pgfmath@def{cos}{1}{0.99985}
\pgfmath@def{cos}{2}{0.99939}    \pgfmath@def{cos}{3}{0.99863}
\pgfmath@def{cos}{4}{0.99756}    \pgfmath@def{cos}{5}{0.99619}
\pgfmath@def{cos}{6}{0.99452}    \pgfmath@def{cos}{7}{0.99255}
\pgfmath@def{cos}{8}{0.99027}    \pgfmath@def{cos}{9}{0.98769}
\pgfmath@def{cos}{10}{0.98481}    \pgfmath@def{cos}{11}{0.98163}
\pgfmath@def{cos}{12}{0.97815}    \pgfmath@def{cos}{13}{0.97437}
\pgfmath@def{cos}{14}{0.97030}    \pgfmath@def{cos}{15}{0.96593}
\pgfmath@def{cos}{16}{0.96126}    \pgfmath@def{cos}{17}{0.95630}
\pgfmath@def{cos}{18}{0.95106}    \pgfmath@def{cos}{19}{0.94552}
\pgfmath@def{cos}{20}{0.93969}    \pgfmath@def{cos}{21}{0.93358}
\pgfmath@def{cos}{22}{0.92718}    \pgfmath@def{cos}{23}{0.92050}
\pgfmath@def{cos}{24}{0.91355}    \pgfmath@def{cos}{25}{0.90631}
\pgfmath@def{cos}{26}{0.89879}    \pgfmath@def{cos}{27}{0.89101}
\pgfmath@def{cos}{28}{0.88295}    \pgfmath@def{cos}{29}{0.87462}
\pgfmath@def{cos}{30}{0.86603}    \pgfmath@def{cos}{31}{0.85717}
\pgfmath@def{cos}{32}{0.84805}    \pgfmath@def{cos}{33}{0.83867}
\pgfmath@def{cos}{34}{0.82904}    \pgfmath@def{cos}{35}{0.81915}
\pgfmath@def{cos}{36}{0.80902}    \pgfmath@def{cos}{37}{0.79864}
\pgfmath@def{cos}{38}{0.78801}    \pgfmath@def{cos}{39}{0.77715}
\pgfmath@def{cos}{40}{0.76604}    \pgfmath@def{cos}{41}{0.75471}
\pgfmath@def{cos}{42}{0.74314}    \pgfmath@def{cos}{43}{0.73135}
\pgfmath@def{cos}{44}{0.71934}    \pgfmath@def{cos}{45}{0.70711}
\pgfmath@def{cos}{46}{0.69466}    \pgfmath@def{cos}{47}{0.68200}
\pgfmath@def{cos}{48}{0.66913}    \pgfmath@def{cos}{49}{0.65606}
\pgfmath@def{cos}{50}{0.64279}    \pgfmath@def{cos}{51}{0.62932}
\pgfmath@def{cos}{52}{0.61566}    \pgfmath@def{cos}{53}{0.60182}
\pgfmath@def{cos}{54}{0.58779}    \pgfmath@def{cos}{55}{0.57358}
\pgfmath@def{cos}{56}{0.55919}    \pgfmath@def{cos}{57}{0.54464}
\pgfmath@def{cos}{58}{0.52992}    \pgfmath@def{cos}{59}{0.51504}
\pgfmath@def{cos}{60}{0.50000}    \pgfmath@def{cos}{61}{0.48481}
\pgfmath@def{cos}{62}{0.46947}    \pgfmath@def{cos}{63}{0.45399}
\pgfmath@def{cos}{64}{0.43837}    \pgfmath@def{cos}{65}{0.42262}
\pgfmath@def{cos}{66}{0.40674}    \pgfmath@def{cos}{67}{0.39073}
\pgfmath@def{cos}{68}{0.37461}    \pgfmath@def{cos}{69}{0.35837}
\pgfmath@def{cos}{70}{0.34202}    \pgfmath@def{cos}{71}{0.32557}
\pgfmath@def{cos}{72}{0.30902}    \pgfmath@def{cos}{73}{0.29237}
\pgfmath@def{cos}{74}{0.27564}    \pgfmath@def{cos}{75}{0.25882}
\pgfmath@def{cos}{76}{0.24192}    \pgfmath@def{cos}{77}{0.22495}
\pgfmath@def{cos}{78}{0.20791}    \pgfmath@def{cos}{79}{0.19081}
\pgfmath@def{cos}{80}{0.17365}    \pgfmath@def{cos}{81}{0.15643}
\pgfmath@def{cos}{82}{0.13917}    \pgfmath@def{cos}{83}{0.12187}
\pgfmath@def{cos}{84}{0.10453}    \pgfmath@def{cos}{85}{0.08716}
\pgfmath@def{cos}{86}{0.06976}    \pgfmath@def{cos}{87}{0.05234}
\pgfmath@def{cos}{88}{0.03490}    \pgfmath@def{cos}{89}{0.01745}
\pgfmath@def{cos}{90}{0.00000}    \pgfmath@def{cos}{91}{-0.01745}
\pgfmath@def{cos}{92}{-0.03490}    \pgfmath@def{cos}{93}{-0.05234}
\pgfmath@def{cos}{94}{-0.06976}    \pgfmath@def{cos}{95}{-0.08716}
\pgfmath@def{cos}{96}{-0.10453}    \pgfmath@def{cos}{97}{-0.12187}
\pgfmath@def{cos}{98}{-0.13917}    \pgfmath@def{cos}{99}{-0.15643}
\pgfmath@def{cos}{100}{-0.17365}    \pgfmath@def{cos}{101}{-0.19081}
\pgfmath@def{cos}{102}{-0.20791}    \pgfmath@def{cos}{103}{-0.22495}
\pgfmath@def{cos}{104}{-0.24192}    \pgfmath@def{cos}{105}{-0.25882}
\pgfmath@def{cos}{106}{-0.27564}    \pgfmath@def{cos}{107}{-0.29237}
\pgfmath@def{cos}{108}{-0.30902}    \pgfmath@def{cos}{109}{-0.32557}
\pgfmath@def{cos}{110}{-0.34202}    \pgfmath@def{cos}{111}{-0.35837}
\pgfmath@def{cos}{112}{-0.37461}    \pgfmath@def{cos}{113}{-0.39073}
\pgfmath@def{cos}{114}{-0.40674}    \pgfmath@def{cos}{115}{-0.42262}
\pgfmath@def{cos}{116}{-0.43837}    \pgfmath@def{cos}{117}{-0.45399}
\pgfmath@def{cos}{118}{-0.46947}    \pgfmath@def{cos}{119}{-0.48481}
\pgfmath@def{cos}{120}{-0.50000}    \pgfmath@def{cos}{121}{-0.51504}
\pgfmath@def{cos}{122}{-0.52992}    \pgfmath@def{cos}{123}{-0.54464}
\pgfmath@def{cos}{124}{-0.55919}    \pgfmath@def{cos}{125}{-0.57358}
\pgfmath@def{cos}{126}{-0.58779}    \pgfmath@def{cos}{127}{-0.60182}
\pgfmath@def{cos}{128}{-0.61566}    \pgfmath@def{cos}{129}{-0.62932}
\pgfmath@def{cos}{130}{-0.64279}    \pgfmath@def{cos}{131}{-0.65606}
\pgfmath@def{cos}{132}{-0.66913}    \pgfmath@def{cos}{133}{-0.68200}
\pgfmath@def{cos}{134}{-0.69466}    \pgfmath@def{cos}{135}{-0.70711}
\pgfmath@def{cos}{136}{-0.71934}    \pgfmath@def{cos}{137}{-0.73135}
\pgfmath@def{cos}{138}{-0.74314}    \pgfmath@def{cos}{139}{-0.75471}
\pgfmath@def{cos}{140}{-0.76604}    \pgfmath@def{cos}{141}{-0.77715}
\pgfmath@def{cos}{142}{-0.78801}    \pgfmath@def{cos}{143}{-0.79864}
\pgfmath@def{cos}{144}{-0.80902}    \pgfmath@def{cos}{145}{-0.81915}
\pgfmath@def{cos}{146}{-0.82904}    \pgfmath@def{cos}{147}{-0.83867}
\pgfmath@def{cos}{148}{-0.84805}    \pgfmath@def{cos}{149}{-0.85717}
\pgfmath@def{cos}{150}{-0.86603}    \pgfmath@def{cos}{151}{-0.87462}
\pgfmath@def{cos}{152}{-0.88295}    \pgfmath@def{cos}{153}{-0.89101}
\pgfmath@def{cos}{154}{-0.89879}    \pgfmath@def{cos}{155}{-0.90631}
\pgfmath@def{cos}{156}{-0.91355}    \pgfmath@def{cos}{157}{-0.92050}
\pgfmath@def{cos}{158}{-0.92718}    \pgfmath@def{cos}{159}{-0.93358}
\pgfmath@def{cos}{160}{-0.93969}    \pgfmath@def{cos}{161}{-0.94552}
\pgfmath@def{cos}{162}{-0.95106}    \pgfmath@def{cos}{163}{-0.95630}
\pgfmath@def{cos}{164}{-0.96126}    \pgfmath@def{cos}{165}{-0.96593}
\pgfmath@def{cos}{166}{-0.97030}    \pgfmath@def{cos}{167}{-0.97437}
\pgfmath@def{cos}{168}{-0.97815}    \pgfmath@def{cos}{169}{-0.98163}
\pgfmath@def{cos}{170}{-0.98481}    \pgfmath@def{cos}{171}{-0.98769}
\pgfmath@def{cos}{172}{-0.99027}    \pgfmath@def{cos}{173}{-0.99255}
\pgfmath@def{cos}{174}{-0.99452}    \pgfmath@def{cos}{175}{-0.99619}
\pgfmath@def{cos}{176}{-0.99756}    \pgfmath@def{cos}{177}{-0.99863}
\pgfmath@def{cos}{178}{-0.99939}    \pgfmath@def{cos}{179}{-0.99985}
\pgfmath@def{cos}{180}{-1.00000}     \pgfmath@def{cos}{181}{-0.99985}

\pgfmath@def{cosfrac}{0}{1.00000}    \pgfmath@def{cosfrac}{1}{0.99995}
\pgfmath@def{cosfrac}{2}{0.99980}    \pgfmath@def{cosfrac}{3}{0.99955}
\pgfmath@def{cosfrac}{4}{0.99920}    \pgfmath@def{cosfrac}{5}{0.99875}
\pgfmath@def{cosfrac}{6}{0.99820}    \pgfmath@def{cosfrac}{7}{0.99755}
\pgfmath@def{cosfrac}{8}{0.99681}    \pgfmath@def{cosfrac}{9}{0.99597}
\pgfmath@def{cosfrac}{10}{0.99503}    \pgfmath@def{cosfrac}{11}{0.99400}
\pgfmath@def{cosfrac}{12}{0.99287}    \pgfmath@def{cosfrac}{13}{0.99165}
\pgfmath@def{cosfrac}{14}{0.99034}    \pgfmath@def{cosfrac}{15}{0.98893}
\pgfmath@def{cosfrac}{16}{0.98744}    \pgfmath@def{cosfrac}{17}{0.98585}
\pgfmath@def{cosfrac}{18}{0.98418}    \pgfmath@def{cosfrac}{19}{0.98242}
\pgfmath@def{cosfrac}{20}{0.98058}    \pgfmath@def{cosfrac}{21}{0.97865}
\pgfmath@def{cosfrac}{22}{0.97664}    \pgfmath@def{cosfrac}{23}{0.97455}
\pgfmath@def{cosfrac}{24}{0.97238}    \pgfmath@def{cosfrac}{25}{0.97014}
\pgfmath@def{cosfrac}{26}{0.96782}    \pgfmath@def{cosfrac}{27}{0.96542}
\pgfmath@def{cosfrac}{28}{0.96296}    \pgfmath@def{cosfrac}{29}{0.96042}
\pgfmath@def{cosfrac}{30}{0.95782}    \pgfmath@def{cosfrac}{31}{0.95515}
\pgfmath@def{cosfrac}{32}{0.95242}    \pgfmath@def{cosfrac}{33}{0.94962}
\pgfmath@def{cosfrac}{34}{0.94677}    \pgfmath@def{cosfrac}{35}{0.94385}
\pgfmath@def{cosfrac}{36}{0.94088}    \pgfmath@def{cosfrac}{37}{0.93786}
\pgfmath@def{cosfrac}{38}{0.93478}    \pgfmath@def{cosfrac}{39}{0.93165}
\pgfmath@def{cosfrac}{40}{0.92847}    \pgfmath@def{cosfrac}{41}{0.92525}
\pgfmath@def{cosfrac}{42}{0.92198}    \pgfmath@def{cosfrac}{43}{0.91866}
\pgfmath@def{cosfrac}{44}{0.91531}    \pgfmath@def{cosfrac}{45}{0.91192}
\pgfmath@def{cosfrac}{46}{0.90849}    \pgfmath@def{cosfrac}{47}{0.90502}
\pgfmath@def{cosfrac}{48}{0.90152}    \pgfmath@def{cosfrac}{49}{0.89799}
\pgfmath@def{cosfrac}{50}{0.89442}    \pgfmath@def{cosfrac}{51}{0.89083}
\pgfmath@def{cosfrac}{52}{0.88721}    \pgfmath@def{cosfrac}{53}{0.88357}
\pgfmath@def{cosfrac}{54}{0.87990}    \pgfmath@def{cosfrac}{55}{0.87621}
\pgfmath@def{cosfrac}{56}{0.87250}    \pgfmath@def{cosfrac}{57}{0.86877}
\pgfmath@def{cosfrac}{58}{0.86503}    \pgfmath@def{cosfrac}{59}{0.86126}
\pgfmath@def{cosfrac}{60}{0.85749}    \pgfmath@def{cosfrac}{61}{0.85370}
\pgfmath@def{cosfrac}{62}{0.84990}    \pgfmath@def{cosfrac}{63}{0.84609}
\pgfmath@def{cosfrac}{64}{0.84227}    \pgfmath@def{cosfrac}{65}{0.83844}
\pgfmath@def{cosfrac}{66}{0.83460}    \pgfmath@def{cosfrac}{67}{0.83077}
\pgfmath@def{cosfrac}{68}{0.82692}    \pgfmath@def{cosfrac}{69}{0.82308}
\pgfmath@def{cosfrac}{70}{0.81923}    \pgfmath@def{cosfrac}{71}{0.81538}
\pgfmath@def{cosfrac}{72}{0.81153}    \pgfmath@def{cosfrac}{73}{0.80768}
\pgfmath@def{cosfrac}{74}{0.80384}    \pgfmath@def{cosfrac}{75}{0.80000}
\pgfmath@def{cosfrac}{76}{0.79616}    \pgfmath@def{cosfrac}{77}{0.79232}
\pgfmath@def{cosfrac}{78}{0.78850}    \pgfmath@def{cosfrac}{79}{0.78468}
\pgfmath@def{cosfrac}{80}{0.78086}    \pgfmath@def{cosfrac}{81}{0.77706}
\pgfmath@def{cosfrac}{82}{0.77326}    \pgfmath@def{cosfrac}{83}{0.76948}
\pgfmath@def{cosfrac}{84}{0.76570}    \pgfmath@def{cosfrac}{85}{0.76193}
\pgfmath@def{cosfrac}{86}{0.75818}    \pgfmath@def{cosfrac}{87}{0.75444}
\pgfmath@def{cosfrac}{88}{0.75071}    \pgfmath@def{cosfrac}{89}{0.74699}
\pgfmath@def{cosfrac}{90}{0.74329}    \pgfmath@def{cosfrac}{91}{0.73960}
\pgfmath@def{cosfrac}{92}{0.73593}    \pgfmath@def{cosfrac}{93}{0.73227}
\pgfmath@def{cosfrac}{94}{0.72862}    \pgfmath@def{cosfrac}{95}{0.72499}
\pgfmath@def{cosfrac}{96}{0.72138}    \pgfmath@def{cosfrac}{97}{0.71779}
\pgfmath@def{cosfrac}{98}{0.71421}    \pgfmath@def{cosfrac}{99}{0.71065}
\pgfmath@def{cosfrac}{100}{0.70710}

% Oh No! Some really loooooong tables.
\pgfmath@def{atan}{0}{0.00000}    \pgfmath@def{atan}{1}{0.05729}
\pgfmath@def{atan}{2}{0.11459}    \pgfmath@def{atan}{3}{0.17188}
\pgfmath@def{atan}{4}{0.22918}    \pgfmath@def{atan}{5}{0.28647}
\pgfmath@def{atan}{6}{0.34377}    \pgfmath@def{atan}{7}{0.40106}
\pgfmath@def{atan}{8}{0.45835}    \pgfmath@def{atan}{9}{0.51564}
\pgfmath@def{atan}{10}{0.57293}    \pgfmath@def{atan}{11}{0.63022}
\pgfmath@def{atan}{12}{0.68751}    \pgfmath@def{atan}{13}{0.74480}
\pgfmath@def{atan}{14}{0.80208}    \pgfmath@def{atan}{15}{0.85937}
\pgfmath@def{atan}{16}{0.91665}    \pgfmath@def{atan}{17}{0.97393}
\pgfmath@def{atan}{18}{1.03121}    \pgfmath@def{atan}{19}{1.08848}
\pgfmath@def{atan}{20}{1.14576}    \pgfmath@def{atan}{21}{1.20303}
\pgfmath@def{atan}{22}{1.26030}    \pgfmath@def{atan}{23}{1.31757}
\pgfmath@def{atan}{24}{1.37483}    \pgfmath@def{atan}{25}{1.43209}
\pgfmath@def{atan}{26}{1.48935}    \pgfmath@def{atan}{27}{1.54661}
\pgfmath@def{atan}{28}{1.60386}    \pgfmath@def{atan}{29}{1.66111}
\pgfmath@def{atan}{30}{1.71835}    \pgfmath@def{atan}{31}{1.77560}
\pgfmath@def{atan}{32}{1.83284}    \pgfmath@def{atan}{33}{1.89007}
\pgfmath@def{atan}{34}{1.94730}    \pgfmath@def{atan}{35}{2.00453}
\pgfmath@def{atan}{36}{2.06175}    \pgfmath@def{atan}{37}{2.11897}
\pgfmath@def{atan}{38}{2.17619}    \pgfmath@def{atan}{39}{2.23340}
\pgfmath@def{atan}{40}{2.29061}    \pgfmath@def{atan}{41}{2.34781}
\pgfmath@def{atan}{42}{2.40500}    \pgfmath@def{atan}{43}{2.46220}
\pgfmath@def{atan}{44}{2.51938}    \pgfmath@def{atan}{45}{2.57657}
\pgfmath@def{atan}{46}{2.63374}    \pgfmath@def{atan}{47}{2.69092}
\pgfmath@def{atan}{48}{2.74808}    \pgfmath@def{atan}{49}{2.80524}
\pgfmath@def{atan}{50}{2.86240}    \pgfmath@def{atan}{51}{2.91955}
\pgfmath@def{atan}{52}{2.97669}    \pgfmath@def{atan}{53}{3.03383}
\pgfmath@def{atan}{54}{3.09097}    \pgfmath@def{atan}{55}{3.14809}
\pgfmath@def{atan}{56}{3.20521}    \pgfmath@def{atan}{57}{3.26232}
\pgfmath@def{atan}{58}{3.31943}    \pgfmath@def{atan}{59}{3.37653}
\pgfmath@def{atan}{60}{3.43363}    \pgfmath@def{atan}{61}{3.49071}
\pgfmath@def{atan}{62}{3.54779}    \pgfmath@def{atan}{63}{3.60487}
\pgfmath@def{atan}{64}{3.66193}    \pgfmath@def{atan}{65}{3.71899}
\pgfmath@def{atan}{66}{3.77604}    \pgfmath@def{atan}{67}{3.83308}
\pgfmath@def{atan}{68}{3.89012}    \pgfmath@def{atan}{69}{3.94715}
\pgfmath@def{atan}{70}{4.00417}    \pgfmath@def{atan}{71}{4.06118}
\pgfmath@def{atan}{72}{4.11819}    \pgfmath@def{atan}{73}{4.17518}
\pgfmath@def{atan}{74}{4.23217}    \pgfmath@def{atan}{75}{4.28915}
\pgfmath@def{atan}{76}{4.34612}    \pgfmath@def{atan}{77}{4.40308}
\pgfmath@def{atan}{78}{4.46004}    \pgfmath@def{atan}{79}{4.51698}
\pgfmath@def{atan}{80}{4.57392}    \pgfmath@def{atan}{81}{4.63084}
\pgfmath@def{atan}{82}{4.68776}    \pgfmath@def{atan}{83}{4.74467}
\pgfmath@def{atan}{84}{4.80157}    \pgfmath@def{atan}{85}{4.85846}
\pgfmath@def{atan}{86}{4.91534}    \pgfmath@def{atan}{87}{4.97221}
\pgfmath@def{atan}{88}{5.02907}    \pgfmath@def{atan}{89}{5.08592}
\pgfmath@def{atan}{90}{5.14276}    \pgfmath@def{atan}{91}{5.19959}
\pgfmath@def{atan}{92}{5.25641}    \pgfmath@def{atan}{93}{5.31322}
\pgfmath@def{atan}{94}{5.37002}    \pgfmath@def{atan}{95}{5.42681}
\pgfmath@def{atan}{96}{5.48359}    \pgfmath@def{atan}{97}{5.54035}
\pgfmath@def{atan}{98}{5.59711}    \pgfmath@def{atan}{99}{5.65385}
\pgfmath@def{atan}{100}{5.71059}    \pgfmath@def{atan}{101}{5.76731}
\pgfmath@def{atan}{102}{5.82402}    \pgfmath@def{atan}{103}{5.88072}
\pgfmath@def{atan}{104}{5.93741}    \pgfmath@def{atan}{105}{5.99409}
\pgfmath@def{atan}{106}{6.05075}    \pgfmath@def{atan}{107}{6.10741}
\pgfmath@def{atan}{108}{6.16405}    \pgfmath@def{atan}{109}{6.22068}
\pgfmath@def{atan}{110}{6.27729}    \pgfmath@def{atan}{111}{6.33390}
\pgfmath@def{atan}{112}{6.39049}    \pgfmath@def{atan}{113}{6.44707}
\pgfmath@def{atan}{114}{6.50364}    \pgfmath@def{atan}{115}{6.56019}
\pgfmath@def{atan}{116}{6.61673}    \pgfmath@def{atan}{117}{6.67326}
\pgfmath@def{atan}{118}{6.72978}    \pgfmath@def{atan}{119}{6.78628}
\pgfmath@def{atan}{120}{6.84277}    \pgfmath@def{atan}{121}{6.89924}
\pgfmath@def{atan}{122}{6.95571}    \pgfmath@def{atan}{123}{7.01216}
\pgfmath@def{atan}{124}{7.06859}    \pgfmath@def{atan}{125}{7.12501}
\pgfmath@def{atan}{126}{7.18142}    \pgfmath@def{atan}{127}{7.23781}
\pgfmath@def{atan}{128}{7.29419}    \pgfmath@def{atan}{129}{7.35056}
\pgfmath@def{atan}{130}{7.40691}    \pgfmath@def{atan}{131}{7.46324}
\pgfmath@def{atan}{132}{7.51957}    \pgfmath@def{atan}{133}{7.57587}
\pgfmath@def{atan}{134}{7.63217}    \pgfmath@def{atan}{135}{7.68844}
\pgfmath@def{atan}{136}{7.74471}    \pgfmath@def{atan}{137}{7.80095}
\pgfmath@def{atan}{138}{7.85719}    \pgfmath@def{atan}{139}{7.91340}
\pgfmath@def{atan}{140}{7.96961}    \pgfmath@def{atan}{141}{8.02579}
\pgfmath@def{atan}{142}{8.08196}    \pgfmath@def{atan}{143}{8.13812}
\pgfmath@def{atan}{144}{8.19426}    \pgfmath@def{atan}{145}{8.25038}
\pgfmath@def{atan}{146}{8.30649}    \pgfmath@def{atan}{147}{8.36258}
\pgfmath@def{atan}{148}{8.41866}    \pgfmath@def{atan}{149}{8.47472}
\pgfmath@def{atan}{150}{8.53076}    \pgfmath@def{atan}{151}{8.58679}
\pgfmath@def{atan}{152}{8.64280}    \pgfmath@def{atan}{153}{8.69879}
\pgfmath@def{atan}{154}{8.75477}    \pgfmath@def{atan}{155}{8.81073}
\pgfmath@def{atan}{156}{8.86667}    \pgfmath@def{atan}{157}{8.92260}
\pgfmath@def{atan}{158}{8.97851}    \pgfmath@def{atan}{159}{9.03440}
\pgfmath@def{atan}{160}{9.09027}    \pgfmath@def{atan}{161}{9.14613}
\pgfmath@def{atan}{162}{9.20197}    \pgfmath@def{atan}{163}{9.25779}
\pgfmath@def{atan}{164}{9.31359}    \pgfmath@def{atan}{165}{9.36938}
\pgfmath@def{atan}{166}{9.42515}    \pgfmath@def{atan}{167}{9.48090}
\pgfmath@def{atan}{168}{9.53663}    \pgfmath@def{atan}{169}{9.59235}
\pgfmath@def{atan}{170}{9.64804}    \pgfmath@def{atan}{171}{9.70372}
\pgfmath@def{atan}{172}{9.75938}    \pgfmath@def{atan}{173}{9.81502}
\pgfmath@def{atan}{174}{9.87064}    \pgfmath@def{atan}{175}{9.92624}
\pgfmath@def{atan}{176}{9.98182}    \pgfmath@def{atan}{177}{10.03739}
\pgfmath@def{atan}{178}{10.09294}    \pgfmath@def{atan}{179}{10.14846}
\pgfmath@def{atan}{180}{10.20397}    \pgfmath@def{atan}{181}{10.25946}
\pgfmath@def{atan}{182}{10.31493}    \pgfmath@def{atan}{183}{10.37037}
\pgfmath@def{atan}{184}{10.42580}    \pgfmath@def{atan}{185}{10.48121}
\pgfmath@def{atan}{186}{10.53660}    \pgfmath@def{atan}{187}{10.59197}
\pgfmath@def{atan}{188}{10.64732}    \pgfmath@def{atan}{189}{10.70265}
\pgfmath@def{atan}{190}{10.75796}    \pgfmath@def{atan}{191}{10.81325}
\pgfmath@def{atan}{192}{10.86852}    \pgfmath@def{atan}{193}{10.92377}
\pgfmath@def{atan}{194}{10.97900}    \pgfmath@def{atan}{195}{11.03420}
\pgfmath@def{atan}{196}{11.08939}    \pgfmath@def{atan}{197}{11.14456}
\pgfmath@def{atan}{198}{11.19970}    \pgfmath@def{atan}{199}{11.25483}
\pgfmath@def{atan}{200}{11.30993}    \pgfmath@def{atan}{201}{11.36501}
\pgfmath@def{atan}{202}{11.42007}    \pgfmath@def{atan}{203}{11.47511}
\pgfmath@def{atan}{204}{11.53013}    \pgfmath@def{atan}{205}{11.58512}
\pgfmath@def{atan}{206}{11.64010}    \pgfmath@def{atan}{207}{11.69505}
\pgfmath@def{atan}{208}{11.74998}    \pgfmath@def{atan}{209}{11.80489}
\pgfmath@def{atan}{210}{11.85977}    \pgfmath@def{atan}{211}{11.91464}
\pgfmath@def{atan}{212}{11.96948}    \pgfmath@def{atan}{213}{12.02430}
\pgfmath@def{atan}{214}{12.07910}    \pgfmath@def{atan}{215}{12.13388}
\pgfmath@def{atan}{216}{12.18863}    \pgfmath@def{atan}{217}{12.24336}
\pgfmath@def{atan}{218}{12.29807}    \pgfmath@def{atan}{219}{12.35275}
\pgfmath@def{atan}{220}{12.40741}    \pgfmath@def{atan}{221}{12.46205}
\pgfmath@def{atan}{222}{12.51667}    \pgfmath@def{atan}{223}{12.57126}
\pgfmath@def{atan}{224}{12.62583}    \pgfmath@def{atan}{225}{12.68038}
\pgfmath@def{atan}{226}{12.73490}    \pgfmath@def{atan}{227}{12.78940}
\pgfmath@def{atan}{228}{12.84388}    \pgfmath@def{atan}{229}{12.89833}
\pgfmath@def{atan}{230}{12.95276}    \pgfmath@def{atan}{231}{13.00717}
\pgfmath@def{atan}{232}{13.06155}    \pgfmath@def{atan}{233}{13.11590}
\pgfmath@def{atan}{234}{13.17024}    \pgfmath@def{atan}{235}{13.22455}
\pgfmath@def{atan}{236}{13.27883}    \pgfmath@def{atan}{237}{13.33309}
\pgfmath@def{atan}{238}{13.38733}    \pgfmath@def{atan}{239}{13.44154}
\pgfmath@def{atan}{240}{13.49573}    \pgfmath@def{atan}{241}{13.54989}
\pgfmath@def{atan}{242}{13.60403}    \pgfmath@def{atan}{243}{13.65814}
\pgfmath@def{atan}{244}{13.71223}    \pgfmath@def{atan}{245}{13.76630}
\pgfmath@def{atan}{246}{13.82034}    \pgfmath@def{atan}{247}{13.87435}
\pgfmath@def{atan}{248}{13.92834}    \pgfmath@def{atan}{249}{13.98230}
\pgfmath@def{atan}{250}{14.03624}    \pgfmath@def{atan}{251}{14.09015}
\pgfmath@def{atan}{252}{14.14404}    \pgfmath@def{atan}{253}{14.19790}
\pgfmath@def{atan}{254}{14.25174}    \pgfmath@def{atan}{255}{14.30555}
\pgfmath@def{atan}{256}{14.35933}    \pgfmath@def{atan}{257}{14.41309}
\pgfmath@def{atan}{258}{14.46682}    \pgfmath@def{atan}{259}{14.52053}
\pgfmath@def{atan}{260}{14.57421}    \pgfmath@def{atan}{261}{14.62787}
\pgfmath@def{atan}{262}{14.68149}    \pgfmath@def{atan}{263}{14.73510}
\pgfmath@def{atan}{264}{14.78867}    \pgfmath@def{atan}{265}{14.84222}
\pgfmath@def{atan}{266}{14.89575}    \pgfmath@def{atan}{267}{14.94924}
\pgfmath@def{atan}{268}{15.00271}    \pgfmath@def{atan}{269}{15.05615}
\pgfmath@def{atan}{270}{15.10957}    \pgfmath@def{atan}{271}{15.16296}
\pgfmath@def{atan}{272}{15.21632}    \pgfmath@def{atan}{273}{15.26966}
\pgfmath@def{atan}{274}{15.32297}    \pgfmath@def{atan}{275}{15.37625}
\pgfmath@def{atan}{276}{15.42950}    \pgfmath@def{atan}{277}{15.48273}
\pgfmath@def{atan}{278}{15.53593}    \pgfmath@def{atan}{279}{15.58910}
\pgfmath@def{atan}{280}{15.64224}    \pgfmath@def{atan}{281}{15.69536}
\pgfmath@def{atan}{282}{15.74845}    \pgfmath@def{atan}{283}{15.80151}
\pgfmath@def{atan}{284}{15.85454}    \pgfmath@def{atan}{285}{15.90755}
\pgfmath@def{atan}{286}{15.96052}    \pgfmath@def{atan}{287}{16.01347}
\pgfmath@def{atan}{288}{16.06640}    \pgfmath@def{atan}{289}{16.11929}
\pgfmath@def{atan}{290}{16.17215}    \pgfmath@def{atan}{291}{16.22499}
\pgfmath@def{atan}{292}{16.27780}    \pgfmath@def{atan}{293}{16.33058}
\pgfmath@def{atan}{294}{16.38333}    \pgfmath@def{atan}{295}{16.43605}
\pgfmath@def{atan}{296}{16.48875}    \pgfmath@def{atan}{297}{16.54142}
\pgfmath@def{atan}{298}{16.59405}    \pgfmath@def{atan}{299}{16.64666}
\pgfmath@def{atan}{300}{16.69924}    \pgfmath@def{atan}{301}{16.75179}
\pgfmath@def{atan}{302}{16.80431}    \pgfmath@def{atan}{303}{16.85680}
\pgfmath@def{atan}{304}{16.90927}    \pgfmath@def{atan}{305}{16.96170}
\pgfmath@def{atan}{306}{17.01411}    \pgfmath@def{atan}{307}{17.06648}
\pgfmath@def{atan}{308}{17.11883}    \pgfmath@def{atan}{309}{17.17114}
\pgfmath@def{atan}{310}{17.22343}    \pgfmath@def{atan}{311}{17.27569}
\pgfmath@def{atan}{312}{17.32792}    \pgfmath@def{atan}{313}{17.38012}
\pgfmath@def{atan}{314}{17.43228}    \pgfmath@def{atan}{315}{17.48442}
\pgfmath@def{atan}{316}{17.53653}    \pgfmath@def{atan}{317}{17.58861}
\pgfmath@def{atan}{318}{17.64066}    \pgfmath@def{atan}{319}{17.69268}
\pgfmath@def{atan}{320}{17.74467}    \pgfmath@def{atan}{321}{17.79663}
\pgfmath@def{atan}{322}{17.84855}    \pgfmath@def{atan}{323}{17.90045}
\pgfmath@def{atan}{324}{17.95232}    \pgfmath@def{atan}{325}{18.00416}
\pgfmath@def{atan}{326}{18.05596}    \pgfmath@def{atan}{327}{18.10774}
\pgfmath@def{atan}{328}{18.15949}    \pgfmath@def{atan}{329}{18.21120}
\pgfmath@def{atan}{330}{18.26289}    \pgfmath@def{atan}{331}{18.31454}
\pgfmath@def{atan}{332}{18.36616}    \pgfmath@def{atan}{333}{18.41775}
\pgfmath@def{atan}{334}{18.46931}    \pgfmath@def{atan}{335}{18.52084}
\pgfmath@def{atan}{336}{18.57234}    \pgfmath@def{atan}{337}{18.62381}
\pgfmath@def{atan}{338}{18.67525}    \pgfmath@def{atan}{339}{18.72665}
\pgfmath@def{atan}{340}{18.77803}    \pgfmath@def{atan}{341}{18.82937}
\pgfmath@def{atan}{342}{18.88068}    \pgfmath@def{atan}{343}{18.93196}
\pgfmath@def{atan}{344}{18.98321}    \pgfmath@def{atan}{345}{19.03443}
\pgfmath@def{atan}{346}{19.08562}    \pgfmath@def{atan}{347}{19.13677}
\pgfmath@def{atan}{348}{19.18789}    \pgfmath@def{atan}{349}{19.23898}
\pgfmath@def{atan}{350}{19.29004}    \pgfmath@def{atan}{351}{19.34107}
\pgfmath@def{atan}{352}{19.39206}    \pgfmath@def{atan}{353}{19.44303}
\pgfmath@def{atan}{354}{19.49396}    \pgfmath@def{atan}{355}{19.54486}
\pgfmath@def{atan}{356}{19.59572}    \pgfmath@def{atan}{357}{19.64656}
\pgfmath@def{atan}{358}{19.69736}    \pgfmath@def{atan}{359}{19.74813}
\pgfmath@def{atan}{360}{19.79887}    \pgfmath@def{atan}{361}{19.84958}
\pgfmath@def{atan}{362}{19.90025}    \pgfmath@def{atan}{363}{19.95089}
\pgfmath@def{atan}{364}{20.00150}    \pgfmath@def{atan}{365}{20.05208}
\pgfmath@def{atan}{366}{20.10262}    \pgfmath@def{atan}{367}{20.15313}
\pgfmath@def{atan}{368}{20.20361}    \pgfmath@def{atan}{369}{20.25406}
\pgfmath@def{atan}{370}{20.30447}    \pgfmath@def{atan}{371}{20.35485}
\pgfmath@def{atan}{372}{20.40520}    \pgfmath@def{atan}{373}{20.45551}
\pgfmath@def{atan}{374}{20.50579}    \pgfmath@def{atan}{375}{20.55604}
\pgfmath@def{atan}{376}{20.60626}    \pgfmath@def{atan}{377}{20.65644}
\pgfmath@def{atan}{378}{20.70659}    \pgfmath@def{atan}{379}{20.75670}
\pgfmath@def{atan}{380}{20.80679}    \pgfmath@def{atan}{381}{20.85684}
\pgfmath@def{atan}{382}{20.90685}    \pgfmath@def{atan}{383}{20.95684}
\pgfmath@def{atan}{384}{21.00678}    \pgfmath@def{atan}{385}{21.05670}
\pgfmath@def{atan}{386}{21.10658}    \pgfmath@def{atan}{387}{21.15643}
\pgfmath@def{atan}{388}{21.20625}    \pgfmath@def{atan}{389}{21.25603}
\pgfmath@def{atan}{390}{21.30578}    \pgfmath@def{atan}{391}{21.35549}
\pgfmath@def{atan}{392}{21.40517}    \pgfmath@def{atan}{393}{21.45482}
\pgfmath@def{atan}{394}{21.50444}    \pgfmath@def{atan}{395}{21.55402}
\pgfmath@def{atan}{396}{21.60356}    \pgfmath@def{atan}{397}{21.65307}
\pgfmath@def{atan}{398}{21.70255}    \pgfmath@def{atan}{399}{21.75200}
\pgfmath@def{atan}{400}{21.80140}    \pgfmath@def{atan}{401}{21.85078}
\pgfmath@def{atan}{402}{21.90012}    \pgfmath@def{atan}{403}{21.94943}
\pgfmath@def{atan}{404}{21.99870}    \pgfmath@def{atan}{405}{22.04794}
\pgfmath@def{atan}{406}{22.09715}    \pgfmath@def{atan}{407}{22.14632}
\pgfmath@def{atan}{408}{22.19546}    \pgfmath@def{atan}{409}{22.24456}
\pgfmath@def{atan}{410}{22.29362}    \pgfmath@def{atan}{411}{22.34266}
\pgfmath@def{atan}{412}{22.39166}    \pgfmath@def{atan}{413}{22.44062}
\pgfmath@def{atan}{414}{22.48955}    \pgfmath@def{atan}{415}{22.53845}
\pgfmath@def{atan}{416}{22.58731}    \pgfmath@def{atan}{417}{22.63613}
\pgfmath@def{atan}{418}{22.68492}    \pgfmath@def{atan}{419}{22.73368}
\pgfmath@def{atan}{420}{22.78240}    \pgfmath@def{atan}{421}{22.83109}
\pgfmath@def{atan}{422}{22.87974}    \pgfmath@def{atan}{423}{22.92836}
\pgfmath@def{atan}{424}{22.97694}    \pgfmath@def{atan}{425}{23.02549}
\pgfmath@def{atan}{426}{23.07400}    \pgfmath@def{atan}{427}{23.12248}
\pgfmath@def{atan}{428}{23.17092}    \pgfmath@def{atan}{429}{23.21933}
\pgfmath@def{atan}{430}{23.26770}    \pgfmath@def{atan}{431}{23.31604}
\pgfmath@def{atan}{432}{23.36434}    \pgfmath@def{atan}{433}{23.41261}
\pgfmath@def{atan}{434}{23.46084}    \pgfmath@def{atan}{435}{23.50904}
\pgfmath@def{atan}{436}{23.55720}    \pgfmath@def{atan}{437}{23.60532}
\pgfmath@def{atan}{438}{23.65341}    \pgfmath@def{atan}{439}{23.70147}
\pgfmath@def{atan}{440}{23.74949}    \pgfmath@def{atan}{441}{23.79747}
\pgfmath@def{atan}{442}{23.84542}    \pgfmath@def{atan}{443}{23.89334}
\pgfmath@def{atan}{444}{23.94122}    \pgfmath@def{atan}{445}{23.98906}
\pgfmath@def{atan}{446}{24.03687}    \pgfmath@def{atan}{447}{24.08464}
\pgfmath@def{atan}{448}{24.13238}    \pgfmath@def{atan}{449}{24.18008}
\pgfmath@def{atan}{450}{24.22774}    \pgfmath@def{atan}{451}{24.27537}
\pgfmath@def{atan}{452}{24.32296}    \pgfmath@def{atan}{453}{24.37052}
\pgfmath@def{atan}{454}{24.41804}    \pgfmath@def{atan}{455}{24.46553}
\pgfmath@def{atan}{456}{24.51298}    \pgfmath@def{atan}{457}{24.56040}
\pgfmath@def{atan}{458}{24.60778}    \pgfmath@def{atan}{459}{24.65512}
\pgfmath@def{atan}{460}{24.70243}    \pgfmath@def{atan}{461}{24.74970}
\pgfmath@def{atan}{462}{24.79693}    \pgfmath@def{atan}{463}{24.84413}
\pgfmath@def{atan}{464}{24.89130}    \pgfmath@def{atan}{465}{24.93842}
\pgfmath@def{atan}{466}{24.98551}    \pgfmath@def{atan}{467}{25.03257}
\pgfmath@def{atan}{468}{25.07959}    \pgfmath@def{atan}{469}{25.12657}
\pgfmath@def{atan}{470}{25.17352}    \pgfmath@def{atan}{471}{25.22043}
\pgfmath@def{atan}{472}{25.26731}    \pgfmath@def{atan}{473}{25.31414}
\pgfmath@def{atan}{474}{25.36095}    \pgfmath@def{atan}{475}{25.40771}
\pgfmath@def{atan}{476}{25.45444}    \pgfmath@def{atan}{477}{25.50114}
\pgfmath@def{atan}{478}{25.54780}    \pgfmath@def{atan}{479}{25.59442}
\pgfmath@def{atan}{480}{25.64100}    \pgfmath@def{atan}{481}{25.68755}
\pgfmath@def{atan}{482}{25.73406}    \pgfmath@def{atan}{483}{25.78054}
\pgfmath@def{atan}{484}{25.82698}    \pgfmath@def{atan}{485}{25.87338}
\pgfmath@def{atan}{486}{25.91975}    \pgfmath@def{atan}{487}{25.96608}
\pgfmath@def{atan}{488}{26.01237}    \pgfmath@def{atan}{489}{26.05863}
\pgfmath@def{atan}{490}{26.10485}    \pgfmath@def{atan}{491}{26.15103}
\pgfmath@def{atan}{492}{26.19718}    \pgfmath@def{atan}{493}{26.24329}
\pgfmath@def{atan}{494}{26.28937}    \pgfmath@def{atan}{495}{26.33541}
\pgfmath@def{atan}{496}{26.38141}    \pgfmath@def{atan}{497}{26.42737}
\pgfmath@def{atan}{498}{26.47330}    \pgfmath@def{atan}{499}{26.51919}
\pgfmath@def{atan}{500}{26.56505}    \pgfmath@def{atan}{501}{26.61086}
\pgfmath@def{atan}{502}{26.65665}    \pgfmath@def{atan}{503}{26.70239}
\pgfmath@def{atan}{504}{26.74810}    \pgfmath@def{atan}{505}{26.79377}
\pgfmath@def{atan}{506}{26.83941}    \pgfmath@def{atan}{507}{26.88500}
\pgfmath@def{atan}{508}{26.93057}    \pgfmath@def{atan}{509}{26.97609}
\pgfmath@def{atan}{510}{27.02158}    \pgfmath@def{atan}{511}{27.06703}
\pgfmath@def{atan}{512}{27.11244}    \pgfmath@def{atan}{513}{27.15782}
\pgfmath@def{atan}{514}{27.20316}    \pgfmath@def{atan}{515}{27.24846}
\pgfmath@def{atan}{516}{27.29373}    \pgfmath@def{atan}{517}{27.33896}
\pgfmath@def{atan}{518}{27.38415}    \pgfmath@def{atan}{519}{27.42931}
\pgfmath@def{atan}{520}{27.47443}    \pgfmath@def{atan}{521}{27.51951}
\pgfmath@def{atan}{522}{27.56455}    \pgfmath@def{atan}{523}{27.60956}
\pgfmath@def{atan}{524}{27.65453}    \pgfmath@def{atan}{525}{27.69947}
\pgfmath@def{atan}{526}{27.74437}    \pgfmath@def{atan}{527}{27.78923}
\pgfmath@def{atan}{528}{27.83405}    \pgfmath@def{atan}{529}{27.87884}
\pgfmath@def{atan}{530}{27.92359}    \pgfmath@def{atan}{531}{27.96830}
\pgfmath@def{atan}{532}{28.01297}    \pgfmath@def{atan}{533}{28.05761}
\pgfmath@def{atan}{534}{28.10221}    \pgfmath@def{atan}{535}{28.14678}
\pgfmath@def{atan}{536}{28.19130}    \pgfmath@def{atan}{537}{28.23579}
\pgfmath@def{atan}{538}{28.28025}    \pgfmath@def{atan}{539}{28.32466}
\pgfmath@def{atan}{540}{28.36904}    \pgfmath@def{atan}{541}{28.41338}
\pgfmath@def{atan}{542}{28.45769}    \pgfmath@def{atan}{543}{28.50196}
\pgfmath@def{atan}{544}{28.54619}    \pgfmath@def{atan}{545}{28.59038}
\pgfmath@def{atan}{546}{28.63454}    \pgfmath@def{atan}{547}{28.67865}
\pgfmath@def{atan}{548}{28.72274}    \pgfmath@def{atan}{549}{28.76678}
\pgfmath@def{atan}{550}{28.81079}    \pgfmath@def{atan}{551}{28.85476}
\pgfmath@def{atan}{552}{28.89869}    \pgfmath@def{atan}{553}{28.94259}
\pgfmath@def{atan}{554}{28.98645}    \pgfmath@def{atan}{555}{29.03027}
\pgfmath@def{atan}{556}{29.07405}    \pgfmath@def{atan}{557}{29.11780}
\pgfmath@def{atan}{558}{29.16151}    \pgfmath@def{atan}{559}{29.20519}
\pgfmath@def{atan}{560}{29.24882}    \pgfmath@def{atan}{561}{29.29242}
\pgfmath@def{atan}{562}{29.33598}    \pgfmath@def{atan}{563}{29.37951}
\pgfmath@def{atan}{564}{29.42299}    \pgfmath@def{atan}{565}{29.46644}
\pgfmath@def{atan}{566}{29.50986}    \pgfmath@def{atan}{567}{29.55323}
\pgfmath@def{atan}{568}{29.59657}    \pgfmath@def{atan}{569}{29.63987}
\pgfmath@def{atan}{570}{29.68314}    \pgfmath@def{atan}{571}{29.72636}
\pgfmath@def{atan}{572}{29.76955}    \pgfmath@def{atan}{573}{29.81270}
\pgfmath@def{atan}{574}{29.85582}    \pgfmath@def{atan}{575}{29.89890}
\pgfmath@def{atan}{576}{29.94194}    \pgfmath@def{atan}{577}{29.98494}
\pgfmath@def{atan}{578}{30.02791}    \pgfmath@def{atan}{579}{30.07084}
\pgfmath@def{atan}{580}{30.11373}    \pgfmath@def{atan}{581}{30.15658}
\pgfmath@def{atan}{582}{30.19940}    \pgfmath@def{atan}{583}{30.24218}
\pgfmath@def{atan}{584}{30.28492}    \pgfmath@def{atan}{585}{30.32763}
\pgfmath@def{atan}{586}{30.37030}    \pgfmath@def{atan}{587}{30.41293}
\pgfmath@def{atan}{588}{30.45552}    \pgfmath@def{atan}{589}{30.49808}
\pgfmath@def{atan}{590}{30.54060}    \pgfmath@def{atan}{591}{30.58308}
\pgfmath@def{atan}{592}{30.62553}    \pgfmath@def{atan}{593}{30.66794}
\pgfmath@def{atan}{594}{30.71031}    \pgfmath@def{atan}{595}{30.75264}
\pgfmath@def{atan}{596}{30.79494}    \pgfmath@def{atan}{597}{30.83720}
\pgfmath@def{atan}{598}{30.87942}    \pgfmath@def{atan}{599}{30.92160}
\pgfmath@def{atan}{600}{30.96375}    \pgfmath@def{atan}{601}{31.00586}
\pgfmath@def{atan}{602}{31.04794}    \pgfmath@def{atan}{603}{31.08997}
\pgfmath@def{atan}{604}{31.13197}    \pgfmath@def{atan}{605}{31.17393}
\pgfmath@def{atan}{606}{31.21586}    \pgfmath@def{atan}{607}{31.25775}
\pgfmath@def{atan}{608}{31.29960}    \pgfmath@def{atan}{609}{31.34141}
\pgfmath@def{atan}{610}{31.38319}    \pgfmath@def{atan}{611}{31.42493}
\pgfmath@def{atan}{612}{31.46663}    \pgfmath@def{atan}{613}{31.50829}
\pgfmath@def{atan}{614}{31.54992}    \pgfmath@def{atan}{615}{31.59151}
\pgfmath@def{atan}{616}{31.63306}    \pgfmath@def{atan}{617}{31.67458}
\pgfmath@def{atan}{618}{31.71606}    \pgfmath@def{atan}{619}{31.75750}
\pgfmath@def{atan}{620}{31.79891}    \pgfmath@def{atan}{621}{31.84028}
\pgfmath@def{atan}{622}{31.88161}    \pgfmath@def{atan}{623}{31.92290}
\pgfmath@def{atan}{624}{31.96416}    \pgfmath@def{atan}{625}{32.00538}
\pgfmath@def{atan}{626}{32.04656}    \pgfmath@def{atan}{627}{32.08771}
\pgfmath@def{atan}{628}{32.12882}    \pgfmath@def{atan}{629}{32.16989}
\pgfmath@def{atan}{630}{32.21092}    \pgfmath@def{atan}{631}{32.25192}
\pgfmath@def{atan}{632}{32.29288}    \pgfmath@def{atan}{633}{32.33381}
\pgfmath@def{atan}{634}{32.37469}    \pgfmath@def{atan}{635}{32.41554}
\pgfmath@def{atan}{636}{32.45636}    \pgfmath@def{atan}{637}{32.49713}
\pgfmath@def{atan}{638}{32.53787}    \pgfmath@def{atan}{639}{32.57857}
\pgfmath@def{atan}{640}{32.61924}    \pgfmath@def{atan}{641}{32.65987}
\pgfmath@def{atan}{642}{32.70046}    \pgfmath@def{atan}{643}{32.74101}
\pgfmath@def{atan}{644}{32.78153}    \pgfmath@def{atan}{645}{32.82201}
\pgfmath@def{atan}{646}{32.86246}    \pgfmath@def{atan}{647}{32.90286}
\pgfmath@def{atan}{648}{32.94323}    \pgfmath@def{atan}{649}{32.98357}
\pgfmath@def{atan}{650}{33.02386}    \pgfmath@def{atan}{651}{33.06412}
\pgfmath@def{atan}{652}{33.10435}    \pgfmath@def{atan}{653}{33.14453}
\pgfmath@def{atan}{654}{33.18468}    \pgfmath@def{atan}{655}{33.22479}
\pgfmath@def{atan}{656}{33.26487}    \pgfmath@def{atan}{657}{33.30491}
\pgfmath@def{atan}{658}{33.34491}    \pgfmath@def{atan}{659}{33.38488}
\pgfmath@def{atan}{660}{33.42481}    \pgfmath@def{atan}{661}{33.46470}
\pgfmath@def{atan}{662}{33.50455}    \pgfmath@def{atan}{663}{33.54437}
\pgfmath@def{atan}{664}{33.58416}    \pgfmath@def{atan}{665}{33.62390}
\pgfmath@def{atan}{666}{33.66361}    \pgfmath@def{atan}{667}{33.70328}
\pgfmath@def{atan}{668}{33.74292}    \pgfmath@def{atan}{669}{33.78252}
\pgfmath@def{atan}{670}{33.82208}    \pgfmath@def{atan}{671}{33.86161}
\pgfmath@def{atan}{672}{33.90110}    \pgfmath@def{atan}{673}{33.94055}
\pgfmath@def{atan}{674}{33.97997}    \pgfmath@def{atan}{675}{34.01935}
\pgfmath@def{atan}{676}{34.05869}    \pgfmath@def{atan}{677}{34.09800}
\pgfmath@def{atan}{678}{34.13727}    \pgfmath@def{atan}{679}{34.17650}
\pgfmath@def{atan}{680}{34.21570}    \pgfmath@def{atan}{681}{34.25486}
\pgfmath@def{atan}{682}{34.29398}    \pgfmath@def{atan}{683}{34.33307}
\pgfmath@def{atan}{684}{34.37212}    \pgfmath@def{atan}{685}{34.41114}
\pgfmath@def{atan}{686}{34.45012}    \pgfmath@def{atan}{687}{34.48906}
\pgfmath@def{atan}{688}{34.52797}    \pgfmath@def{atan}{689}{34.56684}
\pgfmath@def{atan}{690}{34.60567}    \pgfmath@def{atan}{691}{34.64447}
\pgfmath@def{atan}{692}{34.68323}    \pgfmath@def{atan}{693}{34.72195}
\pgfmath@def{atan}{694}{34.76064}    \pgfmath@def{atan}{695}{34.79930}
\pgfmath@def{atan}{696}{34.83791}    \pgfmath@def{atan}{697}{34.87649}
\pgfmath@def{atan}{698}{34.91504}    \pgfmath@def{atan}{699}{34.95354}
\pgfmath@def{atan}{700}{34.99202}    \pgfmath@def{atan}{701}{35.03045}
\pgfmath@def{atan}{702}{35.06885}    \pgfmath@def{atan}{703}{35.10721}
\pgfmath@def{atan}{704}{35.14554}    \pgfmath@def{atan}{705}{35.18383}
\pgfmath@def{atan}{706}{35.22209}    \pgfmath@def{atan}{707}{35.26031}
\pgfmath@def{atan}{708}{35.29849}    \pgfmath@def{atan}{709}{35.33664}
\pgfmath@def{atan}{710}{35.37475}    \pgfmath@def{atan}{711}{35.41282}
\pgfmath@def{atan}{712}{35.45086}    \pgfmath@def{atan}{713}{35.48886}
\pgfmath@def{atan}{714}{35.52683}    \pgfmath@def{atan}{715}{35.56476}
\pgfmath@def{atan}{716}{35.60266}    \pgfmath@def{atan}{717}{35.64052}
\pgfmath@def{atan}{718}{35.67834}    \pgfmath@def{atan}{719}{35.71613}
\pgfmath@def{atan}{720}{35.75388}    \pgfmath@def{atan}{721}{35.79160}
\pgfmath@def{atan}{722}{35.82928}    \pgfmath@def{atan}{723}{35.86692}
\pgfmath@def{atan}{724}{35.90453}    \pgfmath@def{atan}{725}{35.94211}
\pgfmath@def{atan}{726}{35.97965}    \pgfmath@def{atan}{727}{36.01715}
\pgfmath@def{atan}{728}{36.05461}    \pgfmath@def{atan}{729}{36.09204}
\pgfmath@def{atan}{730}{36.12944}    \pgfmath@def{atan}{731}{36.16680}
\pgfmath@def{atan}{732}{36.20412}    \pgfmath@def{atan}{733}{36.24141}
\pgfmath@def{atan}{734}{36.27866}    \pgfmath@def{atan}{735}{36.31588}
\pgfmath@def{atan}{736}{36.35306}    \pgfmath@def{atan}{737}{36.39021}
\pgfmath@def{atan}{738}{36.42732}    \pgfmath@def{atan}{739}{36.46440}
\pgfmath@def{atan}{740}{36.50144}    \pgfmath@def{atan}{741}{36.53844}
\pgfmath@def{atan}{742}{36.57541}    \pgfmath@def{atan}{743}{36.61234}
\pgfmath@def{atan}{744}{36.64924}    \pgfmath@def{atan}{745}{36.68611}
\pgfmath@def{atan}{746}{36.72293}    \pgfmath@def{atan}{747}{36.75973}
\pgfmath@def{atan}{748}{36.79648}    \pgfmath@def{atan}{749}{36.83321}
\pgfmath@def{atan}{750}{36.86989}    \pgfmath@def{atan}{751}{36.90654}
\pgfmath@def{atan}{752}{36.94316}    \pgfmath@def{atan}{753}{36.97974}
\pgfmath@def{atan}{754}{37.01629}    \pgfmath@def{atan}{755}{37.05280}
\pgfmath@def{atan}{756}{37.08928}    \pgfmath@def{atan}{757}{37.12572}
\pgfmath@def{atan}{758}{37.16212}    \pgfmath@def{atan}{759}{37.19849}
\pgfmath@def{atan}{760}{37.23483}    \pgfmath@def{atan}{761}{37.27113}
\pgfmath@def{atan}{762}{37.30740}    \pgfmath@def{atan}{763}{37.34363}
\pgfmath@def{atan}{764}{37.37982}    \pgfmath@def{atan}{765}{37.41598}
\pgfmath@def{atan}{766}{37.45211}    \pgfmath@def{atan}{767}{37.48820}
\pgfmath@def{atan}{768}{37.52426}    \pgfmath@def{atan}{769}{37.56028}
\pgfmath@def{atan}{770}{37.59627}    \pgfmath@def{atan}{771}{37.63222}
\pgfmath@def{atan}{772}{37.66814}    \pgfmath@def{atan}{773}{37.70402}
\pgfmath@def{atan}{774}{37.73987}    \pgfmath@def{atan}{775}{37.77568}
\pgfmath@def{atan}{776}{37.81146}    \pgfmath@def{atan}{777}{37.84720}
\pgfmath@def{atan}{778}{37.88291}    \pgfmath@def{atan}{779}{37.91859}
\pgfmath@def{atan}{780}{37.95423}    \pgfmath@def{atan}{781}{37.98983}
\pgfmath@def{atan}{782}{38.02540}    \pgfmath@def{atan}{783}{38.06094}
\pgfmath@def{atan}{784}{38.09644}    \pgfmath@def{atan}{785}{38.13191}
\pgfmath@def{atan}{786}{38.16734}    \pgfmath@def{atan}{787}{38.20274}
\pgfmath@def{atan}{788}{38.23811}    \pgfmath@def{atan}{789}{38.27344}
\pgfmath@def{atan}{790}{38.30873}    \pgfmath@def{atan}{791}{38.34399}
\pgfmath@def{atan}{792}{38.37922}    \pgfmath@def{atan}{793}{38.41441}
\pgfmath@def{atan}{794}{38.44957}    \pgfmath@def{atan}{795}{38.48469}
\pgfmath@def{atan}{796}{38.51979}    \pgfmath@def{atan}{797}{38.55484}
\pgfmath@def{atan}{798}{38.58986}    \pgfmath@def{atan}{799}{38.62485}
\pgfmath@def{atan}{800}{38.65980}    \pgfmath@def{atan}{801}{38.69472}
\pgfmath@def{atan}{802}{38.72961}    \pgfmath@def{atan}{803}{38.76446}
\pgfmath@def{atan}{804}{38.79928}    \pgfmath@def{atan}{805}{38.83406}
\pgfmath@def{atan}{806}{38.86881}    \pgfmath@def{atan}{807}{38.90353}
\pgfmath@def{atan}{808}{38.93821}    \pgfmath@def{atan}{809}{38.97285}
\pgfmath@def{atan}{810}{39.00747}    \pgfmath@def{atan}{811}{39.04205}
\pgfmath@def{atan}{812}{39.07659}    \pgfmath@def{atan}{813}{39.11111}
\pgfmath@def{atan}{814}{39.14558}    \pgfmath@def{atan}{815}{39.18003}
\pgfmath@def{atan}{816}{39.21444}    \pgfmath@def{atan}{817}{39.24882}
\pgfmath@def{atan}{818}{39.28316}    \pgfmath@def{atan}{819}{39.31747}
\pgfmath@def{atan}{820}{39.35175}    \pgfmath@def{atan}{821}{39.38599}
\pgfmath@def{atan}{822}{39.42020}    \pgfmath@def{atan}{823}{39.45438}
\pgfmath@def{atan}{824}{39.48852}    \pgfmath@def{atan}{825}{39.52263}
\pgfmath@def{atan}{826}{39.55670}    \pgfmath@def{atan}{827}{39.59074}
\pgfmath@def{atan}{828}{39.62475}    \pgfmath@def{atan}{829}{39.65873}
\pgfmath@def{atan}{830}{39.69267}    \pgfmath@def{atan}{831}{39.72658}
\pgfmath@def{atan}{832}{39.76045}    \pgfmath@def{atan}{833}{39.79429}
\pgfmath@def{atan}{834}{39.82810}    \pgfmath@def{atan}{835}{39.86188}
\pgfmath@def{atan}{836}{39.89562}    \pgfmath@def{atan}{837}{39.92933}
\pgfmath@def{atan}{838}{39.96300}    \pgfmath@def{atan}{839}{39.99665}
\pgfmath@def{atan}{840}{40.03025}    \pgfmath@def{atan}{841}{40.06383}
\pgfmath@def{atan}{842}{40.09737}    \pgfmath@def{atan}{843}{40.13088}
\pgfmath@def{atan}{844}{40.16436}    \pgfmath@def{atan}{845}{40.19781}
\pgfmath@def{atan}{846}{40.23122}    \pgfmath@def{atan}{847}{40.26459}
\pgfmath@def{atan}{848}{40.29794}    \pgfmath@def{atan}{849}{40.33125}
\pgfmath@def{atan}{850}{40.36453}    \pgfmath@def{atan}{851}{40.39778}
\pgfmath@def{atan}{852}{40.43099}    \pgfmath@def{atan}{853}{40.46417}
\pgfmath@def{atan}{854}{40.49732}    \pgfmath@def{atan}{855}{40.53044}
\pgfmath@def{atan}{856}{40.56352}    \pgfmath@def{atan}{857}{40.59657}
\pgfmath@def{atan}{858}{40.62959}    \pgfmath@def{atan}{859}{40.66257}
\pgfmath@def{atan}{860}{40.69553}    \pgfmath@def{atan}{861}{40.72845}
\pgfmath@def{atan}{862}{40.76133}    \pgfmath@def{atan}{863}{40.79419}
\pgfmath@def{atan}{864}{40.82701}    \pgfmath@def{atan}{865}{40.85980}
\pgfmath@def{atan}{866}{40.89256}    \pgfmath@def{atan}{867}{40.92528}
\pgfmath@def{atan}{868}{40.95798}    \pgfmath@def{atan}{869}{40.99064}
\pgfmath@def{atan}{870}{41.02326}    \pgfmath@def{atan}{871}{41.05586}
\pgfmath@def{atan}{872}{41.08842}    \pgfmath@def{atan}{873}{41.12095}
\pgfmath@def{atan}{874}{41.15345}    \pgfmath@def{atan}{875}{41.18592}
\pgfmath@def{atan}{876}{41.21836}    \pgfmath@def{atan}{877}{41.25076}
\pgfmath@def{atan}{878}{41.28313}    \pgfmath@def{atan}{879}{41.31547}
\pgfmath@def{atan}{880}{41.34777}    \pgfmath@def{atan}{881}{41.38005}
\pgfmath@def{atan}{882}{41.41229}    \pgfmath@def{atan}{883}{41.44450}
\pgfmath@def{atan}{884}{41.47668}    \pgfmath@def{atan}{885}{41.50882}
\pgfmath@def{atan}{886}{41.54094}    \pgfmath@def{atan}{887}{41.57302}
\pgfmath@def{atan}{888}{41.60507}    \pgfmath@def{atan}{889}{41.63709}
\pgfmath@def{atan}{890}{41.66908}    \pgfmath@def{atan}{891}{41.70103}
\pgfmath@def{atan}{892}{41.73296}    \pgfmath@def{atan}{893}{41.76485}
\pgfmath@def{atan}{894}{41.79671}    \pgfmath@def{atan}{895}{41.82854}
\pgfmath@def{atan}{896}{41.86034}    \pgfmath@def{atan}{897}{41.89210}
\pgfmath@def{atan}{898}{41.92383}    \pgfmath@def{atan}{899}{41.95554}
\pgfmath@def{atan}{900}{41.98721}    \pgfmath@def{atan}{901}{42.01885}
\pgfmath@def{atan}{902}{42.05046}    \pgfmath@def{atan}{903}{42.08203}
\pgfmath@def{atan}{904}{42.11358}    \pgfmath@def{atan}{905}{42.14509}
\pgfmath@def{atan}{906}{42.17657}    \pgfmath@def{atan}{907}{42.20802}
\pgfmath@def{atan}{908}{42.23944}    \pgfmath@def{atan}{909}{42.27083}
\pgfmath@def{atan}{910}{42.30219}    \pgfmath@def{atan}{911}{42.33352}
\pgfmath@def{atan}{912}{42.36481}    \pgfmath@def{atan}{913}{42.39607}
\pgfmath@def{atan}{914}{42.42731}    \pgfmath@def{atan}{915}{42.45851}
\pgfmath@def{atan}{916}{42.48968}    \pgfmath@def{atan}{917}{42.52082}
\pgfmath@def{atan}{918}{42.55193}    \pgfmath@def{atan}{919}{42.58300}
\pgfmath@def{atan}{920}{42.61405}    \pgfmath@def{atan}{921}{42.64507}
\pgfmath@def{atan}{922}{42.67605}    \pgfmath@def{atan}{923}{42.70701}
\pgfmath@def{atan}{924}{42.73793}    \pgfmath@def{atan}{925}{42.76882}
\pgfmath@def{atan}{926}{42.79968}    \pgfmath@def{atan}{927}{42.83051}
\pgfmath@def{atan}{928}{42.86131}    \pgfmath@def{atan}{929}{42.89208}
\pgfmath@def{atan}{930}{42.92282}    \pgfmath@def{atan}{931}{42.95353}
\pgfmath@def{atan}{932}{42.98421}    \pgfmath@def{atan}{933}{43.01485}
\pgfmath@def{atan}{934}{43.04547}    \pgfmath@def{atan}{935}{43.07605}
\pgfmath@def{atan}{936}{43.10661}    \pgfmath@def{atan}{937}{43.13713}
\pgfmath@def{atan}{938}{43.16763}    \pgfmath@def{atan}{939}{43.19809}
\pgfmath@def{atan}{940}{43.22853}    \pgfmath@def{atan}{941}{43.25893}
\pgfmath@def{atan}{942}{43.28930}    \pgfmath@def{atan}{943}{43.31964}
\pgfmath@def{atan}{944}{43.34996}    \pgfmath@def{atan}{945}{43.38024}
\pgfmath@def{atan}{946}{43.41049}    \pgfmath@def{atan}{947}{43.44071}
\pgfmath@def{atan}{948}{43.47090}    \pgfmath@def{atan}{949}{43.50106}
\pgfmath@def{atan}{950}{43.53119}    \pgfmath@def{atan}{951}{43.56130}
\pgfmath@def{atan}{952}{43.59137}    \pgfmath@def{atan}{953}{43.62141}
\pgfmath@def{atan}{954}{43.65142}    \pgfmath@def{atan}{955}{43.68140}
\pgfmath@def{atan}{956}{43.71135}    \pgfmath@def{atan}{957}{43.74127}
\pgfmath@def{atan}{958}{43.77116}    \pgfmath@def{atan}{959}{43.80102}
\pgfmath@def{atan}{960}{43.83086}    \pgfmath@def{atan}{961}{43.86066}
\pgfmath@def{atan}{962}{43.89043}    \pgfmath@def{atan}{963}{43.92017}
\pgfmath@def{atan}{964}{43.94988}    \pgfmath@def{atan}{965}{43.97957}
\pgfmath@def{atan}{966}{44.00922}    \pgfmath@def{atan}{967}{44.03884}
\pgfmath@def{atan}{968}{44.06844}    \pgfmath@def{atan}{969}{44.09800}
\pgfmath@def{atan}{970}{44.12754}    \pgfmath@def{atan}{971}{44.15704}
\pgfmath@def{atan}{972}{44.18652}    \pgfmath@def{atan}{973}{44.21597}
\pgfmath@def{atan}{974}{44.24538}    \pgfmath@def{atan}{975}{44.27477}
\pgfmath@def{atan}{976}{44.30413}    \pgfmath@def{atan}{977}{44.33346}
\pgfmath@def{atan}{978}{44.36276}    \pgfmath@def{atan}{979}{44.39203}
\pgfmath@def{atan}{980}{44.42127}    \pgfmath@def{atan}{981}{44.45048}
\pgfmath@def{atan}{982}{44.47966}    \pgfmath@def{atan}{983}{44.50882}
\pgfmath@def{atan}{984}{44.53794}    \pgfmath@def{atan}{985}{44.56704}
\pgfmath@def{atan}{986}{44.59610}    \pgfmath@def{atan}{987}{44.62514}
\pgfmath@def{atan}{988}{44.65415}    \pgfmath@def{atan}{989}{44.68313}
\pgfmath@def{atan}{990}{44.71208}    \pgfmath@def{atan}{991}{44.74100}
\pgfmath@def{atan}{992}{44.76989}    \pgfmath@def{atan}{993}{44.79876}
\pgfmath@def{atan}{994}{44.82759}    \pgfmath@def{atan}{995}{44.85640}
\pgfmath@def{atan}{996}{44.88517}    \pgfmath@def{atan}{997}{44.91392}
\pgfmath@def{atan}{998}{44.94264}    \pgfmath@def{atan}{999}{44.97133}
\pgfmath@def{atan}{1000}{45.00000}

\pgfmath@def{acos}{0}{90.00000}    \pgfmath@def{acos}{1}{89.94270}
\pgfmath@def{acos}{2}{89.88540}    \pgfmath@def{acos}{3}{89.82811}
\pgfmath@def{acos}{4}{89.77081}    \pgfmath@def{acos}{5}{89.71352}
\pgfmath@def{acos}{6}{89.65622}    \pgfmath@def{acos}{7}{89.59892}
\pgfmath@def{acos}{8}{89.54162}    \pgfmath@def{acos}{9}{89.48433}
\pgfmath@def{acos}{10}{89.42703}    \pgfmath@def{acos}{11}{89.36973}
\pgfmath@def{acos}{12}{89.31243}    \pgfmath@def{acos}{13}{89.25513}
\pgfmath@def{acos}{14}{89.19783}    \pgfmath@def{acos}{15}{89.14053}
\pgfmath@def{acos}{16}{89.08322}    \pgfmath@def{acos}{17}{89.02592}
\pgfmath@def{acos}{18}{88.96862}    \pgfmath@def{acos}{19}{88.91131}
\pgfmath@def{acos}{20}{88.85400}    \pgfmath@def{acos}{21}{88.79670}
\pgfmath@def{acos}{22}{88.73939}    \pgfmath@def{acos}{23}{88.68208}
\pgfmath@def{acos}{24}{88.62476}    \pgfmath@def{acos}{25}{88.56745}
\pgfmath@def{acos}{26}{88.51014}    \pgfmath@def{acos}{27}{88.45282}
\pgfmath@def{acos}{28}{88.39550}    \pgfmath@def{acos}{29}{88.33818}
\pgfmath@def{acos}{30}{88.28086}    \pgfmath@def{acos}{31}{88.22354}
\pgfmath@def{acos}{32}{88.16622}    \pgfmath@def{acos}{33}{88.10889}
\pgfmath@def{acos}{34}{88.05156}    \pgfmath@def{acos}{35}{87.99423}
\pgfmath@def{acos}{36}{87.93690}    \pgfmath@def{acos}{37}{87.87957}
\pgfmath@def{acos}{38}{87.82223}    \pgfmath@def{acos}{39}{87.76489}
\pgfmath@def{acos}{40}{87.70755}    \pgfmath@def{acos}{41}{87.65021}
\pgfmath@def{acos}{42}{87.59286}    \pgfmath@def{acos}{43}{87.53552}
\pgfmath@def{acos}{44}{87.47817}    \pgfmath@def{acos}{45}{87.42081}
\pgfmath@def{acos}{46}{87.36346}    \pgfmath@def{acos}{47}{87.30610}
\pgfmath@def{acos}{48}{87.24874}    \pgfmath@def{acos}{49}{87.19138}
\pgfmath@def{acos}{50}{87.13401}    \pgfmath@def{acos}{51}{87.07664}
\pgfmath@def{acos}{52}{87.01927}    \pgfmath@def{acos}{53}{86.96190}
\pgfmath@def{acos}{54}{86.90452}    \pgfmath@def{acos}{55}{86.84714}
\pgfmath@def{acos}{56}{86.78975}    \pgfmath@def{acos}{57}{86.73237}
\pgfmath@def{acos}{58}{86.67497}    \pgfmath@def{acos}{59}{86.61758}
\pgfmath@def{acos}{60}{86.56018}    \pgfmath@def{acos}{61}{86.50278}
\pgfmath@def{acos}{62}{86.44538}    \pgfmath@def{acos}{63}{86.38797}
\pgfmath@def{acos}{64}{86.33056}    \pgfmath@def{acos}{65}{86.27314}
\pgfmath@def{acos}{66}{86.21572}    \pgfmath@def{acos}{67}{86.15830}
\pgfmath@def{acos}{68}{86.10087}    \pgfmath@def{acos}{69}{86.04344}
\pgfmath@def{acos}{70}{85.98601}    \pgfmath@def{acos}{71}{85.92857}
\pgfmath@def{acos}{72}{85.87113}    \pgfmath@def{acos}{73}{85.81368}
\pgfmath@def{acos}{74}{85.75623}    \pgfmath@def{acos}{75}{85.69877}
\pgfmath@def{acos}{76}{85.64131}    \pgfmath@def{acos}{77}{85.58385}
\pgfmath@def{acos}{78}{85.52638}    \pgfmath@def{acos}{79}{85.46891}
\pgfmath@def{acos}{80}{85.41143}    \pgfmath@def{acos}{81}{85.35395}
\pgfmath@def{acos}{82}{85.29646}    \pgfmath@def{acos}{83}{85.23897}
\pgfmath@def{acos}{84}{85.18147}    \pgfmath@def{acos}{85}{85.12397}
\pgfmath@def{acos}{86}{85.06646}    \pgfmath@def{acos}{87}{85.00895}
\pgfmath@def{acos}{88}{84.95144}    \pgfmath@def{acos}{89}{84.89392}
\pgfmath@def{acos}{90}{84.83639}    \pgfmath@def{acos}{91}{84.77886}
\pgfmath@def{acos}{92}{84.72132}    \pgfmath@def{acos}{93}{84.66378}
\pgfmath@def{acos}{94}{84.60623}    \pgfmath@def{acos}{95}{84.54868}
\pgfmath@def{acos}{96}{84.49112}    \pgfmath@def{acos}{97}{84.43355}
\pgfmath@def{acos}{98}{84.37598}    \pgfmath@def{acos}{99}{84.31841}
\pgfmath@def{acos}{100}{84.26083}    \pgfmath@def{acos}{101}{84.20324}
\pgfmath@def{acos}{102}{84.14564}    \pgfmath@def{acos}{103}{84.08805}
\pgfmath@def{acos}{104}{84.03044}    \pgfmath@def{acos}{105}{83.97283}
\pgfmath@def{acos}{106}{83.91521}    \pgfmath@def{acos}{107}{83.85759}
\pgfmath@def{acos}{108}{83.79996}    \pgfmath@def{acos}{109}{83.74232}
\pgfmath@def{acos}{110}{83.68468}    \pgfmath@def{acos}{111}{83.62703}
\pgfmath@def{acos}{112}{83.56938}    \pgfmath@def{acos}{113}{83.51171}
\pgfmath@def{acos}{114}{83.45405}    \pgfmath@def{acos}{115}{83.39637}
\pgfmath@def{acos}{116}{83.33869}    \pgfmath@def{acos}{117}{83.28100}
\pgfmath@def{acos}{118}{83.22330}    \pgfmath@def{acos}{119}{83.16560}
\pgfmath@def{acos}{120}{83.10789}    \pgfmath@def{acos}{121}{83.05018}
\pgfmath@def{acos}{122}{82.99245}    \pgfmath@def{acos}{123}{82.93472}
\pgfmath@def{acos}{124}{82.87698}    \pgfmath@def{acos}{125}{82.81924}
\pgfmath@def{acos}{126}{82.76149}    \pgfmath@def{acos}{127}{82.70373}
\pgfmath@def{acos}{128}{82.64596}    \pgfmath@def{acos}{129}{82.58819}
\pgfmath@def{acos}{130}{82.53040}    \pgfmath@def{acos}{131}{82.47261}
\pgfmath@def{acos}{132}{82.41482}    \pgfmath@def{acos}{133}{82.35701}
\pgfmath@def{acos}{134}{82.29920}    \pgfmath@def{acos}{135}{82.24138}
\pgfmath@def{acos}{136}{82.18355}    \pgfmath@def{acos}{137}{82.12571}
\pgfmath@def{acos}{138}{82.06786}    \pgfmath@def{acos}{139}{82.01001}
\pgfmath@def{acos}{140}{81.95215}    \pgfmath@def{acos}{141}{81.89428}
\pgfmath@def{acos}{142}{81.83640}    \pgfmath@def{acos}{143}{81.77851}
\pgfmath@def{acos}{144}{81.72062}    \pgfmath@def{acos}{145}{81.66272}
\pgfmath@def{acos}{146}{81.60480}    \pgfmath@def{acos}{147}{81.54688}
\pgfmath@def{acos}{148}{81.48895}    \pgfmath@def{acos}{149}{81.43102}
\pgfmath@def{acos}{150}{81.37307}    \pgfmath@def{acos}{151}{81.31511}
\pgfmath@def{acos}{152}{81.25715}    \pgfmath@def{acos}{153}{81.19917}
\pgfmath@def{acos}{154}{81.14119}    \pgfmath@def{acos}{155}{81.08320}
\pgfmath@def{acos}{156}{81.02520}    \pgfmath@def{acos}{157}{80.96719}
\pgfmath@def{acos}{158}{80.90917}    \pgfmath@def{acos}{159}{80.85114}
\pgfmath@def{acos}{160}{80.79310}    \pgfmath@def{acos}{161}{80.73505}
\pgfmath@def{acos}{162}{80.67699}    \pgfmath@def{acos}{163}{80.61893}
\pgfmath@def{acos}{164}{80.56085}    \pgfmath@def{acos}{165}{80.50276}
\pgfmath@def{acos}{166}{80.44466}    \pgfmath@def{acos}{167}{80.38656}
\pgfmath@def{acos}{168}{80.32844}    \pgfmath@def{acos}{169}{80.27031}
\pgfmath@def{acos}{170}{80.21218}    \pgfmath@def{acos}{171}{80.15403}
\pgfmath@def{acos}{172}{80.09587}    \pgfmath@def{acos}{173}{80.03770}
\pgfmath@def{acos}{174}{79.97953}    \pgfmath@def{acos}{175}{79.92134}
\pgfmath@def{acos}{176}{79.86314}    \pgfmath@def{acos}{177}{79.80493}
\pgfmath@def{acos}{178}{79.74671}    \pgfmath@def{acos}{179}{79.68848}
\pgfmath@def{acos}{180}{79.63024}    \pgfmath@def{acos}{181}{79.57198}
\pgfmath@def{acos}{182}{79.51372}    \pgfmath@def{acos}{183}{79.45545}
\pgfmath@def{acos}{184}{79.39716}    \pgfmath@def{acos}{185}{79.33886}
\pgfmath@def{acos}{186}{79.28056}    \pgfmath@def{acos}{187}{79.22224}
\pgfmath@def{acos}{188}{79.16391}    \pgfmath@def{acos}{189}{79.10556}
\pgfmath@def{acos}{190}{79.04721}    \pgfmath@def{acos}{191}{78.98885}
\pgfmath@def{acos}{192}{78.93047}    \pgfmath@def{acos}{193}{78.87208}
\pgfmath@def{acos}{194}{78.81368}    \pgfmath@def{acos}{195}{78.75527}
\pgfmath@def{acos}{196}{78.69685}    \pgfmath@def{acos}{197}{78.63841}
\pgfmath@def{acos}{198}{78.57997}    \pgfmath@def{acos}{199}{78.52151}
\pgfmath@def{acos}{200}{78.46304}    \pgfmath@def{acos}{201}{78.40455}
\pgfmath@def{acos}{202}{78.34606}    \pgfmath@def{acos}{203}{78.28755}
\pgfmath@def{acos}{204}{78.22903}    \pgfmath@def{acos}{205}{78.17050}
\pgfmath@def{acos}{206}{78.11195}    \pgfmath@def{acos}{207}{78.05339}
\pgfmath@def{acos}{208}{77.99482}    \pgfmath@def{acos}{209}{77.93624}
\pgfmath@def{acos}{210}{77.87764}    \pgfmath@def{acos}{211}{77.81903}
\pgfmath@def{acos}{212}{77.76041}    \pgfmath@def{acos}{213}{77.70178}
\pgfmath@def{acos}{214}{77.64313}    \pgfmath@def{acos}{215}{77.58447}
\pgfmath@def{acos}{216}{77.52579}    \pgfmath@def{acos}{217}{77.46711}
\pgfmath@def{acos}{218}{77.40841}    \pgfmath@def{acos}{219}{77.34969}
\pgfmath@def{acos}{220}{77.29096}    \pgfmath@def{acos}{221}{77.23222}
\pgfmath@def{acos}{222}{77.17347}    \pgfmath@def{acos}{223}{77.11470}
\pgfmath@def{acos}{224}{77.05591}    \pgfmath@def{acos}{225}{76.99712}
\pgfmath@def{acos}{226}{76.93831}    \pgfmath@def{acos}{227}{76.87948}
\pgfmath@def{acos}{228}{76.82064}    \pgfmath@def{acos}{229}{76.76179}
\pgfmath@def{acos}{230}{76.70292}    \pgfmath@def{acos}{231}{76.64404}
\pgfmath@def{acos}{232}{76.58515}    \pgfmath@def{acos}{233}{76.52624}
\pgfmath@def{acos}{234}{76.46731}    \pgfmath@def{acos}{235}{76.40837}
\pgfmath@def{acos}{236}{76.34942}    \pgfmath@def{acos}{237}{76.29045}
\pgfmath@def{acos}{238}{76.23147}    \pgfmath@def{acos}{239}{76.17247}
\pgfmath@def{acos}{240}{76.11346}    \pgfmath@def{acos}{241}{76.05443}
\pgfmath@def{acos}{242}{75.99538}    \pgfmath@def{acos}{243}{75.93632}
\pgfmath@def{acos}{244}{75.87725}    \pgfmath@def{acos}{245}{75.81816}
\pgfmath@def{acos}{246}{75.75906}    \pgfmath@def{acos}{247}{75.69994}
\pgfmath@def{acos}{248}{75.64080}    \pgfmath@def{acos}{249}{75.58165}
\pgfmath@def{acos}{250}{75.52248}    \pgfmath@def{acos}{251}{75.46330}
\pgfmath@def{acos}{252}{75.40410}    \pgfmath@def{acos}{253}{75.34489}
\pgfmath@def{acos}{254}{75.28566}    \pgfmath@def{acos}{255}{75.22641}
\pgfmath@def{acos}{256}{75.16715}    \pgfmath@def{acos}{257}{75.10787}
\pgfmath@def{acos}{258}{75.04857}    \pgfmath@def{acos}{259}{74.98926}
\pgfmath@def{acos}{260}{74.92993}    \pgfmath@def{acos}{261}{74.87059}
\pgfmath@def{acos}{262}{74.81123}    \pgfmath@def{acos}{263}{74.75185}
\pgfmath@def{acos}{264}{74.69245}    \pgfmath@def{acos}{265}{74.63304}
\pgfmath@def{acos}{266}{74.57361}    \pgfmath@def{acos}{267}{74.51417}
\pgfmath@def{acos}{268}{74.45471}    \pgfmath@def{acos}{269}{74.39523}
\pgfmath@def{acos}{270}{74.33573}    \pgfmath@def{acos}{271}{74.27621}
\pgfmath@def{acos}{272}{74.21668}    \pgfmath@def{acos}{273}{74.15713}
\pgfmath@def{acos}{274}{74.09757}    \pgfmath@def{acos}{275}{74.03798}
\pgfmath@def{acos}{276}{73.97838}    \pgfmath@def{acos}{277}{73.91876}
\pgfmath@def{acos}{278}{73.85912}    \pgfmath@def{acos}{279}{73.79946}
\pgfmath@def{acos}{280}{73.73979}    \pgfmath@def{acos}{281}{73.68010}
\pgfmath@def{acos}{282}{73.62039}    \pgfmath@def{acos}{283}{73.56066}
\pgfmath@def{acos}{284}{73.50091}    \pgfmath@def{acos}{285}{73.44115}
\pgfmath@def{acos}{286}{73.38136}    \pgfmath@def{acos}{287}{73.32156}
\pgfmath@def{acos}{288}{73.26174}    \pgfmath@def{acos}{289}{73.20190}
\pgfmath@def{acos}{290}{73.14204}    \pgfmath@def{acos}{291}{73.08216}
\pgfmath@def{acos}{292}{73.02226}    \pgfmath@def{acos}{293}{72.96235}
\pgfmath@def{acos}{294}{72.90241}    \pgfmath@def{acos}{295}{72.84246}
\pgfmath@def{acos}{296}{72.78248}    \pgfmath@def{acos}{297}{72.72249}
\pgfmath@def{acos}{298}{72.66248}    \pgfmath@def{acos}{299}{72.60244}
\pgfmath@def{acos}{300}{72.54239}    \pgfmath@def{acos}{301}{72.48232}
\pgfmath@def{acos}{302}{72.42223}    \pgfmath@def{acos}{303}{72.36212}
\pgfmath@def{acos}{304}{72.30198}    \pgfmath@def{acos}{305}{72.24183}
\pgfmath@def{acos}{306}{72.18166}    \pgfmath@def{acos}{307}{72.12147}
\pgfmath@def{acos}{308}{72.06125}    \pgfmath@def{acos}{309}{72.00102}
\pgfmath@def{acos}{310}{71.94077}    \pgfmath@def{acos}{311}{71.88049}
\pgfmath@def{acos}{312}{71.82019}    \pgfmath@def{acos}{313}{71.75988}
\pgfmath@def{acos}{314}{71.69954}    \pgfmath@def{acos}{315}{71.63918}
\pgfmath@def{acos}{316}{71.57880}    \pgfmath@def{acos}{317}{71.51840}
\pgfmath@def{acos}{318}{71.45798}    \pgfmath@def{acos}{319}{71.39754}
\pgfmath@def{acos}{320}{71.33707}    \pgfmath@def{acos}{321}{71.27658}
\pgfmath@def{acos}{322}{71.21608}    \pgfmath@def{acos}{323}{71.15555}
\pgfmath@def{acos}{324}{71.09499}    \pgfmath@def{acos}{325}{71.03442}
\pgfmath@def{acos}{326}{70.97382}    \pgfmath@def{acos}{327}{70.91321}
\pgfmath@def{acos}{328}{70.85257}    \pgfmath@def{acos}{329}{70.79190}
\pgfmath@def{acos}{330}{70.73122}    \pgfmath@def{acos}{331}{70.67051}
\pgfmath@def{acos}{332}{70.60978}    \pgfmath@def{acos}{333}{70.54903}
\pgfmath@def{acos}{334}{70.48826}    \pgfmath@def{acos}{335}{70.42746}
\pgfmath@def{acos}{336}{70.36664}    \pgfmath@def{acos}{337}{70.30579}
\pgfmath@def{acos}{338}{70.24493}    \pgfmath@def{acos}{339}{70.18404}
\pgfmath@def{acos}{340}{70.12312}    \pgfmath@def{acos}{341}{70.06218}
\pgfmath@def{acos}{342}{70.00122}    \pgfmath@def{acos}{343}{69.94024}
\pgfmath@def{acos}{344}{69.87923}    \pgfmath@def{acos}{345}{69.81820}
\pgfmath@def{acos}{346}{69.75714}    \pgfmath@def{acos}{347}{69.69606}
\pgfmath@def{acos}{348}{69.63496}    \pgfmath@def{acos}{349}{69.57383}
\pgfmath@def{acos}{350}{69.51268}    \pgfmath@def{acos}{351}{69.45150}
\pgfmath@def{acos}{352}{69.39030}    \pgfmath@def{acos}{353}{69.32908}
\pgfmath@def{acos}{354}{69.26783}    \pgfmath@def{acos}{355}{69.20655}
\pgfmath@def{acos}{356}{69.14525}    \pgfmath@def{acos}{357}{69.08393}
\pgfmath@def{acos}{358}{69.02258}    \pgfmath@def{acos}{359}{68.96120}
\pgfmath@def{acos}{360}{68.89980}    \pgfmath@def{acos}{361}{68.83837}
\pgfmath@def{acos}{362}{68.77692}    \pgfmath@def{acos}{363}{68.71544}
\pgfmath@def{acos}{364}{68.65394}    \pgfmath@def{acos}{365}{68.59241}
\pgfmath@def{acos}{366}{68.53086}    \pgfmath@def{acos}{367}{68.46928}
\pgfmath@def{acos}{368}{68.40767}    \pgfmath@def{acos}{369}{68.34604}
\pgfmath@def{acos}{370}{68.28438}    \pgfmath@def{acos}{371}{68.22269}
\pgfmath@def{acos}{372}{68.16098}    \pgfmath@def{acos}{373}{68.09924}
\pgfmath@def{acos}{374}{68.03748}    \pgfmath@def{acos}{375}{67.97568}
\pgfmath@def{acos}{376}{67.91386}    \pgfmath@def{acos}{377}{67.85202}
\pgfmath@def{acos}{378}{67.79014}    \pgfmath@def{acos}{379}{67.72824}
\pgfmath@def{acos}{380}{67.66631}    \pgfmath@def{acos}{381}{67.60436}
\pgfmath@def{acos}{382}{67.54237}    \pgfmath@def{acos}{383}{67.48036}
\pgfmath@def{acos}{384}{67.41832}    \pgfmath@def{acos}{385}{67.35626}
\pgfmath@def{acos}{386}{67.29416}    \pgfmath@def{acos}{387}{67.23204}
\pgfmath@def{acos}{388}{67.16988}    \pgfmath@def{acos}{389}{67.10770}
\pgfmath@def{acos}{390}{67.04550}    \pgfmath@def{acos}{391}{66.98326}
\pgfmath@def{acos}{392}{66.92099}    \pgfmath@def{acos}{393}{66.85870}
\pgfmath@def{acos}{394}{66.79637}    \pgfmath@def{acos}{395}{66.73402}
\pgfmath@def{acos}{396}{66.67164}    \pgfmath@def{acos}{397}{66.60923}
\pgfmath@def{acos}{398}{66.54679}    \pgfmath@def{acos}{399}{66.48432}
\pgfmath@def{acos}{400}{66.42182}    \pgfmath@def{acos}{401}{66.35929}
\pgfmath@def{acos}{402}{66.29673}    \pgfmath@def{acos}{403}{66.23414}
\pgfmath@def{acos}{404}{66.17152}    \pgfmath@def{acos}{405}{66.10887}
\pgfmath@def{acos}{406}{66.04619}    \pgfmath@def{acos}{407}{65.98348}
\pgfmath@def{acos}{408}{65.92074}    \pgfmath@def{acos}{409}{65.85796}
\pgfmath@def{acos}{410}{65.79516}    \pgfmath@def{acos}{411}{65.73233}
\pgfmath@def{acos}{412}{65.66946}    \pgfmath@def{acos}{413}{65.60657}
\pgfmath@def{acos}{414}{65.54364}    \pgfmath@def{acos}{415}{65.48068}
\pgfmath@def{acos}{416}{65.41769}    \pgfmath@def{acos}{417}{65.35467}
\pgfmath@def{acos}{418}{65.29161}    \pgfmath@def{acos}{419}{65.22853}
\pgfmath@def{acos}{420}{65.16541}    \pgfmath@def{acos}{421}{65.10226}
\pgfmath@def{acos}{422}{65.03908}    \pgfmath@def{acos}{423}{64.97586}
\pgfmath@def{acos}{424}{64.91261}    \pgfmath@def{acos}{425}{64.84933}
\pgfmath@def{acos}{426}{64.78602}    \pgfmath@def{acos}{427}{64.72267}
\pgfmath@def{acos}{428}{64.65929}    \pgfmath@def{acos}{429}{64.59588}
\pgfmath@def{acos}{430}{64.53244}    \pgfmath@def{acos}{431}{64.46896}
\pgfmath@def{acos}{432}{64.40544}    \pgfmath@def{acos}{433}{64.34190}
\pgfmath@def{acos}{434}{64.27832}    \pgfmath@def{acos}{435}{64.21470}
\pgfmath@def{acos}{436}{64.15105}    \pgfmath@def{acos}{437}{64.08737}
\pgfmath@def{acos}{438}{64.02365}    \pgfmath@def{acos}{439}{63.95990}
\pgfmath@def{acos}{440}{63.89611}    \pgfmath@def{acos}{441}{63.83229}
\pgfmath@def{acos}{442}{63.76844}    \pgfmath@def{acos}{443}{63.70455}
\pgfmath@def{acos}{444}{63.64062}    \pgfmath@def{acos}{445}{63.57666}
\pgfmath@def{acos}{446}{63.51266}    \pgfmath@def{acos}{447}{63.44863}
\pgfmath@def{acos}{448}{63.38456}    \pgfmath@def{acos}{449}{63.32045}
\pgfmath@def{acos}{450}{63.25631}    \pgfmath@def{acos}{451}{63.19213}
\pgfmath@def{acos}{452}{63.12792}    \pgfmath@def{acos}{453}{63.06367}
\pgfmath@def{acos}{454}{62.99938}    \pgfmath@def{acos}{455}{62.93506}
\pgfmath@def{acos}{456}{62.87070}    \pgfmath@def{acos}{457}{62.80630}
\pgfmath@def{acos}{458}{62.74187}    \pgfmath@def{acos}{459}{62.67740}
\pgfmath@def{acos}{460}{62.61289}    \pgfmath@def{acos}{461}{62.54834}
\pgfmath@def{acos}{462}{62.48376}    \pgfmath@def{acos}{463}{62.41913}
\pgfmath@def{acos}{464}{62.35447}    \pgfmath@def{acos}{465}{62.28977}
\pgfmath@def{acos}{466}{62.22504}    \pgfmath@def{acos}{467}{62.16026}
\pgfmath@def{acos}{468}{62.09545}    \pgfmath@def{acos}{469}{62.03059}
\pgfmath@def{acos}{470}{61.96570}    \pgfmath@def{acos}{471}{61.90077}
\pgfmath@def{acos}{472}{61.83580}    \pgfmath@def{acos}{473}{61.77079}
\pgfmath@def{acos}{474}{61.70574}    \pgfmath@def{acos}{475}{61.64065}
\pgfmath@def{acos}{476}{61.57552}    \pgfmath@def{acos}{477}{61.51035}
\pgfmath@def{acos}{478}{61.44514}    \pgfmath@def{acos}{479}{61.37988}
\pgfmath@def{acos}{480}{61.31459}    \pgfmath@def{acos}{481}{61.24926}
\pgfmath@def{acos}{482}{61.18389}    \pgfmath@def{acos}{483}{61.11847}
\pgfmath@def{acos}{484}{61.05302}    \pgfmath@def{acos}{485}{60.98752}
\pgfmath@def{acos}{486}{60.92199}    \pgfmath@def{acos}{487}{60.85641}
\pgfmath@def{acos}{488}{60.79078}    \pgfmath@def{acos}{489}{60.72512}
\pgfmath@def{acos}{490}{60.65941}    \pgfmath@def{acos}{491}{60.59367}
\pgfmath@def{acos}{492}{60.52787}    \pgfmath@def{acos}{493}{60.46204}
\pgfmath@def{acos}{494}{60.39616}    \pgfmath@def{acos}{495}{60.33025}
\pgfmath@def{acos}{496}{60.26428}    \pgfmath@def{acos}{497}{60.19828}
\pgfmath@def{acos}{498}{60.13223}    \pgfmath@def{acos}{499}{60.06613}
\pgfmath@def{acos}{500}{60.00000}    \pgfmath@def{acos}{501}{59.93381}
\pgfmath@def{acos}{502}{59.86759}    \pgfmath@def{acos}{503}{59.80132}
\pgfmath@def{acos}{504}{59.73500}    \pgfmath@def{acos}{505}{59.66864}
\pgfmath@def{acos}{506}{59.60224}    \pgfmath@def{acos}{507}{59.53579}
\pgfmath@def{acos}{508}{59.46929}    \pgfmath@def{acos}{509}{59.40275}
\pgfmath@def{acos}{510}{59.33617}    \pgfmath@def{acos}{511}{59.26953}
\pgfmath@def{acos}{512}{59.20285}    \pgfmath@def{acos}{513}{59.13613}
\pgfmath@def{acos}{514}{59.06936}    \pgfmath@def{acos}{515}{59.00254}
\pgfmath@def{acos}{516}{58.93568}    \pgfmath@def{acos}{517}{58.86876}
\pgfmath@def{acos}{518}{58.80180}    \pgfmath@def{acos}{519}{58.73480}
\pgfmath@def{acos}{520}{58.66774}    \pgfmath@def{acos}{521}{58.60064}
\pgfmath@def{acos}{522}{58.53349}    \pgfmath@def{acos}{523}{58.46629}
\pgfmath@def{acos}{524}{58.39905}    \pgfmath@def{acos}{525}{58.33175}
\pgfmath@def{acos}{526}{58.26441}    \pgfmath@def{acos}{527}{58.19702}
\pgfmath@def{acos}{528}{58.12957}    \pgfmath@def{acos}{529}{58.06208}
\pgfmath@def{acos}{530}{57.99454}    \pgfmath@def{acos}{531}{57.92695}
\pgfmath@def{acos}{532}{57.85931}    \pgfmath@def{acos}{533}{57.79162}
\pgfmath@def{acos}{534}{57.72388}    \pgfmath@def{acos}{535}{57.65608}
\pgfmath@def{acos}{536}{57.58824}    \pgfmath@def{acos}{537}{57.52035}
\pgfmath@def{acos}{538}{57.45240}    \pgfmath@def{acos}{539}{57.38441}
\pgfmath@def{acos}{540}{57.31636}    \pgfmath@def{acos}{541}{57.24826}
\pgfmath@def{acos}{542}{57.18010}    \pgfmath@def{acos}{543}{57.11190}
\pgfmath@def{acos}{544}{57.04364}    \pgfmath@def{acos}{545}{56.97533}
\pgfmath@def{acos}{546}{56.90697}    \pgfmath@def{acos}{547}{56.83855}
\pgfmath@def{acos}{548}{56.77008}    \pgfmath@def{acos}{549}{56.70156}
\pgfmath@def{acos}{550}{56.63298}    \pgfmath@def{acos}{551}{56.56435}
\pgfmath@def{acos}{552}{56.49567}    \pgfmath@def{acos}{553}{56.42693}
\pgfmath@def{acos}{554}{56.35813}    \pgfmath@def{acos}{555}{56.28928}
\pgfmath@def{acos}{556}{56.22038}    \pgfmath@def{acos}{557}{56.15141}
\pgfmath@def{acos}{558}{56.08240}    \pgfmath@def{acos}{559}{56.01333}
\pgfmath@def{acos}{560}{55.94420}    \pgfmath@def{acos}{561}{55.87501}
\pgfmath@def{acos}{562}{55.80577}    \pgfmath@def{acos}{563}{55.73647}
\pgfmath@def{acos}{564}{55.66712}    \pgfmath@def{acos}{565}{55.59770}
\pgfmath@def{acos}{566}{55.52823}    \pgfmath@def{acos}{567}{55.45871}
\pgfmath@def{acos}{568}{55.38912}    \pgfmath@def{acos}{569}{55.31947}
\pgfmath@def{acos}{570}{55.24977}    \pgfmath@def{acos}{571}{55.18001}
\pgfmath@def{acos}{572}{55.11019}    \pgfmath@def{acos}{573}{55.04030}
\pgfmath@def{acos}{574}{54.97036}    \pgfmath@def{acos}{575}{54.90036}
\pgfmath@def{acos}{576}{54.83030}    \pgfmath@def{acos}{577}{54.76018}
\pgfmath@def{acos}{578}{54.69000}    \pgfmath@def{acos}{579}{54.61976}
\pgfmath@def{acos}{580}{54.54945}    \pgfmath@def{acos}{581}{54.47909}
\pgfmath@def{acos}{582}{54.40866}    \pgfmath@def{acos}{583}{54.33817}
\pgfmath@def{acos}{584}{54.26762}    \pgfmath@def{acos}{585}{54.19701}
\pgfmath@def{acos}{586}{54.12633}    \pgfmath@def{acos}{587}{54.05559}
\pgfmath@def{acos}{588}{53.98479}    \pgfmath@def{acos}{589}{53.91392}
\pgfmath@def{acos}{590}{53.84299}    \pgfmath@def{acos}{591}{53.77199}
\pgfmath@def{acos}{592}{53.70093}    \pgfmath@def{acos}{593}{53.62981}
\pgfmath@def{acos}{594}{53.55862}    \pgfmath@def{acos}{595}{53.48736}
\pgfmath@def{acos}{596}{53.41604}    \pgfmath@def{acos}{597}{53.34466}
\pgfmath@def{acos}{598}{53.27320}    \pgfmath@def{acos}{599}{53.20168}
\pgfmath@def{acos}{600}{53.13010}    \pgfmath@def{acos}{601}{53.05844}
\pgfmath@def{acos}{602}{52.98672}    \pgfmath@def{acos}{603}{52.91494}
\pgfmath@def{acos}{604}{52.84308}    \pgfmath@def{acos}{605}{52.77115}
\pgfmath@def{acos}{606}{52.69916}    \pgfmath@def{acos}{607}{52.62710}
\pgfmath@def{acos}{608}{52.55497}    \pgfmath@def{acos}{609}{52.48276}
\pgfmath@def{acos}{610}{52.41049}    \pgfmath@def{acos}{611}{52.33815}
\pgfmath@def{acos}{612}{52.26574}    \pgfmath@def{acos}{613}{52.19326}
\pgfmath@def{acos}{614}{52.12070}    \pgfmath@def{acos}{615}{52.04808}
\pgfmath@def{acos}{616}{51.97538}    \pgfmath@def{acos}{617}{51.90261}
\pgfmath@def{acos}{618}{51.82976}    \pgfmath@def{acos}{619}{51.75685}
\pgfmath@def{acos}{620}{51.68386}    \pgfmath@def{acos}{621}{51.61080}
\pgfmath@def{acos}{622}{51.53766}    \pgfmath@def{acos}{623}{51.46445}
\pgfmath@def{acos}{624}{51.39117}    \pgfmath@def{acos}{625}{51.31781}
\pgfmath@def{acos}{626}{51.24437}    \pgfmath@def{acos}{627}{51.17086}
\pgfmath@def{acos}{628}{51.09728}    \pgfmath@def{acos}{629}{51.02361}
\pgfmath@def{acos}{630}{50.94987}    \pgfmath@def{acos}{631}{50.87606}
\pgfmath@def{acos}{632}{50.80216}    \pgfmath@def{acos}{633}{50.72819}
\pgfmath@def{acos}{634}{50.65414}    \pgfmath@def{acos}{635}{50.58001}
\pgfmath@def{acos}{636}{50.50580}    \pgfmath@def{acos}{637}{50.43152}
\pgfmath@def{acos}{638}{50.35715}    \pgfmath@def{acos}{639}{50.28270}
\pgfmath@def{acos}{640}{50.20818}    \pgfmath@def{acos}{641}{50.13357}
\pgfmath@def{acos}{642}{50.05888}    \pgfmath@def{acos}{643}{49.98411}
\pgfmath@def{acos}{644}{49.90926}    \pgfmath@def{acos}{645}{49.83432}
\pgfmath@def{acos}{646}{49.75930}    \pgfmath@def{acos}{647}{49.68420}
\pgfmath@def{acos}{648}{49.60902}    \pgfmath@def{acos}{649}{49.53375}
\pgfmath@def{acos}{650}{49.45839}    \pgfmath@def{acos}{651}{49.38296}
\pgfmath@def{acos}{652}{49.30743}    \pgfmath@def{acos}{653}{49.23182}
\pgfmath@def{acos}{654}{49.15613}    \pgfmath@def{acos}{655}{49.08035}
\pgfmath@def{acos}{656}{49.00448}    \pgfmath@def{acos}{657}{48.92852}
\pgfmath@def{acos}{658}{48.85248}    \pgfmath@def{acos}{659}{48.77634}
\pgfmath@def{acos}{660}{48.70012}    \pgfmath@def{acos}{661}{48.62381}
\pgfmath@def{acos}{662}{48.54741}    \pgfmath@def{acos}{663}{48.47092}
\pgfmath@def{acos}{664}{48.39434}    \pgfmath@def{acos}{665}{48.31767}
\pgfmath@def{acos}{666}{48.24091}    \pgfmath@def{acos}{667}{48.16405}
\pgfmath@def{acos}{668}{48.08710}    \pgfmath@def{acos}{669}{48.01006}
\pgfmath@def{acos}{670}{47.93293}    \pgfmath@def{acos}{671}{47.85570}
\pgfmath@def{acos}{672}{47.77838}    \pgfmath@def{acos}{673}{47.70096}
\pgfmath@def{acos}{674}{47.62345}    \pgfmath@def{acos}{675}{47.54585}
\pgfmath@def{acos}{676}{47.46814}    \pgfmath@def{acos}{677}{47.39034}
\pgfmath@def{acos}{678}{47.31244}    \pgfmath@def{acos}{679}{47.23445}
\pgfmath@def{acos}{680}{47.15635}    \pgfmath@def{acos}{681}{47.07816}
\pgfmath@def{acos}{682}{46.99987}    \pgfmath@def{acos}{683}{46.92147}
\pgfmath@def{acos}{684}{46.84298}    \pgfmath@def{acos}{685}{46.76439}
\pgfmath@def{acos}{686}{46.68569}    \pgfmath@def{acos}{687}{46.60690}
\pgfmath@def{acos}{688}{46.52800}    \pgfmath@def{acos}{689}{46.44899}
\pgfmath@def{acos}{690}{46.36989}    \pgfmath@def{acos}{691}{46.29068}
\pgfmath@def{acos}{692}{46.21136}    \pgfmath@def{acos}{693}{46.13194}
\pgfmath@def{acos}{694}{46.05241}    \pgfmath@def{acos}{695}{45.97278}
\pgfmath@def{acos}{696}{45.89304}    \pgfmath@def{acos}{697}{45.81319}
\pgfmath@def{acos}{698}{45.73323}    \pgfmath@def{acos}{699}{45.65317}
\pgfmath@def{acos}{700}{45.57299}    \pgfmath@def{acos}{701}{45.49271}
\pgfmath@def{acos}{702}{45.41231}    \pgfmath@def{acos}{703}{45.33180}
\pgfmath@def{acos}{704}{45.25118}    \pgfmath@def{acos}{705}{45.17045}
\pgfmath@def{acos}{706}{45.08961}    \pgfmath@def{acos}{707}{45.00865}
\pgfmath@def{acos}{708}{44.92757}    \pgfmath@def{acos}{709}{44.84638}
\pgfmath@def{acos}{710}{44.76508}    \pgfmath@def{acos}{711}{44.68366}
\pgfmath@def{acos}{712}{44.60212}    \pgfmath@def{acos}{713}{44.52046}
\pgfmath@def{acos}{714}{44.43869}    \pgfmath@def{acos}{715}{44.35680}
\pgfmath@def{acos}{716}{44.27478}    \pgfmath@def{acos}{717}{44.19265}
\pgfmath@def{acos}{718}{44.11039}    \pgfmath@def{acos}{719}{44.02802}
\pgfmath@def{acos}{720}{43.94552}    \pgfmath@def{acos}{721}{43.86289}
\pgfmath@def{acos}{722}{43.78014}    \pgfmath@def{acos}{723}{43.69727}
\pgfmath@def{acos}{724}{43.61427}    \pgfmath@def{acos}{725}{43.53115}
\pgfmath@def{acos}{726}{43.44790}    \pgfmath@def{acos}{727}{43.36452}
\pgfmath@def{acos}{728}{43.28101}    \pgfmath@def{acos}{729}{43.19737}
\pgfmath@def{acos}{730}{43.11360}    \pgfmath@def{acos}{731}{43.02970}
\pgfmath@def{acos}{732}{42.94567}    \pgfmath@def{acos}{733}{42.86151}
\pgfmath@def{acos}{734}{42.77721}    \pgfmath@def{acos}{735}{42.69278}
\pgfmath@def{acos}{736}{42.60821}    \pgfmath@def{acos}{737}{42.52351}
\pgfmath@def{acos}{738}{42.43867}    \pgfmath@def{acos}{739}{42.35370}
\pgfmath@def{acos}{740}{42.26858}    \pgfmath@def{acos}{741}{42.18333}
\pgfmath@def{acos}{742}{42.09793}    \pgfmath@def{acos}{743}{42.01240}
\pgfmath@def{acos}{744}{41.92672}    \pgfmath@def{acos}{745}{41.84090}
\pgfmath@def{acos}{746}{41.75493}    \pgfmath@def{acos}{747}{41.66882}
\pgfmath@def{acos}{748}{41.58257}    \pgfmath@def{acos}{749}{41.49617}
\pgfmath@def{acos}{750}{41.40962}    \pgfmath@def{acos}{751}{41.32292}
\pgfmath@def{acos}{752}{41.23607}    \pgfmath@def{acos}{753}{41.14908}
\pgfmath@def{acos}{754}{41.06193}    \pgfmath@def{acos}{755}{40.97463}
\pgfmath@def{acos}{756}{40.88717}    \pgfmath@def{acos}{757}{40.79956}
\pgfmath@def{acos}{758}{40.71180}    \pgfmath@def{acos}{759}{40.62388}
\pgfmath@def{acos}{760}{40.53580}    \pgfmath@def{acos}{761}{40.44756}
\pgfmath@def{acos}{762}{40.35916}    \pgfmath@def{acos}{763}{40.27061}
\pgfmath@def{acos}{764}{40.18189}    \pgfmath@def{acos}{765}{40.09300}
\pgfmath@def{acos}{766}{40.00396}    \pgfmath@def{acos}{767}{39.91474}
\pgfmath@def{acos}{768}{39.82537}    \pgfmath@def{acos}{769}{39.73582}
\pgfmath@def{acos}{770}{39.64611}    \pgfmath@def{acos}{771}{39.55622}
\pgfmath@def{acos}{772}{39.46617}    \pgfmath@def{acos}{773}{39.37594}
\pgfmath@def{acos}{774}{39.28554}    \pgfmath@def{acos}{775}{39.19496}
\pgfmath@def{acos}{776}{39.10421}    \pgfmath@def{acos}{777}{39.01328}
\pgfmath@def{acos}{778}{38.92218}    \pgfmath@def{acos}{779}{38.83089}
\pgfmath@def{acos}{780}{38.73942}    \pgfmath@def{acos}{781}{38.64777}
\pgfmath@def{acos}{782}{38.55594}    \pgfmath@def{acos}{783}{38.46392}
\pgfmath@def{acos}{784}{38.37171}    \pgfmath@def{acos}{785}{38.27932}
\pgfmath@def{acos}{786}{38.18673}    \pgfmath@def{acos}{787}{38.09396}
\pgfmath@def{acos}{788}{38.00100}    \pgfmath@def{acos}{789}{37.90784}
\pgfmath@def{acos}{790}{37.81448}    \pgfmath@def{acos}{791}{37.72093}
\pgfmath@def{acos}{792}{37.62719}    \pgfmath@def{acos}{793}{37.53324}
\pgfmath@def{acos}{794}{37.43909}    \pgfmath@def{acos}{795}{37.34474}
\pgfmath@def{acos}{796}{37.25019}    \pgfmath@def{acos}{797}{37.15542}
\pgfmath@def{acos}{798}{37.06046}    \pgfmath@def{acos}{799}{36.96528}
\pgfmath@def{acos}{800}{36.86989}    \pgfmath@def{acos}{801}{36.77429}
\pgfmath@def{acos}{802}{36.67848}    \pgfmath@def{acos}{803}{36.58245}
\pgfmath@def{acos}{804}{36.48621}    \pgfmath@def{acos}{805}{36.38974}
\pgfmath@def{acos}{806}{36.29305}    \pgfmath@def{acos}{807}{36.19615}
\pgfmath@def{acos}{808}{36.09901}    \pgfmath@def{acos}{809}{36.00165}
\pgfmath@def{acos}{810}{35.90406}    \pgfmath@def{acos}{811}{35.80625}
\pgfmath@def{acos}{812}{35.70820}    \pgfmath@def{acos}{813}{35.60991}
\pgfmath@def{acos}{814}{35.51139}    \pgfmath@def{acos}{815}{35.41263}
\pgfmath@def{acos}{816}{35.31364}    \pgfmath@def{acos}{817}{35.21440}
\pgfmath@def{acos}{818}{35.11491}    \pgfmath@def{acos}{819}{35.01518}
\pgfmath@def{acos}{820}{34.91520}    \pgfmath@def{acos}{821}{34.81497}
\pgfmath@def{acos}{822}{34.71449}    \pgfmath@def{acos}{823}{34.61375}
\pgfmath@def{acos}{824}{34.51276}    \pgfmath@def{acos}{825}{34.41150}
\pgfmath@def{acos}{826}{34.30999}    \pgfmath@def{acos}{827}{34.20821}
\pgfmath@def{acos}{828}{34.10616}    \pgfmath@def{acos}{829}{34.00385}
\pgfmath@def{acos}{830}{33.90126}    \pgfmath@def{acos}{831}{33.79840}
\pgfmath@def{acos}{832}{33.69526}    \pgfmath@def{acos}{833}{33.59184}
\pgfmath@def{acos}{834}{33.48814}    \pgfmath@def{acos}{835}{33.38416}
\pgfmath@def{acos}{836}{33.27989}    \pgfmath@def{acos}{837}{33.17533}
\pgfmath@def{acos}{838}{33.07047}    \pgfmath@def{acos}{839}{32.96532}
\pgfmath@def{acos}{840}{32.85988}    \pgfmath@def{acos}{841}{32.75413}
\pgfmath@def{acos}{842}{32.64807}    \pgfmath@def{acos}{843}{32.54171}
\pgfmath@def{acos}{844}{32.43504}    \pgfmath@def{acos}{845}{32.32806}
\pgfmath@def{acos}{846}{32.22076}    \pgfmath@def{acos}{847}{32.11314}
\pgfmath@def{acos}{848}{32.00520}    \pgfmath@def{acos}{849}{31.89693}
\pgfmath@def{acos}{850}{31.78833}    \pgfmath@def{acos}{851}{31.67939}
\pgfmath@def{acos}{852}{31.57012}    \pgfmath@def{acos}{853}{31.46051}
\pgfmath@def{acos}{854}{31.35056}    \pgfmath@def{acos}{855}{31.24026}
\pgfmath@def{acos}{856}{31.12961}    \pgfmath@def{acos}{857}{31.01860}
\pgfmath@def{acos}{858}{30.90724}    \pgfmath@def{acos}{859}{30.79551}
\pgfmath@def{acos}{860}{30.68341}    \pgfmath@def{acos}{861}{30.57095}
\pgfmath@def{acos}{862}{30.45811}    \pgfmath@def{acos}{863}{30.34489}
\pgfmath@def{acos}{864}{30.23128}    \pgfmath@def{acos}{865}{30.11729}
\pgfmath@def{acos}{866}{30.00291}    \pgfmath@def{acos}{867}{29.88813}
\pgfmath@def{acos}{868}{29.77294}    \pgfmath@def{acos}{869}{29.65736}
\pgfmath@def{acos}{870}{29.54136}    \pgfmath@def{acos}{871}{29.42494}
\pgfmath@def{acos}{872}{29.30810}    \pgfmath@def{acos}{873}{29.19084}
\pgfmath@def{acos}{874}{29.07315}    \pgfmath@def{acos}{875}{28.95502}
\pgfmath@def{acos}{876}{28.83645}    \pgfmath@def{acos}{877}{28.71743}
\pgfmath@def{acos}{878}{28.59796}    \pgfmath@def{acos}{879}{28.47803}
\pgfmath@def{acos}{880}{28.35763}    \pgfmath@def{acos}{881}{28.23677}
\pgfmath@def{acos}{882}{28.11542}    \pgfmath@def{acos}{883}{27.99360}
\pgfmath@def{acos}{884}{27.87128}    \pgfmath@def{acos}{885}{27.74847}
\pgfmath@def{acos}{886}{27.62516}    \pgfmath@def{acos}{887}{27.50134}
\pgfmath@def{acos}{888}{27.37700}    \pgfmath@def{acos}{889}{27.25214}
\pgfmath@def{acos}{890}{27.12675}    \pgfmath@def{acos}{891}{27.00082}
\pgfmath@def{acos}{892}{26.87434}    \pgfmath@def{acos}{893}{26.74731}
\pgfmath@def{acos}{894}{26.61973}    \pgfmath@def{acos}{895}{26.49157}
\pgfmath@def{acos}{896}{26.36283}    \pgfmath@def{acos}{897}{26.23351}
\pgfmath@def{acos}{898}{26.10359}    \pgfmath@def{acos}{899}{25.97306}
\pgfmath@def{acos}{900}{25.84193}    \pgfmath@def{acos}{901}{25.71017}
\pgfmath@def{acos}{902}{25.57778}    \pgfmath@def{acos}{903}{25.44475}
\pgfmath@def{acos}{904}{25.31106}    \pgfmath@def{acos}{905}{25.17671}
\pgfmath@def{acos}{906}{25.04169}    \pgfmath@def{acos}{907}{24.90598}
\pgfmath@def{acos}{908}{24.76958}    \pgfmath@def{acos}{909}{24.63247}
\pgfmath@def{acos}{910}{24.49464}    \pgfmath@def{acos}{911}{24.35608}
\pgfmath@def{acos}{912}{24.21678}    \pgfmath@def{acos}{913}{24.07672}
\pgfmath@def{acos}{914}{23.93588}    \pgfmath@def{acos}{915}{23.79427}
\pgfmath@def{acos}{916}{23.65185}    \pgfmath@def{acos}{917}{23.50863}
\pgfmath@def{acos}{918}{23.36457}    \pgfmath@def{acos}{919}{23.21967}
\pgfmath@def{acos}{920}{23.07391}    \pgfmath@def{acos}{921}{22.92728}
\pgfmath@def{acos}{922}{22.77975}    \pgfmath@def{acos}{923}{22.63132}
\pgfmath@def{acos}{924}{22.48195}    \pgfmath@def{acos}{925}{22.33164}
\pgfmath@def{acos}{926}{22.18036}    \pgfmath@def{acos}{927}{22.02810}
\pgfmath@def{acos}{928}{21.87483}    \pgfmath@def{acos}{929}{21.72053}
\pgfmath@def{acos}{930}{21.56518}    \pgfmath@def{acos}{931}{21.40876}
\pgfmath@def{acos}{932}{21.25124}    \pgfmath@def{acos}{933}{21.09260}
\pgfmath@def{acos}{934}{20.93281}    \pgfmath@def{acos}{935}{20.77185}
\pgfmath@def{acos}{936}{20.60969}    \pgfmath@def{acos}{937}{20.44630}
\pgfmath@def{acos}{938}{20.28165}    \pgfmath@def{acos}{939}{20.11570}
\pgfmath@def{acos}{940}{19.94844}    \pgfmath@def{acos}{941}{19.77982}
\pgfmath@def{acos}{942}{19.60981}    \pgfmath@def{acos}{943}{19.43837}
\pgfmath@def{acos}{944}{19.26546}    \pgfmath@def{acos}{945}{19.09105}
\pgfmath@def{acos}{946}{18.91509}    \pgfmath@def{acos}{947}{18.73754}
\pgfmath@def{acos}{948}{18.55835}    \pgfmath@def{acos}{949}{18.37748}
\pgfmath@def{acos}{950}{18.19487}    \pgfmath@def{acos}{951}{18.01047}
\pgfmath@def{acos}{952}{17.82423}    \pgfmath@def{acos}{953}{17.63609}
\pgfmath@def{acos}{954}{17.44598}    \pgfmath@def{acos}{955}{17.25385}
\pgfmath@def{acos}{956}{17.05962}    \pgfmath@def{acos}{957}{16.86322}
\pgfmath@def{acos}{958}{16.66457}    \pgfmath@def{acos}{959}{16.46359}
\pgfmath@def{acos}{960}{16.26020}    \pgfmath@def{acos}{961}{16.05430}
\pgfmath@def{acos}{962}{15.84580}    \pgfmath@def{acos}{963}{15.63459}
\pgfmath@def{acos}{964}{15.42057}    \pgfmath@def{acos}{965}{15.20360}
\pgfmath@def{acos}{966}{14.98357}    \pgfmath@def{acos}{967}{14.76033}
\pgfmath@def{acos}{968}{14.53374}    \pgfmath@def{acos}{969}{14.30364}
\pgfmath@def{acos}{970}{14.06986}    \pgfmath@def{acos}{971}{13.83221}
\pgfmath@def{acos}{972}{13.59049}    \pgfmath@def{acos}{973}{13.34447}
\pgfmath@def{acos}{974}{13.09392}    \pgfmath@def{acos}{975}{12.83856}
\pgfmath@def{acos}{976}{12.57811}    \pgfmath@def{acos}{977}{12.31225}
\pgfmath@def{acos}{978}{12.04060}    \pgfmath@def{acos}{979}{11.76278}
\pgfmath@def{acos}{980}{11.47834}    \pgfmath@def{acos}{981}{11.18676}
\pgfmath@def{acos}{982}{10.88748}    \pgfmath@def{acos}{983}{10.57984}
\pgfmath@def{acos}{984}{10.26309}    \pgfmath@def{acos}{985}{9.93636}
\pgfmath@def{acos}{986}{9.59863}    \pgfmath@def{acos}{987}{9.24870}
\pgfmath@def{acos}{988}{8.88512}    \pgfmath@def{acos}{989}{8.50614}
\pgfmath@def{acos}{990}{8.10961}    \pgfmath@def{acos}{991}{7.69281}
\pgfmath@def{acos}{992}{7.25224}    \pgfmath@def{acos}{993}{6.78328}
\pgfmath@def{acos}{994}{6.27958}    \pgfmath@def{acos}{995}{5.73196}
\pgfmath@def{acos}{996}{5.12640}    \pgfmath@def{acos}{997}{4.43922}
\pgfmath@def{acos}{998}{3.62430}    \pgfmath@def{acos}{999}{2.56255}
\pgfmath@def{acos}{1000}{0.00000}



% Local Variables:
% tab-width: 2
% End:


==> pgfmathparser.code.tex <==

\newdimen\pgfmath@dimen
\newcount\pgfmath@count
\newbox\pgfmath@box
\newtoks\pgfmath@toks

\newif\ifpgfmath@quickparse
\newif\ifpgfmathfloat
\newif\ifpgfmathunitsdeclared
\newif\ifpgfmathmathunitsdeclared
\newif\ifpgfmathignoreunitscale

\let\pgfmath@protected@edef=\edef
\ifcsname protected@edef\endcsname
  \let\pgfmath@protected@edef=\protected@edef
\fi

\def\pgfmathprint#1{\pgfmathparse{#1}\pgfmathresult}

\def\pgfmathparse{%
  \begingroup
    \pgfmath@catcodes
    \pgfmath@quickparsefalse
    % Test for the fpu library
    \ifpgfmathfloat
      \let\pgfmath@parse@next=\pgfmathfloatparsenumber
    \else
      \let\pgfmath@parse@next=\pgfmathparse@
    \fi
    \pgfmath@parse@next}

\def\pgfmath@catcodes{% Maybe unnecessary.
  \catcode`\==12 %
  \catcode`\,=12 %
  \catcode`\|=12 %
  \catcode`\&=12 %
}

\def\pgfmathqparse{%
  \begingroup
    \pgfmath@catcodes
    \pgfmath@quickparsetrue
    \pgfmathparse@}

\def\pgfmathparse@#1{%
    % No (math) units yet.
    \global\pgfmathunitsdeclaredfalse
    \global\pgfmathmathunitsdeclaredfalse
    % Expand expression so any remaining CSs are registers
    % or box dimensions (i.e. |\wd|, |\ht|, |\dp|).
    \pgfmath@protected@edef\pgfmath@expression{#1}%
    %
    \expandafter\pgfmathparse@trynumber@loop\pgfmath@expression\pgfmath@parse@stop
    %
    % this here is the _real_ parser. it is invoked by
    % \pgfmathparse@trynumber@loop if that says "this is no number"
    %\pgfmathparse@@\pgfmath@parse@stop%
}

\def\pgfmath@parse@stop{\pgfmath@parse@stop}% equals only itself

\def\pgfmathparse@trynumber@token{numeric}
\begingroup
\def\\{\global\let\pgf@let@space@token= } \\ % now, \pgf@let@space@token is a space token
\endgroup

% This a "fast-lane": if the expressions consist merely of number
% tokens, we can simply return the number as-is.
%
% This is significantly faster and should resemble the 80% use-case.
%
% #1 a single token
\def\pgfmathparse@trynumber@loop{%
    \futurelet\pgfmath@token@let\pgfmathparse@trynumber@loop@
}%
\def\pgfmathparse@trynumber@loop@#1{%
    \ifx\pgfmath@token@let\pgf@let@space@token
        % Hm. we found a white space... and we have no support for
        % trimming. That means we have to assume that the white space
        % occurred somewhere in the middle - and fall back to the
        % expensive method.
        \def\pgfmath@parse@next{\pgfmathparse@@#1}%
    \else
        \ifx\pgfmath@token@let\bgroup%
            % oh! We found '{' #1.
            % Well, these braces appear to be special; fall back to
            % the complicated routine...
            \let\pgfmath@parse@next=\pgfmathparse@@
        \else
            \ifx\pgfmath@token@let\pgfmath@parse@stop
                % Ah: we have passed the check! The expression consists only
                % of 0123456789. , so do not parse anything and return it
                % as-is!
                \let\pgfmath@parse@next=\pgfmathparse@expression@is@number
            \else
                \expandafter\ifx\csname pgfmath@token@\pgfmathparse@trynumber@token @\string#1\endcsname\relax%
                    % hm. It is none of 0123456789.
                    \let\pgfmath@parse@next=\pgfmathparse@@
                \else
                    % continue... we only found one of 0123456789. so
                    % far...
                    \let\pgfmath@parse@next=\pgfmathparse@trynumber@loop
                \fi
            \fi
        \fi
    \fi
    \pgfmath@parse@next
}%

\def\pgfmathparse@expression@is@number{%
    \let\pgfmathresult=\pgfmath@expression
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup
  \ignorespaces
}%
\def\pgfmathparse@@#1\pgfmath@parse@stop{%
    % We are inside a group (opened in |\pgfmathparse| or
    % |\pgfmathqparse|).
    % Stuff for calc compatibility.
    \let\real=\pgfmath@calc@real
    \let\minof=\pgfmath@calc@minof
    \let\maxof=\pgfmath@calc@maxof
    \let\ratio=\pgfmath@calc@ratio
    \let\widthof=\pgfmath@calc@widthof
    \let\heightof=\pgfmath@calc@heightof
    \let\depthof=\pgfmath@calc@depthof
    % Restore font (defined in pgfmathutil.code.tex)
    \pgfmath@selectfont
    % Set up stack.
    \pgfmath@stack@operation={{}{}{}}%
    \pgfmath@stack@operand={{}{}{}}%
    \let\pgfmath@stack@operation@top=\pgfmath@stack@empty
    \let\pgfmath@stack@operand@top=\pgfmath@stack@empty
    % An expression always begins with an operand.
    \expandafter\pgfmath@bgroup@strip\expandafter{\pgfmath@expression}%
    % |\pgfmath@bgroup@stripped| is the result of
    % |\pgfmath@bgroup@strip|
    \expandafter\pgfmath@parse@@operand\pgfmath@bgroup@stripped @@@@\pgfmath@parse@stop%
}

\def\pgfmath@parse@end#1\pgfmath@parse@stop{%
    \pgfmathpostparse
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup
  \ignorespaces}

\let\pgfmathpostparse=\relax

% For compatibility with older version.
%
\def\pgfmathscaleresult{%
  \ifpgfmathunitsdeclared
  \else
    \ifpgfmathignoreunitscale
    \else
       \afterassignment\pgfmath@gobbletilpgfmath@%
      \pgfmath@x\pgfmathresultunitscale pt\relax\pgfmath@%
      \expandafter\pgfmath@x\pgfmathresult\pgfmath@x%
      \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
    \fi
  \fi
}

\def\pgfmathsetresultunitscale#1{\def\pgfmathresultunitscale{#1}}

\def\pgfmathresultunitscale{1}


% A utility function which evaluates expression '#1' and invokes '#2'
% if the expression is true and '#3' if it is false.
\def\pgfmathifexpression#1#2#3{%
    \pgfmathparse{#1}%
    \pgfmath@iftrue{#2}{#3}%
}%
% Executes '#1' if \pgfmathresult is 'true', '#2' otherwise.
% WARNING : overwritten in fpu lib!
\def\pgfmath@iftrue{%
    \ifdim\pgfmathresult pt=1.0pt %
        \let\pgfmath@next=\pgfutil@firstoftwo
    \else
        \let\pgfmath@next=\pgfutil@secondoftwo
    \fi
    \pgfmath@next%
}%

% Stuff for computability with the calc package.
%
\def\pgfmath@calc@real#1{#1}
\def\pgfmath@calc@minof#1#2{min(#1,#2)}
\def\pgfmath@calc@maxof#1#2{max(#1,#2)}
\def\pgfmath@calc@ratio#1#2{#1/#2}
\def\pgfmath@calc@widthof#1{width("#1")}
\def\pgfmath@calc@heightof#1{height("#1")}
\def\pgfmath@calc@depthof#1{depth("#1")}

\def\pgfmath@bgroup{\string\pgfmath@bgroup}
\def\pgfmath@egroup{\string\pgfmath@egroup}
\def\pgfmath@egroup@token{\pgfmath@egroup}

\def\pgfmath@text@@{@}
\def\pgfmath@text@operator{operator}
\def\pgfmath@text@function{function}
\def\pgfmath@dots{...}
\def\pgfmath@char@zero{0}
\def\pgfmath@char@quote{"}
\def\pgfmath@char@exclamation{!}
\def\pgfmath@char@plus{+}
\def\pgfmath@char@minus{-}
\def\pgfmath@char@period{.}
\def\pgfmath@char@leftangle{<}
\def\pgfmath@char@leftbracket{[}
\pgfmath@toks={#}
\edef\pgfmath@char@hash{\the\pgfmath@toks}

\def\pgfmath@tokens@make#1#2{%
  % Defines for each token or balanced text in |#2| a control sequence
  % |\pgfmath@token@<#1>@\string<one token from #2>| and stores |#2|
  % in it.
  \def\pgfmath@prefix{#1}%
  % Note the empty group |{}| at the end that ends the loop in
  % |\pgfmath@token@@make|.
  \expandafter\pgfmath@tokens@@make#2{}}

\def\pgfmath@tokens@@make#1{%
  \def\pgfmath@token{#1}%
  \ifx\pgfmath@token\pgfmath@empty
    % End of loop: all tokens or balanced texts were parsed.
  \else
    \pgfmath@namedef{pgfmath@token@\pgfmath@prefix @\string#1}{#1}%
    \expandafter\pgfmath@tokens@@make%
  \fi}

\pgfmath@tokens@make{box}{\wd\ht\dp}
\ifx\dimexpr\@undefined\else % needed for classic tex
  \pgfmath@tokens@make{dimexpr}{\dimexpr\glueexpr}
\fi
\pgfmath@tokens@make{unit}{{bp}{cc}{cm}{dd}{em}{ex}{in}{mm}{pc}{pt}{sp}}
\ifx\pdftexversion\@undefined\else % for pdfTeX
  \pgfmath@tokens@make{unit}{{nc}{nd}{px}}
\fi
\ifx\directlua\@undefined\else % for LuaTeX
  \pgfmath@tokens@make{unit}{{nc}{nd}{px}}
\fi
\ifx\kanjiskip\@undefined\else % for pTeX, upTeX
  \pgfmath@tokens@make{unit}{{H}{Q}{zh}{zw}}
\fi
%
\pgfmath@tokens@make{mathunit}{{mu}}
\pgfmath@tokens@make{numeric}{.0123456789}
\pgfmath@tokens@make{number}{0123456789}
\pgfmath@tokens@make{functional}{_abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ}
\pgfmath@tokens@make{exponent}{eE}
\pgfmath@tokens@make{group}{{()}{[]}{\pgfmath@bgroup\pgfmath@egroup}}
\pgfmath@tokens@make{specials}{@)]\pgfmath@egroup}
\pgfmath@tokens@make{hexadecimal}{0123456789ABCDEFabcdef}
\pgfmath@tokens@make{octal}{01234567}
\pgfmath@tokens@make{binary}{01}

\pgfmath@namedef{pgfmath@base@0x}{16}
\pgfmath@namedef{pgfmath@base@0X}{16}
\pgfmath@namedef{pgfmath@base@0b}{2}
\pgfmath@namedef{pgfmath@base@0B}{2}

% Determine if a register is a count or a dimension/skip register.
\newif\ifpgfmath@dimen@
\def\pgfmath@dimen@#1{%
  \begingroup
    \afterassignment\pgfmath@dimen@@%
    #1=0.0pt\relax\pgfmath@}
\def\pgfmath@dimen@@#1#2\pgfmath@{%
  \endgroup
  \ifx#1.%
    \pgfmath@dimen@false
  \else
    \pgfmath@dimen@true
  \fi}

\def\pgfmath@parse@ifbgroup#1#2{%
  \let\pgfmath@parse@bgroup@after=#1%
  \let\pgfmath@parse@nobgroup@after=#2%
  \futurelet\pgfmath@token@let%
  \pgfmath@parse@@ifbgroup}

\def\pgfmath@parse@@ifbgroup{%
  \ifx\pgfmath@token@let\bgroup
    \let\pgfmath@parse@next=\pgfmath@parse@@@ifbgroup
  \else
    % |\pgfmath@sptoken| defined in \file{pgfmathutil.code.tex}.
    \ifx\pgfmath@token@let\pgfmath@sptoken
      \let\pgfmath@parse@next=\pgfmath@parse@@@@ifbgroup
    \else
      \let\pgfmath@parse@next=\pgfmath@parse@nobgroup@after
    \fi
  \fi
  \pgfmath@parse@next}

% TT: If false, octal parsing is switched off (needed for time parsing)
\newif\ifpgfmath@octalparsing
\pgfmath@octalparsingtrue

% I (CJ) *think* it replaces |{| and |}| by |\pgfmath@bgroup| and
% |\pgfmath@egroup|?
\def\pgfmath@parse@@@ifbgroup#1{%
  \pgfmath@parse@bgroup@after\pgfmath@bgroup#1\pgfmath@egroup}

{
\def\:{\pgfmath@parse@@@@ifbgroup}
\expandafter\gdef\: {\futurelet\pgfmath@token@let\pgfmath@parse@@ifbgroup}
}

% Parse an operand.
\def\pgfmath@parse@operand{%
  \expandafter\pgfmath@parse@@operand\pgfmath@token@next}

% This is the entry point for the parser. It is called at the end of
% |\pgfmathparse@| with the following syntax
% |\expandafter\pgfmath@parse@@operand\pgfmath@bgroup@stripped
% @@@@\pgfmath@parse@stop|.
% Note: we are inside a group.
\def\pgfmath@parse@@operand{%
  \pgfmath@parse@ifbgroup{\pgfmath@parse@@operand}{\pgfmath@parse@@operand@}}

% An operand is
% * |+| (unary plus),
% * |-| (unary minus),
% * a prefix operator
\def\pgfmath@parse@@operand@#1{%
  \def\pgfmath@token{#1}%
  \ifx\pgfmath@token\pgfmath@char@plus
    % Unary (prefix) plus
    \let\pgfmath@parse@next=\pgfmath@parse@@operand%
  \else
    \ifx\pgfmath@token\pgfmath@char@minus
      % Unary (prefix) minus
      \pgfmath@stack@push@operation{neg}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand
    \else
      % See |\pgfmathdeclareoperator| (below). Note that |+| and |-|
      % that are also declared as operators have been tested before so
      % they should never be parsed as binary (infix) operator at this stage.
      \expandafter\ifx\csname pgfmath@operation@\expandafter\string\pgfmath@token @prefix\endcsname\pgfmath@token
        \let\pgfmath@parse@next=\pgfmath@parse@prefix@operator
      \else
        \ifpgfmath@quickparse
          \let\pgfmath@parse@next=\pgfmath@qparse@operand
        \else
          \let\pgfmath@number=\pgfmath@empty
          \expandafter\ifx\csname pgfmath@token@functional@\string#1\endcsname\relax%
            \let\pgfmath@base=\pgfmath@empty%
            \let\pgfmath@token@next=\pgfmath@token%
            \if#10% Check for octal prefix.
              \ifpgfmath@octalparsing%
                \def\pgfmath@base{8}%
              \fi%
            \fi%
            \let\pgfmath@parse@next=\pgfmath@parse@number%
          \else%
            \let\pgfmath@function=\pgfmath@token%
            \let\pgfmath@parse@next=\pgfmath@parse@function%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}

% Parse prefix operators.
%
\def\pgfmath@parse@prefix@operator{%
  \ifx\pgfmath@token\pgfmath@char@quote% Quote character.
    \let\pgfmath@parse@next=\pgfmath@parse@operand@quote%
  \else%
    \ifx\pgfmath@token\pgfmath@char@exclamation% Prefix !.
      \pgfmath@stack@push@operation{not}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \else% Anything else, just push and hope.
      \expandafter\pgfmath@stack@push@operation\expandafter{\pgfmath@token}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \fi%
  \fi%
  \pgfmath@parse@next%
}%


% Quote part of an expression.
%
\def\pgfmath@parse@operand@quote#1"{%
  \def\pgfmathresult{#1}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Quick operand parsing. Should always have units.
% No functions, base conversion, quoting or scientific notation
% are permitted.
\def\pgfmath@qparse@operand{%
  \afterassignment\pgfmath@qparse@@operand%
  \pgfmath@dimen\pgfmath@token}
\def\pgfmath@qparse@@operand{%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Parse a number, which can take the form:
%
% 1. An integer, or a decimal, with or without units.
% 2. A dimension/skip or a count register.
% 3. A dimension register preceded by a number or count register.
% 4. A box dimension (e.g., \wd\mybox).
% 5. A box dimension preceded by a number or a count register.
% 6. Scientific notation (e.g., 1.234567e-10).
% 7. A binary, hexadecimal, or octal number.
%
\def\pgfmath@parse@number{\pgfmath@parse@ifbgroup{\pgfmath@parse@number}{\pgfmath@parse@number@}}
\def\pgfmath@parse@number@#1{%
  \let\pgfmath@token=\pgfmath@token@next%
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@number}

\def\pgfmath@parse@@number{%
  \ifx\pgfmath@token\pgfmath@egroup@token%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmath@number}%
    \let\pgfmath@parse@next=\pgfmath@parse@@@operator%
  \else%
    \expandafter\ifcat\pgfmath@token\relax% A CS?
      \expandafter\ifx\csname pgfmath@token@dimexpr@\expandafter\string\pgfmath@token\endcsname\relax%
        \expandafter\ifx\pgfmath@token\numexpr%
          \let\pgfmath@parse@next=\pgfmath@parse@numexpr%
        \else%
          \expandafter\ifx\pgfmath@token\muexpr%
            \let\pgfmath@parse@next=\pgfmath@parse@muexpr%
          \else%
            \expandafter\ifx\csname pgfmath@token@box@\expandafter\string\pgfmath@token\endcsname\relax%
              % So, is the CS is a dimension or a count register?
              \expandafter\pgfmath@dimen@\pgfmath@token%
              \ifpgfmath@dimen@% A dimension register.
                \global\pgfmathunitsdeclaredtrue%
                \pgfmath@dimen=\pgfmath@number\pgfmath@token%
                \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
                \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                \let\pgfmath@parse@next=\pgfmath@parse@operator%
              \else% A count register.
                \pgfmath@count=\pgfmath@token%
                \expandafter\def\expandafter\pgfmath@number\expandafter{\the\pgfmath@count}%
                \expandafter\ifcat\pgfmath@token@next\relax%
                  % A CS following a count register should be \wd, \ht or \dp.
                  \let\pgfmath@parse@next=\pgfmath@parse@number%
                \else%
                  \let\pgfmathresult=\pgfmath@number%
                  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                  \let\pgfmath@parse@next=\pgfmath@parse@operator%
                \fi%
              \fi%
            \else%
              % This should be a box specification, for example, 0.5\wd\mybox.
              \global\pgfmathunitsdeclaredtrue%
              \pgfmath@dimen=\pgfmath@number\pgfmath@token\pgfmath@token@next%
              \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
              \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
              \let\pgfmath@parse@next=\pgfmath@parse@@operator%
            \fi%
          \fi%
        \fi%
      \else%
        \global\pgfmathunitsdeclaredtrue%
        \let\pgfmath@parse@next=\pgfmath@parse@dimexpr%
      \fi%
    \else%
      \expandafter\ifx\csname pgfmath@token@numeric@\expandafter\string\pgfmath@token\endcsname\relax%
        % It isn't numeric (i.e., 012345679.), so it might be units...
        % first double-character units...
        \expandafter\ifx\csname pgfmath@token@unit@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
        % then single-character units...
        \expandafter\ifx\csname pgfmath@token@unit@\pgfmath@token\endcsname\relax%
          % ...or the exponent characters...
          \expandafter\ifx\csname pgfmath@token@exponent@\pgfmath@token\endcsname\relax%
            % ...or a base prefix...
            \expandafter\ifx\csname pgfmath@base@\pgfmath@number\pgfmath@token\endcsname\relax%
              % ...or a math unit...
              \expandafter\ifx\csname pgfmath@token@mathunit@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
                % ...none of the above...
                  \ifx\pgfmath@base\pgfmath@empty%
                    \let\pgfmathresult=\pgfmath@number%
                  \else%
                    \ifx\pgfmath@number\pgfmath@char@zero%
                      \let\pgfmathresult=\pgfmath@number%
                    \else%
                      % Convert from octal.
                      \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{8}{10}%
                    \fi%
                  \fi%
                  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                  \let\pgfmath@parse@next=\pgfmath@parse@@@operator%
              \else%
                % ...here, it is a math unit (mu). Treat it as a pt.
                \global\pgfmathunitsdeclaredtrue%
                \global\pgfmathmathunitsdeclaredtrue%
                \pgfmath@dimen=\pgfmath@number pt\relax%
                \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
                \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                \let\pgfmath@parse@next=\pgfmath@parse@@operator%
              \fi%
            \else%
              % ...here, it is a base prefix 0x, 0X, 0b or 0B
              \expandafter\let\expandafter\pgfmath@base\expandafter=%
                \csname pgfmath@base@\pgfmath@number\pgfmath@token\endcsname%
              \let\pgfmath@parse@next=\pgfmath@parse@base%
            \fi%
          \else% ... and here, it is the exponent characters.
            \let\pgfmath@parse@next=\pgfmath@parse@exponent%
          \fi%
        \else% ...but here it is single-character units.
          \global\pgfmathunitsdeclaredtrue%
          \pgfmath@dimen=\pgfmath@number\pgfmath@token\relax%
          \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
          \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
          \let\pgfmath@parse@next=\pgfmath@parse@@operator%
        \fi%
        \else% ...but here it is double-character units.
          \global\pgfmathunitsdeclaredtrue%
          \pgfmath@dimen=\pgfmath@number\pgfmath@token\pgfmath@token@next\relax%
          \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
          \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
          \let\pgfmath@parse@next=\pgfmath@parse@@operator%
        \fi%
      \else% It is numeric.
        \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgfmath@number%
          \expandafter\expandafter\expandafter{\expandafter\pgfmath@number\pgfmath@token}%
        \ifx\pgfmath@token\pgfmath@char@period%
          \let\pgfmath@base=\pgfmath@empty%
        \fi%
        \let\pgfmath@parse@next=\pgfmath@parse@number%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}


% Parse a \dimexpr
\def\pgfmath@parse@dimexpr{%
  \afterassignment\pgfmath@parse@dimexpr@%
  \expandafter\expandafter\expandafter\pgfmath@dimen\expandafter\pgfmath@token\pgfmath@token@next%
}
\def\pgfmath@parse@dimexpr@{%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}


% Parse a \muexpr
\def\pgfmath@parse@muexpr{%
  \begingroup%
    \afterassignment\pgfmath@parse@muexpr@%
    \expandafter\expandafter\expandafter\muskip\expandafter\expandafter\expandafter0\expandafter\pgfmath@token\expandafter\pgfmath@token@next%
}
\def\pgfmath@parse@muexpr@{%
  \expandafter\endgroup%
  \expandafter\edef\expandafter\pgfmathresult\expandafter{\expandafter\pgfMATH@STRIPMU\the\muskip0}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

{
\catcode`\m=12
\catcode`\u=12
\gdef\pgfMATH@STRIPMU#1mu{#1}
}


% Parse a \numexpr
\def\pgfmath@parse@numexpr{%
  \afterassignment\pgfmath@parse@numexpr@%
  \expandafter\expandafter\expandafter\pgfmath@count\expandafter\pgfmath@token\pgfmath@token@next%
}
\def\pgfmath@parse@numexpr@#1{%
  \expandafter\def\expandafter\pgfmath@number\expandafter{\the\pgfmath@count}%
  \def\pgfmath@token@next{#1}%
  \expandafter\ifcat\pgfmath@token@next\relax%
    % A CS following a count register should be \wd, \ht or \dp.
    \let\pgfmath@parse@next=\pgfmath@parse@number%
  \else%
    \let\pgfmathresult=\pgfmath@number%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \fi%
  \pgfmath@parse@next%
}


% Parse the exponent of a number.
%
% REMARK: this method will be overwritten by the FPU library. Please
% keep changes consistent...
\def\pgfmath@parse@exponent{%
  \afterassignment\pgfmath@parse@@exponent%
  \pgfmath@count\pgfmath@token@next}
\def\pgfmath@parse@@exponent{%
  \pgfmathscientific{\pgfmath@number}{\the\pgfmath@count}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Parse binary or hexadecimal numbers (octal numbers done elsewhere).
%
\def\pgfmath@parse@base{%
  \ifnum\pgfmath@base=2\relax%
    \let\pgfmath@parse@next=\pgfmath@parse@binary%
  \else%
    \ifnum\pgfmath@base=16\relax%
      \let\pgfmath@parse@next=\pgfmath@parse@hexadecimal%
    \else%
      \pgfmath@error{Unexpected numerical base `\pgfmath@base'}{}%
      \def\pgfmathresult{0}%
      \let\pgfmath@parse@next=\pgfmath@parse@end%
    \fi%
  \fi%
  \let\pgfmath@number=\pgfmath@empty%
  \expandafter\pgfmath@parse@next\pgfmath@token@next%
}

\def\pgfmath@parse@binary#1{%
  \expandafter\ifx\csname pgfmath@token@binary@#1\endcsname\relax%
    \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{2}{10}%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \def\pgfmath@token@next{#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \else%
    \expandafter\def\expandafter\pgfmath@number\expandafter{\pgfmath@number#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@binary%
  \fi%
  \pgfmath@parse@next%
}

\def\pgfmath@parse@hexadecimal#1{%
  \expandafter\ifx\csname pgfmath@token@hexadecimal@#1\endcsname\relax%
    \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{16}{10}%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \def\pgfmath@token@next{#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \else%
    \expandafter\def\expandafter\pgfmath@number\expandafter{\pgfmath@number#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@hexadecimal%
  \fi%
  \pgfmath@parse@next%
}

% Parse a function.
%
\def\pgfmath@parse@function{\pgfmath@parse@ifbgroup{\pgfmath@parse@function}{\pgfmath@parse@@function}}
\def\pgfmath@parse@function@{\futurelet\pgfmath@token@let\pgfmath@parse@@function}
\def\pgfmath@parse@@function{%
  \ifx\pgfmath@token@let\pgfmath@sptoken%
    \let\pgfmath@token=\pgfmath@empty%
    \let\pgfmath@parse@next=\pgfmath@parse@@@@function%
  \else%
    \let\pgfmath@parse@next=\pgfmath@parse@@@function%
  \fi%
  \pgfmath@parse@next}

\def\pgfmath@parse@@@function#1{%
  \expandafter\ifx\csname pgfmath@token@functional@\expandafter\string#1\endcsname\relax%
    \expandafter\ifx\csname pgfmath@token@number@\expandafter\string#1\endcsname\relax%
      \def\pgfmath@token{#1}% Not from A-Z, a-z, 0-9, or _.
      \let\pgfmath@parse@next=\pgfmath@parse@@@@function%
    \else% It is from 0-9.
      \expandafter\def\expandafter\pgfmath@function\expandafter{\pgfmath@function#1}%
      \let\pgfmath@parse@next=\pgfmath@parse@function@%
    \fi%
  \else% It is from  A-Z, a-z, or _.
    \edef\pgfmath@function{\pgfmath@function#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@function@%
  \fi%
  \pgfmath@parse@next}

\def\pgfmath@parse@@@@function{%
  \expandafter\ifx\csname pgfmath@function@\pgfmath@function\endcsname\relax%
    \pgfmath@error{Unknown function `\pgfmath@function'}{}%
    \def\pgfmathresult{0}%
    \let\pgfmath@parse@next=\pgfmath@parse@end%
  \else%
    \expandafter\ifnum\csname pgfmath@operation@\pgfmath@function @arity\endcsname=0\relax%
     % Functions with zero arity are called directly.
      \csname pgfmath\pgfmath@function @\endcsname%
      \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operator%
    \else% Otherwise, they are pushed onto the operator stack
      \expandafter\pgfmath@stack@push@operation\expandafter{\pgfmath@function}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \fi%
  \fi%
  \expandafter\pgfmath@parse@next\pgfmath@token}

% Parse an operator.
%
\def\pgfmath@parse@operator{\pgfmath@parse@ifbgroup{\pgfmath@parse@operator}{\pgfmath@parse@operator@}}%
\def\pgfmath@parse@operator@#1{% Get one token.
  \let\pgfmath@token=\pgfmath@token@next%
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@@operator}

\def\pgfmath@parse@@operator{\pgfmath@parse@ifbgroup{\pgfmath@parse@@operator}{\pgfmath@parse@@operator@}}%
\def\pgfmath@parse@@operator@#1{% Get first token...
  \def\pgfmath@token{#1}%
  \pgfmath@parse@ifbgroup{\pgfmath@parse@@operator@@}{\pgfmath@parse@@operator@@}}%
\def\pgfmath@parse@@operator@@#1{% ...and second token.
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@@operator}

\def\pgfmath@parse@@@operator{%
  \expandafter\ifx\csname pgfmath@operator@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
    % Not a double character operator.
    \expandafter\ifx\csname pgfmath@operator@\pgfmath@token\endcsname\relax%
      % Not a single character operator.
      \pgfmath@error{Unknown operator `\pgfmath@token' or `\pgfmath@token\pgfmath@token@next'}{}%
      \def\pgfmathresult{0}%
    \let\pgfmath@parse@next=\pgfmath@parse@end%
    \else%
      \expandafter\pgfmath@operation@process\expandafter{\pgfmath@token}%
      \ifx\pgfmath@token\pgfmath@text@@%
        \let\pgfmath@parse@next=\pgfmath@parse@end%
      \else%
        \expandafter\ifx\csname pgfmath@operation@\pgfmath@token @postfix\endcsname\pgfmath@token%
          % Postfix operators are followed by an operator.
          \ifx\pgfmath@token@next\pgfmath@char@leftbracket% Except [.
            \let\pgfmath@parse@next=\pgfmath@parse@operand%
          \else%
            \let\pgfmath@parse@next=\pgfmath@parse@operator%
          \fi%
        \else%
          % Any other operator is followed by an operand.
          \let\pgfmath@parse@next=\pgfmath@parse@operand%
        \fi%
      \fi%
    \fi%
  \else%
    % A double character operator...
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
      \pgfmath@token\expandafter\expandafter\expandafter%
        {\expandafter\pgfmath@token\pgfmath@token@next}%
    \expandafter\pgfmath@operation@process\expandafter{\pgfmath@token}%
    % ...is always followed by an operand.
    \let\pgfmath@parse@next=\pgfmath@parse@@operand%
  \fi%
  \pgfmath@parse@next%
}


% Process an operation.
%
\def\pgfmath@operation@process#1{%
  \def\pgfmath@operator{#1}%
  \ifx\pgfmath@stack@operation@top\pgfmath@stack@empty%
  \else%
    \pgfmath@operation@@process%
  \fi%
  \expandafter\ifx\csname pgfmath@token@specials@#1\endcsname\relax%
    \pgfmath@stack@push@operation{#1}%
  \fi%
}

% Process the operation stack.
%
\def\pgfmath@operation@@process{%
  \ifx\pgfmath@stack@operation@top\pgfmath@stack@empty%
    \let\pgfmath@parse@next=\relax%
  \else%
    \ifnum\csname pgfmath@operation@\pgfmath@operator @precedence\endcsname>%
      \csname pgfmath@operation@\pgfmath@stack@operation@top @precedence\endcsname\relax%
      % If the precedence of the scanned operator is greater than the
      % precedence of the operator at the top of the stack, do nothing.
      \let\pgfmath@parse@next=\relax%
    \else%
      \let\pgfmath@stack@operation@last=\pgfmath@stack@operation@top%
      \expandafter\ifx\csname pgfmath@operator@\pgfmath@stack@operation@top\endcsname\relax%
        \pgfmath@function@@@process%
      \else%
        \pgfmath@operator@@@process%
      \fi%
      \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
      \expandafter\ifx\csname pgfmath@token@group@\pgfmath@stack@operation@last\pgfmath@operator\endcsname\relax%
        \let\pgfmath@parse@next=\pgfmath@operation@@process%
      \else%
        \let\pgfmath@parse@next=\relax%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}

% Process an operator.
%
\def\pgfmath@operator@@@process{% Process an operator.
  \pgfmath@stack@pop@operation\pgfmath@@operator%
  \pgfmath@stack@pop@operand\pgfmath@operand@a%
  \ifcase\csname pgfmath@operation@\pgfmath@@operator @arity\endcsname\relax%
    % Zero arity operators (!).
  \or%
    \pgfmath@operator@@@@process{\pgfmath@operand@a}%
  \or%
    \pgfmath@stack@pop@operand\pgfmath@operand@b%
    \pgfmath@operator@@@@process{\pgfmath@operand@b}{\pgfmath@operand@a}%
  \or%
    \pgfmath@stack@pop@operand\pgfmath@operand@b%
    \expandafter\pgfmath@operator@@@@process\expandafter%
      {\expandafter\pgfmath@operand@b\expandafter}\pgfmath@operand@a%
  \else%
    % No operators with more than tenary arity.
  \fi%
}

\def\pgfmath@operator@@@@process{%
  \csname pgfmath%
    \csname pgfmath@operation@\pgfmath@@operator @name\endcsname%
  @\endcsname}

% Process a function.
%
\def\pgfmath@function@@@process{% Process a function.
  \ifnum\csname pgfmath@operation@\pgfmath@stack@operation@top @arity\endcsname>0\relax%
    \pgfmath@stack@pop@operation\pgfmath@@function%
    \pgfmath@stack@pop@operand\pgfmath@@operand%
    \ifnum\csname pgfmath@operation@\pgfmath@@function @arity\endcsname>1\relax%
      \ifnum\csname pgfmath@operation@\pgfmath@@function @arity\endcsname>9\relax%
        \csname pgfmath\pgfmath@@function @\endcsname{\pgfmath@@operand}%
      \else%
        \expandafter\pgfmath@function@@@@process\pgfmath@@operand%
      \fi
    \else%
      \expandafter\pgfmath@function@@@@process\expandafter{\pgfmath@@operand}%
    \fi%
  \fi%
}

\def\pgfmath@function@@@@process{\csname pgfmath\pgfmath@@function @\endcsname}

% Stack.
%
\newtoks\pgfmath@stack@operand
\newtoks\pgfmath@stack@operation
\let\pgfmath@stack@empty=\pgfmath@empty

\def\pgfmath@stack@push#1#2{%
  \def\pgfmath@stack@top{#2}%
  \expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
      {\expandafter\pgfmath@stack@top\expandafter}\the#1}}%

\def\pgfmath@stack@pop#1#2{\expandafter\pgfmath@stack@@pop\the#1\pgfmath@stack@stop{#1}{#2}}
\def\pgfmath@stack@@pop#1#2#3\pgfmath@stack@stop#4#5{\def#5{#1}#4={{#2}#3}\def\pgfmath@stack@top{#2}}

\def\pgfmath@stack@push@operation#1{%
  \pgfmath@stack@push\pgfmath@stack@operation{#1}%
  \let\pgfmath@stack@operation@top=\pgfmath@stack@top}

\def\pgfmath@stack@pop@operation#1{%
  \pgfmath@stack@pop\pgfmath@stack@operation{#1}%
  \let\pgfmath@stack@operation@top=\pgfmath@stack@top}

% REMARK: This method will be overwritten by the FPU library. Please
% keep any changes consistent.
\def\pgfmath@stack@push@operand#1{%
  \pgfmath@stack@push\pgfmath@stack@operand{#1}%
  \let\pgfmath@stack@operand@top=\pgfmath@stack@top}

\def\pgfmath@stack@pop@operand#1{%
  \pgfmath@stack@pop\pgfmath@stack@operand{#1}%
  \let\pgfmath@stack@operand@top=\pgfmath@stack@top}


% Declare an operator for the parser.
%
% It is not recommended that new operators be created as
% the parser is not fully robust for arbitrary operators.
%
\def\pgfmathdeclareoperator#1#2#3#4#5{%
  \ifx\pgfmath@operatorlist\pgfutil@empty
    \edef\pgfmath@operatorlist{{\string#1}}%
  \else
    \edef\pgfmath@operatorlist{\pgfmath@operatorlist,{\string#1}}%
  \fi
  \pgfmath@namedef{pgfmath@operator@\string#1}{#1}%
  \pgfmath@namedef{pgfmath@operation@\string#1@name}{#2}%
  \pgfmath@namedef{pgfmath@operation@\string#1@arity}{#3}%
  \pgfmath@namedef{pgfmath@operation@\string#1@#4}{#1}%
  \pgfmath@namedef{pgfmath@operation@\string#1@precedence}{#5}%
}

\def\pgfmath@operatorlist{}

\pgfmathdeclareoperator{+}{add}     {2}{infix}{500}
\pgfmathdeclareoperator{-}{subtract}{2}{infix}{500}
\pgfmathdeclareoperator{*}{multiply}{2}{infix}{700}
\pgfmathdeclareoperator{/}{divide}  {2}{infix}{700}
\pgfmathdeclareoperator{^}{pow}     {2}{infix}{900}

\pgfmathdeclareoperator{<} {}       {1}{prefix} {1}

\pgfmathdeclareoperator{>} {greater}   {2}{infix} {250}
\pgfmathdeclareoperator{<} {less}      {2}{infix} {250}
\pgfmathdeclareoperator{==}{equal}     {2}{infix} {250}
\pgfmathdeclareoperator{>=}{notless}   {2}{infix} {250}
\pgfmathdeclareoperator{<=}{notgreater}{2}{infix} {250}
\pgfmathdeclareoperator{&&}{and}       {2}{infix} {200}
\pgfmathdeclareoperator{||}{or}        {2}{infix} {200}
\pgfmathdeclareoperator{!=}{notequal}  {2}{infix} {250}
\pgfmathdeclareoperator{!} {not}       {1}{prefix}{975}
\pgfmathdeclareoperator{?} {ifthenelse}{3}{infix} {100}
\pgfmathdeclareoperator{:} {@@collect}  {2}{infix}{101}

\pgfmathdeclareoperator{!}{factorial}{1}{postfix}{800}% Must be defined after prefix ! operator.
\pgfmathdeclareoperator{r}{deg}      {1}{postfix}{600}

\pgfmathdeclareoperator{,}{@collect}   {2}{infix}  {10}
\pgfmathdeclareoperator{[}{@startindex}{2}{prefix} {7}
\pgfmathdeclareoperator{]}{@endindex}  {0}{postfix}{6}
\pgfmathdeclareoperator{(}{@startgroup}{1}{prefix} {5}
\pgfmathdeclareoperator{)}{@endgroup}  {0}{postfix}{4}

\pgfmathdeclareoperator{\pgfmath@bgroup}{@startarray}{1}{prefix} {3}
\pgfmathdeclareoperator{\pgfmath@egroup}{@endarray}  {1}{postfix}{2}%

% Special operators.
\pgfmathdeclareoperator{"}{}{1}{prefix}{1}
\pgfmathdeclareoperator{@}{}{0}{postfix}{0}

% Internal functions.

% Begin and end parenthesis ().
%
\def\pgfmath@startgroup@#1{\pgfmath@protected@edef\pgfmathresult{#1}}
\def\pgfmath@endgroup@{}% Never actually called.

% Begin and end array access [].
%
\def\pgfmath@startindex@#1#2{%
  \expandafter\pgfmatharray@#1{#2}%
  \expandafter\pgfmath@bgroup@strip\expandafter{\pgfmathresult}%
  \ifx\pgfmath@token@let\bgroup%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmathresult}}%
  \fi}
\def\pgfmath@endindex@{}% Never actually called.

% Begin and end array {}.
%
\def\pgfmath@startarray@#1{\expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{#1}}}
\def\pgfmath@endarray@#1{\expandafter\def\expandafter\pgfmathresult\expandafter{#1}}% Never actually called.


\def\pgfmath@@collect@#1#2{%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgfmathresult\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
      {\expandafter#1\expandafter}\expandafter{#2}}%
}
% Collect items separated by ,.
%
\def\pgfmath@collect@#1#2{%
  \expandafter\def\expandafter\pgfmath@collect@original\expandafter{#1}%
  \expandafter\pgfmath@bgroup@strip\expandafter{#1}%
  \ifx\pgfmath@token@let\bgroup%
    \ifx\pgfmath@collect@original\pgfmath@bgroup@stripped%
      \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmath@bgroup@stripped}%
    \else%
      \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmath@bgroup@stripped}}%
    \fi%
  \else%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmath@bgroup@stripped}}%
  \fi%
  \expandafter\pgfmath@bgroup@strip\expandafter{#2}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgfmathresult\expandafter\expandafter\expandafter%
      {\expandafter\pgfmathresult\expandafter{\pgfmath@bgroup@stripped}}%
}

% Strip braces from a token sequence.
%
\def\pgfmath@bgroup@strip#1{%
  \def\pgfmath@bgroup@strip@last{#1}%
  \pgfmath@bgroup@@strip{#1}\pgfmath@\pgfmath@@\pgfmath@@@}

\def\pgfmath@bgroup@strip@#1{%
  \def\pgfmath@bgroup@strip@last{#1}%
  \pgfmath@bgroup@@strip#1\pgfmath@\pgfmath@@\pgfmath@@@}

\def\pgfmath@bgroup@pgfmath@{\pgfmath@}

\def\pgfmath@bgroup@@strip{%
  \futurelet\pgfmath@token@let\pgfmath@bgroup@@@strip}

\def\pgfmath@bgroup@@@strip#1#2#3\pgfmath@@@{%
  \ifx\pgfmath@token@let\bgroup
    \def\pgfmath@bgroup@test{#2}%
    \ifx\pgfmath@bgroup@test\pgfmath@bgroup@pgfmath@
      \def\pgfmath@next{\pgfmath@bgroup@strip@{#1}}%
    \else
      \let\pgfmath@bgroup@stripped=\pgfmath@bgroup@strip@last
      \let\pgfmath@next=\relax
    \fi
  \else
    \pgfmath@bgroup@@@@strip#1#2#3%
    \let\pgfmath@next=\relax
  \fi
  \pgfmath@next}

\def\pgfmath@bgroup@@@@strip#1\pgfmath@\pgfmath@@{%
  \def\pgfmath@bgroup@stripped{#1}}

% Local Variables:
% tab-width: 2
% End:


==> pgfmathutil.code.tex <==
% Copyright 2019 Mark Wibrow
%
% but subject to the LaTeX Project Public License
% (http://www.latex-project.org/lppl.txt)
%
% and the GNU Public License
% (http://www.gnu.org/licenses/gpl.txt)
%

% This file defines utilities common to the \pgfmath files.
%
% Version 1.414213 29/9/2007

\def\pgfmathincluded{}

% Helper macros for \pgfmath@ifregister
%
\def\pgfmath@grabv#1#2#3#4#5#6#7\pgfmath@grabv{#2#3#4#5\ifx#6!!\fi}
\def\pgfmath@ifskip@extract#1{\expandafter\pgfmath@grabv\meaning#1!!!!!!\pgfmath@grabv}
\def\pgfmath@iftoks@extract#1{\expandafter\pgfmath@grabv\meaning#1!!!!!!\pgfmath@grabv}

\def\pgfmath@grabvi#1#2#3#4#5#6#7#8\pgfmath@grabvi{#2#3#4#5#6\ifx#7!!\fi}
\def\pgfmath@ifdimen@extract#1{\expandafter\pgfmath@grabvi\meaning#1!!!!!!\pgfmath@grabvi}
\def\pgfmath@ifcount@extract#1{\expandafter\pgfmath@grabvi\meaning#1!!!!!!\pgfmath@grabvi}

\def\pgfmath@grabvii#1#2#3#4#5#6#7#8#9\pgfmath@grabvii{#2#3#4#5#6#7\ifx#8!!\fi}
\def\pgfmath@ifmuskip@extract#1{\expandafter\pgfmath@grabvii\meaning#1!!!!!!\pgfmath@grabvii}

% \pgfmath@ifdimen@unguarded
%
% Check if #2 is a register of type #1.
% Credits to Frank: https://tex.stackexchange.com/a/56905
%
% #1 register type (count, dimen, skip, muskip, toks)
% #2 single token
%
\def\pgfmath@ifregister@unguarded#1#2{%
    \expandafter\ifx\csname\csname pgfmath@if#1@extract\endcsname{#2}\expandafter\endcsname\csname #1\endcsname
        \expandafter\pgfutil@firstoftwo
    \else
        \expandafter\pgfutil@secondoftwo
    \fi}

% \pgfmath@ifregister
%
% Checks if a token is a a certain type of register
%
% #1 register type (count, dimen, skip, muskip, toks)
% #2 single token
%
\def\pgfmath@ifregister#1#2{%
    \pgfutil@IfUndefined{pgfmath@if#1@extract}%
        {\errmessage{Package PGF Math Error: Cannot test for #1 register}}%
        {\pgfutil@IfUndefined{\csname pgfmath@if#1@extract\endcsname{#2}}%
            {\pgfutil@secondoftwo}}%
            {\pgfmath@ifregister@unguarded{#1}{#2}}}

% \pgfmath@ensureregister
%
% Ensure a control sequence exists as a TeX count/dimen register.
%
% #1 - count or dimen.
% #2 - a control sequence.
%
\def\pgfmath@ensureregister#1#2{%
    \pgfmath@ifregister{#1}{#2}%
        {}%
        {\csname new#1\endcsname#2}%
}

% Check registers exist. If not, create them.
%
\pgfmath@ensureregister{dimen}{\pgf@x}
\pgfmath@ensureregister{dimen}{\pgf@xa}
\pgfmath@ensureregister{dimen}{\pgf@xb}
\pgfmath@ensureregister{dimen}{\pgf@xc}

\pgfmath@ensureregister{dimen}{\pgf@y}
\pgfmath@ensureregister{dimen}{\pgf@ya}
\pgfmath@ensureregister{dimen}{\pgf@yb}
\pgfmath@ensureregister{dimen}{\pgf@yc}

\pgfmath@ensureregister{dimen}{\pgfutil@tempdima}
\pgfmath@ensureregister{dimen}{\pgfutil@tempdimb}

\pgfmath@ensureregister{count}{\c@pgf@counta}
\pgfmath@ensureregister{count}{\c@pgf@countb}
\pgfmath@ensureregister{count}{\c@pgf@countc}
\pgfmath@ensureregister{count}{\c@pgf@countd}

\pgfmath@ensureregister{count}{\pgfutil@tempcnta}
\pgfmath@ensureregister{count}{\pgfutil@tempcntb}

% Alias for \pgfmath.
%
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\pgfmath@tempdima\pgfutil@tempdima
\let\pgfmath@tempdimb\pgfutil@tempdimb

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc
\let\c@pgfmath@countd\c@pgf@countd

\let\pgfmath@tempcnta\pgfutil@tempcnta
\let\pgfmath@tempcntb\pgfutil@tempcntb

% Now check if pgfutil and pgf@sys stuff exists. If it does, fine.
% Just \let pgfmath versions. If not, define pgfmath versions (Arghhh).
%

% \...ifnextchar
%
\ifx\pgfutil@ifnextchar\pgfmath@undefined%
    \long\def\pgfmath@ifnextchar#1#2#3{%
  \let\pgfmath@reserved@d#1%
  \def\pgfmath@reserved@a{#2}%
  \def\pgfmath@reserved@b{#3}%
  \futurelet\pgfmath@let@token\pgfmath@ifnch}
    \def\pgfmath@ifnch{%
      \ifx\pgfmath@let@token\pgfmath@sptoken%
        \let\pgfmath@reserved@c\pgfmath@xifnch%
      \else%
        \ifx\pgfmath@let@token\pgfmath@reserved@d%
          \let\pgfmath@reserved@c\pgfmath@reserved@a%
        \else%
          \let\pgfmath@reserved@c\pgfmath@reserved@b%
        \fi%
      \fi%
      \pgfmath@reserved@c}
    {%
      \def\:{\global\let\pgfmath@sptoken= } \:
      \def\:{\pgfmath@xifnch} \expandafter\gdef\: {\futurelet\pgfmath@let@token\pgfmath@ifnch}
    }%
\else%
    \let\pgfmath@ifnextchar\pgfutil@ifnextchar%
    % Still need to define \pgfmath@sptoken (cannot \let).
    {%
        \def\:{\global\let\pgfmath@sptoken= } \:
    }%
\fi%

% \...ifundefined
%
\ifx\pgfutil@ifundefined\pgfmath@undefined%
    \long\def\pgfmath@ifundefined#1{%
      \expandafter\ifx\csname#1\endcsname\relax%
        \expandafter\pgfmath@firstoftwo%
      \else%
        \expandafter\pgfmath@secondoftwo%
      \fi}%
\else%
    \let\pgfmath@ifundefined\pgfutil@ifundefined%
\fi%

% \...selectfont
%
\ifx\pgfutil@selectfont\pgfmath@undefined%
    \ifx\selectfont\pgfmath@undefined%
        \let\pgfmath@selectfont\rm% Plain TeX and ConTeXt.
    \else%
        \let\pgfmath@selectfont\selectfont% LaTeX.
    \fi%
\else%
    \let\pgfmath@selectfont\pgfutil@selectfont%
\fi%

% New definition easier than fussing around with let.
%
\newif\ifpgfmath@in@
\def\pgfmath@in@#1#2{%
 \def\pgfmath@in@@##1#1##2##3\pgfmath@in@@{%
  \ifx\pgfmath@in@##2\pgfmath@in@false\else\pgfmath@in@true\fi}%
 \pgfmath@in@@#2#1\pgfmath@in@\pgfmath@in@@}


% \...tonumber
%
\ifx\pgf@sys@tonumber\pgfmath@undefined%
  {\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}
    \def\pgfmath@tonumber#1{\expandafter\Pgf@geT\the#1}
\else%
    \let\pgfmath@tonumber\pgf@sys@tonumber%
\fi%


% \PackageWarning and \PackageError
%
\ifx\PackageWarning\pgfmath@undefined
    \def\pgfmath@PackageWarning#1#2{\immediate\write-1{Package #1: Warning! #2.}}%
\else%
    \let\pgfmath@PackageWarning\PackageWarning%
\fi%
\ifx\PackageError\pgfmath@undefined
    \def\pgfmath@PackageError#1#2#3{\errmessage{Package #1 Error: #2.}}%
\else%
    \let\pgfmath@PackageError\PackageError%
\fi%

\def\pgfmath@error#1#2{%
    \pgfmath@PackageError{PGF Math}{%
        #1%
        \pgfutil@ifundefined{pgfmath@expression}{}{ (in '\pgfmath@expression')}%
    }{#2}%
}
\def\pgfmath@warning#1{%
    \pgfmath@PackageWarning{PGF Math}{%
        #1%
        \pgfutil@ifundefined{pgfmath@expression}{}{ (in '\pgfmath@expression')}%
    }%
}

% \pgfmath@pt
%
% Needed to test for 'pt' resulting from expansion using \the.
%
{\catcode`\p=12\catcode`\t=12\gdef\PgfmaTh@PT{pt}}
\edef\pgfmath@pt{\PgfmaTh@PT}%

% \pgfmath@empty
%
% A handy macro.
%
\def\pgfmath@empty{}

\def\pgfmath@firstoftwo#1#2{#1}
\def\pgfmath@secondoftwo#1#2{#2}

% \pgfmath@gobbletilpgfmath@
%
% Gobble stream until \pgfmath@ {which is undefined}.
%
\def\pgfmath@gobbletilpgfmath@#1\pgfmath@{}
\def\pgfmath@gobbleone#1{}%


\def\pgfmath@namedef#1{\expandafter\def\csname#1\endcsname}
\def\pgfmath@nameedef#1{\expandafter\edef\csname#1\endcsname}

% \pgfmathloop
%
% A version of the standard TeX and LaTeX
% \loop, with an additional macro \pgfmathcounter
% (which is *not* a TeX counter) which keeps
% track of the iterations.
%
\newif\ifpgfmathcontinueloop
\def\pgfmathloop#1\repeatpgfmathloop{%
    \def\pgfmathcounter{1}%
    \def\pgfmath@iterate{%
        #1\relax%
        {% Do this inside a group, just in case...
            \c@pgfmath@counta\pgfmathcounter%
            \advance\c@pgfmath@counta1\relax%
            \xdef\pgfmathloop@temp{\the\c@pgfmath@counta}%
        }%
        \edef\pgfmathcounter{\pgfmathloop@temp}%
        \expandafter\pgfmath@iterate\fi}%
    \pgfmath@iterate\let\pgfmath@iterate\relax}
\let\repeatpgfmathloop\fi
\def\pgfmathbreakloop{\let\pgfmath@iterate\relax}%

% \pgfmath@returnone
%
% #1 - a dimension representing a number or dimension.
%
% Changed by TT: made faster and simpler since it is used
% *heavily*. #1 must be something that can be assigned to a
% dimension.
%
\def\pgfmath@returnone#1\endgroup{%
  \pgfmath@x#1%
  \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
  \expandafter\endgroup\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmath@temp}%
}

\let\pgfmathreturn=\pgfmath@returnone

% \pgfmath@smuggleone
%
% Smuggle a macro outside a group.
%
% Changed by TT: Speedup by insisting, that smuggleone is directly
% followed by \endgroup
%
\def\pgfmath@smuggleone#1\endgroup{%
  \expandafter\endgroup\expandafter\def\expandafter#1\expandafter{#1}}

\let\pgfmathsmuggle=\pgfmath@smuggleone


==> pgfmoduledecorations.code.tex <==
% Copyright 2019 by Mark Wibrow and Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% The following naming conventions are (more or less) observed:
%
% `decorated'  : the path that is being decorated.
% `decoration' : any path created/left by the automaton
% `decorate'   : generic use where distinction is probably unimportant
%                (e.g. internal macros).



% These should be moved.
%
\def\pgfgetpath#1{\pgfsyssoftpath@getcurrentpath{#1}}%
\def\pgfsetpath#1{\pgfsyssoftpath@setcurrentpath{#1}}%


% Required registers.
%
\newdimen\pgfdecoratedcompleteddistance
\newdimen\pgfdecoratedremainingdistance
\newdimen\pgfdecoratedinputsegmentcompleteddistance
\newdimen\pgfdecoratedinputsegmentremainingdistance
\newdimen\pgf@decorate@distancetomove

\newcount\pgf@decorate@repeatstate


% Extra options used in all libraries

\newdimen\pgfdecorationsegmentamplitude
\newdimen\pgfdecorationsegmentlength
\pgfdecorationsegmentamplitude2.5pt
\pgfdecorationsegmentlength10pt
\def\pgfdecorationsegmentangle{45}%
\def\pgfdecorationsegmentaspect{0.5}%
\def\pgfmetadecorationsegmentamplitude{2.5pt}%
\def\pgfmetadecorationsegmentlength{1cm}%

\pgfkeys{%
  /pgf/decoration/.code={\pgfkeys{/pgf/decoration/.cd,#1}},
  /pgf/decoration/.cd,
  amplitude/.code={\pgfmathsetlength\pgfdecorationsegmentamplitude{#1}},
  meta-amplitude/.store in=\pgfmetadecorationsegmentamplitude,
  segment length/.code={\pgfmathsetlength\pgfdecorationsegmentlength{#1}},
  meta-segment length/.store in=\pgfmetadecorationsegmentlength,
  angle/.code={\pgfmathparse{#1}\let\pgfdecorationsegmentangle\pgfmathresult},
  aspect/.code={\pgfmathparse{#1}\let\pgfdecorationsegmentaspect\pgfmathresult},
  start radius/.initial=2.5pt,
  end radius/.initial=2.5pt,
  radius/.style={start radius=#1,end radius=#1},
  path has corners/.is if=pgfdecoratepathhascorners,
  reverse path/.is if=pgf@decorate@inputsegmentobjects@reverse,
}%
\newif\ifpgfdecoratepathhascorners
\newif\ifpgf@decorate@inputsegmentobjects@reverse

% Declare a decoration
%
% #1 = name of the decoration
% #2 = initial state
% #3 = states
%
% This command declares a new decoration for later use.
% Inside the code of #3 the command \state may be used. This command
% will only be defined while #3 is executed.
%
% Example:
%
% \pgfdeclaredecoration{zigzag}{q}
% {
%   \state{q}[width=10pt]
%   {
%     \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%     \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%     \pgfpathlineto{\pgfpoint{10pt}{0pt}}
%   }
%   \state{final}
%   {
%     \pgfpathlineto{\pgfpointdecoratedpathlast}
%   }
% }

\long\def\pgfdeclaredecoration#1#2#3{%
  \let\pgf@mod@dec@next=\pgf@mod@dec@firstofone%
  \pgfifmetadecoration{#1}{%
    \pgferror{You cannot declare a decoration of the same
      name as a meta-decoration}%
    \let\pgf@mod@dec@next=\pgfutil@gobble%
  }{}%
  \pgf@mod@dec@next
  {%
    \def\pgf@decorate@name{#1}%
    \pgfutil@namedef{pgf@decorate@@#1@initial}{#2}%
    \let\pgf@orig@state\state%
    \let\state\pgf@decorate@state
    #3%
    \let\state\pgf@orig@state%
  }%
}%

\def\pgf@decorate@state#1{\pgfutil@ifnextchar[{\pgf@decorate@@start#1}{\pgf@decorate@@start#1[]}}%}%
\def\pgf@decorate@@start#1[#2]#3{%
  \pgfutil@namedef{pgf@decorate@@\pgf@decorate@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@decorate@@\pgf@decorate@name @#1@code}{#3}%
}%
\long\def\pgf@mod@dec@firstofone#1{#1}%


% Test whether something is a decoration
%
% #1 = name
% #2 = if-code
% #3 = else-code
%
% Example:
%
% \pgfifdecoration{zigzag}{Exists}{Does not exist}

\def\pgfifdecoration#1#2#3{\pgfutil@ifundefined{pgf@decorate@@#1@initial}{#3}{#2}}%



% Declare a meta decoration
%
% #1 = name of the meta decoration
% #2 = initial state
% #3 = states
%
% This command declares a new meta decoration for later use.
% Inside the code of #3 the command \state may be used.

\long\def\pgfdeclaremetadecoration#1#2#3{%
  \let\pgf@mod@dec@next=\pgf@mod@dec@firstofone%
  \pgfifdecoration{#1}{%
    \pgferror{You cannot declare a meta-decoration of the
      same name as a decoration}%
    \let\pgf@mod@dec@next=\pgfutil@gobble%
  }{}%
  \pgf@mod@dec@next{%
    \def\pgf@metadecoration@name{#1}%
    \pgfutil@namedef{pgf@metadecoration@@#1@initial}{#2}%
    \let\pgf@orig@state\state%
    \let\state\pgf@metadecoration@state
    #3%
    \let\state\pgf@orig@state%
  }%
}%

\def\pgf@metadecoration@state#1{\pgfutil@ifnextchar[{\pgf@metadecoration@@state#1}{\pgf@metadecoration@@state#1[]}}%}%
\def\pgf@metadecoration@@state#1[#2]#3{%
  \pgfutil@namedef{pgf@metadecoration@@\pgf@metadecoration@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@metadecoration@@\pgf@metadecoration@name @#1@code}{#3}%
}%


% Test whether something is a meta-decoration
%
% #1 = name
% #2 = if-code
% #3 = else-code
%
% Example:
%
% \pgfifmetadecoration{zigzag}{Exists}{Does not exist}

\def\pgfifmetadecoration#1#2#3{\pgfutil@ifundefined{pgf@metadecoration@@#1@initial}{#3}{#2}}%





\let\pgfdecoratebeforecode\pgfutil@empty
\let\pgfdecorateaftercode\pgfutil@empty

% \pgfdecoratepath
%
% Decorate a path.
%
% \pgfdecoratebeforecode and \pgfdecorateaftercode can be used to
% execute code before and after the decoration.
%
% #1 - the name of the decoration.
% #2 - a (non-empty) path specification.
%
% Example:
%
%  \pgfdeclaredecoration{circles}{red circles}{
%    \state{red circles}[width=10pt, repeat state=2, next state=blue circles]
%    {
%      \pgfmathparse{round(rnd*100)}
%      \pgfsetstrokecolor{red!\pgfmathresult!brown}
%      \pgfsetfillcolor{orange!\pgfmathresult!yellow}
%      \pgfpathcircle{\pgfpointorigin}{2.5pt}
%      \pgfusepath{stroke,fill}
%    }
%    \state{blue circles}[width=10pt, repeat state=1, next state=red circles]
%    {
%      \pgfmathparse{round(rnd*100)}
%      \pgfsetstrokecolor{blue!\pgfmathresult!gray}
%      \pgfsetfillcolor{blue!\pgfmathresult!white}
%      \pgfpathcircle{\pgfpointorigin}{2.5pt}
%      \pgfusepath{stroke,fill}
%    }
%    \state{final}{}
%  }
%
%  \pgfpicture
%    \pgfdecoratepath{circles}
%    {
%      \pgfpathmoveto{\pgfpointorigin}
%      \pgfpathcurveto{\pgfpoint{0cm}{3cm}}{\pgfpoint{4cm}{0cm}}{\pgfpoint{4cm}{3cm}}
%    }
%  \endpgfpicture
%
\long\def\pgfdecoratepath#1#2{%
  \pgfdecoration{{#1}{\pgfdecoratedpathlength}{\pgfdecoratebeforecode}{\pgfdecorateaftercode}}%
  #2%
  \endpgfdecoration}%




% \pgfdecoratecurrentpath
%
% Decorate the current/existing path, but (unavoidably) destroys it.
%
% \pgfdecoratebeforecode and \pgfdecorateaftercode can be used to
% execute code before and after the decoration.
%
% #1 - the name of the decoration.
%
% Example:
%
%  \pgfdeclaredecoration{stars}{move}{
%    \state{move}[width=7.5pt, next state=star]{}
%    \state{star}[width=7.5pt, next state=move]
%    {
%      \pgfmathparse{round(rnd*100)}
%      \pgfsetfillcolor{yellow!\pgfmathresult!orange}
%      \pgfsetstrokecolor{yellow!\pgfmathresult!red}
%      \pgfmathparse{rnd*.75+.25}
%      \pgftransformscale{\pgfmathresult}
%      \pgfnode{star}{center}{}{}{\pgfusepath{stroke,fill}}
%    }
%    \state{final}
%    {
%      \pgfpathmoveto{\pgfpointdecoratedpathlast}
%    }
%  }
%
%  \pgfpicture
%    \pgfpathmoveto{\pgfpointorigin}
%    \pgfpathcurveto{\pgfqpoint{0cm}{2cm}}{\pgfqpoint{3cm}{2cm}}{\pgfqpoint{3cm}{0cm}}
%    \pgfpathcurveto{\pgfqpoint{3cm}{-3cm}}{\pgfqpoint{0cm}{0cm}}{\pgfqpoint{0cm}{-3cm}}
%    \pgfpathcurveto{\pgfqpoint{0cm}{-5cm}}{\pgfqpoint{3cm}{-5cm}}{\pgfqpoint{3cm}{-3cm}}
%    \pgfdecoratecurrentpath{stars}
%  \endpgfpicture
%
\def\pgfdecoratecurrentpath#1{%
  \pgfgetpath\pgf@decorate@currentpath%
  \pgfsetpath\pgfutil@empty%
  \pgfdecoration{{#1}{\pgfdecoratedpathlength}{\pgfdecoratebeforecode}{\pgfdecorateaftercode}}%
    \pgfsetpath\pgf@decorate@currentpath%
  \endpgfdecoration}%




% Environment \pgfdecoration \endpgfdecoration
%
% Decorates a path with multiple decorations.
%
% Definitions:
%
% `existing path'
%    - any unused path existing prior to the environment.
%
% `decorated path'
%   - the path that is being decorated.
%
%  `decoration path'
%    - any unused path left by the decoration automaton.
%
% The action of the environment is as follows:
%
%  1. Any existing path is saved.
%  2. Construction commands are executed forming the decorated path.
%  3. If the first command in the decorated path is not a `move to',
%     the last known position from the existing path is inserted.
%  4. The saved existing path is reinstalled.
%  5. The decoration automaton is executed along the decorated path.
%
% Parameters:
%
% #1 - a comma separated list of decoration specifications.
%
% A decoration specification takes the format:
%
% {<name>}{<distance>}{<before code>}{<after code>}
%
% The decoration <name> is applied to a section of the decorated
% path from the last point on the decorated path the decoration
% automaton reached to <distance> from that point.
%
% When <distance>} is parsed, the dimension
% \pgfdecoratedreminingdistance holds the distance remaining on the
% entire decorated path, and the macro \pgfdecoratedpathlength holds
% the total length of the entire decorated path.
% After <distance> is parsed, both are set to to the value of
% <distance> for the automaton to decorate current section of the
% decorated path.
%
% <before code> is executed just before the decoration automaton
% starts and <after code> is executed just after the automaton stops.
% If <before code> or <after code> are empty, they can be omitted.
% The macros \pgfdecoratedpathfirst and \pgfdecoratedpathlast
% will be set up as the first and last points on the current section
% of the decorated path.
%
% When the environment exits, the following macros will be set up:
%
%  \pgfdecorateexistingpath
%    - the existing path.
%
%  \pgfdecoratedpath
%    - the decorated path.
%
%  \pgfdecorationpath
%    - any unused decoration path.
%
%  \pgfpointdecoratedpathlast
%   - the last point on the decorated path.
%
% Examples (require pgfdecorations library):
%
%  \pgfpicture
%  \pgfdecoration
%    {
%      {lineto}{\pgfdecoratedpathlength/3},
%      {zigzag}{\pgfdecoratedpathlength/3},
%      {lineto}{\pgfdecoratedpathlength/3}
%    }
%    \pgfpathmoveto{\pgfpointorigin}
%    \pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%  \endpgfdecoration
%  \pgfusepath{stroke}
%  \endpgfpicture
%
%
%  \pgfpicture
%  \pgfdecoration
%    {
%      {lineto}{\pgfdecoratedpathlength/5}{}{\pgfusepath{stroke}},
%      {zigzag}{\pgfdecoratedpathlength/5}
%        {
%          \pgfpathmoveto{\pgfpointdecoratedpathfirst}
%        }
%        {
%          \pgfsetstrokecolor{red}
%          \pgfusepath{stroke}
%        },
%      {lineto}{\pgfdecoratedpathlength/5}
%        {
%          \pgfpathmoveto{\pgfpointdecoratedpathfirst}
%        }
%        {
%          \pgfsetstrokecolor{black}
%          \pgfusepath{stroke}
%        },
%      {zigzag}{\pgfdecoratedpathlength/5}
%        {
%          \pgfpathmoveto{\pgfpointdecoratedpathfirst}
%        }
%        {
%          \pgfsetstrokecolor{red}
%          \pgfusepath{stroke}
%        },
%      {lineto}{\pgfdecoratedpathlength/5}
%        {
%          \pgfpathmoveto{\pgfpointdecoratedpathfirst}
%        }
%        {
%          \pgfsetstrokecolor{black}
%          \pgfusepath{stroke}
%        }
%    }
%    \pgfpathmoveto{\pgfpointorigin}
%    \pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%  \endpgfdecoration
%
%  \endpgfpicture
%
%
%
%  \pgfdeclaredecoration{polygons}{move}{
%    \state{move}[width=7.5pt, next state=polygon]{}
%    \state{polygon}[width=7.5pt, next state=move]
%    {
%      \pgfmathparse{round(rnd*100)}
%      \pgfsetfillcolor{green!\pgfmathresult!yellow}
%      \pgfsetstrokecolor{green!\pgfmathresult!brown}
%      \pgfnode{regular polygon}{center}{}{}{\pgfusepath{stroke,fill}}
%    }
%    \state{final}
%    {
%      \pgfpathmoveto{\pgfpointdecoratedpathlast}
%    }
%  }
%
%  \pgfpicture
%  \pgfdecoration
%    {
%      {polygons}{45pt},
%      {lineto}{30pt}
%        {\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%        {
%          \pgfsetstrokecolor{yellow!50!orange}
%          \pgfusepath{stroke}
%        },
%      {polygons}{45pt},
%      {lineto}{30pt}
%        {\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%        {
%          \pgfsetstrokecolor{green!50!blue}
%          \pgfusepath{stroke}
%        },
%      {polygons}{\pgfdecoratedremainingdistance}
%    }
%    \pgfpathmoveto{\pgfpointorigin}
%    \pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%  \endpgfdecoration
%  \endpgfpicture
%
%
%  \pgfpicture
%    \pgfpathmoveto{\pgfpointorigin}
%    \pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%    \pgfgetpath\temppath
%    \pgfsetstrokecolor{red}
%    \pgfusepath{stroke}
%
%    \pgfset{decoration text={Here is some text all the way along this curve!}}
%    \pgfdecoration{{text}{\pgfdecoratedremainingdistance}}
%      \pgfsetpath\temppath
%    \endpgfdecoration
%  \endpgfpicture
%
\def\pgfdecoration#1{%
  \begingroup%
    \def\pgf@decorate@decorationlist{#1}%
    \pgf@decoration@env%
}%

\def\endpgfdecoration{%
    \pgf@decoration@endenv%
    \ifx\pgfdecoratedpath\pgfutil@empty%
    \else%
      %
      % Perform the decoration(s).
      %
      \pgf@decorate@for\pgf@temp:=\pgf@decorate@decorationlist\do{%
        \ifx\pgf@temp\pgfutil@empty%
        \else%
          \expandafter\pgf@decorate@invoke\expandafter{\pgf@temp}%
        \fi%
      }%
    \fi%
    \pgfgetpath\pgfdecorationpath%
    %
    % Take stuff outside the group.
    %
    \global\let\pgf@decorate@decorationpathtemp\pgfdecorationpath%
    \global\let\pgf@decorate@decoratedpathtemp\pgfdecoratedpath%
    \global\let\pgf@decorate@existingpathtemp\pgfdecorateexistingpath%
    \global\let\pgfpoint@decorated@pathlasttemp\pgfpoint@decorated@pathlast%
  \endgroup%
  %
  % Are we in LaTeX?
  %
  \pgfutil@ifnextchar\@checkend{\aftergroup\pgf@decorate@installmacrosatend}%
  {\pgf@decorate@installmacrosatend}%
}%



% Environment \pgfmetadecoration \endpgfmetadecoration
%
% Decorate a path with decoration automatons!
%
% Example:
%
%  \pgfdeclaremetadecoration{fancy line}{line to}{
%    \state{line to}[width=1cm, next state=zigzag]
%    {
%      \decoration{lineto}
%      \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%      \afterdecoration
%      {
%        \pgfsetstrokecolor{black}
%        \pgfusepath{stroke}
%      }
%    }
%    \state{zigzag}[width=2cm, next state=line to]
%    {
%      \decoration{zigzag}
%      \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%      \afterdecoration
%      {
%        \pgfsetstrokecolor{red}
%        \pgfusepath{stroke}
%      }
%    }
%    \state{final}
%    {
%      \decoration{lineto}
%      \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%      \afterdecoration
%      {
%        \pgfsetstrokecolor{black}
%        \pgfusepath{stroke}
%      }
%    }
%  }
%
%  \pgfpicture
%    \pgfmetadecoration{fancy line}
%      \pgfpathmoveto{\pgfpointorigin}
%      \pgfpathcurveto{\pgfqpoint{0cm}{2cm}}{\pgfqpoint{3cm}{2cm}}{\pgfqpoint{3cm}{0cm}}
%      \pgfpathcurveto{\pgfqpoint{3cm}{-3cm}}{\pgfqpoint{0cm}{0cm}}{\pgfqpoint{0cm}{-3cm}}
%      \pgfpathcurveto{\pgfqpoint{0cm}{-5cm}}{\pgfqpoint{3cm}{-5cm}}{\pgfqpoint{3cm}{-3cm}}
%    \endpgfmetadecoration
%  \endpgfpicture
%
\def\pgfmetadecoration#1{%
  \begingroup%
    \let\decoration\pgf@metadecoration@decoration%
    \let\beforedecoration\pgf@metadecoration@beforedecoration%
    \let\afterdecoration\pgf@metadecoration@afterdecoration%
    \def\pgf@metadecoration@name{#1}%
    \pgf@decoration@env%
}%

\def\endpgfmetadecoration{%
    \pgf@decoration@endenv%
    \ifx\pgfdecoratedpath\pgfutil@empty%
    \else%
      \let\pgfmetadecoratedpathlength\pgf@decorate@totalpathlength%
      \def\pgfmetadecoratedinputsegmentremainingdistance{\pgfdecoratedremainingdistance}%
      \def\pgfmetadecoratedinputsegmentcompleteddistance{\pgfdecoratedcompleteddistance}%
      %
      % Perform the meta decoration...
      %
      \expandafter\let\expandafter\pgf@metadecoration@current@state%
      \csname pgf@metadecoration@@\pgf@metadecoration@name @initial\endcsname%
      \pgf@metadecoration@run%
      %
      % ..until the final state.
      %
      \let\pgf@decorate@tempname\pgfutil@empty%
      \let\pgf@decorate@tempbefore\pgfutil@empty%
      \let\pgf@decorate@tempafter\pgfutil@empty%
      \csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @code\endcsname%
      \ifx\pgf@decorate@tempname\pgfutil@empty%
        \def\pgf@decorate@tempname{moveto}
      \fi%
      \pgf@decorate@invoke{%
        {\pgf@decorate@tempname}{\pgfdecoratedremainingdistance}%
        {\pgf@decorate@tempbefore}{\pgf@decorate@tempafter}%
      }%
    \fi%
    \pgfgetpath\pgfdecorationpath%
    %
    % Take stuff outside the group.
    %
     \global\let\pgf@decorate@decorationpathtemp\pgfdecorationpath%
    \global\let\pgf@decorate@decoratedpathtemp\pgfdecoratedpath%
    \global\let\pgf@decorate@existingpathtemp\pgfdecorateexistingpath%
    \global\let\pgfpoint@decorated@pathlasttemp\pgfpoint@decorated@pathlast%
  \endgroup%
  %
  % Are we in LaTeX?
  %
  \pgfutil@ifnextchar\@checkend{\aftergroup\pgf@decorate@installmacrosatend}%
    {\pgf@decorate@installmacrosatend}%
}%






% Internal macro for the decoration environment.
%
\def\pgf@decoration@env{%
  \pgfgetpath\pgfdecorateexistingpath%
  \pgfsetpath\pgfutil@empty%
  \let\pgfdecorationpath\pgfutil@empty%
  \let\pgfdecoratedpath\pgfutil@empty%
  \let\pgfpoint@decorated@pathlast\pgfpointorigin%
  \edef\pgfpoint@decorate@existingpathlast{\pgf@x\the\pgf@path@lastx\pgf@y\the\pgf@path@lasty}%
  %
  % Begin a group so transformations don't mess things up.
  %
  \bgroup%
}%

\def\pgf@decorate@path@check@moveto#1{%
  \expandafter\pgf@decorate@path@@check@moveto#1\pgf@decorate@stop\pgf@decorate@@stop}%

\def\pgf@decorate@token@stop{\pgf@decorate@stop}%
\def\pgf@decorate@path@@check@moveto#1#2#3#4\pgf@decorate@@stop#5#6{%
  \def\pgf@decorate@temp{#4}%
  \pgf@x=#2\relax%
  \pgf@y=#3\relax%
  \ifx\pgf@decorate@temp\pgf@decorate@token@stop%
    #5%
  \else%
    #6%
  \fi%
}%

\def\pgf@decoration@endenv{%
  \egroup%
  \pgftransformreset%
  %
  % Save the existing soft path and restore the existing path.
  %
  \pgfgetpath\pgfdecoratedpath%
  \pgfsetpath\pgfdecorateexistingpath%
  %
  \ifx\pgfdecoratedpath\pgfutil@empty%
    \pgferror{I cannot decorate an empty path}%
  \else%
    %
    % If the path consists of a single moveto token, make it
    % a very small horizontal line.
    %
    \pgf@decorate@path@check@moveto\pgfdecoratedpath{%
      \advance\pgf@x by0.0001pt\relax%
      \edef\pgfdecoratedpath{%
        \expandafter\noexpand\pgfdecoratedpath%
        \noexpand\pgfsyssoftpath@linetotoken{\the\pgf@x}{\the\pgf@y}%
      }%
    }%
    {}%
    %
    % Remove special round tokens and get points.
    %
    \pgfprocessround{\pgfdecoratedpath}{\pgfdecoratedpath}%
    %
    % Parse the soft path into a series of decorated input segment objects.
    %
    \pgf@decorate@parsesoftpath{\pgfdecoratedpath}{\pgf@decorate@inputsegmentobjects}%
    %
    % Setup further options
    %
    \pgfkeys{/pgf/every decoration/.try}%
    %
    % Reverse objects if necessary.
    %
    \ifpgf@decorate@inputsegmentobjects@reverse%
      \pgf@decorate@inputsegmentobjects@reverse{\pgf@decorate@inputsegmentobjects}{\pgf@decorate@inputsegmentobjects}%
    \fi%
    %
    \let\pgf@decorated@remainingdistance\pgf@decorate@totalpathlength%
    %
    \let\pgfpoint@decorated@totalpathfirst\pgfpoint@decorated@firstparsed%
    \let\pgfpoint@decorated@totalpathlast\pgfpoint@decorate@lastnonmovetoparsed%
    %
    \let\pgfpoint@decorated@pathfirst\pgfpoint@decorated@totalpathfirst
    \let\pgfpoint@decorated@pathlast\pgfpoint@decorated@totalpathlast%
    %
    % Set up the first input segment.
    %
    \let\pgf@decorate@currentinputsegmentobjects\pgf@decorate@inputsegmentobjects%
    \let\pgf@decorate@transformtoinputsegment\pgfutil@empty%
    \pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
    \pgf@decorate@processnextinputsegmentobject%
    \pgf@decorate@distancetomove0pt\relax%
  \fi%
}%




\def\pgf@decorate@installmacrosatend{%
  \let\pgfdecorationpath\pgf@decorate@decorationpathtemp%
  \let\pgfdecoratedpath\pgf@decorate@decoratedpathtemp%
  \let\pgfdecorateexistingpath\pgf@decorate@existingpathtemp%
  \let\pgfpoint@decorated@pathlast\pgfpoint@decorated@pathlasttemp%
}%

\let\pgfdecorationpath\pgfutil@empty
\let\pgfdecoratedpath\pgfutil@empty
\let\pgfdecorateexisitingpath\pgfutil@empty

\let\pgfpoint@decorated@pathlast\pgfpointorigin



% A version of \pgfutil@for which doesn't expand each value in #3.
%
\def\pgf@decorate@for#1:=#2\do#3{%
  \def\pgf@decorate@for@var{#1}%
  \def\pgf@decorate@for@action{#3}%
  \expandafter\pgf@decorate@@for#2,\pgf@stop,}%

\def\pgf@decorate@@for#1,{%
  \ifx#1\pgf@stop%
    \expandafter\let\pgf@decorate@for@var\pgfutil@empty%
  \else%
    \expandafter\def\pgf@decorate@for@var{#1}%
    \pgf@decorate@for@action%
    \expandafter\pgf@decorate@@for%
  \fi%
}%


% Invoke a decoration.
%
% #1 - {<name>}{<distance>}{<before code>}{<after code>}
%
\def\pgf@decorate@invoke#1{%
  \pgf@decorate@@invoke#1\pgf@decorate@invoke\pgf@decorate@invoke\pgf@decorate@invoke\pgf@stop}%

\def\pgf@decorate@@invoke#1#2#3#4#5\pgf@stop{%
  \pgfutil@ifundefined{pgf@decorate@@#1@initial}%
  {%
    \pgferror{Unknown decoration `#1'}%
  }%
  {%
    \def\pgf@decorate@name{#1}%
    \ifx\pgf@decorate@invoke#3%
      \let\pgf@decorate@beforecode\pgfutil@empty%
    \else%
      \def\pgf@decorate@beforecode{#3}%
    \fi%
    \ifx\pgf@decorate@invoke#4%
      \let\pgf@decorate@aftercode\pgfutil@empty%
    \else%
      \def\pgf@decorate@aftercode{#4}%
    \fi%
    %
    % Make remaining distance and the decorated path length `public'.
    %
    \pgfdecoratedremainingdistance\pgf@decorated@remainingdistance\relax%
    \let\pgfdecoratedpathlength\pgf@decorate@totalpathlength%
    %
    \pgfmathsetlength\pgf@xa{#2}%
    \ifdim\pgf@xa>\pgf@decorated@remainingdistance\relax%
      \pgf@xa\pgf@decorated@remainingdistance\relax%
    \fi%
    \edef\pgf@decorate@currentpathlength{\the\pgf@xa}%
    %
    % Calculate the distance remaining to the end of the entire path.
    %
    \pgf@xa-\pgf@decorate@currentpathlength\relax%
    \advance\pgf@xa\pgf@decorated@remainingdistance\relax%
    \edef\pgf@decorated@remainingdistance{\the\pgf@xa}%
    %
    % Set up the macros and distances for the current section
    % of the decorated path.
    %
    \let\pgfdecoratedpathlength\pgf@decorate@currentpathlength%
    \pgfdecoratedremainingdistance\pgfdecoratedpathlength\relax%
    \pgfdecoratedcompleteddistance0pt\relax%
    %
    % Execute user-defined code beore decoration.
    %
    \pgf@decorate@beforecode%
    %
    % Run the decoration...
    %
    \expandafter\let\expandafter\pgf@decorate@current@state%
      \csname pgf@decorate@@\pgf@decorate@name @initial\endcsname%
    \pgf@decorate@run%
    %
    % ...until the final state.
    %
    \ifdim\pgf@decorated@remainingdistance<1pt\relax% Should be =0pt, but need to control for inaccuracies.
      \let\pgfpoint@decorated@pathlast\pgfpoint@decorated@totalpathlast%
    \else%
      %
      % Set up \pgfpoint@decorated@pathlast if the end of
      % the total decorated path has not been reached.
      %
      {%
        \pgf@decorate@movealonginputsegment{\the\pgfdecoratedremainingdistance}%
        \pgf@decorate@transformtoinputsegment%
        \pgfpointorigin%
        \pgf@pos@transform@glob%
        \global\pgf@x\pgf@x%
        \global\pgf@y\pgf@y%
      }%
      \edef\pgfpoint@decorated@pathlast{\pgf@x\the\pgf@x\pgf@y\the\pgf@y}%
    \fi%
    {%
      \pgftransformreset%
      \pgf@decorate@transformtoinputsegment%
      \pgf@decorate@additionaltransform%
      \csname pgf@decorate@@\pgf@decorate@name @final@code\endcsname%
    }%
    \pgf@decorate@movealonginputsegment{\the\pgfdecoratedremainingdistance}%
    %
    % Execute user-defined code after decoration.
    %
    \pgf@decorate@aftercode%
    %
    % Update the input segment objects.
    %
    \let\pgf@decorate@additionaltransform\pgfutil@empty%
    \let\pgf@decorate@inputsegmentobjects\pgf@decorate@inputsegmentobjects@aftersplit%
    \let\pgfpoint@decorated@pathfirst\pgfpoint@decorated@pathlast%
   }%
}%



\let\pgf@decorate@transformtoinputsegment\pgfutil@empty%
\let\pgf@decorate@additionaltransform\pgfutil@empty%


% \pgfpointdecoratedpathfirst
%
\def\pgfpointdecoratedpathfirst{%
  {%
    \pgftransforminvert%
    \pgfpoint@decorated@pathfirst%
    \pgf@pos@transform@glob%
    \global\pgf@x\pgf@x%
    \global\pgf@y\pgf@y%
  }%
}%

% \pgfpointdecoratedpathlast
%
\def\pgfpointdecoratedpathlast{%
  {%
    \pgftransforminvert%
    \pgfpoint@decorated@pathlast%
    \pgf@pos@transform@glob%
    \global\pgf@x\pgf@x%
    \global\pgf@y\pgf@y%
  }%
}%

% \pgfpointdecoratedinputsegmentfirst
%
% The first point of the current sub-path.
%
\def\pgfpointdecoratedinputsegmentfirst{%
  {%
    \pgftransforminvert%
    \pgf@decorate@inputsegment@first%
    \pgf@pos@transform@glob%
    \global\pgf@x\pgf@x%
    \global\pgf@y\pgf@y%
  }%
}%

% \pgfpointdecoratedinputsegmentlast
%
% The final point of the current sub-path.
%
\def\pgfpointdecoratedinputsegmentlast{%
  {%
    \pgftransforminvert%
    \pgf@decorate@inputsegment@last%
    \pgf@pos@transform@glob%
    \global\pgf@x\pgf@x%
    \global\pgf@y\pgf@y%
  }%
}%


\def\pgf@final@text{final}%

% Run a normal decoration.
%
\def\pgf@decorate@run{%
  \let\pgf@decorate@next\pgf@decorate@do@state%
  \ifx\pgf@decorate@current@state\pgf@final@text%
    \let\pgf@decorate@next\relax%
  \fi%
  \pgf@decorate@next%
}%

\def\pgf@decorate@do@state{%
  \let\pgf@decorate@next\relax%
  \let\pgf@decorate@next@state\pgf@decorate@current@state%
  %
  % Get the options.
  %
  \let\pgf@decorate@persistent@pre=\relax%
  \let\pgf@decorate@persistent@post=\relax%
  \expandafter\expandafter\expandafter\pgf@decorate@setter
  \expandafter\expandafter\expandafter{\csname pgf@decorate@@\pgf@decorate@name @\pgf@decorate@current@state @options\endcsname}%
  \ifx\pgf@decorate@next\relax%
    \let\pgf@decorate@next\pgf@decorate@do@code%
  \fi%
  \pgf@decorate@next%
}%

\def\pgf@decorate@setter{\pgfqkeys{/pgf/decoration automaton}}%

\pgf@decorate@repeatstate-1\relax

\def\pgf@decorate@do@code{%
  %
  % Execute code.
  %
  \pgf@decorate@persistent@pre%
  {%
    \pgftransformreset%
    \pgf@decorate@transformtoinputsegment%
    \pgf@decorate@additionaltransform%
    \csname pgf@decorate@@\pgf@decorate@name @\pgf@decorate@current@state @code\endcsname%
  }%
  \pgf@decorate@persistent@post%
  \pgf@decorate@movealongpath{\pgf@decorate@width}%
  %
  % Next iteration.
  %
  \ifnum\pgf@decorate@repeatstate>0\relax%
    \advance\pgf@decorate@repeatstate-1\relax%
  \else%
    \pgf@decorate@repeatstate-1\relax%
    \let\pgf@decorate@current@state\pgf@decorate@next@state%
  \fi%
  \pgf@decorate@run%
}%

\pgfkeys{
  /pgf/decoration automaton/width/.code=\def\pgf@decorate@width{#1}\pgf@decorate@switch@if#1 to final\pgf@stop,%
  /pgf/decoration automaton/switch if less than/.code=\pgf@decorate@switch@if#1\pgf@stop,%
  /pgf/decoration automaton/switch if input segment less than/.code=\pgf@decorate@switch@ifinputsegment#1\pgf@stop,%
  /pgf/decoration automaton/next state/.store in=\pgf@decorate@next@state,%
  /pgf/decoration automaton/persistent precomputation/.store in=\pgf@decorate@persistent@pre,%
  /pgf/decoration automaton/persistent postcomputation/.store in=\pgf@decorate@persistent@post,%
  /pgf/decoration automaton/repeat state/.code={%
    \ifnum\pgf@decorate@repeatstate=-1\relax%
      \pgfmathsetcount\pgf@decorate@repeatstate{#1}%
    \fi%
  },%
  /pgf/decoration automaton/if input segment is closepath/.code={%
    \ifpgf@decorate@is@closepath@%
      \pgfkeysalso{#1}%
    \fi%
  },
  /pgf/decoration automaton/auto end on length/.code=\pgf@decorate@auto@end{#1},
  /pgf/decoration automaton/auto corner on length/.code=\pgf@decorate@auto@corner{#1},
}%

\def\pgf@decorate@auto@end#1{%
  \ifx\pgf@decorate@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifpgf@decorate@is@closepath@%
      \ifdim\pgfdecoratedremainingdistance>\pgf@x%
        \ifdim\pgfdecoratedinputsegmentremainingdistance>\pgf@x%
        \else%
          \pgfpathclose%
          \pgf@decorate@movealongpath{\pgfdecoratedinputsegmentremainingdistance}%
          \pgf@decorate@repeatstate-1\relax%
          \let\pgf@decorate@next\pgf@decorate@run%
        \fi%
      \else%
        \pgfpathclose%
        \def\pgf@decorate@current@state{final}%
        \def\pgf@decorate@width{\pgfdecoratedremainingdistance}
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \else%
      \ifdim\pgfdecoratedremainingdistance>\pgf@x%
      \else%
        {%
          \pgftransformreset%
          \pgf@decorate@transformtoinputsegment%
          \pgf@decorate@additionaltransform%
          \pgfpathlineto{\pgfpoint{\pgfdecoratedremainingdistance}{0pt}}
        }%
        \def\pgf@decorate@current@state{final}%
        \def\pgf@decorate@width{\pgfdecoratedremainingdistance}
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}%

\def\pgf@decorate@auto@corner#1{%
  \ifpgfdecoratepathhascorners%
    \ifx\pgf@decorate@next\relax%
      \pgfmathsetlength\pgf@x{#1}%
      \ifdim\pgfdecoratedinputsegmentremainingdistance>\pgf@x%
      \else%
        {%
          \pgftransformreset%
          \pgf@decorate@transformtoinputsegment%
          \pgf@decorate@additionaltransform%
          \pgfpathlineto{\pgfqpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
        }%
        \pgf@decorate@movealongpath{\pgfdecoratedinputsegmentremainingdistance}%
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}%

\def\pgf@decorate@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@decorate@next\relax%
    \ifdim\pgfdecoratedremainingdistance=0pt\relax%
      \def\pgf@decorate@current@state{#2}%
      \pgf@decorate@repeatstate-1\relax%
      \let\pgf@decorate@next\pgf@decorate@run%
    \else%
      \pgfmathsetlength\pgf@x{#1}%
      \ifdim\pgfdecoratedremainingdistance<\pgf@x%
        \def\pgf@decorate@current@state{#2}%
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}%

\def\pgf@decorate@switch@ifinputsegment#1to #2\pgf@stop{%
  \ifx\pgf@decorate@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfdecoratedinputsegmentremainingdistance<\pgf@x%
      \def\pgf@decorate@current@state{#2}%
      \pgf@decorate@repeatstate-1\relax%
      \let\pgf@decorate@next\pgf@decorate@run%
    \fi%
  \fi%
}%




% \pgfsetdecorationsegmenttransformation
%
% Set the additional transform for each decoration state.
%
% Example:
%
% \pgfsetdecorationsegmenttransformation{\pgftransformyshift{5pt}}
%
\def\pgfsetdecorationsegmenttransformation#1{\def\pgf@decorate@additionaltransform{#1}}%
\let\pgf@decorate@additionaltransform\pgfutil@empty%




\def\pgf@metadecoration@decoration#1{%
  \edef\pgf@decorate@tempname{#1}%
}%
\def\pgf@metadecoration@beforedecoration#1{%
  \def\pgf@decorate@tempbefore{#1}%
}%
\def\pgf@metadecoration@afterdecoration#1{%
  \def\pgf@decorate@tempafter{#1}%
}%


\def\pgf@final@text{final}%

% Run a meta decoration.
%
\def\pgf@metadecoration@run{%
  \let\pgf@metadecoration@next\pgf@metadecoration@do@state%
  \ifx\pgf@metadecoration@current@state\pgf@final@text%
    \let\pgf@metadecoration@next\relax%
  \fi%
  \pgf@metadecoration@next%
}%

\def\pgf@metadecoration@do@state{%
  \let\pgf@metadecoration@next\relax%
  \let\pgf@metadecoration@next@state\pgf@metadecoration@current@state%
  %
  % Set up some macros.
  %
  \let\pgfmetadecoratedremainingdistance\pgf@decorated@remainingdistance%
  \pgf@x-\pgfmetadecoratedremainingdistance\relax%
  \advance\pgf@x\pgf@decorate@totalpathlength\relax%
  \edef\pgfmetadecoratedcompleteddistance{\the\pgf@x}%
  %
  % Get the options.
  %
  \expandafter\expandafter\expandafter\pgf@metadecoration@setter
  \expandafter\expandafter\expandafter{\csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @options\endcsname}%
  \ifx\pgf@metadecoration@next\relax%
    \let\pgf@metadecoration@next\pgf@metadecoration@do@code%
  \fi%
  \pgf@metadecoration@next%
}%

\def\pgf@metadecoration@do@code{%
  %
  % Execute code.
  %
  \let\pgf@decorate@tempname\pgfutil@empty%
  \let\pgf@decorate@tempbefore\pgfutil@empty%
  \let\pgf@decorate@tempafter\pgfutil@empty%
  \let\pgfpointmetadecoratedpathfirst\pgfpointdecoratedpathfirst%
  \let\pgfpointmetadecoratedpathlast\pgfpointdecoratedpathlast%
  \csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @code\endcsname%
  \ifx\pgf@decorate@tempname\pgfutil@empty%
    \def\pgf@decorate@tempname{moveto}
  \fi%
  \pgf@decorate@invoke{%
    {\pgf@decorate@tempname}{\pgf@metadecoration@width}%
    {\pgf@decorate@tempbefore}{\pgf@decorate@tempafter}%
  }%
  %
  % Next iteration.
  %
  \let\pgf@metadecoration@current@state\pgf@metadecoration@next@state%
  \pgf@metadecoration@run%
}%

\def\pgf@metadecoration@setter{\pgfqkeys{/pgf/meta-decoration automaton}}%

\pgfkeys{
  /pgf/meta-decoration automaton/width/.code=\def\pgf@metadecoration@width{#1}\pgf@metadecoration@switch@if#1 to final\pgf@stop,%
  /pgf/meta-decoration automaton/switch if less than/.code=\pgf@metadecoration@switch@if#1\pgf@stop,%
  /pgf/meta-decoration automaton/switch if input segment less than/.code=\pgf@metadecoration@switch@ifinputsegment#1\pgf@stop,%
  /pgf/meta-decoration automaton/next state/.store in=\pgf@metadecoration@next@state,%
}%

\def\pgf@metadecoration@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@metadecoration@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgf@decorated@remainingdistance<\pgf@x%
      \def\pgf@metadecoration@current@state{#2}%
      \let\pgf@metadecoration@next\pgf@metadecoration@run%
    \fi%
  \fi%
}%

\def\pgf@metadecoration@switch@ifinputsegment#1to #2\pgf@stop{%
  \ifx\pgf@metadecoration@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfdecoratedinputsegmentremainingdistance<\pgf@x%
      \def\pgf@metadecoration@current@state{#2}%
      \let\pgf@metadecoration@next\pgf@metadecoration@run%
    \fi%
  \fi%
}%



% Move along the path by a specified distance.
%
\def\pgf@decorate@movealongpath#1{%
  \pgfmathsetlength\pgf@decorate@distancetomove{#1}%
  \advance\pgfdecoratedcompleteddistance\pgf@decorate@distancetomove%
  \advance\pgfdecoratedremainingdistance-\pgf@decorate@distancetomove%
  \pgf@decorate@@movealongpath%
}%
\def\pgf@decorate@@movealongpath{%
  \advance\pgfdecoratedinputsegmentcompleteddistance\pgf@decorate@distancetomove%
  \advance\pgfdecoratedinputsegmentremainingdistance-\pgf@decorate@distancetomove%
  \ifdim\pgfdecoratedinputsegmentremainingdistance>0pt\relax%
    \let\pgf@next\pgf@decorate@@@movealongpath%
  \else%
    \pgf@decorate@distancetomove-\pgfdecoratedinputsegmentremainingdistance%
    \pgf@decorate@processnextinputsegmentobject%
    \ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
      \pgfdecoratedremainingdistance0pt\relax%
      \let\pgf@next\relax%
    \else%
      \let\pgf@next\pgf@decorate@@movealongpath%
    \fi%
  \fi%
  \pgf@next%
}%

\def\pgf@decorate@@@movealongpath{%
  %
  % Move along input segment for real.
  %
  \pgf@decorate@movealonginputsegment{\the\pgf@decorate@distancetomove}%
  \pgf@decorate@distancetomove0pt\relax%
  %
  % Grrr. Hacking to control some inaccuracies.
  %
  \ifdim\pgf@decorate@inputsegmenttime pt>1pt\relax%
    \let\pgf@decorate@inputsegmenttimetemp\pgf@decorate@inputsegmenttime%
    \pgf@decorate@processnextinputsegmentobject%
    \pgf@x\pgf@decorate@inputsegmenttimetemp pt\relax%
    \advance\pgf@x-1pt\relax%
    \edef\pgf@decorate@inputsegmenttime{\pgfmath@tonumber{\pgf@x}}%
    \ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
      \pgfdecoratedremainingdistance0pt\relax%
    \fi%
  \fi%
}%

% Return the next input segment object in a macro
%
\def\pgf@decorate@getnextinputsegmentobject#1{%
  \ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
    \let\pgf@next\relax%
  \else%
    \def\pgf@decorate@temp{#1}%
    \let\pgf@next\pgf@decorate@@getnextinputsegmentobject%
  \fi%
  \pgf@next%
}%
\def\pgf@decorate@@getnextinputsegmentobject{%
  \expandafter\pgf@decorate@@@getnextinputsegmentobject\pgf@decorate@currentinputsegmentobjects\pgf@stop}%
\def\pgf@decorate@@@getnextinputsegmentobject#1#2\pgf@stop{%
  \expandafter\def\pgf@decorate@temp{#1}%
  \def\pgf@decorate@currentinputsegmentobjects{#2}}%

% Process the next input segment object.
%
\def\pgf@decorate@processnextinputsegmentobject{%
  \let\pgfdecorationpreviousinputsegment\pgfdecoratecurrentinputsegment%
  \let\pgf@decorate@currentinputsegmentobject\pgf@decorate@nextinputsegmentobject%
  \pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
  %
  % If the current input segment object is a moveto, execute the
  % object macro and get the next input segment object.
  %
  \pgf@decorate@is@closepath@false%
  \pgf@decorate@currentinputsegmentobject%
  \ifx\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentmoveto%
    \pgfpathmoveto{\pgf@decorate@inputsegment@first}%
    \let\pgfdecorationpreviousinputsegment\pgfdecorationcurrentinputsegment%
    \let\pgf@decorate@currentinputsegmentobject\pgf@decorate@nextinputsegmentobject%
    \pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
    \pgf@decorate@is@closepath@false%
    \pgf@decorate@currentinputsegmentobject%
  \fi%
  %
  % Teensy hack in case a path goes nowhere.
  %
  \ifdim\pgfdecoratedinputsegmentlength=0pt\relax%
    \def\pgfdecoratedinputsegmentlength{0.05pt}% Arbitrary choice >0pt.
  \fi%
  \pgfdecoratedinputsegmentremainingdistance\pgfdecoratedinputsegmentlength\relax%
  \pgfdecoratedinputsegmentcompleteddistance0pt\relax%
  \def\pgf@decorate@inputsegmenttime{0}%
  %
  % Get the angle at the start of the input segment.
  %
  \ifx\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentcurveto%
    \pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
    \let\pgfdecoratedangle\pgfmathresult%
    \let\pgfdecoratedinputsegmentstartangle\pgfmathresult%
    \pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
    \let\pgfdecoratedinputsegmentendangle\pgfmathresult%
  \else%
    \pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@last}%
    \let\pgfdecoratedangle\pgfmathresult%
    \let\pgfdecoratedinputsegmentstartangle\pgfmathresult%
    \let\pgfdecoratedinputsegmentendangle\pgfmathresult%
  \fi%
  %
  % Get the angle to the next input segment.
  %
  \begingroup%
    \pgf@decorate@nextinputsegmentobject%
    \global\let\pgf@decorate@temp\pgfdecorationcurrentinputsegment%
    \ifx\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentmoveto%
      \expandafter\pgf@decorate@currentinputsegmentobject%
    \fi%
    \ifx\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentcurveto%
      \pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
    \else%
      \pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@last}%
    \fi%
    \pgf@x-\pgfdecoratedangle pt\relax%
    \advance\pgf@x\pgfmathresult pt\relax%
    \edef\pgfdecoratedangletonextinputsegment{\the\pgf@x}%
    \pgfmath@smuggleone\pgfdecoratedangletonextinputsegment%
  \endgroup%
  \let\pgfdecorationnextinputsegmentobject\pgf@decorate@temp%
}%


%
% Input segment objects
%

\newif\ifpgf@decorate@is@closepath@%

% Input segment types.
%
% These allow comparison with \ifx using
%
% \pgfdecorationcurrentinputsegment
% \pgfdecorationnextinputsegment
% \pgfdecorationcurrentprevioussegment
%
\def\pgfdecorationinputsegmentmoveto{moveto}%
\def\pgfdecorationinputsegmentlineto{lineto}%
\def\pgfdecorationinputsegmentcurveto{curveto}%
\def\pgfdecorationinputsegmentclosepath{closepath}%
\def\pgfdecorationinputsegmentlast{last}%

% Input segment object moveto.
%
\def\pgf@decorate@inputsegmentobject@moveto#1{%
  \def\pgf@decorate@inputsegment@first{#1}%
  \def\pgf@decorate@inputsegment@supporta{#1}%
  \def\pgf@decorate@inputsegment@supportb{#1}%
  \def\pgf@decorate@inputsegment@last{#1}%
  \edef\pgf@decorate@lastmoveto{#1}%
  \def\pgfdecoratedinputsegmentlength{0pt}%
  \let\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentmoveto%
}%

% Input segment object lineto.
%
\def\pgf@decorate@inputsegmentobject@lineto#1#2#3{%
  \def\pgfdecoratedinputsegmentlength{#1}%
  \def\pgf@decorate@inputsegment@first{#2}%
  \def\pgf@decorate@inputsegment@last{#3}%
  %
  % Supports should be defined like this, so if treated as a curve,
  % equal time steps will correspond to equal distances.
  %
  \pgfpointdiff{#2}{#3}%
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
  \pgfextract@process\pgf@decorate@inputsegment@supporta{%
    \pgf@process{#2}%
    \advance\pgf@x0.333333\pgf@xa%
    \advance\pgf@y0.333333\pgf@ya%
  }%
  \pgfextract@process\pgf@decorate@inputsegment@supportb{%
    \pgf@process{#2}%
    \advance\pgf@x0.666666\pgf@xa%
    \advance\pgf@y0.666666\pgf@ya%
  }%
  \let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@line%
  \let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@line%
  \let\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentlineto%
}%

% Input segment object curveto.
%
\def\pgf@decorate@inputsegmentobject@curveto#1#2#3#4#5{%
  \def\pgfdecoratedinputsegmentlength{#1}%
  \def\pgf@decorate@inputsegment@first{#2}%
  \def\pgf@decorate@inputsegment@supporta{#3}%
  \def\pgf@decorate@inputsegment@supportb{#4}%
  \def\pgf@decorate@inputsegment@last{#5}%
  %
  \let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@curve%
  \let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@curve%
  \let\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentcurveto%
}%

% Input segment object closepath.
%
% Treated like a lineto, but flag that it is a closepath.
%
\def\pgf@decorate@inputsegmentobject@closepath#1#2#3{%
  \pgf@decorate@is@closepath@true%
  %
  \def\pgfdecoratedinputsegmentlength{#1}%
  \def\pgf@decorate@inputsegment@first{#2}%
  \def\pgf@decorate@inputsegment@last{#3}%
  %
  \pgfpointdiff{#2}{#3}%
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
  \pgfextract@process\pgf@decorate@inputsegment@supporta{%
    \pgf@process{#2}%
    \advance\pgf@x0.333333\pgf@xa%
    \advance\pgf@y0.333333\pgf@ya%
  }%
  \pgfextract@process\pgf@decorate@inputsegment@supportb{%
    \pgf@process{#2}%
    \advance\pgf@x0.666666\pgf@xa%
    \advance\pgf@y0.666666\pgf@ya%
  }%
  %
  \let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@line%
  \let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@line%
  \let\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentclosepath%
}%


% Input segment object endofinputsegments.
%
\def\pgf@decorate@inputsegmentobject@endofinputsegments{%
  \let\pgfdecorationcurrentinputsegment\pgfdecorationinputsegmentlast%
}%




% This macro controls how the automaton moves along a line sub-path
%
\def\pgf@decorate@movealonginputsegment@line#1{}% Nothing special needed.

% This macro controls how the automaton moves along a curve sub-path.
%
\def\pgf@decorate@movealonginputsegment@curve#1{%
  \ifdim#1=0pt\relax%
  \else%
    \pgfpointcurveattime{\pgf@decorate@inputsegmenttime}%
      {\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
      {\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@decorate@inputsegmenttime pt\relax%
    %
    % Reduce the initial time step, depending on the length
    % of the path. To do: Optimise this step (should also depend on #1).
    %
    \ifdim\pgf@decorate@currentpathlength<128pt\relax%
      \pgf@yb.03125pt\relax%
    \else%
      \ifdim\pgf@decorate@currentpathlength<512pt\relax%
        \pgf@yb.015625pt\relax%
      \else%
        \ifdim\pgf@decorate@currentpathlength<2048pt\relax%
          \pgf@yb.00390625pt\relax%
        \else%
          \pgf@yb.0009765625pt\relax%
        \fi%
      \fi%
    \fi%
    \c@pgf@counta1\relax%
    \pgfutil@tempdima0pt\relax%
    \pgfmathloop%
      \advance\pgf@xb\c@pgf@counta\pgf@yb%
      %
      % We would like to use \pgfpointcurveattime. However, we must not
      % overuse \pgf@process or \pgfmath stuff within this loop,
      % otherwise we increase the chances of save stack overflow.
      %
      \edef\pgf@decorate@temp{%
        \pgf@xa\the\pgf@xa%
        \pgf@xb\the\pgf@xb%
        \pgf@ya\the\pgf@ya%
        \pgf@yb\the\pgf@yb%
      }%
      %
      \pgfpoint@decorate@curveattime{\pgfmath@tonumber{\pgf@xb}}%
        {\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
        {\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
      \pgf@decorate@temp%
      %
      \pgf@xc\pgf@xa%
      \pgf@yc\pgf@ya%
      \pgf@xa\pgf@x%
      \pgf@ya\pgf@y%
      \advance\pgf@x-\pgf@xc%
      \advance\pgf@y-\pgf@yc%
      \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
      \pgfutil@tempdimb\pgfmathresult pt\relax%
      \advance\pgfutil@tempdima\c@pgf@counta\pgfutil@tempdimb%
      \ifnum\c@pgf@counta>0\relax%
        \ifdim\pgfutil@tempdima>#1\relax%
          \c@pgf@counta-\c@pgf@counta%
          \pgf@yb.5\pgf@yb%
        \fi%
      \else%
        \ifdim\pgfutil@tempdima<#1\relax%
          \c@pgf@counta-\c@pgf@counta%
          \pgf@yb.5\pgf@yb%
        \fi%
      \fi%
      \ifdim\pgf@yb=0pt\relax% *Should* be OK.
      \else%
    \repeatpgfmathloop%
    \edef\pgf@decorate@inputsegmenttime{\pgfmath@tonumber{\pgf@xb}}%
    %
    % Now calculate the angle at the new time on the curve.
    %
    % We can use \pgfpointcurveattime safely here.
    %
    \pgfpointcurveattime{\pgf@decorate@inputsegmenttime}%
      {\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
      {\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
    \edef\pgf@marshal{%
      \noexpand\pgfmathanglebetweenpoints%
        {\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}%
        {\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}%
    }%
    \pgf@marshal%
    \let\pgfdecoratedangle\pgfmathresult%
  \fi%
}%

% \pgfpoint@decorate@curveattime
%
% A `quick' version of \pgfpointcurveattime
%
% No parsing and no use of \pgf@process.
% This prevents save stack build up when used inside a loop.
%
\def\pgfpoint@decorate@curveattime#1#2#3#4#5{%
  \edef\pgf@time@s{#1}%
  \pgf@x-\pgf@time@s pt\relax%
  \advance\pgf@x1pt\relax%
  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
  #5\relax%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  #4\relax%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  #3\relax%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  #2\relax%
  % First iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
  % Second iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  % Save x/y
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Third iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
}%


% Applies the necessary transform for a line sub-path.
%
\def\pgf@decorate@transformtoinputsegment@line{%
  \pgftransformshift{%
    \pgfpointlineatdistance{\pgfdecoratedinputsegmentcompleteddistance}{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@last}
  }%
  \pgftransformrotate{\pgfdecoratedangle}%
}%

% Applies the necessary transform for a curve sub-path.
%
\def\pgf@decorate@transformtoinputsegment@curve{%
  \pgfslopedattimetrue%
  \pgfallowupsidedownattimetrue%
  \pgftransformcurveattime{\pgf@decorate@inputsegmenttime}%
    {\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
    {\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
}%





%  \pgf@decorate@parsesoftpath
%
%  Parses an instance of a soft path into intermediate line and curve
%  sub-path objects which the decoration automaton can use to traverse
% the decorated path.
%
%  The soft path should be well formed and only contain `primative'
%  soft path tokens, that is: moveto, lineto, curvetosupporta,
%  curvetosupportb, curveto, rectcorner, rectsize, and closepath.
%  (i.e., all specialround tokens should have removed using
%  \pgfprocessround)
%
%  The overall length of the path is also calculated and returned
%  in the macro \pgfdecoratedpathlength.
%
%  Parameters:
%
%  #1 - a macro containing a well formed soft path.
%  #2 - a macro to store the intermediate sub-path representations.
%
%  Example:
%
%  \pgfpathmoveto{\pgfpointorigin}
%  \pgfpathlineto{\pgfpoint{0pt}{12pt}}
%  \pgfpathlineto{\pgfpoint{12pt}{0pt}}
%  \pgfgetpath\softpath
%
%  \pgf@decorate@parsesoftpath{\softpath}{\parsedsoftpath}
%
%  results in:
%
%  \parsedsoftpath ->
%    {\pgf@decorate@inputsegmentobject@lineto{12pt}{\pgf@x 0pt\pgf@y 0pt}{\pgf@x 0pt\pgf@y 12pt}}
%    {\pgf@decorate@inputsegmentobject@lineto{12pt}{\pgf@x 0pt\pgf@y 12pt}{\pgf@x 12pt\pgf@y 12pt}}
%
%  \pgfdecoratedpathlength ->
%    24pt
%

\def\pgf@decorate@parsesoftpath#1#2{%
  \def\pgf@decorate@inputsegmentobjectsmacro{#2}%
  \let\pgf@decorate@inputsegmentobjects\pgfutil@empty%
  \pgfutil@tempdima0pt\relax%
  \let\pgfpoint@decorate@lastparsed\pgfpoint@decorate@existingpathlast%
  \let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@origin%
  \let\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
  \let\pgfpoint@decorated@firstparsed\pgfutil@empty%
  \expandafter\pgf@decorate@@parsesoftpath#1\pgf@stop%
}%

\def\pgf@decorate@@parsesoftpath#1{%
  \ifx#1\pgf@stop%
    \let\pgf@decorate@queueinputsegmentobject\pgfutil@empty% <- removes final moveto (may not be desirable).
    \pgf@decorate@addtoinputsegmentobjects{\pgf@decorate@inputsegmentobject@endofinputsegments}%
    \pgf@decorate@addtoinputsegmentobjects{\pgf@decorate@inputsegmentobject@endofinputsegments}%
    \expandafter\let\pgf@decorate@inputsegmentobjectsmacro\pgf@decorate@inputsegmentobjects%
    \edef\pgf@decorate@totalpathlength{\the\pgfutil@tempdima}%
    \let\pgf@next\relax%
  \else%
    \ifx#1\pgfsyssoftpath@movetotoken%
      \let\pgf@next\pgf@decorate@parsemoveto%
    \else%
      \ifx#1\pgfsyssoftpath@linetotoken%
        \let\pgf@next\pgf@decorate@parselineto%
      \else%
        \ifx#1\pgfsyssoftpath@curvetosupportatoken%
          \let\pgf@next\pgf@decorate@parsecurveto%
        \else%
          \ifx#1\pgfsyssoftpath@closepathtoken%
            \let\pgf@next\pgf@decorate@parseclosepath%
          \else%
            \ifx#1\pgfsyssoftpath@rectcornertoken%
              \let\pgf@next\pgf@decorate@parserect%
            \else%
              \pgferror{Unrecognised soft path token `#1'}%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@next}%


\def\pgf@decorate@addtoinputsegmentobjects#1{%
  %
  % If there is an input segment object waiting (i.e. a moveto), insert it here.
  %
  \ifx\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
  \else%
    \let\pgf@decorate@temp\pgf@decorate@queueinputsegmentobject%
    \let\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
    \expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
  \fi%
  \ifx\pgfpoint@decorated@firstparsed\pgfutil@empty%
    #1%
    \let\pgfpoint@decorated@firstparsed\pgf@decorate@inputsegment@first%
  \fi%
  \expandafter\def\expandafter\pgf@decorate@inputsegmentobjects\expandafter%
    {\pgf@decorate@inputsegmentobjects{#1}}%
}%

%  Convert \pgfsyssoftpath@movetotoken{<X>}{<Y>} into the following
% representation:
%
%  \pgf@decorate@inputsegmentobject@moveto{\pgf@x X\pgf@y Y}
%
%  The moveto input segment object is not added immediately, so that
%  only the last of multiple movetos is inserted.
%
\def\pgf@decorate@parsemoveto#1#2{%
  \def\pgf@decorate@queueinputsegmentobject{\pgf@decorate@inputsegmentobject@moveto{\pgf@x#1\pgf@y#2}}%
  \def\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
  \pgf@decorate@@parsesoftpath%
}%

% Convert \pgfsyssoftpath@linetotoken{<X>}{<Y>} into the following
% representation:
%
% \pgf@decorate@inputsegmentobject@lineto{<length>}{\pgf@x <Last X> \pgf@y <Last Y}{\pgf@x <X> \pgf@y <Y>}
%
\def\pgf@decorate@parselineto#1#2{%
  \pgf@decorate@linelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
  \advance\pgfutil@tempdima\pgfmathresult pt\relax%
  \edef\pgf@decorate@temp{%
    \noexpand\pgf@decorate@inputsegmentobject@lineto{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
  }%
  \edef\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
  \let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
  \expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
  \pgf@decorate@@parsesoftpath%
}%

% Convert \pgfsyssoftpath@curvetosupportatoken{<Xa>}{<Ya>}...etc
% into the following representation:
%
% \pgf@decorate@inputsegmentobject@curveto{<length>}{\pgf@x <Last X> \pgf@y <Last Y}
%    {\pgf@x <Xa> \pgf@y <Ya>}{\pgf@x <Xb> \pgf@y <Yb>}{\pgf@x <X> \pgf@y <Y>}
%
\def\pgf@decorate@parsecurveto#1#2\pgfsyssoftpath@curvetosupportbtoken#3#4\pgfsyssoftpath@curvetotoken#5#6{%
  \pgf@decorate@curvelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}{\pgf@x#3\pgf@y#4}{\pgf@x#5\pgf@y#6}%
  \advance\pgfutil@tempdima\pgfmathresult pt\relax%
  \edef\pgf@decorate@temp{%
    \noexpand\pgf@decorate@inputsegmentobject@curveto{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}%
      {\pgf@x#1\pgf@y#2}{\pgf@x#3\pgf@y#4}{\pgf@x#5\pgf@y#6}%
  }%
  \expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
  \edef\pgfpoint@decorate@lastparsed{\pgf@x#5\pgf@y#6}%
  \let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
  \pgf@decorate@@parsesoftpath%
}%


\def\pgf@decorate@parseclosepath#1#2{%
  \pgf@decorate@linelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
  \advance\pgfutil@tempdima\pgfmathresult pt\relax%
  \edef\pgf@decorate@temp{%
    \noexpand\pgf@decorate@inputsegmentobject@closepath{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
  }%
  \expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
  \edef\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
  \let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
  \pgf@decorate@@parsesoftpath%
}%

% Convert \pgfsyssoftpath@rectcornertoken{<X>}{<Y>}\pgfsyssoftpath@rectsizetoken{<Xa>}{<Ya>}
% into either (clockwise)
%
% \pgf@decorate@inputsegmentobject@moveto{<X>}{<Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <X> \pgf@y <Y>}{\pgf@x <X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <X> \pgf@y <Ya+Y>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <Xa+X> \pgf@y <Ya+X>}{\pgf@x <Xa+X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <Xa+X> \pgf@y <Y>}{\pgf@x <X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@moveto{<Xa>}{<Ya>}
%
% ...or (anti-clockwise)
%
% \pgf@decorate@inputsegmentobject@moveto{<X>}{<Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <X> \pgf@y <Y>}{\pgf@x <Xa+X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <Xa+X> \pgf@y <Y>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}{\pgf@x <X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <X> \pgf@y <Ya+Y>}{\pgf@x <X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@moveto{<Xa>}{<Ya>}
%
\newif\ifpgfdecoraterectangleclockwise
\def\pgf@decorate@parserect#1#2\pgfsyssoftpath@rectsizetoken#3#4{%
  %
  % Subvert \pgf@decorate@parsesoftpath so parsing macros will
  % return here instead of continuing to parse the soft path.
  %
  \let\pgf@decorate@orig@@parsesoftpath\pgf@decorate@@parsesoftpath%
  \let\pgf@decorate@@parsesoftpath\relax%
  \pgf@decorate@parsemoveto{#1}{#2}%
  \pgf@xa#1\relax%
  \pgf@ya#2\relax%
  \ifpgfdecoraterectangleclockwise%
    \advance\pgf@ya#4%
    \pgf@yb\pgf@ya%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@xa#3%
    \pgf@xb\pgf@xa%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@ya-#4%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@xa-#3%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parseclosepath\pgf@temp%
  \else%
    \advance\pgf@xa#3%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \pgf@xb\pgf@xa%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@ya#4%
    \pgf@yb\pgf@ya%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@xa-#3%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parselineto\pgf@temp%
    \advance\pgf@ya-#4%
    \edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgf@decorate@parseclosepath\pgf@temp%
  \fi%
  %
  % Restore the parsing.
  %
  \let\pgf@decorate@@parsesoftpath\pgf@decorate@orig@@parsesoftpath%
  \edef\pgf@marshal{\noexpand\pgf@decorate@parsemoveto{\the\pgf@xb}{\the\pgf@yb}}%
  \pgf@marshal%
}%




% \pgf@decorate@linelength
%
% Define \pgfmathresult as the distance between #1 and #2 (without units).
%
\def\pgf@decorate@linelength#1#2{%
  \pgf@process{\pgfpointdiff{#1}{#2}}%
  \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
}%

% \pgf@decorate@curvelength
%
% Define \pgfmathresult as the length (without units) of the cubic
% bezier described by #1,#2,#3 and #4.
%
% To approximate the length of the curve P (sort of) use:
%
% curveLength(P,q)
%   Q = subdivideLeft(P);
%    R = subdivideRight(P);
%   return curveLength'(Q,q) + curveLength'(R,q);
%
% curveLength'(P,q)
%    <P1,P2,P3,P4> <- P;
%   P' = P4 - P1;
%   x = P'.x();
%    y = P'.y();
%   if (x < q) && (y < q)
%      return |P'|;
%    else%
%      Q = subdivideLeft(P);
%      R = subdivideRight(P);
%     return curveLength'(Q,q) + curveLength'(R,q);
%
% Where q is some small value (`tolerance').
%
\newif\ifpgf@decorate@subdivide
\def\pgf@decorate@curvelength#1#2#3#4{%
  %
  % Always begin with a subdivision in case #1 = #4.
  %
  \begingroup%
    \pgf@decorate@recursive@subdividecurve@left{#1}{#2}{#3}{#4}%
    \pgfutil@tempdimb\pgfmathresult pt\relax%
    \pgf@decorate@recursive@subdividecurve@right{#1}{#2}{#3}{#4}%
    \advance\pgfutil@tempdimb\pgfmathresult pt\relax%
    \pgfmath@returnone\pgfutil@tempdimb%
  \endgroup%
}%

\def\pgf@decorate@@curvelength#1#2#3#4{%
  \begingroup%
    \pgf@decorate@curvecordlength{#1}{#2}{#3}{#4}%
    \ifpgf@decorate@subdivide%
      \pgf@decorate@recursive@subdividecurve@left{#1}{#2}{#3}{#4}%
      \pgfutil@tempdimb\pgfmathresult pt\relax%
      \pgf@decorate@recursive@subdividecurve@right{#1}{#2}{#3}{#4}%
      \advance\pgfutil@tempdimb\pgfmathresult pt\relax%
      \expandafter\pgfmath@returnone\expandafter\pgfutil@tempdimb%
    \else%
      \expandafter\pgfmath@returnone\expandafter\pgfmathresult\expandafter p\expandafter t\expandafter%
    \fi%
  \endgroup%
}%

\def\pgf@decorate@curvelength@tolerance{1pt}%

\def\pgf@decorate@curvecordlength#1#2#3#4{%
  %
  % Calculate the curve cord vector.
  %
  #4\relax%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  #1\relax%
  \advance\pgf@xa-\pgf@x%
  \advance\pgf@ya-\pgf@y%
  \ifdim\pgf@xa<0pt\relax\pgf@xa-\pgf@xa\fi%
  \ifdim\pgf@ya<0pt\relax\pgf@ya-\pgf@ya\fi%
  %
  % Always subdivide, unless...
  %
  \pgf@decorate@subdividetrue%
  %
  % The cord vector is small.
  %
  \ifdim\pgf@xa<\pgf@decorate@curvelength@tolerance\relax%
    \ifdim\pgf@ya<\pgf@decorate@curvelength@tolerance\relax%
      \pgfmathveclen@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@ya}}%
      \pgf@decorate@subdividefalse%
    \fi%
  \fi%
}%

\def\pgf@decorate@recursive@subdividecurve@left#1#2#3#4{%
  {%
    %
    % The left curve (from t=0 to t=.5)
    %
    #1\relax%
    \pgfutil@tempdima\pgf@x%
    \pgfutil@tempdimb\pgf@y%
    \pgf@xa.5\pgf@x\pgf@ya.5\pgf@y%
    \pgf@xb.25\pgf@x\pgf@yb.25\pgf@y%
    \pgf@xc.125\pgf@x\pgf@yc.125\pgf@y%
    #2\relax%
    \advance\pgf@xa.5\pgf@x\advance\pgf@ya.5\pgf@y%
    \advance\pgf@xb.5\pgf@x\advance\pgf@yb.5\pgf@y%
    \advance\pgf@xc.375\pgf@x\advance\pgf@yc.375\pgf@y%
    #3\relax%
    \advance\pgf@xb.25\pgf@x\advance\pgf@yb.25\pgf@y%
    \advance\pgf@xc.375\pgf@x\advance\pgf@yc.375\pgf@y%
    #4\relax%
    \advance\pgf@xc.125\pgf@x\advance\pgf@yc.125\pgf@y%
    \xdef\pgf@marshal{%
      \noexpand\pgf@decorate@@curvelength%
        {\pgf@x\the\pgfutil@tempdima\pgf@y\the\pgfutil@tempdimb}%
        {\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}{\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}
          {\pgf@x\the\pgf@xc\pgf@y\the\pgf@yc}%
    }%
  }%
  \pgf@marshal%
}%

\def\pgf@decorate@recursive@subdividecurve@right#1#2#3#4{%
  {%
    %
    % The right curve (from t=0.5 to t=1)
    %
    #1\relax%
    \pgfutil@tempdima.125\pgf@x\pgfutil@tempdimb.125\pgf@y%
    #2\relax%
    \advance\pgfutil@tempdima.375\pgf@x\advance\pgfutil@tempdimb.375\pgf@y%
    \pgf@xa.25\pgf@x\pgf@ya.25\pgf@y%
    #3\relax%
    \advance\pgfutil@tempdima.375\pgf@x\advance\pgfutil@tempdimb.375\pgf@y%
    \advance\pgf@xa.5\pgf@x\advance\pgf@ya.5\pgf@y%
    \pgf@xb.5\pgf@x\pgf@yb.5\pgf@y%
    #4\relax%
    \advance\pgfutil@tempdima.125\pgf@x\advance\pgfutil@tempdimb.125\pgf@y%
    \advance\pgf@xa.25\pgf@x\advance\pgf@ya.25\pgf@y%
    \advance\pgf@xb.5\pgf@x\advance\pgf@yb.5\pgf@y%
    \pgf@xc\pgf@x\pgf@yc\pgf@y%
    \xdef\pgf@marshal{%
      \noexpand\pgf@decorate@@curvelength%
        {\pgf@x\the\pgfutil@tempdima\pgf@y\the\pgfutil@tempdimb}%
        {\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}{\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}
          {\pgf@x\the\pgf@xc\pgf@y\the\pgf@yc}%
    }%
  }%
  \pgf@marshal%
}%


% Macro to reverse a set of input segment objects.
%
% #1 - a macro holding the input segment objects.
% #2 - a macro holding the reversed input segment objects.
%
\def\pgf@decorate@inputsegmentobjects@reverse#1#2{%
  \def\pgf@decorate@path@storein{#2}%
  \def\pgf@decorate@inputsegments@@temp{}%
  \expandafter\pgf@decorate@inputsegments@@reverse@pass@first#1\pgf@stop}%

\def\pgf@decorate@inputsegments@@reverse@pass@first#1#2\pgf@stop{%
  \def\pgf@decorate@temp{#1}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgf@decorate@inputsegments@@temp\expandafter\expandafter\expandafter%
      {\expandafter\pgf@decorate@temp\pgf@decorate@inputsegments@@temp}%
  \def\pgf@decorate@test{#2}
  \ifx\pgf@decorate@test\pgfutil@empty%
    \def\pgf@decorate@next{%
      \expandafter\pgf@decorate@inputsegmentobjects@reverse@pass@second\pgf@decorate@inputsegments@@temp\pgf@stop%
    }%
  \else%
    \def\pgf@decorate@next{\pgf@decorate@inputsegments@@reverse@pass@first#2\pgf@stop}%
  \fi%
  \pgf@decorate@next%
}%
\def\pgf@decorate@inputsegmentobjects@reverse@pass@second#1#2#3\pgf@stop{%
  \def\pgf@decorate@inputsegments@temp{#3}%
  \def\pgf@decorate@inputsegments@@temp{}%
  \let\pgf@decorate@current@inputsegmentobject=\pgfutil@empty
  \let\pgf@decorate@last@object=\pgfutil@empty
  \pgf@decorate@inputsegmentobjects@reverse@moveto@waitingtrue%
  \pgf@decorate@inputsegmentobjects@reverse@closepath@waitingfalse%
  \expandafter\pgf@decorate@path@@reverse@pass@second\pgf@decorate@inputsegments@temp\pgf@stop}%


\def\pgf@decorate@path@@reverse@pass@second#1{%
  \ifx#1\pgf@stop%
    \expandafter\def\expandafter\pgf@decorate@inputsegments@@temp\expandafter{%
      \pgf@decorate@inputsegments@@temp%
      {\pgf@decorate@inputsegmentobject@endofinputsegments}%
      {\pgf@decorate@inputsegmentobject@endofinputsegments}
    }%
    \expandafter\let\pgf@decorate@path@storein=\pgf@decorate@inputsegments@@temp%
    \let\pgf@decorate@next=\relax%
  \else%
    \ifx#1\pgf@decorate@inputsegmentobject@moveto%
      \let\pgf@decorate@next=\pgf@decorate@inputsegmentobjects@reverse@moveto%
    \else%
      \ifx#1\pgf@decorate@inputsegmentobject@lineto%
        \let\pgf@decorate@next=\pgf@decorate@inputsegmentobjects@reverse@lineto%
      \else%
        \ifx#1\pgf@decorate@inputsegmentobject@curveto%
          \let\pgf@decorate@next=\pgf@decorate@inputsegmentobjects@reverse@curveto%
        \else%
          \ifx#1\pgf@decorate@inputsegmentobject@closepath%
            \let\pgf@decorate@next=\pgf@decorate@inputsegmentobjects@reverse@closepath%
          \else%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@decorate@next%
}%

\newif\ifpgf@decorate@inputsegmentobjects@reverse@moveto@waiting

\def\pgf@decorate@inputsegmentobjects@reverse@moveto#1{%
  \ifpgf@decorate@inputsegmentobjects@reverse@closepath@waiting%
    \edef\pgf@decorate@current@inputsegmentobject{%
      {\noexpand\pgf@decorate@inputsegmentobject@closepath%
        {\pgf@decorate@reverse@closepath@length}%
        {\pgf@decorate@last}%
        {#1}%
      }%
    }%
    \pgf@decorate@inputsegmentobjects@reverse@closepath@waitingfalse%
  \else%
    \let\pgf@decorate@current@inputsegmentobject=\pgfutil@empty%
  \fi%
  \pgf@decorate@inputsegmentobjects@reverse@moveto@waitingtrue%
  \pgf@decorate@path@@@reverse@pass@second%
}%

\newif\ifpgf@decorate@inputsegmentobjects@reverse@closepath@waiting

\def\pgf@decorate@inputsegmentobjects@reverse@closepath#1#2#3{%
  \pgf@decorate@inputsegmentobjects@reverse@closepath@waitingtrue%
  \def\pgf@decorate@reverse@closepath@length{#1}%
  \def\pgf@decorate@current@inputsegmentobject{}%
  \pgf@decorate@inputsegmentobjects@reverse@lineto{#1}{#2}{#3}%
}%

\def\pgf@decorate@inputsegmentobjects@reverse@lineto#1#2#3#4{%
  \ifpgf@decorate@inputsegmentobjects@reverse@moveto@waiting%
    \def\pgf@decorate@current@inputsegmentobject{{\pgf@decorate@inputsegmentobject@moveto{#3}}}%
    \pgf@decorate@inputsegmentobjects@reverse@moveto@waitingfalse%
  \else%
    \let\pgf@decorate@current@inputsegmentobject=\pgfutil@empty%
  \fi%
  \def\pgf@decorate@append@inputsegmentobject{{\pgf@decorate@inputsegmentobject@lineto{#1}{#3}{#2}}}%
  \ifx#4\pgf@decorate@inputsegmentobject@moveto%
    \ifpgf@decorate@inputsegmentobjects@reverse@closepath@waiting%
      \def\pgf@decorate@append@inputsegmentobject{{\pgf@decorate@inputsegmentobject@closepath{#1}{#3}{#2}}}%
      \pgf@decorate@inputsegmentobjects@reverse@closepath@waitingfalse%
    \else%
      \def\pgf@decorate@append@inputsegmentobject{{\pgf@decorate@inputsegmentobject@lineto{#1}{#3}{#2}}}%
    \fi%
  \fi%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgf@decorate@current@inputsegmentobject\expandafter\expandafter\expandafter%
      {\expandafter\pgf@decorate@current@inputsegmentobject\pgf@decorate@append@inputsegmentobject}
  \def\pgf@decorate@last{#2}%
  \pgf@decorate@path@@@reverse@pass@second#4%
}%

\def\pgf@decorate@inputsegmentobjects@reverse@curveto#1#2#3#4#5{%
  \ifpgf@decorate@inputsegmentobjects@reverse@moveto@waiting%
    \def\pgf@decorate@current@inputsegmentobject{%
      {\pgf@decorate@inputsegmentobject@moveto{#5}}%
      {\pgf@decorate@inputsegmentobject@curveto{#1}{#5}{#4}{#3}{#2}}%
    }%
    \pgf@decorate@inputsegmentobjects@reverse@moveto@waitingfalse%
  \else%
    \def\pgf@decorate@current@inputsegmentobject{{\pgf@decorate@inputsegmentobject@curveto{#1}{#5}{#4}{#3}{#2}}}%
  \fi%
  \def\pgf@decorate@last{#2}%
  \pgf@decorate@path@@@reverse@pass@second%
}%

\def\pgf@decorate@path@@@reverse@pass@second{%
  \ifx\pgf@decorate@current@inputsegmentobject\pgfutil@empty%
  \else%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
      \pgf@decorate@inputsegments@@temp\expandafter\expandafter\expandafter%
        {\expandafter\pgf@decorate@inputsegments@@temp\pgf@decorate@current@inputsegmentobject}%
  \fi%
  \pgf@decorate@path@@reverse@pass@second%
}%





\let\startpgfdecoration=\pgfdecoration
\let\stoppgfdecoration=\endpgfdecoration

\let\startpgfmetadecoration=\pgfmetadecoration
\let\stoppgfmetadecoration=\endpgfmetadecoration



%
% Predefined decorations
%


% Simple decorations.

\pgfdeclaredecoration{lineto}{initial}{%
  \state{initial}[switch if input segment less than=\pgfdecoratedremainingdistance to input segment,
                  width=\pgfdecoratedremainingdistance]
  {
  }%
  \state{input segment}[width=\pgfdecoratedinputsegmentlength,next state=initial]
  {
    \pgfpathlineto{\pgfpointdecoratedinputsegmentlast}
  }%

  \state{final}{\pgfpathlineto{\pgfpointdecoratedpathlast}}%
}%

\pgfdeclaredecoration{moveto}{initial}{%
  \state{initial}[width=\pgfdecoratedremainingdistance]{}%
  \state{final}{\pgfpathmoveto{\pgfpointdecoratedpathlast}}%
}%

% This decorations curves to the end along the line.

\pgfdeclaredecoration{curveto}{initial}{%
  \state{initial}[width=\pgfdecoratedinputsegmentlength/100]
  {
    \pgfpathlineto{\pgfpointorigin}
  }%
  \state{final}{\pgfpathlineto{\pgfpointdecoratedpathlast}}%
}%




% Compatibility with old "snakes":

\let\pgfsnakeremainingdistance=\pgfdecoratedremainingdistance
\let\pgfsnakecompleteddistance=\pgfdecoratedcompleteddistance
\def\pgfsnakeangle{\pgfdecoratedangle}%
\let\pgfdeclaresnake=\pgfdeclaredecoration
\let\pgfsetsnakesegmenttransformation=\pgfsetdecorationsegmenttransformation
\def\pgfpathsnakesto#1#2{%
  \edef\pgf@temp{#1}%
  \expandafter\pgfdecoration\expandafter{\pgf@temp}%
    \pgfpathlineto{#2}%
  \endpgfdecoration%
}%
\def\pgfpathsnaketo#1#2{\pgfpathsnakesto{{#1}{\pgfsnakeremainingdistance}}{#2}}%
\def\pgfpathsnakealongvector#1#2#3{%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfmathparse{#2}%
  \pgf@xa=\pgfmathresult\pgf@xa%
  \pgf@ya=\pgfmathresult\pgf@ya%
  \advance\pgf@xa by\pgf@path@lastx%
  \advance\pgf@ya by\pgf@path@lasty%
  \edef\pgf@snake@lib@temp{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \pgfpathsnaketo{#1}{\pgf@snake@lib@temp}%
}%

\let\pgfsnakesegmentamplitude=\pgfdecorationsegmentamplitude
\let\pgfsnakesegmentlength=\pgfdecorationsegmentlength
\def\pgfsnakesegmentangle{\pgfdecorationsegmentangle}%
\def\pgfsnakesegmentobjectlength{\pgfkeysvalueof{/pgf/decoration/shape start width}}%
\def\pgfsnakesegmentaspect{\pgfdecorationsegmentaspect}%

\pgfset{%
  /pgf/segment amplitude/.style={/pgf/decoration={amplitude=#1,shape height=2*#1}},
  /pgf/segment length/.style={/pgf/decoration={segment length=#1}},
  /pgf/segment angle/.style={/pgf/decoration={angle=#1}},
  /pgf/segment aspect/.style={/pgf/decoration={aspect=#1}},
  /pgf/segment object length/.style={/pgf/decoration={shape width=#1,radius=#1}}}%



\endinput


==> pgfmodulematrix.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmodulematrix.code.tex}

\usepgfmodule{shapes}%

\newif\ifpgfmatrix
\newif\ifpgf@matrix@correct@call

\newif\ifpgf@matrix@fixed

\newcount\pgfmatrixcurrentrow

\newcount\pgfmatrixcurrentcolumn
\newcount\pgf@matrix@numberofcolumns

\let\pgf@matrix@cell=\pgfnodeparttextbox % alias
\let\pgf@matrix@box=\pgf@matrix@cell % alias

\long\def\pgfmatrixbeforeassemblenode#1{%
  \long\def\pgf@matrix@before@assemnble@node{#1}}
\pgfmatrixbeforeassemblenode{}

% Sets the default row or column sep
%
% #1 = default row or column sep list
%
% Description:
%
% Sets the macro \pgfmatrixrowsep or \pgfmatrixcolumnsep to #1.
%
% Example:
%
% \pgfsetmatrixrowsep{5pt}

\def\pgfsetmatrixrowsep#1{\def\pgfmatrixrowsep{#1}}%
\def\pgfsetmatrixcolumnsep#1{\def\pgfmatrixcolumnsep{#1}}%

\def\pgfmatrixrowsep{0pt}%
\def\pgfmatrixcolumnsep{0pt}%



% The pgfmatrix command creates a node that contains a matrix. Like
% the \pgfnode command, it is to be used inside a pgfpicture
% environment.
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
% #5 = inner shift
% #6 = startup code
% #7 = the matrix code (may contain verbatim stuff)
%
% Description:
%
% This command creates a node that contains a matrix. For
% each cell of the matrix, drawing commands may be given. These
% commands will create a cell picture and a bounding box is computed
% for each cell picture. The cell picture is then placed inside the
% cell. The position inside the cell is computed according to the
% following rules:
%
% 1. In each column, the origins of the cell pictures are all on a
%    vertical line.
% 2. In each row, the origins of the cell pictures are all on a
%    horizontal line.
% 3. All cells in the same row have the same height and depth.
% 4. All cells in the same column have the same width.
% 5. The size of cells are chosen minimal such that the boxes fit into
%    the cells and still meet the above requirement.
%
% Next, the whole resulting matrix, which is given as #7, is placed
% inside a node whose name is given as #3, whose shape is #1, and
% whose anchor is #2. This means that the resulting node is shifted
% such that the given anchor lies at the origin. Then, as for a normal
% node, the #4 path usage command is used for the node.
%
% The parameter #5 is an additional negative shift for the node. Normally, such
% a shift could be given beforehand (that is, the shift could be
% preapplied to the current transformation matrix). However, when #5
% is evaluated, you can refer to temporary positions of nodes inside
% the matrix. In detail, the following happens: When the matrix has
% been typeset, all nodes in the matrix temporarily get assigned their
% positions in the matrix box. The origin of this coordinate system is
% at the left baseline end of the matrix box, which corresponds to the
% text anchor. The position #5 is then interpreted inside this
% coordinate system and then used for shifting.
%
% The idea behind using the parameter #5 is the following: If you
% specify "text" as anchor #2 and specify \pgfpointanchor{inner
% node}{some anchor} for parameter #5, where inner node is a node that
% is created in the matrix, then the whole matrix will be shifted such
% that inner node.some anchor lies at the origin of the whole picture.
%
% At the beginning and at the end of each cell, the macros
% \pgfmatrixbegincode and \pgfmatrixendcode are called. Inside these
% macros you can use \pgfmatrixcurrentcolumn and \pgfmatrixcurrentrow
% to access the current row and column.
%
% Before each column except for the first, an extra space given by the
% macro \pgfmatrixcolumnsep is added. Additionally, an extra space
% given by the optional argument of the \pgfmatrixnextcell commands in
% the first line are added, which may vary between columns. Between
% rows, an extra space given by the macro \pgfmatrixrowsep is
% added. You can also change this value for each row by using a \gdef.
%
%
% Lines are ended using the command \pgfmatrixendrow. The command \\
% is \let to be the same, but \\ is sometimes overridden by, say,
% minipage, so it's good to have \pgfmatrixendrow as a "fallback".
%
% Inside the matrix, \\ must be used to end every line ***including
% the last***. You can pass an optional parameter to \\ as in \\[2pt]
% to give an additional space after this particular line.
%
% The usage of \\ at the end of the matrix is important since this
% command is used to find the end of the matrix. What happens is that
% \\ followed by a closing brace ends the matrix.
%
% Inside the matrix, you must use \pgfmatrixnextcell to separate
% columns. The reason is that two columns are used internally for
% every single column shown. The macro \pgfmatrixnextcell is yields
% (more or less) two && (and some further trickery).
%
% The parameter #6 is executed at the beginning of the matrix
% group. It is inside the protecting group of the matrix, but outside
% the matrix itself. It can be used for different purposes: 1) It can be
% used to simplify the next cell macro. 2) It can be used to issue an
% \aftergroup command. 3) It can be used to setup local settings. For
% example, by setting #6 to \let\&=\pgfmatrixnextcell you can use \&
% instead of \pgfmatrixnextcell. You can also set the catcode of & to
% active.
%
%
% Example:
%
% \begin{tikzpicture}
%
%   \draw (0,0) circle (1mm);  % b.north will lie on the center of this circle
%
%   \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{\let\&=\pgfmatrixnextcell}
%   {
%     \draw (0,0) circle (1cm); \& \node (a) [draw] {Hallo}; \\
%     \node (b) [draw] {Welt};  \& \draw (0,0) circle (5mm); \\
%   }
%
%   \draw [->] (a) -- (b);
%
% \end{tikzpicture}

\def\pgfmatrix#1#2#3#4#5#6{%
  \ifpgfmatrix%
    \pgferror{You cannot nest pgfmatrix environments, yet}
  \fi%
  \bgroup%
    \everycr{}%
    #6%
    \def\pgf@matrix@par@shape{#1}%
    \def\pgf@matrix@par@anchor{#2}%
    \def\pgf@matrix@par@name{#3}%
    \def\pgf@matrix@par@usage{#4}%
    \def\pgf@matrix@par@shift{#5}%
    % the matrix must have a name:
    \ifx\pgf@matrix@par@name\pgfutil@empty%
      \def\pgf@matrix@par@name{pgf@matrix@internal}%
    \fi%
    \pgfmatrixcurrentrow=0\relax%
    \pgfmatrixcurrentcolumn=0\relax%
    \pgf@matrix@numberofcolumns=0\relax%
    \let\\=\pgfmatrixendrow%
    \tabskip=0pt%
    \offinterlineskip%
    \pgfmatrixtrue%
    \let\pgf@matrix@node@list=\pgfutil@empty%
    \expandafter\let\csname pgf@matrix@column@finish@1\endcsname=\pgfutil@empty%
    \let\pgf@matrix@row@finish=\pgfutil@empty%
    %
    % Get rid of bgroup
    %
    \afterassignment\pgf@matrix@cont\let\pgf@next=%
}%
\def\pgf@matrix@cont{%
    \setbox\pgf@matrix@box=\hbox\bgroup\vbox\bgroup%
    \halign\bgroup%
    \pgf@matrix@init@row%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }%
    &%
    ##\pgf@matrix@padding&&%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }&%
    ##\pgf@matrix@padding%
    \cr%
}%

\def\pgf@end@matrix{%
      \egroup\egroup%
    \egroup%
    %
    % Inject custom tokens before assembling the node holding the matrix.  Can
    % be used to apply additional settings.
    %
    \pgf@matrix@before@assemnble@node
    %
    % If there are named nodes, we must adjust their coordinates.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      % Ok, this means we got a lot of work to do...
      \pgf@matrix@compute@origin%
      \pgf@matrix@shift@nodes@initial%
    \fi%
    %
    % Compute additional shift
    %
    \pgftransformresetnontranslations%
    \pgftransformshift{\pgf@process{\pgftransformreset\pgf@matrix@par@shift\pgf@x=-\pgf@x\pgf@y=-\pgf@y}}%
    %
    % Create node
    %
    \pgfmultipartnode{\pgf@matrix@par@shape}{\pgf@matrix@par@anchor}{\pgf@matrix@par@name}{\pgf@matrix@par@usage}%
    %
    % If there are named nodes, we must adjust their coordinates, again.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      {%
        \pgftransformreset%
        \pgf@process{\pgfpointanchor{\pgf@matrix@par@name}{text}}%
        \xdef\pgf@matrix@offset{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \pgf@matrix@shift@nodes@secondary{\pgf@matrix@offset}%
      }%
    \fi%
}%




% Ending a cell
%
% #1 = (optional) spacing between previous and next column. This
%      parameter only has an effect in the first row.
%
% Description:
%
% This command ends a cell of a matrix.
%
% Example:
%
% \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{}
% {
%   \draw (0,0) circle (1cm); \pgfmatrixnextcell[1cm] \node (a) [draw] {Hallo}; \\
%   \node (b) [draw] {Welt};  \pgfmatrixnextcell \draw (0,0) circle (5mm); \\
% }

\def\pgfmatrixnextcell{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  \pgfutil@ifnextchar[{\pgf@matrix@cell@cont}{\pgf@matrix@cell@cont[0pt]}}%}%

\def\pgf@matrix@cell@cont[#1]{%
  \xdef\pgf@matrix@last@nextcell@options{#1}%
  &\pgf@matrix@correct@calltrue&%
}%


\def\pgf@matrix@fixed@text{between origins}%
\def\pgf@matrix@natural@text{between borders}%

\def\pgf@matrix@addtolength#1#2{\edef\pgf@temp{#2}\expandafter\pgf@matrix@addtolength@\expandafter#1#2,\pgf@stop}%
\def\pgf@matrix@addtolength@#1#2,#3\pgf@stop{%
  \def\pgf@temp{#2}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \ifx\pgf@temp\pgf@matrix@fixed@text%
      \global\pgf@matrix@fixedtrue%
    \else%
      \ifx\pgf@temp\pgf@matrix@natural@text%
        \global\pgf@matrix@fixedfalse%
      \else%
        \pgfmathaddtolength{#1}{#2}%
      \fi%
    \fi%
  \fi%
  \def\pgf@temp{#3}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgf@matrix@addtolength@#1#3\pgf@stop%
  \fi%
}%



% Init a line

\def\pgf@matrix@init@row{%
  \relax%
  \global\advance\pgfmatrixcurrentrow by 1\relax%
  \global\pgfmatrixcurrentcolumn=0\relax%
  \expandafter\gdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{0pt}%
  \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
}%



% Step the row column number

\def\pgf@matrix@step@column{%
  \relax%
  \global\advance\pgfmatrixcurrentcolumn by1\relax%
}%



% Start a cell

\def\pgf@matrix@startcell{%
  %
  % Step 1: Init the list of nodes for this cell
  %
  \let\pgf@nodecallback=\pgf@matrix@nodecallback%
  %
  % Step 2: Setup the bounding box
  %
  \pgfinterruptboundingbox%
  %
  % Step 3: Reset the transformation matrix
  %
  \pgftransformreset%
  %
  % Step 4: Collect everything in a cell box
  %
  \setbox\pgf@matrix@cell=\hbox\bgroup\bgroup%
    % make sure that cell pictures are not affected if matrices have
    % 'overlay' option on:
    \pgf@relevantforpicturesizetrue
    \pgfsys@beginpicture%
    \normalbaselines%
    % Find out whether the cell is empty:
    \pgfutil@ifnextchar\let%
    {% ok, candidate, check following symbol
      \afterassignment\pgf@matrix@empty@check\let\pgf@matrix@temp=% get rid of \let
    }%
    {% no, not empty
      \pgf@matrix@empty@cell@false%
      \pgfmatrixbegincode%
    }%
}%

\def\pgf@matrix@empty@check{\futurelet\pgf@matrix@check@token\pgf@matrix@empty@check@cont}%
\def\pgf@matrix@empty@check@cont{%
  \ifx\pgf@matrix@check@token\pgf@matrix@signal@cell@end%
    \pgf@matrix@empty@cell@true%
    \expandafter%
    \pgfmatrixemptycode%
    \expandafter%
    \let% reinserted
  \else%
    \pgf@matrix@empty@cell@false%
    \expandafter%
    \pgfmatrixbegincode%
    \expandafter
    \let% reinserted
  \fi%
}%

\newif\ifpgf@matrix@empty@cell@


% End a  cell

\def\pgf@matrix@endcell{%
    \ifpgf@matrix@empty@cell@%
    \else%
      \expandafter\expandafter\expandafter\pgfmatrixendcode%
      \expandafter\ifpgf@matrix@last@cell@in@row\expandafter\pgf@matrix@last@cell@in@rowtrue\expandafter\fi%
    \fi%
    \pgfsys@endpicture%
    \ifnum\pgfmatrixcurrentcolumn<\pgf@matrix@numberofcolumns%
    \else%
    \ifpgf@matrix@last@cell@in@row\else%
    {%
      \global\pgf@matrix@fixedfalse%
      \pgf@x=0pt%
      \pgf@matrix@addtolength{\pgf@x}{\pgfmatrixcolumnsep}%
      \pgf@matrix@addtolength{\pgf@x}{\pgf@matrix@last@nextcell@options}%
      \ifpgf@matrix@fixed%
        \expandafter\pgfutil@g@addto@macro\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
          {\global\pgf@picmaxx=0pt}%
      \fi%
      \advance\pgfmatrixcurrentcolumn by1\relax % only temporary for the following:
      \expandafter\xdef\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@x}%
      \ifpgf@matrix@fixed%
        \expandafter\gdef\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname{\global\pgf@picminx=0pt}%
      \else%
        \expandafter\global\expandafter\let\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname=\pgfutil@empty%
      \fi%
    }%
    \fi\fi%
    % Special case of the empty picture
    \ifdim\pgf@picmaxx=-16000pt\relax%
      \global\pgf@picmaxx=0pt\relax%
      \global\pgf@picminx=0pt\relax%
      \global\pgf@picmaxy=0pt\relax%
      \global\pgf@picminy=0pt\relax%
    \fi%
    \csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
    \pgf@matrix@row@finish%
  \egroup\egroup%
  %
  % Step 5: Horizontal gap
  %
  \ifnum\pgfmatrixcurrentcolumn>1\relax%
    \pgf@y=\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname\relax%
    \advance\pgf@picminx by-\pgf@y%
  \fi%
  %
  % Step 6: Protocol and adjust height and depth
  %
  % Step 6.1: Protocol...
  %
  \ifdim\pgf@picmaxy>\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picmaxy}%
  \fi%
  \ifdim\pgf@picminy<\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picminy}%
  \fi%
  %
  % Step 6.2: and setup.
  %
  \ht\pgf@matrix@cell=\pgf@picmaxy%
  \dp\pgf@matrix@cell=-\pgf@picminy%
  %
  % Step 7: Protocol and adjust left and right width
  %
  % Step 7.1: Protocol...
  %
  \ifnum\pgfmatrixcurrentcolumn>\pgf@matrix@numberofcolumns\relax%
    \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \global\pgf@matrix@numberofcolumns=\pgfmatrixcurrentcolumn\relax%
  \else%
    \ifdim\pgf@picmaxx>\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \fi%
    \ifdim\pgf@picminx<\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \fi%
  \fi%
  %
  % Step 7.2: and setup.
  %
  \xdef\pgf@matrix@paddingskip{\the\pgf@picmaxx}%
  %
  % Step 8: Put in the box now
  %
  \hfil\hskip-\pgf@picminx%
  \wd\pgf@matrix@cell=0pt%
  \box\pgf@matrix@cell%
  %
  % Step 9: End bounding box
  \endpgfinterruptboundingbox%
}%

% Default code for the start and end code
\let\pgfmatrixbegincode=\relax
\let\pgfmatrixendcode=\relax
\let\pgfmatrixemptycode=\relax


% The following callback is called for every node that is produced
% inside a cell

\def\pgf@matrix@nodecallback#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \xdef\pgf@matrix@node@list{\pgf@matrix@node@list,{#1}}%
    \expandafter\xdef\csname pgf@matrix@node@location@#1\endcsname{{\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  \fi%
}%



% Padding code

\def\pgf@matrix@padding{%
  \ifpgf@matrix@correct@call%
  \else%
    \pgferror{Single ampersand used with wrong catcode}%
  \fi%
  \hskip\pgf@matrix@paddingskip\hfil%
}%


% Compute the real positions of the origins

% We must now compute the real positions of the origins of all the
% small pictures. To this end, we need to compute prefix sums. After
% the procedure is done, the minx and the maxy will contain the origin
% positions.

\def\pgf@matrix@compute@origin{%
  %
  % Inverse prefix sum on the vertical positions
  %
  {%
    \ifnum\pgfmatrixcurrentrow>0\relax%
      \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
    \fi
    \c@pgf@counta=\pgfmatrixcurrentrow\relax%
    \loop%
    \ifnum\c@pgf@counta>1\relax%
      \pgf@y=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by\csname pgf@matrix@maxy\the\c@pgf@counta\endcsname\relax
      \advance\c@pgf@counta by-1\relax%
      \pgf@ya=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by-\pgf@ya\relax%
      \expandafter\xdef\csname pgf@matrix@miny\the\c@pgf@counta\endcsname{\the\pgf@y}%
    \repeat%
  }%
  %
  % Prefix sum on the horizontal positions
  %
  {%
    \ifnum\pgf@matrix@numberofcolumns>0\relax%
      \pgf@x=\csname pgf@matrix@minx1\endcsname\relax%
      \pgf@x=-\pgf@x%
      \expandafter\xdef\csname pgf@matrix@minx1\endcsname{\the\pgf@x}%
    \fi
    \c@pgf@counta=1\relax%
    \loop%
    \ifnum\c@pgf@counta<\pgf@matrix@numberofcolumns\relax%
      \pgf@x=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by\csname pgf@matrix@maxx\the\c@pgf@counta\endcsname\relax%
      \advance\c@pgf@counta by1\relax%
      \pgf@xa=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by-\pgf@xa\relax%
      \expandafter\xdef\csname pgf@matrix@minx\the\c@pgf@counta\endcsname{\the\pgf@x}%
    \repeat%
  }%
}%


% Shift the nodes to their origins

% The following procedure shifts all nodes in
% \pgf@matrix@node@list to their location inside a temporary
% picture. This picture will later be shifted again to its final
% position in the real picture.

\def\pgf@matrix@shift@nodes@initial{%
  {%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{%
          \pgf@x=\csname pgf@matrix@minx%
            \expandafter\expandafter\expandafter\pgfutil@secondoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          \pgf@y=\csname pgf@matrix@miny%
            \expandafter\expandafter\expandafter\pgfutil@firstoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          }%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
  }%
}%


% The second shifting, done in the following procedure, shifts all
% nodes to their real positions inside the real picture.

\def\pgf@matrix@shift@nodes@secondary#1{%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{#1}%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
}%


% End of line
\def\pgfmatrixendrow{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end
  \pgf@matrix@last@cell@in@rowtrue%
  \xdef\pgf@matrix@rowsep{\pgfmatrixrowsep}%
  &\pgf@matrix@correct@calltrue%
  \global\pgf@matrix@fixedfalse%
  \pgf@y=0pt%
  \pgf@matrix@addtolength\pgf@y{\pgf@matrix@rowsep}%
  \pgfutil@ifnextchar[{\pgfmatrixendrow@skip}{\pgf@matrix@finish@line}%
}%
\newif\ifpgf@matrix@last@cell@in@row

\def\pgf@matrix@signal@cell@end{\pgf@matrix@signal@cell@end}%
% exact definition does not matter, only needs to be unique.

\def\pgfmatrixendrow@skip[#1]{%
  \pgf@matrix@addtolength\pgf@y{#1}%
  \pgf@matrix@finish@line%
}%

\def\pgf@matrix@finish@line{%
  \global\pgf@y=\pgf@y%
  \pgf@ya=-\pgf@y%
  \global\advance\pgf@ya by\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
  \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@ya}%
  \pgfutil@ifnextchar\egroup{\cr\pgf@end@matrix}{\pgf@matrix@no@eom@found}%
}%

\def\pgf@matrix@eom@found{%
  \cr%
  \pgf@end@matrix%
}%

\def\pgf@matrix@no@eom@found{%
  \cr%
  \noalign{\vskip\pgf@y%
  \ifpgf@matrix@fixed%
    \vskip\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname% unskip
    \vskip\pgf@y%
    \pgf@y=-\pgf@y%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
    \gdef\pgf@matrix@row@finish{\global\pgf@picmaxy=0pt}%
  \else%
    \global\let\pgf@matrix@row@finish=\pgfutil@empty%
  \fi%
  }%
}%


\endinput


==> pgfmoduleplot.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmoduleplot.code.tex}


% PGF's plotting interface works as follows:
%
% In order to plot something, two things need to be done. First, you
% need to provide the coordinates (obviously) of the points that
% should be plotted. The coordinates are given via a long stream of
% commands. These commands are \pgfplotstreamstart, which is
% given exactly once at the beginning, the commands
% \pgfplotstreampoint, \pgfplotstreampointoutlier,
% \pgfplotstreampointundefined, \pgfplotstreamnewdataset, of which
% there are numerous in the middle, the special \pgfplotstreamspecial,
% of which there may be numerous in the middle, and \pgfplotstreamend,
% which must be given at the end. Between these commands arbitrary
% other commands may be given. Here is an example:
%
% ...
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreamnewdataset
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampointoutlier{\pgfpointxy{3}{9}}
% \pgfplotstreamspecial{some handler-dependent special stuff}
% \pgfplotstreamend
%
% By themselves, the \pgfplotstreamxxxx commands do not do anything by
% default. Rather, to ``use'' such a stream, you must first install a
% stream handler. For example, the ``lineto'' handler will simply
% basically every \pgfplotstreampoint into a \pgfpathlineto.
%
% One special things is the handling of "jumps" in a stream. For
% instance, when a lineto handler encounters an "outlier" or a new
% data set, the current line should end and a new subpath should start
% (unless configured otherwise). For this, the special jump handler is
% important.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
%
% \pgfplothandlerlineto
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamend


% The stream commands actually call their ``internal'' versions, which
% are set by the handlers:
\def\pgfplotstreamstart{\pgf@plotstreamstart}%
\def\pgfplotstreampoint#1{\gdef\pgfplotlastpoint{#1}\pgf@plotstreampoint{#1}}%
\def\pgfplotstreampointoutlier#1{\pgfplot@outliers{}{\pgf@plotstreamjump}{\pgfplotstreampoint{#1}}}%
\def\pgfplotstreampointundefined{\pgfplot@outliers{}{\pgf@plotstreamjump}{}}%
\def\pgfplotstreamnewdataset{\pgfplot@outliers{}{\pgf@plotstreamjump}{}}%
\def\pgfplotstreamspecial{\pgf@plotstreamspecial}%
\def\pgfplotstreamend{\pgf@plotstreamend}%

\def\pgfplot@ignorer#1#2#3{#1}%
\def\pgfplot@jumper#1#2#3{#2}%
\def\pgfplot@plotter#1#2#3{#3}%

\let\pgfplot@outliers\pgfplot@jumper
\let\pgfplot@undefined\pgfplot@jumper
\let\pgfplot@newdata\pgfplot@jumper

\pgfset{
  handle outlier points in plots/.is choice,
  handle outlier points in plots/ignore/.code=\let\pgfplot@outliers\pgfplot@ignorer,
  handle outlier points in plots/jump/.code=\let\pgfplot@outliers\pgfplot@jumper,
  handle outlier points in plots/plot/.code=\let\pgfplot@outliers\pgfplot@plotter,
  handle undefined points in plots/.is choice,
  handle undefined points in plots/ignore/.code=\let\pgfplot@undefined\pgfplot@ignorer,
  handle undefined points in plots/jump/.code=\let\pgfplot@undefined\pgfplot@jumper,
  handle new data sets in plots/.is choice,
  handle new data sets in plots/ignore/.code=\let\pgfplot@newdata\pgfplot@ignorer,
  handle new data sets in plots/jump/.code=\let\pgfplot@newdata\pgfplot@jumper,
}%


% Declares a new plot handler
%
% #1 = macro that should install the stream handler subsequently
% #2 = parameter list of said macro.
% #3 = keys as described below
%
% Description:
%
% When you declare a new plot handler, you provide, through keys,
% different "actions" that should be taken when the different stream
% commands are used:
%
% start       = some code to be executed when \pgfplotstreamstart is called
%               for this plothandler
% end         = same for the end of the stream
% point       = code to be executed for a point of the stream
% jump        = code to be executed for a "jump" in the stream
% special     = code to be executed for \pgfplotstreamspecial
% start macro   = here and for the following keys, the to-be-executed
%                 code is stored in the given macro
% end macro     = see above
% jump macro    = see above
% point macro   = see above
% special macro = see above
%
% Example:
%
% \pgfdeclareplothandler{\ultrasimplehandler}{}{
%   point=\pgfpathlineto{##1}
% }

\def\pgfdeclareplothandler#1#2#3{%
  \def#1#2{%
    \pgfkeys{%
      /pgf/plots/@handler options/.cd,
      start=\relax,
      end macro=\relax,
      point macro=\pgfutil@gobble,
      jump macro=\relax,
      special macro=\pgfutil@gobble,%
      #3%
    }%
  }%
}%

\pgfkeys{%
  /pgf/plots/@handler options/.cd,
  start/.code=%
    \gdef\pgf@plotstreamstart{%
      \global\pgf@plot@startedfalse%
      \global\let\pgf@plotstreamend\pgf@plotstreamend@init%
      \global\let\pgf@plotstreampoint\pgf@plotstreampoint@init%
      \global\let\pgf@plotstreamjump\pgf@plotstreamjump@init%
      \global\let\pgf@plotstreamspecial\pgf@plotstreamspecial@init%
      #1%
    },%
  start macro/.code=%
    \gdef\pgf@plotstreamstart{%
      \global\pgf@plot@startedfalse%
      \global\let\pgf@plotstreamend\pgf@plotstreamend@init%
      \global\let\pgf@plotstreampoint\pgf@plotstreampoint@init%
      \global\let\pgf@plotstreamjump\pgf@plotstreamjump@init%
      \global\let\pgf@plotstreamspecial\pgf@plotstreamspecial@init%
      #1%
    },%
  end/.code=\gdef\pgf@plotstreamend@init{#1},
  end macro/.code=\global\let\pgf@plotstreamend@init#1,
  point/.code=\gdef\pgf@plotstreampoint@init##1{#1},
  point macro/.code=\global\let\pgf@plotstreampoint@init#1,
  jump/.code=\gdef\pgf@plotstreamjump@init{#1},
  jump macro/.code=\global\let\pgf@plotstreamjump@init#1,
  special/.code=\gdef\pgf@plotstreamspecial@init##1{#1},
  special macro/.code=\global\let\pgf@plotstreamspecial@init#1,
}%

\newif\ifpgf@plot@started




% Sets the action taken for the first point of a plot to a lineto.
%
% Description:
%
% For certain handlers it makes sense either the start a plot by
% moving to the first point of the plot or to do a lineto to that
% first point. Using this command this action can be set to a lineto.
%
% Example:
%
% \pgfsetlinetofirstplotpoint

\def\pgfsetlinetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathlineto}%


% Sets the action taken for the first point of a plot to a moveto.
%
% Example:
%
% \pgfsetmovetofirstplotpoint

\def\pgfsetmovetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathmoveto}%

\let\pgf@plot@first@action=\pgfpathmoveto




%
% Handlers
%


% This handler converts each plot stream command into a lineto
% command, except for the first, which is converted to the action that
% has previously been specified using \pgfsetlinetofirstplotpoint or
% \pgfsetmovetofirstplotpoint.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerlineto}{}{
  point macro=\pgf@plot@line@handler,
  jump=\global\let\pgf@plotstreampoint\pgf@plot@line@handler@move%
}%

\def\pgf@plot@line@handler#1{%
  \pgf@plot@first@action{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%

\def\pgf@plot@line@handler@move#1{%
  \pgfpathmoveto{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%



% This handler turns creates a series of lineto commands, with the
% last command being a closepath, resulting in a closed path. If a
% jump is encountered, the current subpath is closed and a new subpath
% is started.
%
% Example:
%
% \pgfplothandlerpolygon
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerpolygon}{}{%
  point macro=\pgf@plot@line@handler@close,
  jump macro=\pgf@plot@next@close@and@moveto,
  end macro=\pgf@plot@polygon@stop
}%

\def\pgf@plot@line@handler@close#1{%
  \pgfpathmoveto{#1}%
  \global\pgf@plot@startedtrue%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%

\def\pgf@plot@polygon@stop{%
  \ifpgf@plot@started%
    \pgfpathclose%
  \fi%
  \global\pgf@plot@startedfalse%
}%

\def\pgf@plot@next@close@and@moveto{%
  \ifpgf@plot@started%
    \pgfpathclose%
  \fi%
  \global\let\pgf@plotstreampoint\pgf@plot@line@handler@close%
}%


% More handlers are defined in pgflibraryplothandlers





% This handler discards the plot.
%
% Example:
%
% \pgfplothandlerdiscard
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerdiscard}{}{}%



% This handler records each plot stream command to a macro. This is
% useful if plot commands are difficult to generate and need to be
% ``recycled'' later on.
%
% Example:
%
% \pgfplothandlerrecord{\myplot}
% \pgfplotxyfile{mytable}  % stored in \myplot now
% \pgfplothandlerline
% \myplot
% \pgftransformxshift{1cm}
% \myplot

\pgfdeclareplothandler{\pgfplothandlerrecord}{#1}{%
  start=\gdef#1{\pgfplotstreamstart},
  point=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreampoint{##1}},
  jump=\expandafter\gdef\expandafter#1\expandafter{#1\pgf@plotstreamjump},
  special=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamspecial{##1}},
  end=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend},
}%



% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Each line of the file should begin with two numbers separated by a
% space. Such a line with number #1 and #2 is converted to a
% \pgfplotstreampoint{\pgfpointxy{#1}{#2}}. Extra characters following
% on the line are ignored.
%
% Lines starting with ``%'' and ``#'' are ignored.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyfile#1{%
  \begingroup%
    \def\b@pgfplotsxyfile@scanning@for@first{1}%
    \pgfplotstreamstart%
    \openin\r@pgf@reada=#1
    \ifeof\r@pgf@reada
      \pgfwarning{Plot data file `#1' not found.}
     \else
      \catcode`\#=14
      \catcode`\^^M=5
      \pgf@readxyfile%
    \fi
    \pgfplotstreamend%
  \endgroup%
}%

\let\pgf@savedpar=\par
\def\pgf@partext{\par}%
\def\pgf@readxyfile{%
  \pgfutil@read\r@pgf@reada to \pgf@temp%
  \let\par=\pgf@savedpar%
  \edef\pgf@temp{\pgf@temp}%
  \ifx\pgf@temp\pgfutil@empty%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else\ifx\pgf@temp\pgf@partext%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else%
    \expandafter\pgf@parsexyline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof\r@pgf@reada\else\expandafter\pgf@readxyfile\fi%
}%

\def\pgf@parsexyline#1 #2 #3\pgf@stop{%
  \def\b@pgfplotsxyfile@scanning@for@first{0}%
  \edef\pgf@xyline@flag@val{#3}%
  \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
    \pgfplotstreampointundefined%
  \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
    \pgfplotstreampointoutlier{\pgfpointxy{#1}{#2}}%
  \else%
    \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
  \fi\fi%
}%

\edef\pgf@xyline@flag@out{o\space}%
\edef\pgf@xyline@flag@undef{u\space}%




% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Like xy, except that each line contains three numbers, which are
% converted to xyz coordinates.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyzfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin\r@pgf@reada=#1
    \ifeof\r@pgf@reada
      \pgfwarning{Plot data file `#1' not found.}
    \else
      \catcode`\#=14
      \catcode`\^^M=5
      \pgf@readxyzfile%
    \fi
    \pgfplotstreamend%
  \endgroup%
}%

\def\pgf@readxyzfile{%
  \pgfutil@read\r@pgf@reada to \pgf@temp%
  \ifx\pgf@temp\pgfutil@empty%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else\ifx\pgf@temp\pgf@partext%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else%
    \expandafter\pgf@parsexyzline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof\r@pgf@reada\else\expandafter\pgf@readxyzfile\fi%
}%

\def\pgf@parsexyzline#1 #2 #3 #4\pgf@stop{%
  \def\b@pgfplotsxyfile@scanning@for@first{0}%
  \edef\pgf@xyline@flag@val{#4}%
  \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
    \pgfplotstreampointundefined%
  \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
    \pgfplotstreampointoutlier{\pgfpointxyz{#1}{#2}{#3}}%
  \else%
    \pgfplotstreampoint{\pgfpointxyz{#1}{#2}{#3}}%
  \fi\fi%
}%




% Render a function using gnuplot.
%
% #1 = filename prefix for .gnuplot and .table files (optional,
%      default is \jobname)
% #2 = gnuplot function text
%
% Description:
%
% This command will write a file called #1.gnuplot that sets up
% some gnuplot commands to write output to a file called
% #1.table. Then it calls gnuplot (using the \write18 mechanism)
% to execute the file. Then it reads #2.table using \pgfplotxyfile.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotgnuplot[\jobname]{plot [x=0:5] x*sin(x)}

{%
  \catcode`\%=12
  \catcode`\"=12
  \xdef\pgf@gnuplot@head{set table \noexpand\pgf@plottablefile@quoted; set format "%.5f"}
}%

\let\pgf@plotwrite=\w@pgf@writea
\newif\ifpgf@resample@plot

\pgfkeys{%
  /pgf/plot/gnuplot call/.initial={gnuplot}}%

\def\pgfplotgnuplot{\pgfutil@ifnextchar[{\pgf@plotgnuplot}{\pgf@plotgnuplot[\jobname]}}%}%
\def\pgf@plotgnuplot[#1]#2{%
  \pgf@resample@plottrue%
  \pgfutilpreparefilename{#1.gnuplot}%
  \let\pgf@plotgnuplotfile=\pgfretval
  \pgfutilpreparefilename{#1.table}%
  \let\pgf@plottablefile=\pgfretval
  \let\pgf@plottablefile@quoted=\pgfretvalquoted
  % Check, whether it is up-to-date
  \openin\pgfutil@inputcheck=\pgf@plotgnuplotfile\relax
  \ifeof\pgfutil@inputcheck%
  \else%
    \pgfutil@read\pgfutil@inputcheck to\pgf@temp% ignored
    \pgfutil@read\pgfutil@inputcheck to\pgf@plot@line%
    \closein\pgfutil@inputcheck
    \edef\pgf@plot@code{#2\space}%
    \ifx\pgf@plot@code\pgf@plot@line%
      \openin\pgfutil@inputcheck=\pgfretval\relax
      \ifeof\pgfutil@inputcheck%
      \else%
        \closein\pgfutil@inputcheck
        \pgf@resample@plotfalse%
      \fi%
    \fi%
  \fi
  \ifpgf@resample@plot%
    \immediate\openout\pgf@plotwrite=\pgf@plotgnuplotfile\relax
    \immediate\pgfutil@write\pgf@plotwrite{\pgf@gnuplot@head}%
    \immediate\pgfutil@write\pgf@plotwrite{#2}%
    \immediate\closeout\pgf@plotwrite%
    \pgfutil@shellescape{%
      \pgfkeysvalueof{/pgf/plot/gnuplot call} \pgf@plotgnuplotfile}%
  \fi%
%  \let\pgf@savedparsexyline=\pgf@parsexyline%
%  \let\pgf@parsexyline=\pgf@parsegnuplotxyline%
  \pgfplotxyfile{\pgf@plottablefile}%
%  \let\pgf@parsexyline=\pgf@savedparsexyline%
}%

% \def\pgf@parsegnuplotxyline#1 #2 #3\pgf@stop{%
%   \edef\pgf@xyline@flag@val{#3}%
%   \edef\pgf@xyline@flag@out{o\space}%
%   \edef\pgf@xyline@flag@undef{u\space}%
%   \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
%     \pgfplotstreampointundefined%
%   \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
%     \pgfplotstreampointoutlier{\pgfpointxy{#1}{#2}}%
%   \else%
%     \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
%   \fi\fi%
% }%

% This producer handler plots a function using pgf's mathematical engine.
%
% #1 = variable
% #2 = domain for the variable
% #3 = point, typically defined in terms of the value of the variable
%
% Description:
%
% This producer will iterate the variable #1 over all variables in #2
% (using the \foreach statement). For each value, a plot coordinate
% #3  is created.
%
% Note that this command is pretty slow.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotfunction{\x}{0,0.1,...,3.141}{\pgfpointxy{\x}{sin(\x)}}

\def\pgfplotfunction#1#2#3{%
  \pgfplotstreamstart%
  \foreach#1in{#2}%
  {%
    \pgf@process{#3}%
    \edef\pgf@marshal{\noexpand\pgfplotstreampoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
    \pgf@marshal%
  }
  \pgfplotstreamend%
}%




\endinput


==> pgfmoduleshapes.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmoduleshapes.code.tex}



\newbox\pgfnodeparttextbox


% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% When this command is called, the shape-specific TeX boxes of the
% node must have been setup correctly.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfmultipartnode{rectangle}{center}{hellonode}{\pgfusepath{stroke}}

\def\pgfmultipartnode#1#2#3#4{%
  \pgfutil@ifundefined{pgf@sh@s@#1}%
  {\pgferror{Unknown shape ``#1''}}%
  {%
    {%
      \ifpgflatenodepositioning%
        \pgfsys@beginscope%
      \fi%
      \pgf@outer@adjust@hook%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{#1}% CJ % TT added prefix!
      \csname pgf@sh@s@#1\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{#1}{#2}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@#3\endcsname{%
        \pgf@sh@reanchor{#1}{#2}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{#3}%
      \ifpgflatenodepositioning%
        \pgf@shapes@late@pos@begin%
      \fi%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{#1}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp%
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
      \pgfutil@ifundefined{pgf@sh@bbg@#1}{}
      {{\pgfusetype{.behind background}\pgfidscope\pgfscope\csname pgf@sh@bbg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \pgfutil@ifundefined{pgf@sh@bg@#1}{%
        \global\let\pgfpositionnodelaterpath\pgfutil@empty%
      }%
      {\pgfpushtype%
       \pgfusetype{.background}\csname pgf@sh@bg@#1\endcsname%
        \ifpgflatenodepositioning%
          \pgfsyssoftpath@getcurrentpath\pgfpositionnodelaterpath%
          \pgfprocessround{\pgfpositionnodelaterpath}{\pgfpositionnodelaterpath}%
          \global\let\pgfpositionnodelaterpath\pgfpositionnodelaterpath%
        \fi%
        #4\pgfpoptype}%
      \pgfutil@ifundefined{pgf@sh@fbg@#1}{}
      {{\pgfusetype{.before background}\pgfidscope\pgfscope\csname pgf@sh@fbg@#1\endcsname\endpgfscope\endpgfidscope}}%
      {%
        \expandafter\pgfutil@for\expandafter\pgf@shape@com\expandafter:\expandafter=\csname pgf@sh@boxes@#1\endcsname\do{%
          {%
            \pgfusetype{.\pgf@shape@com}%
            \pgftransformshift{\pgf@sh@reanchor{#1}{\pgf@shape@com}}%
            \pgfapproximatenonlineartransformation%
            \expandafter\pgfqboxsynced\expandafter{\csname pgfnodepart\pgf@shape@com box\endcsname}%
          }%
        }%
      }%
      \pgfutil@ifundefined{pgf@sh@bfg@#1}{}%
      {{\pgfusetype{.behind foreground}\pgfidscope\pgfscope\csname pgf@sh@bfg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \pgfutil@ifundefined{pgf@sh@fg@#1}{}%
      {\pgfpushtype\pgfusetype{.foreground}\csname pgf@sh@fg@#1\endcsname#4\pgfpoptype}%
      \pgfutil@ifundefined{pgf@sh@ffg@#1}{}%
      {{\pgfusetype{.before foreground}\pgfidscope\pgfscope\csname pgf@sh@ffg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \ifpgflatenodepositioning%
        \pgf@shapes@late@pos@end%
        \pgfsys@endscope%
      \else%
        \expandafter\pgf@nodecallback\expandafter{\pgf@node@name}%
      \fi%
    }%
  }%
}%
\let\pgf@outer@adjust@hook\relax

\def\pgf@shapes@late@pos@begin{%
  % Rename node
  \edef\pgf@node@name{not yet positionedPGFINTERNAL\pgf@node@name}%
  % Interrupt bounding box!
  \pgfinterruptboundingbox%
    % Put everything in our box:
    \pgf@relevantforpicturesizetrue%
    \setbox\pgfpositionnodelaterbox=\hbox%
      \bgroup%
        \pgfsys@beginscope%
}%

\def\pgf@shapes@late@pos@end{%
       \pgfsys@endscope%
      \egroup% Close box
    \ifdim\pgf@picminx>\pgf@picmaxx\relax% happens for empty nodes
      \def\pgfpositionnodelaterminx{0.0pt}%
      \let\pgfpositionnodelaterminy\pgfpositionnodelaterminx%
      \let\pgfpositionnodelatermaxx\pgfpositionnodelaterminx%
      \let\pgfpositionnodelatermaxy\pgfpositionnodelaterminx%
    \else%
      \edef\pgfpositionnodelaterminx{\the\pgf@picminx}%
      \edef\pgfpositionnodelaterminy{\the\pgf@picminy}%
      \edef\pgfpositionnodelatermaxx{\the\pgf@picmaxx}%
      \edef\pgfpositionnodelatermaxy{\the\pgf@picmaxy}%
    \fi%
    \let\pgfpositionnodelatername=\pgf@node@name%
    \pgf@positionnodelater@macro%
  \endpgfinterruptboundingbox%
}%

\def\pgf@shift@node#1#2{%
  % This internal command shifts the recorded coordinates for node #1
  % by the vector #2. It is used to
  % correct the position of the node if the recorded coordinate
  % happens to be wrong
  {%
    \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
    \pgf@process{#2}%
    \advance\pgf@pt@x by\pgf@x%
    \advance\pgf@pt@y by\pgf@y%
    \pgfgettransform{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  }%
}%



% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = normal TeX text
% #4 = name for later reference
% #5 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfnode{rectangle}{center}{Hello}{hellonode}{\pgfusepath{stroke}}

\def\pgfnode#1#2#3#4#5{%
  {%
    \setbox\pgfnodeparttextbox=\hbox%
    {%
      \pgfinterruptpicture%
        {#3}%
      \endpgfinterruptpicture%
    }%
    \pgfmultipartnode{#1}{#2}{#4}{#5}%
  }
}%



% Create a node that is positioned later
%
% #1 = macro to be called after the next node has been created
%
% Description:
%
% You can use this command to create a node that is "positioned
% later". The idea is the following: Normally, when a node is created
% using a command like \pgfnode, the node is immediately inserted into
% the current picture. In particular, you have no chance to change the
% position of a created node after it has been create.
%
% Using \pgfpositionnodelater, you can change the default
% behaviour. This command is not a replacement for \pgfnode, but is
% called before such a command and will cause the following to happen:
% The node is created, but not inserted into the picture. Instead, it
% is stored in the box \pgfpositionnodelaterbox. Furthermore, the node
% is not relevant for the picture's bounding box, but a bounding box
% for the node is computed and stored in the macros
% \pgfpositionnodelaterboundboxminx to
% \pgfpositionnodelaterboundboxmaxy. Finally, the
% macro #1 is called with the following macros setup:
%
%   \pgfpositionnodelaterbox
%   A box register (box 0 by default) that stores the node's paths and
%   texts. You should move the contents of this box to a box of your
%   choice.
%
%   \pgfpositionnodelatername
%   The name of the just-created-node. This name will be the
%   originally "desired" name of the box plus the prefix "not yet
%   positioned boxPGFINTERNAL".
%
%   \pgfpositionnodelaterminx
%   \pgfpositionnodelatermaxx
%   \pgfpositionnodelaterminy
%   \pgfpositionnodelatermaxy
%   These four macros store the bounding box as dimensions that are
%   guarenteed to end with "pt".
%
% By setting #1 to \relax (which is the default), you can switch off
% the whole mechanism
%
% Once a late node has been created, you can add arbitrary code in the
% same picture. Then, at some later point, you call
% \pgfpositionnodenow to finally position the node at a given position.
%
% When \pgfpositionnodenow is called, the macros mentioned above
% should have the exact same values they had when #1 is called.

\def\pgfpositionnodelater#1{%
  \let\pgf@positionnodelater@macro=#1%
  \ifx\pgf@positionnodelater@macro\relax%
    \pgflatenodepositioningfalse%
  \else%
    \pgflatenodepositioningtrue%
  \fi%
}%
\newif\ifpgflatenodepositioning
\pgfpositionnodelater{\relax}%
\def\pgfpositionnodelaterbox{0}%




% Position a node that has been scheduled for later insertion
%
% #1 = position in the picture, where the original anchor should go,
%      now
%
% Description:
%
% This command works in concert with \pgfpositionnodelater, see the
% description there. When \pgfpositionnodenow is called, the macros
% \pgfpositionnodelaterbox and so on should be set to the values they
% had when the macro given to \pgfpositionnodelater was called. Then,
% the box described by these macros will be inserted into the picture
% at the position given #1. More precisely, the original node will
% have been positioned such that the anchor given upon invocation is
% at (0,0) and the node is now shifted by #1 before being inserted
% into the actual picture.

\def\pgfpositionnodenow#1{%
  \pgfinterruptpath%
  {%
    \pgfpointtransformed{#1}%
    \edef\pgf@temp@shift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
    \pgftransformreset%
    \pgftransformshift{\pgf@temp@shift}%
    \pgfsys@pictureboxsynced\pgfpositionnodelaterbox%
    \pgf@shift@node{\pgfpositionnodelatername}{\pgf@temp@shift}%
    % Bounding box update...
    \pgfpointtransformed{\pgfqpoint{\pgfpositionnodelaterminx}{\pgfpositionnodelaterminy}}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}
    \pgfpointtransformed{\pgfqpoint{\pgfpositionnodelatermaxx}{\pgfpositionnodelatermaxy}}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}
    % Naming and callbacks
    \expandafter\pgfpositionnodenow@rename\pgfpositionnodelatername\relax%
  }%
  % Late setup%
  {%
    \csname pgf@lns@\pgfpositionnodelatername\endcsname%
    \expandafter\global\expandafter\let\csname pgf@lns@\pgfpositionnodelatername\endcsname\relax%
  }%
  \endpgfinterruptpath%
}%

\def\pgfpositionnodenow@rename not yet positionedPGFINTERNAL#1\relax{%
  \pgfnoderename{#1}{not yet positionedPGFINTERNAL#1}
}%



% "Fake" a node
%
% #1 = node name
%
% Description:
%
% This command will setup things so that it "looks like" a node named
% #1 has been created, but, in reality, no node is created. The idea
% is that a node created in this way can be referenced by systems
% using the late positioning, which will only create the node later
% on.
%
\def\pgffakenode#1{%
  \edef\pgf@temp{\ifpgflatenodepositioning not yet positionedPGFINTERNAL\fi#1}%
  \expandafter\gdef\csname pgf@sh@ns@\pgf@temp\endcsname{coordinate}%
  \expandafter\gdef\csname pgf@sh@np@\pgf@temp\endcsname{\def\centerpoint{\pgfpointorigin}}%
  \expandafter\gdef\csname pgf@sh@nt@\pgf@temp\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
  \expandafter\global\expandafter\let\csname pgf@sh@ma@\pgf@temp\endcsname\pgfutil@empty%
  \expandafter\xdef\csname pgf@sh@pi@\pgf@temp\endcsname{\pgfpictureid}%
}%



% Specify code that should be executed after a node has been created
%
% #1 = node name
% #2 = later code
%
% Description:
%
% This macro allows you to provide some code #2 that will be executed
% right after a node has been positioned using \pgfpositionnodenow. If
% the node has already been positioned (if the late positioning is not
% switched on), nothing happens.

\def\pgfnodepostsetupcode#1#2{%
  \ifpgflatenodepositioning%
    \expandafter\ifx\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname\relax%
      \expandafter\gdef\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname{#2}%
    \else%
      \expandafter\pgfutil@g@addto@macro\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname{#2}%
    \fi%
  \fi%
}%



% Alias a node
%
% #1 = new node name
% #2 = existing node name
%
% Description:
%
% This command allows you to subsequently access the node #2 using the
% name #1.
%
% Example:
%
% \pgfnode{rectangle}{center}{Hallo}{hellonode}{}
% \pgfnodealias{mynode}{hellonode}

\def\pgfnodealias#1#2{%
  \pgf@node@gnamelet{pgf@sh@ns@#1}{pgf@sh@ns@#2}%
  \pgf@node@gnamelet{pgf@sh@np@#1}{pgf@sh@np@#2}%
  \pgf@node@gnamelet{pgf@sh@nt@#1}{pgf@sh@nt@#2}%
  \pgf@node@gnamelet{pgf@sh@pi@#1}{pgf@sh@pi@#2}%
  \pgf@node@gnamelet{pgf@sh@ma@#1}{pgf@sh@ma@#2}%
  \pgf@nodecallback{#1}%
}%
\def\pgf@node@gnamelet#1#2{%
  \expandafter\let\expandafter\pgf@temp\csname #2\endcsname%
  \expandafter\global\expandafter\let\csname #1\endcsname=\pgf@temp%
}%

% Rename a node
%
% #1 = new name
% #2 = old name
%
% Description:
%
% Renames a node. This is like an alias, only the memory used for the
% old name is freed.

\def\pgfnoderename#1#2{%
  \pgfnodealias{#1}{#2}%
  \expandafter\global\expandafter\let\csname pgf@sh@ns@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@np@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@nt@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@pi@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@ma@#2\endcsname\relax
}%




% Quickly create a coordinate node
%
% #1 = name
% #2 = coordinate
%
% Description:
%
% Creates a node of shape coordinate. The following have the same
% effect, only the second is much faster:
%
% { \pgftransformshift{\pgfpoint{1cm}{2cm} \pgfnode{coordinate}{center}{}{foo}{} }
% \pgfcoordinate{foo}{\pgfpoint{1cm}{2cm}}

\def\pgfcoordinate#1#2{%
  \edef\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty% do nothing
  \else%
    \ifpgflatenodepositioning%
      {\pgftransformshift{#2}\pgfnode{coordinate}{center}{}{#1}{}}%
    \else%
      \pgf@process{\pgfpointtransformed{#2}}%
      \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{coordinate}%
      \expandafter\xdef\csname pgf@sh@np@#1\endcsname{%
        \noexpand\def\noexpand\centerpoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      }
      \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
      \expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\pgfutil@empty%
      \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
    \fi%
  \fi%
}%

\def\pgf@sh@redeferredanchor#1#2{% CJ
  \expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @#1\endcsname{#2}}% CJ






\def\pgf@sh@resavedanchor#1#2{%
  \pgf@process{#2}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    }}%
  \pgf@sh@marshal%
}%


\def\pgf@sh@resaveddimen#1#2{%
  {#2\global\pgf@x=\pgf@x}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\the\pgf@x}%
    }}%
  \pgf@sh@marshal%
}%

\def\pgf@sh@resavedmacro#1#2{%
    \let#1\pgfutil@empty%
    \def\addtosavedmacro##1{%
        \expandafter\def\expandafter\pgf@sh@addtomacro@temp\expandafter{#1\noexpand\def\noexpand##1{##1}}%
        {\expandafter\pgfutil@toks@\expandafter{\pgf@sh@addtomacro@temp}\expandafter}%
        \expandafter\def\expandafter#1\expandafter{\the\pgfutil@toks@}%
    }%
  #2\relax%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedmacros{%
      \noexpand\def\noexpand#1{#1}%
    }}%
  \pgf@sh@marshal%
}%

% Invoke an anchor
\def\pgf@sh@reanchor#1#2{%
  \pgfutil@ifundefined{pgf@anchor@#1@#2}%
  {%
    \pgfutil@ifundefined{pgf@anchor@generic@#2}{%
        \pgfmathsetcounter{pgf@counta}{#2}%
        \csname pgf@anchor@#1@border\endcsname{\pgfqpointpolar{\the\c@pgf@counta}{1pt}}%
    }{%
        \csname pgf@anchor@generic@#2\endcsname{#1}%
    }%
  }%
  {\csname pgf@anchor@#1@#2\endcsname}%
}%

% Defines a generic anchor, i.e. one which gets the associated shape
% as first argument.
%
% #1: the anchor name.
% #2: the code of the anchor. It may depend upon '##1', the shape's
% name.
%
% The anchor will be defined locally in the current TeX scope.
%
% If the anchor will be referenced later by \pgfpointanchor, the macro \pgfreferencednodename
% can be used to query the referenced node's name.
% This macro is not defined during node creation.
\def\pgfdeclaregenericanchor#1#2{%
  \expandafter\def\csname pgf@anchor@generic@#1\endcsname##1{#2}%
}%


% Retrieves an anchor of a shape
%
% #1 = name
% #2 = anchor or a number (corresponding to a degree)
%
% Description:
%
% This command yields a point at the anchor of the given named shape.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointanchor{hellonode}{center}}

\def\pgfpointanchor#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\pgfutil@ifundefined{pgf@sh@ns@not yet positionedPGFINTERNAL#1}{%
      \pgferror{No shape named `#1' is known}}{
      % else, fail silently
    }%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      \edef\pgfreferencednodename{#1}% for use inside of anchors.
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname
      \pgf@sh@reanchor{\csname pgf@sh@ns@#1\endcsname}{#2}%
      {%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform@glob%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform@glob%
    }%
  }%
}%

\def\pgf@shape@interpictureshift#1{%
  \expandafter\ifx\csname pgf@sh@pi@#1\endcsname\pgfpictureid%
  \else%
    \pgfsys@getposition{\csname pgf@sh@pi@#1\endcsname}\pgf@shape@original@pos%
    \pgfsys@getposition{\pgfpictureid}\pgf@shape@current@pos%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@current@pos}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@original@pos}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
  \fi%
}%



% Retrieves a border point of a shape
%
% #1 = name
% #2 = another point
%
% Description:
%
% This command yields a point on the border of the shape that is on a
% straight line from the center to the point #2.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointshapeborder{hellonode}{\pgfpoint{2cm}{1cm}}
% \pgfpathlineto{\pgfpoint{2cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfpointshapeborder#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\pgferror{No shape named `#1' is known}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      \edef\pgfreferencednodename{#1}% for use inside of anchors.
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname%
      {%
        \pgf@process{\pgfpointtransformed{#2}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgftransforminvert%
        \pgf@pos@transform@glob%
        \pgf@xa=\pgf@x%
        \pgf@ya=\pgf@y%
        \pgf@process{\csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @center\endcsname}%
        \pgf@process{\pgf@shape@interpictureshift{#1}}%%
        \advance\pgf@xa by-\pgf@x%
        \advance\pgf@ya by-\pgf@y%
        \csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @border\endcsname{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform@glob%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform@glob%
    }%
  }%
}%


% Retrieve the list of node parts of a shape
%
% #1 = a macro
% #2 = a shape name
%
% Description:
%
% Stores the list of node parts of a shape #2 in the macro #1.
%
% Example:
%
% \pgfgetnodeparts\mylist{circle split}
%
% This will set \mylist\ to "text,lower"

\def\pgfgetnodeparts#1#2{%
  \expandafter\let\expandafter#1\csname pgf@sh@boxes@#2\endcsname%
}%


% Declares a shape type
%
% #1 = shape type
% #2 = shape specification
%
% Description:
%
% This command declares a new shape type. The shape specification
% should contain the following commands:
%
% - \savedanchor
%   This command takes two arguments: a name and some code. The point
%   specified by the code (the \pgf@x and \pgf@y values resulting from
%   executing the code, to be precise), will be stored under the given
%   name. Whenever, later on, an anchor is invoked these stored points
%   will be available. The \saveddimen works like \savedanchor, only a
%   single dimension is stored (taken from \pgf@x).
%   When a savedanchor is calculated, the height/width/depth of the
%   boxes mentioned in \nodeparts can be used.
%
% - \anchor
%   Specifies an anchor. This command takes two arguments: an anchor
%   name and some code for computing the anchor. When the anchor
%   computation starts, all shape points and shape dimension will be
%   setup.
%
% - \anchorborder
%   This command should compute a point on the border of the
%   shape. When the code is called, \pgf@x and \pgf@y will have been
%   preinitialised with a direction.
%
% - \behindbackgroundpath
%   Some things to be draw behind everything.
%
% - \backgroundpath
%   A path that is drawn behind the main box. How this path is used
%   depends on how \pgfshape is called.
%
% - \beforebackgroundpath
%   Some things to be draw before the background path, but behind the
%   main box.
%
% - \behindforegroundpath
%   Some things to be draw on top of the main box.
%
% - \foregroundpath
%   A path that is drawn on top of all of the above. How this path is
%   used depends on how \pgfshape is called.
%
% - \beforeforegroundpath
%   Some things to be draw before everything.
%
% - \nodeparts
%   List of node parts that make up the shape. For each entry XYZ in
%   the list there must be a box named \pgfnodepartXYZbox (possibly
%   ``redirected'' to some different box using \let). Each such box
%   will be placed at the anchor XYZ.
%   By default, \nodeparts is just {text}. Thus, there will be one
%   node part box named \pgfnodeparttextbox and this node will be
%   placed at the anchor text.
%
%
% Example:
%
% See the definition of rectangle, below.

\long\def\pgfdeclareshape#1#2{%
  {%
    \def\pgf@sm@shape@name{#1}%
    \let\savedanchor=\pgf@sh@savedanchor
    \let\saveddimen=\pgf@sh@saveddimen
    \let\savedmacro=\pgf@sh@savedmacro% MW
    \let\deferredanchor=\pgf@sh@deferredanchor% CJ
    \let\anchor=\pgf@sh@anchor
    \let\anchorborder=\pgf@sh@anchorborder
    \let\behindbackgroundpath=\pgf@sh@behindbgpath
    \let\backgroundpath=\pgf@sh@bgpath
    \let\beforebackgroundpath=\pgf@sh@beforebgpath
    \let\behindforegroundpath=\pgf@sh@behindfgpath
    \let\foregroundpath=\pgf@sh@fgpath
    \let\beforeforegroundpath=\pgf@sh@beforefgpath
    \let\nodeparts=\pgf@sh@boxes
    \let\inheritsavedanchors=\pgf@sh@inheritsavedanchors
    \let\inheritanchor=\pgf@sh@inheritanchor
    \let\inheritanchorborder=\pgf@sh@inheritanchorborder
    \let\inheritbehindbackgroundpath=\pgf@sh@inheritbehindbgpath
    \let\inheritbackgroundpath=\pgf@sh@inheritbgpath
    \let\inheritbeforebackgroundpath=\pgf@sh@inheritbeforebgpath
    \let\inheritbehindforegroundpath=\pgf@sh@inheritbehindfgpath
    \let\inheritforegroundpath=\pgf@sh@inheritfgpath
    \let\inheritbeforeforegroundpath=\pgf@sh@inheritbeforefgpath
    \let\inheritnodeparts=\pgf@sh@inheritboxes
    \anchorborder{\csname pgf@anchor@#1@center\endcsname}%
    \anchor{text}{\pgfpointorigin}%
    \nodeparts{text}%
    \expandafter\global\expandafter\let\csname pgf@sh@s@\pgf@sm@shape@name\endcsname=\pgfutil@empty%
    #2%
  }%
}%

\def\pgf@sh@savedanchor#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resavedanchor{#1}{#2}}}%
\def\pgf@sh@saveddimen#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resaveddimen{#1}{#2}}}%
 \def\pgf@sh@savedmacro#1#2{% MW
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resavedmacro{#1}{#2}}}% MW
\def\pgf@sh@anchor#1#2{\expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @#1\endcsname{#2}}%
\def\pgf@sh@deferredanchor#1#2{% CJ
  \expandafter\pgfutil@g@addto@macro
    \csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@redeferredanchor{#1}{#2}}}% CJ
\def\pgf@sh@anchorborder#1{\expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @border\endcsname##1{\pgf@process{##1}#1}}%
\long\def\pgf@sh@behindbgpath#1{\expandafter\gdef\csname pgf@sh@bbg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@bgpath#1{\expandafter\gdef\csname pgf@sh@bg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@beforebgpath#1{\expandafter\gdef\csname pgf@sh@fbg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@behindfgpath#1{\expandafter\gdef\csname pgf@sh@bfg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@fgpath#1{\expandafter\gdef\csname pgf@sh@fg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@beforefgpath#1{\expandafter\gdef\csname pgf@sh@ffg@\pgf@sm@shape@name\endcsname{#1}}%
\def\pgf@sh@boxes#1{\expandafter\gdef\csname pgf@sh@boxes@\pgf@sm@shape@name\endcsname{#1}}%

\def\pgf@sh@inheritsavedanchors[from=#1]{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\csname pgf@sh@s@#1\endcsname}}%

\def\pgf@sh@inheritanchor[from=#1]#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\pgf@sm@shape@name @#2\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@#2\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritanchorborder[from=#1]{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\pgf@sm@shape@name @border\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@border\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritor#1#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@sh@#1@\pgf@sm@shape@name\endcsname=\expandafter\noexpand\csname
    pgf@sh@#1@#2\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritbehindbgpath[from=#1]{\pgf@sh@inheritor{bbg}{#1}}%
\def\pgf@sh@inheritbgpath[from=#1]{\pgf@sh@inheritor{bg}{#1}}%
\def\pgf@sh@inheritbeforebgpath[from=#1]{\pgf@sh@inheritor{fbg}{#1}}%
\def\pgf@sh@inheritbehindfgpath[from=#1]{\pgf@sh@inheritor{bfg}{#1}}%
\def\pgf@sh@inheritfgpath[from=#1]{\pgf@sh@inheritor{fg}{#1}}%
\def\pgf@sh@inheritbeforefgpath[from=#1]{\pgf@sh@inheritor{ffg}{#1}}%
\def\pgf@sh@inheritboxes[from=#1]{\pgf@sh@inheritor{boxes}{#1}}%



%
% Coordinate. This shape is special: It is only used to reference a
% point for later usage. Nothing is drawn, all anchors are identical
% to the center.
%

\pgfdeclareshape{coordinate}
{%
  \savedanchor\centerpoint{%
    % x
    \pgf@x=.5\wd\pgfnodeparttextbox%
    % y
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by -.5\dp\pgfnodeparttextbox%
  }%

  \anchor{center}{\centerpoint}%
  \anchor{north}{\centerpoint}%
  \anchor{north west}{\centerpoint}%
  \anchor{north east}{\centerpoint}%
  \anchor{west}{\centerpoint}%
  \anchor{east}{\centerpoint}%
  \anchor{mid}{\centerpoint}%
  \anchor{mid west}{\centerpoint}%
  \anchor{mid east}{\centerpoint}%
  \anchor{base}{\centerpoint}%
  \anchor{base west}{\centerpoint}%
  \anchor{base east}{\centerpoint}%
  \anchor{south}{\centerpoint}%
  \anchor{south west}{\centerpoint}%
  \anchor{south east}{\centerpoint}%
  \anchorborder{\centerpoint}%

  \nodeparts{}% no text
}%


% Value keys for shapes:
%
% /pgf/inner xsep     : recommended inner x separation
% /pgf/inner ysep     : recommended inner y separation
% /pgf/outer xsep     : recommended outer x separation
% /pgf/outer ysep     : recommended outer y separation
% /pgf/minimum width  : recommended minimum width
% /pgf/minimum height : recommended minimum height

\pgfset{
  inner xsep/.initial     =.3333em,
  inner ysep/.initial     =.3333em,
  inner sep/.style        ={/pgf/inner xsep=#1,/pgf/inner ysep=#1},
  outer xsep/.initial     =.5\pgflinewidth,
  outer ysep/.initial     =.5\pgflinewidth,
  outer sep/.code         =\pgf@handle@outer@sep{#1},
  minimum width/.initial  =1pt,
  minimum height/.initial =1pt,
  minimum size/.style     ={/pgf/minimum width=#1,/pgf/minimum height=#1},
}%



\def\pgf@handle@outer@sep#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@auto@text%
    \def\pgf@outer@adjust@hook{%
      \pgftransformationadjustments%
      \pgfkeyssetvalue{/pgf/outer xsep}{.5\pgflinewidth*\pgfhorizontaltransformationadjustment}%
      \pgfkeyssetvalue{/pgf/outer ysep}{.5\pgflinewidth*\pgfverticaltransformationadjustment}%
      \pgf@outer@auto@adjust@hook%
    }%
  \else%
    \pgfkeyssetvalue{/pgf/outer xsep}{#1}%
    \pgfkeyssetvalue{/pgf/outer ysep}{#1}%
  \fi%
}%
\def\pgf@auto@text{auto}%

\let\pgf@outer@auto@adjust@hook\relax


% Keys for rotating the shape border.
% (may not be supported by all shapes)
%
% /pgf/shape border uses incircle : Calculate the shape border using the incircle
%                                   around the node contents (+inner sep).
%
% /pgf/shape border rotate        : Angle of independent border rotation.

\newif\ifpgfshapeborderusesincircle
\pgfkeys{/pgf/shape border uses incircle/.is if=pgfshapeborderusesincircle}%
\pgfkeys{/pgf/shape border rotate/.initial=0}%

%
% Rectangle
%

\pgfdeclareshape{rectangle}
{%
  \savedanchor\northeast{%
    % Calculate x
    %
    % First, is width < minimum width?
    \pgf@x=\the\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by 2\pgf@xc%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    % Now, calculate right border: .5\wd\pgfnodeparttextbox + .5 \pgf@x + outer sep
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    % Calculate y
    %
    % First, is height+depth < minimum height?
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by 2\pgf@yc%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    % Now, calculate upper border: .5\ht-.5\dp + .5 \pgf@y + outer sep
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    \advance\pgf@y by.5\ht\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }%

  \savedanchor\southwest{%
      % Calculate x
      %
      % First, is width < minimum width?
      \pgf@x=\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
      \advance\pgf@x by 2\pgf@xc%
      \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
      \ifdim\pgf@x<\pgf@xb%
        % yes, too small. Enlarge...
        \pgf@x=\pgf@xb%
      \fi%
      % Now, calculate left border: .5\wd\pgfnodeparttextbox - .5 \pgf@x - outer sep
      \pgf@x=-.5\pgf@x%
      \advance\pgf@x by.5\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
      \advance\pgf@x by-\pgf@xa%
      % Calculate y
      %
      % First, is height+depth < minimum height?
      \pgf@y=\ht\pgfnodeparttextbox%
      \advance\pgf@y by\dp\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
      \advance\pgf@y by 2\pgf@yc%
      \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
      \ifdim\pgf@y<\pgf@yb%
        % yes, too small. Enlarge...
        \pgf@y=\pgf@yb%
      \fi%
       % Now, calculate upper border: .5\ht-.5\dp - .5 \pgf@y - outer sep
      \pgf@y=-.5\pgf@y%
      \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
      \advance\pgf@y by.5\ht\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
      \advance\pgf@y by-\pgf@ya%
  }%

  %
  % Anchors
  %
  \anchor{center}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \pgf@y=.5\pgf@y%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base}{\pgf@anchor@rectangle@center\pgf@y=0pt}%
  \anchor{north}{
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }%
  \anchor{south}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }%
  \anchor{west}{
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid west}{\southwest\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base west}{\southwest\pgf@y=0pt}%
  \anchor{north west}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa}%
  \anchor{south west}{\southwest}%
  \anchor{east}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid east}{\northeast\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base east}{\northeast\pgf@y=0pt}%
  \anchor{north east}{\northeast}%
  \anchor{south east}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
  }%
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%

  %
  % Background path
  %
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  }%
}%


% Special current path start coordinate:
\expandafter\def\csname pgf@sh@ns@current subpath start\endcsname{coordinate}%
\expandafter\def\csname pgf@sh@np@current subpath start\endcsname{%
  \def\centerpoint{\expandafter\pgfqpoint\pgfsyssoftpath@lastmoveto}%
}%
\expandafter\def\csname pgf@sh@nt@current subpath start\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current subpath start\endcsname{\pgfpictureid}%



% Special  current bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current bounding box\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
  \def\northeast{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
}%
\expandafter\def\csname pgf@sh@nt@current bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current bounding box\endcsname{\pgfpictureid}%


% Special  current path bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current path bounding box\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current path bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@pathminx}{\pgf@pathminy}}%
  \def\northeast{\pgfqpoint{\pgf@pathmaxx}{\pgf@pathmaxy}}%
}%
\expandafter\def\csname pgf@sh@nt@current path bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current path bounding box\endcsname{\pgfpictureid}%


% Special  current page bounding box rectangle:
\expandafter\def\csname pgf@sh@ns@current page\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current page\endcsname{%
  \def\southwest{\pgfpointorigin}%
  \def\northeast{\pgfpoint{\pgfsys@thepagewidth}{\pgfsys@thepageheight}}%
}%
\expandafter\def\csname pgf@sh@nt@current page\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current page\endcsname{pgfpageorigin}%


% Special scope bounding box rectangle:
\pgfkeys{/pgf/local bounding box/.code={%
    \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
    \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
      \def\southwest{\pgfqpoint{\csname pgf@lbb@minx@#1\endcsname}{\csname pgf@lbb@miny@#1\endcsname}}%
      \def\northeast{\pgfqpoint{\csname pgf@lbb@maxx@#1\endcsname}{\csname pgf@lbb@maxy@#1\endcsname}}%
    }
    \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
    \expandafter\gdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}
    \expandafter\gdef\csname pgf@lbb@maxx@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@minx@#1\endcsname{16000pt}%
    \expandafter\gdef\csname pgf@lbb@maxy@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@miny@#1\endcsname{16000pt}%
    \pgf@size@hookedtrue%
    \expandafter\def\expandafter\pgf@path@size@hook\expandafter{\pgf@path@size@hook\pgf@lbb@do{#1}}
  },
  /pgf/freeze local bounding box/.code={%
    {%
      \csname pgf@sh@np@#1\endcsname%
      \southwest%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \northeast%
      \expandafter\xdef\csname pgf@sh@np@#1\endcsname{%
        \noexpand\def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
        \noexpand\def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      }%
    }%
  },
}%
\def\pgf@lbb@do#1{%
  \ifdim\pgf@size@hook@x<\csname pgf@lbb@minx@#1\endcsname\expandafter\xdef\csname pgf@lbb@minx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@x>\csname pgf@lbb@maxx@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@y<\csname pgf@lbb@miny@#1\endcsname\expandafter\xdef\csname pgf@lbb@miny@#1\endcsname{\the\pgf@size@hook@y}\fi%
  \ifdim\pgf@size@hook@y>\csname pgf@lbb@maxy@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxy@#1\endcsname{\the\pgf@size@hook@y}\fi%
}%

%
% Circle
%

\pgfdeclareshape{circle}
%
% Draws a circle around the text
%
{%
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }%

  \saveddimen\radius{%
    %
    % Calculate ``height radius''
    %
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yb%
    %
    % Calculate ``width radius''
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    %
    % Calculate length of radius vector:
    %
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    %
    % If necessary, adjust radius so that the size requirements are
    % met:
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    %
    % Now, add larger of outer separations.
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }%

  %
  % Anchors
  %
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base}{\centerpoint\pgf@y=0pt}%
  \anchor{north}{\centerpoint\advance\pgf@y by\radius}%
  \anchor{south}{\centerpoint\advance\pgf@y by-\radius}%
  \anchor{west}{\centerpoint\advance\pgf@x by-\radius}%
  \anchor{east}{\centerpoint\advance\pgf@x by\radius}%
  \anchor{mid west}{\centerpoint\advance\pgf@x by-\radius\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{mid east}{\centerpoint\advance\pgf@x by\radius\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base west}{\centerpoint\advance\pgf@x by-\radius\pgf@y=0pt}%
  \anchor{base east}{\centerpoint\advance\pgf@x by\radius\pgf@y=0pt}%
  \anchor{north west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }%
  \anchor{south west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }%
  \anchor{north east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }%
  \anchor{south east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }%
  \anchorborder{%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\radius}{\radius}}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%

  %
  % Background path
  %
  \backgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
  }%
}%





\endinput


==> pgfrcs.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ifx\eTeXrevision\undefined%
  \pgfutil@packageerror{PGF}{PGF requires etex in extended mode}{}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

\ifnum\eTeXversion<2
  \pgfutil@packageerror{PGF}{PGF requires etex version 2}{}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

% The purpose of this file is to define the command
% \ProvidesPackageRCS, which should be followed by an RCS id
% string. This command will also be available in plain TeX, where it
% prints out a message to the log.

\pgfutil@IfFileExists{pgf.revision.tex}{\input pgf.revision.tex } {%
    \def\pgfrevision{0}%
    \def\pgfversion{0.0}%
    \def\pgfversiondatetime{2014-07-01 00:00:00 +100}%
    \def\pgfrevisiondatetime{2014-07-01 00:00:00 +100}%
    \def\pgfversiondate{2014/07/01}%
    \def\pgfrevisiondate{2014/07/01}%
}

\begingroup
\catcode`\"=12
\pgfutil@IfUndefined{directlua}{}{%
    \directlua{pgf = {}; pgf.pgfversion = "\pgfversion"}%
}%
\endgroup

% \def\pgftypesetversion{\oldstylenums{3}.\oldstylenums{0}.\oldstylenums{1}}
% XXX : implement pretty-printing:
% which is better? 'version' is something like 3.0.1 . revision is
% 3.0.1-151-g62184b3 which might be better for instable builds
%\let\pgftypesetversion=\pgfversion
\let\pgftypesetversion=\pgfrevision


\ifx\pgfrcsloaded\undefined
\def\pgfrcsloaded{}

\edef\pgfrcsatcode{\the\catcode`\@}
\catcode`\@=11

% not used in PGF, deprecated
\def\ProvidesFileRCS{%
    \let\pgfrcs@final=\ProvidesFileRCS@
	\pgfrcs@parseinput
}
\def\ProvidesFileRCS@#1{%
    \ProvidesFile{#1}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]%
}

\def\pgf@remove@ext#1.#2\relax{%
    \def\pgfretval{#1}%
}%

\def\ProvidesPackageRCS{%
	\let\pgfrcs@final=\ProvidesPackageRCS@
	\pgfrcs@parseinput
}
\def\ProvidesPackageRCS@#1{%
    \pgf@remove@ext#1.\relax
    \edef\pgfrcs@marshal{{\pgfretval}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]}%
    \expandafter\ProvidesPackage\pgfrcs@marshal
}

% not used in PGF, deprecated
\def\ProvidesClassRCS{%
	\let\pgfrcs@final=\ProvidesClassRCS@
	\pgfrcs@parseinput
}
\def\ProvidesClassRCS@#1{%
    \pgf@remove@ext#1.\relax
    \edef\pgfrcs@marshal{{\pgfretval}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]}%
    \expandafter\ProvidesClass\pgfrcs@marshal
}

\def\pgfrcs@parseinput@bracket{[}%
\def\pgfrcs@parseinput@dollarsign{$}%

\def\pgfrcs@parseinput#1{%
	\def\pgfrcs@parseinput@{#1}%
	\ifx\pgfrcs@parseinput@\pgfrcs@parseinput@bracket%
		% still accept it if someone has written his own pgfrcs files with headers of sorts
		% \ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.7 2010/04/11 07:09:19 username Exp $
		\let\next=\pgfrcs@parseinput@opt
	\else
		\ifx\pgfrcs@parseinput@\pgfrcs@parseinput@dollarsign
			% still accept it if someone has written his own pgfrcs files with headers of sorts
			% \ProvidesPackageRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.7 2010/04/11 07:09:19 username Exp $
			\let\next\pgfrcs@parseinput@dollar
		\else
			% the new, normal pgf-way is \ProvidesPackageRCS{pgfcore.code.tex}
			\def\next{\pgfrcs@final{#1}}%
		\fi
	\fi
	\next
}
\def\pgfrcs@parseinput@opt#1] ${%
	% just backwards compatibility -- ignore the information, but parse the input tokens:
	\pgfrcs@parseinput@dollar
}%
\def\pgfrcs@parseinput@dollar#1${%
	\pgf@parseid $#1$%
	% we ignore pretty much everything except for the file name:
	\edef\pgfrcs@parseinput@{\pgf@rcsfile.\pgf@rcssuffix}%
	\expandafter\pgfrcs@final\expandafter{\pgfrcs@parseinput@}%
}%
% Get date and version from RCS Ids
\def\pgf@parseid $#1: #2.#3,v #4 #5/#6/#7 #8${%
  \pgf@parsercsfile$#2/$
  \def\pgf@rcssuffix{#3}
  \def\pgf@rcsrevision{#4}
  \def\pgf@rcsdate{#5/#6/#7}
}
\def\pgf@parsercsfile$#1/#2${
  \def\pgf@temp{#2}
  \ifx\pgf@temp\pgfutil@empty
    \def\pgf@rcsfile{#1}
  \else
    \pgf@parsercsfile$#2$
  \fi}


\ifx\ProvidesPackage\@undefined
    % plain tex
    \def\ProvidesPackage#1[#2]{\wlog{Loading package #1 version #2.}}
\fi

\ifx\ProvidesFile\@undefined
    % plain tex
    \def\ProvidesFile#1[#2]{\wlog{Loading file #1 version #2.}}
\fi

\ProvidesPackageRCS{pgfrcs.code.tex}

\catcode`\@=\pgfrcsatcode

\fi


% Local Variables:
% coding: undecided-unix
% End:


==> pgfsys.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgfsys.code.tex}


% Load key mechanism
\input pgfkeys.code.tex

% "pgf" is a family
\pgfkeys{/pgf/.is family}
\def\pgfset{\pgfqkeys{/pgf}}

% This if is needed *very* early
\newif\ifpgfpicture


%
% The following conversion functions are used to convert from TeX
% dimensions to postscript/pdf points.
%
{\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}

\def\pgf@sys@tonumber#1{\expandafter\Pgf@geT\the#1}

\def\pgf@sys@bp@correct#1{#1=0.99627#1}

\def\pgf@sys@bp#1{%
  {%
    \pgf@x=#1\relax%
    \pgf@x=0.99627\pgf@x%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \pgfutil@toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\pgfutil@toks@}%
  }%
}
\def\pgf@sys@pt#1{%
  {%
    \pgf@x=#1\relax%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \pgfutil@toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\pgfutil@toks@}%
  }%
}


% internal dimensions that are always present when pgsys is loaded.
\newdimen\pgf@x
\newdimen\pgf@y
\newdimen\pgf@xa
\newdimen\pgf@ya
\newdimen\pgf@xb
\newdimen\pgf@yb
\newdimen\pgf@xc
\newdimen\pgf@yc
\newdimen\pgf@xd
\newdimen\pgf@yd

\newwrite\w@pgf@writea
\newread\r@pgf@reada
\let\pgfutil@inputcheck=\r@pgf@reada

% internal counters that are always present when pgfsys is loaded
\newcount\c@pgf@counta
\newcount\c@pgf@countb
\newcount\c@pgf@countc
\newcount\c@pgf@countd

\newtoks\t@pgf@toka
\newtoks\t@pgf@tokb
\newtoks\t@pgf@tokc

% Ensure that math registers are the same (math is broken in case it
% is loaded first)
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc
\let\c@pgfmath@countd\c@pgf@countd





% In the following dummy definitions of the pgf system commands are
% given. The individual drivers must overwrite these definitions,
% preferably all of them. If some system command is used that has not
% been overwritten, the command fails with a warning.
%
% In some cases, some pgf system commands are just shorthands for a
% series of more complicated commands. In this case, a default
% implementation is given in this file, but a driver may choose to
% overwrite this default implementation with a more efficient
% version. For example, a closestroke is the same as a closepath
% followed by a stroking, but in pdf there is a special shorthand for
% this. So, the pdf driver overwrites \pgfsys@closestroke, while the
% postscript driver does not.
%
% The commands for which default implementations are available are
% given at the end.

\def\pgf@sys@fail#1{%
  \expandafter\ifx\csname pgf@sys@fail@#1\endcsname\pgfutil@empty%
  \else%
    \expandafter\global\expandafter\let\csname pgf@sys@fail@#1\endcsname=\pgfutil@empty%
    \pgfwarning{Your graphic driver \pgfsysdriver\space does not support #1. This warning is given only once}%
  \fi%
}



%
% Invocation commands
%

\def\pgfsys@invoke{\pgf@sys@fail{invoking specials}}
% This command is used whenever some literal text needs to be inserted
% into the resulting .pdf, .ps, or .dvi file. Note that most
% \pgfsys@xxxx commands will not directly call this command, but,
% rather, use the protocolling mechanism to record their literal
% text. It is then left to the discretion of the protocolling
% mechanism to insert the literal text at some appropriate, later
% time.
%
% This command should only be called when \pgfsys@beginpicture has
% been called previously and when the picture has not been suspended
% using \pgfsys@beginhbox.

\def\pgfsys@outerinvoke{\pgfsys@invoke}
% This command can be used to insert protocolled graphic commands
% outside any picture. This is extremely dangerous, but sometimes
% useful. By default, this command does the same as inside pictures.



%
%
% Path construction commands
%
%

\def\pgfsys@moveto#1#2{\pgf@sys@fail{path constructions}}
% This command is used to start a path at a specific point (#1,#2)
% or to move the current point of the current path to (#1,#2)
% without drawing anything upon stroking (the current path is
% `interrupted').
%
% The arguments must be dimensions (like |10pt|).
%
% Example:
%
% \pgfsys@moveto{10pt}{10pt}
% \pgfsys@lineto{0pt}{0pt}
% \pgfsys@stroke
%
% This will draw a line from (10pt,10pt) to the origin of the picture.

\def\pgfsys@lineto#1#2{\pgf@sys@fail{path constructions}}
% Continue the current path to (#1,#2) with a line.

\def\pgfsys@curveto#1#2#3#4#5#6{\pgf@sys@fail{path constructions}}
% Continue the current path with a bezier curve to (#5,#6). The
% control points of the curve are at (#1,#2) and (#3,#4).

\def\pgfsys@rect#1#2#3#4{\pgf@sys@fail{path constructions}}
% Append a rectangle to the current path whose lower left corner is at
% (#1,#2) and whose width/height is given by (#3,#4).
%
% This command can be `mapped back' to moveto and lineto commands, but
% it is included since pdf has a special, quick version of this command.

\def\pgfsys@closepath{\pgf@sys@fail{path constructions}}
% Close the current path. This results in joining the current point of
% the path with the point specified by the last moveto
% operation. Typically, this is preferable over using lineto to the
% last point specified by a moveto, since the line starting at this
% point and the line ending at this point will be smoothly joined by
% closepath.
%
% Example:
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@closepath
% \pgfsys@stroke
%
% versus
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
%
% The difference between the above will be that in the second triangle
% the corner at the origin will be wrong; it will just be the overlay
% of two lines going in different directions, not a sharp pointed
% corner.






%
%
% Stroking and filling commands
%
%

\def\pgfsys@stroke{\pgf@sys@fail{path usage}}
% Stroke the current path (as if it were drawn with a pen). A number
% of so-called graphic state parameters influence this, which can be
% set in different ways:
%
% - linewidth
%   The `thickness' of the line. A width of 0 is the thinnest width
%   renderable on the device. On a high-resolution printer this may
%   become invisible and should be avoided. A good choice is 0.4pt,
%   which is the default.
%
% - stroke color
%   This special color is used for stroking. If it is not set, the
%   current color is used.
%
% - cap
%   The cap describes how the endings of lines a drawn. A round cap
%   adds a little half circle to these endings. A butt cap ends the
%   lines exactly at the end (or start) point without anything
%   added. A rectangular cap ends the lines like the butt cap, but the
%   lines protrude over the endpoint by the line thickness. (See also
%   the pdf or postscript manual). If the path has been closed, no cap
%   is drawn.
%
% - join
%   This describes how a bend (a join) in a path is rendered. A round
%   join draws bends using small arcs. A bevel join just draws the two
%   lines and then fills the join minimally so that it becomes
%   convex. A miter join extends the lines so that they form a single
%   sharp corner, but only up to a certain miter limit. (See the pdf
%   or postscript manual once more).
%
% - dash
%   The line may be dashed according to a dashing pattern.
%
% - clipping area
%   If a clipping area is established, only those parts of the path
%   that are inside the clipping area will be drawn.
%
% In addition to stroking a path, the path may also be used for
% clipping after it has been stroked. This will happen if the
% \pgfsys@clipnext is used prior to this command, see there for
% details.

\def\pgfsys@fill{\pgf@sys@fail{path usage}}
% This command fills the area surrounded by the current path. If the
% path has not yet been closed, it is closed prior to filling. The
% path itself is not stroked. For self-intersecting paths or paths
% consisting of multiple parts, the nonzero winding number rule is
% used to determine whether a point is inside or outside the
% path, except if \ifpgfsys@eorule holds -- in which case the even-odd
% rule should be used. (See the pdf or postscript manual for details.)
%
% The following graphic state parameters influence the filling:
%
% - fill color
%   If the fill color is not especially set, the current color is
%   used.
%
% - clipping area
%   If a clipping area is established, only those parts of the filling
%   area that are inside the clipping area will be drawn.
%
% In addition to filling the path, the path will also be used for
% clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@fillstroke{\pgf@sys@fail{path usage}}
% First, the path is filled, then the path is stroked. If the fill and
% stroke colors are the same (or if they are not specified and the
% current color is used), this yields almost the same as a
% \pgfsys@fill. However, due to the line thickness of the stroked
% path, the fillstroked area will be slightly larger.
%
% In addition to stroking and filling the path, the path will also be
% used for clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@clipnext{\pgf@sys@fail{path usage}}
% This command should be issued after a path has been constructed, but
% before it has been stroked and/or filled or discarded. When the
% command is used, the next stroking/filling/discarding command will
% first be executed normally. Then, afterwards, the just-used path
% will be used for subsequent clipping. If there has already been a
% clipping region, this region is intersected with the new clipping
% path (the clipping cannot get bigger). The nonzero winding number
% rule is used to determine whether a point is inside or outside the
% clipping area or the even-odd rule, depending on whether
% \ifpgfsys@eorule holds.

\def\pgfsys@discardpath{\pgf@sys@fail{path usage}}
% Normally, this command should `throw away' the current path.
% However, after \pgfsys@clipnext has been called, the current path
% should subsequently be used for clipping. See \pgfsys@clipnext for
% details.

\def\pgfsys@closestroke{\pgfsys@closepath\pgfsys@stroke}
% This command should have the same effect as first closing the path
% and then stroking it.

\newif\ifpgfsys@eorule
% Decides, whether even-odd filling and clipping is
% to be used or normal the non-zero winding number rule. See the
% pdf-documentation for details on what these rules are.




%
%
% Stroking options
%
%
\def\pgfsys@setlinewidth#1{\pgf@sys@fail{setting the line width}}
% Sets the width of lines, when stroked, to #1, which must be a TeX
% dimension (as text).

\def\pgfsys@buttcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a butt cap. See \pgfsys@stroke.

\def\pgfsys@roundcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a round cap. See \pgfsys@stroke.

\def\pgfsys@rectcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a rectangular cap. See \pgfsys@stroke.

\def\pgfsys@miterjoin{\pgf@sys@fail{setting the line join}}
% Sets the join to a miter join. See \pgfsys@stroke.

\def\pgfsys@setmiterlimit#1{\pgf@sys@fail{setting the line cap}}
% Sets the miter limit of lines to #1. See the pdf or postscript
% documentation.

\def\pgfsys@roundjoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a round join. See \pgfsys@stroke.

\def\pgfsys@beveljoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a bevel join. See \pgfsys@stroke.

\def\pgfsys@setdash#1#2{\pgf@sys@fail{setting the dashing pattern}}
% Sets the dashing patter. #1 should be a list of lengths separated by
% commas. #2 should be a single dimension.
%
% The list of values in #1 is used to determine the lengths of the
% `on' phases of the dashing and of the `off' phases. For example, if
% #1 is `3pt,4pt', then the dashing pattern is `3pt on followed by 4pt
% off, followed by 3pt on, followed by 4pt off, and so on'. A pattern
% of `.5pt,4pt,3pt,1.5pt' means `.5pt on, 4pt off, 3pt on, 1.5pt off, .5pt on,
% ...'. If the number of entries is odd, the last one is used twice,
% so `3pt' means `3pt on, 3pt off, 3pt on, 3pt off,...'. An empty list
% means `always on'.
%
% The second argument determines the `phase' of the pattern. For
% example, for a pattern of `3pt,4pt' and a phase of `1pt', the pattern
% would start: `2pt on, 4pt off, 3pt on, 4pt off, 3pt on, 4pt off...'.





%
%
% Color stuff
%
%

\def\pgfsys@color@rgb@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given rgb tuple
% (numbers between 0 and 1).
%
% Example: Make stroked text dark red: \pgfsys@color@rgb@stroke{0.5}{0}{0}
%
% The special stroking color is only used if the stroking color has
% been set since the last \pgfutil@color command. Thus, each \pgfutil@color command
% should reset both the stroking and filling colors.

\def\pgfsys@color@rgb@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given rgb tuple
% (numbers between 0 and 1). This color may be different from the
% stroking color.

\def\pgfsys@color@rgb#1#2#3{\pgfsys@color@rgb@stroke{#1}{#2}{#3}\pgfsys@color@rgb@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations. This is a
% ``low-level'' version of the \pgfutil@color command. It is currently only
% used by the plain tex version to support colors.

\def\pgfsys@color@cmyk@stroke#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cymk tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmyk@fill#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cymk tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmyk#1#2#3#4{\pgfsys@color@cmyk@stroke{#1}{#2}{#3}{#4}\pgfsys@color@cmyk@fill{#1}{#2}{#3}{#4}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@cmy@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cym tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmy@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cym tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmy#1#2#3{\pgfsys@color@cmy@stroke{#1}{#2}{#3}\pgfsys@color@cmy@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@gray@stroke#1{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given gray level
% (number between 0 and 1).

\def\pgfsys@color@gray@fill#1{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given gray level
% (number between 0 and 1).

\def\pgfsys@color@gray#1{\pgfsys@color@gray@stroke{#1}\pgfsys@color@gray@fill{#1}}
% Sets the color used for filling and stroking operations.

\newif\ifpgfsys@color@reset@inorder
% This if decides whether the color resetting of the
% \pgfsys@color@reset command may assume that all color commands are
% given ``in order.'' This means that this command will not be called,
% say, at the beginning of a box that is later inserted at a point
% where a fill color was actively set. This may allow the command to
% produce more compact code when it ``knows'' that no special fill or
% stroke color has been set.
\pgfsys@color@reset@inordertrue


\def\pgfsys@color@reset{}
% This command will be called when the \pgfutil@color command is used. It
% should purge any internal settings of stroking and filling
% color. After this call, till the next use of a command like
% \pgfsys@color@rgb@fill, the current color installed by the \pgfutil@color
% command should be used.

\def\pgfsys@color@unstacked#1{}
% This slightly obscure command causes the color stack to be
% tricked. When called, this command should set the current color to
% #1 without causing any change in the color stack.

\def\pgfsys@text@to@black@hook{}
% Another slightly obscure command that allows tikz to hack into
% dvisvgm's color management inside text nodes. The problem is that
% the color "black" is special for dvisvgm.



%
%
% Coordinate system transformations
%
%

\def\pgfsys@transformcm#1#2#3#4#5#6{\pgf@sys@fail{transformations}}
% Perform a concatenation of the low-level current transformation
% matrix with the matrix given by the values #1 to #6. The
% transformation matrix is a transformation on a homogeneous
% 2D-coordinate system. See the pdf or postscript manual for details.

\def\pgfsys@transformshift#1#2{\pgfsys@transformcm{1}{0}{0}{1}{#1}{#2}}
% This command will change the origin of the low-level coordinate
% system to (#1,#2).

\def\pgfsys@transformxyscale#1#2{\pgfsys@transformcm{#1}{0}{0}{#2}{0bp}{0bp}}
% This command will scale the low-level coordinate system (and
% everything that is drawn) by a factor of #1 in x-directed and #2 in
% y-direction. Note that this applies to everything, including
% lines. So a scaled line will have a different width and may even
% have a different width when going along the x-axis and when going
% along the y-axis, if the scaling is different in these directions.

\def\pgfsys@viewboxmeet#1#2#3#4#5#6#7#8{\pgfsys@beginscope\pgf@sys@default@viewbox@impl{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{<}}
% Consider the two rectangles R with lower left corner
% (#5,#6) and upper right (#7,#8) and S with lower left corner
% (#1,#2) and upper right (#3,#4). Now, consider the transformation
% that scales and translates R so that the result T has the same
% center as S and has maximal size while still being inside S. This
% transformation gets installed in a new graphics group, which must be
% ended with a corresponding \pgfsys@endviewbox.

\def\pgfsys@viewboxslice#1#2#3#4#5#6#7#8{\pgfsys@beginscope\pgf@sys@default@viewbox@impl{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{>}}
% Works like \pgfsys@viewboxmeet, but R3 will have minimal size so
% that in contains all of R2.

\def\pgfsys@endviewbox{\pgfsys@endscope}
% Ends a viewbox scope started by either of the previous two commands.


\def\pgf@sys@default@viewbox@impl#1#2#3#4#5#6#7#8#9{{%
    \pgf@x#1%
    \pgf@y#2%
    \pgf@xa#3%
    \pgf@ya#4%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgfmathdivide@\pgf@xa\pgf@ya%
    \let\aspectr\pgfmathresult%
    \pgf@xb#5%
    \pgf@yb#6%
    \pgf@xc#7%
    \pgf@yc#8%
    \advance\pgf@xc by-\pgf@xb%
    \advance\pgf@yc by-\pgf@yb%
    \pgfmathdivide@\pgf@xc\pgf@yc%
    \let\aspects\pgfmathresult%
    \ifdim\aspectr pt#9\aspects pt%
      \pgfmathdivide@\pgf@xa\pgf@xc%
    \else%
      \pgfmathdivide@\pgf@ya\pgf@yc%
    \fi%
    \advance\pgf@x by.5\pgf@xa%
    \advance\pgf@xb by.5\pgf@xc%
    \advance\pgf@y by.5\pgf@ya%
    \advance\pgf@yb by.5\pgf@yc%
    \pgfsys@transformcm{\pgfmathresult}{0}{0}{\pgfmathresult}{\pgf@x}{\pgf@y}%
    \pgfsys@transformcm{1}{0}{0}{1}{-\pgf@xb}{-\pgf@yb}%
  }%
}




%
%
% Graphic state saving and restoring.
%
%

\def\pgfsys@beginscope{\pgf@sys@fail{scoping}}
% Saves the current graphic state on a graphic state stack. All
% changes to the graphic state parameters mentioned for \pgfsys@stroke
% and \pgfsys@fill will be local to the current graphic state and will
% the old values will be restored after endscope is used.
%
% WARNING: pdf and postscript differ with respect to the question of
% whether the current path is part of the graphic state or not. For
% this reason, you should never use this command unless the path is
% currently empty. For example, it might be a good idea to use
% discardpath prior to calling this command.

\def\pgfsys@endscope{\pgf@sys@fail{scoping}}
% Restores the last saved graphic state.

\def\pgfsys@begin@idscope{%
  \begingroup%
    \edef\pgf@sys@cacheref{\pgfsys@id@refcurrent}%
    \expandafter\let\expandafter\pgfsys@beg@save\csname pgf@sys@att@beg@\pgf@sys@cacheref\endcsname%
    \expandafter\let\expandafter\pgfsys@end@save\csname pgf@sys@att@end@\pgf@sys@cacheref\endcsname%
    \ifx\pgfsys@beg@save\relax%
      \ifx\pgfsys@end@save\relax%
      \else%
        \pgfsys@call@save%
      \fi%
    \else%
      \pgfsys@call@save%
    \fi%
    \pgfsys@invalidate@currentid%
      \begingroup%
}
% Starts an "id scope" where the current value of \pgfsys@use@id and
% \pgfsys@use@type is used. If the combination has been used before,
% nothing happens. Otherwise, depending of the driver, a graphic
% scope may or may not be created. To ensure that a graphic scope is
% created, use \pgfsys@beginscope additionally.

\def\pgfsys@call@save{%
  \pgfsys@beginscope%
  \pgfsys@beg@save%
  \expandafter\global\expandafter\let\csname pgf@sys@att@beg@\pgfsys@id@refcurrent\endcsname\relax%
  \expandafter\global\expandafter\let\csname pgf@sys@att@end@\pgfsys@id@refcurrent\endcsname\relax%
}

\def\pgfsys@end@idscope{
      \endgroup%
    \ifx\pgfsys@beg@save\relax%
      \ifx\pgfsys@end@save\relax%
      \else%
        \pgfsys@call@end%
      \fi%
    \else%
      \pgfsys@call@end%
    \fi%
  \endgroup
}
% Ends an id scope.

\def\pgfsys@call@end{%
  \pgfsys@end@save%
  \pgfsys@endscope%
}


\def\pgfsys@begin@text{}
% Inside a text box you should not use graphics command. However, TikZ
% needs to insert some color commands at the beginnings of text
% boxes. For most drivers, this is not a problem; except for SVG,
% where every change of the graphics state opens a scope and needs a
% closing scope. This command should be used at the beginning of text
% boxes containing such color commands and the matching
% \pgfsys@end@text at the end. If the box does not contain commands
% that change the graphics state, this command is not needed.

\def\pgfsys@end@text{}
% Closes a \pgfsys@begin@text.



%
%
% Id management (all of these commands have a default implementation
% any typically need not be redefined by a driver)
%
%

% The id count
\newcount\pgf@sys@id@count

\def\pgfsys@new@id#1{%
  \edef#1{pgf\the\pgf@sys@id@count}%
  \global\advance\pgf@sys@id@count by1\relax%
}
% Creates a new id and stores it in the macro #1.

\def\pgfsys@use@id#1{%
  \edef\pgf@sys@id@current@id{#1}%
  \let\pgfsys@current@type\pgfutil@empty%
}
\let\pgf@sys@id@current@id\pgfutil@empty
% Sets the id to be used for the next graphic object (group, box, or
% path). The type is reset to be empty. #1 must be a macro name that
% has previously been set using \pgfsys@new@id.
%
% Each combination of id and type can be used only once, on a second
% use nothing happens.

\def\pgfsys@clear@id{%
  \let\pgf@sys@id@current@id\pgfutil@empty%
}
% Clears the current id, so nothing can be referenced.

\def\pgfsys@use@type#1{%
  \edef\pgfsys@current@type{#1}%
  \pgfsys@register@type\pgfsys@current@type%
}
\let\pgfsys@current@type\pgfutil@empty
% Sets the type to be used for the next graphic object.

\def\pgfsys@append@type#1{%
  \ifx\pgfsys@current@type\pgfutil@empty%
    \pgfsys@use@type{#1}%
  \else%
    \pgfsys@use@type{\pgfsys@current@type.#1}%
  \fi%
}
% Appends something to the current type

\def\pgfsys@register@type#1{%
  \expandafter\let\expandafter\pgf@sys@temp\csname pgf@sys@reg@type@#1\endcsname%
  \ifx\pgf@sys@temp\relax%
    {%
      \c@pgf@counta\pgf@sys@type@count\relax%
      \global\advance\c@pgf@counta by1\relax%
      \edef\pgf@sys@type@count{\the\c@pgf@counta}%
      \expandafter\xdef\csname pgf@sys@reg@type@#1\endcsname{y\the\c@pgf@counta}%
    }%
  \fi%
}
% Registers a type with the system. Must be called before any use of
% the type
\def\pgf@sys@reg@type@{}
\def\pgf@sys@reg@type@background{b}
\def\pgf@sys@reg@type@path{p}
\def\pgf@sys@reg@type@text{t}
\expandafter\def\csname pgf@sys@reg@type@background.path\endcsname{bp}
\def\pgf@sys@type@count{0}

\def\pgfsys@push@type{%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgf@sys@typestack%
  \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgfsys@current@type%
    \expandafter\expandafter\expandafter{\expandafter\pgfsys@current@type\expandafter}%
    \expandafter\def\expandafter\pgf@sys@typestack\expandafter{\pgf@sys@typestack}}%
}
\let\pgf@sys@typestack\pgfutil@empty
% Pushes the current type onto a global stack. This is useful for
% temporarily changing the type without creating \TeX scopes.

\def\pgfsys@pop@type{\pgf@sys@typestack}
% Pops the last id from the stack.

\def\pgfsys@id@ref#1#2{#1\csname pgf@sys@reg@type@#2\endcsname}
% Expands to a text that can be inserted as a reference. #1 must be a
% reference created \pgfsys@new@id, #2 must be a type that has been
% registered using \pgfsys@id@register@type.

\def\pgfsys@id@refcurrent{\pgfsys@id@ref{\pgf@sys@id@current@id}{\pgfsys@current@type}}
% Expands to a text that can be inserted as a reference to the current
% id-type pair in use.

\def\pgfsys@invalidate@currentid{%
  \expandafter\global\expandafter\let\csname pgf@sys@id@keylist@\pgfsys@id@refcurrent\endcsname\pgfutil@empty%
}
% Mark the current id-type pair as used.

\def\pgfsys@attach@to@id#1#2#3#4{%
  \pgfsys@register@type{#2}%
  \expandafter\def\expandafter\pgf@sys@tempbeg\expandafter{\csname pgf@sys@att@beg@\pgfsys@id@ref{#1}{#2}\endcsname}%
  \expandafter\def\expandafter\pgf@sys@tempend\expandafter{\csname pgf@sys@att@end@\pgfsys@id@ref{#1}{#2}\endcsname}%
  \expandafter\ifx\pgf@sys@tempbeg\relax%
    \expandafter\let\pgf@sys@tempbeg\pgfutil@empty%
  \fi%
  \expandafter\ifx\pgf@sys@tempend\relax%
    \expandafter\let\pgf@sys@tempend\pgfutil@empty%
  \fi%
  \expandafter\let\expandafter\pgf@sys@tempbeg@cont\pgf@sys@tempbeg%
  \expandafter\let\expandafter\pgf@sys@tempend@cont\pgf@sys@tempend%
  \expandafter\expandafter\expandafter\gdef\expandafter\pgf@sys@tempbeg\expandafter{\pgf@sys@tempbeg@cont#3}%
  \def\pgf@sys@temp{#4}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\pgf@sys@tempend\expandafter\expandafter\expandafter{\expandafter\pgf@sys@temp\pgf@sys@tempend@cont}%
}
% Attaches some code to an id-type pair so that when the id's scope
% gets created, #3 is added at the beginning and #4 is added at the
% end.

\def\pgfsys@if@fresh@id#1#2#3#4{%
  \edef\pgf@sys@temp{#1}%
  \ifx\pgf@sys@temp\pgfutil@empty% empty id always counts as "has been used"
    #4%
  \else%
    \pgfsys@register@type{#2}%
    \expandafter\ifx\csname pgf@sys@id@keylist@\pgfsys@id@ref{#1}{#2}\endcsname\pgfutil@empty%
      % has already been used!
      #4%
    \else%
      #3%
    \fi%
  \fi%
}
% Checks whether a given id-type pair #1-#2 has not been used, yet. If
% so, #3 is executed, otherwise #4.

\def\pgfsys@if@fresh@currentid#1#2{%
  \ifx\pgf@sys@id@current@id\pgfutil@empty% empty id always counts as "has been used"
    #2%
  \else%
    \expandafter\ifx\csname pgf@sys@id@keylist@\pgfsys@id@refcurrent\endcsname\pgfutil@empty%
      % has already been used!
      #2%
    \else%
      #1%
    \fi%
  \fi%
}
% Checks whether the current id-type pair in use has not been used,
% yet. If so, #1 is executed, otherwise #2.




%
%
% Special commands
%
%

\def\pgfsys@imagesuffixlist{}
% A list of suffixes, separated by `:', that will be tried when
% searching for an image.



%
%
% Transparency
%
%

\def\pgfsys@opacity#1{\pgfsys@stroke@opacity{#1}\pgfsys@fill@opacity{#1}}
% Ideally, this should sets the opacity of all operations, treating
% the group as a transparency group with 1 meaning fully opaque, 0
% meaning fully transparent. Since most drivers do not support this,
% the fallback is to set the stroke and fill opacity at the same
% time. This is not quite the same, however.

\def\pgfsys@stroke@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of stroking operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@fill@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of filling operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@transparencygroupfrombox#1{\pgf@sys@fail{transparency groups}}
% This takes a TeX box and converts it into a transparency
% group. This means that any transparency settings apply to the box as
% a whole. For instance, if a box contains two overlapping black
% circles and you draw them normally with 50% transparency, then the
% overlap will be darker than the rest. By comparison, if the circles
% are part of a transparency group, the overlap will get the same
% color as the rest.
%
% The following settings modify the behaviour of a transparency group:

\newif\ifpgfsys@transparency@group@isolated
\newif\ifpgfsys@transparency@group@knockout


\def\pgfsys@blend@mode#1{\pgf@sys@fail{blend mode}}
% Sets the current blend mode. See the PDF specification for details
% on blend modes.


\def\pgfsys@definemask{\pgf@sys@fail{image masks}}
% This command declares a mask for usage with images. It works similar
% to \pgfsys@defineimage: Certain macros are set when the command is
% called. The result should be to set the macro \pgf@mask to a pdf
% object count that can subsequently be used as a soft mask. The
% following macros will be set when this command is invoked:
%
% - \pgf@filename
%   File name of the mask to be defined.
%
% - \pgf@maskmatte
%   The so-called matte of the mask (see the pdf documentation for
%   details). The matte is a color specification consisting of 1, 3 or
%   4 numbers between 0 and 1. The number of numbers depends on the
%   number of color channels in the image (not in the mask!). It will
%   be assumed that the image has been preblended with this color.

\def\pgfsys@fadingfrombox#1#2{\pgf@sys@fail{fadings}}
% Declares an fading named #1. The parameter #2 must be a
% box. Its contents luminosity determines the opacity of the resulting
% mask.

\def\pgfsys@usefading#1#2#3#4#5#6#7{\pgf@sys@fail{fadings}}
% Installs a previously declared fading #1 in the current graphics
% state. Parameters #2 to #7 specify a transformation cm that should
% be applied to the mask before it is used.

\def\pgfsys@clipfading{}
% This default implementation is a no-op for all drivers except `dvips'
% where we have to set the clipping path _before_ installing the fading (used in
% \pgfsetfadingforcurrentpath, \pgfsetfadingforcurrentpathstroked commands of
% the basic layer)


%
%
% Shading commands
%
%

\def\pgfsys@horishading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a horizontal shading for later use. The effect of this
% command should be the definition of a macro called `@pgfshading#1!'
% (or \csname @pdfshading#1!\endcsname, to be precise). When invoked,
% this new macro should insert a shading at the current position.
%
% #1 is the name of the shading, which is also used in the output
% macro name. #2 is the height of the shading and must be given as a
% TeX dimension like `2cm' or `10pt'. #3 is a shading color
% specification as specified in the pgfuserguide. The shading
% specification implicitly fixes the width of the shading.
%
% When `@pgfshading#1!' is invoked, it should insert a box of height
% #2 and the width implicit in the shading declaration.

\def\pgfsys@vertshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Like horishading, only for vertical shadings. This time, the height
% of the shading is implicit in #3 and the width is given as #2.

\def\pgfsys@radialshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a radial shading. Like the previous macros, this command
% should setup the macro `@pgfshading#1!', which upon invocation
% should insert a radial shading whose size is implicit in #3.
%
% The parameter #2 is a pgf point specification if the starting point
% of the shading. See the pgfuserguide for details.

\def\pgfsys@functionalshading#1#2#3#4{\pgf@sys@fail{shadings (functional)}\pgf@sys@noshading{#1}}
% Declares a shading using a PostScript-like function that provides a
% color for each point. Like the previous macros, this command
% should setup the macro `@pgfshading#1!' so that it will produce a
% box containing the desired shading.
%
% Parameter #1 is the name of the shading. Parameter #4 is a
% Postscript-like function (type 4 function of the PDF specification)
% as described in Section 3.9.4 of the PDF Specification version 1.7.
% Parameter #2 and #3 are pgf point specifications that specifies the
% lower left and upper right coordinate.
%
% When function #4 is evaluated, the coordinate of the current
% point will be on the (virtual) PostScript stack in bp units. After
% the function has been evaluated, the stack should consist of three
% numbers (not integers! - the Apple PDF renderer is broken in this
% regard, so add cvr's at the end if needed) that represent the red,
% green, and blue components of the color.
%
% A buggy #4 will result is *totally unpredictable chaos* during
% rendering.

\def\pgf@sys@noshading#1{\expandafter\global\expandafter\let\csname @pgfshading#1!\endcsname=\pgfutil@empty}




%
%
% Pattern stuff
%
%

\def\pgfsys@declarepattern#1#2#3#4#5#6#7#8#9{\pgf@sys@fail{patterns}}
% This command declares a new colored or uncolored pattern. Uncolored
% patterns have no inherent color, the color is provided when they are
% set. Colored patters have an inherent color.
% #1       = name of the pattern (must be a plain suffix for use in
%            postscript/pdf/etc.)
% #2 to #5 = four coordinates describing the corners of a bounding box
%            of pattern cells
% #6       = x-step
% #7       = y-step
% #8       = pattern code
% #9       = 0 if uncolored patter, 1 if colored pattern.

\def\pgfsys@setpatternuncolored#1#2#3#4{\pgf@sys@fail{patterns}}
% Sets an uncolored pattern #1 as filling color. The numbers #2, #3,
% #4 must be an rgb-value to be used as the color of the pattern.

\def\pgfsys@setpatterncolored#1{\pgf@sys@fail{patterns}}
% Sets an colored pattern #1 as filling color.





%
%
% Animations
%
%


\newif\ifpgfsysanimationsupported
% Will be set to true by a driver when animations are supported. Note
% that snapshots are always supported.


\def\pgfsys@animate#1{\pgf@sys@fail{animations}}
% Adds an animation of the attribute #1 to the current scope.
% The configuration of the animation (like start times, etc.) is taken
% from the current values of the animation keys, which are configured
% using calls to \pgfsys@animation@..., which setup an animation
% key for the local scope. This means that you typically setup these
% keys in a scope and at the end of the scope call \pgfsys@animate.
%
% Some keys accumulate (like begin or keytime), most do not. In those
% cases, the last call overrides the previous one.
%
% Not all value types make sense or are allowed, it depends on the
% specific \pgfsys@animate call.
%
% Example:
%
% {
%   \pgfsys@animation@offset{10}{begin}%
%   \pgfsys@animation@event{}{click}{1}{begin}%
%   \pgfsys@animation@time{5}{1}{1}{0}{0}
%   \pgfsys@animation@val@scalar{1}
%   \pgfsys@animation@time{8}{1}{1}{0}{0}
%   \pgfsys@animation@val@scalar{0.5}
%   \pgfsys@animation@sum%
%   \pgfsys@animate{fillopacity}%
% }
%
% When a driver does not support a specific attribute #1, it should
% issue a \pgf@sys@fail. Typical attributes are things like "opacity"
% or "linewidth" or "dash".
%
% The following values are permissible for "#1":
%
% "opacity" adds an animation of the opacity.
% Type: scalar
%
% "fillopacity" adds an animation of the fill opacity.
% Type: scalar
%
% "strokeopacity" adds an animation of the stroke opacity.
% Type: scalar
%
% "visibility" adds an animation of the visibility.
% Type: text ("visible" or "hidden")
%
% "linewidth" adds an animation of the line width.
% Type: dimension
%
% "dash" adds an animation of the dash.
% Type: dash
%
% "translate" adds an animation of the transformation.
% Type: translate
%
% "scale" adds an animation of the transformation.
% Type: scale
%
% "rotate" adds an animation of the transformation.
% Type: scalar
%
% "skewx" adds an animation of the transformation.
% Type: scalar
%
% "skewy" adds an animation of the transformation.
% Type: scalar
%
% "motion" adds a movement along a path.
% Type: motion
%
% "strokecolor" adds an animation of the stroke color.
% Type: color
%
% "fillcolor" adds an animation of the fill color.
% Type: color
%
% "viewbox" adds an animation of the view box.
% Type: view box
%
% "path" adds an animation of the path to the path specified by
% \pgfsys@animation@whom
% Type: path
%
% "syncbase" adds a sync base to the animation. A sync base does not animate
% anything by itself, but other animations can begin and end relative
% to it.
%
% "none" suppresses the animation
% Type: any




% Animation timing :
%
% You specify an animation using a timeline. A timeline consists of a
% sequence of times together with values for these times. The times
% must be given in increasing order. You use the command
% \pgfsys@animation@time to specify a time and
% \pgfsys@animation@val@... to specify a value. The time must be
% specified first, the time--value is created when the value command is
% used.
%
% Times are given in seconds (so 0.01 is one hundredth of a second).
%
% The animation's timeline will start with the first time mentioned
% (not necessarily zero and not necessarily a positive value) and ends
% with the last value. The duration is the difference between these
% two values.

\def\pgfsys@animation@restart@always{}
% Specifies that the animation can always restart

\def\pgfsys@animation@restart@never{}
% Specifies that the animation should never restart

\def\pgfsys@animation@restart@whennotactive{}
% Specifies that the animation should only restart when it is not active

\def\pgfsys@animation@repeat#1{}
% #1 must be a number

\def\pgfsys@animation@repeat@indefinite{}
% Repeats forever

\def\pgfsys@animation@repeat@dur#1{}
% #1 must be a clock value

\def\pgfsys@animation@freezeatend{}
% Specifies that the last value of the animation remains in force at
% the end

\def\pgfsys@animation@removeatend{}
% Specifies that the effect of the animation is removed at the end

\def\pgfsys@animation@time#1#2#3#4#5{}
% Specifies a time together with spline control points for the entry
% and the exit to this time. The value #1 is a time in seconds (so 60
% means 1 minute, 0.001 means one millisecond). The values #2 and #3
% specify the control point of the spline *entering* the time point,
% while the values #4 and #5 specify the control point of the spline
% *leaving* the time point. They are all dimensionless values between
% 0 and 1. For a linear animation, set the first two to 1 and the last
% two to 0.
%
% Example:
% \pgfsys@animation@time{5}{1}{1}{0.25}{0.1}
% \pgfsys@animation@val@scalar{80}
% \pgfsys@animation@time{8}{.75}{1}{0}{0}
% \pgfsys@animation@val@scalar{90}
%
% In SVG, this will create the following entries:
% begin     = +5s
% duration  = 3s
% keyTimes  = 0;1
% values    = 80;90
% keySpline = 0.25 0.1 0.75 1
%
% For the key spline, note that the entry spline controls of the first
% time and the exit spline controls of the last point are dropped.
%
%
% When the exit spline takes the special values #4="stay" and #5="0",
% the attribute's value "stays" until the next value for the next time
% (it "jumps" to the next value then). This corresponds, roughly, to
% an "infinite" #4.
%
% Similarly, when the entry spline takes the special value #2="jump"
% and #3="1", the value immediately jumps from the previous value to
% the next value when the previous value was "created".

\def\pgfsys@stay@text{{stay}{0}}
\def\pgfsys@jump@text{{jump}{1}}

\def\pgfsys@animation@base{}
% Think of this command as setting the value of the attribute in the
% timeline before the timeline starts. Normally, an animation only
% influences the timeline while the animation is running (which may be
% forever) and before and after the animation is running, the
% attribute's value is not modified by the animation (so, it is just
% inherited from the surrounding scope). When a base value is set,
% while the animation is not running, this value is used. For most
% attributes you can achieve the same effect by surrounding the
% to-be-animated object by a scope and setting the value there, but
% using bases is often more convenient and, for instance for the
% visibility attribute, it is necessary to use a base.
%
% Note that when a backend driver does not support animations, base
% values will not be depicted unless a snapshot is used explicitly.

\def\pgfsys@animation@offset#1#2{}
% #1 must be a value in seconds, #2 is the target "begin" or "end" to
% which this offset is appended.

\def\pgfsys@animation@syncbegin#1#2#3#4{}
% #1 is the id of a sync base (obtained by
% \pgfsys@new@id), #2 is the id type (or empty), #3 is an optional
% offset, #4 is the target.

\def\pgfsys@animation@syncend#1#2#3#4{}
% Like the previous command.

\def\pgfsys@animation@event#1#2#3#4#5{}
% #1 is the optional id of another element (obtained by
% \pgfsys@new@id), #2 is the optional type of the id, #3 is an event
% name, #4 is an optional offset, #5 is the target.

\def\pgfsys@animation@repeat@event#1#2#3#4#5{}
% #1 is the optional id of another element, #2 is the type, #3 is a
% repeat count, and #4 is an optional offset, #5 is the target.

\def\pgfsys@animation@accesskey#1#2#3{}
% #1 is a character, #2 is an optional offset, #3 is the target.

\def\pgf@sys@begin@text{begin}


% Accumulation

\def\pgfsys@animation@accumulate{}
% Corresponds to accumulate="sum" in SVG

\def\pgfsys@animation@noaccumulate{}
% Corresponds to accumulate="none" in SVG


% Targeting

\def\pgfsys@animation@whom#1#2{}
% Sets the target of the animation. #1 must be an id previously
% created using \pgfsys@new@id and #2 must be empty or a type
% previously created using \pgfsys@new@id@type


% Attribute definitions

\def\pgfsys@animation@rotatealong{}
% Applicable only to motion animations. Indicates that the
% to-be-animated group should be rotated automatically so that it
% points along the path as time progresses.

\def\pgfsys@animation@norotatealong{}
% Corresponds to rotate="0"

\def\pgfsys@animation@movealong#1{}
% Applicable only to motion animations. #1 is a softpath along which
% the movement will be done.

\def\pgfsys@animation@tip@markers#1#2{}
% Applicable only to path animations. #1 and #2 are markers (declared
% using \pgfsys@marker@declare) that store marker symbols to be added
% at the start and at the end of the to-be-animated path. If empty, no
% markers are added.

\def\pgfsys@animation@canvas@transform#1#2{}
% #1 is some code that may call \pgfsys@transformcm at most once. It
% will be executed when a canvas transformation animation is
% installed for a scope id. #2 is some further codes that may also
% call \pgfsys@transformcm at most once. It will be installed right
% after the animation.
%
% Typically, #1 is some pgf coordinate shift followed by
% {\pgflowlevelsynccm} and #2 is \pgftransforminvert followed by
% \pgflowlevelsynccm.



% Values

\def\pgfsys@animation@val@current{}
% The current value of the attribute. At least with SVG, this can only
% be used for the first value and, then, only if there is only one
% other value.

\def\pgfsys@animation@val@text#1{}
% #1 should be some text.

\def\pgfsys@animation@val@scalar#1{}
% #1 should be a single value.

\def\pgfsys@animation@val@dimension#1{}
% #1 must be a dimension.

\def\pgfsys@animation@val@color@rgb#1#2#3{}
% #1,#2,#3 must be an rgb tuple

\def\pgfsys@animation@val@color@cmyk#1#2#3#4{}
% #1,#2,#3,#4 must be an cmyk tuple

\def\pgfsys@animation@val@color@cmy#1#2#3{}
% #1,#2,#3 must be an cmy tuple

\def\pgfsys@animation@val@color@gray#1{}
% #1 must be a gray value

\def\pgfsys@animation@val@path#1{}
% #1 must consist of path-construction tokens (as returned by the
% softpath layer)

\def\pgfsys@animation@val@translate#1#2{}
% #1,#2 must be dimensions

\def\pgfsys@animation@val@scale#1#2{}
% #1,#2 must be dimensionless

\def\pgfsys@animation@val@viewbox#1#2#3#4{}
% #1,#2 describe the lower left, #3,#4 the upper right corner of the
% view box.

\def\pgfsys@animation@val@dash#1#2{}
% #1,#2 have the syntax of \pgfsys@setdash.



%
%
% Markers
%
%

\def\pgfsys@marker@declare#1#2{%
  {%
    \pgfpicturetrue%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@marker@temp%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    \pgfsys@beginscope%
    #2%
    \pgfsys@endscope%
    \xdef#1{\the\pgf@sys@id@count}%
    \expandafter\expandafter\expandafter\global\expandafter\pgfsysprotocol@getcurrentprotocol\csname pgf@sys@marker@prot@#1\endcsname%
    \pgfsys@marker@declare@% curtesy hook
    \pgfsysprotocol@setcurrentprotocol\pgfsys@marker@temp%
    \global\advance\pgf@sys@id@count by1\relax%
  }%
}
\let\pgfsys@marker@declare@\relax
% Declares a new marker symbol whose code is in #2. #1 should be a
% macro name, which will be set to a unique
% value by which the marker can be referenced later on. #2 should be
% code that, when executed, produces recordable code.

\def\pgfsys@marker@use#1{%
  \pgfsysprotocol@literal{\csname pgf@sys@marker@prot@#1\endcsname}%
}
% Draws the marker symbol not at the end of a path, but simply with
% the current transformation matrix






%
%
% RDF
%
%

\def\pgfsys@rdf@about#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute "about" with value #1 to the next
% idscope. The RDF-spec says: "a SafeCURIEorCURIEorIRI, used for
% stating what the data is about (a 'subject' in RDF terminology);"

\def\pgfsys@rdf@content#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute content with value #1 to the next
% idscope. The RDF-spec says: "a CDATA string, for supplying
% machine-readable content for a literal (a 'literal object', in RDF
% terminology);"

\def\pgfsys@rdf@datatype#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute datatype with value #1 to the next
% idscope. The RDF-spec says: "a TERMorCURIEorAbsIRI representing a
% datatype, to express the datatype of a literal;"

\def\pgfsys@rdf@href#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute href with value #1 to the next idscope
% The RDF-spec says: "a traditionally navigable IRI for
% expressing the partner resource of a relationship (a 'resource
% object', in RDF terminology);"

\def\pgfsys@rdf@inlist{\pgf@sys@fail{rdf}}
% Adds the rdf attribute inlist to the next idscope. The
% RDF-spec says: "An attribute used to indicate that the object
% associated with a rel or property attribute on the same element is
% to be added to the list for that predicate. The value of this
% attribute must be ignored. Presence of this attribute causes a list
% to be created if it does not already exist."

\def\pgfsys@rdf@prefix#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf prefix attribute to the next
% idscope. Can be called several times, in which case all values of #1
% are concatenated with whitespaces. The RDF-spec says: "a white space
% separated list of prefix-name IRI pairs of the form NCName ':' ' '+
% xsd:anyURI"

\def\pgfsys@rdf@property#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf property attribute to the next
% idscope. Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between a subject and either a resource object if
% given or some literal text (also a 'predicate');"

\def\pgfsys@rdf@rel#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf rel attribute to the next
% next idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of
% TERMorCURIEorAbsIRIs, used for expressing relationships between two
% resources ('predicates' in RDF terminology);"

\def\pgfsys@rdf@resource#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute resource with value #1 to the next idscope. The
% RDF-spec says: "a SafeCURIEorCURIEorIRI for expressing the partner
% resource of a relationship that is not intended to be navigable
% (e.g., a 'clickable' link) (also an 'object');"

\def\pgfsys@rdf@rev#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf rev attribute to the next
% idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of
% TERMorCURIEorAbsIRIs, used for expressing reverse relationships
% between two resources (also 'predicates');

\def\pgfsys@rdf@src#1{\pgf@sys@fail{rdf}}
% Adds an rdf attribute src with value #1 to the next idscope. The
% RDF-spec says: "an IRI for expressing the partner resource of a
% relationship when the resource is embedded (also a 'resource
% object');"

\def\pgfsys@rdf@typeof#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf typeof attribute to the next
% idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of TERMorCURIEorAbsIRIs
% that indicate the RDF type(s) to associate with a subject;"

\def\pgfsys@rdf@vocab#1{\pgf@sys@fail{rdf}}
% Adds an rdf attribute vocab with value #1 to the next idscope. The
% RDF-spec says: "an IRI that defines the mapping to use when a TERM
% is referenced in an attribute value. See General Use of Terms in
% Attributes and the section on Vocabulary Expansion."



%
%
% Page size stuff
%
%

\def\pgfsys@papersize#1#2{\pgf@sys@fail{papersize}}
% This command sets the paper size in a portable way. It tries to do
% so "locally" for the current page, but what really happens depends
% strongly on the driver. For instance, dvips will use whatever is
% used with the first call to this command that is part of the
% shipped-out document and will ignore all other uses. In contrast,
% pdftex will use the current value of the papersize for each page
% and, additionally, setting the papersize is local to the current TeX
% group.
% #1 = width
% #2 = height

\def\pgfsys@global@papersize#1#2{\pgfsys@papersize{#1}{#2}}
% This command does the same as the papersize command, only for
% drivers that support this, \global is used to set the papersize.
% #1 = width
% #2 = height

\def\pgfsys@prepare@papersize#1#2{\pgfsys@papersize{#1}{#2}}
% Like \pgfsys@papersize, this prepares the paper size in a portable
% way -- but it is supposed to be a preparation step before the
% document has started. Drivers may decide to postpone the action
% until the document has started.
%
% The root cause why I added this method is that image externalization
% seems to suffer from the fact that some drivers need a "prepared"
% routine whereas others must not have a prepared routine and have to
% apply the action right-away. This method is the solution for image
% externalization.
% #1 = width
% #2 = height

\ifx\paperheight\@undefined
  \def\pgfsys@thepageheight{\the\vsize} % this is wrong, but I do not
                                % know how to compute the page height
                                % in plain tex.
  \def\pgfsys@thepagewidth{\the\hsize}
\else
  \def\pgfsys@thepageheight{\paperheight}
  \def\pgfsys@thepagewidth{\paperwidth}
\fi


%
%
% Position tracking commands
%
%

% Marks the current position on the page. This position can later be
% referenced using \pgfsys@getposition
\def\pgfsys@markposition#1{\pgf@sys@fail{marking the current position}}

% Sets #2 to a pgfpoint macro that returns the position #1 is
% returned in a coordinate system where the x-axis goes right and the
% y-axis goes up. The origin of this coordinate system may or may not
% lie in the lower left corner; you should shift the coordinate system
% to the position "pgfpageorigin" to make sure that the origin is at
% the lower left corner. Typically, getting this position
% requires two runs of TeX. On the first run, the macro will be set to
% \relax, indicating that the position is not available.
%
% If #1 is set to the special position "pgfpageorigin", the position
% of the the lower left page corner is returned.

\def\pgfsys@getposition#1#2{\let#2=\relax}



%
%
% Commands having a default implementation. These commands only need
% not be implemented by drivers if this results in a better
% performance.
%
%


\def\pgfsys@shadingoutsidepgfpicture#1{%
  #1%
}
% This command gets the definition of a shading (@pgfshadingxxxx!) as
% an argument and should insert this shading into the normal text.
%
% This command has a default implementation.


\def\pgfsys@shadinginsidepgfpicture#1{%
  \pgf@makehbox{#1}%
  \setbox\pgf@hbox=\hbox{\hskip-.5\wd\pgf@hbox\lower.5\ht\pgf@hbox\hbox{\box\pgf@hbox}}%
  \pgfqbox{\pgf@hbox}%
}
% This command works like \pgfsys@shadingoutsidepgfpicture, only it is
% called when a shading should be inserted inside a picture. This
% command should insert the shading centered on the origin (which will
% typically have been low-level translated somewhere else.)
%
% This command has a default implementation.


\def\pgfsys@hbox#1{%
  \pgfsys@begin@idscope%
  \pgfsys@beginscope%
    \setbox#1=\hbox{\box#1}%
    \wd#1=0pt%
    \ht#1=0pt%
    \dp#1=0pt%
    \box#1%
  \pgfsys@endscope%
  \pgfsys@end@idscope%
}
% Called to insert a TeX hbox into a pgfpicture.

\def\pgfsys@hboxsynced#1{%
  \pgfsys@beginscope\pgflowlevelsynccm\pgfsys@hbox#1\pgfsys@endscope%
}%
% Called to insert box #1 into a pgfpicture, but with the current
% coordinate transformation matrix synced with the canvas
% transformation matrix and surrounded by a scope.
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfsys@hbox#1. However, a
% ``TeX-translation'' is used for the translation part of the
% transformation cm. This will ensure that hyperlinks ``survive'' at
% least translations.

\def\pgfsys@pictureboxsynced#1{%
  {%
    \setbox0=\hbox{\pgfsys@beginpicture\box#1\pgfsys@endpicture}%
    \pgfsys@hboxsynced0%
  }%
}
% Basically, this should do the same as doing a (scoped) low level sync
% followed by inserting the box #1 directly into the output
% stream. However, the default implementation uses \pgfsys@hboxsynced
% in conjunction with \pgfsys@beginpicture to ensure that, if
% possible, hyperlinks survive in pdfs. Drivers that are sensitive to
% picture-in-picture scopes should replace this implementation by
% \pgfsys@beginscope\pgflowlevelsynccm\box#1\pgfsys@endscope

\def\pgfsys@beginpicture{}
% Called at the beginning of a pgfpicture. Used to setup things.

\def\pgfsys@endpicture{}
% Called at the end of a pgfpicture.

\def\pgfsys@typesetpicturebox#1{%
  \pgf@ya=\pgf@shift@baseline\relax%
  \advance\pgf@ya by-\pgf@picminy\relax%
  %
  %
  \advance\pgf@picmaxy by-\pgf@picminy\relax% maxy is now the height
  \advance\pgf@picmaxx by-\pgf@picminx\relax% maxx is now the width
  \setbox#1=\hbox{\hskip-\pgf@picminx\lower\pgf@picminy\box#1}%
  \ht#1=\pgf@picmaxy%
  \wd#1=\pgf@picmaxx%
  \dp#1=0pt%
  \leavevmode%
  \pgf@xa=\pgf@trimleft@final\relax  \ifdim\pgf@xa=0pt \else\kern\pgf@xa\fi
  \raise-\pgf@ya\box#1%
  \pgf@xa=\pgf@trimright@final\relax \ifdim\pgf@xa=0pt \else\kern\pgf@xa\fi
}
% Called after a picture has been typeset in box #1. This
% command should insert the box into the normal TeX code. The box #1
% will still be a ``raw'' box that contains only the \special's. The
% job of this command is to resize and shift this box according to the
% baseline shift and the size of the box.
%
% This command has a default implementation.

\def\pgfsys@beginpurepicture{\pgfsys@beginpicture}
% This version of the beginpicture command can be used for pictures
% that are guaranteed not to contain any hboxes. In this case, a
% driver might provide a more compact version of the command.

\def\pgfsys@endpurepicture{\pgfsys@endpicture}
% Called at the end of a ``pure'' pgfpicture.

\def\pgfsys@defineimage{%
  \ifx\pgf@imagewidth\pgfutil@empty\else\edef\pgf@imagewidth{width=\pgf@imagewidth,}\fi%
  \ifx\pgf@imageheight\pgfutil@empty\else\edef\pgf@imageheight{height=\pgf@imageheight,}\fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepage{page=\pgf@imagepage,}\fi%
  \edef\pgf@image{\noexpand\includegraphics[\pgf@imageheight\pgf@imagewidth]{\pgf@filename}}%
}
% Called, when an image should be defined.
%
% This command does not take any parameters. Instead, certain macros
% will be preinstalled with appropriate values when this command is
% invoked. These are:
%
% - \pgf@filename
%   File name of the image to be defined.
%
% - \pgf@imagewidth
%   Will be set to the desired (scaled) width of the image.
%
% - \pgf@imageheight
%   Will be set to the desired (scaled) height of the image.
%
%   If this macro and also the height macro are empty, the image
%   should have its `natural' size.
%
%   If exactly only of them is specified, the undefined value the
%   image is scaled so that the aspect ratio is kept.
%
%   If both are set, the image is scaled in both directions
%   independently, possibly changing the aspect ratio.
%
%
% The following macros presumable mostly make sense for drivers that
% can handle pdf:
%
% - \pgf@imagepage
%   The desired page number to be extracted from a multi-page
%   `image'.
%
% - \pgf@imagemask
%   If set, it will be set to `/SMask x 0 R', where x is the pdf
%   object number of a soft mask to be applied to the image.
%
% - \pgf@imageinterpolate
%   If set, it will be set to `/Interpolate true' or  `/Interpolate
%   false', indicating whether the image should be interpolated in
%   pdf.
%
%
% The command should now setup the macro \pgf@image such that calling
% this macro will result in typesetting the image. Thus, \pgf@image is
% the `return value' of the command.


\def\pgfsys@defobject#1#2#3#4{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfpicturetrue%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    \pgfsys@beginscope%
    #4%
    \pgfsys@endscope%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@@temp%
    \expandafter\global\expandafter\let\csname #1\endcsname=\pgfsys@@temp%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Declares an object for later use. The idea is that the object can be
% precached in some way and then be rendered more quickly when used
% several times. For example, an arrow head might be defined and
% prerendered in this way.
%
% The parameter #1 is the name for later use. #2 and #3 are pgf points
% specifying a bounding box for the object. #4 is the code for the
% object. The code may only contain protocolable code.


\def\pgfsys@useobject#1#2{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedfalse%
    #2%
    \expandafter\pgfsysprotocol@setcurrentprotocol\csname #1\endcsname%
    \pgfsysprotocol@invokecurrentprotocol%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Renders a previously declared object. The first parameter is the
% name of the object. The second parameter is extra code that
% should be executed right *before* the object is rendered. Typically,
% this will be some transformation code.


\def\pgfsys@begininvisible{\pgfsys@transformcm{1}{0}{0}{1}{2000bp}{2000bp}}
% Between this command and the closing endinvisible, all output should
% be suppressed. Nothing should be drawn at all, which includes all
% paths, images and shadings. This command typically should not open a
% graphic scope.

\def\pgfsys@endinvisible{\pgfsys@transformcm{1}{0}{0}{1}{-2000bp}{-2000bp}}
% Ends the invisibility section, unless invisibility blocks have been
% nested. In this case, only the `last' one restores visibility.

\def\pgfsys@begininvisiblescope{\pgfsys@beginscope\pgfsys@begininvisible}
% Works like pgfsys@begininvisible, but it may open a graphics scope.

\def\pgfsys@endinvisiblescope{\pgfsys@endinvisible\pgfsys@endscope}
% Closes the invisibility scope.


\def\pgfsys@atbegindocument{}
% This command will be executed at the begin of the document. If for
% whatever reason this is not done, you may wish to execute this
% command yourself. It will setup certain specials that need to be
% inserted into the resulting .pdf/.ps/.xxx file.





% Discern the driver:

% Default driver:
\ifx\pgfsysdriver\@undefined
  \pgfutil@guessdriver
\fi

\input pgf.cfg

\immediate\write-1{Driver file for pgf: \pgfsysdriver}
\pgfutil@InputIfFileExists{\pgfsysdriver}{}{%
  \pgferror{Driver file ``\pgfsysdriver'' not found.}}



% This will insert always-present-specials at the beginning of the
% code.
\AtBeginDocument{
  \pgfsys@atbegindocument
  \let\pgfsys@atbegindocument=\pgfutil@empty
}



% Read aux file in plain and context mode:

\pgfutil@aux@read@hook


\endinput


==> pgfsyssoftpath.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfsyssoftpath.code.tex}


% This package provides the pgf system path abstraction layer. This
% layer is used to construct paths first ``abstractly.'' These
% abstract paths can still be modified, before they are ``made
% concrete.''
%
% An abstract path consists of a sequence of basic building blocks,
% each of which is a tuple consisting of two numbers (specifying a
% coordinate) and a token. Possible tokens are:
%
% 1. moveto
% 2. lineto
% 3. rectcorner
% 4. rectsize
% 5. curvetosupporta
% 6. curvetosupportb
% 7. curveto
% 8. closepath
% 9. specialround
%
% A curveto must always be preceded by a curvetosupporta and a
% curvetosupportb. A non-empty path must always begin with a
% moveto. The coordinates of a closepath are non-specified, currently,
% but they might be set to the coordinate of the path segment start,
% in the future.


% Access to the current path:
%
% Lots of stuff is added to the current path and it can get very long
% (containing literally tens of thousands of tokens). For such macros,
% adding things using a simple "g@addtomacro" takes more and more
% time, resulting in quadratic runtime. To avoid this, ideally, one
% would collect things in an array and then use a divide and conquer
% merger. A simple intermediate solution is the following, implemented
% here: We have the path and two buffers. New tokens are added to the
% first buffer, which is quite small. When it overflow, its contents
% is added to the second buffer, which is large. If that buffer
% overflow, the contents is finally added to the main path (which can
% have arbitrary length). Whenever the main path is set or read, the
% buffers are flushed.
%
% Because of this buffering, it is imperative that the main path is
% accessed only via appropriate interface macros.



% The current path
\let\pgfsyssoftpath@thepath=\pgfutil@empty
\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
\newcount\pgfsyssoftpath@smallbuffer@items
\newcount\pgfsyssoftpath@bigbuffer@items

\def\pgfsyssoftpath@flushbuffers{%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
    \expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer}%
  \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
  \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
  \global\pgfsyssoftpath@bigbuffer@items0\relax%
  \global\pgfsyssoftpath@smallbuffer@items0\relax%
}

% Getting and setting the current path
\def\pgfsyssoftpath@getcurrentpath#1{%
  \pgfsyssoftpath@flushbuffers%
  \let#1=\pgfsyssoftpath@thepath%
}

\def\pgfsyssoftpath@setcurrentpath#1{%
  \global\let\pgfsyssoftpath@thepath=#1%
  \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
  \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
  \global\pgfsyssoftpath@bigbuffer@items0\relax%
  \global\pgfsyssoftpath@smallbuffer@items0\relax%
}


% Invoking the current path (slightly optimized)
\def\pgfsyssoftpath@invokecurrentpath{%
  \pgfsyssoftpath@thepath%
  \pgfsyssoftpath@bigbuffer%
  \pgfsyssoftpath@smallbuffer%
}

\def\pgfsyssoftpath@flushcurrentpath{%
  \pgfsyssoftpath@invokecurrentpath%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
}

% Add an item at the end
\def\pgfsyssoftpath@addtocurrentpath#1{%
  \global\advance\pgfsyssoftpath@smallbuffer@items by1\relax%
  \ifnum\pgfsyssoftpath@smallbuffer@items<40\relax% good number?
    \expandafter\gdef\expandafter\pgfsyssoftpath@smallbuffer\expandafter{\pgfsyssoftpath@smallbuffer#1}%
  \else%
    \pgfsyssoftpath@smalloverflow{#1}%
  \fi%
}
\def\pgfsyssoftpath@smalloverflow#1{%
  \global\advance\pgfsyssoftpath@bigbuffer@items by1\relax%
  \ifnum\pgfsyssoftpath@bigbuffer@items<30\relax% good number?
    \expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\pgfsyssoftpath@bigbuffer%
    \expandafter\expandafter\expandafter{\expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer#1}%
    \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty%
    \global\pgfsyssoftpath@smallbuffer@items0\relax%
  \else%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\pgfsyssoftpath@thepath
      \expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer#1}%
    \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
    \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
    \global\pgfsyssoftpath@bigbuffer@items0\relax%
    \global\pgfsyssoftpath@smallbuffer@items0\relax%
  \fi%
}



\def\pgfsyssoftpath@lastmoveto{{0pt}{0pt}}

\newif\ifpgfsyssoftpathmovetorelevant
\pgfsyssoftpathmovetorelevanttrue

% Add a moveto element to the current path
\def\pgfsyssoftpath@moveto#1#2{%
  \edef\pgfsyssoftpath@coord{{#1}{#2}}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\expandafter{\expandafter\pgfsyssoftpath@movetotoken\pgfsyssoftpath@coord}%
  \ifpgfsyssoftpathmovetorelevant%
    \global\let\pgfsyssoftpath@lastmoveto\pgfsyssoftpath@coord%
  \fi%
}

% Add a lineto element to the current path
\def\pgfsyssoftpath@lineto#1#2{%
  \edef\pgfsyssoftpath@coord{{#1}{#2}}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\expandafter{\expandafter\pgfsyssoftpath@linetotoken\pgfsyssoftpath@coord}%
}


% Add curveto elements to the current path
\def\pgfsyssoftpath@curveto#1#2#3#4#5#6{%
  \edef\pgfsyssoftpath@temp{{%
      \noexpand\pgfsyssoftpath@curvetosupportatoken{#1}{#2}%
      \noexpand\pgfsyssoftpath@curvetosupportbtoken{#3}{#4}%
      \noexpand\pgfsyssoftpath@curvetotoken{#5}{#6}%
    }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}


% Add rectangle elements to the current path
\def\pgfsyssoftpath@rect#1#2#3#4{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@rectcornertoken{#1}{#2}%
    \noexpand\pgfsyssoftpath@rectsizetoken{#3}{#4}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Add closepath element to the current path
\def\pgfsyssoftpath@closepath{%
  \expandafter\pgfsyssoftpath@addtocurrentpath\expandafter{\expandafter\pgfsyssoftpath@closepathtoken\pgfsyssoftpath@lastmoveto}%
}

% Add special element to the current path
\def\pgfsyssoftpath@specialround#1#2{%
  \edef\pgfsyssoftpath@temp{{#1}{#2}}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\expandafter{\expandafter\pgfsyssoftpath@specialroundtoken\pgfsyssoftpath@temp}%
}

% Marshallers
\def\pgfsyssoftpath@movetotoken#1#2{\pgfsys@moveto{#1}{#2}}
\def\pgfsyssoftpath@linetotoken#1#2{\pgfsys@lineto{#1}{#2}}
\def\pgfsyssoftpath@rectcornertoken#1#2#3#4#5{\pgfsys@rect{#1}{#2}{#4}{#5}} % #3 = \pgfsyssoftpath@rectsizetoken
\def\pgfsyssoftpath@curvetosupportatoken#1#2#3#4#5#6#7#8{\pgfsys@curveto{#1}{#2}{#4}{#5}{#7}{#8}}
\def\pgfsyssoftpath@closepathtoken#1#2{\pgfsys@closepath}
\let\pgfsyssoftpath@specialroundtoken=\pgfutil@gobbletwo
\def\pgfsyssoftpath@curvetosupportbtoken#1#2{curvetotokenb} % make sure this \ifx-equal only to itself
\def\pgfsyssoftpath@curvetotoken#1#2{curvetotoken}% make sure this \ifx-equal only to itself


\endinput

%%% Local Variables:
%%% mode: latex
%%% End:


==> pgfutil-common-lists.tex <==
% Copyright 2019 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% This list here is a general re-implementation of the list used in
% the PGF system layer.
% It employs two collect-buffers to reduce the runtime.
%
% - It has pre-asymptotical runtime O(N), but is O(N^2) asymptotically.
% - It requires only 5 macros per list.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Usage:
% \pgfapplistnewempty\macro
\def\pgfapplistnewempty#1{%
    \expandafter\let\csname pgfapp@#1\endcsname=\pgfutil@empty
    \expandafter\let\csname pgfapp@#1@smallbuf\endcsname=\pgfutil@empty
    \expandafter\let\csname pgfapp@#1@bigbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfapp@#1@smallbuf@c\endcsname{0}%
    \expandafter\def\csname pgfapp@#1@bigbuf@c\endcsname{0}%
}%

% #1: the item to append
% #2: the list as macro name
\long\def\pgfapplistpushback#1\to#2{%
    \begingroup
        \c@pgf@counta=\csname pgfapp@#2@smallbuf@c\endcsname\relax
        \advance\c@pgf@counta by1
        \xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
    \endgroup
    \expandafter\let\csname pgfapp@#2@smallbuf@c\endcsname=\pgf@glob@TMPa
    \ifnum\csname pgfapp@#2@smallbuf@c\endcsname<40
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
        \expandafter\edef\csname pgfapp@#2@smallbuf\endcsname{\the\t@pgf@toka}%
    \else
        \pgfapplistpushback@smallbufoverfl{#1}{#2}%
    \fi
}%
\long\def\pgfapplistpushback@smallbufoverfl#1#2{%
    \begingroup
        \c@pgf@counta=\csname pgfapp@#2@bigbuf@c\endcsname\relax
        \advance\c@pgf@counta by1
        \xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
    \endgroup
    \expandafter\let\csname pgfapp@#2@bigbuf@c\endcsname=\pgf@glob@TMPa
    %
    \ifnum\csname pgfapp@#2@bigbuf@c\endcsname<30
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2@bigbuf\endcsname}%
        \t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
        \expandafter\edef\csname pgfapp@#2@bigbuf\endcsname{\the\t@pgf@toka\the\t@pgf@tokb}%
        \expandafter\let\csname pgfapp@#2@smallbuf\endcsname=\pgfutil@empty
        \expandafter\def\csname pgfapp@#2@smallbuf@c\endcsname{0}%
    \else%
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2\endcsname}%
        \t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#2@bigbuf\endcsname}%
        \t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
        \expandafter\edef\csname pgfapp@#2\endcsname{\the\t@pgf@toka\the\t@pgf@tokb\the\t@pgf@tokc}%
        \expandafter\let\csname pgfapp@#2@smallbuf\endcsname=\pgfutil@empty
        \expandafter\def\csname pgfapp@#2@smallbuf@c\endcsname{0}%
        \expandafter\let\csname pgfapp@#2@bigbuf\endcsname=\pgfutil@empty
        \expandafter\def\csname pgfapp@#2@bigbuf@c\endcsname{0}%
    \fi%
}%
\def\pgfapplist@flushbuffers#1{%
    \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#1\endcsname}%
    \t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#1@bigbuf\endcsname}%
    \t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfapp@#1@smallbuf\endcsname}%
    \expandafter\edef\csname pgfapp@#1\endcsname{\the\t@pgf@toka\the\t@pgf@tokb\the\t@pgf@tokc}%
    \expandafter\let\csname pgfapp@#1@smallbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfapp@#1@smallbuf@c\endcsname{0}%
    \expandafter\let\csname pgfapp@#1@bigbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfapp@#1@bigbuf@c\endcsname{0}%
}%

\def\pgfapplistlet#1=#2{%
    \pgfapplist@flushbuffers{#2}%
    \expandafter\let\expandafter#1\csname pgfapp@#2\endcsname
}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% A variant of applist which has the same runtime requirements, but
% does PUSH FRONT only.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Usage:
% \pgfprependlistnewempty{list}
\def\pgfprependlistnewempty#1{%
    \expandafter\let\csname pgfpPRP@#1\endcsname=\pgfutil@empty
    \expandafter\let\csname pgfpPRP@#1@smallbuf\endcsname=\pgfutil@empty
    \expandafter\let\csname pgfpPRP@#1@bigbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfpPRP@#1@smallbuf@c\endcsname{0}%
    \expandafter\def\csname pgfpPRP@#1@bigbuf@c\endcsname{0}%
}%

% #1: the item to prepend
% #2: the list as macro name
\long\def\pgfprependlistpushfront#1\to#2{%
    \begingroup
        \c@pgf@counta=\csname pgfpPRP@#2@smallbuf@c\endcsname\relax
        \advance\c@pgf@counta by1
        \xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
    \endgroup
    \expandafter\let\csname pgfpPRP@#2@smallbuf@c\endcsname=\pgf@glob@TMPa
    \ifnum\csname pgfpPRP@#2@smallbuf@c\endcsname<40
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@smallbuf\endcsname}%
        \t@pgf@tokb={#1}%
        \expandafter\edef\csname pgfpPRP@#2@smallbuf\endcsname{\the\t@pgf@tokb\the\t@pgf@toka}%
    \else
        \pgfprependlistpushfront@smallbufoverfl{#1}{#2}%
    \fi
}%
\long\def\pgfprependlistpushfront@smallbufoverfl#1#2{%
    \begingroup
        \c@pgf@counta=\csname pgfpPRP@#2@bigbuf@c\endcsname\relax
        \advance\c@pgf@counta by1
        \xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
    \endgroup
    \expandafter\let\csname pgfpPRP@#2@bigbuf@c\endcsname=\pgf@glob@TMPa
    %
    \ifnum\csname pgfpPRP@#2@bigbuf@c\endcsname<30
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@bigbuf\endcsname}%
        \t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@smallbuf\endcsname}%
        \t@pgf@tokc={#1}%
        \expandafter\edef\csname pgfpPRP@#2@bigbuf\endcsname{\the\t@pgf@tokc\the\t@pgf@tokb\the\t@pgf@toka}%
        \expandafter\let\csname pgfpPRP@#2@smallbuf\endcsname=\pgfutil@empty
        \expandafter\def\csname pgfpPRP@#2@smallbuf@c\endcsname{0}%
    \else%
        \pgfprependlist@flushbuffers{#2}%
        \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2\endcsname}%
        \t@pgf@tokb={#1}%
        \expandafter\edef\csname pgfpPRP@#2\endcsname{\the\t@pgf@tokb\the\t@pgf@toka}%
    \fi%
}%
\def\pgfprependlist@flushbuffers#1{%
    \t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1\endcsname}%
    \t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1@bigbuf\endcsname}%
    \t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1@smallbuf\endcsname}%
    \expandafter\edef\csname pgfpPRP@#1\endcsname{\the\t@pgf@tokc\the\t@pgf@tokb\the\t@pgf@toka}%
    \expandafter\let\csname pgfpPRP@#1@smallbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfpPRP@#1@smallbuf@c\endcsname{0}%
    \expandafter\let\csname pgfpPRP@#1@bigbuf\endcsname=\pgfutil@empty
    \expandafter\def\csname pgfpPRP@#1@bigbuf@c\endcsname{0}%
}%
\def\pgfprependlistlet#1=#2{%
    \pgfprependlist@flushbuffers{#2}%
    \expandafter\let\expandafter#1\csname pgfpPRP@#2\endcsname
}%


==> pgfutil-common.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


%
% This file provides utility commands that are used throughout pgf.
%
% For most commands, the definition of these commands is just given
% below. We cannot use the LaTeX definition of these commands since
% LaTeX may not be the current format and since LaTeX packages tend to
% redefine these commands.
%
% For some commands the actual definition of the format (like latex or
% context) is to be preferred over the generic definition below. In
% this case, the definition of the format is installed when the file
% pgfutil-XXXX.tex is read, where XXXX is the format name (latex,
% plain, or context).



\catcode`\@=11\relax


% Which format is loaded?
\newif\ifpgfutil@format@is@latex
\newif\ifpgfutil@format@is@plain
\newif\ifpgfutil@format@is@context


% Simple stuff

% \pgfutil@trimspaces{<token list>}
%
% Removes spaces on both sides of <token list>.  Same as trimspaces.sty
\catcode`\Q=3
\def\pgfutil@trimspaces#1{%
  \romannumeral-`0\pgfutil@trimspaces@\noexpand#1Q Q}
\def\pgfutil@trimspaces@#1 Q{\pgfutil@trimspaces@@#1Q}
\def\pgfutil@trimspaces@@#1Q#2{#1}
\catcode`\Q=11

% \pgfutil@ifempty{<cs>}{<true code>}{<false code>}
%
% Check if <cs> is equal to \pgfutil@empty
%
% This macro is expandable.
\def\pgfutil@ifempty#1{%
  \ifx#1\pgfutil@empty
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

% \pgfutil@ifundefined{<macro name with backslash>}
%  {<is undefined code>}{<is defined code>}
%
% This will let #1 to \relax if it undefined.
%
% This macro is expandable.
\def\pgfutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

% A variant of \pgfutil@ifundefined which will NOT let #1 to \relax it
% is undefined.
\def\pgfutil@IfUndefined#1{%
  \ifcsname#1\endcsname
    \expandafter\pgfutil@secondoftwo
  \else
    \expandafter\pgfutil@firstoftwo
  \fi
}
\long\def\pgfutil@firstofone#1{#1}
\long\def\pgfutil@firstoftwo#1#2{#1}
\long\def\pgfutil@secondoftwo#1#2{#2}
\def\pgfutil@empty{}
\long\def\pgfutil@gobble@until@relax#1\relax{}
\long\def\pgfutil@gobble#1{}
\long\def\pgfutil@gobbletwo#1#2{}
\def\pgfutil@namedef#1{\expandafter\def\csname #1\endcsname}
\def\pgfutil@namelet#1{\expandafter\pgfutil@@namelet\csname#1\endcsname}
\def\pgfutil@@namelet#1#2{\expandafter\let\expandafter#1\csname#2\endcsname}
\long\def\pgfutil@g@addto@macro#1#2{%
  \begingroup
    \pgfutil@toks@\expandafter{#1#2}%
    \xdef#1{\the\pgfutil@toks@}%
 \endgroup}
\newif\ifpgfutil@tempswa
\newif\ifpgfutil@tempswb

% \pgfutil@pushmacro
% \pgfutil@popmacro
%
% Macro stack.  Allows pushing a macro over \egroup.  Taken from ConTeXt

\let\pgfutil@pushmacro@string\pgfutil@empty

\def\pgfutil@pushmacro#1{%
    \xdef\pgfutil@pushmacro@string{\string#1}%
    \ifcsname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\else
        % \newcount is \outer in Plain
        \csname newcount\expandafter\endcsname\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname
    \fi
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname 1\relax
    \global\expandafter\let\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname#1%
}

\def\pgfutil@popmacro#1{%
    \xdef\pgfutil@pushmacro@string{\string#1}%
    \expandafter\let\expandafter#1\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname -1\relax
}

% pgfutil@ifnextchar

\long\def\pgfutil@ifnextchar#1#2#3{%
  \let\pgfutil@reserved@d=#1%
  \def\pgfutil@reserved@a{#2}%
  \def\pgfutil@reserved@b{#3}%
  \futurelet\pgfutil@let@token\pgfutil@ifnch}
\def\pgfutil@ifnch{%
  \ifx\pgfutil@let@token\pgfutil@sptoken
    \let\pgfutil@reserved@c\pgfutil@xifnch
  \else
    \ifx\pgfutil@let@token\pgfutil@reserved@d
      \let\pgfutil@reserved@c\pgfutil@reserved@a
    \else
      \let\pgfutil@reserved@c\pgfutil@reserved@b
    \fi
  \fi
  \pgfutil@reserved@c}
{%
  \def\:{\global\let\pgfutil@sptoken= } \:
  \def\:{\pgfutil@xifnch} \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ifnch}
}

% pgfutil@ignorespaces

\def\pgfutil@ignorespaces
  {\ifx\pgfutil@let@token\pgfutil@sptoken
     \expandafter\pgfutil@ignorespaces@helper
   \else
     \expandafter\pgfutil@next
   \fi}

{
  \def\:{\pgfutil@ignorespaces@helper}
  \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ignorespaces}
}

% pgfutil@in@

\newif\ifpgfutil@in@

% Usage:
% \pgfutil@in@{one}{three two one}
% \ifpgfutil@in@
%     -> will be true!
% \else
% \fi
%
% \pgfutil@in@{,}{1234,456567}
% \ifpgfutil@in@
%     -> will be true!
% \else
% \fi
\def\pgfutil@in@#1#2{%
 \def\pgfutil@in@@##1#1##2##3\pgfutil@in@@{%
  \ifx\pgfutil@in@##2\pgfutil@in@false\else\pgfutil@in@true\fi}%
 \pgfutil@in@@#2#1\pgfutil@in@\pgfutil@in@@}


% pgfutil@for

\def\pgfutil@nnil{\pgfutil@nil}
\def\pgfutil@fornoop#1\@@#2#3{}
\long\def\pgfutil@for#1:=#2\do#3{%
  \expandafter\def\expandafter\pgfutil@fortmp\expandafter{#2}%
  \ifx\pgfutil@fortmp\pgfutil@empty \else
    \expandafter\pgfutil@forloop#2,\pgfutil@nil,\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\pgfutil@nnil \else
       #5\def#4{#2}\ifx #4\pgfutil@nnil \else#5\pgfutil@iforloop #3\@@#4{#5}\fi\fi}
\long\def\pgfutil@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@iforloop\fi#2\@@#3{#4}}
\def\pgfutil@tfor#1:={\pgfutil@tf@r#1 }
\long\def\pgfutil@tf@r#1#2\do#3{\def\pgfutil@fortmp{#2}\ifx\pgfutil@fortmp\pgfutil@space\else
    \pgfutil@tforloop#2\pgfutil@nil\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@tforloop\fi#2\@@#3{#4}}

\def\pgfutil@space{ }

% pgfutil@IfFileExists

\chardef\pgfutil@inputcheck0
\def\pgfutil@IfFileExists#1#2#3{%
  \openin\pgfutil@inputcheck=#1 %
  \ifeof\pgfutil@inputcheck
     #3\relax
  \else
    #2\relax
  \fi
  \closein\pgfutil@inputcheck}

\def\pgfutil@InputIfFileExists#1#2#3{\pgfutil@IfFileExists{#1}{\input #1\relax#2}{#3}}%


% pgfutil@loop (from plain.tex)

\def\pgfutil@loop#1\pgfutil@repeat{\def\pgfutil@body{#1}\pgfutil@iterate}
\def\pgfutil@iterate{\pgfutil@body \let\pgfutil@next\pgfutil@iterate \else\let\pgfutil@next\relax\fi \pgfutil@next}
\let\pgfutil@repeat=\fi % this makes \loop...\if...\repeat skippable


% \pgfutil@switch
%
% #1: string to switch on
% #2: sequence of label-value pairs
%
% Example:
%
% \pgfutil@switch{foo}{%
%   {foo}{1}%
%   {bar}{2}%
%   {default}{X}%
% }
%
% If a statement with the label `default' exists it will be executed
% if no other label matches.

\long\def\pgfutil@switch#1#2{%
  \begingroup
    \def\pgfutil@switch@selected{}%
    \pgfutil@switch@collect@statements#2{}{}%
    \ifcsname pgfutil@switch@choice@\detokenize{#1}\endcsname
      \expandafter\let\expandafter\pgfutil@switch@selected\csname pgfutil@switch@choice@\detokenize{#1}\endcsname
    \else
      \ifdefined\pgfutil@switch@choice@default
        \let\pgfutil@switch@selected\pgfutil@switch@choice@default
      \fi
    \fi
  \expandafter\endgroup\pgfutil@switch@selected
}

\long\def\pgfutil@switch@collect@statements#1{%
  \if\relax\detokenize{#1}\relax
  \else
    \afterassignment\pgfutil@switch@collect@statements
    \expandafter\def\csname pgfutil@switch@choice@\detokenize{#1}\expandafter\endcsname
  \fi
}


% aux-read-hook

\let\pgfutil@aux@read@hook=\relax


% Tokens for the end of the typesetting -- they will be added at the
% end of every job (hopefully...).

\newtoks\pgfutil@everybye


%
% PDF-Resource management -- might seem strange that this is here, but
% it turns out to be the correct place since latex and context handle
% this stuff quite differently
%

% Adding something to the pdf-resources:

\def\pgfutil@addpdfresource@extgs#1{\pgf@sys@addpdfresource@extgs@plain{#1}}
\def\pgfutil@addpdfresource@colorspaces#1{\pgf@sys@addpdfresource@colorspaces@plain{#1}}
\def\pgfutil@addpdfresource@patterns#1{\pgf@sys@addpdfresource@patterns@plain{#1}}
\def\pgfutil@setuppdfresources{\pgf@sys@setuppdfresources@plain}


% Inserts the argument at the begin of the current page (hopefully)

\let\pgfutil@insertatbegincurrentpage=\relax


% Ragged left and ragged right

\def\pgfutil@raggedright{\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}
\def\pgfutil@raggedleft{\leftskip\z@ plus2em \rightskip\z@ \spaceskip.3333em \xspaceskip.5em\parfillskip0pt\relax}


% Error Messages
\def\pgfutil@packageerror#1#2#3{\errhelp{#3}\errmessage{Package #1 Error: #2}}
\def\pgfutil@packagewarning#1#2{\immediate\write17{Package #1: Warning! #2.}}
\def\pgferror#1{\pgfutil@packageerror{pgf}{#1}{}}
\def\pgfwarning#1{\pgfutil@packagewarning{pgf}{#1}}


% Library files inclusion


% Include a library file.
%
% #1 = List of names of library file.
%
% Description:
%
% This command includes a list of library files. For each file X in the
% list, the file pgflibraryX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgflibrary{arrows}
% \usepgflibrary[patterns,snakes]

\def\usepgflibrary{\pgfutil@ifnextchar[{\use@pgflibrary}{\use@@pgflibrary}}%}
\def\use@pgflibrary[#1]{\use@@pgflibrary{#1}}
\def\use@@pgflibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname pgf@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@library@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@library@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \pgfutil@InputIfFileExists{pgflibrary\pgf@temp.code.tex}{}{%
          \pgferror{I did not find the pgf library
            '\pgf@temp'. I looked for the file named
            pgflibrary\pgf@temp.code.tex, but could not find it in in
            the current texmf trees.}
        }%
      \catcode`\@=\csname pgf@library@#1@atcode\endcsname
      \catcode`\|=\csname pgf@library@#1@barcode\endcsname
      \catcode`\$=\csname pgf@library@#1@dollarcode\endcsname
      \fi%
    \fi
  }%
}


% Include a module file.
%
% #1 = List of names of module files.
%
% Description:
%
% This command includes a list of module files. For each file X in the
% list, the file pgfmoduleX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgfmodule{matrix}

\def\usepgfmodule{\pgfutil@ifnextchar[{\use@pgfmodule}{\use@@pgfmodule}}%}
\def\use@pgfmodule[#1]{\use@@pgfmodule{#1}}
\def\use@@pgfmodule#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@module@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@module@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@module@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@module@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@module@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \input pgfmodule\pgf@temp.code.tex
      \catcode`\@=\csname pgf@module@#1@atcode\endcsname
      \catcode`\|=\csname pgf@module@#1@barcode\endcsname
      \catcode`\$=\csname pgf@module@#1@dollarcode\endcsname
    \fi%
  }%
}

\def\pgfutilensuremath#1{%
  \ifmmode#1\else$#1$\fi
}


%
% Guess the driver:
%

\begingroup
    \catcode`\"=12
    \edef\pgf@loc@TMPa{"}%
    %
    % prepares file names by checking for double colons.
    %
    % If '#1' is a usual file name without anything fancy, \pgfretval
    % will simply contain it. However, if '#1' contains double colons
    % (introduces, for example, by pdftex because there are white
    % spaces in '#1'), the routine
    % - removes the double colons,
    % - re-inserts them outside of the string.
    %
    % \pgfutilpreparefilename{file.tex} -> file.tex
    % \pgfutilpreparefilename{"A file name".file} -> "A file name.file"
    %
    % The resulting file name is returned in '\pgfretval',
    % furthermore, a *quoted* version of the file name is returned in
    % \pgfretvalquoted. The latter result is to have some sort of
    % output normalisation: if the file name as such contains double
    % quotes, we don't want to insert another set of them.
    %
    % This special handling has the following purposes:
    % 1. Both, treatment of white spaces and double colons is not
    % properly defined in TeX. Thus, we should only work with them if
    % necessary and maintain backwards compatibility as far as
    % possible.
    % 2. It *should* work if there are spaces.
    %
    \gdef\pgfutilpreparefilename#1{%
        \begingroup
            \ifnum\the\catcode`\"=13
                \pgfutilconvertdcolon
            \fi
            \xdef\pgf@temp{#1}%
        \endgroup
        \expandafter\pgfutil@in@\expandafter"\expandafter{\pgf@temp}%
        \ifpgfutil@in@
            \def\pgf@loc@TMPa{\pgfutilstrreplace{"}{}}%
            \expandafter\pgf@loc@TMPa\expandafter{\pgf@temp}%
            \edef\pgfretval{"\pgfretval"}% re-insert quotes! Otherwise, TeX can't use the file name.
            \let\pgfretvalquoted=\pgfretval
        \else
            \let\pgfretval=\pgf@temp
            \edef\pgfretvalquoted{"\pgfretval"}%
        \fi
    }%
    \catcode`\"=13
    \xdef\pgfutilconvertdcolon{%
        \noexpand\def\noexpand"{\pgf@loc@TMPa}%
    }%
\endgroup

% Converts an arbitrary command (without arguments) to a string in which all characters
% have category 12.
%
% #1: a macro name (which takes no arguments)
% #2: a macro name which will be assigned to '#1' converted to string.
%
% This uses '\meaning#1' hackery.
\def\pgfutil@command@to@string#1#2{%
    \expandafter\pgfutil@command@to@string@@\meaning#1\pgfutil@EOI{#2}%
}%
\xdef\pgfutil@glob@TMPa{\meaning\pgfutil@empty}%
\expandafter\def\expandafter\pgfutil@command@to@string@@\pgfutil@glob@TMPa#1\pgfutil@EOI#2{%
    \def#2{#1}%
}%
\begingroup
\catcode`\|=0
\catcode`\\=12
|gdef|pgfutil@backslash@as@other{\}%
|endgroup

% Checks if the token sequence #1 (unexpanded) contains a macro and
% invokes #2 if so and #3 if not.
\def\pgfutilifcontainsmacro#1#2#3{%
    \def\pgf@marshal{#1}%
    \pgfutil@command@to@string\pgf@marshal\pgf@marshal
    \edef\pgf@marshal{\noexpand\pgfutil@in@{\pgfutil@backslash@as@other}{\pgf@marshal}}%
    \pgf@marshal
    \ifpgfutil@in@
        \def\pgf@marshal{#2}%
    \else
        \def\pgf@marshal{#3}%
    \fi
    \pgf@marshal
}%

% Tests if string '#2' starts with pattern '#1'.
%
% If so, it executes #3 and defines \pgfretval to contain the
% suffix which is not equal to #1. Otherwise it executes #4.
\def\pgfutilifstartswith#1#2#3#4{%
    \def\pgfutilifstartswith@ ##1#1##2\pgf@EOI{%
        \def\pgfutil@tmp{##1}%
        \ifx\pgfutil@tmp\pgfutil@empty
            % Ah - a hit!
            %
            % define \pgfretval to be the suffix...
            \def\pgfutil@tmp#1####1\pgf@EOI{%
                \def\pgfretval{####1}%
            }%
            \pgfutil@tmp#2\pgf@EOI%
            %
            % ... and execute the <true> code:
            #3\relax%
        \else
            % hm. No such prefix.
            #4\relax%
        \fi
    }%
    \pgfutilifstartswith@#2--#1\pgf@EOI%
}%

% Usage:
% \pgfutilstrreplace{<token>}{<replacement>}{<string>}
%
% -> will assign the modified string into \pgfretval.
%
% #1: the string to search (one or more tokens)
% #2: zero, one or more tokens which will be inserted instead of '#1'.
% #3: the string to search in
\long\def\pgfutilstrreplace#1#2#3{%
    \def\pgfretval{}%
    \long\def\pgfutil@search@and@replace@@##1#1##2\pgf@EOI{%
        \expandafter\def\expandafter\pgfretval\expandafter{\pgfretval ##1#2}%
        \pgfutil@search@and@replace@loop{#1}{##2}%
    }%
    \pgfutil@search@and@replace@loop{#1}{#3}%
}
\long\def\pgfutil@search@and@replace@loop#1#2{%
    \pgfutil@in@{#1}{#2}%
    \ifpgfutil@in@
        \def\pgf@loc@TMPa{\pgfutil@search@and@replace@@ #2\pgf@EOI}%
    \else
        \expandafter\def\expandafter\pgfretval\expandafter{\pgfretval #2}%
        \let\pgf@loc@TMPa=\relax
    \fi
    \pgf@loc@TMPa
}%

% Solves a linear equation system of size 2x2 using gauss elimination.
%
% It employs TeX register arithmetics to do so.
% #1: should contain 4 sets of braces with matrix entries,
%     {<a11>}{<a12>}
%     {<a21>}{<a22>}
%     where each entry should be a number without unit.
%     It is acceptable if '#1' is a macro which expands to the expected
%     format.
% #2: should contain 2 sets of braces with the right-hand-side,
%     {<r1>}{<r2>}
%     where each entry should be a number without unit.
%     It is acceptable if '#2' is a macro which expands to the expected
%     format.
%
% It will assign \pgfmathresult to contain two sets of braces with the
% result.
%
% Example:
% \pgfutilsolvetwotwoleq{
%     {0.24}{1}
%     {-0.97}{0}
% }{
%     {-7}
%     {18}
% }
% -> yields \pgfmathresult={−18.55618}{−2.54642}
%
% The algorithm employs column pivotisation.
%
% If the matrix is singular, the routine will return {}.
\def\pgfutilsolvetwotwoleq#1#2{%
    \begingroup
        \dimendef\aa=0
        \dimendef\ab=1
        \dimendef\ba=2
        \dimendef\bb=3
        \dimendef\ra=4
        \dimendef\rb=5
        \dimendef\tmpa=6
        \dimendef\tmpb=7
        \edef\pgf@temp{#1}%
        \expandafter\pgfutilsolvetwotwoleq@A\pgf@temp
        \edef\pgf@temp{#2}%
        \expandafter\pgfutilsolvetwotwoleq@r\pgf@temp
        %
        \pgfutilsolvetwotwoleq@ifislarger\aa\ba{%
            % identity "permutation":
            \def\Pa{a}%
            \def\Pb{b}%
        }{%
            % permutation matrix: switch rows!
            \def\Pa{b}%
            \def\Pb{a}%
        }%
        % \pivot := 1/aa
        \tmpa=\csname m\Pa a\endcsname pt %
        \ifdim\tmpa<0pt \tmpa=-\tmpa\fi
        \ifdim\tmpa<0.0001pt
            % singular matrix!
            \let\pgfmathresult=\pgfutil@empty
        \else
            \pgfmathreciprocal@
                {\csname m\Pa a\endcsname}%
            \let\pivot=\pgfmathresult
            %
            % \factor := 1/aa * ba
            \csname \Pb a\endcsname=\pivot\csname \Pb a\endcsname
            \edef\factor{\expandafter\pgf@sys@tonumber\csname \Pb a\endcsname}%
            %
            % bb -= ba/aa * ab
            \tmpa=-\factor\csname \Pa b\endcsname
            \advance\csname \Pb b\endcsname by\tmpa
            %
            % rb -= ba/aa * ra
            \tmpa=-\factor\csname r\Pa\endcsname
            \advance\csname r\Pb\endcsname by\tmpa
            %
            \tmpa=\csname \Pb b\endcsname%
            \ifdim\tmpa<0pt \tmpa=-\tmpa\fi
            \ifdim\tmpa<0.0001pt
                % singular matrix!
                \let\pgfmathresult=\pgfutil@empty
            \else
                % xb := rb / bb (the modified rb and modified bb!)
                \pgfmathdivide@
                    {\expandafter\pgf@sys@tonumber\csname r\Pb\endcsname}
                    {\expandafter\pgf@sys@tonumber\csname \Pb b\endcsname}%
                \expandafter\let\csname pgfmathresult\Pb\endcsname=\pgfmathresult
                %
                % ra := ra - xb * ab
                \tmpa=\csname pgfmathresult\Pb\endcsname\csname \Pa b\endcsname
                \advance\csname r\Pa\endcsname by-\tmpa
                %
                % xa := 1/aa * ra  (the modified ra!)
                \tmpa=\pivot\csname r\Pa\endcsname
                \expandafter\edef\csname pgfmathresult\Pa\endcsname{\pgf@sys@tonumber\tmpa}%
                %
                \edef\pgfmathresult{%
                    {\csname pgfmathresult\Pa\endcsname}%
                    {\csname pgfmathresult\Pb\endcsname}%
                }%
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%

\def\pgfutilsolvetwotwoleq@ifislarger#1#2#3#4{%
    \tmpa=#1
    \ifdim\tmpa<0pt
        \multiply\tmpa by-1
    \fi
    \tmpb=#2
    \ifdim\tmpb<0pt
        \multiply\tmpb by-1
    \fi
    \ifdim\tmpa>\tmpb
        #3%
    \else
        #4%
    \fi
}%

\def\pgfutilsolvetwotwoleqfloat@ifislarger#1#2#3#4{%
    \pgfmathfloatabs@{#1}\let\tmpa=\pgfmathresult
    \pgfmathfloatabs@{#2}\let\tmpb=\pgfmathresult
    \pgfmathfloatlessthan@{\tmpb}{\tmpa}%
    \ifpgfmathfloatcomparison
        #3%
    \else
        #4%
    \fi
}%
\def\pgfutilsolvetwotwoleq@A#1#2#3#4{%
    \def\maa{#1}\def\mab{#2}%
    \def\mba{#3}\def\mbb{#3}%
    \aa=#1pt \ab=#2pt
    \ba=#3pt \bb=#4pt
}
\def\pgfutilsolvetwotwoleq@r#1#2{%
    \ra=#1pt \rb=#2pt
}%
\def\pgfutilsolvetwotwoleqfloat@A#1#2#3#4{%
    \pgfmathfloatparsenumber{#1}\let\maa=\pgfmathresult
    \pgfmathfloatparsenumber{#2}\let\mab=\pgfmathresult
    \pgfmathfloatparsenumber{#3}\let\mba=\pgfmathresult
    \pgfmathfloatparsenumber{#4}\let\mbb=\pgfmathresult
}
\def\pgfutilsolvetwotwoleqfloat@r#1#2{%
    \pgfmathfloatparsenumber{#1}\let\ra=\pgfmathresult
    \pgfmathfloatparsenumber{#2}\let\rb=\pgfmathresult
}%

% Same as \pgfutilsolvetwotwoleq, but using floating point
% arithmetics. The return value is still in fixed point.
\def\pgfutilsolvetwotwoleqfloat#1#2{%
    \begingroup
        \pgfmathfloatcreate{1}{1.0}{-4}% FIXME : use a smaller threshold for FPU?
        \let\thresh=\pgfmathresult
        %
        \edef\pgf@temp{#1}%
        \expandafter\pgfutilsolvetwotwoleqfloat@A\pgf@temp
        \edef\pgf@temp{#2}%
        \expandafter\pgfutilsolvetwotwoleqfloat@r\pgf@temp
        %
        \pgfutilsolvetwotwoleqfloat@ifislarger\maa\mba{%
            % identity "permutation":
            \def\Pa{a}%
            \def\Pb{b}%
        }{%
            % permutation matrix: switch rows!
            \def\Pa{b}%
            \def\Pb{a}%
        }%
        % \pivot := 1/aa
        \expandafter\pgfmathfloatabs@\expandafter{\csname m\Pa a\endcsname}%
        \let\tmpa=\pgfmathresult
        \pgfmathfloatlessthan@{\tmpa}{\thresh}%
        \ifpgfmathfloatcomparison
            % singular matrix!
            \let\pgfmathresult=\pgfutil@empty
        \else
            \expandafter\pgfmathfloatreciprocal@\expandafter{\csname m\Pa a\endcsname}%
            \let\pivot=\pgfmathresult
            %
            % \factor := 1/aa * ba
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pb a\endcsname}{\pivot}%
            \let\factor=\pgfmathresult
            \expandafter\let\csname m\Pb a\endcsname=\factor
            %
            % bb -= ba/aa * ab
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pa b\endcsname}{\factor}%
            \let\tmpa=\pgfmathresult
            \expandafter\pgfmathfloatsubtract@\expandafter{\csname m\Pb b\endcsname}{\tmpa}%
            \expandafter\let\csname m\Pb b\endcsname=\pgfmathresult
            %
            % rb -= ba/aa * ra
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname r\Pa\endcsname}{\factor}%
            \let\tmpa=\pgfmathresult
            \expandafter\pgfmathfloatsubtract@\expandafter{\csname r\Pb\endcsname}{\tmpa}%
            \expandafter\let\csname r\Pb\endcsname=\pgfmathresult
            %
            \expandafter\pgfmathfloatabs@\expandafter{\csname m\Pb b\endcsname}%
            \let\tmpa=\pgfmathresult
            \pgfmathfloatlessthan@{\tmpa}{\thresh}%
            \ifpgfmathfloatcomparison
                % singular matrix!
                \let\pgfmathresult=\pgfutil@empty
            \else
                % xb := rb / bb (the modified rb and modified bb!)
                \edef\pgf@marshal{%
                    \noexpand\pgfmathfloatdivide@
                        {\csname r\Pb\endcsname}
                        {\csname m\Pb b\endcsname}%
                }%
                \pgf@marshal
                \expandafter\let\csname pgfmathresult\Pb\endcsname=\pgfmathresult
                \let\tmpa=\pgfmathresult
                %
                % ra := ra - xb * ab
                \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pa b\endcsname}{\tmpa}%
                \let\tmpa=\pgfmathresult
                \expandafter\pgfmathfloatsubtract@\expandafter{\csname r\Pa\endcsname}{\tmpa}%
                \expandafter\let\csname r\Pa\endcsname=\pgfmathresult
                %
                % xa := 1/aa * ra  (the modified ra!)
                \expandafter\pgfmathfloatmultiply@\expandafter{\csname r\Pa\endcsname}{\pivot}%
                \expandafter\let\csname pgfmathresult\Pa\endcsname=\pgfmathresult
                %
                \edef\pgfmathresult{%
                    {\csname pgfmathresult\Pa\endcsname}%
                    {\csname pgfmathresult\Pb\endcsname}%
                }%
                \expandafter\pgfutilsolvetwotwoleqfloat@to@pgf@range\pgfmathresult
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%


\def\pgfutilsolvetwotwoleqfloat@to@pgf@range#1#2{%
    \pgfmathfloatcreate{1}{1.6}{4}\let\pgfutilsolvetwotwoleqfloat@to@pgf@range@max=\pgfmathresult
    \pgfmathfloatabs@{#1}%
    \expandafter\pgfmathfloatlessthan@\expandafter{\pgfmathresult}{\pgfutilsolvetwotwoleqfloat@to@pgf@range@max}%
    \ifpgfmathfloatcomparison
        \pgfmathfloatabs@{#2}%
        \expandafter\pgfmathfloatlessthan@\expandafter{\pgfmathresult}{\pgfutilsolvetwotwoleqfloat@to@pgf@range@max}%
        \ifpgfmathfloatcomparison
            % ok.
            \pgfmathfloattofixed{#1}\let\tmpa=\pgfmathresult
            \pgfmathfloattofixed{#2}%
            \edef\pgfmathresult{{\tmpa}{\pgfmathresult}}%
        \else
            % singular (because PGF cannot represent its result
            \let\pgfmathresult=\pgfutil@empty
        \fi
    \else
        % singular (because PGF cannot represent its result
        \let\pgfmathresult=\pgfutil@empty
    \fi
}%

% there are funny programs which overwrite \read and \write (like
% tabularx).
\let\pgfutil@write=\write
\let\pgfutil@read=\read

% curtesy for latex:
\let\pgfutil@protect\relax

% Used by latex for doing reruns
% #1 = an internal label
% #2 = a to-be-tested text
\def\pgfutil@check@rerun#1#2{}

% new tempdims:
\newdimen\pgfutil@tempdima
\newdimen\pgfutil@tempdimb


% luatex stuff
% We assume luatex version > 0.39:
%   - \directlua <general text> will work
%   - \directlua is the only luatex primitive that we can assume
%     accessible without being prefixed by the format via
%     tex.enableprimitives.
% Ideas taken from the ifluatex package (Heiko Oberdiek)
\let\pgfutil@ifluatex\iffalse
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
\else
  \expandafter\let\csname pgfutil@ifluatex\expandafter\endcsname
    \csname iftrue\endcsname
\fi

\pgfutil@ifluatex
  \let\pgfutil@directlua\directlua
  \pgfutil@directlua{%
    tex.enableprimitives('pgfutil@',{'luaescapestring'})}
\else
  \def\pgfutil@directlua#1{}
  \def\pgfutil@luaescapestring#1{}
\fi


\def\pgfutil@shellescape@lua@eightseven#1{%
    \pgfutil@directlua{os.execute("\pgfutil@luaescapestring{#1}")}%
}%
\def\pgfutil@shellescape#1{%
    \immediate\write18{#1}%
}%
\pgfutil@IfUndefined{directlua}{%
}{%
    \pgfutil@IfUndefined{lastsavedimageresourcepages}{%
        % Ah - an old version of luatex. It still supports \write18
    }{%
        % take the new variant...
        \let\pgfutil@shellescape=\pgfutil@shellescape@lua@eightseven
    }%
}%

% End of luatex stuff

% Advances a number stored in a macro and writes the result back into
% the macro.
% #1 is a macro containing a number.
\def\pgfutil@advancestringcounter#1{%
    \begingroup
        \c@pgf@counta=#1\relax
        \advance\c@pgf@counta by1
        \edef#1{\the\c@pgf@counta}%
        \pgfmath@smuggleone#1%
    \endgroup
}%
\input pgfutil-common-lists.tex

\endinput


==> tikz.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{tikz.code.tex}


\def\tikzerror#1{\pgfutil@packageerror{tikz}{#1}{}}

% Always-present libraries (|\usepgflibrary| defined in
% \file{pgfutil-common.tex}).
\usepgflibrary{plothandlers}

\newdimen\tikz@lastx
\newdimen\tikz@lasty
\newdimen\tikz@lastxsaved
\newdimen\tikz@lastysaved
\newdimen\tikz@lastmovetox
\newdimen\tikz@lastmovetoy

\newdimen\tikzleveldistance
\newdimen\tikzsiblingdistance

\newbox\tikz@figbox
\newbox\tikz@figbox@bg
\newbox\tikz@tempbox
\newbox\tikz@tempbox@bg

\newcount\tikztreelevel
\newcount\tikznumberofchildren
\newcount\tikznumberofcurrentchild

\newcount\tikz@fig@count

\newif\iftikz@node@is@a@label
\newif\iftikz@snaked
\newif\iftikz@decoratepath

\let\tikz@options\pgfutil@empty
% |\tikz@addoption| adds \texttt{#1} at the end of the replacement
% text of |\tikz@options| without expansion.
\def\tikz@addoption#1{%
  \expandafter\def\expandafter\tikz@options\expandafter{\tikz@options#1}}%
% Same as |tikz@addoption| for |\tikz@mode|. Note that |\tikz@mode| is
% initially let to |\pgfutil@empty| later (see path usage options).
\def\tikz@addmode#1{%
  \expandafter\def\expandafter\tikz@mode\expandafter{\tikz@mode#1}}%
% Same as |tikz@addoption| for |\tikz@transform|. Works even if
% |\tikz@transform| is not defined. In that case, nothing is added to
% |\tikz@transform|: \texttt{#1} is expanded.
\def\tikz@addtransform#1{%
  \ifx\tikz@transform\relax
    #1%
  \else
    \expandafter\def\expandafter\tikz@transform\expandafter{\tikz@transform#1}%
  \fi
}%


% TikZ options management.

% Setting up the tikz key family (key management needs
% \file{pgfkeys.code.tex});
\pgfkeys{/tikz/.is family}%

% |\tikzset| is a shortcut to set keys that belongs to the tikz
% family.
\def\tikzset{\pgfqkeys{/tikz}}%

% Note: |\tikzoption| is supported for compatibility only. |\tikzset|
% should be used instead.
\def\tikzoption#1{%
  \pgfutil@ifnextchar[%]
    {\tikzoption@opt{#1}}{\tikzoption@noopt{#1}}}%
\def\tikzoption@opt#1[#2]#3{%
  \pgfkeysdef{/tikz/#1}{#3}%
  \pgfkeyssetvalue{/tikz/#1/.@def}{#2}}%
\def\tikzoption@noopt#1#2{%
  \pgfkeysdef{/tikz/#1}{#2}%
  \pgfkeyssetvalue{/tikz/#1/.@def}{\pgfkeysvaluerequired}}%

% Baseline options
\tikzoption{baseline}[0pt]{%
  \pgfutil@ifnextchar(%)
    {\tikz@baseline@coordinate}{\tikz@baseline@simple}#1\@nil}%
\def\tikz@baseline@simple#1\@nil{\pgfsetbaseline{#1}}%
\def\tikz@baseline@coordinate#1\@nil{%
  \pgfsetbaselinepointlater{\tikz@scan@one@point\pgfutil@firstofone#1}}%

\tikzoption{trim left}[0pt]{\pgfutil@ifnextchar({\tikz@trim@coordinate{left}}{\tikz@trim@simple{left}}#1\@nil}%)%
\tikzoption{trim right}{\pgfutil@ifnextchar({\tikz@trim@coordinate{right}}{\tikz@trim@simple{right}}#1\@nil}%)%
\def\tikz@trim@simple#1#2\@nil{\csname pgfsettrim#1\endcsname{#2}}%
\def\tikz@trim@coordinate#1#2\@nil{\csname pgfsettrim#1pointlater\endcsname{\tikz@scan@one@point\pgfutil@firstofone#2}}%

% Draw options
\tikzoption{line width}{\tikz@semiaddlinewidth{#1}}%

\def\tikz@semiaddlinewidth#1{\tikz@addoption{\pgfsetlinewidth{#1}}\pgfmathsetlength\pgflinewidth{#1}}%

\tikzoption{cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}%
\tikzoption{join}{\tikz@addoption{\csname pgfset#1join\endcsname}}%
\tikzoption{line cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}%
\tikzoption{line join}{\tikz@addoption{\csname pgfset#1join\endcsname}}%
\tikzoption{miter limit}{\tikz@addoption{\pgfsetmiterlimit{#1}}}%

\tikzoption{dash pattern}{% syntax: on 2pt off 3pt on 4pt ...
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi}%
\tikzoption{dash phase}{%
  \def\tikz@dashphase{#1}%
  \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
  \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
}%
\tikzoption{dash}{\tikz@parse@full@dash#1\pgf@stop}%
\def\tikz@parse@full@dash#1phase#2\pgf@stop{%
  \def\tikz@dashphase{#2}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi%
}%
\def\tikz@dashphase{0pt}%
\def\tikz@dashpattern{}%

\def\tikz@scandashon n#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashoff}}%
\def\tikz@scandashoff ff#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashon}}%

% use a decoration to expand the `off' section of a dash pattern.
% https://tex.stackexchange.com/a/133357
\tikzset{
    dash expand off/.code={%
        \ifcsname tikz@library@decorations@loaded\endcsname\else
            \tikzerror{You need \string\usetikzlibrary{decorations} for ``dash offexpand''}%
        \fi
        \tikz@addoption{%
            \pgfgetpath\currentpath
            \pgfprocessround{\currentpath}{\currentpath}%
            \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
            % Parse \on and \off from the current path
            \edef\on{\expandafter\pgfutil@firstoftwo\tikz@dashpattern}%
            \edef\off{\expandafter\pgfutil@secondoftwo\tikz@dashpattern}%
            % \dashphase = max(\on - \dashphase, 0)
            \pgfmathsubtract@{\on}{\tikz@dashphase}%
            \pgfmathmax@{\pgfmathresult}{0}%
            \edef\dashphase{\the\dimexpr\pgfmathresult pt\relax}%
            % \rest = \pgf@decorate@totalpathlength - \on
            \edef\rest{\expandafter\pgf@sys@tonumber\dimexpr\pgf@decorate@totalpathlength - \on + 2\dimexpr\dashphase\relax\relax}%
            % \onoff = \on + \off
            \edef\onoff{\expandafter\pgf@sys@tonumber\dimexpr\on+\off\relax}%
            % \nfullonoff = max(floor(\rest/\onoff), 1)
            \pgfmathdivide@{\rest}{\onoff}%
            \pgfmathfloor@{\pgfmathresult}%
            \pgfmathmax@{\pgfmathresult}{1}%
            % \offexpand = max(\rest/\nfullonoff - \on, \off)
            \pgfmathdivide@{\rest}{\pgfmathresult}%
            \pgfmathsubtract@{\pgfmathresult}{\on}%
            \pgfmathmax@{\pgfmathresult}{\off}%
            \edef\tikz@marshal{\noexpand\pgfsetdash{{\on}{\pgfmathresult}}{\dashphase}}%
            \tikz@marshal
        }%
    }
}

\tikzoption{draw opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}}}%

% Double draw options
\tikzoption{double}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@doublefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \pgfsetinnerstrokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@doubletrue}%
    \tikzset{every double/.try}%
  \fi}%
\tikzoption{double distance}{%
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@setup{%
    \pgf@x=\the\pgf@x%
    \advance\pgf@x by2\pgflinewidth%
    \pgflinewidth=\pgf@x%
    \noexpand\pgfsetlinewidth{\pgflinewidth}%
    \noexpand\pgfsetinnerlinewidth{\the\pgf@x}%
  }%
  \tikzset{double}}%
\def\tikz@double@setup{%
  \pgf@x=2\pgflinewidth%
  \advance\pgf@x by0.6pt%
  \pgflinewidth=\pgf@x%
  \pgfsetlinewidth{\pgflinewidth}%
  \pgfsetinnerlinewidth{0.6pt}%
}%
\tikzset{double distance between line centers/.code={
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@setup{%
    \pgf@x=\pgflinewidth%
    \pgf@xa=\the\pgf@x%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@xa by-\pgflinewidth%
    \pgflinewidth=\pgf@x%
    \noexpand\pgfsetlinewidth{\pgflinewidth}%
    \noexpand\pgfsetinnerlinewidth{\pgf@xa}%
  }%
  \tikzset{double}}}%
\tikzset{double equal sign distance/.style={double distance between line centers=0.45ex}}%




% Fill options

\tikzoption{even odd rule}[]{\tikz@addoption{\pgfseteorule}}%
\tikzoption{nonzero rule}[]{\tikz@addoption{\pgfsetnonzerorule}}%

\tikzoption{fill opacity}{\tikz@addoption{\pgfsetfillopacity{#1}}}%


% Joined fill/draw options

\tikzoption{opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}\pgfsetfillopacity{#1}}}%


% Blend mode

\tikzset{blend mode/.code={\tikz@addoption{\pgfsetblendmode{#1}}}}%


% Main color options
\tikzoption{color}{%
  \tikz@addoption{%
    \ifx\tikz@fillcolor\pgfutil@empty%
      \ifx\tikz@strokecolor\pgfutil@empty%
      \else%
        \pgfsys@color@reset@inorderfalse%
        \let\tikz@strokecolor\pgfutil@empty%
        \let\tikz@fillcolor\pgfutil@empty%
      \fi%
    \else%
      \pgfsys@color@reset@inorderfalse%
      \let\tikz@strokecolor\pgfutil@empty%
      \let\tikz@fillcolor\pgfutil@empty%
    \fi%
    \pgfutil@colorlet{tikz@color}{#1}%
    \pgfutil@colorlet{.}{tikz@color}%
    %
    \pgfsetcolor{.}%
    \pgfsys@color@reset@inordertrue%
  }%
  \def\tikz@textcolor{#1}}%



% Rounding options
\tikzoption{rounded corners}[4pt]{\pgfsetcornersarced{\pgfpoint{#1}{#1}}}%
\tikzoption{sharp corners}[]{\pgfsetcornersarced{\pgfpointorigin}}%

% Radii and arc options
\tikzset{x radius/.initial=0pt}%
\tikzset{y radius/.initial=0pt}%
\tikzset{%
  radius/.code={%
    \pgfmathparse{#1}%
    \ifpgfmathunitsdeclared
      \pgfkeyssetevalue{/tikz/x radius}{\pgfmathresult pt}%
      \pgfkeyssetevalue{/tikz/y radius}{\pgfmathresult pt}%
    \else
      \pgfkeyssetevalue{/tikz/x radius}{\pgfmathresult}%
      \pgfkeyssetevalue{/tikz/y radius}{\pgfmathresult}%
    \fi
  }%
}%
\tikzset{start angle/.initial=}%
\tikzset{end angle/.initial=}%
\tikzset{delta angle/.initial=}%


% Coordinate options
\tikzoption{x}{\tikz@handle@vec{\pgfsetxvec}{\tikz@handle@x}#1\relax}%
\tikzoption{y}{\tikz@handle@vec{\pgfsetyvec}{\tikz@handle@y}#1\relax}%
\tikzoption{z}{\tikz@handle@vec{\pgfsetzvec}{\tikz@handle@z}#1\relax}%

\def\tikz@handle@vec#1#2{\pgfutil@ifnextchar({\tikz@handle@coordinate#1}{\tikz@handle@single#2}}%
\def\tikz@handle@coordinate#1{\tikz@scan@one@point#1}%
\def\tikz@handle@single#1#2\relax{#1{#2}}%
\def\tikz@handle@x#1{\pgfsetxvec{\pgfpoint{#1}{0pt}}}%
\def\tikz@handle@y#1{\pgfsetyvec{\pgfpoint{0pt}{#1}}}%
\def\tikz@handle@z#1{\pgfsetzvec{\pgfpoint{#1}{#1}}}%


% Transformation options
\tikzoption{scale}{\tikz@addtransform{\pgftransformscale{#1}}}%
\tikzoption{scale around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformscale}\tikz@doaround{#1}}}%
\tikzoption{xscale}{\tikz@addtransform{\pgftransformxscale{#1}}}%
\tikzoption{xslant}{\tikz@addtransform{\pgftransformxslant{#1}}}%
\tikzoption{yscale}{\tikz@addtransform{\pgftransformyscale{#1}}}%
\tikzoption{yslant}{\tikz@addtransform{\pgftransformyslant{#1}}}%
\tikzoption{rotate}{\tikz@addtransform{\pgftransformrotate{#1}}}%
\tikzoption{rotate around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformrotate}\tikz@doaround{#1}}}%
\def\tikz@doaround#1{%
  \edef\tikz@temp{#1}% get rid of active stuff
  \expandafter\tikz@doparseA\tikz@temp%
}%
\def\tikz@doparseA#1:{%
  \def\tikz@temp@rot{#1}%
  \tikz@scan@one@point\tikz@doparseB%
}%
\def\tikz@doparseB#1{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@aroundaction{\tikz@temp@rot}%
  \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
}%

\tikzoption{shift}{\tikz@addtransform{\tikz@scan@one@point\pgftransformshift#1\relax}}%
\tikzoption{xshift}{\tikz@addtransform{\pgftransformxshift{#1}}}%
\tikzoption{yshift}{\tikz@addtransform{\pgftransformyshift{#1}}}%
\tikzoption{cm}{\tikz@addtransform{\tikz@parse@cm#1\relax}}%
\tikzoption{reset cm}[]{\tikz@addtransform{\pgftransformreset}}%
\tikzoption{shift only}[]{\tikz@addtransform{\pgftransformresetnontranslations}}%

\def\tikz@parse@cm#1,#2,#3,#4,{%
  \def\tikz@p@cm{{#1}{#2}{#3}{#4}}%
  \tikz@scan@one@point\tikz@parse@cmA}%
\def\tikz@parse@cmA#1{%
  \expandafter\pgftransformcm\tikz@p@cm{#1}%
}%

\tikzset{transform canvas/.code=%
  {%
    \tikz@addoption
    {%
      {%
        \pgftransformreset%
        \let\tikz@transform=\relax%
        \tikzset{#1}%
        \pgflowlevelsynccm%
      }%
      \pgf@relevantforpicturesizefalse%
    }%
  }%
}%

\tikzset{turn/.code={%
    \pgf@x=0pt%
    \pgf@y\pgf@x%
    \pgf@process{\tikz@tangent}%
    \advance\pgf@x by-\tikz@lastx%
    \advance\pgf@y by-\tikz@lasty%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@x=-\pgf@x%
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@ya}}%
    {\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@x}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  }%
}%

\def\tikz@tangent@lookup{%
  \pgfgetpath\tikz@temp%
  \pgfprocesspathextractpoints\tikz@temp%
  \pgfpointsecondlastonpath%
}%

% Code for rotating the xyz coordinate system
% around the x, y, or z vector.
%
\def\tikz@xyz@rotate@let{%
  \let\pgf@z=\pgf@yc%
  \let\pgf@za=\pgf@xc%
}%

\def\tikz@xyz@rotate@xyz@xaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@x=#1\relax%
  \pgf@ya=#2\relax%
  \pgf@za=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@y=\tikz@xyz@cos\pgf@ya%
  \advance\pgf@y by-\tikz@xyz@sin\pgf@za%
  \pgf@z=\tikz@xyz@sin\pgf@ya%
  \advance\pgf@z by\tikz@xyz@cos\pgf@za%
}%

\def\tikz@xyz@rotate@xyz@yaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@xa=#1\relax%
  \pgf@y=#2\relax%
  \pgf@za=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@x=\tikz@xyz@cos\pgf@xa%
  \advance\pgf@x by\tikz@xyz@sin\pgf@za%
  \pgf@z=-\tikz@xyz@sin\pgf@xa%
  \advance\pgf@z by\tikz@xyz@cos\pgf@za%
}%

\def\tikz@xyz@rotate@xyz@zaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@xa=#1\relax%
  \pgf@ya=#2\relax%
  \pgf@z=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@x=\tikz@xyz@cos\pgf@xa%
  \advance\pgf@x by-\tikz@xyz@sin\pgf@ya%
  \pgf@y=\tikz@xyz@sin\pgf@xa%
  \advance\pgf@y by\tikz@xyz@cos\pgf@ya%
}%

\tikzset{rotate around x/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@xaxis{0pt}{1pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@yvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@xaxis{0pt}{0pt}{1pt}{\tikz@xyz@angle}%
    \pgfsetzvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetyvec{\tikz@xyz@rotate@yvec}%
  },
  rotate around y/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@yaxis{1pt}{0pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@xvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@yaxis{0pt}{0pt}{1pt}{\tikz@xyz@angle}%
    \pgfsetzvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetxvec{\tikz@xyz@rotate@xvec}%
  },
  rotate around z/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@zaxis{1pt}{0pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@xvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@zaxis{0pt}{1pt}{0pt}{\tikz@xyz@angle}%
    \pgfsetyvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetxvec{\tikz@xyz@rotate@xvec}%
  },
}%

% Grid options
\tikzoption{xstep}{\def\tikz@grid@x{#1}}%
\tikzoption{ystep}{\def\tikz@grid@y{#1}}%
\tikzoption{step}{\tikz@handle@vec{\tikz@step@point}{\tikz@step@single}#1\relax}%
\def\tikz@step@single#1{\def\tikz@grid@x{#1}\def\tikz@grid@y{#1}}%
\def\tikz@step@point#1{\pgf@process{#1}\edef\tikz@grid@x{\the\pgf@x}\edef\tikz@grid@y{\the\pgf@y}}%

\def\tikz@grid@x{1cm}%
\def\tikz@grid@y{1cm}%


% Current point updates
\newif\iftikz@current@point@local
\tikzset{current point is local/.is if=tikz@current@point@local}%

% Path usage options
\newif\iftikz@mode@double
\newif\iftikz@mode@fill
\newif\iftikz@mode@draw
\newif\iftikz@mode@clip
\newif\iftikz@mode@boundary
\newif\iftikz@mode@shade
\newif\iftikz@mode@fade@path
\newif\iftikz@mode@fade@scope
\let\tikz@mode=\pgfutil@empty

\def\tikz@nonetext{none}%

\tikzoption{path only}[]{\let\tikz@mode=\pgfutil@empty}%
\tikzset{
  shade/.is choice,
  shade/.default=true,
  shade/true/.code=\tikz@addmode{\tikz@mode@shadetrue},
  shade/false/.code=\tikz@addmode{\tikz@mode@shadefalse},
  shade/none/.code=\tikz@addmode{\tikz@mode@shadefalse},
}%

\tikzoption{fill}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillcolor{#1}}%
      \def\tikz@fillcolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}%
\tikzoption{draw}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@drawfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetstrokecolor{#1}}%
      \def\tikz@strokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@drawtrue}%
  \fi%
}%
\tikzoption{clip}[]{\tikz@addmode{\tikz@mode@cliptrue}}%
\tikzoption{use as bounding box}[]{\tikz@addmode{\tikz@mode@boundarytrue}}%

\tikzoption{save path}{\tikz@addmode{\pgfsyssoftpath@getcurrentpath#1\global\let#1=#1}}%
\tikzoption{use path}{\tikz@addmode{\pgfsyssoftpath@setcurrentpath#1}}%

\let\tikz@fillcolor=\pgfutil@empty
\let\tikz@strokecolor=\pgfutil@empty

% Insert a path using an option
\tikzset{insert path/.code=\tikz@scan@next@command#1\pgf@stop}%

% Pattern options
\tikzset{pattern/.code=\tikzerror{You need to say \string\usetikzlibrary{patterns}},
         pattern color/.style=pattern}%

% Path pictures
\tikzset{path picture/.code=\tikz@addmode{\def\tikz@path@picture{#1}}}%

% Fading options
\tikzset{path fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@pathfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@path@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@pathtrue}%
  \fi%
  },
  path fading/.default=,
  scope fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@scopefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@scope@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@scopetrue}%
  \fi%
  },
  scope fading/.default=}%
\tikzset{fit fading/.is if=tikz@fade@adjust}%
\tikzset{fading transform/.store in=\tikz@fade@transform}%
\tikzset{fading angle/.style={fading transform={rotate=#1}}}%

\newif\iftikz@fade@adjust%
\tikz@fade@adjusttrue%
\let\tikz@fade@transform\pgfutil@empty%

\pgfutil@colorlet{transparent}{pgftransparent}%
\def\tikz@do@fade@transform{\let\tikz@transform=\relax\expandafter\tikzset\expandafter{\tikz@fade@transform}}%



% Transparency groups
\newif\iftikz@transparency@group%
\tikzset{/tikz/transparency group/.code=\tikz@transparency@grouptrue\def\tikz@transparency@group@options{isolated=true,#1}\let\tikz@blend@group\pgfutil@empty}%
\tikzset{/tikz/blend group/.code=\tikz@transparency@grouptrue\def\tikz@transparency@group@options{isolated=true}\def\tikz@blend@group{\pgfsetblendmode{#1}}}%

\let\tikz@blend@group\pgfutil@empty

% Shading options
\tikzoption{shading}{\def\tikz@shading{#1}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{shading angle}{\def\tikz@shade@angle{#1}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{top color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{bottom color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{middle color}{%
  \pgfutil@colorlet{tikz@axis@middle}{#1}%
  \def\tikz@shading{axis}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{left color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{right color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{ball}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{inner color}{\pgfutil@colorlet{tikz@radial@inner}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{outer color}{\pgfutil@colorlet{tikz@radial@outer}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}%

\def\tikz@shading{axis}%
\def\tikz@shade@angle{0}%

\pgfdeclareverticalshading[tikz@axis@top,tikz@axis@middle,tikz@axis@bottom]{axis}{100bp}{%
  color(0bp)=(tikz@axis@bottom);
  color(25bp)=(tikz@axis@bottom);
  color(50bp)=(tikz@axis@middle);
  color(75bp)=(tikz@axis@top);
  color(100bp)=(tikz@axis@top)}%

\pgfutil@colorlet{tikz@axis@top}{gray}%
\pgfutil@colorlet{tikz@axis@middle}{gray!50!white}%
\pgfutil@colorlet{tikz@axis@bottom}{white}%

\pgfdeclareradialshading[tikz@ball]{ball}{\pgfqpoint{-10bp}{10bp}}{%
 color(0bp)=(tikz@ball!15!white);
 color(9bp)=(tikz@ball!75!white);
 color(18bp)=(tikz@ball!70!black);
 color(25bp)=(tikz@ball!50!black);
 color(50bp)=(black)}%

\pgfutil@colorlet{tikz@ball}{blue}%

\pgfdeclareradialshading[tikz@radial@inner,tikz@radial@outer]{radial}{\pgfpointorigin}{%
 color(0bp)=(tikz@radial@inner);
 color(25bp)=(tikz@radial@outer);
 color(50bp)=(tikz@radial@outer)}%

\pgfutil@colorlet{tikz@radial@inner}{gray}%
\pgfutil@colorlet{tikz@radial@outer}{white}%


% Pin options
\tikzset{
  pin distance/.store in=\tikz@pin@distance,
  pin distance=3ex,
  pin position/.store in=\tikz@pin@default@pos,
  pin position=above,
  pin edge/.store in=\tikz@pin@edge@style,
  pin edge={},
  tikz@pin@post/.code={\global\let\tikz@pin@edge@style@smuggle=\tikz@pin@edge@style},
  tikz@pre@pin@edge/.code={%
    \toks0=\expandafter{\tikz@pin@edge@style@smuggle}%
    \edef\pgf@marshal{\noexpand\tikzset{tikz@pin@options/.style={\the\toks0}}}%
    \pgf@marshal
  },%
}%

\tikzset{%
  pin/.code={%
    \begingroup
      \ifnum\the\catcode`\:=\active\relax
        \def\tikz@next{%
          \endgroup
          \tikz@parse@pin@active@i{#1}}%
      \else
        \def\tikz@next{%
          \endgroup
          \pgfutil@ifnextchar[%]
            {\tikz@parse@pin@nonactive}
            {\tikz@parse@pin@nonactive[]}#1:\pgf@nil}%
      \fi
    \tikz@next}}%

\begingroup
  \catcode`\:=\active\relax

  \gdef\tikz@parse@pin@active@i#1{%
    \pgfutil@ifnextchar[%]
      {\tikz@parse@pin@active}
      {\tikz@parse@pin@active[]}#1:\pgf@nil}%

  \long\gdef\tikz@parse@pin@active[#1]#2:#3\pgf@nil{%
    \def\tikz@temp{#3}%
    \ifx\tikz@temp\pgfutil@empty
      % no position, use default
      \tikz@@parse@pin@active[#1]\tikz@pin@default@pos:#2:\pgf@nil%
    \else
      \tikz@@parse@pin@active[#1]#2:#3\pgf@nil%
    \fi}%

  \long\gdef\tikz@@parse@pin@active[#1]#2:#3:\pgf@nil{%
    \tikzset{%
      append after command = {%
        \bgroup
          [current point is local = true]
          \pgfextra{\let\tikz@save@last@node=\tikzlastnode\tikz@node@is@a@labelfalse}%
          node [tikz@label@angle = #2,
                anchor=@auto,
                every pin,
                #1,
                append after command = {%
                  (\tikz@save@last@node)
                  edge [every pin edge,
                        tikz@pre@pin@edge,
                        tikz@pin@options]
                  (\tikzlastnode)},
                tikz@label@post = \tikz@pin@distance,
                tikz@pin@post] {#3}
        \egroup}}}%
\endgroup

\long\def\tikz@parse@pin@nonactive[#1]#2:#3\pgf@nil{%
  \def\tikz@temp{#3}%
  \ifx\tikz@temp\pgfutil@empty
    % no position, use default
    \tikz@@parse@pin@nonactive[#1]\tikz@pin@default@pos:#2:\pgf@nil%
  \else
    \tikz@@parse@pin@nonactive[#1]#2:#3\pgf@nil%
  \fi}%

\long\def\tikz@@parse@pin@nonactive[#1]#2:#3:\pgf@nil{%
  \tikzset{%
    append after command = {%
      \bgroup
        [current point is local = true]
        \pgfextra{\let\tikz@save@last@node=\tikzlastnode\tikz@node@is@a@labelfalse}%
        node [tikz@label@angle = #2,
              anchor=@auto,
              every pin,
              #1,
              append after command = {%
                (\tikz@save@last@node)
                edge [every pin edge,
                      tikz@pre@pin@edge,
                      tikz@pin@options]
                (\tikzlastnode)},
              tikz@label@post = \tikz@pin@distance,
              tikz@pin@post] {#3}
      \egroup}}}%

% Label and pin options

\tikzset{
  label distance/.store in=\tikz@label@distance,
  label distance=0pt,
  label position/.store in=\tikz@label@default@pos,
  label position=above,
  absolute/.is if=tikz@absolute,
  tikz@label@angle/.store in=\tikz@label@angle
}%

\newif\iftikz@absolute
\def\tikz@on@text{center}%

\tikzset{tikz@label@post/.code 2 args={
  \edef\tikz@label@angle{\tikz@label@angle}%
  \expandafter\pgfkeys@spdef\expandafter\tikz@label@angle\expandafter{\tikz@label@angle}%
  \csname tikz@label@angle@is@\tikz@label@angle\endcsname
  \ifx\tikz@label@angle\tikz@on@text%
    \def\tikz@node@at{\pgfpointanchor{\tikzlastnode}{center}}%
    \def\tikz@anchor{center}%
  \else%
    \iftikz@absolute%
      \pgftransformreset%
      \pgf@process{%
        \pgfpointshapeborder{\tikzlastnode}%
        {\pgfpointadd{\pgfpointanchor{\tikzlastnode}{center}}{\pgfpointpolar{\tikz@label@angle}{1pt}}}}%
      \edef\tikz@node@at{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      \tikz@compute@direction{\tikz@label@angle}%
      \tikz@addtransform{\pgftransformshift{\pgfpointpolar{\tikz@label@angle}{#1}}}%
    \else%
      \pgf@process{\pgfpointanchor{\tikzlastnode}{\tikz@label@angle}}%
      \edef\tikz@node@at{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      \pgf@xb=\pgf@x%
      \pgf@yb=\pgf@y%
      \pgf@process{\pgfpointanchor{\tikzlastnode}{center}}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@y%
      \tikz@label@simplefalse%
      \ifdim\pgf@xc=\pgf@xb\relax%
        \ifdim\pgf@yc=\pgf@yb\relax%
          \tikz@label@simpletrue%
        \fi%
      \fi%
      \iftikz@label@simple%
        \tikz@compute@direction{\tikz@label@angle}%
        \tikz@addtransform{\pgftransformshift{\pgfpointpolar{\tikz@label@angle}{#1}}}%
      \else%
        \pgf@process{\pgfpointnormalised{%
            \pgfpointdiff{\pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}}{\pgfpointtransformed{\pgfqpoint{\pgf@xb}{\pgf@yb}}}}}%
        \edef\pgf@marshal{%
          \noexpand\tikz@addtransform{\noexpand\pgftransformshift{\noexpand\pgfpointscale{#1}{
                \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}}%
        \pgf@marshal%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgf@x=\pgf@yc%
        \pgf@y=-\pgf@xc%
        \ifx\tikz@anchor\tikz@auto@text%
          \tikz@auto@anchor%
        \fi%
      \fi%
    \fi%
  \fi}
}%

\newif\iftikz@label@simple%

\tikzset{%
  label/.code={%
    \begingroup
      \ifnum\the\catcode`\:=\active\relax
        \def\tikz@next{%
          \endgroup
          \tikz@parse@label@active@i{#1}}%
      \else
        \def\tikz@next{%
          \endgroup
          \pgfutil@ifnextchar[%]
            {\tikz@parse@label@nonactive}
            {\tikz@parse@label@nonactive[]}#1:\pgf@nil}%
      \fi
    \tikz@next}}%

\begingroup
  \catcode`\:=\active\relax

  \gdef\tikz@parse@label@active@i#1{%
    \pgfutil@ifnextchar[%]
      {\tikz@parse@label@active}
      {\tikz@parse@label@active[]}#1:\pgf@nil}%

  \gdef\tikz@parse@label@active[#1]#2:#3\pgf@nil{%
    \def\tikz@temp{#3}%
    \ifx\tikz@temp\pgfutil@empty
    % no position, use default
      \tikz@@parse@label@active[#1]\tikz@label@default@pos:#2:\pgf@nil%
    \else
      \def\tikz@temp{#2}%
      \ifx\tikz@temp\pgfutil@empty
        \tikz@@parse@label@active[#1]\tikz@label@default@pos:#3\pgf@nil%
      \else
        \tikz@@parse@label@active[#1]#2:#3\pgf@nil%
      \fi
    \fi
  }%

  \gdef\tikz@@parse@label@active[#1]#2:#3:\pgf@nil{%
    \tikzset{%
      append after command = {%
        \bgroup
          [current point is local=true]
          \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name\tikz@node@is@a@labelfalse}
          node [tikz@label@angle = #2,
                anchor=@auto,
                every label,
                #1,
                tikz@label@post = \tikz@label@distance] {\iftikz@handle@active@nodes\expandafter\scantokens\else\expandafter\pgfutil@firstofone\fi{#3\noexpand}}
          \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}
        \egroup}}}%
\endgroup

\def\tikz@parse@label@nonactive[#1]#2:#3\pgf@nil{%
  \def\tikz@temp{#3}%
  \ifx\tikz@temp\pgfutil@empty
    % no position, use default
    \tikz@@parse@label@nonactive[#1]\tikz@label@default@pos:#2:\pgf@nil%
  \else
    \def\tikz@temp{#2}%
    \ifx\tikz@temp\pgfutil@empty
      \tikz@@parse@label@nonactive[#1]\tikz@label@default@pos:#3\pgf@nil%
    \else
      \tikz@@parse@label@nonactive[#1]#2:#3\pgf@nil%
    \fi
  \fi
}%

\def\tikz@@parse@label@nonactive[#1]#2:#3:\pgf@nil{%
  \tikzset{%
    append after command = {%
      \bgroup
        [current point is local=true]
        \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name\tikz@node@is@a@labelfalse}
        node [tikz@label@angle = #2,
              anchor=@auto,
              every label,
              #1,
              tikz@label@post = \tikz@label@distance] {\iftikz@handle@active@nodes\expandafter\scantokens\else\expandafter\pgfutil@firstofone\fi{#3\noexpand}}
        \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}
      \egroup}}}%

\expandafter\def\csname tikz@label@angle@is@right\endcsname{\def\tikz@label@angle{0}}%
\expandafter\def\csname tikz@label@angle@is@above right\endcsname{\def\tikz@label@angle{45}}%
\expandafter\def\csname tikz@label@angle@is@above\endcsname{\def\tikz@label@angle{90}}%
\expandafter\def\csname tikz@label@angle@is@above left\endcsname{\def\tikz@label@angle{135}}%
\expandafter\def\csname tikz@label@angle@is@left\endcsname{\def\tikz@label@angle{180}}%
\expandafter\def\csname tikz@label@angle@is@below left\endcsname{\def\tikz@label@angle{225}}%
\expandafter\def\csname tikz@label@angle@is@below\endcsname{\def\tikz@label@angle{270}}%
\expandafter\def\csname tikz@label@angle@is@below right\endcsname{\def\tikz@label@angle{315}}%

\def\tikz@compute@direction#1{%
  \ifx\tikz@anchor\tikz@auto@text%
  \let\tikz@do@auto@anchor=\relax
  \pgfmathsetcount{\c@pgf@counta}{#1}%
  \ifnum\c@pgf@counta<0\relax
    \advance\c@pgf@counta by 360\relax%
  \fi%
  \ifnum\c@pgf@counta>359\relax
    \advance\c@pgf@counta by-360\relax%
  \fi%
  \ifnum\c@pgf@counta<4\relax%
    \def\tikz@anchor{west}%
  \else\ifnum\c@pgf@counta<87\relax%
    \def\tikz@anchor{south west}%
  \else\ifnum\c@pgf@counta<94\relax%
    \def\tikz@anchor{south}%
  \else\ifnum\c@pgf@counta<177\relax%
    \def\tikz@anchor{south east}%
  \else\ifnum\c@pgf@counta<184\relax%
    \def\tikz@anchor{east}%
  \else\ifnum\c@pgf@counta<267\relax%
    \def\tikz@anchor{north east}%
  \else\ifnum\c@pgf@counta<274\relax%
    \def\tikz@anchor{north}%
  \else\ifnum\c@pgf@counta<357\relax%
    \def\tikz@anchor{north west}%
  \else%
    \def\tikz@anchor{west}%
  \fi\fi\fi\fi\fi\fi\fi\fi%
  \fi%
}%
\def\tikz@auto@text{@auto}%

% General node options
\tikzset{
  name/.code={\edef\tikz@fig@name{\tikz@pp@name{#1}}\let\tikz@id@name\tikz@fig@name},%
  name prefix/.initial=,%
  name suffix/.initial=%
}%
\def\tikz@pp@name#1{\csname pgfk@/tikz/name prefix\endcsname#1\csname pgfk@/tikz/name suffix\endcsname}%


\tikzset{
  node contents/.code=\def\tikz@node@content{#1},
  pic type/.code=\def\tikz@node@content{#1}, % alias
}%

\tikzset{
  behind path/.code=\def\tikz@whichbox{\tikz@figbox@bg},
  in front of path/.code=\def\tikz@whichbox{\tikz@figbox}
}%
\def\tikz@whichbox{\tikz@figbox}%

\tikzoption{at}{\tikz@scan@one@point\tikz@set@at#1}%
\def\tikz@set@at#1{\def\tikz@node@at{#1}}%

\tikzoption{shape}{\edef\tikz@shape{#1}}%

\tikzoption{nodes}{\tikzset{every node/.append style={#1}}}%

\tikzset{alias/.code={%
    \tikz@fig@mustbenamed
    \begingroup
    \toks0=\expandafter{\tikz@alias}%
    \edef\pgf@temp{\noexpand\pgfnodealias{\tikz@pp@name{#1}}{\noexpand\tikz@fig@name}}%
    \toks1=\expandafter{\pgf@temp}%
    \xdef\pgf@marshal{%
        \noexpand\def\noexpand\tikz@alias{\the\toks0 \the\toks1 }%
    }%
    \endgroup
    \pgf@marshal
}}%

% deprecated:
\def\tikzaddafternodepathoption#1{#1\tikzset{prefix after command={\pgfextra{#1}}}}%
\tikzset{after node path/.style={append after command={#1}}}%


% Pic options
\newif\iftikz@node@is@pic
\tikzset{pic text/.store in=\tikzpictext}%
\let\tikzpictext\relax
\tikzset{pic text options/.store in=\tikzpictextoptions}%
\let\tikzpictextoptions\pgfutil@empty


% Anchoring

\tikzoption{anchor}{\def\tikz@anchor{#1}\let\tikz@do@auto@anchor=\relax}%

\tikzoption{left}[]{\def\tikz@anchor{east}\tikz@possibly@transform{x}{-}{#1}}%
\tikzoption{right}[]{\def\tikz@anchor{west}\tikz@possibly@transform{x}{}{#1}}%
\tikzoption{above}[]{\def\tikz@anchor{south}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{below}[]{\def\tikz@anchor{north}\tikz@possibly@transform{y}{-}{#1}}%
\tikzoption{above left}[]%
  {\def\tikz@anchor{south east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{above right}[]%
  {\def\tikz@anchor{south west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{below left}[]%
  {\def\tikz@anchor{north east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{-}{#1}}%
\tikzoption{below right}[]%
  {\def\tikz@anchor{north west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{-}{#1}}%
\tikzset{centered/.code=\def\tikz@anchor{center}}%

\tikzoption{node distance}{\def\tikz@node@distance{#1}}%
\def\tikz@node@distance{1cm}%

% The following are deprecated:
\tikzoption{above of}{\tikz@of{#1}{90}}%
\tikzoption{below of}{\tikz@of{#1}{-90}}%
\tikzoption{left of}{\tikz@of{#1}{180}}%
\tikzoption{right of}{\tikz@of{#1}{0}}%
\tikzoption{above left of}{\tikz@of{#1}{135}}%
\tikzoption{below left of}{\tikz@of{#1}{-135}}%
\tikzoption{above right of}{\tikz@of{#1}{45}}%
\tikzoption{below right of}{\tikz@of{#1}{-45}}%
\def\tikz@of#1#2{%
  \def\tikz@anchor{center}%
  \let\tikz@do@auto@anchor=\relax%
  \tikz@addtransform{%
    \expandafter\tikz@extract@node@dist\tikz@node@distance and\pgf@stop%
    \pgftransformshift{\pgfpointpolar{#2}{\tikz@extracted@node@distance}}}%
  \def\tikz@node@at{\pgfpointanchor{\tikz@pp@name{#1}}{center}}}%
\def\tikz@extract@node@dist#1and#2\pgf@stop{%
  \def\tikz@extracted@node@distance{#1}}%

\tikzset{
  transform shape nonlinear/.is choice,
  transform shape nonlinear/.default=true,
  transform shape nonlinear/true/.code=\let\tikz@nlt\relax,
  transform shape nonlinear/false/.code=\def\tikz@nlt{\pgfapproximatenonlineartranslation},
  transform shape nonlinear=false,
}%


\tikzoption{transform shape}[true]{%
  \csname tikz@fullytransformed#1\endcsname%
  \iftikz@fullytransformed%
    \pgfresetnontranslationattimefalse%
  \else%
    \pgfresetnontranslationattimetrue%
  \fi%
}%

\newif\iftikz@fullytransformed
\pgfresetnontranslationattimetrue%

\def\tikz@anchor{center}%
\def\tikz@shape{rectangle}%

\def\tikz@possibly@transform#1#2#3{%
  \let\tikz@do@auto@anchor=\relax%
  \def\tikz@test{#3}%
  \ifx\tikz@test\pgfutil@empty%
  \else%
    \pgfmathsetlength{\pgf@x}{#3}%
    \pgf@x=#2\pgf@x\relax%
    \edef\tikz@marshal{\noexpand\tikz@addtransform{%
        \expandafter\noexpand\csname  pgftransform#1shift\endcsname{\the\pgf@x}}}%
    \tikz@marshal%
  \fi%
}%


% Inter-picture options
\tikzoption{remember picture}[true]{\csname pgfrememberpicturepositiononpage#1\endcsname}
\tikzset{
    overlay/.is choice,
    overlay/true/.code={\pgf@relevantforpicturesizefalse},
    overlay/false/.code={\pgf@relevantforpicturesizetrue},
    overlay/.default=true
}



% Line/curve label placement options
\tikzoption{sloped}[true]{\csname pgfslopedattime#1\endcsname}%
\tikzoption{allow upside down}[true]{\csname pgfallowupsidedownattime#1\endcsname}%

\tikzoption{pos}{\edef\tikz@time{#1}\ifx\tikz@time\pgfutil@empty\else\pgfmathsetmacro\tikz@time{\tikz@time}\fi}%

\tikzoption{auto}[]{\csname tikz@install@auto@anchor@#1\endcsname}%
\tikzoption{swap}[]{%
  \def\tikz@temp{left}%
  \ifx\tikz@auto@anchor@direction\tikz@temp%
    \def\tikz@auto@anchor@direction{right}%
  \else%
    \def\tikz@auto@anchor@direction{left}%
  \fi%
}%
\tikzset{'/.style=swap}% shorthand


\def\tikz@install@auto@anchor@{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on}%
\def\tikz@install@auto@anchor@false{\let\tikz@do@auto@anchor=\relax}%
\def\tikz@install@auto@anchor@left{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{left}}%
\def\tikz@install@auto@anchor@right{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{right}}%

\let\tikz@do@auto@anchor=\relax%

\def\tikz@auto@anchor@on{\csname tikz@auto@anchor@\tikz@auto@anchor@direction\endcsname}

\def\tikz@auto@anchor@left{\tikz@auto@pre\tikz@auto@anchor\tikz@auto@post}%
\def\tikz@auto@anchor@right{\tikz@auto@pre\tikz@auto@anchor@prime\tikz@auto@post}%

\def\tikz@auto@anchor@direction{left}%

% Text options
\tikzoption{text}{\def\tikz@textcolor{#1}}%
\tikzoption{font}{\def\tikz@textfont{#1}}%
\tikzoption{node font}{\def\tikz@node@textfont{#1}}%
\tikzoption{text opacity}{\def\tikz@textopacity{#1}}%
\tikzoption{text width}{\def\tikz@text@width{#1}}%
\tikzoption{text height}{\def\tikz@text@height{#1}}%
\tikzoption{text depth}{\def\tikz@text@depth{#1}}%
\tikzoption{text ragged}[]%
{\def\tikz@text@action{\pgfutil@raggedright\rightskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}}%
\tikzoption{text badly ragged}[]{\def\tikz@text@action{\pgfutil@raggedright\relax}}%
\tikzoption{text ragged left}[]%
{\def\tikz@text@action{\pgfutil@raggedleft\leftskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}}%
\tikzoption{text badly ragged left}[]{\def\tikz@text@action{\pgfutil@raggedleft\relax}}%
\tikzoption{text justified}[]{\def\tikz@text@action{\leftskip0pt\rightskip0pt\relax}}%
\tikzoption{text centered}[]{\def\tikz@text@action{%
  \leftskip0pt plus2em%
  \rightskip0pt plus2em%
  \spaceskip.3333em \xspaceskip.5em%
  \parfillskip=0pt%
  \iftikz@warn@for@narrow@centered\else\hbadness10000\fi%
  \let\\=\@centercr% for latex
  \relax}}%
\tikzoption{text badly centered}[]%
{\def\tikz@text@action{%
  \let\\=\@centercr% for latex
  \parfillskip=0pt%
  \rightskip\pgfutil@flushglue%
  \leftskip\pgfutil@flushglue\relax}}%
\tikzset{badness warnings for centered text/.is if=tikz@warn@for@narrow@centered}%
\newif\iftikz@warn@for@narrow@centered

\def\tikz@text@reset{%
  \let\tikz@text@width=\pgfutil@empty
  \let\tikz@text@height=\pgfutil@empty
  \let\tikz@text@depth=\pgfutil@empty
  \let\tikz@textcolor=\pgfutil@empty
  \let\tikz@textfont=\pgfutil@empty
  \let\tikz@textopacity=\pgfutil@empty
  \let\tikz@node@textfont=\pgfutil@empty
  \def\tikz@text@action{\pgfutil@raggedright\rightskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}%
}
\tikz@text@reset


% Alignment
\tikzset{
  node halign header/.initial=,
  align/.is choice,
  align/left/.style  ={text ragged,node halign header=\tikz@align@left@header},
  align/flush left/.style  ={text badly ragged,node halign header=\tikz@align@left@header},
  align/right/.style ={text ragged left,node halign header=\tikz@align@right@header},
  align/flush right/.style ={text badly ragged left,node halign header=\tikz@align@right@header},
  align/center/.style={text centered,node halign header=\tikz@align@center@header},
  align/flush center/.style={text badly centered,node halign header=\tikz@align@center@header},
  align/justify/.style ={text justified,node halign header=\tikz@align@left@header},
  align/none/.style ={text justified,node halign header=},
}%
\def\tikz@align@left@header{##\hfil\cr}%
\def\tikz@align@right@header{\hfil##\cr}%
\def\tikz@align@center@header{\hfil##\hfil\cr}%



% Arrow options
\tikzoption{arrows}{\tikz@processarrows{#1}}%


\tikzoption{>}{\pgfdeclarearrow{name=<->,means={#1}}}%
\pgfdeclarearrow{name=|<->|,   means={>[sep=0pt].|}}%

\tikzoption{shorten <}{\pgfsetshortenstart{#1}}%
\tikzoption{shorten >}{\pgfsetshortenend{#1}}%

\def\tikz@processarrows#1{%
  \def\tikz@current@arrows{#1}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else%
    \pgfsetarrows{#1}%
  \fi%
}%

\def\tikz@current@arrows{-}%

% Parabola options
\tikzoption{bend}{\tikz@scan@one@point\tikz@set@parabola@bend#1\relax}%
\tikzoption{bend pos}{\def\tikz@parabola@bend@factor{#1}}%
\tikzoption{parabola height}{%
  \def\tikz@parabola@bend@factor{.5}%
  \def\tikz@parabola@bend{\pgfpointadd{\pgfpoint{0pt}{#1}}{\tikz@last@position@saved}}}%

\def\tikz@parabola@bend{\tikz@last@position@saved}%
\def\tikz@parabola@bend@factor{0}%

\def\tikz@set@parabola@bend#1{\def\tikz@parabola@bend{#1}}%

% Axis options
\tikzoption{domain}{\edef\tikz@plot@domain{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}%
\tikzoption{range}{\def\tikz@plot@range{#1}}%
\tikzoption{yrange}{\def\tikz@plot@range{#1}}%
\let\tikz@plot@range=\pgfutil@empty
\tikzoption{xrange}{\def\tikz@plot@xrange{#1}}%
\let\tikz@plot@xrange=\pgfutil@empty

% Plot options
\tikzoption{smooth}[]{\let\tikz@plot@handler=\pgfplothandlercurveto}%
\tikzoption{smooth cycle}[]{\let\tikz@plot@handler=\pgfplothandlerclosedcurve}%
\tikzoption{sharp plot}[]{\let\tikz@plot@handler\pgfplothandlerlineto}%
\tikzoption{sharp cycle}[]{\let\tikz@plot@handler\pgfplothandlerpolygon}%

\tikzoption{tension}{\pgfsetplottension{#1}}%

\tikzoption{xcomb}[]{\let\tikz@plot@handler=\pgfplothandlerxcomb}%
\tikzoption{ycomb}[]{\let\tikz@plot@handler=\pgfplothandlerycomb}%
\tikzoption{polar comb}[]{\let\tikz@plot@handler=\pgfplothandlerpolarcomb}%
\tikzoption{ybar}[]{\let\tikz@plot@handler=\pgfplothandlerybar}%
\tikzoption{ybar interval}[]{\let\tikz@plot@handler=\pgfplothandlerybarinterval}%
\tikzoption{xbar interval}[]{\let\tikz@plot@handler=\pgfplothandlerxbarinterval}%
\tikzoption{xbar}[]{\let\tikz@plot@handler=\pgfplothandlerxbar}%
\tikzoption{const plot}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}%
\tikzoption{const plot mark left}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}%
\tikzoption{const plot mark right}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkright}%
\tikzoption{const plot mark mid}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkmid}%
\tikzoption{jump mark right}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkright}%
\tikzoption{jump mark mid}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkmid}%
\tikzoption{jump mark left}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkleft}%

\tikzoption{raw gnuplot}[true]{\csname tikz@plot@raw@gnuplot#1\endcsname}%
\tikzoption{prefix}{\def\tikz@plot@prefix{#1}}%
\tikzoption{id}{\def\tikz@plot@id{#1}}%

\tikzoption{samples}{\pgfmathsetmacro\tikz@plot@samples{max(2,#1)}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}%
\tikzoption{samples at}{\def\tikz@plot@samplesat{#1}}%
\tikzoption{parametric}[true]{\csname tikz@plot@parametric#1\endcsname}%

\tikzoption{variable}{\def\tikz@plot@var{#1}}%

\tikzoption{only marks}[]{\let\tikz@plot@handler\pgfplothandlerdiscard}%

\tikzoption{mark}{%
    \def\tikz@plot@mark{#1}%
    \def\tikz@temp{none}%
    \ifx\tikz@temp\tikz@plot@mark
        \let\tikz@plot@mark=\pgfutil@empty
    \fi
}%
\tikzset{
    no marks/.style={mark=none},%
    no markers/.style={mark=none},%
    every mark/.style={},
    mark options/.style={%
        every mark/.style={#1}%
    }}%
\tikzoption{mark size}{\pgfsetplotmarksize{#1}}%

\tikzoption{mark indices}{\def\tikz@mark@list{#1}}%
\tikzoption{mark phase}{\pgfsetplotmarkphase{#1}}%
\tikzoption{mark repeat}{\pgfsetplotmarkrepeat{#1}}%

\let\tikz@mark@list=\pgfutil@empty

\let\tikz@plot@handler=\pgfplothandlerlineto
\let\tikz@plot@mark=\pgfutil@empty

\def\tikz@plot@samples{25}%
\def\tikz@plot@domain{-5:5}%
\def\tikz@plot@var{\x}%
\def\tikz@plot@samplesat{-5,-4.5833333,...,5}%
\def\tikz@plot@samples@recalc#1:#2\relax{%
  \begingroup
  \pgfmathparse{#1}%
  \let\tikz@temp@start=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\tikz@temp@end=\pgfmathresult%
  \pgfmathsetmacro\tikz@temp@diff{(\tikz@temp@end-\tikz@temp@start)/(\tikz@plot@samples-1)}%
  %
  % this particular item is for backwards compatibility.
  % Pgfplots <= 1.8 called 'samples' in a context where the 'fpu' was
  % active... and I fear there is no simple solution to replace the
  % new \ifdim below. Sorry.
  \pgfkeys{/pgf/fpu/output format/fixed/.try}%
  %
  \pgfmathsetmacro\tikz@temp@diff@abs{abs(\tikz@temp@diff)}%
  \ifdim\tikz@temp@diff@abs pt<0.0001pt\relax%
    \edef\tikz@plot@samplesat{\tikz@temp@start,\tikz@temp@end}%
  \else%
    \pgfmathparse{\tikz@temp@start+\tikz@temp@diff}%
    \edef\tikz@plot@samplesat{\tikz@temp@start,\pgfmathresult,...,\tikz@temp@end}%
  \fi%
  \pgfmath@smuggleone\tikz@plot@samplesat
  \endgroup
}%


\def\tikz@plot@prefix{\jobname.}%
\def\tikz@plot@id{pgf-plot}%

\newif\iftikz@plot@parametric
\newif\iftikz@plot@raw@gnuplot


%
% To and edge options
%
\tikzoption{to path}{\def\tikz@to@path{#1}}%

\def\tikz@to@path{-- (\tikztotarget) \tikztonodes}%

\tikzset{edge macro/.store in=\tikz@edge@macro}%
\let\tikz@edge@macro\pgfutil@empty

\tikzset{
  edge node/.code={
    \expandafter\def\expandafter\tikz@tonodes\expandafter{\tikz@tonodes #1}
  },
  edge label/.style={/tikz/edge node={node[auto]{#1}}},
  edge label'/.style={/tikz/edge node={node[auto,swap]{#1}}},
}%


% After command options
\tikzset{
  append after command/.code=\expandafter\def\expandafter\tikz@after@path\expandafter{\tikz@after@path#1},
  prefix after command/.code={%
    \def\tikz@temp{#1}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\tikz@after@path%
    \expandafter\expandafter\expandafter{%
      \expandafter\tikz@temp\tikz@after@path}%
  },
}%
\let\tikz@after@path\pgfutil@empty


% Tree options
\newif\iftikz@child@missing
\pgfkeys{/tikz/missing/.is if=tikz@child@missing}%

\tikzset{edge from parent macro/.initial=\tikz@edge@from@parent@macro}%
\def\tikz@edge@from@parent@macro#1#2{
  [style=edge from parent, #1, /utils/exec=\tikz@node@is@a@labeltrue] \tikz@edge@to@parent@path #2}%

\tikzoption{edge from parent path}{\def\tikz@edge@to@parent@path{#1}}%

\tikzoption{parent anchor}{\def\tikzparentanchor{.#1}\ifx\tikzparentanchor\tikz@border@text\let\tikzparentanchor\pgfutil@empty\fi}%
\tikzoption{child anchor}{\def\tikzchildanchor{.#1}\ifx\tikzchildanchor\tikz@border@text\let\tikzchildanchor\pgfutil@empty\fi}%

\tikzoption{level distance}{\pgfmathsetlength\tikzleveldistance{#1}}%
\tikzoption{sibling distance}{\pgfmathsetlength\tikzsiblingdistance{#1}}%

\tikzoption{growth function}{\let\tikz@grow=#1}%

\tikzset{grow siblings on line/.style={growth function=\tikz@grow@direction}}%

\tikzoption{growth parent anchor}{\def\tikz@growth@anchor{#1}}%
\tikzoption{grow}{\tikz@set@growth{#1}\edef\tikz@special@level{\the\tikztreelevel}}%
\tikzoption{grow'}{\tikz@set@growth{#1}\tikz@swap@growth\edef\tikz@special@level{\the\tikztreelevel}}%

\def\tikz@growth@anchor{center}%

\def\tikz@special@level{-1}% never

\def\tikz@swap@growth{%
  % Swap left and right
  \let\tikz@temp=\tikz@angle@grow@right%
  \let\tikz@angle@grow@right=\tikz@angle@grow@left%
  \let\tikz@angle@grow@left=\tikz@temp%
}%

\def\tikz@set@growth#1{%
  \let\tikz@grow=\tikz@grow@direction%
  \expandafter\ifx\csname tikz@grow@direction@#1\endcsname\relax%
    \c@pgf@counta=#1\relax%
  \else%
    \c@pgf@counta=\csname tikz@grow@direction@#1\endcsname%
  \fi%
  \edef\tikz@angle@grow{\the\c@pgf@counta}%
  \advance\c@pgf@counta by-90\relax%
  \edef\tikz@angle@grow@left{\the\c@pgf@counta}%
  \advance\c@pgf@counta by180\relax%
  \edef\tikz@angle@grow@right{\the\c@pgf@counta}%
}%

\def\tikz@border@text{.border}%
\let\tikzparentanchor=\pgfutil@empty
\let\tikzchildanchor=\pgfutil@empty
\def\tikz@edge@to@parent@path{(\tikzparentnode\tikzparentanchor) -- (\tikzchildnode\tikzchildanchor)}%

\tikzleveldistance=15mm%
\tikzsiblingdistance=15mm%

\def\tikz@grow@direction@down{-90}%
\def\tikz@grow@direction@up{90}%
\def\tikz@grow@direction@left{180}%
\def\tikz@grow@direction@right{0}%

\def\tikz@grow@direction@south{-90}%
\def\tikz@grow@direction@north{90}%
\def\tikz@grow@direction@west{180}%
\def\tikz@grow@direction@east{0}%

\expandafter\def\csname tikz@grow@direction@north east\endcsname{45}%
\expandafter\def\csname tikz@grow@direction@north west\endcsname{135}%
\expandafter\def\csname tikz@grow@direction@south east\endcsname{-45}%
\expandafter\def\csname tikz@grow@direction@south west\endcsname{-135}%

\def\tikz@grow@direction{%
  \pgftransformshift{\pgfpointpolar{\tikz@angle@grow}{\tikzleveldistance}}%
  \ifnum\tikztreelevel=\tikz@special@level%
  \else%
    \pgf@xc=.5\tikzsiblingdistance%
    \c@pgf@counta=\tikznumberofchildren%
    \advance\c@pgf@counta by1\relax%
    \pgfutil@tempdima=\c@pgf@counta\pgf@xc%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@left}{\pgfutil@tempdima}}%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@right}{\tikznumberofcurrentchild\tikzsiblingdistance}}%
  \fi%
}%

\tikzset{grow=down}%


% Snakes are in a lib:
\tikzset{snake/.code=\tikzerror{You need to say \string\usetikzlibrary{snakes}}}%

% Decorations
\tikzset{decorate/.code=\tikzerror{You need to load a  decoration library}}%

% Matrix options
\usepgfmodule{matrix}%

\tikzoption{matrix}[true]{\csname tikz@is@matrix#1\endcsname}%

\tikzoption{matrix anchor}{\def\tikz@matrix@anchor{#1}}%

\tikzoption{column sep}{\def\pgfmatrixcolumnsep{#1}}%
\tikzoption{row sep}{\def\pgfmatrixrowsep{#1}}%

\tikzoption{cells}{\tikzset{every cell/.append style={#1}}}%

\tikzoption{ampersand replacement}{\def\tikz@ampersand@replacement{#1}}%

\newif\iftikz@is@matrix
\let\tikz@matrix@anchor=\pgfutil@empty
\let\tikz@ampersand@replacement=\pgfutil@empty


% Automatic shorthand management
\tikzset{%
  handle active characters in code/.is if=tikz@handle@active@code,
  handle active characters in nodes/.is if=tikz@handle@active@nodes,
}%
\newif\iftikz@handle@active@code
\newif\iftikz@handle@active@nodes


% Execute option
\tikzoption{execute at begin picture}{\expandafter\def\expandafter\tikz@atbegin@picture\expandafter{\tikz@atbegin@picture#1}}%
\tikzoption{execute at end picture}{\expandafter\def\expandafter\tikz@atend@picture\expandafter{\tikz@atend@picture#1}}%
\tikzoption{execute at begin scope}{\expandafter\def\expandafter\tikz@atbegin@scope\expandafter{\tikz@atbegin@scope#1}}%
\tikzoption{execute at end scope}{\expandafter\def\expandafter\tikz@atend@scope\expandafter{\tikz@atend@scope#1}}%
\tikzoption{execute at begin to}{\expandafter\def\expandafter\tikz@atbegin@to\expandafter{\tikz@atbegin@to#1}}%
\tikzoption{execute at end to}{\expandafter\def\expandafter\tikz@atend@to\expandafter{\tikz@atend@to#1}}%
\tikzoption{execute at begin node}{\expandafter\def\expandafter\tikz@atbegin@node\expandafter{\tikz@atbegin@node#1}}%
\tikzoption{execute at end node}{\expandafter\def\expandafter\tikz@atend@node\expandafter{\tikz@atend@node#1}}%
\tikzoption{execute at begin matrix}{\expandafter\def\expandafter\tikz@atbegin@matrix\expandafter{\tikz@atbegin@matrix#1}}%
\tikzoption{execute at end matrix}{\expandafter\def\expandafter\tikz@atend@matrix\expandafter{\tikz@atend@matrix#1}}%
\tikzoption{execute at begin cell}{\expandafter\def\expandafter\tikz@atbegin@cell\expandafter{\tikz@atbegin@cell#1}}%
\tikzoption{execute at end cell}{\expandafter\def\expandafter\tikz@atend@cell\expandafter{\tikz@atend@cell#1}}%
\tikzoption{execute at empty cell}{\expandafter\def\expandafter\tikz@at@emptycell\expandafter{\tikz@at@emptycell#1}}%

\let\tikz@atbegin@picture=\pgfutil@empty
\let\tikz@atend@picture=\pgfutil@empty
\let\tikz@atbegin@scope=\pgfutil@empty
\let\tikz@atend@scope=\pgfutil@empty
\let\tikz@atbegin@to=\pgfutil@empty
\let\tikz@atend@to=\pgfutil@empty
\let\tikz@atbegin@node=\pgfutil@empty
\let\tikz@atend@node=\pgfutil@empty
\let\tikz@atbegin@cell=\pgfutil@empty
\let\tikz@atend@cell=\pgfutil@empty
\let\tikz@at@emptycell=\pgfutil@empty
\let\tikz@atbegin@matrix=\pgfutil@empty
\let\tikz@atend@matrix=\pgfutil@empty


% Pre and post actions
\tikzset{preaction/.code=\expandafter\def\expandafter\tikz@preactions\expandafter{\tikz@preactions\tikz@extra@preaction{#1}}}%
\tikzset{postaction/.code=\expandafter\def\expandafter\tikz@postactions\expandafter{\tikz@postactions\tikz@extra@postaction{#1}}}%
\let\tikz@preactions=\pgfutil@empty
\let\tikz@postactions=\pgfutil@empty

% Styles
\tikzoption{set style}{\tikzstyle#1}%

% Handled in a special way.
\def\tikzstyle{\pgfutil@ifnextchar\bgroup\tikz@style@parseA\tikz@style@parseB}%
\def\tikz@style@parseB#1={\tikz@style@parseA{#1}=}%
\def\tikz@style@parseA#1#2=#3[#4]{% check for an optional argument
  \pgfutil@in@[{#2}%]
  \ifpgfutil@in@%
    \tikz@style@parseC{#1}#2={#4}%
  \else%
    \tikz@style@parseD{#1}#2={#4}%
  \fi%
}%

\def\tikz@style@parseC#1[#2]#3=#4{%
  \pgfkeys{/tikz/#1/.default={#2}}%
  \pgfutil@in@+{#3}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#4}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#4}}%
  \fi}%
\def\tikz@style@parseD#1#2=#3{%
  \pgfutil@in@+{#2}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#3}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#3}}%
  \fi}%


%
%
% Predefined styles
%
%

\tikzset{help lines/.style=              {color=gray,line width=0.2pt}}%

\tikzset{every picture/.style=           {}}%
\tikzset{every path/.style=              {}}%
\tikzset{every scope/.style=             {}}%
\tikzset{every plot/.style=              {}}%
\tikzset{every node/.style=              {}}%
\tikzset{every child/.style=             {}}%
\tikzset{every child node/.style=        {}}%
\tikzset{every to/.style=                {}}%
\tikzset{every cell/.style=              {}}%
\tikzset{every matrix/.style=            {}}%
\tikzset{every edge/.style=              {draw}}%
\tikzset{every label/.style=             {draw=none,fill=none}}%
\tikzset{every pin/.style=               {draw=none,fill=none}}%
\tikzset{every pin edge/.style=          {help lines}}%

\tikzset{ultra thin/.style=              {line width=0.1pt}}%
\tikzset{very thin/.style=               {line width=0.2pt}}%
\tikzset{thin/.style=                    {line width=0.4pt}}%
\tikzset{semithick/.style=               {line width=0.6pt}}%
\tikzset{thick/.style=                   {line width=0.8pt}}%
\tikzset{very thick/.style=              {line width=1.2pt}}%
\tikzset{ultra thick/.style=             {line width=1.6pt}}%

\tikzset{solid/.style=                   {dash pattern=}}%
\tikzset{dotted/.style=                  {dash pattern=on \pgflinewidth off 2pt}}%
\tikzset{densely dotted/.style=          {dash pattern=on \pgflinewidth off 1pt}}%
\tikzset{loosely dotted/.style=          {dash pattern=on \pgflinewidth off 4pt}}%
\tikzset{dashed/.style=                  {dash pattern=on 3pt off 3pt}}%
\tikzset{densely dashed/.style=          {dash pattern=on 3pt off 2pt}}%
\tikzset{loosely dashed/.style=          {dash pattern=on 3pt off 6pt}}%
\tikzset{dashdotted/.style=              {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{dash dot/.style=                {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dashdotted/.style=      {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{densely dash dot/.style=        {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dashdotted/.style=      {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{loosely dash dot/.style=        {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{dashdotdotted/.style=           {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dashdotdotted/.style=   {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dashdotdotted/.style=   {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{dash dot dot/.style=         {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dash dot dot/.style=   {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dash dot dot/.style=   {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt on \the\pgflinewidth off 4pt}}%


\tikzset{transparent/.style=             {opacity=0}}%
\tikzset{ultra nearly transparent/.style={opacity=0.05}}%
\tikzset{very nearly transparent/.style= {opacity=0.1}}%
\tikzset{nearly transparent/.style=      {opacity=0.25}}%
\tikzset{semitransparent/.style=         {opacity=0.5}}%
\tikzset{nearly opaque/.style=           {opacity=0.75}}%
\tikzset{very nearly opaque/.style=      {opacity=0.9}}%
\tikzset{ultra nearly opaque/.style=     {opacity=0.95}}%
\tikzset{opaque/.style=                  {opacity=1}}%

\tikzset{at start/.style=                {pos=0}}%
\tikzset{very near start/.style=         {pos=0.125}}%
\tikzset{near start/.style=              {pos=0.25}}%
\tikzset{midway/.style=                  {pos=0.5}}%
\tikzset{near end/.style=                {pos=0.75}}%
\tikzset{very near end/.style=           {pos=0.875}}%
\tikzset{at end/.style=                  {pos=1}}%

\tikzset{bend at start/.style=           {bend pos=0,bend={+(0,0)}}}%
\tikzset{bend at end/.style=             {bend pos=1,bend={+(0,0)}}}%

\tikzset{edge from parent/.style=        {draw}}%



% Animation callbacks
\tikzset{
  animate/.code=\tikzerror{You need to say \string\usetikzlibrary{animations} to use animations}
}

% ID callbacks
\newif\iftikz@is@node
\let\tikz@id@name\pgfutil@empty
\let\tikz@id@hook\pgfutil@empty
\def\tikz@call@id@hook{\ifx\tikz@id@hook\pgfutil@empty\else\tikz@id@hook\pgfuseid{\tikz@id@name}\fi}%


% RDF stuff
\let\tikz@clear@rdf@options\relax
\let\tikz@do@rdf@post@options\relax
\let\tikz@do@rdf@pre@options\relax


%
% Setting keys
%

\pgfkeys{/tikz/style/.style=#1}%

\pgfkeys{/tikz/.unknown/.code=%
  % Is it a pgf key?
  \let\tikz@key\pgfkeyscurrentname%
  \pgfkeys{/pgf/\tikz@key/.try={#1}}%
  \ifpgfkeyssuccess%
  \else%
    \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
    \ifpgfutil@in@%
      % this is a color!
      \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
      \edef\tikz@textcolor{\tikz@key}%
    \else%
      \pgfutil@doifcolorelse{\tikz@key}
      {%
        \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
        \edef\tikz@textcolor{\tikz@key}%
      }%
      {%
        % Ok, second chance: This might be an arrow specification:
        \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          % Ah, an arrow spec!
          \expandafter\tikz@processarrows\expandafter{\tikz@key}%
        \else%
          % Ok, third chance: A shape!
          \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
            \pgfkeys{/errors/unknown key/.expand
              once=\expandafter{\expandafter/\expandafter t\expandafter i\expandafter k\expandafter z\expandafter/\tikz@key}{#1}}%
          \else%
            \edef\tikz@shape{\tikz@key}%
          \fi%
        \fi%
      }%
    \fi%
  \fi%
}%
\def\tikz@compat@color@set#1{%
  \pgfutil@color{#1}\pgfutil@colorlet{pgffillcolor}{#1}%
  \expandafter\let\expandafter\pgf@temp\csname\string\color@pgffillcolor\endcsname%
  % for arrow tips:
  \global\let\pgf@strokecolor@global=\pgf@temp
  \global\let\pgf@fillcolor@global=\pgf@temp
}%

\def\tikz@startup@env{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\expandafter\tikz@origsemi\expandafter=\tikz@activesemicolon\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\expandafter\tikz@origcolon\expandafter=\tikz@activecolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\expandafter\tikz@origbar\expandafter=\tikz@activebar\fi%
  \tikz@deactivatthings%
  \iftikz@handle@active@code%
    \tikz@switchoff@shorthands%
  \fi%
}%

%
% Main TikZ Environment
%
\newif\iftikz@inside@picture
\tikz@inside@picturefalse
\def\tikz@check@inside@picture{%
  \iftikz@inside@picture%
    \pgfwarning{Nesting tikzpictures is NOT supported}%
  \fi%
  \tikz@inside@picturetrue%
}

\def\tikzpicture{%
  \begingroup%
    \tikz@startup@env%
    \tikz@collect@scope@anims\tikz@picture}%
\def\tikz@picture[#1]{%
  %\tikz@check@inside@picture%
  \pgfpicture%
  \let\tikz@atbegin@picture=\pgfutil@empty%
  \let\tikz@atend@picture=\pgfutil@empty%
  \let\tikz@transform=\relax%
  \def\tikz@time{.5}%
  \tikz@installcommands%
  \scope[every picture,#1]%
  \iftikz@handle@active@code%
    \tikz@switchoff@shorthands%
  \fi%
  \expandafter\tikz@atbegin@picture%
  \tikz@lib@scope@check%
}%
\def\endtikzpicture{%
    \tikz@atend@picture%
    \global\let\pgf@shift@baseline@smuggle=\pgf@baseline%
    \global\let\pgf@trimleft@final@smuggle=\pgf@trimleft%
    \global\let\pgf@trimright@final@smuggle=\pgf@trimright%
    \global\let\pgf@remember@smuggle=\ifpgfrememberpicturepositiononpage%
    \pgf@remember@layerlist@globally
    \endscope%
    \let\pgf@baseline=\pgf@shift@baseline@smuggle%
    \let\pgf@trimleft=\pgf@trimleft@final@smuggle%
    \let\pgf@trimright=\pgf@trimright@final@smuggle%
    \let\ifpgfrememberpicturepositiononpage=\pgf@remember@smuggle%
    \pgf@restore@layerlist@from@global
  \endpgfpicture\endgroup}%


% Inlined picture
%
% #1 - some code to be put in a tikzpicture environment.
%
% If the command is not followed by braces, everything up to the next
% semicolon is used as argument.
%
% Example:
%
% The rectangle \tikz{\draw (0,0) rectangle (1em,1ex)} has width 1em and
% height 1ex.


\def\tikz{%
  \begingroup%
    \tikz@startup@env%
    \tikz@collect@scope@anims\tikz@opt}%
\def\tikz@opt[#1]{\tikzpicture[#1]\pgfutil@ifnextchar\bgroup{\tikz@}{\tikz@@single}}%
\def\tikz@{\bgroup\tikz@auto@end@pathtrue\aftergroup\endtikzpicture\aftergroup\endgroup\let\pgf@temp=}%
\def\tikz@@single#1{%
  \expandafter\ifx\csname tikz@protected@command\string#1\endcsname\relax%
    \expandafter\tikz@@%
  \else%
    \begingroup\def\tikz@path@do@at@end{\endgroup\endtikzpicture\endgroup}%
  \fi%
  #1%
}%

\expandafter\let\csname tikz@protected@command\string\draw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\pattern\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\fill\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\filldraw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\shade\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\shadedraw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\clip\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\graph\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\useasboundingbox\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\node\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\coordinate\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\matrix\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\datavisualization\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\path\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\pic\endcsname\pgfutil@empty%

% Comment by TT: I hope I fixed the \tikz \foreach problem. The new
% version will take a conservative approach and will only do fancy
% stuff when the next keyword after \tikz is one of the following:
% \draw, \fill, \filldraw, \graph, \matrix,
\def\tikz@@{%
  \let\tikz@next=\tikz@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@collectactivesemicolon%
  \fi%
  \tikz@next}%
\def\tikz@collectnormalsemicolon#1;{#1;\endtikzpicture\endgroup}
{
  \catcode`\;=\active
  \gdef\tikz@collectactivesemicolon#1;{#1;\endtikzpicture\endgroup}
}%
% End old code

% Invokes '#1' if the command is invoked within a tikzpicture and
% '#2' if not.
\def\tikzifinpicture#1#2{%
    \pgfutil@ifundefined{filldraw}{#2}{#1}% TT: This is a wrong
                                % test! Who uses this?...
}%


\def\tikz@collect@scope@anims#1{%
  \pgfutil@ifnextchar[#1{#1[]}%]
}%

%
% Environment for scoping graphic state settings
%
\def\tikz@scope@env{%
  \pgfscope%
  \begingroup%
  \let\tikz@atbegin@scope=\pgfutil@empty%
  \let\tikz@atend@scope=\pgfutil@empty%
  \let\tikz@options=\pgfutil@empty%
  \tikz@clear@rdf@options%
  \let\tikz@mode=\pgfutil@empty%
  \let\tikz@id@name=\pgfutil@empty%
  \tikz@transparency@groupfalse%
  \tikzset{every scope/.try}%
  \tikz@collect@scope@anims\tikz@scope@opt%
}%
\def\tikz@scope@opt[#1]{%
  \tikzset{#1}%
  \tikz@options%
  \tikz@do@rdf@pre@options%
  \iftikz@transparency@group\expandafter\pgftransparencygroup\expandafter[\tikz@transparency@group@options]\tikz@blend@group\fi%
  \tikz@is@nodefalse%
  \tikz@call@id@hook%
  \pgfidscope%
    \tikz@do@rdf@post@options%
    \begingroup%
      \let\tikz@id@name\pgfutil@empty%
      \expandafter\tikz@atbegin@scope%
      \expandafter\pgfclearid%
      \tikz@lib@scope@check%
}%
\def\endtikz@scope@env{%
      \tikz@atend@scope%
    \endgroup%
  \endpgfidscope%
  \iftikz@transparency@group\endpgftransparencygroup\fi%
  \endgroup%
  \endpgfscope%
  \tikz@lib@scope@check%
}%


\def\tikz@scoped{\tikz@collect@scope@anims\tikz@scoped@opt}%
\def\tikz@scoped@opt[#1]{\scope[#1]\pgfutil@ifnextchar\bgroup{\tikz@scoped@}{\tikz@scoped@@single}}%
\def\tikz@scoped@{\bgroup\tikz@auto@end@pathtrue\aftergroup\endscope\let\pgf@temp=}%
\def\tikz@scoped@@single#1{%
  \expandafter\ifx\csname tikz@scoped@protected@command\string#1\endcsname\relax%
    \expandafter\tikz@scoped@@%
  \else%
    \begingroup\def\tikz@scoped@path@do@at@end{\endgroup\endscope}%
  \fi%
  #1%
}%
\def\tikz@scoped@@{%
  \let\tikz@scoped@next=\tikz@scoped@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@scoped@next=\tikz@scoped@collectactivesemicolon%
  \fi%
  \tikz@scoped@next}%
\def\tikz@scoped@collectnormalsemicolon#1;{#1;\endscope}
{
  \catcode`\;=\active
  \gdef\tikz@scoped@collectactivesemicolon#1;{#1;\endscope}
}%


% Install a shortcut command which is only valid inside of a
% tikzpicture.
%
% It works in the same way as the '\path' shortcut does: it introduces
% a \let#1=#2 at the beginning of tikzpicture.
%
% #1: shortcut command inside of tikzpicture
% #2: real command name
\def\tikzaddtikzonlycommandshortcutlet#1#2{%
    \expandafter\def\expandafter\tikz@installcommands\expandafter{\tikz@installcommands
        \let#1=#2%
    }%
}%

% Has the same effect as \tikzaddtikzonlycommandshortcutlet but uses
% \def#1{#2} instead of \let.
\def\tikzaddtikzonlycommandshortcutdef#1#2{%
    \expandafter\def\expandafter\tikz@installcommands\expandafter{\tikz@installcommands
        \def#1{#2}%
    }%
}%

%
% Install the abbreviated commands
%
\def\tikz@installcommands{%
  \let\tikz@origscope=\scope%
  \let\tikz@origscoped=\scoped%
  \let\tikz@origendscope=\endscope%
  \let\tikz@origstartscope=\startscope%
  \let\tikz@origstopscope=\stopscope%
  \let\tikz@origpath=\path%
  \let\tikz@origagainpath=\againpath%
  \let\tikz@origdraw=\draw%
  \let\tikz@origpattern=\pattern%
  \let\tikz@origfill=\fill%
  \let\tikz@origfilldraw=\filldraw%
  \let\tikz@origshade=\shade%
  \let\tikz@origshadedraw=\shadedraw%
  \let\tikz@origclip=\clip%
  \let\tikz@origuseasboundingbox=\useasboundingbox%
  \let\tikz@orignode=\node%
  \let\tikz@origpic=\pic%
  \let\tikz@origcoordinate=\coordinate%
  \let\tikz@origmatrix=\matrix%
  \let\tikz@origcalendar=\calendar%
  \let\tikz@origdv=\datavisualization%
  \let\tikz@origgraph=\graph%
  %
  \let\scope=\tikz@scope@env%
  \let\scoped=\tikz@scoped%
  \let\endscope=\endtikz@scope@env%
  \let\startscope=\scope%
  \let\stopscope=\endscope%
  \let\path=\tikz@command@path%
  \let\againpath=\tikz@command@againpath%
  %
  \def\draw{\path[draw]}%
  \def\pattern{\path[pattern]}%
  \def\fill{\path[fill]}%
  \def\filldraw{\path[fill,draw]}%
  \def\shade{\path[shade]}%
  \def\shadedraw{\path[shade,draw]}%
  \def\clip{\path[clip]}%
  \def\graph{\path graph}%
  \def\useasboundingbox{\path[use as bounding box]}%
  \def\node{\tikz@path@overlay{node}}%
  \def\pic{\tikz@path@overlay{pic}}%
  \def\coordinate{\tikz@path@overlay{coordinate}}%
  \def\matrix{\tikz@path@overlay{node[matrix]}}%
  \def\calendar{\tikz@lib@cal@calendar}%
  \def\datavisualization{\tikz@lib@datavisualization}%
}%
\ifx\tikz@lib@cal@calendar\@undefined
\def\tikz@lib@cal@calendar{\tikzerror{You need to say \string\usetikzlibrary{calendar} to use the \string\calendar{} command}}%
\fi
\ifx\tikz@lib@datavisualization\@undefined
\def\tikz@lib@datavisualization{\tikzerror{You need to say \string\usetikzlibrary{datavisualization} to use the \string\datavisualization{} command}}%
\fi

\def\tikz@path@overlay#1{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar<{\tikz@path@overlayed{#1}}{\path #1}}%
\def\tikz@path@overlayed#1<#2>{\path<#2> #1}%

\def\tikz@uninstallcommands{%
  \let\scope=\tikz@origscope%
  \let\scoped=\tikz@origscoped%
  \let\endscope=\tikz@origendscope%
  \let\startscope=\tikz@origstartscope%
  \let\stopscope=\tikz@origstopscope%
  \let\path=\tikz@origpath%
  \let\againpath=\tikz@origagainpath%
  \let\draw=\tikz@origdraw%
  \let\pattern=\tikz@origpattern%
  \let\fill=\tikz@origfill%
  \let\filldraw=\tikz@origfilldraw%
  \let\shade=\tikz@origshade%
  \let\shadedraw=\tikz@origshadedraw%
  \let\clip=\tikz@origclip%
  \let\useasboundingbox=\tikz@origuseasboundingbox%
  \let\node=\tikz@orignode%
  \let\pic=\tikz@origpic%
  \let\coordinate=\tikz@origcoordinate%
  \let\matrix=\tikz@origmatrix%
  \let\calendar=\tikz@origcalendar%
  \let\datavisualization=\tikz@origdv%
  \let\graph=\tikz@origgraph%
}%


{%
  \catcode`\;=12
  \gdef\tikz@nonactivesemicolon{;}%
  \catcode`\:=12
  \gdef\tikz@nonactivecolon{:}%
  \catcode`\|=12
  \gdef\tikz@nonactivebar{|}%
  \catcode`\!=12
  \gdef\tikz@nonactiveexlmark{!}%
  \catcode`\;=\active
  \catcode`\:=\active
  \catcode`\|=\active
  \catcode`\"=\active
  \catcode`\!=\active
  \gdef\tikz@activesemicolon{;}%
  \gdef\tikz@activecolon{:}%
  \gdef\tikz@activebar{|}%
  \gdef\tikz@activequotes{"}%
  \global\let\tikz@active@quotes@token="%
  \gdef\tikz@activeexlmark{!}%
  \gdef\tikz@deactivatthings{%
    \def;{\tikz@nonactivesemicolon}%
    \def:{\tikz@nonactivecolon}%
    \def|{\tikz@nonactivebar}%
    \def!{\tikz@nonactiveexlmark}%
  }%
}%

\let\tikz@orig@shorthands\pgfutil@empty
\def\tikz@switchoff@shorthands{%
  \ifx\tikz@orig@shorthands\pgfutil@empty%
    \edef\tikz@orig@shorthands{%
      \catcode\noexpand`\noexpand\;\the\catcode`\;\relax%
      \catcode\noexpand`\noexpand\:\the\catcode`\:\relax%
      \catcode\noexpand`\noexpand\|\the\catcode`\|\relax%
      \catcode\noexpand`\noexpand\!\the\catcode`\!\relax%
      \catcode\noexpand`\noexpand\,\the\catcode`\,\relax%
      \catcode\noexpand`\noexpand\<\the\catcode`\<\relax%
      \catcode\noexpand`\noexpand\>\the\catcode`\>\relax%
      \catcode\noexpand`\noexpand\"\the\catcode`\"\relax%
      \catcode\noexpand`\noexpand\'\the\catcode`\'\relax%
      \catcode\noexpand`\noexpand\-\the\catcode`\-\relax%
      \catcode\noexpand`\noexpand\=\the\catcode`\=\relax%
      \catcode\noexpand`\noexpand\.\the\catcode`\.\relax%
      \catcode\noexpand`\noexpand\$\the\catcode`\$\relax%
    }%
    \catcode`\;12\relax%
    \catcode`\:12\relax%
    \catcode`\|12\relax%
    \catcode`\!12\relax%
    \catcode`\,12\relax%
    \catcode`\<12\relax%
    \catcode`\>12\relax%
    \catcode`\"12\relax%
    \catcode`\'12\relax%
    \catcode`\-12\relax%
    \catcode`\=12\relax%
    \catcode`\.12\relax%
    \catcode`\$3\relax%
  \fi%
}%



% Constructs a path and draws/fills them according to the current
% settings.

\def\tikz@command@path{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar[{\tikz@check@earg}%]
  {\pgfutil@ifnextchar<{\tikz@doopt}{\tikz@@command@path}}}%
\pgfutil@protected\def\tikz@signal@path{\tikz@signal@path}%
\def\tikz@check@earg[#1]{%
  \pgfutil@ifnextchar<{\tikz@swap@args[#1]}{\tikz@@command@path[#1]}}
\def\tikz@swap@args[#1]<#2>{\tikz@command@path<#2>[#1]}%

\def\tikz@doopt{%
  \let\tikz@next=\tikz@eargnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@eargactivesemicolon%
  \fi%
  \tikz@next}%
\long\def\tikz@eargnormalsemicolon<#1>#2;{\alt<#1>{\tikz@@command@path#2;}{\tikz@path@do@at@end}}%
{
  \catcode`\;=\active
  \long\global\def\tikz@eargactivesemicolon<#1>#2;{\alt<#1>{\tikz@@command@path#2;}{\tikz@path@do@at@end}}%
}

\def\tikz@@command@path{%
  \edef\tikzscope@linewidth{\the\pgflinewidth}%
  \begingroup%
    \setbox\tikz@figbox=\box\pgfutil@voidb@x%
    \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
    \let\tikz@path@do@at@end=\tikz@lib@scope@check%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@mode=\pgfutil@empty%
    \let\tikz@moveto@waiting=\relax%
    \let\tikz@timer=\relax%
    \let\tikz@tangent=\relax%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \let\tikz@preactions=\pgfutil@empty%
    \let\tikz@postactions=\pgfutil@empty%
    \tikz@snakedfalse%
    \tikz@decoratepathfalse%
    \tikz@node@is@a@labelfalse%
    \tikz@expandcount=100\relax%
    \pgf@path@lastx=0pt%
    \pgf@path@lasty=0pt%
    \tikz@lastx=0pt%
    \tikz@lasty=0pt%
    \tikz@lastxsaved=0pt%
    \tikz@lastysaved=0pt%
    \tikzset{every path/.try}%
    \tikz@scan@next@command%
}%
\def\tikz@scan@next@command{%
  \ifx\tikz@collected@onpath\pgfutil@empty%
  \else%
    \tikz@invoke@collected@onpath%
  \fi%
  \afterassignment\tikz@handle\let\pgf@let@token=%
}%
\newcount\tikz@expandcount
\let\tikz@collected@onpath=\pgfutil@empty%

% Central dispatcher for commands
\def\tikz@handle{%
  \let\pgfutil@next=\tikz@expand%
  \ifx\pgf@let@token(%)
    \let\pgfutil@next=\tikz@movetoabs%
  \else%
    \ifx\pgf@let@token+%
      \let\pgfutil@next=\tikz@movetorel%
    \else%
      \ifx\pgf@let@token-%
        \let\pgfutil@next=\tikz@lineto%
      \else%
        \ifx\pgf@let@token.%
          \let\pgfutil@next=\tikz@dot%
        \else%
          \ifx\pgf@let@token r%
            \let\pgfutil@next=\tikz@rect%
          \else%
            \ifx\pgf@let@token n%
              \let\pgfutil@next=\tikz@fig%
            \else%
              \ifx\pgf@let@token[%]
                \let\pgfutil@next=\tikz@parse@options%
              \else%
                \ifx\pgf@let@token c%
                  \let\pgfutil@next=\tikz@cchar%
                \else%
                  \ifx\pgf@let@token\bgroup%
                    \let\pgfutil@next=\tikz@beginscope%
                  \else%
                    \ifx\pgf@let@token\egroup%
                      \let\pgfutil@next=\tikz@endscope%
                    \else%
                      \ifx\pgf@let@token;%
                        \let\pgfutil@next=\tikz@finish%
                      \else%
                        \let\pgfutil@next=\tikz@handle@more%
                      \fi%
                    \fi%
                  \fi%
                \fi%
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgfutil@next%
}%

% Continued...
\def\tikz@handle@more{%
  \ifx\pgf@let@token a%
    \let\pgfutil@next=\tikz@a@char%
  \else%
    \ifx\pgf@let@token e%
      \let\pgfutil@next=\tikz@e@char%
    \else%
      \ifx\pgf@let@token g%
        \let\pgfutil@next=\tikz@g@char%
      \else%
        \ifx\pgf@let@token s%
           \let\pgfutil@next=\tikz@schar%
        \else%
          \ifx\pgf@let@token |%
             \let\pgfutil@next=\tikz@vh@lineto%
          \else%
            \ifx\pgf@let@token p%
              \let\pgfutil@next=\tikz@pchar%
              \pgfsetmovetofirstplotpoint%
            \else%
              \ifx\pgf@let@token t%
                \let\pgfutil@next=\tikz@to%
              \else%
                \ifx\pgf@let@token\pgfextra%
                  \let\pgfutil@next=\tikz@extra%
                \else%
                  \ifx\pgf@let@token\foreach%
                    \let\pgfutil@next=\tikz@foreach%
                  \else%
                    \ifx\pgf@let@token f%
                      \let\pgfutil@next=\tikz@fchar%
                    \else%
                      \ifx\pgf@let@token\pgf@stop%
                        \let\pgfutil@next=\relax%
                      \else%
                        \ifx\pgf@let@token\par%
                          \let\pgfutil@next=\tikz@scan@next@command%
                        \else%
                          \ifx\pgf@let@token d%
                            \let\pgfutil@next=\tikz@decoration%
                          \else%
                            \ifx\pgf@let@token l%
                              \let\pgfutil@next=\tikz@l@char%
                            \else%
                              \ifx\pgf@let@token:%
                                \let\pgfutil@next=\tikz@colon@char%
                              \else%
                                \let\pgfutil@next=\tikz@expand%
                              \fi%
                            \fi%
                          \fi%
                        \fi%
                      \fi%
                    \fi%
                  \fi%
                \fi%
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \ifx\pgfutil@next\tikz@expand\else\tikz@expandcount=100\relax\fi%
  \pgfutil@next%
}%

\def\tikz@l@char{%
  \pgfutil@ifnextchar e{\tikz@let@command}{%
    \pgfutil@ifnextchar i{\tikz@lsystem}{%
      \pgfutil@ifnextchar-{\tikz@@lsystem}{\tikz@expand}%
    }%
  }%
}%

\def\tikz@lsystem{%
  \tikzerror{You need to say \string\usetikzlibrary{lindenmayersystems} to draw Lindenmayer systems}
}%

\def\tikz@@lsystem{%
  \tikzerror{You need to say \string\usetikzlibrary{lindenmayersystems} to draw L-systems}
}%

\def\tikz@pchar{\pgfutil@ifnextchar l{\tikz@plot}{\pgfutil@ifnextchar i{\tikz@subpicture}{\tikz@parabola}}}%
\def\tikz@cchar{%
  \pgfutil@ifnextchar i{\tikz@circle}%
  {\pgfutil@ifnextchar h{\tikz@children}{\tikz@cochar}}}%
\def\tikz@cochar o{%
  \pgfutil@ifnextchar o{\tikz@coordinate}{\tikz@cosine}}%
\def\tikz@e@char{%
  \pgfutil@ifnextchar l{\tikz@ellipse}{\tikz@@e@char}}%
\def\tikz@a@char{%
  \pgfutil@ifnextchar r{\tikz@arcA}{\tikzerror{Arc expected}}}%
\def\tikz@@e@char dge{%
  \pgfutil@ifnextchar f{\tikz@edgetoparent}{\tikz@edge@plain}}%

\def\tikz@schar{\pgfutil@ifnextchar i{\tikz@sine}{\tikz@svg@path}}%

\def\tikz@g@char r{\pgfutil@ifnextchar i{\tikz@grid}{\tikz@graph}}%

% svg syntax
% svg[options] {...}

\def\tikz@svg@path{%
  \tikzerror{You need to say \string\usetikzlibrary{svg.path} to use the svg path command}
}%


\def\tikz@finish{%
  % Rendering pipeline
  %
  % Step 1: The path background box
  %
  \box\tikz@figbox@bg%
  %
  % Step 2: Decorate path
  %
  \iftikz@decoratepath%
    \tikz@lib@dec@decorate@path%
  \fi%
  %
  % Step 3: Preactions
  %
  \pgfsyssoftpath@getcurrentpath\tikz@actions@path%
  \edef\tikz@restorepathsize{%
    \global\pgf@pathmaxx=\the\pgf@pathmaxx%
    \global\pgf@pathmaxy=\the\pgf@pathmaxy%
    \global\pgf@pathminx=\the\pgf@pathminx%
    \global\pgf@pathminy=\the\pgf@pathminy%
  }%
  \tikz@preactions%
  %
  % Step 4: Reset modes
  %
  \let\tikz@path@picture=\pgfutil@empty%
  \tikz@mode@fillfalse%
  \tikz@mode@drawfalse%
  \tikz@mode@doublefalse%
  \tikz@mode@clipfalse%
  \tikz@mode@boundaryfalse%
  \tikz@mode@fade@pathfalse%
  \tikz@mode@fade@scopefalse%
  \edef\tikz@pathextend{%
    {\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
    {\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
  }%
  \tikz@mode% installs the mode settings
  % Path fading counts as an option:
  \iftikz@mode@fade@path%
    \tikz@addoption{%
      \iftikz@fade@adjust%
        \iftikz@mode@draw%
          \pgfsetfadingforcurrentpathstroked{\tikz@path@fading}{\tikz@do@fade@transform}%
        \else%
          \pgfsetfadingforcurrentpath{\tikz@path@fading}{\tikz@do@fade@transform}%
        \fi%
      \else%
        \pgfsetfading{\tikz@path@fading}{\tikz@do@fade@transform}%
      \fi%
      \tikz@mode@fade@pathfalse% no more fading...
    }%
  \fi%
  %
  % Step 5: Install scope fading
  %
  \iftikz@mode@fade@scope%
    \iftikz@fade@adjust%
      \iftikz@mode@draw%
        \pgfsetfadingforcurrentpathstroked{\tikz@scope@fading}{\tikz@do@fade@transform}%
      \else%
        \pgfsetfadingforcurrentpath{\tikz@scope@fading}{\tikz@do@fade@transform}%
      \fi%
    \else%
      \pgfsetfading{\tikz@scope@fading}{\tikz@do@fade@transform}%
    \fi%
    \tikz@mode@fade@scopefalse%
  \fi%
  %
  % Step 5': Setup options
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
    \pgfsys@beginscope%
      \let\pgfscope@stroke@color=\pgf@strokecolor@global%
      \let\pgfscope@fill@color=\pgf@fillcolor@global%
      \begingroup%
        \tikz@options%
  \fi%
  \tikz@do@rdf@pre@options%
  %
  % Step 5'': Setup animations
  %
  \tikz@is@nodefalse%
  \tikz@call@id@hook%
  \iftikz@mode@clip\else%
    \pgfidscope%
      \tikz@do@rdf@post@options%
      \begingroup%
  \fi% open an animation scope here, unless clipping is done
  %
  % Step 6: Do a fill if shade or a path picture follows.
  %
  \iftikz@mode@fill%
    \iftikz@mode@shade%
      \pgfsyssoftpath@getcurrentpath\tikz@temppath
      \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
      \pgfsyssoftpath@setcurrentpath\tikz@temppath%
      \pgfsyssoftpath@invokecurrentpath%
      \pgfpushtype%
      \pgfusetype{.path fill}%
      \pgfsys@fill%
      \pgfpoptype%
      \tikz@mode@fillfalse% no more filling...
    \else%
      \ifx\tikz@path@picture\pgfutil@empty%
      \else%
        \pgfsyssoftpath@getcurrentpath\tikz@temppath
        \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
        \pgfsyssoftpath@setcurrentpath\tikz@temppath%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfpushtype%
        \pgfusetype{.path fill}%
        \pgfsys@fill%
        \pgfpoptype%
        \tikz@mode@fillfalse% no more filling...
      \fi%
    \fi%
  \fi%
  %
  % Step 7: Do a shade if necessary.
  %
  \iftikz@mode@shade%
    \pgfsyssoftpath@getcurrentpath\tikz@temppath
    \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
    \pgfsyssoftpath@setcurrentpath\tikz@temppath%
    \pgfpushtype%
    \pgfusetype{.path shade}%
    \pgfshadepath{\tikz@shading}{\tikz@shade@angle}%
    \pgfpoptype%
    \tikz@mode@shadefalse% no more shading...
  \fi%
  %
  % Step 8: Do a path picture if necessary.
  %
  \ifx\tikz@path@picture\pgfutil@empty%
  \else%
    \begingroup%
      \pgfusetype{.path picture}%
      \pgfidscope%
      \pgfsys@beginscope%
        \let\tikz@id@name\pgfutil@empty%
        \pgfclearid%
        \pgfsyssoftpath@getcurrentpath\tikz@temppath
        \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
        \pgfsyssoftpath@setcurrentpath\tikz@temppath%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsys@clipnext%
        \pgfsys@discardpath%
        \pgf@relevantforpicturesizefalse%
        \expandafter\def\csname pgf@sh@ns@path picture bounding box\endcsname{rectangle}
        \expandafter\edef\csname pgf@sh@np@path picture bounding box\endcsname{%
          \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
          \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
        }
        \expandafter\def\csname pgf@sh@nt@path picture bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
        \expandafter\def\csname pgf@sh@pi@path picture bounding box\endcsname{\pgfpictureid}
        \pgfinterruptpath%
          \tikz@path@picture%
        \endpgfinterruptpath%
      \pgfsys@endscope%
      \endpgfidscope%
    \endgroup%
    \let\tikz@path@picture=\pgfutil@empty%
  \fi%
  %
  % Step 9: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
      % Change line width
      \begingroup%
        \pgfsys@beginscope%
          \tikz@double@setup%
    \fi%
  \fi%
  %
  % Step 10: Do stroke/fill/clip as needed
  %
  \pgfpushtype%
  \edef\tikz@temp{\noexpand\pgfusepath{%
    \iftikz@mode@fill fill,\fi%
    \iftikz@mode@draw draw,\fi%
    \iftikz@mode@clip clip\fi%
    }}%
  \pgfusetype{.path}%
  \tikz@temp%
  \pgfpoptype%
  \tikz@mode@fillfalse% no more filling
  %
  % Step 11: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
        \pgfsys@endscope%
      \endgroup%
    \fi%
  \fi%
  \tikz@mode@drawfalse% no more stroking
  %
  % Step 12: Postactions
  %
  \tikz@postactions%
  %
  % Step 13: Add labels and nodes
  %
  \box\tikz@figbox%
  %
  % Step 14: Close animations
  %
  \iftikz@mode@clip\else\endgroup\endpgfidscope\fi%
  %
  % Step 14: Close option brace
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
      \endgroup%
      \global\let\pgf@strokecolor@global=\pgfscope@stroke@color%
      \global\let\pgf@fillcolor@global=\pgfscope@fill@color%
    \pgfsys@endscope%
    \iftikz@mode@clip%
      \tikzerror{Extra options not allowed for clipping path command.}%
    \fi%
  \fi%
  \iftikz@mode@clip%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \iftikz@mode@boundary%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \endgroup%
  \global\pgflinewidth=\tikzscope@linewidth%
  \tikz@path@do@at@end%
}%
\let\tikz@lib@scope@check\pgfutil@empty% this is a hook for the scopes library
\def\tikz@path@do@at@end{\tikz@lib@scope@check}%
\def\tikz@@pathtext{@path}%

\def\pgf@outer@auto@adjust@hook{%
  {%
    \tikz@mode@drawfalse%
    \tikz@mode%
    \expandafter%
  }%
  \iftikz@mode@draw\else%
    \pgfkeyslet{/pgf/outer xsep}\pgf@zero@text
    \pgfkeyslet{/pgf/outer ysep}\pgf@zero@text
  \fi%
}%

% Extra actions

\def\tikz@extra@preaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \path[#1];% do extra path
      \pgfsyssoftpath@setcurrentpath\tikz@actions@path% restore
      \tikz@restorepathsize%
    \pgfsys@endscope%
  }%
}%

\def\tikz@extra@postaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \tikz@restorepathsize%
      \path[#1]\pgfextra{\pgfsyssoftpath@setcurrentpath\tikz@actions@path};% do extra path
      \pgf@resetpathsizes%
    \pgfsys@endscope%
  }%
}%



\def\tikz@skip#1{\tikz@scan@next@command#1}%
\def\tikz@expand{%
  \advance\tikz@expandcount by -1
  \ifnum\tikz@expandcount<0\relax%
    \tikzerror{Giving up on this path. Did you forget a semicolon?}%
    \let\pgfutil@next=\tikz@finish%
  \else%
    \let\pgfutil@next=\tikz@@expand
  \fi%
  \pgfutil@next}%

\def\tikz@@expand{%
  \expandafter\tikz@scan@next@command\pgf@let@token}%



% Syntax for scopes:
% {scoped path commands}

\newif\iftikz@auto@end@path

\def\tikz@beginscope{\begingroup\tikz@auto@end@pathfalse\tikz@scan@next@command}%
\def\tikz@endscope{%
  \iftikz@auto@end@path\expandafter\tikz@finish\expandafter\egroup\else\expandafter\tikz@@endscope\fi%
}%
\def\tikz@@endscope{%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
    \global\let\tikz@tangent@temp\tikz@tangent%
    \edef\tikz@marshal{%
      \tikz@lastx=\the\tikz@lastx%
      \tikz@lasty=\the\tikz@lasty%
      \iftikz@current@point@local%
      \else%
        \tikz@lastxsaved=\the\tikz@lastxsaved%
        \tikz@lastysaved=\the\tikz@lastysaved%
        \ifx\tikz@moveto@waiting\relax%
          \let\tikz@moveto@waiting\relax%
        \else%
          \def\noexpand\tikz@moveto@waiting{\tikz@moveto@waiting}%
        \fi%
        \iftikz@shapeborder%
          \noexpand\tikz@shapebordertrue%
          \def\noexpand\tikz@shapeborder@name{\tikz@shapeborder@name}%
        \else%
          \noexpand\tikz@shapeborderfalse%
        \fi%
      \fi%
    }%
    \expandafter%
  \endgroup\tikz@marshal%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \let\tikz@tangent\tikz@tangent@temp%
  \tikz@scan@next@command}%


% Syntax for pgfextra:
% \pgfextra {normal tex text}
% \pgfextra normal tex text \endpgfextra

\def\tikz@extra{\pgfutil@ifnextchar\bgroup\tikz@@extra\relax}%
\long\def\tikz@@extra#1{#1\tikz@scan@next@command}%
\let\endpgfextra=\tikz@scan@next@command

\def\pgfextra{pgfextra}%


% Syntax for foreach:
%
% foreach \var in {list} {path text}
%
% or
%
% \foreach \var in {list} {path text}
%
% Example:
%
% \draw (0,0) \foreach \x in {1,2,3} {-- (\x,0) circle (1cm)} -- (5,5);

\def\tikz@fchar oreach{\tikz@foreach}%

\def\tikz@foreach{%
  \def\pgffor@beginhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \expandafter\tikz@scan@next@command\pgfutil@firstofone}%
  \def\pgffor@endhook{\pgfextra{%
      \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
      \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
      \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
      \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
      \global\setbox\tikz@tempbox=\box\tikz@figbox%
      \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
      \pgfutil@gobble}}%
  \def\pgffor@afterhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \let\pgffor@beginhook\relax%
    \let\pgffor@endhook\relax%
    \let\pgffor@afterhook\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \tikz@scan@next@command}%
  \global\setbox\tikz@tempbox=\box\tikz@figbox%
  \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
  \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
  \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
  \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
  \foreach}%


% Syntax for againpath:
% \againpath \somepathname

\def\tikz@command@againpath#1{%
  \pgfextra{%
    \pgfsyssoftpath@getcurrentpath\tikz@temp%
    \expandafter\pgfutil@g@addto@macro\expandafter\tikz@temp\expandafter{#1}%
    \pgfsyssoftpath@setcurrentpath\tikz@temp%
  }%
}%


% animation syntax
% :attribute = {...}

\def\tikz@colon@char#1=#2{%
  \tikz@scan@next@command{[animate={myself:{#1}={#2}}]}%
}%



%
% When this if is set, a just-scanned point is a shape and its border
% position still needs to be determined, depending on subsequent
% commands.
%

\newif\iftikz@shapeborder


% Syntax for moveto:
% <point>
\def\tikz@movetoabs{\tikz@moveto(}%
\def\tikz@movetorel{\tikz@moveto+}%
\def\tikz@moveto{%
  \tikz@scan@one@point{\tikz@@moveto}}%
\def\tikz@@moveto#1{%
    \tikz@make@last@position{#1}%
  \iftikz@shapeborder%
    % ok, the moveto will have to wait. flag that we have a moveto in
    % waiting:
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@@movetosave{\tikz@last@position}%
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \tikz@scan@next@command%
}%

  % Wrapper around \pgfpathmoveto that adds a save
\def\tikz@@movetosave#1{%
  {\pgftransformreset
    \pgf@process{#1}%
    \xdef\tikz@marshal{%
      \tikz@lastmovetox=\the\pgf@x\relax%
      \tikz@lastmovetoy=\the\pgf@y\relax%
    }%
  }%
  \tikz@marshal
  \pgfpathmoveto{#1}%
}%

  
\let\tikz@moveto@waiting=\relax % normally, nothing is waiting...

\def\tikz@flush@moveto{%
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \tikz@@movetosave{\tikz@last@position}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}%


\def\tikz@flush@moveto@toward#1#2#3{%
  % #1 = a point towards which the last moveto should be corrected
  % #2 = a dimension to which the corrected x-coordinate should be stored
  % #3 = a dimension for the corrected y-coordinate
  \ifx\tikz@moveto@waiting\relax%
    % do nothing
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{#1}}%
    #2=\pgf@x%
    #3=\pgf@y%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \tikz@@movetosave{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}%


%
% Collecting labels on the path
%

\def\tikz@collect@coordinate@onpath#1c{%
  \pgfutil@ifnextchar y{\tikz@cycle@expander@add#1}{\tikz@collect@coordinate@onpath@{#1}}}%
\def\tikz@collect@coordinate@onpath@#1oordinate{%
  \pgfutil@ifnextchar[{\tikz@@collect@coordinate@opt#1}{\tikz@@collect@coordinate@opt#1[]}}%}%
\def\tikz@@collect@coordinate@opt#1[#2]{%
  \pgfutil@ifnextchar({\tikz@@collect@coordinate#1[#2]}{%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2]{}}}%}%
\def\tikz@@collect@coordinate#1[#2](#3){%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2](#3){}}%

\newif\iftikz@collect@pic

\def\tikz@collect@label@onpath#1node{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath node}%
  \let\tikz@collect@cont#1%
  \tikz@collect@picfalse%
  \tikz@collect@label@scan}%

\def\tikz@collect@pic@onpath#1pic{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath pic}%
  \let\tikz@collect@cont#1
  \tikz@collect@pictrue%
  \tikz@collect@label@scan}%

\def\tikz@collect@label@scan{%
  \pgfutil@ifnextchar f{\tikz@collect@nodes}{%
    \pgfutil@ifnextchar({\tikz@collect@paran}%
    {\pgfutil@ifnextchar[{\tikz@collect@options}%
      {\pgfutil@ifnextchar:{\tikz@collect@animation}%
        {\pgfutil@ifnextchar\bgroup{\tikz@collect@arg}%
          {\tikz@collect@cont}}}}}%
}%}}%

\def\tikz@collect@nodes foreach#1in{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath foreach#1in}%
  \pgfutil@ifnextchar\bgroup\tikz@collect@nodes@group\tikz@collect@nodes@one%
}%
\def\tikz@collect@nodes@one#1{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath #1}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@nodes@group#1{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
  \tikz@collect@label@scan%
}%

\def\tikz@collect@animation#1=#2{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1={#2}}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@paran#1){%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1)}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@options#1]{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1]}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@arg#1{%
  \iftikz@handle@active@nodes%
    \iftikz@collect@pic%
      \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
    \else%
      \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{\scantokens{#1}}}%
    \fi%
  \else%
    \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
  \fi%
  \tikz@collect@cont%
}%

\def\tikz@invoke@collected@onpath{%
  \tikz@node@is@a@labeltrue%
  \let\tikz@temp=\tikz@collected@onpath%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \expandafter\tikz@scan@next@command\tikz@temp\pgf@stop%
  \tikz@node@is@a@labelfalse%
}%


%
% Macros for the cycle command
%

\def\tikz@cycle@expander#1{\pgfutil@ifnextchar c{\tikz@cycle@expander@{#1}}{#1}}%
\def\tikz@cycle@expander@#1c{\pgfutil@ifnextchar y{\tikz@cycle@expander@add{#1}}{#1c}}%
\def\tikz@cycle@expander@add#1ycle{#1(current subpath start)--cycle}%




% Syntax for lineto:
% -- <point>

\def\tikz@lineto{%
  \pgfutil@ifnextchar |%
  {\expandafter\tikz@hv@lineto\pgfutil@gobble}%
  {\expandafter\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikz@hv@lineto\pgfutil@gobble}%
    {\expandafter\tikz@lineto@mid\pgfutil@gobble}}}%
\def\tikz@lineto@mid{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@lineto@mid}%
  {%
    \pgfutil@ifnextchar c{\tikz@close}{%
      \pgfutil@ifnextchar p{\tikz@lineto@plot@or@pic}{\tikz@scan@one@point{\tikz@@lineto}}}}}%
\def\tikz@lineto@plot@or@pic p{%
  \pgfutil@ifnextchar i{\tikz@collect@pic@onpath\tikz@lineto@mid p}{%
    \pgfsetlinetofirstplotpoint\tikz@plot}%
}%
\def\tikz@@lineto#1{%
  % Record the starting point for later labels on the path:
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate end
    \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@last@position}}%
    \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \tikz@make@last@position{#1}%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    % target is a reasonable point...
    % Record the starting point for later labels on the path:
    \tikz@make@last@position{#1}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@line%
  \let\tikz@tangent\tikz@timer@start%
  \tikz@scan@next@command%
}%

% snake or lineto?
\def\tikz@path@lineto#1{%
  \iftikz@snaked%
    {
      \pgfsyssoftpathmovetorelevantfalse%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }
  \else%
    \pgfpathlineto{#1}%
  \fi%
}%

% snake or lineto?
\def\tikz@path@close#1{%
  \iftikz@snaked%
    {%
      \pgftransformreset%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }%
  \fi%
  \pgfpathclose%
}%


% Syntax for lineto horizontal/vertical:
% -| <point>

\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@hv@lineto}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@hv@lineto}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@hv@lineto}%
    {\tikz@scan@one@point{\tikz@@hv@lineto}}}}}%
\def\tikz@@hv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@yc=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \edef\tikz@tangent{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@x\pgf@yc%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yc}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
  \fi%
  \let\tikz@timer=\tikz@timer@hvline%
  \tikz@scan@next@command%
}%

% Syntax for lineto vertical/horizontal:
% |- <point>

\def\tikz@vh@lineto-{\tikz@vh@lineto@next}%
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@vh@lineto@next}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@vh@lineto@next}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@vh@lineto@next}%
    {\tikz@scan@one@point\tikz@@vh@lineto}}}}%
\def\tikz@@vh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx%
  \tikz@make@last@position{#1}%
  \edef\tikz@tangent{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@y%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xc}{\tikz@lasty}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@vhline%
  \tikz@scan@next@command%
}%

% Syntax for cycle:
% -- cycle
\def\tikz@close c{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@lineto@mid c}% oops, a coordinate
  {\tikz@@close c}}%
\def\tikz@@close cycle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \tikz@make@last@position{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \tikz@path@close{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \def\pgfstrokehook{}%
  \edef\tikz@timer@end{%\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \noexpand\pgfqpoint{\the\tikz@lastmovetox}{\the\tikz@lastmovetoy}}%
  \let\tikz@timer=\tikz@timer@line%
  \let\tikz@tangent\tikz@timer@start%
  \tikz@scan@next@command%
}%


% Syntax for options:
% [options]
\def\tikz@parse@options#1]{%
  \tikzset{#1}%
  \tikz@scan@next@command%
}%

% Syntax for edges:
% edge [options] (coordinate)
% edge [options] node {node text} (coordinate)
% edge :attribute={...} [options] node {node text} (coordinate)
\def\tikz@edge@plain{%
  \begingroup%
    \ifx\tikz@to@use@whom\pgfutil@undefined\else\tikz@to@use@whom\fi
    \let\tikz@to@or@edge@function=\tikz@do@edge%
    \let\tikz@@to@local@options\pgfutil@empty%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \tikz@to@or@edge}%

% Syntax for to paths:
% to [options] (coordinate)
% to [options] node {node text} (coordinate)
% to :attribute={...} [options] node {node text} (coordinate)
\def\tikz@to o{%
  \tikz@to@use@last@coordinate%
  \let\tikz@to@or@edge@function=\tikz@do@to%
  \let\tikz@@to@local@options\pgfutil@empty%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@to@or@edge}%

\def\tikz@to@or@edge{%
  \pgfutil@ifnextchar[{\tikz@to@or@edge@option}{%
    \pgfutil@ifnextchar:{\tikz@to@or@edge@animation}{%
      \tikz@@to@collect}}%]
}%
\def\tikz@to@or@edge@option[#1]{%
  \expandafter\def\expandafter\tikz@@to@local@options\expandafter{\tikz@@to@local@options,#1}%
  \tikz@to@or@edge%
}%
\def\tikz@to@or@edge@animation:#1=#2{%
  \expandafter\def\expandafter\tikz@@to@local@options\expandafter{\tikz@@to@local@options,%
    animate={myself:{#1}={#2}}}%
  \tikz@to@or@edge%
}%
\def\tikz@@to@collect{%
  \pgfutil@ifnextchar(\tikz@@to@or@edge@coordinate%)
  {\pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@to@collect}%
    {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@to@collect}%
      {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@to@collect}%
        {\pgfutil@ifnextchar +{\tikz@scan@one@point\tikz@@to@or@edge@math}%
          {\tikzerror{(, +, coordinate, pic, or node expected}%)
            \tikz@@to@or@edge@coordinate()}}}}}%
}%

\def\tikz@@to@or@edge@coordinate({%
  \pgfutil@ifnextchar${%$
    % Ok, parse directly
    \tikz@scan@one@point\tikz@@to@or@edge@math(%
  }{%
    \pgfutil@ifnextchar[{%]
      \tikz@scan@one@point\tikz@@to@or@edge@math(%
    }{%
      \tikz@@to@or@edge@@coordinate(%
    }%
  }%
}%
\def\tikz@@to@or@edge@math#1{%
  \pgf@process{#1}%
  \iftikz@updatecurrent\else
    \tikz@updatenextfalse
  \fi
  \edef\tikztotarget{\the\pgf@x,\the\pgf@y}%
  \tikz@to@or@edge@function%
}%

\def\tikz@@to@or@edge@@coordinate(#1){%
  \def\tikztotarget{#1}%
  \tikz@to@or@edge@function%
}%

\def\tikz@do@edge{%
  \ifx\tikz@edge@macro\pgfutil@empty%
    \setbox\tikz@whichbox=\hbox\bgroup%
      \unhbox\tikz@whichbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@transform=\pgfutil@empty%
              \let\tikz@options=\pgfutil@empty%
              \tikz@clear@rdf@options%
              \let\tikz@tonodes=\tikz@collected@onpath%
              \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
              \let\tikz@collected@onpath=\pgfutil@empty%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \pgfidscope%
              \tikz@do@rdf@post@options%
              \tikz@transform%
              \let\tikz@transform=\relax%
              % Typeset node:
              \let\tikz@after@path\pgfutil@empty%
              \tikz@atbegin@to%
                \tikz@enable@edge@quotes%
                \path[style=every edge]\expandafter[\tikz@@to@local@options](\tikztostart)\tikz@to@path
                \pgfextra{\global\let\tikz@after@path@smuggle=\tikz@after@path};%
              \tikz@atend@to%
              \endpgfidscope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
    \global\setbox\tikz@tempbox=\box\tikz@whichbox%
    \expandafter\endgroup%
    \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox%
  \else%
      \expandafter\expandafter\expandafter\tikz@edge@macro%
      \expandafter\expandafter\expandafter{\expandafter\tikz@@to@local@options\expandafter}\expandafter{\tikz@collected@onpath}%
    \endgroup%
    \let\tikz@after@path@smuggle=\pgfutil@empty%
  \fi%
  \expandafter\tikz@scan@next@command\tikz@after@path@smuggle%
}%

\def\tikz@do@to{%
  \let\tikz@tonodes=\tikz@collected@onpath%
  \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@scan@next@command%
  {%
    \pgfextra{\let\tikz@after@path\pgfutil@empty}%
    \pgfextra{\tikz@atbegin@to}%
    \pgfextra{\tikz@enable@edge@quotes}%
    [style=every to]\expandafter[\tikz@@to@local@options]\tikz@to@path%
    \pgfextra{\tikz@atend@to}%
    \pgf@stop%
    \expandafter\tikz@scan@next@command\expandafter%
  }\tikz@after@path%
  \pgfextra{\tikz@updatenexttrue\tikz@updatecurrenttrue}%
}%


\def\tikz@to@use@last@coordinate{%
  \iftikz@shapeborder%
    \edef\tikztostart{\tikz@shapeborder@name}%
  \else%
    \edef\tikztostart{\the\tikz@lastx,\the\tikz@lasty}%
  \fi%
}%
\def\tikz@to@use@last@fig@name{%
  \edef\tikztostart{\tikz@to@last@fig@name}%
}%



% Syntax for graph path command:
% graph [options] {...}
% See the graph library for details

\def\tikz@graph aph{\tikz@lib@graph@parser}%

\def\tikz@lib@graph@parser{\pgfutil@ifnextchar[\tikz@graph@error{\tikz@graph@error[]}}%]%
\def\tikz@graph@error[#1]#2{%
  \tikzerror{You need to say \string\usetikzlibrary{graphs} in order to use the graph syntax}%
  \tikz@lib@graph@parser@done%
}%

\def\tikz@lib@graph@parser@done{%
  \tikz@scan@next@command%
}%




% Syntax for edge from parent:
% edge from parent [options]
\def\tikz@edgetoparent from parent{\pgfutil@ifnextchar[\tikz@@edgetoparent{\tikz@@edgetoparent[]}}%}%
\def\tikz@@edgetoparent[#1]{%
  \let\tikz@edge@to@parent@needed=\pgfutil@empty%
  \def\tikz@edgetoparent@options{#1}%
  \begingroup%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \tikz@edgetoparentcollect%
}%
\def\tikz@edgetoparentcollect{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@edgetoparentcollect}%
  {%
      \expandafter%
    \endgroup%
    \expandafter\tikz@edgetoparent@rollout\expandafter{\tikz@collected@onpath}%
  }%
}%

\def\tikz@edgetoparent@rollout#1{%
  \pgfkeysgetvalue{/tikz/edge from parent macro}\tikz@etop@temp
  \expandafter\tikz@scan@next@command\expandafter\tikz@etop@temp\expandafter{\tikz@edgetoparent@options}{#1}%
}%


% Syntax for bezier curves
% .. controls(point) and (point) .. (target)
% .. controls(point) .. (target)
% .. (target) % currently not supported

\def\tikz@dot.{\tikz@@dot}%
\def\tikz@@dot{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@dot}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@dot}%
  {\pgfutil@ifnextchar c{\tikz@curveto@double}{\tikz@curveto@auto}}}%
}%

\def\tikz@curveto@double co{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@@dot co}
  {\tikz@cureveto@@double}}%
\def\tikz@cureveto@@double ntrols#1{%
  \tikz@scan@one@point\tikz@curveA#1%
}%
\def\tikz@curveA#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{#1}%
    \xdef\tikz@curve@first{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  \pgfutil@ifnextchar a
  {\tikz@curveBand}%
  {\let\tikz@curve@second\tikz@curve@first\tikz@curveCdots}%
}%
\def\tikz@curveBand and{%
  \tikz@scan@one@point\tikz@curveB%
}%
\def\tikz@curveB#1{%
  \def\tikz@curve@second{#1}%
  \tikz@curveCdots}
\def\tikz@curveCdots{%
  \afterassignment\tikz@curveCdot\let\pgfutil@next=}%
\def\tikz@curveCdot.{%
  \ifx\pgfutil@next.%
  \else%
    \tikzerror{Dot expected}%
  \fi%
  \iftikz@updatenext
    \tikz@updatecurrenttrue%
  \fi
  \tikz@curveCcheck%
}%
\def\tikz@curveCcheck{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@curveCcheck}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@curveCcheck}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@curveCcheck}
    {\tikz@scan@one@point\tikz@curveC}}}%
}%
\def\tikz@curveC#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{\tikz@curve@second}%
    \xdef\tikz@curve@second{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  %
  % Start recalculating things in case start and end are shapes.
  %
  % First, the start:
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{\tikz@curve@first}}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \tikz@@movetosave{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@timer@cont@one=\tikz@curve@first%
  \let\tikz@timer@cont@two=\tikz@curve@second%
  % Second, the end:
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate third
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@curve@second}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
      \global\let\tikz@timer@end@temp=\tikz@curve@third% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
    \let\tikz@timer@end=\tikz@curve@third
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \let\tikz@timer=\tikz@timer@curve%
  \let\tikz@tangent=\tikz@curve@second%
  \tikz@scan@next@command%
}%


% Syntax for rectangles:
% rectangle <corner point>
\def\tikz@rect ectangle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \tikz@@rect}%
\def\tikz@@rect{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@rect}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@rect}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@rect}%
    {
      \pgf@xa=\tikz@lastx\relax%
      \pgf@ya=\tikz@lasty\relax%
      \tikz@scan@one@point\tikz@rectB}}}}%
\def\tikz@rectB#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \let\tikz@timer=\tikz@timer@line%
          \tikz@@movetosave{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@ya}}%
  \iftikz@snaked%
    \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \fi%
  \pgfpathclose%
          \tikz@@movetosave{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \def\pgfstrokehook{}%
  \let\tikz@tangent\relax%
  \tikz@scan@next@command%
}%



% Syntax for grids:
% grid <corner point>
\def\tikz@grid id{%
  \tikz@flush@moveto%
  \pgf@xa=\tikz@lastx\relax%
  \pgf@ya=\tikz@lasty\relax%
  \pgfutil@ifnextchar[{\tikz@gridA}{\tikz@gridA[]}}%}%
\def\tikz@gridA[#1]{%
  \def\tikz@grid@options{#1}%
  \tikz@cycle@expander{\tikz@scan@one@point\tikz@gridB}}%
\def\tikz@gridB#1{%
  \tikz@make@last@position{#1}%
  \let\tikz@tangent\relax%
  {%
    \let\tikz@after@path\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@grid@options}
    \tikz@checkunit{\tikz@grid@x}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{\tikz@grid@x}{0pt}}%
    \else%
      \pgf@process{\pgfpointxy{\tikz@grid@x}{0}}%
    \fi%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \tikz@checkunit{\tikz@grid@y}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{0pt}{\tikz@grid@y}}%
    \else%
      \pgf@process{\pgfpointxy{0}{\tikz@grid@y}}%
    \fi%
    \advance\pgf@xb by\pgf@x%
    \advance\pgf@yb by\pgf@y%
    \pgfpathgrid[stepx=\pgf@xb,stepy=\pgf@yb]%
      {\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \expandafter}%
  \expandafter\tikz@scan@next@command\tikz@after@path%
}%



% Syntax for plot:
% plot [local options] ...    % starts with a moveto
% -- plot [local options] ... % starts with a lineto
\def\tikz@plot lot{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar[{\tikz@@plot}{\tikz@@plot[]}}%}%
\def\tikz@@plot[#1]{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \begingroup%
    \let\tikz@after@path\pgfutil@empty%
    \let\tikz@options=\pgfutil@empty%
    \tikzset{every plot/.try}%
    \tikzset{#1}%
    \pgfutil@ifnextchar f{\tikz@plot@f}%
    {\pgfutil@ifnextchar c{\tikz@plot@scan@points}%
      {\pgfutil@ifnextchar ({\tikz@plot@expression}{%
      \tikzerror{Cannot parse this plotting data}%
       \endgroup}}}}%
\def\tikz@plot@f f{\pgfutil@ifnextchar i{\tikz@plot@file}{\tikz@plot@function}}%

\def\tikz@plot@file ile#1{\def\tikz@plot@data{\pgfplotxyfile{#1}}\tikz@@@plot}%
\def\tikz@plot@scan@points coordinates#1{%
  \pgfplothandlerrecord\tikz@plot@data%
  \pgfplotstreamstart%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}
  {\tikz@scan@one@point\tikz@plot@next@point}%
  #1\pgf@stop%
}%
\def\tikz@plot@next@point#1{%
  \pgfplotstreampoint{#1}%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}%
  {\tikz@scan@one@point\tikz@plot@next@point}%
}%
\def\tikz@plot@function unction#1{%
  \def\tikz@plot@filename{\tikz@plot@prefix\tikz@plot@id}%
  \iftikz@plot@raw@gnuplot%
    \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{#1}}%
  \else%
    \iftikz@plot@parametric%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          set parametric;
          plot [t=\tikz@plot@domain]
          [\tikz@plot@xrange]
          [\tikz@plot@range]
          #1}}%
    \else%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          plot [x=\tikz@plot@domain]
          \ifx\tikz@plot@range\pgfutil@empty\else[\tikz@plot@range]\fi
          #1}}%
    \fi%
  \fi%
  \tikz@@@plot%
}%

\def\tikz@plot@no@resample{%
  \pgfutil@IfFileExists{\tikz@plot@filename.table}%
  {\def\tikz@plot@data{\pgfplotxyfile{\tikz@plot@filename.table}}}%
  {}%
}%

\def\tikz@plot@expression(#1){%
  \edef\tikz@plot@data{\noexpand\pgfplotfunction{\expandafter\noexpand\tikz@plot@var}{\tikz@plot@samplesat}}%
  \expandafter\def\expandafter\tikz@plot@data\expandafter{\tikz@plot@data{\tikz@scan@one@point\pgfutil@firstofone(#1)}}%
  \tikz@@@plot%
}%

\def\tikz@@@plot{%
    \def\pgfplotlastpoint{\pgfpointorigin}%
    \tikz@plot@handler%
    \tikz@plot@data%
    \global\let\tikz@@@temp=\pgfplotlastpoint%
    \ifx\tikz@plot@mark\pgfutil@empty%
    \else%
      % Marks are drawn after the path.
      \setbox\tikz@whichbox=\hbox{%
        \unhbox\tikz@whichbox%
        \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@options=\pgfutil@empty%
              \let\tikz@transform=\pgfutil@empty%
              \tikzset{every mark}%
              \tikz@options%
              \ifx\tikz@mark@list\pgfutil@empty%
                \pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
              \else
                \pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
              \fi
              \tikz@plot@data%
            \endpgfscope
          \endpgfinterruptpath%
        }}%
      }%
    \fi%
    \global\setbox\tikz@tempbox=\box\tikz@whichbox%
    \global\let\tikz@after@path@smuggle=\tikz@after@path
  \expandafter\endgroup%
  \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox%
  \tikz@make@last@position{\tikz@@@temp}%
  \expandafter\tikz@scan@next@command\tikz@after@path@smuggle%
}%


\pgfdeclareplotmark{ball}
{%
  \def\tikz@shading{ball}%
  \shade (0pt,0pt) circle (\pgfplotmarksize);%
}%




% Syntax for cosine curves:
% cos <end of quarter-period>
\def\tikz@cosine s{\tikz@cycle@expander{\tikz@scan@one@point\tikz@@cosine}}
\def\tikz@@cosine#1{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathcosine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}%

% Syntax for sine curves:
% sin <end of quarter-period>
\def\tikz@sine in{\tikz@cycle@expander{\tikz@scan@one@point\tikz@@sine}}
\def\tikz@@sine#1{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathsine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}%

% Syntax for parabolas:
% parabola[options] bend <coordinate> <coordinate>
\def\tikz@parabola arabola{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \pgfutil@ifnextchar[{\tikz@parabola@options}{\tikz@parabola@options[]}}%}%

\def\tikz@parabola@options[#1]{%
  \def\tikz@parabola@option{#1}%
  \pgfutil@ifnextchar b{\tikz@parabola@scan@bend}{\tikz@cycle@expander{\tikz@scan@one@point\tikz@parabola@semifinal}}}%
\def\tikz@parabola@scan@bend bend{\tikz@scan@one@point\tikz@parabola@scan@bendB}%
\def\tikz@parabola@scan@bendB#1{%
  \def\tikz@parabola@bend{#1}%
  \tikz@cycle@expander{\tikz@scan@one@point\tikz@parabola@semifinal}%
}%
\def\tikz@parabola@semifinal#1{%
  \tikz@flush@moveto%
  % Save original start:
  \pgf@xb=\tikz@lastx%
  \pgf@yb=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \pgf@xc=\tikz@lastx%
  \pgf@yc=\tikz@lasty%
  \begingroup% now calculate bend:
    \let\tikz@after@path\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@parabola@option}%
    \tikz@lastxsaved=\tikz@parabola@bend@factor\tikz@lastx%
    \tikz@lastysaved=\tikz@parabola@bend@factor\tikz@lasty%
    \advance\tikz@lastxsaved by\pgf@xb%
    \advance\tikz@lastysaved by\pgf@yb%
    \advance\tikz@lastxsaved by-\tikz@parabola@bend@factor\pgf@xb%
    \advance\tikz@lastysaved by-\tikz@parabola@bend@factor\pgf@yb%
    \expandafter\tikz@make@last@position\expandafter{\tikz@parabola@bend}%
    % Calculate delta from bend
    \advance\pgf@xc by-\tikz@lastx%
    \advance\pgf@yc by-\tikz@lasty%
    % Ok, now calculate delta to bend
    \advance\tikz@lastx by-\pgf@xb%
    \advance\tikz@lasty by-\pgf@yb%
    \xdef\tikz@parabola@b{{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \expandafter\endgroup%
  \expandafter\expandafter\expandafter\pgfpathparabola\expandafter\tikz@parabola@b%
  \expandafter\tikz@scan@next@command\tikz@after@path%
}%


% Syntax for circles:
% circle [options] % where options should set, at least, radius
% circle (radius) % deprecated
%
% Syntax for ellipses:
% ellipse [options] % identical to circle.
% ellipse (x-radius and y-radius) % deprecated
%
% radii can be dimensionless, then they are in the xy-system
\def\tikz@circle ircle{\tikz@flush@moveto\tikz@@circle}%
\def\tikz@ellipse llipse{\tikz@flush@moveto\tikz@@circle}%
\def\tikz@@circle{%
  \let\tikz@tangent\relax%
  \pgfutil@ifnextchar(\tikz@@@circle
  {\pgfutil@ifnextchar[\tikz@circle@opt{%])
    \advance\tikz@expandcount by -10\relax% go down quickly
    \ifnum\tikz@expandcount<0\relax%
      \let\pgfutil@next=\tikz@@circle@normal%
    \else%
      \let\pgfutil@next=\tikz@@circle@scanexpand%
    \fi%
    \pgfutil@next%
  }}%
}%
\def\tikz@@circle@scanexpand{\expandafter\tikz@@circle}%
\def\tikz@@circle@normal{\tikz@circle@opt[]}%

\def\tikz@circle@opt[#1]{%
  {%
    \def\tikz@node@at{\tikz@last@position}%
    \let\tikz@transform=\pgfutil@empty%
    \tikzset{every circle/.try,#1}%
    \pgftransformshift{\tikz@node@at}%
    \tikz@transform%
    \tikz@do@ellipse{\pgfkeysvalueof{/tikz/x radius}}{\pgfkeysvalueof{/tikz/y radius}}
  }%
  \tikz@scan@next@command%
}%

\def\tikz@@@circle(#1){%
  {%
    \pgftransformshift{\tikz@last@position}%
    \pgfutil@in@{ and }{#1}%
    \ifpgfutil@in@%
      \tikz@@ellipseB(#1)%
    \else%
      \tikz@do@circle{#1}%
    \fi%
  }%
  \tikz@scan@next@command%
}%
\def\tikz@@ellipseB(#1 and #2){%
  \tikz@do@ellipse{#1}{#2}%
}%
\def\tikz@do@circle#1{%
  \pgfmathparse{#1}%
  \let\tikz@ellipse@x=\pgfmathresult
  \ifpgfmathunitsdeclared
    \pgfpathellipse{\pgfpointorigin}%
      {\pgfqpoint{\tikz@ellipse@x pt}{0pt}}%
      {\pgfpoint{0pt}{\tikz@ellipse@x pt}}%
  \else
    \pgfpathellipse{\pgfpointorigin}%
      {\pgfpointxy{\tikz@ellipse@x}{0}}%
      {\pgfpointxy{0}{\tikz@ellipse@x}}%
  \fi
}
\def\tikz@do@ellipse#1#2{
  \pgfmathparse{#1}%
  \let\tikz@ellipse@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \pgfpathellipse{\pgfpointorigin}{%
        \pgfqpoint{\tikz@ellipse@x pt}{0pt}}{\pgfpoint{0pt}{\tikz@ellipse@y pt}}%
    \else%
      \tikzerror{You cannot mix dimensions and dimensionless values in an ellipse}%
    \fi%
  \else%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikzerror{You cannot mix dimensions and dimensionless values in an ellipse}%
    \else%
      \pgfpathellipse{\pgfpointorigin}{%
        \pgfpointxy{\tikz@ellipse@x}{0}}{\pgfpointxy{0}{\tikz@ellipse@y}}%
    \fi%
  \fi%
}%

% Syntax for arcs:
% arc [options]
%
% (The syntax with parentheses is deprecated.)
\def\tikz@arcA rc{\tikz@flush@moveto\tikz@arc@cont}%
\def\tikz@arc@cont{%
  \pgfutil@ifnextchar(%)
  {\tikz@@arcto}{%
    \pgfutil@ifnextchar[%]
    {\tikz@arc@opt}%
    {%
      \advance\tikz@expandcount by -10\relax% go down quickly
      \ifnum\tikz@expandcount<0\relax%
        \let\pgfutil@next=\tikz@@arc@normal%
      \else%
        \let\pgfutil@next=\tikz@@arc@scanexpand%
      \fi%
      \pgfutil@next%
    }%
  }%
}%
\def\tikz@@arc@scanexpand{\expandafter\tikz@arc@cont}%
\def\tikz@@arc@normal{\tikz@arc@opt[]}%


\def\tikz@arc@opt[#1]{%
  {%
    \tikzset{every arc/.try,#1}%
    \pgfkeysgetvalue{/tikz/start angle}\tikz@s
    \pgfkeysgetvalue{/tikz/end angle}\tikz@e
    \pgfkeysgetvalue{/tikz/delta angle}\tikz@d
    \ifx\tikz@s\pgfutil@empty%
      \pgfmathsetmacro\tikz@s{\tikz@e-\tikz@d}
    \else
      \ifx\tikz@e\pgfutil@empty%
        \pgfmathsetmacro\tikz@e{\tikz@s+\tikz@d}
      \fi%
    \fi%
    \xdef\pgf@marshal{\noexpand%
    \tikz@do@arc{\tikz@s}{\tikz@e}
      {\pgfkeysvalueof{/tikz/x radius}}
      {\pgfkeysvalueof{/tikz/y radius}}}%
  }%
  \pgf@marshal%
  \tikz@arcfinal%
}%

\def\tikz@@arcto(#1){%
  \edef\tikz@temp{(#1)}%
  \expandafter\tikz@@@arcto@check@slashand\tikz@temp%
}%

\def\tikz@@@arcto@check@slashand(#1:#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \tikz@parse@arc@and(#1:#2:#3)%
  \else%
    \tikz@parse@arc@and(#1:#2:{#3} and {#3})%
  \fi%
  \tikz@arcfinal%
}%

\def\tikz@parse@arc@and(#1:#2:#3 and #4){%
  \tikz@do@arc{#1}{#2}{#3}{#4}%
}%
\def\tikz@do@arc#1#2#3#4{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgfmathsetmacro\tikz@timer@start@angle{#1}%
  \pgfmathsetmacro\tikz@timer@end@angle{#2}%
  \pgfmathparse{#3}%
  \let\tikz@arc@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikz@@@arcfinal{\pgfpatharc{\tikz@timer@start@angle}{\tikz@timer@end@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{\tikz@timer@start@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{\tikz@timer@end@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}%
      \edef\tikz@timer@zero@axis{\noexpand\pgfqpoint{\tikz@arc@x pt}{0pt}}
      \edef\tikz@timer@ninety@axis{\noexpand\pgfqpoint{0pt}{\tikz@arc@y pt}}
    \else%
      \tikzerror{You cannot mix dimensions and dimensionless values in an arc}%
    \fi%
  \else%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikzerror{You cannot mix dimensions and dimensionless values in an arc}%
    \else%
      \tikz@@@arcfinal{\pgfpatharcaxes{\tikz@timer@start@angle}{\tikz@timer@end@angle}{\pgfpointxy{\tikz@arc@x}{0}}{\pgfpointxy{0}{\tikz@arc@y}}}
      {\pgfpointpolarxy{\tikz@timer@start@angle}{\tikz@arc@x and \tikz@arc@y}}{\pgfpointpolarxy{\tikz@timer@end@angle}{\tikz@arc@x and \tikz@arc@y}}%
      \pgf@process{\pgfpointxy{\tikz@arc@x}{0}}
      \edef\tikz@timer@zero@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      \pgf@process{\pgfpointxy{0}{\tikz@arc@y}}
      \edef\tikz@timer@ninety@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
     \fi%
  \fi%
}%

\def\tikz@@@arcfinal#1#2#3{%
  #1%
  \pgf@process{#2}
  \xdef\tikz@arc@save@first{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgf@process{#3}
  \xdef\tikz@arc@save@second{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
}%

\def\tikz@arcfinal{%
  \pgf@process{\tikz@arc@save@first}%
  \advance\tikz@lastx by-\pgf@x%
  \advance\tikz@lasty by-\pgf@y%
  \pgf@process{\tikz@arc@save@second}%
  \advance\tikz@lastx by\pgf@x%
  \advance\tikz@lasty by\pgf@y%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \let\tikz@timer=\tikz@timer@arc%
  \tikz@scan@next@command%
}%


% Syntax for coordinates:
% coordinate[options] (coordinate name) at (point)
% where ``at (point)'' is optional
\def\tikz@coordinate ordinate{%
  \pgfutil@ifnextchar[{\tikz@@coordinate@opt}{\tikz@@coordinate@opt[]}}%
\def\tikz@@coordinate@opt[#1]{%
  \pgfutil@ifnextchar({\tikz@@coordinate[#1]}
  {\tikz@fig ode[shape=coordinate,#1]{}}}%}%
\def\tikz@@coordinate[#1](#2){%
  \pgfutil@ifnextchar a{\tikz@@coordinate@at[#1](#2)}
  {\tikz@fig ode[shape=coordinate,#1](#2){}}}%
\def\tikz@@coordinate@at[#1](#2)a{%
  \pgfutil@ifnextchar t{\tikz@@coordinate@@at[#1](#2)a}%
  {\tikz@fig ode[shape=coordinate,#1](#2){}a}%
}%
\def\tikz@@coordinate@@at[#1](#2)at#3({%
  \def\tikz@coordinate@caller{\tikz@fig ode[shape=coordinate,#1](#2)at}%
  \tikz@scan@one@point\tikz@@coordinate@at@math(%
}%
\def\tikz@@coordinate@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@temp{(\the\pgf@x,\the\pgf@y)}%
  \expandafter\tikz@coordinate@caller\tikz@temp{}%
}%



% Syntax for nodes:
% node foreach \var in {list} ... :attribute={...} [options] (node name) at (pos) {label text}
%
% all of :attribute, [options], (node name), at(pos), and foreach are
% optional. There can be multiple options and the ordering is not
% important as in node[draw] (a) [rotate=10] {text}, *except* that all
% foreach statements must come first.
%
% A label text always ``ends'' the node.
%
\def\tikz@fig ode{%
  \pgfutil@ifnextchar a\tikz@test@also{%
    \pgfutil@ifnextchar f{\tikz@nodes@start}\tikz@normal@fig}}%
\def\tikz@test@also a{\pgfutil@ifnextchar l\tikz@node@also{\tikz@normal@fig a}}%
\def\tikz@normal@fig{%
  \edef\tikz@save@line@width{\the\pgflinewidth}%
  \begingroup%
  \let\tikz@fig@name=\pgfutil@empty%
    \begingroup%
      \tikz@is@matrixfalse%
      \let\nodepart=\tikz@nodepart%
      \let\tikz@atbegin@scope=\pgfutil@empty%
      \let\tikz@atend@scope=\pgfutil@empty%
      \let\tikz@do@after@node=\tikz@scan@next@command%
      \let\tikz@options=\pgfutil@empty%
      \tikz@clear@rdf@options%
      \let\tikz@id@name=\pgfutil@empty%
      \let\tikz@after@path=\pgfutil@empty%
      \let\tikz@transform=\pgfutil@empty%
      \let\tikz@mode=\pgfutil@empty%
      \tikz@decoratepathfalse%
      \let\tikz@preactions=\pgfutil@empty%
      \let\tikz@postactions=\pgfutil@empty%
      \let\tikz@alias=\pgfutil@empty%
      \def\tikz@node@at{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \let\tikz@time@for@matrix\tikz@time%
      \let\tikz@node@content\relax%
      \pgfgetpath\tikzpathuptonow%
      \iftikz@node@is@a@label%
      \else%
        \let\tikz@time\pgfutil@empty%
      \fi%
      \tikz@node@reset@hook%
      \tikzset{every node/.try}%
      \tikz@@scan@fig}%
\def\tikz@@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar:{\tikz@fig@scan@animation}%
        {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
          {\tikzerror{A node must have a (possibly empty) label text}%
            \tikz@fig@main{}}}}}}}%}}%
\def\tikz@fig@scan@at at{%
  \tikz@scan@one@point\tikz@@fig@scan@at}%
\def\tikz@@fig@scan@at#1{%
  \def\tikz@node@at{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@name(#1){%
    \pgfkeysvalueof{/tikz/name/.@cmd}#1\pgfeov% CF : this is now ALWAYS consistent with 'name=' option; allows overrides.
    \tikz@@scan@fig}%
% make it \long to allow \par in "pin" options etc:
\long\def\tikz@fig@scan@options[#1]{\iftikz@node@is@pic\tikz@enable@pic@quotes\else\tikz@enable@node@quotes\fi\tikzset{#1}\ifx\tikz@node@content\relax\expandafter\tikz@@scan@fig\else\tikz@expand@node@contents\fi}%
\def\tikz@fig@scan@animation:#1=#2{\tikzset{animate={myself:{#1}={#2}}}\tikz@@scan@fig}%
\def\tikz@expand@node@contents{%
  \expandafter\tikz@@scan@fig\expandafter{\tikz@node@content}%
}%
\let\tikz@node@reset@hook=\pgfutil@empty%
\let\tikz@node@begin@hook=\pgfutil@empty%
\def\tikz@fig@main{%
  \iftikz@node@is@pic%
    \tikz@node@is@picfalse%
    \expandafter\tikz@subpicture@handle%
  \else%
    \afterassignment\tikz@@fig@main\expandafter\let\expandafter\next\expandafter=%
  \fi}%
\def\tikz@@fig@main{%
    \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
    {\tikzerror{Unknown shape ``\tikz@shape.'' Using ``rectangle'' instead}%
      \def\tikz@shape{rectangle}}%
    {}%
    \expandafter\xdef\csname tikz@dcl@coord@\tikz@fig@name\endcsname{%
      \csname tikz@scan@point@coordinate\endcsname}%
    \tikzset{every \tikz@shape\space node/.try}%
    \tikz@node@textfont%
    \tikz@node@begin@hook%
    \iftikz@is@matrix%
      \let\tikz@next=\tikz@do@matrix%
    \else%
      \let\tikz@next=\tikz@do@fig%
    \fi%
    \tikz@next%
}%
\let\tikz@nodepart@list\pgfutil@empty
\def\tikz@do@fig{%
    % Ok, reset all node part boxes
    \pgfutil@for\tikz@temp:=\tikz@nodepart@list\do{%
      \expandafter\setbox\csname pgfnodepart\tikz@temp box\endcsname=\box\pgfutil@voidb@x%
    }%
    \setbox\pgfnodeparttextbox=\hbox%
      \bgroup%
        \pgfinterruptpicture%
        \pgfsys@begin@text%
          \pgfsys@text@to@black@hook%
          \tikzset{every text node part/.try}%
          \ifx\tikz@textopacity\pgfutil@empty%
          \else%
            \pgfsetfillopacity{\tikz@textopacity}%
            \pgfsetstrokeopacity{\tikz@textopacity}%
          \fi%
          \ifx\tikz@text@width\pgfutil@empty%
            \tikz@textfont%
          \else%
            \begingroup%
                \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
              \pgfutil@minipage[t]{\pgf@x}\leavevmode\hbox{}%
                \tikz@textfont%
                \tikz@text@action%
          \fi%
          \tikz@atbegin@node%
          \bgroup%
            \aftergroup\unskip%
            % Some color stuff has been moved from here to outside; this is
            % necessary for support of dvisvgm and of animation
            % snapshots.
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
              \pgfutil@color{\tikz@textcolor}%
            \fi%
            \setbox\tikz@figbox=\box\pgfutil@voidb@x%
            \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
            \tikz@uninstallcommands%
            \iftikz@handle@active@code%
              \tikz@orig@shorthands%
              \let\tikz@orig@shorthands\pgfutil@empty%
            \fi%
            \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
            \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
            \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
            \aftergroup\tikz@fig@collectresetcolor%
            \tikz@signal@halign@check%
            \tikz@text@reset%
            \tikz@halign@check%
            \ignorespaces%
}%
\def\tikz@fig@collectresetcolor{%
  % Hacks for special packages that mess with \aftergroup
  \pgfutil@ifnextchar\reset@color% hack for color package
  {\reset@color\afterassignment\tikz@fig@collectresetcolor\let\tikz@temp=}\tikz@fig@boxdone%
}%
\def\tikz@fig@boxdone{%
            \tikz@atend@node%
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
              \pgfutil@endminipage%
            \endgroup%
          \fi%
        \pgfsys@end@text%
        \endpgfinterruptpicture%
      \egroup%
    \pgfutil@ifnextchar c{\tikz@fig@mustbenamed\tikz@fig@continue}%
    {\pgfutil@ifnextchar[{\tikz@fig@mustbenamed\tikz@fig@continue}%
      {\pgfutil@ifnextchar t{\tikz@fig@mustbenamed\tikz@fig@continue}
        {\pgfutil@ifnextchar e{\tikz@fig@mustbenamed\tikz@fig@continue}
          {\ifx\tikz@after@path\pgfutil@empty\expandafter\tikz@fig@continue\else\expandafter\tikz@fig@mustbenamed\expandafter\tikz@fig@continue\fi}}}}}%}%

\tikzset{
  matrix/inner style/every cell/.code={%
    \tikzset{every cell/.try={\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  },
  matrix/inner style/column/.code={%
    \tikzset{column \the\pgfmatrixcurrentcolumn/.try}%
  },
  matrix/inner style/even odd column/.code={
    \ifodd\pgfmatrixcurrentcolumn%
      \tikzset{every odd column/.try}%
    \else%
      \tikzset{every even column/.try}%
    \fi
  },
  matrix/inner style/row/.code={%
    \tikzset{row \the\pgfmatrixcurrentrow/.try}%
  },
  matrix/inner style/even odd row/.code={%
    \ifodd\pgfmatrixcurrentrow%
      \tikzset{every odd row/.try}%
    \else%
      \tikzset{every even row/.try}%
    \fi
  },
  matrix/inner style/cell/.code={%
    \tikzset{row \the\pgfmatrixcurrentrow\space column \the\pgfmatrixcurrentcolumn/.try}%
  },
  matrix/inner style order/.store in=\tikz@common@matrix@code@styleorder,
  matrix/inner style order={
    every cell,
    column,
    even odd column,
    row,
    even odd row,
    cell
  },
}%

\def\tikz@do@matrix{%
    \tikzset{every matrix/.try}%
    \tikz@node@transformations%
    \tikz@fig@mustbenamed%
    \setbox\tikz@whichbox=\hbox\bgroup%
      \unhbox\tikz@whichbox%
      \hbox\bgroup\bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \ifx\tikz@time\pgfutil@empty\let\tikz@time\tikz@time@for@matrix\fi%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \tikz@is@nodefalse%
              \tikz@call@id@hook%
              \pgfidscope%
                \tikz@do@rdf@post@options%
                \begingroup%
                \let\tikz@id@name\pgfutil@empty%
                \pgfclearid%
                \setbox\tikz@figbox=\box\pgfutil@voidb@x%
                \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
                \let\tikzmatrixname=\tikz@fig@name%
                \edef\tikz@m@anchor{\ifx\tikz@matrix@anchor\pgfutil@empty\tikz@anchor\else\tikz@matrix@anchor\fi}%
                \expandafter\pgfutil@in@\expandafter{\expandafter.\expandafter}\expandafter{\tikz@m@anchor}%
                \ifpgfutil@in@%
                  \expandafter\tikz@matrix@split\tikz@m@anchor\relax%
                \else%
                  \def\tikz@matrix@shift{\pgfpointorigin}%
                \fi%
                \let\tikz@transform=\relax%
                \pgfmatrixbeforeassemblenode{\tikzset{every outer matrix/.try}}%
                \pgfmatrix%
                {\tikz@shape}%
                {\tikz@m@anchor}%
                {\tikz@fig@name}%
                {%
                  \pgfutil@tempdima=\pgflinewidth%
                  {\begingroup\tikz@finish}%
                  \global\pgflinewidth=\pgfutil@tempdima%
                }%
                {\tikz@matrix@shift}%
                {%
                  \tikz@matrix@make@active@ampersand%
                  \def\pgfmatrixbegincode{%
                    \pgfsys@beginscope%
                    \tikz@common@matrix@code%
                    \tikz@atbegin@cell%
                  }%
                  \def\tikz@common@matrix@code{%
                    \let\tikz@options=\pgfutil@empty%
                    \let\tikz@mode=\pgfutil@empty%
                    \pgfutil@for\pgf@temp:=\tikz@common@matrix@code@styleorder\do{%
                      \toks0=\expandafter{\romannumeral-`0\expandafter\pgfutil@trimspaces\expandafter{\pgf@temp}}%
                      \def\pgf@marshal{}%
                      \pgfutil@ifempty\pgf@temp{}{%
                        \edef\pgf@marshal{\noexpand\tikzset{matrix/inner style/.cd,\the\toks0}}%
                      }%
                      \pgf@marshal
                    }%
                    \tikz@options%
                  }%
                  \def\pgfmatrixendcode{%
                    \tikz@atend@cell%
                    \pgfsys@endscope%
                  }%
                  \def\pgfmatrixemptycode{%
                    \pgfsys@beginscope%
                    \tikz@common@matrix@code%
                    \tikz@at@emptycell%
                    \pgfsys@endscope%
                  }%
                  \tikz@atbegin@matrix%
                  \aftergroup\tikz@do@matrix@cont}%
                \bgroup%
}%
\def\tikz@do@matrix@cont{%
                \tikz@atend@matrix%
              \endgroup%
              \endpgfidscope%
            \endpgfscope
          \endpgfinterruptpath%
      \egroup\egroup%
    \egroup%
    %
    \tikz@node@finish%
}%
{%
  \catcode`\&=13
  \gdef\tikz@matrix@make@active@ampersand{%
    \ifx\tikz@ampersand@replacement\pgfutil@empty%
      \catcode`\&=13%
      \let&=\pgfmatrixnextcell%
    \else%
      \expandafter\let\tikz@ampersand@replacement=\pgfmatrixnextcell%
    \fi%
  }%
}%


\def\tikz@matrix@split#1.#2\relax{%
  \def\tikz@m@anchor{text}%
  \def\tikz@matrix@shift{\pgfpointanchor{#1}{#2}}%
}%

\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    % Node transformation
    %
    \tikz@node@transformations%
    \tikz@nlt%
    %
    \setbox\tikz@whichbox=\hbox{%
      \unhbox\tikz@whichbox%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \tikz@is@nodetrue%
              \tikz@call@id@hook%
              \pgfidscope%
                \tikz@do@rdf@post@options%
                \let\tikz@id@name\pgfutil@empty%
                \setbox\tikz@figbox=\box\pgfutil@voidb@x%
                \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
                % Add color modifications to text box
                \setbox\pgfnodeparttextbox=\hbox{{%
                    \pgfsys@begin@text% Colors moved here...
                    \ifx\tikz@textcolor\pgfutil@empty%
                    \else%
                      \pgfutil@colorlet{.}{\tikz@textcolor}%
                    \fi%
                    \pgfsetcolor{.}%
                    \pgfusetype{.text}%
                    \pgfidscope%
                      \box\pgfnodeparttextbox%
                    \endpgfidscope%
                    \pgfsys@end@text%
                  }}%
                \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                  \pgfutil@tempdima=\pgflinewidth%
                  {\begingroup\tikz@finish}%
                  \global\pgflinewidth=\pgfutil@tempdima%
                }%
              \endpgfidscope%
            \endpgfscope%
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}%


\def\tikz@fig@mustbenamed{%
  \ifx\tikz@fig@name\pgfutil@empty%
    % Assign a dummy name
    \global\advance\tikz@fig@count by1\relax
    \edef\tikz@fig@name{tikz@f@\the\tikz@fig@count}%
    \let\tikz@id@name\tikz@fig@name%
  \fi%
}%

\def\tikz@node@transformations{%
  %
  % Possibly, we are ``online''
  %
  \ifx\tikz@time\pgfutil@empty%
    \pgftransformshift{\tikz@node@at}%
    \iftikz@fullytransformed%
    \else%
      \pgftransformresetnontranslations%
    \fi%
  \else%
    \tikz@do@auto@anchor%
    \tikz@timer%
  \fi%
  % Invoke local transformations
  \tikz@transform%
}%

\def\tikz@node@finish{%
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@path@smuggle=\tikz@after@path%
    % shift box outside group
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \endgroup\endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \global\pgflinewidth=\tikz@save@line@width%
  \tikz@do@after@path@smuggle%
  \tikz@node@is@picfalse
  \tikz@do@after@node%
}%
\let\tikz@fig@continue@orig=\tikz@fig@continue

\def\tikz@do@after@node{\tikz@scan@next@command}%

\def\tikz@do@after@path@smuggle{%
  \let\tikz@to@last@fig@name=\tikz@last@fig@name%
  \let\tikz@to@use@whom=\tikz@to@use@last@fig@name%
  \let\tikzlastnode=\tikz@last@fig@name%
  \ifx\tikz@after@path@smuggle\pgfutil@empty%
  \else%
    \ifpgflatenodepositioning%
      \expandafter\expandafter\expandafter\tikz@call@late%
      \expandafter\expandafter\expandafter{\expandafter\tikz@last@fig@name\expandafter}\expandafter{\tikz@after@path@smuggle}%
    \else%
      \tikz@scan@next@command{\tikz@after@path@smuggle}\pgf@stop%
    \fi%
  \fi%
}%

\def\tikz@call@late#1#2{\pgfnodepostsetupcode{#1}{\path[late options={name={#1},append after command={#2}}];}}%

\newif\iftikz@do@align

% Alignment handling
\def\tikz@signal@halign@check{%
  \tikz@do@alignfalse
  \ifx\tikz@text@width\pgfutil@empty%
    \pgfkeysgetvalue{/tikz/node halign header}\tikz@align@header%
    \ifx\tikz@align@header\pgfutil@empty%
    \else%
      \tikz@do@aligntrue%
    \fi%
  \fi%
}
\def\tikz@halign@check{%
  \iftikz@do@align%
    % Bingo
    \setbox\tikz@align@aligned@box=\box\pgfutil@voidb@x% void
    \let\\=\tikz@align@newline%
    \expandafter\tikz@start@align%
  \fi%
}%
\def\tikz@align@newline{\pgfutil@protect\tikz@align@newline@}%
\def\tikz@align@newline@{\unskip\pgfutil@ifnextchar[\tikz@@align@newline{\tikz@@align@newline[0pt]}}%}%
\def\tikz@@align@newline[#1]{\egroup\tikz@align@continue\pgfmathparse{#1}\let\tikz@align@temp=\pgfmathresult\tikz@start@align}%
% Two safe boxes for alignment:
\let\tikz@align@aligned@box=\pgfnodeparttextbox
\let\tikz@align@line@box=\tikz@figbox

\def\tikz@start@align{%
  % Start collecting text:
  \setbox\tikz@align@line@box=\hbox\bgroup\bgroup%
    \aftergroup\tikz@align@collectresetcolor\ignorespaces%
}%
\def\tikz@align@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\tikz@align@collectresetcolor\let\tikz@temp=}%
  {\tikz@align@end@check}%
}%
\def\tikz@align@end@check{%
  \egroup%
  \ifvoid\tikz@align@aligned@box%
    \setbox\tikz@align@aligned@box=\box\tikz@align@line@box%
  \else%
    \setbox\tikz@align@aligned@box=\vbox{%
      \expandafter\expandafter\expandafter\halign\expandafter\expandafter\expandafter{\tikz@align@header%
        \box\tikz@align@aligned@box\cr%
        \noalign{\vskip\tikz@align@temp pt}%
        \unhbox\tikz@align@line@box\unskip\cr}}%
  \fi%
  \pgfutil@ifnextchar\tikz@align@continue{}
  {%
    % Main continue
      \box\tikz@align@aligned@box%
    \egroup%
  }%
}%
\def\tikz@align@continue{\tikz@@align@continue}%
\let\tikz@@align@continue=\pgfutil@empty


\def\tikz@node@also lso{\pgfutil@ifnextchar[\tikz@node@also@opt{\tikz@node@also@opt[]}}%
\def\tikz@node@also@opt[#1]{
  \pgfutil@ifnextchar(%)
  {\tikz@node@also@opt@cont[#1]}%
  {\tikzerror{Syntax error in node also: ``('' expected.}%
    \tikz@scan@next@command}%
}%
\def\tikz@node@also@opt@cont[#1](#2){\tikzset{late options={name=#2,#1}}\tikz@scan@next@command}%



% Syntax for parts of  nodes:
% node ... {... \nodepart[options]{name} ... \nodepart{name} ...}

\def\tikz@nodepart{\pgfutil@ifnextchar[\tikz@@nodepart{\tikz@@nodepart[]}}%}%
\def\tikz@@nodepart[#1]#2{%
  \tikz@atend@node%
  \unskip%
  \gdef\tikz@nodepart@options{#1}%
  \gdef\tikz@nodepart@name{#2}%
  \global\let\tikz@fig@continue=\tikz@nodepart@continue%
  \pgfutil@ifnextchar x{\egroup\relax}{\egroup\relax}% gobble spaces
}%
\def\tikz@nodepart@continue{%
  \global\let\tikz@fig@continue=\tikz@fig@continue@orig%
  \ifx\tikz@nodepart@list\pgfutil@empty%
    \let\tikz@nodepart@list\tikz@nodepart@name%
  \else%
    \edef\tikz@nodepart@list{\tikz@nodepart@list,\tikz@nodepart@name}%
  \fi%
  % Now start new box:
   \expandafter\setbox\csname pgfnodepart\tikz@nodepart@name box\endcsname=\hbox%
      \bgroup%
        \pgfinterruptpicture%
        \pgfsys@begin@text%
        \pgfsys@text@to@black@hook%
        \tikzset{every \tikz@nodepart@name\space node part/.try}%
        \expandafter\tikzset\expandafter{\tikz@nodepart@options}%
        \ifx\tikz@textopacity\pgfutil@empty%
        \else%
          \pgfsetfillopacity{\tikz@textopacity}%
          \pgfsetstrokeopacity{\tikz@textopacity}%
        \fi%
        % Colors moved here...
        \ifx\tikz@textcolor\pgfutil@empty%
        \else%
          \pgfutil@colorlet{.}{\tikz@textcolor}%
        \fi%
        \pgfsetcolor{.}%
          \ifx\tikz@text@width\pgfutil@empty%
            \tikz@textfont%
          \else%
            \begingroup%
              \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
              \pgfutil@minipage[t]{\pgf@x}\leavevmode\hbox{}%
                \tikz@textfont%
                \tikz@text@action%
          \fi%
          \bgroup%
            \aftergroup\unskip%
            \setbox\tikz@figbox=\box\pgfutil@voidb@x%
            \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
            \tikz@uninstallcommands%
            \iftikz@handle@active@code%
              \tikz@orig@shorthands%
              \let\tikz@orig@shorthands\pgfutil@empty%
            \fi%
            \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
            \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
            \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
            \tikz@atbegin@node%
            \aftergroup\tikz@fig@collectresetcolor%
            \tikz@signal@halign@check%
            \tikz@text@reset%
            \tikz@halign@check%
            \ignorespaces%
}%


%
% Node foreach
%

\def\tikz@nodes@start{%
  \let\tikz@nodes@list\pgfutil@empty%
  \iftikz@node@is@pic%
    \def\tikz@nodes@collect{pic }%
  \else%
    \def\tikz@nodes@collect{node }%
  \fi%
  \tikz@nodes%
}%
\def\tikz@nodes foreach{\pgfutil@ifnextchar x\tikz@nodes@\tikz@nodes@}% get rid of spaces
\def\tikz@nodes@#1in{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list\foreach#1in}%
  \pgfutil@ifnextchar\bgroup\tikz@nodes@group\tikz@nodes@one%
}%
\def\tikz@nodes@one#1{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list#1}%
  \pgfutil@ifnextchar f\tikz@nodes\tikz@nodes@scan%
}%
\def\tikz@nodes@group#1{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list{#1}}%
  \pgfutil@ifnextchar f\tikz@nodes\tikz@nodes@scan%
}%
\def\tikz@nodes@scan{%
  \pgfutil@ifnextchar a{\tikz@nodes@at}%
  {\pgfutil@ifnextchar({\tikz@nodes@name}%
    {\pgfutil@ifnextchar[{\tikz@nodes@opt}%
      {\pgfutil@ifnextchar\bgroup{\tikz@nodes@main}%
      {\tikzerror{Nodes must have a (possibly empty) label text}%
        \tikz@fig@main{}}}}}}%}}%

% Look ahead whether the next character is a (.  If that is the case, we scan
% until ), otherwise we grab a single token and append.
\def\tikz@nodes@at at{\pgfutil@ifnextchar({\tikz@nodes@at@}{\tikz@nodes@at@@}}%
\def\tikz@nodes@at@#1){%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect at#1)}%
  \tikz@nodes@scan}%
\def\tikz@nodes@at@@#1{%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect at#1}%
  \tikz@nodes@scan}%

\def\tikz@nodes@name#1){%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect#1)}%
  \tikz@nodes@scan}%
\def\tikz@nodes@opt#1]{%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect#1]}%
  \tikz@nodes@scan}%
\def\tikz@nodes@main#1{%
  \iftikz@handle@active@nodes%
    \iftikz@node@is@pic%
      \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{#1}}%
    \else%
      \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{\scantokens{#1}}}%
    \fi%
  \else%
    \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{#1}}%
  \fi%
  % Ok, got everything.
  % Now, start building parse text.
  \global\setbox\tikz@tempbox=\box\tikz@figbox%
  \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \tikz@nodes@list{%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \expandafter\tikz@scan@next@command\tikz@nodes@collect\pgfextra\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  }%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \tikz@scan@next@command%
}%



%
% "late" options can be used to "redo" a node
%
\tikzset{late options/.code=\tikz@late@options{#1}}%
\def\tikz@late@options#1{%
  % Do a "virtual" node:
  \begingroup%
    \iftikz@shapeborder%
      \let\tikz@fig@name=\tikz@shapeborder@name%
    \else%
      \let\tikz@fig@name=\pgfutil@empty%
    \fi%
    \tikz@is@matrixfalse%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@after@path=\pgfutil@empty%
    \let\tikz@afternodepathoptions=\pgfutil@empty%
    \let\tikz@alias=\pgfutil@empty%
    \let\tikz@transform=\pgfutil@empty%
    \tikz@decoratepathfalse%
    \tikz@node@reset@hook%
    \tikz@enable@node@quotes%
    \tikzset{every node/.try,#1}%
    \ifx\tikz@fig@name\pgfutil@empty%
      \tikzerror{Late options must reference some existing node}%
    \fi%
    \tikz@node@begin@hook%
    \tikz@alias%
    \tikzgdlatenodeoptionacallback{\tikz@fig@name}%
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@path@smuggle=\tikz@after@path%
  \endgroup%
  \tikz@do@after@path@smuggle%
}%


% Auto placement

\def\tikz@auto@pre{%
  \begingroup
    \pgfresetnontranslationattimefalse
    \ifpgfslopedattime
      \pgfslopedattimefalse%
    \else
      \pgfslopedattimetrue%
    \fi
    \pgfallowupsidedownattimetrue%
    \tikz@timer%
    \pgf@x=\pgf@pt@aa pt%
    \pgf@y=\pgf@pt@ab pt%
    \pgfpointnormalised{}%
}%

\def\tikz@auto@post{%
    \global\let\tikz@anchor@smuggle=\tikz@anchor%
  \endgroup%
  \let\tikz@anchor=\tikz@anchor@smuggle%
}%

\def\tikz@auto@anchor{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south west}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north west}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{east}%
      \else%
        \def\tikz@anchor{west}%
      \fi%
    \fi\fi%
}%

\def\tikz@auto@anchor@prime{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north east}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south east}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{west}%
      \else%
        \def\tikz@anchor{east}%
      \fi%
    \fi\fi%
}%


%
% Callbacks: Please see the documentation of the graph drawing
% lib for info on these callbacks
%
\def\tikzgdeventcallback#1#2{}%
\def\tikzgdeventgroupcallback#1{}%
\def\tikzgdlatenodeoptionacallback#1{}%

% Syntax for trees:
% node {...} child [options] {...} child [options] {...} ...
% node {...} child [options] foreach \var in {list} [options] {...} ...

\def\tikz@children{%
  % Start collecting the children:
  \let\tikz@children@list=\pgfutil@empty%
  \tikznumberofchildren=0\relax%
  \tikz@collect@children c}%

\def\tikz@collect@children{\pgfutil@ifnextchar c{\tikz@collect@children@cchar}{\tikz@children@collected}}%
\def\tikz@collect@children@cchar c{\pgfutil@ifnextchar h{\tikz@collect@child}{\tikz@children@collected c}}%
\def\tikz@collect@child hild{\pgfutil@ifnextchar[{\tikz@collect@childA}{\tikz@collect@childA[]}}%}%
\def\tikz@collect@childA[#1]{\pgfutil@ifnextchar f{\tikz@collect@children@foreach[#1]}{\tikz@collect@childB[#1]}}%
\def\tikz@collect@childB[#1]{%
  \advance\tikznumberofchildren by1\relax
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list \tikz@childnode[#1]}%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@child@code}{\tikz@collect@child@code{}}}%
\def\tikz@collect@child@code#1{%
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list{#1}}%
  \tikz@collect@children%
}%
\def\tikz@collect@children@foreach[#1]foreach#2in#3{%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@children@foreachA{#1}{#2}{#3}}{\tikz@collect@children@foreachA{#1}{#2}{#3}{}}}%
\def\tikz@collect@children@foreachA#1#2#3#4{%
  \expandafter\def\expandafter\tikz@children@list\expandafter
    {\tikz@children@list\tikz@childrennodes[#1]{#2}{#3}{#4}}%
  \c@pgf@counta=\tikznumberofchildren%
  \foreach#2in{#3}%
  {%
    \global\advance\c@pgf@counta by1\relax%
  }%
  \tikznumberofchildren=\c@pgf@counta%
  \tikz@collect@children%
}%
\long\def\tikz@children@collected{%
  \begingroup%
    \advance\tikztreelevel by 1\relax%
    \tikzgdeventgroupcallback{descendants}%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@transform=\pgfutil@empty%
    \tikzset{level/.try=\the\tikztreelevel,level \the\tikztreelevel/.try}%
    \tikz@transform%
    \let\tikz@transform=\relax%
    \let\tikzparentnode=\tikz@last@fig@name%
    \ifx\tikz@grow\relax\else%
      % Transform to center of node
      \pgftransformshift{\pgfpointanchor{\tikzparentnode}{\tikz@growth@anchor}}%
    \fi%
    \tikznumberofcurrentchild=0\relax%
    \tikz@children@list%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \tikz@scan@next@command%
}%

% Syntax for children:
%
% child [all children options] foreach \var in {values} [child options] {...}
\def\tikz@childrennodes[#1]#2#3#4{%
  \c@pgf@counta=\tikznumberofcurrentchild\relax%
  \setbox\tikz@tempbox=\box\tikz@figbox%
  \setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \foreach#2in{#3}{%
    \tikznumberofcurrentchild=\c@pgf@counta\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \tikz@childnode[#1]{#4}%
    % we must now make the current child number and the figbox survive
    % the group
    \global\c@pgf@counta=\tikznumberofcurrentchild\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  }%
  \tikznumberofcurrentchild=\c@pgf@counta\relax%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
}%


% Syntax for child:
%
% child
%
% child[options]
%
% child[options] {node (name) {child node text} ...
%   edge from parent[options] node {label text} node {label text}}

\def\tikz@childnode[#1]#2{%
  \advance\tikznumberofcurrentchild by1\relax%
  {\tikzset{every child/.try,#1}\expandafter}%
  \iftikz@child@missing%
    \tikzgdeventcallback{node}{}%
  \else%
  \setbox\tikz@whichbox=\hbox\bgroup%
    \unhbox\tikz@whichbox%
    \hbox\bgroup\bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \tikzset{every child/.try,#1}%
            \tikz@options%
            \tikz@transform%
            \let\tikz@transform=\relax%
            \tikz@grow%
            % Typeset node:
            \edef\tikz@parent@node@name{[name=\tikzparentnode-\the\tikznumberofcurrentchild,style=every child node]}%
            \def\tikz@child@node@text{[shape=coordinate]{}}
            \tikz@parse@child@node#2\pgf@stop%
            \expandafter\expandafter\expandafter\node
            \expandafter\tikz@parent@node@name
              \tikz@child@node@text
              \pgfextra{\global\let\tikz@childnode@name=\tikz@last@fig@name};%
            \let\tikzchildnode=\tikz@childnode@name%
            {%
              \def\tikz@edge@to@parent@needed{edge from parent}
              \ifx\tikz@child@node@rest\pgfutil@empty%
                \path edge from parent;%
              \else%
                \path \tikz@child@node@rest \tikz@edge@to@parent@needed;%
              \fi%
            }%
        \endpgfscope%
      \endpgfinterruptpath%
    \egroup\egroup%
  \egroup%
  \fi%
}%

\def\tikz@parse@child@node{%
  \pgfutil@ifnextchar n{\tikz@parse@child@node@n}%
  {\pgfutil@ifnextchar c{\tikz@parse@child@node@c}%
    {\pgfutil@ifnextchar\pgf@stop\tikz@parse@child@node@rest\tikz@parse@child@node@expand}}}%
\def\tikz@parse@child@node@expand{%
  \advance\tikz@expandcount by-1\relax%
  \ifnum\tikz@expandcount<0\relax%
    \expandafter\tikz@parse@child@node@rest%
  \else%
    \expandafter\expandafter\expandafter\tikz@parse@child@node%
  \fi%
}%
\def\tikz@parse@child@node@rest#1\pgf@stop{\tikz@expandcount=100\relax\def\tikz@child@node@rest{#1}}%
\def\tikz@parse@child@node@c c{\tikz@expandcount=100\pgfutil@ifnextchar o{\tikz@parse@child@node@co}{\tikz@parse@child@node@rest c}}%
\def\tikz@parse@child@node@co o{\pgfutil@ifnextchar o{\tikz@parse@child@node@coordinate}{\tikz@parse@child@node@rest co}}%
\def\tikz@parse@child@node@coordinate ordinate{%
  \pgfutil@ifnextchar ({\tikz@@parse@child@node@coordinate}{%
    \def\tikz@child@node@text{[shape=coordinate]{}}%
    \tikz@parse@child@node@rest}}%}%
\def\tikz@@parse@child@node@coordinate(#1){%
  \pgfutil@ifnextchar a{\tikz@p@c@n@c@at(#1)}{%
    \def\tikz@child@node@text{[shape=coordinate,name=#1]{}}%
    \tikz@parse@child@node@rest}}%
\def\tikz@p@c@n@c@at(#1)at#2({%
  \def\tikz@child@node@text@pre{[shape=coordinate,name=#1]at}%
  \tikz@scan@one@point\tikz@p@c@n@c@at@math(%
}%
\def\tikz@p@c@n@c@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{(\the\pgf@x,\the\pgf@y){}}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text@pre\tikz@marshal}%
  \tikz@parse@child@node@rest%
}%
\def\tikz@parse@child@node@n node{\tikz@expandcount=100%
  \let\tikz@child@node@text=\pgfutil@empty%
  \tikz@p@c@s}%
\def\tikz@p@c@s{%
  \pgfutil@ifnextchar a{\tikz@p@c@s@at}
  {\pgfutil@ifnextchar ({\tikz@p@c@s@paran}
    {\pgfutil@ifnextchar [{\tikz@p@c@s@bra}
      {\pgfutil@ifnextchar \bgroup{\tikz@p@c@s@group}
        {\tikzerror{Cannot parse this node}}}}}}%}}%
\def\tikz@p@c@s@at at#1({%
  \tikz@scan@one@point\tikz@p@c@s@at@math(%
}%
\def\tikz@p@c@s@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{ at(\the\pgf@x,\the\pgf@y)}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text\tikz@marshal}
  \tikz@p@c@s}%
\def\tikz@p@c@s@paran(#1){%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text(#1)}
  \tikz@p@c@s}%
\def\tikz@p@c@s@bra[#1]{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text[#1]}
  \tikz@p@c@s}%
\def\tikz@p@c@s@group#1{%
  \iftikz@handle@active@nodes%
    \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{\scantokens{#1}}}%
  \else%
    \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{#1}}
  \fi%
  \tikz@parse@child@node@rest%
}%



%
% Syntax for decorated subpaths:
%
% decorate [option] { subpath }
%
\def\tikz@decoration ecorate{%
  \pgfutil@ifnextchar[{\tikz@lib@decoration}{\tikz@lib@decoration[]}%]
}%

\def\tikz@lib@decoration[#1]#2{\tikzerror{You need to load a decoration library}}%

% The decorate path command:
\def\tikz@lib@dec@decorate@path{\tikzerror{You need to load a decoration library}}%



%
% Syntax for let :
%
% let \p1 = (coordinate), \p2 = (coordinate),... in
%
\def\tikz@let@command et#1in{%
  \tikzerror{You need to say \string\usetikzlibrary{calc} to use the let command}%
  \tikz@scan@next@command%
}%


%
% Syntax for pictures:
%
% as for nodes, but with "pic" instead of "node"
%
\newif\iftikz@node@is@pic
\def\tikz@subpicture ic{\tikz@node@is@pictrue\tikz@scan@next@command node}%
\def\tikz@subpicture@handle#1{%
  \pgfkeys@spdef\tikz@temp{#1}%
  \expandafter\tikz@subpicture@handle@\expandafter{\tikz@temp}%
}%
\def\tikz@subpicture@handle@#1{
  \pgfkeys{/tikz/pics/.cd,#1}%
  \tikz@node@transformations%
  \let\tikz@transform=\relax%
  \let\tikz@picmode\tikz@mode%
  \tikzset{name prefix ../.style/.expanded={/tikz/name prefix=\pgfkeysvalueof{/tikz/name prefix}}}%
  \ifx\tikz@fig@name\pgfutil@empty\else%
    \tikzset{name prefix/.expanded=\tikz@fig@name}%
  \fi%
  \pgfkeysvalueof{/tikz/pics/setup code}%
  \pgfkeysgetvalue{/tikz/pics/code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@whichbox=\hbox\bgroup%
    \unhbox\tikz@whichbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \pgfkeysgetvalue{/tikz/pics/foreground code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every front pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \pgfkeysgetvalue{/tikz/pics/background code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@figbox@bg=\hbox\bgroup%
    \unhbox\tikz@figbox@bg%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every behind pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \tikz@node@finish%
}%
\tikzset{
  pic actions/.code=\tikz@addmode{\tikz@picmode}
}%

% Setting up the picture codes:
\tikzset{
  pics/setup code/.initial=,
  pics/code/.initial=,
  pics/background code/.initial=,
  pics/foreground code/.initial=
}%

% Defining pictures:

\def\tikzdeclarepic#1#2{\pgfkeys{/tikz/#1/.cd,#2}}%

\pgfkeysdef{/handlers/.pic}{%
  \edef\pgf@temp{\pgfkeyscurrentpath}%
  \edef\pgf@temp{\expandafter\tikz@smuggle@pics@in\pgf@temp\pgf@stop}%
  \expandafter\pgfkeys\expandafter{\pgf@temp/.style={code={#1}}}%
}%
\def\tikz@smuggle@pics@in/tikz/#1\pgf@stop{/tikz/pics/#1}%

%
% Timers
%

\def\tikz@timer@line{%
  \pgftransformlineattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@end}%
}%

\def\tikz@timer@vhline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}%

\def\tikz@timer@hvline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}%

\def\tikz@timer@curve{%
  \pgftransformcurveattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@cont@one}{\tikz@timer@cont@two}{\tikz@timer@end}%
}%


\def\tikz@timer@arc{%
  \pgfmathcos@{\tikz@timer@start@angle}%
  \let\tikz@angle@cos\pgfmathresult%
  \pgfmathsin@{\tikz@timer@start@angle}%
  \let\tikz@angle@sin\pgfmathresult%
  \pgftransformarcaxesattime{\tikz@time}{%
    \pgfpointdiff{%
      \pgfpointadd{%
        \pgfpointscale{\tikz@angle@cos}{\tikz@timer@zero@axis}%
      }{%
        \pgfpointscale{\tikz@angle@sin}{\tikz@timer@ninety@axis}%
      }%
    }%
    {\tikz@timer@start}%
  }%
  {\tikz@timer@zero@axis}%
  {\tikz@timer@ninety@axis}%
  {\tikz@timer@start@angle}{\tikz@timer@end@angle}%
}%



%
% Coordinate systems
%

\def\tikzdeclarecoordinatesystem#1#2{%
  \expandafter\def\csname tikz@parse@cs@#1\endcsname(##1){%
    \pgf@process{%
      #2%
      \global\let\tikz@smubble@b=\tikz@shapeborder@name%
    }%
    \let\tikz@shapeborder@name=\tikz@smubble@b%
    \edef\tikz@return@coordinate{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
}%
\def\tikzaliascoordinatesystem#1#2{%
  \edef\pgf@marshal{\noexpand\let\expandafter\noexpand\csname
    tikz@parse@cs@#1\endcsname=\expandafter\noexpand\csname
    tikz@parse@cs@#2\endcsname}%
  \pgf@marshal%
}%


% Default coordinate systems:

\tikzdeclarecoordinatesystem{canvas}
{%
  \tikzset{cs/.cd,x=0pt,y=0pt,#1}%
  \pgfpoint{\tikz@cs@x}{\tikz@cs@y}%
}%

\tikzdeclarecoordinatesystem{canvas polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0cm,#1}%
  \pgfpointpolar{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}%

\tikzdeclarecoordinatesystem{xyz}
{%
  \tikzset{cs/.cd,x=0,y=0,z=0,#1}%
  \pgfpointxyz{\tikz@cs@x}{\tikz@cs@y}{\tikz@cs@z}%
}%

\tikzdeclarecoordinatesystem{xyz polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0,#1}%
  \pgfpointpolarxy{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}%
\tikzaliascoordinatesystem{xy polar}{xyz polar}%


\tikzdeclarecoordinatesystem{node}
{%
  \tikzset{cs/.cd,name=,anchor=none,angle=none,#1}%
  \ifx\tikz@cs@anchor\tikz@nonetext%
    \ifx\tikz@cs@angle\tikz@nonetext%
      \expandafter\ifx\csname pgf@sh@ns@\tikz@cs@node\endcsname\tikz@coordinate@text%
      \else
        \aftergroup\tikz@shapebordertrue%
        \edef\tikz@shapeborder@name{\tikz@pp@name{\tikz@cs@node}}%
      \fi%
      \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{center}%
    \else%
      \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{\tikz@cs@angle}%
    \fi%
  \else%
    \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{\tikz@cs@anchor}%
  \fi%
}%

% Intersection coordinates
\tikzset{cs/first line/.code=\def\tikz@cs@line@a{#1}\def\tikz@cs@type@a{line}}%
\tikzset{cs/second line/.code=\def\tikz@cs@line@b{#1}\def\tikz@cs@type@b{line}}%

\tikzset{cs/first node/.code=\tikz@cs@unpack{\tikz@cs@node@a}{\tikz@cs@type@a}{#1}}%
\tikzset{cs/second node/.code=\tikz@cs@unpack{\tikz@cs@node@b}{\tikz@cs@type@b}{#1}}%

\def\tikz@cs@unpack#1#2#3{%
  \expandafter\ifx\csname pgf@sh@ns@#3\endcsname\relax%
    \tikzerror{Undefined node ``#3''}%
  \else%
    \def#1{#3}%
    \edef#2{\csname pgf@sh@ns@#3\endcsname}%
  \fi%
}%

\tikzset{cs/solution/.initial=1}%

\tikzset{cs/horizontal line through/.store in=\tikz@cs@hori@line}%
\tikzset{cs/vertical line through/.store in=\tikz@cs@vert@line}%

\tikzdeclarecoordinatesystem{intersection}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\ifx\csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname\relax%
    \tikzerror{I do not know how to compute the intersection
    of a \tikz@cs@type@a and a \tikz@cs@type@b. Try saying
    \string\usetikzlibrary{calc}}%
    \pgfpointorigin%
  \else%
    \csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname%
  \fi%
}%

\def\tikz@intersect@line@and@line{%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@a%
  \pgf@xa=\pgf@xc%
  \pgf@ya=\pgf@yc%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@b%
  \edef\pgf@marshal{%
    {\noexpand\pgfpointintersectionoflines%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}%
  \pgf@marshal%
}%

\def\tikz@parse@line#1--{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \tikz@scan@one@point\pgf@process%
}%


\tikzdeclarecoordinatesystem{perpendicular}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@a\tikz@cs@hori@line%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@b\tikz@cs@vert@line%
  \pgfqpoint{\the\pgf@xb}{\the\pgf@ya}
}%

\tikzdeclarecoordinatesystem{barycentric}
{%
  {%
    \pgf@xa=0pt% point
    \pgf@ya=0pt%
    \pgf@xb=0pt% sum
    \tikz@bary@dolist#1,=,%
    \pgfmathparse{1/\the\pgf@xb}%
    \global\pgf@x=\pgfmathresult\pgf@xa%
    \global\pgf@y=\pgfmathresult\pgf@ya%
  }%
}%

\def\tikz@bary@dolist#1=#2,{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \pgfmathparse{#2}%
    \advance\pgf@xa by\pgfmathresult\pgf@x%
    \advance\pgf@ya by\pgfmathresult\pgf@y%
    \advance\pgf@xb by\pgfmathresult pt%
    \expandafter\tikz@bary@dolist%
  \fi%
}%

\tikzset{cs/x/.store in=\tikz@cs@x}%
\tikzset{cs/y/.store in=\tikz@cs@y}%
\tikzset{cs/z/.store in=\tikz@cs@z}%
\tikzset{cs/angle/.store in=\tikz@cs@angle}%
\tikzset{cs/x radius/.store in=\tikz@cs@xradius}%
\tikzset{cs/y radius/.store in=\tikz@cs@yradius}%
\tikzset{cs/radius/.style={/tikz/cs/x radius=#1,/tikz/cs/y radius=#1}}%
\tikzset{cs/name/.store in=\tikz@cs@node}%
\tikzset{cs/anchor/.store in=\tikz@cs@anchor}%



%
% Coordinate management
%


% Last position visited
\def\tikz@last@position{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
\def\tikz@last@position@saved{\pgfqpoint{\tikz@lastxsaved}{\tikz@lastysaved}}%

% Make given point the last position visited
\def\tikz@make@last@position#1{%
  \pgf@process{#1}%
  \tikz@lastx=\pgf@x\relax%
  \tikz@lasty=\pgf@y\relax%
  \iftikz@updatecurrent%
    \tikz@lastxsaved=\pgf@x\relax%
    \tikz@lastysaved=\pgf@y\relax%
  \fi%
  \iftikz@updatenext
    \tikz@updatecurrenttrue%
  \fi
}%

\newif\iftikz@updatecurrent
\tikz@updatecurrenttrue
\newif\iftikz@updatenext
\tikz@updatenexttrue



% Scanner: Scans a point or a relative point.
% It then calls the first parameter with the argument set to an
% appropriate pgf command representing that point.

\def\tikz@scan@one@point#1{%
  \let\tikz@to@use@whom=\tikz@to@use@last@coordinate%
  \tikz@shapeborderfalse%
  \pgfutil@ifnextchar+{\tikz@scan@relative#1}{\tikz@scan@absolute#1}}%
\def\tikz@scan@absolute#1{%
  \pgfutil@ifnextchar({\tikz@scan@@absolute#1}%)
  {%
    \advance\tikz@expandcount by -1
    \ifnum\tikz@expandcount<0\relax%
      \let\pgfutil@next=\tikz@@scangiveup%
    \else%
      \let\pgfutil@next=\tikz@@scanexpand%
    \fi%
    \pgfutil@next{#1}%
  }%
}%
\def\tikz@@scanexpand#1{\expandafter\tikz@scan@one@point\expandafter#1}%
\def\tikz@@scangiveup#1{\tikzerror{Cannot parse this coordinate}#1{\pgfpointorigin}}%
\def\tikz@scan@@absolute#1({%
  \pgfutil@ifnextchar[% uhoh... options!
  {\def\tikz@scan@point@recall{#1}\tikz@scan@options}%
  {\tikz@@@scan@@absolute#1(}%
}%

\def\tikz@scan@options[#1]#2{%
  \def\tikz@scan@point@options{#1}%
  \tikz@@@scan@@absolute\tikz@scan@handle@options(#2%
}%

\def\tikz@scan@handle@options#1{%
  {%
    % Ok, compute point with options set and zero transformation
    % matrix:
    \pgftransformreset%
    \let\tikz@transform=\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@scan@point@options}%
    \tikz@transform%
    \pgf@process{\pgfpointtransformed{#1}}%
    \xdef\tikz@marshal{\expandafter\noexpand\tikz@scan@point@recall{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  }%
  \tikz@marshal%
}%

\def\tikz@@@scan@@absolute#1({%
  \pgfutil@ifnextchar{$}%$
  {\tikz@parse@calculator#1(}
  {\tikz@scan@no@calculator#1(}%
}%
\def\tikz@scan@no@calculator#1(#2){%
  \edef\tikz@scan@point@coordinate{(#2)}%
  \expandafter\tikz@@scan@@no@calculator\expandafter#1\tikz@scan@point@coordinate%
}%
\def\tikz@@scan@@no@calculator#1(#2){%
  \pgfutil@in@{cs:}{#2}%
  \ifpgfutil@in@%
    \let\pgfutil@next\tikz@parse@coordinatesystem%
  \else%
    \pgfutil@in@{intersection }{#2}%
    \ifpgfutil@in@%
      \let\pgfutil@next\tikz@parse@intersection%
    \else%
      \pgfutil@in@|{#2}%
      \ifpgfutil@in@
        \pgfutil@in@{-|}{#2}%
        \ifpgfutil@in@
          \let\pgfutil@next\tikz@parse@hv%
        \else%
          \let\pgfutil@next\tikz@parse@vh%
        \fi%
      \else%
        \pgfutil@in@:{#2}%
        \ifpgfutil@in@
          \let\pgfutil@next\tikz@parse@polar%
        \else%
          \pgfutil@in@,{#2}%
          \ifpgfutil@in@%
            \let\pgfutil@next\tikz@parse@regular%
          \else%
            \let\pgfutil@next\tikz@parse@node%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgfutil@next#1(#2)%
}%

\def\tikz@parse@calculator#1($#2$){%
  \tikzerror{You need to say \string\usetikzlibrary{calc} for coordinate calculation}%
  #1{\pgfpointorigin}%
}%

\def\tikz@parse@coordinatesystem#1(#2 cs:#3){%
  \let\tikz@return@coordinate=\pgfpointorigin%
  \pgfutil@ifundefined{tikz@parse@cs@#2}
  {\tikzerror{Unknown coordinate system '#2'}}
  {\csname tikz@parse@cs@#2\endcsname(#3)}%
  \expandafter#1\expandafter{\tikz@return@coordinate}%
}%


\newif\iftikz@isdimension
\def\tikz@checkunit#1{%
  \pgfmathparse{#1}%
  \let\iftikz@isdimension=\ifpgfmathunitsdeclared%
}%

\def\tikz@parse@polar#1(#2:#3){%
  \pgfutil@ifundefined{tikz@polar@dir@#2}
  {\tikz@@parse@polar#1({#2}:{#3})}
  {\tikz@@parse@polar#1(\csname tikz@polar@dir@#2\endcsname:{#3})}%
}%
\def\tikz@@parse@polar#1(#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \edef\tikz@args{({#2}:#3)}%
  \else%
    \edef\tikz@args{({#2}:{#3} and {#3})}%
  \fi%
  \expandafter\tikz@@@parse@polar\expandafter#1\tikz@args%
}%
\def\tikz@@@parse@polar#1(#2:#3 and #4){%
  \tikz@checkunit{#3}%
  \iftikz@isdimension%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \def\tikz@next{#1{\pgfpointpolar{#2}{#3 and #4}}}%
    \else%
      \tikzerror{You cannot mix dimension and dimensionless values for polar coordinates}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \fi%
  \else%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \tikzerror{You cannot mix dimension and dimensionless values for polar coordinates}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \else%
      \def\tikz@next{#1{\pgfpointpolarxy{#2}{#3 and #4}}}%
    \fi%
  \fi%
  \tikz@next%
}%
\def\tikz@polar@dir@up{90}%
\def\tikz@polar@dir@down{-90}%
\def\tikz@polar@dir@left{180}%
\def\tikz@polar@dir@right{0}%
\def\tikz@polar@dir@north{90}%
\def\tikz@polar@dir@south{-90}%
\def\tikz@polar@dir@east{0}%
\def\tikz@polar@dir@west{180}%
\expandafter\def\csname tikz@polar@dir@north east\endcsname{45}%
\expandafter\def\csname tikz@polar@dir@north west\endcsname{135}%
\expandafter\def\csname tikz@polar@dir@south east\endcsname{-45}%
\expandafter\def\csname tikz@polar@dir@south west\endcsname{-135}%


% MW:
% Check to see if the y-coordinate is inside {}. If it is, scan it and
% reinsert it into the stream inside an extra group.
%
\def\tikz@parse@regular#1(#2,{%
    \pgfutil@ifnextchar\bgroup{\tikz@@parse@regular#1{#2}}{\tikz@@@parse@regular#1{#2}}%
}%
\def\tikz@@parse@regular#1#2#3{%
    \pgfutil@ifnextchar[{% Uh oh! An array index.
        \tikz@@@parse@regular#1{#2}{#3}}%
      {\tikz@@@parse@regular#1{#2}{{#3}}}}%

% Originally \def\tikz@parse@regular#1(#2,#3){%
%
\def\tikz@@@parse@regular#1#2#3){%
  \pgfutil@in@,{#3}%
  \ifpgfutil@in@%
    \tikz@parse@splitxyz{#1}{#2}#3,%
  \else%
    \tikz@checkunit{#2}%
    \iftikz@isdimension%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\pgfutil@next{#1{\pgfpoint{#2}{#3}}}%
      \else%
        \def\pgfutil@next{#1{\pgfpointadd{\pgfpoint{#2}{0pt}}{\pgfpointxy{0}{#3}}}}%
      \fi%
    \else%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\pgfutil@next{#1{\pgfpointadd{\pgfpoint{0pt}{#3}}{\pgfpointxy{#2}{0}}}}%
      \else%
        \def\pgfutil@next{#1{\pgfpointxy{#2}{#3}}}%
      \fi%
    \fi%
  \fi%
  \pgfutil@next%
}%

\def\tikz@parse@splitxyz#1#2#3,#4,{%
  \def\pgfutil@next{#1{\pgfpointxyz{#2}{#3}{#4}}}%
}%

\def\tikz@coordinate@text{coordinate}%

\def\tikz@parse@node#1(#2){%
  \pgfutil@in@.{#2}% Ok, flag this
  \ifpgfutil@in@
    \tikz@calc@anchor#2\tikz@stop%
  \else%
    \tikz@calc@anchor#2.center\tikz@stop% to be on the save side, in
                                % case iftikz@shapeborder is ignored...
    \ifcsname pgf@sh@ns@\tikz@pp@name{#2}\endcsname
      \expandafter\ifx\csname pgf@sh@ns@\tikz@pp@name{#2}\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{\tikz@pp@name{#2}}%
      \fi%
    \else\ifcsname pgf@sh@ns@#2\endcsname
      \expandafter\ifx\csname pgf@sh@ns@#2\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{#2}%
      \fi%
    \fi\fi
  \fi%
  \edef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}%

\def\tikz@calc@anchor#1.#2\tikz@stop{%
  % Check if a shape with name prefix exists, otherwise try the global name
  % without prefix.
  \ifcsname pgf@sh@ns@\tikz@pp@name{#1}\endcsname%
    \pgfpointanchor{\tikz@pp@name{#1}}{#2}%
  \else
    \pgfpointanchor{#1}{#2}%
  \fi
}%


\def\tikz@parse@hv#1(#2){%
  \pgfutil@in@{ -| }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@hvboth%
  \else%
    \pgfutil@in@{ -|}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@hvleft%
    \else%
      \pgfutil@in@{-| }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@hvright%
      \else%
        \let\tikz@next=\tikz@parse@hvdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}%
\def\tikz@parse@hvboth#1(#2 -| #3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvleft#1(#2 -|#3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvright#1(#2-| #3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvdone#1(#2-|#3){\tikz@parse@vhdone#1({#3}|-{#2})}%

\def\tikz@parse@vh#1(#2){%
  \pgfutil@in@{ |- }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@vhboth%
  \else%
    \pgfutil@in@{ |-}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@vhleft%
    \else%
      \pgfutil@in@{|- }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@vhright%
      \else%
        \let\tikz@next=\tikz@parse@vhdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}%
\def\tikz@parse@vhboth#1(#2 |- #3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhleft#1(#2 |-#3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhright#1(#2|- #3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhdone#1(#2|-#3){%
  {%
    \tikz@@@scan@@absolute\tikz@parse@vh@mid(#2)%
    \tikz@@@scan@@absolute\tikz@parse@vh@end(#3)%
    \xdef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  }%
  \tikz@marshal%
}%
\def\tikz@parse@vh@mid#1{\pgf@process{#1}\pgf@xa=\pgf@x}%
\def\tikz@parse@vh@end#1{\pgf@process{#1}\pgf@ya=\pgf@y}%

\def\tikz@parse@intersection#1(intersection{%
  \pgfutil@ifnextchar o{%
    \tikz@parse@main@intersection#1 1%
  }{%
    \tikz@parse@main@intersection#1%
  }%
}%
\def\tikz@parse@main@intersection#1#2of #3 and #4){%
  \tikzset{cs/solution=#2}%
  \pgfutil@in@{--}{#3}%
  \ifpgfutil@in@%
    \tikz@reparse@line{first}#3\pgf@stop%
  \else%
    \tikzset{cs/first node=#3}%
  \fi%
  \pgfutil@in@{--}{#4}%
  \ifpgfutil@in@%
    \tikz@reparse@line{second}#4\pgf@stop%
  \else%
    \tikzset{cs/second node=#4}%
  \fi%
  \tikz@parse@cs@intersection()% advanced hackery...
  \edef\pgf@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \pgf@marshal%
}%
\def\tikz@reparse@line#1#2--#3\pgf@stop{%
  \tikzset{cs/#1 line={(#2)--(#3)}}%
}%


\def\tikz@parse@intersection@a#1{\pgf@process{#1}\pgf@xa=\pgf@x\pgf@ya=\pgf@y}%
\def\tikz@parse@intersection@b#1{\pgf@process{#1}\pgf@xb=\pgf@x\pgf@yb=\pgf@y}%

\def\tikz@scan@relative#1+{%
  \pgfutil@ifnextchar+{\tikz@scan@plusplus#1}{\tikz@scan@oneplus#1}}%

\def\tikz@scan@plusplus#1+{%
  \def\tikz@doafter{#1}%
  \tikz@scan@absolute\tikz@add%
}%
\def\tikz@add#1{%
  \tikz@doafter{\pgfpointadd{#1}{\tikz@last@position@saved}}%
}%
\def\tikz@scan@oneplus#1{%
  \def\tikz@doafter{#1}%
  \tikz@updatecurrentfalse%
  \tikz@scan@absolute\tikz@add%
}%



%
% Quote handling
%

\let\tikz@enable@node@quotes\relax
\let\tikz@enable@edge@quotes\relax
\let\tikz@enable@pic@quotes\relax



% Loading further libraries

% Include a library file.
%
% #1 = List of names of library file.
%
% Description:
%
% This command includes a list of TikZ library files. For each file X in the
% list, the file tikzlibraryX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% If no file tikzlibraryX.code.tex exists, the file
% pgflibraryX.code.tex is tried instead. If this file, also, does not
% exist, an error message is printed.
%
% Example:
%
% \usetikzlibrary{arrows}
% \usetikzlibrary[patterns,topaths]

\def\usetikzlibrary{\pgfutil@ifnextchar[{\use@tikzlibrary}{\use@@tikzlibrary}}%}%
\def\use@tikzlibrary[#1]{\use@@tikzlibrary{#1}}%
\def\use@@tikzlibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikz@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikz@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikz@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikz@library@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname tikz@library@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \pgfutil@InputIfFileExists{tikzlibrary\pgf@temp.code.tex}{}{
        \pgfutil@IfFileExists{pgflibrary\pgf@temp.code.tex}{%
          \expandafter\usepgflibrary\expandafter{\pgf@temp}%
        }{%
          \tikzerror{I did not find the tikz library
            '\pgf@temp'. I looked for files named
            tikzlibrary\pgf@temp.code.tex and
            pgflibrary\pgf@temp.code.tex, but neither
            could be found in the current texmf trees.}
        }}%
      \catcode`\@=\csname tikz@library@#1@atcode\endcsname
      \catcode`\|=\csname tikz@library@#1@barcode\endcsname
      \catcode`\$=\csname tikz@library@#1@dollarcode\endcsname
      \fi%
    \fi
  }%
}%


% Always-present libraries:

\usetikzlibrary{topaths}%




\endinput


==> tikzlibraryarrows.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryarrows.code.tex}

\usepgflibrary{arrows}%

\endinput


==> tikzlibrarycalc.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibrarycalc.code.tex}

%
%
% Part I: The let path command
%
%


%
% Syntax: let \p{name1} = (coord), \p{name2} = (coord), ... in ...
%
% Currently (this may get more fancy in the future), the (coord)s are
% evaluated one by one. If the first evaluates to, say, (10pt,20pt),
% the macro \p{name1} is set to "10pt,20pt" (without parentheses), the
% macro \x{name1} is set to "10pt" and the macro \y{name1} is set to
% "20pt".
%
% If you use a number for {name}, you need no parentheses, so you
% could write:
%
% \draw let
%         \p1 = (1,1),
%         \p2 = ($ 2.5*(3,2) $)
%       in
%         (\x1,\x2) -- (\y1,\y2);

\def\tikz@let@command et{%
  \let\p=\tikz@cc@dop%
  \let\x=\tikz@cc@dox%
  \let\y=\tikz@cc@doy%
  \let\n=\tikz@cc@don%
  \pgfutil@ifnextchar i{\tikz@cc@stop@let}{\tikz@cc@handle@line}%
}%
\def\tikz@cc@handle@line{%
  \pgfutil@ifnextchar\p{%
    \tikz@cc@handle@coor%
  }{%
    \pgfutil@ifnextchar\n{%
      \tikz@cc@handle@num%
    }{%
      \pgfutil@ifnextchar i{%
        \tikz@cc@stop@let
      }{%
        \tikzerror{``\string\p'' or ``\string\n'' expected}%
      }%
    }%
  }%
}%
\def\tikz@cc@handle@num\n#1#2=#3{%
  \pgfmathparse{#3}%
  \expandafter\edef\csname tikz@cc@n@#1\endcsname{\pgfmathresult\ifpgfmathunitsdeclared pt\fi}
  \pgfutil@ifnextchar,{\tikz@cc@handle@nextline}{\tikz@cc@stop@let}%
}%
\def\tikz@cc@handle@coor\p#1#2={%
  \def\tikz@cc@coord@name{#1}%
  \tikz@scan@one@point\tikz@cc@dolet%
}%
\def\tikz@cc@dolet#1{%
  \pgf@process{#1}%
  \expandafter\edef\csname tikz@cc@p@\tikz@cc@coord@name\endcsname{\the\pgf@x,\the\pgf@y}%
  \expandafter\edef\csname tikz@cc@x@\tikz@cc@coord@name\endcsname{\the\pgf@x}%
  \expandafter\edef\csname tikz@cc@y@\tikz@cc@coord@name\endcsname{\the\pgf@y}%
  \pgfutil@ifnextchar,{\tikz@cc@handle@nextline}{\tikz@cc@stop@let}%
}%
\def\tikz@cc@handle@nextline,{%
  \tikz@cc@handle@line%
}%
\def\tikz@cc@stop@let in{%
  \tikz@scan@next@command%
}%

\def\tikz@cc@dop#1{\csname tikz@cc@p@#1\endcsname}%
\def\tikz@cc@dox#1{\csname tikz@cc@x@#1\endcsname}%
\def\tikz@cc@doy#1{\csname tikz@cc@y@#1\endcsname}%
\def\tikz@cc@don#1{\csname tikz@cc@n@#1\endcsname}%



%
%
% Part II: The ($...$) parser
%
%

\def\tikz@parse@calculator#1(${%$
  \def\tikz@cc@command{#1}%
  \begingroup%
    %
    % Parse main computation. It's a series of optional factors in front
    % of coordinates.
    %
    \pgf@xa=0pt% We accumulate the result in here.
    \pgf@ya=0pt%
    \tikz@cc@parse+%
}%

\def\tikz@cc@parse{%
  \pgfutil@ifnextchar${%$
    % Ok, we found the end...
    \tikz@cc@end%
  }
  {\pgfutil@ifnextchar+{%
      % Ok, we found a coordinate...
      \tikz@cc@add%
    }{%
      \pgfutil@ifnextchar-{%
        \tikz@cc@sub%
      }{%
        \tikzerror{+ or - expected}%
        \tikz@cc@end$%$
      }%
    }%
  }%
}%

%
% The end is reached with $
%
\def\tikz@cc@end$#1){%$
    \xdef\tikz@marshal{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \endgroup%
  \expandafter\tikz@cc@command\expandafter{\tikz@marshal}%
}%


%
% Another coordinate with +/-, possibly with a factor
%
\def\tikz@cc@add+{%
  \def\tikz@cc@factor{1}%
  \tikz@cc@factororcoordinate%
}%
\def\tikz@cc@sub-{%
  \def\tikz@cc@factor{-1}%
  \tikz@cc@factororcoordinate%
}%

%
% Check for a factor: If we see a (, its a coordinate...
%
\def\tikz@cc@factororcoordinate{%
  \pgfutil@ifnextchar({%)
    % Ok, found coordinate
    \tikz@cc@coordinate%
  }{%
    \tikz@cc@parse@factor%
  }%
}%

%
% ... otherwise it's a factor. It ends at ...*(
%
\def\tikz@cc@parse@factor#1*({%
  \pgfmathparse{#1*\tikz@cc@factor}%
  \let\tikz@cc@factor=\pgfmathresult%
  \tikz@cc@coordinate(%)
}%

\def\tikz@cc@coordinate{%
  \tikz@scan@absolute\tikz@cc@after@coordinate%
}%
\def\tikz@cc@after@coordinate#1{%
  \pgf@process{#1}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \tikz@cc@mid@checks%
}%


%
% A coordinate can be followed by !...!(...)
%

\def\tikz@cc@mid@checks{%
  \ifnum\the\catcode`\!=\active\relax
    \expandafter\tikz@cc@mid@checks@active
  \else
    \expandafter\tikz@cc@mid@checks@nonactive
  \fi
}%

\def\tikz@cc@mid@checks@nonactive{%
  \pgfutil@ifnextchar!{%
    \tikz@cc@mid@nonactive%
  }{%
    \advance\pgf@xa by\tikz@cc@factor\pgf@xb
    \advance\pgf@ya by\tikz@cc@factor\pgf@yb
    \tikz@cc@parse%
  }%
}%

\def\tikz@cc@mid@nonactive!{%
  \pgfutil@ifnextchar({%
    \tikz@scan@one@point\tikz@cc@project%
  }{%
    \tikz@cc@mid@num@nonactive%
  }%
}%

\begingroup
  \catcode`\!=\active
  \gdef\tikz@cc@mid@checks@active{%
    \pgfutil@ifnextchar!{%
      \tikz@cc@mid@active%
    }{%
      \advance\pgf@xa by\tikz@cc@factor\pgf@xb
      \advance\pgf@ya by\tikz@cc@factor\pgf@yb
      \tikz@cc@parse%
    }%
  }%

  \gdef\tikz@cc@mid@active!{%
    \pgfutil@ifnextchar({%
      \tikz@scan@one@point\tikz@cc@project%
    }{%
      \tikz@cc@mid@num@active%
    }%
  }%
\endgroup

%
% Partway case: (coord a)!number!(coord b)
%
% Returns the position that is at <number> fraction on the way from a
% to b. This, (a)!0!(b) is (a), (a)!.5!(b) is the middle and (a)!1!(b)
% is (b)
%

\def\tikz@cc@mid@num@nonactive#1!{\tikz@cc@mid@num{#1}}%

\begingroup
  \catcode`\!=\active
  \gdef\tikz@cc@mid@num@active#1!{\tikz@cc@mid@num{#1}}%
\endgroup

\def\tikz@cc@mid@num#1{%
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared%
    \let\tikz@cc@mid@unit=\pgfmathresult%
    \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@unit%
  \else%
    \let\tikz@cc@mid@factor=\pgfmathresult%
    \pgfmathparse{1-\tikz@cc@mid@factor}%
    \let\tikz@cc@mid@factor@one=\pgfmathresult%
    \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@num%
  \fi%
}%

\def\tikz@cc@after@num#1{%
  \pgf@process{#1}%
  \pgf@xb=\tikz@cc@mid@factor@one\pgf@xb%
  \pgf@yb=\tikz@cc@mid@factor@one\pgf@yb%
  \advance\pgf@xb by\tikz@cc@mid@factor\pgf@x%
  \advance\pgf@yb by\tikz@cc@mid@factor\pgf@y%
  \tikz@cc@mid@checks%
}%



%
% Distance case: (coord a)!dimension!(coord b)
%
% Returns the position that is at <dimension> removed from (coord a)
% in the direction of (coord b).
%

\def\tikz@cc@after@unit#1{%
  \pgf@process{#1}%
  \advance\pgf@x by-\pgf@xb%
  \advance\pgf@y by-\pgf@yb%
  \pgf@process{\pgfpointnormalised{}}%
  \advance\pgf@xb by\tikz@cc@mid@unit\pgf@x%
  \advance\pgf@yb by\tikz@cc@mid@unit\pgf@y%
  \tikz@cc@mid@checks%
}%

%
% Projection case: (a)!(p)!(b)
%
% Projection of p on line from a to b
%
\def\tikz@cc@project#1{%
  \pgf@process{#1}%
  % Save in c
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \begingroup
    \ifnum\the\catcode`\!=\active
      \def\tikz@next{%
        \endgroup
        \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@project
        \tikz@cc@scan@ex@active}%
    \else
      \def\tikz@next{%
        \endgroup
        \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@project
        \tikz@cc@scan@ex@nonactive}%
    \fi
    \tikz@next%
}%

\def\tikz@cc@scan@ex@nonactive!{}%

\begingroup
  \catcode`\!=\active
  \gdef\tikz@cc@scan@ex@active!{}%
\endgroup

\def\tikz@cc@after@project#1{%
  \pgf@process{#1}%
  % Ok, now we need to project (xc,yc) on the line (xb,xc) to (x,y)
  \advance\pgf@x by-\pgf@xb%
  \advance\pgf@y by-\pgf@yb%
  \advance\pgf@xc by-\pgf@xb%
  \advance\pgf@yc by-\pgf@yb%
  \pgf@process{\pgfpointnormalised{}}%
  % Scalar product
  \pgf@xc=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
  \advance\pgf@xc by\pgf@sys@tonumber{\pgf@yc}\pgf@y%
  % and add
  \advance\pgf@xb by\pgf@sys@tonumber{\pgf@xc}\pgf@x%
  \advance\pgf@yb by\pgf@sys@tonumber{\pgf@xc}\pgf@y%
  \tikz@cc@mid@checks%
}%

%
% Rotational scanner: radius:(x)
%

\def\tikz@cc@scan@rot#1{%
  \pgfutil@ifnextchar({%)
    \tikz@scan@one@point#1% normal
  }%
  {%
    \def\tikz@cc@scan@rot@cmd{#1}%
    \ifnum\the\catcode`\:=\active\relax
      \expandafter\tikz@cc@scan@one@rot@active%
    \else
      \expandafter\tikz@cc@scan@one@rot@nonactive%
    \fi
  }%
}%

\def\tikz@cc@scan@one@rot@nonactive#1:{%
  \def\tikz@cc@scan@rot@angle{#1}%
  \tikz@scan@one@point\tikz@cc@handle@rot%
}%

\begingroup
  \catcode`\:=\active
  \gdef\tikz@cc@scan@one@rot@active#1:{%
    \def\tikz@cc@scan@rot@angle{#1}%
    \tikz@scan@one@point\tikz@cc@handle@rot%
  }%
\endgroup

\def\tikz@cc@handle@rot#1{%
  \pgf@process{#1}%
  % Ok, now we need to rotate x/y around xb/xb by ...rot@angle
  {%
    \pgftransformreset%
    % Save them...
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgftransformshift{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
    \pgftransformrotate{\tikz@cc@scan@rot@angle}%
    \pgftransformshift{\pgfqpoint{-\pgf@xb}{-\pgf@yb}}%
    \pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
    \expandafter
  }%
  \edef\tikz@marshal{\noexpand\tikz@cc@scan@rot@cmd{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}%




%
%
% Part III: Calculation coordinate systems
%
%

% Tangent cs: Keys are a node and a point. Depending on the type of
% node, the appropriate tangent computation should be done.

\tikzdeclarecoordinatesystem{tangent}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\ifx\csname tikz@tangent@\tikz@cs@type\endcsname\relax%
    \tikzerror{I do not know how to compute the tangent to
    a \tikz@cs@type}%
    \pgfpointorigin%
  \else%
    \expandafter\tikz@scan@one@point\expandafter\tikz@lib@do@tangent\tikz@cs@point%
  \fi%
}%

\tikzset{cs/node/.code=\tikz@cs@unpack{\tikz@cs@node}{\tikz@cs@type}{#1}}%
\tikzset{cs/point/.store in=\tikz@cs@point}%

\def\tikz@lib@do@tangent{\csname tikz@tangent@\tikz@cs@type\endcsname}%

\def\tikz@tangent@coordinate#1{%
  \pgfpointanchor{\tikz@cs@node}{center}%
}%

\def\tikz@tangent@circle#1{%
  {%
    % Step 1: Compute the transformed position of the input:
    \pgf@process{\pgfpointtransformed{#1}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    %
    % Step 2: Compute vector from center of circle to transformed #1
    %
    \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikz@cs@node}{center}}}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    %
    % Step 2: Reset transformations, they distract...
    %
    \pgftransformreset%
    %
    % Step 3: Transform to the center of the circle.
    %
    \pgftransformshift{\pgfpointanchor{\tikz@cs@node}{center}}%
    %
    % Step 4: Compute the radius
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node}{east}}%
    \pgf@xc=\pgf@x%
    %
    % Now, (xa,ya) is a point. Compute the tangent from this point to
    % a circle around the origin of radius xc.
    %
    % acos(radius/veclen(xa,ya)) is the angle of the tangent.
    \pgfmathparse{veclen(\the\pgf@xa,\the\pgf@ya)}
    \pgfmathparse{acos(\the\pgf@xc/\pgfmathresult)}
    \ifnum\pgfkeysvalueof{/tikz/cs/solution}>1\relax%
      \pgfmathparse{0-\pgfmathresult}%
    \fi%
    \let\tikz@lib@temp=\pgfmathresult%
    %
    % Now \pgfmathparse contains the desired angle. Use this to
    % compute the correct position on the circle...
    %
    % But, first, rotate to the point.
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \pgf@ya=-\pgf@y%
    \pgftransformcm{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
    % Finally, rotate...
    \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@lib@temp}{\the\pgf@xc}}}%
    %
    % Ok, undo transformations...
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}%


% Implementation of intersections


\def\tikz@intersect@circle@and@circle{%
  {%
    \pgftransformreset% transformations only confuse us, here...
    %
    % Compute origin and radius of first circle
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@a}{center}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointanchor{\tikz@cs@node@a}{east}}%
    \advance\pgf@x by-\pgf@xa%
    \pgf@xc=\pgf@x% ok, pgf@xc is first radius, (xa,ya) is center
    %
    % Compute origin and radius of second circle
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{center}}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{east}}%
    \advance\pgf@x by-\pgf@xb%
    \pgf@yc=\pgf@x% \pgf@yc is second radius, (xb,yb) is center
    %
    \pgf@process{%
      \pgfpointintersectionofcircles{\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\pgf@xb}{\pgf@yb}}{\pgf@xc}{\pgf@yc}{\pgfkeysvalueof{/tikz/cs/solution}}%
    }%
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process,
  % reinstall transformations...
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}%


\def\tikz@intersect@line@and@circle{%
  {%
    %
    % Step 1: Get line
    %
    \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@a%
    \pgf@process{\pgfpointtransformed{}}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{\pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    %
    % Step 2: Subtract center of circle
    %
    \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikz@cs@node@b}{center}}}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    %
    % Step 3: Reset transformations, they distract...
    %
    \pgftransformreset%
    %
    % Step 4: Transform to the center of the circle.
    %
    \pgftransformshift{\pgfpointanchor{\tikz@cs@node@b}{center}}%
    %
    % Step 5: Compute the radius
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{east}}%
    \edef\tikz@lib@saved@radius{\pgf@sys@tonumber{\pgf@x}}%
    %
    % Step 6: Compute projection of origin on line (xa,ya) -- (xb,yb),
    % store in (xa,ya)
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@process{\pgfpointnormalised{}}%
    % Scalar product
    \pgf@xc=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \advance\pgf@xc by\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \pgf@xc=-\pgf@xc%
    % and add
    \advance\pgf@xa by\pgf@sys@tonumber{\pgf@xc}\pgf@x%
    \advance\pgf@ya by\pgf@sys@tonumber{\pgf@xc}\pgf@y%
    %
    % Now, we have a triangle with a right angle at (xa,ya). The
    % second point of the triangle is the origin. The third point is
    % sought.
    % Save x/y
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    % Square radius
    \pgf@xb=\tikz@lib@saved@radius pt%
    %
    % First, make numbers smaller, in case they are too large
    %
    \c@pgf@counta=1\relax%
    \loop%
    \ifdim\pgf@xb>50pt%
      \multiply\c@pgf@counta by2\relax%
      \divide\pgf@xa by2\relax%
      \divide\pgf@ya by2\relax%
      \divide\pgf@xb by2\relax%
    \repeat%
    \pgf@xb=\pgf@sys@tonumber{\pgf@xb}\pgf@xb%
    % Subtract xa^2 + ya^2
    \pgf@yb=\pgf@sys@tonumber{\pgf@xa}\pgf@xa%
    \advance\pgf@xb by-\pgf@yb%
    \pgf@yb=\pgf@sys@tonumber{\pgf@ya}\pgf@ya%
    \advance\pgf@xb by-\pgf@yb%
    % Square root
    \ifdim\pgf@xb<0pt%
      \pgf@xb=0pt%
    \fi%
    \pgfmathsqrt@{\pgf@sys@tonumber{\pgf@xb}}%
    \pgfmathmultiply@{\pgfmathresult}{\the\c@pgf@counta}%
    \multiply\pgf@xa by\c@pgf@counta\relax%
    \multiply\pgf@ya by\c@pgf@counta\relax%
    \ifnum\pgfkeysvalueof{/tikz/cs/solution}>1\relax%
      \pgfmathsubtract{0}{\pgfmathresult}%
    \fi%
    % Ok, now add things...
    \advance\pgf@xa by \pgfmathresult\pgf@xc%
    \advance\pgf@ya by \pgfmathresult\pgf@yc%
    \pgf@process{\pgfpointtransformed{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    % Ok, undo transformations...
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}%

\def\tikz@intersect@circle@and@line{%
  % Swap
  {%
    \let\tikz@cs@node@b=\tikz@cs@node@a%
    \let\tikz@cs@line@a=\tikz@cs@line@b%
    \tikz@intersect@line@and@circle%
  }%
}%


==> tikzlibrarycd.code.tex <==
% tikzlibrarycd.code.tex [2018/11/19 v0.9f Commutative diagrams with TikZ]
%
% Copyright 2011, 2012, 2014, 2018 by Augusto Stoffel
%
% This program is free software: you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation, either version 3 of the License, or
% (at your option) any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
% 
% You should have received a copy of the GNU General Public License
% along with this program.  If not, see <http://www.gnu.org/licenses/>.

\usetikzlibrary{matrix,quotes,arrows.meta}

\newif\iftikzcd@mathmode

\def\tikzcdset{\pgfqkeys{/tikz/commutative diagrams}}

\tikzcdset{
  arrows/.code={\tikzcdset{every arrow/.append style={#1}}},
  labels/.code={\tikzcdset{every label/.append style={#1}}},
  cells/.code={\tikzcdset{every cell/.append style={#1}}},
  diagrams/.code={\tikzcdset{every diagram/.append style={#1}}},
  execute before arrows/.code={%
    \expandafter\def%
    \expandafter\tikzcd@before@paths@hook%
    \expandafter{\tikzcd@before@paths@hook#1}},
  to/.code={\tikzcd@setarrowend\tikzcd@ar@target{#1}},
  from/.code={\tikzcd@setarrowend\tikzcd@ar@start{#1}},
  shorten/.style={
    /tikz/shorten <=#1,
    /tikz/shorten >=#1},
  description/.style={
    /tikz/anchor=center,
    /tikz/fill=\pgfkeysvalueof{/tikz/commutative diagrams/background color}},
  marking/.style={
    /tikz/font=,
    /tikz/sloped,
    /tikz/shape=asymmetrical rectangle,
    /tikz/anchor=center},
  phantom/.style={
    /tikz/draw=none,
    /tikz/commutative diagrams/labels={
      /tikz/font=,
      /tikz/anchor=center}},
  crossing over/.style={
    /tikz/preaction={
      /tikz/draw=\pgfkeysvalueof{/tikz/commutative diagrams/background color},
      /tikz/arrows=-,
      /tikz/line width=\pgfkeysvalueof{/tikz/commutative diagrams/crossing over clearance}}},
  cramped/.code={\tikzcdset{
    every matrix/.append style={inner sep=+-0.3em},
    every cell/.append style={inner sep=+0.3em}}},
  row sep/.code={\tikzcd@sep{row}{#1}},
  column sep/.code={\tikzcd@sep{column}{#1}},
  sep/.code={\tikzcdset{row sep={#1},column sep={#1}}},
  math mode/.is if=tikzcd@mathmode,
  arrow style/.is choice}

\def\tikzcd@sep#1#2{%
  \pgfkeysifdefined{/tikz/commutative diagrams/#1 sep/#2}%
    {\pgfkeysgetvalue{/tikz/commutative diagrams/#1 sep/#2}\tikzcd@temp%
     \pgfkeysalso{/tikz/#1 sep/.expand once=\tikzcd@temp}}%
    {\pgfkeysalso{/tikz/#1 sep={#2}}}}

\def\tikzcd@setarrowend#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@\tikzcdmatrixname-#2}%
    {%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp#2\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef#1{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \def#1{#2}%
      \fi%
    }{%
      \def#1{\tikzcdmatrixname-#2}%
    }}
    
% The unknown key handler and direction argument parser
\tikzcdset{
  .unknown/.code={%
    \ifpgfkeysaddeddefaultpath%
      \c@pgf@counta=0%
      \c@pgf@countb=0%
      \let\tikzcd@temp=\tikzcd@parse%
      \expandafter\tikzcd@temp\pgfkeyscurrentname\relax%
      \ifx\tikzcd@temp\pgfutil@empty% true if it was a direction parameter
        \advance\c@pgf@counta by\tikzcd@currentrow%
        \advance\c@pgf@countb by\tikzcd@currentcolumn%
        \edef\tikzcd@ar@target{\tikzcdmatrixname-\the\c@pgf@counta-\the\c@pgf@countb}%
      \else%
        \pgfqkeys{/tikz}{\pgfkeyscurrentname={#1}}%
      \fi%
    \else%
      \def\pgfutilnext{\pgfkeysvalueof{/handlers/.unknown/.@cmd}#1\pgfeov}\pgfutilnext%
    \fi}}

\def\tikzcd@parse#1{% parser for arrow direction argument
  \ifx#1r\advance\c@pgf@countb by1\else%
   \ifx#1d\advance\c@pgf@counta by1\else%
    \ifx#1l\advance\c@pgf@countb by-1\else%
     \ifx#1u\advance\c@pgf@counta by-1\else%
      \ifx#1\relax\let\tikzcd@temp\pgfutil@empty%
       \else\let\tikzcd@temp\pgfutil@gobble@until@relax\fi\fi\fi\fi\fi%
  \tikzcd@temp}

% The `tikzcd' environment
\def\tikzcd{%
  \iffalse{\fi\ifnum0=`}\fi% standard trick to allow nesting of tabular-like environments (cf. the tabularx manual)
  \pgfutil@ifnextchar&% if we get an & here, it will be returned with the wrong catcode to the input stream
    {\expandafter\tikzcd@@\expandafter\pgfmatrixnextcell\pgfutil@gobble}%
    {\tikzcd@@}}

\def\tikzcd@@{\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@}{\tikzcd@[]}}

\def\tikzcd@[#1]{%
  \tikzpicture[/tikz/commutative diagrams/.cd,every diagram,#1]%
  \ifx\arrow\tikzcd@arrow%
    \pgfutil@packageerror{tikz-cd}{Diagrams cannot be nested}{}%
  \fi%
  \let\arrow\tikzcd@arrow%
  \let\ar\tikzcd@arrow%
  \def\rar{\tikzcd@xar{r}}%
  \def\lar{\tikzcd@xar{l}}%
  \def\dar{\tikzcd@xar{d}}%
  \def\uar{\tikzcd@xar{u}}%
  \def\urar{\tikzcd@xar{ur}}%
  \def\ular{\tikzcd@xar{ul}}%
  \def\drar{\tikzcd@xar{dr}}%
  \def\dlar{\tikzcd@xar{dl}}%
  \global\let\tikzcd@savedpaths\pgfutil@empty%
  \matrix[%
    /tikz/matrix of \iftikzcd@mathmode math \fi nodes,%
    /tikz/every cell/.append code={\tikzcdset{every cell}},%
    /tikz/commutative diagrams/.cd,every matrix]%
  \bgroup}

\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths%
  \endgroup%
  \endtikzpicture%
  \ifnum0=`{}\fi}

% The arrow commands
\def\tikzcd@arrow{%
  \relax% this was added to avoid errors when a cell starts with \arrow, but it seems unnecessary now
  \edef\tikzcd@temp{%
    \noexpand\def\noexpand\tikzcd@currentcolumn{\the\pgfmatrixcurrentcolumn}%
    \noexpand\def\noexpand\tikzcd@currentrow{\the\pgfmatrixcurrentrow}%
    \noexpand\def\noexpand\tikzcd@lineno{\the\inputlineno}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@savedpaths\expandafter{\tikzcd@temp}%
  \pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@arrow}{\tikzcd@ar@old[]}}

\def\tikzcd@@arrow[#1]{\pgfutil@ifnextchar\bgroup{\tikzcd@ar@old[#1]}{\tikzcd@ar@new[#1]}}

\def\tikzcd@ar@new[#1]{% new syntax
  \pgfutil@g@addto@macro\tikzcd@savedpaths{%
    \path[/tikz/commutative diagrams/.cd,every arrow,#1]%
    (\tikzcd@ar@start\tikzcd@startanchor) to (\tikzcd@ar@target\tikzcd@endanchor); }}

\def\tikzcd@ar@old[#1]#2{% old syntax
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{to={#2},#1}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{to={#2},#1}[]}%
      {\tikzcd@ar@new[to={#2},#1]}}}

\def\tikzcd@ar@getlabel#1[#2]#3{%
  \pgfutil@ifnextchar[%
    {\tikzcd@handle@shortcuts@next\tikzcd@ar@getlabel{#1,"{#3}"{#2}}}%
    {\pgfutil@ifnextchar\bgroup%
      {\tikzcd@ar@getlabel{#1,"{#3}"{#2}}[]}%
      {\tikzcd@ar@new[#1,"{#3}"{#2}]}}}

\def\tikzcd@xar#1{\relax\pgfutil@ifnextchar[{\tikzcd@handle@shortcuts@next\tikzcd@@xar{#1}}{\tikzcd@arrow[]{#1}}}
\def\tikzcd@@xar#1[#2]{\tikzcd@arrow[#2]{#1}}

\def\tikzcd@handle@shortcuts@next{% expand next macro using standard catcodes
  \iftikz@handle@active@code%
    \begingroup%
      \tikz@switchoff@shorthands\expandafter%
    \endgroup\expandafter%
  \fi}

\def\tikzcd@ar@target{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}
\def\tikzcd@ar@start{\tikzcdmatrixname-\tikzcd@currentrow-\tikzcd@currentcolumn}

\def\tikzcd@forward@quotes#1{\tikzset{every to/.append style={#1}}}

\let\tikzcd@before@paths@hook\pgfutil@empty

% `start anchor', `end anchor', and `shift' keys
\def\tikzcd@setanchor#1[#2]#3\relax{%
  \ifx\relax#2\relax\else%
    \tikzcdset{@#1transform/.append style={#2},@shiftabletopath}%
  \fi%
  \ifx\relax#3\relax%
    \pgfutil@namelet{tikzcd@#1anchor}{pgfutil@empty}%
  \else%
    \pgfutil@namedef{tikzcd@#1anchor}{.#3}%
  \fi}

\tikzcdset{
  @shiftabletopath/.style={
    /tikz/execute at begin to={%
      \begingroup%
        \def\tikz@tonodes{coordinate[pos=0,commutative diagrams/@starttransform/.try](tikzcd@nodea) %
                          coordinate[pos=1,commutative diagrams/@endtransform/.try](tikzcd@nodeb)}%
        \path (\tikztostart) \tikz@to@path;%
      \endgroup%
      \def\tikztostart{tikzcd@nodea}%
      \def\tikztotarget{tikzcd@nodeb}%
      \tikzset{insert path={(tikzcd@nodea)}}},
    /tikz/commutative diagrams/@shiftabletopath/.code={}},
  start anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{start}}{\tikzcd@setanchor{start}[]}#1\relax},%]
  end anchor/.code={%
    \pgfutil@ifnextchar[{\tikzcd@setanchor{end}}{\tikzcd@setanchor{end}[]}#1\relax},%]
  start anchor=,
  end anchor=,
  shift left/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/execute at begin to={%
      \pgfpointnormalised{%
        \pgfpointdiff{\pgfpointanchor{tikzcd@nodeb}{center}}{\pgfpointanchor{tikzcd@nodea}{center}}}%
      \pgfgetlastxy{\tikzcd@x}{\tikzcd@y}%
      \pgfmathparse{#1}%
      \ifpgfmathunitsdeclared\else
        \pgfmathparse{\pgfmathresult*\pgfkeysvalueof{/tikz/commutative diagrams/shift left/.@def}}
      \fi
      \coordinate (tikzcd@nodea) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodea);%
      \coordinate (tikzcd@nodeb) at ([shift={(\pgfmathresult*\tikzcd@y,-\pgfmathresult*\tikzcd@x)}]tikzcd@nodeb);%
      \tikzset{insert path={(tikzcd@nodea)}}}},
  shift right/.style={
    /tikz/commutative diagrams/shift left={-(#1)}},
  transform nodes/.style={
    /tikz/commutative diagrams/@shiftabletopath,
    /tikz/commutative diagrams/@starttransform/.append style={#1},
    /tikz/commutative diagrams/@endtransform/.append style={#1}},
  shift/.style={
    /tikz/shift={#1},% we need this for labels to receive a shift
    /tikz/commutative diagrams/transform nodes={/tikz/shift={#1}}},
  xshift/.style={
    /tikz/xshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/xshift={#1}}},
  yshift/.style={
    /tikz/yshift={#1},
    /tikz/commutative diagrams/transform nodes={/tikz/yshift={#1}}}}

% pgfmath functions to obtain math fontdimens
\pgfutil@ifluatex

  \directlua{tex.enableprimitives('tikzcd@', {'Umathaxis', 'Umathfractionrule'})}

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\tikzcd@Umathaxis\textstyle%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\tikzcd@Umathfractionrule\textstyle%
    \endgroup}

\else% if using (pdf)tex

  \pgfmathdeclarefunction{axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      \pgfmathreturn\the\fontdimen22\textfont2%
    \endgroup}

  \pgfmathdeclarefunction{rule_thickness}{0}{%
    \begingroup%
      $\relax$%
      \pgfmathreturn\the\fontdimen8\textfont3%
    \endgroup}

\fi

% The shape used inside matrices
\pgfdeclareshape{asymmetrical rectangle} {
  \inheritsavedanchors[from={rectangle}]
  \inheritanchor[from={rectangle}]{base}
  \inheritanchor[from={rectangle}]{north}
  \inheritanchor[from={rectangle}]{south}
  \inheritanchor[from={rectangle}]{base west}
  \inheritanchor[from={rectangle}]{north west}
  \inheritanchor[from={rectangle}]{south west}
  \inheritanchor[from={rectangle}]{base east}
  \inheritanchor[from={rectangle}]{north east}
  \inheritanchor[from={rectangle}]{south east}
  \inheritanchor[from={rectangle}]{mid}
  \inheritanchor[from={rectangle}]{mid west}
  \inheritanchor[from={rectangle}]{mid east}
  \inheritbackgroundpath[from={rectangle}]
  \anchor{center}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{west}{\pgf@anchor@rectangle@west\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{east}{\pgf@anchor@rectangle@east\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}}
  \anchor{real center}{\pgf@anchor@rectangle@center}
  \anchor{real west}{\pgf@anchor@rectangle@west}
  \anchor{real east}{\pgf@anchor@rectangle@east}
  \anchorborder{%
    \pgfmathsetlength\pgfutil@tempdima%
      {\pgfkeysvalueof{/tikz/commutative diagrams/center yshift}}%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \ifdim\pgf@yb>0pt%
      \northeast%
      \pgf@yc=\pgf@y%
      \advance\pgf@yc by-\pgfutil@tempdima%
    \else%
      \southwest%
      \pgf@yc=-\pgf@y%
      \advance\pgf@yc by\pgfutil@tempdima%
    \fi
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgfutil@tempdima%
  }%
}%

% Computer modern arrow tips
\pgfkeys{
  cm to/.tip={Computer Modern Rightarrow[length=+0pt 6.2]},
  cm bold to/.tip={cm to[scale=0.667]},
  cm double to/.tip={cm to[sep=+0pt -2.6]cm to},
  cm bar/.tip={Bar[width=+0pt 8.2 0.89,line cap=round]},
  cm left hook/.tip={Hooks[width=+0pt 10.8,length=+0pt 3.6,harpoon,line cap=round]},
  cm implies/.tip={Implies},
  cm left to/.tip={cm to[left]},
  cm right to/.tip={cm to[right]},
  cm right hook/.tip={cm left hook[swap]},
  cm to reversed/.tip={cm to[reversed]},
  cm */.tip={Circle[length=+0pt 7.6]},
  cm o/.tip={cm *[open]},
  cm |/.tip={cm bar}}%|

% The `Glyph' meta arrow tip
\pgfqkeys{/pgf/arrow keys}{
  glyph math command/.code={% if csname #1 is undefined, we want it to remain so
    \pgfarrowsaddtooptions{\def\tikzcd@glyph{$\begingroup\expandafter\endgroup\csname #1\endcsname$}}},
  glyph axis/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@axis{#1}}},
  glyph length/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@len{#1}}},
  glyph shorten/.code={\pgfarrowsaddtooptions{\pgfmathsetlengthmacro\tikzcd@glyph@shorten{#1}}}}

\pgfdeclarearrow{
  name=Glyph,
  cache=false,
  bending mode=none,
  parameters={\tikzcd@glyph@len,\tikzcd@glyph@shorten},
  setup code={%
    \pgfarrowssettipend{\tikzcd@glyph@len\advance\pgf@x by\tikzcd@glyph@shorten}},
  defaults={
    glyph axis=axis_height,
    glyph length=+0.9ex,
    glyph shorten=+-0.1ex},
  drawing code={%
    \pgfpathrectangle{\pgfpoint{+0pt}{+-1ex}}{\pgfpoint{+\tikzcd@glyph@len}{+2ex}}%
    \pgfusepathqclip%
    \pgftransformxshift{+\tikzcd@glyph@len}%
    \pgftransformyshift{+-\tikzcd@glyph@axis}%
    \pgftext[right,base]{\tikzcd@glyph}}}

% Arrow tip selection styles
\tikzcdset{
  double line/.code={\tikzset{%
    double equal sign distance,
    double=\pgfkeysvalueof{/tikz/commutative diagrams/background color}}},
  dashed/.style={/tikz/dash pattern={on 7\pgflinewidth off 4\pgflinewidth}},
  tikzcd to/.tip={cm to},
  tikzcd bar/.tip={cm bar},
  tikzcd left hook/.tip={cm left hook},
  tikzcd double to/.tip={cm double to},
  tikzcd implies/.tip={Implies},
  tikzcd right hook/.tip={tikzcd left hook[swap]},
  tikzcd left to/.tip={tikzcd to[harpoon]},
  tikzcd right to/.tip={tikzcd left to[swap]},
  tikzcd to reversed/.tip={tikzcd to[reversed]},
  tikzcd cap/.tip={},
  tikzcd implies cap/.tip={},
  tikzcd implies bar/.tip={tikzcd bar},
  no tail/.code={\pgfsetarrowsstart{tikzcd cap}},
  to head/.code={\pgfsetarrowsend{tikzcd to}},
  maps to/.code={\pgfsetarrowsstart{tikzcd bar}},
  hook/.code={\pgfsetarrowsstart{tikzcd right hook}},
  hook'/.code={\pgfsetarrowsstart{tikzcd left hook}},
  harpoon/.code={\pgfsetarrowsend{tikzcd left to}},
  harpoon'/.code={\pgfsetarrowsend{tikzcd right to}},
  two heads/.code={\pgfsetarrowsend{tikzcd double to}},
  tail/.code={\pgfsetarrowsstart{tikzcd to reversed}},
  rightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd to}},
  Rightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies}},
  leftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd cap}},
  Leftarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies cap}},
  leftrightarrow/.code={\pgfsetarrows{tikzcd to-tikzcd to}},
  Leftrightarrow/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies}},
  mapsto/.code={\pgfsetarrows{tikzcd bar-tikzcd to}},
  mapsfrom/.code={\pgfsetarrows{tikzcd to-tikzcd bar}},
  Mapsto/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies bar-tikzcd implies}},
  Mapsfrom/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies-tikzcd implies bar}},
  hookrightarrow/.code={\pgfsetarrows{tikzcd right hook-tikzcd to}},
  hookleftarrow/.code={\pgfsetarrows{tikzcd to-tikzcd left hook}},
  rightharpoonup/.code={\pgfsetarrows{tikzcd cap-tikzcd left to}},
  rightharpoondown/.code={\pgfsetarrows{tikzcd cap-tikzcd right to}},
  leftharpoonup/.code={\pgfsetarrows{tikzcd right to-tikzcd cap}},
  leftharpoondown/.code={\pgfsetarrows{tikzcd left to-tikzcd cap}},
  rightarrowtail/.code={\pgfsetarrows{tikzcd to reversed-tikzcd to}},
  leftarrowtail/.code={\pgfsetarrows{tikzcd to-tikzcd to reversed}},
  twoheadrightarrow/.code={\pgfsetarrows{tikzcd cap-tikzcd double to}},
  twoheadleftarrow/.code={\pgfsetarrows{tikzcd double to-tikzcd cap}},
  no head/.code={\pgfsetarrowsend{tikzcd cap}},
  dash/.code={\pgfsetarrows{tikzcd cap-tikzcd cap}},
  dashrightarrow/.code={\tikzcdset{rightarrow,dashed}},
  dashleftarrow/.code={\tikzcdset{leftarrow,dashed}},
  equal/.code={\tikzcdset{double line}\pgfsetarrows{tikzcd implies cap-tikzcd implies cap}},
  equals/.code={\tikzcdset{equal}},
  rightsquigarrow/.code={\tikzcdset{rightarrow,squiggly}},
  leftsquigarrow/.code={\tikzcdset{leftarrow,squiggly}},
  leftrightsquigarrow/.code={\tikzcdset{leftrightarrow,squiggly}},
  squiggly/.code={%
    \pgfutil@ifundefined{tikz@library@decorations.pathmorphing@loaded}%
      {\pgfutil@packageerror{tikz-cd}{You need to say %
      \string\usetikzlibrary{decorations.pathmorphing} to use squiggly arrows}{}}{}%
    \pgfkeysalso{
      /tikz/decorate,
      /tikz/decoration={
        zigzag,
        segment length=9.25\pgflinewidth,
        amplitude=1.9\pgflinewidth,
        post=lineto, post length=6\pgflinewidth,
        pre=lineto, pre length=6\pgflinewidth,
        #1}}}}

% The `Latin Modern' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/Latin Modern}{%
  \tikzcdset{
    tikzcd bar/.tip={Bar[width=+0pt 12 .992,line cap=round]},
    tikzcd left hook/.tip={Hooks[width=+0pt 15,length=+0pt 4.2,arc=190,harpoon,line cap=round]}}}

% The `tikz' arrow style
\pgfkeysdef{/tikz/commutative diagrams/arrow style/tikz}{%
  \tikzcdset{
    tikzcd to/.tip={>},
    tikzcd bar/.tip={Bar[width=+3pt 4 0.9]},
    tikzcd left hook/.tip={Hooks[harpoon]},
    tikzcd double to/.tip={tikzcd to[]tikzcd to}}}

% The `math font' arrow style
%
% If your font does not define the command \mapsfrom, do so by saying
%   \def\mapsfrom{\pgfpicture\pgfsetbaseline{+0pt}\pgftransformxscale{-1}\pgftext[base]{$\mapsto$}\endpgfpicture}
%
% The method used to guess the correct value of `double distance'
% inside the `double line' style is not robust at all.  If it fails,
% set
%   \tikzcdset{double line/.append style={double distance=2*rule_thickness}}
% and find the correct value for `double distance' by trial and error
% (or measure the distance between the \Rightarrow stems in a font
% editor).
%
\pgfkeysdef{/tikz/commutative diagrams/arrow style/math font}{%
  \tikzcdset{
    tikzcd to/.tip={Glyph[glyph math command=rightarrow]},
    tikzcd cap/.tip={Glyph[glyph math command=leftarrow]},
    tikzcd to reversed/.tip={Glyph[glyph math command=leftarrowtail]},
    tikzcd bar/.tip={Glyph[glyph math command=mapsfrom]},
    tikzcd left hook/.tip={Glyph[glyph math command=hookleftarrow]},
    tikzcd right hook/.tip={Glyph[glyph math command=hookleftarrow, swap]},
    tikzcd implies/.tip={Glyph[glyph math command=Rightarrow, glyph length=1.2ex]},
    tikzcd implies cap/.tip={Glyph[glyph math command=Leftarrow]},
    tikzcd implies bar/.tip={Glyph[glyph math command=Mapsfrom]},
    tikzcd double to/.tip={Glyph[glyph math command=twoheadrightarrow, glyph length=1.4ex]},
    tikzcd left to/.tip={Glyph[glyph math command=rightharpoonup]},
    tikzcd right to/.tip={Glyph[glyph math command=rightharpoonup,swap]},
    double line/.append code={\tikzset{double distance={2*(height("$=$")-axis_height-rule_thickness)}}},
    dashed/.code={\tikzset{dash pattern=on 0.8ex off 0.4ex, dash phase=0.8ex}},
    squiggly/.default={pre length=1ex, post length=1ex}}}

% Default settings
\tikzcdset{
  every arrow/.style={
    /tikz/draw,
    /tikz/line width=rule_thickness,
    /tikz/commutative diagrams/rightarrow},
  every label/.style={
    /tikz/auto,
    /tikz/font=\everymath\expandafter{\the\everymath\scriptstyle},
    /tikz/inner sep=+0.5ex},
  every cell/.style={
    /tikz/shape={asymmetrical rectangle},
    /tikz/inner xsep=+1ex,
    /tikz/inner ysep=+0.85ex},
  every matrix/.style={/tikz/inner sep=+0pt},
  every diagram/.style={
    /tikz/commutative diagrams/row sep=normal,
    /tikz/commutative diagrams/column sep=normal,
    /tikz/baseline=+0pt},
  1-row diagram/.style={/tikz/baseline/.expanded=(\tikzcdmatrixname.base)},
  math mode=true,
  center yshift/.initial=axis_height,
  row sep/huge/.initial=+3.6em,
  row sep/large/.initial=+2.7em,
  row sep/normal/.initial=+1.8em,
  row sep/scriptsize/.initial=+1.35em,
  row sep/small/.initial=+0.9em,
  row sep/tiny/.initial=+0.45em,
  column sep/huge/.initial=+4.8em,
  column sep/large/.initial=+3.6em,
  column sep/normal/.initial=+2.4em,
  column sep/scriptsize/.initial=+1.8em,
  column sep/small/.initial=+1.2em,
  column sep/tiny/.initial=+0.6em,
  crossing over clearance/.initial=+1.5ex,
  shift left/.default=+0.56ex,
  shift right/.default=1,
  background color/.initial=white}

% ConTeXt-specific stuff
\pgfutil@IfUndefined{starttikzpicture}{}{%
  \def\starttikzcd{\tikzcd}
  \def\stoptikzcd{\endtikzcd}
  \tikzcdset{
    every matrix/.append code={%
      \def\NC{\pgfmatrixnextcell}%
      \def\NR{\pgfmatrixendrow}}}
}

\endinput


==> tikzlibrarydecorations.code.tex <==
% Copyright 2018 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}%

% Define the basic decoration stuff for tikz. Load more libraries to
% "actually use" decorations

\tikzset{decorate/.is if=tikz@decoratepath,
  /pgf/decoration/name/.store in=\tikz@decoration@name,
  /pgf/decoration/.unknown/.code=%
    \pgfifdecoration{\pgfkeyscurrentname}{\edef\tikz@decoration@name{\pgfkeyscurrentname}}
    {\pgfifmetadecoration{\pgfkeyscurrentname}{\edef\tikz@decoration@name{\pgfkeyscurrentname}}
    {\pgfkeys{/errors/unknown
        key={/pgf/decoration/\pgfkeyscurrentname}{#1}}}},%
  /pgf/decoration/raise/.code={\def\tikz@dec@shift{\pgftransformyshift{#1}}\tikz@dec@trans},
  /pgf/decoration/mirror/.code={%
    \csname if#1\endcsname
      \def\tikz@dec@mirror{\pgftransformyscale{-1}}%
    \else%
      \let\tikz@dec@mirror=\relax%
    \fi%
    \tikz@dec@trans%
  },
  /pgf/decoration/mirror/.default=true,
  /pgf/decoration/transform/.code={%
    {%
      \pgftransformreset%
      \def\tikz@transform{}%
      \pgfkeysalso{/tikz/.cd, #1}%
      \expandafter\gdef\expandafter\tikz@g@temptransform\expandafter{\tikz@transform}%
    }%
    \let\tikz@dec@user@transform=\tikz@g@temptransform%
    \tikz@dec@trans%
  },%
  /pgf/decoration/pre/.initial=lineto,
  /pgf/decoration/post/.initial=lineto,
  /pgf/decoration/pre length/.initial=0pt,
  /pgf/decoration/post length/.initial=0pt,
}%

\let\tikz@decoration@name=\tikz@nonetext

\def\tikz@dec@trans{\pgfsetdecorationsegmenttransformation{\tikz@dec@user@transform\tikz@dec@mirror\tikz@dec@shift}}%
\let\tikz@dec@user@transform=\relax
\let\tikz@dec@shift=\relax
\let\tikz@dec@mirror=\relax

\pgfdeclaremetadecoration{tikz@internal}{pre}{%
  \state{pre}[width=\pgfkeysvalueof{/pgf/decoration/pre length}, next state=main]
  {
    \tikz@dec@trans
    \decoration{\pgfkeysvalueof{/pgf/decoration/pre}}
  }%
  \state{main}[width=\pgfmetadecoratedremainingdistance-\pgfkeysvalueof{/pgf/decoration/post length}, next state=final]
  {
    \tikz@dec@trans
    \decoration{\tikz@decoration@name}
  }%
  \state{final}
  {
    \tikz@dec@trans
    \decoration{\pgfkeysvalueof{/pgf/decoration/post}}
  }%
}%


\newif\iftikz@metadecoration

\def\tikz@lib@dec@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}%

\def\tikz@lib@decoration[#1]{%
  \begingroup%
    % Just to be on the save side...
    %
    % Now, let's parse the options:
    \tikzset{#1}%
    %
    \ifx\tikz@decoration@name\tikz@nonetext%
    % Ok, let's forget about this decoration stuff...
    \else
      \expandafter\tikz@lib@do@dec%
    \fi%
      % Now, we expect a brace.
      \pgfutil@ifnextchar\bgroup{%
        \begingroup%
          \tikz@auto@end@pathfalse%
          \aftergroup\tikz@enddecoration%
          \afterassignment\tikz@scan@next@command%
          \let\tikz@lib@next% gobble \bgroup%
      }%
      {%
        \tikzerror{A decoration must begin with a brace}%
        \tikz@enddecoration%
      }%
}%
\def\tikz@lib@do@dec{%
  % Ok, now what?
  \pgfifmetadecoration{\tikz@decoration@name}%
  {\expandafter\pgfmetadecoration\expandafter{\tikz@decoration@name}}%
  {%
    \pgfifdecoration{\tikz@decoration@name}%
    {\tikz@lib@dec@startdecoration}%
    {\tikzerror{Unknown (meta-)decoration '\tikz@decoration@name'. Perhaps you
        misspelled it?}}%
  }%
  \ifx\pgfdecorateexistingpath\pgfutil@empty%
    \pgfpathmoveto{\pgfqpoint{\the\tikz@lastxsaved}{\the\tikz@lastysaved}}%
  \fi%
}%
\newbox\tikz@lib@dec@box
\def\tikz@enddecoration{%
    \global\setbox\tikz@lib@dec@box=\box\tikz@tempbox%
    \ifx\tikz@decoration@name\tikz@nonetext%
    % ignore this.
    \else
      % Ok, now what?
      \iftikz@metadecoration%
        \endpgfmetadecoration%
      \else%
        \tikz@lib@dec@stopdecoration%
      \fi%
    \fi
  \endgroup%
  \setbox\tikz@tempbox=\box\tikz@lib@dec@box%
}%


\def\tikz@lib@dec@decorate@path{%
  \ifx\tikz@decoration@name\tikz@nonetext%
  \else%
    \pgfgetpath\tikz@lib@dec@currentpath%
    \pgfsetpath\pgfutil@empty%
    \pgfifmetadecoration{\tikz@decoration@name}
    {
      \expandafter\pgfmetadecoration\expandafter{\tikz@decoration@name}%
        \pgfsetpath\tikz@lib@dec@currentpath%
      \endpgfmetadecoration%
    }
    {
      \pgfifdecoration{\tikz@decoration@name}
      {
        \tikz@lib@dec@startdecoration%
          \pgfsetpath\tikz@lib@dec@currentpath%
        \tikz@lib@dec@stopdecoration%
      }
      {
        \tikzerror{Unknown (meta-)decoration '\tikz@decoration@name'. Perhaps
          you misspelled it?}
      }
    }
  \fi%
}%

\def\tikz@lib@dec@zpttext{0pt}%

\newif\iftikz@lib@dec@temp
\def\tikz@lib@dec@startdecoration{%
  \pgfkeysgetvalue{/pgf/decoration/pre length}{\tikz@lib@pre}%
  \pgfkeysgetvalue{/pgf/decoration/post length}{\tikz@lib@post}%
  \tikz@lib@dec@tempfalse%
  \ifx\tikz@lib@pre\tikz@lib@dec@zpttext%
    \ifx\tikz@lib@post\tikz@lib@dec@zpttext%
    \else%
      \tikz@lib@dec@temptrue%
    \fi%
  \else%
    \tikz@lib@dec@temptrue%
  \fi%
  \iftikz@lib@dec@temp%
    \pgfmetadecoration{tikz@internal}%
  \else%
    \expandafter\pgfdecoration\expandafter{\expandafter{\tikz@decoration@name}{\pgfdecoratedpathlength}{}{}}%
  \fi%
}%

\def\tikz@lib@dec@stopdecoration{%
  \iftikz@lib@dec@temp%
    \endpgfmetadecoration%
  \else%
    \endpgfdecoration%
  \fi%
}%


\endinput


==> tikzlibrarydecorations.pathreplacing.code.tex <==
% Copyright 2018 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}%
\usepgflibrary{decorations.pathreplacing}%


\def\tikz@lib@dec@installinputsegmentpoints{%
    \pgf@process{\pgf@decorate@inputsegment@first}%
    \edef\tikzinputsegmentfirst{\the\pgf@x,\the\pgf@y}%
    %
    \pgf@process{\pgf@decorate@inputsegment@last}%
    \edef\tikzinputsegmentlast{\the\pgf@x,\the\pgf@y}%
    %
    \pgf@process{\pgf@decorate@inputsegment@supporta}%
    \edef\tikzinputsegmentsupporta{\the\pgf@x,\the\pgf@y}%
    %
    \pgf@process{\pgf@decorate@inputsegment@supportb}%
    \edef\tikzinputsegmentsupportb{\the\pgf@x,\the\pgf@y}%
}%

\pgfkeys{
    /pgf/decoration/.cd,
        moveto code/.code=\def\pgfdecoratedinputsegmentmovetocode{\tikz@lib@dec@installinputsegmentpoints#1},
        lineto code/.code=\def\pgfdecoratedinputsegmentlinetocode{\tikz@lib@dec@installinputsegmentpoints#1},
        curveto code/.code=\def\pgfdecoratedinputsegmentcurvetocode{\tikz@lib@dec@installinputsegmentpoints#1},
        closepath code/.code=\def\pgfdecoratedinputsegmentclosepathcode{\tikz@lib@dec@installinputsegmentpoints#1}
}%

\endinput


==> tikzlibrarymatrix.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibrarymatrix.code.tex}


% A matrix of nodes contains a node in each cell.

\tikzset{matrix of nodes/.style={%
   matrix,%
   cells={anchor=base},%
   execute at begin cell=\tikz@lib@matrix@start@cell,%
   execute at end cell=\tikz@lib@matrix@end@cell,%
   execute at empty cell=\tikz@lib@matrix@empty@cell,
   execute at begin matrix=\iftikz@handle@active@code\tikz@orig@shorthands\fi,%
}}%

\def\tikz@lib@matrix@empty@cell{\iftikz@lib@matrix@empty\node[name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]{};\fi}%

\newif\iftikz@lib@matrix@plain

\def\tikz@lib@matrix@start@cell{%
  \pgfutil@ifnextchar|{\tikz@lib@matrix@with@options}{\tikz@lib@matrix@normal@start@cell}}%

\def\tikz@lib@matrix@with@options|#1|{\tikz@lib@matrix@plainfalse\node%
  [name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]#1\bgroup\tikz@lib@matrix@startup}%


\def\tikz@lib@matrix@normal@start@cell{\pgfutil@ifnextchar\let{\tikz@lib@matrix@check}{\tikz@lib@matrix@plainfalse\node
  [name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]\bgroup\tikz@lib@matrix@startup}}%

\def\tikz@lib@matrix@check#1{% evil hackery to find out about start of path
  \pgfutil@ifnextchar\tikz@signal@path{\tikz@lib@matrix@plaintrue\let}{\tikz@lib@matrix@plainfalse\node
  [name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]\bgroup\tikz@lib@matrix@startup\let}%
}%

\def\tikz@lib@matrix@end@cell{%
  \iftikz@lib@matrix@plain%
  \else%
    \expandafter\egroup\expandafter;%
  \fi%
}%

\def\tikz@lib@matrix@startup{%
  \pgfutil@ifnextchar\bgroup{%
    % Save meaning of \\:
    \let\tikz@lib@matrix@saved@eol=\\%
    % Now smuggle meaning inside following group.
    \let\\=\pgfmatrixendrow%
    \afterassignment\tikz@lib@matrix@smuggle%
    \let\tikz@next}
  {\let\\=\pgfmatrixendrow}%
}%
\def\tikz@lib@matrix@smuggle{%
  \bgroup%
  \let\\=\tikz@lib@matrix@saved@eol%
}%


% Fill empty nodes in a matrix of nodes

\newif\iftikz@lib@matrix@empty

\tikzoption{nodes in empty cells}[true]{\csname tikz@lib@matrix@empty#1\endcsname}%


% Same as a matrix of nodes, but switch on math mode in each cell
\tikzset{matrix of math nodes/.style={%
  matrix of nodes,
  nodes={%
   execute at begin node=$,%
   execute at end node=$%
  }%
}}%



% Provide a delimiter

\tikzoption{left delimiter}{\tikzset{append after command={\tikz@delimiter%
    {south east}%
    {south west}%
    {every delimiter,every left delimiter}%
    {south}%
    {north}%
    {#1}%
    {.}%
    {\pgf@y}}}}%

\tikzoption{right delimiter}{\tikzset{append after command={\tikz@delimiter%
    {south west}%
    {south east}%
    {every delimiter,every right delimiter}%
    {south}%
    {north}%
    {.}%
    {#1}%
    {\pgf@y}}}}%

\tikzoption{above delimiter}{\tikzset{append after command={\tikz@delimiter%
    {south east}%
    {north west}%
    {every delimiter,every above delimiter,rotate=-90}%
    {west}%
    {east}%
    {#1}%
    {.}%
    {\pgf@x}}}}%

\tikzoption{below delimiter}{\tikzset{append after command={\tikz@delimiter%
    {south west}%
    {south west}%
    {every delimiter,every below delimiter,rotate=-90}%
    {west}%
    {east}%
    {.}%
    {#1}%
    {\pgf@x}}}}%

\def\tikz@delimiter#1#2#3#4#5#6#7#8{%
  \bgroup
    \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
    node[outer sep=0pt,inner sep=0pt,draw=none,fill=none,anchor=#1,at=(\tikz@last@fig@name.#2),#3]
    {%
      {\nullfont\pgf@process{\pgfpointdiff{\pgfpointanchor{\tikz@last@fig@name}{#4}}{\pgfpointanchor{\tikz@last@fig@name}{#5}}}}%
      $\left#6\vcenter{\hrule height .5#8 depth .5#8 width0pt}\right#7$%
    }
    \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
  \egroup%
}%

\tikzset{every delimiter/.style={}}%
\tikzset{every left delimiter/.style={}}%
\tikzset{every right delimiter/.style={}}%
\tikzset{every above delimiter/.style={}}%
\tikzset{every below delimiter/.style={}}%

\endinput


==> tikzlibrarypatterns.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibrarypatterns.code.tex}

\usepgflibrary{patterns}%

\tikzoption{pattern color}{\edef\tikz@pattern@color{#1}}%
\tikzoption{pattern}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillpattern{#1}{\tikz@pattern@color}}%
      \def\tikz@pattern{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}%
\def\tikz@pattern@color{black}%
\def\tikz@pattern{dots}%

\endinput


==> tikzlibraryquotes.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryquotes.code.tex}

\def\tikz@quote@parser#1{\tikz@quote@@parser#1\pgf@stop}%
\def\tikz@quote@@parser"#1"{%
  \pgfutil@ifnextchar\bgroup{%
    \tikz@quote@@parser@group{#1}}{%
    \pgfutil@ifnextchar'{%
      \tikz@quote@@parser@apo{#1}}{%
      \tikz@quote@@parser@normal{#1}}}}%
\def\tikz@quote@@parser@apo#1'{%
  \pgfutil@ifnextchar\bgroup{\tikz@quote@@parser@apo@group{#1}}{\tikz@quote@@parser@apo@normal{#1}}}%
\def\tikz@quote@@parser@group#1#2#3\pgf@stop{%
  \expandafter\def\expandafter\tikz@temp\expandafter{\tikz@quotes@as{#1}{#2}}%
  \expandafter\pgfkeysalso\expandafter{\tikz@temp}%
}%
\def\tikz@quote@@parser@normal#1#2\pgf@stop{%
  \expandafter\def\expandafter\tikz@temp\expandafter{\tikz@quotes@as{#1}{#2}}%
  \expandafter\pgfkeysalso\expandafter{\tikz@temp}%
}%
\def\tikz@quote@@parser@apo@group#1#2#3\pgf@stop{%
  \expandafter\def\expandafter\tikz@temp\expandafter{\tikz@quotes@as{#1}{',#2}}%
  \expandafter\pgfkeysalso\expandafter{\tikz@temp}%
}%
\def\tikz@quote@@parser@apo@normal#1#2\pgf@stop{%
  \expandafter\def\expandafter\tikz@temp\expandafter{\tikz@quotes@as{#1}{',#2}}%
  \expandafter\pgfkeysalso\expandafter{\tikz@temp}%
}%

\pgfkeys{/handlers/first char syntax=true}%

\def\tikz@enable@node@quotes{%
  \pgfkeyssetvalue{/handlers/first char syntax/the character "}{\tikz@quote@parser}%
  \let\tikz@quotes@as\tikz@node@quotes@as%
}%
\def\tikz@enable@edge@quotes{%
  \pgfkeyssetvalue{/handlers/first char syntax/the character "}{\tikz@quote@parser}%
  \let\tikz@quotes@as\tikz@edge@quotes@as%
}%
\def\tikz@enable@pic@quotes{%
  \pgfkeyssetvalue{/handlers/first char syntax/the character "}{\tikz@quote@parser}%
  \let\tikz@quotes@as\tikz@pic@quotes@as%
}%

\tikzset{
  node quotes mean/.code={\def\tikz@node@quotes@as##1##2{#1}},
  edge quotes mean/.code={\def\tikz@edge@quotes@as##1##2{#1}},
  pic quotes mean/.code={\def\tikz@pic@quotes@as##1##2{#1}},
  quotes mean pin/.style={node quotes mean={
      pin={[direction shorthands,every pin quotes/.try,##2]##1}}},
  quotes mean label/.style={node quotes mean={
      label={[direction shorthands,every label quotes/.try,##2]##1}}},
  quotes mean label,
  edge quotes mean={edge node={node [every edge quotes,#2]{#1}}},
  pic quotes mean={pic text={#1},pic text options={every pic quotes/.try,#2}},
  every edge quotes/.style={auto},
  direction shorthands/.code={%
    \pgfkeyslet{/tikz/centered/.@cmd}\tikz@label@@centered
    \pgfkeyslet{/tikz/above/.@cmd}\tikz@label@@above
    \pgfkeyslet{/tikz/below/.@cmd}\tikz@label@@below
    \pgfkeyslet{/tikz/left/.@cmd}\tikz@label@@left
    \pgfkeyslet{/tikz/right/.@cmd}\tikz@label@@right
    \pgfkeyslet{/tikz/above left/.@cmd}\tikz@label@@above@left
    \pgfkeyslet{/tikz/above right/.@cmd}\tikz@label@@above@right
    \pgfkeyslet{/tikz/below left/.@cmd}\tikz@label@@below@left
    \pgfkeyslet{/tikz/below right/.@cmd}\tikz@label@@below@right
  }
}%

\def\tikz@label@@centered#1\pgfeov{\pgfkeysalso{label position=center,pin position=center}}%
\def\tikz@label@@above#1\pgfeov{\pgfkeysalso{label position=90,pin position=90}}%
\def\tikz@label@@below#1\pgfeov{\pgfkeysalso{label position=-90,pin position=-90}}%
\def\tikz@label@@left#1\pgfeov{\pgfkeysalso{label position=180,pin position=180}}%
\def\tikz@label@@right#1\pgfeov{\pgfkeysalso{label position=0,pin position=0}}%
\def\tikz@label@@above@left#1\pgfeov{\pgfkeysalso{label position=135,pin position=135}}%
\def\tikz@label@@below@left#1\pgfeov{\pgfkeysalso{label position=-135,pin position=-135}}%
\def\tikz@label@@above@right#1\pgfeov{\pgfkeysalso{label position=45,pin position=45}}%
\def\tikz@label@@below@right#1\pgfeov{\pgfkeysalso{label position=-45,pin position=-45}}%



\endinput


==> tikzlibraryshapes.arrows.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.arrows.code.tex}

\usepgflibrary{shapes.arrows}%

\pgfkeys{/tikz/arrow box arrows/.code={\pgf@lib@arrowbox@parsearrows{#1}}}%

\endinput


==> tikzlibraryshapes.callouts.code.tex <==
% Copyright 2018 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.callouts}%

\pgfkeys{/tikz/callout absolute pointer/.code={%
    \tikz@scan@one@point\tikz@lib@callout@checkforplus#1\relax%
    }%
}%

\def\tikz@lib@callout@checkforplus#1{%
    \pgfutil@ifnextchar+{\def\tikz@lib@callout@originalpoint{#1}\tikz@lib@callout@scan@relative}%
        {\pgf@lib@callout@makeabsolutepointer{#1}}}%

\def\tikz@lib@callout@scan@relative+{%
    \pgfutil@ifnextchar+{\tikz@lib@callout@scan@plusplus}{\tikz@lib@callout@scan@plus}}%
\def\tikz@lib@callout@scan@plusplus+{\tikz@scan@one@point\tikz@lib@callout@add}%
\def\tikz@lib@callout@scan@plus{\tikz@scan@one@point\tikz@lib@callout@add}%
\def\tikz@lib@callout@add#1{%
    \expandafter\pgf@lib@callout@makeabsolutepointer\expandafter{%
        \expandafter\pgfpointadd\expandafter{\tikz@lib@callout@originalpoint}{#1}}%
}%

\pgfkeys{/tikz/callout relative pointer/.code={%
        \tikz@scan@one@point\pgf@lib@callout@makerelativepointer#1\relax%
    }%
}%

\endinput


==> tikzlibraryshapes.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.code.tex}

\usetikzlibrary{shapes.geometric}%
\usetikzlibrary{shapes.misc}%
\usetikzlibrary{shapes.symbols}%
\usetikzlibrary{shapes.arrows}%
\usetikzlibrary{shapes.callouts}%
\usetikzlibrary{shapes.multipart}%

\endinput


==> tikzlibraryshapes.geometric.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.geometric.code.tex}

\usepgflibrary{shapes.geometric}%

\endinput


==> tikzlibraryshapes.misc.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.misc.code.tex}

\usepgflibrary{shapes.misc}%

\endinput


==> tikzlibraryshapes.multipart.code.tex <==
% Copyright 2018 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.multipart.code.tex}

\usepgflibrary{shapes.multipart}%

\pgfkeys{/tikz/rectangle split/parts/.code={%
    \pgfkeys{/pgf/rectangle split parts=#1}%
    }%
}%

\pgfkeys{/tikz/rectangle split use custom fill/.code={%
    \pgfkeys{/pgf/rectangle split use custom fill=#1}%
    \pgfkeys{/tikz/fill=none}}%
}%

\pgfkeys{/tikz/rectangle split draw splits/.is if=pgfrectanglesplitdrawsplits}%

\pgfkeys{/tikz/rectangle split part align/.code={%
        \pgfkeys{/pgf/rectangle split part align={#1}}%
    }%
}%

\pgfkeys{/tikz/rectangle split part fill/.code={%
        \pgfkeys{/pgf/rectangle split part fill={#1}}%
    }%
}%

\endinput


==> tikzlibraryshapes.symbols.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibraryshapes.symbols.code.tex}

\pgfkeysifdefined{/tikz/shape border uses incircle}{}{%
    \pgfkeys{/tikz/shape border uses incircle/.is if=pgfshapeborderusesincircle}}%

\usepgflibrary{shapes.symbols}%

\endinput


==> tikzlibrarytopaths.code.tex <==
% Copyright 2020 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{tikzlibrarytopaths.code.tex}


% Move to

\tikzset{move to/.style=                 {to path={(\tikztotarget) \tikztonodes}}}


% Straight to

\tikzset{line to/.style=                 {to path={-- (\tikztotarget) \tikztonodes}}}


% Curved to

\tikzset{every curve to/.style=          {}}
\tikzset{curve to/.style=                {to path=\tikz@to@curve@path}}

\tikzoption{bend angle}{\pgfmathsetmacro\tikz@to@bend{#1}}

\tikzoption{bend left}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgfmathsetmacro\tikz@to@bend{#1}%
  \fi%
  \let\tikz@to@out=\tikz@to@bend%
  \pgfmathsetmacro\tikz@to@in{180-(\tikz@to@out)}%
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{bend right}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgfmathsetmacro\tikz@to@bend{#1}%
  \fi%
  % Now, negate
  \pgfmathsetmacro\tikz@to@out{-(\tikz@to@bend)}
  \pgfmathsetmacro\tikz@to@in{180-(\tikz@to@out)}
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{relative}[true]{\csname tikz@to@relative#1\endcsname}
\newif\iftikz@to@relative
\tikz@to@relativefalse

\tikzoption{in}{\def\tikz@to@in{#1}\tikz@to@switch@on}
\tikzoption{out}{\def\tikz@to@out{#1}\tikz@to@switch@on}

\tikzoption{in looseness}{\tikz@to@set@in@looseness{#1}}
\tikzoption{out looseness}{\tikz@to@set@out@looseness{#1}}
\tikzoption{looseness}{\tikz@to@set@in@looseness{#1}\tikz@to@set@out@looseness{#1}}

\tikzoption{in control}{\tikz@to@set@in@control{#1}}
\tikzoption{out control}{\tikz@to@set@out@control{#1}}
\tikzoption{controls}{\tikz@to@parse@controls#1\pgf@stop}

\tikzoption{in min distance}{\tikz@to@set@distances{#1}{}{}{}}
\tikzoption{in max distance}{\tikz@to@set@distances{}{#1}{}{}}
\tikzoption{in distance}{\tikz@to@set@distances{#1}{#1}{}{}}
\tikzoption{out min distance}{\tikz@to@set@distances{}{}{#1}{}}
\tikzoption{out max distance}{\tikz@to@set@distances{}{}{}{#1}}
\tikzoption{out distance}{\tikz@to@set@distances{}{}{#1}{#1}}
\tikzoption{min distance}{\tikz@to@set@distances{#1}{}{#1}{}}
\tikzoption{max distance}{\tikz@to@set@distances{}{#1}{}{#1}}
\tikzoption{distance}{\tikz@to@set@distances{#1}{#1}{#1}{#1}}

\def\tikz@to@set@distances#1#2#3#4{%
  \tikz@to@setifnotempy{#1}{\tikz@to@in@min}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#2}{\tikz@to@in@max}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#3}{\tikz@to@out@min}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@setifnotempy{#4}{\tikz@to@out@max}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@switch@on%
}

\def\tikz@to@setifnotempy#1#2#3{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty\else\def#2{#1}#3\fi%
}


\def\tikz@to@set@in@looseness#1{%
  \pgfmathsetmacro\tikz@to@in@looseness{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@looseness%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@looseness#1{%
  \pgfmathsetmacro\tikz@to@out@looseness{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
  \tikz@to@switch@on%
}

\def\tikz@to@parse@controls#1and#2\pgf@stop{\tikz@to@set@in@control{#2}\tikz@to@set@out@control{#1}}

\def\tikz@to@set@in@control#1{%
  \def\tikz@to@in@control{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@control%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@control#1{%
  \def\tikz@to@out@control{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@control%
  \tikz@to@switch@on%
}


\def\tikz@to@bend{30}

\def\tikz@to@out{45}
\def\tikz@to@in{135}

\def\tikz@to@out@looseness{1}
\def\tikz@to@in@looseness{1}

\def\tikz@to@in@min{0pt}
\def\tikz@to@in@max{10000pt}
\def\tikz@to@out@min{0pt}
\def\tikz@to@out@max{10000pt}

\def\tikz@to@switch@on{\let\tikz@to@path=\tikz@to@curve@path}

\def\tikz@to@curve@path{%
  [every curve to]
  \pgfextra{\iftikz@to@relative\tikz@to@compute@relative\else\tikz@to@compute\fi}
  \tikz@computed@path
  \pgfextra{\tikz@updatenexttrue\tikz@updatecurrenttrue}%
  \tikztonodes%
}

\def\tikz@to@modify#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {}%
  {\edef#1{#1.#2}}
}%

\def\tikz@to@compute{%
  \let\tikz@tofrom=\tikztostart%
  \let\tikz@toto=\tikztotarget%
  \tikz@to@modify\tikz@tofrom\tikz@to@out%
  \tikz@to@modify\tikz@toto\tikz@to@in%
  \ifx\tikz@to@start@compute\tikz@to@start@compute@looseness%
    \tikz@to@compute@distance%
  \else%
    \ifx\tikz@from@start@compute\tikz@to@start@compute@looseness%
      \tikz@to@compute@distance%
    \fi%
  \fi%
  \tikz@to@start@compute%
  \tikz@to@end@compute%
  \edef\tikz@computed@path{.. controls \tikz@computed@start and \tikz@computed@end .. (\tikztotarget)}
}

\def\tikz@to@compute@distance{\tikz@scan@one@point\tikz@@to@compute@distance(\tikz@tofrom)}
\def\tikz@@to@compute@distance#1{%
  \def\tikz@first@point{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@distance(\tikz@toto)}
\def\tikz@@@to@compute@distance#1{%
  \iftikz@updatecurrent\else
    \tikz@updatenextfalse
  \fi
  \def\tikz@second@point{#1}%
  \tikz@to@compute@distance@main%
}
\def\tikz@to@compute@distance@main{%
  \pgf@process{\pgfpointdiff{\tikz@first@point}{\tikz@second@point}}%
  \ifdim\pgf@x<0pt\pgf@xa=-\pgf@x\else\pgf@xa=\pgf@x\fi%
  \ifdim\pgf@y<0pt\pgf@ya=-\pgf@y\else\pgf@ya=\pgf@y\fi%
  %
  % Calculate length of second to first vector:
  %
  \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
  \ifdim\pgf@x>\pgf@y%
    \c@pgf@counta=\pgf@x%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@xa=16\pgf@xa\relax%
      \divide\pgf@xa by\c@pgf@counta%
      \pgf@xa=16\pgf@xa\relax%
    \fi%
  \else%
    \c@pgf@counta=\pgf@y%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@ya=16\pgf@ya\relax%
      \divide\pgf@ya by\c@pgf@counta%
      \pgf@xa=16\pgf@ya\relax%
    \fi%
  \fi%
  \pgf@x=0.3915\pgf@xa%
  \pgf@xa=\tikz@to@out@looseness\pgf@x%
  \pgf@xb=\tikz@to@in@looseness\pgf@x%
  % Adjust as necessary
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@min}
  \ifdim\pgf@xa<\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@max}
  \ifdim\pgf@xa>\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@min}
  \ifdim\pgf@xb<\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@max}
  \ifdim\pgf@xb>\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
}

\def\tikz@to@start@compute@looseness{%
  \edef\tikz@computed@start{([shift=({\tikz@to@out}:\the\pgf@xa)]\tikz@tofrom)}%
}
\def\tikz@to@end@compute@looseness{%
  \edef\tikz@computed@end{([shift=({\tikz@to@in}:\the\pgf@xb)]\tikz@toto)}%
}
\def\tikz@to@start@compute@control{%
  \let\tikz@computed@start=\tikz@to@out@control%
}
\def\tikz@to@end@compute@control{%
  \let\tikz@computed@end=\tikz@to@in@control%
}

\let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
\let\tikz@to@end@compute=\tikz@to@end@compute@looseness%




% Relative curves

\def\tikz@to@compute@relative{%
  \tikz@scan@one@point\tikz@@to@compute@relative(\tikztostart)%
}
\def\tikz@@to@compute@relative#1{%
  \def\tikz@tofrom{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@relative(\tikztotarget)%
}
\def\tikz@@@to@compute@relative#1{%
  \def\tikz@toto{#1}%
  \begingroup
    %
    % Adjust start and target so that they lie on the border in the
    % rotated coordinate system.
    %
    \pgfutil@ifundefined{pgf@sh@ns@\tikztostart}
    {%
      \let\tikz@first@point=\tikz@tofrom%
      \let\tikz@tostart@tikz=\pgfutil@empty
    }%
    {%
      % Start computation of new start.
      {%
        \tikz@tofrom%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{\tikz@to@out}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@toto}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztostart}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@tofrom@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@first@point=\tikz@tofrom@smuggle%
      \tikz@first@point%
      \edef\tikz@tostart@tikz{(\the\pgf@x,\the\pgf@y)}%
    }%
    \pgfutil@ifundefined{pgf@sh@ns@\tikztotarget}
    {%
      \let\tikz@second@point=\tikz@toto%
    }%
    {%
      % Start computation of new target.
      {%
        \tikz@toto%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{180}%
          \pgftransformrotate{\tikz@to@in}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@tofrom}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztotarget}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@toto@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@second@point=\tikz@toto@smuggle%
    }%
    \tikz@second@point%
    \edef\tikz@totarget@tikz{(\the\pgf@x,\the\pgf@y)}%
    %
    % Compute distances
    %
    \tikz@to@compute@distance@main%
    \edef\tikz@to@first@distance{\the\pgf@xa}%
    \edef\tikz@to@second@distance{\the\pgf@xb}%
    %
    % Next step: Establish a transformed coordinate system so that the (modified)
    % start is at the origin and the (modified) target is at (1,0)
    %
    \pgftransformreset%
    \pgf@process{\tikz@first@point}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@second@point}%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgfpointnormalised{}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@xb=-\pgf@x%
    \pgf@yb=-\pgf@y%
    %
    % Now compute the control points.
    %
    {%
      \pgftransformshift{\tikz@first@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@out}{\tikz@to@first@distance}}}%
      \xdef\tikz@computed@start{(\the\pgf@x,\the\pgf@y)}%
    }
    {%
      \pgftransformshift{\tikz@second@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@in}{\tikz@to@second@distance}}}%
      \xdef\tikz@computed@end{(\the\pgf@x,\the\pgf@y)}%
    }
    \xdef\tikz@computed@path{
      \tikz@tostart@tikz
      .. controls \tikz@computed@start and \tikz@computed@end ..
      \tikz@totarget@tikz}%
  \endgroup
}



% Loops

\tikzset{loop/.style=                    {to path={
  \pgfextra{\let\tikztotarget=\tikztostart}
  [looseness=8,min distance=5mm,every loop]
  \tikz@to@curve@path
  }}}

\tikzset{every loop/.style=              {->,shorten >=1pt}}

\tikzset{loop right/.style=              {right,out=15,in=-15,loop}}
\tikzset{loop above/.style=              {above,out=105,in=75,loop}}
\tikzset{loop left/.style=               {left,out=195,in=165,loop}}
\tikzset{loop below/.style=              {below,out=285,in=255,loop}}





\endinput

